SmartTrack: Efficient Predictive Race Detection

Widely used data race detectors, including the state-of-the-art FastTrack algorithm, incur performance costs that are acceptable for regular in-house testing, but miss races detectable from the analyzed execution. Predictive analyses detect more data races in an analyzed execution than FastTrack detects, but at significantly higher performance cost. This paper presents SmartTrack, an algorithm that optimizes predictive race detection analyses, including two analyses from prior work and a new analysis introduced in this paper. SmartTrack's algorithm incorporates two main optimizations: (1) epoch and ownership optimizations from prior work, applied to predictive analysis for the first time; and (2) novel conflicting critical section optimizations introduced by this paper. Our evaluation shows that SmartTrack achieves performance competitive with FastTrack-a qualitative improvement in the state of the art for data race detection.

==> CAPO-Opt-analysis.tex <==
\begin{algorithm}
\caption{\hfill \CAPO analysis with potential optimization}

\small
\begin{algorithmic}[1]

	\Procedure{Acquire}{$t,m$}
		\State Create a new vector clock $C_m$
	\EndProcedure
	
	\Procedure{Release}{$t,m$}
		\State $C_m \gets C_t$ \Comment{Update the vector clock that was shallowed-copied (\ie, reference was copied) during this CS}
		%\LineCommentx{$\lambda_{m,x}^r$ and $\lambda_{m,x}^w$ are vectors of vector clocks}
		%\lForEach{$x \in R_m$}{$\lambda_{m,x}^r(t) \gets C$} \Comment{Store a \emph{ref} to $C$}
		%\lForEach{$x \in W_m$}{$\lambda_{m,x}^w(t) \gets C$} \Comment{Store a \emph{ref} to $C$}
		%\State $R_m \gets W_m \gets \emptyset$
		\State $C_t(t) \gets C_t(t) + 1$
	\EndProcedure
	
	\LineCommentx{$\lambda_{m,x}^w$ is a vector clock, and $\lambda_{m,x}^r$ is a vector of vector clocks}
	
	\Procedure{Read}{$t,x$}
		\ForEach {$m \in \textnormal{HeldLocks}(t)$}
			\If {$\lambda_{m,x}^w(t) < C_t(t)$}
				\State $C_t \gets C_t \sqcup \lambda_{m,x}^w$
			\EndIf
			%\State $C_t \gets C_t \sqcup \LockVarQ{m}{x}{w}$
			\State $\lambda_{m,x}^r(t) \gets_\mathit{shallow} C_m$ \Comment{Store a \emph{reference} to $C_m$}
			%\State $R_m \gets R_m \cup \{x\}$
		\EndFor
		\lIf {$W_x \not\sqsubseteq C_t$}{\Race{\CAPO}}
		\State $R_x(t) \gets C_t(t)$
	\EndProcedure
	
	\Procedure{Write}{$t,x$}
		\ForEach {$m \in \textnormal{HeldLocks}(t)$}
			\If {$\lambda_{m,x}^w(t) < C_t(t)$}
				\State $C_t \gets C_t \sqcup \lambda_{m,x}^w$
			\EndIf
			\If {$\lambda_{m,x}^r \ne \emptyset$}
				\State{$C_t \gets C_t \sqcup \big(\!\sqcup_{u \ne t} \lambda_{m,x}^r(u)\big)$}
				\State $\lambda_{m,x}^r \gets \emptyset$
			\EndIf
			%\State $C_t \gets C_t \sqcup \big( \LockVarQ{m}{x}{r} \sqcup \LockVarQ{m}{x}{w}\big)$
			\State $\lambda_{m,x}^w \gets_\mathit{shallow} C_m$ \Comment{Store a \emph{reference} to $C_m$}
			%\State $W_m \gets W_m \cup \{x\}$
		\EndFor
		\lIf {$W_x \not\sqsubseteq C_t$}{\Race{\CAPO}}
		\lIf {$R_x \not\sqsubseteq C_t$}{\Race{\CAPO}}
		\State $W_x(t) \gets C_t(t)$
	\EndProcedure

\end{algorithmic}
\label{alg:CAPO-Opt-VC}
\end{algorithm}

==> CAPO-analysis.tex <==
\begin{algorithm}
\caption{\hfill \CAPO analysis at each event type}

\small
\begin{algorithmic}[1]

	\Procedure{Acquire}{$t,m$}
		
	\EndProcedure
	
	\Procedure{Release}{$t,m$}
		\lForEach{$x \in R_m$}{$\LockVarQ{m}{x}{r} \gets \LockVarQ{m}{x}{r} \sqcup C_t$} \label{alg:CAPO-VC:TrackRuleARead}
		\lForEach{$x \in W_m$}{$\LockVarQ{m}{x}{w} \gets \LockVarQ{m}{x}{w} \sqcup C_t$} \label{alg:CAPO-VC:TrackRuleAWrite}
		\State $R_m \gets W_m \gets \emptyset$
		\State $C_t(t) \gets C_t(t) + 1$ \label{line:CAPO-VC:Ctinc}
	\EndProcedure
	
	\Procedure{Read}{$t,x$}
		\ForEach {$m \in \textnormal{HeldLocks}(t)$}
			\State $C_t \gets C_t \sqcup \LockVarQ{m}{x}{w}$ \label{alg:CAPO-VC:RuleARead}
			\State $R_m \gets R_m \cup \{x\}$
		\EndFor
		\lIf {$W_x \not\sqsubseteq C_t$}{\Race{\CAPO}} \label{alg:CAPO-VC:write-read-race}
		\State $R_x(t) \gets C_t(t)$ \label{alg:CAPO-VC:updateRx}
	\EndProcedure
	
	\Procedure{Write}{$t,x$}
		\ForEach {$m \in \textnormal{HeldLocks}(t)$}
			\State $C_t \gets C_t \sqcup \big( \LockVarQ{m}{x}{r} \sqcup \LockVarQ{m}{x}{w}\big)$ \label{alg:CAPO-VC:RuleAWrite}
			\State $W_m \gets W_m \cup \{x\}$
		\EndFor
		\lIf {$W_x \not\sqsubseteq C_t$}{\Race{\CAPO}} \label{alg:CAPO-VC:write-write-race}
		\lIf {$R_x \not\sqsubseteq C_t$}{\Race{\CAPO}} \label{alg:CAPO-VC:read-write-race}
		\State $W_x(t) \gets C_t(t)$ \label{alg:CAPO-VC:updateWx}
	\EndProcedure

\end{algorithmic}
\label{alg:CAPO-VC}
\end{algorithm}

==> CAPO-definition.tex <==
\begin{definition}[\CapoFull]
\label{def:capo}

Given a trace \tr,
\CAPOOrdered{}{} is the smallest relation that satisfies the following properties:

\begin{enumerate}[leftmargin=*,label=(\alph*)]

%   \item[(a), (c), (d)] Same as \DC rules~(a), (c), and (d), but for \CAPO instead of DC.
  \item[(a)] Same as \DC \Rule{a}, but with \ltCAPO replacing \ltDC.
%   \item If two critical sections on the same lock contain \conflictingEvents,
%   then the first critical section is ordered by \CAPO to the second \conflictingEvent.
%   % %
%   That is, \CAPOOrdered{\event{r}{_1}}{\event{e}{_2}} if
%   \event{r}{_1} and \event{r}{_2} are release events on the same lock,
%   \TROrdered{\event{r}{_1}}{\event{r}{_2}},
%   $\event{e}{_1} \in \CS{\event{r}{_1}}$, $\event{e}{_2} \in \CS{\event{r}{_2}}$, and
%   \conflicts{\event{e}{_1}}{\event{e}{_2}}.
  
  \item[(c)] Same as \DC \Rule{c}, but with \ltCAPO replacing \ltDC.
%   \item Two events are ordered by \CAPO if they are ordered by \PO.
%   That is, \CAPOOrdered{\event{e}{}}{\event{e}{'}}
%   if \POOrdered{\event{e}{}}{\event{e}{'}}.
  
  \item[(d)] Same as \DC \Rule{d}, but with \ltCAPO replacing \ltDC.
%   \item \CAPO is transitively closed.
%   That is, \CAPOOrdered{\event{e}{}}{\event{e}{'}} 
%   if $\exists e'' \mid \CAPOOrdered{\event{e}{}}{\event{e}{''}} \land \CAPOOrdered{\event{e}{''}}{\event{e}{'}}$.
\end{enumerate}

\end{definition}

==> CAPO-implementation.tex <==
\begin{itemize}[leftmargin=*]

\item a vector clock $C_t$ for each thread $t$;

\item an epoch $t@c$ for each thread $t$ with clock $c$;

\item a vector clock $C_m$ for each lock $m$; 

\item a vector clock $C_x$ for each program variable, representing the read shared vector clock;

\item an epoch $x_r@c$ and $x_w@c$ for each program variable, representing the latest read and write to $x$ respectively;

\item vector clocks \LockVarQ{m}{x}{r} and \LockVarQ{m}{x}{w} that represent joined critical sections on lock $m$
that have read and written $x$;

\item a set of variables read and written by each lock $m$'s ongoing critical section (if any),
$R_m$ and $W_m$; and

\end{itemize}

\begin{algorithm}
\caption{\hfill Implementation of \CAPO analysis at acquire and release event types}
\begin{small}
\raggedright The pair of a thread $t$ and a clock $c$ is an \emph{epoch}.\\
\raggedright An \emph{epoch} is represented as: $e = t@c$.
\smallskip\hrule\smallskip
\end{small}

\small
\begin{algorithmic}[1]

	\Procedure{Acquire}{$t,m$}
		\State $C_t(t) \gets C_t(t) + 1$
		\State $t@c \gets t@C_t(t)$
	\EndProcedure
	
	\Procedure{AcquireHardEdge}{$t,m$}
		\State $C_t(t) \gets C_t(t) + 1$
		\State $t@c \gets t@C_t(t)$
		\State $C_t \gets C_t \sqcup C_m$ \Comment{Called by postWait}
		\State $t@c \gets t@C_t(t)$
	\EndProcedure
	
	\Procedure{Release}{$t,m$} \Comment{Called by preWait}
		\lForEach{$x \in R_m$}{$\LockVarQ{m}{x}{r} \gets \LockVarQ{m}{x}{r} \sqcup C_t$} \label{alg:CAPO-VC:TrackRuleARead}
		\lForEach{$x \in W_m$}{$\LockVarQ{m}{x}{w} \gets \LockVarQ{m}{x}{w} \sqcup C_t$} \label{alg:CAPO-VC:TrackRuleAWrite}
		\State $C_m \gets C_m \sqcup C_t$ \Comment{Used for hard notify -> wait edge}
		\State $R_m \gets W_m \gets \emptyset$ 
		\LineCommentxx{$\LockVarQ{m}{x}{r}$ and $\LockVarQ{m}{x}{w}$ are shrunk if weak variable references have been reclaimed.}
		\State $C_t(t) \gets C_t(t) + 1$ \label{line:CAPO-VC:Ctinc}
		\State $t@c \gets t@C_t(t)$
	\EndProcedure
	
\end{algorithmic}
\label{alg:CAPO-VC-implementation:acq-rel}
\end{algorithm}

\begin{algorithm}
\caption{\hfill Implementation of \CAPO analysis at read event type}
\begin{small}
\raggedright The pair of a thread $t$ and a clock $c$ is an \emph{epoch}.\\
\raggedright An \emph{epoch} is represented as: $e = t@c$. \\
\raggedright A helper function to retrieve an epoch's corresponding thread: $tid(e) = t$. \\
\raggedright The helper function $leq(t@c_1, t@c_2) = c_1 \leq c_2$. \\
\raggedright The helper function $nleq(t@c_1, t@c_2) = c_1 \nleq c_2$.
\smallskip\hrule\smallskip
\end{small}

\small
\begin{algorithmic}[1]
	
	\Procedure{ReadFastPath}{$t,x$}
		\State $w \gets x_w@c$; $r \gets x_r@c$ \Comment{Set epoch for simplicity}
		\If {$r = t@c \lor (x_r \textnormal{ is Read\_Shared} \land C_x(t) = t@c)$}
			\State return \textbf{True} \Comment{Read Same $\lor$ Read Shared Same Epoch}
		\EndIf
		
		\If{$\nexists m \mid m \in \textnormal{HeldLocks}(t)$}
			\State $\textnormal{\bf Lock on } x$
			\If {$tid(w) \neq t \land nleq(w, C_t(tid(w)))$}
				\State $\textnormal{Set BadVarState}$; return \textbf{False} \Comment{Wr-Rd Race}
			\EndIf
			
			\If {$r \textnormal{ is NOT Read\_Shared}$}
				\If {$tid(r) = t \lor leq(r, C_t(tid(r)))$} 
					\State $r \gets t@c$ \Comment{Read Exclusive}
				\Else {} \Comment{Read Share}
					\State $C_x(tid(r)) \gets r$
					\State $C_x(t) \gets C_x(t) \cup t@c$ \Comment{Now Read Shared}
				\EndIf
			\EndIf %lElse is part of if, but must be seperate to format correctly in document 
			\lElse {$C_x(t) \gets t@c$} \Comment{Read Shared}
			
			\State $\textnormal{\bf Unlock on } x$
			\State return \textbf{True}
		\EndIf
		\lElse{return \textbf{False}}
	\EndProcedure
	
	\Procedure{Read}{$t,x$}
		\State $w \gets x_w@c$; $r \gets x_r@c$ \Comment{Set epoch for simplicity}
		\LineCommentxx{Omitting class initialization Code}
		
		\ForEach {$m \in \textnormal{HeldLocks}(t)$} \Comment{Rule (a)}
			\State $C_t \gets C_t \sqcup \LockVarQ{m}{x}{w}$
			\State $R_m \gets R_m \cup \{x\}$
		\EndFor
		
		
		\If {$r = t@c \lor (x_r \textnormal{ is Read\_Shared} \land C_x(t) = t@c)$}
			\State return \Comment{Read Same Epoch $\lor$ Read Shared Same Epoch}
		\EndIf
		
		\State $\textnormal{\bf Lock on } x$
		\If {$tid(w) \neq t \land nleq(w, C_t(tid(w)))$}
			\State Write-Read Race; return
		\EndIf
		
		\If {$r \textnormal{ is NOT Read\_Shared}$}
			\If {$tid(r = t \lor leq(r, C_t(tid(r))))$} 
				\State $r \gets t@c$ \Comment{Read Exclusive}
			\Else {} \Comment{Read Share}
				\State $C_x(tid(r)) \gets r$
				\State $C_x(t) \gets C_x(t) \cup t@c$ \Comment{Now Read Shared}
			\EndIf
		\EndIf %lElse is part of if, but must be seperate to format correctly in document
		\lElse {$C_x(t) \gets t@c$} \Comment{Read Shared}

		\State $\textnormal{\bf Unlock on } x$
	\EndProcedure
	
\end{algorithmic}
\label{alg:CAPO-VC-implementation:rd}
\end{algorithm}

\begin{algorithm}
\caption{\hfill Implementation of \CAPO analysis at write event types}
\begin{small}
\raggedright The pair of a thread $t$ and a clock $c$ is an \emph{epoch}.\\
\raggedright An \emph{epoch} is represented as: $e = t@c$. \\
\raggedright A helper function to retrieve an epoch's corresponding thread: $tid(e) = t$. \\
\raggedright The helper function $leq(t@c_1, t@c_2) = c_1 \leq c_2$. \\
\raggedright The helper function $nleq(t@c_1, t@c_2) = c_1 \nleq c_2$.
\smallskip\hrule\smallskip
\end{small}

\small
\begin{algorithmic}[1]
	
	\Procedure{WriteFastPath}{$t,x$}
		\State $w \gets x_w@c$; $r \gets x_r@c$ \Comment{Set epoch for simplicity}
		\lIf {$w = t@c$}{return \textbf{True}} \Comment{Write Same Epoch}
		
		\If {$\nexists m \mid m \in \textnormal{HeldLocks}(t)$}
			\State $\textnormal{\bf Lock on } x$
			\If {$tid(w) \neq t \land nleq(w, C_t(tid(w)))$}
				\State $\textnormal{Set BadVarState}$; return \textbf{False} \Comment{Wr-Wr Race}
			\EndIf
			
			\If {$r \textnormal{ is NOT Read\_Shared}$}
				\If {$tid(r) \neq t \land nleq(r, C_t(tid(r)))$}
					\State $\textnormal{Set BadVarState}$; return \textbf{False} \Comment{Rd-Wr Race}
				\EndIf
				\lElse {} \Comment{Write Exclusive}
			\Else {}
				\If {$C_t \sqsubseteq C_x$}
					\State $\textnormal{Set BadVarState}$; return \textbf{False} \Comment{Rd(S)-Wr Race}
				\EndIf
				\lElse {} \Comment{Write Shared}
			\EndIf
			\State $w \gets t@c$
			\State $\textnormal{\bf Unlock on } x$
			\State return \textbf{True}
		\EndIf %lElse is part of if, but must be seperate to format correctly in document
		\lElse {return \textbf{False}}
	\EndProcedure
	
	\Procedure{Write}{$t,x$}
		\State $w \gets x_w@c$; $r \gets x_r@c$ \Comment{Set epoch for simplicity}
		\LineCommentxx{Omitting class initialization Code}
		
		\ForEach {$m \in \textnormal{HeldLocks}(t)$} \Comment{Rule (a)}
			\State $C_t \gets C_t \sqcup \big( \LockVarQ{m}{x}{r} \sqcup \LockVarQ{m}{x}{w}\big)$
			\State $W_m \gets W_m \cup \{x\}$
		\EndFor
		
		\lIf {$w = t@c$}{return} \Comment{Write Same Epoch}
		
		\State $\textnormal{\bf Lock on } x$
		\If {$tid(w) \neq t \land nleq(x_w@c, C_t(tid(w)))$}
			\State Write-Write Race
		\EndIf
		\If {$r \textnormal{ is NOT Read\_Shared}$}
			\If {$tid(r) \neq t \land nleq(r, C_t(tid(r)))$}
				\State Read-Write Race
			\EndIf
		\Else{}
			\lIf {$C_t \sqsubseteq C_x$}{Read(Shared)-Write Race}
			%lElse is part of if, but must be seperate to format correctly in document
			\lElse{} \Comment{Write Shared}
		\EndIf
		\State $w \gets t@c$
		\State $\textnormal{\bf Unlock on } x$
	\EndProcedure

\end{algorithmic}
\label{alg:CAPO-VC-implementation:wr}
\end{algorithm}

==> DC-logic-table.tex <==
\begin{table*}[t]
\begin{minipage}{1\textwidth}
\small
\centering
\begin{tabular}{@{}|c|llll|@{}}\hline
Event 	& Case Check & Order Check & Update & Rule \\\hline
\hline 	& $R_x = v \land \VCepoch{C_t}{t} \in v$ & & & \textsc{Read Shared Same Epoch} \\\cline{2-5}
\readOp	& $R_x = v$ & \partialOrdered{W_x}{C_t} & $\VCepoch{R_x}{t} \coloneqq \VCepoch{C_t}{t}$ & \textsc{Read Shared} \\\cline{3-5}
		& & \npartialOrdered{W_x}{C_t} & $C_t \coloneqq C_t \sqcup W_x; \VCepoch{R_x}{t} \coloneqq \VCepoch{C_t}{t}$ & \textsc{Write-Read Race} \\\cline{2-5}
		& $m \in HeldLocks(t)$ & & $C_t \coloneqq C_t \sqcup L_{m,x}^{w}$ & \textsc{Rule(a) Write-Read Sink}\\\hline
\hline 	& $W_x = v \land \VCepoch{C_t}{t} \in v$ & & & \textsc{Write Same Epoch} \\\cline{2-5}
\writeOp& $W_x = v \land R_x = v$ & $\partialOrdered{R_x}{C_t} \land \partialOrdered{W_x}{C_t}$ & $\VCepoch{W_x}{t} \coloneqq \VCepoch{C_t}{t}$ & \textsc{Write Shared} \\\cline{3-5}
		& & $\npartialOrdered{R_x}{C_t} \lor \npartialOrdered{W_x}{C_t}$ & $C_t \coloneqq C_t \sqcup W_x; C_t \coloneqq C_t \sqcup R_x$ & \textsc{Write-Write Race} \\\cline{5-5}
		& & & $\VCepoch{W_x}{t} \coloneqq \VCepoch{C_t}{t} $ & \textsc{Read-Write Race} \\\cline{2-5}
		& $m \in HeldLocks(t)$ & & $C_t \coloneqq C_t \sqcup L_{m,x}^{w}$ & \textsc{Rule(a) Write-Write Sink}\\\cline{4-5}
		& & & $C_t \coloneqq C_t \sqcup L_{m,x}^{r}$ & \textsc{Rule(a) Read-Write Sink}\\\hline
\hline	\acquireOp & $t' \neq t$ & & $Acq_{m,t'}(t)\textnormal{.Enque}(C_t)$ & \textsc{Rule(b)} \\\hline
\hline 	& & & $\VCepoch{C_t}{t} \coloneqq \VCepoch{C_t}{t} + 1$ & \textsc{Release} \\\cline{2-5}
		& $t' \neq t$ & & $Rel_{m,t'}(t)\textnormal{.Enque}(C_t)$ & \textsc{Rule(b) Source} \\\cline{3-5}
		& & $Acq_{m,t}(t')\textnormal{.Front}() \sqsubseteq C_t$ & $C_t \coloneqq C_t \sqcup Rel_{m,t}(t')\textnormal{.Deque}()$ & \textsc{Rule(b) Sink} \\\cline{2-5}
		\releaseOp & $x \in CS(\releaseOp)$ & & $L_{m,x}^{r} \coloneqq L_{m,x}^{r} \sqcup C_t$ & \textsc{Rule(a) Read Source} \\\cline{4-5}
		& & & $L_{m,x}^{w} \coloneqq L_{m,x}^{w} \sqcup C_t$ & \textsc{Rule(a) Write Source} \\\hline
\end{tabular}
\caption{Simple \DCFull Analysis logic.}
\label{tab:analysis-logic:doesnt-commute-simple}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\small
\centering
\begin{tabular}{@{}|c|llll|@{}}\hline
Event 	& Case Check & Order Check & Update & Rule \\\hline
\hline 	& $R_x$ = \VCepoch{C_t}{t} & & & \textsc{Read Same Epoch} \\\cline{2-5}
		& $R_x = v \land \VCepoch{C_t}{t} \in v$ & & & \textsc{Read Shared Same Epoch} \\\cline{2-5}
\readOp	& $R_x$ = \epoch{c}{u} & $\strictPartialOrdered{R_x}{C_t} \land \strictPartialOrdered{W_x}{C_t}$ & $R_x \coloneqq \VCepoch{C_t}{t}$ & \textsc{Read Exclusive} \\\cline{3-5}
		& & \strictPartialOrdered{W_x}{C_t} & $R_x \coloneqq \{\epoch{c}{u}, \VCepoch{C_t}{t}\}$ & \textsc{Read Share} \\\cline{2-5}
		& $R_x = v$ & \strictPartialOrdered{W_x}{C_t} & $\VCepoch{R_x}{t} \coloneqq \VCepoch{C_t}{t}$ & \textsc{Read Shared} \\\cline{2-5}
		& $tid(W_x) \neq t$ & \nstrictPartialOrdered{W_x}{C_t} & $C_t(tid(W_x)) \coloneqq W_x$ & \textsc{Write-Read Race}\\\cline{2-5}
		& $m \in HeldLocks(t)$ & $\nstrictPartialOrdered{\VCepoch{\lambda_{m,x}^{w}}{tid(W_x)}}{\VCepoch{C_t}{tid(W_x)}}$ & $C_t \coloneqq C_t \sqcup \lambda_{m,x}^{w}$ & \textsc{Rule(a) Write-Read Sink}\\\cline{3-5}
		& & & $\lambda_{m,x}^{r}(t) \coloneqq C_m$ & \textsc{Rule(a) Read Source} \\\hline
\hline 	& $W_x$ = \VCepoch{C_t}{t} & & & \textsc{Write Same Epoch} \\\cline{2-5}
		& $R_x$ = \epoch{c}{u} & $\strictPartialOrdered{R_x}{C_t} \land \strictPartialOrdered{W_x}{C_t}$ & $W_x \coloneqq \VCepoch{C_t}{t}$ & \textsc{Write Exclusive} \\\cline{2-5}
		& $R_x = v$ & $\partialOrdered{R_x}{C_t} \land \strictPartialOrdered{W_x}{C_t}$ & \sout{$R_x \coloneqq \epoch{0}{t_0}$}, $W_x \coloneqq \VCepoch{C_t}{t}$ & \textsc{Write Shared} \\\cline{2-5}
		& $tid(W_x) \neq t$ & \nstrictPartialOrdered{W_x}{C_t} & $\big\{C_t(tid(W_x)) \coloneqq W_x \land$ & \textsc{Write-Write Race} \\\cline{2-3}\cline{5-5}
\writeOp& $R_x = \epoch{c}{u}$ & \nstrictPartialOrdered{R_x}{C_t} & $\big(C_t(tid(R_x)) \coloneqq R_x \lor$ & \textsc{Read-Write Race} \\\cline{2-3}\cline{5-5}
		& $R_x = v$ & \npartialOrdered{R_x}{C_t} & $C_t \coloneqq C_t \sqcup R_x\big)\big\}$ & \textsc{Read(Shared)-Write Race}\\\cline{2-5}
		& $m \in HeldLocks(t)$ & $\nstrictPartialOrdered{\VCepoch{\lambda_{m,x}^{w}}{tid(W_x)}}{\VCepoch{C_t}{tid(W_x)}}$ & $C_t \coloneqq C_t \sqcup \lambda_{m,x}^{w}$ & \textsc{Rule(a) Write-Write Sink}\\\cline{3-5}
		& & $\nstrictPartialOrdered{\VCepoch{\lambda_{m,x}^{r}(t')}{t'}}{\VCepoch{C_t}{t'}}$ & $C_t \coloneqq C_t \sqcup \lambda_{m,x}^{r}(t')$ & \textsc{Rule(a) Read-Write Sink}\\\cline{4-5}
		& & & $\lambda_{m,x}^{r} \coloneqq C_m $ & \textsc{Rule(a) Read Source}\\\cline{3-5}
		& & & $\lambda_{m,x}^{w} \coloneqq C_m$ & \textsc{Rule(a) Write Source} \\\hline
\hline	\acquireOp & & & $C_m \coloneqq \textnormal{new VC}$ & \textsc{Rule(a)} \\\hline
\hline 	\releaseOp & & & $\VCepoch{C_t}{t} \coloneqq \VCepoch{C_t}{t} + 1$ & \textsc{Release} \\\cline{2-5}
		& & & $C_m \coloneqq C_t$ & \textsc{Rule(a)} \\\hline
\end{tabular}
\caption{Epoch Optimization \CAPOFull Analysis logic. \DC Rule(b) from Table~\ref{tab:analysis-logic:doesnt-commute-simple} wouldn't change.}
\label{tab:analysis-logic:capo}
\end{minipage}
\end{table*}

==> DO-definition.tex <==
\begin{definition}[\DoFull]
\label{def:do}

Given a trace \tr,
\DOOrdered{}{} is the smallest relation that satisfies the following
properties:

\begin{enumerate}[label=(\alph*)]
  \item If two critical sections on the same lock contain \conflictingEvents,
  then the latest critical section on the same lock that 
  the first critical section is \PO ordered to
  is ordered by \DO to the second conflicting event.
  % % 
  That is, \DOOrdered{\event{r}{'}}{\event{e}{_2}} if
  $\event{e}{_1} \in \CS{\event{r}{_1}} \mid \EqPOOrdered{\event{r}{_1}}{\event{r}{'}}$, 
  $\event{e}{_2} \in \CS{\event{r}{_2}}$,
  $\nexists \event{r}{''} \mid \POOrdered{\event{r}{'}}{\TROrdered{\event{r}{''}}{\event{r}{_2}}}$,
  where \event{r}{_1}, \event{r}{'}, \event{r}{''}, and \event{r}{_2} are release events on the same lock,
  \conflicts{\event{e}{_1}}{\event{e}{_2}}, \EqTROrdered{\event{r}{_1}}{\event{r}{_2}},
  and \TROrdered{\event{r}{'}}{\event{r}{_2}}.
  
%   \item If two critical sections on the same lock contain \conflictingEvents,
%   then the first critical section is ordered by \DO to the second
%   \conflictingEvent.
%   % %
%   That is, \DOOrdered{\event{r}{_1}}{\event{e}{_2}}
%   if $\event{e}{_1} \in \CS{\event{r}{_1}}$, $\event{e}{_2} \in \CS{\event{r}{_2}}$,
%   \event{r}{_1} and \event{r}{_2} are release events on the same lock,
%   \conflicts{\event{e}{_1}}{\event{e}{_2}}, and 
%   \TROrdered{\event{r}{_1}}{\event{r}{_2}}.
  
  \item Two events are ordered by \DO if they are ordered by \PO.
  That is, \DOOrdered{\event{e}{}}{\event{e}{'}}
  if \POOrdered{\event{e}{}}{\event{e}{'}}.
  
  \item \DO is transitively closed.
  That is, \DOOrdered{\event{e}{}}{\event{e}{'}} 
  if $\exists e'' \mid \DOOrdered{\event{e}{}}{\event{e}{''}} \land \DOOrdered{\event{e}{''}}{\event{e}{'}}$.
\end{enumerate}

\end{definition}

==> EO-analysis.tex <==
\begin{algorithm}
\caption{\hfill \CAPO\_RelOpt analysis}

\small
\begin{algorithmic}[1]

	\Procedure{Acquire}{$t,m$}
		\State $O_{m,t} \gets \emptyset$
	\EndProcedure
	
	\Procedure{Release}{$t,m$}
		\State $CA \gets \emptyset$ \Comment{$CA$ is an ordered list of conflicting accesses}
		\ForEach {$\textnormal{thread } t' \ne t$}
			\State $CA \gets CA \cup (O_{m,t} \cap O_{m,t'}^{'})$ 
			\State $O_{m,t'}^{'} \gets \neg \big( O_{m,t'}^{'} \cap CA \big)$ \Comment{Maintain edge events}
		\EndFor
		\State $C_{t}^{'} \gets C_t$ \Comment{Temporary old $C_t$ for race detection}
		\If {$CA \ne \emptyset$} \Comment{Do nothing if $\emptyset$}
			\State $C_t \gets C_t \sqcup L_{m}$
		\EndIf
		\ForEach {$C_x \in A_{m}$} \Comment{$C_x$ is the VC of a variable in $A_{m}$}
			\If {$V(C_x, O_{m,t}) \textnormal{ is \PO before } top(CA)$}
				\lIf {$C_x \not\sqsubseteq C_{t}^{'}$}{\Race{\CAPO}}
			\Else
				\lIf {$C_x \not\sqsubseteq C_t$}{\Race{\CAPO}}
			\EndIf
		\EndFor
		\State $A_{m} \gets \emptyset$
		\State $L_{m} \gets C_t$
		\State $O_{m,t}^{'} \gets O_{m,t}^{'} \cup O_{m,t}$ 
		\State $C_t(t) \gets C_t(t) + 1$
	\EndProcedure
	
	\Procedure{Read}{$t,x$}
		\ForEach {$m \in \textnormal{HeldLocks}(t)$}
			\State $O_{m,t} \gets O_{m,t} \oplus x$
			\lIf {$W_x \not\sqsubseteq C_t$}{$A_{m} \gets A_{m} \oplus W_x$}
		\EndFor
		\lIf {$\textnormal{HeldLocks}(t) = \emptyset \land W_x \not\sqsubseteq C_t$}{\Race{\CAPO}}
		\State $R_x(t) \gets C_t(t)$
	\EndProcedure
	
	\Procedure{Write}{$t,x$}
		\ForEach {$m \in \textnormal{HeldLocks}(t)$}
			\State $O_{m,t} \gets O_{m,t} \oplus x$
			\lIf {$W_x \not\sqsubseteq C_t$}{$A_{m} \gets A_{m} \oplus W_x$}
			\lIf {$R_x \not\sqsubseteq C_t$}{$A_{m} \gets A_{m} \oplus R_x$}
		\EndFor
		\If {$\textnormal{HeldLocks}(t) = \emptyset$}
			\lIf {$W_x \not\sqsubseteq C_t$}{\Race{\CAPO}}
			\lIf {$R_x \not\sqsubseteq C_t$}{\Race{\CAPO}}
		\EndIf
		\State $W_x(t) \gets C_t(t)$
	\EndProcedure

\end{algorithmic}
\label{alg:EO-VC}
\end{algorithm}

\begin{algorithm}
\caption{\hfill \EO analysis at each event type}

\small
\begin{algorithmic}[1]

	\Procedure{Acquire}{$t,m$}
		\ForEach{$n \in HeldLocks(t) \mid n \neq m$} \Comment{Nested locks}
			\State $W_m \gets W_m \cup W_n$
			\State $R_m \gets R_m \cup R_n$
		\EndFor
	\EndProcedure
	
	\Procedure{Release}{$t,m$}
		\ForEach{$x \in W_m$}
			\State $C_t \gets C_t \sqcup \big( \LockVarQ{m}{x}{r} \sqcup \LockVarQ{m}{x}{w}\big)$
		\EndFor
		\ForEach{$x \in R_m \setminus (R_m \cap W_m)$}
			\State $C_t \gets C_t \sqcup \LockVarQ{m}{x}{r}$
		\EndFor
		\lForEach{$x \in R_m$}{$\LockVarQ{m}{x}{r} \gets \LockVarQ{m}{x}{r} \sqcup C_t$}
		\lForEach{$x \in W_m$}{$\LockVarQ{m}{x}{w} \gets \LockVarQ{m}{x}{w} \sqcup C_t$}
		\State $R_m \gets W_m \gets \emptyset$
		\State $C_t(t) \gets C_t(t) + 1$ \label{line:CAPO-VC:Ctinc}
	\EndProcedure
	
	\Procedure{Read}{$t,x$}
		\ForEach {$t' \neq t$}
			\ForEach {$m \in \big( L_{x,t'}^{w} \cap \textnormal{HeldLocks}(t) \big)$}
				\State $R_m \gets R_m \cup \{x\}$
			\EndFor
			\lIf{$L_{x,t'}^{w} \cap \textnormal{HeldLocks}(t) = \emptyset \land W_x \not\sqsubseteq C_t$}{\Race{\EO}} \label{alg:EO-VC:write-read-race}
		\EndFor
		\State $R_x(t) \gets C_t(t)$ \label{alg:CAPO-VC:updateRx}
	\EndProcedure
	
	\Procedure{Write}{$t,x$}
		\ForEach {$t' \neq t$}
			\ForEach {$m \in \big( (L_{x,t'}^{w} \cup L_{x,t'}^{r}) \cap \textnormal{HeldLocks}(t) \big)$}
				\State $W_m \gets W_m \cup \{x\}$
			\EndFor
			\lIf{$L_{x,t'}^{w} \cap \textnormal{HeldLocks}(t) = \emptyset \land W_x \not\sqsubseteq C_t$}{\Race{\EO}} \label{alg:EO-VC:write-write-race}
			\LineComment{$L_{x,t'}^{w}$ is the set of locks held by thread $t'$ at the last write $x$.}
			\lIf{$L_{x,t'}^{r} \cap \textnormal{HeldLocks}(t) = \emptyset \land R_x \not\sqsubseteq C_t$}{\Race{\EO}} \label{alg:EO-VC:read-write-race}
			\LineComment{$L_{x,t'}^{r}$ is the set of locks held by thread $t'$ at the last read $x$.}
		\EndFor
		\State $W_x(t) \gets C_t(t)$ \label{alg:CAPO-VC:updateWx}
	\EndProcedure

\end{algorithmic}
\label{alg:EO-VC}
\end{algorithm}

==> EO-definition.tex <==
\begin{definition}[\EoFull]
\label{def:eo}

Given a trace \tr,
\EOOrdered{}{} is the smallest relation that satisfies the following
properties:

\begin{enumerate}[label=(\alph*)]
  \item Release events on the same lock are ordered by \EO
  if their critical sections contain \conflictingEvents.
  % %
  That is, \EOOrdered{\event{r}{_1}}{\event{r}{_2}} if
  \event{r}{_1} and \event{r}{_2} are release events on the same lock,
  \TROrdered{\event{r}{_1}}{\event{r}{_2}},
  $\event{e}{_1} \in \CS{\event{r}{_1}}$,
  $\event{e}{_2} \in \CS{\event{r}{_2}}$, and
  \conflicts{\event{e}{_1}}{\event{e}{_2}}.
  
  \item Two events are ordered by \EO if they are ordered by \PO.
  That is, \EOOrdered{\event{e}{}}{\event{e}{'}}
  if \POOrdered{\event{e}{}}{\event{e}{'}}.
  
  \item \EO is transitively closed.
  That is, \EOOrdered{\event{e}{}}{\event{e}{'}} 
  if $\exists e'' \mid \EOOrdered{\event{e}{}}{\event{e}{''}} \land 
  \EOOrdered{\event{e}{''}}{\event{e}{'}}$.
\end{enumerate}

\end{definition}

A trace has a \Race{\EO} if it has two conflicting events unordered by \EO that hold no common lock.
That is, a trace \tr has an \Race{\EO} on events \event{e}{} and \event{e}{'} if
\TROrdered{\event{e}{}}{\event{e}{'}}, 
\conflicts{\event{e}{}}{\event{e}{'}},
\nEOOrdered{\event{e}{}}{\event{e}{'}}, and
$\lockset{\event{e}{}} \cap \lockset{\event{e}{'}} = \emptyset$.


Note: Desired goal is to have race detection calculated by joining the earliest \conflictingEvents pair's
earlier release to the second conflicting access. This creates a \CAPO \Rule{a} edge
that is used to determine if a race with any access in the current later critical section
is a \CAPO race. Using this method of detecting races, the vindication process remains
correct. If we attempt to vindicate a non-\CAPO race, the \EO event graph would not be
sufficient in detecting false races and the approach would then be unsound.
Figure~\ref{fig:eo-counter-example} 
shows an example of a non-\CAPO race that an event graph built from the
\EO relation would incorrectly reorder to find a race. Though it is possible for the
forward validation to catch this incorrect reordering, the non-\CAPO race should NOT
be detected if possible. Avoiding detecting of the non-\CAPO race prevents cases that the
\EO event graph could not correctly attempt to reorder; thus resulting in a sound approach.

\begin{figure*}
\renewcommand{\arraystretch}{\smalltablerowheight}
\small
\centering 
\hfill
\subfloat[Example execution. The arrows represent \EO ordering (excluding \PO ordering).]{
\centering
\sf
\begin{tabular}{@{}ll@{}} 
\textnormal{Thread 1} & \textnormal{Thread 2} \\\hline
\Write{z} \\
\Acquire{m} \\
\Write{x} \\
\Release{m}\tikzmark{1} \\
& \Acquire{m} \\
& \Read{x} \\
& \Read{z} \\
& \tikzmark{2}\Release{m}
\end{tabular}%
\label{fig:EO-unsoundness}
}
\link{1}{2}%
\hfill
\subfloat[Incorrectly reordered trace of (a) demonstrating a non-predictable race reported.]{
\centering
\sf
\begin{tabular}{@{}ll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} \\\hline 
& \Acquire{m} \\
& \Read{x} \\
\Write{z} \\
& \Read{z}
\\ \\ \\ \\ \\
\end{tabular}%
\label{fig:EO-unsoundness:reorder}
}\hfill\hfill

\caption{The execution in (a) does not have a predictable race
or a \CAPO-race (\CAPOOrdered{\Write{z}}{\Read{z}}) but 
does have a \EO-race (\nEOOrdered{\Write{z}}{\Read{z}}).
Since the \Sync{m} events contain \conflictingEvents, 
the latest \RelT{m}{T1} is \eoFull to \RelT{m}{T2} 
which is weaker than the distinct \CAPOOrdered{\RelT{m}{T1}}{\ReadT{x}{T2}}.
\Sync{m} is an abbreviation for the sequence \Acquire{m}\code{;} \Read{mVar}\code{;} \Write{mVar}\code{;} \Release{m}.}
\label{fig:eo-counter-example}
\end{figure*}


==> HB-logic-table.tex <==
\begin{table*}[t]
\begin{minipage}{1\textwidth}
\small
\centering
\begin{tabular}{@{}|c|llll|@{}}\hline
Event 	& Case Check & Order Check & Update & Rule \\\hline
\hline 	& $R_x = v \land \VCepoch{C_t}{t} \in v$ & & & \textsc{Read Shared Same Epoch} \\\cline{2-5}
\readOp	& $R_x = v$ & \partialOrdered{W_x}{C_t} & $\VCepoch{R_x}{t} \coloneqq \VCepoch{C_t}{t}$ & \textsc{Read Shared} \\\cline{3-5}
		& & \npartialOrdered{W_x}{C_t} & $C_t \coloneqq C_t \sqcup W_x; \VCepoch{R_x}{t} \coloneqq \VCepoch{C_t}{t}$ & \textsc{Write-Read Race} \\\hline
\hline 	& $W_x = v \land \VCepoch{C_t}{t} \in v$ & & & \textsc{Write Same Epoch} \\\cline{2-5}
\writeOp& $W_x = v \land R_x = v$ & $\partialOrdered{R_x}{C_t} \land \partialOrdered{W_x}{C_t}$ & $\VCepoch{W_x}{t} \coloneqq \VCepoch{C_t}{t}$ & \textsc{Write Shared} \\\cline{3-5}
		& & $\npartialOrdered{R_x}{C_t} \lor \npartialOrdered{W_x}{C_t}$ & $C_t \coloneqq C_t \sqcup W_x; C_t \coloneqq C_t \sqcup R_x$ & \textsc{Write-Write Race} \\\cline{5-5}
		& & & $\VCepoch{W_x}{t} \coloneqq \VCepoch{C_t}{t} $ & \textsc{Read-Write Race} \\\hline
\hline	\acquireOp & $L_m = v$ & & $C_t \coloneqq C_t \sqcup L_m$ & \textsc{Acquire} \\\hline
\hline 	\releaseOp & & & $\VCepoch{C_t}{t} \coloneqq \VCepoch{C_t}{t} + 1$ & \textsc{Release} \\\hline
\end{tabular}
\caption{Simple \HBFull Analysis logic.}
\label{tab:analysis-logic}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\small
\centering
\begin{tabular}{@{}|c|llll|@{}}\hline
Event 	& Case Check & Order Check & Update & Rule \\\hline
\hline 	& $R_x$ = \VCepoch{C_t}{t} & & & \textsc{Read Same Epoch} \\\cline{2-5}
		& $R_x = v \land \VCepoch{C_t}{t} \in v$ & & & \textsc{Read Shared Same Epoch} \\\cline{2-5}
\readOp	& $R_x = \epoch{c}{u}$ & $\strictPartialOrdered{R_x}{C_t} \land \strictPartialOrdered{W_x}{C_t}$ & $R_x \coloneqq \VCepoch{C_t}{t}$ & \textsc{Read Exclusive} \\\cline{3-5}
		& & \strictPartialOrdered{W_x}{C_t} & $R_x \coloneqq \{\epoch{c}{u}, \VCepoch{C_t}{t}\}$ & \textsc{Read Share} \\\cline{2-5}
		& $R_x = v$ & \strictPartialOrdered{W_x}{C_t} & $\VCepoch{R_x}{t} \coloneqq \VCepoch{C_t}{t}$ & \textsc{Read Shared} \\\cline{2-5}
		& $tid(W_x) \neq t$ & \nstrictPartialOrdered{W_x}{C_t} & $C_t(tid(W_x)) \coloneqq W_x$ & \textsc{Write-Read Race}\\\hline
\hline 	& $W_x$ = \VCepoch{C_t}{t} & & & \textsc{Write Same Epoch} \\\cline{2-5}
		& $R_x$ = \epoch{c}{u} & $\strictPartialOrdered{R_x}{C_t} \land \strictPartialOrdered{W_x}{C_t}$ & $W_x \coloneqq \VCepoch{C_t}{t}$ & \textsc{Write Exclusive} \\\cline{2-5} 
		& $R_x = v$ & $\partialOrdered{R_x}{C_t} \land \strictPartialOrdered{W_x}{C_t}$ & \sout{$R_x \coloneqq \epoch{0}{t_0}$}, $W_x \coloneqq \VCepoch{C_t}{t}$ & \textsc{Write Shared} \\\cline{2-5}
\writeOp& $tid(W_x) \neq t$ & \nstrictPartialOrdered{W_x}{C_t} & $\big\{C_t(tid(W_x)) \coloneqq W_x \land$ & \textsc{Write-Write Race} \\\cline{2-3}\cline{5-5}
		& $R_x = \epoch{c}{u}$ & \nstrictPartialOrdered{R_x}{C_t} & $\big(C_t(tid(R_x)) \coloneqq R_x \lor$ & \textsc{Read-Write Race} \\\cline{2-3}\cline{5-5}
		& $R_x = v$ & \npartialOrdered{R_x}{C_t} & $C_t \coloneqq C_t \sqcup R_x\big)\big\}$ & \textsc{Read(Shared)-Write Race}\\\hline
\hline	\acquireOp & $L_m = v$ & & $C_t \coloneqq C_t \sqcup L_m$ & \textsc{Acquire} \\\hline
\hline 	\releaseOp & & & $\VCepoch{C_t}{t} \coloneqq \VCepoch{C_t}{t} + 1$ & \textsc{Release} \\\hline
\end{tabular}
\caption{Epoch Optimization \HBFull Analysis logic.}
\label{tab:analysis-logic:epoch-optimization}
\end{minipage}
\end{table*}

==> PIP-analysis.tex <==
\begin{algorithm}
\caption{\hfill \DO analysis at each event type}

\small
\begin{algorithmic}[1]

	\Procedure{Acquire}{$t,m$}

	\EndProcedure
	
	\Procedure{Release}{$t,m$}
		\State $\LockVarQ{t}{m}{} \gets \LockVarQ{t}{m}{} \sqcup C_t$ \label{alg:DO-VC:TrackRuleA}
% 		\State $\LockVarQ{t}{m}{w} \gets \LockVarQ{t}{m}{w} \sqcup C_t$ \label{alg:DO-VC:TrackRuleAWrite}
% 		\State $R_m \gets W_m \gets \emptyset$
		\State $C_t(t) \gets C_t(t) + 1$ \label{line:DO-VC:Ctinc}
	\EndProcedure
	
	\Procedure{Read}{$t,x$}
		\ForEach {$m \in \textnormal{HeldLocks}(t)$}
			\If {$x \not\in R_{m,t}$} 
				\LineCommentxx {Invariant: $x$ in at most one $W_{m,t'}$}
				\If {$x \in W_{m,t'} \mid t' \ne t$}
					\State $C_t \gets C_t \sqcup \LockVarQ{t'}{m}{}$ \label{alg:DO-VC:RuleARead}
				\EndIf
				\State $R_{m,t} \gets R_{m,t} \cup \{x\}$
			\EndIf
		\EndFor
		\lIf {$W_x \not\sqsubseteq C_t$}{\Race{\DO}} \label{alg:DO-VC:write-read-race}
		\State $R_x(t) \gets C_t(t)$ \label{alg:DO-VC:updateRx}
	\EndProcedure
	
	\Procedure{Write}{$t,x$}
		\ForEach {$m \in \textnormal{HeldLocks}(t)$}
			\ForEach {thread $t' \ne t$}
				\If{$x \in R_{m,t'} \lor x \in W_{m,t'}$}
					\State $C_t \gets C_t \sqcup \LockVarQ{t'}{m}{}$ \label{alg:DO-VC:RuleAWrite}
	% 				\State $C_t \gets C_t \sqcup \big( \LockVarQ{t}{m}{r} \sqcup \LockVarQ{t}{m}{w}\big)$ \label{alg:DO-VC:RuleAWrite} 
					\State $R_{m,t'} \gets R_{m,t'} \setminus \{x\}$
					\State $W_{m,t'} \gets W_{m,t'} \setminus \{x\}$
				\EndIf
			\EndFor
			%\State $R_{m,t} \gets R_{m,t} \setminus \{x\}$ \Comment{Not strictly necessary}
			\State $W_{m,t} \gets W_{m,t} \cup \{x\}$
		\EndFor
		\lIf {$W_x \not\sqsubseteq C_t$}{\Race{\DO}} \label{alg:DO-VC:write-write-race}
		\lIf {$R_x \not\sqsubseteq C_t$}{\Race{\DO}} \label{alg:DO-VC:read-write-race}
		\State $W_x(t) \gets C_t(t)$ \label{alg:DO-VC:updateWx}
	\EndProcedure

\end{algorithmic}
\label{alg:DO-VC}
\end{algorithm}

==> PIP-implementation.tex <==
\begin{itemize}[leftmargin=*]

\item a vector clock $C_t$ for each thread $t$;

\item an epoch $t@c$ for each thread $t$ with clock $c$;

\item a vector clock $C_m$ for each lock $m$; 

\item a vector clock $C_x$ for each program variable, representing the read shared vector clock;

\item an epoch $x_r@c$ and $x_w@c$ for each program variable, representing the latest read and write to $x$ respectively;

\item vector clocks \LockVarThrQRd{m}{x}{t} that represent joined latest critical sections on lock $m$
that have read $x$ by thread $t$;

\item vector clock \LockVarThrQWr{m}{x}{t} that represent the latest critical section on lock $m$ that has written $x$ by thread $t$;

\item vector clocks \PerThrLockQ{m}{t} that represent the VC of the latest release on lock $m$ per thread $t$ 

\end{itemize}

\begin{algorithm}
\caption{\hfill Implementation of \PIP analysis at acquire and release event types}
\begin{small}
\raggedright The pair of a thread $t$ and a clock $c$ is an \emph{epoch}.\\
\raggedright An \emph{epoch} is represented as: $e = t@c$.
\smallskip\hrule\smallskip
\end{small}

\small
\begin{algorithmic}[1]

	\Procedure{Acquire}{$t,m$} \Comment{\textbf{Same as CAPO}}
		\State $C_t(t) \gets C_t(t) + 1$
		\State $t@c \gets t@C_t(t)$
	\EndProcedure
	
	\Procedure{AcquireHardEdge}{$t,m$} \Comment{\textbf{Same as CAPO}}
		\State $C_t(t) \gets C_t(t) + 1$
		\State $t@c \gets t@C_t(t)$
		\State $C_t \gets C_t \sqcup C_m$ \Comment{Called by postWait}
		\State $t@c \gets t@C_t(t)$
	\EndProcedure
	
	\Procedure{Release}{$t,m$} \Comment{Called by preWait}
		\State $\PerThrLockQ{m}{t} \gets \PerThrLockQ{m}{t} \sqcup C_t$ 
		
		\State $C_m \gets C_m \sqcup C_t$ \Comment{Used for hard notify -> wait edge}
		\LineCommentxx{$\LockVarThrQRd{m}{x}{t}$ and $\LockVarThrQWr{m}{x}{t}$ are shrunk if weak variable references have been reclaimed.}
		\State $C_t(t) \gets C_t(t) + 1$
		\State $t@c \gets t@C_t(t)$
	\EndProcedure
	
\end{algorithmic}
\label{alg:PIP-VC-implementation:acq-rel}
\end{algorithm}

\begin{algorithm}
\caption{\hfill Implementation of \PIP analysis at read event type}
\begin{small}
\raggedright The pair of a thread $t$ and a clock $c$ is an \emph{epoch}.\\
\raggedright An \emph{epoch} is represented as: $e = t@c$. \\
\raggedright A helper function to retrieve an epoch's corresponding thread: $tid(e) = t$. \\
\raggedright The helper function $leq(t@c_1, t@c_2) = c_1 \leq c_2$. \\
\raggedright The helper function $nleq(t@c_1, t@c_2) = c_1 \nleq c_2$. \\
\raggedright A helper function to retrieve the thread from LockVarThr: $Thr(\LockVarThrQWr{m}{x}{t}) = t$, $Thr(\LockVarThrQRd{m}{x}{t}) = t$.
\smallskip\hrule\smallskip
\end{small}

\small
\begin{algorithmic}[1]
	
	\Procedure{ReadFastPath}{$t,x$} \Comment{\textbf{Same as CAPO}}
		\State $w \gets x_w@c$; $r \gets x_r@c$ \Comment{Set epoch for simplicity}
		\If {$r = t@c \lor (x_r \textnormal{ is Read\_Shared} \land C_x(t) = t@c)$}
			\State return \textbf{True} \Comment{Read Same $\lor$ Read Shared Same Epoch}
		\EndIf
		
		\If{$\nexists m \mid m \in \textnormal{HeldLocks}(t)$}
			\State $\textnormal{\bf Lock on } x$
			\If {$tid(w) \neq t \land nleq(w, C_t(tid(w)))$}
				\State $\textnormal{Set BadVarState}$; return \textbf{False} \Comment{Wr-Rd Race}
			\EndIf
			
			\If {$r \textnormal{ is NOT Read\_Shared}$}
				\If {$tid(r) = t \lor leq(r, C_t(tid(r)))$} 
					\State $r \gets t@c$ \Comment{Read Exclusive}
				\Else {} \Comment{Read Share}
					\State $C_x(tid(r)) \gets r$
					\State $C_x(t) \gets C_x(t) \cup t@c$ \Comment{Now Read Shared}
				\EndIf
			\EndIf %lElse is part of if, but must be seperate to format correctly in document 
			\lElse {$C_x(t) \gets t@c$} \Comment{Read Shared}
			
			\State $\textnormal{\bf Unlock on } x$
			\State return \textbf{True}
		\EndIf
		\lElse{return \textbf{False}}
	\EndProcedure
	
	\Procedure{Read}{$t,x$}
		\State $w \gets x_w@c$; $r \gets x_r@c$ \Comment{Set epoch for simplicity}
		\LineCommentxx{Omitting class initialization Code}
		
		\ForEach {$m \in \textnormal{HeldLocks}(t)$} \Comment{Relaxed Rule (a)}
			\If {$Thr(\LockVarThrQRd{m}{x}{t}) \neq t$} \Comment{Read Shared}
				\If {$Thr(\LockVarThrQWr{m}{x}{t}) \neq t$} \Comment{\nPOOrdered{\textnormal{prior } \Write{x}}{\Read{x}}}
					\State $C_t \gets C_t \sqcup \PerThrLockQ{m}{Thr(\LockVarThrQWr{m}{x}{t})}$
					\State $t@c \gets C_t(t)$
				\EndIf
				
				\State $\LockVarThrQRd{m}{x}{t} \gets \LockVarThrQRd{m}{x}{t} \sqcup x_m^t$
			\EndIf
		\EndFor
		
		\If {$r = t@c \lor (x_r \textnormal{ is Read\_Shared} \land C_x(t) = t@c)$}
			\State return \Comment{Read Same Epoch $\lor$ Read Shared Same Epoch}
		\EndIf
		
		\State $\textnormal{\bf Lock on } x$
		\If {$tid(w) \neq t \land nleq(w, C_t(tid(w)))$}
			\State Write-Read Race; return
		\EndIf
		
		\If {$r \textnormal{ is NOT Read\_Shared}$}
			\If {$tid(r = t \lor leq(r, C_t(tid(r))))$} 
				\State $r \gets t@c$ \Comment{Read Exclusive}
			\Else {} \Comment{Read Share}
				\State $C_x(tid(r)) \gets r$
				\State $C_x(t) \gets C_x(t) \cup t@c$ \Comment{Now Read Shared}
			\EndIf
		\EndIf %lElse is part of if, but must be seperate to format correctly in document
		\lElse {$C_x(t) \gets t@c$} \Comment{Read Shared}

		\State $\textnormal{\bf Unlock on } x$
	\EndProcedure
	
\end{algorithmic}
\label{alg:PIP-VC-implementation:rd}
\end{algorithm}

\begin{algorithm}
\caption{\hfill Implementation of \PIP analysis at write event types}
\begin{small}
\raggedright The pair of a thread $t$ and a clock $c$ is an \emph{epoch}.\\
\raggedright An \emph{epoch} is represented as: $e = t@c$. \\
\raggedright A helper function to retrieve an epoch's corresponding thread: $tid(e) = t$. \\
\raggedright The helper function $leq(t@c_1, t@c_2) = c_1 \leq c_2$. \\
\raggedright The helper function $nleq(t@c_1, t@c_2) = c_1 \nleq c_2$. \\
\raggedright A helper function to retrieve the thread from LockVarThr: $Thr(\LockVarThrQWr{m}{x}{t}) = t$, $Thr(\LockVarThrQRd{m}{x}{t}) = t$.
\smallskip\hrule\smallskip
\end{small}

\small
\begin{algorithmic}[1]
	
	\Procedure{WriteFastPath}{$t,x$} \Comment{\textbf{Same as CAPO}}
		\State $w \gets x_w@c$; $r \gets x_r@c$ \Comment{Set epoch for simplicity}
		\lIf {$w = t@c$}{return \textbf{True}} \Comment{Write Same Epoch}
		
		\If {$\nexists m \mid m \in \textnormal{HeldLocks}(t)$}
			\State $\textnormal{\bf Lock on } x$
			\If {$tid(w) \neq t \land nleq(w, C_t(tid(w)))$}
				\State $\textnormal{Set BadVarState}$; return \textbf{False} \Comment{Wr-Wr Race}
			\EndIf
			
			\If {$r \textnormal{ is NOT Read\_Shared}$}
				\If {$tid(r) \neq t \land nleq(r, C_t(tid(r)))$}
					\State $\textnormal{Set BadVarState}$; return \textbf{False} \Comment{Rd-Wr Race}
				\EndIf
				\lElse {} \Comment{Write Exclusive}
			\Else {}
				\If {$C_t \sqsubseteq C_x$}
					\State $\textnormal{Set BadVarState}$; return \textbf{False} \Comment{Rd(S)-Wr Race}
				\EndIf
				\lElse {} \Comment{Write Shared}
			\EndIf
			\State $w \gets t@c$
			\State $\textnormal{\bf Unlock on } x$
			\State return \textbf{True}
		\EndIf %lElse is part of if, but must be seperate to format correctly in document
		\lElse {return \textbf{False}}
	\EndProcedure
	
	\Procedure{Write}{$t,x$}
		\State $w \gets x_w@c$; $r \gets x_r@c$ \Comment{Set epoch for simplicity}
		\LineCommentxx{Omitting class initialization Code}
		
		\ForEach {$m \in \textnormal{HeldLocks}(t)$} \Comment{Relaxed Rule (a)}
			\If {$Thr(\LockVarThrQWr{m}{x}{t}) \neq t$} \Comment{Write Shared}
				\State $C_t \gets C_t \sqcup \PerThrLockQ{m}{Thr(\LockVarThrQWr{m}{x}{t})}$
				\State $t@c \gets C_t(t)$
			\EndIf
			
			\ForEach{$t' \neq t \mid t' \in \LockVarThrQRd{m}{x}{t}$}
				\State $C_t \gets C_t \sqcup \PerThrLockQ{m}{t'}$
				\State $t@c \gets C_t(t)$
			\EndFor
			
			\State $\LockVarThrQRd{m}{x}{t} \gets \LockVarThrQRd{m}{x}{t} \setminus x$
			\State $\LockVarThrQWr{m}{x}{t} \gets x_m^t$
		\EndFor
		
		\lIf {$w = t@c$}{return} \Comment{Write Same Epoch}
		
		\State $\textnormal{\bf Lock on } x$
		\If {$tid(w) \neq t \land nleq(x_w@c, C_t(tid(w)))$}
			\State Write-Write Race
		\EndIf
		\If {$r \textnormal{ is NOT Read\_Shared}$}
			\If {$tid(r) \neq t \land nleq(r, C_t(tid(r)))$}
				\State Read-Write Race
			\EndIf
		\Else{}
			\lIf {$C_t \sqsubseteq C_x$}{Read(Shared)-Write Race}
			%lElse is part of if, but must be seperate to format correctly in document
			\lElse{} \Comment{Write Shared}
		\EndIf
		\State $w \gets t@c$
		\State $\textnormal{\bf Unlock on } x$
	\EndProcedure

\end{algorithmic}
\label{alg:PIP-VC-implementation:wr}
\end{algorithm}

==> RE-alternate-analysis.tex <==
\begin{algorithm} [H]
\caption{\hfill \DCO analysis with \Rule{a} optimization}
\jake{Alternate representation of last access metadata and \Rule{a} metadata. 
This is mostly just a quick sketch to see what the possible change might look like.
\mike{I like it but I think there's an issue:
$L_r^x$ can be either a list or a vector of lists.
Loading $r \gets C' \mid \langle C', \bot \rangle \in $ head($L_{x}^{r}$) initially in Read or Write
doesn't seem type-correct when $L_r^x$ may actually be a vector of lists.
In particular, it's hard to reconcile that operation with possibly accessing $L_x^r(u)$ later in Read or Write.}}

\newcommand\Ht{\ensuremath{H_t}\xspace}

\small
\begin{algorithmic}[1]

	\Procedure{Acquire}{$t$, $m$}
		\lForEach{$t' \neq t$}{$\AcqMQ{m}{t'}{t}$.Enque($C_t$)}
		\State $C_m \gets$ new vector clock
		\State $C_m(t) \gets \infty$
		\State $\Ht \gets \langle C_m, m \rangle \oplus \Ht$ \Comment{Uses shallow copy of $C_m$}
	\EndProcedure
	
	\Procedure{Release}{$t$, $m$}
		\ForEach{$t' \neq t$}
			\While{$\AcqMQ{m}{t}{t'}\textnormal{.Front()} \sqsubseteq C_t$}
				\State $\AcqMQ{m}{t}{t'}$.Deque() 
				\State $C_t \gets C_t \sqcup \RelMQ{m}{t}{t'}$.Deque()
			\EndWhile
		\EndFor
		\lForEach{$t' \neq t$}{$\RelMQ{m}{t'}{t}$.Enque($C_t$)}
		\State $\Ht \gets$ rest(\Ht) \Comment{rest() returns list without first element}
		\State $C_m \gets C_t$ \Comment{Update shallow-copied vector clock}
		\State $C_t(t) \gets C_t(t) + 1$
	\EndProcedure
	
	\Procedure{Read}{$t$, $x$} \Comment{{\bf Sr} is Source; {\bf Si} is Sink}
		\State \textbf{let} $r \gets C' \mid \langle C', \bot \rangle \in $ head($L_{x}^{r}$)
		\lIf {$r = C_t(t)$}{\textbf{return}} \Comment{Same-Epoch}
		\lIf {$r(t) = C_t(t)$}{\textbf{return}} \Comment{Shr-Same-Epoch}
		\If {$r = \epoch{c}{t}$} \Comment{Read-Owned}
			\State $L_{x}^{r} \gets \langle C_t(t), \bot \rangle \oplus \Ht$
		\ElsIf {$r = \epoch{c}{u}$}
			\State \textbf{let} $\epoch{c'}{u} = \left\{\begin{tabular}{@{}l@{\;\;}l@{}} $C'(u)$ s.t.\ $\langle C', \_ \rangle = \textnormal{tail}(L_x^r)$ & if $L_x^r \ne \langle\rangle$ \\
			                                                  $r$ & otherwise \\\end{tabular}\right.$
			\If {$\epoch{c'}{u} \le C_t(u)$} \Comment{Read-Exclusive}
				\State $L_{x}^{r} \gets \langle C_t(t), \bot \rangle \oplus \Ht$
			\Else \Comment{Read-Share}
				\State \textbf{let} $s \gets \textnormal{tid}(w)$
				\lIf {$\neg$\textsc{CSCheck}($L_x^w$, $s$)}{\textbf{race}}
				\State $L_{x}^{r} \gets \{L_{x}^{r}, \langle C_t(t), \bot \rangle \oplus \Ht\}$
			\EndIf
		\ElsIf {$r(t) = \epoch{c}{t}$} \Comment{Read-Shared-Owned}
			\State $L_{x}^{r}(t) \gets \langle C_t(t), \bot \rangle \oplus \Ht$
		\Else \Comment{Read-Shared}
			\State \textbf{let} $s \gets \textnormal{tid}(w)$
			\lIf {$\neg$\textsc{CSCheck}($L_x^w$, $s$)}{\textbf{race}}
			\State $L_{x}^{r}(t) \gets \langle C_t(t), \bot \rangle \oplus \Ht$
		\EndIf
	\EndProcedure
	
	\Procedure{Write}{$t$, $x$}
		\State \textbf{let} $r \gets C' \mid \langle C', \bot \rangle \in $ head($L_{x}^{r}$)
		\State \textbf{let} $w \gets C' \mid \langle C', \bot \rangle \in $ head($L_{x}^{w}$)
		\lIf {$w = C_t(t)$} \textbf{return} \Comment{Same-Epoch}
		\If {$r = \epoch{c}{t}$} \textbf{skip} \Comment{Write-Owned (skips to line~\ref{line:WDC-O:write:update})}
		\ElsIf {$r = \epoch{c}{u}$} \Comment{Write-Exclusive}
			\lIf {$\neg$\textsc{CSCheck}($L_x^r$, $u$)}{\textbf{race}}
		\Else \Comment{Write-Shared}
			\ForEach {$u \neq t$}
				\lIf {$\neg$\textsc{CSCheck}($L_x^r(u)$, $u$)}{\textbf{race}}
			\EndFor
		\EndIf
		\State $L_{x}^{w} \gets L_{x}^{r} \gets \langle C_t(t), \bot \rangle \oplus \Ht$ \Comment{Write-Owned; -Exc; -Shr}
	\EndProcedure

	\Procedure{CSCheck}{$L$, $u$}
		\ForEach {$\langle C', m \rangle \textnormal{ in } L$ in right-to-left order}
			\If {$C'(u) \leq C_t(u)$}
				\State \textbf{return} true
			\ElsIf {$m \in \textnormal{heldby}(t)$}
 				\State $C_t \gets C_t \sqcup C'$ \Comment{Rule(a) {\bf Si}}
				\State \textbf{return} true
			\EndIf
		\EndFor
		\State \textbf{return} false
	\EndProcedure

\end{algorithmic}
\label{alg:RE-VC-alt}
\end{algorithm}

==> RE-example.tex <==
\begin{figure*}
\renewcommand{\arraystretch}{\smalltablerowheight}
\small
\centering 
\hfill
\subfloat[Example execution. The arrows represent \RE ordering (excluding \PO ordering).]{
\centering
\sf
\begin{tabular}{@{}lll@{}} 
\textnormal{Thread 1} & \textnormal{Thread 2} & \textnormal{Thread 3} \\\hline
\Acquire{p} \\
\Acquire{m} \\
\Write{x} \\
\Release{m}\tikzmark{3} \\
\Write{z} \\
\Release{p}\tikzmark{1} \\
& \Acquire{m} \\
& \tikzmark{4}\Read{x} \\
& \Release{m}\tikzmark{7} \\
& \Write{y} \\
& \Acquire{p} \\
& \tikzmark{2}\Read{x}\tikzmark{5} \\
& \Release{p} \\
& & \Acquire{m} \\
& & \tikzmark{6}\tikzmark{8}\Write{x} \\
& & \Release{m} \\
& & \Read{y} \\
& & \Read{z}
\end{tabular}%
\link{1}{2}
\link{3}{4}
\link{5}{6}
\linkdash{7}{8}
\label{fig:RE-example}
}
\hfill
\subfloat[Similar example execution as (a) without the critical section on lock \code{p} in thread T2.]{
\centering
\sf
\begin{tabular}{@{}lll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} & \textnormal{Thread 3} \\\hline 
\Acquire{p} \\
\Acquire{m} \\
\Write{x} \\
\Release{m}\tikzmark{1} \\
\Write{z} \\
\Release{p} \\
& \Acquire{m} \\
& \tikzmark{2}\Read{x} \\
& \Release{m}\tikzmark{5} \\
& \Write{y} \\
& {\bf \Read{x}}\tikzmark{3} \\
& & \Acquire{m} \\
& & \tikzmark{4}\tikzmark{6}\Write{x} \\
& & \Release{m} \\
& & \Read{y} \\
& & \Read{z}
\\ \\
\end{tabular}%
\link{1}{2}
\link{3}{4}
\linkdash{5}{6}
\label{fig:RE-example:race-edge}
}
\hfill
\subfloat[A \RE-race exists on \code{z} (\protect\nREOrdered{\WriteT{z}{T1}}{\ReadT{z}{T3}}) but no predictable race exists.]{
\centering
\sf
\begin{tabular}{@{}lll@{}}
\textnormal{Thread 1} & \textnormal{Thread 2} & \textnormal{Thread 3} \\\hline
\Write{z} \\
\Acquire{m} \\
\Write{x} \\
\Release{m}\tikzmark{1} \\
& \Acquire{m} \\
& \Acquire{p} \\
& \tikzmark{2}\Read{x} \\
& \Release{p}\tikzmark{5} \\
& \Release{m} \\
& {\bf \Read{x}}\tikzmark{3} \\
& & \Acquire{p} \\
& & \tikzmark{4}\tikzmark{6}\Write{x} \\
& & \Release{p} \\
& & \Read{z}
\\ \\ \\ \\
\end{tabular}%
\link{1}{2}
\link{3}{4}
\linkdash{5}{6}
\label{fig:RE-example:counter-example}
}
\hfill\hfill
\caption{Dashed arrows indicate redundant Rule(a) edges that are not established by \RE.
The execution in (a) has a predictable race and \RE-race on \code{x}
(\protect\nREOrdered{\ReadT{x}{T2}}{\WriteT{x}{T3}})
but no \RE-race on \code{y} in either example.
The race edge from \ReadT{x}{T2} to \WriteT{x}{T3} ``mends'' the race by establishing
order based on the observed order; effectively removing the race from the execution.
This best effort approach results in the execution containing no predictable race on \code{y}
in either example.
Similar for the execution in (a), showing no predictable race and no \RE-race on \code{z}.
The execution in (b) however has a predictable race and \RE-race on \code{z} (\protect\nREOrdered{\WriteT{z}{T1}}{\ReadT{z}{T3}}).}
\label{fig:re-example}
\end{figure*}

==> WCP-definition.tex <==
\begin{definition}[\WcpFull]

Given a trace \tr,
\WCPOrdered{}{} is the smallest relation that satisfies the following properties:

\begin{enumerate}[label=(\alph*)]  
  \item If two critical sections on the same lock contain \conflictingEvents,
  then the first critical section is ordered by \WCP to the second \conflictingEvent.
  % %
  That is, \WCPOrdered{\event{r}{_1}}{\event{e}{_2}}
  if $\event{e}{_1} \in \CS{\event{r}{_1}}$, $\event{e}{_2} \in \CS{\event{r}{_2}}$,
  \event{r}{_1} and \event{r}{_2} are release events on the same lock,
  \conflicts{\event{e}{_1}}{\event{e}{_2}}, and 
  \TROrdered{\event{r}{_1}}{\event{r}{_2}}.
  
  \item Release events on the same lock are ordered by \WCP
  if their critical sections contain \WCP-ordered events.
  Because of the next rule, this rule can be expressed simply as follows:
  \WCPOrdered{\event{r}{_1}}{\event{r}{_2}} if
  \event{r}{_1} and \event{r}{_2} are release events on the same lock and
  \WCPOrdered{\getAcquire{\event{r}{_1}}}{\event{r}{_2}}.
  
  \item \WCP is closed under left and right composition with \HB.
  That is, \WCPOrdered{e}{e'} 
  if $\exists e'' \mid \WCPOrdered{\HBOrdered{e}{e''}}{e'} \lor
                       \HBOrdered{\WCPOrdered{e}{e''}}{e'}$.
\end{enumerate}
\label{def:weak-causally-precedes}
\end{definition}

==> analyses.tex <==
\section{Analyses}

The following notation and terminology follow the \WCP paper's~\cite{wcp}.
A vector clock $C : \mathit{Tid} \mapsto \mathit{Val}$ maps
each thread to a nonnegative integer. Operations on vector clocks are
pointwise comparison ($\sqsubseteq$) and pointwise join ($\sqcup$):
\begin{eqnarray*}
  C_1 \sqsubseteq C_2 & \iff & \forall t . C_1(t) \leq C_2(t) \\
  C_1 \sqcup C_2 & \equiv & \lambda t . \mathit{max(C_1(t), C_2(t))}
\end{eqnarray*}

%%%%%%
\subsection{\DC Analysis}
\DC analysis, detailed in Algorithm~\ref{alg:Vindicator-VC}, handles each kind
of event in a trace and maintains the following analysis state:

\begin{itemize}[leftmargin=*]

\item a vector clock $C_t$ for each thread $t$;

\item vector clocks for each program variable, $R_x$ and $W_x$, representing the last read and write to $x$ by each thread;

\item vector clocks \LockVarQ{m}{x}{r} and \LockVarQ{m}{x}{w} that represent joined critical sections on lock $m$
that have read and written $x$;

\item a set of variables read and written by each lock $m$'s ongoing critical section (if any),
$R_m$ and $W_m$; and

\item for each lock, two queues for each pair of threads, \AcqMQ{m}{t}{t'} and \RelMQ{m}{t}{t'}, explained below.

\end{itemize}

\input{DC-analysis}

\noindent
Initially,
every vector clock maps all threads to 0,
and every set and queue is empty. 

At each release event $r$ executed by $t$,
the analysis increments $t$'s logical time $C_t(t)$ (line~\ref{line:WDC-VC:Ctinc}).
This action discerns events that occur before and after $r$,
since later the analysis may order $r$ to an event by another thread.

The analysis orders events by \DC \Rule{a} as follows.
At a read or write to $x$ by $t$ in a critical section on lock $m$,
the analysis joins $C_t$ with all prior critical sections on $m$ that have performed \conflictingEvents to $x$
(lines~\ref{alg:WDC-VC:RuleARead} and \ref{alg:WDC-VC:RuleAWrite}).
The analysis updates \LockVarQ{m}{x}{r} and \LockVarQ{m}{x}{w} at each release of $m$
based on which variables the latest critical section on $m$ accessed
(lines~\ref{alg:WDC-VC:TrackRuleARead}--\ref{alg:WDC-VC:TrackRuleAWrite}).

To order events by \Rule{b} of \DC,
the analysis uses the queues of vector clocks, \AcqMQ{m}{t}{t'} and \RelMQ{m}{t}{t'}.
\AcqMQ{m}{t}{t'} is a queue of vector clocks, each of which corresponds to an acquire of lock $m$ by $t'$ that
has \emph{not} been determined to be \DC ordered to the most recent release of $m$ by $t$.
\RelMQ{m}{t}{t'} maintains a queue of vector clocks for the release events corresponding to
each acquire event represented in \AcqMQ{m}{t}{t'}.

These queues of vector clocks help to order events by \DC \Rule{b}:
at $t$'s release of $m$,
the analysis checks whether the release is ordered to a prior acquire of $m$ by each thread $t'$,
by checking $\AcqMQ{m}{t}{t'}\textnormal{.Front()} \sqsubseteq C_t$ (line~\ref{alg:WDC-VC:RuleBCheck}).
If so, the algorithm orders the release corresponding to $\AcqMQ{m}{t}{t'}\textnormal{.Front()}$
to $t$'s release of $m$ (line~\ref{alg:WDC-VC:RelMQDeque}).
It is sufficient to use a queue and check only the head (line~\ref{alg:WDC-VC:RuleBCheck}):
other vector clocks in the queue will pass the check only if the head also passes the check (since \PO implies \DC).  

At each read and write, \DC analysis maintains the logical time of each thread's last read and write to $x$
(lines~\ref{alg:WDC-VC:updateRx} and \ref{alg:WDC-VC:updateWx}).
The analysis checks for \races{\DC} by checking for \DC ordering with prior \conflictingEvents to $x$;
a failed check indicates a \race{\DC}
(lines~\ref{alg:WDC-VC:write-read-race}, \ref{alg:WDC-VC:write-write-race}, and \ref{alg:WDC-VC:read-write-race}).

%%%%%%
\subsection{\CAPO Analysis}
\CAPO analysis, detailed in Algorithm~\ref{alg:CAPO-VC}, handles each kind
of event in a trace and maintains the following analysis state:

\begin{itemize}[leftmargin=*]

\item a vector clock $C_t$ for each thread $t$;

\item vector clocks for each program variable, $R_x$ and $W_x$, representing the last read and write to $x$ by each thread;

\item vector clocks \LockVarQ{m}{x}{r} and \LockVarQ{m}{x}{w} that represent joined critical sections on lock $m$
that have read and written $x$; and

\item a set of variables read and written by each lock $m$'s ongoing critical section (if any),
$R_m$ and $W_m$.

\end{itemize}

\input{CAPO-analysis}

\noindent
Initially,
every vector clock maps all threads to 0,
and every set and queue is empty. 

At each release event $r$ executed by $t$,
the analysis increments $t$'s logical time $C_t(t)$ (line~\ref{line:CAPO-VC:Ctinc}).
This action discerns events that occur before and after $r$,
since later the analysis may order $r$ to an event by another thread.

The analysis orders events by \CAPO \Rule{a} as follows.
At a read or write to $x$ by $t$ in a critical section on lock $m$,
the analysis joins $C_t$ with all prior critical sections on $m$ that have performed \conflictingEvents to $x$
(lines~\ref{alg:CAPO-VC:RuleARead} and \ref{alg:CAPO-VC:RuleAWrite}).
The analysis updates \LockVarQ{m}{x}{r} and \LockVarQ{m}{x}{w} at each release of $m$
based on which variables the latest critical section on $m$ accessed
(lines~\ref{alg:CAPO-VC:TrackRuleARead}--\ref{alg:CAPO-VC:TrackRuleAWrite}).

At each read and write, \CAPO analysis maintains the logical time of each thread's last read and write to $x$
(lines~\ref{alg:CAPO-VC:updateRx} and \ref{alg:CAPO-VC:updateWx}).
The analysis checks for \races {\CAPO} by checking for \CAPO ordering with prior \conflictingEvents to $x$;
a failed check indicates a \race{\CAPO}
(lines~\ref{alg:CAPO-VC:write-read-race}, \ref{alg:CAPO-VC:write-write-race}, and \ref{alg:CAPO-VC:read-write-race}).

%%%%%%
\subsection{CAPO-Opt Analysis}
\CAPO-Opt analysis, detailed in Algorithm~\ref{alg:CAPO-Opt-VC}, handles each kind
of event in a trace and maintains the following analysis state:

\begin{itemize}[leftmargin=*]

\item a vector clock $C_t$ for each thread $t$;

\item a vector clock $C_m$ for each lock $m$;

\item vector clocks for each program variable, $R_x$ and $W_x$, representing the last read and write to $x$ by each thread; and

\item a vector clock $\lambda_{m,x}^w$ and a vector of vector clocks $\lambda_{m,x}^r$,
that represent critical sections on lock $m$ that have read and written $x$.

\end{itemize}

\input{CAPO-Opt-analysis}

%%%%%%
\subsection{\EO Analysis}
\EO analysis, detailed in Algorithm~\ref{alg:EO-VC}, handles each kind
of event in a trace and maintains the following analysis state:

\begin{itemize}[leftmargin=*]

\item $\lambda_{m,x}^w$ is a vector clock, and $\lambda_{m,x}^r$ is a vector of vector clocks;

\item $O_{m,t}$ is an ordered list of program variable access instances per lock per thread;

\item $O_{m,t}^{'}$ is $O_{m,t}$ of the prior critical section of the same lock per thread;

\item $A_{m}$ is a set of vector clocks for each access instance;

\item $V(C, O_{m,t})$ is a helper function that takes a vector clock and $O_{m,t}$ and returns the order of the access from $O_{m}$;

\item $top(CA)$ is a helper function that takes a set of variables and returns the first element of the set;

\item $bot(CA)$ is a helper function that takes a set of variables and returns the last element of the set; and

\item $L_{m}$ is the vector clock of the last release operation of the lock $m$.

\end{itemize}

\input{EO-analysis}

\begin{itemize}
  \item []\textbf{\EO:} Only order release operations and perform lazy race detection using 
the order events execute within a critical section. More specifically:
  \item Record the order of read/write events within a critical section as a set.
  \item At release events, perform an intersection of the read/write set with 
a prior release's read/write set of the same lock for each thread.
  \item If the intersection is empty, no further operation needs to be performed 
since the two CS do not access conflicting events and no rule (a) is established.
  \item If the intersection produces a common variable then rule (a) would have been established
and therefore the two CS are ordered by rule (b), thus the two release events establish an edge between them.
  \item At read/write events, do not update VC but check for races.
  \item Create an ordered list of potential race vector clocks.
  \item Then at the release event, determine if the potential race came before or after 
the earilest event that would have established rule (a).
  \item If before rule (a) event, use the clock's $C_t$ before the rule (b) is established to determine if a race occurred.
  \item If after rule (a) event, use the updated $C_t$ after rule (b) has been established to determine if a race occurred. 
\end{itemize}

%%%%%%
\subsection{\RE Analysis}
\RE analysis, detailed in Algorithm~\ref{alg:RE-VC}, handles each kind
of event in a trace and maintains the following analysis state:

\begin{itemize}[leftmargin=*]

\item a vector clock $C_t$ for each thread $t$;

\item a vector clock $C_m$ for each lock $m$;

\item vector clocks for each program variable, $R_x$ and $W_x$, representing the last read and write to $x$ by each thread; and

\item a vector clock $\lambda_{m,x}^w$ and a vector of vector clocks $\lambda_{m,x}^r$,
that represent critical sections on lock $m$ that have read and written $x$.

\end{itemize}

\input{RE-analysis}

\input{RE-example}

On second thought, it seems that ``rule~(a) metadata''
cannot exactly follow the same representation as the last-access metadata.
In particular, at least in some cases, the rule~(a) metadata needs to be updated to a vector
even when the last-access metadata can be updated to a new epoch (the ``read exclusive'' case).
Figure~\ref{fig:re-read-exclusive-issue} has an example.

\begin{figure}
\renewcommand{\arraystretch}{\smalltablerowheight}
\small
\centering 
\sf
\begin{tabular}{@{}lll@{}} 
\textnormal{Thread 1} & \textnormal{Thread 2} & \textnormal{Thread 3} \\\hline
\Acquire{m} \\
\Read{x} \\
\Sync{o}\tikzmark{1} \\
\ldots \\
\Release{m}\tikzmark{5} \\
& \tikzmark{2}\Sync{o} \\
& \Read{x} \\
& \Sync{p}\tikzmark{3} \\
& & \tikzmark{4}\Sync{p} \\
& & \Acquire{m} \\
& & \tikzmark{6}\Write{x} \\
& & \ldots \\
& & \Release{m} \\
\end{tabular}%
\link{1}{2}
\link{3}{4}
\linkdash{5}{6}
\caption{Using the FastTrack read exclusive optimization, Thread~2's read will update \code{x}'s read metadata to be \code{c@T2}.
If the RE optimization also updates \code{x}'s rule~(a) metadata so that it only stores information for \thr{T2}'s read,
then at the write to \code{x}, the dotted edge will \textbf{not} be established, which is incorrect.}
\label{fig:re-read-exclusive-issue}
\end{figure}

%%%%%%
\subsection{\PIP Analysis}
\DO analysis, detailed in Algorithm~\ref{alg:DO-VC}, handles each kind
of event in a trace and maintains the following analysis state:

\begin{itemize}[leftmargin=*]

\item a vector clock $C_t$ for each thread $t$;

\item vector clocks for each program variable, $R_x$ and $W_x$, representing the last read and write to $x$ by each thread;

\item vector clocks \LockVarQ{t}{m}{} that represent joined critical sections on lock $m$; and

\item a set of variables read and written by each lock $m$'s ongoing critical section (if any) per thread,
$R_{m,t}$ and $W_{m,t}$.

\end{itemize}

\input{PIP-analysis}

\noindent
Initially,
every vector clock maps all threads to 0,
and every set and queue is empty. 

At each release event $r$ executed by $t$,
the analysis increments $t$'s logical time $C_t(t)$ (line~\ref{line:DO-VC:Ctinc}).
This action discerns events that occur before and after $r$,
since later the analysis may order $r$ to an event by another thread.

The analysis orders events by \DO \Rule{a} as follows.
At a read or write to $x$ by $t$ in a critical section on lock $m$,
the analysis joins $C_t$ with all prior critical sections on $m$ that have performed \conflictingEvents to $x$
(lines~\ref{alg:DO-VC:RuleARead} and \ref{alg:DO-VC:RuleAWrite}).
The analysis updates \LockVarQ{m}{x}{r} and \LockVarQ{m}{x}{w} at each release of $m$
based on which variables the latest critical section on $m$ accessed
(line~\ref{alg:DO-VC:TrackRuleA}).  

At each read and write, \DO analysis maintains the logical time of each thread's last read and write to $x$
(lines~\ref{alg:DO-VC:updateRx} and \ref{alg:DO-VC:updateWx}).
The analysis checks for \races{\DO} by checking for \DO ordering with prior \conflictingEvents to $x$;
a failed check indicates a \race{\DO}
(lines~\ref{alg:DO-VC:write-read-race}, \ref{alg:DO-VC:write-write-race}, and \ref{alg:DO-VC:read-write-race}).



==> analysis-barriers.tex <==
\subsection{Analysis Barriers}

\begin{table*}[t]
\small
\centering
\begin{tabular}{@{}rll|rll|rll@{}}\hline
Location & x & 												& Clock & c & : $Z^{+}$ 								& Lock VCs & $L$ & : Lock $\rightarrow$ VC \\
Thread ID & t, u &											& Epoch & e, \epoch{c}{t} & : Clock $\times$ Thread ID	& Last Reads & $R$ & : Location $\rightarrow$ $\big($Epoch $\cup$ VC$\big)$ \\
Operation & a, b & $\Coloneqq \writeOp | \readOp | \ldots$	& VC & $v$ & : Thread ID $\rightarrow$ Epoch 			& Last Writes & $W$ & : Location $\rightarrow$ Epoch \\
Trace & T & $\Coloneqq$ Operation*							& Thread VCs & $C$ & : Thread ID $\rightarrow$ VC		& Epoch TID & $tid(e)$ & : Epoch $\rightarrow$ Thread ID
\end{tabular}
\caption{Syntax for analysis logic tables.}
\label{tab:syntax}
\end{table*}

%\input{HB-logic-table}
%\input{DC-logic-table}

\begin{table*}[t]
\begin{adjustwidth}{-1.5cm}{}
\small
\centering
\begin{tabular}{@{}|c|llll|@{}}\hline
Event 	& Case Check & Order Check & Update & Rule \\\hline
\hline 	& $R_x = \VCepoch{C_t}{t}$ & & & \textsc{Read Same Epoch} \\\cline{2-5}
\readOp	& $R_x = v \land \VCepoch{C_t}{t} \in v$ & & & \textsc{Read Shared Same Epoch} \\\hline
\writeOp& $W_x = \VCepoch{C_t}{t}$ & & & \textsc{Write Same Epoch} \\\hline
\hline  & $R_x = \epoch{c}{t}$ & & $R_x \coloneqq \VCepoch{C_t}{t}$ & \textsc{Read Owned} \\\cline{4-5}
		& & & $L_{x}^{r} \coloneqq \HeldLocks{t}$ & \textsc{Rule(a) Read Owned \bf{Source}} \\\cline{2-5}
\readOp	& $R_x = v \land \VCepoch{C_t}{t} \in v$ & & $\VCepoch{R_x}{t} \coloneqq \VCepoch{C_t}{t}$ & \textsc{Read Shared Owned} \\\cline{4-5}
		& & & $L_{x}^{r}[t] \coloneqq \HeldLocks{t}$ & \textsc{Rule(a) Read Shared Owned \bf{Source}} \\\hline
\writeOp& $R_x = \epoch{c}{t}$ & & $\VCepoch{R_x}{t} \coloneqq \VCepoch{C_t}{t}; \VCepoch{W_x}{t} \coloneqq \VCepoch{C_t}{t}$ & \textsc{Write Owned} \\\cline{4-5}
		& & & $L_{x}^{w} \coloneqq \HeldLocks{t}; L_{x}^{r} \coloneqq \HeldLocks{t}$ & \textsc{Rule(a) Write Owned \bf{Source}} \\\hline
\hline	& $R_x = \epoch{c}{u} \mid u \neq t$ & $\big(C_{m} \leftmapsto L_{x}^{r}(m) \land \strictPartialOrdered{\VCepoch{C_{m}}{u}}{\VCepoch{C_t}{u}}\big)$ & & \\
\readOp	& & $\lor \big(L_{x}^{r} = \emptyset \land \strictPartialOrdered{\VCepoch{R_{x}}{u}}{\VCepoch{C_t}{u}}\big)$ & $R_x \coloneqq \VCepoch{C_t}{t}$ & \textsc{Read Exclusive} \\\hline
\writeOp& $R_x = \epoch{c}{u} \mid u \neq t$ & $\strictPartialOrdered{R_x}{C_t} \land \strictPartialOrdered{W_x}{C_t}$ & $R_x \coloneqq \VCepoch{C_t}{t}; W_x \coloneqq \VCepoch{C_t}{t}$ & \textsc{Write Exclusive} \\\hline
\hline	& $R_x = \epoch{c}{u} \mid u \neq t$ & $C_{m} \leftmapsto L_{x}^{r}(m) \land \nstrictPartialOrdered{\VCepoch{C_{m}}{u}}{\VCepoch{C_t}{u}}$ & & \\
		& & $\land \nstrictPartialOrdered{W_x}{C_t}$ & $\textsc{Race}$ & \textsc{Write-Read Race} \\\cline{3-5}
		& & $C_{m} \leftmapsto L_{x}^{r}(m) \land \nstrictPartialOrdered{\VCepoch{C_{m}}{u}}{\VCepoch{C_t}{u}}$ & $R_x \coloneqq \{\epoch{c}{u}, \VCepoch{C_t}{t}\}$ & \textsc{Read Share} \\\cline{4-5}
		& & $\land \strictPartialOrdered{W_x}{C_t}$ & $L_{x}^{r} \coloneqq \{\epoch{L_{x}^{r}}{u}, \HeldLocks{t}\}$ & \textsc{Rule(a) Read Share \bf{Source}} \\\cline{3-5}
		& & $\big(C_{m} \leftmapsto L_{x}^{r}(m) \land \nstrictPartialOrdered{\VCepoch{C_{m}}{u}}{\VCepoch{C_t}{u}}\big)$ & & \\
		& & $\land \big(C_{m} \leftmapsto L_{x}^{w}(m) \land \nstrictPartialOrdered{\VCepoch{C_{m}}{wt}}{\VCepoch{C_t}{wt}}\big)$ & $C_t \coloneqq C_t \sqcup C_{m} \mid C_{m} \leftmapsto L_{x}^{w}(m)$ & \textsc{Rule(a) Write-Read Share \bf{Sink}} \\\cline{2-5}
\readOp	& $R_x = v$ & \nstrictPartialOrdered{W_x}{C_t} & $\textsc{Race}$ & \textsc{Write-Read Race} \\\cline{3-5}
		& & \strictPartialOrdered{W_x}{C_t} & $\VCepoch{R_x}{t} \coloneqq \VCepoch{C_t}{t}$ & \textsc{Read Shared} \\\cline{4-5}
		& & & $L_{x}^{r}[t] \coloneqq \HeldLocks{t}$ & \textsc{Rule(a) Read Shared \bf{Source}} \\\cline{3-5}
		& & $C_{m} \leftmapsto L_{x}^{w}(m) \land \nstrictPartialOrdered{\VCepoch{C_{m}}{wt}}{\VCepoch{C_t}{wt}}$ & $C_t \coloneqq C_t \sqcup C_{m} \mid C_{m} \leftmapsto L_{x}^{w}(m)$ & \textsc{Rule(a) Write-Read Share \bf{Sink}} \\\hline
\hline	& $R_x = v$ & $\partialOrdered{R_x}{C_t}$ & $R_x \coloneqq \VCepoch{C_t}{t}; W_x \coloneqq \VCepoch{C_t}{t}$ & \textsc{Write Shared} \\\cline{3-5}
		& & & $L_{x}^{w} \coloneqq \HeldLocks{t}; L_{x}^{r} \coloneqq \HeldLocks{t}$ & \textsc{Rule(a) Write Shared \bf{Source}} \\\cline{3-5}
\writeOp& & \npartialOrdered{R_x}{C_t} & $\textsc{Race}$ & \textsc{Read(Shr)-Write Race}\\\cline{3-5}
		& & $C_{m} \leftmapsto L_{x}^{r}[t'](m) \land \nstrictPartialOrdered{\VCepoch{C_{m}}{t'}}{\VCepoch{C_t}{t'}}$ & $C_t \coloneqq C_t \sqcup C_{m} \mid C_{m} \leftmapsto L_{x}^{r}[t'](m)$ & \textsc{Rule(a) Read(Shr)-Write \bf{Sink}} \\\cline{2-5}
		& $R_x = \epoch{c}{u}$ & \nstrictPartialOrdered{R_x}{C_t} & $\textsc{Race}$ & \textsc{Read-Write Race} \\\cline{3-5}
		& & $C_{m} \leftmapsto L_{x}^{r}(m) \land \nstrictPartialOrdered{\VCepoch{C_{m}}{u}}{\VCepoch{C_t}{u}}$ & $C_t \coloneqq C_t \sqcup C_{m} \mid C_{m} \leftmapsto L_{x}^{r}(m)$ & \textsc{Rule(a) Read-Write \bf{Sink}} \\\hline
\hline  \textsc{Race} & $\big\{C_t(wt) \coloneqq W_x \land$ & $\big(C_t(rt) \coloneqq R_x \lor$ & $C_t \coloneqq C_t \sqcup R_x\big)\big\}$ & \textsc{Race} \\\hline
\hline	\acquireOp & & & $C_m \coloneqq \textnormal{new VC}; \VCepoch{C_m}{t} \coloneqq \infty$ & \\
		& & & $\HeldLocks{t} \coloneqq \HeldLocks{t} \oplus C_m$ & \textsc{Rule(a)} \\\hline
\hline 	\releaseOp & & & $\VCepoch{C_t}{t} \coloneqq \VCepoch{C_t}{t} + 1$ & \textsc{Release} \\\cline{2-5}
		& & & $C_m \coloneqq C_t$ & \\
		& & & $\HeldLocks{t} \coloneqq \HeldLocks{t} \setminus C_m$ & \textsc{Rule(a)} \\\hline
\end{tabular}
\jake{Note: \textsc{Race} is one large update spread over the columns for Case Check, Order Check, and Update.}
\jake{Another Note: \HeldLocks{t} is the set of locks currently held by the thread.}
\caption{Epoch Optimization \RE Analysis logic. Note: \textsc{Race} is one large update spread over the columns for Case Check, Order Check, and Update.
\HeldLocks{t} returns the currently held locks from outer most to inner most. $rT$ is $tid(R_x)$. $wT$ is $tid(W_x)$.}
\label{tab:analysis-logic:capo-re}
\end{adjustwidth}
\end{table*}

==> contributions.tex <==

\section*{Contributions} 

\begin{itemize}

\item Use epochs and FastTrack2 optimizations~\cite{fasttrack,fasttrack2}
(including the FastTrack optimizations introduced in the FIB paper~\cite{fib}?)
for last-access metadata.

\item Use epoch/FastTrack2-like optimizations for rule~(a) computations.

\item Eliminate DC rule~(b) for performance--soundness tradeoff (new analysis called \CAPO).

\item Eliminate constraint graph construction and instead rely on the observations that
  \begin{enumerate}
  \item most DC- and \CAPO-races are true predictable races and
  \item multithreaded record \& replay is really fast during record, especially if you're already detecting the data races~\cite{castor,ireplayer}.
  \end{enumerate}

\item Evaluation of all of the above, comparing HB, WCP, DC, and \CAPO with and without the optimizations.

\end{itemize}

\mike{The first two contributions are algorithmic contributions.
To show the new algorithm(s), I think we need to use a level of detail and notation that shows
epochs and read vectors and such.}


==> definitions.tex <==
\section{Definitions}

\input{DC-definition}
\input{CAPO-definition}
\input{DO-definition}
\input{EO-definition}

% \input{CAPO-implementation}
% \input{PIP-implementation}

==> duplicate-results.tex <==

\section{Results duplicating result tables for different configuration
without including confidence intervals}

% Table for benchmark stats such as event counts, thread counts, number of locks held counts 
\begin{table}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\nfpet}[2]{#2M} %no same-epoch event total
% \newcommand{\nfpet}[2]{(#1M + #2M)} %no same-epoch event total
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\tot}[1]{#1~M}
\newcommand{\per}[1]{\ifthenelse{\equal{#1}{\cna}}{\cna}{#1\%}}
\newcommand{\cna}{---} %em-dash. (--) for en-dash
\input{result-macros/PIP_fastTool_noCoresSet_noStatCollection}
% \input{result-macros/PIP_fastTool_noCoresSet}
%
\small
\centering
\begin{tabular}{@{}l|rr|Hrr|rrr@{}}
& & & Size & \mc{2}{c|}{Events} & \mc{3}{c@{}}{Locks held at NSEAs} \\
Program & \mc{2}{c|}{\#Thr} & (LoC) & All & NSEAs & $\geq 1$ & $\geq 2$ & $\geq 3$ \\\hline 
\bench{avrora} 	& \FASTavroraTotalThreads	& (\FASTavroraMaxLiveThreads)	& & \et{\FASTavroraEvents}   & \nfpet{\avroraRECAPONoFPOtherTotal}{\avroraRECAPONoFPEventTotal} 	& \per{\avroraRECAPOOneLockHeld} 	& \per{\avroraRECAPOTwoNestedLocks} 	& \per{\avroraRECAPOThreeNestedLocks} \\
\bench{batik} 	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& & \et{\FASTbatikEvents}    & \nfpet{\batikRECAPONoFPOtherTotal}{\batikRECAPONoFPEventTotal}		& \per{\batikRECAPOOneLockHeld} 	& \per{\batikRECAPOTwoNestedLocks} 		& \per{\batikRECAPOThreeNestedLocks} \\
\bench{h2} 		& \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & & \et{\FASThtwoEvents}     & \nfpet{\htwoRECAPONoFPOtherTotal}{\htwoRECAPONoFPEventTotal}		& \per{\htwoRECAPOOneLockHeld} 		& \per{\htwoRECAPOTwoNestedLocks} 		& \per{\htwoRECAPOThreeNestedLocks} \\
\bench{jython} 	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& & \et{\FASTjythonEvents}   & \nfpet{\jythonRECAPONoFPOtherTotal}{\jythonRECAPONoFPEventTotal}	& \per{\jythonRECAPOOneLockHeld} 	& \per{\jythonRECAPOTwoNestedLocks} 	& \per{\jythonRECAPOThreeNestedLocks} \\
\bench{luindex} & \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& & \et{\FASTluindexEvents}  & \nfpet{\luindexRECAPONoFPOtherTotal}{\luindexRECAPONoFPEventTotal}	& \per{\luindexRECAPOOneLockHeld} 	& \per{\luindexRECAPOTwoNestedLocks} 	& \per{\luindexRECAPOThreeNestedLocks} \\
\bench{lusearch}& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& & \et{\FASTlusearchEvents} & \nfpet{\lusearchRECAPONoFPOtherTotal}{\lusearchRECAPONoFPEventTotal}& \per{\lusearchRECAPOOneLockHeld}	& \per{\lusearchRECAPOTwoNestedLocks} 	& \per{\lusearchRECAPOThreeNestedLocks} \\
\bench{pmd}		& \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & & \et{\FASTpmdEvents}      & \nfpet{\pmdRECAPONoFPOtherTotal}{\pmdRECAPONoFPEventTotal}			& \per{\pmdRECAPOOneLockHeld} 		& \per{\pmdRECAPOTwoNestedLocks} 		& \per{\pmdRECAPOThreeNestedLocks} \\
\bench{sunflow} & \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& & \et{\FASTsunflowEvents}  & \nfpet{\sunflowRECAPONoFPOtherTotal}{\sunflowRECAPONoFPEventTotal}	& \per{\sunflowRECAPOOneLockHeld} 	& \per{\sunflowRECAPOTwoNestedLocks} 	& \per{\sunflowRECAPOThreeNestedLocks} \\
\bench{tomcat} 	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& & \et{\FASTtomcatEvents}   & \nfpet{\tomcatRECAPONoFPOtherTotal}{\tomcatRECAPONoFPEventTotal}	& \per{\tomcatRECAPOOneLockHeld} 	& \per{\tomcatRECAPOTwoNestedLocks} 	& \per{\tomcatRECAPOThreeNestedLocks} \\
\bench{xalan} 	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& & \et{\FASTxalanEvents}    & \nfpet{\xalanRECAPONoFPOtherTotal}{\xalanRECAPONoFPEventTotal}		& \per{\xalanRECAPOOneLockHeld} 	& \per{\xalanRECAPOTwoNestedLocks} 		& \per{\xalanRECAPOThreeNestedLocks} \\
\end{tabular}

\jake{Only \# Thr is collected w/o stat collection.  
Configuration: 10 trials, without setting
cores, without stat collection but with new thread count methodology.
Slow tool is not used in these values.}

\caption{Run-time characteristics of the evaluated programs. ``NSEAs'' are \emph{non-same-epoch accesses}.}
\label{tab:characteristics:bench-stats}
\end{table}

% Separate table with Events, #Thr, Base Time, FT for all benchmarks
\begin{table}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\baseMem}[1]{#1~MB} %base memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_noCoresSet_noStatCollection}
%
\small
\centering
\newcommand{\ics}{\;}
\begin{tabular}{@{}l|HHHHHHcc|rr|rr@{}}
& \mc{2}{Z}{} & \mc{2}{Z}{} & Base & \mc{3}{c|}{\HB} & \mc{2}{c|}{Unopt-\DC} & \mc{2}{c@{}}{Unopt-\CAPO} \\
Program & \mc{2}{Z}{Events} & \mc{2}{Z}{\#Thr} & time & RR\FTTwoAbbrv & \FTTwoAbbrv & \FTO & w/ G & w/o G & w/ G & w/o G \\\hline 
\bench{avrora} 	& \et{\FASTavroraEvents}   & \enfp{\FASTavroraNoFPEvents}	& \FASTavroraTotalThreads 	& (\FASTavroraMaxLiveThreads)	& \base{\FASTavroraBaseTime}   & \roh{\FASTavroraFTTime}   & \roh{\FASTavroraHBTime}	& \roh{\FASTavroraFTOHBTime}	& \roh{\SLOWavroraDCExcTime}	& \roh{\SLOWavroraDCnoGExcTime}	& \roh{\SLOWavroraCAPOExcTime}	& \roh{\SLOWavroraCAPOnoGExcTime}\\
\bench{batik} 	& \et{\FASTbatikEvents}    & \enfp{\FASTbatikNoFPEvents}	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& \base{\FASTbatikBaseTime}    & \roh{\FASTbatikFTTime}    & \roh{\FASTbatikHBTime}   	& \roh{\FASTbatikFTOHBTime}		& \roh{\SLOWbatikDCExcTime}	& \roh{\SLOWbatikDCnoGExcTime}		& \roh{\SLOWbatikCAPOExcTime}	& \roh{\SLOWbatikCAPOnoGExcTime} \\
\bench{h2} 		& \et{\FASThtwoEvents}     & \enfp{\FASThtwoNoFPEvents}	    & \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & \base{\FASThtwoBaseTime}     & \roh{\FASThtwoFTTime}     & \roh{\FASThtwoHBTime}    	& \roh{\FASThtwoFTOHBTime}		& \roh{\SLOWhtwoDCExcTime}		& \roh{\SLOWhtwoDCnoGExcTime}		& \roh{\SLOWhtwoCAPOExcTime}	& \roh{\SLOWhtwoCAPOnoGExcTime}\\
\bench{jython} 	& \et{\FASTjythonEvents}   & \enfp{\FASTjythonNoFPEvents}	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& \base{\FASTjythonBaseTime}   & \roh{\FASTjythonFTTime}   & \roh{\FASTjythonHBTime} 	& \roh{\FASTjythonFTOHBTime}	& \roh{\SLOWjythonDCExcTime}	& \roh{\SLOWjythonDCnoGExcTime}	& \roh{\SLOWjythonCAPOExcTime}	& \roh{\SLOWjythonCAPOnoGExcTime} \\
\bench{luindex} & \et{\FASTluindexEvents}  & \enfp{\FASTluindexNoFPEvents}	& \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& \base{\FASTluindexBaseTime}  & \roh{\FASTluindexFTTime}  & \roh{\FASTluindexHBTime} 	& \roh{\FASTluindexFTOHBTime}	& \roh{\SLOWluindexDCExcTime}	& \roh{\SLOWluindexDCnoGExcTime}	& \roh{\SLOWluindexCAPOExcTime}	& \roh{\SLOWluindexCAPOnoGExcTime} \\
\bench{lusearch}& \et{\FASTlusearchEvents} & \enfp{\FASTlusearchNoFPEvents}	& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& \base{\FASTlusearchBaseTime} & \roh{\FASTlusearchFTTime} & \roh{\FASTlusearchHBTime}	& \roh{\FASTlusearchFTOHBTime}	& \roh{\SLOWlusearchDCExcTime}	& \roh{\SLOWlusearchDCnoGExcTime}	& \roh{\SLOWlusearchCAPOExcTime}& \roh{\SLOWlusearchCAPOnoGExcTime} \\
\bench{pmd}		& \et{\FASTpmdEvents}      & \enfp{\FASTpmdNoFPEvents}      & \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & \base{\FASTpmdBaseTime}      & \roh{\FASTpmdFTTime}      & \roh{\FASTpmdHBTime}		& \roh{\FASTpmdFTOHBTime}		& \roh{\SLOWpmdDCExcTime}		& \roh{\SLOWpmdDCnoGExcTime}		& \roh{\SLOWpmdCAPOExcTime}		& \roh{\SLOWpmdCAPOnoGExcTime} \\
\bench{sunflow} & \et{\FASTsunflowEvents}  & \enfp{\FASTsunflowNoFPEvents}	& \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& \base{\FASTsunflowBaseTime}  & \roh{\FASTsunflowFTTime}  & \roh{\FASTsunflowHBTime}	& \roh{\FASTsunflowFTOHBTime}	& \roh{\SLOWsunflowDCExcTime}	& \roh{\SLOWsunflowDCnoGExcTime}	& \roh{\SLOWsunflowCAPOExcTime}	& \roh{\SLOWsunflowCAPOnoGExcTime} \\
\bench{tomcat} 	& \et{\FASTtomcatEvents}   & \enfp{\FASTtomcatNoFPEvents}	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& \base{\FASTtomcatBaseTime}   & \roh{\FASTtomcatFTTime}   & \roh{\FASTtomcatHBTime} 	& \roh{\FASTtomcatFTOHBTime}	& \roh{\SLOWtomcatDCExcTime}	& \roh{\SLOWtomcatDCnoGExcTime}	& \roh{\SLOWtomcatCAPOExcTime}	& \roh{\SLOWtomcatCAPOnoGExcTime} \\
\bench{xalan} 	& \et{\FASTxalanEvents}    & \enfp{\FASTxalanNoFPEvents}	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& \base{\FASTxalanBaseTime}    & \roh{\FASTxalanFTTime}    & \roh{\FASTxalanHBTime}		& \roh{\FASTxalanFTOHBTime}		& \roh{\SLOWxalanDCExcTime}	& \roh{\SLOWxalanDCnoGExcTime} 	& \roh{\SLOWxalanCAPOExcTime}	& \roh{\SLOWxalanCAPOnoGExcTime}\\\hline
geomean	& &	& &	& & \roh{\FASTFTTimeGeoMean} & \roh{\FASTHBTimeGeoMean} & \roh{\FASTFTOHBTimeGeoMean} & \roh{\SLOWDCExcTimeGeoMean} & \roh{\SLOWDCnoGExcTimeGeoMean} & \roh{\SLOWCAPOExcTimeGeoMean} & \roh{\SLOWCAPOnoGExcTimeGeoMean} \\
\mc{1}{c|}{} & \mc{12}{c}{Run time} \\
\end{tabular}%
\hfill\mbox{\vline height 3cm depth 2.5cm}\hfill\null
\begin{tabular}{@{}HHHHHHHcc|rr|rr@{}}
& \mc{2}{Z}{} & \mc{2}{Z}{} & Base & \mc{3}{c|}{\HB} & \mc{2}{c|}{Unopt-\DC} & \mc{2}{c@{}}{Unopt-\CAPO} \\
Program & \mc{2}{Z}{Events} & \mc{2}{Z}{\#Thr} & memory & RR\FTTwoAbbrv & \FTTwoAbbrv & \FTO & w/ G & w/o G & w/ G & w/o G \\\hline 
\bench{avrora} 	& \et{\FASTavroraEvents}   & \enfp{\FASTavroraNoFPEvents}	& \FASTavroraTotalThreads 	& (\FASTavroraMaxLiveThreads)	& \baseMem{\FASTavroraBaseMem}   & \mem{\FASTavroraFTMem}   & \mem{\FASTavroraHBMem}	& \mem{\FASTavroraFTOHBMem}	& \mem{\SLOWavroraDCExcMem}	& \mem{\SLOWavroraDCnoGExcMem}	& \mem{\SLOWavroraCAPOExcMem}	& \mem{\SLOWavroraCAPOnoGExcMem}\\
\bench{batik} 	& \et{\FASTbatikEvents}    & \enfp{\FASTbatikNoFPEvents}	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& \baseMem{\FASTbatikBaseMem}    & \mem{\FASTbatikFTMem}    & \mem{\FASTbatikHBMem}   	& \mem{\FASTbatikFTOHBMem}		& \mem{\SLOWbatikDCExcMem}	& \mem{\SLOWbatikDCnoGExcMem}		& \mem{\SLOWbatikCAPOExcMem}	& \mem{\SLOWbatikCAPOnoGExcMem} \\
\bench{h2} 		& \et{\FASThtwoEvents}     & \enfp{\FASThtwoNoFPEvents}	    & \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & \baseMem{\FASThtwoBaseMem}     & \mem{\FASThtwoFTMem}     & \mem{\FASThtwoHBMem}    	& \mem{\FASThtwoFTOHBMem}		& \mem{\SLOWhtwoDCExcMem}		& \mem{\SLOWhtwoDCnoGExcMem}		& \mem{\SLOWhtwoCAPOExcMem}	& \mem{\SLOWhtwoCAPOnoGExcMem}\\
\bench{jython} 	& \et{\FASTjythonEvents}   & \enfp{\FASTjythonNoFPEvents}	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& \baseMem{\FASTjythonBaseMem}   & \mem{\FASTjythonFTMem}   & \mem{\FASTjythonHBMem} 	& \mem{\FASTjythonFTOHBMem}	& \mem{\SLOWjythonDCExcMem}	& \mem{\SLOWjythonDCnoGExcMem}	& \mem{\SLOWjythonCAPOExcMem}	& \mem{\SLOWjythonCAPOnoGExcMem} \\
\bench{luindex} & \et{\FASTluindexEvents}  & \enfp{\FASTluindexNoFPEvents}	& \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& \baseMem{\FASTluindexBaseMem}  & \mem{\FASTluindexFTMem}  & \mem{\FASTluindexHBMem} 	& \mem{\FASTluindexFTOHBMem}	& \mem{\SLOWluindexDCExcMem}	& \mem{\SLOWluindexDCnoGExcMem}	& \mem{\SLOWluindexCAPOExcMem}	& \mem{\SLOWluindexCAPOnoGExcMem} \\
\bench{lusearch}& \et{\FASTlusearchEvents} & \enfp{\FASTlusearchNoFPEvents}	& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& \baseMem{\FASTlusearchBaseMem} & \mem{\FASTlusearchFTMem} & \mem{\FASTlusearchHBMem}	& \mem{\FASTlusearchFTOHBMem}	& \mem{\SLOWlusearchDCExcMem}	& \mem{\SLOWlusearchDCnoGExcMem}	& \mem{\SLOWlusearchCAPOExcMem}& \mem{\SLOWlusearchCAPOnoGExcMem} \\
\bench{pmd}		& \et{\FASTpmdEvents}      & \enfp{\FASTpmdNoFPEvents}      & \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & \baseMem{\FASTpmdBaseMem}      & \mem{\FASTpmdFTMem}      & \mem{\FASTpmdHBMem}		& \mem{\FASTpmdFTOHBMem}		& \mem{\SLOWpmdDCExcMem}		& \mem{\SLOWpmdDCnoGExcMem}		& \mem{\SLOWpmdCAPOExcMem}		& \mem{\SLOWpmdCAPOnoGExcMem} \\
\bench{sunflow} & \et{\FASTsunflowEvents}  & \enfp{\FASTsunflowNoFPEvents}	& \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& \baseMem{\FASTsunflowBaseMem}  & \mem{\FASTsunflowFTMem}  & \mem{\FASTsunflowHBMem}	& \mem{\FASTsunflowFTOHBMem}	& \mem{\SLOWsunflowDCExcMem}	& \mem{\SLOWsunflowDCnoGExcMem}	& \mem{\SLOWsunflowCAPOExcMem}	& \mem{\SLOWsunflowCAPOnoGExcMem} \\
\bench{tomcat} 	& \et{\FASTtomcatEvents}   & \enfp{\FASTtomcatNoFPEvents}	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& \baseMem{\FASTtomcatBaseMem}   & \mem{\FASTtomcatFTMem}   & \mem{\FASTtomcatHBMem} 	& \mem{\FASTtomcatFTOHBMem}	& \mem{\SLOWtomcatDCExcMem}	& \mem{\SLOWtomcatDCnoGExcMem}	& \mem{\SLOWtomcatCAPOExcMem}	& \mem{\SLOWtomcatCAPOnoGExcMem} \\
\bench{xalan} 	& \et{\FASTxalanEvents}    & \enfp{\FASTxalanNoFPEvents}	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& \baseMem{\FASTxalanBaseMem}    & \mem{\FASTxalanFTMem}    & \mem{\FASTxalanHBMem}		& \mem{\FASTxalanFTOHBMem}		& \mem{\SLOWxalanDCExcMem}	& \mem{\SLOWxalanDCnoGExcMem} 	& \mem{\SLOWxalanCAPOExcMem}	& \mem{\SLOWxalanCAPOnoGExcMem}\\\hline
geomean	& &	& &	& & \mem{\FASTFTMemGeoMean} & \mem{\FASTHBMemGeoMean} & \mem{\FASTFTOHBMemGeoMean} & \mem{\SLOWDCExcMemGeoMean} & \mem{\SLOWDCnoGExcMemGeoMean} & \mem{\SLOWCAPOExcMemGeoMean} & \mem{\SLOWCAPOnoGExcMemGeoMean} \\
\mc{13}{c}{Memory usage} \\
\end{tabular}

\jake{Configuration: 10 trials, without setting cores, without stat collection but with new thread count methodology.
Unopt- updated.}

\caption{Run time and memory usage for FastTrack-based \HB analyses
and for unoptimized \DC and \CAPO analyses, relative to uninstrumented execution.}
\label{tab:performance:fasttrack}
\end{table}

%The following are three tables stacked together
% Table for geometric mean of all relations with various optimizations for all DaCapo benchmarks
\begin{table}[t]
\begin{empty}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_noCoresSet_noStatCollection}
%
\small
\centering
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWHBTimeGeoMean}			& \roh{\FASTFTOHBTimeGeoMean}	& \rna \\
\WCP	& \rna							& \roh{\SLOWWCPTimeGeoMean}			& \roh{\FASTFTOWCPTimeGeoMean}	& \roh{\FASTREWCPTimeGeoMean} \\
\DC		& \roh{\SLOWDCExcTimeGeoMean}	& \roh{\SLOWDCnoGExcTimeGeoMean}	& \roh{\FASTFTODCTimeGeoMean}	& \roh{\FASTREDCTimeGeoMean} \\
\CAPO	& \roh{\SLOWCAPOExcTimeGeoMean}	& \roh{\SLOWCAPOnoGExcTimeGeoMean}	& \roh{\FASTFTOCAPOTimeGeoMean}	& \roh{\FASTRECAPOTimeGeoMean} \\
\mc{2}{H}{} & \mc{3}{c}{Run time} \\
\end{tabular}
\hspace*{1em}
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \mem{\SLOWHBMemGeoMean}			& \mem{\FASTFTOHBMemGeoMean}	& \rna \\
\WCP	& \rna							& \mem{\SLOWWCPMemGeoMean}			& \mem{\FASTFTOWCPMemGeoMean}	& \mem{\FASTREWCPMemGeoMean} \\
\DC		& \mem{\SLOWDCExcMemGeoMean}	& \mem{\SLOWDCnoGExcMemGeoMean}	& \mem{\FASTFTODCMemGeoMean}	& \mem{\FASTREDCMemGeoMean} \\
\CAPO	& \mem{\SLOWCAPOExcMemGeoMean}	& \mem{\SLOWCAPOnoGExcMemGeoMean}	& \mem{\FASTFTOCAPOMemGeoMean}	& \mem{\FASTRECAPOMemGeoMean} \\
\mc{2}{H}{} & \mc{3}{c}{Memory usage} \\
\end{tabular}

\jake{Configuration: 10 trials, without setting cores, without stat collection but with new thread count methodology.
Unopt- updated.}

\caption{Geometric mean of run time and memory usage across the evaluated programs.}
\label{tab:performance:geoMean}
\end{empty}
\medskip
% Combined benchmarks table for 10 trials of all relations with various optimizations
\begin{empty}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_noCoresSet_noStatCollection}
%
\smaller
\centering
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWavroraHBTime}			& \roh{\FASTavroraFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWavroraWCPTime}			& \roh{\FASTavroraFTOWCPTime}	& \roh{\FASTavroraREWCPTime} \\
\DC		& \roh{\SLOWavroraDCExcTime}	& \roh{\SLOWavroraDCnoGExcTime}	& \roh{\FASTavroraFTODCTime}	& \roh{\FASTavroraREDCTime} \\
\CAPO	& \roh{\SLOWavroraCAPOExcTime}	& \roh{\SLOWavroraCAPOnoGExcTime}	& \roh{\FASTavroraFTOCAPOTime}	& \roh{\FASTavroraRECAPOTime} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWbatikHBTime}			& \roh{\FASTbatikFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWbatikWCPTime}			& \roh{\FASTbatikFTOWCPTime}	& \roh{\FASTbatikREWCPTime} \\
\DC		& \roh{\SLOWbatikDCExcTime}	& \roh{\SLOWbatikDCnoGExcTime}	& \roh{\FASTbatikFTODCTime}	& \roh{\FASTbatikREDCTime} \\
\CAPO	& \roh{\SLOWbatikCAPOExcTime}	& \roh{\SLOWbatikCAPOnoGExcTime}	& \roh{\FASTbatikFTOCAPOTime}	& \roh{\FASTbatikRECAPOTime} \\
		& \mc{4}{c}{\bench{batik}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWhtwoHBTime}			& \roh{\FASThtwoFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWhtwoWCPTime}			& \roh{\FASThtwoFTOWCPTime}	& \roh{\FASThtwoREWCPTime} \\
\DC		& \roh{\SLOWhtwoDCExcTime}	& \roh{\SLOWhtwoDCnoGExcTime}	& \roh{\FASThtwoFTODCTime}	& \roh{\FASThtwoREDCTime} \\
\CAPO	& \roh{\SLOWhtwoCAPOExcTime}	& \roh{\SLOWhtwoCAPOnoGExcTime}	& \roh{\FASThtwoFTOCAPOTime}	& \roh{\FASThtwoRECAPOTime} \\
		& \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWjythonHBTime}			& \roh{\FASTjythonFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWjythonWCPTime}			& \roh{\FASTjythonFTOWCPTime}	& \roh{\FASTjythonREWCPTime} \\
\DC		& \roh{\SLOWjythonDCExcTime}	& \roh{\SLOWjythonDCnoGExcTime}	& \roh{\FASTjythonFTODCTime}	& \roh{\FASTjythonREDCTime} \\
\CAPO	& \roh{\SLOWjythonCAPOExcTime}	& \roh{\SLOWjythonCAPOnoGExcTime}	& \roh{\FASTjythonFTOCAPOTime}	& \roh{\FASTjythonRECAPOTime} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWluindexHBTime}			& \roh{\FASTluindexFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWluindexWCPTime}			& \roh{\FASTluindexFTOWCPTime}	& \roh{\FASTluindexREWCPTime} \\
\DC		& \roh{\SLOWluindexDCExcTime}	& \roh{\SLOWluindexDCnoGExcTime}	& \roh{\FASTluindexFTODCTime}	& \roh{\FASTluindexREDCTime} \\
\CAPO	& \roh{\SLOWluindexCAPOExcTime}	& \roh{\SLOWluindexCAPOnoGExcTime}	& \roh{\FASTluindexFTOCAPOTime}	& \roh{\FASTluindexRECAPOTime} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWlusearchHBTime}			& \roh{\FASTlusearchFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWlusearchWCPTime}			& \roh{\FASTlusearchFTOWCPTime}	& \roh{\FASTlusearchREWCPTime} \\
\DC		& \roh{\SLOWlusearchDCExcTime}	& \roh{\SLOWlusearchDCnoGExcTime}	& \roh{\FASTlusearchFTODCTime}	& \roh{\FASTlusearchREDCTime} \\
\CAPO	& \roh{\SLOWlusearchCAPOExcTime}	& \roh{\SLOWlusearchCAPOnoGExcTime}	& \roh{\FASTlusearchFTOCAPOTime}	& \roh{\FASTlusearchRECAPOTime} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{lusearch}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWpmdHBTime}			& \roh{\FASTpmdFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWpmdWCPTime}			& \roh{\FASTpmdFTOWCPTime}	& \roh{\FASTpmdREWCPTime} \\
\DC		& \roh{\SLOWpmdDCExcTime}	& \roh{\SLOWpmdDCnoGExcTime}	& \roh{\FASTpmdFTODCTime}	& \roh{\FASTpmdREDCTime} \\
\CAPO	& \roh{\SLOWpmdCAPOExcTime}	& \roh{\SLOWpmdCAPOnoGExcTime}	& \roh{\FASTpmdFTOCAPOTime}	& \roh{\FASTpmdRECAPOTime} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWsunflowHBTime}			& \roh{\FASTsunflowFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWsunflowWCPTime}			& \roh{\FASTsunflowFTOWCPTime}	& \roh{\FASTsunflowREWCPTime} \\
\DC		& \roh{\SLOWsunflowDCExcTime}	& \roh{\SLOWsunflowDCnoGExcTime}	& \roh{\FASTsunflowFTODCTime}	& \roh{\FASTsunflowREDCTime} \\
\CAPO	& \roh{\SLOWsunflowCAPOExcTime}	& \roh{\SLOWsunflowCAPOnoGExcTime}	& \roh{\FASTsunflowFTOCAPOTime}	& \roh{\FASTsunflowRECAPOTime} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWtomcatHBTime}			& \roh{\FASTtomcatFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWtomcatWCPTime}			& \roh{\FASTtomcatFTOWCPTime}	& \roh{\FASTtomcatREWCPTime} \\
\DC		& \roh{\SLOWtomcatDCExcTime}	& \roh{\SLOWtomcatDCnoGExcTime}	& \roh{\FASTtomcatFTODCTime}	& \roh{\FASTtomcatREDCTime} \\
\CAPO	& \roh{\SLOWtomcatCAPOExcTime}	& \roh{\SLOWtomcatCAPOnoGExcTime}	& \roh{\FASTtomcatFTOCAPOTime}	& \roh{\FASTtomcatRECAPOTime} \\
		& \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWxalanHBTime}			& \roh{\FASTxalanFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWxalanWCPTime}			& \roh{\FASTxalanFTOWCPTime}	& \roh{\FASTxalanREWCPTime} \\
\DC		& \roh{\SLOWxalanDCExcTime}	& \roh{\SLOWxalanDCnoGExcTime}	& \roh{\FASTxalanFTODCTime}	& \roh{\FASTxalanREDCTime} \\
\CAPO	& \roh{\SLOWxalanCAPOExcTime}	& \roh{\SLOWxalanCAPOnoGExcTime}	& \roh{\FASTxalanFTOCAPOTime}	& \roh{\FASTxalanRECAPOTime} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\end{empty}

\jake{Configuration: 10 trials, without setting cores, without stat collection but with new thread count methodology.
Unopt- updated.}

\caption{Run time, relative to uninstrumented execution, of various analyses for each evaluated program.}
\label{tab:performance:allDaCapo}
\medskip
% Table for 10 trials of all relations with various optimizations for all DaCapo benchmarks
\begin{empty}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_noCoresSet_noStatCollection}
%
\smaller
\centering
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWavroraHBMem}		& \mem{\FASTavroraFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWavroraWCPMem}		& \mem{\FASTavroraFTOWCPMem}	& \mem{\FASTavroraREWCPMem} \\
\DC		& \mem{\SLOWavroraDCExcMem}	& \mem{\SLOWavroraDCnoGExcMem}	& \mem{\FASTavroraFTODCMem}		& \mem{\FASTavroraREDCMem} \\
\CAPO	& \mem{\SLOWavroraCAPOExcMem}	& \mem{\SLOWavroraCAPOnoGExcMem}& \mem{\FASTavroraFTOCAPOMem}	& \mem{\FASTavroraRECAPOMem} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWbatikHBMem}		& \mem{\FASTbatikFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWbatikWCPMem}		& \mem{\FASTbatikFTOWCPMem}	& \mem{\FASTbatikREWCPMem} \\
\DC		& \mem{\SLOWbatikDCExcMem}	& \mem{\SLOWbatikDCnoGExcMem}	& \mem{\FASTbatikFTODCMem}		& \mem{\FASTbatikREDCMem} \\
\CAPO	& \mem{\SLOWbatikCAPOExcMem}	& \mem{\SLOWbatikCAPOnoGExcMem}& \mem{\FASTbatikFTOCAPOMem}	& \mem{\FASTbatikRECAPOMem} \\
		& \mc{4}{c}{\bench{batik}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWhtwoHBMem}		& \mem{\FASThtwoFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWhtwoWCPMem}		& \mem{\FASThtwoFTOWCPMem}	& \mem{\FASThtwoREWCPMem} \\
\DC		& \mem{\SLOWhtwoDCExcMem}	& \mem{\SLOWhtwoDCnoGExcMem}	& \mem{\FASThtwoFTODCMem}		& \mem{\FASThtwoREDCMem} \\
\CAPO	& \mem{\SLOWhtwoCAPOExcMem}	& \mem{\SLOWhtwoCAPOnoGExcMem}& \mem{\FASThtwoFTOCAPOMem}	& \mem{\FASThtwoRECAPOMem} \\
		& \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWjythonHBMem}		& \mem{\FASTjythonFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWjythonWCPMem}		& \mem{\FASTjythonFTOWCPMem}	& \mem{\FASTjythonREWCPMem} \\
\DC		& \mem{\SLOWjythonDCExcMem}	& \mem{\SLOWjythonDCnoGExcMem}	& \mem{\FASTjythonFTODCMem}		& \mem{\FASTjythonREDCMem} \\
\CAPO	& \mem{\SLOWjythonCAPOExcMem}	& \mem{\SLOWjythonCAPOnoGExcMem}& \mem{\FASTjythonFTOCAPOMem}	& \mem{\FASTjythonRECAPOMem} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWluindexHBMem}		& \mem{\FASTluindexFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWluindexWCPMem}		& \mem{\FASTluindexFTOWCPMem}	& \mem{\FASTluindexREWCPMem} \\
\DC		& \mem{\SLOWluindexDCExcMem}	& \mem{\SLOWluindexDCnoGExcMem}	& \mem{\FASTluindexFTODCMem}		& \mem{\FASTluindexREDCMem} \\
\CAPO	& \mem{\SLOWluindexCAPOExcMem}	& \mem{\SLOWluindexCAPOnoGExcMem}& \mem{\FASTluindexFTOCAPOMem}	& \mem{\FASTluindexRECAPOMem} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWlusearchHBMem}		& \mem{\FASTlusearchFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWlusearchWCPMem}		& \mem{\FASTlusearchFTOWCPMem}	& \mem{\FASTlusearchREWCPMem} \\
\DC		& \mem{\SLOWlusearchDCExcMem}	& \mem{\SLOWlusearchDCnoGExcMem}	& \mem{\FASTlusearchFTODCMem}		& \mem{\FASTlusearchREDCMem} \\
\CAPO	& \mem{\SLOWlusearchCAPOExcMem}	& \mem{\SLOWlusearchCAPOnoGExcMem}& \mem{\FASTlusearchFTOCAPOMem}	& \mem{\FASTlusearchRECAPOMem} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{lusearch}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWpmdHBMem}		& \mem{\FASTpmdFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWpmdWCPMem}		& \mem{\FASTpmdFTOWCPMem}	& \mem{\FASTpmdREWCPMem} \\
\DC		& \mem{\SLOWpmdDCExcMem}	& \mem{\SLOWpmdDCnoGExcMem}	& \mem{\FASTpmdFTODCMem}		& \mem{\FASTpmdREDCMem} \\
\CAPO	& \mem{\SLOWpmdCAPOExcMem}	& \mem{\SLOWpmdCAPOnoGExcMem}& \mem{\FASTpmdFTOCAPOMem}	& \mem{\FASTpmdRECAPOMem} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWsunflowHBMem}		& \mem{\FASTsunflowFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWsunflowWCPMem}		& \mem{\FASTsunflowFTOWCPMem}	& \mem{\FASTsunflowREWCPMem} \\
\DC		& \mem{\SLOWsunflowDCExcMem}	& \mem{\SLOWsunflowDCnoGExcMem}	& \mem{\FASTsunflowFTODCMem}		& \mem{\FASTsunflowREDCMem} \\
\CAPO	& \mem{\SLOWsunflowCAPOExcMem}	& \mem{\SLOWsunflowCAPOnoGExcMem}& \mem{\FASTsunflowFTOCAPOMem}	& \mem{\FASTsunflowRECAPOMem} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWtomcatHBMem}		& \mem{\FASTtomcatFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWtomcatWCPMem}		& \mem{\FASTtomcatFTOWCPMem}	& \mem{\FASTtomcatREWCPMem} \\
\DC		& \mem{\SLOWtomcatDCExcMem}	& \mem{\SLOWtomcatDCnoGExcMem}	& \mem{\FASTtomcatFTODCMem}		& \mem{\FASTtomcatREDCMem} \\
\CAPO	& \mem{\SLOWtomcatCAPOExcMem}	& \mem{\SLOWtomcatCAPOnoGExcMem}& \mem{\FASTtomcatFTOCAPOMem}	& \mem{\FASTtomcatRECAPOMem} \\
		& \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWxalanHBMem}		& \mem{\FASTxalanFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWxalanWCPMem}		& \mem{\FASTxalanFTOWCPMem}	& \mem{\FASTxalanREWCPMem} \\
\DC		& \mem{\SLOWxalanDCExcMem}	& \mem{\SLOWxalanDCnoGExcMem}	& \mem{\FASTxalanFTODCMem}		& \mem{\FASTxalanREDCMem} \\
\CAPO	& \mem{\SLOWxalanCAPOExcMem}	& \mem{\SLOWxalanCAPOnoGExcMem}& \mem{\FASTxalanFTOCAPOMem}	& \mem{\FASTxalanRECAPOMem} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\end{empty}

\jake{Configuration: 10 trials, without setting cores, without stat collection but with new thread count methodology.
Unopt- updated.}

\caption{Memory usage, relative to uninstrumented execution, of various analyses for each evaluated program.}
\label{tab:memory:allDaCapo}
\end{table}

% Table for 10 trials of all relations with various optimizations for xalan benchmark
\begin{table}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
% \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;Mb$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\sdr}[2]{#1{\;}(#2)}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_noCoresSet_noStatCollection}
%
\smaller
\centering
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWavroraHB}{\SLOWavroraHBDynamic}					& \sdr{\FASTavroraFTOHB}{\FASTavroraFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWavroraWCP}{\SLOWavroraWCPDynamic}				& \sdr{\FASTavroraFTOWCP}{\FASTavroraFTOWCPDynamic}		& \sdr{\FASTavroraREWCP}{\FASTavroraREWCPDynamic} \\
\DC		& \sdr{\SLOWavroraDCExc}{\SLOWavroraDCExcDynamic}		& \sdr{\SLOWavroraDCnoGExc}{\SLOWavroraDCnoGExcDynamic}	& \sdr{\FASTavroraFTODC}{\FASTavroraFTODCDynamic}		& \sdr{\FASTavroraREDC}{\FASTavroraREDCDynamic} \\
\CAPO	& \sdr{\SLOWavroraCAPOExc}{\SLOWavroraCAPOExcDynamic}	& \sdr{\SLOWavroraCAPOnoGExc}{\SLOWavroraCAPOnoGExcDynamic}	& \sdr{\FASTavroraFTOCAPO}{\FASTavroraFTOCAPODynamic}	& \sdr{\FASTavroraRECAPO}{\FASTavroraRECAPODynamic} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWhtwoHB}{\SLOWhtwoHBDynamic}					& \sdr{\FASThtwoFTOHB}{\FASThtwoFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWhtwoWCP}{\SLOWhtwoWCPDynamic}				& \sdr{\FASThtwoFTOWCP}{\FASThtwoFTOWCPDynamic}		& \sdr{\FASThtwoREWCP}{\FASThtwoREWCPDynamic} \\
\DC		& \sdr{\SLOWhtwoDCExc}{\SLOWhtwoDCExcDynamic}		& \sdr{\SLOWhtwoDCnoGExc}{\SLOWhtwoDCnoGExcDynamic}	& \sdr{\FASThtwoFTODC}{\FASThtwoFTODCDynamic}		& \sdr{\FASThtwoREDC}{\FASThtwoREDCDynamic} \\
\CAPO	& \sdr{\SLOWhtwoCAPOExc}{\SLOWhtwoCAPOExcDynamic}	& \sdr{\SLOWhtwoCAPOnoGExc}{\SLOWhtwoCAPOnoGExcDynamic}	& \sdr{\FASThtwoFTOCAPO}{\FASThtwoFTOCAPODynamic}	& \sdr{\FASThtwoRECAPO}{\FASThtwoRECAPODynamic} \\
		& \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWjythonHB}{\SLOWjythonHBDynamic}					& \sdr{\FASTjythonFTOHB}{\FASTjythonFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWjythonWCP}{\SLOWjythonWCPDynamic}				& \sdr{\FASTjythonFTOWCP}{\FASTjythonFTOWCPDynamic}		& \sdr{\FASTjythonREWCP}{\FASTjythonREWCPDynamic} \\
\DC		& \sdr{\SLOWjythonDCExc}{\SLOWjythonDCExcDynamic}		& \sdr{\SLOWjythonDCnoGExc}{\SLOWjythonDCnoGExcDynamic}	& \sdr{\FASTjythonFTODC}{\FASTjythonFTODCDynamic}		& \sdr{\FASTjythonREDC}{\FASTjythonREDCDynamic} \\
\CAPO	& \sdr{\SLOWjythonCAPOExc}{\SLOWjythonCAPOExcDynamic}	& \sdr{\SLOWjythonCAPOnoGExc}{\SLOWjythonCAPOnoGExcDynamic}	& \sdr{\FASTjythonFTOCAPO}{\FASTjythonFTOCAPODynamic}	& \sdr{\FASTjythonRECAPO}{\FASTjythonRECAPODynamic} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWluindexHB}{\SLOWluindexHBDynamic}					& \sdr{\FASTluindexFTOHB}{\FASTluindexFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWluindexWCP}{\SLOWluindexWCPDynamic}				& \sdr{\FASTluindexFTOWCP}{\FASTluindexFTOWCPDynamic}		& \sdr{\FASTluindexREWCP}{\FASTluindexREWCPDynamic} \\
\DC		& \sdr{\SLOWluindexDCExc}{\SLOWluindexDCExcDynamic}		& \sdr{\SLOWluindexDCnoGExc}{\SLOWluindexDCnoGExcDynamic}	& \sdr{\FASTluindexFTODC}{\FASTluindexFTODCDynamic}		& \sdr{\FASTluindexREDC}{\FASTluindexREDCDynamic} \\
\CAPO	& \sdr{\SLOWluindexCAPOExc}{\SLOWluindexCAPOExcDynamic}	& \sdr{\SLOWluindexCAPOnoGExc}{\SLOWluindexCAPOnoGExcDynamic}	& \sdr{\FASTluindexFTOCAPO}{\FASTluindexFTOCAPODynamic}	& \sdr{\FASTluindexRECAPO}{\FASTluindexRECAPODynamic} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWpmdHB}{\SLOWpmdHBDynamic}					& \sdr{\FASTpmdFTOHB}{\FASTpmdFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWpmdWCP}{\SLOWpmdWCPDynamic}				& \sdr{\FASTpmdFTOWCP}{\FASTpmdFTOWCPDynamic}		& \sdr{\FASTpmdREWCP}{\FASTpmdREWCPDynamic} \\
\DC		& \sdr{\SLOWpmdDCExc}{\SLOWpmdDCExcDynamic}		& \sdr{\SLOWpmdDCnoGExc}{\SLOWpmdDCnoGExcDynamic}	& \sdr{\FASTpmdFTODC}{\FASTpmdFTODCDynamic}		& \sdr{\FASTpmdREDC}{\FASTpmdREDCDynamic} \\
\CAPO	& \sdr{\SLOWpmdCAPOExc}{\SLOWpmdCAPOExcDynamic}	& \sdr{\SLOWpmdCAPOnoGExc}{\SLOWpmdCAPOnoGExcDynamic}	& \sdr{\FASTpmdFTOCAPO}{\FASTpmdFTOCAPODynamic}	& \sdr{\FASTpmdRECAPO}{\FASTpmdRECAPODynamic} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWsunflowHB}{\SLOWsunflowHBDynamic}					& \sdr{\FASTsunflowFTOHB}{\FASTsunflowFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWsunflowWCP}{\SLOWsunflowWCPDynamic}				& \sdr{\FASTsunflowFTOWCP}{\FASTsunflowFTOWCPDynamic}		& \sdr{\FASTsunflowREWCP}{\FASTsunflowREWCPDynamic} \\
\DC		& \sdr{\SLOWsunflowDCExc}{\SLOWsunflowDCExcDynamic}		& \sdr{\SLOWsunflowDCnoGExc}{\SLOWsunflowDCnoGExcDynamic}	& \sdr{\FASTsunflowFTODC}{\FASTsunflowFTODCDynamic}		& \sdr{\FASTsunflowREDC}{\FASTsunflowREDCDynamic} \\
\CAPO	& \sdr{\SLOWsunflowCAPOExc}{\SLOWsunflowCAPOExcDynamic}	& \sdr{\SLOWsunflowCAPOnoGExc}{\SLOWsunflowCAPOnoGExcDynamic}	& \sdr{\FASTsunflowFTOCAPO}{\FASTsunflowFTOCAPODynamic}	& \sdr{\FASTsunflowRECAPO}{\FASTsunflowRECAPODynamic} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWtomcatHB}{\SLOWtomcatHBDynamic}					& \sdr{\FASTtomcatFTOHB}{\FASTtomcatFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWtomcatWCP}{\SLOWtomcatWCPDynamic}				& \sdr{\FASTtomcatFTOWCP}{\FASTtomcatFTOWCPDynamic}		& \sdr{\FASTtomcatREWCP}{\FASTtomcatREWCPDynamic} \\
\DC		& \sdr{\SLOWtomcatDCExc}{\SLOWtomcatDCExcDynamic}		& \sdr{\SLOWtomcatDCnoGExc}{\SLOWtomcatDCnoGExcDynamic}	& \sdr{\FASTtomcatFTODC}{\FASTtomcatFTODCDynamic}		& \sdr{\FASTtomcatREDC}{\FASTtomcatREDCDynamic} \\
\CAPO	& \sdr{\SLOWtomcatCAPOExc}{\SLOWtomcatCAPOExcDynamic}	& \sdr{\SLOWtomcatCAPOnoGExc}{\SLOWtomcatCAPOnoGExcDynamic}	& \sdr{\FASTtomcatFTOCAPO}{\FASTtomcatFTOCAPODynamic}	& \sdr{\FASTtomcatRECAPO}{\FASTtomcatRECAPODynamic} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWxalanHB}{\SLOWxalanHBDynamic}					& \sdr{\FASTxalanFTOHB}{\FASTxalanFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWxalanWCP}{\SLOWxalanWCPDynamic}				& \sdr{\FASTxalanFTOWCP}{\FASTxalanFTOWCPDynamic}		& \sdr{\FASTxalanREWCP}{\FASTxalanREWCPDynamic} \\
\DC		& \sdr{\SLOWxalanDCExc}{\SLOWxalanDCExcDynamic}		& \sdr{\SLOWxalanDCnoGExc}{\SLOWxalanDCnoGExcDynamic}	& \sdr{\FASTxalanFTODC}{\FASTxalanFTODCDynamic}		& \sdr{\FASTxalanREDC}{\FASTxalanREDCDynamic} \\
\CAPO	& \sdr{\SLOWxalanCAPOExc}{\SLOWxalanCAPOExcDynamic}	& \sdr{\SLOWxalanCAPOnoGExc}{\SLOWxalanCAPOnoGExcDynamic}	& \sdr{\FASTxalanFTOCAPO}{\FASTxalanFTOCAPODynamic}	& \sdr{\FASTxalanRECAPO}{\FASTxalanRECAPODynamic} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}

\jake{Configuration: 10 trials, without setting cores, without stat collection but with new thread count methodology.
Unopt- updated.}

\caption{Average races reported by various analyses for each evaluated program
(excluding \bench{batik} and \bench{lusearch}, for which all analyses report no races).
In each cell, the first value is statically distinct races
(\ie, distinct program locations) and the second value, in parentheses, is total dynamic races.}
\label{tab:race:allDaCapo}
\end{table}

%%%%%%%%%%%%%%%%%%%%New Set of Tables%%%%%%%%%%%%%%%%%%%%%%

\section{Results duplicating result tables for update extra metadata for ST-*}

%The following are three tables stacked together
% Table for geometric mean of all relations with various optimizations for all DaCapo benchmarks
\begin{table}[t]
\begin{empty}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOptQuiet}
%
\small
\centering
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWHBTimeGeoMean}			& \roh{\FASTFTOHBTimeGeoMean}	& \rna \\
\WCP	& \rna							& \roh{\SLOWWCPTimeGeoMean}			& \roh{\FASTFTOWCPTimeGeoMean}	& \roh{\FASTREWCPTimeGeoMean} \\
\DC		& \roh{\SLOWDCExcTimeGeoMean}	& \roh{\SLOWDCnoGExcTimeGeoMean}	& \roh{\FASTFTODCTimeGeoMean}	& \roh{\FASTREDCTimeGeoMean} \\
\CAPO	& \roh{\SLOWCAPOExcTimeGeoMean}	& \roh{\SLOWCAPOnoGExcTimeGeoMean}	& \roh{\FASTFTOCAPOTimeGeoMean}	& \roh{\FASTRECAPOTimeGeoMean} \\
\mc{2}{H}{} & \mc{3}{c}{Run time} \\
\end{tabular}
\hspace*{1em}
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \mem{\SLOWHBMemGeoMean}			& \mem{\FASTFTOHBMemGeoMean}	& \rna \\
\WCP	& \rna							& \mem{\SLOWWCPMemGeoMean}			& \mem{\FASTFTOWCPMemGeoMean}	& \mem{\FASTREWCPMemGeoMean} \\
\DC		& \mem{\SLOWDCExcMemGeoMean}	& \mem{\SLOWDCnoGExcMemGeoMean}	& \mem{\FASTFTODCMemGeoMean}	& \mem{\FASTREDCMemGeoMean} \\
\CAPO	& \mem{\SLOWCAPOExcMemGeoMean}	& \mem{\SLOWCAPOnoGExcMemGeoMean}	& \mem{\FASTFTOCAPOMemGeoMean}	& \mem{\FASTRECAPOMemGeoMean} \\
\mc{2}{H}{} & \mc{3}{c}{Memory usage} \\
\end{tabular}

\jake{Configuration: 10 trials, no stats collected.
Unopt-* results are the latest evaluation of removing setting cores to 8.
FTO-* and ST-* also remove setting cores to 8 and only initialize extra metadata if used.}

\caption{Geometric mean of run time and memory usage across the evaluated programs.}
\label{tab:performance:geoMean-Ex}
\end{empty}
\medskip
% Combined benchmarks table for 10 trials of all relations with various optimizations
\begin{empty}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOptQuiet}
%
\smaller
\centering
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWavroraHBTime}			& \roh{\FASTavroraFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWavroraWCPTime}			& \roh{\FASTavroraFTOWCPTime}	& \roh{\FASTavroraREWCPTime} \\
\DC		& \roh{\SLOWavroraDCExcTime}	& \roh{\SLOWavroraDCnoGExcTime}	& \roh{\FASTavroraFTODCTime}	& \roh{\FASTavroraREDCTime} \\
\CAPO	& \roh{\SLOWavroraCAPOExcTime}	& \roh{\SLOWavroraCAPOnoGExcTime}	& \roh{\FASTavroraFTOCAPOTime}	& \roh{\FASTavroraRECAPOTime} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWbatikHBTime}			& \roh{\FASTbatikFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWbatikWCPTime}			& \roh{\FASTbatikFTOWCPTime}	& \roh{\FASTbatikREWCPTime} \\
\DC		& \roh{\SLOWbatikDCExcTime}	& \roh{\SLOWbatikDCnoGExcTime}	& \roh{\FASTbatikFTODCTime}	& \roh{\FASTbatikREDCTime} \\
\CAPO	& \roh{\SLOWbatikCAPOExcTime}	& \roh{\SLOWbatikCAPOnoGExcTime}	& \roh{\FASTbatikFTOCAPOTime}	& \roh{\FASTbatikRECAPOTime} \\
		& \mc{4}{c}{\bench{batik}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWhtwoHBTime}			& \roh{\FASThtwoFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWhtwoWCPTime}			& \roh{\FASThtwoFTOWCPTime}	& \roh{\FASThtwoREWCPTime} \\
\DC		& \roh{\SLOWhtwoDCExcTime}	& \roh{\SLOWhtwoDCnoGExcTime}	& \roh{\FASThtwoFTODCTime}	& \roh{\FASThtwoREDCTime} \\
\CAPO	& \roh{\SLOWhtwoCAPOExcTime}	& \roh{\SLOWhtwoCAPOnoGExcTime}	& \roh{\FASThtwoFTOCAPOTime}	& \roh{\FASThtwoRECAPOTime} \\
		& \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWjythonHBTime}			& \roh{\FASTjythonFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWjythonWCPTime}			& \roh{\FASTjythonFTOWCPTime}	& \roh{\FASTjythonREWCPTime} \\
\DC		& \roh{\SLOWjythonDCExcTime}	& \roh{\SLOWjythonDCnoGExcTime}	& \roh{\FASTjythonFTODCTime}	& \roh{\FASTjythonREDCTime} \\
\CAPO	& \roh{\SLOWjythonCAPOExcTime}	& \roh{\SLOWjythonCAPOnoGExcTime}	& \roh{\FASTjythonFTOCAPOTime}	& \roh{\FASTjythonRECAPOTime} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWluindexHBTime}			& \roh{\FASTluindexFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWluindexWCPTime}			& \roh{\FASTluindexFTOWCPTime}	& \roh{\FASTluindexREWCPTime} \\
\DC		& \roh{\SLOWluindexDCExcTime}	& \roh{\SLOWluindexDCnoGExcTime}	& \roh{\FASTluindexFTODCTime}	& \roh{\FASTluindexREDCTime} \\
\CAPO	& \roh{\SLOWluindexCAPOExcTime}	& \roh{\SLOWluindexCAPOnoGExcTime}	& \roh{\FASTluindexFTOCAPOTime}	& \roh{\FASTluindexRECAPOTime} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWlusearchHBTime}			& \roh{\FASTlusearchFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWlusearchWCPTime}			& \roh{\FASTlusearchFTOWCPTime}	& \roh{\FASTlusearchREWCPTime} \\
\DC		& \roh{\SLOWlusearchDCExcTime}	& \roh{\SLOWlusearchDCnoGExcTime}	& \roh{\FASTlusearchFTODCTime}	& \roh{\FASTlusearchREDCTime} \\
\CAPO	& \roh{\SLOWlusearchCAPOExcTime}	& \roh{\SLOWlusearchCAPOnoGExcTime}	& \roh{\FASTlusearchFTOCAPOTime}	& \roh{\FASTlusearchRECAPOTime} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{lusearch}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWpmdHBTime}			& \roh{\FASTpmdFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWpmdWCPTime}			& \roh{\FASTpmdFTOWCPTime}	& \roh{\FASTpmdREWCPTime} \\
\DC		& \roh{\SLOWpmdDCExcTime}	& \roh{\SLOWpmdDCnoGExcTime}	& \roh{\FASTpmdFTODCTime}	& \roh{\FASTpmdREDCTime} \\
\CAPO	& \roh{\SLOWpmdCAPOExcTime}	& \roh{\SLOWpmdCAPOnoGExcTime}	& \roh{\FASTpmdFTOCAPOTime}	& \roh{\FASTpmdRECAPOTime} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWsunflowHBTime}			& \roh{\FASTsunflowFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWsunflowWCPTime}			& \roh{\FASTsunflowFTOWCPTime}	& \roh{\FASTsunflowREWCPTime} \\
\DC		& \roh{\SLOWsunflowDCExcTime}	& \roh{\SLOWsunflowDCnoGExcTime}	& \roh{\FASTsunflowFTODCTime}	& \roh{\FASTsunflowREDCTime} \\
\CAPO	& \roh{\SLOWsunflowCAPOExcTime}	& \roh{\SLOWsunflowCAPOnoGExcTime}	& \roh{\FASTsunflowFTOCAPOTime}	& \roh{\FASTsunflowRECAPOTime} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWtomcatHBTime}			& \roh{\FASTtomcatFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWtomcatWCPTime}			& \roh{\FASTtomcatFTOWCPTime}	& \roh{\FASTtomcatREWCPTime} \\
\DC		& \roh{\SLOWtomcatDCExcTime}	& \roh{\SLOWtomcatDCnoGExcTime}	& \roh{\FASTtomcatFTODCTime}	& \roh{\FASTtomcatREDCTime} \\
\CAPO	& \roh{\SLOWtomcatCAPOExcTime}	& \roh{\SLOWtomcatCAPOnoGExcTime}	& \roh{\FASTtomcatFTOCAPOTime}	& \roh{\FASTtomcatRECAPOTime} \\
		& \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWxalanHBTime}			& \roh{\FASTxalanFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWxalanWCPTime}			& \roh{\FASTxalanFTOWCPTime}	& \roh{\FASTxalanREWCPTime} \\
\DC		& \roh{\SLOWxalanDCExcTime}	& \roh{\SLOWxalanDCnoGExcTime}	& \roh{\FASTxalanFTODCTime}	& \roh{\FASTxalanREDCTime} \\
\CAPO	& \roh{\SLOWxalanCAPOExcTime}	& \roh{\SLOWxalanCAPOnoGExcTime}	& \roh{\FASTxalanFTOCAPOTime}	& \roh{\FASTxalanRECAPOTime} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\end{empty}

\jake{Configuration: 10 trials, no stats collected.
Unopt-* results are the latest evaluation of removing setting cores to 8.
FTO-* and ST-* also remove setting cores to 8 and only initialize extra metadata if used.}
\caption{Run time, relative to uninstrumented execution, of various analyses for each evaluated program.}
\label{tab:performance:allDaCapo}
\medskip
% Table for 10 trials of all relations with various optimizations for all DaCapo benchmarks
\begin{empty}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOptQuiet}
%
\smaller
\centering
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWavroraHBMem}		& \mem{\FASTavroraFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWavroraWCPMem}		& \mem{\FASTavroraFTOWCPMem}	& \mem{\FASTavroraREWCPMem} \\
\DC		& \mem{\SLOWavroraDCExcMem}	& \mem{\SLOWavroraDCnoGExcMem}	& \mem{\FASTavroraFTODCMem}		& \mem{\FASTavroraREDCMem} \\
\CAPO	& \mem{\SLOWavroraCAPOExcMem}	& \mem{\SLOWavroraCAPOnoGExcMem}& \mem{\FASTavroraFTOCAPOMem}	& \mem{\FASTavroraRECAPOMem} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWbatikHBMem}		& \mem{\FASTbatikFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWbatikWCPMem}		& \mem{\FASTbatikFTOWCPMem}	& \mem{\FASTbatikREWCPMem} \\
\DC		& \mem{\SLOWbatikDCExcMem}	& \mem{\SLOWbatikDCnoGExcMem}	& \mem{\FASTbatikFTODCMem}		& \mem{\FASTbatikREDCMem} \\
\CAPO	& \mem{\SLOWbatikCAPOExcMem}	& \mem{\SLOWbatikCAPOnoGExcMem}& \mem{\FASTbatikFTOCAPOMem}	& \mem{\FASTbatikRECAPOMem} \\
		& \mc{4}{c}{\bench{batik}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWhtwoHBMem}		& \mem{\FASThtwoFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWhtwoWCPMem}		& \mem{\FASThtwoFTOWCPMem}	& \mem{\FASThtwoREWCPMem} \\
\DC		& \mem{\SLOWhtwoDCExcMem}	& \mem{\SLOWhtwoDCnoGExcMem}	& \mem{\FASThtwoFTODCMem}		& \mem{\FASThtwoREDCMem} \\
\CAPO	& \mem{\SLOWhtwoCAPOExcMem}	& \mem{\SLOWhtwoCAPOnoGExcMem}& \mem{\FASThtwoFTOCAPOMem}	& \mem{\FASThtwoRECAPOMem} \\
		& \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWjythonHBMem}		& \mem{\FASTjythonFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWjythonWCPMem}		& \mem{\FASTjythonFTOWCPMem}	& \mem{\FASTjythonREWCPMem} \\
\DC		& \mem{\SLOWjythonDCExcMem}	& \mem{\SLOWjythonDCnoGExcMem}	& \mem{\FASTjythonFTODCMem}		& \mem{\FASTjythonREDCMem} \\
\CAPO	& \mem{\SLOWjythonCAPOExcMem}	& \mem{\SLOWjythonCAPOnoGExcMem}& \mem{\FASTjythonFTOCAPOMem}	& \mem{\FASTjythonRECAPOMem} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWluindexHBMem}		& \mem{\FASTluindexFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWluindexWCPMem}		& \mem{\FASTluindexFTOWCPMem}	& \mem{\FASTluindexREWCPMem} \\
\DC		& \mem{\SLOWluindexDCExcMem}	& \mem{\SLOWluindexDCnoGExcMem}	& \mem{\FASTluindexFTODCMem}		& \mem{\FASTluindexREDCMem} \\
\CAPO	& \mem{\SLOWluindexCAPOExcMem}	& \mem{\SLOWluindexCAPOnoGExcMem}& \mem{\FASTluindexFTOCAPOMem}	& \mem{\FASTluindexRECAPOMem} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWlusearchHBMem}		& \mem{\FASTlusearchFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWlusearchWCPMem}		& \mem{\FASTlusearchFTOWCPMem}	& \mem{\FASTlusearchREWCPMem} \\
\DC		& \mem{\SLOWlusearchDCExcMem}	& \mem{\SLOWlusearchDCnoGExcMem}	& \mem{\FASTlusearchFTODCMem}		& \mem{\FASTlusearchREDCMem} \\
\CAPO	& \mem{\SLOWlusearchCAPOExcMem}	& \mem{\SLOWlusearchCAPOnoGExcMem}& \mem{\FASTlusearchFTOCAPOMem}	& \mem{\FASTlusearchRECAPOMem} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{lusearch}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWpmdHBMem}		& \mem{\FASTpmdFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWpmdWCPMem}		& \mem{\FASTpmdFTOWCPMem}	& \mem{\FASTpmdREWCPMem} \\
\DC		& \mem{\SLOWpmdDCExcMem}	& \mem{\SLOWpmdDCnoGExcMem}	& \mem{\FASTpmdFTODCMem}		& \mem{\FASTpmdREDCMem} \\
\CAPO	& \mem{\SLOWpmdCAPOExcMem}	& \mem{\SLOWpmdCAPOnoGExcMem}& \mem{\FASTpmdFTOCAPOMem}	& \mem{\FASTpmdRECAPOMem} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWsunflowHBMem}		& \mem{\FASTsunflowFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWsunflowWCPMem}		& \mem{\FASTsunflowFTOWCPMem}	& \mem{\FASTsunflowREWCPMem} \\
\DC		& \mem{\SLOWsunflowDCExcMem}	& \mem{\SLOWsunflowDCnoGExcMem}	& \mem{\FASTsunflowFTODCMem}		& \mem{\FASTsunflowREDCMem} \\
\CAPO	& \mem{\SLOWsunflowCAPOExcMem}	& \mem{\SLOWsunflowCAPOnoGExcMem}& \mem{\FASTsunflowFTOCAPOMem}	& \mem{\FASTsunflowRECAPOMem} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWtomcatHBMem}		& \mem{\FASTtomcatFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWtomcatWCPMem}		& \mem{\FASTtomcatFTOWCPMem}	& \mem{\FASTtomcatREWCPMem} \\
\DC		& \mem{\SLOWtomcatDCExcMem}	& \mem{\SLOWtomcatDCnoGExcMem}	& \mem{\FASTtomcatFTODCMem}		& \mem{\FASTtomcatREDCMem} \\
\CAPO	& \mem{\SLOWtomcatCAPOExcMem}	& \mem{\SLOWtomcatCAPOnoGExcMem}& \mem{\FASTtomcatFTOCAPOMem}	& \mem{\FASTtomcatRECAPOMem} \\
		& \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWxalanHBMem}		& \mem{\FASTxalanFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWxalanWCPMem}		& \mem{\FASTxalanFTOWCPMem}	& \mem{\FASTxalanREWCPMem} \\
\DC		& \mem{\SLOWxalanDCExcMem}	& \mem{\SLOWxalanDCnoGExcMem}	& \mem{\FASTxalanFTODCMem}		& \mem{\FASTxalanREDCMem} \\
\CAPO	& \mem{\SLOWxalanCAPOExcMem}	& \mem{\SLOWxalanCAPOnoGExcMem}& \mem{\FASTxalanFTOCAPOMem}	& \mem{\FASTxalanRECAPOMem} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\end{empty}

\jake{Configuration: 10 trials, no stats collected.
Unopt-* results are the latest evaluation of removing setting cores to 8.
FTO-* and ST-* also remove setting cores to 8 and only initialize extra metadata if used.}

\caption{Memory usage, relative to uninstrumented execution, of various analyses for each evaluated program.}
\label{tab:memory:allDaCapo}
\end{table}

% Table for 10 trials of all relations with various optimizations for xalan benchmark
\begin{table}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
% \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;Mb$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\sdr}[2]{#1{\;}(#2)}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOptQuiet}
%
\smaller
\centering
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWavroraHB}{\SLOWavroraHBDynamic}					& \sdr{\FASTavroraFTOHB}{\FASTavroraFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWavroraWCP}{\SLOWavroraWCPDynamic}				& \sdr{\FASTavroraFTOWCP}{\FASTavroraFTOWCPDynamic}		& \sdr{\FASTavroraREWCP}{\FASTavroraREWCPDynamic} \\
\DC		& \sdr{\SLOWavroraDCExc}{\SLOWavroraDCExcDynamic}		& \sdr{\SLOWavroraDCnoGExc}{\SLOWavroraDCnoGExcDynamic}	& \sdr{\FASTavroraFTODC}{\FASTavroraFTODCDynamic}		& \sdr{\FASTavroraREDC}{\FASTavroraREDCDynamic} \\
\CAPO	& \sdr{\SLOWavroraCAPOExc}{\SLOWavroraCAPOExcDynamic}	& \sdr{\SLOWavroraCAPOnoGExc}{\SLOWavroraCAPOnoGExcDynamic}	& \sdr{\FASTavroraFTOCAPO}{\FASTavroraFTOCAPODynamic}	& \sdr{\FASTavroraRECAPO}{\FASTavroraRECAPODynamic} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWhtwoHB}{\SLOWhtwoHBDynamic}					& \sdr{\FASThtwoFTOHB}{\FASThtwoFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWhtwoWCP}{\SLOWhtwoWCPDynamic}				& \sdr{\FASThtwoFTOWCP}{\FASThtwoFTOWCPDynamic}		& \sdr{\FASThtwoREWCP}{\FASThtwoREWCPDynamic} \\
\DC		& \sdr{\SLOWhtwoDCExc}{\SLOWhtwoDCExcDynamic}		& \sdr{\SLOWhtwoDCnoGExc}{\SLOWhtwoDCnoGExcDynamic}	& \sdr{\FASThtwoFTODC}{\FASThtwoFTODCDynamic}		& \sdr{\FASThtwoREDC}{\FASThtwoREDCDynamic} \\
\CAPO	& \sdr{\SLOWhtwoCAPOExc}{\SLOWhtwoCAPOExcDynamic}	& \sdr{\SLOWhtwoCAPOnoGExc}{\SLOWhtwoCAPOnoGExcDynamic}	& \sdr{\FASThtwoFTOCAPO}{\FASThtwoFTOCAPODynamic}	& \sdr{\FASThtwoRECAPO}{\FASThtwoRECAPODynamic} \\
		& \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWjythonHB}{\SLOWjythonHBDynamic}					& \sdr{\FASTjythonFTOHB}{\FASTjythonFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWjythonWCP}{\SLOWjythonWCPDynamic}				& \sdr{\FASTjythonFTOWCP}{\FASTjythonFTOWCPDynamic}		& \sdr{\FASTjythonREWCP}{\FASTjythonREWCPDynamic} \\
\DC		& \sdr{\SLOWjythonDCExc}{\SLOWjythonDCExcDynamic}		& \sdr{\SLOWjythonDCnoGExc}{\SLOWjythonDCnoGExcDynamic}	& \sdr{\FASTjythonFTODC}{\FASTjythonFTODCDynamic}		& \sdr{\FASTjythonREDC}{\FASTjythonREDCDynamic} \\
\CAPO	& \sdr{\SLOWjythonCAPOExc}{\SLOWjythonCAPOExcDynamic}	& \sdr{\SLOWjythonCAPOnoGExc}{\SLOWjythonCAPOnoGExcDynamic}	& \sdr{\FASTjythonFTOCAPO}{\FASTjythonFTOCAPODynamic}	& \sdr{\FASTjythonRECAPO}{\FASTjythonRECAPODynamic} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWluindexHB}{\SLOWluindexHBDynamic}					& \sdr{\FASTluindexFTOHB}{\FASTluindexFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWluindexWCP}{\SLOWluindexWCPDynamic}				& \sdr{\FASTluindexFTOWCP}{\FASTluindexFTOWCPDynamic}		& \sdr{\FASTluindexREWCP}{\FASTluindexREWCPDynamic} \\
\DC		& \sdr{\SLOWluindexDCExc}{\SLOWluindexDCExcDynamic}		& \sdr{\SLOWluindexDCnoGExc}{\SLOWluindexDCnoGExcDynamic}	& \sdr{\FASTluindexFTODC}{\FASTluindexFTODCDynamic}		& \sdr{\FASTluindexREDC}{\FASTluindexREDCDynamic} \\
\CAPO	& \sdr{\SLOWluindexCAPOExc}{\SLOWluindexCAPOExcDynamic}	& \sdr{\SLOWluindexCAPOnoGExc}{\SLOWluindexCAPOnoGExcDynamic}	& \sdr{\FASTluindexFTOCAPO}{\FASTluindexFTOCAPODynamic}	& \sdr{\FASTluindexRECAPO}{\FASTluindexRECAPODynamic} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWpmdHB}{\SLOWpmdHBDynamic}					& \sdr{\FASTpmdFTOHB}{\FASTpmdFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWpmdWCP}{\SLOWpmdWCPDynamic}				& \sdr{\FASTpmdFTOWCP}{\FASTpmdFTOWCPDynamic}		& \sdr{\FASTpmdREWCP}{\FASTpmdREWCPDynamic} \\
\DC		& \sdr{\SLOWpmdDCExc}{\SLOWpmdDCExcDynamic}		& \sdr{\SLOWpmdDCnoGExc}{\SLOWpmdDCnoGExcDynamic}	& \sdr{\FASTpmdFTODC}{\FASTpmdFTODCDynamic}		& \sdr{\FASTpmdREDC}{\FASTpmdREDCDynamic} \\
\CAPO	& \sdr{\SLOWpmdCAPOExc}{\SLOWpmdCAPOExcDynamic}	& \sdr{\SLOWpmdCAPOnoGExc}{\SLOWpmdCAPOnoGExcDynamic}	& \sdr{\FASTpmdFTOCAPO}{\FASTpmdFTOCAPODynamic}	& \sdr{\FASTpmdRECAPO}{\FASTpmdRECAPODynamic} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWsunflowHB}{\SLOWsunflowHBDynamic}					& \sdr{\FASTsunflowFTOHB}{\FASTsunflowFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWsunflowWCP}{\SLOWsunflowWCPDynamic}				& \sdr{\FASTsunflowFTOWCP}{\FASTsunflowFTOWCPDynamic}		& \sdr{\FASTsunflowREWCP}{\FASTsunflowREWCPDynamic} \\
\DC		& \sdr{\SLOWsunflowDCExc}{\SLOWsunflowDCExcDynamic}		& \sdr{\SLOWsunflowDCnoGExc}{\SLOWsunflowDCnoGExcDynamic}	& \sdr{\FASTsunflowFTODC}{\FASTsunflowFTODCDynamic}		& \sdr{\FASTsunflowREDC}{\FASTsunflowREDCDynamic} \\
\CAPO	& \sdr{\SLOWsunflowCAPOExc}{\SLOWsunflowCAPOExcDynamic}	& \sdr{\SLOWsunflowCAPOnoGExc}{\SLOWsunflowCAPOnoGExcDynamic}	& \sdr{\FASTsunflowFTOCAPO}{\FASTsunflowFTOCAPODynamic}	& \sdr{\FASTsunflowRECAPO}{\FASTsunflowRECAPODynamic} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWtomcatHB}{\SLOWtomcatHBDynamic}					& \sdr{\FASTtomcatFTOHB}{\FASTtomcatFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWtomcatWCP}{\SLOWtomcatWCPDynamic}				& \sdr{\FASTtomcatFTOWCP}{\FASTtomcatFTOWCPDynamic}		& \sdr{\FASTtomcatREWCP}{\FASTtomcatREWCPDynamic} \\
\DC		& \sdr{\SLOWtomcatDCExc}{\SLOWtomcatDCExcDynamic}		& \sdr{\SLOWtomcatDCnoGExc}{\SLOWtomcatDCnoGExcDynamic}	& \sdr{\FASTtomcatFTODC}{\FASTtomcatFTODCDynamic}		& \sdr{\FASTtomcatREDC}{\FASTtomcatREDCDynamic} \\
\CAPO	& \sdr{\SLOWtomcatCAPOExc}{\SLOWtomcatCAPOExcDynamic}	& \sdr{\SLOWtomcatCAPOnoGExc}{\SLOWtomcatCAPOnoGExcDynamic}	& \sdr{\FASTtomcatFTOCAPO}{\FASTtomcatFTOCAPODynamic}	& \sdr{\FASTtomcatRECAPO}{\FASTtomcatRECAPODynamic} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWxalanHB}{\SLOWxalanHBDynamic}					& \sdr{\FASTxalanFTOHB}{\FASTxalanFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWxalanWCP}{\SLOWxalanWCPDynamic}				& \sdr{\FASTxalanFTOWCP}{\FASTxalanFTOWCPDynamic}		& \sdr{\FASTxalanREWCP}{\FASTxalanREWCPDynamic} \\
\DC		& \sdr{\SLOWxalanDCExc}{\SLOWxalanDCExcDynamic}		& \sdr{\SLOWxalanDCnoGExc}{\SLOWxalanDCnoGExcDynamic}	& \sdr{\FASTxalanFTODC}{\FASTxalanFTODCDynamic}		& \sdr{\FASTxalanREDC}{\FASTxalanREDCDynamic} \\
\CAPO	& \sdr{\SLOWxalanCAPOExc}{\SLOWxalanCAPOExcDynamic}	& \sdr{\SLOWxalanCAPOnoGExc}{\SLOWxalanCAPOnoGExcDynamic}	& \sdr{\FASTxalanFTOCAPO}{\FASTxalanFTOCAPODynamic}	& \sdr{\FASTxalanRECAPO}{\FASTxalanRECAPODynamic} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}

\jake{Configuration: 10 trials, no stats collected.
Unopt-* results are the latest evaluation of removing setting cores to 8.
FTO-* and ST-* also remove setting cores to 8 and only initialize extra metadata if used.}

\caption{Average races reported by various analyses for each evaluated program
(excluding \bench{batik} and \bench{lusearch}, for which all analyses report no races).
In each cell, the first value is statically distinct races
(\ie, distinct program locations) and the second value, in parentheses, is total dynamic races.}
\label{tab:race:allDaCapo}
\end{table}

\section{Results duplicating result tables for different configuration
including confidence intervals}

\begin{table}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
% \input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOptQuiet}
%
\small
\centering
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWavroraHBTime}{\SLOWavroraHBTimeCI}			& \vci{\FASTavroraFTOHBTime}{\FASTavroraFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWavroraWCPTime}{\SLOWavroraWCPTimeCI}			& \vci{\FASTavroraFTOWCPTime}{\FASTavroraFTOWCPTimeCI}	& \vci{\FASTavroraREWCPTime}{\FASTavroraREWCPTimeCI} \\
\DC		& \vci{\SLOWavroraDCExcTime}{\SLOWavroraDCExcTimeCI}	& \vci{\SLOWavroraDCnoGExcTime}{\SLOWavroraDCnoGExcTimeCI}	& \vci{\FASTavroraFTODCTime}{\FASTavroraFTODCTimeCI}	& \vci{\FASTavroraREDCTime}{\FASTavroraREDCTimeCI} \\
\CAPO	& \vci{\SLOWavroraCAPOExcTime}{\SLOWavroraCAPOExcTimeCI}	& \vci{\SLOWavroraCAPOnoGExcTime}{\SLOWavroraCAPOnoGExcTimeCI}	& \vci{\FASTavroraFTOCAPOTime}{\FASTavroraFTOCAPOTimeCI}	& \vci{\FASTavroraRECAPOTime}{\FASTavroraRECAPOTimeCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWbatikHBTime}{\SLOWbatikHBTimeCI}			& \vci{\FASTbatikFTOHBTime}{\FASTbatikFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWbatikWCPTime}{\SLOWbatikWCPTimeCI}			& \vci{\FASTbatikFTOWCPTime}{\FASTbatikFTOWCPTimeCI}	& \vci{\FASTbatikREWCPTime}{\FASTbatikREWCPTimeCI} \\
\DC		& \vci{\SLOWbatikDCExcTime}{\SLOWbatikDCExcTimeCI}	& \vci{\SLOWbatikDCnoGExcTime}{\SLOWbatikDCnoGExcTimeCI}	& \vci{\FASTbatikFTODCTime}{\FASTbatikFTODCTimeCI}	& \vci{\FASTbatikREDCTime}{\FASTbatikREDCTimeCI} \\
\CAPO	& \vci{\SLOWbatikCAPOExcTime}{\SLOWbatikCAPOExcTimeCI}	& \vci{\SLOWbatikCAPOnoGExcTime}{\SLOWbatikCAPOnoGExcTimeCI}	& \vci{\FASTbatikFTOCAPOTime}{\FASTbatikFTOCAPOTimeCI}	& \vci{\FASTbatikRECAPOTime}{\FASTbatikRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{batik}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWhtwoHBTime}{\SLOWhtwoHBTimeCI}			& \vci{\FASThtwoFTOHBTime}{\FASThtwoFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWhtwoWCPTime}{\SLOWhtwoWCPTimeCI}			& \vci{\FASThtwoFTOWCPTime}{\FASThtwoFTOWCPTimeCI}	& \vci{\FASThtwoREWCPTime}{\FASThtwoREWCPTimeCI} \\
\DC		& \vci{\SLOWhtwoDCExcTime}{\SLOWhtwoDCExcTimeCI}	& \vci{\SLOWhtwoDCnoGExcTime}{\SLOWhtwoDCnoGExcTimeCI}	& \vci{\FASThtwoFTODCTime}{\FASThtwoFTODCTimeCI}	& \vci{\FASThtwoREDCTime}{\FASThtwoREDCTimeCI} \\
\CAPO	& \vci{\SLOWhtwoCAPOExcTime}{\SLOWhtwoCAPOExcTimeCI}	& \vci{\SLOWhtwoCAPOnoGExcTime}{\SLOWhtwoCAPOnoGExcTimeCI}	& \vci{\FASThtwoFTOCAPOTime}{\FASThtwoFTOCAPOTimeCI}	& \vci{\FASThtwoRECAPOTime}{\FASThtwoRECAPOTimeCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWjythonHBTime}{\SLOWjythonHBTimeCI}			& \vci{\FASTjythonFTOHBTime}{\FASTjythonFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWjythonWCPTime}{\SLOWjythonWCPTimeCI}			& \vci{\FASTjythonFTOWCPTime}{\FASTjythonFTOWCPTimeCI}	& \vci{\FASTjythonREWCPTime}{\FASTjythonREWCPTimeCI} \\
\DC		& \vci{\SLOWjythonDCExcTime}{\SLOWjythonDCExcTimeCI}	& \vci{\SLOWjythonDCnoGExcTime}{\SLOWjythonDCnoGExcTimeCI}	& \vci{\FASTjythonFTODCTime}{\FASTjythonFTODCTimeCI}	& \vci{\FASTjythonREDCTime}{\FASTjythonREDCTimeCI} \\
\CAPO	& \vci{\SLOWjythonCAPOExcTime}{\SLOWjythonCAPOExcTimeCI}	& \vci{\SLOWjythonCAPOnoGExcTime}{\SLOWjythonCAPOnoGExcTimeCI}	& \vci{\FASTjythonFTOCAPOTime}{\FASTjythonFTOCAPOTimeCI}	& \vci{\FASTjythonRECAPOTime}{\FASTjythonRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWluindexHBTime}{\SLOWluindexHBTimeCI}			& \vci{\FASTluindexFTOHBTime}{\FASTluindexFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWluindexWCPTime}{\SLOWluindexWCPTimeCI}			& \vci{\FASTluindexFTOWCPTime}{\FASTluindexFTOWCPTimeCI}	& \vci{\FASTluindexREWCPTime}{\FASTluindexREWCPTimeCI} \\
\DC		& \vci{\SLOWluindexDCExcTime}{\SLOWluindexDCExcTimeCI}	& \vci{\SLOWluindexDCnoGExcTime}{\SLOWluindexDCnoGExcTimeCI}	& \vci{\FASTluindexFTODCTime}{\FASTluindexFTODCTimeCI}	& \vci{\FASTluindexREDCTime}{\FASTluindexREDCTimeCI} \\
\CAPO	& \vci{\SLOWluindexCAPOExcTime}{\SLOWluindexCAPOExcTimeCI}	& \vci{\SLOWluindexCAPOnoGExcTime}{\SLOWluindexCAPOnoGExcTimeCI}	& \vci{\FASTluindexFTOCAPOTime}{\FASTluindexFTOCAPOTimeCI}	& \vci{\FASTluindexRECAPOTime}{\FASTluindexRECAPOTimeCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWlusearchHBTime}{\SLOWlusearchHBTimeCI}			& \vci{\FASTlusearchFTOHBTime}{\FASTlusearchFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWlusearchWCPTime}{\SLOWlusearchWCPTimeCI}			& \vci{\FASTlusearchFTOWCPTime}{\FASTlusearchFTOWCPTimeCI}	& \vci{\FASTlusearchREWCPTime}{\FASTlusearchREWCPTimeCI} \\
\DC		& \vci{\SLOWlusearchDCExcTime}{\SLOWlusearchDCExcTimeCI}	& \vci{\SLOWlusearchDCnoGExcTime}{\SLOWlusearchDCnoGExcTimeCI}	& \vci{\FASTlusearchFTODCTime}{\FASTlusearchFTODCTimeCI}	& \vci{\FASTlusearchREDCTime}{\FASTlusearchREDCTimeCI} \\
\CAPO	& \vci{\SLOWlusearchCAPOExcTime}{\SLOWlusearchCAPOExcTimeCI}	& \vci{\SLOWlusearchCAPOnoGExcTime}{\SLOWlusearchCAPOnoGExcTimeCI}	& \vci{\FASTlusearchFTOCAPOTime}{\FASTlusearchFTOCAPOTimeCI}	& \vci{\FASTlusearchRECAPOTime}{\FASTlusearchRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{lusearch}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWpmdHBTime}{\SLOWpmdHBTimeCI}			& \vci{\FASTpmdFTOHBTime}{\FASTpmdFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWpmdWCPTime}{\SLOWpmdWCPTimeCI}			& \vci{\FASTpmdFTOWCPTime}{\FASTpmdFTOWCPTimeCI}	& \vci{\FASTpmdREWCPTime}{\FASTpmdREWCPTimeCI} \\
\DC		& \vci{\SLOWpmdDCExcTime}{\SLOWpmdDCExcTimeCI}	& \vci{\SLOWpmdDCnoGExcTime}{\SLOWpmdDCnoGExcTimeCI}	& \vci{\FASTpmdFTODCTime}{\FASTpmdFTODCTimeCI}	& \vci{\FASTpmdREDCTime}{\FASTpmdREDCTimeCI} \\
\CAPO	& \vci{\SLOWpmdCAPOExcTime}{\SLOWpmdCAPOExcTimeCI}	& \vci{\SLOWpmdCAPOnoGExcTime}{\SLOWpmdCAPOnoGExcTimeCI}	& \vci{\FASTpmdFTOCAPOTime}{\FASTpmdFTOCAPOTimeCI}	& \vci{\FASTpmdRECAPOTime}{\FASTpmdRECAPOTimeCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWsunflowHBTime}{\SLOWsunflowHBTimeCI}			& \vci{\FASTsunflowFTOHBTime}{\FASTsunflowFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWsunflowWCPTime}{\SLOWsunflowWCPTimeCI}			& \vci{\FASTsunflowFTOWCPTime}{\FASTsunflowFTOWCPTimeCI}	& \vci{\FASTsunflowREWCPTime}{\FASTsunflowREWCPTimeCI} \\
\DC		& \vci{\SLOWsunflowDCExcTime}{\SLOWsunflowDCExcTimeCI}	& \vci{\SLOWsunflowDCnoGExcTime}{\SLOWsunflowDCnoGExcTimeCI}	& \vci{\FASTsunflowFTODCTime}{\FASTsunflowFTODCTimeCI}	& \vci{\FASTsunflowREDCTime}{\FASTsunflowREDCTimeCI} \\
\CAPO	& \vci{\SLOWsunflowCAPOExcTime}{\SLOWsunflowCAPOExcTimeCI}	& \vci{\SLOWsunflowCAPOnoGExcTime}{\SLOWsunflowCAPOnoGExcTimeCI}	& \vci{\FASTsunflowFTOCAPOTime}{\FASTsunflowFTOCAPOTimeCI}	& \vci{\FASTsunflowRECAPOTime}{\FASTsunflowRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWtomcatHBTime}{\SLOWtomcatHBTimeCI}			& \vci{\FASTtomcatFTOHBTime}{\FASTtomcatFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWtomcatWCPTime}{\SLOWtomcatWCPTimeCI}			& \vci{\FASTtomcatFTOWCPTime}{\FASTtomcatFTOWCPTimeCI}	& \vci{\FASTtomcatREWCPTime}{\FASTtomcatREWCPTimeCI} \\
\DC		& \vci{\SLOWtomcatDCExcTime}{\SLOWtomcatDCExcTimeCI}	& \vci{\SLOWtomcatDCnoGExcTime}{\SLOWtomcatDCnoGExcTimeCI}	& \vci{\FASTtomcatFTODCTime}{\FASTtomcatFTODCTimeCI}	& \vci{\FASTtomcatREDCTime}{\FASTtomcatREDCTimeCI} \\
\CAPO	& \vci{\SLOWtomcatCAPOExcTime}{\SLOWtomcatCAPOExcTimeCI}	& \vci{\SLOWtomcatCAPOnoGExcTime}{\SLOWtomcatCAPOnoGExcTimeCI}	& \vci{\FASTtomcatFTOCAPOTime}{\FASTtomcatFTOCAPOTimeCI}	& \vci{\FASTtomcatRECAPOTime}{\FASTtomcatRECAPOTimeCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWxalanHBTime}{\SLOWxalanHBTimeCI}			& \vci{\FASTxalanFTOHBTime}{\FASTxalanFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWxalanWCPTime}{\SLOWxalanWCPTimeCI}			& \vci{\FASTxalanFTOWCPTime}{\FASTxalanFTOWCPTimeCI}	& \vci{\FASTxalanREWCPTime}{\FASTxalanREWCPTimeCI} \\
\DC		& \vci{\SLOWxalanDCExcTime}{\SLOWxalanDCExcTimeCI}	& \vci{\SLOWxalanDCnoGExcTime}{\SLOWxalanDCnoGExcTimeCI}	& \vci{\FASTxalanFTODCTime}{\FASTxalanFTODCTimeCI}	& \vci{\FASTxalanREDCTime}{\FASTxalanREDCTimeCI} \\
\CAPO	& \vci{\SLOWxalanCAPOExcTime}{\SLOWxalanCAPOExcTimeCI}	& \vci{\SLOWxalanCAPOnoGExcTime}{\SLOWxalanCAPOnoGExcTimeCI}	& \vci{\FASTxalanFTOCAPOTime}{\FASTxalanFTOCAPOTimeCI}	& \vci{\FASTxalanRECAPOTime}{\FASTxalanRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\jake{Configuration: 10 trials, no stats collected.
Unopt-* results are the latest evaluation of removing setting cores to 8.
FTO-* and ST-* also remove setting cores to 8 and only initialize extra metadata if used.}
\caption{Run time, relative to uninstrumented execution, of various analyses for each evaluated program
with 95\% confidence intervals.}
\label{tab:performance:allDaCapo:CI}
\end{table}
% Table for 10 trials of all relations with various optimizations for all DaCapo benchmarks
\begin{table}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
%memory \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$Gb$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
% \input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOptQuiet}
%
\small
\centering
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWavroraHBMem}{\SLOWavroraHBMemCI}		& \vci{\FASTavroraFTOHBMem}{\FASTavroraFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWavroraWCPMem}{\SLOWavroraWCPMemCI}		& \vci{\FASTavroraFTOWCPMem}{\FASTavroraFTOWCPMemCI}	& \vci{\FASTavroraREWCPMem}{\FASTavroraREWCPMemCI} \\
\DC		& \vci{\SLOWavroraDCExcMem}{\SLOWavroraDCExcMemCI}	& \vci{\SLOWavroraDCnoGExcMem}{\SLOWavroraDCnoGExcMemCI}	& \vci{\FASTavroraFTODCMem}{\FASTavroraFTODCMemCI}		& \vci{\FASTavroraREDCMem}{\FASTavroraREDCMemCI} \\
\CAPO	& \vci{\SLOWavroraCAPOExcMem}{\SLOWavroraCAPOExcMemCI}	& \vci{\SLOWavroraCAPOnoGExcMem}{\SLOWavroraCAPOnoGExcMemCI}& \vci{\FASTavroraFTOCAPOMem}{\FASTavroraFTOCAPOMemCI}	& \vci{\FASTavroraRECAPOMem}{\FASTavroraRECAPOMemCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWbatikHBMem}{\SLOWbatikHBMemCI}		& \vci{\FASTbatikFTOHBMem}{\FASTbatikFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWbatikWCPMem}{\SLOWbatikWCPMemCI}		& \vci{\FASTbatikFTOWCPMem}{\FASTbatikFTOWCPMemCI}	& \vci{\FASTbatikREWCPMem}{\FASTbatikREWCPMemCI} \\
\DC		& \vci{\SLOWbatikDCExcMem}{\SLOWbatikDCExcMemCI}	& \vci{\SLOWbatikDCnoGExcMem}{\SLOWbatikDCnoGExcMemCI}	& \vci{\FASTbatikFTODCMem}{\FASTbatikFTODCMemCI}		& \vci{\FASTbatikREDCMem}{\FASTbatikREDCMemCI} \\
\CAPO	& \vci{\SLOWbatikCAPOExcMem}{\SLOWbatikCAPOExcMemCI}	& \vci{\SLOWbatikCAPOnoGExcMem}{\SLOWbatikCAPOnoGExcMemCI}& \vci{\FASTbatikFTOCAPOMem}{\FASTbatikFTOCAPOMemCI}	& \vci{\FASTbatikRECAPOMem}{\FASTbatikRECAPOMemCI} \\
		& \mc{4}{c}{\bench{batik}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWhtwoHBMem}{\SLOWhtwoHBMemCI}		& \vci{\FASThtwoFTOHBMem}{\FASThtwoFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWhtwoWCPMem}{\SLOWhtwoWCPMemCI}		& \vci{\FASThtwoFTOWCPMem}{\FASThtwoFTOWCPMemCI}	& \vci{\FASThtwoREWCPMem}{\FASThtwoREWCPMemCI} \\
\DC		& \vci{\SLOWhtwoDCExcMem}{\SLOWhtwoDCExcMemCI}	& \vci{\SLOWhtwoDCnoGExcMem}{\SLOWhtwoDCnoGExcMemCI}	& \vci{\FASThtwoFTODCMem}{\FASThtwoFTODCMemCI}		& \vci{\FASThtwoREDCMem}{\FASThtwoREDCMemCI} \\
\CAPO	& \vci{\SLOWhtwoCAPOExcMem}{\SLOWhtwoCAPOExcMemCI}	& \vci{\SLOWhtwoCAPOnoGExcMem}{\SLOWhtwoCAPOnoGExcMemCI}& \vci{\FASThtwoFTOCAPOMem}{\FASThtwoFTOCAPOMemCI}	& \vci{\FASThtwoRECAPOMem}{\FASThtwoRECAPOMemCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWjythonHBMem}{\SLOWjythonHBMemCI}		& \vci{\FASTjythonFTOHBMem}{\FASTjythonFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWjythonWCPMem}{\SLOWjythonWCPMemCI}		& \vci{\FASTjythonFTOWCPMem}{\FASTjythonFTOWCPMemCI}	& \vci{\FASTjythonREWCPMem}{\FASTjythonREWCPMemCI} \\
\DC		& \vci{\SLOWjythonDCExcMem}{\SLOWjythonDCExcMemCI}	& \vci{\SLOWjythonDCnoGExcMem}{\SLOWjythonDCnoGExcMemCI}	& \vci{\FASTjythonFTODCMem}{\FASTjythonFTODCMemCI}		& \vci{\FASTjythonREDCMem}{\FASTjythonREDCMemCI} \\
\CAPO	& \vci{\SLOWjythonCAPOExcMem}{\SLOWjythonCAPOExcMemCI}	& \vci{\SLOWjythonCAPOnoGExcMem}{\SLOWjythonCAPOnoGExcMemCI}& \vci{\FASTjythonFTOCAPOMem}{\FASTjythonFTOCAPOMemCI}	& \vci{\FASTjythonRECAPOMem}{\FASTjythonRECAPOMemCI} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWluindexHBMem}{\SLOWluindexHBMemCI}		& \vci{\FASTluindexFTOHBMem}{\FASTluindexFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWluindexWCPMem}{\SLOWluindexWCPMemCI}		& \vci{\FASTluindexFTOWCPMem}{\FASTluindexFTOWCPMemCI}	& \vci{\FASTluindexREWCPMem}{\FASTluindexREWCPMemCI} \\
\DC		& \vci{\SLOWluindexDCExcMem}{\SLOWluindexDCExcMemCI}	& \vci{\SLOWluindexDCnoGExcMem}{\SLOWluindexDCnoGExcMemCI}	& \vci{\FASTluindexFTODCMem}{\FASTluindexFTODCMemCI}		& \vci{\FASTluindexREDCMem}{\FASTluindexREDCMemCI} \\
\CAPO	& \vci{\SLOWluindexCAPOExcMem}{\SLOWluindexCAPOExcMemCI}	& \vci{\SLOWluindexCAPOnoGExcMem}{\SLOWluindexCAPOnoGExcMemCI}& \vci{\FASTluindexFTOCAPOMem}{\FASTluindexFTOCAPOMemCI}	& \vci{\FASTluindexRECAPOMem}{\FASTluindexRECAPOMemCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWlusearchHBMem}{\SLOWlusearchHBMemCI}		& \vci{\FASTlusearchFTOHBMem}{\FASTlusearchFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWlusearchWCPMem}{\SLOWlusearchWCPMemCI}		& \vci{\FASTlusearchFTOWCPMem}{\FASTlusearchFTOWCPMemCI}	& \vci{\FASTlusearchREWCPMem}{\FASTlusearchREWCPMemCI} \\
\DC		& \vci{\SLOWlusearchDCExcMem}{\SLOWlusearchDCExcMemCI}	& \vci{\SLOWlusearchDCnoGExcMem}{\SLOWlusearchDCnoGExcMemCI}	& \vci{\FASTlusearchFTODCMem}{\FASTlusearchFTODCMemCI}		& \vci{\FASTlusearchREDCMem}{\FASTlusearchREDCMemCI} \\
\CAPO	& \vci{\SLOWlusearchCAPOExcMem}{\SLOWlusearchCAPOExcMemCI}	& \vci{\SLOWlusearchCAPOnoGExcMem}{\SLOWlusearchCAPOnoGExcMemCI}& \vci{\FASTlusearchFTOCAPOMem}{\FASTlusearchFTOCAPOMemCI}	& \vci{\FASTlusearchRECAPOMem}{\FASTlusearchRECAPOMemCI} \\
		& \mc{4}{c}{\bench{lusearch}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWpmdHBMem}{\SLOWpmdHBMemCI}		& \vci{\FASTpmdFTOHBMem}{\FASTpmdFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWpmdWCPMem}{\SLOWpmdWCPMemCI}		& \vci{\FASTpmdFTOWCPMem}{\FASTpmdFTOWCPMemCI}	& \vci{\FASTpmdREWCPMem}{\FASTpmdREWCPMemCI} \\
\DC		& \vci{\SLOWpmdDCExcMem}{\SLOWpmdDCExcMemCI}	& \vci{\SLOWpmdDCnoGExcMem}{\SLOWpmdDCnoGExcMemCI}	& \vci{\FASTpmdFTODCMem}{\FASTpmdFTODCMemCI}		& \vci{\FASTpmdREDCMem}{\FASTpmdREDCMemCI} \\
\CAPO	& \vci{\SLOWpmdCAPOExcMem}{\SLOWpmdCAPOExcMemCI}	& \vci{\SLOWpmdCAPOnoGExcMem}{\SLOWpmdCAPOnoGExcMemCI}& \vci{\FASTpmdFTOCAPOMem}{\FASTpmdFTOCAPOMemCI}	& \vci{\FASTpmdRECAPOMem}{\FASTpmdRECAPOMemCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWsunflowHBMem}{\SLOWsunflowHBMemCI}		& \vci{\FASTsunflowFTOHBMem}{\FASTsunflowFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWsunflowWCPMem}{\SLOWsunflowWCPMemCI}		& \vci{\FASTsunflowFTOWCPMem}{\FASTsunflowFTOWCPMemCI}	& \vci{\FASTsunflowREWCPMem}{\FASTsunflowREWCPMemCI} \\
\DC		& \vci{\SLOWsunflowDCExcMem}{\SLOWsunflowDCExcMemCI}	& \vci{\SLOWsunflowDCnoGExcMem}{\SLOWsunflowDCnoGExcMemCI}	& \vci{\FASTsunflowFTODCMem}{\FASTsunflowFTODCMemCI}		& \vci{\FASTsunflowREDCMem}{\FASTsunflowREDCMemCI} \\
\CAPO	& \vci{\SLOWsunflowCAPOExcMem}{\SLOWsunflowCAPOExcMemCI}	& \vci{\SLOWsunflowCAPOnoGExcMem}{\SLOWsunflowCAPOnoGExcMemCI}& \vci{\FASTsunflowFTOCAPOMem}{\FASTsunflowFTOCAPOMemCI}	& \vci{\FASTsunflowRECAPOMem}{\FASTsunflowRECAPOMemCI} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWtomcatHBMem}{\SLOWtomcatHBMemCI}		& \vci{\FASTtomcatFTOHBMem}{\FASTtomcatFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWtomcatWCPMem}{\SLOWtomcatWCPMemCI}		& \vci{\FASTtomcatFTOWCPMem}{\FASTtomcatFTOWCPMemCI}	& \vci{\FASTtomcatREWCPMem}{\FASTtomcatREWCPMemCI} \\
\DC		& \vci{\SLOWtomcatDCExcMem}{\SLOWtomcatDCExcMemCI}	& \vci{\SLOWtomcatDCnoGExcMem}{\SLOWtomcatDCnoGExcMemCI}	& \vci{\FASTtomcatFTODCMem}{\FASTtomcatFTODCMemCI}		& \vci{\FASTtomcatREDCMem}{\FASTtomcatREDCMemCI} \\
\CAPO	& \vci{\SLOWtomcatCAPOExcMem}{\SLOWtomcatCAPOExcMemCI}	& \vci{\SLOWtomcatCAPOnoGExcMem}{\SLOWtomcatCAPOnoGExcMemCI}& \vci{\FASTtomcatFTOCAPOMem}{\FASTtomcatFTOCAPOMemCI}	& \vci{\FASTtomcatRECAPOMem}{\FASTtomcatRECAPOMemCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWxalanHBMem}{\SLOWxalanHBMemCI}		& \vci{\FASTxalanFTOHBMem}{\FASTxalanFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWxalanWCPMem}{\SLOWxalanWCPMemCI}		& \vci{\FASTxalanFTOWCPMem}{\FASTxalanFTOWCPMemCI}	& \vci{\FASTxalanREWCPMem}{\FASTxalanREWCPMemCI} \\
\DC		& \vci{\SLOWxalanDCExcMem}{\SLOWxalanDCExcMemCI}	& \vci{\SLOWxalanDCnoGExcMem}{\SLOWxalanDCnoGExcMemCI}	& \vci{\FASTxalanFTODCMem}{\FASTxalanFTODCMemCI}		& \vci{\FASTxalanREDCMem}{\FASTxalanREDCMemCI} \\
\CAPO	& \vci{\SLOWxalanCAPOExcMem}{\SLOWxalanCAPOExcMemCI}	& \vci{\SLOWxalanCAPOnoGExcMem}{\SLOWxalanCAPOnoGExcMemCI}& \vci{\FASTxalanFTOCAPOMem}{\FASTxalanFTOCAPOMemCI}	& \vci{\FASTxalanRECAPOMem}{\FASTxalanRECAPOMemCI} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\jake{Configuration: 10 trials, no stats collected.
Unopt-* results are the latest evaluation of removing setting cores to 8.
FTO-* and ST-* also remove setting cores to 8 and only initialize extra metadata if used.}
\caption{Memory usage, relative to uninstrumented execution, of various analyses for each evaluated program
with 95\% confidence intervals.}
\label{tab:memory:allDaCapo:CI}
\end{table}

\begin{table}
% \begin{adjustwidth}{-1.5cm}{}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
% \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;Mb$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\sdr}[4]{\vci{#1}{#2}{\;}(\vci{#3}{#4})}
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}#1}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOptQuiet}
%
\smaller
\centering
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWavroraHB}{\SLOWavroraHBCI}{\SLOWavroraHBDynamic}{\SLOWavroraHBDynamicCI}					& \sdr{\FASTavroraFTOHB}{\FASTavroraFTOHBCI}{\FASTavroraFTOHBDynamic}{\FASTavroraFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWavroraWCP}{\SLOWavroraWCPCI}{\SLOWavroraWCPDynamic}{\SLOWavroraWCPDynamicCI}				& \sdr{\FASTavroraFTOWCP}{\FASTavroraFTOWCPCI}{\FASTavroraFTOWCPDynamic}{\FASTavroraFTOWCPDynamicCI}		& \sdr{\FASTavroraREWCP}{\FASTavroraREWCPCI}{\FASTavroraREWCPDynamic}{\FASTavroraREWCPDynamicCI} \\
\DC		& \sdr{\SLOWavroraDCExc}{\SLOWavroraDCExcCI}{\SLOWavroraDCExcDynamic}{\SLOWavroraDCExcDynamicCI}		& \sdr{\SLOWavroraDCnoGExc}{\SLOWavroraDCnoGExcCI}{\SLOWavroraDCnoGExcDynamic}{\SLOWavroraDCnoGExcDynamicCI}	& \sdr{\FASTavroraFTODC}{\FASTavroraFTODCCI}{\FASTavroraFTODCDynamic}{\FASTavroraFTODCDynamicCI}		& \sdr{\FASTavroraREDC}{\FASTavroraREDCCI}{\FASTavroraREDCDynamic}{\FASTavroraREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWavroraCAPOExc}{\SLOWavroraCAPOExcCI}{\SLOWavroraCAPOExcDynamic}{\SLOWavroraCAPOExcDynamicCI}	& \sdr{\SLOWavroraCAPOnoGExc}{\SLOWavroraCAPOnoGExcCI}{\SLOWavroraCAPOnoGExcDynamic}{\SLOWavroraCAPOnoGExcDynamicCI}	& \sdr{\FASTavroraFTOCAPO}{\FASTavroraFTOCAPOCI}{\FASTavroraFTOCAPODynamic}{\FASTavroraFTOCAPODynamicCI}	& \sdr{\FASTavroraRECAPO}{\FASTavroraRECAPOCI}{\FASTavroraRECAPODynamic}{\FASTavroraRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\medskip\\
% \begin{tabular}{@{}HHlll@{}}
%         & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
% \HB		& \rna													& \sdr{\SLOWbatikHB}{\SLOWbatikHBCI}{\SLOWbatikHBDynamic}{\SLOWbatikHBDynamicCI}					& \sdr{\FASTbatikFTOHB}{\FASTbatikFTOHBCI}{\FASTbatikFTOHBDynamic}{\FASTbatikFTOHBDynamicCI}		& \rna \\
% \WCP	& \rna													& \sdr{\SLOWbatikWCP}{\SLOWbatikWCPCI}{\SLOWbatikWCPDynamic}{\SLOWbatikWCPDynamicCI}				& \sdr{\FASTbatikFTOWCP}{\FASTbatikFTOWCPCI}{\FASTbatikFTOWCPDynamic}{\FASTbatikFTOWCPDynamicCI}		& \sdr{\FASTbatikREWCP}{\FASTbatikREWCPCI}{\FASTbatikREWCPDynamic}{\FASTbatikREWCPDynamicCI} \\
% \DC		& \sdr{\SLOWbatikDCExc}{\SLOWbatikDCExcCI}{\SLOWbatikDCExcDynamic}{\SLOWbatikDCExcDynamicCI}		& \sdr{\SLOWbatikDCnoGExc}{\SLOWbatikDCnoGExcCI}{\SLOWbatikDCnoGExcDynamic}{\SLOWbatikDCnoGExcDynamicCI}	& \sdr{\FASTbatikFTODC}{\FASTbatikFTODCCI}{\FASTbatikFTODCDynamic}{\FASTbatikFTODCDynamicCI}		& \sdr{\FASTbatikREDC}{\FASTbatikREDCCI}{\FASTbatikREDCDynamic}{\FASTbatikREDCDynamicCI} \\
% \CAPO	& \sdr{\SLOWbatikCAPOExc}{\SLOWbatikCAPOExcCI}{\SLOWbatikCAPOExcDynamic}{\SLOWbatikCAPOExcDynamicCI}	& \sdr{\SLOWbatikCAPOnoGExc}{\SLOWbatikCAPOnoGExcCI}{\SLOWbatikCAPOnoGExcDynamic}{\SLOWbatikCAPOnoGExcDynamicCI}	& \sdr{\FASTbatikFTOCAPO}{\FASTbatikFTOCAPOCI}{\FASTbatikFTOCAPODynamic}{\FASTbatikFTOCAPODynamicCI}	& \sdr{\FASTbatikRECAPO}{\FASTbatikRECAPOCI}{\FASTbatikRECAPODynamic}{\FASTbatikRECAPODynamicCI} \\
% 		& \mc{4}{c}{\bench{batik}} \\
% \end{tabular}
% \hfill
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWhtwoHB}{\SLOWhtwoHBCI}{\SLOWhtwoHBDynamic}{\SLOWhtwoHBDynamicCI}					& \sdr{\FASThtwoFTOHB}{\FASThtwoFTOHBCI}{\FASThtwoFTOHBDynamic}{\FASThtwoFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWhtwoWCP}{\SLOWhtwoWCPCI}{\SLOWhtwoWCPDynamic}{\SLOWhtwoWCPDynamicCI}				& \sdr{\FASThtwoFTOWCP}{\FASThtwoFTOWCPCI}{\FASThtwoFTOWCPDynamic}{\FASThtwoFTOWCPDynamicCI}		& \sdr{\FASThtwoREWCP}{\FASThtwoREWCPCI}{\FASThtwoREWCPDynamic}{\FASThtwoREWCPDynamicCI} \\
\DC		& \sdr{\SLOWhtwoDCExc}{\SLOWhtwoDCExcCI}{\SLOWhtwoDCExcDynamic}{\SLOWhtwoDCExcDynamicCI}		& \sdr{\SLOWhtwoDCnoGExc}{\SLOWhtwoDCnoGExcCI}{\SLOWhtwoDCnoGExcDynamic}{\SLOWhtwoDCnoGExcDynamicCI}	& \sdr{\FASThtwoFTODC}{\FASThtwoFTODCCI}{\FASThtwoFTODCDynamic}{\FASThtwoFTODCDynamicCI}		& \sdr{\FASThtwoREDC}{\FASThtwoREDCCI}{\FASThtwoREDCDynamic}{\FASThtwoREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWhtwoCAPOExc}{\SLOWhtwoCAPOExcCI}{\SLOWhtwoCAPOExcDynamic}{\SLOWhtwoCAPOExcDynamicCI}	& \sdr{\SLOWhtwoCAPOnoGExc}{\SLOWhtwoCAPOnoGExcCI}{\SLOWhtwoCAPOnoGExcDynamic}{\SLOWhtwoCAPOnoGExcDynamicCI}	& \sdr{\FASThtwoFTOCAPO}{\FASThtwoFTOCAPOCI}{\FASThtwoFTOCAPODynamic}{\FASThtwoFTOCAPODynamicCI}	& \sdr{\FASThtwoRECAPO}{\FASThtwoRECAPOCI}{\FASThtwoRECAPODynamic}{\FASThtwoRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWjythonHB}{\SLOWjythonHBCI}{\SLOWjythonHBDynamic}{\SLOWjythonHBDynamicCI}					& \sdr{\FASTjythonFTOHB}{\FASTjythonFTOHBCI}{\FASTjythonFTOHBDynamic}{\FASTjythonFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWjythonWCP}{\SLOWjythonWCPCI}{\SLOWjythonWCPDynamic}{\SLOWjythonWCPDynamicCI}				& \sdr{\FASTjythonFTOWCP}{\FASTjythonFTOWCPCI}{\FASTjythonFTOWCPDynamic}{\FASTjythonFTOWCPDynamicCI}		& \sdr{\FASTjythonREWCP}{\FASTjythonREWCPCI}{\FASTjythonREWCPDynamic}{\FASTjythonREWCPDynamicCI} \\
\DC		& \sdr{\SLOWjythonDCExc}{\SLOWjythonDCExcCI}{\SLOWjythonDCExcDynamic}{\SLOWjythonDCExcDynamicCI}		& \sdr{\SLOWjythonDCnoGExc}{\SLOWjythonDCnoGExcCI}{\SLOWjythonDCnoGExcDynamic}{\SLOWjythonDCnoGExcDynamicCI}	& \sdr{\FASTjythonFTODC}{\FASTjythonFTODCCI}{\FASTjythonFTODCDynamic}{\FASTjythonFTODCDynamicCI}		& \sdr{\FASTjythonREDC}{\FASTjythonREDCCI}{\FASTjythonREDCDynamic}{\FASTjythonREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWjythonCAPOExc}{\SLOWjythonCAPOExcCI}{\SLOWjythonCAPOExcDynamic}{\SLOWjythonCAPOExcDynamicCI}	& \sdr{\SLOWjythonCAPOnoGExc}{\SLOWjythonCAPOnoGExcCI}{\SLOWjythonCAPOnoGExcDynamic}{\SLOWjythonCAPOnoGExcDynamicCI}	& \sdr{\FASTjythonFTOCAPO}{\FASTjythonFTOCAPOCI}{\FASTjythonFTOCAPODynamic}{\FASTjythonFTOCAPODynamicCI}	& \sdr{\FASTjythonRECAPO}{\FASTjythonRECAPOCI}{\FASTjythonRECAPODynamic}{\FASTjythonRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWluindexHB}{\SLOWluindexHBCI}{\SLOWluindexHBDynamic}{\SLOWluindexHBDynamicCI}					& \sdr{\FASTluindexFTOHB}{\FASTluindexFTOHBCI}{\FASTluindexFTOHBDynamic}{\FASTluindexFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWluindexWCP}{\SLOWluindexWCPCI}{\SLOWluindexWCPDynamic}{\SLOWluindexWCPDynamicCI}				& \sdr{\FASTluindexFTOWCP}{\FASTluindexFTOWCPCI}{\FASTluindexFTOWCPDynamic}{\FASTluindexFTOWCPDynamicCI}		& \sdr{\FASTluindexREWCP}{\FASTluindexREWCPCI}{\FASTluindexREWCPDynamic}{\FASTluindexREWCPDynamicCI} \\
\DC		& \sdr{\SLOWluindexDCExc}{\SLOWluindexDCExcCI}{\SLOWluindexDCExcDynamic}{\SLOWluindexDCExcDynamicCI}		& \sdr{\SLOWluindexDCnoGExc}{\SLOWluindexDCnoGExcCI}{\SLOWluindexDCnoGExcDynamic}{\SLOWluindexDCnoGExcDynamicCI}	& \sdr{\FASTluindexFTODC}{\FASTluindexFTODCCI}{\FASTluindexFTODCDynamic}{\FASTluindexFTODCDynamicCI}		& \sdr{\FASTluindexREDC}{\FASTluindexREDCCI}{\FASTluindexREDCDynamic}{\FASTluindexREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWluindexCAPOExc}{\SLOWluindexCAPOExcCI}{\SLOWluindexCAPOExcDynamic}{\SLOWluindexCAPOExcDynamicCI}	& \sdr{\SLOWluindexCAPOnoGExc}{\SLOWluindexCAPOnoGExcCI}{\SLOWluindexCAPOnoGExcDynamic}{\SLOWluindexCAPOnoGExcDynamicCI}	& \sdr{\FASTluindexFTOCAPO}{\FASTluindexFTOCAPOCI}{\FASTluindexFTOCAPODynamic}{\FASTluindexFTOCAPODynamicCI}	& \sdr{\FASTluindexRECAPO}{\FASTluindexRECAPOCI}{\FASTluindexRECAPODynamic}{\FASTluindexRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
% \hfill
% \begin{tabular}{@{}HHlll@{}}
%         & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
% \HB		& \rna													& \sdr{\SLOWlusearchHB}{\SLOWlusearchHBCI}{\SLOWlusearchHBDynamic}{\SLOWlusearchHBDynamicCI}					& \sdr{\FASTlusearchFTOHB}{\FASTlusearchFTOHBCI}{\FASTlusearchFTOHBDynamic}{\FASTlusearchFTOHBDynamicCI}		& \rna \\
% \WCP	& \rna													& \sdr{\SLOWlusearchWCP}{\SLOWlusearchWCPCI}{\SLOWlusearchWCPDynamic}{\SLOWlusearchWCPDynamicCI}				& \sdr{\FASTlusearchFTOWCP}{\FASTlusearchFTOWCPCI}{\FASTlusearchFTOWCPDynamic}{\FASTlusearchFTOWCPDynamicCI}		& \sdr{\FASTlusearchREWCP}{\FASTlusearchREWCPCI}{\FASTlusearchREWCPDynamic}{\FASTlusearchREWCPDynamicCI} \\
% \DC		& \sdr{\SLOWlusearchDCExc}{\SLOWlusearchDCExcCI}{\SLOWlusearchDCExcDynamic}{\SLOWlusearchDCExcDynamicCI}		& \sdr{\SLOWlusearchDCnoGExc}{\SLOWlusearchDCnoGExcCI}{\SLOWlusearchDCnoGExcDynamic}{\SLOWlusearchDCnoGExcDynamicCI}	& \sdr{\FASTlusearchFTODC}{\FASTlusearchFTODCCI}{\FASTlusearchFTODCDynamic}{\FASTlusearchFTODCDynamicCI}		& \sdr{\FASTlusearchREDC}{\FASTlusearchREDCCI}{\FASTlusearchREDCDynamic}{\FASTlusearchREDCDynamicCI} \\
% \CAPO	& \sdr{\SLOWlusearchCAPOExc}{\SLOWlusearchCAPOExcCI}{\SLOWlusearchCAPOExcDynamic}{\SLOWlusearchCAPOExcDynamicCI}	& \sdr{\SLOWlusearchCAPOnoGExc}{\SLOWlusearchCAPOnoGExcCI}{\SLOWlusearchCAPOnoGExcDynamic}{\SLOWlusearchCAPOnoGExcDynamicCI}	& \sdr{\FASTlusearchFTOCAPO}{\FASTlusearchFTOCAPOCI}{\FASTlusearchFTOCAPODynamic}{\FASTlusearchFTOCAPODynamicCI}	& \sdr{\FASTlusearchRECAPO}{\FASTlusearchRECAPOCI}{\FASTlusearchRECAPODynamic}{\FASTlusearchRECAPODynamicCI} \\
% 		& \mc{4}{c}{\bench{lusearch}} \\
% \end{tabular}
% \hfill
\medskip\\
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWpmdHB}{\SLOWpmdHBCI}{\SLOWpmdHBDynamic}{\SLOWpmdHBDynamicCI}					& \sdr{\FASTpmdFTOHB}{\FASTpmdFTOHBCI}{\FASTpmdFTOHBDynamic}{\FASTpmdFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWpmdWCP}{\SLOWpmdWCPCI}{\SLOWpmdWCPDynamic}{\SLOWpmdWCPDynamicCI}				& \sdr{\FASTpmdFTOWCP}{\FASTpmdFTOWCPCI}{\FASTpmdFTOWCPDynamic}{\FASTpmdFTOWCPDynamicCI}		& \sdr{\FASTpmdREWCP}{\FASTpmdREWCPCI}{\FASTpmdREWCPDynamic}{\FASTpmdREWCPDynamicCI} \\
\DC		& \sdr{\SLOWpmdDCExc}{\SLOWpmdDCExcCI}{\SLOWpmdDCExcDynamic}{\SLOWpmdDCExcDynamicCI}		& \sdr{\SLOWpmdDCnoGExc}{\SLOWpmdDCnoGExcCI}{\SLOWpmdDCnoGExcDynamic}{\SLOWpmdDCnoGExcDynamicCI}	& \sdr{\FASTpmdFTODC}{\FASTpmdFTODCCI}{\FASTpmdFTODCDynamic}{\FASTpmdFTODCDynamicCI}		& \sdr{\FASTpmdREDC}{\FASTpmdREDCCI}{\FASTpmdREDCDynamic}{\FASTpmdREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWpmdCAPOExc}{\SLOWpmdCAPOExcCI}{\SLOWpmdCAPOExcDynamic}{\SLOWpmdCAPOExcDynamicCI}	& \sdr{\SLOWpmdCAPOnoGExc}{\SLOWpmdCAPOnoGExcCI}{\SLOWpmdCAPOnoGExcDynamic}{\SLOWpmdCAPOnoGExcDynamicCI}	& \sdr{\FASTpmdFTOCAPO}{\FASTpmdFTOCAPOCI}{\FASTpmdFTOCAPODynamic}{\FASTpmdFTOCAPODynamicCI}	& \sdr{\FASTpmdRECAPO}{\FASTpmdRECAPOCI}{\FASTpmdRECAPODynamic}{\FASTpmdRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWsunflowHB}{\SLOWsunflowHBCI}{\SLOWsunflowHBDynamic}{\SLOWsunflowHBDynamicCI}					& \sdr{\FASTsunflowFTOHB}{\FASTsunflowFTOHBCI}{\FASTsunflowFTOHBDynamic}{\FASTsunflowFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWsunflowWCP}{\SLOWsunflowWCPCI}{\SLOWsunflowWCPDynamic}{\SLOWsunflowWCPDynamicCI}				& \sdr{\FASTsunflowFTOWCP}{\FASTsunflowFTOWCPCI}{\FASTsunflowFTOWCPDynamic}{\FASTsunflowFTOWCPDynamicCI}		& \sdr{\FASTsunflowREWCP}{\FASTsunflowREWCPCI}{\FASTsunflowREWCPDynamic}{\FASTsunflowREWCPDynamicCI} \\
\DC		& \sdr{\SLOWsunflowDCExc}{\SLOWsunflowDCExcCI}{\SLOWsunflowDCExcDynamic}{\SLOWsunflowDCExcDynamicCI}		& \sdr{\SLOWsunflowDCnoGExc}{\SLOWsunflowDCnoGExcCI}{\SLOWsunflowDCnoGExcDynamic}{\SLOWsunflowDCnoGExcDynamicCI}	& \sdr{\FASTsunflowFTODC}{\FASTsunflowFTODCCI}{\FASTsunflowFTODCDynamic}{\FASTsunflowFTODCDynamicCI}		& \sdr{\FASTsunflowREDC}{\FASTsunflowREDCCI}{\FASTsunflowREDCDynamic}{\FASTsunflowREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWsunflowCAPOExc}{\SLOWsunflowCAPOExcCI}{\SLOWsunflowCAPOExcDynamic}{\SLOWsunflowCAPOExcDynamicCI}	& \sdr{\SLOWsunflowCAPOnoGExc}{\SLOWsunflowCAPOnoGExcCI}{\SLOWsunflowCAPOnoGExcDynamic}{\SLOWsunflowCAPOnoGExcDynamicCI}	& \sdr{\FASTsunflowFTOCAPO}{\FASTsunflowFTOCAPOCI}{\FASTsunflowFTOCAPODynamic}{\FASTsunflowFTOCAPODynamicCI}	& \sdr{\FASTsunflowRECAPO}{\FASTsunflowRECAPOCI}{\FASTsunflowRECAPODynamic}{\FASTsunflowRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWtomcatHB}{\SLOWtomcatHBCI}{\SLOWtomcatHBDynamic}{\SLOWtomcatHBDynamicCI}					& \sdr{\FASTtomcatFTOHB}{\FASTtomcatFTOHBCI}{\FASTtomcatFTOHBDynamic}{\FASTtomcatFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWtomcatWCP}{\SLOWtomcatWCPCI}{\SLOWtomcatWCPDynamic}{\SLOWtomcatWCPDynamicCI}				& \sdr{\FASTtomcatFTOWCP}{\FASTtomcatFTOWCPCI}{\FASTtomcatFTOWCPDynamic}{\FASTtomcatFTOWCPDynamicCI}		& \sdr{\FASTtomcatREWCP}{\FASTtomcatREWCPCI}{\FASTtomcatREWCPDynamic}{\FASTtomcatREWCPDynamicCI} \\
\DC		& \sdr{\SLOWtomcatDCExc}{\SLOWtomcatDCExcCI}{\SLOWtomcatDCExcDynamic}{\SLOWtomcatDCExcDynamicCI}		& \sdr{\SLOWtomcatDCnoGExc}{\SLOWtomcatDCnoGExcCI}{\SLOWtomcatDCnoGExcDynamic}{\SLOWtomcatDCnoGExcDynamicCI}	& \sdr{\FASTtomcatFTODC}{\FASTtomcatFTODCCI}{\FASTtomcatFTODCDynamic}{\FASTtomcatFTODCDynamicCI}		& \sdr{\FASTtomcatREDC}{\FASTtomcatREDCCI}{\FASTtomcatREDCDynamic}{\FASTtomcatREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWtomcatCAPOExc}{\SLOWtomcatCAPOExcCI}{\SLOWtomcatCAPOExcDynamic}{\SLOWtomcatCAPOExcDynamicCI}	& \sdr{\SLOWtomcatCAPOnoGExc}{\SLOWtomcatCAPOnoGExcCI}{\SLOWtomcatCAPOnoGExcDynamic}{\SLOWtomcatCAPOnoGExcDynamicCI}	& \sdr{\FASTtomcatFTOCAPO}{\FASTtomcatFTOCAPOCI}{\FASTtomcatFTOCAPODynamic}{\FASTtomcatFTOCAPODynamicCI}	& \sdr{\FASTtomcatRECAPO}{\FASTtomcatRECAPOCI}{\FASTtomcatRECAPODynamic}{\FASTtomcatRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWxalanHB}{\SLOWxalanHBCI}{\SLOWxalanHBDynamic}{\SLOWxalanHBDynamicCI}					& \sdr{\FASTxalanFTOHB}{\FASTxalanFTOHBCI}{\FASTxalanFTOHBDynamic}{\FASTxalanFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWxalanWCP}{\SLOWxalanWCPCI}{\SLOWxalanWCPDynamic}{\SLOWxalanWCPDynamicCI}				& \sdr{\FASTxalanFTOWCP}{\FASTxalanFTOWCPCI}{\FASTxalanFTOWCPDynamic}{\FASTxalanFTOWCPDynamicCI}		& \sdr{\FASTxalanREWCP}{\FASTxalanREWCPCI}{\FASTxalanREWCPDynamic}{\FASTxalanREWCPDynamicCI} \\
\DC		& \sdr{\SLOWxalanDCExc}{\SLOWxalanDCExcCI}{\SLOWxalanDCExcDynamic}{\SLOWxalanDCExcDynamicCI}		& \sdr{\SLOWxalanDCnoGExc}{\SLOWxalanDCnoGExcCI}{\SLOWxalanDCnoGExcDynamic}{\SLOWxalanDCnoGExcDynamicCI}	& \sdr{\FASTxalanFTODC}{\FASTxalanFTODCCI}{\FASTxalanFTODCDynamic}{\FASTxalanFTODCDynamicCI}		& \sdr{\FASTxalanREDC}{\FASTxalanREDCCI}{\FASTxalanREDCDynamic}{\FASTxalanREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWxalanCAPOExc}{\SLOWxalanCAPOExcCI}{\SLOWxalanCAPOExcDynamic}{\SLOWxalanCAPOExcDynamicCI}	& \sdr{\SLOWxalanCAPOnoGExc}{\SLOWxalanCAPOnoGExcCI}{\SLOWxalanCAPOnoGExcDynamic}{\SLOWxalanCAPOnoGExcDynamicCI}	& \sdr{\FASTxalanFTOCAPO}{\FASTxalanFTOCAPOCI}{\FASTxalanFTOCAPODynamic}{\FASTxalanFTOCAPODynamicCI}	& \sdr{\FASTxalanRECAPO}{\FASTxalanRECAPOCI}{\FASTxalanRECAPODynamic}{\FASTxalanRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\jake{Configuration: 10 trials, no stats collected.
Unopt-* results are the latest evaluation of removing setting cores to 8.
FTO-* and ST-* also remove setting cores to 8 and only initialize extra metadata if used.}
\caption{Average races reported by various analyses for each evaluated program
(excluding \bench{batik} and \bench{lusearch}, for which all analyses report no races).
In each cell, the first value is statically distinct races
(\ie, distinct program locations), and the second value, in parentheses, is total dynamic races,
both with 95\% confidence intervals.}
\label{tab:race:allDaCapo:CI}
\end{table}


%%%%%%%%%%%%%%%%%%%%New Set of Tables%%%%%%%%%%%%%%%%%%%%%%

\section{Results duplicating result tables for initializing extra metadata to null 
and setting back to null when Ex is empty for ST-*}

%The following are three tables stacked together
% Table for geometric mean of all relations with various optimizations for all DaCapo benchmarks
\begin{table}[t]
\begin{empty}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOpt2Quiet}
%
\small
\centering
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWHBTimeGeoMean}			& \roh{\FASTFTOHBTimeGeoMean}	& \rna \\
\WCP	& \rna							& \roh{\SLOWWCPTimeGeoMean}			& \roh{\FASTFTOWCPTimeGeoMean}	& \roh{\FASTREWCPTimeGeoMean} \\
\DC		& \roh{\SLOWDCExcTimeGeoMean}	& \roh{\SLOWDCnoGExcTimeGeoMean}	& \roh{\FASTFTODCTimeGeoMean}	& \roh{\FASTREDCTimeGeoMean} \\
\CAPO	& \roh{\SLOWCAPOExcTimeGeoMean}	& \roh{\SLOWCAPOnoGExcTimeGeoMean}	& \roh{\FASTFTOCAPOTimeGeoMean}	& \roh{\FASTRECAPOTimeGeoMean} \\
\mc{2}{H}{} & \mc{3}{c}{Run time} \\
\end{tabular}
\hspace*{1em}
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \mem{\SLOWHBMemGeoMean}			& \mem{\FASTFTOHBMemGeoMean}	& \rna \\
\WCP	& \rna							& \mem{\SLOWWCPMemGeoMean}			& \mem{\FASTFTOWCPMemGeoMean}	& \mem{\FASTREWCPMemGeoMean} \\
\DC		& \mem{\SLOWDCExcMemGeoMean}	& \mem{\SLOWDCnoGExcMemGeoMean}	& \mem{\FASTFTODCMemGeoMean}	& \mem{\FASTREDCMemGeoMean} \\
\CAPO	& \mem{\SLOWCAPOExcMemGeoMean}	& \mem{\SLOWCAPOnoGExcMemGeoMean}	& \mem{\FASTFTOCAPOMemGeoMean}	& \mem{\FASTRECAPOMemGeoMean} \\
\mc{2}{H}{} & \mc{3}{c}{Memory usage} \\
\end{tabular}

\jake{Configuration: 10 trials, no stats collected.
Unopt-* results are the latest evaluation of removing setting cores to 8.
FTO-* and ST-* also remove setting cores to 8 and initialize extra metadata to null
and sets extra metadata to null if empty.}

\caption{Geometric mean of run time and memory usage across the evaluated programs.}
\label{tab:performance:geoMean-Ex}
\end{empty}
\medskip
% Combined benchmarks table for 10 trials of all relations with various optimizations
\begin{empty}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOpt2Quiet}
%
\smaller
\centering
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWavroraHBTime}			& \roh{\FASTavroraFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWavroraWCPTime}			& \roh{\FASTavroraFTOWCPTime}	& \roh{\FASTavroraREWCPTime} \\
\DC		& \roh{\SLOWavroraDCExcTime}	& \roh{\SLOWavroraDCnoGExcTime}	& \roh{\FASTavroraFTODCTime}	& \roh{\FASTavroraREDCTime} \\
\CAPO	& \roh{\SLOWavroraCAPOExcTime}	& \roh{\SLOWavroraCAPOnoGExcTime}	& \roh{\FASTavroraFTOCAPOTime}	& \roh{\FASTavroraRECAPOTime} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWbatikHBTime}			& \roh{\FASTbatikFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWbatikWCPTime}			& \roh{\FASTbatikFTOWCPTime}	& \roh{\FASTbatikREWCPTime} \\
\DC		& \roh{\SLOWbatikDCExcTime}	& \roh{\SLOWbatikDCnoGExcTime}	& \roh{\FASTbatikFTODCTime}	& \roh{\FASTbatikREDCTime} \\
\CAPO	& \roh{\SLOWbatikCAPOExcTime}	& \roh{\SLOWbatikCAPOnoGExcTime}	& \roh{\FASTbatikFTOCAPOTime}	& \roh{\FASTbatikRECAPOTime} \\
		& \mc{4}{c}{\bench{batik}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWhtwoHBTime}			& \roh{\FASThtwoFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWhtwoWCPTime}			& \roh{\FASThtwoFTOWCPTime}	& \roh{\FASThtwoREWCPTime} \\
\DC		& \roh{\SLOWhtwoDCExcTime}	& \roh{\SLOWhtwoDCnoGExcTime}	& \roh{\FASThtwoFTODCTime}	& \roh{\FASThtwoREDCTime} \\
\CAPO	& \roh{\SLOWhtwoCAPOExcTime}	& \roh{\SLOWhtwoCAPOnoGExcTime}	& \roh{\FASThtwoFTOCAPOTime}	& \roh{\FASThtwoRECAPOTime} \\
		& \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWjythonHBTime}			& \roh{\FASTjythonFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWjythonWCPTime}			& \roh{\FASTjythonFTOWCPTime}	& \roh{\FASTjythonREWCPTime} \\
\DC		& \roh{\SLOWjythonDCExcTime}	& \roh{\SLOWjythonDCnoGExcTime}	& \roh{\FASTjythonFTODCTime}	& \roh{\FASTjythonREDCTime} \\
\CAPO	& \roh{\SLOWjythonCAPOExcTime}	& \roh{\SLOWjythonCAPOnoGExcTime}	& \roh{\FASTjythonFTOCAPOTime}	& \roh{\FASTjythonRECAPOTime} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWluindexHBTime}			& \roh{\FASTluindexFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWluindexWCPTime}			& \roh{\FASTluindexFTOWCPTime}	& \roh{\FASTluindexREWCPTime} \\
\DC		& \roh{\SLOWluindexDCExcTime}	& \roh{\SLOWluindexDCnoGExcTime}	& \roh{\FASTluindexFTODCTime}	& \roh{\FASTluindexREDCTime} \\
\CAPO	& \roh{\SLOWluindexCAPOExcTime}	& \roh{\SLOWluindexCAPOnoGExcTime}	& \roh{\FASTluindexFTOCAPOTime}	& \roh{\FASTluindexRECAPOTime} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWlusearchHBTime}			& \roh{\FASTlusearchFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWlusearchWCPTime}			& \roh{\FASTlusearchFTOWCPTime}	& \roh{\FASTlusearchREWCPTime} \\
\DC		& \roh{\SLOWlusearchDCExcTime}	& \roh{\SLOWlusearchDCnoGExcTime}	& \roh{\FASTlusearchFTODCTime}	& \roh{\FASTlusearchREDCTime} \\
\CAPO	& \roh{\SLOWlusearchCAPOExcTime}	& \roh{\SLOWlusearchCAPOnoGExcTime}	& \roh{\FASTlusearchFTOCAPOTime}	& \roh{\FASTlusearchRECAPOTime} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{lusearch}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWpmdHBTime}			& \roh{\FASTpmdFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWpmdWCPTime}			& \roh{\FASTpmdFTOWCPTime}	& \roh{\FASTpmdREWCPTime} \\
\DC		& \roh{\SLOWpmdDCExcTime}	& \roh{\SLOWpmdDCnoGExcTime}	& \roh{\FASTpmdFTODCTime}	& \roh{\FASTpmdREDCTime} \\
\CAPO	& \roh{\SLOWpmdCAPOExcTime}	& \roh{\SLOWpmdCAPOnoGExcTime}	& \roh{\FASTpmdFTOCAPOTime}	& \roh{\FASTpmdRECAPOTime} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWsunflowHBTime}			& \roh{\FASTsunflowFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWsunflowWCPTime}			& \roh{\FASTsunflowFTOWCPTime}	& \roh{\FASTsunflowREWCPTime} \\
\DC		& \roh{\SLOWsunflowDCExcTime}	& \roh{\SLOWsunflowDCnoGExcTime}	& \roh{\FASTsunflowFTODCTime}	& \roh{\FASTsunflowREDCTime} \\
\CAPO	& \roh{\SLOWsunflowCAPOExcTime}	& \roh{\SLOWsunflowCAPOnoGExcTime}	& \roh{\FASTsunflowFTOCAPOTime}	& \roh{\FASTsunflowRECAPOTime} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWtomcatHBTime}			& \roh{\FASTtomcatFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWtomcatWCPTime}			& \roh{\FASTtomcatFTOWCPTime}	& \roh{\FASTtomcatREWCPTime} \\
\DC		& \roh{\SLOWtomcatDCExcTime}	& \roh{\SLOWtomcatDCnoGExcTime}	& \roh{\FASTtomcatFTODCTime}	& \roh{\FASTtomcatREDCTime} \\
\CAPO	& \roh{\SLOWtomcatCAPOExcTime}	& \roh{\SLOWtomcatCAPOnoGExcTime}	& \roh{\FASTtomcatFTOCAPOTime}	& \roh{\FASTtomcatRECAPOTime} \\
		& \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWxalanHBTime}			& \roh{\FASTxalanFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWxalanWCPTime}			& \roh{\FASTxalanFTOWCPTime}	& \roh{\FASTxalanREWCPTime} \\
\DC		& \roh{\SLOWxalanDCExcTime}	& \roh{\SLOWxalanDCnoGExcTime}	& \roh{\FASTxalanFTODCTime}	& \roh{\FASTxalanREDCTime} \\
\CAPO	& \roh{\SLOWxalanCAPOExcTime}	& \roh{\SLOWxalanCAPOnoGExcTime}	& \roh{\FASTxalanFTOCAPOTime}	& \roh{\FASTxalanRECAPOTime} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\end{empty}

\jake{Configuration: 10 trials, no stats collected.
Unopt-* results are the latest evaluation of removing setting cores to 8.
FTO-* and ST-* also remove setting cores to 8 and initialize extra metadata to null
and sets extra metadata to null if empty.}
\caption{Run time, relative to uninstrumented execution, of various analyses for each evaluated program.}
\label{tab:performance:allDaCapo}
\medskip
% Table for 10 trials of all relations with various optimizations for all DaCapo benchmarks
\begin{empty}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOpt2Quiet}
%
\smaller
\centering
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWavroraHBMem}		& \mem{\FASTavroraFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWavroraWCPMem}		& \mem{\FASTavroraFTOWCPMem}	& \mem{\FASTavroraREWCPMem} \\
\DC		& \mem{\SLOWavroraDCExcMem}	& \mem{\SLOWavroraDCnoGExcMem}	& \mem{\FASTavroraFTODCMem}		& \mem{\FASTavroraREDCMem} \\
\CAPO	& \mem{\SLOWavroraCAPOExcMem}	& \mem{\SLOWavroraCAPOnoGExcMem}& \mem{\FASTavroraFTOCAPOMem}	& \mem{\FASTavroraRECAPOMem} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWbatikHBMem}		& \mem{\FASTbatikFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWbatikWCPMem}		& \mem{\FASTbatikFTOWCPMem}	& \mem{\FASTbatikREWCPMem} \\
\DC		& \mem{\SLOWbatikDCExcMem}	& \mem{\SLOWbatikDCnoGExcMem}	& \mem{\FASTbatikFTODCMem}		& \mem{\FASTbatikREDCMem} \\
\CAPO	& \mem{\SLOWbatikCAPOExcMem}	& \mem{\SLOWbatikCAPOnoGExcMem}& \mem{\FASTbatikFTOCAPOMem}	& \mem{\FASTbatikRECAPOMem} \\
		& \mc{4}{c}{\bench{batik}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWhtwoHBMem}		& \mem{\FASThtwoFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWhtwoWCPMem}		& \mem{\FASThtwoFTOWCPMem}	& \mem{\FASThtwoREWCPMem} \\
\DC		& \mem{\SLOWhtwoDCExcMem}	& \mem{\SLOWhtwoDCnoGExcMem}	& \mem{\FASThtwoFTODCMem}		& \mem{\FASThtwoREDCMem} \\
\CAPO	& \mem{\SLOWhtwoCAPOExcMem}	& \mem{\SLOWhtwoCAPOnoGExcMem}& \mem{\FASThtwoFTOCAPOMem}	& \mem{\FASThtwoRECAPOMem} \\
		& \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWjythonHBMem}		& \mem{\FASTjythonFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWjythonWCPMem}		& \mem{\FASTjythonFTOWCPMem}	& \mem{\FASTjythonREWCPMem} \\
\DC		& \mem{\SLOWjythonDCExcMem}	& \mem{\SLOWjythonDCnoGExcMem}	& \mem{\FASTjythonFTODCMem}		& \mem{\FASTjythonREDCMem} \\
\CAPO	& \mem{\SLOWjythonCAPOExcMem}	& \mem{\SLOWjythonCAPOnoGExcMem}& \mem{\FASTjythonFTOCAPOMem}	& \mem{\FASTjythonRECAPOMem} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWluindexHBMem}		& \mem{\FASTluindexFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWluindexWCPMem}		& \mem{\FASTluindexFTOWCPMem}	& \mem{\FASTluindexREWCPMem} \\
\DC		& \mem{\SLOWluindexDCExcMem}	& \mem{\SLOWluindexDCnoGExcMem}	& \mem{\FASTluindexFTODCMem}		& \mem{\FASTluindexREDCMem} \\
\CAPO	& \mem{\SLOWluindexCAPOExcMem}	& \mem{\SLOWluindexCAPOnoGExcMem}& \mem{\FASTluindexFTOCAPOMem}	& \mem{\FASTluindexRECAPOMem} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWlusearchHBMem}		& \mem{\FASTlusearchFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWlusearchWCPMem}		& \mem{\FASTlusearchFTOWCPMem}	& \mem{\FASTlusearchREWCPMem} \\
\DC		& \mem{\SLOWlusearchDCExcMem}	& \mem{\SLOWlusearchDCnoGExcMem}	& \mem{\FASTlusearchFTODCMem}		& \mem{\FASTlusearchREDCMem} \\
\CAPO	& \mem{\SLOWlusearchCAPOExcMem}	& \mem{\SLOWlusearchCAPOnoGExcMem}& \mem{\FASTlusearchFTOCAPOMem}	& \mem{\FASTlusearchRECAPOMem} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{lusearch}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWpmdHBMem}		& \mem{\FASTpmdFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWpmdWCPMem}		& \mem{\FASTpmdFTOWCPMem}	& \mem{\FASTpmdREWCPMem} \\
\DC		& \mem{\SLOWpmdDCExcMem}	& \mem{\SLOWpmdDCnoGExcMem}	& \mem{\FASTpmdFTODCMem}		& \mem{\FASTpmdREDCMem} \\
\CAPO	& \mem{\SLOWpmdCAPOExcMem}	& \mem{\SLOWpmdCAPOnoGExcMem}& \mem{\FASTpmdFTOCAPOMem}	& \mem{\FASTpmdRECAPOMem} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWsunflowHBMem}		& \mem{\FASTsunflowFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWsunflowWCPMem}		& \mem{\FASTsunflowFTOWCPMem}	& \mem{\FASTsunflowREWCPMem} \\
\DC		& \mem{\SLOWsunflowDCExcMem}	& \mem{\SLOWsunflowDCnoGExcMem}	& \mem{\FASTsunflowFTODCMem}		& \mem{\FASTsunflowREDCMem} \\
\CAPO	& \mem{\SLOWsunflowCAPOExcMem}	& \mem{\SLOWsunflowCAPOnoGExcMem}& \mem{\FASTsunflowFTOCAPOMem}	& \mem{\FASTsunflowRECAPOMem} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWtomcatHBMem}		& \mem{\FASTtomcatFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWtomcatWCPMem}		& \mem{\FASTtomcatFTOWCPMem}	& \mem{\FASTtomcatREWCPMem} \\
\DC		& \mem{\SLOWtomcatDCExcMem}	& \mem{\SLOWtomcatDCnoGExcMem}	& \mem{\FASTtomcatFTODCMem}		& \mem{\FASTtomcatREDCMem} \\
\CAPO	& \mem{\SLOWtomcatCAPOExcMem}	& \mem{\SLOWtomcatCAPOnoGExcMem}& \mem{\FASTtomcatFTOCAPOMem}	& \mem{\FASTtomcatRECAPOMem} \\
		& \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWxalanHBMem}		& \mem{\FASTxalanFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWxalanWCPMem}		& \mem{\FASTxalanFTOWCPMem}	& \mem{\FASTxalanREWCPMem} \\
\DC		& \mem{\SLOWxalanDCExcMem}	& \mem{\SLOWxalanDCnoGExcMem}	& \mem{\FASTxalanFTODCMem}		& \mem{\FASTxalanREDCMem} \\
\CAPO	& \mem{\SLOWxalanCAPOExcMem}	& \mem{\SLOWxalanCAPOnoGExcMem}& \mem{\FASTxalanFTOCAPOMem}	& \mem{\FASTxalanRECAPOMem} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\end{empty}

\jake{Configuration: 10 trials, no stats collected.
Unopt-* results are the latest evaluation of removing setting cores to 8.
FTO-* and ST-* also remove setting cores to 8 and initialize extra metadata to null
and sets extra metadata to null if empty.}

\caption{Memory usage, relative to uninstrumented execution, of various analyses for each evaluated program.}
\label{tab:memory:allDaCapo}
\end{table}

% Table for 10 trials of all relations with various optimizations for xalan benchmark
\begin{table}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
% \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;Mb$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\sdr}[2]{#1{\;}(#2)}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOpt2Quiet}
%
\smaller
\centering
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWavroraHB}{\SLOWavroraHBDynamic}					& \sdr{\FASTavroraFTOHB}{\FASTavroraFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWavroraWCP}{\SLOWavroraWCPDynamic}				& \sdr{\FASTavroraFTOWCP}{\FASTavroraFTOWCPDynamic}		& \sdr{\FASTavroraREWCP}{\FASTavroraREWCPDynamic} \\
\DC		& \sdr{\SLOWavroraDCExc}{\SLOWavroraDCExcDynamic}		& \sdr{\SLOWavroraDCnoGExc}{\SLOWavroraDCnoGExcDynamic}	& \sdr{\FASTavroraFTODC}{\FASTavroraFTODCDynamic}		& \sdr{\FASTavroraREDC}{\FASTavroraREDCDynamic} \\
\CAPO	& \sdr{\SLOWavroraCAPOExc}{\SLOWavroraCAPOExcDynamic}	& \sdr{\SLOWavroraCAPOnoGExc}{\SLOWavroraCAPOnoGExcDynamic}	& \sdr{\FASTavroraFTOCAPO}{\FASTavroraFTOCAPODynamic}	& \sdr{\FASTavroraRECAPO}{\FASTavroraRECAPODynamic} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWhtwoHB}{\SLOWhtwoHBDynamic}					& \sdr{\FASThtwoFTOHB}{\FASThtwoFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWhtwoWCP}{\SLOWhtwoWCPDynamic}				& \sdr{\FASThtwoFTOWCP}{\FASThtwoFTOWCPDynamic}		& \sdr{\FASThtwoREWCP}{\FASThtwoREWCPDynamic} \\
\DC		& \sdr{\SLOWhtwoDCExc}{\SLOWhtwoDCExcDynamic}		& \sdr{\SLOWhtwoDCnoGExc}{\SLOWhtwoDCnoGExcDynamic}	& \sdr{\FASThtwoFTODC}{\FASThtwoFTODCDynamic}		& \sdr{\FASThtwoREDC}{\FASThtwoREDCDynamic} \\
\CAPO	& \sdr{\SLOWhtwoCAPOExc}{\SLOWhtwoCAPOExcDynamic}	& \sdr{\SLOWhtwoCAPOnoGExc}{\SLOWhtwoCAPOnoGExcDynamic}	& \sdr{\FASThtwoFTOCAPO}{\FASThtwoFTOCAPODynamic}	& \sdr{\FASThtwoRECAPO}{\FASThtwoRECAPODynamic} \\
		& \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWjythonHB}{\SLOWjythonHBDynamic}					& \sdr{\FASTjythonFTOHB}{\FASTjythonFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWjythonWCP}{\SLOWjythonWCPDynamic}				& \sdr{\FASTjythonFTOWCP}{\FASTjythonFTOWCPDynamic}		& \sdr{\FASTjythonREWCP}{\FASTjythonREWCPDynamic} \\
\DC		& \sdr{\SLOWjythonDCExc}{\SLOWjythonDCExcDynamic}		& \sdr{\SLOWjythonDCnoGExc}{\SLOWjythonDCnoGExcDynamic}	& \sdr{\FASTjythonFTODC}{\FASTjythonFTODCDynamic}		& \sdr{\FASTjythonREDC}{\FASTjythonREDCDynamic} \\
\CAPO	& \sdr{\SLOWjythonCAPOExc}{\SLOWjythonCAPOExcDynamic}	& \sdr{\SLOWjythonCAPOnoGExc}{\SLOWjythonCAPOnoGExcDynamic}	& \sdr{\FASTjythonFTOCAPO}{\FASTjythonFTOCAPODynamic}	& \sdr{\FASTjythonRECAPO}{\FASTjythonRECAPODynamic} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWluindexHB}{\SLOWluindexHBDynamic}					& \sdr{\FASTluindexFTOHB}{\FASTluindexFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWluindexWCP}{\SLOWluindexWCPDynamic}				& \sdr{\FASTluindexFTOWCP}{\FASTluindexFTOWCPDynamic}		& \sdr{\FASTluindexREWCP}{\FASTluindexREWCPDynamic} \\
\DC		& \sdr{\SLOWluindexDCExc}{\SLOWluindexDCExcDynamic}		& \sdr{\SLOWluindexDCnoGExc}{\SLOWluindexDCnoGExcDynamic}	& \sdr{\FASTluindexFTODC}{\FASTluindexFTODCDynamic}		& \sdr{\FASTluindexREDC}{\FASTluindexREDCDynamic} \\
\CAPO	& \sdr{\SLOWluindexCAPOExc}{\SLOWluindexCAPOExcDynamic}	& \sdr{\SLOWluindexCAPOnoGExc}{\SLOWluindexCAPOnoGExcDynamic}	& \sdr{\FASTluindexFTOCAPO}{\FASTluindexFTOCAPODynamic}	& \sdr{\FASTluindexRECAPO}{\FASTluindexRECAPODynamic} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWpmdHB}{\SLOWpmdHBDynamic}					& \sdr{\FASTpmdFTOHB}{\FASTpmdFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWpmdWCP}{\SLOWpmdWCPDynamic}				& \sdr{\FASTpmdFTOWCP}{\FASTpmdFTOWCPDynamic}		& \sdr{\FASTpmdREWCP}{\FASTpmdREWCPDynamic} \\
\DC		& \sdr{\SLOWpmdDCExc}{\SLOWpmdDCExcDynamic}		& \sdr{\SLOWpmdDCnoGExc}{\SLOWpmdDCnoGExcDynamic}	& \sdr{\FASTpmdFTODC}{\FASTpmdFTODCDynamic}		& \sdr{\FASTpmdREDC}{\FASTpmdREDCDynamic} \\
\CAPO	& \sdr{\SLOWpmdCAPOExc}{\SLOWpmdCAPOExcDynamic}	& \sdr{\SLOWpmdCAPOnoGExc}{\SLOWpmdCAPOnoGExcDynamic}	& \sdr{\FASTpmdFTOCAPO}{\FASTpmdFTOCAPODynamic}	& \sdr{\FASTpmdRECAPO}{\FASTpmdRECAPODynamic} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWsunflowHB}{\SLOWsunflowHBDynamic}					& \sdr{\FASTsunflowFTOHB}{\FASTsunflowFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWsunflowWCP}{\SLOWsunflowWCPDynamic}				& \sdr{\FASTsunflowFTOWCP}{\FASTsunflowFTOWCPDynamic}		& \sdr{\FASTsunflowREWCP}{\FASTsunflowREWCPDynamic} \\
\DC		& \sdr{\SLOWsunflowDCExc}{\SLOWsunflowDCExcDynamic}		& \sdr{\SLOWsunflowDCnoGExc}{\SLOWsunflowDCnoGExcDynamic}	& \sdr{\FASTsunflowFTODC}{\FASTsunflowFTODCDynamic}		& \sdr{\FASTsunflowREDC}{\FASTsunflowREDCDynamic} \\
\CAPO	& \sdr{\SLOWsunflowCAPOExc}{\SLOWsunflowCAPOExcDynamic}	& \sdr{\SLOWsunflowCAPOnoGExc}{\SLOWsunflowCAPOnoGExcDynamic}	& \sdr{\FASTsunflowFTOCAPO}{\FASTsunflowFTOCAPODynamic}	& \sdr{\FASTsunflowRECAPO}{\FASTsunflowRECAPODynamic} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWtomcatHB}{\SLOWtomcatHBDynamic}					& \sdr{\FASTtomcatFTOHB}{\FASTtomcatFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWtomcatWCP}{\SLOWtomcatWCPDynamic}				& \sdr{\FASTtomcatFTOWCP}{\FASTtomcatFTOWCPDynamic}		& \sdr{\FASTtomcatREWCP}{\FASTtomcatREWCPDynamic} \\
\DC		& \sdr{\SLOWtomcatDCExc}{\SLOWtomcatDCExcDynamic}		& \sdr{\SLOWtomcatDCnoGExc}{\SLOWtomcatDCnoGExcDynamic}	& \sdr{\FASTtomcatFTODC}{\FASTtomcatFTODCDynamic}		& \sdr{\FASTtomcatREDC}{\FASTtomcatREDCDynamic} \\
\CAPO	& \sdr{\SLOWtomcatCAPOExc}{\SLOWtomcatCAPOExcDynamic}	& \sdr{\SLOWtomcatCAPOnoGExc}{\SLOWtomcatCAPOnoGExcDynamic}	& \sdr{\FASTtomcatFTOCAPO}{\FASTtomcatFTOCAPODynamic}	& \sdr{\FASTtomcatRECAPO}{\FASTtomcatRECAPODynamic} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWxalanHB}{\SLOWxalanHBDynamic}					& \sdr{\FASTxalanFTOHB}{\FASTxalanFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWxalanWCP}{\SLOWxalanWCPDynamic}				& \sdr{\FASTxalanFTOWCP}{\FASTxalanFTOWCPDynamic}		& \sdr{\FASTxalanREWCP}{\FASTxalanREWCPDynamic} \\
\DC		& \sdr{\SLOWxalanDCExc}{\SLOWxalanDCExcDynamic}		& \sdr{\SLOWxalanDCnoGExc}{\SLOWxalanDCnoGExcDynamic}	& \sdr{\FASTxalanFTODC}{\FASTxalanFTODCDynamic}		& \sdr{\FASTxalanREDC}{\FASTxalanREDCDynamic} \\
\CAPO	& \sdr{\SLOWxalanCAPOExc}{\SLOWxalanCAPOExcDynamic}	& \sdr{\SLOWxalanCAPOnoGExc}{\SLOWxalanCAPOnoGExcDynamic}	& \sdr{\FASTxalanFTOCAPO}{\FASTxalanFTOCAPODynamic}	& \sdr{\FASTxalanRECAPO}{\FASTxalanRECAPODynamic} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}

\jake{Configuration: 10 trials, no stats collected.
Unopt-* results are the latest evaluation of removing setting cores to 8.
FTO-* and ST-* also remove setting cores to 8 and initialize extra metadata to null
and sets extra metadata to null if empty.}

\caption{Average races reported by various analyses for each evaluated program
(excluding \bench{batik} and \bench{lusearch}, for which all analyses report no races).
In each cell, the first value is statically distinct races
(\ie, distinct program locations) and the second value, in parentheses, is total dynamic races.}
\label{tab:race:allDaCapo}
\end{table}

\section{Results duplicating above set of result tables with including confidence intervals}

\begin{table}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
% \input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOpt2Quiet}
%
\small
\centering
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWavroraHBTime}{\SLOWavroraHBTimeCI}			& \vci{\FASTavroraFTOHBTime}{\FASTavroraFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWavroraWCPTime}{\SLOWavroraWCPTimeCI}			& \vci{\FASTavroraFTOWCPTime}{\FASTavroraFTOWCPTimeCI}	& \vci{\FASTavroraREWCPTime}{\FASTavroraREWCPTimeCI} \\
\DC		& \vci{\SLOWavroraDCExcTime}{\SLOWavroraDCExcTimeCI}	& \vci{\SLOWavroraDCnoGExcTime}{\SLOWavroraDCnoGExcTimeCI}	& \vci{\FASTavroraFTODCTime}{\FASTavroraFTODCTimeCI}	& \vci{\FASTavroraREDCTime}{\FASTavroraREDCTimeCI} \\
\CAPO	& \vci{\SLOWavroraCAPOExcTime}{\SLOWavroraCAPOExcTimeCI}	& \vci{\SLOWavroraCAPOnoGExcTime}{\SLOWavroraCAPOnoGExcTimeCI}	& \vci{\FASTavroraFTOCAPOTime}{\FASTavroraFTOCAPOTimeCI}	& \vci{\FASTavroraRECAPOTime}{\FASTavroraRECAPOTimeCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWbatikHBTime}{\SLOWbatikHBTimeCI}			& \vci{\FASTbatikFTOHBTime}{\FASTbatikFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWbatikWCPTime}{\SLOWbatikWCPTimeCI}			& \vci{\FASTbatikFTOWCPTime}{\FASTbatikFTOWCPTimeCI}	& \vci{\FASTbatikREWCPTime}{\FASTbatikREWCPTimeCI} \\
\DC		& \vci{\SLOWbatikDCExcTime}{\SLOWbatikDCExcTimeCI}	& \vci{\SLOWbatikDCnoGExcTime}{\SLOWbatikDCnoGExcTimeCI}	& \vci{\FASTbatikFTODCTime}{\FASTbatikFTODCTimeCI}	& \vci{\FASTbatikREDCTime}{\FASTbatikREDCTimeCI} \\
\CAPO	& \vci{\SLOWbatikCAPOExcTime}{\SLOWbatikCAPOExcTimeCI}	& \vci{\SLOWbatikCAPOnoGExcTime}{\SLOWbatikCAPOnoGExcTimeCI}	& \vci{\FASTbatikFTOCAPOTime}{\FASTbatikFTOCAPOTimeCI}	& \vci{\FASTbatikRECAPOTime}{\FASTbatikRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{batik}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWhtwoHBTime}{\SLOWhtwoHBTimeCI}			& \vci{\FASThtwoFTOHBTime}{\FASThtwoFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWhtwoWCPTime}{\SLOWhtwoWCPTimeCI}			& \vci{\FASThtwoFTOWCPTime}{\FASThtwoFTOWCPTimeCI}	& \vci{\FASThtwoREWCPTime}{\FASThtwoREWCPTimeCI} \\
\DC		& \vci{\SLOWhtwoDCExcTime}{\SLOWhtwoDCExcTimeCI}	& \vci{\SLOWhtwoDCnoGExcTime}{\SLOWhtwoDCnoGExcTimeCI}	& \vci{\FASThtwoFTODCTime}{\FASThtwoFTODCTimeCI}	& \vci{\FASThtwoREDCTime}{\FASThtwoREDCTimeCI} \\
\CAPO	& \vci{\SLOWhtwoCAPOExcTime}{\SLOWhtwoCAPOExcTimeCI}	& \vci{\SLOWhtwoCAPOnoGExcTime}{\SLOWhtwoCAPOnoGExcTimeCI}	& \vci{\FASThtwoFTOCAPOTime}{\FASThtwoFTOCAPOTimeCI}	& \vci{\FASThtwoRECAPOTime}{\FASThtwoRECAPOTimeCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWjythonHBTime}{\SLOWjythonHBTimeCI}			& \vci{\FASTjythonFTOHBTime}{\FASTjythonFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWjythonWCPTime}{\SLOWjythonWCPTimeCI}			& \vci{\FASTjythonFTOWCPTime}{\FASTjythonFTOWCPTimeCI}	& \vci{\FASTjythonREWCPTime}{\FASTjythonREWCPTimeCI} \\
\DC		& \vci{\SLOWjythonDCExcTime}{\SLOWjythonDCExcTimeCI}	& \vci{\SLOWjythonDCnoGExcTime}{\SLOWjythonDCnoGExcTimeCI}	& \vci{\FASTjythonFTODCTime}{\FASTjythonFTODCTimeCI}	& \vci{\FASTjythonREDCTime}{\FASTjythonREDCTimeCI} \\
\CAPO	& \vci{\SLOWjythonCAPOExcTime}{\SLOWjythonCAPOExcTimeCI}	& \vci{\SLOWjythonCAPOnoGExcTime}{\SLOWjythonCAPOnoGExcTimeCI}	& \vci{\FASTjythonFTOCAPOTime}{\FASTjythonFTOCAPOTimeCI}	& \vci{\FASTjythonRECAPOTime}{\FASTjythonRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWluindexHBTime}{\SLOWluindexHBTimeCI}			& \vci{\FASTluindexFTOHBTime}{\FASTluindexFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWluindexWCPTime}{\SLOWluindexWCPTimeCI}			& \vci{\FASTluindexFTOWCPTime}{\FASTluindexFTOWCPTimeCI}	& \vci{\FASTluindexREWCPTime}{\FASTluindexREWCPTimeCI} \\
\DC		& \vci{\SLOWluindexDCExcTime}{\SLOWluindexDCExcTimeCI}	& \vci{\SLOWluindexDCnoGExcTime}{\SLOWluindexDCnoGExcTimeCI}	& \vci{\FASTluindexFTODCTime}{\FASTluindexFTODCTimeCI}	& \vci{\FASTluindexREDCTime}{\FASTluindexREDCTimeCI} \\
\CAPO	& \vci{\SLOWluindexCAPOExcTime}{\SLOWluindexCAPOExcTimeCI}	& \vci{\SLOWluindexCAPOnoGExcTime}{\SLOWluindexCAPOnoGExcTimeCI}	& \vci{\FASTluindexFTOCAPOTime}{\FASTluindexFTOCAPOTimeCI}	& \vci{\FASTluindexRECAPOTime}{\FASTluindexRECAPOTimeCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWlusearchHBTime}{\SLOWlusearchHBTimeCI}			& \vci{\FASTlusearchFTOHBTime}{\FASTlusearchFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWlusearchWCPTime}{\SLOWlusearchWCPTimeCI}			& \vci{\FASTlusearchFTOWCPTime}{\FASTlusearchFTOWCPTimeCI}	& \vci{\FASTlusearchREWCPTime}{\FASTlusearchREWCPTimeCI} \\
\DC		& \vci{\SLOWlusearchDCExcTime}{\SLOWlusearchDCExcTimeCI}	& \vci{\SLOWlusearchDCnoGExcTime}{\SLOWlusearchDCnoGExcTimeCI}	& \vci{\FASTlusearchFTODCTime}{\FASTlusearchFTODCTimeCI}	& \vci{\FASTlusearchREDCTime}{\FASTlusearchREDCTimeCI} \\
\CAPO	& \vci{\SLOWlusearchCAPOExcTime}{\SLOWlusearchCAPOExcTimeCI}	& \vci{\SLOWlusearchCAPOnoGExcTime}{\SLOWlusearchCAPOnoGExcTimeCI}	& \vci{\FASTlusearchFTOCAPOTime}{\FASTlusearchFTOCAPOTimeCI}	& \vci{\FASTlusearchRECAPOTime}{\FASTlusearchRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{lusearch}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWpmdHBTime}{\SLOWpmdHBTimeCI}			& \vci{\FASTpmdFTOHBTime}{\FASTpmdFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWpmdWCPTime}{\SLOWpmdWCPTimeCI}			& \vci{\FASTpmdFTOWCPTime}{\FASTpmdFTOWCPTimeCI}	& \vci{\FASTpmdREWCPTime}{\FASTpmdREWCPTimeCI} \\
\DC		& \vci{\SLOWpmdDCExcTime}{\SLOWpmdDCExcTimeCI}	& \vci{\SLOWpmdDCnoGExcTime}{\SLOWpmdDCnoGExcTimeCI}	& \vci{\FASTpmdFTODCTime}{\FASTpmdFTODCTimeCI}	& \vci{\FASTpmdREDCTime}{\FASTpmdREDCTimeCI} \\
\CAPO	& \vci{\SLOWpmdCAPOExcTime}{\SLOWpmdCAPOExcTimeCI}	& \vci{\SLOWpmdCAPOnoGExcTime}{\SLOWpmdCAPOnoGExcTimeCI}	& \vci{\FASTpmdFTOCAPOTime}{\FASTpmdFTOCAPOTimeCI}	& \vci{\FASTpmdRECAPOTime}{\FASTpmdRECAPOTimeCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWsunflowHBTime}{\SLOWsunflowHBTimeCI}			& \vci{\FASTsunflowFTOHBTime}{\FASTsunflowFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWsunflowWCPTime}{\SLOWsunflowWCPTimeCI}			& \vci{\FASTsunflowFTOWCPTime}{\FASTsunflowFTOWCPTimeCI}	& \vci{\FASTsunflowREWCPTime}{\FASTsunflowREWCPTimeCI} \\
\DC		& \vci{\SLOWsunflowDCExcTime}{\SLOWsunflowDCExcTimeCI}	& \vci{\SLOWsunflowDCnoGExcTime}{\SLOWsunflowDCnoGExcTimeCI}	& \vci{\FASTsunflowFTODCTime}{\FASTsunflowFTODCTimeCI}	& \vci{\FASTsunflowREDCTime}{\FASTsunflowREDCTimeCI} \\
\CAPO	& \vci{\SLOWsunflowCAPOExcTime}{\SLOWsunflowCAPOExcTimeCI}	& \vci{\SLOWsunflowCAPOnoGExcTime}{\SLOWsunflowCAPOnoGExcTimeCI}	& \vci{\FASTsunflowFTOCAPOTime}{\FASTsunflowFTOCAPOTimeCI}	& \vci{\FASTsunflowRECAPOTime}{\FASTsunflowRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWtomcatHBTime}{\SLOWtomcatHBTimeCI}			& \vci{\FASTtomcatFTOHBTime}{\FASTtomcatFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWtomcatWCPTime}{\SLOWtomcatWCPTimeCI}			& \vci{\FASTtomcatFTOWCPTime}{\FASTtomcatFTOWCPTimeCI}	& \vci{\FASTtomcatREWCPTime}{\FASTtomcatREWCPTimeCI} \\
\DC		& \vci{\SLOWtomcatDCExcTime}{\SLOWtomcatDCExcTimeCI}	& \vci{\SLOWtomcatDCnoGExcTime}{\SLOWtomcatDCnoGExcTimeCI}	& \vci{\FASTtomcatFTODCTime}{\FASTtomcatFTODCTimeCI}	& \vci{\FASTtomcatREDCTime}{\FASTtomcatREDCTimeCI} \\
\CAPO	& \vci{\SLOWtomcatCAPOExcTime}{\SLOWtomcatCAPOExcTimeCI}	& \vci{\SLOWtomcatCAPOnoGExcTime}{\SLOWtomcatCAPOnoGExcTimeCI}	& \vci{\FASTtomcatFTOCAPOTime}{\FASTtomcatFTOCAPOTimeCI}	& \vci{\FASTtomcatRECAPOTime}{\FASTtomcatRECAPOTimeCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWxalanHBTime}{\SLOWxalanHBTimeCI}			& \vci{\FASTxalanFTOHBTime}{\FASTxalanFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWxalanWCPTime}{\SLOWxalanWCPTimeCI}			& \vci{\FASTxalanFTOWCPTime}{\FASTxalanFTOWCPTimeCI}	& \vci{\FASTxalanREWCPTime}{\FASTxalanREWCPTimeCI} \\
\DC		& \vci{\SLOWxalanDCExcTime}{\SLOWxalanDCExcTimeCI}	& \vci{\SLOWxalanDCnoGExcTime}{\SLOWxalanDCnoGExcTimeCI}	& \vci{\FASTxalanFTODCTime}{\FASTxalanFTODCTimeCI}	& \vci{\FASTxalanREDCTime}{\FASTxalanREDCTimeCI} \\
\CAPO	& \vci{\SLOWxalanCAPOExcTime}{\SLOWxalanCAPOExcTimeCI}	& \vci{\SLOWxalanCAPOnoGExcTime}{\SLOWxalanCAPOnoGExcTimeCI}	& \vci{\FASTxalanFTOCAPOTime}{\FASTxalanFTOCAPOTimeCI}	& \vci{\FASTxalanRECAPOTime}{\FASTxalanRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\jake{Configuration: 10 trials, no stats collected.
Unopt-* results are the latest evaluation of removing setting cores to 8.
FTO-* and ST-* also remove setting cores to 8 and initialize extra metadata to null
and sets extra metadata to null if empty.}
\caption{Run time, relative to uninstrumented execution, of various analyses for each evaluated program
with 95\% confidence intervals.}
\label{tab:performance:allDaCapo:CI}
\end{table}
% Table for 10 trials of all relations with various optimizations for all DaCapo benchmarks
\begin{table}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
%memory \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$Gb$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
% \input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOpt2Quiet}
%
\small
\centering
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWavroraHBMem}{\SLOWavroraHBMemCI}		& \vci{\FASTavroraFTOHBMem}{\FASTavroraFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWavroraWCPMem}{\SLOWavroraWCPMemCI}		& \vci{\FASTavroraFTOWCPMem}{\FASTavroraFTOWCPMemCI}	& \vci{\FASTavroraREWCPMem}{\FASTavroraREWCPMemCI} \\
\DC		& \vci{\SLOWavroraDCExcMem}{\SLOWavroraDCExcMemCI}	& \vci{\SLOWavroraDCnoGExcMem}{\SLOWavroraDCnoGExcMemCI}	& \vci{\FASTavroraFTODCMem}{\FASTavroraFTODCMemCI}		& \vci{\FASTavroraREDCMem}{\FASTavroraREDCMemCI} \\
\CAPO	& \vci{\SLOWavroraCAPOExcMem}{\SLOWavroraCAPOExcMemCI}	& \vci{\SLOWavroraCAPOnoGExcMem}{\SLOWavroraCAPOnoGExcMemCI}& \vci{\FASTavroraFTOCAPOMem}{\FASTavroraFTOCAPOMemCI}	& \vci{\FASTavroraRECAPOMem}{\FASTavroraRECAPOMemCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWbatikHBMem}{\SLOWbatikHBMemCI}		& \vci{\FASTbatikFTOHBMem}{\FASTbatikFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWbatikWCPMem}{\SLOWbatikWCPMemCI}		& \vci{\FASTbatikFTOWCPMem}{\FASTbatikFTOWCPMemCI}	& \vci{\FASTbatikREWCPMem}{\FASTbatikREWCPMemCI} \\
\DC		& \vci{\SLOWbatikDCExcMem}{\SLOWbatikDCExcMemCI}	& \vci{\SLOWbatikDCnoGExcMem}{\SLOWbatikDCnoGExcMemCI}	& \vci{\FASTbatikFTODCMem}{\FASTbatikFTODCMemCI}		& \vci{\FASTbatikREDCMem}{\FASTbatikREDCMemCI} \\
\CAPO	& \vci{\SLOWbatikCAPOExcMem}{\SLOWbatikCAPOExcMemCI}	& \vci{\SLOWbatikCAPOnoGExcMem}{\SLOWbatikCAPOnoGExcMemCI}& \vci{\FASTbatikFTOCAPOMem}{\FASTbatikFTOCAPOMemCI}	& \vci{\FASTbatikRECAPOMem}{\FASTbatikRECAPOMemCI} \\
		& \mc{4}{c}{\bench{batik}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWhtwoHBMem}{\SLOWhtwoHBMemCI}		& \vci{\FASThtwoFTOHBMem}{\FASThtwoFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWhtwoWCPMem}{\SLOWhtwoWCPMemCI}		& \vci{\FASThtwoFTOWCPMem}{\FASThtwoFTOWCPMemCI}	& \vci{\FASThtwoREWCPMem}{\FASThtwoREWCPMemCI} \\
\DC		& \vci{\SLOWhtwoDCExcMem}{\SLOWhtwoDCExcMemCI}	& \vci{\SLOWhtwoDCnoGExcMem}{\SLOWhtwoDCnoGExcMemCI}	& \vci{\FASThtwoFTODCMem}{\FASThtwoFTODCMemCI}		& \vci{\FASThtwoREDCMem}{\FASThtwoREDCMemCI} \\
\CAPO	& \vci{\SLOWhtwoCAPOExcMem}{\SLOWhtwoCAPOExcMemCI}	& \vci{\SLOWhtwoCAPOnoGExcMem}{\SLOWhtwoCAPOnoGExcMemCI}& \vci{\FASThtwoFTOCAPOMem}{\FASThtwoFTOCAPOMemCI}	& \vci{\FASThtwoRECAPOMem}{\FASThtwoRECAPOMemCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWjythonHBMem}{\SLOWjythonHBMemCI}		& \vci{\FASTjythonFTOHBMem}{\FASTjythonFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWjythonWCPMem}{\SLOWjythonWCPMemCI}		& \vci{\FASTjythonFTOWCPMem}{\FASTjythonFTOWCPMemCI}	& \vci{\FASTjythonREWCPMem}{\FASTjythonREWCPMemCI} \\
\DC		& \vci{\SLOWjythonDCExcMem}{\SLOWjythonDCExcMemCI}	& \vci{\SLOWjythonDCnoGExcMem}{\SLOWjythonDCnoGExcMemCI}	& \vci{\FASTjythonFTODCMem}{\FASTjythonFTODCMemCI}		& \vci{\FASTjythonREDCMem}{\FASTjythonREDCMemCI} \\
\CAPO	& \vci{\SLOWjythonCAPOExcMem}{\SLOWjythonCAPOExcMemCI}	& \vci{\SLOWjythonCAPOnoGExcMem}{\SLOWjythonCAPOnoGExcMemCI}& \vci{\FASTjythonFTOCAPOMem}{\FASTjythonFTOCAPOMemCI}	& \vci{\FASTjythonRECAPOMem}{\FASTjythonRECAPOMemCI} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWluindexHBMem}{\SLOWluindexHBMemCI}		& \vci{\FASTluindexFTOHBMem}{\FASTluindexFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWluindexWCPMem}{\SLOWluindexWCPMemCI}		& \vci{\FASTluindexFTOWCPMem}{\FASTluindexFTOWCPMemCI}	& \vci{\FASTluindexREWCPMem}{\FASTluindexREWCPMemCI} \\
\DC		& \vci{\SLOWluindexDCExcMem}{\SLOWluindexDCExcMemCI}	& \vci{\SLOWluindexDCnoGExcMem}{\SLOWluindexDCnoGExcMemCI}	& \vci{\FASTluindexFTODCMem}{\FASTluindexFTODCMemCI}		& \vci{\FASTluindexREDCMem}{\FASTluindexREDCMemCI} \\
\CAPO	& \vci{\SLOWluindexCAPOExcMem}{\SLOWluindexCAPOExcMemCI}	& \vci{\SLOWluindexCAPOnoGExcMem}{\SLOWluindexCAPOnoGExcMemCI}& \vci{\FASTluindexFTOCAPOMem}{\FASTluindexFTOCAPOMemCI}	& \vci{\FASTluindexRECAPOMem}{\FASTluindexRECAPOMemCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWlusearchHBMem}{\SLOWlusearchHBMemCI}		& \vci{\FASTlusearchFTOHBMem}{\FASTlusearchFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWlusearchWCPMem}{\SLOWlusearchWCPMemCI}		& \vci{\FASTlusearchFTOWCPMem}{\FASTlusearchFTOWCPMemCI}	& \vci{\FASTlusearchREWCPMem}{\FASTlusearchREWCPMemCI} \\
\DC		& \vci{\SLOWlusearchDCExcMem}{\SLOWlusearchDCExcMemCI}	& \vci{\SLOWlusearchDCnoGExcMem}{\SLOWlusearchDCnoGExcMemCI}	& \vci{\FASTlusearchFTODCMem}{\FASTlusearchFTODCMemCI}		& \vci{\FASTlusearchREDCMem}{\FASTlusearchREDCMemCI} \\
\CAPO	& \vci{\SLOWlusearchCAPOExcMem}{\SLOWlusearchCAPOExcMemCI}	& \vci{\SLOWlusearchCAPOnoGExcMem}{\SLOWlusearchCAPOnoGExcMemCI}& \vci{\FASTlusearchFTOCAPOMem}{\FASTlusearchFTOCAPOMemCI}	& \vci{\FASTlusearchRECAPOMem}{\FASTlusearchRECAPOMemCI} \\
		& \mc{4}{c}{\bench{lusearch}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWpmdHBMem}{\SLOWpmdHBMemCI}		& \vci{\FASTpmdFTOHBMem}{\FASTpmdFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWpmdWCPMem}{\SLOWpmdWCPMemCI}		& \vci{\FASTpmdFTOWCPMem}{\FASTpmdFTOWCPMemCI}	& \vci{\FASTpmdREWCPMem}{\FASTpmdREWCPMemCI} \\
\DC		& \vci{\SLOWpmdDCExcMem}{\SLOWpmdDCExcMemCI}	& \vci{\SLOWpmdDCnoGExcMem}{\SLOWpmdDCnoGExcMemCI}	& \vci{\FASTpmdFTODCMem}{\FASTpmdFTODCMemCI}		& \vci{\FASTpmdREDCMem}{\FASTpmdREDCMemCI} \\
\CAPO	& \vci{\SLOWpmdCAPOExcMem}{\SLOWpmdCAPOExcMemCI}	& \vci{\SLOWpmdCAPOnoGExcMem}{\SLOWpmdCAPOnoGExcMemCI}& \vci{\FASTpmdFTOCAPOMem}{\FASTpmdFTOCAPOMemCI}	& \vci{\FASTpmdRECAPOMem}{\FASTpmdRECAPOMemCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWsunflowHBMem}{\SLOWsunflowHBMemCI}		& \vci{\FASTsunflowFTOHBMem}{\FASTsunflowFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWsunflowWCPMem}{\SLOWsunflowWCPMemCI}		& \vci{\FASTsunflowFTOWCPMem}{\FASTsunflowFTOWCPMemCI}	& \vci{\FASTsunflowREWCPMem}{\FASTsunflowREWCPMemCI} \\
\DC		& \vci{\SLOWsunflowDCExcMem}{\SLOWsunflowDCExcMemCI}	& \vci{\SLOWsunflowDCnoGExcMem}{\SLOWsunflowDCnoGExcMemCI}	& \vci{\FASTsunflowFTODCMem}{\FASTsunflowFTODCMemCI}		& \vci{\FASTsunflowREDCMem}{\FASTsunflowREDCMemCI} \\
\CAPO	& \vci{\SLOWsunflowCAPOExcMem}{\SLOWsunflowCAPOExcMemCI}	& \vci{\SLOWsunflowCAPOnoGExcMem}{\SLOWsunflowCAPOnoGExcMemCI}& \vci{\FASTsunflowFTOCAPOMem}{\FASTsunflowFTOCAPOMemCI}	& \vci{\FASTsunflowRECAPOMem}{\FASTsunflowRECAPOMemCI} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWtomcatHBMem}{\SLOWtomcatHBMemCI}		& \vci{\FASTtomcatFTOHBMem}{\FASTtomcatFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWtomcatWCPMem}{\SLOWtomcatWCPMemCI}		& \vci{\FASTtomcatFTOWCPMem}{\FASTtomcatFTOWCPMemCI}	& \vci{\FASTtomcatREWCPMem}{\FASTtomcatREWCPMemCI} \\
\DC		& \vci{\SLOWtomcatDCExcMem}{\SLOWtomcatDCExcMemCI}	& \vci{\SLOWtomcatDCnoGExcMem}{\SLOWtomcatDCnoGExcMemCI}	& \vci{\FASTtomcatFTODCMem}{\FASTtomcatFTODCMemCI}		& \vci{\FASTtomcatREDCMem}{\FASTtomcatREDCMemCI} \\
\CAPO	& \vci{\SLOWtomcatCAPOExcMem}{\SLOWtomcatCAPOExcMemCI}	& \vci{\SLOWtomcatCAPOnoGExcMem}{\SLOWtomcatCAPOnoGExcMemCI}& \vci{\FASTtomcatFTOCAPOMem}{\FASTtomcatFTOCAPOMemCI}	& \vci{\FASTtomcatRECAPOMem}{\FASTtomcatRECAPOMemCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWxalanHBMem}{\SLOWxalanHBMemCI}		& \vci{\FASTxalanFTOHBMem}{\FASTxalanFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWxalanWCPMem}{\SLOWxalanWCPMemCI}		& \vci{\FASTxalanFTOWCPMem}{\FASTxalanFTOWCPMemCI}	& \vci{\FASTxalanREWCPMem}{\FASTxalanREWCPMemCI} \\
\DC		& \vci{\SLOWxalanDCExcMem}{\SLOWxalanDCExcMemCI}	& \vci{\SLOWxalanDCnoGExcMem}{\SLOWxalanDCnoGExcMemCI}	& \vci{\FASTxalanFTODCMem}{\FASTxalanFTODCMemCI}		& \vci{\FASTxalanREDCMem}{\FASTxalanREDCMemCI} \\
\CAPO	& \vci{\SLOWxalanCAPOExcMem}{\SLOWxalanCAPOExcMemCI}	& \vci{\SLOWxalanCAPOnoGExcMem}{\SLOWxalanCAPOnoGExcMemCI}& \vci{\FASTxalanFTOCAPOMem}{\FASTxalanFTOCAPOMemCI}	& \vci{\FASTxalanRECAPOMem}{\FASTxalanRECAPOMemCI} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\jake{Configuration: 10 trials, no stats collected.
Unopt-* results are the latest evaluation of removing setting cores to 8.
FTO-* and ST-* also remove setting cores to 8 and initialize extra metadata to null
and sets extra metadata to null if empty.}
\caption{Memory usage, relative to uninstrumented execution, of various analyses for each evaluated program
with 95\% confidence intervals.}
\label{tab:memory:allDaCapo:CI}
\end{table}

\begin{table}
% \begin{adjustwidth}{-1.5cm}{}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
% \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;Mb$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\sdr}[4]{\vci{#1}{#2}{\;}(\vci{#3}{#4})}
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}#1}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOpt2Quiet}
%
\smaller
\centering
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWavroraHB}{\SLOWavroraHBCI}{\SLOWavroraHBDynamic}{\SLOWavroraHBDynamicCI}					& \sdr{\FASTavroraFTOHB}{\FASTavroraFTOHBCI}{\FASTavroraFTOHBDynamic}{\FASTavroraFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWavroraWCP}{\SLOWavroraWCPCI}{\SLOWavroraWCPDynamic}{\SLOWavroraWCPDynamicCI}				& \sdr{\FASTavroraFTOWCP}{\FASTavroraFTOWCPCI}{\FASTavroraFTOWCPDynamic}{\FASTavroraFTOWCPDynamicCI}		& \sdr{\FASTavroraREWCP}{\FASTavroraREWCPCI}{\FASTavroraREWCPDynamic}{\FASTavroraREWCPDynamicCI} \\
\DC		& \sdr{\SLOWavroraDCExc}{\SLOWavroraDCExcCI}{\SLOWavroraDCExcDynamic}{\SLOWavroraDCExcDynamicCI}		& \sdr{\SLOWavroraDCnoGExc}{\SLOWavroraDCnoGExcCI}{\SLOWavroraDCnoGExcDynamic}{\SLOWavroraDCnoGExcDynamicCI}	& \sdr{\FASTavroraFTODC}{\FASTavroraFTODCCI}{\FASTavroraFTODCDynamic}{\FASTavroraFTODCDynamicCI}		& \sdr{\FASTavroraREDC}{\FASTavroraREDCCI}{\FASTavroraREDCDynamic}{\FASTavroraREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWavroraCAPOExc}{\SLOWavroraCAPOExcCI}{\SLOWavroraCAPOExcDynamic}{\SLOWavroraCAPOExcDynamicCI}	& \sdr{\SLOWavroraCAPOnoGExc}{\SLOWavroraCAPOnoGExcCI}{\SLOWavroraCAPOnoGExcDynamic}{\SLOWavroraCAPOnoGExcDynamicCI}	& \sdr{\FASTavroraFTOCAPO}{\FASTavroraFTOCAPOCI}{\FASTavroraFTOCAPODynamic}{\FASTavroraFTOCAPODynamicCI}	& \sdr{\FASTavroraRECAPO}{\FASTavroraRECAPOCI}{\FASTavroraRECAPODynamic}{\FASTavroraRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\medskip\\
% \begin{tabular}{@{}HHlll@{}}
%         & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
% \HB		& \rna													& \sdr{\SLOWbatikHB}{\SLOWbatikHBCI}{\SLOWbatikHBDynamic}{\SLOWbatikHBDynamicCI}					& \sdr{\FASTbatikFTOHB}{\FASTbatikFTOHBCI}{\FASTbatikFTOHBDynamic}{\FASTbatikFTOHBDynamicCI}		& \rna \\
% \WCP	& \rna													& \sdr{\SLOWbatikWCP}{\SLOWbatikWCPCI}{\SLOWbatikWCPDynamic}{\SLOWbatikWCPDynamicCI}				& \sdr{\FASTbatikFTOWCP}{\FASTbatikFTOWCPCI}{\FASTbatikFTOWCPDynamic}{\FASTbatikFTOWCPDynamicCI}		& \sdr{\FASTbatikREWCP}{\FASTbatikREWCPCI}{\FASTbatikREWCPDynamic}{\FASTbatikREWCPDynamicCI} \\
% \DC		& \sdr{\SLOWbatikDCExc}{\SLOWbatikDCExcCI}{\SLOWbatikDCExcDynamic}{\SLOWbatikDCExcDynamicCI}		& \sdr{\SLOWbatikDCnoGExc}{\SLOWbatikDCnoGExcCI}{\SLOWbatikDCnoGExcDynamic}{\SLOWbatikDCnoGExcDynamicCI}	& \sdr{\FASTbatikFTODC}{\FASTbatikFTODCCI}{\FASTbatikFTODCDynamic}{\FASTbatikFTODCDynamicCI}		& \sdr{\FASTbatikREDC}{\FASTbatikREDCCI}{\FASTbatikREDCDynamic}{\FASTbatikREDCDynamicCI} \\
% \CAPO	& \sdr{\SLOWbatikCAPOExc}{\SLOWbatikCAPOExcCI}{\SLOWbatikCAPOExcDynamic}{\SLOWbatikCAPOExcDynamicCI}	& \sdr{\SLOWbatikCAPOnoGExc}{\SLOWbatikCAPOnoGExcCI}{\SLOWbatikCAPOnoGExcDynamic}{\SLOWbatikCAPOnoGExcDynamicCI}	& \sdr{\FASTbatikFTOCAPO}{\FASTbatikFTOCAPOCI}{\FASTbatikFTOCAPODynamic}{\FASTbatikFTOCAPODynamicCI}	& \sdr{\FASTbatikRECAPO}{\FASTbatikRECAPOCI}{\FASTbatikRECAPODynamic}{\FASTbatikRECAPODynamicCI} \\
% 		& \mc{4}{c}{\bench{batik}} \\
% \end{tabular}
% \hfill
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWhtwoHB}{\SLOWhtwoHBCI}{\SLOWhtwoHBDynamic}{\SLOWhtwoHBDynamicCI}					& \sdr{\FASThtwoFTOHB}{\FASThtwoFTOHBCI}{\FASThtwoFTOHBDynamic}{\FASThtwoFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWhtwoWCP}{\SLOWhtwoWCPCI}{\SLOWhtwoWCPDynamic}{\SLOWhtwoWCPDynamicCI}				& \sdr{\FASThtwoFTOWCP}{\FASThtwoFTOWCPCI}{\FASThtwoFTOWCPDynamic}{\FASThtwoFTOWCPDynamicCI}		& \sdr{\FASThtwoREWCP}{\FASThtwoREWCPCI}{\FASThtwoREWCPDynamic}{\FASThtwoREWCPDynamicCI} \\
\DC		& \sdr{\SLOWhtwoDCExc}{\SLOWhtwoDCExcCI}{\SLOWhtwoDCExcDynamic}{\SLOWhtwoDCExcDynamicCI}		& \sdr{\SLOWhtwoDCnoGExc}{\SLOWhtwoDCnoGExcCI}{\SLOWhtwoDCnoGExcDynamic}{\SLOWhtwoDCnoGExcDynamicCI}	& \sdr{\FASThtwoFTODC}{\FASThtwoFTODCCI}{\FASThtwoFTODCDynamic}{\FASThtwoFTODCDynamicCI}		& \sdr{\FASThtwoREDC}{\FASThtwoREDCCI}{\FASThtwoREDCDynamic}{\FASThtwoREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWhtwoCAPOExc}{\SLOWhtwoCAPOExcCI}{\SLOWhtwoCAPOExcDynamic}{\SLOWhtwoCAPOExcDynamicCI}	& \sdr{\SLOWhtwoCAPOnoGExc}{\SLOWhtwoCAPOnoGExcCI}{\SLOWhtwoCAPOnoGExcDynamic}{\SLOWhtwoCAPOnoGExcDynamicCI}	& \sdr{\FASThtwoFTOCAPO}{\FASThtwoFTOCAPOCI}{\FASThtwoFTOCAPODynamic}{\FASThtwoFTOCAPODynamicCI}	& \sdr{\FASThtwoRECAPO}{\FASThtwoRECAPOCI}{\FASThtwoRECAPODynamic}{\FASThtwoRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWjythonHB}{\SLOWjythonHBCI}{\SLOWjythonHBDynamic}{\SLOWjythonHBDynamicCI}					& \sdr{\FASTjythonFTOHB}{\FASTjythonFTOHBCI}{\FASTjythonFTOHBDynamic}{\FASTjythonFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWjythonWCP}{\SLOWjythonWCPCI}{\SLOWjythonWCPDynamic}{\SLOWjythonWCPDynamicCI}				& \sdr{\FASTjythonFTOWCP}{\FASTjythonFTOWCPCI}{\FASTjythonFTOWCPDynamic}{\FASTjythonFTOWCPDynamicCI}		& \sdr{\FASTjythonREWCP}{\FASTjythonREWCPCI}{\FASTjythonREWCPDynamic}{\FASTjythonREWCPDynamicCI} \\
\DC		& \sdr{\SLOWjythonDCExc}{\SLOWjythonDCExcCI}{\SLOWjythonDCExcDynamic}{\SLOWjythonDCExcDynamicCI}		& \sdr{\SLOWjythonDCnoGExc}{\SLOWjythonDCnoGExcCI}{\SLOWjythonDCnoGExcDynamic}{\SLOWjythonDCnoGExcDynamicCI}	& \sdr{\FASTjythonFTODC}{\FASTjythonFTODCCI}{\FASTjythonFTODCDynamic}{\FASTjythonFTODCDynamicCI}		& \sdr{\FASTjythonREDC}{\FASTjythonREDCCI}{\FASTjythonREDCDynamic}{\FASTjythonREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWjythonCAPOExc}{\SLOWjythonCAPOExcCI}{\SLOWjythonCAPOExcDynamic}{\SLOWjythonCAPOExcDynamicCI}	& \sdr{\SLOWjythonCAPOnoGExc}{\SLOWjythonCAPOnoGExcCI}{\SLOWjythonCAPOnoGExcDynamic}{\SLOWjythonCAPOnoGExcDynamicCI}	& \sdr{\FASTjythonFTOCAPO}{\FASTjythonFTOCAPOCI}{\FASTjythonFTOCAPODynamic}{\FASTjythonFTOCAPODynamicCI}	& \sdr{\FASTjythonRECAPO}{\FASTjythonRECAPOCI}{\FASTjythonRECAPODynamic}{\FASTjythonRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWluindexHB}{\SLOWluindexHBCI}{\SLOWluindexHBDynamic}{\SLOWluindexHBDynamicCI}					& \sdr{\FASTluindexFTOHB}{\FASTluindexFTOHBCI}{\FASTluindexFTOHBDynamic}{\FASTluindexFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWluindexWCP}{\SLOWluindexWCPCI}{\SLOWluindexWCPDynamic}{\SLOWluindexWCPDynamicCI}				& \sdr{\FASTluindexFTOWCP}{\FASTluindexFTOWCPCI}{\FASTluindexFTOWCPDynamic}{\FASTluindexFTOWCPDynamicCI}		& \sdr{\FASTluindexREWCP}{\FASTluindexREWCPCI}{\FASTluindexREWCPDynamic}{\FASTluindexREWCPDynamicCI} \\
\DC		& \sdr{\SLOWluindexDCExc}{\SLOWluindexDCExcCI}{\SLOWluindexDCExcDynamic}{\SLOWluindexDCExcDynamicCI}		& \sdr{\SLOWluindexDCnoGExc}{\SLOWluindexDCnoGExcCI}{\SLOWluindexDCnoGExcDynamic}{\SLOWluindexDCnoGExcDynamicCI}	& \sdr{\FASTluindexFTODC}{\FASTluindexFTODCCI}{\FASTluindexFTODCDynamic}{\FASTluindexFTODCDynamicCI}		& \sdr{\FASTluindexREDC}{\FASTluindexREDCCI}{\FASTluindexREDCDynamic}{\FASTluindexREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWluindexCAPOExc}{\SLOWluindexCAPOExcCI}{\SLOWluindexCAPOExcDynamic}{\SLOWluindexCAPOExcDynamicCI}	& \sdr{\SLOWluindexCAPOnoGExc}{\SLOWluindexCAPOnoGExcCI}{\SLOWluindexCAPOnoGExcDynamic}{\SLOWluindexCAPOnoGExcDynamicCI}	& \sdr{\FASTluindexFTOCAPO}{\FASTluindexFTOCAPOCI}{\FASTluindexFTOCAPODynamic}{\FASTluindexFTOCAPODynamicCI}	& \sdr{\FASTluindexRECAPO}{\FASTluindexRECAPOCI}{\FASTluindexRECAPODynamic}{\FASTluindexRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
% \hfill
% \begin{tabular}{@{}HHlll@{}}
%         & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
% \HB		& \rna													& \sdr{\SLOWlusearchHB}{\SLOWlusearchHBCI}{\SLOWlusearchHBDynamic}{\SLOWlusearchHBDynamicCI}					& \sdr{\FASTlusearchFTOHB}{\FASTlusearchFTOHBCI}{\FASTlusearchFTOHBDynamic}{\FASTlusearchFTOHBDynamicCI}		& \rna \\
% \WCP	& \rna													& \sdr{\SLOWlusearchWCP}{\SLOWlusearchWCPCI}{\SLOWlusearchWCPDynamic}{\SLOWlusearchWCPDynamicCI}				& \sdr{\FASTlusearchFTOWCP}{\FASTlusearchFTOWCPCI}{\FASTlusearchFTOWCPDynamic}{\FASTlusearchFTOWCPDynamicCI}		& \sdr{\FASTlusearchREWCP}{\FASTlusearchREWCPCI}{\FASTlusearchREWCPDynamic}{\FASTlusearchREWCPDynamicCI} \\
% \DC		& \sdr{\SLOWlusearchDCExc}{\SLOWlusearchDCExcCI}{\SLOWlusearchDCExcDynamic}{\SLOWlusearchDCExcDynamicCI}		& \sdr{\SLOWlusearchDCnoGExc}{\SLOWlusearchDCnoGExcCI}{\SLOWlusearchDCnoGExcDynamic}{\SLOWlusearchDCnoGExcDynamicCI}	& \sdr{\FASTlusearchFTODC}{\FASTlusearchFTODCCI}{\FASTlusearchFTODCDynamic}{\FASTlusearchFTODCDynamicCI}		& \sdr{\FASTlusearchREDC}{\FASTlusearchREDCCI}{\FASTlusearchREDCDynamic}{\FASTlusearchREDCDynamicCI} \\
% \CAPO	& \sdr{\SLOWlusearchCAPOExc}{\SLOWlusearchCAPOExcCI}{\SLOWlusearchCAPOExcDynamic}{\SLOWlusearchCAPOExcDynamicCI}	& \sdr{\SLOWlusearchCAPOnoGExc}{\SLOWlusearchCAPOnoGExcCI}{\SLOWlusearchCAPOnoGExcDynamic}{\SLOWlusearchCAPOnoGExcDynamicCI}	& \sdr{\FASTlusearchFTOCAPO}{\FASTlusearchFTOCAPOCI}{\FASTlusearchFTOCAPODynamic}{\FASTlusearchFTOCAPODynamicCI}	& \sdr{\FASTlusearchRECAPO}{\FASTlusearchRECAPOCI}{\FASTlusearchRECAPODynamic}{\FASTlusearchRECAPODynamicCI} \\
% 		& \mc{4}{c}{\bench{lusearch}} \\
% \end{tabular}
% \hfill
\medskip\\
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWpmdHB}{\SLOWpmdHBCI}{\SLOWpmdHBDynamic}{\SLOWpmdHBDynamicCI}					& \sdr{\FASTpmdFTOHB}{\FASTpmdFTOHBCI}{\FASTpmdFTOHBDynamic}{\FASTpmdFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWpmdWCP}{\SLOWpmdWCPCI}{\SLOWpmdWCPDynamic}{\SLOWpmdWCPDynamicCI}				& \sdr{\FASTpmdFTOWCP}{\FASTpmdFTOWCPCI}{\FASTpmdFTOWCPDynamic}{\FASTpmdFTOWCPDynamicCI}		& \sdr{\FASTpmdREWCP}{\FASTpmdREWCPCI}{\FASTpmdREWCPDynamic}{\FASTpmdREWCPDynamicCI} \\
\DC		& \sdr{\SLOWpmdDCExc}{\SLOWpmdDCExcCI}{\SLOWpmdDCExcDynamic}{\SLOWpmdDCExcDynamicCI}		& \sdr{\SLOWpmdDCnoGExc}{\SLOWpmdDCnoGExcCI}{\SLOWpmdDCnoGExcDynamic}{\SLOWpmdDCnoGExcDynamicCI}	& \sdr{\FASTpmdFTODC}{\FASTpmdFTODCCI}{\FASTpmdFTODCDynamic}{\FASTpmdFTODCDynamicCI}		& \sdr{\FASTpmdREDC}{\FASTpmdREDCCI}{\FASTpmdREDCDynamic}{\FASTpmdREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWpmdCAPOExc}{\SLOWpmdCAPOExcCI}{\SLOWpmdCAPOExcDynamic}{\SLOWpmdCAPOExcDynamicCI}	& \sdr{\SLOWpmdCAPOnoGExc}{\SLOWpmdCAPOnoGExcCI}{\SLOWpmdCAPOnoGExcDynamic}{\SLOWpmdCAPOnoGExcDynamicCI}	& \sdr{\FASTpmdFTOCAPO}{\FASTpmdFTOCAPOCI}{\FASTpmdFTOCAPODynamic}{\FASTpmdFTOCAPODynamicCI}	& \sdr{\FASTpmdRECAPO}{\FASTpmdRECAPOCI}{\FASTpmdRECAPODynamic}{\FASTpmdRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWsunflowHB}{\SLOWsunflowHBCI}{\SLOWsunflowHBDynamic}{\SLOWsunflowHBDynamicCI}					& \sdr{\FASTsunflowFTOHB}{\FASTsunflowFTOHBCI}{\FASTsunflowFTOHBDynamic}{\FASTsunflowFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWsunflowWCP}{\SLOWsunflowWCPCI}{\SLOWsunflowWCPDynamic}{\SLOWsunflowWCPDynamicCI}				& \sdr{\FASTsunflowFTOWCP}{\FASTsunflowFTOWCPCI}{\FASTsunflowFTOWCPDynamic}{\FASTsunflowFTOWCPDynamicCI}		& \sdr{\FASTsunflowREWCP}{\FASTsunflowREWCPCI}{\FASTsunflowREWCPDynamic}{\FASTsunflowREWCPDynamicCI} \\
\DC		& \sdr{\SLOWsunflowDCExc}{\SLOWsunflowDCExcCI}{\SLOWsunflowDCExcDynamic}{\SLOWsunflowDCExcDynamicCI}		& \sdr{\SLOWsunflowDCnoGExc}{\SLOWsunflowDCnoGExcCI}{\SLOWsunflowDCnoGExcDynamic}{\SLOWsunflowDCnoGExcDynamicCI}	& \sdr{\FASTsunflowFTODC}{\FASTsunflowFTODCCI}{\FASTsunflowFTODCDynamic}{\FASTsunflowFTODCDynamicCI}		& \sdr{\FASTsunflowREDC}{\FASTsunflowREDCCI}{\FASTsunflowREDCDynamic}{\FASTsunflowREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWsunflowCAPOExc}{\SLOWsunflowCAPOExcCI}{\SLOWsunflowCAPOExcDynamic}{\SLOWsunflowCAPOExcDynamicCI}	& \sdr{\SLOWsunflowCAPOnoGExc}{\SLOWsunflowCAPOnoGExcCI}{\SLOWsunflowCAPOnoGExcDynamic}{\SLOWsunflowCAPOnoGExcDynamicCI}	& \sdr{\FASTsunflowFTOCAPO}{\FASTsunflowFTOCAPOCI}{\FASTsunflowFTOCAPODynamic}{\FASTsunflowFTOCAPODynamicCI}	& \sdr{\FASTsunflowRECAPO}{\FASTsunflowRECAPOCI}{\FASTsunflowRECAPODynamic}{\FASTsunflowRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWtomcatHB}{\SLOWtomcatHBCI}{\SLOWtomcatHBDynamic}{\SLOWtomcatHBDynamicCI}					& \sdr{\FASTtomcatFTOHB}{\FASTtomcatFTOHBCI}{\FASTtomcatFTOHBDynamic}{\FASTtomcatFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWtomcatWCP}{\SLOWtomcatWCPCI}{\SLOWtomcatWCPDynamic}{\SLOWtomcatWCPDynamicCI}				& \sdr{\FASTtomcatFTOWCP}{\FASTtomcatFTOWCPCI}{\FASTtomcatFTOWCPDynamic}{\FASTtomcatFTOWCPDynamicCI}		& \sdr{\FASTtomcatREWCP}{\FASTtomcatREWCPCI}{\FASTtomcatREWCPDynamic}{\FASTtomcatREWCPDynamicCI} \\
\DC		& \sdr{\SLOWtomcatDCExc}{\SLOWtomcatDCExcCI}{\SLOWtomcatDCExcDynamic}{\SLOWtomcatDCExcDynamicCI}		& \sdr{\SLOWtomcatDCnoGExc}{\SLOWtomcatDCnoGExcCI}{\SLOWtomcatDCnoGExcDynamic}{\SLOWtomcatDCnoGExcDynamicCI}	& \sdr{\FASTtomcatFTODC}{\FASTtomcatFTODCCI}{\FASTtomcatFTODCDynamic}{\FASTtomcatFTODCDynamicCI}		& \sdr{\FASTtomcatREDC}{\FASTtomcatREDCCI}{\FASTtomcatREDCDynamic}{\FASTtomcatREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWtomcatCAPOExc}{\SLOWtomcatCAPOExcCI}{\SLOWtomcatCAPOExcDynamic}{\SLOWtomcatCAPOExcDynamicCI}	& \sdr{\SLOWtomcatCAPOnoGExc}{\SLOWtomcatCAPOnoGExcCI}{\SLOWtomcatCAPOnoGExcDynamic}{\SLOWtomcatCAPOnoGExcDynamicCI}	& \sdr{\FASTtomcatFTOCAPO}{\FASTtomcatFTOCAPOCI}{\FASTtomcatFTOCAPODynamic}{\FASTtomcatFTOCAPODynamicCI}	& \sdr{\FASTtomcatRECAPO}{\FASTtomcatRECAPOCI}{\FASTtomcatRECAPODynamic}{\FASTtomcatRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hl@{\;\;}l@{\;\;}l@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWxalanHB}{\SLOWxalanHBCI}{\SLOWxalanHBDynamic}{\SLOWxalanHBDynamicCI}					& \sdr{\FASTxalanFTOHB}{\FASTxalanFTOHBCI}{\FASTxalanFTOHBDynamic}{\FASTxalanFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWxalanWCP}{\SLOWxalanWCPCI}{\SLOWxalanWCPDynamic}{\SLOWxalanWCPDynamicCI}				& \sdr{\FASTxalanFTOWCP}{\FASTxalanFTOWCPCI}{\FASTxalanFTOWCPDynamic}{\FASTxalanFTOWCPDynamicCI}		& \sdr{\FASTxalanREWCP}{\FASTxalanREWCPCI}{\FASTxalanREWCPDynamic}{\FASTxalanREWCPDynamicCI} \\
\DC		& \sdr{\SLOWxalanDCExc}{\SLOWxalanDCExcCI}{\SLOWxalanDCExcDynamic}{\SLOWxalanDCExcDynamicCI}		& \sdr{\SLOWxalanDCnoGExc}{\SLOWxalanDCnoGExcCI}{\SLOWxalanDCnoGExcDynamic}{\SLOWxalanDCnoGExcDynamicCI}	& \sdr{\FASTxalanFTODC}{\FASTxalanFTODCCI}{\FASTxalanFTODCDynamic}{\FASTxalanFTODCDynamicCI}		& \sdr{\FASTxalanREDC}{\FASTxalanREDCCI}{\FASTxalanREDCDynamic}{\FASTxalanREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWxalanCAPOExc}{\SLOWxalanCAPOExcCI}{\SLOWxalanCAPOExcDynamic}{\SLOWxalanCAPOExcDynamicCI}	& \sdr{\SLOWxalanCAPOnoGExc}{\SLOWxalanCAPOnoGExcCI}{\SLOWxalanCAPOnoGExcDynamic}{\SLOWxalanCAPOnoGExcDynamicCI}	& \sdr{\FASTxalanFTOCAPO}{\FASTxalanFTOCAPOCI}{\FASTxalanFTOCAPODynamic}{\FASTxalanFTOCAPODynamicCI}	& \sdr{\FASTxalanRECAPO}{\FASTxalanRECAPOCI}{\FASTxalanRECAPODynamic}{\FASTxalanRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\jake{Configuration: 10 trials, no stats collected.
Unopt-* results are the latest evaluation of removing setting cores to 8.
FTO-* and ST-* also remove setting cores to 8 and initialize extra metadata to null
and sets extra metadata to null if empty.}
\caption{Average races reported by various analyses for each evaluated program
(excluding \bench{batik} and \bench{lusearch}, for which all analyses report no races).
In each cell, the first value is statically distinct races
(\ie, distinct program locations), and the second value, in parentheses, is total dynamic races,
both with 95\% confidence intervals.}
\label{tab:race:allDaCapo:CI}
\end{table}

==> extra-data-counts-tables.tex <==
\begin{table*}[t]
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\newcommand{\tot}[1]{#1{\;}M}
\input{result-macros/PIP_fastTool_noRaceLimit}
%  
\small
\centering
\begin{tabular}{@{}l|rl|rr|rr|rr@{}}
& \mc{8}{c@{}}{\FastTool Extra Data Counts: CAPO-Opt Rule A or CAPO-Opt (A)}  \\
Program & Events & (NoFPEvents) & Rd (A) Succ & Rd (A) Total & WrWr(A) Succ & WrWr(A) Total & WrRd(A) Succ & WrRd(A) Total \\\hline
\bench{avrora} 	& \et{\avroraEvents} & (\et{\avroraNoFPEvents}) 	& \per{\avroraReadRuleASuc} 	& \tot{\avroraReadRuleATot} 	& \per{\avroraWriteWriteRuleASuc} 	& \tot{\avroraWriteWriteRuleATot} 	& \per{\avroraWriteReadRuleASuc} 	& \tot{\avroraWriteReadRuleATot} \\
\bench{batik} 	& \et{\batikEvents} & (\et{\batikNoFPEvents}) 		& \per{\batikReadRuleASuc} 		& \tot{\batikReadRuleATot} 		& \per{\batikWriteWriteRuleASuc} 	& \tot{\batikWriteWriteRuleATot} 	& \per{\batikWriteReadRuleASuc} 	& \tot{\batikWriteReadRuleATot} \\
\bench{h2} 		& \et{\htwoEvents} & (\et{\htwoNoFPEvents}) 		& \per{\htwoReadRuleASuc}		& \tot{\htwoReadRuleATot} 		& \per{\htwoWriteWriteRuleASuc} 	& \tot{\htwoWriteWriteRuleATot} 	& \per{\htwoWriteReadRuleASuc} 		& \tot{\htwoWriteReadRuleATot} \\
\bench{jython} 	& \et{\jythonEvents} & (\et{\jythonNoFPEvents}) 	& \per{\jythonReadRuleASuc} 	& \tot{\jythonReadRuleATot} 	& \per{\jythonWriteWriteRuleASuc} 	& \tot{\jythonWriteWriteRuleATot} 	& \per{\jythonWriteReadRuleASuc}	& \tot{\jythonWriteReadRuleATot} \\
\bench{luindex} & \et{\luindexEvents} & (\et{\luindexNoFPEvents}) 	& \per{\luindexReadRuleASuc} 	& \tot{\luindexReadRuleATot}	& \per{\luindexWriteWriteRuleASuc} 	& \tot{\luindexWriteWriteRuleATot} 	& \per{\luindexWriteReadRuleASuc} 	& \tot{\luindexWriteReadRuleATot} \\
\bench{lusearch}& \et{\lusearchEvents} & (\et{\lusearchNoFPEvents})	& \per{\lusearchReadRuleASuc}	& \tot{\lusearchReadRuleATot}	& \per{\lusearchWriteWriteRuleASuc} & \tot{\lusearchWriteWriteRuleATot} & \per{\lusearchWriteReadRuleASuc} 	& \tot{\lusearchWriteReadRuleATot} \\
\bench{pmd} 	& \et{\pmdEvents} & (\et{\pmdNoFPEvents}) 			& \per{\pmdReadRuleASuc} 		& \tot{\pmdReadRuleATot} 		& \per{\pmdWriteWriteRuleASuc} 		& \tot{\pmdWriteWriteRuleATot} 		& \per{\pmdWriteReadRuleASuc} 		& \tot{\pmdWriteReadRuleATot} \\
\bench{sunflow} & \et{\sunflowEvents} & (\et{\sunflowNoFPEvents}) 	& \per{\sunflowReadRuleASuc} 	& \tot{\sunflowReadRuleATot}	& \per{\sunflowWriteWriteRuleASuc} 	& \tot{\sunflowWriteWriteRuleATot} 	& \per{\sunflowWriteReadRuleASuc} 	& \tot{\sunflowWriteReadRuleATot} \\
\bench{tomcat} 	& \et{\tomcatEvents} & (\et{\tomcatNoFPEvents}) 	& \per{\tomcatReadRuleASuc} 	& \tot{\tomcatReadRuleATot} 	& \per{\tomcatWriteWriteRuleASuc} 	& \tot{\tomcatWriteWriteRuleATot} 	& \per{\tomcatWriteReadRuleASuc} 	& \tot{\tomcatWriteReadRuleATot} \\
\bench{xalan} 	& \et{\xalanEvents} & (\et{\xalanNoFPEvents}) 		& \per{\xalanReadRuleASuc} 		& \tot{\xalanReadRuleATot}		& \per{\xalanWriteWriteRuleASuc} 	& \tot{\xalanWriteWriteRuleATot} 	& \per{\xalanWriteReadRuleASuc} 	& \tot{\xalanWriteReadRuleATot} \\\hline
\end{tabular}
%  
\caption{CAPO-Opt Rule A counts.}
\label{tab:extra-data-counts:ruleA}
\end{table*}

\begin{table*}[t]
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\newcommand{\tot}[1]{#1{\;}M}
\input{result-macros/PIP_fastTool_noRaceLimit}
%  
\small
\centering
\begin{tabular}{@{}l|rl|r|rrr|rrr@{}}
& \mc{9}{c@{}}{\FastTool Extra Data Counts: CAPO Rd/Wr Sets}  \\
Program & Events & (NoFPEvents) & Total Clears & Rd Set 0 & Rd Set 1 & Rd Set Gt1 & Wr Set 0 & Wr Set 1 & Wr Set Gt1 \\\hline
\bench{avrora} 	& \et{\avroraEvents} & (\et{\avroraNoFPEvents}) 	& \tot{\avroraTotalSetClears} 	& \per{\avroraReadSetZero} 	& \per{\avroraReadSetOne} 	& \per{\avroraReadSetGtOne} 	& \per{\avroraWriteSetZero} 	& \per{\avroraWriteSetOne} 	& \per{\avroraWriteSetGtOne} \\
\bench{batik} 	& \et{\batikEvents} & (\et{\batikNoFPEvents}) 		& \tot{\batikTotalSetClears} 	& \per{\batikReadSetZero} 	& \per{\batikReadSetOne} 	& \per{\batikReadSetGtOne} 		& \per{\batikWriteSetZero} 		& \per{\batikWriteSetOne} 	& \per{\batikWriteSetGtOne} \\
\bench{h2} 		& \et{\htwoEvents} & (\et{\htwoNoFPEvents}) 		& \tot{\htwoTotalSetClears}		& \per{\htwoReadSetZero} 	& \per{\htwoReadSetOne} 	& \per{\htwoReadSetGtOne} 		& \per{\htwoWriteSetZero} 		& \per{\htwoWriteSetOne} 	& \per{\htwoWriteSetGtOne} \\
\bench{jython} 	& \et{\jythonEvents} & (\et{\jythonNoFPEvents}) 	& \tot{\jythonTotalSetClears} 	& \per{\jythonReadSetZero} 	& \per{\jythonReadSetOne} 	& \per{\jythonReadSetGtOne} 	& \per{\jythonWriteSetZero} 	& \per{\jythonWriteSetOne} 	& \per{\jythonWriteSetGtOne} \\
\bench{luindex} & \et{\luindexEvents} & (\et{\luindexNoFPEvents}) 	& \tot{\luindexTotalSetClears} 	& \per{\luindexReadSetZero}	& \per{\luindexReadSetOne} 	& \per{\luindexReadSetGtOne} 	& \per{\luindexWriteSetZero} 	& \per{\luindexWriteSetOne} & \per{\luindexWriteSetGtOne} \\
\bench{lusearch}& \et{\lusearchEvents} & (\et{\lusearchNoFPEvents})	& \tot{\lusearchTotalSetClears}	& \per{\lusearchReadSetZero}& \per{\lusearchReadSetOne} & \per{\lusearchReadSetGtOne} 	& \per{\lusearchWriteSetZero} 	& \per{\lusearchWriteSetOne}& \per{\lusearchWriteSetGtOne} \\
\bench{pmd} 	& \et{\pmdEvents} & (\et{\pmdNoFPEvents}) 			& \tot{\pmdTotalSetClears} 		& \per{\pmdReadSetZero} 	& \per{\pmdReadSetOne} 		& \per{\pmdReadSetGtOne} 		& \per{\pmdWriteSetZero} 		& \per{\pmdWriteSetOne} 	& \per{\pmdWriteSetGtOne} \\
\bench{sunflow} & \et{\sunflowEvents} & (\et{\sunflowNoFPEvents}) 	& \tot{\sunflowTotalSetClears} 	& \per{\sunflowReadSetZero}	& \per{\sunflowReadSetOne} 	& \per{\sunflowReadSetGtOne} 	& \per{\sunflowWriteSetZero} 	& \per{\sunflowWriteSetOne} & \per{\sunflowWriteSetGtOne} \\
\bench{tomcat} 	& \et{\tomcatEvents} & (\et{\tomcatNoFPEvents}) 	& \tot{\tomcatTotalSetClears} 	& \per{\tomcatReadSetZero} 	& \per{\tomcatReadSetOne} 	& \per{\tomcatReadSetGtOne} 	& \per{\tomcatWriteSetZero} 	& \per{\tomcatWriteSetOne} 	& \per{\tomcatWriteSetGtOne} \\
\bench{xalan} 	& \et{\xalanEvents} & (\et{\xalanNoFPEvents}) 		& \tot{\xalanTotalSetClears} 	& \per{\xalanReadSetZero}	& \per{\xalanReadSetOne} 	& \per{\xalanReadSetGtOne} 		& \per{\xalanWriteSetZero} 		& \per{\xalanWriteSetOne} 	& \per{\xalanWriteSetGtOne} \\\hline
\end{tabular}
%  
\caption{CAPO set counts.}
\label{tab:extra-data-counts:CAPOSets}
\end{table*}

\begin{table*}[t]
\begin{adjustwidth}{-1cm}{}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\newcommand{\tot}[1]{#1{\;}M}
\input{result-macros/PIP_fastTool_noRaceLimit}
%  
\small
\centering
\begin{tabular}{@{}l|rl|r|rrrrrr@{}}
& \mc{9}{c@{}}{\FastTool Extra Data Counts: CAPO Rd Maps}  \\
Program & Events & (NoFPEvents) & Total Clears & Rd Map 0 & Rd Map 1 & Rd Map 10 & Rd Map 100 & Rd Map 1000 & Rd Map Gt1000 \\\hline
\bench{avrora} 	& \et{\avroraEvents} & (\et{\avroraNoFPEvents}) 	& \tot{\avroraTotalMapClears} 	& \per{\avroraReadMapZero} 	& \per{\avroraReadMapOne} 	& \per{\avroraReadMapTen} 	& \per{\avroraReadMapHund} 	& \per{\avroraReadMapThou} 	& \per{\avroraReadMapGtThou} \\
\bench{batik} 	& \et{\batikEvents} & (\et{\batikNoFPEvents}) 		& \tot{\batikTotalMapClears} 	& \per{\batikReadMapZero} 	& \per{\batikReadMapOne} 	& \per{\batikReadMapTen} 	& \per{\batikReadMapHund} 	& \per{\batikReadMapThou} 	& \per{\batikReadMapGtThou} \\
\bench{h2} 		& \et{\htwoEvents} & (\et{\htwoNoFPEvents}) 		& \tot{\htwoTotalMapClears}		& \per{\htwoReadMapZero} 	& \per{\htwoReadMapOne} 	& \per{\htwoReadMapTen} 	& \per{\htwoReadMapHund} 	& \per{\htwoReadMapThou} 	& \per{\htwoReadMapGtThou} \\
\bench{jython} 	& \et{\jythonEvents} & (\et{\jythonNoFPEvents}) 	& \tot{\jythonTotalMapClears} 	& \per{\jythonReadMapZero} 	& \per{\jythonReadMapOne} 	& \per{\jythonReadMapTen} 	& \per{\jythonReadMapHund} 	& \per{\jythonReadMapThou} 	& \per{\jythonReadMapGtThou} \\
\bench{luindex} & \et{\luindexEvents} & (\et{\luindexNoFPEvents}) 	& \tot{\luindexTotalMapClears} 	& \per{\luindexReadMapZero}	& \per{\luindexReadMapOne} 	& \per{\luindexReadMapTen} 	& \per{\luindexReadMapHund} & \per{\luindexReadMapThou} & \per{\luindexReadMapGtThou} \\
\bench{lusearch}& \et{\lusearchEvents} & (\et{\lusearchNoFPEvents})	& \tot{\lusearchTotalMapClears}	& \per{\lusearchReadMapZero}& \per{\lusearchReadMapOne} & \per{\lusearchReadMapTen} & \per{\lusearchReadMapHund}& \per{\lusearchReadMapThou}& \per{\lusearchReadMapGtThou} \\
\bench{pmd} 	& \et{\pmdEvents} & (\et{\pmdNoFPEvents}) 			& \tot{\pmdTotalMapClears} 		& \per{\pmdReadMapZero} 	& \per{\pmdReadMapOne} 		& \per{\pmdReadMapTen} 		& \per{\pmdReadMapHund} 	& \per{\pmdReadMapThou} 	& \per{\pmdReadMapGtThou} \\
\bench{sunflow} & \et{\sunflowEvents} & (\et{\sunflowNoFPEvents}) 	& \tot{\sunflowTotalMapClears} 	& \per{\sunflowReadMapZero}	& \per{\sunflowReadMapOne} 	& \per{\sunflowReadMapTen} 	& \per{\sunflowReadMapHund} & \per{\sunflowReadMapThou} & \per{\sunflowReadMapGtThou} \\
\bench{tomcat} 	& \et{\tomcatEvents} & (\et{\tomcatNoFPEvents}) 	& \tot{\tomcatTotalMapClears} 	& \per{\tomcatReadMapZero} 	& \per{\tomcatReadMapOne} 	& \per{\tomcatReadMapTen} 	& \per{\tomcatReadMapHund} 	& \per{\tomcatReadMapThou} 	& \per{\tomcatReadMapGtThou} \\
\bench{xalan} 	& \et{\xalanEvents} & (\et{\xalanNoFPEvents}) 		& \tot{\xalanTotalMapClears} 	& \per{\xalanReadMapZero}	& \per{\xalanReadMapOne} 	& \per{\xalanReadMapTen} 	& \per{\xalanReadMapHund} 	& \per{\xalanReadMapThou} 	& \per{\xalanReadMapGtThou} \\\hline
\end{tabular}
%  
\caption{CAPO Rd map counts.}
\label{tab:extra-data-counts:CAPORdMaps}
\end{adjustwidth}
\end{table*}

\begin{table*}[t]
\begin{adjustwidth}{-1cm}{}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\newcommand{\tot}[1]{#1{\;}M}
\input{result-macros/PIP_fastTool_noRaceLimit}
%  
\small
\centering
\begin{tabular}{@{}l|rl|r|rrrrrr@{}}
& \mc{9}{c@{}}{\FastTool Extra Data Counts: CAPO Wr Maps}  \\
Program & Events & (NoFPEvents) & Total Clears & Wr Map 0 & Wr Map 1 & Wr Map 10 & Wr Map 100 & Wr Map 1000 & Wr Map Gt1000 \\\hline
\bench{avrora} 	& \et{\avroraEvents} & (\et{\avroraNoFPEvents}) 	& \tot{\avroraTotalMapClears} 	& \per{\avroraWriteMapZero} 	& \per{\avroraWriteMapOne} 	& \per{\avroraWriteMapTen} 	& \per{\avroraWriteMapHund} 	& \per{\avroraWriteMapThou} 	& \per{\avroraWriteMapGtThou} \\
\bench{batik} 	& \et{\batikEvents} & (\et{\batikNoFPEvents}) 		& \tot{\batikTotalMapClears} 	& \per{\batikWriteMapZero} 	& \per{\batikWriteMapOne} 	& \per{\batikWriteMapTen} 	& \per{\batikWriteMapHund} 	& \per{\batikWriteMapThou} 	& \per{\batikWriteMapGtThou} \\
\bench{h2} 		& \et{\htwoEvents} & (\et{\htwoNoFPEvents}) 		& \tot{\htwoTotalMapClears}		& \per{\htwoWriteMapZero} 	& \per{\htwoWriteMapOne} 	& \per{\htwoWriteMapTen} 	& \per{\htwoWriteMapHund} 	& \per{\htwoWriteMapThou} 	& \per{\htwoWriteMapGtThou} \\
\bench{jython} 	& \et{\jythonEvents} & (\et{\jythonNoFPEvents}) 	& \tot{\jythonTotalMapClears} 	& \per{\jythonWriteMapZero} 	& \per{\jythonWriteMapOne} 	& \per{\jythonWriteMapTen} 	& \per{\jythonWriteMapHund} 	& \per{\jythonWriteMapThou} 	& \per{\jythonWriteMapGtThou} \\
\bench{luindex} & \et{\luindexEvents} & (\et{\luindexNoFPEvents}) 	& \tot{\luindexTotalMapClears} 	& \per{\luindexWriteMapZero}	& \per{\luindexWriteMapOne} 	& \per{\luindexWriteMapTen} 	& \per{\luindexWriteMapHund} & \per{\luindexWriteMapThou} & \per{\luindexWriteMapGtThou} \\
\bench{lusearch}& \et{\lusearchEvents} & (\et{\lusearchNoFPEvents})	& \tot{\lusearchTotalMapClears}	& \per{\lusearchWriteMapZero}& \per{\lusearchWriteMapOne} & \per{\lusearchWriteMapTen} & \per{\lusearchWriteMapHund}& \per{\lusearchWriteMapThou}& \per{\lusearchWriteMapGtThou} \\
\bench{pmd} 	& \et{\pmdEvents} & (\et{\pmdNoFPEvents}) 			& \tot{\pmdTotalMapClears} 		& \per{\pmdWriteMapZero} 	& \per{\pmdWriteMapOne} 		& \per{\pmdWriteMapTen} 		& \per{\pmdWriteMapHund} 	& \per{\pmdWriteMapThou} 	& \per{\pmdWriteMapGtThou} \\
\bench{sunflow} & \et{\sunflowEvents} & (\et{\sunflowNoFPEvents}) 	& \tot{\sunflowTotalMapClears} 	& \per{\sunflowWriteMapZero}	& \per{\sunflowWriteMapOne} 	& \per{\sunflowWriteMapTen} 	& \per{\sunflowWriteMapHund} & \per{\sunflowWriteMapThou} & \per{\sunflowWriteMapGtThou} \\
\bench{tomcat} 	& \et{\tomcatEvents} & (\et{\tomcatNoFPEvents}) 	& \tot{\tomcatTotalMapClears} 	& \per{\tomcatWriteMapZero} 	& \per{\tomcatWriteMapOne} 	& \per{\tomcatWriteMapTen} 	& \per{\tomcatWriteMapHund} 	& \per{\tomcatWriteMapThou} 	& \per{\tomcatWriteMapGtThou} \\
\bench{xalan} 	& \et{\xalanEvents} & (\et{\xalanNoFPEvents}) 		& \tot{\xalanTotalMapClears} 	& \per{\xalanWriteMapZero}	& \per{\xalanWriteMapOne} 	& \per{\xalanWriteMapTen} 	& \per{\xalanWriteMapHund} 	& \per{\xalanWriteMapThou} 	& \per{\xalanWriteMapGtThou} \\\hline
\end{tabular}
%  
\caption{CAPO Wr map counts.}
\label{tab:extra-data-counts:CAPOWrMaps}
\end{adjustwidth}
\end{table*}

\begin{table*}[t]
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\newcommand{\tot}[1]{#1{\;}M}
\input{result-macros/PIP_fastTool_raceEdgeAdd_lockCount}
%  
\small
\centering
\begin{tabular}{@{}l|rl|r|rrr@{}}
& \mc{6}{c@{}}{\FastTool Extra Data Counts 2: Locks Held During Access Event}  \\
Program & Events & (NoFPEvents) & Held Lock Total & One Lock Held & Two Nested Locks & Many Nested Locks \\\hline
\bench{avrora} 	& \et{\avroraEvents} & (\et{\avroraNoFPEvents}) 	& \tot{\avroraHoldLocksTotal} 	& \per{\avroraOneLockHeld} 	& \per{\avroraTwoNestedLocks} 	& \per{\avroraManyNestedLocks} \\
\bench{batik} 	& \et{\batikEvents} & (\et{\batikNoFPEvents}) 		& \tot{\batikHoldLocksTotal} 	& \per{\batikOneLockHeld} 	& \per{\batikTwoNestedLocks} 	& \per{\batikManyNestedLocks} \\
\bench{h2} 		& \et{\htwoEvents} & (\et{\htwoNoFPEvents}) 		& \tot{\htwoHoldLocksTotal}		& \per{\htwoOneLockHeld} 	& \per{\htwoTwoNestedLocks} 	& \per{\htwoManyNestedLocks} \\
\bench{jython} 	& \et{\jythonEvents} & (\et{\jythonNoFPEvents}) 	& \tot{\jythonHoldLocksTotal} 	& \per{\jythonOneLockHeld} 	& \per{\jythonTwoNestedLocks} 	& \per{\jythonManyNestedLocks} \\
\bench{luindex} & \et{\luindexEvents} & (\et{\luindexNoFPEvents}) 	& \tot{\luindexHoldLocksTotal} 	& \per{\luindexOneLockHeld}	& \per{\luindexTwoNestedLocks} 	& \per{\luindexManyNestedLocks} \\
\bench{lusearch}& \et{\lusearchEvents} & (\et{\lusearchNoFPEvents})	& \tot{\lusearchHoldLocksTotal}	& \per{\lusearchOneLockHeld}& \per{\lusearchTwoNestedLocks} & \per{\lusearchManyNestedLocks} \\
\bench{pmd} 	& \et{\pmdEvents} & (\et{\pmdNoFPEvents}) 			& \tot{\pmdHoldLocksTotal} 		& \per{\pmdOneLockHeld} 	& \per{\pmdTwoNestedLocks} 		& \per{\pmdManyNestedLocks} \\
\bench{sunflow} & \et{\sunflowEvents} & (\et{\sunflowNoFPEvents}) 	& \tot{\sunflowHoldLocksTotal} 	& \per{\sunflowOneLockHeld}	& \per{\sunflowTwoNestedLocks} 	& \per{\sunflowManyNestedLocks} \\
\bench{tomcat} 	& \et{\tomcatEvents} & (\et{\tomcatNoFPEvents}) 	& \tot{\tomcatHoldLocksTotal} 	& \per{\tomcatOneLockHeld} 	& \per{\tomcatTwoNestedLocks} 	& \per{\tomcatManyNestedLocks} \\
\bench{xalan} 	& \et{\xalanEvents} & (\et{\xalanNoFPEvents}) 		& \tot{\xalanHoldLocksTotal} 	& \per{\xalanOneLockHeld}	& \per{\xalanTwoNestedLocks} 	& \per{\xalanManyNestedLocks} \\\hline
\end{tabular}
%  
\caption{Locks Held During Access Events.}
\label{tab:extra-data-counts-2:locksHeld}
\end{table*}

==> fast-tool-event-counts.tex <==
\begin{table*}[t]
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\input{result-macros/PIP_fastTool_noRaceLimit}
%  
\small
\centering
\begin{tabular}{@{}l|rl|rr|rr|rr@{}}
& \mc{8}{c@{}}{\FastTool Extra: Access Event Counts}  \\
Program & Events & (NoFPEvents) & Read Total & Write Total & Access In CS & Access Out CS & Acq/Rel Total & Other Total \\\hline
\bench{avrora} 	& \et{\avroraEvents} & (\et{\avroraNoFPEvents}) 		& \per{\avroraReadTotal} 		& \per{\avroraWriteTotal} 	& \per{\avroraNoFPAccessInCS} 		& \per{\avroraNoFPAccessOutCS} 	& \per{\avroraAcqRelTotal} & \per{\avroraOtherTotal} \\
\bench{batik} 	& \et{\batikEvents} & (\et{\batikNoFPEvents}) 		& \per{\batikReadTotal} 		& \per{\batikWriteTotal} 		& \per{\batikNoFPAccessInCS} 		& \per{\batikNoFPAccessOutCS} 	& \per{\batikAcqRelTotal} & \per{\batikOtherTotal} \\
\bench{h2} 		& \et{\htwoEvents} & (\et{\htwoNoFPEvents}) 			& \per{\htwoReadTotal}		& \per{\htwoWriteTotal} 		& \per{\htwoNoFPAccessInCS} 		& \per{\htwoNoFPAccessOutCS} 	& \per{\htwoAcqRelTotal} & \per{\htwoOtherTotal} \\
\bench{jython} 	& \et{\jythonEvents} & (\et{\jythonNoFPEvents}) 		& \per{\jythonReadTotal} 		& \per{\jythonWriteTotal} 	& \per{\jythonNoFPAccessInCS} 		& \per{\jythonNoFPAccessOutCS} 	& \per{\jythonAcqRelTotal} & \per{\jythonOtherTotal} \\
\bench{luindex} & \et{\luindexEvents} & (\et{\luindexNoFPEvents}) 	& \per{\luindexReadTotal} 	& \per{\luindexWriteTotal}	& \per{\luindexNoFPAccessInCS} 		& \per{\luindexNoFPAccessOutCS} 	& \per{\luindexAcqRelTotal} & \per{\luindexOtherTotal} \\
\bench{lusearch}& \et{\lusearchEvents} & (\et{\lusearchNoFPEvents})	& \per{\lusearchReadTotal}	& \per{\lusearchWriteTotal}	& \per{\lusearchNoFPAccessInCS} 		& \per{\lusearchNoFPAccessOutCS} 	& \per{\lusearchAcqRelTotal} & \per{\lusearchOtherTotal} \\
\bench{pmd} 	& \et{\pmdEvents} & (\et{\pmdNoFPEvents}) 			& \per{\pmdReadTotal} 		& \per{\pmdWriteTotal} 		& \per{\pmdNoFPAccessInCS} 		& \per{\pmdNoFPAccessOutCS} 	& \per{\pmdAcqRelTotal} & \per{\pmdOtherTotal} \\
\bench{sunflow} & \et{\sunflowEvents} & (\et{\sunflowNoFPEvents}) 	& \per{\sunflowReadTotal} 	& \per{\sunflowWriteTotal}	& \per{\sunflowNoFPAccessInCS} 		& \per{\sunflowNoFPAccessOutCS} 	& \per{\sunflowAcqRelTotal} & \per{\sunflowOtherTotal} \\
\bench{tomcat} 	& \et{\tomcatEvents} & (\et{\tomcatNoFPEvents}) 		& \per{\tomcatReadTotal} 		& \per{\tomcatWriteTotal} 	& \per{\tomcatNoFPAccessInCS} 		& \per{\tomcatNoFPAccessOutCS} 	& \per{\tomcatAcqRelTotal} & \per{\tomcatOtherTotal} \\
\bench{xalan} 	& \et{\xalanEvents} & (\et{\xalanNoFPEvents}) 		& \per{\xalanReadTotal} 		& \per{\xalanWriteTotal}		& \per{\xalanNoFPAccessInCS} 		& \per{\xalanNoFPAccessOutCS} 	& \per{\xalanAcqRelTotal} & \per{\xalanOtherTotal} \\\hline
\end{tabular}
%  
\caption{Access event counts.}
\label{tab:fast-tool-event-counts:access}
\end{table*}

\begin{table*}[t]
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\input{result-macros/PIP_fastTool_noRaceLimit}
%  
\small
\centering
\begin{tabular}{@{}l|r|rr|rrrrr@{}}
& \mc{8}{c@{}}{\FastTool Extra: Read Event Counts}  \\
Program & Read Total & In CS & Out CS & Same Ep & Shared-Same Ep & Exclusive & Share & Shared \\\hline
\bench{avrora} 	& \et{\avroraNoFPReadTotal} & \per{\avroraReadInCS} 		& \per{\avroraReadOutCS} 		& \per{\avroraReadSameEp} 	& \per{\avroraReadSharedSameEp} & \per{\avroraReadExclusive} & \per{\avroraReadShare} & \per{\avroraReadShared} \\
\bench{batik} 	& \et{\batikNoFPReadTotal} & \per{\batikReadInCS} 		& \per{\batikReadOutCS} 		& \per{\batikReadSameEp} 		& \per{\batikReadSharedSameEp} & \per{\batikReadExclusive} & \per{\batikReadShare} & \per{\batikReadShared} \\
\bench{h2} 		& \et{\htwoNoFPReadTotal} & \per{\htwoReadInCS} 			& \per{\htwoReadOutCS}		& \per{\htwoReadSameEp} 		& \per{\htwoReadSharedSameEp} & \per{\htwoReadExclusive} & \per{\htwoReadShare} & \per{\htwoReadShared} \\
\bench{jython} 	& \et{\jythonNoFPReadTotal} & \per{\jythonReadInCS} 		& \per{\jythonReadOutCS} 		& \per{\jythonReadSameEp} 	& \per{\jythonReadSharedSameEp} & \per{\jythonReadExclusive} & \per{\jythonReadShare} & \per{\jythonReadShared} \\
\bench{luindex} & \et{\luindexNoFPReadTotal} & \per{\luindexReadInCS} 	& \per{\luindexReadOutCS} 	& \per{\luindexReadSameEp}	& \per{\luindexReadSharedSameEp} & \per{\luindexReadExclusive} & \per{\luindexReadShare} & \per{\luindexReadShared} \\
\bench{lusearch}& \et{\lusearchNoFPReadTotal} & \per{\lusearchReadInCS}	& \per{\lusearchReadOutCS}	& \per{\lusearchReadSameEp}	& \per{\lusearchReadSharedSameEp} & \per{\lusearchReadExclusive} & \per{\lusearchReadShare} & \per{\lusearchReadShared} \\
\bench{pmd} 	& \et{\pmdNoFPReadTotal} & \per{\pmdReadInCS} 			& \per{\pmdReadOutCS} 		& \per{\pmdReadSameEp} 		& \per{\pmdReadSharedSameEp} & \per{\pmdReadExclusive} & \per{\pmdReadShare} & \per{\pmdReadShared} \\
\bench{sunflow} & \et{\sunflowNoFPReadTotal} & \per{\sunflowReadInCS} 	& \per{\sunflowReadOutCS} 	& \per{\sunflowReadSameEp}	& \per{\sunflowReadSharedSameEp} & \per{\sunflowReadExclusive} & \per{\sunflowReadShare} & \per{\sunflowReadShared} \\
\bench{tomcat} 	& \et{\tomcatNoFPReadTotal} & \per{\tomcatReadInCS} 		& \per{\tomcatReadOutCS} 		& \per{\tomcatReadSameEp} 	& \per{\tomcatReadSharedSameEp} & \per{\tomcatReadExclusive} & \per{\tomcatReadShare} & \per{\tomcatReadShared} \\
\bench{xalan} 	& \et{\xalanNoFPReadTotal} & \per{\xalanReadInCS} 		& \per{\xalanReadOutCS} 		& \per{\xalanReadSameEp}		& \per{\xalanReadSharedSameEp} & \per{\xalanReadExclusive} & \per{\xalanReadShare} & \per{\xalanReadShared} \\\hline
\end{tabular}
%  
\caption{Read event counts.}
\label{tab:fast-tool-event-counts:read}
\end{table*}

\begin{table*}[t]
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\input{result-macros/PIP_fastTool_noRaceLimit}
%  
\small
\centering
\begin{tabular}{@{}l|r|rr|r|rrr@{}}
& \mc{7}{c@{}}{\FastTool Extra: Write Event Counts}  \\
Program & Honest Writes & In CS & Out CS & Write Total & Same Ep & Exclusive & Shared \\\hline
\bench{avrora} 	& \et{\avroraNoFPHonestWriteTotal} & \per{\avroraWriteInCS} 		& \per{\avroraWriteOutCS} 		& \et{\avroraNoFPWriteTotal} & \per{\avroraWriteSameEp} 	& \per{\avroraWriteExclusive} & \per{\avroraWriteShared} \\
\bench{batik} 	& \et{\batikNoFPHonestWriteTotal} & \per{\batikWriteInCS} 		& \per{\batikWriteOutCS} 		& \et{\batikNoFPWriteTotal} & \per{\batikWriteSameEp} 		& \per{\batikWriteExclusive} & \per{\batikWriteShared} \\
\bench{h2} 		& \et{\htwoNoFPHonestWriteTotal} & \per{\htwoWriteInCS} 			& \per{\htwoWriteOutCS}		& \et{\htwoNoFPWriteTotal} & \per{\htwoWriteSameEp} 		& \per{\htwoWriteExclusive} & \per{\htwoWriteShared} \\
\bench{jython} 	& \et{\jythonNoFPHonestWriteTotal} & \per{\jythonWriteInCS} 		& \per{\jythonWriteOutCS} 		& \et{\jythonNoFPWriteTotal} & \per{\jythonWriteSameEp} 	& \per{\jythonWriteExclusive} & \per{\jythonWriteShared} \\
\bench{luindex} & \et{\luindexNoFPHonestWriteTotal} & \per{\luindexWriteInCS} 	& \per{\luindexWriteOutCS} 	& \et{\luindexNoFPWriteTotal} & \per{\luindexWriteSameEp}	& \per{\luindexWriteExclusive} & \per{\luindexWriteShared} \\
\bench{lusearch}& \et{\lusearchNoFPHonestWriteTotal} & \per{\lusearchWriteInCS}	& \per{\lusearchWriteOutCS}	& \et{\lusearchNoFPWriteTotal} & \per{\lusearchWriteSameEp}	& \per{\lusearchWriteExclusive} & \per{\lusearchWriteShared} \\
\bench{pmd} 	& \et{\pmdNoFPHonestWriteTotal} & \per{\pmdWriteInCS} 			& \per{\pmdWriteOutCS} 		& \et{\pmdNoFPWriteTotal} & \per{\pmdWriteSameEp} 		& \per{\pmdWriteExclusive} & \per{\pmdWriteShared} \\
\bench{sunflow} & \et{\sunflowNoFPHonestWriteTotal} & \per{\sunflowWriteInCS} 	& \per{\sunflowWriteOutCS} 	& \et{\sunflowNoFPWriteTotal} & \per{\sunflowWriteSameEp}	& \per{\sunflowWriteExclusive} & \per{\sunflowWriteShared} \\
\bench{tomcat} 	& \et{\tomcatNoFPHonestWriteTotal} & \per{\tomcatWriteInCS} 		& \per{\tomcatWriteOutCS} 		& \et{\tomcatNoFPWriteTotal} & \per{\tomcatWriteSameEp} 	& \per{\tomcatWriteExclusive} & \per{\tomcatWriteShared} \\
\bench{xalan} 	& \et{\xalanNoFPHonestWriteTotal} & \per{\xalanWriteInCS} 		& \per{\xalanWriteOutCS} 		& \et{\xalanNoFPWriteTotal} & \per{\xalanWriteSameEp}		& \per{\xalanWriteExclusive} & \per{\xalanWriteShared} \\\hline
\end{tabular}
%  
\caption{Write event counts.}
\label{tab:fast-tool-event-counts:write}
\end{table*}

\begin{table*}[t]
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\newcommand{\per}[1]{#1\%}
\input{result-macros/PIP_fastTool_noRaceLimit}
%  
\small
\centering
\begin{tabular}{@{}l|r|r|r|rrrrrrr@{}}
& \mc{10}{c@{}}{\FastTool Extra: Other Event Counts}  \\
Program & Other Total & Acq/Rel & No Acq/Rel Total & Fork & Join & PreWait & PostWait & Volatile & ClassInit & ClassAccess \\\hline
\bench{avrora} 	& \avroraNoFPOtherTotal & \per{\avroraAcqRelOtherTotal} 		& \avroraNoAcqRelOtherTotal 		& \per{\avroraFork} 	& \per{\avroraJoin} & \per{\avroraPreWait} & \per{\avroraPostWait} & \per{\avroraVolatileTotal} & \per{\avroraClassInit} & \per{\avroraClassAccess} \\
\bench{batik} 	& \batikNoFPOtherTotal & \per{\batikAcqRelOtherTotal} 		& \batikNoAcqRelOtherTotal 		& \per{\batikFork} 		& \per{\batikJoin} & \per{\batikPreWait} & \per{\batikPostWait} & \per{\batikVolatileTotal} & \per{\batikClassInit} & \per{\batikClassAccess}\\
\bench{h2} 		& \htwoNoFPOtherTotal & \per{\htwoAcqRelOtherTotal} 			& \htwoNoAcqRelOtherTotal		& \per{\htwoFork} 		& \per{\htwoJoin} & \per{\htwoPreWait} & \per{\htwoPostWait} & \per{\htwoVolatileTotal} & \per{\htwoClassInit} & \per{\htwoClassAccess} \\
\bench{jython} 	& \jythonNoFPOtherTotal & \per{\jythonAcqRelOtherTotal} 		& \jythonNoAcqRelOtherTotal 		& \per{\jythonFork} 	& \per{\jythonJoin} & \per{\jythonPreWait} & \per{\jythonPostWait} & \per{\jythonVolatileTotal} & \per{\jythonClassInit} & \per{\jythonClassAccess} \\
\bench{luindex} & \luindexNoFPOtherTotal & \per{\luindexAcqRelOtherTotal} 	& \luindexNoAcqRelOtherTotal 	& \per{\luindexFork}	& \per{\luindexJoin} & \per{\luindexPreWait} & \per{\luindexPostWait} & \per{\luindexVolatileTotal} & \per{\luindexClassInit} & \per{\luindexClassAccess} \\
\bench{lusearch}& \lusearchNoFPOtherTotal & \per{\lusearchAcqRelOtherTotal}	& \lusearchNoAcqRelOtherTotal	& \per{\lusearchFork}	& \per{\lusearchJoin} & \per{\lusearchPreWait} & \per{\lusearchPostWait} & \per{\lusearchVolatileTotal} & \per{\lusearchClassInit} & \per{\lusearchClassAccess} \\
\bench{pmd} 	& \pmdNoFPOtherTotal & \per{\pmdAcqRelOtherTotal} 			& \pmdNoAcqRelOtherTotal 		& \per{\pmdFork} 		& \per{\pmdJoin} & \per{\pmdPreWait} & \per{\pmdPostWait} & \per{\pmdVolatileTotal} & \per{\pmdClassInit} & \per{\pmdClassAccess} \\
\bench{sunflow} & \sunflowNoFPOtherTotal & \per{\sunflowAcqRelOtherTotal} 	& \sunflowNoAcqRelOtherTotal 	& \per{\sunflowFork}	& \per{\sunflowJoin} & \per{\sunflowPreWait} & \per{\sunflowPostWait} & \per{\sunflowVolatileTotal} & \per{\sunflowClassInit} & \per{\sunflowClassAccess} \\
\bench{tomcat} 	& \tomcatNoFPOtherTotal & \per{\tomcatAcqRelOtherTotal} 		& \tomcatNoAcqRelOtherTotal 		& \per{\tomcatFork} 	& \per{\tomcatJoin} & \per{\tomcatPreWait} & \per{\tomcatPostWait} & \per{\tomcatVolatileTotal} & \per{\tomcatClassInit} & \per{\tomcatClassAccess} \\
\bench{xalan} 	& \xalanNoFPOtherTotal & \per{\xalanAcqRelOtherTotal} 		& \xalanNoAcqRelOtherTotal 		& \per{\xalanFork}		& \per{\xalanJoin} & \per{\xalanPreWait} & \per{\xalanPostWait} & \per{\xalanVolatileTotal} & \per{\xalanClassInit} & \per{\xalanClassAccess} \\\hline
\end{tabular}
%  
\caption{Other event counts.}
\label{tab:fast-tool-event-counts:other}
\end{table*}

\begin{table*}[t]
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\newcommand{\per}[1]{#1\%}
\input{result-macros/PIP_fastTool_noRaceLimit}
%  
\small
\centering
\begin{tabular}{@{}l|r|rrrr@{}}
& \mc{5}{c@{}}{\FastTool Extra: Race Type Counts}  \\
Program & Race Total & Wr-Rd Race & Wr-Wr Race & Rd-Wr Race & Rd(Shd)-Wr Race \\\hline
\bench{avrora} 	& \avroraRaceTotal & \per{\avroraWrRdRace} 		& \per{\avroraWrWrRace} 		& \per{\avroraRdWrRace} 	& \per{\avroraRdShWrRace} \\
\bench{batik} 	& \batikRaceTotal & \per{\batikWrRdRace} 		& \per{\batikWrWrRace} 		& \per{\batikRdWrRace} 		& \per{\batikRdShWrRace} \\
\bench{h2} 		& \htwoRaceTotal & \per{\htwoWrRdRace} 			& \per{\htwoWrWrRace}		& \per{\htwoRdWrRace} 		& \per{\htwoRdShWrRace} \\
\bench{jython} 	& \jythonRaceTotal & \per{\jythonWrRdRace} 		& \per{\jythonWrWrRace} 		& \per{\jythonRdWrRace} 	& \per{\jythonRdShWrRace} \\
\bench{luindex} & \luindexRaceTotal & \per{\luindexWrRdRace} 	& \per{\luindexWrWrRace} 	& \per{\luindexRdWrRace}	& \per{\luindexRdShWrRace} \\
\bench{lusearch}& \lusearchRaceTotal & \per{\lusearchWrRdRace}	& \per{\lusearchWrWrRace}	& \per{\lusearchRdWrRace}	& \per{\lusearchRdShWrRace} \\
\bench{pmd} 	& \pmdRaceTotal & \per{\pmdWrRdRace} 			& \per{\pmdWrWrRace} 		& \per{\pmdRdWrRace} 		& \per{\pmdRdShWrRace} \\
\bench{sunflow} & \sunflowRaceTotal & \per{\sunflowWrRdRace} 	& \per{\sunflowWrWrRace} 	& \per{\sunflowRdWrRace}	& \per{\sunflowRdShWrRace} \\
\bench{tomcat} 	& \tomcatRaceTotal & \per{\tomcatWrRdRace} 		& \per{\tomcatWrWrRace} 		& \per{\tomcatRdWrRace} 	& \per{\tomcatRdShWrRace} \\
\bench{xalan} 	& \xalanRaceTotal & \per{\xalanWrRdRace} 		& \per{\xalanWrWrRace} 		& \per{\xalanRdWrRace}		& \per{\xalanRdShWrRace} \\\hline
\end{tabular}
%  
\caption{Other event counts.}
\label{tab:fast-tool-event-counts:raceType}
\end{table*}

==> fast-tool-extra-tables-2.tex <==
\begin{table*}[t]
\newcommand\DCwoG{\DC}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_fastTool_shortestRaceEdge}
 
\small
\centering
\begin{tabular}{@{}l|rl|rl||r|rrrrrrrrr}
& \mc{2}{c|}{} & \mc{2}{c||}{} & Base & \mc{8}{c}{\FastTool Extra 2: Slowdown (normalized to Base time)} \\
Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & time & Empty & \FT & \HB & \WCP & \DC & \CAPO & \CAPO-Opt & \CAPO-Opt-Alt \\\hline 
\bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraTotalThreads 	& (\avroraMaxLiveThreads)	& \base{\avroraBaseTime}   & \roh{\avroraEmptyTime}   & \roh{\avroraFTTime}   & \roh{\avroraHBTime}   & \roh{\avroraWCPTime}   & \roh{\avroraDCTime} 	& \roh{\avroraCAPOTime} 	& \roh{\avroraCAPOOPTTime} & \roh{\avroraCAPOOPTALTTime} \\
\bench{batik} 		& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikTotalThreads 	& (\batikMaxLiveThreads)	& \base{\batikBaseTime}    & \roh{\batikEmptyTime}    & \roh{\batikFTTime}    & \roh{\batikHBTime}    & \roh{\batikWCPTime}    & \roh{\batikDCTime}    & \roh{\batikCAPOTime} 		& \roh{\batikCAPOOPTTime} & \roh{\batikCAPOOPTALTTime} \\
\bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoTotalThreads 	& (\htwoMaxLiveThreads)	    & \base{\htwoBaseTime}     & \roh{\htwoEmptyTime}     & \roh{\htwoFTTime}     & \roh{\htwoHBTime}     & \roh{\htwoWCPTime}     & \roh{\htwoDCTime}     & \roh{\htwoCAPOTime} 		& \roh{\htwoCAPOOPTTime} & \roh{\htwoCAPOOPTALTTime} \\
\bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonTotalThreads	& (\jythonMaxLiveThreads)	& \base{\jythonBaseTime}   & \roh{\jythonEmptyTime}   & \roh{\jythonFTTime}   & \roh{\jythonHBTime} 	 & \roh{\jythonWCPTime}   & \roh{\jythonDCTime} 	 & \roh{\jythonCAPOTime} 	& \roh{\jythonCAPOOPTTime} & \roh{\jythonCAPOOPTALTTime} \\
\bench{luindex} 	& \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexTotalThreads	& (\luindexMaxLiveThreads)	& \base{\luindexBaseTime}  & \roh{\luindexEmptyTime}  & \roh{\luindexFTTime}  & \roh{\luindexHBTime}  & \roh{\luindexWCPTime}  & \roh{\luindexDCTime}  & \roh{\luindexCAPOTime} 	& \roh{\luindexCAPOOPTTime} & \roh{\luindexCAPOOPTALTTime} \\
\bench{lusearch}	& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchTotalThreads	& (\lusearchMaxLiveThreads)	& \base{\lusearchBaseTime} & \roh{\lusearchEmptyTime} & \roh{\lusearchFTTime} & \roh{\lusearchHBTime} & \roh{\lusearchWCPTime} & \roh{\lusearchDCTime} & \roh{\lusearchCAPOTime}	& \roh{\lusearchCAPOOPTTime} & \roh{\lusearchCAPOOPTALTTime} \\
\bench{pmd}		& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdTotalThreads	    & (\pmdMaxLiveThreads)	    & \base{\pmdBaseTime}      & \roh{\pmdEmptyTime}      & \roh{\pmdFTTime}      & \roh{\pmdHBTime}      & \roh{\pmdWCPTime}      & \roh{\pmdDCTime}	     & \roh{\pmdCAPOTime} 		& \roh{\pmdCAPOOPTTime} & \roh{\pmdCAPOOPTALTTime} \\
\bench{sunflow} 	& \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowTotalThreads	& (\sunflowMaxLiveThreads)	& \base{\sunflowBaseTime}  & \roh{\sunflowEmptyTime}  & \roh{\sunflowFTTime}  & \roh{\sunflowHBTime}	 & \roh{\sunflowWCPTime}  & \roh{\sunflowDCTime}  & \roh{\sunflowCAPOTime} 	& \roh{\sunflowCAPOOPTTime} & \roh{\sunflowCAPOOPTALTTime} \\
\bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatTotalThreads	& (\tomcatMaxLiveThreads)	& \base{\tomcatBaseTime}   & \roh{\tomcatEmptyTime}   & \roh{\tomcatFTTime}   & \roh{\tomcatHBTime} 	 & \roh{\tomcatWCPTime}   & \roh{\tomcatDCTime}   & \roh{\tomcatCAPOTime} 	& \roh{\tomcatCAPOOPTTime} & \roh{\tomcatCAPOOPTALTTime} \\
\bench{xalan} 		& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanTotalThreads	& (\xalanMaxLiveThreads)	& \base{\xalanBaseTime}    & \roh{\xalanEmptyTime}    & \roh{\xalanFTTime}    & \roh{\xalanHBTime}    & \roh{\xalanWCPTime}    & \roh{\xalanDCTime}    & \roh{\xalanCAPOTime} 		& \roh{\xalanCAPOOPTTime} & \roh{\xalanCAPOOPTALTTime} 
\end{tabular}

% \notes{
% \jake{Raw results for all the tables and figures in
% evaluation can be found here:
% \url{http://cse-dcse101008d.cse.ohio-state.edu/exp-products/PIP\_test/}}
% }

\caption{Run time for \fasttool and other analysis
configurations.
All values (except thread counts) are rounded to 2 significant figures.
The table reports \PIP's slowdown relative to uninstrumented execution
as the first value in the \emph{\Approach} column
(\eg, \protect\roh{\avroraDCTime} for \bench{avrora}).
The text explains other values.} 

\label{tab:performance}
\end{table*}
 
\begin{table*}[t]
\newcommand\DCwoG{\DC}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_fastTool_shortestRaceEdge}
 
\small
\centering
\begin{tabular}{@{}l|rl|rl||rrrrrrr}
& \mc{2}{c|}{} & \mc{2}{c||}{} & \mc{7}{c}{\FastTool Extra 2: Memory usage (GB)} \\
Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & \FT & \HB & \WCP & \DC & \CAPO & \CAPO-Opt & \CAPO-Opt-Alt \\\hline 
\bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraTotalThreads 	& (\avroraMaxLiveThreads)	& \mem{\avroraFTMem}	& \mem{\avroraHBMem}	 	& \mem{\avroraWCPMem} 	& \mem{\avroraDCMem} 	& \mem{\avroraCAPOMem} 		& \mem{\avroraCAPOOPTMem} & \mem{\avroraCAPOOPTALTMem} \\
\bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikTotalThreads 	& (\batikMaxLiveThreads)	& \mem{\batikFTMem}	& \mem{\batikHBMem} 		& \mem{\batikWCPMem} 	& \mem{\batikDCMem} 	& \mem{\batikCAPOMem} 		& \mem{\batikCAPOOPTMem} & \mem{\batikCAPOOPTALTMem} \\
\bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoTotalThreads 	& (\htwoMaxLiveThreads)	    & \mem{\htwoFTMem}	    & \mem{\htwoHBMem} 		& \mem{\htwoWCPMem} 		& \mem{\htwoDCMem} 		& \mem{\htwoCAPOMem} 		& \mem{\htwoCAPOOPTMem} & \mem{\htwoCAPOOPTALTMem} \\
\bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonTotalThreads	& (\jythonMaxLiveThreads)	& \mem{\jythonFTMem}	& \mem{\jythonHBMem} 	& \mem{\jythonWCPMem} 	& \mem{\jythonDCMem} 	& \mem{\jythonCAPOMem} 		& \mem{\jythonCAPOOPTMem} & \mem{\jythonCAPOOPTALTMem} \\
\bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexTotalThreads	& (\luindexMaxLiveThreads)	& \mem{\luindexFTMem}	& \mem{\luindexHBMem} 	& \mem{\luindexWCPMem} 	& \mem{\luindexDCMem} 	& \mem{\luindexCAPOMem} 	& \mem{\luindexCAPOOPTMem} & \mem{\luindexCAPOOPTALTMem} \\
\bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchTotalThreads	& (\lusearchMaxLiveThreads)	& \mem{\lusearchFTMem}	& \mem{\lusearchHBMem} 	& \mem{\lusearchWCPMem}	& \mem{\lusearchDCMem} 	& \mem{\lusearchCAPOMem}	& \mem{\lusearchCAPOOPTMem} & \mem{\lusearchCAPOOPTALTMem} \\
\bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdTotalThreads	    & (\pmdMaxLiveThreads)	    & \mem{\pmdFTMem}	    & \mem{\pmdHBMem} 		& \mem{\pmdWCPMem} 		& \mem{\pmdDCMem} 		& \mem{\pmdCAPOMem} 		& \mem{\pmdCAPOOPTMem} & \mem{\pmdCAPOOPTALTMem} \\
\bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowTotalThreads	& (\sunflowMaxLiveThreads)	& \mem{\sunflowFTMem}	& \mem{\sunflowHBMem}	& \mem{\sunflowWCPMem} 	& \mem{\sunflowDCMem} 	& \mem{\sunflowCAPOMem} 	& \mem{\sunflowCAPOOPTMem} & \mem{\sunflowCAPOOPTALTMem} \\
\bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatTotalThreads	& (\tomcatMaxLiveThreads)	& \mem{\tomcatFTMem}	& \mem{\tomcatHBMem} 	& \mem{\tomcatWCPMem} 	& \mem{\tomcatDCMem} 	& \mem{\tomcatCAPOMem} 		& \mem{\tomcatCAPOOPTMem} & \mem{\tomcatCAPOOPTALTMem} \\
\bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanTotalThreads	& (\xalanMaxLiveThreads)	& \mem{\xalanFTMem}	& \mem{\xalanHBMem} 		& \mem{\xalanWCPMem} 	& \mem{\xalanDCMem} 	& \mem{\xalanCAPOMem} 		& \mem{\xalanCAPOOPTMem} & \mem{\xalanCAPOOPTALTMem}
\end{tabular}
 
% \notes{
% \jake{Raw results for all the tables and figures in
% evaluation can be found here:
% \url{http://cse-dcse101008d.cse.ohio-state.edu/exp-products/PIP\_test/}}
% }

\caption{Memory usage for \fasttool and other analysis
configurations.
All values are rounded to 2 significant figures.
The text explains other values.} 

\label{tab:memory}
\end{table*}
 
\begin{table*}[t]
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\newcommand{\ci}[1]{\ensuremath{\pm{\;}#1}}
\input{result-macros/PIP_fastTool_shortestRaceEdge}
%  
\small
\centering
\begin{tabular}{@{}l|rlrl|rlrl|rlrl@{}}
\et{}{} & \mc{12}{c@{}}{\FastTool Extra 2: Statically distinct races (dynamic races)}  \\
Program \et{Events}{\#Thr} & \mc{4}{c|}{\FT-races} & \mc{4}{c|}{\HB-races} & \mc{4}{c}{\WCP-races} \\\hline
\bench{avrora} 	\et{\avroraEvents}{\avroraThreads} 		& \avroraFT & \ci{\avroraFTCI} 		& (\avroraFTDynamic) & \ci{\avroraFTDynamicCI}		& \avroraHB & \ci{\avroraHBCI} 		& (\avroraHBDynamic) & \ci{\avroraHBDynamicCI}		& \avroraWCP & \ci{\avroraWCPCI} 		& (\avroraWCPDynamic) & \ci{\avroraWCPDynamicCI} \\
\bench{batik} 	\et{\batikEvents}{\batikThreads} 		& \batikFT & \ci{\batikFTCI} 		& (\batikFTDynamic) & \ci{\batikFTDynamicCI} 		& \batikHB & \ci{\batikHBCI} 		& (\batikHBDynamic) & \ci{\batikHBDynamicCI} 		& \batikWCP & \ci{\batikWCPCI} 			& (\batikWCPDynamic) & \ci{\batikWCPDynamicCI} \\
\bench{h2} 		\et{\htwoEvents}{\htwoThreads} 			& \htwoFT & \ci{\htwoFTCI} 			& (\htwoFTDynamic) & \ci{\htwoFTDynamicCI}			& \htwoHB & \ci{\htwoHBCI} 			& (\htwoHBDynamic) & \ci{\htwoHBDynamicCI} 			& \htwoWCP & \ci{\htwoWCPCI} 			& (\htwoWCPDynamic) & \ci{\htwoWCPDynamicCI} \\
\bench{jython} 	\et{\jythonEvents}{\jythonThreads} 		& \jythonFT & \ci{\jythonFTCI} 		& (\jythonFTDynamic) & \ci{\jythonFTDynamicCI}		& \jythonHB & \ci{\jythonHBCI} 		& (\jythonHBDynamic) & \ci{\jythonHBDynamicCI} 		& \jythonWCP & \ci{\jythonWCPCI} 		& (\jythonWCPDynamic) & \ci{\jythonWCPDynamicCI} \\
\bench{luindex} \et{\luindexEvents}{\luindexThreads} 	& \luindexFT & \ci{\luindexFTCI} 	& (\luindexFTDynamic) & \ci{\luindexFTDynamicCI}	& \luindexHB & \ci{\luindexHBCI} 	& (\luindexHBDynamic) & \ci{\luindexHBDynamicCI} 	& \luindexWCP & \ci{\luindexWCPCI} 		& (\luindexWCPDynamic) & \ci{\luindexWCPDynamicCI} \\
\bench{lusearch}\et{\lusearchEvents}{\lusearchThreads}	& \lusearchFT & \ci{\lusearchFTCI} 	& (\lusearchFTDynamic) & \ci{\lusearchFTDynamicCI}	& \lusearchHB & \ci{\lusearchHBCI} 	& (\lusearchHBDynamic) & \ci{\lusearchHBDynamicCI}	& \lusearchWCP & \ci{\lusearchWCPCI} 	& (\lusearchWCPDynamic) & \ci{\lusearchWCPDynamicCI} \\
\bench{pmd} 	\et{\pmdEvents}{\pmdThreads} 			& \pmdFT & \ci{\pmdFTCI} 			& (\pmdFTDynamic) & \ci{\pmdFTDynamicCI}			& \pmdHB & \ci{\pmdHBCI} 			& (\pmdHBDynamic) & \ci{\pmdHBDynamicCI} 			& \pmdWCP & \ci{\pmdWCPCI}	 			& (\pmdWCPDynamic) & \ci{\pmdWCPDynamicCI} \\
\bench{sunflow} \et{\sunflowEvents}{\sunflowThreads} 	& \sunflowFT & \ci{\sunflowFTCI} 	& (\sunflowFTDynamic) & \ci{\sunflowFTDynamicCI} 	& \sunflowHB & \ci{\sunflowHBCI} 	& (\sunflowHBDynamic) & \ci{\sunflowHBDynamicCI} 	& \sunflowWCP & \ci{\sunflowWCPCI} 		& (\sunflowWCPDynamic) & \ci{\sunflowWCPDynamicCI} \\
\bench{tomcat} 	\et{\tomcatEvents}{\tomcatThreads} 		& \tomcatFT & \ci{\tomcatFTCI} 		& (\tomcatFTDynamic) & \ci{\tomcatFTDynamicCI}		& \tomcatHB & \ci{\tomcatHBCI} 		& (\tomcatHBDynamic) & \ci{\tomcatHBDynamicCI} 		& \tomcatWCP & \ci{\tomcatWCPCI} 		& (\tomcatWCPDynamic) & \ci{\tomcatWCPDynamicCI} \\
\bench{xalan} 	\et{\xalanEvents}{\xalanThreads} 		& \xalanFT & \ci{\xalanFTCI} 		& (\xalanFTDynamic) & \ci{\xalanFTDynamicCI}		& \xalanHB & \ci{\xalanHBCI} 		& (\xalanHBDynamic) & \ci{\xalanHBDynamicCI} 		& \xalanWCP & \ci{\xalanWCPCI} 			& (\xalanWCPDynamic) & \ci{\xalanWCPDynamicCI} \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\newcommand{\ci}[1]{\ensuremath{\pm{\;}#1}}
\input{result-macros/PIP_fastTool_shortestRaceEdge}
%  
\small
\centering
\begin{tabular}{@{}l|rlrl|rlrl@{}}
\et{}{} & \mc{8}{c@{}}{\FastTool Extra 2: Statically distinct races (dynamic races)}  \\
Program \et{Events}{\#Thr} & \mc{4}{c|}{\DC-races} & \mc{4}{c}{\CAPO-races} \\\hline
\bench{avrora} 	\et{\avroraEvents}{\avroraThreads} 		& \avroraWDC & \ci{\avroraWDCCI} 	& (\avroraWDCDynamic) & \ci{\avroraWDCDynamicCI}	& \avroraCAPO & \ci{\avroraCAPOCI}		& (\avroraCAPODynamic) & \ci{\avroraCAPODynamicCI} \\
\bench{batik} 	\et{\batikEvents}{\batikThreads} 		& \batikWDC & \ci{\batikWDCCI} 		& (\batikWDCDynamic) & \ci{\batikWDCDynamicCI}		& \batikCAPO & \ci{\batikCAPOCI} 		& (\batikCAPODynamic) & \ci{\batikCAPODynamicCI} \\
\bench{h2} 		\et{\htwoEvents}{\htwoThreads} 			& \htwoWDC & \ci{\htwoWDCCI} 		& (\htwoWDCDynamic) & \ci{\htwoWDCDynamicCI}		& \htwoCAPO & \ci{\htwoCAPOCI} 			& (\htwoCAPODynamic) & \ci{\htwoCAPODynamicCI} \\
\bench{jython} 	\et{\jythonEvents}{\jythonThreads} 		& \jythonWDC & \ci{\jythonWDCCI} 	& (\jythonWDCDynamic) & \ci{\jythonWDCDynamicCI}	& \jythonCAPO & \ci{\jythonCAPOCI} 		& (\jythonCAPODynamic) & \ci{\jythonCAPODynamicCI} \\
\bench{luindex} \et{\luindexEvents}{\luindexThreads} 	& \luindexWDC & \ci{\luindexWDCCI} 	& (\luindexWDCDynamic) & \ci{\luindexWDCDynamicCI}	& \luindexCAPO & \ci{\luindexCAPOCI} 	& (\luindexCAPODynamic) & \ci{\luindexCAPODynamicCI} \\
\bench{lusearch}\et{\lusearchEvents}{\lusearchThreads}	& \lusearchWDC & \ci{\lusearchWDCCI}& (\lusearchWDCDynamic) & \ci{\lusearchWDCDynamicCI}& \lusearchCAPO & \ci{\lusearchCAPOCI} 	& (\lusearchCAPODynamic) & \ci{\lusearchCAPODynamicCI} \\
\bench{pmd} 	\et{\pmdEvents}{\pmdThreads} 			& \pmdWDC & \ci{\pmdWDCCI} 			& (\pmdWDCDynamic) & \ci{\pmdWDCDynamicCI}			& \pmdCAPO & \ci{\pmdCAPOCI} 			& (\pmdCAPODynamic) & \ci{\pmdCAPODynamicCI} \\
\bench{sunflow} \et{\sunflowEvents}{\sunflowThreads} 	& \sunflowWDC & \ci{\sunflowWDCCI} 	& (\sunflowWDCDynamic) & \ci{\sunflowWDCDynamicCI}	& \sunflowCAPO & \ci{\sunflowCAPOCI} 	& (\sunflowCAPODynamic) & \ci{\sunflowCAPODynamicCI} \\
\bench{tomcat} 	\et{\tomcatEvents}{\tomcatThreads} 		& \tomcatWDC & \ci{\tomcatWDCCI} 	& (\tomcatWDCDynamic) & \ci{\tomcatWDCDynamicCI}	& \tomcatCAPO & \ci{\tomcatCAPOCI} 		& (\tomcatCAPODynamic) & \ci{\tomcatCAPODynamicCI} \\
\bench{xalan} 	\et{\xalanEvents}{\xalanThreads} 		& \xalanWDC & \ci{\xalanWDCCI} 		& (\xalanWDCDynamic) & \ci{\xalanWDCDynamicCI}		& \xalanCAPO & \ci{\xalanCAPOCI} 		& (\xalanCAPODynamic) & \ci{\xalanCAPODynamicCI} \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\newcommand{\ci}[1]{\ensuremath{\pm{\;}#1}}
\input{result-macros/PIP_fastTool_shortestRaceEdge}
%  
\small
\centering
\begin{tabular}{@{}l|rlrl|rlrl|rlrl@{}}
\et{}{} & \mc{12}{c@{}}{\FastTool Extra 2: Statically distinct races (dynamic races)}  \\
Program \et{Events}{\#Thr} & \mc{4}{c|}{\CAPO-races} & \mc{4}{c|@{}}{\CAPO-Opt-races} & \mc{4}{c@{}}{Opt-Alt-races} \\\hline
\bench{avrora} 	\et{\avroraEvents}{\avroraThreads} 		& \avroraCAPO & \ci{\avroraCAPOCI} 		& (\avroraCAPODynamic) & \ci{\avroraCAPODynamicCI}		& \avroraCAPOOPT & \ci{\avroraCAPOOPTCI} 	& (\avroraCAPOOPTDynamic) & \ci{\avroraCAPOOPTDynamicCI}	& \avroraCAPOOPTALT & \ci{\avroraCAPOOPTALTCI} 		& (\avroraCAPOOPTALTDynamic) & \ci{\avroraCAPOOPTALTDynamicCI} \\
\bench{batik} 	\et{\batikEvents}{\batikThreads} 		& \batikCAPO & \ci{\batikCAPOCI} 		& (\batikCAPODynamic) & \ci{\batikCAPODynamicCI} 		& \batikCAPOOPT & \ci{\batikCAPOOPTCI} 		& (\batikCAPOOPTDynamic) & \ci{\batikCAPOOPTDynamicCI} 		& \batikCAPOOPTALT & \ci{\batikCAPOOPTALTCI} 		& (\batikCAPOOPTALTDynamic) & \ci{\batikCAPOOPTALTDynamicCI} \\
\bench{h2} 		\et{\htwoEvents}{\htwoThreads} 			& \htwoCAPO & \ci{\htwoCAPOCI} 			& (\htwoCAPODynamic) & \ci{\htwoCAPODynamicCI}			& \htwoCAPOOPT & \ci{\htwoCAPOOPTCI} 		& (\htwoCAPOOPTDynamic) & \ci{\htwoCAPOOPTDynamicCI} 		& \htwoCAPOOPTALT & \ci{\htwoCAPOOPTALTCI} 			& (\htwoCAPOOPTALTDynamic) & \ci{\htwoCAPOOPTALTDynamicCI} \\
\bench{jython} 	\et{\jythonEvents}{\jythonThreads} 		& \jythonCAPO & \ci{\jythonCAPOCI} 		& (\jythonCAPODynamic) & \ci{\jythonCAPODynamicCI}		& \jythonCAPOOPT & \ci{\jythonCAPOOPTCI} 	& (\jythonCAPOOPTDynamic) & \ci{\jythonCAPOOPTDynamicCI} 	& \jythonCAPOOPTALT & \ci{\jythonCAPOOPTALTCI} 		& (\jythonCAPOOPTALTDynamic) & \ci{\jythonCAPOOPTALTDynamicCI} \\
\bench{luindex} \et{\luindexEvents}{\luindexThreads} 	& \luindexCAPO & \ci{\luindexCAPOCI} 	& (\luindexCAPODynamic) & \ci{\luindexCAPODynamicCI}	& \luindexCAPOOPT & \ci{\luindexCAPOOPTCI} 	& (\luindexCAPOOPTDynamic) & \ci{\luindexCAPOOPTDynamicCI} 	& \luindexCAPOOPTALT & \ci{\luindexCAPOOPTALTCI} 	& (\luindexCAPOOPTALTDynamic) & \ci{\luindexCAPOOPTALTDynamicCI} \\
\bench{lusearch}\et{\lusearchEvents}{\lusearchThreads}	& \lusearchCAPO & \ci{\lusearchCAPOCI} 	& (\lusearchCAPODynamic) & \ci{\lusearchCAPODynamicCI}	& \lusearchCAPOOPT & \ci{\lusearchCAPOOPTCI}& (\lusearchCAPOOPTDynamic) & \ci{\lusearchCAPOOPTDynamicCI}& \lusearchCAPOOPTALT & \ci{\lusearchCAPOOPTALTCI} 	& (\lusearchCAPOOPTALTDynamic) & \ci{\lusearchCAPOOPTALTDynamicCI} \\
\bench{pmd} 	\et{\pmdEvents}{\pmdThreads} 			& \pmdCAPO & \ci{\pmdCAPOCI} 			& (\pmdCAPODynamic) & \ci{\pmdCAPODynamicCI}			& \pmdCAPOOPT & \ci{\pmdCAPOOPTCI} 			& (\pmdCAPOOPTDynamic) & \ci{\pmdCAPOOPTDynamicCI} 			& \pmdCAPOOPTALT & \ci{\pmdCAPOOPTALTCI}	 		& (\pmdCAPOOPTALTDynamic) & \ci{\pmdCAPOOPTALTDynamicCI} \\
\bench{sunflow} \et{\sunflowEvents}{\sunflowThreads} 	& \sunflowCAPO & \ci{\sunflowCAPOCI} 	& (\sunflowCAPODynamic) & \ci{\sunflowCAPODynamicCI} 	& \sunflowCAPOOPT & \ci{\sunflowCAPOOPTCI} 	& (\sunflowCAPOOPTDynamic) & \ci{\sunflowCAPOOPTDynamicCI} 	& \sunflowCAPOOPTALT & \ci{\sunflowCAPOOPTALTCI} 	& (\sunflowCAPOOPTALTDynamic) & \ci{\sunflowCAPOOPTALTDynamicCI} \\
\bench{tomcat} 	\et{\tomcatEvents}{\tomcatThreads} 		& \tomcatCAPO & \ci{\tomcatCAPOCI} 		& (\tomcatCAPODynamic) & \ci{\tomcatCAPODynamicCI}		& \tomcatCAPOOPT & \ci{\tomcatCAPOOPTCI} 	& (\tomcatCAPOOPTDynamic) & \ci{\tomcatCAPOOPTDynamicCI} 	& \tomcatCAPOOPTALT & \ci{\tomcatCAPOOPTALTCI} 		& (\tomcatCAPOOPTALTDynamic) & \ci{\tomcatCAPOOPTALTDynamicCI} \\
\bench{xalan} 	\et{\xalanEvents}{\xalanThreads} 		& \xalanCAPO & \ci{\xalanCAPOCI} 		& (\xalanCAPODynamic) & \ci{\xalanCAPODynamicCI}		& \xalanCAPOOPT & \ci{\xalanCAPOOPTCI} 		& (\xalanCAPOOPTDynamic) & \ci{\xalanCAPOOPTDynamicCI} 		& \xalanCAPOOPTALT & \ci{\xalanCAPOOPTALTCI} 		& (\xalanCAPOOPTALTDynamic) & \ci{\xalanCAPOOPTALTDynamicCI} \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\caption{\FT-, \HB-, \WCP-, \DC-, \CAPO-, and \PIP-races detected by our implementation.
Each result is the average of 10 trials, rounded to the nearest integer.
Races are identified by single second site.}
 % Each result is from a single trial.}
\label{tab:coverage-dc}
\end{table*}


\begin{table*}[t]
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\newcommand{\ci}[1]{\ensuremath{\pm{\;}#1}}
\newcommand{\ciRange}[2]{(#1--#2)}
\input{result-macros/PIP_fastTool_shortestRaceEdge}
%  
\small
\centering
\begin{tabular}{@{}l|rlr|rlr|rlr@{}}
\et{}{} & \mc{9}{c@{}}{\FastTool Extra 2: Statically distinct races (dynamic races)}  \\
Program \et{Events}{\#Thr} & \mc{3}{c|}{\FT-races} & \mc{3}{c|}{\HB-races} & \mc{3}{c}{\WCP-races} \\\hline
\bench{avrora} 	\et{\avroraEvents}{\avroraThreads} 		& \avroraFT & \ci{\avroraFTCI} 		& \ciRange{\avroraFTDynamicCIMIN}{\avroraFTDynamicCIMAX}	& \avroraHB & \ci{\avroraHBCI} 		& \ciRange{\avroraHBDynamicCIMIN}{\avroraHBDynamicCIMAX}	& \avroraWCP & \ci{\avroraWCPCI} 		& \ciRange{\avroraWCPDynamicCIMIN}{\avroraWCPDynamicCIMAX} \\
\bench{batik} 	\et{\batikEvents}{\batikThreads} 		& \batikFT & \ci{\batikFTCI} 		& \ciRange{\batikFTDynamicCIMIN}{\batikFTDynamicCIMAX} 		& \batikHB & \ci{\batikHBCI} 		& \ciRange{\batikHBDynamicCIMIN}{\batikHBDynamicCIMAX} 		& \batikWCP & \ci{\batikWCPCI} 			& \ciRange{\batikWCPDynamicCIMIN}{\batikWCPDynamicCIMAX} \\
\bench{h2} 		\et{\htwoEvents}{\htwoThreads} 			& \htwoFT & \ci{\htwoFTCI} 			& \ciRange{\htwoFTDynamicCIMIN}{\htwoFTDynamicCIMAX}		& \htwoHB & \ci{\htwoHBCI} 			& \ciRange{\htwoHBDynamicCIMIN}{\htwoHBDynamicCIMAX} 		& \htwoWCP & \ci{\htwoWCPCI} 			& \ciRange{\htwoWCPDynamicCIMIN}{\htwoWCPDynamicCIMAX} \\
\bench{jython} 	\et{\jythonEvents}{\jythonThreads} 		& \jythonFT & \ci{\jythonFTCI} 		& \ciRange{\jythonFTDynamicCIMIN}{\jythonFTDynamicCIMAX}	& \jythonHB & \ci{\jythonHBCI} 		& \ciRange{\jythonHBDynamicCIMIN}{\jythonHBDynamicCIMAX} 	& \jythonWCP & \ci{\jythonWCPCI} 		& \ciRange{\jythonWCPDynamicCIMIN}{\jythonWCPDynamicCIMAX} \\
\bench{luindex} \et{\luindexEvents}{\luindexThreads} 	& \luindexFT & \ci{\luindexFTCI} 	& \ciRange{\luindexFTDynamicCIMIN}{\luindexFTDynamicCIMAX}	& \luindexHB & \ci{\luindexHBCI} 	& \ciRange{\luindexHBDynamicCIMIN}{\luindexHBDynamicCIMAX} 	& \luindexWCP & \ci{\luindexWCPCI} 		& \ciRange{\luindexWCPDynamicCIMIN}{\luindexWCPDynamicCIMAX} \\
\bench{lusearch}\et{\lusearchEvents}{\lusearchThreads}	& \lusearchFT & \ci{\lusearchFTCI} 	& \ciRange{\lusearchFTDynamicCIMIN}{\lusearchFTDynamicCIMAX}& \lusearchHB & \ci{\lusearchHBCI} 	& \ciRange{\lusearchHBDynamicCIMIN}{\lusearchHBDynamicCIMAX}& \lusearchWCP & \ci{\lusearchWCPCI} 	& \ciRange{\lusearchWCPDynamicCIMIN}{\lusearchWCPDynamicCIMAX} \\
\bench{pmd} 	\et{\pmdEvents}{\pmdThreads} 			& \pmdFT & \ci{\pmdFTCI} 			& \ciRange{\pmdFTDynamicCIMIN}{\pmdFTDynamicCIMAX}			& \pmdHB & \ci{\pmdHBCI} 			& \ciRange{\pmdHBDynamicCIMIN}{\pmdHBDynamicCIMAX} 			& \pmdWCP & \ci{\pmdWCPCI}	 			& \ciRange{\pmdWCPDynamicCIMIN}{\pmdWCPDynamicCIMAX} \\
\bench{sunflow} \et{\sunflowEvents}{\sunflowThreads} 	& \sunflowFT & \ci{\sunflowFTCI} 	& \ciRange{\sunflowFTDynamicCIMIN}{\sunflowFTDynamicCIMAX} 	& \sunflowHB & \ci{\sunflowHBCI} 	& \ciRange{\sunflowHBDynamicCIMIN}{\sunflowHBDynamicCIMAX} 	& \sunflowWCP & \ci{\sunflowWCPCI} 		& \ciRange{\sunflowWCPDynamicCIMIN}{\sunflowWCPDynamicCIMAX} \\
\bench{tomcat} 	\et{\tomcatEvents}{\tomcatThreads} 		& \tomcatFT & \ci{\tomcatFTCI} 		& \ciRange{\tomcatFTDynamicCIMIN}{\tomcatFTDynamicCIMAX}	& \tomcatHB & \ci{\tomcatHBCI} 		& \ciRange{\tomcatHBDynamicCIMIN}{\tomcatHBDynamicCIMAX} 	& \tomcatWCP & \ci{\tomcatWCPCI} 		& \ciRange{\tomcatWCPDynamicCIMIN}{\tomcatWCPDynamicCIMAX} \\
\bench{xalan} 	\et{\xalanEvents}{\xalanThreads} 		& \xalanFT & \ci{\xalanFTCI} 		& \ciRange{\xalanFTDynamicCIMIN}{\xalanFTDynamicCIMAX}		& \xalanHB & \ci{\xalanHBCI} 		& \ciRange{\xalanHBDynamicCIMIN}{\xalanHBDynamicCIMAX} 		& \xalanWCP & \ci{\xalanWCPCI} 			& \ciRange{\xalanWCPDynamicCIMIN}{\xalanWCPDynamicCIMAX} \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\newcommand{\ci}[1]{\ensuremath{\pm{\;}#1}}
\newcommand{\ciRange}[2]{(#1--#2)}
\input{result-macros/PIP_fastTool_shortestRaceEdge}
%  
\small
\centering
\begin{tabular}{@{}l|rlr|rlr@{}}
\et{}{} & \mc{6}{c@{}}{\FastTool Extra 2: Statically distinct races (dynamic races)}  \\
Program \et{Events}{\#Thr} & \mc{3}{c|}{\DC-races} & \mc{3}{c}{\CAPO-races} \\\hline
\bench{avrora} 	\et{\avroraEvents}{\avroraThreads} 		& \avroraWDC & \ci{\avroraWDCCI} 	& \ciRange{\avroraWDCDynamicCIMIN}{\avroraWDCDynamicCIMAX}		& \avroraCAPO & \ci{\avroraCAPOCI} 		& \ciRange{\avroraCAPODynamicCIMIN}{\avroraCAPODynamicCIMAX} \\
\bench{batik} 	\et{\batikEvents}{\batikThreads} 		& \batikWDC & \ci{\batikWDCCI} 		& \ciRange{\batikWDCDynamicCIMIN}{\batikWDCDynamicCIMAX} 		& \batikCAPO & \ci{\batikCAPOCI} 		& \ciRange{\batikCAPODynamicCIMIN}{\batikCAPODynamicCIMAX} \\
\bench{h2} 		\et{\htwoEvents}{\htwoThreads} 			& \htwoWDC & \ci{\htwoWDCCI} 		& \ciRange{\htwoWDCDynamicCIMIN}{\htwoWDCDynamicCIMAX}			& \htwoCAPO & \ci{\htwoCAPOCI} 			& \ciRange{\htwoCAPODynamicCIMIN}{\htwoCAPODynamicCIMAX} \\
\bench{jython} 	\et{\jythonEvents}{\jythonThreads} 		& \jythonWDC & \ci{\jythonWDCCI} 	& \ciRange{\jythonWDCDynamicCIMIN}{\jythonWDCDynamicCIMAX}		& \jythonCAPO & \ci{\jythonCAPOCI} 		& \ciRange{\jythonCAPODynamicCIMIN}{\jythonCAPODynamicCIMAX} \\
\bench{luindex} \et{\luindexEvents}{\luindexThreads} 	& \luindexWDC & \ci{\luindexWDCCI} 	& \ciRange{\luindexWDCDynamicCIMIN}{\luindexWDCDynamicCIMAX}	& \luindexCAPO & \ci{\luindexCAPOCI} 	& \ciRange{\luindexCAPODynamicCIMIN}{\luindexCAPODynamicCIMAX} \\
\bench{lusearch}\et{\lusearchEvents}{\lusearchThreads}	& \lusearchWDC & \ci{\lusearchWDCCI}& \ciRange{\lusearchWDCDynamicCIMIN}{\lusearchWDCDynamicCIMAX}	& \lusearchCAPO & \ci{\lusearchCAPOCI} 	& \ciRange{\lusearchCAPODynamicCIMIN}{\lusearchCAPODynamicCIMAX} \\
\bench{pmd} 	\et{\pmdEvents}{\pmdThreads} 			& \pmdWDC & \ci{\pmdWDCCI} 			& \ciRange{\pmdWDCDynamicCIMIN}{\pmdWDCDynamicCIMAX}			& \pmdCAPO & \ci{\pmdCAPOCI} 			& \ciRange{\pmdCAPODynamicCIMIN}{\pmdCAPODynamicCIMAX} \\
\bench{sunflow} \et{\sunflowEvents}{\sunflowThreads} 	& \sunflowWDC & \ci{\sunflowWDCCI} 	& \ciRange{\sunflowWDCDynamicCIMIN}{\sunflowWDCDynamicCIMAX} 	& \sunflowCAPO & \ci{\sunflowCAPOCI} 	& \ciRange{\sunflowCAPODynamicCIMIN}{\sunflowCAPODynamicCIMAX} \\
\bench{tomcat} 	\et{\tomcatEvents}{\tomcatThreads} 		& \tomcatWDC & \ci{\tomcatWDCCI} 	& \ciRange{\tomcatWDCDynamicCIMIN}{\tomcatWDCDynamicCIMAX}		& \tomcatCAPO & \ci{\tomcatCAPOCI} 		& \ciRange{\tomcatCAPODynamicCIMIN}{\tomcatCAPODynamicCIMAX} \\
\bench{xalan} 	\et{\xalanEvents}{\xalanThreads} 		& \xalanWDC & \ci{\xalanWDCCI} 		& \ciRange{\xalanWDCDynamicCIMIN}{\xalanWDCDynamicCIMAX}		& \xalanCAPO & \ci{\xalanCAPOCI} 		& \ciRange{\xalanCAPODynamicCIMIN}{\xalanCAPODynamicCIMAX} \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\newcommand{\ci}[1]{\ensuremath{\pm{\;}#1}}
\newcommand{\ciRange}[2]{(#1--#2)}
\input{result-macros/PIP_fastTool_shortestRaceEdge}
%  
\small
\centering
\begin{tabular}{@{}l|rlr|rlr|rlr@{}}
\et{}{} & \mc{9}{c@{}}{\FastTool Extra 2: Statically distinct races (dynamic races)}  \\
Program \et{Events}{\#Thr} & \mc{3}{c|}{\CAPO-races} & \mc{3}{c|@{}}{\CAPO-Opt-races} & \mc{3}{c@{}}{Opt-Alt-races} \\\hline
\bench{avrora} 	\et{\avroraEvents}{\avroraThreads} 		& \avroraCAPO & \ci{\avroraCAPOCI} 		& \ciRange{\avroraCAPODynamicCIMIN}{\avroraCAPODynamicCIMAX}	& \avroraCAPOOPT & \ci{\avroraCAPOOPTCI} 	& \ciRange{\avroraCAPOOPTDynamicCIMIN}{\avroraCAPOOPTDynamicCIMAX}		& \avroraCAPOOPTALT & \ci{\avroraCAPOOPTALTCI} 		& \ciRange{\avroraCAPOOPTALTDynamicCIMIN}{\avroraCAPOOPTALTDynamicCIMAX} \\
\bench{batik} 	\et{\batikEvents}{\batikThreads} 		& \batikCAPO & \ci{\batikCAPOCI} 		& \ciRange{\batikCAPODynamicCIMIN}{\batikCAPODynamicCIMAX} 		& \batikCAPOOPT & \ci{\batikCAPOOPTCI} 		& \ciRange{\batikCAPOOPTDynamicCIMIN}{\batikCAPOOPTDynamicCIMAX} 		& \batikCAPOOPTALT & \ci{\batikCAPOOPTALTCI} 		& \ciRange{\batikCAPOOPTALTDynamicCIMIN}{\batikCAPOOPTALTDynamicCIMAX} \\
\bench{h2} 		\et{\htwoEvents}{\htwoThreads} 			& \htwoCAPO & \ci{\htwoCAPOCI} 			& \ciRange{\htwoCAPODynamicCIMIN}{\htwoCAPODynamicCIMAX}		& \htwoCAPOOPT & \ci{\htwoCAPOOPTCI} 		& \ciRange{\htwoCAPOOPTDynamicCIMIN}{\htwoCAPOOPTDynamicCIMAX} 			& \htwoCAPOOPTALT & \ci{\htwoCAPOOPTALTCI} 			& \ciRange{\htwoCAPOOPTALTDynamicCIMIN}{\htwoCAPOOPTALTDynamicCIMAX} \\
\bench{jython} 	\et{\jythonEvents}{\jythonThreads} 		& \jythonCAPO & \ci{\jythonCAPOCI} 		& \ciRange{\jythonCAPODynamicCIMIN}{\jythonCAPODynamicCIMAX}	& \jythonCAPOOPT & \ci{\jythonCAPOOPTCI} 	& \ciRange{\jythonCAPOOPTDynamicCIMIN}{\jythonCAPOOPTDynamicCIMAX} 		& \jythonCAPOOPTALT & \ci{\jythonCAPOOPTALTCI} 		& \ciRange{\jythonCAPOOPTALTDynamicCIMIN}{\jythonCAPOOPTALTDynamicCIMAX} \\
\bench{luindex} \et{\luindexEvents}{\luindexThreads} 	& \luindexCAPO & \ci{\luindexCAPOCI} 	& \ciRange{\luindexCAPODynamicCIMIN}{\luindexCAPODynamicCIMAX}	& \luindexCAPOOPT & \ci{\luindexCAPOOPTCI} 	& \ciRange{\luindexCAPOOPTDynamicCIMIN}{\luindexCAPOOPTDynamicCIMAX} 	& \luindexCAPOOPTALT & \ci{\luindexCAPOOPTALTCI} 	& \ciRange{\luindexCAPOOPTALTDynamicCIMIN}{\luindexCAPOOPTALTDynamicCIMAX} \\
\bench{lusearch}\et{\lusearchEvents}{\lusearchThreads}	& \lusearchCAPO & \ci{\lusearchCAPOCI} 	& \ciRange{\lusearchCAPODynamicCIMIN}{\lusearchCAPODynamicCIMAX}& \lusearchCAPOOPT & \ci{\lusearchCAPOOPTCI}& \ciRange{\lusearchCAPOOPTDynamicCIMIN}{\lusearchCAPOOPTDynamicCIMAX}	& \lusearchCAPOOPTALT & \ci{\lusearchCAPOOPTALTCI} 	& \ciRange{\lusearchCAPOOPTALTDynamicCIMIN}{\lusearchCAPOOPTALTDynamicCIMAX} \\
\bench{pmd} 	\et{\pmdEvents}{\pmdThreads} 			& \pmdCAPO & \ci{\pmdCAPOCI} 			& \ciRange{\pmdCAPODynamicCIMIN}{\pmdCAPODynamicCIMAX}			& \pmdCAPOOPT & \ci{\pmdCAPOOPTCI} 			& \ciRange{\pmdCAPOOPTDynamicCIMIN}{\pmdCAPOOPTDynamicCIMAX} 			& \pmdCAPOOPTALT & \ci{\pmdCAPOOPTALTCI}	 		& \ciRange{\pmdCAPOOPTALTDynamicCIMIN}{\pmdCAPOOPTALTDynamicCIMAX} \\
\bench{sunflow} \et{\sunflowEvents}{\sunflowThreads} 	& \sunflowCAPO & \ci{\sunflowCAPOCI} 	& \ciRange{\sunflowCAPODynamicCIMIN}{\sunflowCAPODynamicCIMAX} 	& \sunflowCAPOOPT & \ci{\sunflowCAPOOPTCI} 	& \ciRange{\sunflowCAPOOPTDynamicCIMIN}{\sunflowCAPOOPTDynamicCIMAX} 	& \sunflowCAPOOPTALT & \ci{\sunflowCAPOOPTALTCI} 	& \ciRange{\sunflowCAPOOPTALTDynamicCIMIN}{\sunflowCAPOOPTALTDynamicCIMAX} \\
\bench{tomcat} 	\et{\tomcatEvents}{\tomcatThreads} 		& \tomcatCAPO & \ci{\tomcatCAPOCI} 		& \ciRange{\tomcatCAPODynamicCIMIN}{\tomcatCAPODynamicCIMAX}	& \tomcatCAPOOPT & \ci{\tomcatCAPOOPTCI} 	& \ciRange{\tomcatCAPOOPTDynamicCIMIN}{\tomcatCAPOOPTDynamicCIMAX} 		& \tomcatCAPOOPTALT & \ci{\tomcatCAPOOPTALTCI} 		& \ciRange{\tomcatCAPOOPTALTDynamicCIMIN}{\tomcatCAPOOPTALTDynamicCIMAX} \\
\bench{xalan} 	\et{\xalanEvents}{\xalanThreads} 		& \xalanCAPO & \ci{\xalanCAPOCI} 		& \ciRange{\xalanCAPODynamicCIMIN}{\xalanCAPODynamicCIMAX}		& \xalanCAPOOPT & \ci{\xalanCAPOOPTCI} 		& \ciRange{\xalanCAPOOPTDynamicCIMIN}{\xalanCAPOOPTDynamicCIMAX} 		& \xalanCAPOOPTALT & \ci{\xalanCAPOOPTALTCI} 		& \ciRange{\xalanCAPOOPTALTDynamicCIMIN}{\xalanCAPOOPTALTDynamicCIMAX} \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\caption{\FT-, \HB-, \WCP-, \DC-, \CAPO-, and \PIP-races detected by our implementation.
Each result is the average of 10 trials, rounded to the nearest integer.
Races are identified by single second site.}
 % Each result is from a single trial.}
\label{tab:coverage-dc}
\end{table*}

==> fast-tool-extra-tables-3.tex <==
\begin{table*}[t]
\newcommand\DCwoG{\DC}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
 \newcommand{\rna}{\textbf{N/A}}
 \newcommand{\memna}{$<\,$2}
 \newcommand{\st}[1]{(#1~s)} %static time
 \newcommand{\dt}[1]{#1~s} %dynamic time
 \newcommand{\mem}[1]{#1} %memory
 \newcommand{\et}[1]{#1M} %event total
 \newcommand{\enfp}[1]{(#1M)} %event total, no fast path
 \newcommand{\base}[1]{#1~s} %base time
 \input{result-macros/PIP_fastTool_raceEdgeAdd_lockCount}
 
 \small
 \centering
 \begin{tabular}{@{}l|rl|rl||r|rrrrrrrrr}
 & \mc{2}{c|}{} & \mc{2}{c||}{} & Base & \mc{8}{c}{\FastTool Extra 3: Slowdown (normalized to Base time)} \\
 Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & time & Empty & \FT & \HB & \WCP & \DC & \CAPO & \CAPO-Opt & \CAPO-Opt-Alt \\\hline 
 \bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraTotalThreads 	& (\avroraMaxLiveThreads)	& \base{\avroraBaseTime}   & \roh{\avroraEmptyTime}   & \roh{\avroraFTTime}   & \roh{\avroraHBTime}   & \roh{\avroraWCPTime}   & \roh{\avroraDCTime} 	& \roh{\avroraCAPOTime} 	& \roh{\avroraCAPOOPTTime} & \roh{\avroraCAPOOPTALTTime} \\
 \bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikTotalThreads 	& (\batikMaxLiveThreads)	& \base{\batikBaseTime}    & \roh{\batikEmptyTime}    & \roh{\batikFTTime}    & \roh{\batikHBTime}    & \roh{\batikWCPTime}    & \roh{\batikDCTime}    & \roh{\batikCAPOTime} 		& \roh{\batikCAPOOPTTime} & \roh{\batikCAPOOPTALTTime} \\
 \bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoTotalThreads 	& (\htwoMaxLiveThreads)	    & \base{\htwoBaseTime}     & \roh{\htwoEmptyTime}     & \roh{\htwoFTTime}     & \roh{\htwoHBTime}     & \roh{\htwoWCPTime}     & \roh{\htwoDCTime}     & \roh{\htwoCAPOTime} 		& \roh{\htwoCAPOOPTTime} & \roh{\htwoCAPOOPTALTTime} \\
 \bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonTotalThreads	& (\jythonMaxLiveThreads)	& \base{\jythonBaseTime}   & \roh{\jythonEmptyTime}   & \roh{\jythonFTTime}   & \roh{\jythonHBTime} 	 & \roh{\jythonWCPTime}   & \roh{\jythonDCTime} 	 & \roh{\jythonCAPOTime} 	& \roh{\jythonCAPOOPTTime} & \roh{\jythonCAPOOPTALTTime} \\
 \bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexTotalThreads	& (\luindexMaxLiveThreads)	& \base{\luindexBaseTime}  & \roh{\luindexEmptyTime}  & \roh{\luindexFTTime}  & \roh{\luindexHBTime}  & \roh{\luindexWCPTime}  & \roh{\luindexDCTime}  & \roh{\luindexCAPOTime} 	& \roh{\luindexCAPOOPTTime} & \roh{\luindexCAPOOPTALTTime} \\
 \bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchTotalThreads	& (\lusearchMaxLiveThreads)	& \base{\lusearchBaseTime} & \roh{\lusearchEmptyTime} & \roh{\lusearchFTTime} & \roh{\lusearchHBTime} & \roh{\lusearchWCPTime} & \roh{\lusearchDCTime} & \roh{\lusearchCAPOTime}	& \roh{\lusearchCAPOOPTTime} & \roh{\lusearchCAPOOPTALTTime} \\
 \bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdTotalThreads	    & (\pmdMaxLiveThreads)	    & \base{\pmdBaseTime}      & \roh{\pmdEmptyTime}      & \roh{\pmdFTTime}      & \roh{\pmdHBTime}      & \roh{\pmdWCPTime}      & \roh{\pmdDCTime}	     & \roh{\pmdCAPOTime} 		& \roh{\pmdCAPOOPTTime} & \roh{\pmdCAPOOPTALTTime} \\
 \bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowTotalThreads	& (\sunflowMaxLiveThreads)	& \base{\sunflowBaseTime}  & \roh{\sunflowEmptyTime}  & \roh{\sunflowFTTime}  & \roh{\sunflowHBTime}	 & \roh{\sunflowWCPTime}  & \roh{\sunflowDCTime}  & \roh{\sunflowCAPOTime} 	& \roh{\sunflowCAPOOPTTime} & \roh{\sunflowCAPOOPTALTTime} \\
 \bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatTotalThreads	& (\tomcatMaxLiveThreads)	& \base{\tomcatBaseTime}   & \roh{\tomcatEmptyTime}   & \roh{\tomcatFTTime}   & \roh{\tomcatHBTime} 	 & \roh{\tomcatWCPTime}   & \roh{\tomcatDCTime}   & \roh{\tomcatCAPOTime} 	& \roh{\tomcatCAPOOPTTime} & \roh{\tomcatCAPOOPTALTTime} \\
 \bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanTotalThreads	& (\xalanMaxLiveThreads)	& \base{\xalanBaseTime}    & \roh{\xalanEmptyTime}    & \roh{\xalanFTTime}    & \roh{\xalanHBTime}    & \roh{\xalanWCPTime}    & \roh{\xalanDCTime}    & \roh{\xalanCAPOTime} 		& \roh{\xalanCAPOOPTTime} & \roh{\xalanCAPOOPTALTTime} 
 \end{tabular}
 % \notes{
 % \jake{Raw results for all the tables and figures in
 % evaluation can be found here:
 % \url{http://cse-dcse101008d.cse.ohio-state.edu/exp-products/PIP\_test/}}
 % }
 \caption{Run time for \fasttool and other analysis
 configurations.
 All values (except thread counts) are rounded to 2 significant figures.
 The table reports \PIP's slowdown relative to uninstrumented execution
 as the first value in the \emph{\Approach} column
 (\eg, \protect\roh{\avroraDCTime} for \bench{avrora}).
 The text explains other values.} 
 %
 \label{tab:performance}
 \end{table*}
 
 \begin{table*}[t]
 \newcommand\DCwoG{\DC}
 \newcommand{\rzero}{0\xspace}
 \newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
 \newcommand{\rna}{\textbf{N/A}}
 \newcommand{\memna}{$<\,$2}
 \newcommand{\st}[1]{(#1~s)} %static time
 \newcommand{\dt}[1]{#1~s} %dynamic time
 \newcommand{\mem}[1]{#1} %memory
 \newcommand{\et}[1]{#1M} %event total
 \newcommand{\enfp}[1]{(#1M)} %event total, no fast path
 \newcommand{\base}[1]{#1~s} %base time
 \input{result-macros/PIP_fastTool_raceEdgeAdd_lockCount}
 
 \small
 \centering
 \begin{tabular}{@{}l|rl|rl||rrrrrrr}
 & \mc{2}{c|}{} & \mc{2}{c||}{} & \mc{7}{c}{\FastTool Extra 3: Memory usage (GB)} \\
 Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & \FT & \HB & \WCP & \DC & \CAPO & \CAPO-Opt & \CAPO-Opt-Alt \\\hline 
 \bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraTotalThreads 	& (\avroraMaxLiveThreads)	& \mem{\avroraFTMem}	& \mem{\avroraHBMem}	 	& \mem{\avroraWCPMem} 	& \mem{\avroraDCMem} 	& \mem{\avroraCAPOMem} 		& \mem{\avroraCAPOOPTMem} & \mem{\avroraCAPOOPTALTMem} \\
 \bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikTotalThreads 	& (\batikMaxLiveThreads)	& \mem{\batikFTMem}	& \mem{\batikHBMem} 		& \mem{\batikWCPMem} 	& \mem{\batikDCMem} 	& \mem{\batikCAPOMem} 		& \mem{\batikCAPOOPTMem} & \mem{\batikCAPOOPTALTMem} \\
 \bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoTotalThreads 	& (\htwoMaxLiveThreads)	    & \mem{\htwoFTMem}	    & \mem{\htwoHBMem} 		& \mem{\htwoWCPMem} 		& \mem{\htwoDCMem} 		& \mem{\htwoCAPOMem} 		& \mem{\htwoCAPOOPTMem} & \mem{\htwoCAPOOPTALTMem} \\
 \bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonTotalThreads	& (\jythonMaxLiveThreads)	& \mem{\jythonFTMem}	& \mem{\jythonHBMem} 	& \mem{\jythonWCPMem} 	& \mem{\jythonDCMem} 	& \mem{\jythonCAPOMem} 		& \mem{\jythonCAPOOPTMem} & \mem{\jythonCAPOOPTALTMem} \\
 \bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexTotalThreads	& (\luindexMaxLiveThreads)	& \mem{\luindexFTMem}	& \mem{\luindexHBMem} 	& \mem{\luindexWCPMem} 	& \mem{\luindexDCMem} 	& \mem{\luindexCAPOMem} 	& \mem{\luindexCAPOOPTMem} & \mem{\luindexCAPOOPTALTMem} \\
 \bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchTotalThreads	& (\lusearchMaxLiveThreads)	& \mem{\lusearchFTMem}	& \mem{\lusearchHBMem} 	& \mem{\lusearchWCPMem}	& \mem{\lusearchDCMem} 	& \mem{\lusearchCAPOMem}	& \mem{\lusearchCAPOOPTMem} & \mem{\lusearchCAPOOPTALTMem} \\
 \bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdTotalThreads	    & (\pmdMaxLiveThreads)	    & \mem{\pmdFTMem}	    & \mem{\pmdHBMem} 		& \mem{\pmdWCPMem} 		& \mem{\pmdDCMem} 		& \mem{\pmdCAPOMem} 		& \mem{\pmdCAPOOPTMem} & \mem{\pmdCAPOOPTALTMem} \\
 \bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowTotalThreads	& (\sunflowMaxLiveThreads)	& \mem{\sunflowFTMem}	& \mem{\sunflowHBMem}	& \mem{\sunflowWCPMem} 	& \mem{\sunflowDCMem} 	& \mem{\sunflowCAPOMem} 	& \mem{\sunflowCAPOOPTMem} & \mem{\sunflowCAPOOPTALTMem} \\
 \bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatTotalThreads	& (\tomcatMaxLiveThreads)	& \mem{\tomcatFTMem}	& \mem{\tomcatHBMem} 	& \mem{\tomcatWCPMem} 	& \mem{\tomcatDCMem} 	& \mem{\tomcatCAPOMem} 		& \mem{\tomcatCAPOOPTMem} & \mem{\tomcatCAPOOPTALTMem} \\
 \bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanTotalThreads	& (\xalanMaxLiveThreads)	& \mem{\xalanFTMem}	& \mem{\xalanHBMem} 		& \mem{\xalanWCPMem} 	& \mem{\xalanDCMem} 	& \mem{\xalanCAPOMem} 		& \mem{\xalanCAPOOPTMem} & \mem{\xalanCAPOOPTALTMem}
 \end{tabular}
 % \notes{
 % \jake{Raw results for all the tables and figures in
 % evaluation can be found here:
 % \url{http://cse-dcse101008d.cse.ohio-state.edu/exp-products/PIP\_test/}}
 % }
 \caption{Memory usage for \fasttool and other analysis
 configurations.
 All values are rounded to 2 significant figures.
 The text explains other values.} 
 %
 \label{tab:memory}
 \end{table*}
 
\begin{table*}[t]
\begin{adjustwidth}{-1.5cm}{}
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\input{result-macros/PIP_fastTool_raceEdgeAdd_lockCount}
%  
\small
\centering
\begin{tabular}{@{}l|rr|rr|rr|rr|rr|rr|rr@{}}
\et{}{} & \mc{14}{c@{}}{\FastTool Extra 3: Statically distinct races (dynamic races)}  \\
Program \et{Events}{\#Thr} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c|}{\CAPO-races} & \mc{2}{c|@{}}{\CAPO-Opt-races} & \mc{2}{c@{}}{Opt-Alt-races} \\\hline
\bench{avrora} 	\et{\avroraEvents}{\avroraThreads} 		& \avroraFT & (\avroraFTDynamic) 		& \avroraHB & (\avroraHBDynamic) 		& \avroraWCP & (\avroraWCPDynamic)		& \avroraWDC & (\avroraWDCDynamic) 		& \avroraCAPO & (\avroraCAPODynamic) 		& \avroraCAPOOPT & (\avroraCAPOOPTDynamic) 	& \avroraCAPOOPTALT & (\avroraCAPOOPTALTDynamic) \\
\bench{batik} 	\et{\batikEvents}{\batikThreads} 		& \batikFT & (\batikFTDynamic) 		& \batikHB & (\batikHBDynamic) 			& \batikWCP & (\batikWCPDynamic)		& \batikWDC & (\batikWDCDynamic)		& \batikCAPO & (\batikCAPODynamic)		& \batikCAPOOPT & (\batikCAPOOPTDynamic) 			& \batikCAPOOPTALT & (\batikCAPOOPTALTDynamic)\\
\bench{h2} 		\et{\htwoEvents}{\htwoThreads} 			& \htwoFT & (\htwoFTDynamic) 			& \htwoHB & (\htwoHBDynamic) 			& \htwoWCP & (\htwoWCPDynamic)			& \htwoWDC & (\htwoWDCDynamic)			& \htwoCAPO & (\htwoCAPODynamic)			& \htwoCAPOOPT & (\htwoCAPOOPTDynamic) 		& \htwoCAPOOPTALT & (\htwoCAPOOPTALTDynamic)\\
\bench{jython} 	\et{\jythonEvents}{\jythonThreads} 		& \jythonFT & (\jythonFTDynamic) 		& \jythonHB & (\jythonHBDynamic) 		& \jythonWCP & (\jythonWCPDynamic)		& \jythonWDC & (\jythonWDCDynamic)		& \jythonCAPO & (\jythonCAPODynamic)		& \jythonCAPOOPT & (\jythonCAPOOPTDynamic) 	& \jythonCAPOOPTALT & (\jythonCAPOOPTALTDynamic)\\
\bench{luindex} \et{\luindexEvents}{\luindexThreads} 	& \luindexFT & (\luindexFTDynamic) 	& \luindexHB & (\luindexHBDynamic) 		& \luindexWCP & (\luindexWCPDynamic)	& \luindexWDC & (\luindexWDCDynamic)	& \luindexCAPO & (\luindexCAPODynamic)	& \luindexCAPOOPT & (\luindexCAPOOPTDynamic) 		& \luindexCAPOOPTALT & (\luindexCAPOOPTALTDynamic)\\
\bench{lusearch}\et{\lusearchEvents}{\lusearchThreads}	& \lusearchFT & (\lusearchFTDynamic)	& \lusearchHB & (\lusearchHBDynamic)	& \lusearchWCP & (\lusearchWCPDynamic)	& \lusearchWDC & (\lusearchWDCDynamic)	& \lusearchCAPO & (\lusearchCAPODynamic)	& \lusearchCAPOOPT & (\lusearchCAPOOPTDynamic) & \lusearchCAPOOPTALT & (\lusearchCAPOOPTALTDynamic)\\
\bench{pmd} 	\et{\pmdEvents}{\pmdThreads} 			& \pmdFT & (\pmdFTDynamic) 			& \pmdHB & (\pmdHBDynamic) 				& \pmdWCP & (\pmdWCPDynamic)			& \pmdWDC & (\pmdWDCDynamic)			& \pmdCAPO & (\pmdCAPODynamic)			& \pmdCAPOOPT & (\pmdCAPOOPTDynamic) 				& \pmdCAPOOPTALT & (\pmdCAPOOPTALTDynamic)\\
\bench{sunflow} \et{\sunflowEvents}{\sunflowThreads} 	& \sunflowFT & (\sunflowFTDynamic) 	& \sunflowHB & (\sunflowHBDynamic) 		& \sunflowWCP & (\sunflowWCPDynamic)	& \sunflowWDC & (\sunflowWDCDynamic)	& \sunflowCAPO & (\sunflowCAPODynamic)	& \sunflowCAPOOPT & (\sunflowCAPOOPTDynamic) 		& \sunflowCAPOOPTALT & (\sunflowCAPOOPTALTDynamic)\\
\bench{tomcat} 	\et{\tomcatEvents}{\tomcatThreads} 		& \tomcatFT & (\tomcatFTDynamic) 		& \tomcatHB & (\tomcatHBDynamic) 		& \tomcatWCP & (\tomcatWCPDynamic)		& \tomcatWDC & (\tomcatWDCDynamic)		& \tomcatCAPO & (\tomcatCAPODynamic)		& \tomcatCAPOOPT & (\tomcatCAPOOPTDynamic) 	& \tomcatCAPOOPTALT & (\tomcatCAPOOPTALTDynamic)\\
\bench{xalan} 	\et{\xalanEvents}{\xalanThreads} 		& \xalanFT & (\xalanFTDynamic) 		& \xalanHB & (\xalanHBDynamic) 			& \xalanWCP & (\xalanWCPDynamic)		& \xalanWDC & (\xalanWDCDynamic)		& \xalanCAPO & (\xalanCAPODynamic)		& \xalanCAPOOPT & (\xalanCAPOOPTDynamic) 			& \xalanCAPOOPTALT & (\xalanCAPOOPTALTDynamic)\\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\input{result-macros/PIP_fastTool_shortestRaceEdge}
%  
\small
\centering
\begin{tabular}{@{}l|rr|rr|rr|rr|rr|rr|rr@{}}
\et{}{} & \mc{14}{c@{}}{\FastTool Extra 4: Statically distinct races (dynamic races)}  \\
Program \et{Events}{\#Thr} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c|}{\CAPO-races} & \mc{2}{c|@{}}{\CAPO-Opt-races} & \mc{2}{c@{}}{Opt-Alt-races} \\\hline
\bench{avrora} 	\et{\avroraEvents}{\avroraThreads} 		& \avroraFT & (\avroraFTDynamic) 		& \avroraHB & (\avroraHBDynamic) 		& \avroraWCP & (\avroraWCPDynamic)		& \avroraWDC & (\avroraWDCDynamic) 		& \avroraCAPO & (\avroraCAPODynamic) 		& \avroraCAPOOPT & (\avroraCAPOOPTDynamic) 	& \avroraCAPOOPTALT & (\avroraCAPOOPTALTDynamic) \\
\bench{batik} 	\et{\batikEvents}{\batikThreads} 		& \batikFT & (\batikFTDynamic) 		& \batikHB & (\batikHBDynamic) 			& \batikWCP & (\batikWCPDynamic)		& \batikWDC & (\batikWDCDynamic)		& \batikCAPO & (\batikCAPODynamic)		& \batikCAPOOPT & (\batikCAPOOPTDynamic) 			& \batikCAPOOPTALT & (\batikCAPOOPTALTDynamic)\\
\bench{h2} 		\et{\htwoEvents}{\htwoThreads} 			& \htwoFT & (\htwoFTDynamic) 			& \htwoHB & (\htwoHBDynamic) 			& \htwoWCP & (\htwoWCPDynamic)			& \htwoWDC & (\htwoWDCDynamic)			& \htwoCAPO & (\htwoCAPODynamic)			& \htwoCAPOOPT & (\htwoCAPOOPTDynamic) 		& \htwoCAPOOPTALT & (\htwoCAPOOPTALTDynamic)\\
\bench{jython} 	\et{\jythonEvents}{\jythonThreads} 		& \jythonFT & (\jythonFTDynamic) 		& \jythonHB & (\jythonHBDynamic) 		& \jythonWCP & (\jythonWCPDynamic)		& \jythonWDC & (\jythonWDCDynamic)		& \jythonCAPO & (\jythonCAPODynamic)		& \jythonCAPOOPT & (\jythonCAPOOPTDynamic) 	& \jythonCAPOOPTALT & (\jythonCAPOOPTALTDynamic)\\
\bench{luindex} \et{\luindexEvents}{\luindexThreads} 	& \luindexFT & (\luindexFTDynamic) 	& \luindexHB & (\luindexHBDynamic) 		& \luindexWCP & (\luindexWCPDynamic)	& \luindexWDC & (\luindexWDCDynamic)	& \luindexCAPO & (\luindexCAPODynamic)	& \luindexCAPOOPT & (\luindexCAPOOPTDynamic) 		& \luindexCAPOOPTALT & (\luindexCAPOOPTALTDynamic)\\
\bench{lusearch}\et{\lusearchEvents}{\lusearchThreads}	& \lusearchFT & (\lusearchFTDynamic)	& \lusearchHB & (\lusearchHBDynamic)	& \lusearchWCP & (\lusearchWCPDynamic)	& \lusearchWDC & (\lusearchWDCDynamic)	& \lusearchCAPO & (\lusearchCAPODynamic)	& \lusearchCAPOOPT & (\lusearchCAPOOPTDynamic) & \lusearchCAPOOPTALT & (\lusearchCAPOOPTALTDynamic)\\
\bench{pmd} 	\et{\pmdEvents}{\pmdThreads} 			& \pmdFT & (\pmdFTDynamic) 			& \pmdHB & (\pmdHBDynamic) 				& \pmdWCP & (\pmdWCPDynamic)			& \pmdWDC & (\pmdWDCDynamic)			& \pmdCAPO & (\pmdCAPODynamic)			& \pmdCAPOOPT & (\pmdCAPOOPTDynamic) 				& \pmdCAPOOPTALT & (\pmdCAPOOPTALTDynamic)\\
\bench{sunflow} \et{\sunflowEvents}{\sunflowThreads} 	& \sunflowFT & (\sunflowFTDynamic) 	& \sunflowHB & (\sunflowHBDynamic) 		& \sunflowWCP & (\sunflowWCPDynamic)	& \sunflowWDC & (\sunflowWDCDynamic)	& \sunflowCAPO & (\sunflowCAPODynamic)	& \sunflowCAPOOPT & (\sunflowCAPOOPTDynamic) 		& \sunflowCAPOOPTALT & (\sunflowCAPOOPTALTDynamic)\\
\bench{tomcat} 	\et{\tomcatEvents}{\tomcatThreads} 		& \tomcatFT & (\tomcatFTDynamic) 		& \tomcatHB & (\tomcatHBDynamic) 		& \tomcatWCP & (\tomcatWCPDynamic)		& \tomcatWDC & (\tomcatWDCDynamic)		& \tomcatCAPO & (\tomcatCAPODynamic)		& \tomcatCAPOOPT & (\tomcatCAPOOPTDynamic) 	& \tomcatCAPOOPTALT & (\tomcatCAPOOPTALTDynamic)\\
\bench{xalan} 	\et{\xalanEvents}{\xalanThreads} 		& \xalanFT & (\xalanFTDynamic) 		& \xalanHB & (\xalanHBDynamic) 			& \xalanWCP & (\xalanWCPDynamic)		& \xalanWDC & (\xalanWDCDynamic)		& \xalanCAPO & (\xalanCAPODynamic)		& \xalanCAPOOPT & (\xalanCAPOOPTDynamic) 			& \xalanCAPOOPTALT & (\xalanCAPOOPTALTDynamic)\\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\input{result-macros/PIP_fastTool_WCPFix}
%  
\small
\centering
\begin{tabular}{@{}l|rr|rr|rr|rr|rr|rr|rr@{}}
\et{}{} & \mc{14}{c@{}}{\FastTool Extra 5: Statically distinct races (dynamic races)}  \\
Program \et{Events}{\#Thr} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c|}{\CAPO-races} & \mc{2}{c|@{}}{\CAPO-Opt-races} & \mc{2}{c@{}}{Opt-Alt-races} \\\hline
\bench{avrora} 	\et{\avroraEvents}{\avroraThreads} 		& \avroraFT & (\avroraFTDynamic) 		& \avroraHB & (\avroraHBDynamic) 		& \avroraWCP & (\avroraWCPDynamic)		& \avroraWDC & (\avroraWDCDynamic) 		& \avroraCAPO & (\avroraCAPODynamic) 		& \avroraCAPOOPT & (\avroraCAPOOPTDynamic) 	& \avroraCAPOOPTALT & (\avroraCAPOOPTALTDynamic) \\
\bench{batik} 	\et{\batikEvents}{\batikThreads} 		& \batikFT & (\batikFTDynamic) 		& \batikHB & (\batikHBDynamic) 			& \batikWCP & (\batikWCPDynamic)		& \batikWDC & (\batikWDCDynamic)		& \batikCAPO & (\batikCAPODynamic)		& \batikCAPOOPT & (\batikCAPOOPTDynamic) 			& \batikCAPOOPTALT & (\batikCAPOOPTALTDynamic)\\
\bench{h2} 		\et{\htwoEvents}{\htwoThreads} 			& \htwoFT & (\htwoFTDynamic) 			& \htwoHB & (\htwoHBDynamic) 			& \htwoWCP & (\htwoWCPDynamic)			& \htwoWDC & (\htwoWDCDynamic)			& \htwoCAPO & (\htwoCAPODynamic)			& \htwoCAPOOPT & (\htwoCAPOOPTDynamic) 		& \htwoCAPOOPTALT & (\htwoCAPOOPTALTDynamic)\\
\bench{jython} 	\et{\jythonEvents}{\jythonThreads} 		& \jythonFT & (\jythonFTDynamic) 		& \jythonHB & (\jythonHBDynamic) 		& \jythonWCP & (\jythonWCPDynamic)		& \jythonWDC & (\jythonWDCDynamic)		& \jythonCAPO & (\jythonCAPODynamic)		& \jythonCAPOOPT & (\jythonCAPOOPTDynamic) 	& \jythonCAPOOPTALT & (\jythonCAPOOPTALTDynamic)\\
\bench{luindex} \et{\luindexEvents}{\luindexThreads} 	& \luindexFT & (\luindexFTDynamic) 	& \luindexHB & (\luindexHBDynamic) 		& \luindexWCP & (\luindexWCPDynamic)	& \luindexWDC & (\luindexWDCDynamic)	& \luindexCAPO & (\luindexCAPODynamic)	& \luindexCAPOOPT & (\luindexCAPOOPTDynamic) 		& \luindexCAPOOPTALT & (\luindexCAPOOPTALTDynamic)\\
\bench{lusearch}\et{\lusearchEvents}{\lusearchThreads}	& \lusearchFT & (\lusearchFTDynamic)	& \lusearchHB & (\lusearchHBDynamic)	& \lusearchWCP & (\lusearchWCPDynamic)	& \lusearchWDC & (\lusearchWDCDynamic)	& \lusearchCAPO & (\lusearchCAPODynamic)	& \lusearchCAPOOPT & (\lusearchCAPOOPTDynamic) & \lusearchCAPOOPTALT & (\lusearchCAPOOPTALTDynamic)\\
\bench{pmd} 	\et{\pmdEvents}{\pmdThreads} 			& \pmdFT & (\pmdFTDynamic) 			& \pmdHB & (\pmdHBDynamic) 				& \pmdWCP & (\pmdWCPDynamic)			& \pmdWDC & (\pmdWDCDynamic)			& \pmdCAPO & (\pmdCAPODynamic)			& \pmdCAPOOPT & (\pmdCAPOOPTDynamic) 				& \pmdCAPOOPTALT & (\pmdCAPOOPTALTDynamic)\\
\bench{sunflow} \et{\sunflowEvents}{\sunflowThreads} 	& \sunflowFT & (\sunflowFTDynamic) 	& \sunflowHB & (\sunflowHBDynamic) 		& \sunflowWCP & (\sunflowWCPDynamic)	& \sunflowWDC & (\sunflowWDCDynamic)	& \sunflowCAPO & (\sunflowCAPODynamic)	& \sunflowCAPOOPT & (\sunflowCAPOOPTDynamic) 		& \sunflowCAPOOPTALT & (\sunflowCAPOOPTALTDynamic)\\
\bench{tomcat} 	\et{\tomcatEvents}{\tomcatThreads} 		& \tomcatFT & (\tomcatFTDynamic) 		& \tomcatHB & (\tomcatHBDynamic) 		& \tomcatWCP & (\tomcatWCPDynamic)		& \tomcatWDC & (\tomcatWDCDynamic)		& \tomcatCAPO & (\tomcatCAPODynamic)		& \tomcatCAPOOPT & (\tomcatCAPOOPTDynamic) 	& \tomcatCAPOOPTALT & (\tomcatCAPOOPTALTDynamic)\\
\bench{xalan} 	\et{\xalanEvents}{\xalanThreads} 		& \xalanFT & (\xalanFTDynamic) 		& \xalanHB & (\xalanHBDynamic) 			& \xalanWCP & (\xalanWCPDynamic)		& \xalanWDC & (\xalanWDCDynamic)		& \xalanCAPO & (\xalanCAPODynamic)		& \xalanCAPOOPT & (\xalanCAPOOPTDynamic) 			& \xalanCAPOOPTALT & (\xalanCAPOOPTALTDynamic)\\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\caption{\FT-, \HB-, \WCP-, \DC-, \CAPO-, and \PIP-races detected by our implementation.
Each result is the average of 2 trials, rounded to the nearest integer.
Races are identified by field.}
 % Each result is from a single trial.}
\label{tab:coverage-dc}
\end{adjustwidth}
\end{table*}


\begin{table*}[t]
\begin{adjustwidth}{-1.5cm}{}
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\input{result-macros/PIP_fast_slow_eventCountCheck_fastTool}
%  
\small
\centering
\begin{tabular}{@{}l|rl|rr|rr|rr|rr|rr|rr|rr@{}}
& \mc{2}{c|}{} & \mc{14}{c@{}}{\FastTool fast slow eventCountCheck: Statically distinct races (dynamic races)}  \\
Program & \mc{2}{c|}{Events} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c|}{\CAPO-races} & \mc{2}{c|@{}}{\CAPO-Opt-races} & \mc{2}{c@{}}{Opt-Alt-races} \\\hline
\bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraFT & (\avroraFTDynamic) 		& \avroraHB & (\avroraHBDynamic) 		& \avroraWCP & (\avroraWCPDynamic)		& \avroraWDC & (\avroraWDCDynamic) 		& \avroraCAPO & (\avroraCAPODynamic) 		& \avroraCAPOOPT & (\avroraCAPOOPTDynamic) 	& \avroraCAPOOPTALT & (\avroraCAPOOPTALTDynamic) \\
\bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikFT & (\batikFTDynamic) 		& \batikHB & (\batikHBDynamic) 			& \batikWCP & (\batikWCPDynamic)		& \batikWDC & (\batikWDCDynamic)		& \batikCAPO & (\batikCAPODynamic)		& \batikCAPOOPT & (\batikCAPOOPTDynamic) 			& \batikCAPOOPTALT & (\batikCAPOOPTALTDynamic)\\
\bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoFT & (\htwoFTDynamic) 			& \htwoHB & (\htwoHBDynamic) 			& \htwoWCP & (\htwoWCPDynamic)			& \htwoWDC & (\htwoWDCDynamic)			& \htwoCAPO & (\htwoCAPODynamic)			& \htwoCAPOOPT & (\htwoCAPOOPTDynamic) 		& \htwoCAPOOPTALT & (\htwoCAPOOPTALTDynamic)\\
\bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonFT & (\jythonFTDynamic) 		& \jythonHB & (\jythonHBDynamic) 		& \jythonWCP & (\jythonWCPDynamic)		& \jythonWDC & (\jythonWDCDynamic)		& \jythonCAPO & (\jythonCAPODynamic)		& \jythonCAPOOPT & (\jythonCAPOOPTDynamic) 	& \jythonCAPOOPTALT & (\jythonCAPOOPTALTDynamic)\\
\bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexFT & (\luindexFTDynamic) 	& \luindexHB & (\luindexHBDynamic) 		& \luindexWCP & (\luindexWCPDynamic)	& \luindexWDC & (\luindexWDCDynamic)	& \luindexCAPO & (\luindexCAPODynamic)	& \luindexCAPOOPT & (\luindexCAPOOPTDynamic) 		& \luindexCAPOOPTALT & (\luindexCAPOOPTALTDynamic)\\
\bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchFT & (\lusearchFTDynamic)	& \lusearchHB & (\lusearchHBDynamic)	& \lusearchWCP & (\lusearchWCPDynamic)	& \lusearchWDC & (\lusearchWDCDynamic)	& \lusearchCAPO & (\lusearchCAPODynamic)	& \lusearchCAPOOPT & (\lusearchCAPOOPTDynamic) & \lusearchCAPOOPTALT & (\lusearchCAPOOPTALTDynamic)\\
\bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdFT & (\pmdFTDynamic) 			& \pmdHB & (\pmdHBDynamic) 				& \pmdWCP & (\pmdWCPDynamic)			& \pmdWDC & (\pmdWDCDynamic)			& \pmdCAPO & (\pmdCAPODynamic)			& \pmdCAPOOPT & (\pmdCAPOOPTDynamic) 				& \pmdCAPOOPTALT & (\pmdCAPOOPTALTDynamic)\\
\bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowFT & (\sunflowFTDynamic) 	& \sunflowHB & (\sunflowHBDynamic) 		& \sunflowWCP & (\sunflowWCPDynamic)	& \sunflowWDC & (\sunflowWDCDynamic)	& \sunflowCAPO & (\sunflowCAPODynamic)	& \sunflowCAPOOPT & (\sunflowCAPOOPTDynamic) 		& \sunflowCAPOOPTALT & (\sunflowCAPOOPTALTDynamic)\\
\bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatFT & (\tomcatFTDynamic) 		& \tomcatHB & (\tomcatHBDynamic) 		& \tomcatWCP & (\tomcatWCPDynamic)		& \tomcatWDC & (\tomcatWDCDynamic)		& \tomcatCAPO & (\tomcatCAPODynamic)		& \tomcatCAPOOPT & (\tomcatCAPOOPTDynamic) 	& \tomcatCAPOOPTALT & (\tomcatCAPOOPTALTDynamic)\\
\bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanFT & (\xalanFTDynamic) 		& \xalanHB & (\xalanHBDynamic) 			& \xalanWCP & (\xalanWCPDynamic)		& \xalanWDC & (\xalanWDCDynamic)		& \xalanCAPO & (\xalanCAPODynamic)		& \xalanCAPOOPT & (\xalanCAPOOPTDynamic) 			& \xalanCAPOOPTALT & (\xalanCAPOOPTALTDynamic)\\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\input{result-macros/PIP_fast_slow_eventCountCheck_slowTool}
%  
\small
\centering
\begin{tabular}{@{}l|rl|rr|rr|rr|rr|rr|rr|rr@{}}
& \mc{2}{c|}{} & \mc{14}{c@{}}{\SlowTool fast slow eventCountCheck: Statically distinct races (dynamic races)}  \\
Program & \mc{2}{c|}{Events} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} \\\hline
\bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraFT & (\avroraFTDynamic)		& \avroraHB & (\avroraHBDynamic) 		& \avroraWCP & (\avroraWCPDynamic)		& \avroraWDC & (\avroraWDCDynamic) \\
\bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikFT & (\batikFTDynamic)			& \batikHB & (\batikHBDynamic) 			& \batikWCP & (\batikWCPDynamic)		& \batikWDC & (\batikWDCDynamic) \\
\bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoFT & (\htwoFTDynamic)			& \htwoHB & (\htwoHBDynamic) 			& \htwoWCP & (\htwoWCPDynamic)			& \htwoWDC & (\htwoWDCDynamic) \\
\bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonFT & (\jythonFTDynamic)		& \jythonHB & (\jythonHBDynamic) 		& \jythonWCP & (\jythonWCPDynamic)		& \jythonWDC & (\jythonWDCDynamic) \\
\bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexFT & (\luindexFTDynamic)		& \luindexHB & (\luindexHBDynamic) 		& \luindexWCP & (\luindexWCPDynamic)	& \luindexWDC & (\luindexWDCDynamic) \\
\bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchFT & (\lusearchFTDynamic)	& \lusearchHB & (\lusearchHBDynamic)	& \lusearchWCP & (\lusearchWCPDynamic)	& \lusearchWDC & (\lusearchWDCDynamic) \\
\bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdFT & (\pmdFTDynamic)				& \pmdHB & (\pmdHBDynamic) 				& \pmdWCP & (\pmdWCPDynamic)			& \pmdWDC & (\pmdWDCDynamic) \\
\bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowFT & (\sunflowFTDynamic)		& \sunflowHB & (\sunflowHBDynamic) 		& \sunflowWCP & (\sunflowWCPDynamic)	& \sunflowWDC & (\sunflowWDCDynamic) \\
\bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatFT & (\tomcatFTDynamic)		& \tomcatHB & (\tomcatHBDynamic) 		& \tomcatWCP & (\tomcatWCPDynamic)		& \tomcatWDC & (\tomcatWDCDynamic) \\
\bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanFT & (\xalanFTDynamic)			& \xalanHB & (\xalanHBDynamic) 			& \xalanWCP & (\xalanWCPDynamic)		& \xalanWDC & (\xalanWDCDynamic) \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\caption{\FT-, \HB-, \WCP-, \DC-, \CAPO-, and \PIP-races detected by our implementation.
Each result is the average of 2 trials, rounded to the nearest integer.
Races are identified by field.}
 % Each result is from a single trial.}
\label{tab:coverage-dc}
\end{adjustwidth}
\end{table*}

\begin{table*}[t]
\begin{adjustwidth}{-1.5cm}{}
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\newcommand{\ci}[1]{\ensuremath{\pm{\;}#1}}
\newcommand{\ciRange}[2]{(#1--#2)}
\input{result-macros/PIP_slowTool_latestRaceHBTest}
%  
\small
\centering
\begin{tabular}{@{}l|rlr|rlr|rlr|rlr@{}}
\et{}{} & \mc{12}{c@{}}{\SlowTool lastestRaceHBTest: Statically distinct races (dynamic races)}  \\
Program \et{Events}{\#Thr} & \mc{3}{c|}{\HB w/o G w/o REdge-races} & \mc{3}{c|}{\HB w/G w/o REdge-races} & \mc{3}{c|}{\HB w/o G w/ REdge-races} & \mc{3}{c}{\HB w/ G w/ REdge-races} \\\hline
\bench{avrora} 	\et{\avroraEvents}{\avroraThreads} 		& \avroraHB & \ci{\avroraHBCI} 		& \ciRange{\avroraHBDynamicCIMIN}{\avroraHBDynamicCIMAX}	& \avroraHBwG & \ci{\avroraHBwGCI} 		& \ciRange{\avroraHBwGDynamicCIMIN}{\avroraHBwGDynamicCIMAX}	& \avroraHBnoGwRaceEdge & \ci{\avroraHBnoGwRaceEdgeCI} 		& \ciRange{\avroraHBnoGwRaceEdgeDynamicCIMIN}{\avroraHBnoGwRaceEdgeDynamicCIMAX}	& \avroraHBwRaceEdge & \ci{\avroraHBwRaceEdgeCI} 	& \ciRange{\avroraHBwRaceEdgeDynamicCIMIN}{\avroraHBwRaceEdgeDynamicCIMAX} \\
\bench{batik} 	\et{\batikEvents}{\batikThreads} 		& \batikHB & \ci{\batikHBCI} 		& \ciRange{\batikHBDynamicCIMIN}{\batikHBDynamicCIMAX} 		& \batikHBwG & \ci{\batikHBwGCI} 		& \ciRange{\batikHBwGDynamicCIMIN}{\batikHBwGDynamicCIMAX} 		& \batikHBnoGwRaceEdge & \ci{\batikHBnoGwRaceEdgeCI} 		& \ciRange{\batikHBnoGwRaceEdgeDynamicCIMIN}{\batikHBnoGwRaceEdgeDynamicCIMAX}		& \batikHBwRaceEdge & \ci{\batikHBwRaceEdgeCI} 		& \ciRange{\batikHBwRaceEdgeDynamicCIMIN}{\batikHBwRaceEdgeDynamicCIMAX} \\
\bench{h2} 		\et{\htwoEvents}{\htwoThreads} 			& \htwoHB & \ci{\htwoHBCI} 			& \ciRange{\htwoHBDynamicCIMIN}{\htwoHBDynamicCIMAX}		& \htwoHBwG & \ci{\htwoHBwGCI} 			& \ciRange{\htwoHBwGDynamicCIMIN}{\htwoHBwGDynamicCIMAX} 		& \htwoHBnoGwRaceEdge & \ci{\htwoHBnoGwRaceEdgeCI} 			& \ciRange{\htwoHBnoGwRaceEdgeDynamicCIMIN}{\htwoHBnoGwRaceEdgeDynamicCIMAX}		& \htwoHBwRaceEdge & \ci{\htwoHBwRaceEdgeCI} 		& \ciRange{\htwoHBwRaceEdgeDynamicCIMIN}{\htwoHBwRaceEdgeDynamicCIMAX} \\
\bench{jython} 	\et{\jythonEvents}{\jythonThreads} 		& \jythonHB & \ci{\jythonHBCI} 		& \ciRange{\jythonHBDynamicCIMIN}{\jythonHBDynamicCIMAX}	& \jythonHBwG & \ci{\jythonHBwGCI} 		& \ciRange{\jythonHBwGDynamicCIMIN}{\jythonHBwGDynamicCIMAX} 	& \jythonHBnoGwRaceEdge & \ci{\jythonHBnoGwRaceEdgeCI} 		& \ciRange{\jythonHBnoGwRaceEdgeDynamicCIMIN}{\jythonHBnoGwRaceEdgeDynamicCIMAX} 	& \jythonHBwRaceEdge & \ci{\jythonHBwRaceEdgeCI} 	& \ciRange{\jythonHBwRaceEdgeDynamicCIMIN}{\jythonHBwRaceEdgeDynamicCIMAX} \\
\bench{luindex} \et{\luindexEvents}{\luindexThreads} 	& \luindexHB & \ci{\luindexHBCI} 	& \ciRange{\luindexHBDynamicCIMIN}{\luindexHBDynamicCIMAX}	& \luindexHBwG & \ci{\luindexHBwGCI} 	& \ciRange{\luindexHBwGDynamicCIMIN}{\luindexHBwGDynamicCIMAX} 	& \luindexHBnoGwRaceEdge & \ci{\luindexHBnoGwRaceEdgeCI} 	& \ciRange{\luindexHBnoGwRaceEdgeDynamicCIMIN}{\luindexHBnoGwRaceEdgeDynamicCIMAX} 	& \luindexHBwRaceEdge & \ci{\luindexHBwRaceEdgeCI} 	& \ciRange{\luindexHBwRaceEdgeDynamicCIMIN}{\luindexHBwRaceEdgeDynamicCIMAX} \\
\bench{lusearch}\et{\lusearchEvents}{\lusearchThreads}	& \lusearchHB & \ci{\lusearchHBCI} 	& \ciRange{\lusearchHBDynamicCIMIN}{\lusearchHBDynamicCIMAX}& \lusearchHBwG & \ci{\lusearchHBwGCI} 	& \ciRange{\lusearchHBwGDynamicCIMIN}{\lusearchHBwGDynamicCIMAX}& \lusearchHBnoGwRaceEdge & \ci{\lusearchHBnoGwRaceEdgeCI} 	& \ciRange{\lusearchHBnoGwRaceEdgeDynamicCIMIN}{\lusearchHBnoGwRaceEdgeDynamicCIMAX}& \lusearchHBwRaceEdge & \ci{\lusearchHBwRaceEdgeCI}& \ciRange{\lusearchHBwRaceEdgeDynamicCIMIN}{\lusearchHBwRaceEdgeDynamicCIMAX} \\
\bench{pmd} 	\et{\pmdEvents}{\pmdThreads} 			& \pmdHB & \ci{\pmdHBCI} 			& \ciRange{\pmdHBDynamicCIMIN}{\pmdHBDynamicCIMAX}			& \pmdHBwG & \ci{\pmdHBwGCI} 			& \ciRange{\pmdHBwGDynamicCIMIN}{\pmdHBwGDynamicCIMAX} 			& \pmdHBnoGwRaceEdge & \ci{\pmdHBnoGwRaceEdgeCI}	 		& \ciRange{\pmdHBnoGwRaceEdgeDynamicCIMIN}{\pmdHBnoGwRaceEdgeDynamicCIMAX} 			& \pmdHBwRaceEdge & \ci{\pmdHBwRaceEdgeCI}	 		& \ciRange{\pmdHBwRaceEdgeDynamicCIMIN}{\pmdHBwRaceEdgeDynamicCIMAX} \\
\bench{sunflow} \et{\sunflowEvents}{\sunflowThreads} 	& \sunflowHB & \ci{\sunflowHBCI} 	& \ciRange{\sunflowHBDynamicCIMIN}{\sunflowHBDynamicCIMAX} 	& \sunflowHBwG & \ci{\sunflowHBwGCI} 	& \ciRange{\sunflowHBwGDynamicCIMIN}{\sunflowHBwGDynamicCIMAX} 	& \sunflowHBnoGwRaceEdge & \ci{\sunflowHBnoGwRaceEdgeCI} 	& \ciRange{\sunflowHBnoGwRaceEdgeDynamicCIMIN}{\sunflowHBnoGwRaceEdgeDynamicCIMAX} 	& \sunflowHBwRaceEdge & \ci{\sunflowHBwRaceEdgeCI} 	& \ciRange{\sunflowHBwRaceEdgeDynamicCIMIN}{\sunflowHBwRaceEdgeDynamicCIMAX} \\
\bench{tomcat} 	\et{\tomcatEvents}{\tomcatThreads} 		& \tomcatHB & \ci{\tomcatHBCI} 		& \ciRange{\tomcatHBDynamicCIMIN}{\tomcatHBDynamicCIMAX}	& \tomcatHBwG & \ci{\tomcatHBwGCI} 		& \ciRange{\tomcatHBwGDynamicCIMIN}{\tomcatHBwGDynamicCIMAX} 	& \tomcatHBnoGwRaceEdge & \ci{\tomcatHBnoGwRaceEdgeCI} 		& \ciRange{\tomcatHBnoGwRaceEdgeDynamicCIMIN}{\tomcatHBnoGwRaceEdgeDynamicCIMAX} 	& \tomcatHBwRaceEdge & \ci{\tomcatHBwRaceEdgeCI} 	& \ciRange{\tomcatHBwRaceEdgeDynamicCIMIN}{\tomcatHBwRaceEdgeDynamicCIMAX} \\
\bench{xalan} 	\et{\xalanEvents}{\xalanThreads} 		& \xalanHB & \ci{\xalanHBCI} 		& \ciRange{\xalanHBDynamicCIMIN}{\xalanHBDynamicCIMAX}		& \xalanHBwG & \ci{\xalanHBwGCI} 		& \ciRange{\xalanHBwGDynamicCIMIN}{\xalanHBwGDynamicCIMAX} 		& \xalanHBnoGwRaceEdge & \ci{\xalanHBnoGwRaceEdgeCI} 		& \ciRange{\xalanHBnoGwRaceEdgeDynamicCIMIN}{\xalanHBnoGwRaceEdgeDynamicCIMAX} 		& \xalanHBwRaceEdge & \ci{\xalanHBwRaceEdgeCI} 		& \ciRange{\xalanHBwRaceEdgeDynamicCIMIN}{\xalanHBwRaceEdgeDynamicCIMAX} \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\caption{\FT-, \HB-, \WCP-, \DC-, \CAPO-, and \PIP-races detected by our implementation.
Each result is the average of 2 trials, rounded to the nearest integer.
Races are identified by field.}
 % Each result is from a single trial.}
\label{tab:coverage-dc}
\end{adjustwidth}
\end{table*}

\begin{table*}[t]
\begin{adjustwidth}{-1.5cm}{}
\begin{minipage}{0.5\textwidth}
\newcommand\DCwoG{\DC}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_fastTool_raceCountEnabled}

\small
\centering
\begin{tabular}{@{}l|rl|rl||r|rrrrrrrrr}
& \mc{2}{c|}{} & \mc{2}{c||}{} & Base & \mc{8}{c}{\FastTool raceCountEnabled: Slowdown (normalized to Base time)} \\
Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & time & Empty & \FT & \HB & \WCP & \DC & \CAPO & \CAPO-Opt & \CAPO-Opt-Alt \\\hline 
\bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraTotalThreads 	& (\avroraMaxLiveThreads)	& \base{\avroraBaseTime}   & \roh{\avroraEmptyTime}   & \roh{\avroraFTTime}   & \roh{\avroraHBTime}   & \roh{\avroraWCPTime}   & \roh{\avroraDCTime} 	& \roh{\avroraCAPOTime} 	& \roh{\avroraCAPOOPTTime} & \roh{\avroraCAPOOPTALTTime} \\
\bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikTotalThreads 	& (\batikMaxLiveThreads)	& \base{\batikBaseTime}    & \roh{\batikEmptyTime}    & \roh{\batikFTTime}    & \roh{\batikHBTime}    & \roh{\batikWCPTime}    & \roh{\batikDCTime}    & \roh{\batikCAPOTime} 		& \roh{\batikCAPOOPTTime} & \roh{\batikCAPOOPTALTTime} \\
\bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoTotalThreads 	& (\htwoMaxLiveThreads)	    & \base{\htwoBaseTime}     & \roh{\htwoEmptyTime}     & \roh{\htwoFTTime}     & \roh{\htwoHBTime}     & \roh{\htwoWCPTime}     & \roh{\htwoDCTime}     & \roh{\htwoCAPOTime} 		& \roh{\htwoCAPOOPTTime} & \roh{\htwoCAPOOPTALTTime} \\
\bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonTotalThreads	& (\jythonMaxLiveThreads)	& \base{\jythonBaseTime}   & \roh{\jythonEmptyTime}   & \roh{\jythonFTTime}   & \roh{\jythonHBTime} 	 & \roh{\jythonWCPTime}   & \roh{\jythonDCTime} 	 & \roh{\jythonCAPOTime} 	& \roh{\jythonCAPOOPTTime} & \roh{\jythonCAPOOPTALTTime} \\
\bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexTotalThreads	& (\luindexMaxLiveThreads)	& \base{\luindexBaseTime}  & \roh{\luindexEmptyTime}  & \roh{\luindexFTTime}  & \roh{\luindexHBTime}  & \roh{\luindexWCPTime}  & \roh{\luindexDCTime}  & \roh{\luindexCAPOTime} 	& \roh{\luindexCAPOOPTTime} & \roh{\luindexCAPOOPTALTTime} \\
\bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchTotalThreads	& (\lusearchMaxLiveThreads)	& \base{\lusearchBaseTime} & \roh{\lusearchEmptyTime} & \roh{\lusearchFTTime} & \roh{\lusearchHBTime} & \roh{\lusearchWCPTime} & \roh{\lusearchDCTime} & \roh{\lusearchCAPOTime}	& \roh{\lusearchCAPOOPTTime} & \roh{\lusearchCAPOOPTALTTime} \\
\bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdTotalThreads	    & (\pmdMaxLiveThreads)	    & \base{\pmdBaseTime}      & \roh{\pmdEmptyTime}      & \roh{\pmdFTTime}      & \roh{\pmdHBTime}      & \roh{\pmdWCPTime}      & \roh{\pmdDCTime}	     & \roh{\pmdCAPOTime} 		& \roh{\pmdCAPOOPTTime} & \roh{\pmdCAPOOPTALTTime} \\
\bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowTotalThreads	& (\sunflowMaxLiveThreads)	& \base{\sunflowBaseTime}  & \roh{\sunflowEmptyTime}  & \roh{\sunflowFTTime}  & \roh{\sunflowHBTime}	 & \roh{\sunflowWCPTime}  & \roh{\sunflowDCTime}  & \roh{\sunflowCAPOTime} 	& \roh{\sunflowCAPOOPTTime} & \roh{\sunflowCAPOOPTALTTime} \\
\bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatTotalThreads	& (\tomcatMaxLiveThreads)	& \base{\tomcatBaseTime}   & \roh{\tomcatEmptyTime}   & \roh{\tomcatFTTime}   & \roh{\tomcatHBTime} 	 & \roh{\tomcatWCPTime}   & \roh{\tomcatDCTime}   & \roh{\tomcatCAPOTime} 	& \roh{\tomcatCAPOOPTTime} & \roh{\tomcatCAPOOPTALTTime} \\
\bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanTotalThreads	& (\xalanMaxLiveThreads)	& \base{\xalanBaseTime}    & \roh{\xalanEmptyTime}    & \roh{\xalanFTTime}    & \roh{\xalanHBTime}    & \roh{\xalanWCPTime}    & \roh{\xalanDCTime}    & \roh{\xalanCAPOTime} 		& \roh{\xalanCAPOOPTTime} & \roh{\xalanCAPOOPTALTTime} 
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{0.5\textwidth}
\newcommand\DCwoG{\DC}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_fastTool_raceCountCost}

\small
\centering
\begin{tabular}{@{}l|rl|rl||r|rrrrrrrrr}
& \mc{2}{c|}{} & \mc{2}{c||}{} & Base & \mc{8}{c}{\FastTool raceCountCost [disable race counting]: Slowdown (normalized to Base time)} \\
Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & time & Empty & \FT & \HB & \WCP & \DC & \CAPO & \CAPO-Opt & \CAPO-Opt-Alt \\\hline 
\bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraTotalThreads 	& (\avroraMaxLiveThreads)	& \base{\avroraBaseTime}   & \roh{\avroraEmptyTime}   & \roh{\avroraFTTime}   & \roh{\avroraHBTime}   & \roh{\avroraWCPTime}   & \roh{\avroraDCTime} 	& \roh{\avroraCAPOTime} 	& \roh{\avroraCAPOOPTTime} & \roh{\avroraCAPOOPTALTTime} \\
\bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikTotalThreads 	& (\batikMaxLiveThreads)	& \base{\batikBaseTime}    & \roh{\batikEmptyTime}    & \roh{\batikFTTime}    & \roh{\batikHBTime}    & \roh{\batikWCPTime}    & \roh{\batikDCTime}    & \roh{\batikCAPOTime} 		& \roh{\batikCAPOOPTTime} & \roh{\batikCAPOOPTALTTime} \\
\bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoTotalThreads 	& (\htwoMaxLiveThreads)	    & \base{\htwoBaseTime}     & \roh{\htwoEmptyTime}     & \roh{\htwoFTTime}     & \roh{\htwoHBTime}     & \roh{\htwoWCPTime}     & \roh{\htwoDCTime}     & \roh{\htwoCAPOTime} 		& \roh{\htwoCAPOOPTTime} & \roh{\htwoCAPOOPTALTTime} \\
\bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonTotalThreads	& (\jythonMaxLiveThreads)	& \base{\jythonBaseTime}   & \roh{\jythonEmptyTime}   & \roh{\jythonFTTime}   & \roh{\jythonHBTime} 	 & \roh{\jythonWCPTime}   & \roh{\jythonDCTime} 	 & \roh{\jythonCAPOTime} 	& \roh{\jythonCAPOOPTTime} & \roh{\jythonCAPOOPTALTTime} \\
\bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexTotalThreads	& (\luindexMaxLiveThreads)	& \base{\luindexBaseTime}  & \roh{\luindexEmptyTime}  & \roh{\luindexFTTime}  & \roh{\luindexHBTime}  & \roh{\luindexWCPTime}  & \roh{\luindexDCTime}  & \roh{\luindexCAPOTime} 	& \roh{\luindexCAPOOPTTime} & \roh{\luindexCAPOOPTALTTime} \\
\bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchTotalThreads	& (\lusearchMaxLiveThreads)	& \base{\lusearchBaseTime} & \roh{\lusearchEmptyTime} & \roh{\lusearchFTTime} & \roh{\lusearchHBTime} & \roh{\lusearchWCPTime} & \roh{\lusearchDCTime} & \roh{\lusearchCAPOTime}	& \roh{\lusearchCAPOOPTTime} & \roh{\lusearchCAPOOPTALTTime} \\
\bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdTotalThreads	    & (\pmdMaxLiveThreads)	    & \base{\pmdBaseTime}      & \roh{\pmdEmptyTime}      & \roh{\pmdFTTime}      & \roh{\pmdHBTime}      & \roh{\pmdWCPTime}      & \roh{\pmdDCTime}	     & \roh{\pmdCAPOTime} 		& \roh{\pmdCAPOOPTTime} & \roh{\pmdCAPOOPTALTTime} \\
\bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowTotalThreads	& (\sunflowMaxLiveThreads)	& \base{\sunflowBaseTime}  & \roh{\sunflowEmptyTime}  & \roh{\sunflowFTTime}  & \roh{\sunflowHBTime}	 & \roh{\sunflowWCPTime}  & \roh{\sunflowDCTime}  & \roh{\sunflowCAPOTime} 	& \roh{\sunflowCAPOOPTTime} & \roh{\sunflowCAPOOPTALTTime} \\
\bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatTotalThreads	& (\tomcatMaxLiveThreads)	& \base{\tomcatBaseTime}   & \roh{\tomcatEmptyTime}   & \roh{\tomcatFTTime}   & \roh{\tomcatHBTime} 	 & \roh{\tomcatWCPTime}   & \roh{\tomcatDCTime}   & \roh{\tomcatCAPOTime} 	& \roh{\tomcatCAPOOPTTime} & \roh{\tomcatCAPOOPTALTTime} \\
\bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanTotalThreads	& (\xalanMaxLiveThreads)	& \base{\xalanBaseTime}    & \roh{\xalanEmptyTime}    & \roh{\xalanFTTime}    & \roh{\xalanHBTime}    & \roh{\xalanWCPTime}    & \roh{\xalanDCTime}    & \roh{\xalanCAPOTime} 		& \roh{\xalanCAPOOPTTime} & \roh{\xalanCAPOOPTALTTime} 
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{0.5\textwidth}
\newcommand\DCwoG{\DC}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_fastTool_EpochRaceCheck}

\small
\centering
\begin{tabular}{@{}l|rl|rl||r|rrrrrrrrr}
& \mc{2}{c|}{} & \mc{2}{c||}{} & Base & \mc{8}{c}{\FastTool EpochRaceCheck: Slowdown (normalized to Base time)} \\
Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & time & Empty & \FT & \HB & \WCP & \DC & \CAPO & \CAPO-Opt & \CAPO-Opt-Alt \\\hline 
\bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraTotalThreads 	& (\avroraMaxLiveThreads)	& \base{\avroraBaseTime}   & \roh{\avroraEmptyTime}   & \roh{\avroraFTTime}   & \roh{\avroraHBTime}   & \roh{\avroraWCPTime}   & \roh{\avroraDCTime} 	& \roh{\avroraCAPOTime} 	& \roh{\avroraCAPOOPTTime} & \roh{\avroraCAPOOPTALTTime} \\
\bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikTotalThreads 	& (\batikMaxLiveThreads)	& \base{\batikBaseTime}    & \roh{\batikEmptyTime}    & \roh{\batikFTTime}    & \roh{\batikHBTime}    & \roh{\batikWCPTime}    & \roh{\batikDCTime}    & \roh{\batikCAPOTime} 		& \roh{\batikCAPOOPTTime} & \roh{\batikCAPOOPTALTTime} \\
\bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoTotalThreads 	& (\htwoMaxLiveThreads)	    & \base{\htwoBaseTime}     & \roh{\htwoEmptyTime}     & \roh{\htwoFTTime}     & \roh{\htwoHBTime}     & \roh{\htwoWCPTime}     & \roh{\htwoDCTime}     & \roh{\htwoCAPOTime} 		& \roh{\htwoCAPOOPTTime} & \roh{\htwoCAPOOPTALTTime} \\
\bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonTotalThreads	& (\jythonMaxLiveThreads)	& \base{\jythonBaseTime}   & \roh{\jythonEmptyTime}   & \roh{\jythonFTTime}   & \roh{\jythonHBTime} 	 & \roh{\jythonWCPTime}   & \roh{\jythonDCTime} 	 & \roh{\jythonCAPOTime} 	& \roh{\jythonCAPOOPTTime} & \roh{\jythonCAPOOPTALTTime} \\
\bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexTotalThreads	& (\luindexMaxLiveThreads)	& \base{\luindexBaseTime}  & \roh{\luindexEmptyTime}  & \roh{\luindexFTTime}  & \roh{\luindexHBTime}  & \roh{\luindexWCPTime}  & \roh{\luindexDCTime}  & \roh{\luindexCAPOTime} 	& \roh{\luindexCAPOOPTTime} & \roh{\luindexCAPOOPTALTTime} \\
\bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchTotalThreads	& (\lusearchMaxLiveThreads)	& \base{\lusearchBaseTime} & \roh{\lusearchEmptyTime} & \roh{\lusearchFTTime} & \roh{\lusearchHBTime} & \roh{\lusearchWCPTime} & \roh{\lusearchDCTime} & \roh{\lusearchCAPOTime}	& \roh{\lusearchCAPOOPTTime} & \roh{\lusearchCAPOOPTALTTime} \\
\bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdTotalThreads	    & (\pmdMaxLiveThreads)	    & \base{\pmdBaseTime}      & \roh{\pmdEmptyTime}      & \roh{\pmdFTTime}      & \roh{\pmdHBTime}      & \roh{\pmdWCPTime}      & \roh{\pmdDCTime}	     & \roh{\pmdCAPOTime} 		& \roh{\pmdCAPOOPTTime} & \roh{\pmdCAPOOPTALTTime} \\
\bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowTotalThreads	& (\sunflowMaxLiveThreads)	& \base{\sunflowBaseTime}  & \roh{\sunflowEmptyTime}  & \roh{\sunflowFTTime}  & \roh{\sunflowHBTime}	 & \roh{\sunflowWCPTime}  & \roh{\sunflowDCTime}  & \roh{\sunflowCAPOTime} 	& \roh{\sunflowCAPOOPTTime} & \roh{\sunflowCAPOOPTALTTime} \\
\bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatTotalThreads	& (\tomcatMaxLiveThreads)	& \base{\tomcatBaseTime}   & \roh{\tomcatEmptyTime}   & \roh{\tomcatFTTime}   & \roh{\tomcatHBTime} 	 & \roh{\tomcatWCPTime}   & \roh{\tomcatDCTime}   & \roh{\tomcatCAPOTime} 	& \roh{\tomcatCAPOOPTTime} & \roh{\tomcatCAPOOPTALTTime} \\
\bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanTotalThreads	& (\xalanMaxLiveThreads)	& \base{\xalanBaseTime}    & \roh{\xalanEmptyTime}    & \roh{\xalanFTTime}    & \roh{\xalanHBTime}    & \roh{\xalanWCPTime}    & \roh{\xalanDCTime}    & \roh{\xalanCAPOTime} 		& \roh{\xalanCAPOOPTTime} & \roh{\xalanCAPOOPTALTTime} 
\end{tabular}
\end{minipage}
\caption{Run time for \fasttool and other analysis
configurations.} 
%
\label{tab:performance}
\end{adjustwidth}
\end{table*}

\begin{table*}[t]
\begin{adjustwidth}{-1.5cm}{}
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\input{result-macros/PIP_fastTool_WCPFix}
%  
\small
\centering
\begin{tabular}{@{}l|rl|rr|rr|rr|rr|rr|rr|rr@{}}
& \mc{2}{c|}{} & \mc{14}{c@{}}{\FastTool WCPFix: Statically distinct races (dynamic races)}  \\
Program & \mc{2}{c|}{Events} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c|}{\CAPO-races} & \mc{2}{c|@{}}{\CAPO-Opt-races} & \mc{2}{c@{}}{Opt-Alt-races} \\\hline
\bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraFT & (\avroraFTDynamic) 		& \avroraHB & (\avroraHBDynamic) 		& \avroraWCP & (\avroraWCPDynamic)		& \avroraWDC & (\avroraWDCDynamic) 		& \avroraCAPO & (\avroraCAPODynamic) 		& \avroraCAPOOPT & (\avroraCAPOOPTDynamic) 	& \avroraCAPOOPTALT & (\avroraCAPOOPTALTDynamic) \\
\bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikFT & (\batikFTDynamic) 		& \batikHB & (\batikHBDynamic) 			& \batikWCP & (\batikWCPDynamic)		& \batikWDC & (\batikWDCDynamic)		& \batikCAPO & (\batikCAPODynamic)		& \batikCAPOOPT & (\batikCAPOOPTDynamic) 			& \batikCAPOOPTALT & (\batikCAPOOPTALTDynamic)\\
\bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoFT & (\htwoFTDynamic) 			& \htwoHB & (\htwoHBDynamic) 			& \htwoWCP & (\htwoWCPDynamic)			& \htwoWDC & (\htwoWDCDynamic)			& \htwoCAPO & (\htwoCAPODynamic)			& \htwoCAPOOPT & (\htwoCAPOOPTDynamic) 		& \htwoCAPOOPTALT & (\htwoCAPOOPTALTDynamic)\\
\bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonFT & (\jythonFTDynamic) 		& \jythonHB & (\jythonHBDynamic) 		& \jythonWCP & (\jythonWCPDynamic)		& \jythonWDC & (\jythonWDCDynamic)		& \jythonCAPO & (\jythonCAPODynamic)		& \jythonCAPOOPT & (\jythonCAPOOPTDynamic) 	& \jythonCAPOOPTALT & (\jythonCAPOOPTALTDynamic)\\
\bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexFT & (\luindexFTDynamic) 	& \luindexHB & (\luindexHBDynamic) 		& \luindexWCP & (\luindexWCPDynamic)	& \luindexWDC & (\luindexWDCDynamic)	& \luindexCAPO & (\luindexCAPODynamic)	& \luindexCAPOOPT & (\luindexCAPOOPTDynamic) 		& \luindexCAPOOPTALT & (\luindexCAPOOPTALTDynamic)\\
\bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchFT & (\lusearchFTDynamic)	& \lusearchHB & (\lusearchHBDynamic)	& \lusearchWCP & (\lusearchWCPDynamic)	& \lusearchWDC & (\lusearchWDCDynamic)	& \lusearchCAPO & (\lusearchCAPODynamic)	& \lusearchCAPOOPT & (\lusearchCAPOOPTDynamic) & \lusearchCAPOOPTALT & (\lusearchCAPOOPTALTDynamic)\\
\bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdFT & (\pmdFTDynamic) 			& \pmdHB & (\pmdHBDynamic) 				& \pmdWCP & (\pmdWCPDynamic)			& \pmdWDC & (\pmdWDCDynamic)			& \pmdCAPO & (\pmdCAPODynamic)			& \pmdCAPOOPT & (\pmdCAPOOPTDynamic) 				& \pmdCAPOOPTALT & (\pmdCAPOOPTALTDynamic)\\
\bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowFT & (\sunflowFTDynamic) 	& \sunflowHB & (\sunflowHBDynamic) 		& \sunflowWCP & (\sunflowWCPDynamic)	& \sunflowWDC & (\sunflowWDCDynamic)	& \sunflowCAPO & (\sunflowCAPODynamic)	& \sunflowCAPOOPT & (\sunflowCAPOOPTDynamic) 		& \sunflowCAPOOPTALT & (\sunflowCAPOOPTALTDynamic)\\
\bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatFT & (\tomcatFTDynamic) 		& \tomcatHB & (\tomcatHBDynamic) 		& \tomcatWCP & (\tomcatWCPDynamic)		& \tomcatWDC & (\tomcatWDCDynamic)		& \tomcatCAPO & (\tomcatCAPODynamic)		& \tomcatCAPOOPT & (\tomcatCAPOOPTDynamic) 	& \tomcatCAPOOPTALT & (\tomcatCAPOOPTALTDynamic)\\
\bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanFT & (\xalanFTDynamic) 		& \xalanHB & (\xalanHBDynamic) 			& \xalanWCP & (\xalanWCPDynamic)		& \xalanWDC & (\xalanWDCDynamic)		& \xalanCAPO & (\xalanCAPODynamic)		& \xalanCAPOOPT & (\xalanCAPOOPTDynamic) 			& \xalanCAPOOPTALT & (\xalanCAPOOPTALTDynamic)\\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\input{result-macros/PIP_fastTool_EpochRaceCheck}
%  
\small
\centering
\begin{tabular}{@{}l|rl|rr|rr|rr|rr|rr|rr|rr@{}}
& \mc{2}{c|}{} & \mc{14}{c@{}}{\FastTool EpochRaceCheck: Statically distinct races (dynamic races)}  \\
Program & \mc{2}{c|}{Events} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c|}{\CAPO-races} & \mc{2}{c|@{}}{\CAPO-Opt-races} & \mc{2}{c@{}}{Opt-Alt-races} \\\hline
\bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraFT & (\avroraFTDynamic) 		& \avroraHB & (\avroraHBDynamic) 		& \avroraWCP & (\avroraWCPDynamic)		& \avroraWDC & (\avroraWDCDynamic) 		& \avroraCAPO & (\avroraCAPODynamic) 		& \avroraCAPOOPT & (\avroraCAPOOPTDynamic) 	& \avroraCAPOOPTALT & (\avroraCAPOOPTALTDynamic) \\
\bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikFT & (\batikFTDynamic) 		& \batikHB & (\batikHBDynamic) 			& \batikWCP & (\batikWCPDynamic)		& \batikWDC & (\batikWDCDynamic)		& \batikCAPO & (\batikCAPODynamic)		& \batikCAPOOPT & (\batikCAPOOPTDynamic) 			& \batikCAPOOPTALT & (\batikCAPOOPTALTDynamic)\\
\bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoFT & (\htwoFTDynamic) 			& \htwoHB & (\htwoHBDynamic) 			& \htwoWCP & (\htwoWCPDynamic)			& \htwoWDC & (\htwoWDCDynamic)			& \htwoCAPO & (\htwoCAPODynamic)			& \htwoCAPOOPT & (\htwoCAPOOPTDynamic) 		& \htwoCAPOOPTALT & (\htwoCAPOOPTALTDynamic)\\
\bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonFT & (\jythonFTDynamic) 		& \jythonHB & (\jythonHBDynamic) 		& \jythonWCP & (\jythonWCPDynamic)		& \jythonWDC & (\jythonWDCDynamic)		& \jythonCAPO & (\jythonCAPODynamic)		& \jythonCAPOOPT & (\jythonCAPOOPTDynamic) 	& \jythonCAPOOPTALT & (\jythonCAPOOPTALTDynamic)\\
\bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexFT & (\luindexFTDynamic) 	& \luindexHB & (\luindexHBDynamic) 		& \luindexWCP & (\luindexWCPDynamic)	& \luindexWDC & (\luindexWDCDynamic)	& \luindexCAPO & (\luindexCAPODynamic)	& \luindexCAPOOPT & (\luindexCAPOOPTDynamic) 		& \luindexCAPOOPTALT & (\luindexCAPOOPTALTDynamic)\\
\bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchFT & (\lusearchFTDynamic)	& \lusearchHB & (\lusearchHBDynamic)	& \lusearchWCP & (\lusearchWCPDynamic)	& \lusearchWDC & (\lusearchWDCDynamic)	& \lusearchCAPO & (\lusearchCAPODynamic)	& \lusearchCAPOOPT & (\lusearchCAPOOPTDynamic) & \lusearchCAPOOPTALT & (\lusearchCAPOOPTALTDynamic)\\
\bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdFT & (\pmdFTDynamic) 			& \pmdHB & (\pmdHBDynamic) 				& \pmdWCP & (\pmdWCPDynamic)			& \pmdWDC & (\pmdWDCDynamic)			& \pmdCAPO & (\pmdCAPODynamic)			& \pmdCAPOOPT & (\pmdCAPOOPTDynamic) 				& \pmdCAPOOPTALT & (\pmdCAPOOPTALTDynamic)\\
\bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowFT & (\sunflowFTDynamic) 	& \sunflowHB & (\sunflowHBDynamic) 		& \sunflowWCP & (\sunflowWCPDynamic)	& \sunflowWDC & (\sunflowWDCDynamic)	& \sunflowCAPO & (\sunflowCAPODynamic)	& \sunflowCAPOOPT & (\sunflowCAPOOPTDynamic) 		& \sunflowCAPOOPTALT & (\sunflowCAPOOPTALTDynamic)\\
\bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatFT & (\tomcatFTDynamic) 		& \tomcatHB & (\tomcatHBDynamic) 		& \tomcatWCP & (\tomcatWCPDynamic)		& \tomcatWDC & (\tomcatWDCDynamic)		& \tomcatCAPO & (\tomcatCAPODynamic)		& \tomcatCAPOOPT & (\tomcatCAPOOPTDynamic) 	& \tomcatCAPOOPTALT & (\tomcatCAPOOPTALTDynamic)\\
\bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanFT & (\xalanFTDynamic) 		& \xalanHB & (\xalanHBDynamic) 			& \xalanWCP & (\xalanWCPDynamic)		& \xalanWDC & (\xalanWDCDynamic)		& \xalanCAPO & (\xalanCAPODynamic)		& \xalanCAPOOPT & (\xalanCAPOOPTDynamic) 			& \xalanCAPOOPTALT & (\xalanCAPOOPTALTDynamic)\\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\input{result-macros/PIP_fast_slow_eventCountCheck_slowTool}
%  
\small
\centering
\begin{tabular}{@{}l|rl|rr|rr|rr|rr@{}}
& \mc{2}{c|}{} & \mc{8}{c@{}}{\SlowTool fast slow eventCountCheck: Statically distinct races (dynamic races)}  \\
Program & \mc{2}{c|}{Events} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c@{}}{\DC-races} \\\hline
\bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraFT & (\avroraFTDynamic)		& \avroraHB & (\avroraHBDynamic) 		& \avroraWCP & (\avroraWCPDynamic)		& \avroraWDC & (\avroraWDCDynamic) \\
\bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikFT & (\batikFTDynamic)			& \batikHB & (\batikHBDynamic) 			& \batikWCP & (\batikWCPDynamic)		& \batikWDC & (\batikWDCDynamic) \\
\bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoFT & (\htwoFTDynamic)			& \htwoHB & (\htwoHBDynamic) 			& \htwoWCP & (\htwoWCPDynamic)			& \htwoWDC & (\htwoWDCDynamic) \\
\bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonFT & (\jythonFTDynamic)		& \jythonHB & (\jythonHBDynamic) 		& \jythonWCP & (\jythonWCPDynamic)		& \jythonWDC & (\jythonWDCDynamic) \\
\bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexFT & (\luindexFTDynamic)		& \luindexHB & (\luindexHBDynamic) 		& \luindexWCP & (\luindexWCPDynamic)	& \luindexWDC & (\luindexWDCDynamic) \\
\bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchFT & (\lusearchFTDynamic)	& \lusearchHB & (\lusearchHBDynamic)	& \lusearchWCP & (\lusearchWCPDynamic)	& \lusearchWDC & (\lusearchWDCDynamic) \\
\bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdFT & (\pmdFTDynamic)				& \pmdHB & (\pmdHBDynamic) 				& \pmdWCP & (\pmdWCPDynamic)			& \pmdWDC & (\pmdWDCDynamic) \\
\bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowFT & (\sunflowFTDynamic)		& \sunflowHB & (\sunflowHBDynamic) 		& \sunflowWCP & (\sunflowWCPDynamic)	& \sunflowWDC & (\sunflowWDCDynamic) \\
\bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatFT & (\tomcatFTDynamic)		& \tomcatHB & (\tomcatHBDynamic) 		& \tomcatWCP & (\tomcatWCPDynamic)		& \tomcatWDC & (\tomcatWDCDynamic) \\
\bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanFT & (\xalanFTDynamic)			& \xalanHB & (\xalanHBDynamic) 			& \xalanWCP & (\xalanWCPDynamic)		& \xalanWDC & (\xalanWDCDynamic) \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{0.5\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\input{result-macros/PIP_slowTool_noRaceEdge}
%  
\small
\centering
\begin{tabular}{@{}l|rl|rr|rr|rr|rr|rr@{}}
& \mc{2}{c|}{} & \mc{10}{c@{}}{\SlowTool noRaceEdge: Statically distinct races (dynamic races)}  \\
Program & \mc{2}{c|}{Events} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC noG-races} & \mc{2}{c@{}}{\DC-races} \\\hline
\bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraFT & (\avroraFTDynamic)		& \avroraHB & (\avroraHBDynamic) 		& \avroraWCP & (\avroraWCPDynamic)		& \avroraWDCnoG & (\avroraWDCnoGDynamic)	& \avroraWDC & (\avroraWDCDynamic) \\
\bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikFT & (\batikFTDynamic)			& \batikHB & (\batikHBDynamic) 			& \batikWCP & (\batikWCPDynamic)		& \batikWDCnoG & (\batikWDCnoGDynamic)		& \batikWDC & (\batikWDCDynamic) \\
\bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoFT & (\htwoFTDynamic)			& \htwoHB & (\htwoHBDynamic) 			& \htwoWCP & (\htwoWCPDynamic)			& \htwoWDCnoG & (\htwoWDCnoGDynamic)		& \htwoWDC & (\htwoWDCDynamic) \\
\bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonFT & (\jythonFTDynamic)		& \jythonHB & (\jythonHBDynamic) 		& \jythonWCP & (\jythonWCPDynamic)		& \jythonWDCnoG & (\jythonWDCnoGDynamic)	& \jythonWDC & (\jythonWDCDynamic) \\
\bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexFT & (\luindexFTDynamic)		& \luindexHB & (\luindexHBDynamic) 		& \luindexWCP & (\luindexWCPDynamic)	& \luindexWDCnoG & (\luindexWDCnoGDynamic)	& \luindexWDC & (\luindexWDCDynamic) \\
\bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchFT & (\lusearchFTDynamic)	& \lusearchHB & (\lusearchHBDynamic)	& \lusearchWCP & (\lusearchWCPDynamic)	& \lusearchWDCnoG & (\lusearchWDCnoGDynamic)& \lusearchWDC & (\lusearchWDCDynamic) \\
\bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdFT & (\pmdFTDynamic)				& \pmdHB & (\pmdHBDynamic) 				& \pmdWCP & (\pmdWCPDynamic)			& \pmdWDCnoG & (\pmdWDCnoGDynamic)			& \pmdWDC & (\pmdWDCDynamic) \\
\bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowFT & (\sunflowFTDynamic)		& \sunflowHB & (\sunflowHBDynamic) 		& \sunflowWCP & (\sunflowWCPDynamic)	& \sunflowWDCnoG & (\sunflowWDCnoGDynamic)	& \sunflowWDC & (\sunflowWDCDynamic) \\
\bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatFT & (\tomcatFTDynamic)		& \tomcatHB & (\tomcatHBDynamic) 		& \tomcatWCP & (\tomcatWCPDynamic)		& \tomcatWDCnoG & (\tomcatWDCnoGDynamic)	& \tomcatWDC & (\tomcatWDCDynamic) \\
\bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanFT & (\xalanFTDynamic)			& \xalanHB & (\xalanHBDynamic) 			& \xalanWCP & (\xalanWCPDynamic)		& \xalanWDCnoG' & (\xalanWDCnoGDynamic)		& \xalanWDC & (\xalanWDCDynamic) \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\caption{\FT-, \HB-, \WCP-, \DC-, \CAPO-, and \PIP-races detected by our implementation.
Each result is the average of 2 trials, rounded to the nearest integer.
Races are identified by field.}
 % Each result is from a single trial.}
\label{tab:coverage-dc}
\end{adjustwidth}
\end{table*}

==> fast-tool-extra-tables.tex <==
\begin{table*}[t]
\newcommand\DCwoG{\DC}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
 \newcommand{\rna}{\textbf{N/A}}
 \newcommand{\memna}{$<\,$2}
 \newcommand{\st}[1]{(#1~s)} %static time
 \newcommand{\dt}[1]{#1~s} %dynamic time
 \newcommand{\mem}[1]{#1} %memory
 \newcommand{\et}[1]{#1M} %event total
 \newcommand{\enfp}[1]{(#1M)} %event total, no fast path
 \newcommand{\base}[1]{#1~s} %base time
 \input{result-macros/PIP_fastTool_FTAddRaceEdge}
 
 \small
 \centering
 \begin{tabular}{@{}l|rl|rl||r|rrrrrrrrr}
 & \mc{2}{c|}{} & \mc{2}{c||}{} & Base & \mc{8}{c}{\FastTool Extra: Slowdown (normalized to Base time)} \\
 Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & time & Empty & \FT & \HB & \WCP & \DC & \CAPO & \CAPO-Opt & \CAPO-Opt-Alt \\\hline 
 \bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraTotalThreads 	& (\avroraMaxLiveThreads)	& \base{\avroraBaseTime}   & \roh{\avroraEmptyTime}   & \roh{\avroraFTTime}   & \roh{\avroraHBTime}   & \roh{\avroraWCPTime}   & \roh{\avroraDCTime} 	& \roh{\avroraCAPOTime} 	& \roh{\avroraCAPOOPTTime} & \roh{\avroraCAPOOPTALTTime} \\
 \bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikTotalThreads 	& (\batikMaxLiveThreads)	& \base{\batikBaseTime}    & \roh{\batikEmptyTime}    & \roh{\batikFTTime}    & \roh{\batikHBTime}    & \roh{\batikWCPTime}    & \roh{\batikDCTime}    & \roh{\batikCAPOTime} 		& \roh{\batikCAPOOPTTime} & \roh{\batikCAPOOPTALTTime} \\
 \bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoTotalThreads 	& (\htwoMaxLiveThreads)	    & \base{\htwoBaseTime}     & \roh{\htwoEmptyTime}     & \roh{\htwoFTTime}     & \roh{\htwoHBTime}     & \roh{\htwoWCPTime}     & \roh{\htwoDCTime}     & \roh{\htwoCAPOTime} 		& \roh{\htwoCAPOOPTTime} & \roh{\htwoCAPOOPTALTTime} \\
 \bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonTotalThreads	& (\jythonMaxLiveThreads)	& \base{\jythonBaseTime}   & \roh{\jythonEmptyTime}   & \roh{\jythonFTTime}   & \roh{\jythonHBTime} 	 & \roh{\jythonWCPTime}   & \roh{\jythonDCTime} 	 & \roh{\jythonCAPOTime} 	& \roh{\jythonCAPOOPTTime} & \roh{\jythonCAPOOPTALTTime} \\
 \bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexTotalThreads	& (\luindexMaxLiveThreads)	& \base{\luindexBaseTime}  & \roh{\luindexEmptyTime}  & \roh{\luindexFTTime}  & \roh{\luindexHBTime}  & \roh{\luindexWCPTime}  & \roh{\luindexDCTime}  & \roh{\luindexCAPOTime} 	& \roh{\luindexCAPOOPTTime} & \roh{\luindexCAPOOPTALTTime} \\
 \bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchTotalThreads	& (\lusearchMaxLiveThreads)	& \base{\lusearchBaseTime} & \roh{\lusearchEmptyTime} & \roh{\lusearchFTTime} & \roh{\lusearchHBTime} & \roh{\lusearchWCPTime} & \roh{\lusearchDCTime} & \roh{\lusearchCAPOTime}	& \roh{\lusearchCAPOOPTTime} & \roh{\lusearchCAPOOPTALTTime} \\
 \bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdTotalThreads	    & (\pmdMaxLiveThreads)	    & \base{\pmdBaseTime}      & \roh{\pmdEmptyTime}      & \roh{\pmdFTTime}      & \roh{\pmdHBTime}      & \roh{\pmdWCPTime}      & \roh{\pmdDCTime}	     & \roh{\pmdCAPOTime} 		& \roh{\pmdCAPOOPTTime} & \roh{\pmdCAPOOPTALTTime} \\
 \bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowTotalThreads	& (\sunflowMaxLiveThreads)	& \base{\sunflowBaseTime}  & \roh{\sunflowEmptyTime}  & \roh{\sunflowFTTime}  & \roh{\sunflowHBTime}	 & \roh{\sunflowWCPTime}  & \roh{\sunflowDCTime}  & \roh{\sunflowCAPOTime} 	& \roh{\sunflowCAPOOPTTime} & \roh{\sunflowCAPOOPTALTTime} \\
 \bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatTotalThreads	& (\tomcatMaxLiveThreads)	& \base{\tomcatBaseTime}   & \roh{\tomcatEmptyTime}   & \roh{\tomcatFTTime}   & \roh{\tomcatHBTime} 	 & \roh{\tomcatWCPTime}   & \roh{\tomcatDCTime}   & \roh{\tomcatCAPOTime} 	& \roh{\tomcatCAPOOPTTime} & \roh{\tomcatCAPOOPTALTTime} \\
 \bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanTotalThreads	& (\xalanMaxLiveThreads)	& \base{\xalanBaseTime}    & \roh{\xalanEmptyTime}    & \roh{\xalanFTTime}    & \roh{\xalanHBTime}    & \roh{\xalanWCPTime}    & \roh{\xalanDCTime}    & \roh{\xalanCAPOTime} 		& \roh{\xalanCAPOOPTTime} & \roh{\xalanCAPOOPTALTTime} 
 \end{tabular}
 
 % \notes{
 % \jake{Raw results for all the tables and figures in
 % evaluation can be found here:
 % \url{http://cse-dcse101008d.cse.ohio-state.edu/exp-products/PIP\_test/}}
 % }
 
 \caption{Run time for \fasttool and other analysis
 configurations.
 All values (except thread counts) are rounded to 2 significant figures.
 The table reports \PIP's slowdown relative to uninstrumented execution
 as the first value in the \emph{\Approach} column
 (\eg, \protect\roh{\avroraDCTime} for \bench{avrora}).
 The text explains other values.} 
 
 \label{tab:performance}
 \end{table*}
 
 \begin{table*}[t]
 \newcommand\DCwoG{\DC}
 \newcommand{\rzero}{0\xspace}
 \newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
 \newcommand{\rna}{\textbf{N/A}}
 \newcommand{\memna}{$<\,$2}
 \newcommand{\st}[1]{(#1~s)} %static time
 \newcommand{\dt}[1]{#1~s} %dynamic time
 \newcommand{\mem}[1]{#1} %memory
 \newcommand{\et}[1]{#1M} %event total
 \newcommand{\enfp}[1]{(#1M)} %event total, no fast path
 \newcommand{\base}[1]{#1~s} %base time
 \input{result-macros/PIP_fastTool_FTAddRaceEdge}
 
 \small
 \centering
 \begin{tabular}{@{}l|rl|rl||rrrrrrr}
 & \mc{2}{c|}{} & \mc{2}{c||}{} & \mc{7}{c}{\FastTool Extra: Memory usage (GB)} \\
 Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & \FT & \HB & \WCP & \DC & \CAPO & \CAPO-Opt & \CAPO-Opt-Alt \\\hline 
 \bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraTotalThreads 	& (\avroraMaxLiveThreads)	& \mem{\avroraFTMem}	& \mem{\avroraHBMem}	 	& \mem{\avroraWCPMem} 	& \mem{\avroraDCMem} 	& \mem{\avroraCAPOMem} 		& \mem{\avroraCAPOOPTMem} & \mem{\avroraCAPOOPTALTMem} \\
 \bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikTotalThreads 	& (\batikMaxLiveThreads)	& \mem{\batikFTMem}	& \mem{\batikHBMem} 		& \mem{\batikWCPMem} 	& \mem{\batikDCMem} 	& \mem{\batikCAPOMem} 		& \mem{\batikCAPOOPTMem} & \mem{\batikCAPOOPTALTMem} \\
 \bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoTotalThreads 	& (\htwoMaxLiveThreads)	    & \mem{\htwoFTMem}	    & \mem{\htwoHBMem} 		& \mem{\htwoWCPMem} 		& \mem{\htwoDCMem} 		& \mem{\htwoCAPOMem} 		& \mem{\htwoCAPOOPTMem} & \mem{\htwoCAPOOPTALTMem} \\
 \bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonTotalThreads	& (\jythonMaxLiveThreads)	& \mem{\jythonFTMem}	& \mem{\jythonHBMem} 	& \mem{\jythonWCPMem} 	& \mem{\jythonDCMem} 	& \mem{\jythonCAPOMem} 		& \mem{\jythonCAPOOPTMem} & \mem{\jythonCAPOOPTALTMem} \\
 \bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexTotalThreads	& (\luindexMaxLiveThreads)	& \mem{\luindexFTMem}	& \mem{\luindexHBMem} 	& \mem{\luindexWCPMem} 	& \mem{\luindexDCMem} 	& \mem{\luindexCAPOMem} 	& \mem{\luindexCAPOOPTMem} & \mem{\luindexCAPOOPTALTMem} \\
 \bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchTotalThreads	& (\lusearchMaxLiveThreads)	& \mem{\lusearchFTMem}	& \mem{\lusearchHBMem} 	& \mem{\lusearchWCPMem}	& \mem{\lusearchDCMem} 	& \mem{\lusearchCAPOMem}	& \mem{\lusearchCAPOOPTMem} & \mem{\lusearchCAPOOPTALTMem} \\
 \bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdTotalThreads	    & (\pmdMaxLiveThreads)	    & \mem{\pmdFTMem}	    & \mem{\pmdHBMem} 		& \mem{\pmdWCPMem} 		& \mem{\pmdDCMem} 		& \mem{\pmdCAPOMem} 		& \mem{\pmdCAPOOPTMem} & \mem{\pmdCAPOOPTALTMem} \\
 \bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowTotalThreads	& (\sunflowMaxLiveThreads)	& \mem{\sunflowFTMem}	& \mem{\sunflowHBMem}	& \mem{\sunflowWCPMem} 	& \mem{\sunflowDCMem} 	& \mem{\sunflowCAPOMem} 	& \mem{\sunflowCAPOOPTMem} & \mem{\sunflowCAPOOPTALTMem} \\
 \bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatTotalThreads	& (\tomcatMaxLiveThreads)	& \mem{\tomcatFTMem}	& \mem{\tomcatHBMem} 	& \mem{\tomcatWCPMem} 	& \mem{\tomcatDCMem} 	& \mem{\tomcatCAPOMem} 		& \mem{\tomcatCAPOOPTMem} & \mem{\tomcatCAPOOPTALTMem} \\
 \bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanTotalThreads	& (\xalanMaxLiveThreads)	& \mem{\xalanFTMem}	& \mem{\xalanHBMem} 		& \mem{\xalanWCPMem} 	& \mem{\xalanDCMem} 	& \mem{\xalanCAPOMem} 		& \mem{\xalanCAPOOPTMem} & \mem{\xalanCAPOOPTALTMem}
 \end{tabular}
 
 % \notes{
 % \jake{Raw results for all the tables and figures in
 % evaluation can be found here:
 % \url{http://cse-dcse101008d.cse.ohio-state.edu/exp-products/PIP\_test/}}
 % }
 
 \caption{Memory usage for \fasttool and other analysis
 configurations.
 All values are rounded to 2 significant figures.
 The text explains other values.} 
 
 \label{tab:memory}
 \end{table*}
 
\begin{table*}[t]
\begin{adjustwidth}{-1cm}{}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\input{result-macros/PIP_fastTool_FTAddRaceEdge}
%  
\small
\centering
\begin{tabular}{@{}l|rr|rr|rr|rr|rr|rr|rr@{}}
\et{}{} & \mc{14}{c@{}}{\FastTool Extra: Statically distinct races (dynamic races)}  \\
Program \et{Events}{\#Thr} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c|}{\CAPO-races} & \mc{2}{c|@{}}{\CAPO-Opt-races} & \mc{2}{c@{}}{Opt-Alt-races} \\\hline
\bench{avrora} 	\et{\avroraEvents}{\avroraThreads} 		& \avroraFT & (\avroraFTDynamic) 	& \avroraHB & (\avroraHBDynamic) 		& \avroraWCP & (\avroraWCPDynamic)		& \avroraWDC & (\avroraWDCDynamic) 		& \avroraCAPO & (\avroraCAPODynamic) 	& \avroraCAPOOPT & (\avroraCAPOOPTDynamic) 		& \avroraCAPOOPTALT & (\avroraCAPOOPTALTDynamic) \\
\bench{batik} 	\et{\batikEvents}{\batikThreads} 		& \batikFT & (\batikFTDynamic) 		& \batikHB & (\batikHBDynamic) 			& \batikWCP & (\batikWCPDynamic)		& \batikWDC & (\batikWDCDynamic)		& \batikCAPO & (\batikCAPODynamic)		& \batikCAPOOPT & (\batikCAPOOPTDynamic) 		& \batikCAPOOPTALT & (\batikCAPOOPTALTDynamic)\\
\bench{h2} 		\et{\htwoEvents}{\htwoThreads} 			& \htwoFT & (\htwoFTDynamic) 		& \htwoHB & (\htwoHBDynamic) 			& \htwoWCP & (\htwoWCPDynamic)			& \htwoWDC & (\htwoWDCDynamic)			& \htwoCAPO & (\htwoCAPODynamic)		& \htwoCAPOOPT & (\htwoCAPOOPTDynamic) 			& \htwoCAPOOPTALT & (\htwoCAPOOPTALTDynamic)\\
\bench{jython} 	\et{\jythonEvents}{\jythonThreads} 		& \jythonFT & (\jythonFTDynamic) 	& \jythonHB & (\jythonHBDynamic) 		& \jythonWCP & (\jythonWCPDynamic)		& \jythonWDC & (\jythonWDCDynamic)		& \jythonCAPO & (\jythonCAPODynamic)	& \jythonCAPOOPT & (\jythonCAPOOPTDynamic) 		& \jythonCAPOOPTALT & (\jythonCAPOOPTALTDynamic)\\
\bench{luindex} \et{\luindexEvents}{\luindexThreads} 	& \luindexFT & (\luindexFTDynamic) 	& \luindexHB & (\luindexHBDynamic) 		& \luindexWCP & (\luindexWCPDynamic)	& \luindexWDC & (\luindexWDCDynamic)	& \luindexCAPO & (\luindexCAPODynamic)	& \luindexCAPOOPT & (\luindexCAPOOPTDynamic) 	& \luindexCAPOOPTALT & (\luindexCAPOOPTALTDynamic)\\
\bench{lusearch}\et{\lusearchEvents}{\lusearchThreads}	& \lusearchFT & (\lusearchFTDynamic)& \lusearchHB & (\lusearchHBDynamic)	& \lusearchWCP & (\lusearchWCPDynamic)	& \lusearchWDC & (\lusearchWDCDynamic)	& \lusearchCAPO & (\lusearchCAPODynamic)& \lusearchCAPOOPT & (\lusearchCAPOOPTDynamic) 	& \lusearchCAPOOPTALT & (\lusearchCAPOOPTALTDynamic)\\
\bench{pmd} 	\et{\pmdEvents}{\pmdThreads} 			& \pmdFT & (\pmdFTDynamic) 			& \pmdHB & (\pmdHBDynamic) 				& \pmdWCP & (\pmdWCPDynamic)			& \pmdWDC & (\pmdWDCDynamic)			& \pmdCAPO & (\pmdCAPODynamic)			& \pmdCAPOOPT & (\pmdCAPOOPTDynamic) 			& \pmdCAPOOPTALT & (\pmdCAPOOPTALTDynamic)\\
\bench{sunflow} \et{\sunflowEvents}{\sunflowThreads} 	& \sunflowFT & (\sunflowFTDynamic) 	& \sunflowHB & (\sunflowHBDynamic) 		& \sunflowWCP & (\sunflowWCPDynamic)	& \sunflowWDC & (\sunflowWDCDynamic)	& \sunflowCAPO & (\sunflowCAPODynamic)	& \sunflowCAPOOPT & (\sunflowCAPOOPTDynamic) 	& \sunflowCAPOOPTALT & (\sunflowCAPOOPTALTDynamic)\\
\bench{tomcat} 	\et{\tomcatEvents}{\tomcatThreads} 		& \tomcatFT & (\tomcatFTDynamic) 	& \tomcatHB & (\tomcatHBDynamic) 		& \tomcatWCP & (\tomcatWCPDynamic)		& \tomcatWDC & (\tomcatWDCDynamic)		& \tomcatCAPO & (\tomcatCAPODynamic)	& \tomcatCAPOOPT & (\tomcatCAPOOPTDynamic) 		& \tomcatCAPOOPTALT & (\tomcatCAPOOPTALTDynamic)\\
\bench{xalan} 	\et{\xalanEvents}{\xalanThreads} 		& \xalanFT & (\xalanFTDynamic) 		& \xalanHB & (\xalanHBDynamic) 			& \xalanWCP & (\xalanWCPDynamic)		& \xalanWDC & (\xalanWDCDynamic)		& \xalanCAPO & (\xalanCAPODynamic)		& \xalanCAPOOPT & (\xalanCAPOOPTDynamic) 		& \xalanCAPOOPTALT & (\xalanCAPOOPTALTDynamic)\\\hline
Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
%  
\caption{\FT-, \HB-, \WCP-, \DC-, \CAPO-, and \PIP-races detected by our implementation.
Each result is the average of 10 trials, rounded to the nearest integer.
Races are identified using fields, the same method FastTrack uses to identify races.}
 % Each result is from a single trial.}
  
\label{tab:coverage-dc}
\end{adjustwidth}
\end{table*}


==> fast-tool-tables.tex <==
\begin{table*}[t]
\newcommand\DCwoG{\DC}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
 \newcommand{\rna}{\textbf{N/A}}
 \newcommand{\memna}{$<\,$2}
 \newcommand{\st}[1]{(#1~s)} %static time
 \newcommand{\dt}[1]{#1~s} %dynamic time
 \newcommand{\mem}[1]{#1} %memory
 \newcommand{\et}[1]{#1M} %event total
 \newcommand{\enfp}[1]{(#1M)} %event total, no fast path
 \newcommand{\base}[1]{#1~s} %base time
 \input{result-macros-fast-tool}
 
 \small
 \centering
 \begin{tabular}{@{}l|rl|rl||r|rrrrrrrr}
 & \mc{2}{c|}{} & \mc{2}{c||}{} & Base & \mc{7}{c}{\FastTool: Slowdown (normalized to Base time)} \\
 Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & time & Empty & \FT & \HB & \WCP & \DC & \CAPO & \PIP \\\hline 
 \bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraTotalThreads 	& (\avroraMaxLiveThreads)	& \base{\avroraBaseTime}   & \roh{\avroraEmptyTime}   & \roh{\avroraFTTime}   & \roh{\avroraHBTime}   & \roh{\avroraWCPTime}   & \roh{\avroraDCTime} 	& \roh{\avroraCAPOTime} 	& \roh{\avroraPIPTime} \\
 \bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikTotalThreads 	& (\batikMaxLiveThreads)	& \base{\batikBaseTime}    & \roh{\batikEmptyTime}    & \roh{\batikFTTime}    & \roh{\batikHBTime}    & \roh{\batikWCPTime}    & \roh{\batikDCTime}    & \roh{\batikCAPOTime} 		& \roh{\batikPIPTime} \\
 \bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoTotalThreads 	& (\htwoMaxLiveThreads)	    & \base{\htwoBaseTime}     & \roh{\htwoEmptyTime}     & \roh{\htwoFTTime}     & \roh{\htwoHBTime}     & \roh{\htwoWCPTime}     & \roh{\htwoDCTime}     & \roh{\htwoCAPOTime} 		& \roh{\htwoPIPTime} \\
 \bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonTotalThreads	& (\jythonMaxLiveThreads)	& \base{\jythonBaseTime}   & \roh{\jythonEmptyTime}   & \roh{\jythonFTTime}   & \roh{\jythonHBTime} 	 & \roh{\jythonWCPTime}   & \roh{\jythonDCTime} 	 & \roh{\jythonCAPOTime} 	& \roh{\jythonPIPTime} \\
 \bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexTotalThreads	& (\luindexMaxLiveThreads)	& \base{\luindexBaseTime}  & \roh{\luindexEmptyTime}  & \roh{\luindexFTTime}  & \roh{\luindexHBTime}  & \roh{\luindexWCPTime}  & \roh{\luindexDCTime}  & \roh{\luindexCAPOTime} 	& \roh{\luindexPIPTime} \\
 \bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchTotalThreads	& (\lusearchMaxLiveThreads)	& \base{\lusearchBaseTime} & \roh{\lusearchEmptyTime} & \roh{\lusearchFTTime} & \roh{\lusearchHBTime} & \roh{\lusearchWCPTime} & \roh{\lusearchDCTime} & \roh{\lusearchCAPOTime}	& \roh{\lusearchPIPTime} \\
 \bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdTotalThreads	    & (\pmdMaxLiveThreads)	    & \base{\pmdBaseTime}      & \roh{\pmdEmptyTime}      & \roh{\pmdFTTime}      & \roh{\pmdHBTime}      & \roh{\pmdWCPTime}      & \roh{\pmdDCTime}	     & \roh{\pmdCAPOTime} 		& \roh{\pmdPIPTime} \\
 \bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowTotalThreads	& (\sunflowMaxLiveThreads)	& \base{\sunflowBaseTime}  & \roh{\sunflowEmptyTime}  & \roh{\sunflowFTTime}  & \roh{\sunflowHBTime}	 & \roh{\sunflowWCPTime}  & \roh{\sunflowDCTime}  & \roh{\sunflowCAPOTime} 	& \roh{\sunflowPIPTime} \\
 \bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatTotalThreads	& (\tomcatMaxLiveThreads)	& \base{\tomcatBaseTime}   & \roh{\tomcatEmptyTime}   & \roh{\tomcatFTTime}   & \roh{\tomcatHBTime} 	 & \roh{\tomcatWCPTime}   & \roh{\tomcatDCTime}   & \roh{\tomcatCAPOTime} 	& \roh{\tomcatPIPTime} \\
 \bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanTotalThreads	& (\xalanMaxLiveThreads)	& \base{\xalanBaseTime}    & \roh{\xalanEmptyTime}    & \roh{\xalanFTTime}    & \roh{\xalanHBTime}    & \roh{\xalanWCPTime}    & \roh{\xalanDCTime}    & \roh{\xalanCAPOTime} 		& \roh{\xalanPIPTime} 
 \end{tabular}
 
 % \notes{
 % \jake{Raw results for all the tables and figures in
 % evaluation can be found here:
 % \url{http://cse-dcse101008d.cse.ohio-state.edu/exp-products/PIP\_test/}}
 % }
 
 \caption{Run time for \fasttool and other analysis
 configurations.
 All values (except thread counts) are rounded to 2 significant figures.
 The table reports \PIP's slowdown relative to uninstrumented execution
 as the first value in the \emph{\Approach} column
 (\eg, \protect\roh{\avroraDCTime} for \bench{avrora}).
 The text explains other values.} 
 
 \label{tab:performance}
 \end{table*}
 
 \begin{table*}[t]
 \newcommand\DCwoG{\DC}
 \newcommand{\rzero}{0\xspace}
 \newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
 \newcommand{\rna}{\textbf{N/A}}
 \newcommand{\memna}{$<\,$2}
 \newcommand{\st}[1]{(#1~s)} %static time
 \newcommand{\dt}[1]{#1~s} %dynamic time
 \newcommand{\mem}[1]{#1} %memory
 \newcommand{\et}[1]{#1M} %event total
 \newcommand{\enfp}[1]{(#1M)} %event total, no fast path
 \newcommand{\base}[1]{#1~s} %base time
 \input{result-macros-fast-tool}
 
 \small
 \centering
 \begin{tabular}{@{}l|rl|rl||rrrrrr}
 & \mc{2}{c|}{} & \mc{2}{c||}{} & \mc{6}{c}{\FastTool: Memory usage (GB)} \\
 Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & \FT & \HB & \WCP & \DC & \CAPO & \PIP \\\hline 
 \bench{avrora} 	& \et{\avroraEvents}   & \enfp{\avroraNoFPEvents}	& \avroraTotalThreads 	& (\avroraMaxLiveThreads)	& \mem{\avroraFTMem}	& \mem{\avroraHBMem}	 	& \mem{\avroraWCPMem} 	& \mem{\avroraDCMem} 	& \mem{\avroraCAPOMem} 		& \mem{\avroraPIPMem} \\
 \bench{batik} 	& \et{\batikEvents}    & \enfp{\batikNoFPEvents}	& \batikTotalThreads 	& (\batikMaxLiveThreads)	& \mem{\batikFTMem}	& \mem{\batikHBMem} 		& \mem{\batikWCPMem} 	& \mem{\batikDCMem} 	& \mem{\batikCAPOMem} 		& \mem{\batikPIPMem} \\
 \bench{h2} 		& \et{\htwoEvents}     & \enfp{\htwoNoFPEvents}	    & \htwoTotalThreads 	& (\htwoMaxLiveThreads)	    & \mem{\htwoFTMem}	    & \mem{\htwoHBMem} 		& \mem{\htwoWCPMem} 		& \mem{\htwoDCMem} 		& \mem{\htwoCAPOMem} 		& \mem{\htwoPIPMem} \\
 \bench{jython} 	& \et{\jythonEvents}   & \enfp{\jythonNoFPEvents}	& \jythonTotalThreads	& (\jythonMaxLiveThreads)	& \mem{\jythonFTMem}	& \mem{\jythonHBMem} 	& \mem{\jythonWCPMem} 	& \mem{\jythonDCMem} 	& \mem{\jythonCAPOMem} 		& \mem{\jythonPIPMem} \\
 \bench{luindex} & \et{\luindexEvents}  & \enfp{\luindexNoFPEvents}	& \luindexTotalThreads	& (\luindexMaxLiveThreads)	& \mem{\luindexFTMem}	& \mem{\luindexHBMem} 	& \mem{\luindexWCPMem} 	& \mem{\luindexDCMem} 	& \mem{\luindexCAPOMem} 	& \mem{\luindexPIPMem} \\
 \bench{lusearch}& \et{\lusearchEvents} & \enfp{\lusearchNoFPEvents}	& \lusearchTotalThreads	& (\lusearchMaxLiveThreads)	& \mem{\lusearchFTMem}	& \mem{\lusearchHBMem} 	& \mem{\lusearchWCPMem}	& \mem{\lusearchDCMem} 	& \mem{\lusearchCAPOMem}	& \mem{\lusearchPIPMem} \\
 \bench{pmd} 	& \et{\pmdEvents}      & \enfp{\pmdNoFPEvents}      & \pmdTotalThreads	    & (\pmdMaxLiveThreads)	    & \mem{\pmdFTMem}	    & \mem{\pmdHBMem} 		& \mem{\pmdWCPMem} 		& \mem{\pmdDCMem} 		& \mem{\pmdCAPOMem} 		& \mem{\pmdPIPMem} \\
 \bench{sunflow} & \et{\sunflowEvents}  & \enfp{\sunflowNoFPEvents}	& \sunflowTotalThreads	& (\sunflowMaxLiveThreads)	& \mem{\sunflowFTMem}	& \mem{\sunflowHBMem}	& \mem{\sunflowWCPMem} 	& \mem{\sunflowDCMem} 	& \mem{\sunflowCAPOMem} 	& \mem{\sunflowPIPMem} \\
 \bench{tomcat} 	& \et{\tomcatEvents}   & \enfp{\tomcatNoFPEvents}	& \tomcatTotalThreads	& (\tomcatMaxLiveThreads)	& \mem{\tomcatFTMem}	& \mem{\tomcatHBMem} 	& \mem{\tomcatWCPMem} 	& \mem{\tomcatDCMem} 	& \mem{\tomcatCAPOMem} 		& \mem{\tomcatPIPMem} \\
 \bench{xalan} 	& \et{\xalanEvents}    & \enfp{\xalanNoFPEvents}	& \xalanTotalThreads	& (\xalanMaxLiveThreads)	& \mem{\xalanFTMem}	& \mem{\xalanHBMem} 		& \mem{\xalanWCPMem} 	& \mem{\xalanDCMem} 	& \mem{\xalanCAPOMem} 		& \mem{\xalanPIPMem}  
 \end{tabular}
 
 % \notes{
 % \jake{Raw results for all the tables and figures in
 % evaluation can be found here:
 % \url{http://cse-dcse101008d.cse.ohio-state.edu/exp-products/PIP\_test/}}
 % }
 
 \caption{Memory usage for \fasttool and other analysis
 configurations.
 All values are rounded to 2 significant figures.
 The text explains other values.} 
 
 \label{tab:memory}
 \end{table*}
 
 \begin{table*}[t]
 \newcommand{\rcounts}[2]{\textbf{#2} (#1)}
 \newcommand{\rzero}{\textbf{0}}
 \newcommand{\rna}{\textbf{N/A}}
 \newcommand{\et}[2]{}
 \input{result-macros-fast-tool}
%  
 \small
 \centering
 \begin{tabular}{@{}l|rr|rr|rr|rr|rr|rr@{}}
 \et{}{} & \mc{12}{c@{}}{\FastTool: Statically distinct races (dynamic races)}  \\
 Program \et{Events}{\#Thr} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c|}{\CAPO-races} & \mc{2}{c@{}}{\PIP-races} \\\hline
 \bench{avrora} 	\et{\avroraEvents}{\avroraThreads} 		& \avroraFT & (\avroraFTDynamic) 		& \avroraHB & (\avroraHBDynamic) 		& \avroraWCP & (\avroraWCPDynamic)		& \avroraWDC & (\avroraWDCDynamic) 		& \avroraCAPO & (\avroraCAPODynamic) 		& \avroraPIP & (\avroraPIPDynamic) \\
 \bench{batik} 	\et{\batikEvents}{\batikThreads} 		& \batikFT & (\batikFTDynamic) 		& \batikHB & (\batikHBDynamic) 			& \batikWCP & (\batikWCPDynamic)		& \batikWDC & (\batikWDCDynamic)		& \batikCAPO & (\batikCAPODynamic)		& \batikPIP & (\batikPIPDynamic)\\
 \bench{h2} 		\et{\htwoEvents}{\htwoThreads} 			& \htwoFT & (\htwoFTDynamic) 			& \htwoHB & (\htwoHBDynamic) 			& \htwoWCP & (\htwoWCPDynamic)			& \htwoWDC & (\htwoWDCDynamic)			& \htwoCAPO & (\htwoCAPODynamic)			& \htwoPIP & (\htwoPIPDynamic)\\
 \bench{jython} 	\et{\jythonEvents}{\jythonThreads} 		& \jythonFT & (\jythonFTDynamic) 		& \jythonHB & (\jythonHBDynamic) 		& \jythonWCP & (\jythonWCPDynamic)		& \jythonWDC & (\jythonWDCDynamic)		& \jythonCAPO & (\jythonCAPODynamic)		& \jythonPIP & (\jythonPIPDynamic)\\
 \bench{luindex} \et{\luindexEvents}{\luindexThreads} 	& \luindexFT & (\luindexFTDynamic) 	& \luindexHB & (\luindexHBDynamic) 		& \luindexWCP & (\luindexWCPDynamic)	& \luindexWDC & (\luindexWDCDynamic)	& \luindexCAPO & (\luindexCAPODynamic)	& \luindexPIP & (\luindexPIPDynamic)\\
 \bench{lusearch}\et{\lusearchEvents}{\lusearchThreads}	& \lusearchFT & (\lusearchFTDynamic)	& \lusearchHB & (\lusearchHBDynamic)	& \lusearchWCP & (\lusearchWCPDynamic)	& \lusearchWDC & (\lusearchWDCDynamic)	& \lusearchCAPO & (\lusearchCAPODynamic)	& \lusearchPIP & (\lusearchPIPDynamic)\\
 \bench{pmd} 	\et{\pmdEvents}{\pmdThreads} 			& \pmdFT & (\pmdFTDynamic) 			& \pmdHB & (\pmdHBDynamic) 				& \pmdWCP & (\pmdWCPDynamic)			& \pmdWDC & (\pmdWDCDynamic)			& \pmdCAPO & (\pmdCAPODynamic)			& \pmdPIP & (\pmdPIPDynamic)\\
 \bench{sunflow} \et{\sunflowEvents}{\sunflowThreads} 	& \sunflowFT & (\sunflowFTDynamic) 	& \sunflowHB & (\sunflowHBDynamic) 		& \sunflowWCP & (\sunflowWCPDynamic)	& \sunflowWDC & (\sunflowWDCDynamic)	& \sunflowCAPO & (\sunflowCAPODynamic)	& \sunflowPIP & (\sunflowPIPDynamic)\\
 \bench{tomcat} 	\et{\tomcatEvents}{\tomcatThreads} 		& \tomcatFT & (\tomcatFTDynamic) 		& \tomcatHB & (\tomcatHBDynamic) 		& \tomcatWCP & (\tomcatWCPDynamic)		& \tomcatWDC & (\tomcatWDCDynamic)		& \tomcatCAPO & (\tomcatCAPODynamic)		& \tomcatPIP & (\tomcatPIPDynamic)\\
 \bench{xalan} 	\et{\xalanEvents}{\xalanThreads} 		& \xalanFT & (\xalanFTDynamic) 		& \xalanHB & (\xalanHBDynamic) 			& \xalanWCP & (\xalanWCPDynamic)		& \xalanWDC & (\xalanWDCDynamic)		& \xalanCAPO & (\xalanCAPODynamic)		& \xalanPIP & (\xalanPIPDynamic)\\\hline
 Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
 \end{tabular}
%  
 \caption{\FT-, \HB-, \WCP-, \DC-, \CAPO-, and \PIP-races detected by our implementation.
 Each result is the average of 5 trials, rounded to the nearest integer.}
 % Each result is from a single trial.}
  
 \label{tab:coverage-dc}
 \end{table*}

==> misc/annotated-oopsla-2019-reviews <==
# Detailed Response

### Review A

> Cons: From about the middle of section 2.4 through section 4.2, I found the paper very difficult to
> read, probably due to the high ratio of formulae to plain English. The authors should revise the paper
> to explain the various kinds of analyses, and their composites, more simply and intuitively with prose
> (and examples!) separate from the formulae. Although hotcrp says the authors intend to submit an
> artifact, I was unable to find anywhere in the paper that states that the authors plan to make the
> implementation available open-source (but I may have missed it).

--- [Addressed. Added a sentence in the Implementation section with an empty link for the Github URL]

As mentioned above, we'll open-source our implementation.
We'll revise significantly to make the explanations more intuitive as the reviewer suggests.


> The contributions paragraph on page 2 says 
> "We realize *the last two contributions* in SmartTrack, 
> a new algorithm for optimized partial-order-based predictive analysis, 
> including the existing WCP and DC analyses and the new WDC analysis." (emphasis added) 
> This wording is confusing.  
> But it looks to me like SmartTrack includes all three of the optimizations, 
> which together constitute the second and third contributions, 
> and seems to also incorporate the weakly-doesn't-commute analysis part of the first contribution.  
> The authors should clarify.

--- [Addressed. Rewrote the Contributions paragraph on page 2 to clarify the individual contributions
and expanded upon how each contributions addresses the issues of poor performance.]

The paper introduces three optimizations:
1. The weak-doesn't-commute (WDC) relation and analysis
2. Epoch and ownership optimizations
3. Conflict critical section (CCS) optimizations

SmartTrack represents Contributions 2 and 3. 
SmartTrack is orthogonal to WDC: SmartTrack can be applied to WDC analysis and other predictive analyses. 
We'll clarify in the next revision.


> It looks like SmartTrack does not always improve on FTO-{WCP|DC|WDC}, 
> e.g., jython, sunflow, and tomcat show higher overhead for both runtime and memory usage, 
> and there's higher memory usage for lusearch (just DC) and pmd.  Why is this?  
> There is discussion in 5.6 about apparent and actual anomalies for race detection, 
> but no analogous discussion for overhead.
> The paper would be stronger if the authors found, and presented, 
> the cause of the unexpectly low race counts for jython using FTO-WCP.

--- [Addressed. Gathered and included full results for the "extra metadata" performance bug.]
--- [TODO: Mention in cover letter that we also changed our methodology for specifying core count, affecting the results.]

--- [Not Addressed. Still investigating FTO-WCP for jython issue.]

Investigating this issue, 
we have found that our implementation of "extra metadata" ($E_x$) incurs nontrivial performance overheads 
even when the extra metadata is rarely or never used. 
In particular, 
each program variable $x$'s metadata is initialized with two empty hash maps for $E^r_x$ and $E^w_x$, 
leading to significant memory and run-time overhead.

In preliminary experiments,
initializing these fields to null (and creating a map only when needed) 
eliminates the performance anomaly between SmartTrack and FTO, 
actually improving the performance of SmartTrack-based analyses noticeably 
(by 6–9% run time and 31–33% memory usage on average).
We'll collect full updated results for the next version of the paper.


> The paper does not explain how all the different implementations 
> (or perhaps options within the same implementation?) were tested for semantic bugs, 
> what the development effort involved, lines of code, and so on, 
> which I typically see in "my tool runs fast" papers.
> In any case, the implementation should be made available open-source 
> for other researchers to build on.

--- [Not Addressed yet. Still figuring out how to describe development and sanity check of the implementation.] 

As mentioned above, we'll open-source our implementation, 
which consists of a RoadRunner tool and minor modifications to RoadRunner. 
We can describe in the text how we developed and sanity checked the implementation.


### Review B

> The paper says that the performance is comparable to HB 
> and gives a large number of evaluation tables. 
> However the text doesn't give headline figures. 
> For each of your three sets of optimisations how much did they help up the performance.
> Do different kinds of programs benefit differently and if so how and why?

--- [Addressed. I included the speedups corresponding to the individual optimizations for headline figures.
I included a table as well to emphasis the overall contributions, Unopt-* vs. ST-* and ST-* vs. Opt-HB.]

--- [Addressed. I expanded upon Section 5.3 (Run-Time Characteristics) to address
how and why different kinds of programs benefit differently.] 

We'll answer these questions in the text, including giving headline figures. 
Here we also give answers briefly.

The individual optimizations help performance in the following ways:
1. WDC analysis speeds up execution time by 1.1–1.2x compared with DC analysis.
2. Epoch and ownership optimizations (FTO-*) speed up execution time by 1.9–3.0x compared with unoptimized analyses.
3. CCS optimizations speed up execution by 1.5–1.6x compared with FTO-based analyses.

All programs generally benefit from epoch and ownership optimizations, 
which avoid full vector clock operations. 
Programs that perform many accesses holding one or more locks (see Table 2) 
benefit more from CCS optimizations.


> Line 63 says there are 3 major sources of poor performance. 
> What are the poor performance issues that the second and third optimisation provide? 
> If they aren't obvious then perhaps you should start the paragraph by 
> saying there are 3 ways we can improve the performance? 
> After introducing each of these kinds of optimisations can you also say 
> what kind of speedup each one provides? 
> (e.g between x% and y% improvement or approx z% improvement).

--- [Addressed. Rewrote the Contributions paragraph on page 2 to clarify the poor performance issues,
including stating speedups corresponding to the individual optimizations that address each poor performance issue.] 

1. The first source of poor performance is DC's release–release ordering. 
WDC analysis addresses this issue.
2. The second source of poor performance is performing full vector clock operations. 
Epoch and ownership optimizations address this issue.
3. The third source of poor performance is detecting and handling conflicting critical sections. 
CCS optimizations address this issue.

We'll clarify these sources of poor performance and corresponding optimizations upfront in the paper 
and state corresponding speedups.


> Line 408 - could you explain/justify the statement in the paragraph?

--- [Addressed. Included the more intuitive explanation of FastTrack's insights.]

Only the latest write and latest reads since the last write are necessary for detecting the first race soundly, 
as justified in FastTrack [Flanagan and Freund 2009] and FastTrack-Ownership [Wood et al. 2017]. 
Intuitively, if there's no race with the last write and the current access, then either 
(1) the current access doesn't race with any earlier writes or 
(2) the last write races with an earlier write (which would have been detected earlier). 
A similar argument applies to some reads. We'll explain this in the text.


> Line 805 - what is the advantage of continuing after finding a race?

--- [Addressed. Expanded Handling races paragraph to clarify why we continue after the first race.]

In practice, industry-standard race detectors continue detecting races after the first race 
in order to report more races to users. 
Furthermore, continuing after the first race allows us to run our analyses on full executions 
and collect performance and race coverage results.


> Line 1027 - Can you try to include the reasons in the final publication?

--- [Not Addressed. Still investigating FTO-WCP for jython issue.]

We haven't figured it out yet, but we'll try to include it.


> Line 1102 - state why you want predictive analysis rather than just HB in the conclusions. 
> That is state something about not finding races and finding false races.

--- [Addressed. Rewrote the Conclusion section to more distinctly advocate for predictive analysis over HB.]

We'll revise as suggested.


### Review C

> Where this paper is lacking is that the evaluation does not draw any conclusions 
> as to whether the more expensive analyses are worth using instead of the HB analysis.  
> For example, given a fixed time budget, which analysis finds the largest number of static races?
> Does it make sense to run the HB analysis on more traces or the WCP analysis on fewer traces?
> Moreover, what is the overhead of the vindication procedure that DC and WDC require?
> Taking that into account, does it (still) make sense to use these techniques?
> (I understand that these questions are somewhat orthogonal to the contribution of the paper, 
> which is to optimise algorithms XYZ, 
> but I think they are very important for a reader of the paper to understand 
> whether these algorithms are now worth implementing/using.)

--- [Addressed. Added the response to section 5.7 (Summary)]

Evaluating analysis effectiveness across multiple executions is admittedly beyond the scope of the paper. 
A key challenge is the plethora of different options for choosing multiple executions. 
Simply re-executing a program natively is likely to expose a similar set of HB-races, 
while an advanced race-exposing technique could potentially expose HB-races effectively, 
but likely at a higher cost. We'll discuss this issue in the paper.

We emphasize that our optimized DC and WDC analyses do *not* perform vindication. 
They instead report DC- and WDC-races (which are generally true races in practice) without vindication; 
or they can use record & replay techniques to replay an execution 
and collect enough information to perform vindication.


> 42: "Alternatively" - alternative to what?

--- [Addressed. No major revision. Simply changed "Alternatively," to "Alternatives to partial-order-based predictive analysis,"] 

Alternative to partial-order-based predictive analysis.
We'll clarify the text.


> 391: sound -> unsound.
> 
> 466: $R_x = C(t)$ -> $R_x = C_t(t)$

--- [Addressed.]

Thanks, we'll correct these typos.


> 981-995: Do you have any explanation about the different number of races found 
> in the unoptimised and optimised versions of a given algorithm,
> when statistically significant, e.g., pmd and xalan?

--- [Addressed. Added clearly stating the reason for differences in coverage between Unopt- and optimized (FTO-,ST-). Also added to table caption.]

As Lines 1046-1048 explain,
the differences in number of races are attributable to
the unoptimized and optimized analyses having different behavior after detecting the first race
due to their different representations of last-access metadata.


### Review D

> Besides the above, I wonder why the authors distinguish 
> happens-before from "predictive analysis".  
> Isn't happens-before also a predictive analysis technique?  
> It has a lower prediction capability, 
> but falls into the same category as the other predictive runtime analysis techniques, 
> that is, from one execution we can predict other executions.

--- [Addressed. Added clarification to distinguish HB analysis from predictive analysis.]

We agree, but the literature generally distinguishes "predictive analysis" as being able 
to find strictly more races than HB analysis. 
We'll make this more evident in the text.


> Dacapo is not necessarily a great benchmark for data-races; 
> it would be more convincing to use SmartTrack on some large concurrent real-life Java programs.

--- [Addressed. Added disclaimer to the beginning of section 5.6 (Predictable Race Coverage)]

DaCapo consists of real, widely used concurrent programs that are well suited to evaluating performance 
and that also contain data races.
We recognize that the DaCapo suite is not expressly intended for evaluating data race detection,
and we'll mention that in the paper.


*********** INTERNAL NOTES ****************

Evaluating multiple distinct traces, systematically or intelligently, 
using the analyses mentioned in this paper is out of the scope of this paper.
It is not conclusive from our evaluation that more static races will be reported
by HB analysis or predictive analysis within a fixed time budget.

Future work could investigate the effectiveness of thread scheduling using
the analyses mentioned in this paper on the same program.

\jake{I finished collecting 10 trials for the new results we looked at in the last meeting 
(previously only 5 trials).
I added performance improvement percentages over the results in the submitted results 
for WCP (10.64% run and 32.73% mem), DC (10.42% run and 30.9% mem), and WDC (16.87% run and 35.79% mem).
The "extra" change improved performance over the w/o setting core results 
(tables we were comparing during our meeting) by roughly 6%-9% (WCP 5.62%, DC 8.51%, WDC 6.76%) run time 
and 31%-33% (WCP 32.73%, DC 30.91%, WDC 31.46%) memory usage on average.
I'm not sure which you intended to base the improvement upon.}



==> misc/annotated-pldi-2019-reviews <==
PLDI 2019 Paper #63 Reviews and Comments
===========================================================================
Paper #63 Practical Predictive Race Detection


Review #63A
===========================================================================
* Updated: 15 Feb 2019 1:07:03pm EST

Overall merit
-------------
C. I would not accept this paper but will not argue strongly against
   accepting it.

Reviewer expertise
------------------
Y. Knowledgeable

Paper summary
-------------
This paper presents SmartTrack, a series of optimizations for
predictive race detection algorithms to improve their runtime and
memory consumption. The main contribution of this paper is the
conflicting critical section (CCS) optimization. The key insight is
that CCSs can be detected efficiently by maintaining CCS metadata in
addition to last-access metadata. The paper also applies
happens-before optimizations such as epoch and ownership optimizations
(FTO) to predictive race detection algorithms. The paper compares
unoptimized race detection algorithms (HB, WCP, DC, WDC) with the
corresponding FTO and CCS optimized variants. Evaluation on 10 DaCapo
programs shows that the optimizations improve the performance of
predictive race detection algorithms.

Comments for author
-------------------
### Comments after PC meeting

The paper was discussed at the PC meeting. All reviewers appreciated the practical motivation of this work. The proposed optimizations improve the performance of various predictive race detection algorithms. The main concerns were about the novelty of the optimizations. Although the evaluation is extensive, some reviewers would have liked to see how the optimizations work on large/real programs, and how the optimizations impact precision. We hope the detailed comments in the reviews can be used to improve a future revision of this work.

### Original review

Strengths:

+ The proposed optimizations improve the performance of various
predictive race detection algorithms.

+ The optimizations are evaluated on 10 DaCapo benchmarks against
several implementations of happens-before and predictive race
detectors.

Weaknesses:

- Race coverage is not fully evaluated as part of the main paper.

- HB-FTO seems to be as effective and faster than the predictive
  algorithms with ST optimizations for the majority of the benchmarks.

- The quality of race detection is not considered in the evaluation.

- Related work is not described in detail.


Comments:

Predictive race detection is known to be more precise than
happens-before race detection (HB), however it is also more expensive
in terms of runtime and memory. This paper proposes to apply three
optimizations to speedup predictive race detection. The first two
optimizations are epoch and ownership optimizations (FTO), which are
already used in the context of HB algorithms. The paper also proposes
the conflicting critical section (CCS) optimization, which is the main
contribution of this paper. The main insight behind implementing CCS
effectively is to maintain metadata on critical sections for a given
variable in a similar way as metadata for variable accesses is
maintained. Optimized algorithms for "doesn't commute" (DC) are given
as well as discussed for "weak doesn't-commute analysis" (WDC). The
paper is well written, and gives a good amount of background on
happens-before and predictive race detection.

The authors did a good job providing baselines (unoptimized HB, WCP,
DC, WDC) and providing runtime and memory use for the corresponding
optimized algorithms (FT and ST). For the evaluation, the paper uses
10 DaCapo programs. The paper focuses on comparing the various
algorithms in terms of running time and memory usage, but the number
of static and dynamic races can be found in the supplemental
material. I think number of races should be part of the main
evaluation of the paper, thus I would like to encourage the authors to
include this material in the paper.

My main questions are related to the comparison against HB-FTO
(happens before analysis with FTO optimizations). I found it
surprising that HB-FTO is as effective finding static races as the
rest of FTO and ST optimized algorithms for 8 out of 10 programs, and
more efficient for 7 of these programs. The optimized predictive
algorithms are significantly faster than their unoptimized versions,
but it is not clear how these algoritms compare with HB-FTO in terms
of race detection effectiveness when the number of data races it is
the same in most cases. The paper refers to coverage-soundness
tradeoff, however the evaluation does not provide evidence that the
optimized predictive algorithms are more effective in finding races
than HB-FTO. What is the overlap among static races detected by the
various algorithms? How many false races are reported by the various
algorithms? Are there more false races when optimizing the algorithms?

Finally, I found the related work section to be too general. Please
consider describing this work againts closely related work in more
detail instead of giving a one-sentence description for multiple
papers.

>>> \mike{There are some potential TODOs above.}
>>> \jake{The feedback similar to the questions for authors,
>>> ``races should be part of the main evaluation of the paper''
>>> and ``comparison against HB-FTO''?
>>> I agree once the race counting is finalized.}
>>> \jake{In regards to related work,
>>> should we include more types of prior work
>>> or simply expand on what is already mentioned?}

Questions for Authors
---------------------
1. What do you consider to be the most significant challenge in
applying FTO optimizations to predictive race detection algorithms?
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

2. What is the overlap among static races detected by the various
algorithms (HB-FTO vs. WCP-ST, DC-ST, and WDC-ST)?
>>> Not Addressed. Currently investigating counting races by fields.

3. How do the optimized predictive algorithms compare with HB-FTO in
terms of false static races?
>>> Not Addressed. See above.

4. Are there any limitations introduced by the proposed optimizations?
>>> Not Addressed. See above. 

5. Is it possible for the optimizations to have an impact on the
validity or number of the data races detected?
>>> Not Addressed. See above.



Review #63B
===========================================================================

Overall merit
-------------
C. I would not accept this paper but will not argue strongly against
   accepting it.

Reviewer expertise
------------------
Y. Knowledgeable

Paper summary
-------------
The traditional problem of data races is considered. Several recent
papers have been improving on the traditional happens-before (HB) race
detection using so called predictive analyses that find more races
than HB but have a higher overhead than HB. A new set of optimizations
is presented, culminating in the SmartTrack algorithm, that can speed
up predictive analyses using prior work on faster HB analysis. The
results on the standard benchmark set show promising reduction in time
and memory overheads.

Comments for author
-------------------
* Pros:
  - traditional problem of detecting data races
  - new techniques reduce overhead of predictive analyses
  - extensive list of references

* Cons:
  - rather small increment
  - simple extensions of combining two lines of prior work
  - presentation issues
  - unexplained problems with FTO-HB and sunflow

* Section 3.1 does not discuss if there were any challenges in applying
  FTO to DC: is it just a straightforward applications, or are there
  some deeper insights?  We just learn what is being done but not why.
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

* Section 3.2 addresses the "second significant cost".  It's indeed
  the key contribution in terms of both novelty and the length.  But
  the presentation is rather "dense" and hard to follow.  Also, at
  that point in the text it's not clear how big is that "second cost".
  In fact, the various costs are never analyzed in isolation later!
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

* Section 4 (WDC) is a nice contribution and should be expanded more.
  Even if the contribution is simple, it can be practically beneficial.
  The vindication algorithm should be described here in more detail.
  Is this all shortened because WDC does not report more races than DC
  (which we find in section 5.6)?
>>> Not Applicable. WDC and Vindication are both discussed in relevant detail.
>>> \mike{You don't think we should highlight WDC as more of a contribution?}
>>> \jake{I think we are with the latest changes and I agree it should be after working on Dissertation.}

* The evaluation uses a standard set of Java benchmarks.  The runtimes
  (Base time column in Table 3) are rather small.  For table 4, it'd
  help to show the maximum overhead, e.g., 120x for sunflow in table 3.
>>> Addressed.

  Tables 5 and 6 don't contribute much to gaining insights. The number
  of detected races would be more informative.
>>> Not Addressed. Currently investigating counting races by fields. 

* The paper discusses soundness, starting from the background in
  section 2.3 and repeating several times, including middle of section
  4. It's better to refer to *soundiness* when talking about practical
  analyses (as claimed in the title and repeated several times):

  "In Defense of Soundiness: A Manifesto"
  By Benjamin Livshits, Manu Sridharan, Yannis Smaragdakis, Ondřej
  Lhoták, J. Nelson Amaral, Bor-Yuh Evan Chang, Samuel Z. Guyer, Uday
  P. Khedker, Anders Møller, Dimitrios Vardoulakis

  Practical tools have several causes of unsoundness, including
  programs using synchronization not understood by the tools.
>>> Not Applicable. Soundness is defined in the paper as
every race indicates a true predictable race.
>>> \mike{Doesn't the "-iness" issue apply to not only FN freedom but also FP freedom?}
>>> \jake{FN and FP?}

* The formalization is not very rigorous, eg:

  - Each event has an executing thread returned by a helper function thr(e).
    ... presumably the event (tuple) should have that thread info
>>> Addressed as comment in Section 2.1

  - if e <tr e′ ... ordering notation used without being defined
>>> Addressed.

  - every read in tr′ has the same last writer as in tr ... the term
    last writer used without being defined
>>> Addressed.

  - two conflicting accesses unordered by <WCP or <DC, respectively
    ... again some ordering notation used before being defined
>>> Addressed.

  - where a1 is the corresponding acquire event for r1 ... does not
    formally define corresponding, which may be in [53], but this
    paper should be self contained
>>> Addressed.

  - a rule that WCP left- and right-composes with HB ... again not
    described in this paper making it not self contained
>>> Addressed.

  - an epoch is a scalar c@t ... looks more like a pair than scalar
>>> Addressed.

  - it'd be good to mention whether memory locations correspond to all
    field accesses (o.f) and array accesses (a[i])
>>> Addressed.

* The order of presentation can be changed in several places.

  - more intuition, examples, or high-level descriptions can be
    provided before going deeper into details, eg, for DC analysis or
    epoch optimizations; the paper tends to delve rather fast into
    *how* something is done before describing *what* it tries to achieve;
    this is particularly important for algorithm 3, the key contribution;
    I found it rather hard to follow the description -- one can always
    blame a "lazy reviewer/reader", but a better description can
    significantly help
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

  - the use of mutable references is also somewhat unusual in pseudocode
    as most algorithms are presented in a functional style, at least
    first before describing some optimizations based on state updates;
    could the description of SmartTrack-DC benefit by first discussing
    it with copying and then later with updates
>>> Not Applicable. I don't think the algorithms or discussions should
be changed to address this feedback.

  - as I'm struggling to follow page 8, particularly lines 778-799,
    which compares SmartTrack-DC with FTO-DC, a question occurs: why
    introduce FTO-DC at all??  is it useful just to easier describe
    SmartTrack-DC? (I'm personally not finding it to be the case)  or
    is FTO-DC useful by itself as one can build on it without going
    into SmartTrack-DC?  could the paper be better *without* FTO-DC?
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

  - section on DC analysis and performance costs interleaves discussion
    of what the analysis does and what the costs are; it may be better
    to separate these by first presenting the analysis and then the costs
    where each cost is tied back to specific line numbers: three paragraphs
    in lines 321-360
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

  - the same discussion of performance costs does not make it clear if
    the order of discussion (those three paragraphs) is based on the
    amount of overhead or on some other criteria (eg, line numbers in
    the pseudocode); it'd help to add here some summary numbers about
    the overhead from the evaluation section
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

  - the entire FTO, at least intuition not formalization, may be
    presented before going into FTO-DC
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

  - Initially, every vector clock maps ... could be by the description
    of each part of the state, or even explicit in algorithm 1
>>> Not Applicable. I don't think the algorithms or discussions should
be changed to address this feedback.

  - uses epoch optimizations to achieve constant time and space ...
    should describe these optimizations here not later
>>> Not Addressed. If it looks nice, an init procedure could be added to each algorithm
but I don't think it is necessary.
>>> \mike{Huh? Is this responding to the comment immediately above or the one before that?}
>>> \jake{The one above. Sorry for the misplacement.}

  - SmartTrack-DC makes the following unrelated change relative to FTO-DC
    ... should describe *why* this is being done
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

* The paper is not self contained in several places; some were already
  listed above; some stem from the presentation trying to compare with
  both DC and WCP in various places (eg, lines 361-369), but WCP is
  never presented fully; maybe WCP optimizations should be presented
  separately rather than being interleaved with the DC optimizations.
  The vindication algorithm should be described in more detail.
>>> Partially Addressed. I expanded the explanation of WCP relation
but not comprehensively as the above feedback suggests.

* Nitpick:

  - deteciton ... misspelled
>>> Addressed.

Questions for Authors
---------------------
* Section 3.1: does applying FTO to DC have some challenges?
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

* Section 3.2: is there some direct analysis of various costs (not indirect from the overhead reduction after optimizations)?
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

* Section 4: why does WDC not find more races than DC? Does it have more false alarms?
>>> Partially Addressed. The discussion on race counts could be expanded once
investigation of counting races by fields is done.


Review #63C
===========================================================================

Overall merit
-------------
C. I would not accept this paper but will not argue strongly against
   accepting it.

Reviewer expertise
------------------
Z. Some familiarity

Paper summary
-------------
This paper presents techniques to improve the performance of predictive data-race detection. The work extends known ideas implemented in the FastTrack data-race detector (for happens-before analysis) to predictive analyses such as does-not-commute and weak-causally-precedes.  It also introduces a new optimization for detecting conflicting critical sections that is specific to predictive analyses.  The optimizations are implemented and show good results.

Comments for author
-------------------
Strengths
- practical motivation

Weaknesses
- Modest novelty
- Hard to understand the core idea (for a non-expert reviewer)

Your paper focuses on improving the performance of DC analysis.  To understand your contribution, the reader needs to fully understand the definition of DC and its unoptimized implementation.  You present both of these in Section 2 but the presentation is cluttered with details about FastTrack optimizations.  In fact, there are three different explanations being interleaved, for HB, DC, and WCP analyses.  I am not an expert and consequently got lost.   Here is a suggestion that would help me out.  HB analysis does not need to be understood until you are presenting your optimizations since they are inspired by HB analysis.  So postpone the explanation of HB. Also since the same idea works for both DC and WCP, just pick DC which appears to be your favorite anyway and run with it.  Have a small section somewhere that talks informally about how the same idea works for WCP.
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

I had difficulty understanding both Definition 3 and Algorithm 1.
- In definition 3, bullet (b) refers to bullets (c) and (d). This is a really odd way to communicate with the reader who hasn't read (c) and (d) when he is reading (b).
>>> Addressed.

- I was not able to connect Algorithm 1 to Definition 3.
>>> Not Applicable.
>>> \mike{What exactly does "Not Applicable" mean (here and in general)? The above seems like a potentially legitimate criticism that could be addressed.}
>>> \jake{Not Applicable -> Not to be addressed. In light of the other feedback,
>>> I did not think this criticism was dire,
>>> but during DC analysis details we could segment (since it mostly done already) Rule a and b into paragraphs
>>> or include Rule a and b comments within Algorithm 1.}

Section 3 presents your contribution.  By your own admission, Section 3.2 is the most novel part of your paper so shouldn't your presentation start with the detection of conflicting critical sections rather than the FastTrack adaptations?
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

Section 4 presents a new partial order called weak-doesn't-commute (WDC).  Section 5.6 in your evaluation makes the point that the weakening of WDC over DC does not buy you much in terms of finding more bugs.  Why even have this thing in the paper then, especially since it is completely  unrelated to your main focus of performance improvement?
>>> Not Applicable.
>>> \mike{We should try to make it more clear what's the point of WDC / why it's a contribution.}
>>> \jake{I agree now and I think we are doing so with the current changes.}

Your evaluation is good.  But I detected a desire to convince the reader that DC analysis could be made just as efficient as HB analysis.  To me, this seems like comparing apples and oranges.  I would be happy enough to see good performance improvements over baseline DC analysis due to your optimizations which you are doing anyway.  Cutting out the DC vs HB analysis would reduce the clutter in the Evaluation section and make it more pointed.
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS


Response by Jake Roemer <roemer.37@osu.edu>
---------------------------------------------------------------------------
We thank the reviewers for their thorough comments, suggestions, and questions.
The detailed and constructive presentation feedback will be particularly helpful for improving the next revision of the paper.
Here we focus on responding to questions and correcting a few misconceptions.

#### Reviewers A and B ask if there are significant challenges in applying FTO optimizations to predictive race detection.

No prior work has applied FastTrack or FTO optimizations to predictive analyses,
but doing so is relatively straightforward.
As the reviewers have noted, the CCS optimizations are the paper's primary intellectual contribution.

#### Reviewer A asks why FTO-HB sometimes finds more static races than SmartTrack-DC. Do the optimizations have limitations? Can the optimizations affect what races are detected?

The FTO and SmartTrack optimizations do not cause reporting of false races or impact detection of the first race in an execution.
While the optimizations all maintain last-access and conflicting critical section (CCS) metadata correctly for
detecting the first race accurately and avoiding all false races,
they differ in how they detect later races, leading to detecting races at different program memory accesses.

These differences explain why FTO-HB sometimes finds more static races than SmartTrack-DC
(although SmartTrack-DC always finds more dynamic races than FTO-HB).
The extra static races found by FTO-HB are generally related to races found by both FTO-HB and SmartTrack-DC
(i.e., an access to the same memory location as an access also reported by both FTO-HB and SmartTrack-DC).

It is difficult in general to compare race detector coverage quantitatively on programs with multiple related races.
One potential solution we will try is to "bin" static races more coarsely, e.g., by class field / array element type
or allocation site of the racing memory location,
which may better highlight the truly unique races found by an analysis.

#### Reviewer B asks about direct measurement of unoptimized analysis costs.

We agree that the paper does not directly measure the cost of the two significant costs of unoptimized DC analysis identified in Section 2.3.
One way to get closer to a direct comparison is to compare three non-SmartTrack configurations: Unopt-DC, FTO-DC, and FTO-HB.
The comparison between Unopt-DC and FTO-DC -- 33x vs. 15x on average (Table 4) -- estimates the cost of using full
vector clocks compared with epoch optimizations.
The comparison between FTO-DC and FTO-HB -- 15x vs. 7.3x -- estimates the cost of detecting conflicting critical sections
because HB analysis eschews this cost and simply orders all critical sections.
>>> \mike{We could provide this analysis in the background/motivation section that describes predictive analysis costs.}
>>> \jake{I agree. I partly incorporated this information into the evaluation.
>>> I think we should add Unopt-DC vs. FTO-DC to section 2.3 or section 2.5 paragraph Vector clocks
>>> and FTO-DC vs. FTO-HB to section 2.5 paragraph DC Rule (a).}

#### Reviewers B and C ask what benefits and drawbacks WDC provides compared with DC.

The benefit of WDC over DC is that WDC analysis is more straightforward than DC analysis, reducing execution time and memory usage.
The drawback of WDC compared with DC is that WDC has a source of unsoundness that DC does not: no DC rule (b).
WDC analysis can thus, in theory, detect false races that DC analysis does not.
However, in our experiments, all WDC and DC analyses detect only true races
(which we verified by vindicating all DC- and WDC-races detected by unoptimized analyses,
then cross-referencing the static races with the DC- and WDC-races reported by optimized analyses).
Overall, WDC analysis provides better performance with an elevated risk of false races compared with DC analysis.



Review #63D
===========================================================================

Overall merit
-------------
A. I will champion accepting this paper.

Reviewer expertise
------------------
X. Expert

Paper summary
-------------
This paper shows how to optimize predictive dynamic race detectors to achieve performance on par with state-of-the-art non-predictive algorithms. In previous work, predictive algorithms were roughly 4x slower than their non-predictive counterparts. The paper contains two optimizations (epoch-ownership and CCS) each of which contribute roughly a factor of 2 to close this gap. While the epoch-ownership optimizations are similar to those applied in existing optimized non-predictive analyses such as FastTrack, the CCS optimization appears novel.

Comments for author
-------------------
## Strengths

- Well-motivated problem statement and well-written overall.
- Thorough evaluation with good baselines. 
- Exciting and somewhat surprising results.

## Weaknesses

(Each weakness is elaborated on further below.)

1. It is not clear that poor performance (30x instead of 8x) is what's preventing developers from using predictive analysis (or from using dynamic race detection at all.)
>>> Not Addressed.

2. The intro leaves it a little unclear that the results are somewhat surprising, given the nature of predictive analysis.
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

3. The paper should clarify (in intro and evaluation sections) that the evaluation shows that the two optimizations each contribute roughly equally to the final speedups.
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

4. The evaluation could use more discussion.
>>> Partially Addressed. Included emphasizing the individual contributions of FTO and CCS
but could be expanded on more.

## Other feedback

- (Weakness 1) Is there any reason to believe that the performance improvements achieved in this paper will have an impact on developers? I think there might be a stronger story here than you're telling.
>>> Not Addressed.
>>> \mike{I think we can address this.}
>>> \jake{This has been addressed in intro, right?}

- (Weakness 2) The paper somewhat undersells the surprising nature of its results. A priori, it might seem like predictive race detectors (even those based on partial orders) must track much more information than HB detectors. Thus it is surprising that similar performance can be achieved.
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

- (Weakness 3) It would be nice if the intro and first half of the paper would call out the roughly equal contribution of the epoch-ownership optimizations and the CCS optimization. I found myself flipping to the evaluation to see whether both were really important, and it turns out they were, so say so!
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS

- (Weakness 4) The evaluation is heavy on data and light on analysis. If there is nothing interesting about the results on individual benchmark (and there is very little in the text to suggest that there is), then Table 6 could move to an appendix.
>>> Partially Addressed. Included emphasizing the individual contributions of FTO and CCS
but could be expanded on more.

## Lower-level suggestions

(Numbers refer to red line numbers in submitted version of paper.)

- 37-38: repetitive "limitation" and "limited"
>>> Addressed.

- 47: Make it clear that you're about to describe two techniques for implementing predictive analysis: SMT and partial order.
>>> Addressed.

- I really appreciated the pseudocode presentation of the algorithms in this paper, as opposed to inference rules. Future implementors will thank you!
>>> Not Applicable.

- 1059: A description of what's going on with sunflow would be a good way to expand the evaluation's discussion of the per-benchmark results!
>>> Addressed.

- 1124: In Table 4, it might be worth emphasizing somehow that the FTO optimizations applied to non-HB are also new to this paper, even if they are not as intellectually novel as the CCS optimizations. Make sure you give yourself credit for 30x vs 8x rather than 15x vs 8x.
>>> Addressed. Included emphasizing the individual contributions of FTO and CCS



LR2 Response by Michael Bond <mikebond@cse.ohio-state.edu>
---------------------------------------------------------------------------
We thank Reviewer D for the feedback and suggestions,
particularly for how to improve and clarify the paper's story,
which we'll incorporate when revising the paper.

#### Reviewer D mentions the performance anomaly for sunflow.

After the submission deadline, we found a bug in our implementation that 
affected FTO-* analyses, but not SmartTrack-* or other analyses. 
(The bug was that each FTO-* analysis incorrectly performed both read-share and read-exclusive logic 
for the read-share case.) After fixing this bug, we found that sunflow's results 
were in line with expected results, i.e., FTO-HB performed similarly to FastTrack2.
We repeated all experiments and found that only sunflow's performance results were 
significantly affected by the bug, and the paper's overall results and story were not 
significantly affected.


==> misc/annotated-pldi-2020-reviews <==
PLDI 2020 Paper #228 Reviews and Comments
===========================================================================
Paper #228 Efficient Predictive Race Detection

>>> \jake{I'm including comments on the changes I have made in response to each Reviewer.} 

Review #228A
===========================================================================

Overall merit
-------------
C. I would not accept this paper but will not argue strongly against
   accepting it.

Reviewer expertise
------------------
X. Expert

Paper summary
-------------
The paper presents several optimisations to the existing
happens-before algorithms for dynamic race detection in concurrent
Java programs. It extends the FastTrack tool with the technique that
allows to prune the search space for races based on the idea of
conflicting critical sections, while using more expensive to analyse
partial even orders, such as weak-casually-precedes and doesn't
commute. The result is the dynamic analysis that combines the
efficiency of predictive data race detection with the speed of
HB-based analyses, while remaining sound. The evaluation compares the
presented analysis to state of the art in terms of speed and memory
usage, and demonstrates some improvements.

Comments for author
-------------------
Strengths:

* As far as one is concerned about dynamic race detection, the paper
  improves on the state of the art in dynamic race terms of
  performance and memory consumption.

Weaknesses:

* The work doesn't improve on the quality of the analysis - SmartTrack
  doesn't report more races than existing WCP and DC-based analyses.

* The paper only presents an ad-hoc argument towards the soundness of
  the analysis. 

Assuming that there is no better way to detect data races in Java
applications than by running a dynamic analysis based on partial
orders of events, this work could be considered as an impressive
improvement on the state of the art, combining the speed of the HB and
the precision of the predictive data race detection. The paper makes a
convincing argument for this, presenting a detailed performance
comparison with respect to previous works in this family of analyses.

However, the paper misses an important related work [1,2] on sound (in
a dynamic analysis sense) _static_ data race detection, which
outperforms the present approach both in terms of speed and precision.
For instance, for `avrora` SmartTrack only reports 6 races, while the
existing static analyses report 92 true races. For `sunflow` it's 19
versus 42. The exact numbers might, indeed, differ depending on which
version of the benchmark is checked, but overall the comparison shows
that static analysis performs consistently better and takes only a few
seconds. 
\mike{Added a paragraph comparing to RacerD and RacerDX based on corresponding the RacerDX authors.}

Therefore, I'd like the authors to argue that, with their
optimisations, there is a tangible benefit of using SmartTrack instead
(or together) with static analysis. For instance, SmartTrack might
detect different classes of races. Unfortunately, the paper doesn't
really present any qualitative discussion on its result, and
exclusively focuses on the performance improvements.

[Addressed]
>>> \jake{Related work has been updated}

Finally, I'm not satisfied with the presentation of the algorithms, as
the soundness argument is carried over by example. Given the existing
formalisations of HB-based race detection tools [3,4], I find it
reasonable to expect that the soundness of presented conservative
optimisations should be formalised.

Overall, without the necessary rigour and with the comparison to the
recent related work missing, I find this paper to be a bit thin on its
contributions to be accepted to PLDI.

>>> \jake{Should we say anything about the above specifically?
\mike{The concern is technically no longer valid because we added the comparison to related work. ;)}}

[1] Sam Blackshear, Nikos Gorogiannis, Peter W. O'Hearn, Ilya Sergey:
    RacerD: compositional static race detection. PACMPL 2(OOPSLA): 144:1-144:28 (2018)

[2] Nikos Gorogiannis, Peter W. O'Hearn, Ilya Sergey:
    A true positives theorem for a static race detector. PACMPL 3(POPL): 57:1-57:29 (2019)

[3] William Mansky, Yuanfeng Peng, Steve Zdancewic, Joseph Devietti:
    Verifying dynamic race detection. CPP 2017: 151-163

[4] James R. Wilcox, Cormac Flanagan, Stephen N. Freund:
    VerifiedFT: a verified, high-performance precise dynamic race detector. PPOPP 2018: 354-367



Review #228B
===========================================================================

Overall merit
-------------
B. I support accepting this paper but will not champion it.

Reviewer expertise
------------------
Y. Knowledgeable

Paper summary
-------------
This paper introduces algorithmic improvements for improving the scalability of
dynamic predictive analyses. These analyses are capable of finding more bugs
than dynamic happens-before analysis but are typically more expensive. It is
impressive that the optimizations in this paper lower this cost to being
competitive with FastTrack.

Comments for author
-------------------
Finding data races is an important problem. Tools like TSan that are (1)
capable of being applied wholesale to a codebase with little programmer
attention and (2) precise are extremely useful for the working programmer.
The work in this paper offers a way to extend the capability of dynamic data
race detection, using predictive analyses, but without sacrificing (too much)
performance. If these methods were incorporated into a tool for concurrent C
code then I would be keen to use them!

The paper builds from a clear description of happens-before analysis into
predictive analyses and then the main technical contributions: a weaker partial
order WDC and SmartTrack = epoch+ownership optimizations and conflicting
critical section optimizations. 

Weaknesses: The cost of all of these optimizations is that Algorithm 3 is much
more complex and harder to understand than the naive Algorithm 1. How do we
know that these optimizations only effect the performance, rather than the
precision of the analysis? The experimental evaluation is good evidence, but
what would be even better would be a proof of correctness.

>>> \jake{I'm not sure how soundness should be handled.}

Overall, this is a solid paper with contributions to an important problem that
I think is to the standard of PLDI.

Additional feedback:
  - In Sec 5 (results), I could not find a discussion of how many extra reports
    were flagged as a result of WDC analysis compared to DC analysis. This
    would be useful in light of the comment in Sec 3 about "few if any false races
    in practice".
    
[Addressed]
>>> \jake{Changed the comment in Sec 3 about "few if any false races in practice" to:
However, \CAPO analysis detects few if any false races in practice and
our evalution shows that despite \CAPO being weaker than \DC,
\CAPO analysis does \emph{not} report more races than \DC analysis.} 

  - Do the DC and WDC rows of Table 5 including the runtime for vindication?

[Addressed]  
>>> \jake{Updated paper to clarify that the Evaluation section does not include costs for vindication}

  - In Sec 5.5 'SmarkTrack thus enable three kinds of predictive analysis, each
    offering a different coverage-soundness tradeoff'. How do you imagine a
    programmer taking use of these tradeoffs?

[Addressed]
>>> \jake{Included the rebuttal response in the Summary subsection of Evaluation.} 

Minor:
  - Def 1(a). Does `CS(r)` include `r`? And does it also include its
    corresponding acquire `a` event?

[Addressed]
>>> \jake{Expanded CS(r) definition to be inclusive for r and a.}

  - The order of WCP and DC in the paper changes. Sometimes it is 'DC and WCP'
    and other times vice-versa. It would be less taxing (as a reader) if the
    paper fixed on a particular order.

[Addressed]
>>> \jake{Picked the order of HB, WCP, DC, and then WDC and enforced it in the paper.}

  - Consider highlighting the differences in Algorithm 2 from Algorithm 1 and,
    also, Algorithm 3 from Algorithm 2 to help the reader concentate on what's
    important.

[Addressed]
>>> \jake{Added grey highlighting to signify differences between Algo 1 and 2 and Algo 2 and 3.}

Review #228C
===========================================================================

Overall merit
-------------
B. I support accepting this paper but will not champion it.

Reviewer expertise
------------------
Y. Knowledgeable

Paper summary
-------------
The paper proposes optimizations to make predictive race detection more time and space efficient. 
The optimized race detector, SmartTrack, incorporates epoch and ownership techniques from prior 
work in the partial-order analyses. It proposes a novel optimization to track conflicting 
ritical sections. Together, they are shown to reduce the space and time overhead of performing 
predictive race detection.

Comments for author
-------------------
The use of vector clocks and further optimizations like epochs have helped make 
happens-before (HB) analysis more practical. However, HB based race detection can miss certain 
data races. The predictive race detectors work with weaker relations than HB and avoid this 
problem. This paper shows that epoch and ownership optimizations can be applied to predictive 
race detectors based on doesn't-compute (DC) and weak-causally-precedes (WCP) relations. It also 
proposes a weaker notion of DC.

The main contribution of the paper is the new constructions for detecting conflicting critical 
sections (CCS) more efficiently. Unfortunately, the paper presentation became too dense by the 
time I reached this part -- there are multiple algorithmic variants and associated data structures. 
Despite my best efforts and past experience in race detection, I was unable to fully understand 
the exact construction, and the motivation and use of the required meta-data. Though the paper 
seems sound, I am unable to be completely sure of it. The example in Figure 3 also did not help me. 

In my view, the authors spend too much space in building the background concepts and showing their 
contributions incrementally. The authors could instead directly start with an example (or even a 
series of examples), e.g., something parameterized so that the growth of space and time can be 
argued easily, and then explain the optimizations, with emphasis on the CCS related optimization. 
The comparison with other methods and extensions to DC, etc. can be delegated to later sections or 
even an appendix.

The experimentation is thorough and shows impressive results. The authors have clearly spent 
significant efforts here. I am therefore in favor of accepting the paper if any other reviewer 
is confident of the technical content. I would still worry about the accessibility of the work 
to the larger audience.

[Addressed]
>>> \jake{Used example from Figure 4(a) as the running example.
Added example description for Unopt-DC and FTO-DC.}


Review #228D
===========================================================================

Overall merit
-------------
B. I support accepting this paper but will not champion it.

Reviewer expertise
------------------
X. Expert

Paper summary
-------------
This paper proposes a novel optimization technique, called conflicting critical section (CCS), 
as well as several other optimizations of existing but relatively new techniques, 
such as DC and WCP, as well as porting of an optimization from an industrial strength HB race 
detector called FastTrack.  All these together bring the performance of predictive race analysis 
close to the performance of HB analysis engineered in FastTrack, but with the increased 
predictive capability.  That is, more data-races are detected from one execution of the 
program that with FastTrack, at a comparable performance.

Comments for author
-------------------
Dynamic data race detection continues to be an important problem in the PL field and this 
paper makes another step ahead.  The paper is well written, the algorithms are well presented, 
and the challenges are properly explained.  The appendix shows detailed measurements of 
performance on the various Dacapo programs.  All in all, a good paper.  I cannot find any 
technical problems, not even typos or grammar issues.  The title is a bit too pretentious, though.  
Add "SmartTrack" in it, or SCC, to make it more specific to what you do in the paper?

[Addressed]
>>> \jake{'SmartTrack: ' has been added to the title.}

My main reservation is that you are only using Dacapo for experiments, which was not even 
conceived for data-races.  How about JavaGrande?  Or off-the-shelf Java applications, 
like Hadoop?  Missing such other applications makes the reader think that you may only have 
a rough prototype and not a well engineered implementation, which would decrease the value 
of such a nice engineering paper.  The lack of a discussion about instrumentation adds to 
that worry.  Indeed, implementing an efficient instrumentation to do all the data-race analysis 
online, as opposed to post-mortem on a logged trace, is a very challenging problem, almost as 
challenging as the data-race algorithm itself.

Can you explain how you collected the traces and whether your implementation is indeed 
online or not?

[Addressed]
>>> \jake{Mentioned all analyses are online and don't collect traces in Implementation subsection
using the rebuttal text.}

I would avoid calling your SCC contribution "intellectual".  It sounds strange.  You can admit 
upfront that this is an engineering paper, with the clear objective of making existing 
techniques work together and further optimize where opportunities arise, like the SCC.

[Addressed]
>>> \jake{Changed 'intellectual' to 'technical'}

You appear optimistic regarding record & replay tools; have you tried them?  Were you able 
to generate a record log from a predicted trace, and then replay it?

[Addressed]
>>> \jake{Added the following to Vindication subsection.
Admittedly we haven't since it is beyond the scope of this paper. 
The recent practical multithreaded record & replay tools
iReplayer [43] and Castor [49] both target C/C++ programs.}

Finally, there is also some worry that your own implementation of FastTrack is not as 
efficient as the actual industrial tools.  I know you needed your own implementation in order 
to compare the techniques on the same trace, but this is still a worry.  We've seen it in 
the past where unfair claims were made this way.

==> misc/oopsla-2019-rebuttal <==
We thank the reviewers for their thorough comments, suggestions, and questions.

# High-Level Response

Here we address the main high-level feedback, and later we respond to all questions and suggestions in detail.

#### Reviewer A asks why SmartTrack-based analyses do not improve performance over corresponding FTO-based analyses for some programs.

Investigating this issue, we have found that our implementation of "extra metadata" ($E_x$) incurs nontrivial performance overheads even when the extra metadata is rarely or never used. In particular, each program variable $x$'s metadata is initialized with two empty hash maps for $E^r_x$ and $E^w_x$, leading to significant memory and run-time overhead.

In preliminary experiments,
initializing these fields to null (and creating a map only when needed) eliminates the performance anomaly between SmartTrack and FTO, actually improving the performance of SmartTrack-based analyses noticeably (by 6–9% run time and 31–33% memory usage on average).
We'll collect full updated results for the next version of the paper.

#### Reviewer A asks whether we'll make our implementation publicly available and open source.

Yes; we'll publish it on GitHub and provide a link in the final paper if accepted.

#### Reviewer C asks about the tradeoff between running HB analysis on more traces versus running predictive analysis on fewer traces given a fixed time budget.

Evaluating analysis effectiveness across multiple executions is admittedly beyond the scope of the paper. A key challenge is the plethora of different options for choosing multiple executions. Simply re-executing a program natively is likely to expose a similar set of HB-races, while an advanced race-exposing technique could potentially expose HB-races effectively, but likely at a higher cost. We'll discuss this issue in the paper.

We emphasize that our optimized DC and WDC analyses do *not* perform vindication. They instead report DC- and WDC-races (which are generally true races in practice) without vindication; or they can use record & replay techniques to replay an execution and collect enough information to perform vindication.

# Detailed Response

### Review A

> Cons: From about the middle of section 2.4 through section 4.2, I found the paper very difficult to
> read, probably due to the high ratio of formulae to plain English. The authors should revise the paper
> to explain the various kinds of analyses, and their composites, more simply and intuitively with prose
> (and examples!) separate from the formulae. Although hotcrp says the authors intend to submit an
> artifact, I was unable to find anywhere in the paper that states that the authors plan to make the
> implementation available open-source (but I may have missed it).

As mentioned above, we'll open-source our implementation.

We'll revise significantly to make the explanations more intuitive as the reviewer suggests.

> The contributions paragraph on page 2 says 
> "We realize *the last two contributions* in SmartTrack, 
> a new algorithm for optimized partial-order-based predictive analysis, 
> including the existing WCP and DC analyses and the new WDC analysis." (emphasis added) 
> This wording is confusing.  
> But it looks to me like SmartTrack includes all three of the optimizations, 
> which together constitute the second and third contributions, 
> and seems to also incorporate the weakly-doesn't-commute analysis part of the first contribution.  
> The authors should clarify.

The paper introduces three optimizations:

1. The weak-doesn't-commute (WDC) relation and analysis
2. Epoch and ownership optimizations
3. Conflict critical section (CCS) optimizations

SmartTrack represents Contributions 2 and 3. SmartTrack is orthogonal to WDC: SmartTrack can be applied to WDC analysis and other predictive analyses. We'll clarify in the next revision.

> It looks like SmartTrack does not always improve on FTO-{WCP|DC|WDC}, 
> e.g., jython, sunflow, and tomcat show higher overhead for both runtime and memory usage, 
> and there's higher memory usage for lusearch (just DC) and pmd.  Why is this?  
> There is discussion in 5.6 about apparent and actual anomalies for race detection, 
> but no analogous discussion for overhead.
> The paper would be stronger if the authors found, and presented, 
> the cause of the unexpectly low race counts for jython using FTO-WCP.

See our response in "High-Level Response" above.

> The paper does not explain how all the different implementations 
> (or perhaps options within the same implementation?) were tested for semantic bugs, 
> what the development effort involved, lines of code, and so on, 
> which I typically see in "my tool runs fast" papers.
> In any case, the implementation should be made available open-source 
> for other researchers to build on.

As mentioned above, we'll open-source our implementation, which consists of a RoadRunner tool and minor modifications to RoadRunner. We can describe in the text how we developed and sanity checked the implementation.

### Review B

> The paper says that the performance is comparable to HB 
> and gives a large number of evaluation tables. 
> However the text doesn't give headline figures. 
> For each of your three sets of optimisations how much did they help up the performance.
> Do different kinds of programs benefit differently and if so how and why?

We'll answer these questions in the text, including giving headline figures. Here we also give answers briefly.

The individual optimizations help performance in the following ways:
1. WDC analysis speeds up execution time by 1.1–1.2x compared with DC analysis.
2. Epoch and ownership optimizations (FTO-*) speed up execution time by 1.9–3.0x compared with unoptimized analyses.
3. CCS optimizations speed up execution by 1.5–1.6x compared with FTO-based analyses.

All programs generally benefit from epoch and ownership optimizations, which avoid full vector clock operations. Programs that perform many accesses holding one or more locks (see Table 2) benefit more from CCS optimizations.

> Line 63 says there are 3 major sources of poor performance. 
> What are the poor performance issues that the second and third optimisation provide? 
> If they aren't obvious then perhaps you should start the paragraph by 
> saying there are 3 ways we can improve the performance? 
> After introducing each of these kinds of optimisations can you also say 
> what kind of speedup each one provides? 
> (e.g between x% and y% improvement or approx z% improvement).

The first source of poor performance is DC's release–release ordering. WDC analysis addresses this issue.

The second source of poor performance is performing full vector clock operations. Epoch and ownership optimizations address this issue.

The third source of poor performance is detecting and handling conflicting critical sections. CCS optimizations address this issue.

We'll clarify these sources of poor performance and corresponding optimizations upfront in the paper and state corresponding speedups.

> Line 408 - could you explain/justify the statement in the paragraph?

Only the latest write and latest reads since the last write are necessary for detecting the first race soundly, as justified in FastTrack [Flanagan and Freund 2009] and FastTrack-Ownership [Wood et al. 2017]. Intuitively, if there's no race with the last write and the current access, then either (1) the current access doesn't race with any earlier writes or (2) the last write races with an earlier write (which would have been detected earlier). A similar argument applies to some reads. We'll explain this in the text.

> Line 805 - what is the advantage of continuing after finding a race?

In practice, industry-standard race detectors continue detecting races after the first race in order to report more races to users. Furthermore, continuing after the first race allows us to run our analyses on full executions and collect performance and race coverage results.

> Line 1027 - Can you try to include the reasons in the final publication?

We haven't figured it out yet, but we'll try to include it.

> Line 1102 - state why you want predictive analysis rather than just HB in the conclusions. 
> That is state something about not finding races and finding false races.

We'll revise as suggested.

### Review C

> Where this paper is lacking is that the evaluation does not draw any conclusions 
> as to whether the more expensive analyses are worth using instead of the HB analysis.  
> For example, given a fixed time budget, which analysis finds the largest number of static races?
> Does it make sense to run the HB analysis on more traces or the WCP analysis on fewer traces?
> Moreover, what is the overhead of the vindication procedure that DC and WDC require?
> Taking that into account, does it (still) make sense to use these techniques?
> (I understand that these questions are somewhat orthogonal to the contribution of the paper, 
> which is to optimise algorithms XYZ, 
> but I think they are very important for a reader of the paper to understand 
> whether these algorithms are now worth implementing/using.)

See our response in "High-Level Response" above.

> 42: "Alternatively" - alternative to what?

Alternative to partial-order-based predictive analysis.
We'll clarify the text.

> 391: sound -> unsound.
> 
> 466: $R_x = C(t)$ -> $R_x = C_t(t)$

Thanks, we'll correct these typos.

> 981-995: Do you have any explanation about the different number of races found 
> in the unoptimised and optimised versions of a given algorithm,
> when statistically significant, e.g., pmd and xalan?

As Lines 1046-1048 explain,
the differences in number of races are attributable to
the unoptimized and optimized analyses having different behavior after detecting the first race
due to their different representations of last-access metadata.

### Review D

> Besides the above, I wonder why the authors distinguish 
> happens-before from "predictive analysis".  
> Isn't happens-before also a predictive analysis technique?  
> It has a lower prediction capability, 
> but falls into the same category as the other predictive runtime analysis techniques, 
> that is, from one execution we can predict other executions.

We agree, but the literature generally distinguishes "predictive analysis" as being able to find strictly more races than HB analysis. We'll make this more evident in the text.

> Dacapo is not necessarily a great benchmark for data-races; 
> it would be more convincing to use SmartTrack on some large concurrent real-life Java programs.

DaCapo consists of real, widely used concurrent programs that are well suited to evaluating performance and that also contain data races.
We recognize that the DaCapo suite is not expressly intended for evaluating data race detection,
and we'll mention that in the paper.


*********** INTERNAL NOTES ****************

Evaluating multiple distinct traces, systematically or intelligently, 
using the analyses mentioned in this paper is out of the scope of this paper.
It is not conclusive from our evaluation that more static races will be reported
by HB analysis or predictive analysis within a fixed time budget.

Future work could investigate the effectiveness of thread scheduling using
the analyses mentioned in this paper on the same program.

\jake{I finished collecting 10 trials for the new results we looked at in the last meeting (previously only 5 trials).
I added performance improvement percentages over the results in the submitted results for WCP (10.64% run and 32.73% mem), DC (10.42% run and 30.9% mem), and WDC (16.87% run and 35.79% mem).
The "extra" change improved performance over the w/o setting core results (tables we were comparing during our meeting) by roughly 6%-9% (WCP 5.62%, DC 8.51%, WDC 6.76%) run time and 31%-33% (WCP 32.73%, DC 30.91%, WDC 31.46%) memory usage on average.
I'm not sure which you intended to base the improvement upon.}



==> misc/pldi-2019-rebuttal <==
We thank the reviewers for their thorough comments, suggestions, and questions.
The detailed and constructive presentation feedback will be particularly helpful for improving the next revision of the paper.
Here we focus on responding to questions and correcting a few misconceptions.

### Reviewers A and B ask if there are significant challenges in applying FTO optimizations to predictive race detection.

No prior work has applied FastTrack or FTO optimizations to predictive analyses,
but doing so is relatively straightforward.
As the reviewers have noted, the CCS optimizations are the paper's primary intellectual contribution.

#### Reviewer A asks why FTO-HB sometimes finds more static races than SmartTrack-DC. Do the optimizations have limitations? Can the optimizations affect what races are detected?

The FTO and SmartTrack optimizations do not cause reporting of false races or impact detection of the first race in an execution.
While the optimizations all maintain last-access and conflicting critical section (CCS) metadata correctly for
detecting the first race accurately and avoiding all false races,
they differ in how they detect later races, leading to detecting races at different program memory accesses.

These differences explain why FTO-HB sometimes finds more static races than SmartTrack-DC
(although SmartTrack-DC always finds more dynamic races than FTO-HB).
The extra static races found by FTO-HB are generally related to races found by both FTO-HB and SmartTrack-DC
(i.e., an access to the same memory location as an access also reported by both FTO-HB and SmartTrack-DC).

It is difficult in general to compare race detector coverage quantitatively on programs with multiple related races.
One potential solution we will try is to "bin" static races more coarsely, e.g., by class field / array element type
or allocation site of the racing memory location,
which may better highlight the truly unique races found by an analysis.

#### Reviewer B asks about direct measurement of unoptimized analysis costs.

We agree that the paper does not directly measure the cost of the two significant costs of unoptimized DC analysis identified in Section 2.3.
One way to get closer to a direct comparison is to compare three non-SmartTrack configurations: Unopt-DC, FTO-DC, and FTO-HB.
The comparison between Unopt-DC and FTO-DC -- 33x vs. 15x on average (Table 4) -- estimates the cost of using full
vector clocks compared with epoch optimizations.
The comparison between FTO-DC and FTO-HB -- 15x vs. 7.3x -- estimates the cost of detecting conflicting critical sections
because HB analysis eschews this cost and simply orders all critical sections.

#### Reviewers B and C ask what benefits and drawbacks WDC provides compared with DC.

The benefit of WDC over DC is that WDC analysis is more straightforward than DC analysis, reducing execution time and memory usage.
The drawback of WDC compared with DC is that WDC has a source of unsoundness that DC does not: no DC rule (b).
WDC analysis can thus, in theory, detect false races that DC analysis does not.
However, in our experiments, all WDC and DC analyses detect only true races
(which we verified by vindicating all DC- and WDC-races detected by unoptimized analyses,
then cross-referencing the static races with the DC- and WDC-races reported by optimized analyses).
Overall, WDC analysis provides better performance with an elevated risk of false races compared with DC analysis.

%%%%%%%%%%%%%%%% NOTES %%%%%%%%%%%%%%%%%%%%%%

The races reported in Table 13 shows FTO-HB finds as many or more races than other FTO-* and ST-* analyses.
A limitation within the implementation of the proposed optimizations, 
not the optimizations themselves,
is in applying the best effort approach for ordering racing accesses
and in the method of identifying and grouping races.
\mike{It's an experimental issue, not an implementation, right?}

The FTO-* and ST-* analyses use epoch and ownership analysis state
to update and order accesses at a racing event.
The analyses can only guarantee to order the shortest race without full vector clock information,
thus only guaranteeing that every analysis detects the same first race but will differ in detecting subsequent races.

Every analysis evaluated in the paper identifies races using only the information 
at the site of the second, later within the observed execution, racing access to reduce memory overhead.
Identifying races using second site information limits the number of static races detected,
two static races may be identified as the same static race based on the second racing access alone
but does not affect the number of dynamic races.

\mike{I think much of the above two paragraphs may be lost on the reviewer.}

Additionally, a truly fair comparison of static race counts 
requires that each analysis analyze the same observed execution trace.
Our experiments evaluate each analysis on a different execution trace.
\mike{This can go either way in terms of helping or hurting our case.}

Table 13 provides event type counts which correspond to the performance improvements seen
in Table 5 and Table 6 when comparing Unopt- analyses to FTO- analyses.
Table 2 provides counts for lock events which correspond to performance improvements also seen
in Table 5 and Table 6 when comparing FTO- analyses to ST- analyses.
\jake{Should the above stay or be removed?
\mike{Removed, I think}}

\jake{I do not think the following should be included, but maybe it is an important point to address
\mike{There's something to be said for correcting clear misunderstandings (e.g., helps avoid spread of misinformation).}}
#### Reviewer B suggests clarifying soundiness

The use of sound when discussing sound analyses refers to 
a relation or analysis being sound if it finds no race for every execution trace that has no predictable race.
The analyses evaluated in the paper conform to soundiness as a limitation of RoadRunner
which does not provide support for all types of possible synchronization.
\mike{Isn't the main issue that the reviewer thinks sound means no false negatives,
but sound in our paper means no false positives?}

#### Reviewer B asks about the significance of the CCS optimization contribution

The CCS optimization is a significant contribution theoretically and empirically.
The FTO optimizations improve the costs for access events where
the CCS optimizations improve the costs for lock events.
Since predictive partial order analyses require expensive analysis state updates at lock events
the CCS optimizations provide the critical performance improvements necessary for predictive analyses
to be competitive with optimized HB analysis.
Table 2 emphasizes this point by showing the impact, number of, of lock events on the evaluated benchmarks
The impact of these lock event counts can be seen in Table 5
with the significant improvements in performance for h2, luindex, and xalan
comparing FTO- and ST- optimizations.
\mike{I'm not sure what you mean or where you think the reviewer's asking this.
In any case, the answer reads as sort of unhelpful to a reviewer who's genuinely asking/confused, and
the contribution significance would usually be intellectual, not empirical.}
\jake{I reworded Reviewer B's comment about the "second significant cost".
I reworded this answer. Can you review and comment again?}
\mike{I don't think the reviewer is asking about the significance of the CCS optimization contribution.}


==> misc/pldi-2019-rebuttal-2 <==
\jake{I'm adding a lot here, but I mostly stand behind the response addressing sunflow.
Anything in notes I feel was addressed in the first rebuttal}

We thank Reviewer D for the feedback and suggestions,
particularly for how to improve and clarify the paper's story,
which we'll incorporate when revising the paper.

#### Reviewer D mentions the performance anomaly for sunflow.

After the submission deadline we found a bug in our implementation that 
affected FTO-* analyses, but not SmartTrack-* or other analyses. 
(The bug was that each FTO-* analysis incorrectly performed both read-share and read-exclusive logic 
for the read-share case.) After fixing this bug, we found that sunflow's results 
were in line with expected results, i.e., FTO-HB performed similarly to FastTrack2.
We repeated all experiments and found that only sunflow's performance results were 
significantly affected by the bug, and the paper's overall results and story were not 
significantly affected.

%%%%%%%%%%%%%%%% NOTES %%%%%%%%%%%%%%%%%%%%%%

Repeating the experiments in the paper with the fix to the FTO-* analyses
has resulted in the geometric mean of the run time performance between FTO-HB and ST-WDC
changing from 7.3x (FTO-HB) vs. 7.7x (ST-WDC) to 7.0x (FTO-HB) vs. 8.2x (ST-WDC).
Overall, the error has weakened the impact of ST-WDC performance compared to FTO-HB,
but has not weakened the impact of the performance improvement of CCS optimization.
\mike{Why has the run time of ST-WDC changed from 7.7X to 8.2X if the bug didn't affect SmartTrack?}
\mike{In any case, I think we can omit numbers (i.e., omit the above paragraph);
also, then it looks less like we're trying to give new results after the deadline. :) }
\jake{Yeah. I agree. The changes look solid to me. I'm ready to submit if you are.}

Further investigation of sunflow revealed an error in the specific case of 
updating fast path read-share case to read-exclusive.

### Reviewer D asks if the performance improvements to predictive analysis will have an impact on developers.
\jake{(Weakness 1)}
Our contribution advances state-of-the-art predictive dynamic data race detectors.
However, we recognize this is not a solved area with a tool
that will convince developers to use data race detectors more.  

### Reviewer D asks to clarify the additional complexity of predictive analyses (partial-order-based) compared to HB analysis.
\jake{(Weakness 2)}
Partial-order-based analysis discussed in the paper require additional
analysis state to track conflicting accesses within critical sections.
This analysis state is strictly larger than the analysis state tracked by HB analysis
that lends itself to optimizations that follow similar ideas to epoch and ownership optimizations.

- (Weakness 3) It would be nice if the intro and first half of the paper would call out the 
roughly equal contribution of the epoch-ownership optimizations and the CCS optimization. 
I found myself flipping to the evaluation to see whether both were really important, 
and it turns out they were, so say so!
\jake{The above weakness is similar to asking about direct measurement costs,
which we address as #### Reviewer B asks about direct measurement of unoptimized analysis costs,
but being introduced earlier in the paper. 
We could direct the question to the already submitted author response or leave out addressing this weakness.}


- (Weakness 4) The evaluation is heavy on data and light on analysis. 
If there is nothing interesting about the results on individual benchmark 
(and there is very little in the text to suggest that there is), 
then Table 6 could move to an appendix.
\jake{The above weakness relates to most or all of the points made in the first author response.
Should we combine Weakness 3 and 4 with a redirect to the first author response?}

==> misc/pldi-2020-rebuttal <==
We thank the reviewers for their thorough feedback.
We'll address the reviewer's presentation and other suggestions when revising.
Here we focus on responding to reviewer questions.

### Reviewer A asks about the comparison with prior work on static race detection
[Blackshear et al. OOPSLA'18] [Gorogiannis et al. POPL'19].

Thanks for the references to prior work; we'll add discussion of them in the text.
RacerDX [POPL'19] in particular is impressive in that it reports
provably no false races.
Our current reading is that RacerDX's race reports and access paths
(result table's "DX Reps" and "DX #$\pi$" columns in [POPL'19])
are counting races differently from how we count SmartTrack-reported races
(distinct static code locations at which a race is detected). The RacerDX paper states that
"[a]n access path may be accessed at a set of locations.
In the worst case where [all] these accesses are racy,
we may end up with a number of reports that is quadratic in the number of locations."
We'll figure out the exact race-counting methodology used by RacerDX, by contacting the authors if needed,
before the next version of the paper.
It would be interesting to compare directly the races reported by RacerDX and SmartTrack
and measure the degree of overlap.

### Reviewer B asks about WDC analysis race counts compared to DC analysis race counts.

In our experiments, all WDC and DC analyses detect only true races.
We verified this result by cross-referencing all of the static races reported by these optimized analyses
with DC- and WDC-races that were detected and vindicated by unoptimized analyses.

### Reviewer B asks if the DC and WDC rows of Table 5 include the run time for vindication.

Table 5's results do not include vindication's run time;
for a fair comparison, none of the analyses build constraint graphs or perform vindication.
Table 8 in the submitted supplementary material includes results with and without vindication enabled for
unoptimized DC and WDC analyses.

### Reviewer B asks how programmers would choose among analyses with different coverage-soundness-performance tradeoffs.

It depends mainly on a programmer's tolerance for the possibility of false races
(or: deploying with record & replay would allow vindicating reported DC- or WDC-races) and
the observed differences among the analyses for the programmer's application.

### Reviewer C makes several suggestions for improving the presentation.

We'll apply the reviewer's suggestions when revising, e.g.,
driving the exposition with analysis examples.

### Reviewer D suggests changing the title.

Sure, we'll add "SmartTrack" or something else specific to the title.

### Reviewer D asks how traces were collected and whether the implementation is online.

Our analysis implementations try to minimally extend the existing FastTrack
analysis that is part of the publicly available RoadRunner implementation.
Every analysis evaluated in the paper is online.

### Reviewer D asks if we have tried record & replay tools.

Admittedly we haven't. The recent practical multithreaded record & replay tools
iReplayer [43] and Castor [49] both target C/C++ programs.

=============================== NOTES ===================================

### Reviewers A, B, and C express concern about the lack of a proof of soundness for the SmartTrack optimizations.

\jake{I'm not sure how to address this one.
Should we attempt to include a proof or argue that one is not needed for this paper?
\mike{I don't think we have a good response (so we should just omit this Q&A from the response).
We don't have time to do a proof,
we probably shouldn't say we'll do a proof for the final paper, and
saying we don't need a proof is arguing with the reviewers on a subjective (and good) point.}
\mike{To do a correctness proof I guess we'd want to start with formalizing the algorithm,
as FastTrack does using operational semantics, then try to prove it finds a DC-race iff one exists.}}

Reviewer A says:
Finally, I'm not satisfied with the presentation of the algorithms, as
the soundness argument is carried over by example. Given the existing
formalisations of HB-based race detection tools [3,4], I find it
reasonable to expect that the soundness of presented conservative
optimisations should be formalised.

Reviewer B says:
Weaknesses: The cost of all of these optimizations is that Algorithm 3 is much
more complex and harder to understand than the naive Algorithm 1. How do we
know that these optimizations only effect the performance, rather than the
precision of the analysis? The experimental evaluation is good evidence, but
what would be even better would be a proof of correctness.

Reviewer C says:
Despite my best efforts and past experience in race detection, I was unable to fully understand 
the exact construction, and the motivation and use of the required meta-data. Though the paper 
seems sound, I am unable to be completely sure of it. The example in Figure 3 also did not help me.

### Reviewer B asks if `CS(r)` includes `r` and corresponding `a` events.

Yes, `CS(r)` includes both `r` and `a` events.

### Reviewer D says:
My main reservation is that you are only using Dacapo for experiments, which was not even 
conceived for data-races.  How about JavaGrande?  Or off-the-shelf Java applications, 
like Hadoop?  Missing such other applications makes the reader think that you may only have 
a rough prototype and not a well engineered implementation, which would decrease the value 
of such a nice engineering paper.  The lack of a discussion about instrumentation adds to 
that worry.  Indeed, implementing an efficient instrumentation to do all the data-race analysis 
online, as opposed to post-mortem on a logged trace, is a very challenging problem, almost as 
challenging as the data-race algorithm itself.
Can you explain how you collected the traces and whether your implementation is indeed 
online or not?



==> old-result-tables.tex <==
%%% Run-Time Performance
\begin{table*}[t]
\begin{minipage}{1\textwidth}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_slowTool_raceLimitFix_assertCheck}
%
\small
\centering
\begin{tabular}{@{}l|rl|rl||r|Hrrr|rr|rr}
& \mc{2}{c|}{} & \mc{2}{c||}{} & & \mc{8}{c}{\SlowTool: Slowdown (normalized to Base time)} \\
& \mc{2}{c|}{} & \mc{2}{c||}{} & Base & \mc{4}{c|}{} & \mc{2}{c|}{\DC} & \mc{2}{c}{\CAPO} \\
Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & time & Empty & \FT & \HB & \WCP & w/o G & w/ G & w/o G & w/ G \\\hline 
\bench{avrora} 	& \et{\SLOWavroraEvents}   & \enfp{\SLOWavroraNoFPEvents}	& \SLOWavroraTotalThreads 	& (\SLOWavroraMaxLiveThreads)	& \base{\SLOWavroraBaseTime}   & \roh{\SLOWavroraEmptyTime}   & \roh{\SLOWavroraFTTime}		& \roh{\SLOWavroraHBTime}	& \roh{\SLOWavroraWCPTime} 	& \roh{\SLOWavroraWDCnoGTime} 	& \roh{\SLOWavroraWDCTime} 	& \roh{\SLOWavroraCAPOnoGTime}	& \roh{\SLOWavroraCAPOTime} \\
\bench{batik} 	& \et{\SLOWbatikEvents}    & \enfp{\SLOWbatikNoFPEvents}	& \SLOWbatikTotalThreads 	& (\SLOWbatikMaxLiveThreads)	& \base{\SLOWbatikBaseTime}    & \roh{\SLOWbatikEmptyTime}    & \roh{\SLOWbatikFTTime}		& \roh{\SLOWbatikHBTime}	& \roh{\SLOWbatikWCPTime} 	& \roh{\SLOWbatikWDCnoGTime} 	& \roh{\SLOWbatikWDCTime}	& \roh{\SLOWbatikCAPOnoGTime}	& \roh{\SLOWbatikCAPOTime} \\
\bench{h2} 		& \et{\SLOWhtwoEvents}     & \enfp{\SLOWhtwoNoFPEvents}	    & \SLOWhtwoTotalThreads 	& (\SLOWhtwoMaxLiveThreads)	    & \base{\SLOWhtwoBaseTime}     & \roh{\SLOWhtwoEmptyTime}     & \roh{\SLOWhtwoFTTime}		& \roh{\SLOWhtwoHBTime}		& \roh{\SLOWhtwoWCPTime} 	& \roh{\SLOWhtwoWDCnoGTime} 	& \roh{\SLOWhtwoWDCTime}	& \roh{\SLOWhtwoCAPOnoGTime}	& \roh{\SLOWhtwoCAPOTime} \\
\bench{jython} 	& \et{\SLOWjythonEvents}   & \enfp{\SLOWjythonNoFPEvents}	& \SLOWjythonTotalThreads	& (\SLOWjythonMaxLiveThreads)	& \base{\SLOWjythonBaseTime}   & \roh{\SLOWjythonEmptyTime}   & \roh{\SLOWjythonFTTime}		& \roh{\SLOWjythonHBTime}	& \roh{\SLOWjythonWCPTime} 	& \roh{\SLOWjythonWDCnoGTime} 	& \roh{\SLOWjythonWDCTime}	& \roh{\SLOWjythonCAPOnoGTime}	& \roh{\SLOWjythonCAPOTime} \\
\bench{luindex} & \et{\SLOWluindexEvents}  & \enfp{\SLOWluindexNoFPEvents}	& \SLOWluindexTotalThreads	& (\SLOWluindexMaxLiveThreads)	& \base{\SLOWluindexBaseTime}  & \roh{\SLOWluindexEmptyTime}  & \roh{\SLOWluindexFTTime}	& \roh{\SLOWluindexHBTime}	& \roh{\SLOWluindexWCPTime} & \roh{\SLOWluindexWDCnoGTime} 	& \roh{\SLOWluindexWDCTime}	& \roh{\SLOWluindexCAPOnoGTime}	& \roh{\SLOWluindexCAPOTime} \\
\bench{lusearch}& \et{\SLOWlusearchEvents} & \enfp{\SLOWlusearchNoFPEvents}	& \SLOWlusearchTotalThreads	& (\SLOWlusearchMaxLiveThreads)	& \base{\SLOWlusearchBaseTime} & \roh{\SLOWlusearchEmptyTime} & \roh{\SLOWlusearchFTTime}	& \roh{\SLOWlusearchHBTime}	& \roh{\SLOWlusearchWCPTime}& \roh{\SLOWlusearchWDCnoGTime}	& \roh{\SLOWlusearchWDCTime}& \roh{\SLOWlusearchCAPOnoGTime}& \roh{\SLOWlusearchCAPOTime} \\
\bench{pmd} 	& \et{\SLOWpmdEvents}      & \enfp{\SLOWpmdNoFPEvents}      & \SLOWpmdTotalThreads	    & (\SLOWpmdMaxLiveThreads)	    & \base{\SLOWpmdBaseTime}      & \roh{\SLOWpmdEmptyTime}      & \roh{\SLOWpmdFTTime}		& \roh{\SLOWpmdHBTime}		& \roh{\SLOWpmdWCPTime} 	& \roh{\SLOWpmdWDCnoGTime} 		& \roh{\SLOWpmdWDCTime}		& \roh{\SLOWpmdCAPOnoGTime}		& \roh{\SLOWpmdCAPOTime} \\
\bench{sunflow} & \et{\SLOWsunflowEvents}  & \enfp{\SLOWsunflowNoFPEvents}	& \SLOWsunflowTotalThreads	& (\SLOWsunflowMaxLiveThreads)	& \base{\SLOWsunflowBaseTime}  & \roh{\SLOWsunflowEmptyTime}  & \roh{\SLOWsunflowFTTime}	& \roh{\SLOWsunflowHBTime}	& \roh{\SLOWsunflowWCPTime} & \roh{\SLOWsunflowWDCnoGTime} 	& \roh{\SLOWsunflowWDCTime}	& \roh{\SLOWsunflowCAPOnoGTime}	& \roh{\SLOWsunflowCAPOTime} \\
\bench{tomcat} 	& \et{\SLOWtomcatEvents}   & \enfp{\SLOWtomcatNoFPEvents}	& \SLOWtomcatTotalThreads	& (\SLOWtomcatMaxLiveThreads)	& \base{\SLOWtomcatBaseTime}   & \roh{\SLOWtomcatEmptyTime}   & \roh{\SLOWtomcatFTTime}		& \roh{\SLOWtomcatHBTime}	& \roh{\SLOWtomcatWCPTime} 	& \roh{\SLOWtomcatWDCnoGTime} 	& \roh{\SLOWtomcatWDCTime}	& \roh{\SLOWtomcatCAPOnoGTime}	& \roh{\SLOWtomcatCAPOTime} \\
\bench{xalan} 	& \et{\SLOWxalanEvents}    & \enfp{\SLOWxalanNoFPEvents}	& \SLOWxalanTotalThreads	& (\SLOWxalanMaxLiveThreads)	& \base{\SLOWxalanBaseTime}    & \roh{\SLOWxalanEmptyTime}    & \roh{\SLOWxalanFTTime}		& \roh{\SLOWxalanHBTime}	& \roh{\SLOWxalanWCPTime} 	& \roh{\SLOWxalanWDCnoGTime} 	& \roh{\SLOWxalanWDCTime}	& \roh{\SLOWxalanCAPOnoGTime}	& \roh{\SLOWxalanCAPOTime} \\\hline
\end{tabular}
\label{tab:slow-tool:performance}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand\DCwoG{\DC}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
% \input{result-macros/PIP_fastTool_performanceProfile}
% \input{result-macros/PIP_fastTool_CAPORE_raceCheckOptimization}
% \input{result-macros/PIP_fastTool_CAPOOpt_RuleAFix}
% \input{result-macros/PIP_fastTool_CAPORE_FTO}
\input{result-macros/PIP_fastTool_FTO_All}
%
\small
\centering
\begin{tabular}{@{}l|rl|rl||r|HrrrrrHHH@{}}
& \mc{2}{c|}{} & \mc{2}{c||}{} & Base & \mc{9}{c}{\FastTool: Slowdown (normalized to Base time)} \\
Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & time & Empty & \FT & \HB & \WCP & \DC & \CAPO & -Opt & -Opt-Alt & -RE \\\hline 
\bench{avrora} 	& \et{\FASTavroraEvents}   & \enfp{\FASTavroraNoFPEvents}	& \FASTavroraTotalThreads 	& (\FASTavroraMaxLiveThreads)	& \base{\FASTavroraBaseTime}   & \roh{\FASTavroraEmptyTime}   & \roh{\FASTavroraFTTime}   & \roh{\FASTavroraHBTime}   	& \roh{\FASTavroraWCPTime}   & \roh{\FASTavroraDCTime} 	 & \roh{\FASTavroraCAPOTime} 	& \roh{\FASTavroraCAPOOPTTime} 	& \roh{\FASTavroraCAPOOPTALTTime} 	& \roh{\FASTavroraCAPORETime} \\
\bench{batik} 	& \et{\FASTbatikEvents}    & \enfp{\FASTbatikNoFPEvents}	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& \base{\FASTbatikBaseTime}    & \roh{\FASTbatikEmptyTime}    & \roh{\FASTbatikFTTime}    & \roh{\FASTbatikHBTime}    	& \roh{\FASTbatikWCPTime}    & \roh{\FASTbatikDCTime}    & \roh{\FASTbatikCAPOTime} 	& \roh{\FASTbatikCAPOOPTTime} 	& \roh{\FASTbatikCAPOOPTALTTime} 	& \roh{\FASTbatikCAPORETime} \\
\bench{h2} 		& \et{\FASThtwoEvents}     & \enfp{\FASThtwoNoFPEvents}	    & \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & \base{\FASThtwoBaseTime}     & \roh{\FASThtwoEmptyTime}     & \roh{\FASThtwoFTTime}     & \roh{\FASThtwoHBTime}     	& \roh{\FASThtwoWCPTime}     & \roh{\FASThtwoDCTime}     & \roh{\FASThtwoCAPOTime} 		& \roh{\FASThtwoCAPOOPTTime} 	& \roh{\FASThtwoCAPOOPTALTTime} 	& \roh{\FASThtwoCAPORETime} \\
\bench{jython} 	& \et{\FASTjythonEvents}   & \enfp{\FASTjythonNoFPEvents}	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& \base{\FASTjythonBaseTime}   & \roh{\FASTjythonEmptyTime}   & \roh{\FASTjythonFTTime}   & \roh{\FASTjythonHBTime} 	& \roh{\FASTjythonWCPTime}   & \roh{\FASTjythonDCTime} 	 & \roh{\FASTjythonCAPOTime} 	& \roh{\FASTjythonCAPOOPTTime} 	& \roh{\FASTjythonCAPOOPTALTTime} 	& \roh{\FASTjythonCAPORETime} \\
\bench{luindex} & \et{\FASTluindexEvents}  & \enfp{\FASTluindexNoFPEvents}	& \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& \base{\FASTluindexBaseTime}  & \roh{\FASTluindexEmptyTime}  & \roh{\FASTluindexFTTime}  & \roh{\FASTluindexHBTime}  	& \roh{\FASTluindexWCPTime}  & \roh{\FASTluindexDCTime}  & \roh{\FASTluindexCAPOTime} 	& \roh{\FASTluindexCAPOOPTTime} & \roh{\FASTluindexCAPOOPTALTTime} 	& \roh{\FASTluindexCAPORETime} \\
\bench{lusearch}& \et{\FASTlusearchEvents} & \enfp{\FASTlusearchNoFPEvents}	& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& \base{\FASTlusearchBaseTime} & \roh{\FASTlusearchEmptyTime} & \roh{\FASTlusearchFTTime} & \roh{\FASTlusearchHBTime}	& \roh{\FASTlusearchWCPTime} & \roh{\FASTlusearchDCTime} & \roh{\FASTlusearchCAPOTime}	& \roh{\FASTlusearchCAPOOPTTime}& \roh{\FASTlusearchCAPOOPTALTTime}	& \roh{\FASTlusearchCAPORETime} \\
\bench{pmd}		& \et{\FASTpmdEvents}      & \enfp{\FASTpmdNoFPEvents}      & \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & \base{\FASTpmdBaseTime}      & \roh{\FASTpmdEmptyTime}      & \roh{\FASTpmdFTTime}      & \roh{\FASTpmdHBTime}		& \roh{\FASTpmdWCPTime}      & \roh{\FASTpmdDCTime}	     & \roh{\FASTpmdCAPOTime} 		& \roh{\FASTpmdCAPOOPTTime} 	& \roh{\FASTpmdCAPOOPTALTTime} 		& \roh{\FASTpmdCAPORETime} \\
\bench{sunflow} & \et{\FASTsunflowEvents}  & \enfp{\FASTsunflowNoFPEvents}	& \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& \base{\FASTsunflowBaseTime}  & \roh{\FASTsunflowEmptyTime}  & \roh{\FASTsunflowFTTime}  & \roh{\FASTsunflowHBTime}	& \roh{\FASTsunflowWCPTime}  & \roh{\FASTsunflowDCTime}  & \roh{\FASTsunflowCAPOTime} 	& \roh{\FASTsunflowCAPOOPTTime} & \roh{\FASTsunflowCAPOOPTALTTime} 	& \roh{\FASTsunflowCAPORETime} \\
\bench{tomcat} 	& \et{\FASTtomcatEvents}   & \enfp{\FASTtomcatNoFPEvents}	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& \base{\FASTtomcatBaseTime}   & \roh{\FASTtomcatEmptyTime}   & \roh{\FASTtomcatFTTime}   & \roh{\FASTtomcatHBTime} 	& \roh{\FASTtomcatWCPTime}   & \roh{\FASTtomcatDCTime}   & \roh{\FASTtomcatCAPOTime} 	& \roh{\FASTtomcatCAPOOPTTime} 	& \roh{\FASTtomcatCAPOOPTALTTime} 	& \roh{\FASTtomcatCAPORETime} \\
\bench{xalan} 	& \et{\FASTxalanEvents}    & \enfp{\FASTxalanNoFPEvents}	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& \base{\FASTxalanBaseTime}    & \roh{\FASTxalanEmptyTime}    & \roh{\FASTxalanFTTime}    & \roh{\FASTxalanHBTime}		& \roh{\FASTxalanWCPTime}    & \roh{\FASTxalanDCTime}    & \roh{\FASTxalanCAPOTime} 	& \roh{\FASTxalanCAPOOPTTime} 	& \roh{\FASTxalanCAPOOPTALTTime} 	& \roh{\FASTxalanCAPORETime} \\\hline
\end{tabular}
\label{tab:performance}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand\DCwoG{\DC}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_fastTool_FTO_All}
%
\small
\centering
% \begin{tabular}{@{}l|rl|rl||r|Hr|rrrrrH|r@{}}
\begin{tabular}{@{}l|rl|rl||r|Hr|rrrr|rrr@{}}
& \mc{2}{c|}{} & \mc{2}{c||}{} & & \mc{9}{c}{\FastTool: Slowdown (normalized to Base time)} \\
& \mc{2}{c|}{} & \mc{2}{c||}{} & Base & & & \mc{4}{c|}{FTO w/o RE} & \mc{3}{c}{FTO w/ RE} \\
Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & time & Empty & \FT & \HB & \WCP & \DC & \CAPO & \WCP & \DC & \CAPO \\\hline 
\bench{avrora} 	& \et{\FASTavroraEvents}   & \enfp{\FASTavroraNoFPEvents}	& \FASTavroraTotalThreads 	& (\FASTavroraMaxLiveThreads)	& \base{\FASTavroraBaseTime}   & \roh{\FASTavroraEmptyTime}   & \roh{\FASTavroraFTTime}   & \roh{\FASTavroraFTOHBTime}  & \roh{\FASTavroraFTOWCPTime}   & \roh{\FASTavroraFTODCTime} 	& \roh{\FASTavroraFTOCAPOTime}	& \roh{\FASTavroraREWCPTime}	& \roh{\FASTavroraREDCTime}		& \roh{\FASTavroraCAPORETime} \\
\bench{batik} 	& \et{\FASTbatikEvents}    & \enfp{\FASTbatikNoFPEvents}	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& \base{\FASTbatikBaseTime}    & \roh{\FASTbatikEmptyTime}    & \roh{\FASTbatikFTTime}    & \roh{\FASTbatikFTOHBTime}   & \roh{\FASTbatikFTOWCPTime}    & \roh{\FASTbatikFTODCTime}   	& \roh{\FASTbatikFTOCAPOTime} 	& \roh{\FASTbatikREWCPTime}		& \roh{\FASTbatikREDCTime}		& \roh{\FASTbatikCAPORETime} \\
\bench{h2} 		& \et{\FASThtwoEvents}     & \enfp{\FASThtwoNoFPEvents}	    & \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & \base{\FASThtwoBaseTime}     & \roh{\FASThtwoEmptyTime}     & \roh{\FASThtwoFTTime}     & \roh{\FASThtwoFTOHBTime}    & \roh{\FASThtwoFTOWCPTime}     & \roh{\FASThtwoFTODCTime}    	& \roh{\FASThtwoFTOCAPOTime} 	& \roh{\FASThtwoREWCPTime}		& \roh{\FASThtwoREDCTime}		& \roh{\FASThtwoCAPORETime} \\
\bench{jython} 	& \et{\FASTjythonEvents}   & \enfp{\FASTjythonNoFPEvents}	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& \base{\FASTjythonBaseTime}   & \roh{\FASTjythonEmptyTime}   & \roh{\FASTjythonFTTime}   & \roh{\FASTjythonFTOHBTime} 	& \roh{\FASTjythonFTOWCPTime}   & \roh{\FASTjythonFTODCTime} 	& \roh{\FASTjythonFTOCAPOTime} 	& \roh{\FASTjythonREWCPTime}	& \roh{\FASTjythonREDCTime}		& \roh{\FASTjythonCAPORETime} \\
\bench{luindex} & \et{\FASTluindexEvents}  & \enfp{\FASTluindexNoFPEvents}	& \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& \base{\FASTluindexBaseTime}  & \roh{\FASTluindexEmptyTime}  & \roh{\FASTluindexFTTime}  & \roh{\FASTluindexFTOHBTime} & \roh{\FASTluindexFTOWCPTime}  & \roh{\FASTluindexFTODCTime}  	& \roh{\FASTluindexFTOCAPOTime} & \roh{\FASTluindexREWCPTime} 	& \roh{\FASTluindexREDCTime}	& \roh{\FASTluindexCAPORETime} \\
\bench{lusearch}& \et{\FASTlusearchEvents} & \enfp{\FASTlusearchNoFPEvents}	& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& \base{\FASTlusearchBaseTime} & \roh{\FASTlusearchEmptyTime} & \roh{\FASTlusearchFTTime} & \roh{\FASTlusearchFTOHBTime}& \roh{\FASTlusearchFTOWCPTime} & \roh{\FASTlusearchFTODCTime}	& \roh{\FASTlusearchFTOCAPOTime}& \roh{\FASTlusearchREWCPTime}	& \roh{\FASTlusearchREDCTime}	& \roh{\FASTlusearchCAPORETime} \\
\bench{pmd}		& \et{\FASTpmdEvents}      & \enfp{\FASTpmdNoFPEvents}      & \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & \base{\FASTpmdBaseTime}      & \roh{\FASTpmdEmptyTime}      & \roh{\FASTpmdFTTime}      & \roh{\FASTpmdFTOHBTime}		& \roh{\FASTpmdFTOWCPTime}      & \roh{\FASTpmdFTODCTime}	    & \roh{\FASTpmdFTOCAPOTime} 	& \roh{\FASTpmdREWCPTime}		& \roh{\FASTpmdREDCTime}		& \roh{\FASTpmdCAPORETime} \\
\bench{sunflow} & \et{\FASTsunflowEvents}  & \enfp{\FASTsunflowNoFPEvents}	& \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& \base{\FASTsunflowBaseTime}  & \roh{\FASTsunflowEmptyTime}  & \roh{\FASTsunflowFTTime}  & \roh{\FASTsunflowFTOHBTime}	& \roh{\FASTsunflowFTOWCPTime}  & \roh{\FASTsunflowFTODCTime}  	& \roh{\FASTsunflowFTOCAPOTime} & \roh{\FASTsunflowREWCPTime}	& \roh{\FASTsunflowREDCTime}	& \roh{\FASTsunflowCAPORETime} \\
\bench{tomcat} 	& \et{\FASTtomcatEvents}   & \enfp{\FASTtomcatNoFPEvents}	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& \base{\FASTtomcatBaseTime}   & \roh{\FASTtomcatEmptyTime}   & \roh{\FASTtomcatFTTime}   & \roh{\FASTtomcatFTOHBTime} 	& \roh{\FASTtomcatFTOWCPTime}   & \roh{\FASTtomcatFTODCTime}   	& \roh{\FASTtomcatFTOCAPOTime} 	& \roh{\FASTtomcatREWCPTime}	& \roh{\FASTtomcatREDCTime}		& \roh{\FASTtomcatCAPORETime} \\
\bench{xalan} 	& \et{\FASTxalanEvents}    & \enfp{\FASTxalanNoFPEvents}	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& \base{\FASTxalanBaseTime}    & \roh{\FASTxalanEmptyTime}    & \roh{\FASTxalanFTTime}    & \roh{\FASTxalanFTOHBTime}	& \roh{\FASTxalanFTOWCPTime}    & \roh{\FASTxalanFTODCTime}    	& \roh{\FASTxalanFTOCAPOTime} 	& \roh{\FASTxalanREWCPTime}		& \roh{\FASTxalanREDCTime}		& \roh{\FASTxalanCAPORETime} \\\hline
\end{tabular}
\label{tab:performance:fto}
\end{minipage}
\caption{Slow tool performance, memory, and race results.}
\label{tab:slow-tool-stats}
\end{table*}



%%% Memory Overhead
\begin{table*}[t]
\begin{minipage}{1\textwidth}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\input{result-macros/PIP_slowTool_raceLimitFix_assertCheck}
%
\small
\centering
\begin{tabular}{@{}l|rl|rl||rrr|rr|rr}
& \mc{2}{c|}{} & \mc{2}{c||}{} & \mc{7}{c}{\SlowTool: Memory usage (GB)} \\
& \mc{2}{c|}{} & \mc{2}{c||}{} & \mc{3}{c|}{} & \mc{2}{c|}{\DC} & \mc{2}{c}{\CAPO} \\
Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & \FT & \HB & \WCP & w/o G & w/ G & w/o G & w/ G \\\hline 
\bench{avrora} 	& \et{\SLOWavroraEvents}   & \enfp{\SLOWavroraNoFPEvents}	& \SLOWavroraTotalThreads 	& (\SLOWavroraMaxLiveThreads)	& \mem{\SLOWavroraFTMem}   & \mem{\SLOWavroraHBMem}   & \mem{\SLOWavroraWCPMem}		& \mem{\SLOWavroraWDCnoGMem} 	& \mem{\SLOWavroraWDCMem} 	& \mem{\SLOWavroraCAPOnoGMem}	& \mem{\SLOWavroraCAPOMem} \\
\bench{batik} 	& \et{\SLOWbatikEvents}    & \enfp{\SLOWbatikNoFPEvents}	& \SLOWbatikTotalThreads 	& (\SLOWbatikMaxLiveThreads)	& \mem{\SLOWbatikFTMem}    & \mem{\SLOWbatikHBMem} 	  & \mem{\SLOWbatikWCPMem} 		& \mem{\SLOWbatikWDCnoGMem} 	& \mem{\SLOWbatikWDCMem} 	& \mem{\SLOWbatikCAPOnoGMem}	& \mem{\SLOWbatikCAPOMem} \\
\bench{h2} 		& \et{\SLOWhtwoEvents}     & \enfp{\SLOWhtwoNoFPEvents}	    & \SLOWhtwoTotalThreads 	& (\SLOWhtwoMaxLiveThreads)	    & \mem{\SLOWhtwoFTMem} 	   & \mem{\SLOWhtwoHBMem} 	  & \mem{\SLOWhtwoWCPMem} 		& \mem{\SLOWhtwoWDCnoGMem} 		& \mem{\SLOWhtwoWDCMem} 	& \mem{\SLOWhtwoCAPOnoGMem}		& \mem{\SLOWhtwoCAPOMem} \\
\bench{jython} 	& \et{\SLOWjythonEvents}   & \enfp{\SLOWjythonNoFPEvents}	& \SLOWjythonTotalThreads	& (\SLOWjythonMaxLiveThreads)	& \mem{\SLOWjythonFTMem}   & \mem{\SLOWjythonHBMem}   & \mem{\SLOWjythonWCPMem} 	& \mem{\SLOWjythonWDCnoGMem} 	& \mem{\SLOWjythonWDCMem} 	& \mem{\SLOWjythonCAPOnoGMem}	& \mem{\SLOWjythonCAPOMem} \\
\bench{luindex} & \et{\SLOWluindexEvents}  & \enfp{\SLOWluindexNoFPEvents}	& \SLOWluindexTotalThreads	& (\SLOWluindexMaxLiveThreads)	& \mem{\SLOWluindexFTMem}  & \mem{\SLOWluindexHBMem}  & \mem{\SLOWluindexWCPMem} 	& \mem{\SLOWluindexWDCnoGMem} 	& \mem{\SLOWluindexWDCMem} 	& \mem{\SLOWluindexCAPOnoGMem}	& \mem{\SLOWluindexCAPOMem} \\
\bench{lusearch}& \et{\SLOWlusearchEvents} & \enfp{\SLOWlusearchNoFPEvents}	& \SLOWlusearchTotalThreads	& (\SLOWlusearchMaxLiveThreads)	& \mem{\SLOWlusearchFTMem} & \mem{\SLOWlusearchHBMem} & \mem{\SLOWlusearchWCPMem} 	& \mem{\SLOWlusearchWDCnoGMem} 	& \mem{\SLOWlusearchWDCMem}	& \mem{\SLOWlusearchCAPOnoGMem}	& \mem{\SLOWlusearchCAPOMem} \\
\bench{pmd} 	& \et{\SLOWpmdEvents}      & \enfp{\SLOWpmdNoFPEvents}      & \SLOWpmdTotalThreads	    & (\SLOWpmdMaxLiveThreads)	    & \mem{\SLOWpmdFTMem} 	   & \mem{\SLOWpmdHBMem} 	  & \mem{\SLOWpmdWCPMem} 		& \mem{\SLOWpmdWDCnoGMem} 		& \mem{\SLOWpmdWDCMem} 		& \mem{\SLOWpmdCAPOnoGMem}		& \mem{\SLOWpmdCAPOMem} \\
\bench{sunflow} & \et{\SLOWsunflowEvents}  & \enfp{\SLOWsunflowNoFPEvents}	& \SLOWsunflowTotalThreads	& (\SLOWsunflowMaxLiveThreads)	& \mem{\SLOWsunflowFTMem}  & \mem{\SLOWsunflowHBMem}  & \mem{\SLOWsunflowWCPMem}	& \mem{\SLOWsunflowWDCnoGMem} 	& \mem{\SLOWsunflowWDCMem} 	& \mem{\SLOWsunflowCAPOnoGMem}	& \mem{\SLOWsunflowCAPOMem} \\
\bench{tomcat} 	& \et{\SLOWtomcatEvents}   & \enfp{\SLOWtomcatNoFPEvents}	& \SLOWtomcatTotalThreads	& (\SLOWtomcatMaxLiveThreads)	& \mem{\SLOWtomcatFTMem}   & \mem{\SLOWtomcatHBMem}   & \mem{\SLOWtomcatWCPMem} 	& \mem{\SLOWtomcatWDCnoGMem} 	& \mem{\SLOWtomcatWDCMem} 	& \mem{\SLOWtomcatCAPOnoGMem}	& \mem{\SLOWtomcatCAPOMem} \\
\bench{xalan} 	& \et{\SLOWxalanEvents}    & \enfp{\SLOWxalanNoFPEvents}	& \SLOWxalanTotalThreads	& (\SLOWxalanMaxLiveThreads)	& \mem{\SLOWxalanFTMem}    & \mem{\SLOWxalanHBMem} 	  & \mem{\SLOWxalanWCPMem} 		& \mem{\SLOWxalanWDCnoGMem} 	& \mem{\SLOWxalanWDCMem}	& \mem{\SLOWxalanCAPOnoGMem}	& \mem{\SLOWxalanCAPOMem} \\\hline
\end{tabular}
\label{tab:memory}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand\DCwoG{\DC}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
% \input{result-macros/PIP_fastTool_performanceProfile}
% \input{result-macros/PIP_fastTool_CAPORE_raceCheckOptimization}
% \input{result-macros/PIP_fastTool_CAPORE_FTO}
\input{result-macros/PIP_fastTool_FTO_All}
%
\small
\centering
\begin{tabular}{@{}l|rl|rl||r|rrrr|rrrr|rrr@{}}
& \mc{2}{c|}{} & \mc{2}{c||}{} & \mc{12}{c}{\FastTool: Memory usage (GB)} \\
& \mc{2}{c|}{} & \mc{2}{c||}{} & & \mc{4}{c|}{} & \mc{4}{c|}{FTO w/o RE} & \mc{3}{c}{FTO w/ RE} \\
Program & \mc{2}{c|}{Events} & \mc{2}{c||}{\#Thr} & \FT & \HB & \WCP & \DC & \CAPO & \HB & \WCP & \DC & \CAPO & \WCP & \DC & \CAPO \\\hline 
\bench{avrora} 	& \et{\FASTavroraEvents}   & \enfp{\FASTavroraNoFPEvents}	& \FASTavroraTotalThreads 	& (\FASTavroraMaxLiveThreads)	& \mem{\FASTavroraFTMem}	& \mem{\FASTavroraHBMem}	& \mem{\FASTavroraWCPMem} 	& \mem{\FASTavroraDCMem} 	& \mem{\FASTavroraCAPOMem} 		& \mem{\FASTavroraFTOHBMem} 	& \mem{\FASTavroraFTOWCPMem} 	& \mem{\FASTavroraFTODCMem} 	& \mem{\FASTavroraFTOCAPOMem}	& \mem{\FASTavroraREWCPMem}		& \mem{\FASTavroraREDCMem}	& \mem{\FASTavroraCAPOREMem} \\
\bench{batik} 	& \et{\FASTbatikEvents}    & \enfp{\FASTbatikNoFPEvents}	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& \mem{\FASTbatikFTMem}		& \mem{\FASTbatikHBMem} 	& \mem{\FASTbatikWCPMem} 	& \mem{\FASTbatikDCMem} 	& \mem{\FASTbatikCAPOMem} 		& \mem{\FASTbatikFTOHBMem} 		& \mem{\FASTbatikFTOWCPMem} 	& \mem{\FASTbatikFTODCMem} 		& \mem{\FASTbatikFTOCAPOMem}	& \mem{\FASTbatikREWCPMem}		& \mem{\FASTbatikREDCMem}	& \mem{\FASTbatikCAPOREMem} \\
\bench{h2} 		& \et{\FASThtwoEvents}     & \enfp{\FASThtwoNoFPEvents}	    & \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & \mem{\FASThtwoFTMem}	    & \mem{\FASThtwoHBMem} 		& \mem{\FASThtwoWCPMem} 	& \mem{\FASThtwoDCMem} 		& \mem{\FASThtwoCAPOMem} 		& \mem{\FASThtwoFTOHBMem} 		& \mem{\FASThtwoFTOWCPMem} 		& \mem{\FASThtwoFTODCMem} 		& \mem{\FASThtwoFTOCAPOMem}		& \mem{\FASThtwoREWCPMem}		& \mem{\FASThtwoREDCMem}	& \mem{\FASThtwoCAPOREMem} \\
\bench{jython} 	& \et{\FASTjythonEvents}   & \enfp{\FASTjythonNoFPEvents}	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& \mem{\FASTjythonFTMem}	& \mem{\FASTjythonHBMem} 	& \mem{\FASTjythonWCPMem} 	& \mem{\FASTjythonDCMem} 	& \mem{\FASTjythonCAPOMem} 		& \mem{\FASTjythonFTOHBMem} 	& \mem{\FASTjythonFTOWCPMem} 	& \mem{\FASTjythonFTODCMem} 	& \mem{\FASTjythonFTOCAPOMem}	& \mem{\FASTjythonREWCPMem}		& \mem{\FASTjythonREDCMem}	& \mem{\FASTjythonCAPOREMem} \\
\bench{luindex} & \et{\FASTluindexEvents}  & \enfp{\FASTluindexNoFPEvents}	& \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& \mem{\FASTluindexFTMem}	& \mem{\FASTluindexHBMem} 	& \mem{\FASTluindexWCPMem} 	& \mem{\FASTluindexDCMem} 	& \mem{\FASTluindexCAPOMem} 	& \mem{\FASTluindexFTOHBMem} 	& \mem{\FASTluindexFTOWCPMem} 	& \mem{\FASTluindexFTODCMem} 	& \mem{\FASTluindexFTOCAPOMem}	& \mem{\FASTluindexREWCPMem}	& \mem{\FASTluindexREDCMem}	& \mem{\FASTluindexCAPOREMem} \\
\bench{lusearch}& \et{\FASTlusearchEvents} & \enfp{\FASTlusearchNoFPEvents}	& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& \mem{\FASTlusearchFTMem}	& \mem{\FASTlusearchHBMem} 	& \mem{\FASTlusearchWCPMem}	& \mem{\FASTlusearchDCMem} 	& \mem{\FASTlusearchCAPOMem}	& \mem{\FASTlusearchFTOHBMem}	& \mem{\FASTlusearchFTOWCPMem} 	& \mem{\FASTlusearchFTODCMem}	& \mem{\FASTlusearchFTOCAPOMem}	& \mem{\FASTlusearchREWCPMem}	& \mem{\FASTlusearchREDCMem}& \mem{\FASTlusearchCAPOREMem} \\
\bench{pmd} 	& \et{\FASTpmdEvents}      & \enfp{\FASTpmdNoFPEvents}      & \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & \mem{\FASTpmdFTMem}	    & \mem{\FASTpmdHBMem} 		& \mem{\FASTpmdWCPMem} 		& \mem{\FASTpmdDCMem} 		& \mem{\FASTpmdCAPOMem} 		& \mem{\FASTpmdFTOHBMem} 		& \mem{\FASTpmdFTOWCPMem}		& \mem{\FASTpmdFTODCMem} 		& \mem{\FASTpmdFTOCAPOMem}		& \mem{\FASTpmdREWCPMem}		& \mem{\FASTpmdREDCMem}		& \mem{\FASTpmdCAPOREMem} \\
\bench{sunflow} & \et{\FASTsunflowEvents}  & \enfp{\FASTsunflowNoFPEvents}	& \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& \mem{\FASTsunflowFTMem}	& \mem{\FASTsunflowHBMem}	& \mem{\FASTsunflowWCPMem} 	& \mem{\FASTsunflowDCMem} 	& \mem{\FASTsunflowCAPOMem} 	& \mem{\FASTsunflowFTOHBMem} 	& \mem{\FASTsunflowFTOWCPMem} 	& \mem{\FASTsunflowFTODCMem} 	& \mem{\FASTsunflowFTOCAPOMem}	& \mem{\FASTsunflowREWCPMem}	& \mem{\FASTsunflowREDCMem}	& \mem{\FASTsunflowCAPOREMem} \\
\bench{tomcat} 	& \et{\FASTtomcatEvents}   & \enfp{\FASTtomcatNoFPEvents}	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& \mem{\FASTtomcatFTMem}	& \mem{\FASTtomcatHBMem} 	& \mem{\FASTtomcatWCPMem} 	& \mem{\FASTtomcatDCMem} 	& \mem{\FASTtomcatCAPOMem} 		& \mem{\FASTtomcatFTOHBMem} 	& \mem{\FASTtomcatFTOWCPMem} 	& \mem{\FASTtomcatFTODCMem} 	& \mem{\FASTtomcatFTOCAPOMem}	& \mem{\FASTtomcatREWCPMem}		& \mem{\FASTtomcatREDCMem}	& \mem{\FASTtomcatCAPOREMem} \\
\bench{xalan} 	& \et{\FASTxalanEvents}    & \enfp{\FASTxalanNoFPEvents}	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& \mem{\FASTxalanFTMem}		& \mem{\FASTxalanHBMem} 	& \mem{\FASTxalanWCPMem} 	& \mem{\FASTxalanDCMem} 	& \mem{\FASTxalanCAPOMem} 		& \mem{\FASTxalanFTOHBMem} 		& \mem{\FASTxalanFTOWCPMem} 	& \mem{\FASTxalanFTODCMem} 		& \mem{\FASTxalanFTOCAPOMem}	& \mem{\FASTxalanREWCPMem}		& \mem{\FASTxalanREDCMem}	& \mem{\FASTxalanCAPOREMem} \\\hline
\end{tabular}
\end{minipage}
\caption{Fast tool performance, memory, and race results.}
\label{tab:fast-tool-stats}
\end{table*}



%%% Race Coverage
\begin{table*}[t]
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\input{result-macros/PIP_slowTool_raceLimitFix_assertCheck}
%  
\small
\centering
% \begin{tabular}{@{}l|rl|rr|rr|rr|rr|rr|rr|rr@{}}
\begin{tabular}{@{}lHH|rr|rr|rr|rr|rr|rr|rr@{}}
& \mc{2}{c|}{} & \mc{14}{c@{}}{\SlowTool: Second Site [SS] Statically distinct races (dynamic races)}  \\
& \mc{2}{c|}{} & \mc{2}{c|}{} & \mc{2}{c|}{} & \mc{2}{c|}{} & \mc{4}{c|}{\DC-races} & \mc{4}{c}{\CAPO-races} \\
Program & \mc{2}{H|}{Events} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{w/o G} & \mc{2}{c|}{w/ G} & \mc{2}{c|}{w/o G} & \mc{2}{c@{}}{w/ G} \\\hline
\bench{avrora} 	& \et{\SLOWavroraEvents}   & \enfp{\SLOWavroraNoFPEvents}	& \SLOWavroraFT & (\SLOWavroraFTDynamic)	& \SLOWavroraHB & (\SLOWavroraHBDynamic) 		& \SLOWavroraWCP & (\SLOWavroraWCPDynamic)		& \SLOWavroraWDCnoG & (\SLOWavroraWDCnoGDynamic)	& \SLOWavroraWDC & (\SLOWavroraWDCDynamic) 		& \SLOWavroraCAPO & (\SLOWavroraCAPODynamic) \\
\bench{batik} 	& \et{\SLOWbatikEvents}    & \enfp{\SLOWbatikNoFPEvents}	& \SLOWbatikFT & (\SLOWbatikFTDynamic)		& \SLOWbatikHB & (\SLOWbatikHBDynamic) 			& \SLOWbatikWCP & (\SLOWbatikWCPDynamic)		& \SLOWbatikWDCnoG & (\SLOWbatikWDCnoGDynamic)		& \SLOWbatikWDC & (\SLOWbatikWDCDynamic) 		& \SLOWbatikCAPO & (\SLOWbatikCAPODynamic) \\
\bench{h2} 		& \et{\SLOWhtwoEvents}     & \enfp{\SLOWhtwoNoFPEvents}	    & \SLOWhtwoFT & (\SLOWhtwoFTDynamic)		& \SLOWhtwoHB & (\SLOWhtwoHBDynamic) 			& \SLOWhtwoWCP & (\SLOWhtwoWCPDynamic)			& \SLOWhtwoWDCnoG & (\SLOWhtwoWDCnoGDynamic)		& \SLOWhtwoWDC & (\SLOWhtwoWDCDynamic) 			& \SLOWhtwoCAPO & (\SLOWhtwoCAPODynamic) \\
\bench{jython} 	& \et{\SLOWjythonEvents}   & \enfp{\SLOWjythonNoFPEvents}	& \SLOWjythonFT & (\SLOWjythonFTDynamic)	& \SLOWjythonHB & (\SLOWjythonHBDynamic) 		& \SLOWjythonWCP & (\SLOWjythonWCPDynamic)		& \SLOWjythonWDCnoG & (\SLOWjythonWDCnoGDynamic)	& \SLOWjythonWDC & (\SLOWjythonWDCDynamic) 		& \SLOWjythonCAPO & (\SLOWjythonCAPODynamic) \\
\bench{luindex} & \et{\SLOWluindexEvents}  & \enfp{\SLOWluindexNoFPEvents}	& \SLOWluindexFT & (\SLOWluindexFTDynamic)	& \SLOWluindexHB & (\SLOWluindexHBDynamic) 		& \SLOWluindexWCP & (\SLOWluindexWCPDynamic)	& \SLOWluindexWDCnoG & (\SLOWluindexWDCnoGDynamic)	& \SLOWluindexWDC & (\SLOWluindexWDCDynamic) 	& \SLOWluindexCAPO & (\SLOWluindexCAPODynamic) \\
\bench{lusearch}& \et{\SLOWlusearchEvents} & \enfp{\SLOWlusearchNoFPEvents}	& \SLOWlusearchFT & (\SLOWlusearchFTDynamic)& \SLOWlusearchHB & (\SLOWlusearchHBDynamic)	& \SLOWlusearchWCP & (\SLOWlusearchWCPDynamic)	& \SLOWlusearchWDCnoG & (\SLOWlusearchWDCnoGDynamic)& \SLOWlusearchWDC & (\SLOWlusearchWDCDynamic)	& \SLOWlusearchCAPO & (\SLOWlusearchCAPODynamic) \\
\bench{pmd} 	& \et{\SLOWpmdEvents}      & \enfp{\SLOWpmdNoFPEvents}      & \SLOWpmdFT & (\SLOWpmdFTDynamic)			& \SLOWpmdHB & (\SLOWpmdHBDynamic) 				& \SLOWpmdWCP & (\SLOWpmdWCPDynamic)			& \SLOWpmdWDCnoG & (\SLOWpmdWDCnoGDynamic)			& \SLOWpmdWDC & (\SLOWpmdWDCDynamic) 			& \SLOWpmdCAPO & (\SLOWpmdCAPODynamic) \\
\bench{sunflow} & \et{\SLOWsunflowEvents}  & \enfp{\SLOWsunflowNoFPEvents}	& \SLOWsunflowFT & (\SLOWsunflowFTDynamic)	& \SLOWsunflowHB & (\SLOWsunflowHBDynamic) 		& \SLOWsunflowWCP & (\SLOWsunflowWCPDynamic)	& \SLOWsunflowWDCnoG & (\SLOWsunflowWDCnoGDynamic)	& \SLOWsunflowWDC & (\SLOWsunflowWDCDynamic) 	& \SLOWsunflowCAPO & (\SLOWsunflowCAPODynamic) \\
\bench{tomcat} 	& \et{\SLOWtomcatEvents}   & \enfp{\SLOWtomcatNoFPEvents}	& \SLOWtomcatFT & (\SLOWtomcatFTDynamic)	& \SLOWtomcatHB & (\SLOWtomcatHBDynamic) 		& \SLOWtomcatWCP & (\SLOWtomcatWCPDynamic)		& \SLOWtomcatWDCnoG & (\SLOWtomcatWDCnoGDynamic)	& \SLOWtomcatWDC & (\SLOWtomcatWDCDynamic) 		& \SLOWtomcatCAPO & (\SLOWtomcatCAPODynamic) \\
\bench{xalan} 	& \et{\SLOWxalanEvents}    & \enfp{\SLOWxalanNoFPEvents}	& \SLOWxalanFT & (\SLOWxalanFTDynamic)		& \SLOWxalanHB & (\SLOWxalanHBDynamic) 			& \SLOWxalanWCP & (\SLOWxalanWCPDynamic)		& \SLOWxalanWDCnoG & (\SLOWxalanWDCnoGDynamic)		& \SLOWxalanWDC & (\SLOWxalanWDCDynamic) 		& \SLOWxalanCAPO & (\SLOWxalanCAPODynamic) \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\input{result-macros/PIP_slowTool_raceLimitFix_assertCheck}
%  
\small
\centering
% \begin{tabular}{@{}l|rl|rr|rr|rr|rr|rr|rr|rr@{}}
\begin{tabular}{@{}lHH|rr|rr|rr|rr|rr|rr|rr@{}}
& \mc{2}{c|}{} & \mc{14}{c@{}}{\SlowTool: Unordered Pairs [UP] Statically distinct races (dynamic races)}  \\
& \mc{2}{c|}{} & \mc{2}{c|}{} & \mc{2}{c|}{} & \mc{2}{c|}{} & \mc{4}{c|}{\DC-races} & \mc{4}{c}{\CAPO-races} \\
Program & \mc{2}{H|}{Events} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{w/o G} & \mc{2}{c|}{w/ G} & \mc{2}{c|}{w/o G} & \mc{2}{c@{}}{w/ G} \\\hline
\bench{avrora} 	& \et{\SLOWavroraEvents}   & \enfp{\SLOWavroraNoFPEvents}	& \SLOWavroraFT & (\SLOWavroraFTDynamic)		& \SLOWavroraHBUP & (\SLOWavroraHBDynamicUP) 		& \SLOWavroraWCPUP & (\SLOWavroraWCPDynamicUP)		& \SLOWavroraWDCnoGUP & (\SLOWavroraWDCnoGDynamicUP)	& \SLOWavroraWDCUP & (\SLOWavroraWDCDynamicUP) 		& \SLOWavroraCAPOUP & (\SLOWavroraCAPODynamicUP) \\
\bench{batik} 	& \et{\SLOWbatikEvents}    & \enfp{\SLOWbatikNoFPEvents}	& \SLOWbatikFT & (\SLOWbatikFTDynamic)			& \SLOWbatikHBUP & (\SLOWbatikHBDynamicUP) 			& \SLOWbatikWCPUP & (\SLOWbatikWCPDynamicUP)		& \SLOWbatikWDCnoGUP & (\SLOWbatikWDCnoGDynamicUP)		& \SLOWbatikWDCUP & (\SLOWbatikWDCDynamicUP) 		& \SLOWbatikCAPOUP & (\SLOWbatikCAPODynamicUP) \\
\bench{h2} 		& \et{\SLOWhtwoEvents}     & \enfp{\SLOWhtwoNoFPEvents}	    & \SLOWhtwoFT & (\SLOWhtwoFTDynamic)			& \SLOWhtwoHBUP & (\SLOWhtwoHBDynamicUP) 			& \SLOWhtwoWCPUP & (\SLOWhtwoWCPDynamicUP)			& \SLOWhtwoWDCnoGUP & (\SLOWhtwoWDCnoGDynamicUP)		& \SLOWhtwoWDCUP & (\SLOWhtwoWDCDynamicUP) 			& \SLOWhtwoCAPOUP & (\SLOWhtwoCAPODynamicUP) \\
\bench{jython} 	& \et{\SLOWjythonEvents}   & \enfp{\SLOWjythonNoFPEvents}	& \SLOWjythonFT & (\SLOWjythonFTDynamic)		& \SLOWjythonHBUP & (\SLOWjythonHBDynamicUP) 		& \SLOWjythonWCPUP & (\SLOWjythonWCPDynamicUP)		& \SLOWjythonWDCnoGUP & (\SLOWjythonWDCnoGDynamicUP)	& \SLOWjythonWDCUP & (\SLOWjythonWDCDynamicUP) 		& \SLOWjythonCAPOUP & (\SLOWjythonCAPODynamicUP) \\
\bench{luindex} & \et{\SLOWluindexEvents}  & \enfp{\SLOWluindexNoFPEvents}	& \SLOWluindexFT & (\SLOWluindexFTDynamic)		& \SLOWluindexHBUP & (\SLOWluindexHBDynamicUP) 		& \SLOWluindexWCPUP & (\SLOWluindexWCPDynamicUP)	& \SLOWluindexWDCnoGUP & (\SLOWluindexWDCnoGDynamicUP)	& \SLOWluindexWDCUP & (\SLOWluindexWDCDynamicUP) 	& \SLOWluindexCAPOUP & (\SLOWluindexCAPODynamicUP) \\
\bench{lusearch}& \et{\SLOWlusearchEvents} & \enfp{\SLOWlusearchNoFPEvents}	& \SLOWlusearchFT & (\SLOWlusearchFTDynamic)	& \SLOWlusearchHBUP & (\SLOWlusearchHBDynamicUP)	& \SLOWlusearchWCPUP & (\SLOWlusearchWCPDynamicUP)	& \SLOWlusearchWDCnoGUP & (\SLOWlusearchWDCnoGDynamicUP)& \SLOWlusearchWDCUP & (\SLOWlusearchWDCDynamicUP)	& \SLOWlusearchCAPOUP & (\SLOWlusearchCAPODynamicUP) \\
\bench{pmd} 	& \et{\SLOWpmdEvents}      & \enfp{\SLOWpmdNoFPEvents}      & \SLOWpmdFT & (\SLOWpmdFTDynamic)				& \SLOWpmdHBUP & (\SLOWpmdHBDynamicUP) 				& \SLOWpmdWCPUP & (\SLOWpmdWCPDynamicUP)			& \SLOWpmdWDCnoGUP & (\SLOWpmdWDCnoGDynamicUP)			& \SLOWpmdWDCUP & (\SLOWpmdWDCDynamicUP) 			& \SLOWpmdCAPOUP & (\SLOWpmdCAPODynamicUP) \\
\bench{sunflow} & \et{\SLOWsunflowEvents}  & \enfp{\SLOWsunflowNoFPEvents}	& \SLOWsunflowFT & (\SLOWsunflowFTDynamic)		& \SLOWsunflowHBUP & (\SLOWsunflowHBDynamicUP) 		& \SLOWsunflowWCPUP & (\SLOWsunflowWCPDynamicUP)	& \SLOWsunflowWDCnoGUP & (\SLOWsunflowWDCnoGDynamicUP)	& \SLOWsunflowWDCUP & (\SLOWsunflowWDCDynamicUP) 	& \SLOWsunflowCAPOUP & (\SLOWsunflowCAPODynamicUP) \\
\bench{tomcat} 	& \et{\SLOWtomcatEvents}   & \enfp{\SLOWtomcatNoFPEvents}	& \SLOWtomcatFT & (\SLOWtomcatFTDynamic)		& \SLOWtomcatHBUP & (\SLOWtomcatHBDynamicUP) 		& \SLOWtomcatWCPUP & (\SLOWtomcatWCPDynamicUP)		& \SLOWtomcatWDCnoGUP & (\SLOWtomcatWDCnoGDynamicUP)	& \SLOWtomcatWDCUP & (\SLOWtomcatWDCDynamicUP) 		& \SLOWtomcatCAPOUP & (\SLOWtomcatCAPODynamicUP) \\
\bench{xalan} 	& \et{\SLOWxalanEvents}    & \enfp{\SLOWxalanNoFPEvents}	& \SLOWxalanFT & (\SLOWxalanFTDynamic)			& \SLOWxalanHBUP & (\SLOWxalanHBDynamicUP) 			& \SLOWxalanWCPUP & (\SLOWxalanWCPDynamicUP)		& \SLOWxalanWDCnoGUP & (\SLOWxalanWDCnoGDynamicUP)		& \SLOWxalanWDCUP & (\SLOWxalanWDCDynamicUP) 		& \SLOWxalanCAPOUP & (\SLOWxalanCAPODynamicUP) \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
% \notes{
% \jake{Raw results for all the tables and figures in
% evaluation can be found here:
% \url{http://cse-dcse101008d.cse.ohio-state.edu/exp-products/PIP\_test/}}
% }
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
% \input{result-macros/PIP_fastTool_performanceProfile}
% \input{result-macros/PIP_fastTool_CAPORE_raceCheckOptimization}
% \input{result-macros/PIP_fastTool_CAPOOpt_RuleAFix}
% \input{result-macros/PIP_fastTool_CAPORE_FTO}
\input{result-macros/PIP_fastTool_FTO_All}
%  
\small
\centering
\begin{tabular}{@{}l|rr|rr|rr|rr|rr@{}}
\et{}{} & \mc{10}{c@{}}{\FastTool: Statically distinct races (dynamic races)}  \\ 
Program \et{Events}{\#Thr} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c}{\CAPO-races} \\\hline
\bench{avrora} 	\et{\FASTavroraEvents}{\FASTavroraThreads} 		& \FASTavroraFT & (\FASTavroraFTDynamic) 	& \FASTavroraHB & (\FASTavroraHBDynamic) 	& \FASTavroraWCP & (\FASTavroraWCPDynamic)		& \FASTavroraWDC & (\FASTavroraWDCDynamic) 		& \FASTavroraCAPO & (\FASTavroraCAPODynamic) \\
\bench{batik} 	\et{\FASTbatikEvents}{\FASTbatikThreads} 		& \FASTbatikFT & (\FASTbatikFTDynamic) 		& \FASTbatikHB & (\FASTbatikHBDynamic) 		& \FASTbatikWCP & (\FASTbatikWCPDynamic)		& \FASTbatikWDC & (\FASTbatikWDCDynamic)		& \FASTbatikCAPO & (\FASTbatikCAPODynamic) \\
\bench{h2} 		\et{\FASThtwoEvents}{\FASThtwoThreads} 			& \FASThtwoFT & (\FASThtwoFTDynamic) 		& \FASThtwoHB & (\FASThtwoHBDynamic) 		& \FASThtwoWCP & (\FASThtwoWCPDynamic)			& \FASThtwoWDC & (\FASThtwoWDCDynamic)			& \FASThtwoCAPO & (\FASThtwoCAPODynamic) \\
\bench{jython} 	\et{\FASTjythonEvents}{\FASTjythonThreads} 		& \FASTjythonFT & (\FASTjythonFTDynamic) 	& \FASTjythonHB & (\FASTjythonHBDynamic) 	& \FASTjythonWCP & (\FASTjythonWCPDynamic)		& \FASTjythonWDC & (\FASTjythonWDCDynamic)		& \FASTjythonCAPO & (\FASTjythonCAPODynamic) \\
\bench{luindex} \et{\FASTluindexEvents}{\FASTluindexThreads} 	& \FASTluindexFT & (\FASTluindexFTDynamic) 	& \FASTluindexHB & (\FASTluindexHBDynamic) 	& \FASTluindexWCP & (\FASTluindexWCPDynamic)	& \FASTluindexWDC & (\FASTluindexWDCDynamic)	& \FASTluindexCAPO & (\FASTluindexCAPODynamic) \\
\bench{lusearch}\et{\FASTlusearchEvents}{\FASTlusearchThreads}	& \FASTlusearchFT & (\FASTlusearchFTDynamic)& \FASTlusearchHB & (\FASTlusearchHBDynamic)& \FASTlusearchWCP & (\FASTlusearchWCPDynamic)	& \FASTlusearchWDC & (\FASTlusearchWDCDynamic)	& \FASTlusearchCAPO & (\FASTlusearchCAPODynamic) \\
\bench{pmd} 	\et{\FASTpmdEvents}{\FASTpmdThreads} 			& \FASTpmdFT & (\FASTpmdFTDynamic) 			& \FASTpmdHB & (\FASTpmdHBDynamic)			& \FASTpmdWCP & (\FASTpmdWCPDynamic)			& \FASTpmdWDC & (\FASTpmdWDCDynamic)			& \FASTpmdCAPO & (\FASTpmdCAPODynamic) \\
\bench{sunflow} \et{\FASTsunflowEvents}{\FASTsunflowThreads} 	& \FASTsunflowFT & (\FASTsunflowFTDynamic) 	& \FASTsunflowHB & (\FASTsunflowHBDynamic) 	& \FASTsunflowWCP & (\FASTsunflowWCPDynamic)	& \FASTsunflowWDC & (\FASTsunflowWDCDynamic)	& \FASTsunflowCAPO & (\FASTsunflowCAPODynamic) \\
\bench{tomcat} 	\et{\FASTtomcatEvents}{\FASTtomcatThreads} 		& \FASTtomcatFT & (\FASTtomcatFTDynamic) 	& \FASTtomcatHB & (\FASTtomcatHBDynamic) 	& \FASTtomcatWCP & (\FASTtomcatWCPDynamic)		& \FASTtomcatWDC & (\FASTtomcatWDCDynamic)		& \FASTtomcatCAPO & (\FASTtomcatCAPODynamic) \\
\bench{xalan} 	\et{\FASTxalanEvents}{\FASTxalanThreads} 		& \FASTxalanFT & (\FASTxalanFTDynamic) 		& \FASTxalanHB & (\FASTxalanHBDynamic) 		& \FASTxalanWCP & (\FASTxalanWCPDynamic)		& \FASTxalanWDC & (\FASTxalanWDCDynamic)		& \FASTxalanCAPO & (\FASTxalanCAPODynamic) \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
% \notes{
% \jake{Raw results for all the tables and figures in
% evaluation can be found here:
% \url{http://cse-dcse101008d.cse.ohio-state.edu/exp-products/PIP\_test/}}
% }
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
% \input{result-macros/PIP_fastTool_performanceProfile}
% \input{result-macros/PIP_fastTool_CAPORE_raceCheckOptimization}
% \input{result-macros/PIP_fastTool_CAPOOpt_RuleAFix}
% \input{result-macros/PIP_fastTool_CAPORE_FTO}
\input{result-macros/PIP_fastTool_FTO_All}
%  
\small
\centering
\begin{tabular}{@{}l|rr|rr|rr|rr|rr|rr|rr|rr@{}}
\et{}{} & \mc{16}{c@{}}{\FastTool: Statically distinct races (dynamic races)}  \\ 
\et{}{} & \mc{2}{c|}{} & \mc{8}{c|}{FTO w/o RE} & \mc{6}{c}{FTO w/ RE} \\
Program \et{Events}{\#Thr} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c|}{\CAPO-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c|}{\CAPO-races} \\\hline
\bench{avrora} 	\et{\FASTavroraEvents}{\FASTavroraThreads} 		& \FASTavroraFT & (\FASTavroraFTDynamic) 	& \FASTavroraFTOHB & (\FASTavroraFTOHBDynamic) 		& \FASTavroraFTOWCP & (\FASTavroraFTOWCPDynamic)	& \FASTavroraFTODC & (\FASTavroraFTODCDynamic) 		& \FASTavroraFTOCAPO & (\FASTavroraFTOCAPODynamic) 		& \FASTavroraREWCP & (\FASTavroraREWCPDynamic)		& \FASTavroraREDC & (\FASTavroraREDCDynamic) 	& \FASTavroraCAPORE & (\FASTavroraCAPOREDynamic) \\
\bench{batik} 	\et{\FASTbatikEvents}{\FASTbatikThreads} 		& \FASTbatikFT & (\FASTbatikFTDynamic) 		& \FASTbatikFTOHB & (\FASTbatikFTOHBDynamic) 		& \FASTbatikFTOWCP & (\FASTbatikFTOWCPDynamic)		& \FASTbatikFTODC & (\FASTbatikFTODCDynamic)		& \FASTbatikFTOCAPO & (\FASTbatikFTOCAPODynamic)		& \FASTbatikREWCP & (\FASTbatikREWCPDynamic)		& \FASTbatikREDC & (\FASTbatikREDCDynamic)		& \FASTbatikCAPORE & (\FASTbatikCAPOREDynamic) \\
\bench{h2} 		\et{\FASThtwoEvents}{\FASThtwoThreads} 			& \FASThtwoFT & (\FASThtwoFTDynamic) 		& \FASThtwoFTOHB & (\FASThtwoFTOHBDynamic) 			& \FASThtwoFTOWCP & (\FASThtwoFTOWCPDynamic)		& \FASThtwoFTODC & (\FASThtwoFTODCDynamic)			& \FASThtwoFTOCAPO & (\FASThtwoFTOCAPODynamic)			& \FASThtwoREWCP & (\FASThtwoREWCPDynamic)			& \FASThtwoREDC & (\FASThtwoREDCDynamic)		& \FASThtwoCAPORE & (\FASThtwoCAPOREDynamic) \\
\bench{jython} 	\et{\FASTjythonEvents}{\FASTjythonThreads} 		& \FASTjythonFT & (\FASTjythonFTDynamic) 	& \FASTjythonFTOHB & (\FASTjythonFTOHBDynamic) 		& \FASTjythonFTOWCP & (\FASTjythonFTOWCPDynamic)	& \FASTjythonFTODC & (\FASTjythonFTODCDynamic)		& \FASTjythonFTOCAPO & (\FASTjythonFTOCAPODynamic)		& \FASTjythonREWCP & (\FASTjythonREWCPDynamic)		& \FASTjythonREDC & (\FASTjythonREDCDynamic)	& \FASTjythonCAPORE & (\FASTjythonCAPOREDynamic) \\
\bench{luindex} \et{\FASTluindexEvents}{\FASTluindexThreads} 	& \FASTluindexFT & (\FASTluindexFTDynamic) 	& \FASTluindexFTOHB & (\FASTluindexFTOHBDynamic) 	& \FASTluindexFTOWCP & (\FASTluindexFTOWCPDynamic)	& \FASTluindexFTODC & (\FASTluindexFTODCDynamic)	& \FASTluindexFTOCAPO & (\FASTluindexFTOCAPODynamic)	& \FASTluindexREWCP & (\FASTluindexREWCPDynamic)	& \FASTluindexREDC & (\FASTluindexREDCDynamic)	& \FASTluindexCAPORE & (\FASTluindexCAPOREDynamic) \\
\bench{lusearch}\et{\FASTlusearchEvents}{\FASTlusearchThreads}	& \FASTlusearchFT & (\FASTlusearchFTDynamic)& \FASTlusearchFTOHB & (\FASTlusearchFTOHBDynamic)	& \FASTlusearchFTOWCP & (\FASTlusearchFTOWCPDynamic)& \FASTlusearchFTODC & (\FASTlusearchFTODCDynamic)	& \FASTlusearchFTOCAPO & (\FASTlusearchFTOCAPODynamic)	& \FASTlusearchREWCP & (\FASTlusearchREWCPDynamic)	& \FASTlusearchREDC & (\FASTlusearchREDCDynamic)& \FASTlusearchCAPORE & (\FASTlusearchCAPOREDynamic) \\
\bench{pmd} 	\et{\FASTpmdEvents}{\FASTpmdThreads} 			& \FASTpmdFT & (\FASTpmdFTDynamic) 			& \FASTpmdFTOHB & (\FASTpmdFTOHBDynamic)			& \FASTpmdFTOWCP & (\FASTpmdFTOWCPDynamic)			& \FASTpmdFTODC & (\FASTpmdFTODCDynamic)			& \FASTpmdFTOCAPO & (\FASTpmdFTOCAPODynamic)			& \FASTpmdREWCP & (\FASTpmdREWCPDynamic)			& \FASTpmdREDC & (\FASTpmdREDCDynamic)			& \FASTpmdCAPORE & (\FASTpmdCAPOREDynamic) \\
\bench{sunflow} \et{\FASTsunflowEvents}{\FASTsunflowThreads} 	& \FASTsunflowFT & (\FASTsunflowFTDynamic) 	& \FASTsunflowFTOHB & (\FASTsunflowFTOHBDynamic) 	& \FASTsunflowFTOWCP & (\FASTsunflowFTOWCPDynamic)	& \FASTsunflowFTODC & (\FASTsunflowFTODCDynamic)	& \FASTsunflowFTOCAPO & (\FASTsunflowFTOCAPODynamic)	& \FASTsunflowREWCP & (\FASTsunflowREWCPDynamic)	& \FASTsunflowREDC & (\FASTsunflowREDCDynamic)	& \FASTsunflowCAPORE & (\FASTsunflowCAPOREDynamic) \\
\bench{tomcat} 	\et{\FASTtomcatEvents}{\FASTtomcatThreads} 		& \FASTtomcatFT & (\FASTtomcatFTDynamic) 	& \FASTtomcatFTOHB & (\FASTtomcatFTOHBDynamic) 		& \FASTtomcatFTOWCP & (\FASTtomcatFTOWCPDynamic)	& \FASTtomcatFTODC & (\FASTtomcatFTODCDynamic)		& \FASTtomcatFTOCAPO & (\FASTtomcatFTOCAPODynamic)		& \FASTtomcatREWCP & (\FASTtomcatREWCPDynamic)		& \FASTtomcatREDC & (\FASTtomcatREDCDynamic)	& \FASTtomcatCAPORE & (\FASTtomcatCAPOREDynamic) \\
\bench{xalan} 	\et{\FASTxalanEvents}{\FASTxalanThreads} 		& \FASTxalanFT & (\FASTxalanFTDynamic) 		& \FASTxalanFTOHB & (\FASTxalanFTOHBDynamic) 		& \FASTxalanFTOWCP & (\FASTxalanFTOWCPDynamic)		& \FASTxalanFTODC & (\FASTxalanFTODCDynamic)		& \FASTxalanFTOCAPO & (\FASTxalanFTOCAPODynamic)		& \FASTxalanREWCP & (\FASTxalanREWCPDynamic)		& \FASTxalanREDC & (\FASTxalanREDCDynamic)		& \FASTxalanCAPORE & (\FASTxalanCAPOREDynamic) \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\end{table*}




%%% Detailed Race Coverage
% \subsection{Detailed Predictable Race Coverage}
%below are more involved race results with confidence intervals
\begin{table*}[t]
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\vci}[2]{#1{\;}\ci{#2}}
\newcommand{\ci}[1]{\ensuremath{\pm{\;}#1}}
\newcommand{\ciRange}[2]{(#1--#2)}
\input{result-macros/PIP_slowTool_raceLimitFix_assertCheck}
%  
\small
\centering
\begin{tabular}{@{}l|rr|rr|rr|rr|rr|rr|rr@{}}
\et{}{} & \mc{14}{c@{}}{\SlowTool: Second Site [SS] Statically distinct races (dynamic races)}  \\
\et{}{} & \mc{2}{c|}{} & \mc{2}{c|}{} & \mc{2}{c|}{} & \mc{4}{c|}{\DC-races} & \mc{4}{c}{\CAPO-races} \\
Program \et{Events}{\#Thr} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{w/o G} & \mc{2}{c|}{w/ G} & \mc{2}{c|}{w/o G} & \mc{2}{c@{}}{w/ G} \\\hline
\bench{avrora} 	\et{\SLOWavroraEvents}{\SLOWavroraThreads} 		& \vci{\SLOWavroraFT}{\SLOWavroraFTCI} 		& \ciRange{\SLOWavroraFTDynamicCIMIN}{\SLOWavroraFTDynamicCIMAX}	& \vci{\SLOWavroraHB}{\SLOWavroraHBCI} 		& \ciRange{\SLOWavroraHBDynamicCIMIN}{\SLOWavroraHBDynamicCIMAX}	& \vci{\SLOWavroraWCP}{\SLOWavroraWCPCI} 		& \ciRange{\SLOWavroraWCPDynamicCIMIN}{\SLOWavroraWCPDynamicCIMAX} 		& \vci{\SLOWavroraWDC}{\SLOWavroraWDCCI} 		& \ciRange{\SLOWavroraWDCDynamicCIMIN}{\SLOWavroraWDCDynamicCIMAX} \\
\bench{batik} 	\et{\SLOWbatikEvents}{\SLOWbatikThreads} 		& \vci{\SLOWbatikFT}{\SLOWbatikFTCI} 		& \ciRange{\SLOWbatikFTDynamicCIMIN}{\SLOWbatikFTDynamicCIMAX} 		& \vci{\SLOWbatikHB}{\SLOWbatikHBCI} 		& \ciRange{\SLOWbatikHBDynamicCIMIN}{\SLOWbatikHBDynamicCIMAX} 		& \vci{\SLOWbatikWCP}{\SLOWbatikWCPCI} 			& \ciRange{\SLOWbatikWCPDynamicCIMIN}{\SLOWbatikWCPDynamicCIMAX} 		& \vci{\SLOWbatikWDC}{\SLOWbatikWDCCI} 			& \ciRange{\SLOWbatikWDCDynamicCIMIN}{\SLOWbatikWDCDynamicCIMAX} \\
\bench{h2} 		\et{\SLOWhtwoEvents}{\SLOWhtwoThreads} 			& \vci{\SLOWhtwoFT}{\SLOWhtwoFTCI} 			& \ciRange{\SLOWhtwoFTDynamicCIMIN}{\SLOWhtwoFTDynamicCIMAX}		& \vci{\SLOWhtwoHB}{\SLOWhtwoHBCI} 			& \ciRange{\SLOWhtwoHBDynamicCIMIN}{\SLOWhtwoHBDynamicCIMAX} 		& \vci{\SLOWhtwoWCP}{\SLOWhtwoWCPCI} 			& \ciRange{\SLOWhtwoWCPDynamicCIMIN}{\SLOWhtwoWCPDynamicCIMAX} 			& \vci{\SLOWhtwoWDC}{\SLOWhtwoWDCCI} 			& \ciRange{\SLOWhtwoWDCDynamicCIMIN}{\SLOWhtwoWDCDynamicCIMAX} \\
\bench{jython} 	\et{\SLOWjythonEvents}{\SLOWjythonThreads} 		& \vci{\SLOWjythonFT}{\SLOWjythonFTCI} 		& \ciRange{\SLOWjythonFTDynamicCIMIN}{\SLOWjythonFTDynamicCIMAX}	& \vci{\SLOWjythonHB}{\SLOWjythonHBCI} 		& \ciRange{\SLOWjythonHBDynamicCIMIN}{\SLOWjythonHBDynamicCIMAX} 	& \vci{\SLOWjythonWCP}{\SLOWjythonWCPCI} 		& \ciRange{\SLOWjythonWCPDynamicCIMIN}{\SLOWjythonWCPDynamicCIMAX} 		& \vci{\SLOWjythonWDC}{\SLOWjythonWDCCI} 		& \ciRange{\SLOWjythonWDCDynamicCIMIN}{\SLOWjythonWDCDynamicCIMAX} \\
\bench{luindex} \et{\SLOWluindexEvents}{\SLOWluindexThreads} 	& \vci{\SLOWluindexFT}{\SLOWluindexFTCI} 	& \ciRange{\SLOWluindexFTDynamicCIMIN}{\SLOWluindexFTDynamicCIMAX}	& \vci{\SLOWluindexHB}{\SLOWluindexHBCI} 	& \ciRange{\SLOWluindexHBDynamicCIMIN}{\SLOWluindexHBDynamicCIMAX} 	& \vci{\SLOWluindexWCP}{\SLOWluindexWCPCI} 		& \ciRange{\SLOWluindexWCPDynamicCIMIN}{\SLOWluindexWCPDynamicCIMAX} 	& \vci{\SLOWluindexWDC}{\SLOWluindexWDCCI} 		& \ciRange{\SLOWluindexWDCDynamicCIMIN}{\SLOWluindexWDCDynamicCIMAX} \\
\bench{lusearch}\et{\SLOWlusearchEvents}{\SLOWlusearchThreads}	& \vci{\SLOWlusearchFT}{\SLOWlusearchFTCI} 	& \ciRange{\SLOWlusearchFTDynamicCIMIN}{\SLOWlusearchFTDynamicCIMAX}& \vci{\SLOWlusearchHB}{\SLOWlusearchHBCI} 	& \ciRange{\SLOWlusearchHBDynamicCIMIN}{\SLOWlusearchHBDynamicCIMAX}& \vci{\SLOWlusearchWCP}{\SLOWlusearchWCPCI} 	& \ciRange{\SLOWlusearchWCPDynamicCIMIN}{\SLOWlusearchWCPDynamicCIMAX} 	& \vci{\SLOWlusearchWDC}{\SLOWlusearchWDCCI} 	& \ciRange{\SLOWlusearchWDCDynamicCIMIN}{\SLOWlusearchWDCDynamicCIMAX} \\
\bench{pmd} 	\et{\SLOWpmdEvents}{\SLOWpmdThreads} 			& \vci{\SLOWpmdFT}{\SLOWpmdFTCI} 			& \ciRange{\SLOWpmdFTDynamicCIMIN}{\SLOWpmdFTDynamicCIMAX}			& \vci{\SLOWpmdHB}{\SLOWpmdHBCI} 			& \ciRange{\SLOWpmdHBDynamicCIMIN}{\SLOWpmdHBDynamicCIMAX} 			& \vci{\SLOWpmdWCP}{\SLOWpmdWCPCI}	 			& \ciRange{\SLOWpmdWCPDynamicCIMIN}{\SLOWpmdWCPDynamicCIMAX} 			& \vci{\SLOWpmdWDC}{\SLOWpmdWDCCI}	 			& \ciRange{\SLOWpmdWDCDynamicCIMIN}{\SLOWpmdWDCDynamicCIMAX} \\
\bench{sunflow} \et{\SLOWsunflowEvents}{\SLOWsunflowThreads} 	& \vci{\SLOWsunflowFT}{\SLOWsunflowFTCI} 	& \ciRange{\SLOWsunflowFTDynamicCIMIN}{\SLOWsunflowFTDynamicCIMAX} 	& \vci{\SLOWsunflowHB}{\SLOWsunflowHBCI} 	& \ciRange{\SLOWsunflowHBDynamicCIMIN}{\SLOWsunflowHBDynamicCIMAX} 	& \vci{\SLOWsunflowWCP}{\SLOWsunflowWCPCI} 		& \ciRange{\SLOWsunflowWCPDynamicCIMIN}{\SLOWsunflowWCPDynamicCIMAX} 	& \vci{\SLOWsunflowWDC}{\SLOWsunflowWDCCI} 		& \ciRange{\SLOWsunflowWDCDynamicCIMIN}{\SLOWsunflowWDCDynamicCIMAX} \\
\bench{tomcat} 	\et{\SLOWtomcatEvents}{\SLOWtomcatThreads} 		& \vci{\SLOWtomcatFT}{\SLOWtomcatFTCI} 		& \ciRange{\SLOWtomcatFTDynamicCIMIN}{\SLOWtomcatFTDynamicCIMAX}	& \vci{\SLOWtomcatHB}{\SLOWtomcatHBCI} 		& \ciRange{\SLOWtomcatHBDynamicCIMIN}{\SLOWtomcatHBDynamicCIMAX} 	& \vci{\SLOWtomcatWCP}{\SLOWtomcatWCPCI} 		& \ciRange{\SLOWtomcatWCPDynamicCIMIN}{\SLOWtomcatWCPDynamicCIMAX} 		& \vci{\SLOWtomcatWDC}{\SLOWtomcatWDCCI} 		& \ciRange{\SLOWtomcatWDCDynamicCIMIN}{\SLOWtomcatWDCDynamicCIMAX} \\
\bench{xalan} 	\et{\SLOWxalanEvents}{\SLOWxalanThreads} 		& \vci{\SLOWxalanFT}{\SLOWxalanFTCI} 		& \ciRange{\SLOWxalanFTDynamicCIMIN}{\SLOWxalanFTDynamicCIMAX}		& \vci{\SLOWxalanHB}{\SLOWxalanHBCI} 		& \ciRange{\SLOWxalanHBDynamicCIMIN}{\SLOWxalanHBDynamicCIMAX} 		& \vci{\SLOWxalanWCP}{\SLOWxalanWCPCI} 			& \ciRange{\SLOWxalanWCPDynamicCIMIN}{\SLOWxalanWCPDynamicCIMAX} 		& \vci{\SLOWxalanWDC}{\SLOWxalanWDCCI} 			& \ciRange{\SLOWxalanWDCDynamicCIMIN}{\SLOWxalanWDCDynamicCIMAX} \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\newcommand{\vci}[2]{#1{\;}\ci{#2}}
\newcommand{\ci}[1]{\ensuremath{\pm{\;}#1}}
\newcommand{\ciRange}[2]{(#1--#2)}
% \input{result-macros/PIP_fastTool_performanceProfile}
% \input{result-macros/PIP_fastTool_CAPOOpt_RuleAFix}
\input{result-macros/PIP_fastTool_FTO_All}
%  
\small
\centering
\begin{tabular}{@{}l|rr|rr|rr|rr|rr@{}}
\et{}{} & \mc{10}{c@{}}{\FastTool: Statically distinct races (dynamic races)}  \\
Program \et{Events}{\#Thr} & \mc{2}{c|}{\FT-races} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c}{\DC-races} & \mc{2}{c}{\CAPO-races} \\\hline
\bench{avrora} 	\et{\FASTavroraEvents}{\FASTavroraThreads} 		& \vci{\FASTavroraFT}{\FASTavroraFTCI} 		& \ciRange{\FASTavroraFTDynamicCIMIN}{\FASTavroraFTDynamicCIMAX}	& \vci{\FASTavroraHB}{\FASTavroraHBCI} 		& \ciRange{\FASTavroraHBDynamicCIMIN}{\FASTavroraHBDynamicCIMAX}	& \vci{\FASTavroraWCP}{\FASTavroraWCPCI} 		& \ciRange{\FASTavroraWCPDynamicCIMIN}{\FASTavroraWCPDynamicCIMAX} 		& \vci{\FASTavroraDC}{\FASTavroraDCCI} 		& \ciRange{\FASTavroraDCDynamicCIMIN}{\FASTavroraDCDynamicCIMAX} 	& \vci{\FASTavroraCAPO}{\FASTavroraCAPOCI} 		& \ciRange{\FASTavroraCAPODynamicCIMIN}{\FASTavroraCAPODynamicCIMAX} \\
\bench{batik} 	\et{\FASTbatikEvents}{\FASTbatikThreads} 		& \vci{\FASTbatikFT}{\FASTbatikFTCI} 		& \ciRange{\FASTbatikFTDynamicCIMIN}{\FASTbatikFTDynamicCIMAX} 		& \vci{\FASTbatikHB}{\FASTbatikHBCI} 		& \ciRange{\FASTbatikHBDynamicCIMIN}{\FASTbatikHBDynamicCIMAX} 		& \vci{\FASTbatikWCP}{\FASTbatikWCPCI} 			& \ciRange{\FASTbatikWCPDynamicCIMIN}{\FASTbatikWCPDynamicCIMAX} 		& \vci{\FASTbatikDC}{\FASTbatikDCCI} 		& \ciRange{\FASTbatikDCDynamicCIMIN}{\FASTbatikDCDynamicCIMAX} 		& \vci{\FASTbatikCAPO}{\FASTbatikCAPOCI} 		& \ciRange{\FASTbatikCAPODynamicCIMIN}{\FASTbatikCAPODynamicCIMAX} \\
\bench{h2} 		\et{\FASThtwoEvents}{\FASThtwoThreads} 			& \vci{\FASThtwoFT}{\FASThtwoFTCI} 			& \ciRange{\FASThtwoFTDynamicCIMIN}{\FASThtwoFTDynamicCIMAX}		& \vci{\FASThtwoHB}{\FASThtwoHBCI} 			& \ciRange{\FASThtwoHBDynamicCIMIN}{\FASThtwoHBDynamicCIMAX} 		& \vci{\FASThtwoWCP}{\FASThtwoWCPCI} 			& \ciRange{\FASThtwoWCPDynamicCIMIN}{\FASThtwoWCPDynamicCIMAX} 			& \vci{\FASThtwoDC}{\FASThtwoDCCI} 			& \ciRange{\FASThtwoDCDynamicCIMIN}{\FASThtwoDCDynamicCIMAX} 		& \vci{\FASThtwoCAPO}{\FASThtwoCAPOCI} 			& \ciRange{\FASThtwoCAPODynamicCIMIN}{\FASThtwoCAPODynamicCIMAX} \\
\bench{jython} 	\et{\FASTjythonEvents}{\FASTjythonThreads} 		& \vci{\FASTjythonFT}{\FASTjythonFTCI} 		& \ciRange{\FASTjythonFTDynamicCIMIN}{\FASTjythonFTDynamicCIMAX}	& \vci{\FASTjythonHB}{\FASTjythonHBCI} 		& \ciRange{\FASTjythonHBDynamicCIMIN}{\FASTjythonHBDynamicCIMAX} 	& \vci{\FASTjythonWCP}{\FASTjythonWCPCI} 		& \ciRange{\FASTjythonWCPDynamicCIMIN}{\FASTjythonWCPDynamicCIMAX} 		& \vci{\FASTjythonDC}{\FASTjythonDCCI} 		& \ciRange{\FASTjythonDCDynamicCIMIN}{\FASTjythonDCDynamicCIMAX} 	& \vci{\FASTjythonCAPO}{\FASTjythonCAPOCI} 		& \ciRange{\FASTjythonCAPODynamicCIMIN}{\FASTjythonCAPODynamicCIMAX} \\
\bench{luindex} \et{\FASTluindexEvents}{\FASTluindexThreads} 	& \vci{\FASTluindexFT}{\FASTluindexFTCI} 	& \ciRange{\FASTluindexFTDynamicCIMIN}{\FASTluindexFTDynamicCIMAX}	& \vci{\FASTluindexHB}{\FASTluindexHBCI} 	& \ciRange{\FASTluindexHBDynamicCIMIN}{\FASTluindexHBDynamicCIMAX} 	& \vci{\FASTluindexWCP}{\FASTluindexWCPCI} 		& \ciRange{\FASTluindexWCPDynamicCIMIN}{\FASTluindexWCPDynamicCIMAX} 	& \vci{\FASTluindexDC}{\FASTluindexDCCI} 	& \ciRange{\FASTluindexDCDynamicCIMIN}{\FASTluindexDCDynamicCIMAX} 	& \vci{\FASTluindexCAPO}{\FASTluindexCAPOCI} 	& \ciRange{\FASTluindexCAPODynamicCIMIN}{\FASTluindexCAPODynamicCIMAX} \\
\bench{lusearch}\et{\FASTlusearchEvents}{\FASTlusearchThreads}	& \vci{\FASTlusearchFT}{\FASTlusearchFTCI} 	& \ciRange{\FASTlusearchFTDynamicCIMIN}{\FASTlusearchFTDynamicCIMAX}& \vci{\FASTlusearchHB}{\FASTlusearchHBCI} 	& \ciRange{\FASTlusearchHBDynamicCIMIN}{\FASTlusearchHBDynamicCIMAX}& \vci{\FASTlusearchWCP}{\FASTlusearchWCPCI} 	& \ciRange{\FASTlusearchWCPDynamicCIMIN}{\FASTlusearchWCPDynamicCIMAX} 	& \vci{\FASTlusearchDC}{\FASTlusearchDCCI} 	& \ciRange{\FASTlusearchDCDynamicCIMIN}{\FASTlusearchDCDynamicCIMAX}& \vci{\FASTlusearchCAPO}{\FASTlusearchCAPOCI} 	& \ciRange{\FASTlusearchCAPODynamicCIMIN}{\FASTlusearchCAPODynamicCIMAX} \\
\bench{pmd} 	\et{\FASTpmdEvents}{\FASTpmdThreads} 			& \vci{\FASTpmdFT}{\FASTpmdFTCI} 			& \ciRange{\FASTpmdFTDynamicCIMIN}{\FASTpmdFTDynamicCIMAX}			& \vci{\FASTpmdHB}{\FASTpmdHBCI} 			& \ciRange{\FASTpmdHBDynamicCIMIN}{\FASTpmdHBDynamicCIMAX} 			& \vci{\FASTpmdWCP}{\FASTpmdWCPCI}	 			& \ciRange{\FASTpmdWCPDynamicCIMIN}{\FASTpmdWCPDynamicCIMAX} 			& \vci{\FASTpmdDC}{\FASTpmdDCCI}	 		& \ciRange{\FASTpmdDCDynamicCIMIN}{\FASTpmdDCDynamicCIMAX} 			& \vci{\FASTpmdCAPO}{\FASTpmdCAPOCI} 			& \ciRange{\FASTpmdCAPODynamicCIMIN}{\FASTpmdCAPODynamicCIMAX} \\
\bench{sunflow} \et{\FASTsunflowEvents}{\FASTsunflowThreads} 	& \vci{\FASTsunflowFT}{\FASTsunflowFTCI} 	& \ciRange{\FASTsunflowFTDynamicCIMIN}{\FASTsunflowFTDynamicCIMAX} 	& \vci{\FASTsunflowHB}{\FASTsunflowHBCI} 	& \ciRange{\FASTsunflowHBDynamicCIMIN}{\FASTsunflowHBDynamicCIMAX} 	& \vci{\FASTsunflowWCP}{\FASTsunflowWCPCI} 		& \ciRange{\FASTsunflowWCPDynamicCIMIN}{\FASTsunflowWCPDynamicCIMAX} 	& \vci{\FASTsunflowDC}{\FASTsunflowDCCI} 	& \ciRange{\FASTsunflowDCDynamicCIMIN}{\FASTsunflowDCDynamicCIMAX} 	& \vci{\FASTsunflowCAPO}{\FASTsunflowCAPOCI} 	& \ciRange{\FASTsunflowCAPODynamicCIMIN}{\FASTsunflowCAPODynamicCIMAX} \\
\bench{tomcat} 	\et{\FASTtomcatEvents}{\FASTtomcatThreads} 		& \vci{\FASTtomcatFT}{\FASTtomcatFTCI} 		& \ciRange{\FASTtomcatFTDynamicCIMIN}{\FASTtomcatFTDynamicCIMAX}	& \vci{\FASTtomcatHB}{\FASTtomcatHBCI} 		& \ciRange{\FASTtomcatHBDynamicCIMIN}{\FASTtomcatHBDynamicCIMAX} 	& \vci{\FASTtomcatWCP}{\FASTtomcatWCPCI} 		& \ciRange{\FASTtomcatWCPDynamicCIMIN}{\FASTtomcatWCPDynamicCIMAX} 		& \vci{\FASTtomcatDC}{\FASTtomcatDCCI} 		& \ciRange{\FASTtomcatDCDynamicCIMIN}{\FASTtomcatDCDynamicCIMAX} 	& \vci{\FASTtomcatCAPO}{\FASTtomcatCAPOCI} 		& \ciRange{\FASTtomcatCAPODynamicCIMIN}{\FASTtomcatCAPODynamicCIMAX} \\
\bench{xalan} 	\et{\FASTxalanEvents}{\FASTxalanThreads} 		& \vci{\FASTxalanFT}{\FASTxalanFTCI} 		& \ciRange{\FASTxalanFTDynamicCIMIN}{\FASTxalanFTDynamicCIMAX}		& \vci{\FASTxalanHB}{\FASTxalanHBCI} 		& \ciRange{\FASTxalanHBDynamicCIMIN}{\FASTxalanHBDynamicCIMAX} 		& \vci{\FASTxalanWCP}{\FASTxalanWCPCI} 			& \ciRange{\FASTxalanWCPDynamicCIMIN}{\FASTxalanWCPDynamicCIMAX} 		& \vci{\FASTxalanDC}{\FASTxalanDCCI} 		& \ciRange{\FASTxalanDCDynamicCIMIN}{\FASTxalanDCDynamicCIMAX} 		& \vci{\FASTxalanCAPO}{\FASTxalanCAPOCI} 		& \ciRange{\FASTxalanCAPODynamicCIMIN}{\FASTxalanCAPODynamicCIMAX} \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\newcommand{\vci}[2]{#1{\;}\ci{#2}}
\newcommand{\ci}[1]{\ensuremath{\pm{\;}#1}}
\newcommand{\ciRange}[2]{(#1--#2)}
% \input{result-macros/PIP_fastTool_performanceProfile}
% \input{result-macros/PIP_fastTool_CAPOOpt_RuleAFix}
\input{result-macros/PIP_fastTool_FTO_All}
%
\small
\centering
\begin{tabular}{@{}l|rr|rr|rr|rrHHHHHH@{}}
\et{}{} & \mc{14}{c@{}}{\FastTool: Statically distinct races (dynamic races)}  \\
\et{}{} & \mc{8}{c}{FTO w/o G} & \mc{6}{H}{FTO W/ G} \\
Program \et{Events}{\#Thr} & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c}{\CAPO-races} & \mc{2}{H}{\WCP-races} & \mc{2}{H}{\DC-races} & \mc{2}{H}{\CAPO-races} \\\hline
\bench{avrora} 	\et{\FASTavroraEvents}{\FASTavroraThreads} 		& \vci{\FASTavroraFTOHB}{\FASTavroraFTOHBCI} 	& \ciRange{\FASTavroraFTOHBDynamicCIMIN}{\FASTavroraFTOHBDynamicCIMAX}		& \vci{\FASTavroraFTOWCP}{\FASTavroraFTOWCPCI} 		& \ciRange{\FASTavroraFTOWCPDynamicCIMIN}{\FASTavroraFTOWCPDynamicCIMAX} 	& \vci{\FASTavroraFTODC}{\FASTavroraFTODCCI} 	& \ciRange{\FASTavroraFTODCDynamicCIMIN}{\FASTavroraFTODCDynamicCIMAX} 		& \vci{\FASTavroraFTOCAPO}{\FASTavroraFTOCAPOCI} 	& \ciRange{\FASTavroraFTOCAPODynamicCIMIN}{\FASTavroraFTOCAPODynamicCIMAX}		& \vci{\FASTavroraREWCP}{\FASTavroraREWCPCI} 		& \ciRange{\FASTavroraREWCPDynamicCIMIN}{\FASTavroraREWCPDynamicCIMAX} 		& \vci{\FASTavroraREDC}{\FASTavroraREDCCI} 		& \ciRange{\FASTavroraREDCDynamicCIMIN}{\FASTavroraREDCDynamicCIMAX} 	& \vci{\FASTavroraCAPORE}{\FASTavroraCAPORECI} 		& \ciRange{\FASTavroraCAPOREDynamicCIMIN}{\FASTavroraCAPOREDynamicCIMAX} \\
\bench{batik} 	\et{\FASTbatikEvents}{\FASTbatikThreads} 		& \vci{\FASTbatikFTOHB}{\FASTbatikFTOHBCI} 		& \ciRange{\FASTbatikFTOHBDynamicCIMIN}{\FASTbatikFTOHBDynamicCIMAX} 		& \vci{\FASTbatikFTOWCP}{\FASTbatikFTOWCPCI} 		& \ciRange{\FASTbatikFTOWCPDynamicCIMIN}{\FASTbatikFTOWCPDynamicCIMAX} 		& \vci{\FASTbatikFTODC}{\FASTbatikFTODCCI} 		& \ciRange{\FASTbatikFTODCDynamicCIMIN}{\FASTbatikFTODCDynamicCIMAX} 		& \vci{\FASTbatikFTOCAPO}{\FASTbatikFTOCAPOCI} 		& \ciRange{\FASTbatikFTOCAPODynamicCIMIN}{\FASTbatikFTOCAPODynamicCIMAX} 		& \vci{\FASTbatikREWCP}{\FASTbatikREWCPCI} 			& \ciRange{\FASTbatikREWCPDynamicCIMIN}{\FASTbatikREWCPDynamicCIMAX} 		& \vci{\FASTbatikREDC}{\FASTbatikREDCCI} 		& \ciRange{\FASTbatikREDCDynamicCIMIN}{\FASTbatikREDCDynamicCIMAX} 		& \vci{\FASTbatikCAPORE}{\FASTbatikCAPORECI} 		& \ciRange{\FASTbatikCAPOREDynamicCIMIN}{\FASTbatikCAPOREDynamicCIMAX} \\
\bench{h2} 		\et{\FASThtwoEvents}{\FASThtwoThreads} 			& \vci{\FASThtwoFTOHB}{\FASThtwoFTOHBCI} 		& \ciRange{\FASThtwoFTOHBDynamicCIMIN}{\FASThtwoFTOHBDynamicCIMAX} 			& \vci{\FASThtwoFTOWCP}{\FASThtwoFTOWCPCI} 			& \ciRange{\FASThtwoFTOWCPDynamicCIMIN}{\FASThtwoFTOWCPDynamicCIMAX} 		& \vci{\FASThtwoFTODC}{\FASThtwoFTODCCI} 		& \ciRange{\FASThtwoFTODCDynamicCIMIN}{\FASThtwoFTODCDynamicCIMAX} 			& \vci{\FASThtwoFTOCAPO}{\FASThtwoFTOCAPOCI} 		& \ciRange{\FASThtwoFTOCAPODynamicCIMIN}{\FASThtwoFTOCAPODynamicCIMAX} 			& \vci{\FASThtwoREWCP}{\FASThtwoREWCPCI} 			& \ciRange{\FASThtwoREWCPDynamicCIMIN}{\FASThtwoREWCPDynamicCIMAX} 			& \vci{\FASThtwoREDC}{\FASThtwoREDCCI} 			& \ciRange{\FASThtwoREDCDynamicCIMIN}{\FASThtwoREDCDynamicCIMAX} 		& \vci{\FASThtwoCAPORE}{\FASThtwoCAPORECI} 			& \ciRange{\FASThtwoCAPOREDynamicCIMIN}{\FASThtwoCAPOREDynamicCIMAX} \\
\bench{jython} 	\et{\FASTjythonEvents}{\FASTjythonThreads} 		& \vci{\FASTjythonFTOHB}{\FASTjythonFTOHBCI} 	& \ciRange{\FASTjythonFTOHBDynamicCIMIN}{\FASTjythonFTOHBDynamicCIMAX} 		& \vci{\FASTjythonFTOWCP}{\FASTjythonFTOWCPCI} 		& \ciRange{\FASTjythonFTOWCPDynamicCIMIN}{\FASTjythonFTOWCPDynamicCIMAX} 	& \vci{\FASTjythonFTODC}{\FASTjythonFTODCCI} 	& \ciRange{\FASTjythonFTODCDynamicCIMIN}{\FASTjythonFTODCDynamicCIMAX} 		& \vci{\FASTjythonFTOCAPO}{\FASTjythonFTOCAPOCI} 	& \ciRange{\FASTjythonFTOCAPODynamicCIMIN}{\FASTjythonFTOCAPODynamicCIMAX} 		& \vci{\FASTjythonREWCP}{\FASTjythonREWCPCI} 		& \ciRange{\FASTjythonREWCPDynamicCIMIN}{\FASTjythonREWCPDynamicCIMAX} 		& \vci{\FASTjythonREDC}{\FASTjythonREDCCI} 		& \ciRange{\FASTjythonREDCDynamicCIMIN}{\FASTjythonREDCDynamicCIMAX} 	& \vci{\FASTjythonCAPORE}{\FASTjythonCAPORECI} 		& \ciRange{\FASTjythonCAPOREDynamicCIMIN}{\FASTjythonCAPOREDynamicCIMAX} \\
\bench{luindex} \et{\FASTluindexEvents}{\FASTluindexThreads} 	& \vci{\FASTluindexFTOHB}{\FASTluindexFTOHBCI} 	& \ciRange{\FASTluindexFTOHBDynamicCIMIN}{\FASTluindexFTOHBDynamicCIMAX} 	& \vci{\FASTluindexFTOWCP}{\FASTluindexFTOWCPCI} 	& \ciRange{\FASTluindexFTOWCPDynamicCIMIN}{\FASTluindexFTOWCPDynamicCIMAX} 	& \vci{\FASTluindexFTODC}{\FASTluindexFTODCCI} 	& \ciRange{\FASTluindexFTODCDynamicCIMIN}{\FASTluindexFTODCDynamicCIMAX} 	& \vci{\FASTluindexFTOCAPO}{\FASTluindexFTOCAPOCI} 	& \ciRange{\FASTluindexFTOCAPODynamicCIMIN}{\FASTluindexFTOCAPODynamicCIMAX} 	& \vci{\FASTluindexREWCP}{\FASTluindexREWCPCI} 		& \ciRange{\FASTluindexREWCPDynamicCIMIN}{\FASTluindexREWCPDynamicCIMAX} 	& \vci{\FASTluindexREDC}{\FASTluindexREDCCI} 	& \ciRange{\FASTluindexREDCDynamicCIMIN}{\FASTluindexREDCDynamicCIMAX} 	& \vci{\FASTluindexCAPORE}{\FASTluindexCAPORECI} 	& \ciRange{\FASTluindexCAPOREDynamicCIMIN}{\FASTluindexCAPOREDynamicCIMAX} \\
\bench{lusearch}\et{\FASTlusearchEvents}{\FASTlusearchThreads}	& \vci{\FASTlusearchFTOHB}{\FASTlusearchFTOHBCI}& \ciRange{\FASTlusearchFTOHBDynamicCIMIN}{\FASTlusearchFTOHBDynamicCIMAX}	& \vci{\FASTlusearchFTOWCP}{\FASTlusearchFTOWCPCI} 	& \ciRange{\FASTlusearchFTOWCPDynamicCIMIN}{\FASTlusearchFTOWCPDynamicCIMAX}& \vci{\FASTlusearchFTODC}{\FASTlusearchFTODCCI}& \ciRange{\FASTlusearchFTODCDynamicCIMIN}{\FASTlusearchFTODCDynamicCIMAX}	& \vci{\FASTlusearchFTOCAPO}{\FASTlusearchFTOCAPOCI}& \ciRange{\FASTlusearchFTOCAPODynamicCIMIN}{\FASTlusearchFTOCAPODynamicCIMAX}	& \vci{\FASTlusearchREWCP}{\FASTlusearchREWCPCI} 	& \ciRange{\FASTlusearchREWCPDynamicCIMIN}{\FASTlusearchREWCPDynamicCIMAX} 	& \vci{\FASTlusearchREDC}{\FASTlusearchREDCCI} 	& \ciRange{\FASTlusearchREDCDynamicCIMIN}{\FASTlusearchREDCDynamicCIMAX}& \vci{\FASTlusearchCAPORE}{\FASTlusearchCAPORECI} 	& \ciRange{\FASTlusearchCAPOREDynamicCIMIN}{\FASTlusearchCAPOREDynamicCIMAX} \\
\bench{pmd} 	\et{\FASTpmdEvents}{\FASTpmdThreads} 			& \vci{\FASTpmdFTOHB}{\FASTpmdFTOHBCI} 			& \ciRange{\FASTpmdFTOHBDynamicCIMIN}{\FASTpmdFTOHBDynamicCIMAX} 			& \vci{\FASTpmdFTOWCP}{\FASTpmdFTOWCPCI}	 		& \ciRange{\FASTpmdFTOWCPDynamicCIMIN}{\FASTpmdFTOWCPDynamicCIMAX} 			& \vci{\FASTpmdFTODC}{\FASTpmdFTODCCI}	 		& \ciRange{\FASTpmdFTODCDynamicCIMIN}{\FASTpmdFTODCDynamicCIMAX} 			& \vci{\FASTpmdFTOCAPO}{\FASTpmdFTOCAPOCI} 			& \ciRange{\FASTpmdFTOCAPODynamicCIMIN}{\FASTpmdFTOCAPODynamicCIMAX} 			& \vci{\FASTpmdREWCP}{\FASTpmdREWCPCI}	 			& \ciRange{\FASTpmdREWCPDynamicCIMIN}{\FASTpmdREWCPDynamicCIMAX} 			& \vci{\FASTpmdREDC}{\FASTpmdREDCCI}	 		& \ciRange{\FASTpmdREDCDynamicCIMIN}{\FASTpmdREDCDynamicCIMAX} 			& \vci{\FASTpmdCAPORE}{\FASTpmdCAPORECI} 			& \ciRange{\FASTpmdCAPOREDynamicCIMIN}{\FASTpmdCAPOREDynamicCIMAX} \\
\bench{sunflow} \et{\FASTsunflowEvents}{\FASTsunflowThreads} 	& \vci{\FASTsunflowFTOHB}{\FASTsunflowFTOHBCI} 	& \ciRange{\FASTsunflowFTOHBDynamicCIMIN}{\FASTsunflowFTOHBDynamicCIMAX} 	& \vci{\FASTsunflowFTOWCP}{\FASTsunflowFTOWCPCI} 	& \ciRange{\FASTsunflowFTOWCPDynamicCIMIN}{\FASTsunflowFTOWCPDynamicCIMAX} 	& \vci{\FASTsunflowFTODC}{\FASTsunflowFTODCCI} 	& \ciRange{\FASTsunflowFTODCDynamicCIMIN}{\FASTsunflowFTODCDynamicCIMAX} 	& \vci{\FASTsunflowFTOCAPO}{\FASTsunflowFTOCAPOCI} 	& \ciRange{\FASTsunflowFTOCAPODynamicCIMIN}{\FASTsunflowFTOCAPODynamicCIMAX} 	& \vci{\FASTsunflowREWCP}{\FASTsunflowREWCPCI} 		& \ciRange{\FASTsunflowREWCPDynamicCIMIN}{\FASTsunflowREWCPDynamicCIMAX} 	& \vci{\FASTsunflowREDC}{\FASTsunflowREDCCI} 	& \ciRange{\FASTsunflowREDCDynamicCIMIN}{\FASTsunflowREDCDynamicCIMAX} 	& \vci{\FASTsunflowCAPORE}{\FASTsunflowCAPORECI} 	& \ciRange{\FASTsunflowCAPOREDynamicCIMIN}{\FASTsunflowCAPOREDynamicCIMAX} \\
\bench{tomcat} 	\et{\FASTtomcatEvents}{\FASTtomcatThreads} 		& \vci{\FASTtomcatFTOHB}{\FASTtomcatFTOHBCI} 	& \ciRange{\FASTtomcatFTOHBDynamicCIMIN}{\FASTtomcatFTOHBDynamicCIMAX} 		& \vci{\FASTtomcatFTOWCP}{\FASTtomcatFTOWCPCI} 		& \ciRange{\FASTtomcatFTOWCPDynamicCIMIN}{\FASTtomcatFTOWCPDynamicCIMAX} 	& \vci{\FASTtomcatFTODC}{\FASTtomcatFTODCCI} 	& \ciRange{\FASTtomcatFTODCDynamicCIMIN}{\FASTtomcatFTODCDynamicCIMAX} 		& \vci{\FASTtomcatFTOCAPO}{\FASTtomcatFTOCAPOCI} 	& \ciRange{\FASTtomcatFTOCAPODynamicCIMIN}{\FASTtomcatFTOCAPODynamicCIMAX} 		& \vci{\FASTtomcatREWCP}{\FASTtomcatREWCPCI} 		& \ciRange{\FASTtomcatREWCPDynamicCIMIN}{\FASTtomcatREWCPDynamicCIMAX} 		& \vci{\FASTtomcatREDC}{\FASTtomcatREDCCI} 		& \ciRange{\FASTtomcatREDCDynamicCIMIN}{\FASTtomcatREDCDynamicCIMAX} 	& \vci{\FASTtomcatCAPORE}{\FASTtomcatCAPORECI} 		& \ciRange{\FASTtomcatCAPOREDynamicCIMIN}{\FASTtomcatCAPOREDynamicCIMAX} \\
\bench{xalan} 	\et{\FASTxalanEvents}{\FASTxalanThreads} 		& \vci{\FASTxalanFTOHB}{\FASTxalanFTOHBCI} 		& \ciRange{\FASTxalanFTOHBDynamicCIMIN}{\FASTxalanFTOHBDynamicCIMAX} 		& \vci{\FASTxalanFTOWCP}{\FASTxalanFTOWCPCI} 		& \ciRange{\FASTxalanFTOWCPDynamicCIMIN}{\FASTxalanFTOWCPDynamicCIMAX} 		& \vci{\FASTxalanFTODC}{\FASTxalanFTODCCI} 		& \ciRange{\FASTxalanFTODCDynamicCIMIN}{\FASTxalanFTODCDynamicCIMAX} 		& \vci{\FASTxalanFTOCAPO}{\FASTxalanFTOCAPOCI} 		& \ciRange{\FASTxalanFTOCAPODynamicCIMIN}{\FASTxalanFTOCAPODynamicCIMAX} 		& \vci{\FASTxalanREWCP}{\FASTxalanREWCPCI} 			& \ciRange{\FASTxalanREWCPDynamicCIMIN}{\FASTxalanREWCPDynamicCIMAX} 		& \vci{\FASTxalanREDC}{\FASTxalanREDCCI} 		& \ciRange{\FASTxalanREDCDynamicCIMIN}{\FASTxalanREDCDynamicCIMAX} 		& \vci{\FASTxalanCAPORE}{\FASTxalanCAPORECI} 		& \ciRange{\FASTxalanCAPOREDynamicCIMIN}{\FASTxalanCAPOREDynamicCIMAX} \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\newcommand{\vci}[2]{#1{\;}\ci{#2}}
\newcommand{\ci}[1]{\ensuremath{\pm{\;}#1}}
\newcommand{\ciRange}[2]{(#1--#2)}
% \input{result-macros/PIP_fastTool_performanceProfile}
% \input{result-macros/PIP_fastTool_CAPOOpt_RuleAFix}
\input{result-macros/PIP_fastTool_FTO_All}
%
\small
\centering
\begin{tabular}{@{}l|HHHHHHHHrr|rr|rr@{}}
\et{}{} & \mc{14}{c@{}}{\FastTool: Statically distinct races (dynamic races)}  \\
\et{}{} & \mc{8}{H}{FTO w/o G} & \mc{6}{c}{FTO W/ G} \\
Program \et{Events}{\#Thr} & \mc{2}{H}{\HB-races} & \mc{2}{H}{\WCP-races} & \mc{2}{H}{\DC-races} & \mc{2}{H}{\CAPO-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c}{\CAPO-races} \\\hline
\bench{avrora} 	\et{\FASTavroraEvents}{\FASTavroraThreads} 		& \vci{\FASTavroraFTOHB}{\FASTavroraFTOHBCI} 	& \ciRange{\FASTavroraFTOHBDynamicCIMIN}{\FASTavroraFTOHBDynamicCIMAX}		& \vci{\FASTavroraFTOWCP}{\FASTavroraFTOWCPCI} 		& \ciRange{\FASTavroraFTOWCPDynamicCIMIN}{\FASTavroraFTOWCPDynamicCIMAX} 	& \vci{\FASTavroraFTODC}{\FASTavroraFTODCCI} 	& \ciRange{\FASTavroraFTODCDynamicCIMIN}{\FASTavroraFTODCDynamicCIMAX} 		& \vci{\FASTavroraFTOCAPO}{\FASTavroraFTOCAPOCI} 	& \ciRange{\FASTavroraFTOCAPODynamicCIMIN}{\FASTavroraFTOCAPODynamicCIMAX}		& \vci{\FASTavroraREWCP}{\FASTavroraREWCPCI} 		& \ciRange{\FASTavroraREWCPDynamicCIMIN}{\FASTavroraREWCPDynamicCIMAX} 		& \vci{\FASTavroraREDC}{\FASTavroraREDCCI} 		& \ciRange{\FASTavroraREDCDynamicCIMIN}{\FASTavroraREDCDynamicCIMAX} 	& \vci{\FASTavroraCAPORE}{\FASTavroraCAPORECI} 		& \ciRange{\FASTavroraCAPOREDynamicCIMIN}{\FASTavroraCAPOREDynamicCIMAX} \\
\bench{batik} 	\et{\FASTbatikEvents}{\FASTbatikThreads} 		& \vci{\FASTbatikFTOHB}{\FASTbatikFTOHBCI} 		& \ciRange{\FASTbatikFTOHBDynamicCIMIN}{\FASTbatikFTOHBDynamicCIMAX} 		& \vci{\FASTbatikFTOWCP}{\FASTbatikFTOWCPCI} 		& \ciRange{\FASTbatikFTOWCPDynamicCIMIN}{\FASTbatikFTOWCPDynamicCIMAX} 		& \vci{\FASTbatikFTODC}{\FASTbatikFTODCCI} 		& \ciRange{\FASTbatikFTODCDynamicCIMIN}{\FASTbatikFTODCDynamicCIMAX} 		& \vci{\FASTbatikFTOCAPO}{\FASTbatikFTOCAPOCI} 		& \ciRange{\FASTbatikFTOCAPODynamicCIMIN}{\FASTbatikFTOCAPODynamicCIMAX} 		& \vci{\FASTbatikREWCP}{\FASTbatikREWCPCI} 			& \ciRange{\FASTbatikREWCPDynamicCIMIN}{\FASTbatikREWCPDynamicCIMAX} 		& \vci{\FASTbatikREDC}{\FASTbatikREDCCI} 		& \ciRange{\FASTbatikREDCDynamicCIMIN}{\FASTbatikREDCDynamicCIMAX} 		& \vci{\FASTbatikCAPORE}{\FASTbatikCAPORECI} 		& \ciRange{\FASTbatikCAPOREDynamicCIMIN}{\FASTbatikCAPOREDynamicCIMAX} \\
\bench{h2} 		\et{\FASThtwoEvents}{\FASThtwoThreads} 			& \vci{\FASThtwoFTOHB}{\FASThtwoFTOHBCI} 		& \ciRange{\FASThtwoFTOHBDynamicCIMIN}{\FASThtwoFTOHBDynamicCIMAX} 			& \vci{\FASThtwoFTOWCP}{\FASThtwoFTOWCPCI} 			& \ciRange{\FASThtwoFTOWCPDynamicCIMIN}{\FASThtwoFTOWCPDynamicCIMAX} 		& \vci{\FASThtwoFTODC}{\FASThtwoFTODCCI} 		& \ciRange{\FASThtwoFTODCDynamicCIMIN}{\FASThtwoFTODCDynamicCIMAX} 			& \vci{\FASThtwoFTOCAPO}{\FASThtwoFTOCAPOCI} 		& \ciRange{\FASThtwoFTOCAPODynamicCIMIN}{\FASThtwoFTOCAPODynamicCIMAX} 			& \vci{\FASThtwoREWCP}{\FASThtwoREWCPCI} 			& \ciRange{\FASThtwoREWCPDynamicCIMIN}{\FASThtwoREWCPDynamicCIMAX} 			& \vci{\FASThtwoREDC}{\FASThtwoREDCCI} 			& \ciRange{\FASThtwoREDCDynamicCIMIN}{\FASThtwoREDCDynamicCIMAX} 		& \vci{\FASThtwoCAPORE}{\FASThtwoCAPORECI} 			& \ciRange{\FASThtwoCAPOREDynamicCIMIN}{\FASThtwoCAPOREDynamicCIMAX} \\
\bench{jython} 	\et{\FASTjythonEvents}{\FASTjythonThreads} 		& \vci{\FASTjythonFTOHB}{\FASTjythonFTOHBCI} 	& \ciRange{\FASTjythonFTOHBDynamicCIMIN}{\FASTjythonFTOHBDynamicCIMAX} 		& \vci{\FASTjythonFTOWCP}{\FASTjythonFTOWCPCI} 		& \ciRange{\FASTjythonFTOWCPDynamicCIMIN}{\FASTjythonFTOWCPDynamicCIMAX} 	& \vci{\FASTjythonFTODC}{\FASTjythonFTODCCI} 	& \ciRange{\FASTjythonFTODCDynamicCIMIN}{\FASTjythonFTODCDynamicCIMAX} 		& \vci{\FASTjythonFTOCAPO}{\FASTjythonFTOCAPOCI} 	& \ciRange{\FASTjythonFTOCAPODynamicCIMIN}{\FASTjythonFTOCAPODynamicCIMAX} 		& \vci{\FASTjythonREWCP}{\FASTjythonREWCPCI} 		& \ciRange{\FASTjythonREWCPDynamicCIMIN}{\FASTjythonREWCPDynamicCIMAX} 		& \vci{\FASTjythonREDC}{\FASTjythonREDCCI} 		& \ciRange{\FASTjythonREDCDynamicCIMIN}{\FASTjythonREDCDynamicCIMAX} 	& \vci{\FASTjythonCAPORE}{\FASTjythonCAPORECI} 		& \ciRange{\FASTjythonCAPOREDynamicCIMIN}{\FASTjythonCAPOREDynamicCIMAX} \\
\bench{luindex} \et{\FASTluindexEvents}{\FASTluindexThreads} 	& \vci{\FASTluindexFTOHB}{\FASTluindexFTOHBCI} 	& \ciRange{\FASTluindexFTOHBDynamicCIMIN}{\FASTluindexFTOHBDynamicCIMAX} 	& \vci{\FASTluindexFTOWCP}{\FASTluindexFTOWCPCI} 	& \ciRange{\FASTluindexFTOWCPDynamicCIMIN}{\FASTluindexFTOWCPDynamicCIMAX} 	& \vci{\FASTluindexFTODC}{\FASTluindexFTODCCI} 	& \ciRange{\FASTluindexFTODCDynamicCIMIN}{\FASTluindexFTODCDynamicCIMAX} 	& \vci{\FASTluindexFTOCAPO}{\FASTluindexFTOCAPOCI} 	& \ciRange{\FASTluindexFTOCAPODynamicCIMIN}{\FASTluindexFTOCAPODynamicCIMAX} 	& \vci{\FASTluindexREWCP}{\FASTluindexREWCPCI} 		& \ciRange{\FASTluindexREWCPDynamicCIMIN}{\FASTluindexREWCPDynamicCIMAX} 	& \vci{\FASTluindexREDC}{\FASTluindexREDCCI} 	& \ciRange{\FASTluindexREDCDynamicCIMIN}{\FASTluindexREDCDynamicCIMAX} 	& \vci{\FASTluindexCAPORE}{\FASTluindexCAPORECI} 	& \ciRange{\FASTluindexCAPOREDynamicCIMIN}{\FASTluindexCAPOREDynamicCIMAX} \\
\bench{lusearch}\et{\FASTlusearchEvents}{\FASTlusearchThreads}	& \vci{\FASTlusearchFTOHB}{\FASTlusearchFTOHBCI}& \ciRange{\FASTlusearchFTOHBDynamicCIMIN}{\FASTlusearchFTOHBDynamicCIMAX}	& \vci{\FASTlusearchFTOWCP}{\FASTlusearchFTOWCPCI} 	& \ciRange{\FASTlusearchFTOWCPDynamicCIMIN}{\FASTlusearchFTOWCPDynamicCIMAX}& \vci{\FASTlusearchFTODC}{\FASTlusearchFTODCCI}& \ciRange{\FASTlusearchFTODCDynamicCIMIN}{\FASTlusearchFTODCDynamicCIMAX}	& \vci{\FASTlusearchFTOCAPO}{\FASTlusearchFTOCAPOCI}& \ciRange{\FASTlusearchFTOCAPODynamicCIMIN}{\FASTlusearchFTOCAPODynamicCIMAX}	& \vci{\FASTlusearchREWCP}{\FASTlusearchREWCPCI} 	& \ciRange{\FASTlusearchREWCPDynamicCIMIN}{\FASTlusearchREWCPDynamicCIMAX} 	& \vci{\FASTlusearchREDC}{\FASTlusearchREDCCI} 	& \ciRange{\FASTlusearchREDCDynamicCIMIN}{\FASTlusearchREDCDynamicCIMAX}& \vci{\FASTlusearchCAPORE}{\FASTlusearchCAPORECI} 	& \ciRange{\FASTlusearchCAPOREDynamicCIMIN}{\FASTlusearchCAPOREDynamicCIMAX} \\
\bench{pmd} 	\et{\FASTpmdEvents}{\FASTpmdThreads} 			& \vci{\FASTpmdFTOHB}{\FASTpmdFTOHBCI} 			& \ciRange{\FASTpmdFTOHBDynamicCIMIN}{\FASTpmdFTOHBDynamicCIMAX} 			& \vci{\FASTpmdFTOWCP}{\FASTpmdFTOWCPCI}	 		& \ciRange{\FASTpmdFTOWCPDynamicCIMIN}{\FASTpmdFTOWCPDynamicCIMAX} 			& \vci{\FASTpmdFTODC}{\FASTpmdFTODCCI}	 		& \ciRange{\FASTpmdFTODCDynamicCIMIN}{\FASTpmdFTODCDynamicCIMAX} 			& \vci{\FASTpmdFTOCAPO}{\FASTpmdFTOCAPOCI} 			& \ciRange{\FASTpmdFTOCAPODynamicCIMIN}{\FASTpmdFTOCAPODynamicCIMAX} 			& \vci{\FASTpmdREWCP}{\FASTpmdREWCPCI}	 			& \ciRange{\FASTpmdREWCPDynamicCIMIN}{\FASTpmdREWCPDynamicCIMAX} 			& \vci{\FASTpmdREDC}{\FASTpmdREDCCI}	 		& \ciRange{\FASTpmdREDCDynamicCIMIN}{\FASTpmdREDCDynamicCIMAX} 			& \vci{\FASTpmdCAPORE}{\FASTpmdCAPORECI} 			& \ciRange{\FASTpmdCAPOREDynamicCIMIN}{\FASTpmdCAPOREDynamicCIMAX} \\
\bench{sunflow} \et{\FASTsunflowEvents}{\FASTsunflowThreads} 	& \vci{\FASTsunflowFTOHB}{\FASTsunflowFTOHBCI} 	& \ciRange{\FASTsunflowFTOHBDynamicCIMIN}{\FASTsunflowFTOHBDynamicCIMAX} 	& \vci{\FASTsunflowFTOWCP}{\FASTsunflowFTOWCPCI} 	& \ciRange{\FASTsunflowFTOWCPDynamicCIMIN}{\FASTsunflowFTOWCPDynamicCIMAX} 	& \vci{\FASTsunflowFTODC}{\FASTsunflowFTODCCI} 	& \ciRange{\FASTsunflowFTODCDynamicCIMIN}{\FASTsunflowFTODCDynamicCIMAX} 	& \vci{\FASTsunflowFTOCAPO}{\FASTsunflowFTOCAPOCI} 	& \ciRange{\FASTsunflowFTOCAPODynamicCIMIN}{\FASTsunflowFTOCAPODynamicCIMAX} 	& \vci{\FASTsunflowREWCP}{\FASTsunflowREWCPCI} 		& \ciRange{\FASTsunflowREWCPDynamicCIMIN}{\FASTsunflowREWCPDynamicCIMAX} 	& \vci{\FASTsunflowREDC}{\FASTsunflowREDCCI} 	& \ciRange{\FASTsunflowREDCDynamicCIMIN}{\FASTsunflowREDCDynamicCIMAX} 	& \vci{\FASTsunflowCAPORE}{\FASTsunflowCAPORECI} 	& \ciRange{\FASTsunflowCAPOREDynamicCIMIN}{\FASTsunflowCAPOREDynamicCIMAX} \\
\bench{tomcat} 	\et{\FASTtomcatEvents}{\FASTtomcatThreads} 		& \vci{\FASTtomcatFTOHB}{\FASTtomcatFTOHBCI} 	& \ciRange{\FASTtomcatFTOHBDynamicCIMIN}{\FASTtomcatFTOHBDynamicCIMAX} 		& \vci{\FASTtomcatFTOWCP}{\FASTtomcatFTOWCPCI} 		& \ciRange{\FASTtomcatFTOWCPDynamicCIMIN}{\FASTtomcatFTOWCPDynamicCIMAX} 	& \vci{\FASTtomcatFTODC}{\FASTtomcatFTODCCI} 	& \ciRange{\FASTtomcatFTODCDynamicCIMIN}{\FASTtomcatFTODCDynamicCIMAX} 		& \vci{\FASTtomcatFTOCAPO}{\FASTtomcatFTOCAPOCI} 	& \ciRange{\FASTtomcatFTOCAPODynamicCIMIN}{\FASTtomcatFTOCAPODynamicCIMAX} 		& \vci{\FASTtomcatREWCP}{\FASTtomcatREWCPCI} 		& \ciRange{\FASTtomcatREWCPDynamicCIMIN}{\FASTtomcatREWCPDynamicCIMAX} 		& \vci{\FASTtomcatREDC}{\FASTtomcatREDCCI} 		& \ciRange{\FASTtomcatREDCDynamicCIMIN}{\FASTtomcatREDCDynamicCIMAX} 	& \vci{\FASTtomcatCAPORE}{\FASTtomcatCAPORECI} 		& \ciRange{\FASTtomcatCAPOREDynamicCIMIN}{\FASTtomcatCAPOREDynamicCIMAX} \\
\bench{xalan} 	\et{\FASTxalanEvents}{\FASTxalanThreads} 		& \vci{\FASTxalanFTOHB}{\FASTxalanFTOHBCI} 		& \ciRange{\FASTxalanFTOHBDynamicCIMIN}{\FASTxalanFTOHBDynamicCIMAX} 		& \vci{\FASTxalanFTOWCP}{\FASTxalanFTOWCPCI} 		& \ciRange{\FASTxalanFTOWCPDynamicCIMIN}{\FASTxalanFTOWCPDynamicCIMAX} 		& \vci{\FASTxalanFTODC}{\FASTxalanFTODCCI} 		& \ciRange{\FASTxalanFTODCDynamicCIMIN}{\FASTxalanFTODCDynamicCIMAX} 		& \vci{\FASTxalanFTOCAPO}{\FASTxalanFTOCAPOCI} 		& \ciRange{\FASTxalanFTOCAPODynamicCIMIN}{\FASTxalanFTOCAPODynamicCIMAX} 		& \vci{\FASTxalanREWCP}{\FASTxalanREWCPCI} 			& \ciRange{\FASTxalanREWCPDynamicCIMIN}{\FASTxalanREWCPDynamicCIMAX} 		& \vci{\FASTxalanREDC}{\FASTxalanREDCCI} 		& \ciRange{\FASTxalanREDCDynamicCIMIN}{\FASTxalanREDCDynamicCIMAX} 		& \vci{\FASTxalanCAPORE}{\FASTxalanCAPORECI} 		& \ciRange{\FASTxalanCAPOREDynamicCIMIN}{\FASTxalanCAPOREDynamicCIMAX} \\\hline
% Total & \FTTotal & (\FTDynamicTotal) & \HBTotal & (\HBDynamicTotal) & \WCPTotal & (\WCPDynamicTotal) & \WDCTotal & (\WDCDynamicTotal) & \CAPOTotal & (\CAPODynamicTotal) & \PIPTotal & (\PIPDynamicTotal) \\
\end{tabular}
\end{minipage}
\caption{\FT-, \HB-, \WCP-, \DC-, \CAPO-, and \PIP-races detected by our implementation.
Each result is the average of 10 trials, rounded to the nearest integer.
Races are identified by single second site.}
 % Each result is from a single trial.}
\label{tab:coverage-dc}
\end{table*}




%%% Extra Stats
\begin{table*}[t]
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}} 
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\input{result-macros/PIP_fastTool_performanceProfile}
%  
\small
\centering
\begin{tabular}{@{}l|rl|rr|rr|rr@{}}
& \mc{8}{c@{}}{\FastTool: Access Event Counts}  \\
Program & Events & (NoFPEvents) & Read Total & Write Total & Access In CS & Access Out CS & Acq/Rel Total & Other Total \\\hline
\bench{avrora} 	& \et{\avroraEvents} & (\et{\avroraNoFPEvents}) 		& \per{\avroraReadTotal} 		& \per{\avroraWriteTotal} 	& \per{\avroraNoFPAccessInCS} 		& \per{\avroraNoFPAccessOutCS} 	& \per{\avroraAcqRelTotal} & \per{\avroraOtherTotal} \\
\bench{batik} 	& \et{\batikEvents} & (\et{\batikNoFPEvents}) 		& \per{\batikReadTotal} 		& \per{\batikWriteTotal} 		& \per{\batikNoFPAccessInCS} 		& \per{\batikNoFPAccessOutCS} 	& \per{\batikAcqRelTotal} & \per{\batikOtherTotal} \\
\bench{h2} 		& \et{\htwoEvents} & (\et{\htwoNoFPEvents}) 			& \per{\htwoReadTotal}		& \per{\htwoWriteTotal} 		& \per{\htwoNoFPAccessInCS} 		& \per{\htwoNoFPAccessOutCS} 	& \per{\htwoAcqRelTotal} & \per{\htwoOtherTotal} \\
\bench{jython} 	& \et{\jythonEvents} & (\et{\jythonNoFPEvents}) 		& \per{\jythonReadTotal} 		& \per{\jythonWriteTotal} 	& \per{\jythonNoFPAccessInCS} 		& \per{\jythonNoFPAccessOutCS} 	& \per{\jythonAcqRelTotal} & \per{\jythonOtherTotal} \\
\bench{luindex} & \et{\luindexEvents} & (\et{\luindexNoFPEvents}) 	& \per{\luindexReadTotal} 	& \per{\luindexWriteTotal}	& \per{\luindexNoFPAccessInCS} 		& \per{\luindexNoFPAccessOutCS} 	& \per{\luindexAcqRelTotal} & \per{\luindexOtherTotal} \\
\bench{lusearch}& \et{\lusearchEvents} & (\et{\lusearchNoFPEvents})	& \per{\lusearchReadTotal}	& \per{\lusearchWriteTotal}	& \per{\lusearchNoFPAccessInCS} 		& \per{\lusearchNoFPAccessOutCS} 	& \per{\lusearchAcqRelTotal} & \per{\lusearchOtherTotal} \\
\bench{pmd} 	& \et{\pmdEvents} & (\et{\pmdNoFPEvents}) 			& \per{\pmdReadTotal} 		& \per{\pmdWriteTotal} 		& \per{\pmdNoFPAccessInCS} 		& \per{\pmdNoFPAccessOutCS} 	& \per{\pmdAcqRelTotal} & \per{\pmdOtherTotal} \\
\bench{sunflow} & \et{\sunflowEvents} & (\et{\sunflowNoFPEvents}) 	& \per{\sunflowReadTotal} 	& \per{\sunflowWriteTotal}	& \per{\sunflowNoFPAccessInCS} 		& \per{\sunflowNoFPAccessOutCS} 	& \per{\sunflowAcqRelTotal} & \per{\sunflowOtherTotal} \\
\bench{tomcat} 	& \et{\tomcatEvents} & (\et{\tomcatNoFPEvents}) 		& \per{\tomcatReadTotal} 		& \per{\tomcatWriteTotal} 	& \per{\tomcatNoFPAccessInCS} 		& \per{\tomcatNoFPAccessOutCS} 	& \per{\tomcatAcqRelTotal} & \per{\tomcatOtherTotal} \\
\bench{xalan} 	& \et{\xalanEvents} & (\et{\xalanNoFPEvents}) 		& \per{\xalanReadTotal} 		& \per{\xalanWriteTotal}		& \per{\xalanNoFPAccessInCS} 		& \per{\xalanNoFPAccessOutCS} 	& \per{\xalanAcqRelTotal} & \per{\xalanOtherTotal} \\\hline
\end{tabular}
%
\label{tab:fast-tool-event-counts:access}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\input{result-macros/PIP_fastTool_performanceProfile}
%  
\small
\centering
\begin{tabular}{@{}l|r|rr|rrrrr@{}}
& \mc{8}{c@{}}{\FastTool: Read Event Counts}  \\
Program & Read Total & In CS & Out CS & Same Ep & Shared-Same Ep & Exclusive & Share & Shared \\\hline
\bench{avrora} 	& \et{\avroraNoFPReadTotal} & \per{\avroraReadInCS} 		& \per{\avroraReadOutCS} 		& \per{\avroraReadSameEp} 	& \per{\avroraReadSharedSameEp} & \per{\avroraReadExclusive} & \per{\avroraReadShare} & \per{\avroraReadShared} \\
\bench{batik} 	& \et{\batikNoFPReadTotal} & \per{\batikReadInCS} 		& \per{\batikReadOutCS} 		& \per{\batikReadSameEp} 		& \per{\batikReadSharedSameEp} & \per{\batikReadExclusive} & \per{\batikReadShare} & \per{\batikReadShared} \\
\bench{h2} 		& \et{\htwoNoFPReadTotal} & \per{\htwoReadInCS} 			& \per{\htwoReadOutCS}		& \per{\htwoReadSameEp} 		& \per{\htwoReadSharedSameEp} & \per{\htwoReadExclusive} & \per{\htwoReadShare} & \per{\htwoReadShared} \\
\bench{jython} 	& \et{\jythonNoFPReadTotal} & \per{\jythonReadInCS} 		& \per{\jythonReadOutCS} 		& \per{\jythonReadSameEp} 	& \per{\jythonReadSharedSameEp} & \per{\jythonReadExclusive} & \per{\jythonReadShare} & \per{\jythonReadShared} \\
\bench{luindex} & \et{\luindexNoFPReadTotal} & \per{\luindexReadInCS} 	& \per{\luindexReadOutCS} 	& \per{\luindexReadSameEp}	& \per{\luindexReadSharedSameEp} & \per{\luindexReadExclusive} & \per{\luindexReadShare} & \per{\luindexReadShared} \\
\bench{lusearch}& \et{\lusearchNoFPReadTotal} & \per{\lusearchReadInCS}	& \per{\lusearchReadOutCS}	& \per{\lusearchReadSameEp}	& \per{\lusearchReadSharedSameEp} & \per{\lusearchReadExclusive} & \per{\lusearchReadShare} & \per{\lusearchReadShared} \\
\bench{pmd} 	& \et{\pmdNoFPReadTotal} & \per{\pmdReadInCS} 			& \per{\pmdReadOutCS} 		& \per{\pmdReadSameEp} 		& \per{\pmdReadSharedSameEp} & \per{\pmdReadExclusive} & \per{\pmdReadShare} & \per{\pmdReadShared} \\
\bench{sunflow} & \et{\sunflowNoFPReadTotal} & \per{\sunflowReadInCS} 	& \per{\sunflowReadOutCS} 	& \per{\sunflowReadSameEp}	& \per{\sunflowReadSharedSameEp} & \per{\sunflowReadExclusive} & \per{\sunflowReadShare} & \per{\sunflowReadShared} \\
\bench{tomcat} 	& \et{\tomcatNoFPReadTotal} & \per{\tomcatReadInCS} 		& \per{\tomcatReadOutCS} 		& \per{\tomcatReadSameEp} 	& \per{\tomcatReadSharedSameEp} & \per{\tomcatReadExclusive} & \per{\tomcatReadShare} & \per{\tomcatReadShared} \\
\bench{xalan} 	& \et{\xalanNoFPReadTotal} & \per{\xalanReadInCS} 		& \per{\xalanReadOutCS} 		& \per{\xalanReadSameEp}		& \per{\xalanReadSharedSameEp} & \per{\xalanReadExclusive} & \per{\xalanReadShare} & \per{\xalanReadShared} \\\hline
\end{tabular}
%
\label{tab:fast-tool-event-counts:read}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\input{result-macros/PIP_fastTool_performanceProfile}
%  
\small
\centering
\begin{tabular}{@{}l|r|rr|r|rrr@{}}
& \mc{7}{c@{}}{\FastTool: Write Event Counts}  \\
Program & Honest Writes & In CS & Out CS & Write Total & Same Ep & Exclusive & Shared \\\hline
\bench{avrora} 	& \et{\avroraNoFPHonestWriteTotal} & \per{\avroraWriteInCS} 		& \per{\avroraWriteOutCS} 		& \et{\avroraNoFPWriteTotal} & \per{\avroraWriteSameEp} 	& \per{\avroraWriteExclusive} & \per{\avroraWriteShared} \\
\bench{batik} 	& \et{\batikNoFPHonestWriteTotal} & \per{\batikWriteInCS} 		& \per{\batikWriteOutCS} 		& \et{\batikNoFPWriteTotal} & \per{\batikWriteSameEp} 		& \per{\batikWriteExclusive} & \per{\batikWriteShared} \\
\bench{h2} 		& \et{\htwoNoFPHonestWriteTotal} & \per{\htwoWriteInCS} 			& \per{\htwoWriteOutCS}		& \et{\htwoNoFPWriteTotal} & \per{\htwoWriteSameEp} 		& \per{\htwoWriteExclusive} & \per{\htwoWriteShared} \\
\bench{jython} 	& \et{\jythonNoFPHonestWriteTotal} & \per{\jythonWriteInCS} 		& \per{\jythonWriteOutCS} 		& \et{\jythonNoFPWriteTotal} & \per{\jythonWriteSameEp} 	& \per{\jythonWriteExclusive} & \per{\jythonWriteShared} \\
\bench{luindex} & \et{\luindexNoFPHonestWriteTotal} & \per{\luindexWriteInCS} 	& \per{\luindexWriteOutCS} 	& \et{\luindexNoFPWriteTotal} & \per{\luindexWriteSameEp}	& \per{\luindexWriteExclusive} & \per{\luindexWriteShared} \\
\bench{lusearch}& \et{\lusearchNoFPHonestWriteTotal} & \per{\lusearchWriteInCS}	& \per{\lusearchWriteOutCS}	& \et{\lusearchNoFPWriteTotal} & \per{\lusearchWriteSameEp}	& \per{\lusearchWriteExclusive} & \per{\lusearchWriteShared} \\
\bench{pmd} 	& \et{\pmdNoFPHonestWriteTotal} & \per{\pmdWriteInCS} 			& \per{\pmdWriteOutCS} 		& \et{\pmdNoFPWriteTotal} & \per{\pmdWriteSameEp} 		& \per{\pmdWriteExclusive} & \per{\pmdWriteShared} \\
\bench{sunflow} & \et{\sunflowNoFPHonestWriteTotal} & \per{\sunflowWriteInCS} 	& \per{\sunflowWriteOutCS} 	& \et{\sunflowNoFPWriteTotal} & \per{\sunflowWriteSameEp}	& \per{\sunflowWriteExclusive} & \per{\sunflowWriteShared} \\
\bench{tomcat} 	& \et{\tomcatNoFPHonestWriteTotal} & \per{\tomcatWriteInCS} 		& \per{\tomcatWriteOutCS} 		& \et{\tomcatNoFPWriteTotal} & \per{\tomcatWriteSameEp} 	& \per{\tomcatWriteExclusive} & \per{\tomcatWriteShared} \\
\bench{xalan} 	& \et{\xalanNoFPHonestWriteTotal} & \per{\xalanWriteInCS} 		& \per{\xalanWriteOutCS} 		& \et{\xalanNoFPWriteTotal} & \per{\xalanWriteSameEp}		& \per{\xalanWriteExclusive} & \per{\xalanWriteShared} \\\hline
\end{tabular}
%
\label{tab:fast-tool-event-counts:write}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\newcommand{\per}[1]{#1\%}
\input{result-macros/PIP_fastTool_performanceProfile}
%  
\small
\centering
\begin{tabular}{@{}l|r|r|r|rrrrrrr@{}}
& \mc{10}{c@{}}{\FastTool: Other Event Counts}  \\
Program & Other Total & Acq/Rel & No Acq/Rel Total & Fork & Join & PreWait & PostWait & Volatile & ClassInit & ClassAccess \\\hline
\bench{avrora} 	& \avroraNoFPOtherTotal & \per{\avroraAcqRelOtherTotal} 		& \avroraNoAcqRelOtherTotal 		& \per{\avroraFork} 	& \per{\avroraJoin} & \per{\avroraPreWait} & \per{\avroraPostWait} & \per{\avroraVolatileTotal} & \per{\avroraClassInit} & \per{\avroraClassAccess} \\
\bench{batik} 	& \batikNoFPOtherTotal & \per{\batikAcqRelOtherTotal} 		& \batikNoAcqRelOtherTotal 		& \per{\batikFork} 		& \per{\batikJoin} & \per{\batikPreWait} & \per{\batikPostWait} & \per{\batikVolatileTotal} & \per{\batikClassInit} & \per{\batikClassAccess}\\
\bench{h2} 		& \htwoNoFPOtherTotal & \per{\htwoAcqRelOtherTotal} 			& \htwoNoAcqRelOtherTotal		& \per{\htwoFork} 		& \per{\htwoJoin} & \per{\htwoPreWait} & \per{\htwoPostWait} & \per{\htwoVolatileTotal} & \per{\htwoClassInit} & \per{\htwoClassAccess} \\
\bench{jython} 	& \jythonNoFPOtherTotal & \per{\jythonAcqRelOtherTotal} 		& \jythonNoAcqRelOtherTotal 		& \per{\jythonFork} 	& \per{\jythonJoin} & \per{\jythonPreWait} & \per{\jythonPostWait} & \per{\jythonVolatileTotal} & \per{\jythonClassInit} & \per{\jythonClassAccess} \\
\bench{luindex} & \luindexNoFPOtherTotal & \per{\luindexAcqRelOtherTotal} 	& \luindexNoAcqRelOtherTotal 	& \per{\luindexFork}	& \per{\luindexJoin} & \per{\luindexPreWait} & \per{\luindexPostWait} & \per{\luindexVolatileTotal} & \per{\luindexClassInit} & \per{\luindexClassAccess} \\
\bench{lusearch}& \lusearchNoFPOtherTotal & \per{\lusearchAcqRelOtherTotal}	& \lusearchNoAcqRelOtherTotal	& \per{\lusearchFork}	& \per{\lusearchJoin} & \per{\lusearchPreWait} & \per{\lusearchPostWait} & \per{\lusearchVolatileTotal} & \per{\lusearchClassInit} & \per{\lusearchClassAccess} \\
\bench{pmd} 	& \pmdNoFPOtherTotal & \per{\pmdAcqRelOtherTotal} 			& \pmdNoAcqRelOtherTotal 		& \per{\pmdFork} 		& \per{\pmdJoin} & \per{\pmdPreWait} & \per{\pmdPostWait} & \per{\pmdVolatileTotal} & \per{\pmdClassInit} & \per{\pmdClassAccess} \\
\bench{sunflow} & \sunflowNoFPOtherTotal & \per{\sunflowAcqRelOtherTotal} 	& \sunflowNoAcqRelOtherTotal 	& \per{\sunflowFork}	& \per{\sunflowJoin} & \per{\sunflowPreWait} & \per{\sunflowPostWait} & \per{\sunflowVolatileTotal} & \per{\sunflowClassInit} & \per{\sunflowClassAccess} \\
\bench{tomcat} 	& \tomcatNoFPOtherTotal & \per{\tomcatAcqRelOtherTotal} 		& \tomcatNoAcqRelOtherTotal 		& \per{\tomcatFork} 	& \per{\tomcatJoin} & \per{\tomcatPreWait} & \per{\tomcatPostWait} & \per{\tomcatVolatileTotal} & \per{\tomcatClassInit} & \per{\tomcatClassAccess} \\
\bench{xalan} 	& \xalanNoFPOtherTotal & \per{\xalanAcqRelOtherTotal} 		& \xalanNoAcqRelOtherTotal 		& \per{\xalanFork}		& \per{\xalanJoin} & \per{\xalanPreWait} & \per{\xalanPostWait} & \per{\xalanVolatileTotal} & \per{\xalanClassInit} & \per{\xalanClassAccess} \\\hline
\end{tabular}
%
\label{tab:fast-tool-event-counts:other}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[2]{}
\newcommand{\per}[1]{#1\%}
\input{result-macros/PIP_fastTool_performanceProfile}
%  
\small
\centering
\begin{tabular}{@{}l|r|rrrr@{}}
& \mc{5}{c@{}}{\FastTool: Race Type Counts}  \\
Program & Race Total & Wr-Rd Race & Wr-Wr Race & Rd-Wr Race & Rd(Shd)-Wr Race \\\hline
\bench{avrora} 	& \avroraRaceTotal & \per{\avroraWrRdRace} 		& \per{\avroraWrWrRace} 		& \per{\avroraRdWrRace} 	& \per{\avroraRdShWrRace} \\
\bench{batik} 	& \batikRaceTotal & \per{\batikWrRdRace} 		& \per{\batikWrWrRace} 		& \per{\batikRdWrRace} 		& \per{\batikRdShWrRace} \\
\bench{h2} 		& \htwoRaceTotal & \per{\htwoWrRdRace} 			& \per{\htwoWrWrRace}		& \per{\htwoRdWrRace} 		& \per{\htwoRdShWrRace} \\
\bench{jython} 	& \jythonRaceTotal & \per{\jythonWrRdRace} 		& \per{\jythonWrWrRace} 		& \per{\jythonRdWrRace} 	& \per{\jythonRdShWrRace} \\
\bench{luindex} & \luindexRaceTotal & \per{\luindexWrRdRace} 	& \per{\luindexWrWrRace} 	& \per{\luindexRdWrRace}	& \per{\luindexRdShWrRace} \\
\bench{lusearch}& \lusearchRaceTotal & \per{\lusearchWrRdRace}	& \per{\lusearchWrWrRace}	& \per{\lusearchRdWrRace}	& \per{\lusearchRdShWrRace} \\
\bench{pmd} 	& \pmdRaceTotal & \per{\pmdWrRdRace} 			& \per{\pmdWrWrRace} 		& \per{\pmdRdWrRace} 		& \per{\pmdRdShWrRace} \\
\bench{sunflow} & \sunflowRaceTotal & \per{\sunflowWrRdRace} 	& \per{\sunflowWrWrRace} 	& \per{\sunflowRdWrRace}	& \per{\sunflowRdShWrRace} \\
\bench{tomcat} 	& \tomcatRaceTotal & \per{\tomcatWrRdRace} 		& \per{\tomcatWrWrRace} 		& \per{\tomcatRdWrRace} 	& \per{\tomcatRdShWrRace} \\
\bench{xalan} 	& \xalanRaceTotal & \per{\xalanWrRdRace} 		& \per{\xalanWrWrRace} 		& \per{\xalanRdWrRace}		& \per{\xalanRdShWrRace} \\\hline
\end{tabular}
\end{minipage}
%
\label{tab:fast-tool-event-counts:raceType}
\end{table*}
 
%%% CAPO Event Characteristics extra counts
\begin{table*}[t]
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\newcommand{\tot}[1]{#1{\;}M}
\input{result-macros/PIP_fastTool_performanceProfile}
%  
\small
\centering
\begin{tabular}{@{}l|rl|rr|rr|rr@{}}
& \mc{8}{c@{}}{\FastTool: CAPO-Opt Rule A or CAPO-Opt (A)}  \\
Program & Events & (NoFPEvents) & Rd (A) Succ & Rd (A) Total & WrWr(A) Succ & WrWr(A) Total & WrRd(A) Succ & WrRd(A) Total \\\hline
\bench{avrora} 	& \et{\avroraEvents} & (\et{\avroraNoFPEvents}) 	& \per{\avroraReadRuleASuc} 	& \tot{\avroraReadRuleATot} 	& \per{\avroraWriteWriteRuleASuc} 	& \tot{\avroraWriteWriteRuleATot} 	& \per{\avroraWriteReadRuleASuc} 	& \tot{\avroraWriteReadRuleATot} \\
\bench{batik} 	& \et{\batikEvents} & (\et{\batikNoFPEvents}) 		& \per{\batikReadRuleASuc} 		& \tot{\batikReadRuleATot} 		& \per{\batikWriteWriteRuleASuc} 	& \tot{\batikWriteWriteRuleATot} 	& \per{\batikWriteReadRuleASuc} 	& \tot{\batikWriteReadRuleATot} \\
\bench{h2} 		& \et{\htwoEvents} & (\et{\htwoNoFPEvents}) 		& \per{\htwoReadRuleASuc}		& \tot{\htwoReadRuleATot} 		& \per{\htwoWriteWriteRuleASuc} 	& \tot{\htwoWriteWriteRuleATot} 	& \per{\htwoWriteReadRuleASuc} 		& \tot{\htwoWriteReadRuleATot} \\
\bench{jython} 	& \et{\jythonEvents} & (\et{\jythonNoFPEvents}) 	& \per{\jythonReadRuleASuc} 	& \tot{\jythonReadRuleATot} 	& \per{\jythonWriteWriteRuleASuc} 	& \tot{\jythonWriteWriteRuleATot} 	& \per{\jythonWriteReadRuleASuc}	& \tot{\jythonWriteReadRuleATot} \\
\bench{luindex} & \et{\luindexEvents} & (\et{\luindexNoFPEvents}) 	& \per{\luindexReadRuleASuc} 	& \tot{\luindexReadRuleATot}	& \per{\luindexWriteWriteRuleASuc} 	& \tot{\luindexWriteWriteRuleATot} 	& \per{\luindexWriteReadRuleASuc} 	& \tot{\luindexWriteReadRuleATot} \\
\bench{lusearch}& \et{\lusearchEvents} & (\et{\lusearchNoFPEvents})	& \per{\lusearchReadRuleASuc}	& \tot{\lusearchReadRuleATot}	& \per{\lusearchWriteWriteRuleASuc} & \tot{\lusearchWriteWriteRuleATot} & \per{\lusearchWriteReadRuleASuc} 	& \tot{\lusearchWriteReadRuleATot} \\
\bench{pmd} 	& \et{\pmdEvents} & (\et{\pmdNoFPEvents}) 			& \per{\pmdReadRuleASuc} 		& \tot{\pmdReadRuleATot} 		& \per{\pmdWriteWriteRuleASuc} 		& \tot{\pmdWriteWriteRuleATot} 		& \per{\pmdWriteReadRuleASuc} 		& \tot{\pmdWriteReadRuleATot} \\
\bench{sunflow} & \et{\sunflowEvents} & (\et{\sunflowNoFPEvents}) 	& \per{\sunflowReadRuleASuc} 	& \tot{\sunflowReadRuleATot}	& \per{\sunflowWriteWriteRuleASuc} 	& \tot{\sunflowWriteWriteRuleATot} 	& \per{\sunflowWriteReadRuleASuc} 	& \tot{\sunflowWriteReadRuleATot} \\
\bench{tomcat} 	& \et{\tomcatEvents} & (\et{\tomcatNoFPEvents}) 	& \per{\tomcatReadRuleASuc} 	& \tot{\tomcatReadRuleATot} 	& \per{\tomcatWriteWriteRuleASuc} 	& \tot{\tomcatWriteWriteRuleATot} 	& \per{\tomcatWriteReadRuleASuc} 	& \tot{\tomcatWriteReadRuleATot} \\
\bench{xalan} 	& \et{\xalanEvents} & (\et{\xalanNoFPEvents}) 		& \per{\xalanReadRuleASuc} 		& \tot{\xalanReadRuleATot}		& \per{\xalanWriteWriteRuleASuc} 	& \tot{\xalanWriteWriteRuleATot} 	& \per{\xalanWriteReadRuleASuc} 	& \tot{\xalanWriteReadRuleATot} \\\hline
\end{tabular}
%
\label{tab:extra-data-counts:ruleA}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\newcommand{\tot}[1]{#1{\;}M}
\input{result-macros/PIP_fastTool_performanceProfile}
%  
\small
\centering
\begin{tabular}{@{}l|rl|r|rrr|rrr@{}}
& \mc{9}{c@{}}{\FastTool: CAPO Rd/Wr Sets}  \\
Program & Events & (NoFPEvents) & Total Clears & Rd Set 0 & Rd Set 1 & Rd Set Gt1 & Wr Set 0 & Wr Set 1 & Wr Set Gt1 \\\hline
\bench{avrora} 	& \et{\avroraEvents} & (\et{\avroraNoFPEvents}) 	& \tot{\avroraTotalSetClears} 	& \per{\avroraReadSetZero} 	& \per{\avroraReadSetOne} 	& \per{\avroraReadSetGtOne} 	& \per{\avroraWriteSetZero} 	& \per{\avroraWriteSetOne} 	& \per{\avroraWriteSetGtOne} \\
\bench{batik} 	& \et{\batikEvents} & (\et{\batikNoFPEvents}) 		& \tot{\batikTotalSetClears} 	& \per{\batikReadSetZero} 	& \per{\batikReadSetOne} 	& \per{\batikReadSetGtOne} 		& \per{\batikWriteSetZero} 		& \per{\batikWriteSetOne} 	& \per{\batikWriteSetGtOne} \\
\bench{h2} 		& \et{\htwoEvents} & (\et{\htwoNoFPEvents}) 		& \tot{\htwoTotalSetClears}		& \per{\htwoReadSetZero} 	& \per{\htwoReadSetOne} 	& \per{\htwoReadSetGtOne} 		& \per{\htwoWriteSetZero} 		& \per{\htwoWriteSetOne} 	& \per{\htwoWriteSetGtOne} \\
\bench{jython} 	& \et{\jythonEvents} & (\et{\jythonNoFPEvents}) 	& \tot{\jythonTotalSetClears} 	& \per{\jythonReadSetZero} 	& \per{\jythonReadSetOne} 	& \per{\jythonReadSetGtOne} 	& \per{\jythonWriteSetZero} 	& \per{\jythonWriteSetOne} 	& \per{\jythonWriteSetGtOne} \\
\bench{luindex} & \et{\luindexEvents} & (\et{\luindexNoFPEvents}) 	& \tot{\luindexTotalSetClears} 	& \per{\luindexReadSetZero}	& \per{\luindexReadSetOne} 	& \per{\luindexReadSetGtOne} 	& \per{\luindexWriteSetZero} 	& \per{\luindexWriteSetOne} & \per{\luindexWriteSetGtOne} \\
\bench{lusearch}& \et{\lusearchEvents} & (\et{\lusearchNoFPEvents})	& \tot{\lusearchTotalSetClears}	& \per{\lusearchReadSetZero}& \per{\lusearchReadSetOne} & \per{\lusearchReadSetGtOne} 	& \per{\lusearchWriteSetZero} 	& \per{\lusearchWriteSetOne}& \per{\lusearchWriteSetGtOne} \\
\bench{pmd} 	& \et{\pmdEvents} & (\et{\pmdNoFPEvents}) 			& \tot{\pmdTotalSetClears} 		& \per{\pmdReadSetZero} 	& \per{\pmdReadSetOne} 		& \per{\pmdReadSetGtOne} 		& \per{\pmdWriteSetZero} 		& \per{\pmdWriteSetOne} 	& \per{\pmdWriteSetGtOne} \\
\bench{sunflow} & \et{\sunflowEvents} & (\et{\sunflowNoFPEvents}) 	& \tot{\sunflowTotalSetClears} 	& \per{\sunflowReadSetZero}	& \per{\sunflowReadSetOne} 	& \per{\sunflowReadSetGtOne} 	& \per{\sunflowWriteSetZero} 	& \per{\sunflowWriteSetOne} & \per{\sunflowWriteSetGtOne} \\
\bench{tomcat} 	& \et{\tomcatEvents} & (\et{\tomcatNoFPEvents}) 	& \tot{\tomcatTotalSetClears} 	& \per{\tomcatReadSetZero} 	& \per{\tomcatReadSetOne} 	& \per{\tomcatReadSetGtOne} 	& \per{\tomcatWriteSetZero} 	& \per{\tomcatWriteSetOne} 	& \per{\tomcatWriteSetGtOne} \\
\bench{xalan} 	& \et{\xalanEvents} & (\et{\xalanNoFPEvents}) 		& \tot{\xalanTotalSetClears} 	& \per{\xalanReadSetZero}	& \per{\xalanReadSetOne} 	& \per{\xalanReadSetGtOne} 		& \per{\xalanWriteSetZero} 		& \per{\xalanWriteSetOne} 	& \per{\xalanWriteSetGtOne} \\\hline
\end{tabular}
%
\label{tab:extra-data-counts:CAPOSets}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\begin{adjustwidth}{-1cm}{}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\newcommand{\tot}[1]{#1{\;}M}
\input{result-macros/PIP_fastTool_performanceProfile}
%  
\small
\centering
\begin{tabular}{@{}l|rl|r|rrrrrr@{}}
& \mc{9}{c@{}}{\FastTool: CAPO Rd Maps}  \\
Program & Events & (NoFPEvents) & Total Clears & Rd Map 0 & Rd Map 1 & Rd Map 10 & Rd Map 100 & Rd Map 1000 & Rd Map Gt1000 \\\hline
\bench{avrora} 	& \et{\avroraEvents} & (\et{\avroraNoFPEvents}) 	& \tot{\avroraTotalMapClears} 	& \per{\avroraReadMapZero} 	& \per{\avroraReadMapOne} 	& \per{\avroraReadMapTen} 	& \per{\avroraReadMapHund} 	& \per{\avroraReadMapThou} 	& \per{\avroraReadMapGtThou} \\
\bench{batik} 	& \et{\batikEvents} & (\et{\batikNoFPEvents}) 		& \tot{\batikTotalMapClears} 	& \per{\batikReadMapZero} 	& \per{\batikReadMapOne} 	& \per{\batikReadMapTen} 	& \per{\batikReadMapHund} 	& \per{\batikReadMapThou} 	& \per{\batikReadMapGtThou} \\
\bench{h2} 		& \et{\htwoEvents} & (\et{\htwoNoFPEvents}) 		& \tot{\htwoTotalMapClears}		& \per{\htwoReadMapZero} 	& \per{\htwoReadMapOne} 	& \per{\htwoReadMapTen} 	& \per{\htwoReadMapHund} 	& \per{\htwoReadMapThou} 	& \per{\htwoReadMapGtThou} \\
\bench{jython} 	& \et{\jythonEvents} & (\et{\jythonNoFPEvents}) 	& \tot{\jythonTotalMapClears} 	& \per{\jythonReadMapZero} 	& \per{\jythonReadMapOne} 	& \per{\jythonReadMapTen} 	& \per{\jythonReadMapHund} 	& \per{\jythonReadMapThou} 	& \per{\jythonReadMapGtThou} \\
\bench{luindex} & \et{\luindexEvents} & (\et{\luindexNoFPEvents}) 	& \tot{\luindexTotalMapClears} 	& \per{\luindexReadMapZero}	& \per{\luindexReadMapOne} 	& \per{\luindexReadMapTen} 	& \per{\luindexReadMapHund} & \per{\luindexReadMapThou} & \per{\luindexReadMapGtThou} \\
\bench{lusearch}& \et{\lusearchEvents} & (\et{\lusearchNoFPEvents})	& \tot{\lusearchTotalMapClears}	& \per{\lusearchReadMapZero}& \per{\lusearchReadMapOne} & \per{\lusearchReadMapTen} & \per{\lusearchReadMapHund}& \per{\lusearchReadMapThou}& \per{\lusearchReadMapGtThou} \\
\bench{pmd} 	& \et{\pmdEvents} & (\et{\pmdNoFPEvents}) 			& \tot{\pmdTotalMapClears} 		& \per{\pmdReadMapZero} 	& \per{\pmdReadMapOne} 		& \per{\pmdReadMapTen} 		& \per{\pmdReadMapHund} 	& \per{\pmdReadMapThou} 	& \per{\pmdReadMapGtThou} \\
\bench{sunflow} & \et{\sunflowEvents} & (\et{\sunflowNoFPEvents}) 	& \tot{\sunflowTotalMapClears} 	& \per{\sunflowReadMapZero}	& \per{\sunflowReadMapOne} 	& \per{\sunflowReadMapTen} 	& \per{\sunflowReadMapHund} & \per{\sunflowReadMapThou} & \per{\sunflowReadMapGtThou} \\
\bench{tomcat} 	& \et{\tomcatEvents} & (\et{\tomcatNoFPEvents}) 	& \tot{\tomcatTotalMapClears} 	& \per{\tomcatReadMapZero} 	& \per{\tomcatReadMapOne} 	& \per{\tomcatReadMapTen} 	& \per{\tomcatReadMapHund} 	& \per{\tomcatReadMapThou} 	& \per{\tomcatReadMapGtThou} \\
\bench{xalan} 	& \et{\xalanEvents} & (\et{\xalanNoFPEvents}) 		& \tot{\xalanTotalMapClears} 	& \per{\xalanReadMapZero}	& \per{\xalanReadMapOne} 	& \per{\xalanReadMapTen} 	& \per{\xalanReadMapHund} 	& \per{\xalanReadMapThou} 	& \per{\xalanReadMapGtThou} \\\hline
\end{tabular}
%
\label{tab:extra-data-counts:CAPORdMaps}
\end{adjustwidth}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\begin{adjustwidth}{-1cm}{}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\newcommand{\tot}[1]{#1{\;}M}
\input{result-macros/PIP_fastTool_performanceProfile}
%  
\small
\centering
\begin{tabular}{@{}l|rl|r|rrrrrr@{}}
& \mc{9}{c@{}}{\FastTool: CAPO Wr Maps}  \\
Program & Events & (NoFPEvents) & Total Clears & Wr Map 0 & Wr Map 1 & Wr Map 10 & Wr Map 100 & Wr Map 1000 & Wr Map Gt1000 \\\hline
\bench{avrora} 	& \et{\avroraEvents} & (\et{\avroraNoFPEvents}) 	& \tot{\avroraTotalMapClears} 	& \per{\avroraWriteMapZero} 	& \per{\avroraWriteMapOne} 	& \per{\avroraWriteMapTen} 	& \per{\avroraWriteMapHund} 	& \per{\avroraWriteMapThou} 	& \per{\avroraWriteMapGtThou} \\
\bench{batik} 	& \et{\batikEvents} & (\et{\batikNoFPEvents}) 		& \tot{\batikTotalMapClears} 	& \per{\batikWriteMapZero} 	& \per{\batikWriteMapOne} 	& \per{\batikWriteMapTen} 	& \per{\batikWriteMapHund} 	& \per{\batikWriteMapThou} 	& \per{\batikWriteMapGtThou} \\
\bench{h2} 		& \et{\htwoEvents} & (\et{\htwoNoFPEvents}) 		& \tot{\htwoTotalMapClears}		& \per{\htwoWriteMapZero} 	& \per{\htwoWriteMapOne} 	& \per{\htwoWriteMapTen} 	& \per{\htwoWriteMapHund} 	& \per{\htwoWriteMapThou} 	& \per{\htwoWriteMapGtThou} \\
\bench{jython} 	& \et{\jythonEvents} & (\et{\jythonNoFPEvents}) 	& \tot{\jythonTotalMapClears} 	& \per{\jythonWriteMapZero} 	& \per{\jythonWriteMapOne} 	& \per{\jythonWriteMapTen} 	& \per{\jythonWriteMapHund} 	& \per{\jythonWriteMapThou} 	& \per{\jythonWriteMapGtThou} \\
\bench{luindex} & \et{\luindexEvents} & (\et{\luindexNoFPEvents}) 	& \tot{\luindexTotalMapClears} 	& \per{\luindexWriteMapZero}	& \per{\luindexWriteMapOne} 	& \per{\luindexWriteMapTen} 	& \per{\luindexWriteMapHund} & \per{\luindexWriteMapThou} & \per{\luindexWriteMapGtThou} \\
\bench{lusearch}& \et{\lusearchEvents} & (\et{\lusearchNoFPEvents})	& \tot{\lusearchTotalMapClears}	& \per{\lusearchWriteMapZero}& \per{\lusearchWriteMapOne} & \per{\lusearchWriteMapTen} & \per{\lusearchWriteMapHund}& \per{\lusearchWriteMapThou}& \per{\lusearchWriteMapGtThou} \\
\bench{pmd} 	& \et{\pmdEvents} & (\et{\pmdNoFPEvents}) 			& \tot{\pmdTotalMapClears} 		& \per{\pmdWriteMapZero} 	& \per{\pmdWriteMapOne} 		& \per{\pmdWriteMapTen} 		& \per{\pmdWriteMapHund} 	& \per{\pmdWriteMapThou} 	& \per{\pmdWriteMapGtThou} \\
\bench{sunflow} & \et{\sunflowEvents} & (\et{\sunflowNoFPEvents}) 	& \tot{\sunflowTotalMapClears} 	& \per{\sunflowWriteMapZero}	& \per{\sunflowWriteMapOne} 	& \per{\sunflowWriteMapTen} 	& \per{\sunflowWriteMapHund} & \per{\sunflowWriteMapThou} & \per{\sunflowWriteMapGtThou} \\
\bench{tomcat} 	& \et{\tomcatEvents} & (\et{\tomcatNoFPEvents}) 	& \tot{\tomcatTotalMapClears} 	& \per{\tomcatWriteMapZero} 	& \per{\tomcatWriteMapOne} 	& \per{\tomcatWriteMapTen} 	& \per{\tomcatWriteMapHund} 	& \per{\tomcatWriteMapThou} 	& \per{\tomcatWriteMapGtThou} \\
\bench{xalan} 	& \et{\xalanEvents} & (\et{\xalanNoFPEvents}) 		& \tot{\xalanTotalMapClears} 	& \per{\xalanWriteMapZero}	& \per{\xalanWriteMapOne} 	& \per{\xalanWriteMapTen} 	& \per{\xalanWriteMapHund} 	& \per{\xalanWriteMapThou} 	& \per{\xalanWriteMapGtThou} \\\hline
\end{tabular}
%
\end{adjustwidth}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\newcommand{\tot}[1]{#1{\;}M}
\input{result-macros/PIP_fastTool_performanceProfile}
%  
\small
\centering
\begin{tabular}{@{}l|rl|r|rrr@{}}
& \mc{6}{c@{}}{\FastTool: Locks Held During Access Event}  \\
Program & Events & (NoFPEvents) & Held Lock Total & One Lock Held & Two Nested Locks & Many Nested Locks \\\hline
\bench{avrora} 	& \et{\avroraEvents} & (\et{\avroraNoFPEvents}) 	& \tot{\avroraHoldLocksTotal} 	& \per{\avroraOneLockHeld} 	& \per{\avroraTwoNestedLocks} 	& \per{\avroraManyNestedLocks} \\
\bench{batik} 	& \et{\batikEvents} & (\et{\batikNoFPEvents}) 		& \tot{\batikHoldLocksTotal} 	& \per{\batikOneLockHeld} 	& \per{\batikTwoNestedLocks} 	& \per{\batikManyNestedLocks} \\
\bench{h2} 		& \et{\htwoEvents} & (\et{\htwoNoFPEvents}) 		& \tot{\htwoHoldLocksTotal}		& \per{\htwoOneLockHeld} 	& \per{\htwoTwoNestedLocks} 	& \per{\htwoManyNestedLocks} \\
\bench{jython} 	& \et{\jythonEvents} & (\et{\jythonNoFPEvents}) 	& \tot{\jythonHoldLocksTotal} 	& \per{\jythonOneLockHeld} 	& \per{\jythonTwoNestedLocks} 	& \per{\jythonManyNestedLocks} \\
\bench{luindex} & \et{\luindexEvents} & (\et{\luindexNoFPEvents}) 	& \tot{\luindexHoldLocksTotal} 	& \per{\luindexOneLockHeld}	& \per{\luindexTwoNestedLocks} 	& \per{\luindexManyNestedLocks} \\
\bench{lusearch}& \et{\lusearchEvents} & (\et{\lusearchNoFPEvents})	& \tot{\lusearchHoldLocksTotal}	& \per{\lusearchOneLockHeld}& \per{\lusearchTwoNestedLocks} & \per{\lusearchManyNestedLocks} \\
\bench{pmd} 	& \et{\pmdEvents} & (\et{\pmdNoFPEvents}) 			& \tot{\pmdHoldLocksTotal} 		& \per{\pmdOneLockHeld} 	& \per{\pmdTwoNestedLocks} 		& \per{\pmdManyNestedLocks} \\
\bench{sunflow} & \et{\sunflowEvents} & (\et{\sunflowNoFPEvents}) 	& \tot{\sunflowHoldLocksTotal} 	& \per{\sunflowOneLockHeld}	& \per{\sunflowTwoNestedLocks} 	& \per{\sunflowManyNestedLocks} \\
\bench{tomcat} 	& \et{\tomcatEvents} & (\et{\tomcatNoFPEvents}) 	& \tot{\tomcatHoldLocksTotal} 	& \per{\tomcatOneLockHeld} 	& \per{\tomcatTwoNestedLocks} 	& \per{\tomcatManyNestedLocks} \\
\bench{xalan} 	& \et{\xalanEvents} & (\et{\xalanNoFPEvents}) 		& \tot{\xalanHoldLocksTotal} 	& \per{\xalanOneLockHeld}	& \per{\xalanTwoNestedLocks} 	& \per{\xalanManyNestedLocks} \\\hline
\end{tabular}
\end{minipage}
%
\label{tab:extra-data-counts-2:locksHeld}
\end{table*}

%%% Rule{a} Event Characteristics extra counts
\begin{table*}[t]
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\newcommand{\tot}[1]{#1{\;}M}
% \input{result-macros/PIP_fastTool_CAPORE}
\input{result-macros/PIP_fastTool_CAPOOpt_RuleAFix}
%
\small
\centering
\begin{tabular}{@{}l|rl|r|rrrr@{}}
& \mc{7}{c@{}}{\FastTool: Rule(a) Useful Updates: CAPO-Opt configuration}  \\
Program & Events & (NoFPEvents) & Rule(a) Total & One Thr Changed & Two Thr Changed & Many Thr Changed & All Thr Changed \\\hline
\bench{avrora} 	& \et{\avroraEvents} & (\et{\avroraNoFPEvents}) 	& \tot{\avroraTotalRuleASuc} 	& \per{\avroraOneThrChanged} 	& \per{\avroraTwoThrChanged} 	& \per{\avroraManyThrChanged} 	& \per{\avroraAllThrChanged} \\
\bench{batik} 	& \et{\batikEvents} & (\et{\batikNoFPEvents}) 		& \tot{\batikTotalRuleASuc} 	& \per{\batikOneThrChanged} 	& \per{\batikTwoThrChanged} 	& \per{\batikManyThrChanged} 	& \per{\batikAllThrChanged} \\
\bench{h2} 		& \et{\htwoEvents} & (\et{\htwoNoFPEvents}) 		& \tot{\htwoTotalRuleASuc}		& \per{\htwoOneThrChanged} 		& \per{\htwoTwoThrChanged} 		& \per{\htwoManyThrChanged} 	& \per{\htwoAllThrChanged} \\
\bench{jython} 	& \et{\jythonEvents} & (\et{\jythonNoFPEvents}) 	& \tot{\jythonTotalRuleASuc} 	& \per{\jythonOneThrChanged} 	& \per{\jythonTwoThrChanged} 	& \per{\jythonManyThrChanged} 	& \per{\jythonAllThrChanged} \\
\bench{luindex} & \et{\luindexEvents} & (\et{\luindexNoFPEvents}) 	& \tot{\luindexTotalRuleASuc} 	& \per{\luindexOneThrChanged}	& \per{\luindexTwoThrChanged} 	& \per{\luindexManyThrChanged} 	& \per{\luindexAllThrChanged} \\
\bench{lusearch}& \et{\lusearchEvents} & (\et{\lusearchNoFPEvents})	& \tot{\lusearchTotalRuleASuc}	& \per{\lusearchOneThrChanged}	& \per{\lusearchTwoThrChanged} 	& \per{\lusearchManyThrChanged} & \per{\lusearchAllThrChanged} \\
\bench{pmd} 	& \et{\pmdEvents} & (\et{\pmdNoFPEvents}) 			& \tot{\pmdTotalRuleASuc} 		& \per{\pmdOneThrChanged} 		& \per{\pmdTwoThrChanged} 		& \per{\pmdManyThrChanged} 		& \per{\pmdAllThrChanged} \\
\bench{sunflow} & \et{\sunflowEvents} & (\et{\sunflowNoFPEvents}) 	& \tot{\sunflowTotalRuleASuc} 	& \per{\sunflowOneThrChanged}	& \per{\sunflowTwoThrChanged} 	& \per{\sunflowManyThrChanged} 	& \per{\sunflowAllThrChanged} \\
\bench{tomcat} 	& \et{\tomcatEvents} & (\et{\tomcatNoFPEvents}) 	& \tot{\tomcatTotalRuleASuc} 	& \per{\tomcatOneThrChanged} 	& \per{\tomcatTwoThrChanged} 	& \per{\tomcatManyThrChanged} 	& \per{\tomcatAllThrChanged} \\
\bench{xalan} 	& \et{\xalanEvents} & (\et{\xalanNoFPEvents}) 		& \tot{\xalanTotalRuleASuc} 	& \per{\xalanOneThrChanged}		& \per{\xalanTwoThrChanged} 	& \per{\xalanManyThrChanged} 	& \per{\xalanAllThrChanged} \\\hline
\end{tabular}
%
\label{tab:extra-data-counts:ruleA}
\end{minipage}
\\
\hfill
\begin{minipage}{1\textwidth}
\newcommand{\rcounts}[2]{\textbf{#2} (#1)}
\newcommand{\rzero}{\textbf{0}}
\newcommand{\rna}{\textbf{N/A}}
\newcommand{\et}[1]{#1{\;}M}
\newcommand{\per}[1]{#1\%}
\newcommand{\tot}[1]{#1{\;}M}
% \input{result-macros/PIP_fastTool_CAPORE}
\input{result-macros/PIP_fastTool_CAPOOpt_RuleAFix}
%  
\small
\centering
\begin{tabular}{@{}l|rl|rrrr||rr||rrr||rrr@{}}
& \mc{14}{c@{}}{\FastTool: Rule(a) Lock Useful Updates: CAPO-RE-Alt configuration}  \\
& \mc{2}{c|}{} & \mc{4}{c||}{Locks Held} & \mc{2}{c||}{One Lock Held} & \mc{3}{c||}{Two Locks Held} & \mc{3}{c}{Many Locks Held} \\
Program & Events & (NoFPEvents) & Total & One & Two & Many & Total & Succ & Total & In & Out & Total & In Most & Out Most \\\hline
\bench{avrora} 	& \et{\avroraEvents} & (\et{\avroraNoFPEvents}) 	& \tot{\avroraTotalLockHeld} 	& \per{\avroraSingleLockHeld} 	& \per{\avroraTwoLocksHeld} 	& \per{\avroraManyLocksHeld} & \tot{\avroraTotalSingleLockHeld} & \per{\avroraSucSingleLockHeld} & \tot{\avroraTotalTwoLocksHeld} & \per{\avroraSucInnerLockHeld} & \per{\avroraSucOuterLockHeld} & \tot{\avroraTotalManyLocksHeld} & \per{\avroraSucInnerMostLockHeld} & \per{\avroraSucOuterMostLockHeld} \\
\bench{batik} 	& \et{\batikEvents} & (\et{\batikNoFPEvents}) 		& \tot{\batikTotalLockHeld} 	& \per{\batikSingleLockHeld} 	& \per{\batikTwoLocksHeld} 		& \per{\batikManyLocksHeld} & \tot{\batikTotalSingleLockHeld} & \per{\batikSucSingleLockHeld} & \tot{\batikTotalTwoLocksHeld} & \per{\batikSucInnerLockHeld} & \per{\batikSucOuterLockHeld} & \tot{\batikTotalManyLocksHeld} & \per{\batikSucInnerMostLockHeld} & \per{\batikSucOuterMostLockHeld} \\
\bench{h2} 		& \et{\htwoEvents} & (\et{\htwoNoFPEvents}) 		& \tot{\htwoTotalLockHeld}		& \per{\htwoSingleLockHeld} 	& \per{\htwoTwoLocksHeld} 		& \per{\htwoManyLocksHeld} & \tot{\htwoTotalSingleLockHeld} & \per{\htwoSucSingleLockHeld} & \tot{\htwoTotalTwoLocksHeld} & \per{\htwoSucInnerLockHeld} & \per{\htwoSucOuterLockHeld} & \tot{\htwoTotalManyLocksHeld} & \per{\htwoSucInnerMostLockHeld} & \per{\htwoSucOuterMostLockHeld} \\
\bench{jython} 	& \et{\jythonEvents} & (\et{\jythonNoFPEvents}) 	& \tot{\jythonTotalLockHeld} 	& \per{\jythonSingleLockHeld} 	& \per{\jythonTwoLocksHeld} 	& \per{\jythonManyLocksHeld} & \tot{\jythonTotalSingleLockHeld} & \per{\jythonSucSingleLockHeld} & \tot{\jythonTotalTwoLocksHeld} & \per{\jythonSucInnerLockHeld} & \per{\jythonSucOuterLockHeld} & \tot{\jythonTotalManyLocksHeld} & \per{\jythonSucInnerMostLockHeld} & \per{\jythonSucOuterMostLockHeld} \\
\bench{luindex} & \et{\luindexEvents} & (\et{\luindexNoFPEvents}) 	& \tot{\luindexTotalLockHeld} 	& \per{\luindexSingleLockHeld}	& \per{\luindexTwoLocksHeld} 	& \per{\luindexManyLocksHeld} & \tot{\luindexTotalSingleLockHeld} & \per{\luindexSucSingleLockHeld} & \tot{\luindexTotalTwoLocksHeld} & \per{\luindexSucInnerLockHeld} & \per{\luindexSucOuterLockHeld} & \tot{\luindexTotalManyLocksHeld} & \per{\luindexSucInnerMostLockHeld} & \per{\luindexSucOuterMostLockHeld} \\
\bench{lusearch}& \et{\lusearchEvents} & (\et{\lusearchNoFPEvents})	& \tot{\lusearchTotalLockHeld}	& \per{\lusearchSingleLockHeld}	& \per{\lusearchTwoLocksHeld} 	& \per{\lusearchManyLocksHeld} & \tot{\lusearchTotalSingleLockHeld} & \per{\lusearchSucSingleLockHeld} & \tot{\lusearchTotalTwoLocksHeld} & \per{\lusearchSucInnerLockHeld} & \per{\lusearchSucOuterLockHeld} & \tot{\lusearchTotalManyLocksHeld} & \per{\lusearchSucInnerMostLockHeld} & \per{\lusearchSucOuterMostLockHeld} \\
\bench{pmd} 	& \et{\pmdEvents} & (\et{\pmdNoFPEvents}) 			& \tot{\pmdTotalLockHeld} 		& \per{\pmdSingleLockHeld} 		& \per{\pmdTwoLocksHeld} 		& \per{\pmdManyLocksHeld} & \tot{\pmdTotalSingleLockHeld} & \per{\pmdSucSingleLockHeld} & \tot{\pmdTotalTwoLocksHeld} & \per{\pmdSucInnerLockHeld} & \per{\pmdSucOuterLockHeld} & \tot{\pmdTotalManyLocksHeld} & \per{\pmdSucInnerMostLockHeld} & \per{\pmdSucOuterMostLockHeld} \\
\bench{sunflow} & \et{\sunflowEvents} & (\et{\sunflowNoFPEvents}) 	& \tot{\sunflowTotalLockHeld} 	& \per{\sunflowSingleLockHeld}	& \per{\sunflowTwoLocksHeld} 	& \per{\sunflowManyLocksHeld} & \tot{\sunflowTotalSingleLockHeld} & \per{\sunflowSucSingleLockHeld} & \tot{\sunflowTotalTwoLocksHeld} & \per{\sunflowSucInnerLockHeld} & \per{\sunflowSucOuterLockHeld} & \tot{\sunflowTotalManyLocksHeld} & \per{\sunflowSucInnerMostLockHeld} & \per{\sunflowSucOuterMostLockHeld} \\
\bench{tomcat} 	& \et{\tomcatEvents} & (\et{\tomcatNoFPEvents}) 	& \tot{\tomcatTotalLockHeld} 	& \per{\tomcatSingleLockHeld} 	& \per{\tomcatTwoLocksHeld} 	& \per{\tomcatManyLocksHeld} & \tot{\tomcatTotalSingleLockHeld} & \per{\tomcatSucSingleLockHeld} & \tot{\tomcatTotalTwoLocksHeld} & \per{\tomcatSucInnerLockHeld} & \per{\tomcatSucOuterLockHeld} & \tot{\tomcatTotalManyLocksHeld} & \per{\tomcatSucInnerMostLockHeld} & \per{\tomcatSucOuterMostLockHeld} \\
\bench{xalan} 	& \et{\xalanEvents} & (\et{\xalanNoFPEvents}) 		& \tot{\xalanTotalLockHeld} 	& \per{\xalanSingleLockHeld}	& \per{\xalanTwoLocksHeld} 		& \per{\xalanManyLocksHeld} & \tot{\xalanTotalSingleLockHeld} & \per{\xalanSucSingleLockHeld} & \tot{\xalanTotalTwoLocksHeld} & \per{\xalanSucInnerLockHeld} & \per{\xalanSucOuterLockHeld} & \tot{\xalanTotalManyLocksHeld} & \per{\xalanSucInnerMostLockHeld} & \per{\xalanSucOuterMostLockHeld} \\\hline
\end{tabular}
\end{minipage}
%
\label{tab:extra-data-counts-2:locksHeld}
\end{table*}

==> response-results.tex <==
\clearpage
\section{Results in preparation for response with Confidence Intervals}

\mike{In the following four race result tables,
are static races for Unopt-* analyses still counted by static site, not by field ID \& array type?
That's what it looks like based on comparing Unopt analyses to both non-Unopt analyses and the PLDI submission's reslts.}

\mike{Why does FTO-HB detect so many static races for \bench{h2}?
Have you looked at the reported field names and array types for FTO-HB on \bench{h2}
to see that there really are that many unique field names and array types being reported
(and not so many for the other configs running \bench{h2})?
What are those field names and array types?
More generally, have you sanity checked the results?}

\begin{table*}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\sdr}[4]{\vci{#1}{#2}{\;}(\vci{#3}{#4})}
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
% \input{result-macros/PIP_slowTool_AllConfig_memChange}
\input{result-macros/PIP_slowTool_raceEdgeFix}
% \input{result-macros/PIP_fastTool_sunflowCheck}
\input{result-macros/PIP_fastTool_readExclFix}
%
\smaller
\centering
\begin{tabular}{@{}l|llllll@{}}
Relation& w/ G & Unopt- & Epoch- & \FTO- & \REAbbrv- & AGG- \\\hline
\HB		& \rna														& \vci{\SLOWsunflowHBTime}{\SLOWsunflowHBTimeCI}					& \vci{\FASTsunflowHBTime}{\FASTsunflowHBTimeCI}		& \vci{\FASTsunflowFTOHBTime}{\FASTsunflowFTOHBTimeCI}		& \rna 													& \rna \\
\WCP	& \rna														& \vci{\SLOWsunflowWCPTime}{\SLOWsunflowWCPTimeCI}					& \vci{\FASTsunflowWCPTime}{\FASTsunflowWCPTimeCI}		& \vci{\FASTsunflowFTOWCPTime}{\FASTsunflowFTOWCPTimeCI}	& \vci{\FASTsunflowREWCPTime}{\FASTsunflowREWCPTimeCI}	& \rna \\
\DC		& \vci{\SLOWsunflowDCExcTime}{\SLOWsunflowDCExcTimeCI}	& \vci{\SLOWsunflowDCnoGExcTime}{\SLOWsunflowDCnoGExcTimeCI}		& \vci{\FASTsunflowDCTime}{\FASTsunflowDCTimeCI}		& \vci{\FASTsunflowFTODCTime}{\FASTsunflowFTODCTimeCI}		& \vci{\FASTsunflowREDCTime}{\FASTsunflowREDCTimeCI}	& \rna \\
\CAPO	& \vci{\SLOWsunflowCAPOExcTime}{\SLOWsunflowCAPOExcTimeCI}	& \vci{\SLOWsunflowCAPOnoGExcTime}{\SLOWsunflowCAPOnoGExcTimeCI}	& \vci{\FASTsunflowCAPOTime}{\FASTsunflowCAPOTimeCI}	& \vci{\FASTsunflowFTOCAPOTime}{\FASTsunflowFTOCAPOTimeCI}	& \vci{\FASTsunflowRECAPOTime}{\FASTsunflowRECAPOTimeCI}& \vci{\FASTsunflowAGGCAPOTime}{\FASTsunflowAGGCAPOTimeCI} \\
\mc{1}{c}{} & \mc{6}{c}{\bench{sunflow} run-time} \\
\end{tabular}
\hfill
\begin{tabular}{@{}l|llllll@{}}
Relation& w/ G & Unopt- & Epoch- & \FTO- & \REAbbrv- & AGG- \\\hline 
\HB		& \rna													& \vci{\SLOWsunflowHBMem}{\SLOWsunflowHBMemCI}					& \vci{\FASTsunflowHBMem}{\FASTsunflowHBMemCI}		& \vci{\FASTsunflowFTOHBMem}{\FASTsunflowFTOHBMemCI}		& \rna													& \rna \\
\WCP	& \rna													& \vci{\SLOWsunflowWCPMem}{\SLOWsunflowWCPMemCI}				& \vci{\FASTsunflowWCPMem}{\FASTsunflowWCPMemCI}	& \vci{\FASTsunflowFTOWCPMem}{\FASTsunflowFTOWCPMemCI}		& \vci{\FASTsunflowREWCPMem}{\FASTsunflowREWCPMemCI}	& \rna \\
\DC		& \vci{\SLOWsunflowDCExcMem}{\SLOWsunflowDCExcMemCI}	& \vci{\SLOWsunflowDCnoGExcMem}{\SLOWsunflowDCnoGExcMemCI}	& \vci{\FASTsunflowDCMem}{\FASTsunflowDCMemCI}		& \vci{\FASTsunflowFTODCMem}{\FASTsunflowFTODCMemCI}		& \vci{\FASTsunflowREDCMem}{\FASTsunflowREDCMemCI}		& \rna \\
\CAPO	& \vci{\SLOWsunflowCAPOExcMem}{\SLOWsunflowCAPOExcMemCI}& \vci{\SLOWsunflowCAPOnoGExcMem}{\SLOWsunflowCAPOnoGExcMemCI}	& \vci{\FASTsunflowCAPOMem}{\FASTsunflowCAPOMemCI}	& \vci{\FASTsunflowFTOCAPOMem}{\FASTsunflowFTOCAPOMemCI}	& \vci{\FASTsunflowRECAPOMem}{\FASTsunflowRECAPOMemCI}	& \vci{\FASTsunflowAGGCAPOMem}{\FASTsunflowAGGCAPOMemCI} \\
\mc{1}{c}{} & \mc{6}{c}{\bench{sunflow} memory} \\
\end{tabular}
\hfill
\begin{tabular}{@{}l|llllll@{}}
        & w/ G & Unopt- & Epoch- & \FTO- & \REAbbrv- & AGG- \\\hline
\HB		& \rna																										& \sdr{\SLOWsunflowHB}{\SLOWsunflowHBCI}{\SLOWsunflowHBDynamic}{\SLOWsunflowHBDynamicCI}								& \sdr{\FASTsunflowHB}{\FASTsunflowHBCI}{\FASTsunflowHBDynamic}{\FASTsunflowHBDynamicCI}		& \sdr{\FASTsunflowFTOHB}{\FASTsunflowFTOHBCI}{\FASTsunflowFTOHBDynamic}{\FASTsunflowFTOHBDynamicCI}		& \rna																									& \rna \\
\WCP	& \rna																										& \sdr{\SLOWsunflowWCP}{\SLOWsunflowWCPCI}{\SLOWsunflowWCPDynamic}{\SLOWsunflowWCPDynamicCI}							& \sdr{\FASTsunflowWCP}{\FASTsunflowWCPCI}{\FASTsunflowWCPDynamic}{\FASTsunflowWCPDynamicCI}	& \sdr{\FASTsunflowFTOWCP}{\FASTsunflowFTOWCPCI}{\FASTsunflowFTOWCPDynamic}{\FASTsunflowFTOWCPDynamicCI}	& \sdr{\FASTsunflowREWCP}{\FASTsunflowREWCPCI}{\FASTsunflowREWCPDynamic}{\FASTsunflowREWCPDynamicCI}	& \rna \\
\DC		& \sdr{\SLOWsunflowDCExc}{\SLOWsunflowDCExcCI}{\SLOWsunflowDCExcDynamic}{\SLOWsunflowDCExcDynamicCI}	& \sdr{\SLOWsunflowDCnoGExc}{\SLOWsunflowDCnoGExcCI}{\SLOWsunflowDCnoGExcDynamic}{\SLOWsunflowDCnoGExcDynamicCI}	& \sdr{\FASTsunflowDC}{\FASTsunflowDCCI}{\FASTsunflowDCDynamic}{\FASTsunflowDCDynamicCI}		& \sdr{\FASTsunflowFTODC}{\FASTsunflowFTODCCI}{\FASTsunflowFTODCDynamic}{\FASTsunflowFTODCDynamicCI}		& \sdr{\FASTsunflowREDC}{\FASTsunflowREDCCI}{\FASTsunflowREDCDynamic}{\FASTsunflowREDCDynamicCI}		& \rna \\
\CAPO	& \sdr{\SLOWsunflowCAPOExc}{\SLOWsunflowCAPOExcCI}{\SLOWsunflowCAPOExcDynamic}{\SLOWsunflowCAPOExcDynamicCI}& \sdr{\SLOWsunflowCAPOnoGExc}{\SLOWsunflowCAPOnoGExcCI}{\SLOWsunflowCAPOnoGExcDynamic}{\SLOWsunflowCAPOnoGExcDynamicCI}& \sdr{\FASTsunflowCAPO}{\FASTsunflowCAPOCI}{\FASTsunflowCAPODynamic}{\FASTsunflowCAPODynamicCI}& \sdr{\FASTsunflowFTOCAPO}{\FASTsunflowFTOCAPOCI}{\FASTsunflowFTOCAPODynamic}{\FASTsunflowFTOCAPODynamicCI}& \sdr{\FASTsunflowRECAPO}{\FASTsunflowRECAPOCI}{\FASTsunflowRECAPODynamic}{\FASTsunflowRECAPODynamicCI}& \sdr{\FASTsunflowAGGCAPO}{\FASTsunflowAGGCAPOCI}{\FASTsunflowAGGCAPODynamic}{\FASTsunflowAGGCAPODynamicCI} \\
\mc{1}{c}{} & \mc{6}{c}{\bench{sunflow} races} \\
\end{tabular}
\caption{Run time, memory usage, and average races reported, relative to
uninstrumented execution, of various analyses for sunflow program
with 95\% confidence intervals.}
\end{table*}

% Table for geometric mean of all relations with event type counts
\begin{table*}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
% \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!Mb$}} %memory
\newcommand{\et}[1]{#1{\;}M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\per}[1]{\ifthenelse{\equal{#1}{\cna}}{\cna}{#1\%}}
\newcommand{\cna}{---} %em-dash. (--) for en-dash
% \input{result-macros/PIP_fastTool_sunflowCheck}
\input{result-macros/PIP_fastTool_readExclFix}
%
\small
\centering
\renewcommand\bench[1]{\multirow{2}{*}{\code{#1}}}
\begin{tabular}{@{}l|l|r|HHr|r|r|r|r@{}ZZ}
\mc{1}{c}{} & \mc{7}{c}{\bench{sunflow}} \\ \\
				&Event	& & \mc{2}{Z}{Same} & \mc{2}{c|}{Owned} & \mc{3}{c@{}}{Unowned} & \mc{2}{Z}{Locks} \\
Relation		&Type	& Total & Epoch & Shr Epoch & Excl & Shared & Excl & Share & Shared & Held & Not Held \\\hline
				&Read	& \et{\sunflowHBNoFPReadTotal}	& \per{\sunflowHBReadSameEp}	& \per{\sunflowHBReadSharedSameEp}	& \per{\sunflowHBReadOwned} & \per{\sunflowHBReadSharedOwned} & \per{\sunflowHBReadExclusive} & \per{\sunflowHBReadShare} 	& \per{\sunflowHBReadShared} & \per{\sunflowHBReadInCS} & \per{\sunflowHBReadOutCS} \\
Epoch-\HB		&Write	& \et{\sunflowHBNoFPWriteTotal}& \per{\sunflowHBWriteSameEp}	& \rna							& \per{\sunflowHBWriteOwned}& \rna							& \per{\sunflowHBWriteExclusive}& \rna						& \per{\sunflowHBWriteShared}& \per{\sunflowHBWriteInCS} & \per{\sunflowHBWriteOutCS} \\\hline
% \end{tabular}
% \begin{tabular}{@{}l|l|r|HHr|r|r|r|r@{}ZZ}
				&Event	& & \mc{2}{Z}{Same} & \mc{2}{c|}{Owned} & \mc{3}{c@{}}{Unowned} & \mc{2}{Z}{Locks} \\
				&Type	& Total & Epoch & Shr Epoch & Excl & Shared & Excl & Share & Shared & Held & Not Held \\\hline
				&Read	& \et{\sunflowFTOHBNoFPReadTotal}	& \per{\sunflowFTOHBReadSameEp}	& \per{\sunflowFTOHBReadSharedSameEp}	& \per{\sunflowFTOHBReadOwned} & \per{\sunflowFTOHBReadSharedOwned} & \per{\sunflowFTOHBReadExclusive} & \per{\sunflowFTOHBReadShare} 	& \per{\sunflowFTOHBReadShared} & \per{\sunflowFTOHBReadInCS} & \per{\sunflowFTOHBReadOutCS} \\
\FTO-\HB		&Write	& \et{\sunflowFTOHBNoFPWriteTotal}& \per{\sunflowFTOHBWriteSameEp}	& \rna							& \per{\sunflowFTOHBWriteOwned}& \rna							& \per{\sunflowFTOHBWriteExclusive}& \rna						& \per{\sunflowFTOHBWriteShared}& \per{\sunflowFTOHBWriteInCS} & \per{\sunflowFTOHBWriteOutCS} \\\hline
% \end{tabular}
% \begin{tabular}{@{}l|l|r|HHr|r|r|r|r@{}ZZ}
% 				&Event	& & \mc{2}{Z}{Same} & \mc{2}{c|}{Owned} & \mc{3}{c@{}}{Unowned} & \mc{2}{Z}{Locks} \\
% 				&Type	& Total & Epoch & Shr Epoch & Excl & Shared & Excl & Share & Shared & Held & Not Held \\\hline
% 				&Read	& \et{\sunflowWCPNoFPReadTotal}	& \per{\sunflowWCPReadSameEp}	& \per{\sunflowWCPReadSharedSameEp}	& \per{\sunflowWCPReadOwned} & \per{\sunflowWCPReadSharedOwned} & \per{\sunflowWCPReadExclusive} & \per{\sunflowWCPReadShare} 	& \per{\sunflowWCPReadShared} & \per{\sunflowWCPReadInCS} & \per{\sunflowWCPReadOutCS} \\
% Epoch-\WCP		&Write	& \et{\sunflowWCPNoFPWriteTotal}& \per{\sunflowWCPWriteSameEp}	& \rna							& \per{\sunflowWCPWriteOwned}& \rna							& \per{\sunflowWCPWriteExclusive}& \rna						& \per{\sunflowWCPWriteShared}& \per{\sunflowWCPWriteInCS} & \per{\sunflowWCPWriteOutCS} \\\hline
% \end{tabular}
% \begin{tabular}{@{}l|l|r|HHr|r|r|r|r@{}ZZ}
				&Event	& & \mc{2}{Z}{Same} & \mc{2}{c|}{Owned} & \mc{3}{c@{}}{Unowned} & \mc{2}{Z}{Locks} \\
				&Type	& Total & Epoch & Shr Epoch & Excl & Shared & Excl & Share & Shared & Held & Not Held \\\hline
				&Read	& \et{\sunflowFTOWCPNoFPReadTotal}	& \per{\sunflowFTOWCPReadSameEp}	& \per{\sunflowFTOWCPReadSharedSameEp}	& \per{\sunflowFTOWCPReadOwned} & \per{\sunflowFTOWCPReadSharedOwned} & \per{\sunflowFTOWCPReadExclusive} & \per{\sunflowFTOWCPReadShare} 	& \per{\sunflowFTOWCPReadShared} & \per{\sunflowFTOWCPReadInCS} & \per{\sunflowFTOWCPReadOutCS} \\
\FTO-\WCP		&Write	& \et{\sunflowFTOWCPNoFPWriteTotal}& \per{\sunflowFTOWCPWriteSameEp}	& \rna							& \per{\sunflowFTOWCPWriteOwned}& \rna							& \per{\sunflowFTOWCPWriteExclusive}& \rna						& \per{\sunflowFTOWCPWriteShared}& \per{\sunflowFTOWCPWriteInCS} & \per{\sunflowFTOWCPWriteOutCS} \\\hline
% \end{tabular}
% \begin{tabular}{@{}l|l|r|HHr|r|r|r|r@{}ZZ}
				&Event	& & \mc{2}{Z}{Same} & \mc{2}{c|}{Owned} & \mc{3}{c@{}}{Unowned} & \mc{2}{Z}{Locks} \\
				&Type	& Total & Epoch & Shr Epoch & Excl & Shared & Excl & Share & Shared & Held & Not Held \\\hline
				&Read	& \et{\sunflowREWCPNoFPReadTotal}	& \per{\sunflowREWCPReadSameEp}	& \per{\sunflowREWCPReadSharedSameEp}	& \per{\sunflowREWCPReadOwned} & \per{\sunflowREWCPReadSharedOwned} & \per{\sunflowREWCPReadExclusive} & \per{\sunflowREWCPReadShare} 	& \per{\sunflowREWCPReadShared} & \per{\sunflowREWCPReadInCS} & \per{\sunflowREWCPReadOutCS} \\
\REAbbrv-\WCP	&Write	& \et{\sunflowREWCPNoFPWriteTotal}& \per{\sunflowREWCPWriteSameEp}	& \rna							& \per{\sunflowREWCPWriteOwned}& \rna							& \per{\sunflowREWCPWriteExclusive}& \rna						& \per{\sunflowREWCPWriteShared}& \per{\sunflowREWCPWriteInCS} & \per{\sunflowREWCPWriteOutCS} \\\hline
% \end{tabular}
% \begin{tabular}{@{}l|l|r|HHr|r|r|r|r@{}ZZ}
% 				&Event	& & \mc{2}{Z}{Same} & \mc{2}{c|}{Owned} & \mc{3}{c@{}}{Unowned} & \mc{2}{Z}{Locks} \\
% 				&Type	& Total & Epoch & Shr Epoch & Excl & Shared & Excl & Share & Shared & Held & Not Held \\\hline
% 				&Read	& \et{\sunflowDCNoFPReadTotal}	& \per{\sunflowDCReadSameEp}	& \per{\sunflowDCReadSharedSameEp}	& \per{\sunflowDCReadOwned} & \per{\sunflowDCReadSharedOwned} & \per{\sunflowDCReadExclusive} & \per{\sunflowDCReadShare} 	& \per{\sunflowDCReadShared} & \per{\sunflowDCReadInCS} & \per{\sunflowDCReadOutCS} \\
% Epoch-\DC		&Write	& \et{\sunflowDCNoFPWriteTotal}& \per{\sunflowDCWriteSameEp}	& \rna							& \per{\sunflowDCWriteOwned}& \rna							& \per{\sunflowDCWriteExclusive}& \rna						& \per{\sunflowDCWriteShared}& \per{\sunflowDCWriteInCS} & \per{\sunflowDCWriteOutCS} \\\hline
% \end{tabular}
% \begin{tabular}{@{}l|l|r|HHr|r|r|r|r@{}ZZ}
				&Event	& & \mc{2}{Z}{Same} & \mc{2}{c|}{Owned} & \mc{3}{c@{}}{Unowned} & \mc{2}{Z}{Locks} \\
				&Type	& Total & Epoch & Shr Epoch & Excl & Shared & Excl & Share & Shared & Held & Not Held \\\hline
				&Read	& \et{\sunflowFTODCNoFPReadTotal}	& \per{\sunflowFTODCReadSameEp}	& \per{\sunflowFTODCReadSharedSameEp}	& \per{\sunflowFTODCReadOwned} & \per{\sunflowFTODCReadSharedOwned} & \per{\sunflowFTODCReadExclusive} & \per{\sunflowFTODCReadShare} 	& \per{\sunflowFTODCReadShared} & \per{\sunflowFTODCReadInCS} & \per{\sunflowFTODCReadOutCS} \\
\FTO-\DC		&Write	& \et{\sunflowFTODCNoFPWriteTotal}& \per{\sunflowFTODCWriteSameEp}	& \rna							& \per{\sunflowFTODCWriteOwned}& \rna							& \per{\sunflowFTODCWriteExclusive}& \rna						& \per{\sunflowFTODCWriteShared}& \per{\sunflowFTODCWriteInCS} & \per{\sunflowFTODCWriteOutCS} \\\hline
% \end{tabular}
% \begin{tabular}{@{}l|l|r|HHr|r|r|r|r@{}ZZ}
				&Event	& & \mc{2}{Z}{Same} & \mc{2}{c|}{Owned} & \mc{3}{c@{}}{Unowned} & \mc{2}{Z}{Locks} \\
				&Type	& Total & Epoch & Shr Epoch & Excl & Shared & Excl & Share & Shared & Held & Not Held \\\hline
				&Read	& \et{\sunflowREDCNoFPReadTotal}	& \per{\sunflowREDCReadSameEp}	& \per{\sunflowREDCReadSharedSameEp}	& \per{\sunflowREDCReadOwned} & \per{\sunflowREDCReadSharedOwned} & \per{\sunflowREDCReadExclusive} & \per{\sunflowREDCReadShare} 	& \per{\sunflowREDCReadShared} & \per{\sunflowREDCReadInCS} & \per{\sunflowREDCReadOutCS} \\
\REAbbrv-\DC	&Write	& \et{\sunflowREDCNoFPWriteTotal}& \per{\sunflowREDCWriteSameEp}	& \rna							& \per{\sunflowREDCWriteOwned}& \rna							& \per{\sunflowREDCWriteExclusive}& \rna						& \per{\sunflowREDCWriteShared}& \per{\sunflowREDCWriteInCS} & \per{\sunflowREDCWriteOutCS} \\\hline
% \end{tabular}
% \begin{tabular}{@{}l|l|r|HHr|r|r|r|r@{}ZZ}
% 				&Event	& & \mc{2}{Z}{Same} & \mc{2}{c|}{Owned} & \mc{3}{c@{}}{Unowned} & \mc{2}{Z}{Locks} \\
% 				&Type	& Total & Epoch & Shr Epoch & Excl & Shared & Excl & Share & Shared & Held & Not Held \\\hline
% 				&Read	& \et{\sunflowCAPONoFPReadTotal}	& \per{\sunflowCAPOReadSameEp}	& \per{\sunflowCAPOReadSharedSameEp}	& \per{\sunflowCAPOReadOwned} & \per{\sunflowCAPOReadSharedOwned} & \per{\sunflowCAPOReadExclusive} & \per{\sunflowCAPOReadShare} 	& \per{\sunflowCAPOReadShared} & \per{\sunflowCAPOReadInCS} & \per{\sunflowCAPOReadOutCS} \\
% Epoch-\CAPO		&Write	& \et{\sunflowCAPONoFPWriteTotal}& \per{\sunflowCAPOWriteSameEp}	& \rna							& \per{\sunflowCAPOWriteOwned}& \rna							& \per{\sunflowCAPOWriteExclusive}& \rna						& \per{\sunflowCAPOWriteShared}& \per{\sunflowCAPOWriteInCS} & \per{\sunflowCAPOWriteOutCS} \\\hline
% \end{tabular}
% \begin{tabular}{@{}l|l|r|HHr|r|r|r|r@{}ZZ}
				&Event	& & \mc{2}{Z}{Same} & \mc{2}{c|}{Owned} & \mc{3}{c@{}}{Unowned} & \mc{2}{Z}{Locks} \\
				&Type	& Total & Epoch & Shr Epoch & Excl & Shared & Excl & Share & Shared & Held & Not Held \\\hline
				&Read	& \et{\sunflowFTOCAPONoFPReadTotal}	& \per{\sunflowFTOCAPOReadSameEp}	& \per{\sunflowFTOCAPOReadSharedSameEp}	& \per{\sunflowFTOCAPOReadOwned} & \per{\sunflowFTOCAPOReadSharedOwned} & \per{\sunflowFTOCAPOReadExclusive} & \per{\sunflowFTOCAPOReadShare} 	& \per{\sunflowFTOCAPOReadShared} & \per{\sunflowFTOCAPOReadInCS} & \per{\sunflowFTOCAPOReadOutCS} \\
\FTO-\CAPO		&Write	& \et{\sunflowFTOCAPONoFPWriteTotal}& \per{\sunflowFTOCAPOWriteSameEp}	& \rna							& \per{\sunflowFTOCAPOWriteOwned}& \rna							& \per{\sunflowFTOCAPOWriteExclusive}& \rna						& \per{\sunflowFTOCAPOWriteShared}& \per{\sunflowFTOCAPOWriteInCS} & \per{\sunflowFTOCAPOWriteOutCS} \\\hline
% \end{tabular}
% \begin{tabular}{@{}l|l|r|HHr|r|r|r|r@{}ZZ}
				&Event	& & \mc{2}{Z}{Same} & \mc{2}{c|}{Owned} & \mc{3}{c@{}}{Unowned} & \mc{2}{Z}{Locks} \\
				&Type	& Total & Epoch & Shr Epoch & Excl & Shared & Excl & Share & Shared & Held & Not Held \\\hline
				&Read	& \et{\sunflowRECAPONoFPReadTotal}	& \per{\sunflowRECAPOReadSameEp}	& \per{\sunflowRECAPOReadSharedSameEp}	& \per{\sunflowRECAPOReadOwned} & \per{\sunflowRECAPOReadSharedOwned} & \per{\sunflowRECAPOReadExclusive} & \per{\sunflowRECAPOReadShare} 	& \per{\sunflowRECAPOReadShared} & \per{\sunflowRECAPOReadInCS} & \per{\sunflowRECAPOReadOutCS} \\
\REAbbrv-\CAPO	&Write	& \et{\sunflowRECAPONoFPWriteTotal}& \per{\sunflowRECAPOWriteSameEp}	& \rna							& \per{\sunflowRECAPOWriteOwned}& \rna							& \per{\sunflowRECAPOWriteExclusive}& \rna						& \per{\sunflowRECAPOWriteShared}& \per{\sunflowRECAPOWriteInCS} & \per{\sunflowRECAPOWriteOutCS} \\\hline
\end{tabular}
\caption{Frequencies of non-same-epoch reads and writes for various
analyses, for sunflow program.}
% \label{tab:characteristic:event-type}
\end{table*}


\iffalse
%Duplicate result tables from main paper with recent fixes for fast and slow tool
\subsection{PIP FastTool Read-Exclusive Fix and PIP SlowTool Race-Edge Fix}

\begin{table*}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\baseMem}[1]{#1~MB} %base memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
% \input{result-macros/PIP_slowTool_AllConfig_memChange}
\input{result-macros/PIP_slowTool_raceEdgeFix}
\input{result-macros/PIP_fastTool_readExclFix_Quite}
%
\small
\centering
\newcommand{\ics}{\;}
\begin{tabular}{@{}l|HHHHr|lll|l@{\ics}l|l@{\ics}l@{}}
& \mc{2}{Z}{} & \mc{2}{Z}{} & Base & \mc{3}{c|}{\HB} & \mc{2}{c|}{Unopt-\DC} & \mc{2}{c@{}}{Unopt-\CAPO} \\
Program & \mc{2}{Z}{Events} & \mc{2}{Z}{\#Thr} & time & RR\FTTwoAbbrv & \FTTwoAbbrv & \FTO & w/ G & w/o G & w/ G & w/o G \\\hline 
\bench{avrora} 	& \et{\FASTavroraEvents}{\FASTavroraEventsCI}   & \enfp{\FASTavroraNoFPEvents}{\FASTavroraNoFPEventsCI}	& \FASTavroraTotalThreads 	& (\FASTavroraMaxLiveThreads)	& \base{\FASTavroraBaseTime}   & \vci{\FASTavroraFTTime}{\FASTavroraFTTimeCI}   & \vci{\FASTavroraHBTime}{\FASTavroraHBTimeCI}	& \vci{\FASTavroraFTOHBTime}{\FASTavroraFTOHBTimeCI}	& \vci{\SLOWavroraDCExcTime}{\SLOWavroraDCExcTimeCI}	& \vci{\SLOWavroraDCnoGExcTime}{\SLOWavroraDCnoGExcTimeCI}	& \vci{\SLOWavroraCAPOExcTime}{\SLOWavroraCAPOExcTimeCI}	& \vci{\SLOWavroraCAPOnoGExcTime}{\SLOWavroraCAPOnoGExcTimeCI}\\
\bench{batik} 	& \et{\FASTbatikEvents}{\FASTbatikEventsCI}    & \enfp{\FASTbatikNoFPEvents}{\FASTbatikNoFPEventsCI}	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& \base{\FASTbatikBaseTime}    & \vci{\FASTbatikFTTime}{\FASTbatikFTTimeCI}    & \vci{\FASTbatikHBTime}{\FASTbatikHBTimeCI}   	& \vci{\FASTbatikFTOHBTime}{\FASTbatikFTOHBTimeCI}		& \vci{\SLOWbatikDCExcTime}{\SLOWbatikDCExcTimeCI}	& \vci{\SLOWbatikDCnoGExcTime}{\SLOWbatikDCnoGExcTimeCI}		& \vci{\SLOWbatikCAPOExcTime}{\SLOWbatikCAPOExcTimeCI}	& \vci{\SLOWbatikCAPOnoGExcTime}{\SLOWbatikCAPOnoGExcTimeCI} \\
\bench{h2} 		& \et{\FASThtwoEvents}{\FASThtwoEventsCI}     & \enfp{\FASThtwoNoFPEvents}{\FASThtwoNoFPEventsCI}	    & \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & \base{\FASThtwoBaseTime}     & \vci{\FASThtwoFTTime}{\FASThtwoFTTimeCI}     & \vci{\FASThtwoHBTime}{\FASThtwoHBTimeCI}    	& \vci{\FASThtwoFTOHBTime}{\FASThtwoFTOHBTimeCI}		& \vci{\SLOWhtwoDCExcTime}{\SLOWhtwoDCExcTimeCI}		& \vci{\SLOWhtwoDCnoGExcTime}{\SLOWhtwoDCnoGExcTimeCI}		& \vci{\SLOWhtwoCAPOExcTime}{\SLOWhtwoCAPOExcTimeCI}	& \vci{\SLOWhtwoCAPOnoGExcTime}{\SLOWhtwoCAPOnoGExcTimeCI}\\
\bench{jython} 	& \et{\FASTjythonEvents}{\FASTjythonEventsCI}   & \enfp{\FASTjythonNoFPEvents}{\FASTjythonNoFPEventsCI}	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& \base{\FASTjythonBaseTime}   & \vci{\FASTjythonFTTime}{\FASTjythonFTTimeCI}   & \vci{\FASTjythonHBTime}{\FASTjythonHBTimeCI} 	& \vci{\FASTjythonFTOHBTime}{\FASTjythonFTOHBTimeCI}	& \vci{\SLOWjythonDCExcTime}{\SLOWjythonDCExcTimeCI}	& \vci{\SLOWjythonDCnoGExcTime}{\SLOWjythonDCnoGExcTimeCI}	& \vci{\SLOWjythonCAPOExcTime}{\SLOWjythonCAPOExcTimeCI}	& \vci{\SLOWjythonCAPOnoGExcTime}{\SLOWjythonCAPOnoGExcTimeCI} \\
\bench{luindex} & \et{\FASTluindexEvents}{\FASTluindexEventsCI}  & \enfp{\FASTluindexNoFPEvents}{\FASTluindexNoFPEventsCI}	& \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& \base{\FASTluindexBaseTime}  & \vci{\FASTluindexFTTime}{\FASTluindexFTTimeCI}  & \vci{\FASTluindexHBTime}{\FASTluindexHBTimeCI} 	& \vci{\FASTluindexFTOHBTime}{\FASTluindexFTOHBTimeCI}	& \vci{\SLOWluindexDCExcTime}{\SLOWluindexDCExcTimeCI}	& \vci{\SLOWluindexDCnoGExcTime}{\SLOWluindexDCnoGExcTimeCI}	& \vci{\SLOWluindexCAPOExcTime}{\SLOWluindexCAPOExcTimeCI}	& \vci{\SLOWluindexCAPOnoGExcTime}{\SLOWluindexCAPOnoGExcTimeCI} \\
\bench{lusearch}& \et{\FASTlusearchEvents}{\FASTlusearchEventsCI} & \enfp{\FASTlusearchNoFPEvents}{\FASTlusearchNoFPEventsCI}	& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& \base{\FASTlusearchBaseTime} & \vci{\FASTlusearchFTTime}{\FASTlusearchFTTimeCI} & \vci{\FASTlusearchHBTime}{\FASTlusearchHBTimeCI}	& \vci{\FASTlusearchFTOHBTime}{\FASTlusearchFTOHBTimeCI}	& \vci{\SLOWlusearchDCExcTime}{\SLOWlusearchDCExcTimeCI}	& \vci{\SLOWlusearchDCnoGExcTime}{\SLOWlusearchDCnoGExcTimeCI}	& \vci{\SLOWlusearchCAPOExcTime}{\SLOWlusearchCAPOExcTimeCI}& \vci{\SLOWlusearchCAPOnoGExcTime}{\SLOWlusearchCAPOnoGExcTimeCI} \\
\bench{pmd}		& \et{\FASTpmdEvents}{\FASTpmdEventsCI}      & \enfp{\FASTpmdNoFPEvents}{\FASTpmdNoFPEventsCI}      & \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & \base{\FASTpmdBaseTime}      & \vci{\FASTpmdFTTime}{\FASTpmdFTTimeCI}      & \vci{\FASTpmdHBTime}{\FASTpmdHBTimeCI}		& \vci{\FASTpmdFTOHBTime}{\FASTpmdFTOHBTimeCI}		& \vci{\SLOWpmdDCExcTime}{\SLOWpmdDCExcTimeCI}		& \vci{\SLOWpmdDCnoGExcTime}{\SLOWpmdDCnoGExcTimeCI}		& \vci{\SLOWpmdCAPOExcTime}{\SLOWpmdCAPOExcTimeCI}		& \vci{\SLOWpmdCAPOnoGExcTime}{\SLOWpmdCAPOnoGExcTimeCI} \\
\bench{sunflow} & \et{\FASTsunflowEvents}{\FASTsunflowEventsCI}  & \enfp{\FASTsunflowNoFPEvents}{\FASTsunflowNoFPEventsCI}	& \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& \base{\FASTsunflowBaseTime}  & \vci{\FASTsunflowFTTime}{\FASTsunflowFTTimeCI}  & \vci{\FASTsunflowHBTime}{\FASTsunflowHBTimeCI}	& \vci{\FASTsunflowFTOHBTime}{\FASTsunflowFTOHBTimeCI}	& \vci{\SLOWsunflowDCExcTime}{\SLOWsunflowDCExcTimeCI}	& \vci{\SLOWsunflowDCnoGExcTime}{\SLOWsunflowDCnoGExcTimeCI}	& \vci{\SLOWsunflowCAPOExcTime}{\SLOWsunflowCAPOExcTimeCI}	& \vci{\SLOWsunflowCAPOnoGExcTime}{\SLOWsunflowCAPOnoGExcTimeCI} \\
\bench{tomcat} 	& \et{\FASTtomcatEvents}{\FASTtomcatEventsCI}   & \enfp{\FASTtomcatNoFPEvents}{\FASTtomcatNoFPEventsCI}	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& \base{\FASTtomcatBaseTime}   & \vci{\FASTtomcatFTTime}{\FASTtomcatFTTimeCI}   & \vci{\FASTtomcatHBTime}{\FASTtomcatHBTimeCI} 	& \vci{\FASTtomcatFTOHBTime}{\FASTtomcatFTOHBTimeCI}	& \vci{\SLOWtomcatDCExcTime}{\SLOWtomcatDCExcTimeCI}	& \vci{\SLOWtomcatDCnoGExcTime}{\SLOWtomcatDCnoGExcTimeCI}	& \vci{\SLOWtomcatCAPOExcTime}{\SLOWtomcatCAPOExcTimeCI}	& \vci{\SLOWtomcatCAPOnoGExcTime}{\SLOWtomcatCAPOnoGExcTimeCI} \\
\bench{xalan} 	& \et{\FASTxalanEvents}{\FASTxalanEventsCI}    & \enfp{\FASTxalanNoFPEvents}{\FASTxalanNoFPEventsCI}	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& \base{\FASTxalanBaseTime}    & \vci{\FASTxalanFTTime}{\FASTxalanFTTimeCI}    & \vci{\FASTxalanHBTime}{\FASTxalanHBTimeCI}		& \vci{\FASTxalanFTOHBTime}{\FASTxalanFTOHBTimeCI}		& \vci{\SLOWxalanDCExcTime}{\SLOWxalanDCExcTimeCI}	& \vci{\SLOWxalanDCnoGExcTime}{\SLOWxalanDCnoGExcTimeCI} 	& \vci{\SLOWxalanCAPOExcTime}{\SLOWxalanCAPOExcTimeCI}	& \vci{\SLOWxalanCAPOnoGExcTime}{\SLOWxalanCAPOnoGExcTimeCI}\\\hline
geomean	& &	& &	& & \roh{\FASTFTTimeGeoMean} & \roh{\FASTHBTimeGeoMean} & \roh{\FASTFTOHBTimeGeoMean} & \roh{\SLOWDCExcTimeGeoMean} & \roh{\SLOWDCnoGExcTimeGeoMean} & \roh{\SLOWCAPOExcTimeGeoMean} & \roh{\SLOWCAPOnoGExcTimeGeoMean} \\
\mc{1}{c}{} & \mc{12}{c}{Run time} \\
\end{tabular}

\caption{Run-time performance for various FastTrack-based \HB analyses
and for unoptimized \DC and \CAPO analyses, relative to uninstrumented
execution, with 95\% confidence intervals.}
\label{tab:performance:fasttrack:timeCI}
\end{table*}


\begin{table*}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\baseMem}[1]{#1~MB} %base memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
% \input{result-macros/PIP_slowTool_AllConfig_memChange}
\input{result-macros/PIP_slowTool_raceEdgeFix}
\input{result-macros/PIP_fastTool_readExclFix_Quite}
%
\small
\centering
\newcommand{\ics}{\;\;}
\begin{tabular}{@{}l|HHHHr|lll|l@{\ics}l|l@{\ics}l@{}}
& \mc{2}{Z}{} & \mc{2}{Z}{} & Base & \mc{3}{c|}{\HB} & \mc{2}{c|}{Unopt-\DC} & \mc{2}{c@{}}{Unopt-\CAPO} \\
Program & \mc{2}{Z}{Events} & \mc{2}{Z}{\#Thr} & memory & RR\FTTwoAbbrv & \FTTwoAbbrv & \FTO & w/ G & w/o G & w/ G & w/o G \\\hline 
\bench{avrora} 	& \et{\FASTavroraEvents}{\FASTavroraEventsCI}   & \enfp{\FASTavroraNoFPEvents}{\FASTavroraNoFPEventsCI}	& \FASTavroraTotalThreads 	& (\FASTavroraMaxLiveThreads)	& \baseMem{\FASTavroraBaseMem}   & \vci{\FASTavroraFTMem}{\FASTavroraFTMemCI}   & \vci{\FASTavroraHBMem}{\FASTavroraHBMemCI}	& \vci{\FASTavroraFTOHBMem}{\FASTavroraFTOHBMemCI}	& \vci{\SLOWavroraDCExcMem}{\SLOWavroraDCExcMemCI}	& \vci{\SLOWavroraDCnoGExcMem}{\SLOWavroraDCnoGExcMemCI}	& \vci{\SLOWavroraCAPOExcMem}{\SLOWavroraCAPOExcMemCI}	& \vci{\SLOWavroraCAPOnoGExcMem}{\SLOWavroraCAPOnoGExcMemCI}\\
\bench{batik} 	& \et{\FASTbatikEvents}{\FASTbatikEventsCI}    & \enfp{\FASTbatikNoFPEvents}{\FASTbatikNoFPEventsCI}	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& \baseMem{\FASTbatikBaseMem}    & \vci{\FASTbatikFTMem}{\FASTbatikFTMemCI}    & \vci{\FASTbatikHBMem}{\FASTbatikHBMemCI}   	& \vci{\FASTbatikFTOHBMem}{\FASTbatikFTOHBMemCI}		& \vci{\SLOWbatikDCExcMem}{\SLOWbatikDCExcMemCI}	& \vci{\SLOWbatikDCnoGExcMem}{\SLOWbatikDCnoGExcMemCI}		& \vci{\SLOWbatikCAPOExcMem}{\SLOWbatikCAPOExcMemCI}	& \vci{\SLOWbatikCAPOnoGExcMem}{\SLOWbatikCAPOnoGExcMemCI} \\
\bench{h2} 		& \et{\FASThtwoEvents}{\FASThtwoEventsCI}     & \enfp{\FASThtwoNoFPEvents}{\FASThtwoNoFPEventsCI}	    & \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & \baseMem{\FASThtwoBaseMem}     & \vci{\FASThtwoFTMem}{\FASThtwoFTMemCI}     & \vci{\FASThtwoHBMem}{\FASThtwoHBMemCI}    	& \vci{\FASThtwoFTOHBMem}{\FASThtwoFTOHBMemCI}		& \vci{\SLOWhtwoDCExcMem}{\SLOWhtwoDCExcMemCI}		& \vci{\SLOWhtwoDCnoGExcMem}{\SLOWhtwoDCnoGExcMemCI}		& \vci{\SLOWhtwoCAPOExcMem}{\SLOWhtwoCAPOExcMemCI}	& \vci{\SLOWhtwoCAPOnoGExcMem}{\SLOWhtwoCAPOnoGExcMemCI}\\
\bench{jython} 	& \et{\FASTjythonEvents}{\FASTjythonEventsCI}   & \enfp{\FASTjythonNoFPEvents}{\FASTjythonNoFPEventsCI}	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& \baseMem{\FASTjythonBaseMem}   & \vci{\FASTjythonFTMem}{\FASTjythonFTMemCI}   & \vci{\FASTjythonHBMem}{\FASTjythonHBMemCI} 	& \vci{\FASTjythonFTOHBMem}{\FASTjythonFTOHBMemCI}	& \vci{\SLOWjythonDCExcMem}{\SLOWjythonDCExcMemCI}	& \vci{\SLOWjythonDCnoGExcMem}{\SLOWjythonDCnoGExcMemCI}	& \vci{\SLOWjythonCAPOExcMem}{\SLOWjythonCAPOExcMemCI}	& \vci{\SLOWjythonCAPOnoGExcMem}{\SLOWjythonCAPOnoGExcMemCI} \\
\bench{luindex} & \et{\FASTluindexEvents}{\FASTluindexEventsCI}  & \enfp{\FASTluindexNoFPEvents}{\FASTluindexNoFPEventsCI}	& \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& \baseMem{\FASTluindexBaseMem}  & \vci{\FASTluindexFTMem}{\FASTluindexFTMemCI}  & \vci{\FASTluindexHBMem}{\FASTluindexHBMemCI} 	& \vci{\FASTluindexFTOHBMem}{\FASTluindexFTOHBMemCI}	& \vci{\SLOWluindexDCExcMem}{\SLOWluindexDCExcMemCI}	& \vci{\SLOWluindexDCnoGExcMem}{\SLOWluindexDCnoGExcMemCI}	& \vci{\SLOWluindexCAPOExcMem}{\SLOWluindexCAPOExcMemCI}	& \vci{\SLOWluindexCAPOnoGExcMem}{\SLOWluindexCAPOnoGExcMemCI} \\
\bench{lusearch}& \et{\FASTlusearchEvents}{\FASTlusearchEventsCI} & \enfp{\FASTlusearchNoFPEvents}{\FASTlusearchNoFPEventsCI}	& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& \baseMem{\FASTlusearchBaseMem} & \vci{\FASTlusearchFTMem}{\FASTlusearchFTMemCI} & \vci{\FASTlusearchHBMem}{\FASTlusearchHBMemCI}	& \vci{\FASTlusearchFTOHBMem}{\FASTlusearchFTOHBMemCI}	& \vci{\SLOWlusearchDCExcMem}{\SLOWlusearchDCExcMemCI}	& \vci{\SLOWlusearchDCnoGExcMem}{\SLOWlusearchDCnoGExcMemCI}	& \vci{\SLOWlusearchCAPOExcMem}{\SLOWlusearchCAPOExcMemCI}& \vci{\SLOWlusearchCAPOnoGExcMem}{\SLOWlusearchCAPOnoGExcMemCI} \\
\bench{pmd}		& \et{\FASTpmdEvents}{\FASTpmdEventsCI}      & \enfp{\FASTpmdNoFPEvents}{\FASTpmdNoFPEventsCI}      & \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & \baseMem{\FASTpmdBaseMem}      & \vci{\FASTpmdFTMem}{\FASTpmdFTMemCI}      & \vci{\FASTpmdHBMem}{\FASTpmdHBMemCI}		& \vci{\FASTpmdFTOHBMem}{\FASTpmdFTOHBMemCI}		& \vci{\SLOWpmdDCExcMem}{\SLOWpmdDCExcMemCI}		& \vci{\SLOWpmdDCnoGExcMem}{\SLOWpmdDCnoGExcMemCI}		& \vci{\SLOWpmdCAPOExcMem}{\SLOWpmdCAPOExcMemCI}		& \vci{\SLOWpmdCAPOnoGExcMem}{\SLOWpmdCAPOnoGExcMemCI} \\
\bench{sunflow} & \et{\FASTsunflowEvents}{\FASTsunflowEventsCI}  & \enfp{\FASTsunflowNoFPEvents}{\FASTsunflowNoFPEventsCI}	& \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& \baseMem{\FASTsunflowBaseMem}  & \vci{\FASTsunflowFTMem}{\FASTsunflowFTMemCI}  & \vci{\FASTsunflowHBMem}{\FASTsunflowHBMemCI}	& \vci{\FASTsunflowFTOHBMem}{\FASTsunflowFTOHBMemCI}	& \vci{\SLOWsunflowDCExcMem}{\SLOWsunflowDCExcMemCI}	& \vci{\SLOWsunflowDCnoGExcMem}{\SLOWsunflowDCnoGExcMemCI}	& \vci{\SLOWsunflowCAPOExcMem}{\SLOWsunflowCAPOExcMemCI}	& \vci{\SLOWsunflowCAPOnoGExcMem}{\SLOWsunflowCAPOnoGExcMemCI} \\
\bench{tomcat} 	& \et{\FASTtomcatEvents}{\FASTtomcatEventsCI}   & \enfp{\FASTtomcatNoFPEvents}{\FASTtomcatNoFPEventsCI}	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& \baseMem{\FASTtomcatBaseMem}   & \vci{\FASTtomcatFTMem}{\FASTtomcatFTMemCI}   & \vci{\FASTtomcatHBMem}{\FASTtomcatHBMemCI} 	& \vci{\FASTtomcatFTOHBMem}{\FASTtomcatFTOHBMemCI}	& \vci{\SLOWtomcatDCExcMem}{\SLOWtomcatDCExcMemCI}	& \vci{\SLOWtomcatDCnoGExcMem}{\SLOWtomcatDCnoGExcMemCI}	& \vci{\SLOWtomcatCAPOExcMem}{\SLOWtomcatCAPOExcMemCI}	& \vci{\SLOWtomcatCAPOnoGExcMem}{\SLOWtomcatCAPOnoGExcMemCI} \\
\bench{xalan} 	& \et{\FASTxalanEvents}{\FASTxalanEventsCI}    & \enfp{\FASTxalanNoFPEvents}{\FASTxalanNoFPEventsCI}	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& \baseMem{\FASTxalanBaseMem}    & \vci{\FASTxalanFTMem}{\FASTxalanFTMemCI}    & \vci{\FASTxalanHBMem}{\FASTxalanHBMemCI}		& \vci{\FASTxalanFTOHBMem}{\FASTxalanFTOHBMemCI}		& \vci{\SLOWxalanDCExcMem}{\SLOWxalanDCExcMemCI}	& \vci{\SLOWxalanDCnoGExcMem}{\SLOWxalanDCnoGExcMemCI} 	& \vci{\SLOWxalanCAPOExcMem}{\SLOWxalanCAPOExcMemCI}	& \vci{\SLOWxalanCAPOnoGExcMem}{\SLOWxalanCAPOnoGExcMemCI}\\\hline
geomean	& &	& &	& & \mem{\FASTFTMemGeoMean} & \mem{\FASTHBMemGeoMean} & \mem{\FASTFTOHBMemGeoMean} & \mem{\SLOWDCExcMemGeoMean} & \mem{\SLOWDCnoGExcMemGeoMean} & \mem{\SLOWCAPOExcMemGeoMean} & \mem{\SLOWCAPOnoGExcMemGeoMean} \\
\mc{13}{c}{Memory usage} \\
\end{tabular}

\caption{Memory usage for various FastTrack-based \HB analyses
and for unoptimized \DC and \CAPO analyses, relative to uninstrumented
execution, with 95\% confidence intervals.}
\label{tab:performance:fasttrack:memoryCI}
\end{table*}


\begin{table*}[t]
\begin{empty}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
% \input{result-macros/PIP_slowTool_AllConfig_memChange}
\input{result-macros/PIP_slowTool_raceEdgeFix}
\input{result-macros/PIP_fastTool_readExclFix_Quite}
%
\smaller
\centering
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWavroraHBTime}{\SLOWavroraHBTimeCI}			& \vci{\FASTavroraFTOHBTime}{\FASTavroraFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWavroraWCPTime}{\SLOWavroraWCPTimeCI}			& \vci{\FASTavroraFTOWCPTime}{\FASTavroraFTOWCPTimeCI}	& \vci{\FASTavroraREWCPTime}{\FASTavroraREWCPTimeCI} \\
\DC		& \vci{\SLOWavroraDCExcTime}{\SLOWavroraDCExcTimeCI}	& \vci{\SLOWavroraDCnoGExcTime}{\SLOWavroraDCnoGExcTimeCI}	& \vci{\FASTavroraFTODCTime}{\FASTavroraFTODCTimeCI}	& \vci{\FASTavroraREDCTime}{\FASTavroraREDCTimeCI} \\
\CAPO	& \vci{\SLOWavroraCAPOExcTime}{\SLOWavroraCAPOExcTimeCI}	& \vci{\SLOWavroraCAPOnoGExcTime}{\SLOWavroraCAPOnoGExcTimeCI}	& \vci{\FASTavroraFTOCAPOTime}{\FASTavroraFTOCAPOTimeCI}	& \vci{\FASTavroraRECAPOTime}{\FASTavroraRECAPOTimeCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWbatikHBTime}{\SLOWbatikHBTimeCI}			& \vci{\FASTbatikFTOHBTime}{\FASTbatikFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWbatikWCPTime}{\SLOWbatikWCPTimeCI}			& \vci{\FASTbatikFTOWCPTime}{\FASTbatikFTOWCPTimeCI}	& \vci{\FASTbatikREWCPTime}{\FASTbatikREWCPTimeCI} \\
\DC		& \vci{\SLOWbatikDCExcTime}{\SLOWbatikDCExcTimeCI}	& \vci{\SLOWbatikDCnoGExcTime}{\SLOWbatikDCnoGExcTimeCI}	& \vci{\FASTbatikFTODCTime}{\FASTbatikFTODCTimeCI}	& \vci{\FASTbatikREDCTime}{\FASTbatikREDCTimeCI} \\
\CAPO	& \vci{\SLOWbatikCAPOExcTime}{\SLOWbatikCAPOExcTimeCI}	& \vci{\SLOWbatikCAPOnoGExcTime}{\SLOWbatikCAPOnoGExcTimeCI}	& \vci{\FASTbatikFTOCAPOTime}{\FASTbatikFTOCAPOTimeCI}	& \vci{\FASTbatikRECAPOTime}{\FASTbatikRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{batik}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWhtwoHBTime}{\SLOWhtwoHBTimeCI}			& \vci{\FASThtwoFTOHBTime}{\FASThtwoFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWhtwoWCPTime}{\SLOWhtwoWCPTimeCI}			& \vci{\FASThtwoFTOWCPTime}{\FASThtwoFTOWCPTimeCI}	& \vci{\FASThtwoREWCPTime}{\FASThtwoREWCPTimeCI} \\
\DC		& \vci{\SLOWhtwoDCExcTime}{\SLOWhtwoDCExcTimeCI}	& \vci{\SLOWhtwoDCnoGExcTime}{\SLOWhtwoDCnoGExcTimeCI}	& \vci{\FASThtwoFTODCTime}{\FASThtwoFTODCTimeCI}	& \vci{\FASThtwoREDCTime}{\FASThtwoREDCTimeCI} \\
\CAPO	& \vci{\SLOWhtwoCAPOExcTime}{\SLOWhtwoCAPOExcTimeCI}	& \vci{\SLOWhtwoCAPOnoGExcTime}{\SLOWhtwoCAPOnoGExcTimeCI}	& \vci{\FASThtwoFTOCAPOTime}{\FASThtwoFTOCAPOTimeCI}	& \vci{\FASThtwoRECAPOTime}{\FASThtwoRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWjythonHBTime}{\SLOWjythonHBTimeCI}			& \vci{\FASTjythonFTOHBTime}{\FASTjythonFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWjythonWCPTime}{\SLOWjythonWCPTimeCI}			& \vci{\FASTjythonFTOWCPTime}{\FASTjythonFTOWCPTimeCI}	& \vci{\FASTjythonREWCPTime}{\FASTjythonREWCPTimeCI} \\
\DC		& \vci{\SLOWjythonDCExcTime}{\SLOWjythonDCExcTimeCI}	& \vci{\SLOWjythonDCnoGExcTime}{\SLOWjythonDCnoGExcTimeCI}	& \vci{\FASTjythonFTODCTime}{\FASTjythonFTODCTimeCI}	& \vci{\FASTjythonREDCTime}{\FASTjythonREDCTimeCI} \\
\CAPO	& \vci{\SLOWjythonCAPOExcTime}{\SLOWjythonCAPOExcTimeCI}	& \vci{\SLOWjythonCAPOnoGExcTime}{\SLOWjythonCAPOnoGExcTimeCI}	& \vci{\FASTjythonFTOCAPOTime}{\FASTjythonFTOCAPOTimeCI}	& \vci{\FASTjythonRECAPOTime}{\FASTjythonRECAPOTimeCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWluindexHBTime}{\SLOWluindexHBTimeCI}			& \vci{\FASTluindexFTOHBTime}{\FASTluindexFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWluindexWCPTime}{\SLOWluindexWCPTimeCI}			& \vci{\FASTluindexFTOWCPTime}{\FASTluindexFTOWCPTimeCI}	& \vci{\FASTluindexREWCPTime}{\FASTluindexREWCPTimeCI} \\
\DC		& \vci{\SLOWluindexDCExcTime}{\SLOWluindexDCExcTimeCI}	& \vci{\SLOWluindexDCnoGExcTime}{\SLOWluindexDCnoGExcTimeCI}	& \vci{\FASTluindexFTODCTime}{\FASTluindexFTODCTimeCI}	& \vci{\FASTluindexREDCTime}{\FASTluindexREDCTimeCI} \\
\CAPO	& \vci{\SLOWluindexCAPOExcTime}{\SLOWluindexCAPOExcTimeCI}	& \vci{\SLOWluindexCAPOnoGExcTime}{\SLOWluindexCAPOnoGExcTimeCI}	& \vci{\FASTluindexFTOCAPOTime}{\FASTluindexFTOCAPOTimeCI}	& \vci{\FASTluindexRECAPOTime}{\FASTluindexRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWlusearchHBTime}{\SLOWlusearchHBTimeCI}			& \vci{\FASTlusearchFTOHBTime}{\FASTlusearchFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWlusearchWCPTime}{\SLOWlusearchWCPTimeCI}			& \vci{\FASTlusearchFTOWCPTime}{\FASTlusearchFTOWCPTimeCI}	& \vci{\FASTlusearchREWCPTime}{\FASTlusearchREWCPTimeCI} \\
\DC		& \vci{\SLOWlusearchDCExcTime}{\SLOWlusearchDCExcTimeCI}	& \vci{\SLOWlusearchDCnoGExcTime}{\SLOWlusearchDCnoGExcTimeCI}	& \vci{\FASTlusearchFTODCTime}{\FASTlusearchFTODCTimeCI}	& \vci{\FASTlusearchREDCTime}{\FASTlusearchREDCTimeCI} \\
\CAPO	& \vci{\SLOWlusearchCAPOExcTime}{\SLOWlusearchCAPOExcTimeCI}	& \vci{\SLOWlusearchCAPOnoGExcTime}{\SLOWlusearchCAPOnoGExcTimeCI}	& \vci{\FASTlusearchFTOCAPOTime}{\FASTlusearchFTOCAPOTimeCI}	& \vci{\FASTlusearchRECAPOTime}{\FASTlusearchRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{lusearch}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWpmdHBTime}{\SLOWpmdHBTimeCI}			& \vci{\FASTpmdFTOHBTime}{\FASTpmdFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWpmdWCPTime}{\SLOWpmdWCPTimeCI}			& \vci{\FASTpmdFTOWCPTime}{\FASTpmdFTOWCPTimeCI}	& \vci{\FASTpmdREWCPTime}{\FASTpmdREWCPTimeCI} \\
\DC		& \vci{\SLOWpmdDCExcTime}{\SLOWpmdDCExcTimeCI}	& \vci{\SLOWpmdDCnoGExcTime}{\SLOWpmdDCnoGExcTimeCI}	& \vci{\FASTpmdFTODCTime}{\FASTpmdFTODCTimeCI}	& \vci{\FASTpmdREDCTime}{\FASTpmdREDCTimeCI} \\
\CAPO	& \vci{\SLOWpmdCAPOExcTime}{\SLOWpmdCAPOExcTimeCI}	& \vci{\SLOWpmdCAPOnoGExcTime}{\SLOWpmdCAPOnoGExcTimeCI}	& \vci{\FASTpmdFTOCAPOTime}{\FASTpmdFTOCAPOTimeCI}	& \vci{\FASTpmdRECAPOTime}{\FASTpmdRECAPOTimeCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWsunflowHBTime}{\SLOWsunflowHBTimeCI}			& \vci{\FASTsunflowFTOHBTime}{\FASTsunflowFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWsunflowWCPTime}{\SLOWsunflowWCPTimeCI}			& \vci{\FASTsunflowFTOWCPTime}{\FASTsunflowFTOWCPTimeCI}	& \vci{\FASTsunflowREWCPTime}{\FASTsunflowREWCPTimeCI} \\
\DC		& \vci{\SLOWsunflowDCExcTime}{\SLOWsunflowDCExcTimeCI}	& \vci{\SLOWsunflowDCnoGExcTime}{\SLOWsunflowDCnoGExcTimeCI}	& \vci{\FASTsunflowFTODCTime}{\FASTsunflowFTODCTimeCI}	& \vci{\FASTsunflowREDCTime}{\FASTsunflowREDCTimeCI} \\
\CAPO	& \vci{\SLOWsunflowCAPOExcTime}{\SLOWsunflowCAPOExcTimeCI}	& \vci{\SLOWsunflowCAPOnoGExcTime}{\SLOWsunflowCAPOnoGExcTimeCI}	& \vci{\FASTsunflowFTOCAPOTime}{\FASTsunflowFTOCAPOTimeCI}	& \vci{\FASTsunflowRECAPOTime}{\FASTsunflowRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWtomcatHBTime}{\SLOWtomcatHBTimeCI}			& \vci{\FASTtomcatFTOHBTime}{\FASTtomcatFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWtomcatWCPTime}{\SLOWtomcatWCPTimeCI}			& \vci{\FASTtomcatFTOWCPTime}{\FASTtomcatFTOWCPTimeCI}	& \vci{\FASTtomcatREWCPTime}{\FASTtomcatREWCPTimeCI} \\
\DC		& \vci{\SLOWtomcatDCExcTime}{\SLOWtomcatDCExcTimeCI}	& \vci{\SLOWtomcatDCnoGExcTime}{\SLOWtomcatDCnoGExcTimeCI}	& \vci{\FASTtomcatFTODCTime}{\FASTtomcatFTODCTimeCI}	& \vci{\FASTtomcatREDCTime}{\FASTtomcatREDCTimeCI} \\
\CAPO	& \vci{\SLOWtomcatCAPOExcTime}{\SLOWtomcatCAPOExcTimeCI}	& \vci{\SLOWtomcatCAPOnoGExcTime}{\SLOWtomcatCAPOnoGExcTimeCI}	& \vci{\FASTtomcatFTOCAPOTime}{\FASTtomcatFTOCAPOTimeCI}	& \vci{\FASTtomcatRECAPOTime}{\FASTtomcatRECAPOTimeCI} \\
		& \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \vci{\SLOWxalanHBTime}{\SLOWxalanHBTimeCI}			& \vci{\FASTxalanFTOHBTime}{\FASTxalanFTOHBTimeCI}	& \rna \\
\WCP	& \rna							& \vci{\SLOWxalanWCPTime}{\SLOWxalanWCPTimeCI}			& \vci{\FASTxalanFTOWCPTime}{\FASTxalanFTOWCPTimeCI}	& \vci{\FASTxalanREWCPTime}{\FASTxalanREWCPTimeCI} \\
\DC		& \vci{\SLOWxalanDCExcTime}{\SLOWxalanDCExcTimeCI}	& \vci{\SLOWxalanDCnoGExcTime}{\SLOWxalanDCnoGExcTimeCI}	& \vci{\FASTxalanFTODCTime}{\FASTxalanFTODCTimeCI}	& \vci{\FASTxalanREDCTime}{\FASTxalanREDCTimeCI} \\
\CAPO	& \vci{\SLOWxalanCAPOExcTime}{\SLOWxalanCAPOExcTimeCI}	& \vci{\SLOWxalanCAPOnoGExcTime}{\SLOWxalanCAPOnoGExcTimeCI}	& \vci{\FASTxalanFTOCAPOTime}{\FASTxalanFTOCAPOTimeCI}	& \vci{\FASTxalanRECAPOTime}{\FASTxalanRECAPOTimeCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\end{empty}
\caption{Run time, relative to uninstrumented execution, of various analyses for each evaluated program
with 95\% confidence intervals.}
\label{tab:performance:allDaCapo:CI}
% \end{table*}
% Table for 10 trials of all relations with various optimizations for all DaCapo benchmarks
% \begin{table*}[t]
\begin{empty}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
%memory \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$Gb$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
% \input{result-macros/PIP_slowTool_AllConfig_memChange}
\input{result-macros/PIP_slowTool_raceEdgeFix}
\input{result-macros/PIP_fastTool_readExclFix_Quite}
%
\smaller
\centering
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWavroraHBMem}{\SLOWavroraHBMemCI}		& \vci{\FASTavroraFTOHBMem}{\FASTavroraFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWavroraWCPMem}{\SLOWavroraWCPMemCI}		& \vci{\FASTavroraFTOWCPMem}{\FASTavroraFTOWCPMemCI}	& \vci{\FASTavroraREWCPMem}{\FASTavroraREWCPMemCI} \\
\DC		& \vci{\SLOWavroraDCExcMem}{\SLOWavroraDCExcMemCI}	& \vci{\SLOWavroraDCnoGExcMem}{\SLOWavroraDCnoGExcMemCI}	& \vci{\FASTavroraFTODCMem}{\FASTavroraFTODCMemCI}		& \vci{\FASTavroraREDCMem}{\FASTavroraREDCMemCI} \\
\CAPO	& \vci{\SLOWavroraCAPOExcMem}{\SLOWavroraCAPOExcMemCI}	& \vci{\SLOWavroraCAPOnoGExcMem}{\SLOWavroraCAPOnoGExcMemCI}& \vci{\FASTavroraFTOCAPOMem}{\FASTavroraFTOCAPOMemCI}	& \vci{\FASTavroraRECAPOMem}{\FASTavroraRECAPOMemCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWbatikHBMem}{\SLOWbatikHBMemCI}		& \vci{\FASTbatikFTOHBMem}{\FASTbatikFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWbatikWCPMem}{\SLOWbatikWCPMemCI}		& \vci{\FASTbatikFTOWCPMem}{\FASTbatikFTOWCPMemCI}	& \vci{\FASTbatikREWCPMem}{\FASTbatikREWCPMemCI} \\
\DC		& \vci{\SLOWbatikDCExcMem}{\SLOWbatikDCExcMemCI}	& \vci{\SLOWbatikDCnoGExcMem}{\SLOWbatikDCnoGExcMemCI}	& \vci{\FASTbatikFTODCMem}{\FASTbatikFTODCMemCI}		& \vci{\FASTbatikREDCMem}{\FASTbatikREDCMemCI} \\
\CAPO	& \vci{\SLOWbatikCAPOExcMem}{\SLOWbatikCAPOExcMemCI}	& \vci{\SLOWbatikCAPOnoGExcMem}{\SLOWbatikCAPOnoGExcMemCI}& \vci{\FASTbatikFTOCAPOMem}{\FASTbatikFTOCAPOMemCI}	& \vci{\FASTbatikRECAPOMem}{\FASTbatikRECAPOMemCI} \\
		& \mc{4}{c}{\bench{batik}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWhtwoHBMem}{\SLOWhtwoHBMemCI}		& \vci{\FASThtwoFTOHBMem}{\FASThtwoFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWhtwoWCPMem}{\SLOWhtwoWCPMemCI}		& \vci{\FASThtwoFTOWCPMem}{\FASThtwoFTOWCPMemCI}	& \vci{\FASThtwoREWCPMem}{\FASThtwoREWCPMemCI} \\
\DC		& \vci{\SLOWhtwoDCExcMem}{\SLOWhtwoDCExcMemCI}	& \vci{\SLOWhtwoDCnoGExcMem}{\SLOWhtwoDCnoGExcMemCI}	& \vci{\FASThtwoFTODCMem}{\FASThtwoFTODCMemCI}		& \vci{\FASThtwoREDCMem}{\FASThtwoREDCMemCI} \\
\CAPO	& \vci{\SLOWhtwoCAPOExcMem}{\SLOWhtwoCAPOExcMemCI}	& \vci{\SLOWhtwoCAPOnoGExcMem}{\SLOWhtwoCAPOnoGExcMemCI}& \vci{\FASThtwoFTOCAPOMem}{\FASThtwoFTOCAPOMemCI}	& \vci{\FASThtwoRECAPOMem}{\FASThtwoRECAPOMemCI} \\
		& \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWjythonHBMem}{\SLOWjythonHBMemCI}		& \vci{\FASTjythonFTOHBMem}{\FASTjythonFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWjythonWCPMem}{\SLOWjythonWCPMemCI}		& \vci{\FASTjythonFTOWCPMem}{\FASTjythonFTOWCPMemCI}	& \vci{\FASTjythonREWCPMem}{\FASTjythonREWCPMemCI} \\
\DC		& \vci{\SLOWjythonDCExcMem}{\SLOWjythonDCExcMemCI}	& \vci{\SLOWjythonDCnoGExcMem}{\SLOWjythonDCnoGExcMemCI}	& \vci{\FASTjythonFTODCMem}{\FASTjythonFTODCMemCI}		& \vci{\FASTjythonREDCMem}{\FASTjythonREDCMemCI} \\
\CAPO	& \vci{\SLOWjythonCAPOExcMem}{\SLOWjythonCAPOExcMemCI}	& \vci{\SLOWjythonCAPOnoGExcMem}{\SLOWjythonCAPOnoGExcMemCI}& \vci{\FASTjythonFTOCAPOMem}{\FASTjythonFTOCAPOMemCI}	& \vci{\FASTjythonRECAPOMem}{\FASTjythonRECAPOMemCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWluindexHBMem}{\SLOWluindexHBMemCI}		& \vci{\FASTluindexFTOHBMem}{\FASTluindexFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWluindexWCPMem}{\SLOWluindexWCPMemCI}		& \vci{\FASTluindexFTOWCPMem}{\FASTluindexFTOWCPMemCI}	& \vci{\FASTluindexREWCPMem}{\FASTluindexREWCPMemCI} \\
\DC		& \vci{\SLOWluindexDCExcMem}{\SLOWluindexDCExcMemCI}	& \vci{\SLOWluindexDCnoGExcMem}{\SLOWluindexDCnoGExcMemCI}	& \vci{\FASTluindexFTODCMem}{\FASTluindexFTODCMemCI}		& \vci{\FASTluindexREDCMem}{\FASTluindexREDCMemCI} \\
\CAPO	& \vci{\SLOWluindexCAPOExcMem}{\SLOWluindexCAPOExcMemCI}	& \vci{\SLOWluindexCAPOnoGExcMem}{\SLOWluindexCAPOnoGExcMemCI}& \vci{\FASTluindexFTOCAPOMem}{\FASTluindexFTOCAPOMemCI}	& \vci{\FASTluindexRECAPOMem}{\FASTluindexRECAPOMemCI} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWlusearchHBMem}{\SLOWlusearchHBMemCI}		& \vci{\FASTlusearchFTOHBMem}{\FASTlusearchFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWlusearchWCPMem}{\SLOWlusearchWCPMemCI}		& \vci{\FASTlusearchFTOWCPMem}{\FASTlusearchFTOWCPMemCI}	& \vci{\FASTlusearchREWCPMem}{\FASTlusearchREWCPMemCI} \\
\DC		& \vci{\SLOWlusearchDCExcMem}{\SLOWlusearchDCExcMemCI}	& \vci{\SLOWlusearchDCnoGExcMem}{\SLOWlusearchDCnoGExcMemCI}	& \vci{\FASTlusearchFTODCMem}{\FASTlusearchFTODCMemCI}		& \vci{\FASTlusearchREDCMem}{\FASTlusearchREDCMemCI} \\
\CAPO	& \vci{\SLOWlusearchCAPOExcMem}{\SLOWlusearchCAPOExcMemCI}	& \vci{\SLOWlusearchCAPOnoGExcMem}{\SLOWlusearchCAPOnoGExcMemCI}& \vci{\FASTlusearchFTOCAPOMem}{\FASTlusearchFTOCAPOMemCI}	& \vci{\FASTlusearchRECAPOMem}{\FASTlusearchRECAPOMemCI} \\
		& \mc{4}{c}{\bench{lusearch}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWpmdHBMem}{\SLOWpmdHBMemCI}		& \vci{\FASTpmdFTOHBMem}{\FASTpmdFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWpmdWCPMem}{\SLOWpmdWCPMemCI}		& \vci{\FASTpmdFTOWCPMem}{\FASTpmdFTOWCPMemCI}	& \vci{\FASTpmdREWCPMem}{\FASTpmdREWCPMemCI} \\
\DC		& \vci{\SLOWpmdDCExcMem}{\SLOWpmdDCExcMemCI}	& \vci{\SLOWpmdDCnoGExcMem}{\SLOWpmdDCnoGExcMemCI}	& \vci{\FASTpmdFTODCMem}{\FASTpmdFTODCMemCI}		& \vci{\FASTpmdREDCMem}{\FASTpmdREDCMemCI} \\
\CAPO	& \vci{\SLOWpmdCAPOExcMem}{\SLOWpmdCAPOExcMemCI}	& \vci{\SLOWpmdCAPOnoGExcMem}{\SLOWpmdCAPOnoGExcMemCI}& \vci{\FASTpmdFTOCAPOMem}{\FASTpmdFTOCAPOMemCI}	& \vci{\FASTpmdRECAPOMem}{\FASTpmdRECAPOMemCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWsunflowHBMem}{\SLOWsunflowHBMemCI}		& \vci{\FASTsunflowFTOHBMem}{\FASTsunflowFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWsunflowWCPMem}{\SLOWsunflowWCPMemCI}		& \vci{\FASTsunflowFTOWCPMem}{\FASTsunflowFTOWCPMemCI}	& \vci{\FASTsunflowREWCPMem}{\FASTsunflowREWCPMemCI} \\
\DC		& \vci{\SLOWsunflowDCExcMem}{\SLOWsunflowDCExcMemCI}	& \vci{\SLOWsunflowDCnoGExcMem}{\SLOWsunflowDCnoGExcMemCI}	& \vci{\FASTsunflowFTODCMem}{\FASTsunflowFTODCMemCI}		& \vci{\FASTsunflowREDCMem}{\FASTsunflowREDCMemCI} \\
\CAPO	& \vci{\SLOWsunflowCAPOExcMem}{\SLOWsunflowCAPOExcMemCI}	& \vci{\SLOWsunflowCAPOnoGExcMem}{\SLOWsunflowCAPOnoGExcMemCI}& \vci{\FASTsunflowFTOCAPOMem}{\FASTsunflowFTOCAPOMemCI}	& \vci{\FASTsunflowRECAPOMem}{\FASTsunflowRECAPOMemCI} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWtomcatHBMem}{\SLOWtomcatHBMemCI}		& \vci{\FASTtomcatFTOHBMem}{\FASTtomcatFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWtomcatWCPMem}{\SLOWtomcatWCPMemCI}		& \vci{\FASTtomcatFTOWCPMem}{\FASTtomcatFTOWCPMemCI}	& \vci{\FASTtomcatREWCPMem}{\FASTtomcatREWCPMemCI} \\
\DC		& \vci{\SLOWtomcatDCExcMem}{\SLOWtomcatDCExcMemCI}	& \vci{\SLOWtomcatDCnoGExcMem}{\SLOWtomcatDCnoGExcMemCI}	& \vci{\FASTtomcatFTODCMem}{\FASTtomcatFTODCMemCI}		& \vci{\FASTtomcatREDCMem}{\FASTtomcatREDCMemCI} \\
\CAPO	& \vci{\SLOWtomcatCAPOExcMem}{\SLOWtomcatCAPOExcMemCI}	& \vci{\SLOWtomcatCAPOnoGExcMem}{\SLOWtomcatCAPOnoGExcMemCI}& \vci{\FASTtomcatFTOCAPOMem}{\FASTtomcatFTOCAPOMemCI}	& \vci{\FASTtomcatRECAPOMem}{\FASTtomcatRECAPOMemCI} \\
		& \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
		& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \vci{\SLOWxalanHBMem}{\SLOWxalanHBMemCI}		& \vci{\FASTxalanFTOHBMem}{\FASTxalanFTOHBMemCI}		& \rna \\
\WCP	& \rna							& \vci{\SLOWxalanWCPMem}{\SLOWxalanWCPMemCI}		& \vci{\FASTxalanFTOWCPMem}{\FASTxalanFTOWCPMemCI}	& \vci{\FASTxalanREWCPMem}{\FASTxalanREWCPMemCI} \\
\DC		& \vci{\SLOWxalanDCExcMem}{\SLOWxalanDCExcMemCI}	& \vci{\SLOWxalanDCnoGExcMem}{\SLOWxalanDCnoGExcMemCI}	& \vci{\FASTxalanFTODCMem}{\FASTxalanFTODCMemCI}		& \vci{\FASTxalanREDCMem}{\FASTxalanREDCMemCI} \\
\CAPO	& \vci{\SLOWxalanCAPOExcMem}{\SLOWxalanCAPOExcMemCI}	& \vci{\SLOWxalanCAPOnoGExcMem}{\SLOWxalanCAPOnoGExcMemCI}& \vci{\FASTxalanFTOCAPOMem}{\FASTxalanFTOCAPOMemCI}	& \vci{\FASTxalanRECAPOMem}{\FASTxalanRECAPOMemCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\end{empty}
\caption{Memory usage, relative to uninstrumented execution, of various analyses for each evaluated program
with 95\% confidence intervals.}
\label{tab:memory:allDaCapo:CI}
\end{table*}

\begin{table*}[t]
% \begin{adjustwidth}{-1.5cm}{}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
% \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;Mb$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\sdr}[4]{\vci{#1}{#2}{\;}(\vci{#3}{#4})}
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}#1}
% \input{result-macros/PIP_slowTool_AllConfig_memChange}
\input{result-macros/PIP_slowTool_raceEdgeFix}
\input{result-macros/PIP_fastTool_readExclFix_Quite}
%
\smaller
\centering
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWavroraHB}{\SLOWavroraHBCI}{\SLOWavroraHBDynamic}{\SLOWavroraHBDynamicCI}					& \sdr{\FASTavroraFTOHB}{\FASTavroraFTOHBCI}{\FASTavroraFTOHBDynamic}{\FASTavroraFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWavroraWCP}{\SLOWavroraWCPCI}{\SLOWavroraWCPDynamic}{\SLOWavroraWCPDynamicCI}				& \sdr{\FASTavroraFTOWCP}{\FASTavroraFTOWCPCI}{\FASTavroraFTOWCPDynamic}{\FASTavroraFTOWCPDynamicCI}		& \sdr{\FASTavroraREWCP}{\FASTavroraREWCPCI}{\FASTavroraREWCPDynamic}{\FASTavroraREWCPDynamicCI} \\
\DC		& \sdr{\SLOWavroraDCExc}{\SLOWavroraDCExcCI}{\SLOWavroraDCExcDynamic}{\SLOWavroraDCExcDynamicCI}		& \sdr{\SLOWavroraDCnoGExc}{\SLOWavroraDCnoGExcCI}{\SLOWavroraDCnoGExcDynamic}{\SLOWavroraDCnoGExcDynamicCI}	& \sdr{\FASTavroraFTODC}{\FASTavroraFTODCCI}{\FASTavroraFTODCDynamic}{\FASTavroraFTODCDynamicCI}		& \sdr{\FASTavroraREDC}{\FASTavroraREDCCI}{\FASTavroraREDCDynamic}{\FASTavroraREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWavroraCAPOExc}{\SLOWavroraCAPOExcCI}{\SLOWavroraCAPOExcDynamic}{\SLOWavroraCAPOExcDynamicCI}	& \sdr{\SLOWavroraCAPOnoGExc}{\SLOWavroraCAPOnoGExcCI}{\SLOWavroraCAPOnoGExcDynamic}{\SLOWavroraCAPOnoGExcDynamicCI}	& \sdr{\FASTavroraFTOCAPO}{\FASTavroraFTOCAPOCI}{\FASTavroraFTOCAPODynamic}{\FASTavroraFTOCAPODynamicCI}	& \sdr{\FASTavroraRECAPO}{\FASTavroraRECAPOCI}{\FASTavroraRECAPODynamic}{\FASTavroraRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\medskip\\
% \begin{tabular}{@{}HHlll@{}}
%         & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
% \HB		& \rna													& \sdr{\SLOWbatikHB}{\SLOWbatikHBCI}{\SLOWbatikHBDynamic}{\SLOWbatikHBDynamicCI}					& \sdr{\FASTbatikFTOHB}{\FASTbatikFTOHBCI}{\FASTbatikFTOHBDynamic}{\FASTbatikFTOHBDynamicCI}		& \rna \\
% \WCP	& \rna													& \sdr{\SLOWbatikWCP}{\SLOWbatikWCPCI}{\SLOWbatikWCPDynamic}{\SLOWbatikWCPDynamicCI}				& \sdr{\FASTbatikFTOWCP}{\FASTbatikFTOWCPCI}{\FASTbatikFTOWCPDynamic}{\FASTbatikFTOWCPDynamicCI}		& \sdr{\FASTbatikREWCP}{\FASTbatikREWCPCI}{\FASTbatikREWCPDynamic}{\FASTbatikREWCPDynamicCI} \\
% \DC		& \sdr{\SLOWbatikDCExc}{\SLOWbatikDCExcCI}{\SLOWbatikDCExcDynamic}{\SLOWbatikDCExcDynamicCI}		& \sdr{\SLOWbatikDCnoGExc}{\SLOWbatikDCnoGExcCI}{\SLOWbatikDCnoGExcDynamic}{\SLOWbatikDCnoGExcDynamicCI}	& \sdr{\FASTbatikFTODC}{\FASTbatikFTODCCI}{\FASTbatikFTODCDynamic}{\FASTbatikFTODCDynamicCI}		& \sdr{\FASTbatikREDC}{\FASTbatikREDCCI}{\FASTbatikREDCDynamic}{\FASTbatikREDCDynamicCI} \\
% \CAPO	& \sdr{\SLOWbatikCAPOExc}{\SLOWbatikCAPOExcCI}{\SLOWbatikCAPOExcDynamic}{\SLOWbatikCAPOExcDynamicCI}	& \sdr{\SLOWbatikCAPOnoGExc}{\SLOWbatikCAPOnoGExcCI}{\SLOWbatikCAPOnoGExcDynamic}{\SLOWbatikCAPOnoGExcDynamicCI}	& \sdr{\FASTbatikFTOCAPO}{\FASTbatikFTOCAPOCI}{\FASTbatikFTOCAPODynamic}{\FASTbatikFTOCAPODynamicCI}	& \sdr{\FASTbatikRECAPO}{\FASTbatikRECAPOCI}{\FASTbatikRECAPODynamic}{\FASTbatikRECAPODynamicCI} \\
% 		& \mc{4}{c}{\bench{batik}} \\
% \end{tabular}
% \hfill
\begin{tabular}{@{}l|Hlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWhtwoHB}{\SLOWhtwoHBCI}{\SLOWhtwoHBDynamic}{\SLOWhtwoHBDynamicCI}					& \sdr{\FASThtwoFTOHB}{\FASThtwoFTOHBCI}{\FASThtwoFTOHBDynamic}{\FASThtwoFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWhtwoWCP}{\SLOWhtwoWCPCI}{\SLOWhtwoWCPDynamic}{\SLOWhtwoWCPDynamicCI}				& \sdr{\FASThtwoFTOWCP}{\FASThtwoFTOWCPCI}{\FASThtwoFTOWCPDynamic}{\FASThtwoFTOWCPDynamicCI}		& \sdr{\FASThtwoREWCP}{\FASThtwoREWCPCI}{\FASThtwoREWCPDynamic}{\FASThtwoREWCPDynamicCI} \\
\DC		& \sdr{\SLOWhtwoDCExc}{\SLOWhtwoDCExcCI}{\SLOWhtwoDCExcDynamic}{\SLOWhtwoDCExcDynamicCI}		& \sdr{\SLOWhtwoDCnoGExc}{\SLOWhtwoDCnoGExcCI}{\SLOWhtwoDCnoGExcDynamic}{\SLOWhtwoDCnoGExcDynamicCI}	& \sdr{\FASThtwoFTODC}{\FASThtwoFTODCCI}{\FASThtwoFTODCDynamic}{\FASThtwoFTODCDynamicCI}		& \sdr{\FASThtwoREDC}{\FASThtwoREDCCI}{\FASThtwoREDCDynamic}{\FASThtwoREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWhtwoCAPOExc}{\SLOWhtwoCAPOExcCI}{\SLOWhtwoCAPOExcDynamic}{\SLOWhtwoCAPOExcDynamicCI}	& \sdr{\SLOWhtwoCAPOnoGExc}{\SLOWhtwoCAPOnoGExcCI}{\SLOWhtwoCAPOnoGExcDynamic}{\SLOWhtwoCAPOnoGExcDynamicCI}	& \sdr{\FASThtwoFTOCAPO}{\FASThtwoFTOCAPOCI}{\FASThtwoFTOCAPODynamic}{\FASThtwoFTOCAPODynamicCI}	& \sdr{\FASThtwoRECAPO}{\FASThtwoRECAPOCI}{\FASThtwoRECAPODynamic}{\FASThtwoRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWjythonHB}{\SLOWjythonHBCI}{\SLOWjythonHBDynamic}{\SLOWjythonHBDynamicCI}					& \sdr{\FASTjythonFTOHB}{\FASTjythonFTOHBCI}{\FASTjythonFTOHBDynamic}{\FASTjythonFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWjythonWCP}{\SLOWjythonWCPCI}{\SLOWjythonWCPDynamic}{\SLOWjythonWCPDynamicCI}				& \sdr{\FASTjythonFTOWCP}{\FASTjythonFTOWCPCI}{\FASTjythonFTOWCPDynamic}{\FASTjythonFTOWCPDynamicCI}		& \sdr{\FASTjythonREWCP}{\FASTjythonREWCPCI}{\FASTjythonREWCPDynamic}{\FASTjythonREWCPDynamicCI} \\
\DC		& \sdr{\SLOWjythonDCExc}{\SLOWjythonDCExcCI}{\SLOWjythonDCExcDynamic}{\SLOWjythonDCExcDynamicCI}		& \sdr{\SLOWjythonDCnoGExc}{\SLOWjythonDCnoGExcCI}{\SLOWjythonDCnoGExcDynamic}{\SLOWjythonDCnoGExcDynamicCI}	& \sdr{\FASTjythonFTODC}{\FASTjythonFTODCCI}{\FASTjythonFTODCDynamic}{\FASTjythonFTODCDynamicCI}		& \sdr{\FASTjythonREDC}{\FASTjythonREDCCI}{\FASTjythonREDCDynamic}{\FASTjythonREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWjythonCAPOExc}{\SLOWjythonCAPOExcCI}{\SLOWjythonCAPOExcDynamic}{\SLOWjythonCAPOExcDynamicCI}	& \sdr{\SLOWjythonCAPOnoGExc}{\SLOWjythonCAPOnoGExcCI}{\SLOWjythonCAPOnoGExcDynamic}{\SLOWjythonCAPOnoGExcDynamicCI}	& \sdr{\FASTjythonFTOCAPO}{\FASTjythonFTOCAPOCI}{\FASTjythonFTOCAPODynamic}{\FASTjythonFTOCAPODynamicCI}	& \sdr{\FASTjythonRECAPO}{\FASTjythonRECAPOCI}{\FASTjythonRECAPODynamic}{\FASTjythonRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWluindexHB}{\SLOWluindexHBCI}{\SLOWluindexHBDynamic}{\SLOWluindexHBDynamicCI}					& \sdr{\FASTluindexFTOHB}{\FASTluindexFTOHBCI}{\FASTluindexFTOHBDynamic}{\FASTluindexFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWluindexWCP}{\SLOWluindexWCPCI}{\SLOWluindexWCPDynamic}{\SLOWluindexWCPDynamicCI}				& \sdr{\FASTluindexFTOWCP}{\FASTluindexFTOWCPCI}{\FASTluindexFTOWCPDynamic}{\FASTluindexFTOWCPDynamicCI}		& \sdr{\FASTluindexREWCP}{\FASTluindexREWCPCI}{\FASTluindexREWCPDynamic}{\FASTluindexREWCPDynamicCI} \\
\DC		& \sdr{\SLOWluindexDCExc}{\SLOWluindexDCExcCI}{\SLOWluindexDCExcDynamic}{\SLOWluindexDCExcDynamicCI}		& \sdr{\SLOWluindexDCnoGExc}{\SLOWluindexDCnoGExcCI}{\SLOWluindexDCnoGExcDynamic}{\SLOWluindexDCnoGExcDynamicCI}	& \sdr{\FASTluindexFTODC}{\FASTluindexFTODCCI}{\FASTluindexFTODCDynamic}{\FASTluindexFTODCDynamicCI}		& \sdr{\FASTluindexREDC}{\FASTluindexREDCCI}{\FASTluindexREDCDynamic}{\FASTluindexREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWluindexCAPOExc}{\SLOWluindexCAPOExcCI}{\SLOWluindexCAPOExcDynamic}{\SLOWluindexCAPOExcDynamicCI}	& \sdr{\SLOWluindexCAPOnoGExc}{\SLOWluindexCAPOnoGExcCI}{\SLOWluindexCAPOnoGExcDynamic}{\SLOWluindexCAPOnoGExcDynamicCI}	& \sdr{\FASTluindexFTOCAPO}{\FASTluindexFTOCAPOCI}{\FASTluindexFTOCAPODynamic}{\FASTluindexFTOCAPODynamicCI}	& \sdr{\FASTluindexRECAPO}{\FASTluindexRECAPOCI}{\FASTluindexRECAPODynamic}{\FASTluindexRECAPODynamicCI} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\hfill
% \begin{tabular}{@{}HHlll@{}}
%         & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
% \HB		& \rna													& \sdr{\SLOWlusearchHB}{\SLOWlusearchHBCI}{\SLOWlusearchHBDynamic}{\SLOWlusearchHBDynamicCI}					& \sdr{\FASTlusearchFTOHB}{\FASTlusearchFTOHBCI}{\FASTlusearchFTOHBDynamic}{\FASTlusearchFTOHBDynamicCI}		& \rna \\
% \WCP	& \rna													& \sdr{\SLOWlusearchWCP}{\SLOWlusearchWCPCI}{\SLOWlusearchWCPDynamic}{\SLOWlusearchWCPDynamicCI}				& \sdr{\FASTlusearchFTOWCP}{\FASTlusearchFTOWCPCI}{\FASTlusearchFTOWCPDynamic}{\FASTlusearchFTOWCPDynamicCI}		& \sdr{\FASTlusearchREWCP}{\FASTlusearchREWCPCI}{\FASTlusearchREWCPDynamic}{\FASTlusearchREWCPDynamicCI} \\
% \DC		& \sdr{\SLOWlusearchDCExc}{\SLOWlusearchDCExcCI}{\SLOWlusearchDCExcDynamic}{\SLOWlusearchDCExcDynamicCI}		& \sdr{\SLOWlusearchDCnoGExc}{\SLOWlusearchDCnoGExcCI}{\SLOWlusearchDCnoGExcDynamic}{\SLOWlusearchDCnoGExcDynamicCI}	& \sdr{\FASTlusearchFTODC}{\FASTlusearchFTODCCI}{\FASTlusearchFTODCDynamic}{\FASTlusearchFTODCDynamicCI}		& \sdr{\FASTlusearchREDC}{\FASTlusearchREDCCI}{\FASTlusearchREDCDynamic}{\FASTlusearchREDCDynamicCI} \\
% \CAPO	& \sdr{\SLOWlusearchCAPOExc}{\SLOWlusearchCAPOExcCI}{\SLOWlusearchCAPOExcDynamic}{\SLOWlusearchCAPOExcDynamicCI}	& \sdr{\SLOWlusearchCAPOnoGExc}{\SLOWlusearchCAPOnoGExcCI}{\SLOWlusearchCAPOnoGExcDynamic}{\SLOWlusearchCAPOnoGExcDynamicCI}	& \sdr{\FASTlusearchFTOCAPO}{\FASTlusearchFTOCAPOCI}{\FASTlusearchFTOCAPODynamic}{\FASTlusearchFTOCAPODynamicCI}	& \sdr{\FASTlusearchRECAPO}{\FASTlusearchRECAPOCI}{\FASTlusearchRECAPODynamic}{\FASTlusearchRECAPODynamicCI} \\
% 		& \mc{4}{c}{\bench{lusearch}} \\
% \end{tabular}
% \hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWpmdHB}{\SLOWpmdHBCI}{\SLOWpmdHBDynamic}{\SLOWpmdHBDynamicCI}					& \sdr{\FASTpmdFTOHB}{\FASTpmdFTOHBCI}{\FASTpmdFTOHBDynamic}{\FASTpmdFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWpmdWCP}{\SLOWpmdWCPCI}{\SLOWpmdWCPDynamic}{\SLOWpmdWCPDynamicCI}				& \sdr{\FASTpmdFTOWCP}{\FASTpmdFTOWCPCI}{\FASTpmdFTOWCPDynamic}{\FASTpmdFTOWCPDynamicCI}		& \sdr{\FASTpmdREWCP}{\FASTpmdREWCPCI}{\FASTpmdREWCPDynamic}{\FASTpmdREWCPDynamicCI} \\
\DC		& \sdr{\SLOWpmdDCExc}{\SLOWpmdDCExcCI}{\SLOWpmdDCExcDynamic}{\SLOWpmdDCExcDynamicCI}		& \sdr{\SLOWpmdDCnoGExc}{\SLOWpmdDCnoGExcCI}{\SLOWpmdDCnoGExcDynamic}{\SLOWpmdDCnoGExcDynamicCI}	& \sdr{\FASTpmdFTODC}{\FASTpmdFTODCCI}{\FASTpmdFTODCDynamic}{\FASTpmdFTODCDynamicCI}		& \sdr{\FASTpmdREDC}{\FASTpmdREDCCI}{\FASTpmdREDCDynamic}{\FASTpmdREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWpmdCAPOExc}{\SLOWpmdCAPOExcCI}{\SLOWpmdCAPOExcDynamic}{\SLOWpmdCAPOExcDynamicCI}	& \sdr{\SLOWpmdCAPOnoGExc}{\SLOWpmdCAPOnoGExcCI}{\SLOWpmdCAPOnoGExcDynamic}{\SLOWpmdCAPOnoGExcDynamicCI}	& \sdr{\FASTpmdFTOCAPO}{\FASTpmdFTOCAPOCI}{\FASTpmdFTOCAPODynamic}{\FASTpmdFTOCAPODynamicCI}	& \sdr{\FASTpmdRECAPO}{\FASTpmdRECAPOCI}{\FASTpmdRECAPODynamic}{\FASTpmdRECAPODynamicCI} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWsunflowHB}{\SLOWsunflowHBCI}{\SLOWsunflowHBDynamic}{\SLOWsunflowHBDynamicCI}					& \sdr{\FASTsunflowFTOHB}{\FASTsunflowFTOHBCI}{\FASTsunflowFTOHBDynamic}{\FASTsunflowFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWsunflowWCP}{\SLOWsunflowWCPCI}{\SLOWsunflowWCPDynamic}{\SLOWsunflowWCPDynamicCI}				& \sdr{\FASTsunflowFTOWCP}{\FASTsunflowFTOWCPCI}{\FASTsunflowFTOWCPDynamic}{\FASTsunflowFTOWCPDynamicCI}		& \sdr{\FASTsunflowREWCP}{\FASTsunflowREWCPCI}{\FASTsunflowREWCPDynamic}{\FASTsunflowREWCPDynamicCI} \\
\DC		& \sdr{\SLOWsunflowDCExc}{\SLOWsunflowDCExcCI}{\SLOWsunflowDCExcDynamic}{\SLOWsunflowDCExcDynamicCI}		& \sdr{\SLOWsunflowDCnoGExc}{\SLOWsunflowDCnoGExcCI}{\SLOWsunflowDCnoGExcDynamic}{\SLOWsunflowDCnoGExcDynamicCI}	& \sdr{\FASTsunflowFTODC}{\FASTsunflowFTODCCI}{\FASTsunflowFTODCDynamic}{\FASTsunflowFTODCDynamicCI}		& \sdr{\FASTsunflowREDC}{\FASTsunflowREDCCI}{\FASTsunflowREDCDynamic}{\FASTsunflowREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWsunflowCAPOExc}{\SLOWsunflowCAPOExcCI}{\SLOWsunflowCAPOExcDynamic}{\SLOWsunflowCAPOExcDynamicCI}	& \sdr{\SLOWsunflowCAPOnoGExc}{\SLOWsunflowCAPOnoGExcCI}{\SLOWsunflowCAPOnoGExcDynamic}{\SLOWsunflowCAPOnoGExcDynamicCI}	& \sdr{\FASTsunflowFTOCAPO}{\FASTsunflowFTOCAPOCI}{\FASTsunflowFTOCAPODynamic}{\FASTsunflowFTOCAPODynamicCI}	& \sdr{\FASTsunflowRECAPO}{\FASTsunflowRECAPOCI}{\FASTsunflowRECAPODynamic}{\FASTsunflowRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWtomcatHB}{\SLOWtomcatHBCI}{\SLOWtomcatHBDynamic}{\SLOWtomcatHBDynamicCI}					& \sdr{\FASTtomcatFTOHB}{\FASTtomcatFTOHBCI}{\FASTtomcatFTOHBDynamic}{\FASTtomcatFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWtomcatWCP}{\SLOWtomcatWCPCI}{\SLOWtomcatWCPDynamic}{\SLOWtomcatWCPDynamicCI}				& \sdr{\FASTtomcatFTOWCP}{\FASTtomcatFTOWCPCI}{\FASTtomcatFTOWCPDynamic}{\FASTtomcatFTOWCPDynamicCI}		& \sdr{\FASTtomcatREWCP}{\FASTtomcatREWCPCI}{\FASTtomcatREWCPDynamic}{\FASTtomcatREWCPDynamicCI} \\
\DC		& \sdr{\SLOWtomcatDCExc}{\SLOWtomcatDCExcCI}{\SLOWtomcatDCExcDynamic}{\SLOWtomcatDCExcDynamicCI}		& \sdr{\SLOWtomcatDCnoGExc}{\SLOWtomcatDCnoGExcCI}{\SLOWtomcatDCnoGExcDynamic}{\SLOWtomcatDCnoGExcDynamicCI}	& \sdr{\FASTtomcatFTODC}{\FASTtomcatFTODCCI}{\FASTtomcatFTODCDynamic}{\FASTtomcatFTODCDynamicCI}		& \sdr{\FASTtomcatREDC}{\FASTtomcatREDCCI}{\FASTtomcatREDCDynamic}{\FASTtomcatREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWtomcatCAPOExc}{\SLOWtomcatCAPOExcCI}{\SLOWtomcatCAPOExcDynamic}{\SLOWtomcatCAPOExcDynamicCI}	& \sdr{\SLOWtomcatCAPOnoGExc}{\SLOWtomcatCAPOnoGExcCI}{\SLOWtomcatCAPOnoGExcDynamic}{\SLOWtomcatCAPOnoGExcDynamicCI}	& \sdr{\FASTtomcatFTOCAPO}{\FASTtomcatFTOCAPOCI}{\FASTtomcatFTOCAPODynamic}{\FASTtomcatFTOCAPODynamicCI}	& \sdr{\FASTtomcatRECAPO}{\FASTtomcatRECAPOCI}{\FASTtomcatRECAPODynamic}{\FASTtomcatRECAPODynamicCI} \\
        & \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWxalanHB}{\SLOWxalanHBCI}{\SLOWxalanHBDynamic}{\SLOWxalanHBDynamicCI}					& \sdr{\FASTxalanFTOHB}{\FASTxalanFTOHBCI}{\FASTxalanFTOHBDynamic}{\FASTxalanFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWxalanWCP}{\SLOWxalanWCPCI}{\SLOWxalanWCPDynamic}{\SLOWxalanWCPDynamicCI}				& \sdr{\FASTxalanFTOWCP}{\FASTxalanFTOWCPCI}{\FASTxalanFTOWCPDynamic}{\FASTxalanFTOWCPDynamicCI}		& \sdr{\FASTxalanREWCP}{\FASTxalanREWCPCI}{\FASTxalanREWCPDynamic}{\FASTxalanREWCPDynamicCI} \\
\DC		& \sdr{\SLOWxalanDCExc}{\SLOWxalanDCExcCI}{\SLOWxalanDCExcDynamic}{\SLOWxalanDCExcDynamicCI}		& \sdr{\SLOWxalanDCnoGExc}{\SLOWxalanDCnoGExcCI}{\SLOWxalanDCnoGExcDynamic}{\SLOWxalanDCnoGExcDynamicCI}	& \sdr{\FASTxalanFTODC}{\FASTxalanFTODCCI}{\FASTxalanFTODCDynamic}{\FASTxalanFTODCDynamicCI}		& \sdr{\FASTxalanREDC}{\FASTxalanREDCCI}{\FASTxalanREDCDynamic}{\FASTxalanREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWxalanCAPOExc}{\SLOWxalanCAPOExcCI}{\SLOWxalanCAPOExcDynamic}{\SLOWxalanCAPOExcDynamicCI}	& \sdr{\SLOWxalanCAPOnoGExc}{\SLOWxalanCAPOnoGExcCI}{\SLOWxalanCAPOnoGExcDynamic}{\SLOWxalanCAPOnoGExcDynamicCI}	& \sdr{\FASTxalanFTOCAPO}{\FASTxalanFTOCAPOCI}{\FASTxalanFTOCAPODynamic}{\FASTxalanFTOCAPODynamicCI}	& \sdr{\FASTxalanRECAPO}{\FASTxalanRECAPOCI}{\FASTxalanRECAPODynamic}{\FASTxalanRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\caption{Average races reported by various analyses for each evaluated program
(excluding \bench{batik} and \bench{lusearch}, for which all analyses report no races).
In each cell, the first value is statically distinct races
(\ie, distinct program locations) and the second value, in parentheses, is total dynamic races
with 95\% confidence intervals.}
\label{tab:race:allDaCapo:CI}
\end{table*}

% Table for geometric mean of all relations with various optimizations for all DaCapo benchmarks
\begin{table}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
% \input{result-macros/PIP_slowTool_AllConfig_memChange}
\input{result-macros/PIP_slowTool_raceEdgeFix}
\input{result-macros/PIP_fastTool_readExclFix_Quite}
%
\small
\centering
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWHBTimeGeoMean}			& \roh{\FASTFTOHBTimeGeoMean}	& \rna \\
\WCP	& \rna							& \roh{\SLOWWCPTimeGeoMean}			& \roh{\FASTFTOWCPTimeGeoMean}	& \roh{\FASTREWCPTimeGeoMean} \\
\DC		& \roh{\SLOWDCExcTimeGeoMean}	& \roh{\SLOWDCnoGExcTimeGeoMean}	& \roh{\FASTFTODCTimeGeoMean}	& \roh{\FASTREDCTimeGeoMean} \\
\CAPO	& \roh{\SLOWCAPOExcTimeGeoMean}	& \roh{\SLOWCAPOnoGExcTimeGeoMean}	& \roh{\FASTFTOCAPOTimeGeoMean}	& \roh{\FASTRECAPOTimeGeoMean} \\
\mc{2}{H}{} & \mc{3}{c}{Run time} \\
\end{tabular}
\hspace*{1em}
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \mem{\SLOWHBMemGeoMean}			& \mem{\FASTFTOHBMemGeoMean}	& \rna \\
\WCP	& \rna							& \mem{\SLOWWCPMemGeoMean}			& \mem{\FASTFTOWCPMemGeoMean}	& \mem{\FASTREWCPMemGeoMean} \\
\DC		& \mem{\SLOWDCExcMemGeoMean}	& \mem{\SLOWDCnoGExcMemGeoMean}	& \mem{\FASTFTODCMemGeoMean}	& \mem{\FASTREDCMemGeoMean} \\
\CAPO	& \mem{\SLOWCAPOExcMemGeoMean}	& \mem{\SLOWCAPOnoGExcMemGeoMean}	& \mem{\FASTFTOCAPOMemGeoMean}	& \mem{\FASTRECAPOMemGeoMean} \\
\mc{2}{H}{} & \mc{3}{c}{Memory usage} \\
\end{tabular}

\caption{Geometric mean of run time and memory usage across the evaluated programs.}
\label{tab:performance:geoMean}
\end{table}
\fi

\begin{table*}[t]
% \begin{adjustwidth}{-1.5cm}{}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
% \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;Mb$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\sdr}[2]{#1{\;}(#2)}
\input{result-macros/PIP_slowTool_raceEdgeFix_fieldName}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
%\input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_fastTool_fieldRaces}
%
\smaller
\centering
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWavroraHB}{\SLOWavroraHBDynamic}					& \sdr{\FASTavroraFTOHB}{\FASTavroraFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWavroraWCP}{\SLOWavroraWCPDynamic}				& \sdr{\FASTavroraFTOWCP}{\FASTavroraFTOWCPDynamic}		& \sdr{\FASTavroraREWCP}{\FASTavroraREWCPDynamic} \\
\DC		& \sdr{\SLOWavroraDCExc}{\SLOWavroraDCExcDynamic}		& \sdr{\SLOWavroraDCnoGExc}{\SLOWavroraDCnoGExcDynamic}	& \sdr{\FASTavroraFTODC}{\FASTavroraFTODCDynamic}		& \sdr{\FASTavroraREDC}{\FASTavroraREDCDynamic} \\
\CAPO	& \sdr{\SLOWavroraCAPOExc}{\SLOWavroraCAPOExcDynamic}	& \sdr{\SLOWavroraCAPOnoGExc}{\SLOWavroraCAPOnoGExcDynamic}	& \sdr{\FASTavroraFTOCAPO}{\FASTavroraFTOCAPODynamic}	& \sdr{\FASTavroraRECAPO}{\FASTavroraRECAPODynamic} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
% \begin{tabular}{@{}HHrrr@{}}
%         & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
% \HB		& \rna													& \sdr{\SLOWbatikHB}{\SLOWbatikHBDynamic}					& \sdr{\FASTbatikFTOHB}{\FASTbatikFTOHBDynamic}		& \rna \\
% \WCP	& \rna													& \sdr{\SLOWbatikWCP}{\SLOWbatikWCPDynamic}				& \sdr{\FASTbatikFTOWCP}{\FASTbatikFTOWCPDynamic}		& \sdr{\FASTbatikREWCP}{\FASTbatikREWCPDynamic} \\
% \DC		& \sdr{\SLOWbatikDCExc}{\SLOWbatikDCExcDynamic}		& \sdr{\SLOWbatikDCnoGExc}{\SLOWbatikDCnoGExcDynamic}	& \sdr{\FASTbatikFTODC}{\FASTbatikFTODCDynamic}		& \sdr{\FASTbatikREDC}{\FASTbatikREDCDynamic} \\
% \CAPO	& \sdr{\SLOWbatikCAPOExc}{\SLOWbatikCAPOExcDynamic}	& \sdr{\SLOWbatikCAPOnoGExc}{\SLOWbatikCAPOnoGExcDynamic}	& \sdr{\FASTbatikFTOCAPO}{\FASTbatikFTOCAPODynamic}	& \sdr{\FASTbatikRECAPO}{\FASTbatikRECAPODynamic} \\
% 		& \mc{4}{c}{\bench{batik}} \\
% \end{tabular}
% \hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWhtwoHB}{\SLOWhtwoHBDynamic}					& \sdr{\FASThtwoFTOHB}{\FASThtwoFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWhtwoWCP}{\SLOWhtwoWCPDynamic}				& \sdr{\FASThtwoFTOWCP}{\FASThtwoFTOWCPDynamic}		& \sdr{\FASThtwoREWCP}{\FASThtwoREWCPDynamic} \\
\DC		& \sdr{\SLOWhtwoDCExc}{\SLOWhtwoDCExcDynamic}		& \sdr{\SLOWhtwoDCnoGExc}{\SLOWhtwoDCnoGExcDynamic}	& \sdr{\FASThtwoFTODC}{\FASThtwoFTODCDynamic}		& \sdr{\FASThtwoREDC}{\FASThtwoREDCDynamic} \\
\CAPO	& \sdr{\SLOWhtwoCAPOExc}{\SLOWhtwoCAPOExcDynamic}	& \sdr{\SLOWhtwoCAPOnoGExc}{\SLOWhtwoCAPOnoGExcDynamic}	& \sdr{\FASThtwoFTOCAPO}{\FASThtwoFTOCAPODynamic}	& \sdr{\FASThtwoRECAPO}{\FASThtwoRECAPODynamic} \\
		& \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWjythonHB}{\SLOWjythonHBDynamic}					& \sdr{\FASTjythonFTOHB}{\FASTjythonFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWjythonWCP}{\SLOWjythonWCPDynamic}				& \sdr{\FASTjythonFTOWCP}{\FASTjythonFTOWCPDynamic}		& \sdr{\FASTjythonREWCP}{\FASTjythonREWCPDynamic} \\
\DC		& \sdr{\SLOWjythonDCExc}{\SLOWjythonDCExcDynamic}		& \sdr{\SLOWjythonDCnoGExc}{\SLOWjythonDCnoGExcDynamic}	& \sdr{\FASTjythonFTODC}{\FASTjythonFTODCDynamic}		& \sdr{\FASTjythonREDC}{\FASTjythonREDCDynamic} \\
\CAPO	& \sdr{\SLOWjythonCAPOExc}{\SLOWjythonCAPOExcDynamic}	& \sdr{\SLOWjythonCAPOnoGExc}{\SLOWjythonCAPOnoGExcDynamic}	& \sdr{\FASTjythonFTOCAPO}{\FASTjythonFTOCAPODynamic}	& \sdr{\FASTjythonRECAPO}{\FASTjythonRECAPODynamic} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWluindexHB}{\SLOWluindexHBDynamic}					& \sdr{\FASTluindexFTOHB}{\FASTluindexFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWluindexWCP}{\SLOWluindexWCPDynamic}				& \sdr{\FASTluindexFTOWCP}{\FASTluindexFTOWCPDynamic}		& \sdr{\FASTluindexREWCP}{\FASTluindexREWCPDynamic} \\
\DC		& \sdr{\SLOWluindexDCExc}{\SLOWluindexDCExcDynamic}		& \sdr{\SLOWluindexDCnoGExc}{\SLOWluindexDCnoGExcDynamic}	& \sdr{\FASTluindexFTODC}{\FASTluindexFTODCDynamic}		& \sdr{\FASTluindexREDC}{\FASTluindexREDCDynamic} \\
\CAPO	& \sdr{\SLOWluindexCAPOExc}{\SLOWluindexCAPOExcDynamic}	& \sdr{\SLOWluindexCAPOnoGExc}{\SLOWluindexCAPOnoGExcDynamic}	& \sdr{\FASTluindexFTOCAPO}{\FASTluindexFTOCAPODynamic}	& \sdr{\FASTluindexRECAPO}{\FASTluindexRECAPODynamic} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\medskip\\
% \begin{tabular}{@{}HHrrr@{}}
%         & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
% \HB		& \rna													& \sdr{\SLOWlusearchHB}{\SLOWlusearchHBDynamic}					& \sdr{\FASTlusearchFTOHB}{\FASTlusearchFTOHBDynamic}		& \rna \\
% \WCP	& \rna													& \sdr{\SLOWlusearchWCP}{\SLOWlusearchWCPDynamic}				& \sdr{\FASTlusearchFTOWCP}{\FASTlusearchFTOWCPDynamic}		& \sdr{\FASTlusearchREWCP}{\FASTlusearchREWCPDynamic} \\
% \DC		& \sdr{\SLOWlusearchDCExc}{\SLOWlusearchDCExcDynamic}		& \sdr{\SLOWlusearchDCnoGExc}{\SLOWlusearchDCnoGExcDynamic}	& \sdr{\FASTlusearchFTODC}{\FASTlusearchFTODCDynamic}		& \sdr{\FASTlusearchREDC}{\FASTlusearchREDCDynamic} \\
% \CAPO	& \sdr{\SLOWlusearchCAPOExc}{\SLOWlusearchCAPOExcDynamic}	& \sdr{\SLOWlusearchCAPOnoGExc}{\SLOWlusearchCAPOnoGExcDynamic}	& \sdr{\FASTlusearchFTOCAPO}{\FASTlusearchFTOCAPODynamic}	& \sdr{\FASTlusearchRECAPO}{\FASTlusearchRECAPODynamic} \\
% 		& \mc{4}{c}{\bench{lusearch}} \\
% \end{tabular}
% \hfill
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWpmdHB}{\SLOWpmdHBDynamic}					& \sdr{\FASTpmdFTOHB}{\FASTpmdFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWpmdWCP}{\SLOWpmdWCPDynamic}				& \sdr{\FASTpmdFTOWCP}{\FASTpmdFTOWCPDynamic}		& \sdr{\FASTpmdREWCP}{\FASTpmdREWCPDynamic} \\
\DC		& \sdr{\SLOWpmdDCExc}{\SLOWpmdDCExcDynamic}		& \sdr{\SLOWpmdDCnoGExc}{\SLOWpmdDCnoGExcDynamic}	& \sdr{\FASTpmdFTODC}{\FASTpmdFTODCDynamic}		& \sdr{\FASTpmdREDC}{\FASTpmdREDCDynamic} \\
\CAPO	& \sdr{\SLOWpmdCAPOExc}{\SLOWpmdCAPOExcDynamic}	& \sdr{\SLOWpmdCAPOnoGExc}{\SLOWpmdCAPOnoGExcDynamic}	& \sdr{\FASTpmdFTOCAPO}{\FASTpmdFTOCAPODynamic}	& \sdr{\FASTpmdRECAPO}{\FASTpmdRECAPODynamic} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWsunflowHB}{\SLOWsunflowHBDynamic}					& \sdr{\FASTsunflowFTOHB}{\FASTsunflowFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWsunflowWCP}{\SLOWsunflowWCPDynamic}				& \sdr{\FASTsunflowFTOWCP}{\FASTsunflowFTOWCPDynamic}		& \sdr{\FASTsunflowREWCP}{\FASTsunflowREWCPDynamic} \\
\DC		& \sdr{\SLOWsunflowDCExc}{\SLOWsunflowDCExcDynamic}		& \sdr{\SLOWsunflowDCnoGExc}{\SLOWsunflowDCnoGExcDynamic}	& \sdr{\FASTsunflowFTODC}{\FASTsunflowFTODCDynamic}		& \sdr{\FASTsunflowREDC}{\FASTsunflowREDCDynamic} \\
\CAPO	& \sdr{\SLOWsunflowCAPOExc}{\SLOWsunflowCAPOExcDynamic}	& \sdr{\SLOWsunflowCAPOnoGExc}{\SLOWsunflowCAPOnoGExcDynamic}	& \sdr{\FASTsunflowFTOCAPO}{\FASTsunflowFTOCAPODynamic}	& \sdr{\FASTsunflowRECAPO}{\FASTsunflowRECAPODynamic} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWtomcatHB}{\SLOWtomcatHBDynamic}					& \sdr{\FASTtomcatFTOHB}{\FASTtomcatFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWtomcatWCP}{\SLOWtomcatWCPDynamic}				& \sdr{\FASTtomcatFTOWCP}{\FASTtomcatFTOWCPDynamic}		& \sdr{\FASTtomcatREWCP}{\FASTtomcatREWCPDynamic} \\
\DC		& \sdr{\SLOWtomcatDCExc}{\SLOWtomcatDCExcDynamic}		& \sdr{\SLOWtomcatDCnoGExc}{\SLOWtomcatDCnoGExcDynamic}	& \sdr{\FASTtomcatFTODC}{\FASTtomcatFTODCDynamic}		& \sdr{\FASTtomcatREDC}{\FASTtomcatREDCDynamic} \\
\CAPO	& \sdr{\SLOWtomcatCAPOExc}{\SLOWtomcatCAPOExcDynamic}	& \sdr{\SLOWtomcatCAPOnoGExc}{\SLOWtomcatCAPOnoGExcDynamic}	& \sdr{\FASTtomcatFTOCAPO}{\FASTtomcatFTOCAPODynamic}	& \sdr{\FASTtomcatRECAPO}{\FASTtomcatRECAPODynamic} \\
        & \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWxalanHB}{\SLOWxalanHBDynamic}					& \sdr{\FASTxalanFTOHB}{\FASTxalanFTOHBDynamic}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWxalanWCP}{\SLOWxalanWCPDynamic}				& \sdr{\FASTxalanFTOWCP}{\FASTxalanFTOWCPDynamic}		& \sdr{\FASTxalanREWCP}{\FASTxalanREWCPDynamic} \\
\DC		& \sdr{\SLOWxalanDCExc}{\SLOWxalanDCExcDynamic}		& \sdr{\SLOWxalanDCnoGExc}{\SLOWxalanDCnoGExcDynamic}	& \sdr{\FASTxalanFTODC}{\FASTxalanFTODCDynamic}		& \sdr{\FASTxalanREDC}{\FASTxalanREDCDynamic} \\
\CAPO	& \sdr{\SLOWxalanCAPOExc}{\SLOWxalanCAPOExcDynamic}	& \sdr{\SLOWxalanCAPOnoGExc}{\SLOWxalanCAPOnoGExcDynamic}	& \sdr{\FASTxalanFTOCAPO}{\FASTxalanFTOCAPODynamic}	& \sdr{\FASTxalanRECAPO}{\FASTxalanRECAPODynamic} \\
& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\caption{Average races reported for counting races by field name and array type
for all analyses.}
\label{tab:race:allDaCapo}
\end{table*}

\begin{table*}[t]
% \begin{adjustwidth}{-1.5cm}{}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
% \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;Mb$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\sdr}[4]{\vci{#1}{#2}{\;}(\vci{#3}{#4})}
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}#1}
\input{result-macros/PIP_slowTool_raceEdgeFix_fieldName}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
%\input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_fastTool_fieldRaces}
%
\smaller
\centering
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWavroraHB}{\SLOWavroraHBCI}{\SLOWavroraHBDynamic}{\SLOWavroraHBDynamicCI}					& \sdr{\FASTavroraFTOHB}{\FASTavroraFTOHBCI}{\FASTavroraFTOHBDynamic}{\FASTavroraFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWavroraWCP}{\SLOWavroraWCPCI}{\SLOWavroraWCPDynamic}{\SLOWavroraWCPDynamicCI}				& \sdr{\FASTavroraFTOWCP}{\FASTavroraFTOWCPCI}{\FASTavroraFTOWCPDynamic}{\FASTavroraFTOWCPDynamicCI}		& \sdr{\FASTavroraREWCP}{\FASTavroraREWCPCI}{\FASTavroraREWCPDynamic}{\FASTavroraREWCPDynamicCI} \\
\DC		& \sdr{\SLOWavroraDCExc}{\SLOWavroraDCExcCI}{\SLOWavroraDCExcDynamic}{\SLOWavroraDCExcDynamicCI}		& \sdr{\SLOWavroraDCnoGExc}{\SLOWavroraDCnoGExcCI}{\SLOWavroraDCnoGExcDynamic}{\SLOWavroraDCnoGExcDynamicCI}	& \sdr{\FASTavroraFTODC}{\FASTavroraFTODCCI}{\FASTavroraFTODCDynamic}{\FASTavroraFTODCDynamicCI}		& \sdr{\FASTavroraREDC}{\FASTavroraREDCCI}{\FASTavroraREDCDynamic}{\FASTavroraREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWavroraCAPOExc}{\SLOWavroraCAPOExcCI}{\SLOWavroraCAPOExcDynamic}{\SLOWavroraCAPOExcDynamicCI}	& \sdr{\SLOWavroraCAPOnoGExc}{\SLOWavroraCAPOnoGExcCI}{\SLOWavroraCAPOnoGExcDynamic}{\SLOWavroraCAPOnoGExcDynamicCI}	& \sdr{\FASTavroraFTOCAPO}{\FASTavroraFTOCAPOCI}{\FASTavroraFTOCAPODynamic}{\FASTavroraFTOCAPODynamicCI}	& \sdr{\FASTavroraRECAPO}{\FASTavroraRECAPOCI}{\FASTavroraRECAPODynamic}{\FASTavroraRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\medskip\\
% \begin{tabular}{@{}HHlll@{}}
%         & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
% \HB		& \rna													& \sdr{\SLOWbatikHB}{\SLOWbatikHBCI}{\SLOWbatikHBDynamic}{\SLOWbatikHBDynamicCI}					& \sdr{\FASTbatikFTOHB}{\FASTbatikFTOHBCI}{\FASTbatikFTOHBDynamic}{\FASTbatikFTOHBDynamicCI}		& \rna \\
% \WCP	& \rna													& \sdr{\SLOWbatikWCP}{\SLOWbatikWCPCI}{\SLOWbatikWCPDynamic}{\SLOWbatikWCPDynamicCI}				& \sdr{\FASTbatikFTOWCP}{\FASTbatikFTOWCPCI}{\FASTbatikFTOWCPDynamic}{\FASTbatikFTOWCPDynamicCI}		& \sdr{\FASTbatikREWCP}{\FASTbatikREWCPCI}{\FASTbatikREWCPDynamic}{\FASTbatikREWCPDynamicCI} \\
% \DC		& \sdr{\SLOWbatikDCExc}{\SLOWbatikDCExcCI}{\SLOWbatikDCExcDynamic}{\SLOWbatikDCExcDynamicCI}		& \sdr{\SLOWbatikDCnoGExc}{\SLOWbatikDCnoGExcCI}{\SLOWbatikDCnoGExcDynamic}{\SLOWbatikDCnoGExcDynamicCI}	& \sdr{\FASTbatikFTODC}{\FASTbatikFTODCCI}{\FASTbatikFTODCDynamic}{\FASTbatikFTODCDynamicCI}		& \sdr{\FASTbatikREDC}{\FASTbatikREDCCI}{\FASTbatikREDCDynamic}{\FASTbatikREDCDynamicCI} \\
% \CAPO	& \sdr{\SLOWbatikCAPOExc}{\SLOWbatikCAPOExcCI}{\SLOWbatikCAPOExcDynamic}{\SLOWbatikCAPOExcDynamicCI}	& \sdr{\SLOWbatikCAPOnoGExc}{\SLOWbatikCAPOnoGExcCI}{\SLOWbatikCAPOnoGExcDynamic}{\SLOWbatikCAPOnoGExcDynamicCI}	& \sdr{\FASTbatikFTOCAPO}{\FASTbatikFTOCAPOCI}{\FASTbatikFTOCAPODynamic}{\FASTbatikFTOCAPODynamicCI}	& \sdr{\FASTbatikRECAPO}{\FASTbatikRECAPOCI}{\FASTbatikRECAPODynamic}{\FASTbatikRECAPODynamicCI} \\
% 		& \mc{4}{c}{\bench{batik}} \\
% \end{tabular}
% \hfill
\begin{tabular}{@{}l|Hlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWhtwoHB}{\SLOWhtwoHBCI}{\SLOWhtwoHBDynamic}{\SLOWhtwoHBDynamicCI}					& \sdr{\FASThtwoFTOHB}{\FASThtwoFTOHBCI}{\FASThtwoFTOHBDynamic}{\FASThtwoFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWhtwoWCP}{\SLOWhtwoWCPCI}{\SLOWhtwoWCPDynamic}{\SLOWhtwoWCPDynamicCI}				& \sdr{\FASThtwoFTOWCP}{\FASThtwoFTOWCPCI}{\FASThtwoFTOWCPDynamic}{\FASThtwoFTOWCPDynamicCI}		& \sdr{\FASThtwoREWCP}{\FASThtwoREWCPCI}{\FASThtwoREWCPDynamic}{\FASThtwoREWCPDynamicCI} \\
\DC		& \sdr{\SLOWhtwoDCExc}{\SLOWhtwoDCExcCI}{\SLOWhtwoDCExcDynamic}{\SLOWhtwoDCExcDynamicCI}		& \sdr{\SLOWhtwoDCnoGExc}{\SLOWhtwoDCnoGExcCI}{\SLOWhtwoDCnoGExcDynamic}{\SLOWhtwoDCnoGExcDynamicCI}	& \sdr{\FASThtwoFTODC}{\FASThtwoFTODCCI}{\FASThtwoFTODCDynamic}{\FASThtwoFTODCDynamicCI}		& \sdr{\FASThtwoREDC}{\FASThtwoREDCCI}{\FASThtwoREDCDynamic}{\FASThtwoREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWhtwoCAPOExc}{\SLOWhtwoCAPOExcCI}{\SLOWhtwoCAPOExcDynamic}{\SLOWhtwoCAPOExcDynamicCI}	& \sdr{\SLOWhtwoCAPOnoGExc}{\SLOWhtwoCAPOnoGExcCI}{\SLOWhtwoCAPOnoGExcDynamic}{\SLOWhtwoCAPOnoGExcDynamicCI}	& \sdr{\FASThtwoFTOCAPO}{\FASThtwoFTOCAPOCI}{\FASThtwoFTOCAPODynamic}{\FASThtwoFTOCAPODynamicCI}	& \sdr{\FASThtwoRECAPO}{\FASThtwoRECAPOCI}{\FASThtwoRECAPODynamic}{\FASThtwoRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWjythonHB}{\SLOWjythonHBCI}{\SLOWjythonHBDynamic}{\SLOWjythonHBDynamicCI}					& \sdr{\FASTjythonFTOHB}{\FASTjythonFTOHBCI}{\FASTjythonFTOHBDynamic}{\FASTjythonFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWjythonWCP}{\SLOWjythonWCPCI}{\SLOWjythonWCPDynamic}{\SLOWjythonWCPDynamicCI}				& \sdr{\FASTjythonFTOWCP}{\FASTjythonFTOWCPCI}{\FASTjythonFTOWCPDynamic}{\FASTjythonFTOWCPDynamicCI}		& \sdr{\FASTjythonREWCP}{\FASTjythonREWCPCI}{\FASTjythonREWCPDynamic}{\FASTjythonREWCPDynamicCI} \\
\DC		& \sdr{\SLOWjythonDCExc}{\SLOWjythonDCExcCI}{\SLOWjythonDCExcDynamic}{\SLOWjythonDCExcDynamicCI}		& \sdr{\SLOWjythonDCnoGExc}{\SLOWjythonDCnoGExcCI}{\SLOWjythonDCnoGExcDynamic}{\SLOWjythonDCnoGExcDynamicCI}	& \sdr{\FASTjythonFTODC}{\FASTjythonFTODCCI}{\FASTjythonFTODCDynamic}{\FASTjythonFTODCDynamicCI}		& \sdr{\FASTjythonREDC}{\FASTjythonREDCCI}{\FASTjythonREDCDynamic}{\FASTjythonREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWjythonCAPOExc}{\SLOWjythonCAPOExcCI}{\SLOWjythonCAPOExcDynamic}{\SLOWjythonCAPOExcDynamicCI}	& \sdr{\SLOWjythonCAPOnoGExc}{\SLOWjythonCAPOnoGExcCI}{\SLOWjythonCAPOnoGExcDynamic}{\SLOWjythonCAPOnoGExcDynamicCI}	& \sdr{\FASTjythonFTOCAPO}{\FASTjythonFTOCAPOCI}{\FASTjythonFTOCAPODynamic}{\FASTjythonFTOCAPODynamicCI}	& \sdr{\FASTjythonRECAPO}{\FASTjythonRECAPOCI}{\FASTjythonRECAPODynamic}{\FASTjythonRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWluindexHB}{\SLOWluindexHBCI}{\SLOWluindexHBDynamic}{\SLOWluindexHBDynamicCI}					& \sdr{\FASTluindexFTOHB}{\FASTluindexFTOHBCI}{\FASTluindexFTOHBDynamic}{\FASTluindexFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWluindexWCP}{\SLOWluindexWCPCI}{\SLOWluindexWCPDynamic}{\SLOWluindexWCPDynamicCI}				& \sdr{\FASTluindexFTOWCP}{\FASTluindexFTOWCPCI}{\FASTluindexFTOWCPDynamic}{\FASTluindexFTOWCPDynamicCI}		& \sdr{\FASTluindexREWCP}{\FASTluindexREWCPCI}{\FASTluindexREWCPDynamic}{\FASTluindexREWCPDynamicCI} \\
\DC		& \sdr{\SLOWluindexDCExc}{\SLOWluindexDCExcCI}{\SLOWluindexDCExcDynamic}{\SLOWluindexDCExcDynamicCI}		& \sdr{\SLOWluindexDCnoGExc}{\SLOWluindexDCnoGExcCI}{\SLOWluindexDCnoGExcDynamic}{\SLOWluindexDCnoGExcDynamicCI}	& \sdr{\FASTluindexFTODC}{\FASTluindexFTODCCI}{\FASTluindexFTODCDynamic}{\FASTluindexFTODCDynamicCI}		& \sdr{\FASTluindexREDC}{\FASTluindexREDCCI}{\FASTluindexREDCDynamic}{\FASTluindexREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWluindexCAPOExc}{\SLOWluindexCAPOExcCI}{\SLOWluindexCAPOExcDynamic}{\SLOWluindexCAPOExcDynamicCI}	& \sdr{\SLOWluindexCAPOnoGExc}{\SLOWluindexCAPOnoGExcCI}{\SLOWluindexCAPOnoGExcDynamic}{\SLOWluindexCAPOnoGExcDynamicCI}	& \sdr{\FASTluindexFTOCAPO}{\FASTluindexFTOCAPOCI}{\FASTluindexFTOCAPODynamic}{\FASTluindexFTOCAPODynamicCI}	& \sdr{\FASTluindexRECAPO}{\FASTluindexRECAPOCI}{\FASTluindexRECAPODynamic}{\FASTluindexRECAPODynamicCI} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\hfill
% \begin{tabular}{@{}HHlll@{}}
%         & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
% \HB		& \rna													& \sdr{\SLOWlusearchHB}{\SLOWlusearchHBCI}{\SLOWlusearchHBDynamic}{\SLOWlusearchHBDynamicCI}					& \sdr{\FASTlusearchFTOHB}{\FASTlusearchFTOHBCI}{\FASTlusearchFTOHBDynamic}{\FASTlusearchFTOHBDynamicCI}		& \rna \\
% \WCP	& \rna													& \sdr{\SLOWlusearchWCP}{\SLOWlusearchWCPCI}{\SLOWlusearchWCPDynamic}{\SLOWlusearchWCPDynamicCI}				& \sdr{\FASTlusearchFTOWCP}{\FASTlusearchFTOWCPCI}{\FASTlusearchFTOWCPDynamic}{\FASTlusearchFTOWCPDynamicCI}		& \sdr{\FASTlusearchREWCP}{\FASTlusearchREWCPCI}{\FASTlusearchREWCPDynamic}{\FASTlusearchREWCPDynamicCI} \\
% \DC		& \sdr{\SLOWlusearchDCExc}{\SLOWlusearchDCExcCI}{\SLOWlusearchDCExcDynamic}{\SLOWlusearchDCExcDynamicCI}		& \sdr{\SLOWlusearchDCnoGExc}{\SLOWlusearchDCnoGExcCI}{\SLOWlusearchDCnoGExcDynamic}{\SLOWlusearchDCnoGExcDynamicCI}	& \sdr{\FASTlusearchFTODC}{\FASTlusearchFTODCCI}{\FASTlusearchFTODCDynamic}{\FASTlusearchFTODCDynamicCI}		& \sdr{\FASTlusearchREDC}{\FASTlusearchREDCCI}{\FASTlusearchREDCDynamic}{\FASTlusearchREDCDynamicCI} \\
% \CAPO	& \sdr{\SLOWlusearchCAPOExc}{\SLOWlusearchCAPOExcCI}{\SLOWlusearchCAPOExcDynamic}{\SLOWlusearchCAPOExcDynamicCI}	& \sdr{\SLOWlusearchCAPOnoGExc}{\SLOWlusearchCAPOnoGExcCI}{\SLOWlusearchCAPOnoGExcDynamic}{\SLOWlusearchCAPOnoGExcDynamicCI}	& \sdr{\FASTlusearchFTOCAPO}{\FASTlusearchFTOCAPOCI}{\FASTlusearchFTOCAPODynamic}{\FASTlusearchFTOCAPODynamicCI}	& \sdr{\FASTlusearchRECAPO}{\FASTlusearchRECAPOCI}{\FASTlusearchRECAPODynamic}{\FASTlusearchRECAPODynamicCI} \\
% 		& \mc{4}{c}{\bench{lusearch}} \\
% \end{tabular}
% \hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWpmdHB}{\SLOWpmdHBCI}{\SLOWpmdHBDynamic}{\SLOWpmdHBDynamicCI}					& \sdr{\FASTpmdFTOHB}{\FASTpmdFTOHBCI}{\FASTpmdFTOHBDynamic}{\FASTpmdFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWpmdWCP}{\SLOWpmdWCPCI}{\SLOWpmdWCPDynamic}{\SLOWpmdWCPDynamicCI}				& \sdr{\FASTpmdFTOWCP}{\FASTpmdFTOWCPCI}{\FASTpmdFTOWCPDynamic}{\FASTpmdFTOWCPDynamicCI}		& \sdr{\FASTpmdREWCP}{\FASTpmdREWCPCI}{\FASTpmdREWCPDynamic}{\FASTpmdREWCPDynamicCI} \\
\DC		& \sdr{\SLOWpmdDCExc}{\SLOWpmdDCExcCI}{\SLOWpmdDCExcDynamic}{\SLOWpmdDCExcDynamicCI}		& \sdr{\SLOWpmdDCnoGExc}{\SLOWpmdDCnoGExcCI}{\SLOWpmdDCnoGExcDynamic}{\SLOWpmdDCnoGExcDynamicCI}	& \sdr{\FASTpmdFTODC}{\FASTpmdFTODCCI}{\FASTpmdFTODCDynamic}{\FASTpmdFTODCDynamicCI}		& \sdr{\FASTpmdREDC}{\FASTpmdREDCCI}{\FASTpmdREDCDynamic}{\FASTpmdREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWpmdCAPOExc}{\SLOWpmdCAPOExcCI}{\SLOWpmdCAPOExcDynamic}{\SLOWpmdCAPOExcDynamicCI}	& \sdr{\SLOWpmdCAPOnoGExc}{\SLOWpmdCAPOnoGExcCI}{\SLOWpmdCAPOnoGExcDynamic}{\SLOWpmdCAPOnoGExcDynamicCI}	& \sdr{\FASTpmdFTOCAPO}{\FASTpmdFTOCAPOCI}{\FASTpmdFTOCAPODynamic}{\FASTpmdFTOCAPODynamicCI}	& \sdr{\FASTpmdRECAPO}{\FASTpmdRECAPOCI}{\FASTpmdRECAPODynamic}{\FASTpmdRECAPODynamicCI} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWsunflowHB}{\SLOWsunflowHBCI}{\SLOWsunflowHBDynamic}{\SLOWsunflowHBDynamicCI}					& \sdr{\FASTsunflowFTOHB}{\FASTsunflowFTOHBCI}{\FASTsunflowFTOHBDynamic}{\FASTsunflowFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWsunflowWCP}{\SLOWsunflowWCPCI}{\SLOWsunflowWCPDynamic}{\SLOWsunflowWCPDynamicCI}				& \sdr{\FASTsunflowFTOWCP}{\FASTsunflowFTOWCPCI}{\FASTsunflowFTOWCPDynamic}{\FASTsunflowFTOWCPDynamicCI}		& \sdr{\FASTsunflowREWCP}{\FASTsunflowREWCPCI}{\FASTsunflowREWCPDynamic}{\FASTsunflowREWCPDynamicCI} \\
\DC		& \sdr{\SLOWsunflowDCExc}{\SLOWsunflowDCExcCI}{\SLOWsunflowDCExcDynamic}{\SLOWsunflowDCExcDynamicCI}		& \sdr{\SLOWsunflowDCnoGExc}{\SLOWsunflowDCnoGExcCI}{\SLOWsunflowDCnoGExcDynamic}{\SLOWsunflowDCnoGExcDynamicCI}	& \sdr{\FASTsunflowFTODC}{\FASTsunflowFTODCCI}{\FASTsunflowFTODCDynamic}{\FASTsunflowFTODCDynamicCI}		& \sdr{\FASTsunflowREDC}{\FASTsunflowREDCCI}{\FASTsunflowREDCDynamic}{\FASTsunflowREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWsunflowCAPOExc}{\SLOWsunflowCAPOExcCI}{\SLOWsunflowCAPOExcDynamic}{\SLOWsunflowCAPOExcDynamicCI}	& \sdr{\SLOWsunflowCAPOnoGExc}{\SLOWsunflowCAPOnoGExcCI}{\SLOWsunflowCAPOnoGExcDynamic}{\SLOWsunflowCAPOnoGExcDynamicCI}	& \sdr{\FASTsunflowFTOCAPO}{\FASTsunflowFTOCAPOCI}{\FASTsunflowFTOCAPODynamic}{\FASTsunflowFTOCAPODynamicCI}	& \sdr{\FASTsunflowRECAPO}{\FASTsunflowRECAPOCI}{\FASTsunflowRECAPODynamic}{\FASTsunflowRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWtomcatHB}{\SLOWtomcatHBCI}{\SLOWtomcatHBDynamic}{\SLOWtomcatHBDynamicCI}					& \sdr{\FASTtomcatFTOHB}{\FASTtomcatFTOHBCI}{\FASTtomcatFTOHBDynamic}{\FASTtomcatFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWtomcatWCP}{\SLOWtomcatWCPCI}{\SLOWtomcatWCPDynamic}{\SLOWtomcatWCPDynamicCI}				& \sdr{\FASTtomcatFTOWCP}{\FASTtomcatFTOWCPCI}{\FASTtomcatFTOWCPDynamic}{\FASTtomcatFTOWCPDynamicCI}		& \sdr{\FASTtomcatREWCP}{\FASTtomcatREWCPCI}{\FASTtomcatREWCPDynamic}{\FASTtomcatREWCPDynamicCI} \\
\DC		& \sdr{\SLOWtomcatDCExc}{\SLOWtomcatDCExcCI}{\SLOWtomcatDCExcDynamic}{\SLOWtomcatDCExcDynamicCI}		& \sdr{\SLOWtomcatDCnoGExc}{\SLOWtomcatDCnoGExcCI}{\SLOWtomcatDCnoGExcDynamic}{\SLOWtomcatDCnoGExcDynamicCI}	& \sdr{\FASTtomcatFTODC}{\FASTtomcatFTODCCI}{\FASTtomcatFTODCDynamic}{\FASTtomcatFTODCDynamicCI}		& \sdr{\FASTtomcatREDC}{\FASTtomcatREDCCI}{\FASTtomcatREDCDynamic}{\FASTtomcatREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWtomcatCAPOExc}{\SLOWtomcatCAPOExcCI}{\SLOWtomcatCAPOExcDynamic}{\SLOWtomcatCAPOExcDynamicCI}	& \sdr{\SLOWtomcatCAPOnoGExc}{\SLOWtomcatCAPOnoGExcCI}{\SLOWtomcatCAPOnoGExcDynamic}{\SLOWtomcatCAPOnoGExcDynamicCI}	& \sdr{\FASTtomcatFTOCAPO}{\FASTtomcatFTOCAPOCI}{\FASTtomcatFTOCAPODynamic}{\FASTtomcatFTOCAPODynamicCI}	& \sdr{\FASTtomcatRECAPO}{\FASTtomcatRECAPOCI}{\FASTtomcatRECAPODynamic}{\FASTtomcatRECAPODynamicCI} \\
        & \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWxalanHB}{\SLOWxalanHBCI}{\SLOWxalanHBDynamic}{\SLOWxalanHBDynamicCI}					& \sdr{\FASTxalanFTOHB}{\FASTxalanFTOHBCI}{\FASTxalanFTOHBDynamic}{\FASTxalanFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWxalanWCP}{\SLOWxalanWCPCI}{\SLOWxalanWCPDynamic}{\SLOWxalanWCPDynamicCI}				& \sdr{\FASTxalanFTOWCP}{\FASTxalanFTOWCPCI}{\FASTxalanFTOWCPDynamic}{\FASTxalanFTOWCPDynamicCI}		& \sdr{\FASTxalanREWCP}{\FASTxalanREWCPCI}{\FASTxalanREWCPDynamic}{\FASTxalanREWCPDynamicCI} \\
\DC		& \sdr{\SLOWxalanDCExc}{\SLOWxalanDCExcCI}{\SLOWxalanDCExcDynamic}{\SLOWxalanDCExcDynamicCI}		& \sdr{\SLOWxalanDCnoGExc}{\SLOWxalanDCnoGExcCI}{\SLOWxalanDCnoGExcDynamic}{\SLOWxalanDCnoGExcDynamicCI}	& \sdr{\FASTxalanFTODC}{\FASTxalanFTODCCI}{\FASTxalanFTODCDynamic}{\FASTxalanFTODCDynamicCI}		& \sdr{\FASTxalanREDC}{\FASTxalanREDCCI}{\FASTxalanREDCDynamic}{\FASTxalanREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWxalanCAPOExc}{\SLOWxalanCAPOExcCI}{\SLOWxalanCAPOExcDynamic}{\SLOWxalanCAPOExcDynamicCI}	& \sdr{\SLOWxalanCAPOnoGExc}{\SLOWxalanCAPOnoGExcCI}{\SLOWxalanCAPOnoGExcDynamic}{\SLOWxalanCAPOnoGExcDynamicCI}	& \sdr{\FASTxalanFTOCAPO}{\FASTxalanFTOCAPOCI}{\FASTxalanFTOCAPODynamic}{\FASTxalanFTOCAPODynamicCI}	& \sdr{\FASTxalanRECAPO}{\FASTxalanRECAPOCI}{\FASTxalanRECAPODynamic}{\FASTxalanRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\caption{Average races reported for counting races by field name and array type
for all analyses
with 95\% confidence intervals.}
\label{tab:race:allDaCapo:CI}
\end{table*}

\begin{table*}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{#1}
% \newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\baseMem}[1]{#1~MB} %base memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
\input{result-macros/PIP_slowTool_raceEdgeFix_fieldName}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
%\input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_fastTool_fieldRaces}
%
\small
\centering
\newcommand{\ics}{\;}
\begin{tabular}{@{}l|HHHHHlll|l@{\ics}l|l@{\ics}l@{}}
& \mc{2}{Z}{} & \mc{2}{Z}{} & \mc{1}{H}{Base} & \mc{3}{c|}{\HB} & \mc{2}{c|}{Unopt-\DC} & \mc{2}{c@{}}{Unopt-\CAPO} \\
Program & \mc{2}{Z}{Events} & \mc{2}{Z}{\#Thr} & \mc{1}{H}{time} & RR\FTTwoAbbrv & \FTTwoAbbrv & \FTO & w/ G & w/o G & w/ G & w/o G \\\hline 
\bench{avrora} 	& \et{\FASTavroraEvents}{\FASTavroraEventsCI}   & \enfp{\FASTavroraNoFPEvents}{\FASTavroraNoFPEventsCI}	& \FASTavroraTotalThreads 	& (\FASTavroraMaxLiveThreads)	& \base{\FASTavroraBase}   & \vci{\FASTavroraFT}{\FASTavroraFTCI}   & \vci{\FASTavroraHB}{\FASTavroraHBCI}	& \vci{\FASTavroraFTOHB}{\FASTavroraFTOHBCI}	& \vci{\SLOWavroraDCExc}{\SLOWavroraDCExcCI}	& \vci{\SLOWavroraDCnoGExc}{\SLOWavroraDCnoGExcCI}	& \vci{\SLOWavroraCAPOExc}{\SLOWavroraCAPOExcCI}	& \vci{\SLOWavroraCAPOnoGExc}{\SLOWavroraCAPOnoGExcCI}\\
\bench{batik} 	& \et{\FASTbatikEvents}{\FASTbatikEventsCI}    & \enfp{\FASTbatikNoFPEvents}{\FASTbatikNoFPEventsCI}	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& \base{\FASTbatikBase}    & \vci{\FASTbatikFT}{\FASTbatikFTCI}    & \vci{\FASTbatikHB}{\FASTbatikHBCI}   	& \vci{\FASTbatikFTOHB}{\FASTbatikFTOHBCI}		& \vci{\SLOWbatikDCExc}{\SLOWbatikDCExcCI}	& \vci{\SLOWbatikDCnoGExc}{\SLOWbatikDCnoGExcCI}		& \vci{\SLOWbatikCAPOExc}{\SLOWbatikCAPOExcCI}	& \vci{\SLOWbatikCAPOnoGExc}{\SLOWbatikCAPOnoGExcCI} \\
\bench{h2} 		& \et{\FASThtwoEvents}{\FASThtwoEventsCI}     & \enfp{\FASThtwoNoFPEvents}{\FASThtwoNoFPEventsCI}	    & \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & \base{\FASThtwoBase}     & \vci{\FASThtwoFT}{\FASThtwoFTCI}     & \vci{\FASThtwoHB}{\FASThtwoHBCI}    	& \vci{\FASThtwoFTOHB}{\FASThtwoFTOHBCI}		& \vci{\SLOWhtwoDCExc}{\SLOWhtwoDCExcCI}		& \vci{\SLOWhtwoDCnoGExc}{\SLOWhtwoDCnoGExcCI}		& \vci{\SLOWhtwoCAPOExc}{\SLOWhtwoCAPOExcCI}	& \vci{\SLOWhtwoCAPOnoGExc}{\SLOWhtwoCAPOnoGExcCI}\\
\bench{jython} 	& \et{\FASTjythonEvents}{\FASTjythonEventsCI}   & \enfp{\FASTjythonNoFPEvents}{\FASTjythonNoFPEventsCI}	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& \base{\FASTjythonBase}   & \vci{\FASTjythonFT}{\FASTjythonFTCI}   & \vci{\FASTjythonHB}{\FASTjythonHBCI} 	& \vci{\FASTjythonFTOHB}{\FASTjythonFTOHBCI}	& \vci{\SLOWjythonDCExc}{\SLOWjythonDCExcCI}	& \vci{\SLOWjythonDCnoGExc}{\SLOWjythonDCnoGExcCI}	& \vci{\SLOWjythonCAPOExc}{\SLOWjythonCAPOExcCI}	& \vci{\SLOWjythonCAPOnoGExc}{\SLOWjythonCAPOnoGExcCI} \\
\bench{luindex} & \et{\FASTluindexEvents}{\FASTluindexEventsCI}  & \enfp{\FASTluindexNoFPEvents}{\FASTluindexNoFPEventsCI}	& \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& \base{\FASTluindexBase}  & \vci{\FASTluindexFT}{\FASTluindexFTCI}  & \vci{\FASTluindexHB}{\FASTluindexHBCI} 	& \vci{\FASTluindexFTOHB}{\FASTluindexFTOHBCI}	& \vci{\SLOWluindexDCExc}{\SLOWluindexDCExcCI}	& \vci{\SLOWluindexDCnoGExc}{\SLOWluindexDCnoGExcCI}	& \vci{\SLOWluindexCAPOExc}{\SLOWluindexCAPOExcCI}	& \vci{\SLOWluindexCAPOnoGExc}{\SLOWluindexCAPOnoGExcCI} \\
\bench{lusearch}& \et{\FASTlusearchEvents}{\FASTlusearchEventsCI} & \enfp{\FASTlusearchNoFPEvents}{\FASTlusearchNoFPEventsCI}	& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& \base{\FASTlusearchBase} & \vci{\FASTlusearchFT}{\FASTlusearchFTCI} & \vci{\FASTlusearchHB}{\FASTlusearchHBCI}	& \vci{\FASTlusearchFTOHB}{\FASTlusearchFTOHBCI}	& \vci{\SLOWlusearchDCExc}{\SLOWlusearchDCExcCI}	& \vci{\SLOWlusearchDCnoGExc}{\SLOWlusearchDCnoGExcCI}	& \vci{\SLOWlusearchCAPOExc}{\SLOWlusearchCAPOExcCI}& \vci{\SLOWlusearchCAPOnoGExc}{\SLOWlusearchCAPOnoGExcCI} \\
\bench{pmd}		& \et{\FASTpmdEvents}{\FASTpmdEventsCI}      & \enfp{\FASTpmdNoFPEvents}{\FASTpmdNoFPEventsCI}      & \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & \base{\FASTpmdBase}      & \vci{\FASTpmdFT}{\FASTpmdFTCI}      & \vci{\FASTpmdHB}{\FASTpmdHBCI}		& \vci{\FASTpmdFTOHB}{\FASTpmdFTOHBCI}		& \vci{\SLOWpmdDCExc}{\SLOWpmdDCExcCI}		& \vci{\SLOWpmdDCnoGExc}{\SLOWpmdDCnoGExcCI}		& \vci{\SLOWpmdCAPOExc}{\SLOWpmdCAPOExcCI}		& \vci{\SLOWpmdCAPOnoGExc}{\SLOWpmdCAPOnoGExcCI} \\
\bench{sunflow} & \et{\FASTsunflowEvents}{\FASTsunflowEventsCI}  & \enfp{\FASTsunflowNoFPEvents}{\FASTsunflowNoFPEventsCI}	& \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& \base{\FASTsunflowBase}  & \vci{\FASTsunflowFT}{\FASTsunflowFTCI}  & \vci{\FASTsunflowHB}{\FASTsunflowHBCI}	& \vci{\FASTsunflowFTOHB}{\FASTsunflowFTOHBCI}	& \vci{\SLOWsunflowDCExc}{\SLOWsunflowDCExcCI}	& \vci{\SLOWsunflowDCnoGExc}{\SLOWsunflowDCnoGExcCI}	& \vci{\SLOWsunflowCAPOExc}{\SLOWsunflowCAPOExcCI}	& \vci{\SLOWsunflowCAPOnoGExc}{\SLOWsunflowCAPOnoGExcCI} \\
% \bench{tomcat} 	& \et{\FASTtomcatEvents}{\FASTtomcatEventsCI}   & \enfp{\FASTtomcatNoFPEvents}{\FASTtomcatNoFPEventsCI}	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& \base{\FASTtomcatBase}   & \vci{\FASTtomcatFT}{\FASTtomcatFTCI}   & \vci{\FASTtomcatHB}{\FASTtomcatHBCI} 	& \vci{\FASTtomcatFTOHB}{\FASTtomcatFTOHBCI}	& \vci{\SLOWtomcatDCExc}{\SLOWtomcatDCExcCI}	& \vci{\SLOWtomcatDCnoGExc}{\SLOWtomcatDCnoGExcCI}	& \vci{\SLOWtomcatCAPOExc}{\SLOWtomcatCAPOExcCI}	& \vci{\SLOWtomcatCAPOnoGExc}{\SLOWtomcatCAPOnoGExcCI} \\
\bench{xalan} 	& \et{\FASTxalanEvents}{\FASTxalanEventsCI}    & \enfp{\FASTxalanNoFPEvents}{\FASTxalanNoFPEventsCI}	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& \base{\FASTxalanBase}    & \vci{\FASTxalanFT}{\FASTxalanFTCI}    & \vci{\FASTxalanHB}{\FASTxalanHBCI}		& \vci{\FASTxalanFTOHB}{\FASTxalanFTOHBCI}		& \vci{\SLOWxalanDCExc}{\SLOWxalanDCExcCI}	& \vci{\SLOWxalanDCnoGExc}{\SLOWxalanDCnoGExcCI} 	& \vci{\SLOWxalanCAPOExc}{\SLOWxalanCAPOExcCI}	& \vci{\SLOWxalanCAPOnoGExc}{\SLOWxalanCAPOnoGExcCI}\\\hline
% geomean	& &	& &	& & \roh{\FASTFTTimeGeoMean} & \roh{\FASTHBTimeGeoMean} & \roh{\FASTFTOHBTimeGeoMean} & \roh{\SLOWDCExcTimeGeoMean} & \roh{\SLOWDCnoGExcTimeGeoMean} & \roh{\SLOWCAPOExcTimeGeoMean} & \roh{\SLOWCAPOnoGExcTimeGeoMean} \\
\mc{1}{c}{} & \mc{12}{c}{Static Race Counts} \\
\end{tabular}

\mike{Commented out tomcat row so VSCode will stop complaining at me :)}

\caption{Static Race Counts for counting races by field name and array type
for all analyses with 95\% confidence intervals.}
\label{tab:performance:fasttrack:timeCI}
\end{table*}

\begin{table*}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{#1}
% \newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\baseMem}[1]{#1~MB} %base memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
\input{result-macros/PIP_slowTool_raceEdgeFix_fieldName}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
%\input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_fastTool_fieldRaces}
%
\small
\centering
\newcommand{\ics}{\;}
\begin{tabular}{@{}l|HHHHHlll|l@{\ics}l|l@{\ics}l@{}}
& \mc{2}{Z}{} & \mc{2}{Z}{} & \mc{1}{H}{Base} & \mc{3}{c|}{\HB} & \mc{2}{c|}{Unopt-\DC} & \mc{2}{c@{}}{Unopt-\CAPO} \\
Program & \mc{2}{Z}{Events} & \mc{2}{Z}{\#Thr} & \mc{1}{H}{time} & RR\FTTwoAbbrv & \FTTwoAbbrv & \FTO & w/ G & w/o G & w/ G & w/o G \\\hline 
\bench{avrora} 	& \et{\FASTavroraEvents}{\FASTavroraEventsCI}   & \enfp{\FASTavroraNoFPEvents}{\FASTavroraNoFPEventsCI}	& \FASTavroraTotalThreads 	& (\FASTavroraMaxLiveThreads)	& \base{\FASTavroraBase}   & \vci{\FASTavroraFTDynamic}{\FASTavroraFTDynamicCI}   & \vci{\FASTavroraHBDynamic}{\FASTavroraHBDynamicCI}	& \vci{\FASTavroraFTOHBDynamic}{\FASTavroraFTOHBDynamicCI}	& \vci{\SLOWavroraDCExcDynamic}{\SLOWavroraDCExcDynamicCI}	& \vci{\SLOWavroraDCnoGExcDynamic}{\SLOWavroraDCnoGExcDynamicCI}	& \vci{\SLOWavroraCAPOExcDynamic}{\SLOWavroraCAPOExcDynamicCI}	& \vci{\SLOWavroraCAPOnoGExcDynamic}{\SLOWavroraCAPOnoGExcDynamicCI}\\
\bench{batik} 	& \et{\FASTbatikEvents}{\FASTbatikEventsCI}    & \enfp{\FASTbatikNoFPEvents}{\FASTbatikNoFPEventsCI}	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& \base{\FASTbatikBase}    & \vci{\FASTbatikFTDynamic}{\FASTbatikFTDynamicCI}    & \vci{\FASTbatikHBDynamic}{\FASTbatikHBDynamicCI}   	& \vci{\FASTbatikFTOHBDynamic}{\FASTbatikFTOHBDynamicCI}		& \vci{\SLOWbatikDCExcDynamic}{\SLOWbatikDCExcDynamicCI}	& \vci{\SLOWbatikDCnoGExcDynamic}{\SLOWbatikDCnoGExcDynamicCI}		& \vci{\SLOWbatikCAPOExcDynamic}{\SLOWbatikCAPOExcDynamicCI}	& \vci{\SLOWbatikCAPOnoGExcDynamic}{\SLOWbatikCAPOnoGExcDynamicCI} \\
\bench{h2} 		& \et{\FASThtwoEvents}{\FASThtwoEventsCI}     & \enfp{\FASThtwoNoFPEvents}{\FASThtwoNoFPEventsCI}	    & \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & \base{\FASThtwoBase}     & \vci{\FASThtwoFTDynamic}{\FASThtwoFTDynamicCI}     & \vci{\FASThtwoHBDynamic}{\FASThtwoHBDynamicCI}    	& \vci{\FASThtwoFTOHBDynamic}{\FASThtwoFTOHBDynamicCI}		& \vci{\SLOWhtwoDCExcDynamic}{\SLOWhtwoDCExcDynamicCI}		& \vci{\SLOWhtwoDCnoGExcDynamic}{\SLOWhtwoDCnoGExcDynamicCI}		& \vci{\SLOWhtwoCAPOExcDynamic}{\SLOWhtwoCAPOExcDynamicCI}	& \vci{\SLOWhtwoCAPOnoGExcDynamic}{\SLOWhtwoCAPOnoGExcDynamicCI}\\
\bench{jython} 	& \et{\FASTjythonEvents}{\FASTjythonEventsCI}   & \enfp{\FASTjythonNoFPEvents}{\FASTjythonNoFPEventsCI}	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& \base{\FASTjythonBase}   & \vci{\FASTjythonFTDynamic}{\FASTjythonFTDynamicCI}   & \vci{\FASTjythonHBDynamic}{\FASTjythonHBDynamicCI} 	& \vci{\FASTjythonFTOHBDynamic}{\FASTjythonFTOHBDynamicCI}	& \vci{\SLOWjythonDCExcDynamic}{\SLOWjythonDCExcDynamicCI}	& \vci{\SLOWjythonDCnoGExcDynamic}{\SLOWjythonDCnoGExcDynamicCI}	& \vci{\SLOWjythonCAPOExcDynamic}{\SLOWjythonCAPOExcDynamicCI}	& \vci{\SLOWjythonCAPOnoGExcDynamic}{\SLOWjythonCAPOnoGExcDynamicCI} \\
\bench{luindex} & \et{\FASTluindexEvents}{\FASTluindexEventsCI}  & \enfp{\FASTluindexNoFPEvents}{\FASTluindexNoFPEventsCI}	& \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& \base{\FASTluindexBase}  & \vci{\FASTluindexFTDynamic}{\FASTluindexFTDynamicCI}  & \vci{\FASTluindexHBDynamic}{\FASTluindexHBDynamicCI} 	& \vci{\FASTluindexFTOHBDynamic}{\FASTluindexFTOHBDynamicCI}	& \vci{\SLOWluindexDCExcDynamic}{\SLOWluindexDCExcDynamicCI}	& \vci{\SLOWluindexDCnoGExcDynamic}{\SLOWluindexDCnoGExcDynamicCI}	& \vci{\SLOWluindexCAPOExcDynamic}{\SLOWluindexCAPOExcDynamicCI}	& \vci{\SLOWluindexCAPOnoGExcDynamic}{\SLOWluindexCAPOnoGExcDynamicCI} \\
\bench{lusearch}& \et{\FASTlusearchEvents}{\FASTlusearchEventsCI} & \enfp{\FASTlusearchNoFPEvents}{\FASTlusearchNoFPEventsCI}	& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& \base{\FASTlusearchBase} & \vci{\FASTlusearchFTDynamic}{\FASTlusearchFTDynamicCI} & \vci{\FASTlusearchHBDynamic}{\FASTlusearchHBDynamicCI}	& \vci{\FASTlusearchFTOHBDynamic}{\FASTlusearchFTOHBDynamicCI}	& \vci{\SLOWlusearchDCExcDynamic}{\SLOWlusearchDCExcDynamicCI}	& \vci{\SLOWlusearchDCnoGExcDynamic}{\SLOWlusearchDCnoGExcDynamicCI}	& \vci{\SLOWlusearchCAPOExcDynamic}{\SLOWlusearchCAPOExcDynamicCI}& \vci{\SLOWlusearchCAPOnoGExcDynamic}{\SLOWlusearchCAPOnoGExcDynamicCI} \\
\bench{pmd}		& \et{\FASTpmdEvents}{\FASTpmdEventsCI}      & \enfp{\FASTpmdNoFPEvents}{\FASTpmdNoFPEventsCI}      & \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & \base{\FASTpmdBase}      & \vci{\FASTpmdFTDynamic}{\FASTpmdFTDynamicCI}      & \vci{\FASTpmdHBDynamic}{\FASTpmdHBDynamicCI}		& \vci{\FASTpmdFTOHBDynamic}{\FASTpmdFTOHBDynamicCI}		& \vci{\SLOWpmdDCExcDynamic}{\SLOWpmdDCExcDynamicCI}		& \vci{\SLOWpmdDCnoGExcDynamic}{\SLOWpmdDCnoGExcDynamicCI}		& \vci{\SLOWpmdCAPOExcDynamic}{\SLOWpmdCAPOExcDynamicCI}		& \vci{\SLOWpmdCAPOnoGExcDynamic}{\SLOWpmdCAPOnoGExcDynamicCI} \\
\bench{sunflow} & \et{\FASTsunflowEvents}{\FASTsunflowEventsCI}  & \enfp{\FASTsunflowNoFPEvents}{\FASTsunflowNoFPEventsCI}	& \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& \base{\FASTsunflowBase}  & \vci{\FASTsunflowFTDynamic}{\FASTsunflowFTDynamicCI}  & \vci{\FASTsunflowHBDynamic}{\FASTsunflowHBDynamicCI}	& \vci{\FASTsunflowFTOHBDynamic}{\FASTsunflowFTOHBDynamicCI}	& \vci{\SLOWsunflowDCExcDynamic}{\SLOWsunflowDCExcDynamicCI}	& \vci{\SLOWsunflowDCnoGExcDynamic}{\SLOWsunflowDCnoGExcDynamicCI}	& \vci{\SLOWsunflowCAPOExcDynamic}{\SLOWsunflowCAPOExcDynamicCI}	& \vci{\SLOWsunflowCAPOnoGExcDynamic}{\SLOWsunflowCAPOnoGExcDynamicCI} \\
% \bench{tomcat} 	& \et{\FASTtomcatEvents}{\FASTtomcatEventsCI}   & \enfp{\FASTtomcatNoFPEvents}{\FASTtomcatNoFPEventsCI}	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& \base{\FASTtomcatBase}   & \vci{\FASTtomcatFTDynamic}{\FASTtomcatFTDynamicCI}   & \vci{\FASTtomcatHBDynamic}{\FASTtomcatHBDynamicCI} 	& \vci{\FASTtomcatFTOHBDynamic}{\FASTtomcatFTOHBDynamicCI}	& \vci{\SLOWtomcatDCExcDynamic}{\SLOWtomcatDCExcDynamicCI}	& \vci{\SLOWtomcatDCnoGExcDynamic}{\SLOWtomcatDCnoGExcDynamicCI}	& \vci{\SLOWtomcatCAPOExcDynamic}{\SLOWtomcatCAPOExcDynamicCI}	& \vci{\SLOWtomcatCAPOnoGExcDynamic}{\SLOWtomcatCAPOnoGExcDynamicCI} \\
\bench{xalan} 	& \et{\FASTxalanEvents}{\FASTxalanEventsCI}    & \enfp{\FASTxalanNoFPEvents}{\FASTxalanNoFPEventsCI}	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& \base{\FASTxalanBase}    & \vci{\FASTxalanFTDynamic}{\FASTxalanFTDynamicCI}    & \vci{\FASTxalanHBDynamic}{\FASTxalanHBDynamicCI}		& \vci{\FASTxalanFTOHBDynamic}{\FASTxalanFTOHBDynamicCI}		& \vci{\SLOWxalanDCExcDynamic}{\SLOWxalanDCExcDynamicCI}	& \vci{\SLOWxalanDCnoGExcDynamic}{\SLOWxalanDCnoGExcDynamicCI} 	& \vci{\SLOWxalanCAPOExcDynamic}{\SLOWxalanCAPOExcDynamicCI}	& \vci{\SLOWxalanCAPOnoGExcDynamic}{\SLOWxalanCAPOnoGExcDynamicCI}\\\hline
% geomean	& &	& &	& & \roh{\FASTFTTimeGeoMean} & \roh{\FASTHBTimeGeoMean} & \roh{\FASTFTOHBTimeGeoMean} & \roh{\SLOWDCExcTimeGeoMean} & \roh{\SLOWDCnoGExcTimeGeoMean} & \roh{\SLOWCAPOExcTimeGeoMean} & \roh{\SLOWCAPOnoGExcTimeGeoMean} \\
\mc{1}{c}{} & \mc{12}{c}{Dynamic Race Counts} \\
\end{tabular}

\mike{Commented out tomcat row so VSCode will stop complaining at me :)}

\caption{Dynamic Race Counts for counting races by field name and array type
for all analyses with 95\% confidence intervals.}
\label{tab:performance:fasttrack:timeCI}
\end{table*}

%Unordered Pair counts
\begin{table}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{#1}
% \newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\baseMem}[1]{#1~MB} %base memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
% \input{result-macros/PIP_slowTool_raceEdgeFix_fieldName}
% \input{result-macros/PIP_fastTool_fieldRaces}
\input{result-macros/PIP_slowTool_noWriteOrReadRaceEdge_accessMetaUpdate_unorderedPairs}
\input{result-macros/PIP_fastTool_noWriteOrReadRaceEdge_accessMetaUpdate}
%
\small
\centering
\newcommand{\ics}{\;}
\begin{tabular}{@{}l|rr|rr|rr|rr@{}}
 & \mc{8}{c}{Statically distinct races (dynamic races)} \\
Program & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c}{\CAPO-races} \\\hline
% Program & \mc{2}{Z}{Events} & \mc{2}{Z}{\#Thr} & \mc{1}{H}{time} & RR\FTTwoAbbrv & \FTTwoAbbrv & \FTO & w/ G & w/o G & w/ G & w/o G \\\hline 
\bench{avrora} 	& \SLOWavroraHB	& (\SLOWavroraHBDynamic)		& \SLOWavroraWCP	& (\SLOWavroraWCPDynamic) & \SLOWavroraDCnoGExc	& (\SLOWavroraDCnoGExcDynamic)		& \SLOWavroraCAPOnoGExc	& (\SLOWavroraCAPOnoGExcDynamic) \\
\bench{batik} 	& \SLOWbatikHB	& (\SLOWbatikHBDynamic)		& \SLOWbatikWCP		& (\SLOWbatikWCPDynamic) & \SLOWbatikDCnoGExc	& (\SLOWbatikDCnoGExcDynamic)		& \SLOWbatikCAPOnoGExc		& (\SLOWbatikCAPOnoGExcDynamic) \\
\bench{h2} 		& \SLOWhtwoHB	& (\SLOWhtwoHBDynamic)		& \SLOWhtwoWCP		& (\SLOWhtwoWCPDynamic) & \SLOWhtwoDCnoGExc	& (\SLOWhtwoDCnoGExcDynamic)		& \SLOWhtwoCAPOnoGExc		& (\SLOWhtwoCAPOnoGExcDynamic) \\
\bench{jython} 	& \SLOWjythonHB	& (\SLOWjythonHBDynamic)		& \SLOWjythonWCP	& (\SLOWjythonWCPDynamic) & \SLOWjythonDCnoGExc	& (\SLOWjythonDCnoGExcDynamic)		& \SLOWjythonCAPOnoGExc	& (\SLOWjythonCAPOnoGExcDynamic) \\
\bench{luindex} & \SLOWluindexHB	& (\SLOWluindexHBDynamic)	& \SLOWluindexWCP	& (\SLOWluindexWCPDynamic) & \SLOWluindexDCnoGExc	& (\SLOWluindexDCnoGExcDynamic)	& \SLOWluindexCAPOnoGExc	& (\SLOWluindexCAPOnoGExcDynamic) \\
\bench{lusearch}& \SLOWlusearchHB & (\SLOWlusearchHBDynamic)	& \SLOWlusearchWCP	& (\SLOWlusearchWCPDynamic) & \SLOWlusearchDCnoGExc& (\SLOWlusearchDCnoGExcDynamic)	& \SLOWlusearchCAPOnoGExc	& (\SLOWlusearchCAPOnoGExcDynamic) \\
\bench{pmd}		& \SLOWpmdHB		& (\SLOWpmdHBDynamic)		& \SLOWpmdWCP		& (\SLOWpmdWCPDynamic) & \SLOWpmdDCnoGExc		& (\SLOWpmdDCnoGExcDynamic)		& \SLOWpmdCAPOnoGExc		& (\SLOWpmdCAPOnoGExcDynamic) \\
\bench{sunflow} & \SLOWsunflowHB	& (\SLOWsunflowHBDynamic)	& \SLOWsunflowWCP	& (\SLOWsunflowWCPDynamic) & \SLOWsunflowDCnoGExc	& (\SLOWsunflowDCnoGExcDynamic)	& \SLOWsunflowCAPOnoGExc	& (\SLOWsunflowCAPOnoGExcDynamic) \\
\bench{tomcat} 	& \SLOWtomcatHB	& (\SLOWtomcatHBDynamic)		& \SLOWtomcatWCP	& (\SLOWtomcatWCPDynamic) & \SLOWtomcatDCnoGExc	& (\SLOWtomcatDCnoGExcDynamic)		& \SLOWtomcatCAPOnoGExc	& (\SLOWtomcatCAPOnoGExcDynamic) \\
\bench{xalan} 	& \SLOWxalanHB	& (\SLOWxalanHBDynamic) 		& \SLOWxalanWCP		& (\SLOWxalanWCPDynamic) & \SLOWxalanDCnoGExc	& (\SLOWxalanDCnoGExcDynamic) 		& \SLOWxalanCAPOnoGExc		& (\SLOWxalanCAPOnoGExcDynamic) \\\hline
Total & \SLOWHBTotal & (\SLOWHBDynamicTotal) & \SLOWWCPTotal & (\SLOWWCPDynamicTotal) & \SLOWDCnoGExcTotal & (\SLOWDCnoGExcDynamicTotal) & \SLOWCAPOnoGExcTotal & (\SLOWCAPOnoGExcDynamicTotal)
% geomean	& &	& &	& & \roh{\FASTFTTimeGeoMean} & \roh{\FASTHBTimeGeoMean} & \roh{\FASTFTOHBTimeGeoMean} & \roh{\SLOWDCExcTimeGeoMean} & \roh{\SLOWDCnoGExcTimeGeoMean} & \roh{\SLOWCAPOExcTimeGeoMean} & \roh{\SLOWCAPOnoGExcTimeGeoMean} \\
\end{tabular}

\caption{Static and dynamic Race Counts for counting races by unordered pairs
for all analyses.}
\label{tab:performance:fasttrack:timeCI}
\end{table}

%Unordered Pair counts
\begin{table}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{#1}
% \newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\baseMem}[1]{#1~MB} %base memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
% \input{result-macros/PIP_slowTool_raceEdgeFix_fieldName}
% \input{result-macros/PIP_fastTool_fieldRaces}
\input{result-macros/PIP_slowTool_noWriteOrReadRaceEdge_accessMetaUpdate_unorderedPairs}
% \input{result-macros/PIP_fastTool_noWriteOrReadRaceEdge_accessMetaUpdate}
%
\small
\centering
\newcommand{\ics}{\;}
\begin{tabular}{@{}l|rr|rr|rr|rr@{}}
 & \mc{8}{c}{Statically distinct races (dynamic races)} \\
Program & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c}{\CAPO-races} \\\hline
% Program & \mc{2}{Z}{Events} & \mc{2}{Z}{\#Thr} & \mc{1}{H}{time} & RR\FTTwoAbbrv & \FTTwoAbbrv & \FTO & w/ G & w/o G & w/ G & w/o G \\\hline 
\bench{avrora} 	& \SLOWavroraHBCI	& (\SLOWavroraHBDynamicCI)		& \SLOWavroraWCPCI	& (\SLOWavroraWCPDynamicCI) & \SLOWavroraDCnoGExcCI	& (\SLOWavroraDCnoGExcDynamicCI)		& \SLOWavroraCAPOnoGExcCI	& (\SLOWavroraCAPOnoGExcDynamicCI) \\
\bench{batik} 	& \SLOWbatikHBCI	& (\SLOWbatikHBDynamicCI)		& \SLOWbatikWCPCI		& (\SLOWbatikWCPDynamicCI) & \SLOWbatikDCnoGExcCI	& (\SLOWbatikDCnoGExcDynamicCI)		& \SLOWbatikCAPOnoGExcCI		& (\SLOWbatikCAPOnoGExcDynamicCI) \\
\bench{h2} 		& \SLOWhtwoHBCI	& (\SLOWhtwoHBDynamicCI)		& \SLOWhtwoWCPCI		& (\SLOWhtwoWCPDynamicCI) & \SLOWhtwoDCnoGExcCI	& (\SLOWhtwoDCnoGExcDynamicCI)		& \SLOWhtwoCAPOnoGExcCI		& (\SLOWhtwoCAPOnoGExcDynamicCI) \\
\bench{jython} 	& \SLOWjythonHBCI	& (\SLOWjythonHBDynamicCI)		& \SLOWjythonWCPCI	& (\SLOWjythonWCPDynamicCI) & \SLOWjythonDCnoGExcCI	& (\SLOWjythonDCnoGExcDynamicCI)		& \SLOWjythonCAPOnoGExcCI	& (\SLOWjythonCAPOnoGExcDynamicCI) \\
\bench{luindex} & \SLOWluindexHBCI	& (\SLOWluindexHBDynamicCI)	& \SLOWluindexWCPCI	& (\SLOWluindexWCPDynamicCI) & \SLOWluindexDCnoGExcCI	& (\SLOWluindexDCnoGExcDynamicCI)	& \SLOWluindexCAPOnoGExcCI	& (\SLOWluindexCAPOnoGExcDynamicCI) \\
\bench{lusearch}& \SLOWlusearchHBCI & (\SLOWlusearchHBDynamicCI)	& \SLOWlusearchWCPCI	& (\SLOWlusearchWCPDynamicCI) & \SLOWlusearchDCnoGExcCI& (\SLOWlusearchDCnoGExcDynamicCI)	& \SLOWlusearchCAPOnoGExcCI	& (\SLOWlusearchCAPOnoGExcDynamicCI) \\
\bench{pmd}		& \SLOWpmdHBCI		& (\SLOWpmdHBDynamicCI)		& \SLOWpmdWCPCI		& (\SLOWpmdWCPDynamicCI) & \SLOWpmdDCnoGExcCI		& (\SLOWpmdDCnoGExcDynamicCI)		& \SLOWpmdCAPOnoGExcCI		& (\SLOWpmdCAPOnoGExcDynamicCI) \\
\bench{sunflow} & \SLOWsunflowHBCI	& (\SLOWsunflowHBDynamicCI)	& \SLOWsunflowWCPCI	& (\SLOWsunflowWCPDynamicCI) & \SLOWsunflowDCnoGExcCI	& (\SLOWsunflowDCnoGExcDynamicCI)	& \SLOWsunflowCAPOnoGExcCI	& (\SLOWsunflowCAPOnoGExcDynamicCI) \\
\bench{tomcat} 	& \SLOWtomcatHBCI	& (\SLOWtomcatHBDynamicCI)		& \SLOWtomcatWCPCI	& (\SLOWtomcatWCPDynamicCI) & \SLOWtomcatDCnoGExcCI	& (\SLOWtomcatDCnoGExcDynamicCI)		& \SLOWtomcatCAPOnoGExcCI	& (\SLOWtomcatCAPOnoGExcDynamicCI) \\
\bench{xalan} 	& \SLOWxalanHBCI	& (\SLOWxalanHBDynamicCI) 		& \SLOWxalanWCPCI		& (\SLOWxalanWCPDynamicCI) & \SLOWxalanDCnoGExcCI	& (\SLOWxalanDCnoGExcDynamicCI) 		& \SLOWxalanCAPOnoGExcCI		& (\SLOWxalanCAPOnoGExcDynamicCI) \\\hline
% geomean	& &	& &	& & \roh{\FASTFTTimeGeoMean} & \roh{\FASTHBTimeGeoMean} & \roh{\FASTFTOHBTimeGeoMean} & \roh{\SLOWDCExcTimeGeoMean} & \roh{\SLOWDCnoGExcTimeGeoMean} & \roh{\SLOWCAPOExcTimeGeoMean} & \roh{\SLOWCAPOnoGExcTimeGeoMean} \\
\end{tabular}

\caption{Static and dynamic Confidence Intervals for 95\% Race Counts
for counting races by unordered pairs for all analyses.}
\label{tab:performance:fasttrack:timeCI}
\end{table}

%Run time for Unordered Pair counts
\begin{table}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{#1}
% \newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\baseMem}[1]{#1~MB} %base memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
% \input{result-macros/PIP_slowTool_raceEdgeFix_fieldName}
% \input{result-macros/PIP_fastTool_fieldRaces}
\input{result-macros/PIP_slowTool_noWriteOrReadRaceEdge_accessMetaUpdate_unorderedPairs}
\input{result-macros/PIP_fastTool_noWriteOrReadRaceEdge_accessMetaUpdate}
%
\small
\centering
\newcommand{\ics}{\;}
\begin{tabular}{@{}l|rr|rr|rr|rr@{}}
 & \mc{8}{c}{Statically distinct races (dynamic races)} \\
Program & \mc{2}{c|}{\HB-races} & \mc{2}{c|}{\WCP-races} & \mc{2}{c|}{\DC-races} & \mc{2}{c}{\CAPO-races} \\\hline
% Program & \mc{2}{Z}{Events} & \mc{2}{Z}{\#Thr} & \mc{1}{H}{time} & RR\FTTwoAbbrv & \FTTwoAbbrv & \FTO & w/ G & w/o G & w/ G & w/o G \\\hline 
\bench{avrora} 	& \SLOWavroraHBTime	& (\SLOWavroraHBTimeDynamic)		& \SLOWavroraWCPTime	& (\SLOWavroraWCPTimeDynamic) & \SLOWavroraDCnoGExcTime	& (\SLOWavroraDCnoGExcTimeDynamic)		& \SLOWavroraCAPOnoGExcTime	& (\SLOWavroraCAPOnoGExcTimeDynamic) \\
\bench{batik} 	& \SLOWbatikHBTime	& (\SLOWbatikHBTimeDynamic)		& \SLOWbatikWCPTime		& (\SLOWbatikWCPTimeDynamic) & \SLOWbatikDCnoGExcTime	& (\SLOWbatikDCnoGExcTimeDynamic)		& \SLOWbatikCAPOnoGExcTime		& (\SLOWbatikCAPOnoGExcTimeDynamic) \\
\bench{h2} 		& \SLOWhtwoHBTime	& (\SLOWhtwoHBTimeDynamic)		& \SLOWhtwoWCPTime		& (\SLOWhtwoWCPTimeDynamic) & \SLOWhtwoDCnoGExcTime	& (\SLOWhtwoDCnoGExcTimeDynamic)		& \SLOWhtwoCAPOnoGExcTime		& (\SLOWhtwoCAPOnoGExcTimeDynamic) \\
\bench{jython} 	& \SLOWjythonHBTime	& (\SLOWjythonHBTimeDynamic)		& \SLOWjythonWCPTime	& (\SLOWjythonWCPTimeDynamic) & \SLOWjythonDCnoGExcTime	& (\SLOWjythonDCnoGExcTimeDynamic)		& \SLOWjythonCAPOnoGExcTime	& (\SLOWjythonCAPOnoGExcTimeDynamic) \\
\bench{luindex} & \SLOWluindexHBTime	& (\SLOWluindexHBTimeDynamic)	& \SLOWluindexWCPTime	& (\SLOWluindexWCPTimeDynamic) & \SLOWluindexDCnoGExcTime	& (\SLOWluindexDCnoGExcTimeDynamic)	& \SLOWluindexCAPOnoGExcTime	& (\SLOWluindexCAPOnoGExcTimeDynamic) \\
\bench{lusearch}& \SLOWlusearchHBTime & (\SLOWlusearchHBTimeDynamic)	& \SLOWlusearchWCPTime	& (\SLOWlusearchWCPTimeDynamic) & \SLOWlusearchDCnoGExcTime& (\SLOWlusearchDCnoGExcTimeDynamic)	& \SLOWlusearchCAPOnoGExcTime	& (\SLOWlusearchCAPOnoGExcTimeDynamic) \\
\bench{pmd}		& \SLOWpmdHBTime		& (\SLOWpmdHBTimeDynamic)		& \SLOWpmdWCPTime		& (\SLOWpmdWCPTimeDynamic) & \SLOWpmdDCnoGExcTime		& (\SLOWpmdDCnoGExcTimeDynamic)		& \SLOWpmdCAPOnoGExcTime		& (\SLOWpmdCAPOnoGExcTimeDynamic) \\
\bench{sunflow} & \SLOWsunflowHBTime	& (\SLOWsunflowHBTimeDynamic)	& \SLOWsunflowWCPTime	& (\SLOWsunflowWCPTimeDynamic) & \SLOWsunflowDCnoGExcTime	& (\SLOWsunflowDCnoGExcTimeDynamic)	& \SLOWsunflowCAPOnoGExcTime	& (\SLOWsunflowCAPOnoGExcTimeDynamic) \\
\bench{tomcat} 	& \SLOWtomcatHBTime	& (\SLOWtomcatHBTimeDynamic)		& \SLOWtomcatWCPTime	& (\SLOWtomcatWCPTimeDynamic) & \SLOWtomcatDCnoGExcTime	& (\SLOWtomcatDCnoGExcTimeDynamic)		& \SLOWtomcatCAPOnoGExcTime	& (\SLOWtomcatCAPOnoGExcTimeDynamic) \\
\bench{xalan} 	& \SLOWxalanHBTime	& (\SLOWxalanHBTimeDynamic) 		& \SLOWxalanWCPTime		& (\SLOWxalanWCPTimeDynamic) & \SLOWxalanDCnoGExcTime	& (\SLOWxalanDCnoGExcTimeDynamic) 		& \SLOWxalanCAPOnoGExcTime		& (\SLOWxalanCAPOnoGExcTimeDynamic) \\\hline
Total & \SLOWHBTimeGeoMean & (\SLOWHBDynamicTotal) & \SLOWWCPTimeGeoMean & (\SLOWWCPDynamicTotal) & \SLOWDCnoGExcTimeGeoMean & (\SLOWDCnoGExcDynamicTotal) & \SLOWCAPOnoGExcTimeGeoMean & (\SLOWCAPOnoGExcDynamicTotal)
% geomean	& &	& &	& & \roh{\FASTFTTimeGeoMean} & \roh{\FASTHBTimeGeoMean} & \roh{\FASTFTOHBTimeGeoMean} & \roh{\SLOWDCExcTimeGeoMean} & \roh{\SLOWDCnoGExcTimeGeoMean} & \roh{\SLOWCAPOExcTimeGeoMean} & \roh{\SLOWCAPOnoGExcTimeGeoMean} \\
\end{tabular}

\caption{Run time for all analyses.}
\label{tab:performance:fasttrack:timeCI}
\end{table}

\begin{table}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{#1}
% \newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\baseMem}[1]{#1~MB} %base memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
\input{result-macros/PIP_slowTool_raceEdgeFix_fieldName}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
%\input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_fastTool_fieldRaces}
%
\small
\centering
\newcommand{\ics}{\;}
\begin{tabular}{@{}l|HHHHHlll|l@{\ics}l|l@{\ics}l@{}}
& \mc{2}{Z}{} & \mc{2}{Z}{} & \mc{1}{H}{Base} & \mc{3}{c|}{\HB} & \mc{2}{c|}{Unopt-\DC} & \mc{2}{c@{}}{Unopt-\CAPO} \\
Program & \mc{2}{Z}{Events} & \mc{2}{Z}{\#Thr} & \mc{1}{H}{time} & RR\FTTwoAbbrv & \FTTwoAbbrv & \FTO & w/ G & w/o G & w/ G & w/o G \\\hline 
\bench{avrora} 	& \et{\FASTavroraEvents}{\FASTavroraEventsCI}   & \enfp{\FASTavroraNoFPEvents}{\FASTavroraNoFPEventsCI}	& \FASTavroraTotalThreads 	& (\FASTavroraMaxLiveThreads)	& \base{\FASTavroraBase}   & \vci{\FASTavroraFTDynamic}{\FASTavroraFTDynamicCI}   & \vci{\FASTavroraHBDynamic}{\FASTavroraHBDynamicCI}	& \vci{\FASTavroraFTOHBDynamic}{\FASTavroraFTOHBDynamicCI}	& \vci{\SLOWavroraDCExcDynamic}{\SLOWavroraDCExcDynamicCI}	& \vci{\SLOWavroraDCnoGExcDynamic}{\SLOWavroraDCnoGExcDynamicCI}	& \vci{\SLOWavroraCAPOExcDynamic}{\SLOWavroraCAPOExcDynamicCI}	& \vci{\SLOWavroraCAPOnoGExcDynamic}{\SLOWavroraCAPOnoGExcDynamicCI}\\
\bench{batik} 	& \et{\FASTbatikEvents}{\FASTbatikEventsCI}    & \enfp{\FASTbatikNoFPEvents}{\FASTbatikNoFPEventsCI}	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& \base{\FASTbatikBase}    & \vci{\FASTbatikFTDynamic}{\FASTbatikFTDynamicCI}    & \vci{\FASTbatikHBDynamic}{\FASTbatikHBDynamicCI}   	& \vci{\FASTbatikFTOHBDynamic}{\FASTbatikFTOHBDynamicCI}		& \vci{\SLOWbatikDCExcDynamic}{\SLOWbatikDCExcDynamicCI}	& \vci{\SLOWbatikDCnoGExcDynamic}{\SLOWbatikDCnoGExcDynamicCI}		& \vci{\SLOWbatikCAPOExcDynamic}{\SLOWbatikCAPOExcDynamicCI}	& \vci{\SLOWbatikCAPOnoGExcDynamic}{\SLOWbatikCAPOnoGExcDynamicCI} \\
\bench{h2} 		& \et{\FASThtwoEvents}{\FASThtwoEventsCI}     & \enfp{\FASThtwoNoFPEvents}{\FASThtwoNoFPEventsCI}	    & \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & \base{\FASThtwoBase}     & \vci{\FASThtwoFTDynamic}{\FASThtwoFTDynamicCI}     & \vci{\FASThtwoHBDynamic}{\FASThtwoHBDynamicCI}    	& \vci{\FASThtwoFTOHBDynamic}{\FASThtwoFTOHBDynamicCI}		& \vci{\SLOWhtwoDCExcDynamic}{\SLOWhtwoDCExcDynamicCI}		& \vci{\SLOWhtwoDCnoGExcDynamic}{\SLOWhtwoDCnoGExcDynamicCI}		& \vci{\SLOWhtwoCAPOExcDynamic}{\SLOWhtwoCAPOExcDynamicCI}	& \vci{\SLOWhtwoCAPOnoGExcDynamic}{\SLOWhtwoCAPOnoGExcDynamicCI}\\
\bench{jython} 	& \et{\FASTjythonEvents}{\FASTjythonEventsCI}   & \enfp{\FASTjythonNoFPEvents}{\FASTjythonNoFPEventsCI}	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& \base{\FASTjythonBase}   & \vci{\FASTjythonFTDynamic}{\FASTjythonFTDynamicCI}   & \vci{\FASTjythonHBDynamic}{\FASTjythonHBDynamicCI} 	& \vci{\FASTjythonFTOHBDynamic}{\FASTjythonFTOHBDynamicCI}	& \vci{\SLOWjythonDCExcDynamic}{\SLOWjythonDCExcDynamicCI}	& \vci{\SLOWjythonDCnoGExcDynamic}{\SLOWjythonDCnoGExcDynamicCI}	& \vci{\SLOWjythonCAPOExcDynamic}{\SLOWjythonCAPOExcDynamicCI}	& \vci{\SLOWjythonCAPOnoGExcDynamic}{\SLOWjythonCAPOnoGExcDynamicCI} \\
\bench{luindex} & \et{\FASTluindexEvents}{\FASTluindexEventsCI}  & \enfp{\FASTluindexNoFPEvents}{\FASTluindexNoFPEventsCI}	& \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& \base{\FASTluindexBase}  & \vci{\FASTluindexFTDynamic}{\FASTluindexFTDynamicCI}  & \vci{\FASTluindexHBDynamic}{\FASTluindexHBDynamicCI} 	& \vci{\FASTluindexFTOHBDynamic}{\FASTluindexFTOHBDynamicCI}	& \vci{\SLOWluindexDCExcDynamic}{\SLOWluindexDCExcDynamicCI}	& \vci{\SLOWluindexDCnoGExcDynamic}{\SLOWluindexDCnoGExcDynamicCI}	& \vci{\SLOWluindexCAPOExcDynamic}{\SLOWluindexCAPOExcDynamicCI}	& \vci{\SLOWluindexCAPOnoGExcDynamic}{\SLOWluindexCAPOnoGExcDynamicCI} \\
\bench{lusearch}& \et{\FASTlusearchEvents}{\FASTlusearchEventsCI} & \enfp{\FASTlusearchNoFPEvents}{\FASTlusearchNoFPEventsCI}	& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& \base{\FASTlusearchBase} & \vci{\FASTlusearchFTDynamic}{\FASTlusearchFTDynamicCI} & \vci{\FASTlusearchHBDynamic}{\FASTlusearchHBDynamicCI}	& \vci{\FASTlusearchFTOHBDynamic}{\FASTlusearchFTOHBDynamicCI}	& \vci{\SLOWlusearchDCExcDynamic}{\SLOWlusearchDCExcDynamicCI}	& \vci{\SLOWlusearchDCnoGExcDynamic}{\SLOWlusearchDCnoGExcDynamicCI}	& \vci{\SLOWlusearchCAPOExcDynamic}{\SLOWlusearchCAPOExcDynamicCI}& \vci{\SLOWlusearchCAPOnoGExcDynamic}{\SLOWlusearchCAPOnoGExcDynamicCI} \\
\bench{pmd}		& \et{\FASTpmdEvents}{\FASTpmdEventsCI}      & \enfp{\FASTpmdNoFPEvents}{\FASTpmdNoFPEventsCI}      & \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & \base{\FASTpmdBase}      & \vci{\FASTpmdFTDynamic}{\FASTpmdFTDynamicCI}      & \vci{\FASTpmdHBDynamic}{\FASTpmdHBDynamicCI}		& \vci{\FASTpmdFTOHBDynamic}{\FASTpmdFTOHBDynamicCI}		& \vci{\SLOWpmdDCExcDynamic}{\SLOWpmdDCExcDynamicCI}		& \vci{\SLOWpmdDCnoGExcDynamic}{\SLOWpmdDCnoGExcDynamicCI}		& \vci{\SLOWpmdCAPOExcDynamic}{\SLOWpmdCAPOExcDynamicCI}		& \vci{\SLOWpmdCAPOnoGExcDynamic}{\SLOWpmdCAPOnoGExcDynamicCI} \\
\bench{sunflow} & \et{\FASTsunflowEvents}{\FASTsunflowEventsCI}  & \enfp{\FASTsunflowNoFPEvents}{\FASTsunflowNoFPEventsCI}	& \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& \base{\FASTsunflowBase}  & \vci{\FASTsunflowFTDynamic}{\FASTsunflowFTDynamicCI}  & \vci{\FASTsunflowHBDynamic}{\FASTsunflowHBDynamicCI}	& \vci{\FASTsunflowFTOHBDynamic}{\FASTsunflowFTOHBDynamicCI}	& \vci{\SLOWsunflowDCExcDynamic}{\SLOWsunflowDCExcDynamicCI}	& \vci{\SLOWsunflowDCnoGExcDynamic}{\SLOWsunflowDCnoGExcDynamicCI}	& \vci{\SLOWsunflowCAPOExcDynamic}{\SLOWsunflowCAPOExcDynamicCI}	& \vci{\SLOWsunflowCAPOnoGExcDynamic}{\SLOWsunflowCAPOnoGExcDynamicCI} \\
% \bench{tomcat} 	& \et{\FASTtomcatEvents}{\FASTtomcatEventsCI}   & \enfp{\FASTtomcatNoFPEvents}{\FASTtomcatNoFPEventsCI}	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& \base{\FASTtomcatBase}   & \vci{\FASTtomcatFTDynamic}{\FASTtomcatFTDynamicCI}   & \vci{\FASTtomcatHBDynamic}{\FASTtomcatHBDynamicCI} 	& \vci{\FASTtomcatFTOHBDynamic}{\FASTtomcatFTOHBDynamicCI}	& \vci{\SLOWtomcatDCExcDynamic}{\SLOWtomcatDCExcDynamicCI}	& \vci{\SLOWtomcatDCnoGExcDynamic}{\SLOWtomcatDCnoGExcDynamicCI}	& \vci{\SLOWtomcatCAPOExcDynamic}{\SLOWtomcatCAPOExcDynamicCI}	& \vci{\SLOWtomcatCAPOnoGExcDynamic}{\SLOWtomcatCAPOnoGExcDynamicCI} \\
\bench{xalan} 	& \et{\FASTxalanEvents}{\FASTxalanEventsCI}    & \enfp{\FASTxalanNoFPEvents}{\FASTxalanNoFPEventsCI}	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& \base{\FASTxalanBase}    & \vci{\FASTxalanFTDynamic}{\FASTxalanFTDynamicCI}    & \vci{\FASTxalanHBDynamic}{\FASTxalanHBDynamicCI}		& \vci{\FASTxalanFTOHBDynamic}{\FASTxalanFTOHBDynamicCI}		& \vci{\SLOWxalanDCExcDynamic}{\SLOWxalanDCExcDynamicCI}	& \vci{\SLOWxalanDCnoGExcDynamic}{\SLOWxalanDCnoGExcDynamicCI} 	& \vci{\SLOWxalanCAPOExcDynamic}{\SLOWxalanCAPOExcDynamicCI}	& \vci{\SLOWxalanCAPOnoGExcDynamic}{\SLOWxalanCAPOnoGExcDynamicCI}\\\hline
% geomean	& &	& &	& & \roh{\FASTFTTimeGeoMean} & \roh{\FASTHBTimeGeoMean} & \roh{\FASTFTOHBTimeGeoMean} & \roh{\SLOWDCExcTimeGeoMean} & \roh{\SLOWDCnoGExcTimeGeoMean} & \roh{\SLOWCAPOExcTimeGeoMean} & \roh{\SLOWCAPOnoGExcTimeGeoMean} \\
\mc{1}{c}{} & \mc{12}{c}{Dynamic Race Counts} \\
\end{tabular}

\caption{Dynamic Race Counts for counting races by unordered pairs
for all analyses with 95\% confidence intervals.}
\label{tab:performance:fasttrack:timeCI}
\end{table}

% No race edge second static site
\begin{table*}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{#1}
% \newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\baseMem}[1]{#1~MB} %base memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
%\input{result-macros/PIP_slowTool_raceEdgeFix_fieldName}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
%\input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_slowTool_noWriteOrReadRaceEdge}
\input{result-macros/PIP_fastTool_noWriteOrReadRaceEdge}
%
\small
\centering
\newcommand{\ics}{\;}
\begin{tabular}{@{}l|HHHHHlll|l@{\ics}l|l@{\ics}l@{}}
& \mc{2}{Z}{} & \mc{2}{Z}{} & \mc{1}{H}{Base} & \mc{3}{c|}{\HB} & \mc{2}{c|}{Unopt-\DC} & \mc{2}{c@{}}{Unopt-\CAPO} \\
Program & \mc{2}{Z}{Events} & \mc{2}{Z}{\#Thr} & \mc{1}{H}{time} & RR\FTTwoAbbrv & \FTTwoAbbrv & \FTO & w/ G & w/o G & w/ G & w/o G \\\hline 
\bench{avrora} 	& \et{\FASTavroraEvents}{\FASTavroraEventsCI}   & \enfp{\FASTavroraNoFPEvents}{\FASTavroraNoFPEventsCI}	& \FASTavroraTotalThreads 	& (\FASTavroraMaxLiveThreads)	& \base{\FASTavroraBase}   & \vci{\FASTavroraFT}{\FASTavroraFTCI}   & \vci{\FASTavroraHB}{\FASTavroraHBCI}	& \vci{\FASTavroraFTOHB}{\FASTavroraFTOHBCI}	& \vci{\SLOWavroraDCExc}{\SLOWavroraDCExcCI}	& \vci{\SLOWavroraDCnoGExc}{\SLOWavroraDCnoGExcCI}	& \vci{\SLOWavroraCAPOExc}{\SLOWavroraCAPOExcCI}	& \vci{\SLOWavroraCAPOnoGExc}{\SLOWavroraCAPOnoGExcCI}\\
\bench{batik} 	& \et{\FASTbatikEvents}{\FASTbatikEventsCI}    & \enfp{\FASTbatikNoFPEvents}{\FASTbatikNoFPEventsCI}	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& \base{\FASTbatikBase}    & \vci{\FASTbatikFT}{\FASTbatikFTCI}    & \vci{\FASTbatikHB}{\FASTbatikHBCI}   	& \vci{\FASTbatikFTOHB}{\FASTbatikFTOHBCI}		& \vci{\SLOWbatikDCExc}{\SLOWbatikDCExcCI}	& \vci{\SLOWbatikDCnoGExc}{\SLOWbatikDCnoGExcCI}		& \vci{\SLOWbatikCAPOExc}{\SLOWbatikCAPOExcCI}	& \vci{\SLOWbatikCAPOnoGExc}{\SLOWbatikCAPOnoGExcCI} \\
\bench{h2} 		& \et{\FASThtwoEvents}{\FASThtwoEventsCI}     & \enfp{\FASThtwoNoFPEvents}{\FASThtwoNoFPEventsCI}	    & \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & \base{\FASThtwoBase}     & \vci{\FASThtwoFT}{\FASThtwoFTCI}     & \vci{\FASThtwoHB}{\FASThtwoHBCI}    	& \vci{\FASThtwoFTOHB}{\FASThtwoFTOHBCI}		& \vci{\SLOWhtwoDCExc}{\SLOWhtwoDCExcCI}		& \vci{\SLOWhtwoDCnoGExc}{\SLOWhtwoDCnoGExcCI}		& \vci{\SLOWhtwoCAPOExc}{\SLOWhtwoCAPOExcCI}	& \vci{\SLOWhtwoCAPOnoGExc}{\SLOWhtwoCAPOnoGExcCI}\\
\bench{jython} 	& \et{\FASTjythonEvents}{\FASTjythonEventsCI}   & \enfp{\FASTjythonNoFPEvents}{\FASTjythonNoFPEventsCI}	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& \base{\FASTjythonBase}   & \vci{\FASTjythonFT}{\FASTjythonFTCI}   & \vci{\FASTjythonHB}{\FASTjythonHBCI} 	& \vci{\FASTjythonFTOHB}{\FASTjythonFTOHBCI}	& \vci{\SLOWjythonDCExc}{\SLOWjythonDCExcCI}	& \vci{\SLOWjythonDCnoGExc}{\SLOWjythonDCnoGExcCI}	& \vci{\SLOWjythonCAPOExc}{\SLOWjythonCAPOExcCI}	& \vci{\SLOWjythonCAPOnoGExc}{\SLOWjythonCAPOnoGExcCI} \\
\bench{luindex} & \et{\FASTluindexEvents}{\FASTluindexEventsCI}  & \enfp{\FASTluindexNoFPEvents}{\FASTluindexNoFPEventsCI}	& \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& \base{\FASTluindexBase}  & \vci{\FASTluindexFT}{\FASTluindexFTCI}  & \vci{\FASTluindexHB}{\FASTluindexHBCI} 	& \vci{\FASTluindexFTOHB}{\FASTluindexFTOHBCI}	& \vci{\SLOWluindexDCExc}{\SLOWluindexDCExcCI}	& \vci{\SLOWluindexDCnoGExc}{\SLOWluindexDCnoGExcCI}	& \vci{\SLOWluindexCAPOExc}{\SLOWluindexCAPOExcCI}	& \vci{\SLOWluindexCAPOnoGExc}{\SLOWluindexCAPOnoGExcCI} \\
\bench{lusearch}& \et{\FASTlusearchEvents}{\FASTlusearchEventsCI} & \enfp{\FASTlusearchNoFPEvents}{\FASTlusearchNoFPEventsCI}	& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& \base{\FASTlusearchBase} & \vci{\FASTlusearchFT}{\FASTlusearchFTCI} & \vci{\FASTlusearchHB}{\FASTlusearchHBCI}	& \vci{\FASTlusearchFTOHB}{\FASTlusearchFTOHBCI}	& \vci{\SLOWlusearchDCExc}{\SLOWlusearchDCExcCI}	& \vci{\SLOWlusearchDCnoGExc}{\SLOWlusearchDCnoGExcCI}	& \vci{\SLOWlusearchCAPOExc}{\SLOWlusearchCAPOExcCI}& \vci{\SLOWlusearchCAPOnoGExc}{\SLOWlusearchCAPOnoGExcCI} \\
\bench{pmd}		& \et{\FASTpmdEvents}{\FASTpmdEventsCI}      & \enfp{\FASTpmdNoFPEvents}{\FASTpmdNoFPEventsCI}      & \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & \base{\FASTpmdBase}      & \vci{\FASTpmdFT}{\FASTpmdFTCI}      & \vci{\FASTpmdHB}{\FASTpmdHBCI}		& \vci{\FASTpmdFTOHB}{\FASTpmdFTOHBCI}		& \vci{\SLOWpmdDCExc}{\SLOWpmdDCExcCI}		& \vci{\SLOWpmdDCnoGExc}{\SLOWpmdDCnoGExcCI}		& \vci{\SLOWpmdCAPOExc}{\SLOWpmdCAPOExcCI}		& \vci{\SLOWpmdCAPOnoGExc}{\SLOWpmdCAPOnoGExcCI} \\
\bench{sunflow} & \et{\FASTsunflowEvents}{\FASTsunflowEventsCI}  & \enfp{\FASTsunflowNoFPEvents}{\FASTsunflowNoFPEventsCI}	& \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& \base{\FASTsunflowBase}  & \vci{\FASTsunflowFT}{\FASTsunflowFTCI}  & \vci{\FASTsunflowHB}{\FASTsunflowHBCI}	& \vci{\FASTsunflowFTOHB}{\FASTsunflowFTOHBCI}	& \vci{\SLOWsunflowDCExc}{\SLOWsunflowDCExcCI}	& \vci{\SLOWsunflowDCnoGExc}{\SLOWsunflowDCnoGExcCI}	& \vci{\SLOWsunflowCAPOExc}{\SLOWsunflowCAPOExcCI}	& \vci{\SLOWsunflowCAPOnoGExc}{\SLOWsunflowCAPOnoGExcCI} \\
% \bench{tomcat} 	& \et{\FASTtomcatEvents}{\FASTtomcatEventsCI}   & \enfp{\FASTtomcatNoFPEvents}{\FASTtomcatNoFPEventsCI}	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& \base{\FASTtomcatBase}   & \vci{\FASTtomcatFT}{\FASTtomcatFTCI}   & \vci{\FASTtomcatHB}{\FASTtomcatHBCI} 	& \vci{\FASTtomcatFTOHB}{\FASTtomcatFTOHBCI}	& \vci{\SLOWtomcatDCExc}{\SLOWtomcatDCExcCI}	& \vci{\SLOWtomcatDCnoGExc}{\SLOWtomcatDCnoGExcCI}	& \vci{\SLOWtomcatCAPOExc}{\SLOWtomcatCAPOExcCI}	& \vci{\SLOWtomcatCAPOnoGExc}{\SLOWtomcatCAPOnoGExcCI} \\
\bench{xalan} 	& \et{\FASTxalanEvents}{\FASTxalanEventsCI}    & \enfp{\FASTxalanNoFPEvents}{\FASTxalanNoFPEventsCI}	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& \base{\FASTxalanBase}    & \vci{\FASTxalanFT}{\FASTxalanFTCI}    & \vci{\FASTxalanHB}{\FASTxalanHBCI}		& \vci{\FASTxalanFTOHB}{\FASTxalanFTOHBCI}		& \vci{\SLOWxalanDCExc}{\SLOWxalanDCExcCI}	& \vci{\SLOWxalanDCnoGExc}{\SLOWxalanDCnoGExcCI} 	& \vci{\SLOWxalanCAPOExc}{\SLOWxalanCAPOExcCI}	& \vci{\SLOWxalanCAPOnoGExc}{\SLOWxalanCAPOnoGExcCI}\\\hline
% geomean	& &	& &	& & \roh{\FASTFTTimeGeoMean} & \roh{\FASTHBTimeGeoMean} & \roh{\FASTFTOHBTimeGeoMean} & \roh{\SLOWDCExcTimeGeoMean} & \roh{\SLOWDCnoGExcTimeGeoMean} & \roh{\SLOWCAPOExcTimeGeoMean} & \roh{\SLOWCAPOnoGExcTimeGeoMean} \\
\mc{1}{c}{} & \mc{12}{c}{Static Race Counts} \\
\end{tabular}

\caption{Static Race Counts {\bf with no race edge} for counting races
by {\bf second static site} for all analyses with 95\% confidence intervals.}
\label{tab:performance:fasttrack:timeCI}
\end{table*}

\begin{table*}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{#1}
% \newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\baseMem}[1]{#1~MB} %base memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
%\input{result-macros/PIP_slowTool_raceEdgeFix_fieldName}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
%\input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_slowTool_noWriteOrReadRaceEdge}
\input{result-macros/PIP_fastTool_noWriteOrReadRaceEdge}
%
\smaller
\smaller
\centering
\newcommand{\ics}{\;}
\begin{tabular}{@{}l|HHHHHlll|l@{\ics}l|l@{\ics}l@{}}
& \mc{2}{Z}{} & \mc{2}{Z}{} & \mc{1}{H}{Base} & \mc{3}{c|}{\HB} & \mc{2}{c|}{Unopt-\DC} & \mc{2}{c@{}}{Unopt-\CAPO} \\
Program & \mc{2}{Z}{Events} & \mc{2}{Z}{\#Thr} & \mc{1}{H}{time} & RR\FTTwoAbbrv & \FTTwoAbbrv & \FTO & w/ G & w/o G & w/ G & w/o G \\\hline 
\bench{avrora} 	& \et{\FASTavroraEvents}{\FASTavroraEventsCI}   & \enfp{\FASTavroraNoFPEvents}{\FASTavroraNoFPEventsCI}	& \FASTavroraTotalThreads 	& (\FASTavroraMaxLiveThreads)	& \base{\FASTavroraBase}   & \vci{\FASTavroraFTDynamic}{\FASTavroraFTDynamicCI}   & \vci{\FASTavroraHBDynamic}{\FASTavroraHBDynamicCI}	& \vci{\FASTavroraFTOHBDynamic}{\FASTavroraFTOHBDynamicCI}	& \vci{\SLOWavroraDCExcDynamic}{\SLOWavroraDCExcDynamicCI}	& \vci{\SLOWavroraDCnoGExcDynamic}{\SLOWavroraDCnoGExcDynamicCI}	& \vci{\SLOWavroraCAPOExcDynamic}{\SLOWavroraCAPOExcDynamicCI}	& \vci{\SLOWavroraCAPOnoGExcDynamic}{\SLOWavroraCAPOnoGExcDynamicCI}\\
\bench{batik} 	& \et{\FASTbatikEvents}{\FASTbatikEventsCI}    & \enfp{\FASTbatikNoFPEvents}{\FASTbatikNoFPEventsCI}	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& \base{\FASTbatikBase}    & \vci{\FASTbatikFTDynamic}{\FASTbatikFTDynamicCI}    & \vci{\FASTbatikHBDynamic}{\FASTbatikHBDynamicCI}   	& \vci{\FASTbatikFTOHBDynamic}{\FASTbatikFTOHBDynamicCI}		& \vci{\SLOWbatikDCExcDynamic}{\SLOWbatikDCExcDynamicCI}	& \vci{\SLOWbatikDCnoGExcDynamic}{\SLOWbatikDCnoGExcDynamicCI}		& \vci{\SLOWbatikCAPOExcDynamic}{\SLOWbatikCAPOExcDynamicCI}	& \vci{\SLOWbatikCAPOnoGExcDynamic}{\SLOWbatikCAPOnoGExcDynamicCI} \\
\bench{h2} 		& \et{\FASThtwoEvents}{\FASThtwoEventsCI}     & \enfp{\FASThtwoNoFPEvents}{\FASThtwoNoFPEventsCI}	    & \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & \base{\FASThtwoBase}     & \vci{\FASThtwoFTDynamic}{\FASThtwoFTDynamicCI}     & \vci{\FASThtwoHBDynamic}{\FASThtwoHBDynamicCI}    	& \vci{\FASThtwoFTOHBDynamic}{\FASThtwoFTOHBDynamicCI}		& \vci{\SLOWhtwoDCExcDynamic}{\SLOWhtwoDCExcDynamicCI}		& \vci{\SLOWhtwoDCnoGExcDynamic}{\SLOWhtwoDCnoGExcDynamicCI}		& \vci{\SLOWhtwoCAPOExcDynamic}{\SLOWhtwoCAPOExcDynamicCI}	& \vci{\SLOWhtwoCAPOnoGExcDynamic}{\SLOWhtwoCAPOnoGExcDynamicCI}\\
\bench{jython} 	& \et{\FASTjythonEvents}{\FASTjythonEventsCI}   & \enfp{\FASTjythonNoFPEvents}{\FASTjythonNoFPEventsCI}	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& \base{\FASTjythonBase}   & \vci{\FASTjythonFTDynamic}{\FASTjythonFTDynamicCI}   & \vci{\FASTjythonHBDynamic}{\FASTjythonHBDynamicCI} 	& \vci{\FASTjythonFTOHBDynamic}{\FASTjythonFTOHBDynamicCI}	& \vci{\SLOWjythonDCExcDynamic}{\SLOWjythonDCExcDynamicCI}	& \vci{\SLOWjythonDCnoGExcDynamic}{\SLOWjythonDCnoGExcDynamicCI}	& \vci{\SLOWjythonCAPOExcDynamic}{\SLOWjythonCAPOExcDynamicCI}	& \vci{\SLOWjythonCAPOnoGExcDynamic}{\SLOWjythonCAPOnoGExcDynamicCI} \\
\bench{luindex} & \et{\FASTluindexEvents}{\FASTluindexEventsCI}  & \enfp{\FASTluindexNoFPEvents}{\FASTluindexNoFPEventsCI}	& \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& \base{\FASTluindexBase}  & \vci{\FASTluindexFTDynamic}{\FASTluindexFTDynamicCI}  & \vci{\FASTluindexHBDynamic}{\FASTluindexHBDynamicCI} 	& \vci{\FASTluindexFTOHBDynamic}{\FASTluindexFTOHBDynamicCI}	& \vci{\SLOWluindexDCExcDynamic}{\SLOWluindexDCExcDynamicCI}	& \vci{\SLOWluindexDCnoGExcDynamic}{\SLOWluindexDCnoGExcDynamicCI}	& \vci{\SLOWluindexCAPOExcDynamic}{\SLOWluindexCAPOExcDynamicCI}	& \vci{\SLOWluindexCAPOnoGExcDynamic}{\SLOWluindexCAPOnoGExcDynamicCI} \\
\bench{lusearch}& \et{\FASTlusearchEvents}{\FASTlusearchEventsCI} & \enfp{\FASTlusearchNoFPEvents}{\FASTlusearchNoFPEventsCI}	& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& \base{\FASTlusearchBase} & \vci{\FASTlusearchFTDynamic}{\FASTlusearchFTDynamicCI} & \vci{\FASTlusearchHBDynamic}{\FASTlusearchHBDynamicCI}	& \vci{\FASTlusearchFTOHBDynamic}{\FASTlusearchFTOHBDynamicCI}	& \vci{\SLOWlusearchDCExcDynamic}{\SLOWlusearchDCExcDynamicCI}	& \vci{\SLOWlusearchDCnoGExcDynamic}{\SLOWlusearchDCnoGExcDynamicCI}	& \vci{\SLOWlusearchCAPOExcDynamic}{\SLOWlusearchCAPOExcDynamicCI}& \vci{\SLOWlusearchCAPOnoGExcDynamic}{\SLOWlusearchCAPOnoGExcDynamicCI} \\
\bench{pmd}		& \et{\FASTpmdEvents}{\FASTpmdEventsCI}      & \enfp{\FASTpmdNoFPEvents}{\FASTpmdNoFPEventsCI}      & \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & \base{\FASTpmdBase}      & \vci{\FASTpmdFTDynamic}{\FASTpmdFTDynamicCI}      & \vci{\FASTpmdHBDynamic}{\FASTpmdHBDynamicCI}		& \vci{\FASTpmdFTOHBDynamic}{\FASTpmdFTOHBDynamicCI}		& \vci{\SLOWpmdDCExcDynamic}{\SLOWpmdDCExcDynamicCI}		& \vci{\SLOWpmdDCnoGExcDynamic}{\SLOWpmdDCnoGExcDynamicCI}		& \vci{\SLOWpmdCAPOExcDynamic}{\SLOWpmdCAPOExcDynamicCI}		& \vci{\SLOWpmdCAPOnoGExcDynamic}{\SLOWpmdCAPOnoGExcDynamicCI} \\
\bench{sunflow} & \et{\FASTsunflowEvents}{\FASTsunflowEventsCI}  & \enfp{\FASTsunflowNoFPEvents}{\FASTsunflowNoFPEventsCI}	& \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& \base{\FASTsunflowBase}  & \vci{\FASTsunflowFTDynamic}{\FASTsunflowFTDynamicCI}  & \vci{\FASTsunflowHBDynamic}{\FASTsunflowHBDynamicCI}	& \vci{\FASTsunflowFTOHBDynamic}{\FASTsunflowFTOHBDynamicCI}	& \vci{\SLOWsunflowDCExcDynamic}{\SLOWsunflowDCExcDynamicCI}	& \vci{\SLOWsunflowDCnoGExcDynamic}{\SLOWsunflowDCnoGExcDynamicCI}	& \vci{\SLOWsunflowCAPOExcDynamic}{\SLOWsunflowCAPOExcDynamicCI}	& \vci{\SLOWsunflowCAPOnoGExcDynamic}{\SLOWsunflowCAPOnoGExcDynamicCI} \\
% \bench{tomcat} 	& \et{\FASTtomcatEvents}{\FASTtomcatEventsCI}   & \enfp{\FASTtomcatNoFPEvents}{\FASTtomcatNoFPEventsCI}	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& \base{\FASTtomcatBase}   & \vci{\FASTtomcatFTDynamic}{\FASTtomcatFTDynamicCI}   & \vci{\FASTtomcatHBDynamic}{\FASTtomcatHBDynamicCI} 	& \vci{\FASTtomcatFTOHBDynamic}{\FASTtomcatFTOHBDynamicCI}	& \vci{\SLOWtomcatDCExcDynamic}{\SLOWtomcatDCExcDynamicCI}	& \vci{\SLOWtomcatDCnoGExcDynamic}{\SLOWtomcatDCnoGExcDynamicCI}	& \vci{\SLOWtomcatCAPOExcDynamic}{\SLOWtomcatCAPOExcDynamicCI}	& \vci{\SLOWtomcatCAPOnoGExcDynamic}{\SLOWtomcatCAPOnoGExcDynamicCI} \\
\bench{xalan} 	& \et{\FASTxalanEvents}{\FASTxalanEventsCI}    & \enfp{\FASTxalanNoFPEvents}{\FASTxalanNoFPEventsCI}	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& \base{\FASTxalanBase}    & \vci{\FASTxalanFTDynamic}{\FASTxalanFTDynamicCI}    & \vci{\FASTxalanHBDynamic}{\FASTxalanHBDynamicCI}		& \vci{\FASTxalanFTOHBDynamic}{\FASTxalanFTOHBDynamicCI}		& \vci{\SLOWxalanDCExcDynamic}{\SLOWxalanDCExcDynamicCI}	& \vci{\SLOWxalanDCnoGExcDynamic}{\SLOWxalanDCnoGExcDynamicCI} 	& \vci{\SLOWxalanCAPOExcDynamic}{\SLOWxalanCAPOExcDynamicCI}	& \vci{\SLOWxalanCAPOnoGExcDynamic}{\SLOWxalanCAPOnoGExcDynamicCI}\\\hline
% geomean	& &	& &	& & \roh{\FASTFTTimeGeoMean} & \roh{\FASTHBTimeGeoMean} & \roh{\FASTFTOHBTimeGeoMean} & \roh{\SLOWDCExcTimeGeoMean} & \roh{\SLOWDCnoGExcTimeGeoMean} & \roh{\SLOWCAPOExcTimeGeoMean} & \roh{\SLOWCAPOnoGExcTimeGeoMean} \\
\mc{1}{c}{} & \mc{12}{c}{Dynamic Race Counts} \\
\end{tabular}

\caption{Dynamic Race Counts {\bf with no race edge} for counting
races by {\bf second static site} for all analyses with 95\% confidence intervals.}
\label{tab:performance:fasttrack:timeCI}
\end{table*}

\begin{table*}[t]
% \begin{adjustwidth}{-1.5cm}{}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
% \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;Mb$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\sdr}[4]{\vci{#1}{#2}{\;}(\vci{#3}{#4})}
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}#1}
%\input{result-macros/PIP_slowTool_raceEdgeFix_fieldName}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
%\input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_slowTool_noWriteOrReadRaceEdge}
\input{result-macros/PIP_fastTool_noWriteOrReadRaceEdge}
%
\smaller
\centering
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWavroraHB}{\SLOWavroraHBCI}{\SLOWavroraHBDynamic}{\SLOWavroraHBDynamicCI}					& \sdr{\FASTavroraFTOHB}{\FASTavroraFTOHBCI}{\FASTavroraFTOHBDynamic}{\FASTavroraFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWavroraWCP}{\SLOWavroraWCPCI}{\SLOWavroraWCPDynamic}{\SLOWavroraWCPDynamicCI}				& \sdr{\FASTavroraFTOWCP}{\FASTavroraFTOWCPCI}{\FASTavroraFTOWCPDynamic}{\FASTavroraFTOWCPDynamicCI}		& \sdr{\FASTavroraREWCP}{\FASTavroraREWCPCI}{\FASTavroraREWCPDynamic}{\FASTavroraREWCPDynamicCI} \\
\DC		& \sdr{\SLOWavroraDCExc}{\SLOWavroraDCExcCI}{\SLOWavroraDCExcDynamic}{\SLOWavroraDCExcDynamicCI}		& \sdr{\SLOWavroraDCnoGExc}{\SLOWavroraDCnoGExcCI}{\SLOWavroraDCnoGExcDynamic}{\SLOWavroraDCnoGExcDynamicCI}	& \sdr{\FASTavroraFTODC}{\FASTavroraFTODCCI}{\FASTavroraFTODCDynamic}{\FASTavroraFTODCDynamicCI}		& \sdr{\FASTavroraREDC}{\FASTavroraREDCCI}{\FASTavroraREDCDynamic}{\FASTavroraREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWavroraCAPOExc}{\SLOWavroraCAPOExcCI}{\SLOWavroraCAPOExcDynamic}{\SLOWavroraCAPOExcDynamicCI}	& \sdr{\SLOWavroraCAPOnoGExc}{\SLOWavroraCAPOnoGExcCI}{\SLOWavroraCAPOnoGExcDynamic}{\SLOWavroraCAPOnoGExcDynamicCI}	& \sdr{\FASTavroraFTOCAPO}{\FASTavroraFTOCAPOCI}{\FASTavroraFTOCAPODynamic}{\FASTavroraFTOCAPODynamicCI}	& \sdr{\FASTavroraRECAPO}{\FASTavroraRECAPOCI}{\FASTavroraRECAPODynamic}{\FASTavroraRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\medskip\\
% \begin{tabular}{@{}HHlll@{}}
%         & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
% \HB		& \rna													& \sdr{\SLOWbatikHB}{\SLOWbatikHBCI}{\SLOWbatikHBDynamic}{\SLOWbatikHBDynamicCI}					& \sdr{\FASTbatikFTOHB}{\FASTbatikFTOHBCI}{\FASTbatikFTOHBDynamic}{\FASTbatikFTOHBDynamicCI}		& \rna \\
% \WCP	& \rna													& \sdr{\SLOWbatikWCP}{\SLOWbatikWCPCI}{\SLOWbatikWCPDynamic}{\SLOWbatikWCPDynamicCI}				& \sdr{\FASTbatikFTOWCP}{\FASTbatikFTOWCPCI}{\FASTbatikFTOWCPDynamic}{\FASTbatikFTOWCPDynamicCI}		& \sdr{\FASTbatikREWCP}{\FASTbatikREWCPCI}{\FASTbatikREWCPDynamic}{\FASTbatikREWCPDynamicCI} \\
% \DC		& \sdr{\SLOWbatikDCExc}{\SLOWbatikDCExcCI}{\SLOWbatikDCExcDynamic}{\SLOWbatikDCExcDynamicCI}		& \sdr{\SLOWbatikDCnoGExc}{\SLOWbatikDCnoGExcCI}{\SLOWbatikDCnoGExcDynamic}{\SLOWbatikDCnoGExcDynamicCI}	& \sdr{\FASTbatikFTODC}{\FASTbatikFTODCCI}{\FASTbatikFTODCDynamic}{\FASTbatikFTODCDynamicCI}		& \sdr{\FASTbatikREDC}{\FASTbatikREDCCI}{\FASTbatikREDCDynamic}{\FASTbatikREDCDynamicCI} \\
% \CAPO	& \sdr{\SLOWbatikCAPOExc}{\SLOWbatikCAPOExcCI}{\SLOWbatikCAPOExcDynamic}{\SLOWbatikCAPOExcDynamicCI}	& \sdr{\SLOWbatikCAPOnoGExc}{\SLOWbatikCAPOnoGExcCI}{\SLOWbatikCAPOnoGExcDynamic}{\SLOWbatikCAPOnoGExcDynamicCI}	& \sdr{\FASTbatikFTOCAPO}{\FASTbatikFTOCAPOCI}{\FASTbatikFTOCAPODynamic}{\FASTbatikFTOCAPODynamicCI}	& \sdr{\FASTbatikRECAPO}{\FASTbatikRECAPOCI}{\FASTbatikRECAPODynamic}{\FASTbatikRECAPODynamicCI} \\
% 		& \mc{4}{c}{\bench{batik}} \\
% \end{tabular}
% \hfill
\begin{tabular}{@{}l|Hlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWhtwoHB}{\SLOWhtwoHBCI}{\SLOWhtwoHBDynamic}{\SLOWhtwoHBDynamicCI}					& \sdr{\FASThtwoFTOHB}{\FASThtwoFTOHBCI}{\FASThtwoFTOHBDynamic}{\FASThtwoFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWhtwoWCP}{\SLOWhtwoWCPCI}{\SLOWhtwoWCPDynamic}{\SLOWhtwoWCPDynamicCI}				& \sdr{\FASThtwoFTOWCP}{\FASThtwoFTOWCPCI}{\FASThtwoFTOWCPDynamic}{\FASThtwoFTOWCPDynamicCI}		& \sdr{\FASThtwoREWCP}{\FASThtwoREWCPCI}{\FASThtwoREWCPDynamic}{\FASThtwoREWCPDynamicCI} \\
\DC		& \sdr{\SLOWhtwoDCExc}{\SLOWhtwoDCExcCI}{\SLOWhtwoDCExcDynamic}{\SLOWhtwoDCExcDynamicCI}		& \sdr{\SLOWhtwoDCnoGExc}{\SLOWhtwoDCnoGExcCI}{\SLOWhtwoDCnoGExcDynamic}{\SLOWhtwoDCnoGExcDynamicCI}	& \sdr{\FASThtwoFTODC}{\FASThtwoFTODCCI}{\FASThtwoFTODCDynamic}{\FASThtwoFTODCDynamicCI}		& \sdr{\FASThtwoREDC}{\FASThtwoREDCCI}{\FASThtwoREDCDynamic}{\FASThtwoREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWhtwoCAPOExc}{\SLOWhtwoCAPOExcCI}{\SLOWhtwoCAPOExcDynamic}{\SLOWhtwoCAPOExcDynamicCI}	& \sdr{\SLOWhtwoCAPOnoGExc}{\SLOWhtwoCAPOnoGExcCI}{\SLOWhtwoCAPOnoGExcDynamic}{\SLOWhtwoCAPOnoGExcDynamicCI}	& \sdr{\FASThtwoFTOCAPO}{\FASThtwoFTOCAPOCI}{\FASThtwoFTOCAPODynamic}{\FASThtwoFTOCAPODynamicCI}	& \sdr{\FASThtwoRECAPO}{\FASThtwoRECAPOCI}{\FASThtwoRECAPODynamic}{\FASThtwoRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWjythonHB}{\SLOWjythonHBCI}{\SLOWjythonHBDynamic}{\SLOWjythonHBDynamicCI}					& \sdr{\FASTjythonFTOHB}{\FASTjythonFTOHBCI}{\FASTjythonFTOHBDynamic}{\FASTjythonFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWjythonWCP}{\SLOWjythonWCPCI}{\SLOWjythonWCPDynamic}{\SLOWjythonWCPDynamicCI}				& \sdr{\FASTjythonFTOWCP}{\FASTjythonFTOWCPCI}{\FASTjythonFTOWCPDynamic}{\FASTjythonFTOWCPDynamicCI}		& \sdr{\FASTjythonREWCP}{\FASTjythonREWCPCI}{\FASTjythonREWCPDynamic}{\FASTjythonREWCPDynamicCI} \\
\DC		& \sdr{\SLOWjythonDCExc}{\SLOWjythonDCExcCI}{\SLOWjythonDCExcDynamic}{\SLOWjythonDCExcDynamicCI}		& \sdr{\SLOWjythonDCnoGExc}{\SLOWjythonDCnoGExcCI}{\SLOWjythonDCnoGExcDynamic}{\SLOWjythonDCnoGExcDynamicCI}	& \sdr{\FASTjythonFTODC}{\FASTjythonFTODCCI}{\FASTjythonFTODCDynamic}{\FASTjythonFTODCDynamicCI}		& \sdr{\FASTjythonREDC}{\FASTjythonREDCCI}{\FASTjythonREDCDynamic}{\FASTjythonREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWjythonCAPOExc}{\SLOWjythonCAPOExcCI}{\SLOWjythonCAPOExcDynamic}{\SLOWjythonCAPOExcDynamicCI}	& \sdr{\SLOWjythonCAPOnoGExc}{\SLOWjythonCAPOnoGExcCI}{\SLOWjythonCAPOnoGExcDynamic}{\SLOWjythonCAPOnoGExcDynamicCI}	& \sdr{\FASTjythonFTOCAPO}{\FASTjythonFTOCAPOCI}{\FASTjythonFTOCAPODynamic}{\FASTjythonFTOCAPODynamicCI}	& \sdr{\FASTjythonRECAPO}{\FASTjythonRECAPOCI}{\FASTjythonRECAPODynamic}{\FASTjythonRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWluindexHB}{\SLOWluindexHBCI}{\SLOWluindexHBDynamic}{\SLOWluindexHBDynamicCI}					& \sdr{\FASTluindexFTOHB}{\FASTluindexFTOHBCI}{\FASTluindexFTOHBDynamic}{\FASTluindexFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWluindexWCP}{\SLOWluindexWCPCI}{\SLOWluindexWCPDynamic}{\SLOWluindexWCPDynamicCI}				& \sdr{\FASTluindexFTOWCP}{\FASTluindexFTOWCPCI}{\FASTluindexFTOWCPDynamic}{\FASTluindexFTOWCPDynamicCI}		& \sdr{\FASTluindexREWCP}{\FASTluindexREWCPCI}{\FASTluindexREWCPDynamic}{\FASTluindexREWCPDynamicCI} \\
\DC		& \sdr{\SLOWluindexDCExc}{\SLOWluindexDCExcCI}{\SLOWluindexDCExcDynamic}{\SLOWluindexDCExcDynamicCI}		& \sdr{\SLOWluindexDCnoGExc}{\SLOWluindexDCnoGExcCI}{\SLOWluindexDCnoGExcDynamic}{\SLOWluindexDCnoGExcDynamicCI}	& \sdr{\FASTluindexFTODC}{\FASTluindexFTODCCI}{\FASTluindexFTODCDynamic}{\FASTluindexFTODCDynamicCI}		& \sdr{\FASTluindexREDC}{\FASTluindexREDCCI}{\FASTluindexREDCDynamic}{\FASTluindexREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWluindexCAPOExc}{\SLOWluindexCAPOExcCI}{\SLOWluindexCAPOExcDynamic}{\SLOWluindexCAPOExcDynamicCI}	& \sdr{\SLOWluindexCAPOnoGExc}{\SLOWluindexCAPOnoGExcCI}{\SLOWluindexCAPOnoGExcDynamic}{\SLOWluindexCAPOnoGExcDynamicCI}	& \sdr{\FASTluindexFTOCAPO}{\FASTluindexFTOCAPOCI}{\FASTluindexFTOCAPODynamic}{\FASTluindexFTOCAPODynamicCI}	& \sdr{\FASTluindexRECAPO}{\FASTluindexRECAPOCI}{\FASTluindexRECAPODynamic}{\FASTluindexRECAPODynamicCI} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\hfill
% \begin{tabular}{@{}HHlll@{}}
%         & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
% \HB		& \rna													& \sdr{\SLOWlusearchHB}{\SLOWlusearchHBCI}{\SLOWlusearchHBDynamic}{\SLOWlusearchHBDynamicCI}					& \sdr{\FASTlusearchFTOHB}{\FASTlusearchFTOHBCI}{\FASTlusearchFTOHBDynamic}{\FASTlusearchFTOHBDynamicCI}		& \rna \\
% \WCP	& \rna													& \sdr{\SLOWlusearchWCP}{\SLOWlusearchWCPCI}{\SLOWlusearchWCPDynamic}{\SLOWlusearchWCPDynamicCI}				& \sdr{\FASTlusearchFTOWCP}{\FASTlusearchFTOWCPCI}{\FASTlusearchFTOWCPDynamic}{\FASTlusearchFTOWCPDynamicCI}		& \sdr{\FASTlusearchREWCP}{\FASTlusearchREWCPCI}{\FASTlusearchREWCPDynamic}{\FASTlusearchREWCPDynamicCI} \\
% \DC		& \sdr{\SLOWlusearchDCExc}{\SLOWlusearchDCExcCI}{\SLOWlusearchDCExcDynamic}{\SLOWlusearchDCExcDynamicCI}		& \sdr{\SLOWlusearchDCnoGExc}{\SLOWlusearchDCnoGExcCI}{\SLOWlusearchDCnoGExcDynamic}{\SLOWlusearchDCnoGExcDynamicCI}	& \sdr{\FASTlusearchFTODC}{\FASTlusearchFTODCCI}{\FASTlusearchFTODCDynamic}{\FASTlusearchFTODCDynamicCI}		& \sdr{\FASTlusearchREDC}{\FASTlusearchREDCCI}{\FASTlusearchREDCDynamic}{\FASTlusearchREDCDynamicCI} \\
% \CAPO	& \sdr{\SLOWlusearchCAPOExc}{\SLOWlusearchCAPOExcCI}{\SLOWlusearchCAPOExcDynamic}{\SLOWlusearchCAPOExcDynamicCI}	& \sdr{\SLOWlusearchCAPOnoGExc}{\SLOWlusearchCAPOnoGExcCI}{\SLOWlusearchCAPOnoGExcDynamic}{\SLOWlusearchCAPOnoGExcDynamicCI}	& \sdr{\FASTlusearchFTOCAPO}{\FASTlusearchFTOCAPOCI}{\FASTlusearchFTOCAPODynamic}{\FASTlusearchFTOCAPODynamicCI}	& \sdr{\FASTlusearchRECAPO}{\FASTlusearchRECAPOCI}{\FASTlusearchRECAPODynamic}{\FASTlusearchRECAPODynamicCI} \\
% 		& \mc{4}{c}{\bench{lusearch}} \\
% \end{tabular}
% \hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWpmdHB}{\SLOWpmdHBCI}{\SLOWpmdHBDynamic}{\SLOWpmdHBDynamicCI}					& \sdr{\FASTpmdFTOHB}{\FASTpmdFTOHBCI}{\FASTpmdFTOHBDynamic}{\FASTpmdFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWpmdWCP}{\SLOWpmdWCPCI}{\SLOWpmdWCPDynamic}{\SLOWpmdWCPDynamicCI}				& \sdr{\FASTpmdFTOWCP}{\FASTpmdFTOWCPCI}{\FASTpmdFTOWCPDynamic}{\FASTpmdFTOWCPDynamicCI}		& \sdr{\FASTpmdREWCP}{\FASTpmdREWCPCI}{\FASTpmdREWCPDynamic}{\FASTpmdREWCPDynamicCI} \\
\DC		& \sdr{\SLOWpmdDCExc}{\SLOWpmdDCExcCI}{\SLOWpmdDCExcDynamic}{\SLOWpmdDCExcDynamicCI}		& \sdr{\SLOWpmdDCnoGExc}{\SLOWpmdDCnoGExcCI}{\SLOWpmdDCnoGExcDynamic}{\SLOWpmdDCnoGExcDynamicCI}	& \sdr{\FASTpmdFTODC}{\FASTpmdFTODCCI}{\FASTpmdFTODCDynamic}{\FASTpmdFTODCDynamicCI}		& \sdr{\FASTpmdREDC}{\FASTpmdREDCCI}{\FASTpmdREDCDynamic}{\FASTpmdREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWpmdCAPOExc}{\SLOWpmdCAPOExcCI}{\SLOWpmdCAPOExcDynamic}{\SLOWpmdCAPOExcDynamicCI}	& \sdr{\SLOWpmdCAPOnoGExc}{\SLOWpmdCAPOnoGExcCI}{\SLOWpmdCAPOnoGExcDynamic}{\SLOWpmdCAPOnoGExcDynamicCI}	& \sdr{\FASTpmdFTOCAPO}{\FASTpmdFTOCAPOCI}{\FASTpmdFTOCAPODynamic}{\FASTpmdFTOCAPODynamicCI}	& \sdr{\FASTpmdRECAPO}{\FASTpmdRECAPOCI}{\FASTpmdRECAPODynamic}{\FASTpmdRECAPODynamicCI} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWsunflowHB}{\SLOWsunflowHBCI}{\SLOWsunflowHBDynamic}{\SLOWsunflowHBDynamicCI}					& \sdr{\FASTsunflowFTOHB}{\FASTsunflowFTOHBCI}{\FASTsunflowFTOHBDynamic}{\FASTsunflowFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWsunflowWCP}{\SLOWsunflowWCPCI}{\SLOWsunflowWCPDynamic}{\SLOWsunflowWCPDynamicCI}				& \sdr{\FASTsunflowFTOWCP}{\FASTsunflowFTOWCPCI}{\FASTsunflowFTOWCPDynamic}{\FASTsunflowFTOWCPDynamicCI}		& \sdr{\FASTsunflowREWCP}{\FASTsunflowREWCPCI}{\FASTsunflowREWCPDynamic}{\FASTsunflowREWCPDynamicCI} \\
\DC		& \sdr{\SLOWsunflowDCExc}{\SLOWsunflowDCExcCI}{\SLOWsunflowDCExcDynamic}{\SLOWsunflowDCExcDynamicCI}		& \sdr{\SLOWsunflowDCnoGExc}{\SLOWsunflowDCnoGExcCI}{\SLOWsunflowDCnoGExcDynamic}{\SLOWsunflowDCnoGExcDynamicCI}	& \sdr{\FASTsunflowFTODC}{\FASTsunflowFTODCCI}{\FASTsunflowFTODCDynamic}{\FASTsunflowFTODCDynamicCI}		& \sdr{\FASTsunflowREDC}{\FASTsunflowREDCCI}{\FASTsunflowREDCDynamic}{\FASTsunflowREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWsunflowCAPOExc}{\SLOWsunflowCAPOExcCI}{\SLOWsunflowCAPOExcDynamic}{\SLOWsunflowCAPOExcDynamicCI}	& \sdr{\SLOWsunflowCAPOnoGExc}{\SLOWsunflowCAPOnoGExcCI}{\SLOWsunflowCAPOnoGExcDynamic}{\SLOWsunflowCAPOnoGExcDynamicCI}	& \sdr{\FASTsunflowFTOCAPO}{\FASTsunflowFTOCAPOCI}{\FASTsunflowFTOCAPODynamic}{\FASTsunflowFTOCAPODynamicCI}	& \sdr{\FASTsunflowRECAPO}{\FASTsunflowRECAPOCI}{\FASTsunflowRECAPODynamic}{\FASTsunflowRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWtomcatHB}{\SLOWtomcatHBCI}{\SLOWtomcatHBDynamic}{\SLOWtomcatHBDynamicCI}					& \sdr{\FASTtomcatFTOHB}{\FASTtomcatFTOHBCI}{\FASTtomcatFTOHBDynamic}{\FASTtomcatFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWtomcatWCP}{\SLOWtomcatWCPCI}{\SLOWtomcatWCPDynamic}{\SLOWtomcatWCPDynamicCI}				& \sdr{\FASTtomcatFTOWCP}{\FASTtomcatFTOWCPCI}{\FASTtomcatFTOWCPDynamic}{\FASTtomcatFTOWCPDynamicCI}		& \sdr{\FASTtomcatREWCP}{\FASTtomcatREWCPCI}{\FASTtomcatREWCPDynamic}{\FASTtomcatREWCPDynamicCI} \\
\DC		& \sdr{\SLOWtomcatDCExc}{\SLOWtomcatDCExcCI}{\SLOWtomcatDCExcDynamic}{\SLOWtomcatDCExcDynamicCI}		& \sdr{\SLOWtomcatDCnoGExc}{\SLOWtomcatDCnoGExcCI}{\SLOWtomcatDCnoGExcDynamic}{\SLOWtomcatDCnoGExcDynamicCI}	& \sdr{\FASTtomcatFTODC}{\FASTtomcatFTODCCI}{\FASTtomcatFTODCDynamic}{\FASTtomcatFTODCDynamicCI}		& \sdr{\FASTtomcatREDC}{\FASTtomcatREDCCI}{\FASTtomcatREDCDynamic}{\FASTtomcatREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWtomcatCAPOExc}{\SLOWtomcatCAPOExcCI}{\SLOWtomcatCAPOExcDynamic}{\SLOWtomcatCAPOExcDynamicCI}	& \sdr{\SLOWtomcatCAPOnoGExc}{\SLOWtomcatCAPOnoGExcCI}{\SLOWtomcatCAPOnoGExcDynamic}{\SLOWtomcatCAPOnoGExcDynamicCI}	& \sdr{\FASTtomcatFTOCAPO}{\FASTtomcatFTOCAPOCI}{\FASTtomcatFTOCAPODynamic}{\FASTtomcatFTOCAPODynamicCI}	& \sdr{\FASTtomcatRECAPO}{\FASTtomcatRECAPOCI}{\FASTtomcatRECAPODynamic}{\FASTtomcatRECAPODynamicCI} \\
        & \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWxalanHB}{\SLOWxalanHBCI}{\SLOWxalanHBDynamic}{\SLOWxalanHBDynamicCI}					& \sdr{\FASTxalanFTOHB}{\FASTxalanFTOHBCI}{\FASTxalanFTOHBDynamic}{\FASTxalanFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWxalanWCP}{\SLOWxalanWCPCI}{\SLOWxalanWCPDynamic}{\SLOWxalanWCPDynamicCI}				& \sdr{\FASTxalanFTOWCP}{\FASTxalanFTOWCPCI}{\FASTxalanFTOWCPDynamic}{\FASTxalanFTOWCPDynamicCI}		& \sdr{\FASTxalanREWCP}{\FASTxalanREWCPCI}{\FASTxalanREWCPDynamic}{\FASTxalanREWCPDynamicCI} \\
\DC		& \sdr{\SLOWxalanDCExc}{\SLOWxalanDCExcCI}{\SLOWxalanDCExcDynamic}{\SLOWxalanDCExcDynamicCI}		& \sdr{\SLOWxalanDCnoGExc}{\SLOWxalanDCnoGExcCI}{\SLOWxalanDCnoGExcDynamic}{\SLOWxalanDCnoGExcDynamicCI}	& \sdr{\FASTxalanFTODC}{\FASTxalanFTODCCI}{\FASTxalanFTODCDynamic}{\FASTxalanFTODCDynamicCI}		& \sdr{\FASTxalanREDC}{\FASTxalanREDCCI}{\FASTxalanREDCDynamic}{\FASTxalanREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWxalanCAPOExc}{\SLOWxalanCAPOExcCI}{\SLOWxalanCAPOExcDynamic}{\SLOWxalanCAPOExcDynamicCI}	& \sdr{\SLOWxalanCAPOnoGExc}{\SLOWxalanCAPOnoGExcCI}{\SLOWxalanCAPOnoGExcDynamic}{\SLOWxalanCAPOnoGExcDynamicCI}	& \sdr{\FASTxalanFTOCAPO}{\FASTxalanFTOCAPOCI}{\FASTxalanFTOCAPODynamic}{\FASTxalanFTOCAPODynamicCI}	& \sdr{\FASTxalanRECAPO}{\FASTxalanRECAPOCI}{\FASTxalanRECAPODynamic}{\FASTxalanRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\caption{Static and Dynamic Race Counts {\bf with no race edge} for counting
races by {\bf second static site} for all analyses with 95\% confidence intervals.}
\label{tab:race:allDaCapo:CI}
\end{table*}

% No race edge field name array type
\begin{table*}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{#1}
% \newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\baseMem}[1]{#1~MB} %base memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
%\input{result-macros/PIP_slowTool_raceEdgeFix_fieldName}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
%\input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_slowTool_noWriteOrReadRaceEdge_fieldName}
\input{result-macros/PIP_fastTool_noWriteOrReadRaceEdge_fieldName}
%
\small
\centering
\newcommand{\ics}{\;}
\begin{tabular}{@{}l|HHHHHlll|l@{\ics}l|l@{\ics}l@{}}
& \mc{2}{Z}{} & \mc{2}{Z}{} & \mc{1}{H}{Base} & \mc{3}{c|}{\HB} & \mc{2}{c|}{Unopt-\DC} & \mc{2}{c@{}}{Unopt-\CAPO} \\
Program & \mc{2}{Z}{Events} & \mc{2}{Z}{\#Thr} & \mc{1}{H}{time} & RR\FTTwoAbbrv & \FTTwoAbbrv & \FTO & w/ G & w/o G & w/ G & w/o G \\\hline 
\bench{avrora} 	& \et{\FASTavroraEvents}{\FASTavroraEventsCI}   & \enfp{\FASTavroraNoFPEvents}{\FASTavroraNoFPEventsCI}	& \FASTavroraTotalThreads 	& (\FASTavroraMaxLiveThreads)	& \base{\FASTavroraBase}   & \vci{\FASTavroraFT}{\FASTavroraFTCI}   & \vci{\FASTavroraHB}{\FASTavroraHBCI}	& \vci{\FASTavroraFTOHB}{\FASTavroraFTOHBCI}	& \vci{\SLOWavroraDCExc}{\SLOWavroraDCExcCI}	& \vci{\SLOWavroraDCnoGExc}{\SLOWavroraDCnoGExcCI}	& \vci{\SLOWavroraCAPOExc}{\SLOWavroraCAPOExcCI}	& \vci{\SLOWavroraCAPOnoGExc}{\SLOWavroraCAPOnoGExcCI}\\
\bench{batik} 	& \et{\FASTbatikEvents}{\FASTbatikEventsCI}    & \enfp{\FASTbatikNoFPEvents}{\FASTbatikNoFPEventsCI}	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& \base{\FASTbatikBase}    & \vci{\FASTbatikFT}{\FASTbatikFTCI}    & \vci{\FASTbatikHB}{\FASTbatikHBCI}   	& \vci{\FASTbatikFTOHB}{\FASTbatikFTOHBCI}		& \vci{\SLOWbatikDCExc}{\SLOWbatikDCExcCI}	& \vci{\SLOWbatikDCnoGExc}{\SLOWbatikDCnoGExcCI}		& \vci{\SLOWbatikCAPOExc}{\SLOWbatikCAPOExcCI}	& \vci{\SLOWbatikCAPOnoGExc}{\SLOWbatikCAPOnoGExcCI} \\
\bench{h2} 		& \et{\FASThtwoEvents}{\FASThtwoEventsCI}     & \enfp{\FASThtwoNoFPEvents}{\FASThtwoNoFPEventsCI}	    & \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & \base{\FASThtwoBase}     & \vci{\FASThtwoFT}{\FASThtwoFTCI}     & \vci{\FASThtwoHB}{\FASThtwoHBCI}    	& \vci{\FASThtwoFTOHB}{\FASThtwoFTOHBCI}		& \vci{\SLOWhtwoDCExc}{\SLOWhtwoDCExcCI}		& \vci{\SLOWhtwoDCnoGExc}{\SLOWhtwoDCnoGExcCI}		& \vci{\SLOWhtwoCAPOExc}{\SLOWhtwoCAPOExcCI}	& \vci{\SLOWhtwoCAPOnoGExc}{\SLOWhtwoCAPOnoGExcCI}\\
\bench{jython} 	& \et{\FASTjythonEvents}{\FASTjythonEventsCI}   & \enfp{\FASTjythonNoFPEvents}{\FASTjythonNoFPEventsCI}	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& \base{\FASTjythonBase}   & \vci{\FASTjythonFT}{\FASTjythonFTCI}   & \vci{\FASTjythonHB}{\FASTjythonHBCI} 	& \vci{\FASTjythonFTOHB}{\FASTjythonFTOHBCI}	& \vci{\SLOWjythonDCExc}{\SLOWjythonDCExcCI}	& \vci{\SLOWjythonDCnoGExc}{\SLOWjythonDCnoGExcCI}	& \vci{\SLOWjythonCAPOExc}{\SLOWjythonCAPOExcCI}	& \vci{\SLOWjythonCAPOnoGExc}{\SLOWjythonCAPOnoGExcCI} \\
\bench{luindex} & \et{\FASTluindexEvents}{\FASTluindexEventsCI}  & \enfp{\FASTluindexNoFPEvents}{\FASTluindexNoFPEventsCI}	& \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& \base{\FASTluindexBase}  & \vci{\FASTluindexFT}{\FASTluindexFTCI}  & \vci{\FASTluindexHB}{\FASTluindexHBCI} 	& \vci{\FASTluindexFTOHB}{\FASTluindexFTOHBCI}	& \vci{\SLOWluindexDCExc}{\SLOWluindexDCExcCI}	& \vci{\SLOWluindexDCnoGExc}{\SLOWluindexDCnoGExcCI}	& \vci{\SLOWluindexCAPOExc}{\SLOWluindexCAPOExcCI}	& \vci{\SLOWluindexCAPOnoGExc}{\SLOWluindexCAPOnoGExcCI} \\
\bench{lusearch}& \et{\FASTlusearchEvents}{\FASTlusearchEventsCI} & \enfp{\FASTlusearchNoFPEvents}{\FASTlusearchNoFPEventsCI}	& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& \base{\FASTlusearchBase} & \vci{\FASTlusearchFT}{\FASTlusearchFTCI} & \vci{\FASTlusearchHB}{\FASTlusearchHBCI}	& \vci{\FASTlusearchFTOHB}{\FASTlusearchFTOHBCI}	& \vci{\SLOWlusearchDCExc}{\SLOWlusearchDCExcCI}	& \vci{\SLOWlusearchDCnoGExc}{\SLOWlusearchDCnoGExcCI}	& \vci{\SLOWlusearchCAPOExc}{\SLOWlusearchCAPOExcCI}& \vci{\SLOWlusearchCAPOnoGExc}{\SLOWlusearchCAPOnoGExcCI} \\
\bench{pmd}		& \et{\FASTpmdEvents}{\FASTpmdEventsCI}      & \enfp{\FASTpmdNoFPEvents}{\FASTpmdNoFPEventsCI}      & \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & \base{\FASTpmdBase}      & \vci{\FASTpmdFT}{\FASTpmdFTCI}      & \vci{\FASTpmdHB}{\FASTpmdHBCI}		& \vci{\FASTpmdFTOHB}{\FASTpmdFTOHBCI}		& \vci{\SLOWpmdDCExc}{\SLOWpmdDCExcCI}		& \vci{\SLOWpmdDCnoGExc}{\SLOWpmdDCnoGExcCI}		& \vci{\SLOWpmdCAPOExc}{\SLOWpmdCAPOExcCI}		& \vci{\SLOWpmdCAPOnoGExc}{\SLOWpmdCAPOnoGExcCI} \\
\bench{sunflow} & \et{\FASTsunflowEvents}{\FASTsunflowEventsCI}  & \enfp{\FASTsunflowNoFPEvents}{\FASTsunflowNoFPEventsCI}	& \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& \base{\FASTsunflowBase}  & \vci{\FASTsunflowFT}{\FASTsunflowFTCI}  & \vci{\FASTsunflowHB}{\FASTsunflowHBCI}	& \vci{\FASTsunflowFTOHB}{\FASTsunflowFTOHBCI}	& \vci{\SLOWsunflowDCExc}{\SLOWsunflowDCExcCI}	& \vci{\SLOWsunflowDCnoGExc}{\SLOWsunflowDCnoGExcCI}	& \vci{\SLOWsunflowCAPOExc}{\SLOWsunflowCAPOExcCI}	& \vci{\SLOWsunflowCAPOnoGExc}{\SLOWsunflowCAPOnoGExcCI} \\
% \bench{tomcat} 	& \et{\FASTtomcatEvents}{\FASTtomcatEventsCI}   & \enfp{\FASTtomcatNoFPEvents}{\FASTtomcatNoFPEventsCI}	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& \base{\FASTtomcatBase}   & \vci{\FASTtomcatFT}{\FASTtomcatFTCI}   & \vci{\FASTtomcatHB}{\FASTtomcatHBCI} 	& \vci{\FASTtomcatFTOHB}{\FASTtomcatFTOHBCI}	& \vci{\SLOWtomcatDCExc}{\SLOWtomcatDCExcCI}	& \vci{\SLOWtomcatDCnoGExc}{\SLOWtomcatDCnoGExcCI}	& \vci{\SLOWtomcatCAPOExc}{\SLOWtomcatCAPOExcCI}	& \vci{\SLOWtomcatCAPOnoGExc}{\SLOWtomcatCAPOnoGExcCI} \\
\bench{xalan} 	& \et{\FASTxalanEvents}{\FASTxalanEventsCI}    & \enfp{\FASTxalanNoFPEvents}{\FASTxalanNoFPEventsCI}	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& \base{\FASTxalanBase}    & \vci{\FASTxalanFT}{\FASTxalanFTCI}    & \vci{\FASTxalanHB}{\FASTxalanHBCI}		& \vci{\FASTxalanFTOHB}{\FASTxalanFTOHBCI}		& \vci{\SLOWxalanDCExc}{\SLOWxalanDCExcCI}	& \vci{\SLOWxalanDCnoGExc}{\SLOWxalanDCnoGExcCI} 	& \vci{\SLOWxalanCAPOExc}{\SLOWxalanCAPOExcCI}	& \vci{\SLOWxalanCAPOnoGExc}{\SLOWxalanCAPOnoGExcCI}\\\hline
% geomean	& &	& &	& & \roh{\FASTFTTimeGeoMean} & \roh{\FASTHBTimeGeoMean} & \roh{\FASTFTOHBTimeGeoMean} & \roh{\SLOWDCExcTimeGeoMean} & \roh{\SLOWDCnoGExcTimeGeoMean} & \roh{\SLOWCAPOExcTimeGeoMean} & \roh{\SLOWCAPOnoGExcTimeGeoMean} \\
\mc{1}{c}{} & \mc{12}{c}{Static Race Counts} \\
\end{tabular}

\caption{Static Race Counts {\bf with no race edge} for counting races
by {\bf field name and array type} for all analyses with 95\% confidence intervals.}
\label{tab:performance:fasttrack:timeCI}
\end{table*}

\begin{table*}[t]
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{#1}
% \newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rzero}}{0}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
\newcommand{\baseMem}[1]{#1~MB} %base memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
%\input{result-macros/PIP_slowTool_raceEdgeFix_fieldName}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
%\input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_slowTool_noWriteOrReadRaceEdge_fieldName}
\input{result-macros/PIP_fastTool_noWriteOrReadRaceEdge_fieldName}
%
\smaller
\smaller
\centering
\newcommand{\ics}{\;}
\begin{tabular}{@{}l|HHHHHlll|l@{\ics}l|l@{\ics}l@{}}
& \mc{2}{Z}{} & \mc{2}{Z}{} & \mc{1}{H}{Base} & \mc{3}{c|}{\HB} & \mc{2}{c|}{Unopt-\DC} & \mc{2}{c@{}}{Unopt-\CAPO} \\
Program & \mc{2}{Z}{Events} & \mc{2}{Z}{\#Thr} & \mc{1}{H}{time} & RR\FTTwoAbbrv & \FTTwoAbbrv & \FTO & w/ G & w/o G & w/ G & w/o G \\\hline 
\bench{avrora} 	& \et{\FASTavroraEvents}{\FASTavroraEventsCI}   & \enfp{\FASTavroraNoFPEvents}{\FASTavroraNoFPEventsCI}	& \FASTavroraTotalThreads 	& (\FASTavroraMaxLiveThreads)	& \base{\FASTavroraBase}   & \vci{\FASTavroraFTDynamic}{\FASTavroraFTDynamicCI}   & \vci{\FASTavroraHBDynamic}{\FASTavroraHBDynamicCI}	& \vci{\FASTavroraFTOHBDynamic}{\FASTavroraFTOHBDynamicCI}	& \vci{\SLOWavroraDCExcDynamic}{\SLOWavroraDCExcDynamicCI}	& \vci{\SLOWavroraDCnoGExcDynamic}{\SLOWavroraDCnoGExcDynamicCI}	& \vci{\SLOWavroraCAPOExcDynamic}{\SLOWavroraCAPOExcDynamicCI}	& \vci{\SLOWavroraCAPOnoGExcDynamic}{\SLOWavroraCAPOnoGExcDynamicCI}\\
\bench{batik} 	& \et{\FASTbatikEvents}{\FASTbatikEventsCI}    & \enfp{\FASTbatikNoFPEvents}{\FASTbatikNoFPEventsCI}	& \FASTbatikTotalThreads 	& (\FASTbatikMaxLiveThreads)	& \base{\FASTbatikBase}    & \vci{\FASTbatikFTDynamic}{\FASTbatikFTDynamicCI}    & \vci{\FASTbatikHBDynamic}{\FASTbatikHBDynamicCI}   	& \vci{\FASTbatikFTOHBDynamic}{\FASTbatikFTOHBDynamicCI}		& \vci{\SLOWbatikDCExcDynamic}{\SLOWbatikDCExcDynamicCI}	& \vci{\SLOWbatikDCnoGExcDynamic}{\SLOWbatikDCnoGExcDynamicCI}		& \vci{\SLOWbatikCAPOExcDynamic}{\SLOWbatikCAPOExcDynamicCI}	& \vci{\SLOWbatikCAPOnoGExcDynamic}{\SLOWbatikCAPOnoGExcDynamicCI} \\
\bench{h2} 		& \et{\FASThtwoEvents}{\FASThtwoEventsCI}     & \enfp{\FASThtwoNoFPEvents}{\FASThtwoNoFPEventsCI}	    & \FASThtwoTotalThreads 	& (\FASThtwoMaxLiveThreads)	    & \base{\FASThtwoBase}     & \vci{\FASThtwoFTDynamic}{\FASThtwoFTDynamicCI}     & \vci{\FASThtwoHBDynamic}{\FASThtwoHBDynamicCI}    	& \vci{\FASThtwoFTOHBDynamic}{\FASThtwoFTOHBDynamicCI}		& \vci{\SLOWhtwoDCExcDynamic}{\SLOWhtwoDCExcDynamicCI}		& \vci{\SLOWhtwoDCnoGExcDynamic}{\SLOWhtwoDCnoGExcDynamicCI}		& \vci{\SLOWhtwoCAPOExcDynamic}{\SLOWhtwoCAPOExcDynamicCI}	& \vci{\SLOWhtwoCAPOnoGExcDynamic}{\SLOWhtwoCAPOnoGExcDynamicCI}\\
\bench{jython} 	& \et{\FASTjythonEvents}{\FASTjythonEventsCI}   & \enfp{\FASTjythonNoFPEvents}{\FASTjythonNoFPEventsCI}	& \FASTjythonTotalThreads	& (\FASTjythonMaxLiveThreads)	& \base{\FASTjythonBase}   & \vci{\FASTjythonFTDynamic}{\FASTjythonFTDynamicCI}   & \vci{\FASTjythonHBDynamic}{\FASTjythonHBDynamicCI} 	& \vci{\FASTjythonFTOHBDynamic}{\FASTjythonFTOHBDynamicCI}	& \vci{\SLOWjythonDCExcDynamic}{\SLOWjythonDCExcDynamicCI}	& \vci{\SLOWjythonDCnoGExcDynamic}{\SLOWjythonDCnoGExcDynamicCI}	& \vci{\SLOWjythonCAPOExcDynamic}{\SLOWjythonCAPOExcDynamicCI}	& \vci{\SLOWjythonCAPOnoGExcDynamic}{\SLOWjythonCAPOnoGExcDynamicCI} \\
\bench{luindex} & \et{\FASTluindexEvents}{\FASTluindexEventsCI}  & \enfp{\FASTluindexNoFPEvents}{\FASTluindexNoFPEventsCI}	& \FASTluindexTotalThreads	& (\FASTluindexMaxLiveThreads)	& \base{\FASTluindexBase}  & \vci{\FASTluindexFTDynamic}{\FASTluindexFTDynamicCI}  & \vci{\FASTluindexHBDynamic}{\FASTluindexHBDynamicCI} 	& \vci{\FASTluindexFTOHBDynamic}{\FASTluindexFTOHBDynamicCI}	& \vci{\SLOWluindexDCExcDynamic}{\SLOWluindexDCExcDynamicCI}	& \vci{\SLOWluindexDCnoGExcDynamic}{\SLOWluindexDCnoGExcDynamicCI}	& \vci{\SLOWluindexCAPOExcDynamic}{\SLOWluindexCAPOExcDynamicCI}	& \vci{\SLOWluindexCAPOnoGExcDynamic}{\SLOWluindexCAPOnoGExcDynamicCI} \\
\bench{lusearch}& \et{\FASTlusearchEvents}{\FASTlusearchEventsCI} & \enfp{\FASTlusearchNoFPEvents}{\FASTlusearchNoFPEventsCI}	& \FASTlusearchTotalThreads	& (\FASTlusearchMaxLiveThreads)	& \base{\FASTlusearchBase} & \vci{\FASTlusearchFTDynamic}{\FASTlusearchFTDynamicCI} & \vci{\FASTlusearchHBDynamic}{\FASTlusearchHBDynamicCI}	& \vci{\FASTlusearchFTOHBDynamic}{\FASTlusearchFTOHBDynamicCI}	& \vci{\SLOWlusearchDCExcDynamic}{\SLOWlusearchDCExcDynamicCI}	& \vci{\SLOWlusearchDCnoGExcDynamic}{\SLOWlusearchDCnoGExcDynamicCI}	& \vci{\SLOWlusearchCAPOExcDynamic}{\SLOWlusearchCAPOExcDynamicCI}& \vci{\SLOWlusearchCAPOnoGExcDynamic}{\SLOWlusearchCAPOnoGExcDynamicCI} \\
\bench{pmd}		& \et{\FASTpmdEvents}{\FASTpmdEventsCI}      & \enfp{\FASTpmdNoFPEvents}{\FASTpmdNoFPEventsCI}      & \FASTpmdTotalThreads	    & (\FASTpmdMaxLiveThreads)	    & \base{\FASTpmdBase}      & \vci{\FASTpmdFTDynamic}{\FASTpmdFTDynamicCI}      & \vci{\FASTpmdHBDynamic}{\FASTpmdHBDynamicCI}		& \vci{\FASTpmdFTOHBDynamic}{\FASTpmdFTOHBDynamicCI}		& \vci{\SLOWpmdDCExcDynamic}{\SLOWpmdDCExcDynamicCI}		& \vci{\SLOWpmdDCnoGExcDynamic}{\SLOWpmdDCnoGExcDynamicCI}		& \vci{\SLOWpmdCAPOExcDynamic}{\SLOWpmdCAPOExcDynamicCI}		& \vci{\SLOWpmdCAPOnoGExcDynamic}{\SLOWpmdCAPOnoGExcDynamicCI} \\
\bench{sunflow} & \et{\FASTsunflowEvents}{\FASTsunflowEventsCI}  & \enfp{\FASTsunflowNoFPEvents}{\FASTsunflowNoFPEventsCI}	& \FASTsunflowTotalThreads	& (\FASTsunflowMaxLiveThreads)	& \base{\FASTsunflowBase}  & \vci{\FASTsunflowFTDynamic}{\FASTsunflowFTDynamicCI}  & \vci{\FASTsunflowHBDynamic}{\FASTsunflowHBDynamicCI}	& \vci{\FASTsunflowFTOHBDynamic}{\FASTsunflowFTOHBDynamicCI}	& \vci{\SLOWsunflowDCExcDynamic}{\SLOWsunflowDCExcDynamicCI}	& \vci{\SLOWsunflowDCnoGExcDynamic}{\SLOWsunflowDCnoGExcDynamicCI}	& \vci{\SLOWsunflowCAPOExcDynamic}{\SLOWsunflowCAPOExcDynamicCI}	& \vci{\SLOWsunflowCAPOnoGExcDynamic}{\SLOWsunflowCAPOnoGExcDynamicCI} \\
% \bench{tomcat} 	& \et{\FASTtomcatEvents}{\FASTtomcatEventsCI}   & \enfp{\FASTtomcatNoFPEvents}{\FASTtomcatNoFPEventsCI}	& \FASTtomcatTotalThreads	& (\FASTtomcatMaxLiveThreads)	& \base{\FASTtomcatBase}   & \vci{\FASTtomcatFTDynamic}{\FASTtomcatFTDynamicCI}   & \vci{\FASTtomcatHBDynamic}{\FASTtomcatHBDynamicCI} 	& \vci{\FASTtomcatFTOHBDynamic}{\FASTtomcatFTOHBDynamicCI}	& \vci{\SLOWtomcatDCExcDynamic}{\SLOWtomcatDCExcDynamicCI}	& \vci{\SLOWtomcatDCnoGExcDynamic}{\SLOWtomcatDCnoGExcDynamicCI}	& \vci{\SLOWtomcatCAPOExcDynamic}{\SLOWtomcatCAPOExcDynamicCI}	& \vci{\SLOWtomcatCAPOnoGExcDynamic}{\SLOWtomcatCAPOnoGExcDynamicCI} \\
\bench{xalan} 	& \et{\FASTxalanEvents}{\FASTxalanEventsCI}    & \enfp{\FASTxalanNoFPEvents}{\FASTxalanNoFPEventsCI}	& \FASTxalanTotalThreads	& (\FASTxalanMaxLiveThreads)	& \base{\FASTxalanBase}    & \vci{\FASTxalanFTDynamic}{\FASTxalanFTDynamicCI}    & \vci{\FASTxalanHBDynamic}{\FASTxalanHBDynamicCI}		& \vci{\FASTxalanFTOHBDynamic}{\FASTxalanFTOHBDynamicCI}		& \vci{\SLOWxalanDCExcDynamic}{\SLOWxalanDCExcDynamicCI}	& \vci{\SLOWxalanDCnoGExcDynamic}{\SLOWxalanDCnoGExcDynamicCI} 	& \vci{\SLOWxalanCAPOExcDynamic}{\SLOWxalanCAPOExcDynamicCI}	& \vci{\SLOWxalanCAPOnoGExcDynamic}{\SLOWxalanCAPOnoGExcDynamicCI}\\\hline
% geomean	& &	& &	& & \roh{\FASTFTTimeGeoMean} & \roh{\FASTHBTimeGeoMean} & \roh{\FASTFTOHBTimeGeoMean} & \roh{\SLOWDCExcTimeGeoMean} & \roh{\SLOWDCnoGExcTimeGeoMean} & \roh{\SLOWCAPOExcTimeGeoMean} & \roh{\SLOWCAPOnoGExcTimeGeoMean} \\
\mc{1}{c}{} & \mc{12}{c}{Dynamic Race Counts} \\
\end{tabular}

\caption{Dynamic Race Counts {\bf with no race edge} for counting
races by {\bf field name and array type} for all analyses with 95\% confidence intervals.}
\label{tab:performance:fasttrack:timeCI}
\end{table*}

\begin{table*}[t]
% \begin{adjustwidth}{-1.5cm}{}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
% \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;Mb$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\sdr}[4]{\vci{#1}{#2}{\;}(\vci{#3}{#4})}
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}#1}
%\input{result-macros/PIP_slowTool_raceEdgeFix_fieldName}
% \input{result-macros/PIP_slowTool_raceEdgeFix}
%\input{result-macros/PIP_fastTool_readExclFix_Quite}
\input{result-macros/PIP_slowTool_noWriteOrReadRaceEdge_fieldName}
\input{result-macros/PIP_fastTool_noWriteOrReadRaceEdge_fieldName}
%
\smaller
\centering
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWavroraHB}{\SLOWavroraHBCI}{\SLOWavroraHBDynamic}{\SLOWavroraHBDynamicCI}					& \sdr{\FASTavroraFTOHB}{\FASTavroraFTOHBCI}{\FASTavroraFTOHBDynamic}{\FASTavroraFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWavroraWCP}{\SLOWavroraWCPCI}{\SLOWavroraWCPDynamic}{\SLOWavroraWCPDynamicCI}				& \sdr{\FASTavroraFTOWCP}{\FASTavroraFTOWCPCI}{\FASTavroraFTOWCPDynamic}{\FASTavroraFTOWCPDynamicCI}		& \sdr{\FASTavroraREWCP}{\FASTavroraREWCPCI}{\FASTavroraREWCPDynamic}{\FASTavroraREWCPDynamicCI} \\
\DC		& \sdr{\SLOWavroraDCExc}{\SLOWavroraDCExcCI}{\SLOWavroraDCExcDynamic}{\SLOWavroraDCExcDynamicCI}		& \sdr{\SLOWavroraDCnoGExc}{\SLOWavroraDCnoGExcCI}{\SLOWavroraDCnoGExcDynamic}{\SLOWavroraDCnoGExcDynamicCI}	& \sdr{\FASTavroraFTODC}{\FASTavroraFTODCCI}{\FASTavroraFTODCDynamic}{\FASTavroraFTODCDynamicCI}		& \sdr{\FASTavroraREDC}{\FASTavroraREDCCI}{\FASTavroraREDCDynamic}{\FASTavroraREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWavroraCAPOExc}{\SLOWavroraCAPOExcCI}{\SLOWavroraCAPOExcDynamic}{\SLOWavroraCAPOExcDynamicCI}	& \sdr{\SLOWavroraCAPOnoGExc}{\SLOWavroraCAPOnoGExcCI}{\SLOWavroraCAPOnoGExcDynamic}{\SLOWavroraCAPOnoGExcDynamicCI}	& \sdr{\FASTavroraFTOCAPO}{\FASTavroraFTOCAPOCI}{\FASTavroraFTOCAPODynamic}{\FASTavroraFTOCAPODynamicCI}	& \sdr{\FASTavroraRECAPO}{\FASTavroraRECAPOCI}{\FASTavroraRECAPODynamic}{\FASTavroraRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\medskip\\
% \begin{tabular}{@{}HHlll@{}}
%         & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
% \HB		& \rna													& \sdr{\SLOWbatikHB}{\SLOWbatikHBCI}{\SLOWbatikHBDynamic}{\SLOWbatikHBDynamicCI}					& \sdr{\FASTbatikFTOHB}{\FASTbatikFTOHBCI}{\FASTbatikFTOHBDynamic}{\FASTbatikFTOHBDynamicCI}		& \rna \\
% \WCP	& \rna													& \sdr{\SLOWbatikWCP}{\SLOWbatikWCPCI}{\SLOWbatikWCPDynamic}{\SLOWbatikWCPDynamicCI}				& \sdr{\FASTbatikFTOWCP}{\FASTbatikFTOWCPCI}{\FASTbatikFTOWCPDynamic}{\FASTbatikFTOWCPDynamicCI}		& \sdr{\FASTbatikREWCP}{\FASTbatikREWCPCI}{\FASTbatikREWCPDynamic}{\FASTbatikREWCPDynamicCI} \\
% \DC		& \sdr{\SLOWbatikDCExc}{\SLOWbatikDCExcCI}{\SLOWbatikDCExcDynamic}{\SLOWbatikDCExcDynamicCI}		& \sdr{\SLOWbatikDCnoGExc}{\SLOWbatikDCnoGExcCI}{\SLOWbatikDCnoGExcDynamic}{\SLOWbatikDCnoGExcDynamicCI}	& \sdr{\FASTbatikFTODC}{\FASTbatikFTODCCI}{\FASTbatikFTODCDynamic}{\FASTbatikFTODCDynamicCI}		& \sdr{\FASTbatikREDC}{\FASTbatikREDCCI}{\FASTbatikREDCDynamic}{\FASTbatikREDCDynamicCI} \\
% \CAPO	& \sdr{\SLOWbatikCAPOExc}{\SLOWbatikCAPOExcCI}{\SLOWbatikCAPOExcDynamic}{\SLOWbatikCAPOExcDynamicCI}	& \sdr{\SLOWbatikCAPOnoGExc}{\SLOWbatikCAPOnoGExcCI}{\SLOWbatikCAPOnoGExcDynamic}{\SLOWbatikCAPOnoGExcDynamicCI}	& \sdr{\FASTbatikFTOCAPO}{\FASTbatikFTOCAPOCI}{\FASTbatikFTOCAPODynamic}{\FASTbatikFTOCAPODynamicCI}	& \sdr{\FASTbatikRECAPO}{\FASTbatikRECAPOCI}{\FASTbatikRECAPODynamic}{\FASTbatikRECAPODynamicCI} \\
% 		& \mc{4}{c}{\bench{batik}} \\
% \end{tabular}
% \hfill
\begin{tabular}{@{}l|Hlll@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWhtwoHB}{\SLOWhtwoHBCI}{\SLOWhtwoHBDynamic}{\SLOWhtwoHBDynamicCI}					& \sdr{\FASThtwoFTOHB}{\FASThtwoFTOHBCI}{\FASThtwoFTOHBDynamic}{\FASThtwoFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWhtwoWCP}{\SLOWhtwoWCPCI}{\SLOWhtwoWCPDynamic}{\SLOWhtwoWCPDynamicCI}				& \sdr{\FASThtwoFTOWCP}{\FASThtwoFTOWCPCI}{\FASThtwoFTOWCPDynamic}{\FASThtwoFTOWCPDynamicCI}		& \sdr{\FASThtwoREWCP}{\FASThtwoREWCPCI}{\FASThtwoREWCPDynamic}{\FASThtwoREWCPDynamicCI} \\
\DC		& \sdr{\SLOWhtwoDCExc}{\SLOWhtwoDCExcCI}{\SLOWhtwoDCExcDynamic}{\SLOWhtwoDCExcDynamicCI}		& \sdr{\SLOWhtwoDCnoGExc}{\SLOWhtwoDCnoGExcCI}{\SLOWhtwoDCnoGExcDynamic}{\SLOWhtwoDCnoGExcDynamicCI}	& \sdr{\FASThtwoFTODC}{\FASThtwoFTODCCI}{\FASThtwoFTODCDynamic}{\FASThtwoFTODCDynamicCI}		& \sdr{\FASThtwoREDC}{\FASThtwoREDCCI}{\FASThtwoREDCDynamic}{\FASThtwoREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWhtwoCAPOExc}{\SLOWhtwoCAPOExcCI}{\SLOWhtwoCAPOExcDynamic}{\SLOWhtwoCAPOExcDynamicCI}	& \sdr{\SLOWhtwoCAPOnoGExc}{\SLOWhtwoCAPOnoGExcCI}{\SLOWhtwoCAPOnoGExcDynamic}{\SLOWhtwoCAPOnoGExcDynamicCI}	& \sdr{\FASThtwoFTOCAPO}{\FASThtwoFTOCAPOCI}{\FASThtwoFTOCAPODynamic}{\FASThtwoFTOCAPODynamicCI}	& \sdr{\FASThtwoRECAPO}{\FASThtwoRECAPOCI}{\FASThtwoRECAPODynamic}{\FASThtwoRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWjythonHB}{\SLOWjythonHBCI}{\SLOWjythonHBDynamic}{\SLOWjythonHBDynamicCI}					& \sdr{\FASTjythonFTOHB}{\FASTjythonFTOHBCI}{\FASTjythonFTOHBDynamic}{\FASTjythonFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWjythonWCP}{\SLOWjythonWCPCI}{\SLOWjythonWCPDynamic}{\SLOWjythonWCPDynamicCI}				& \sdr{\FASTjythonFTOWCP}{\FASTjythonFTOWCPCI}{\FASTjythonFTOWCPDynamic}{\FASTjythonFTOWCPDynamicCI}		& \sdr{\FASTjythonREWCP}{\FASTjythonREWCPCI}{\FASTjythonREWCPDynamic}{\FASTjythonREWCPDynamicCI} \\
\DC		& \sdr{\SLOWjythonDCExc}{\SLOWjythonDCExcCI}{\SLOWjythonDCExcDynamic}{\SLOWjythonDCExcDynamicCI}		& \sdr{\SLOWjythonDCnoGExc}{\SLOWjythonDCnoGExcCI}{\SLOWjythonDCnoGExcDynamic}{\SLOWjythonDCnoGExcDynamicCI}	& \sdr{\FASTjythonFTODC}{\FASTjythonFTODCCI}{\FASTjythonFTODCDynamic}{\FASTjythonFTODCDynamicCI}		& \sdr{\FASTjythonREDC}{\FASTjythonREDCCI}{\FASTjythonREDCDynamic}{\FASTjythonREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWjythonCAPOExc}{\SLOWjythonCAPOExcCI}{\SLOWjythonCAPOExcDynamic}{\SLOWjythonCAPOExcDynamicCI}	& \sdr{\SLOWjythonCAPOnoGExc}{\SLOWjythonCAPOnoGExcCI}{\SLOWjythonCAPOnoGExcDynamic}{\SLOWjythonCAPOnoGExcDynamicCI}	& \sdr{\FASTjythonFTOCAPO}{\FASTjythonFTOCAPOCI}{\FASTjythonFTOCAPODynamic}{\FASTjythonFTOCAPODynamicCI}	& \sdr{\FASTjythonRECAPO}{\FASTjythonRECAPOCI}{\FASTjythonRECAPODynamic}{\FASTjythonRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWluindexHB}{\SLOWluindexHBCI}{\SLOWluindexHBDynamic}{\SLOWluindexHBDynamicCI}					& \sdr{\FASTluindexFTOHB}{\FASTluindexFTOHBCI}{\FASTluindexFTOHBDynamic}{\FASTluindexFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWluindexWCP}{\SLOWluindexWCPCI}{\SLOWluindexWCPDynamic}{\SLOWluindexWCPDynamicCI}				& \sdr{\FASTluindexFTOWCP}{\FASTluindexFTOWCPCI}{\FASTluindexFTOWCPDynamic}{\FASTluindexFTOWCPDynamicCI}		& \sdr{\FASTluindexREWCP}{\FASTluindexREWCPCI}{\FASTluindexREWCPDynamic}{\FASTluindexREWCPDynamicCI} \\
\DC		& \sdr{\SLOWluindexDCExc}{\SLOWluindexDCExcCI}{\SLOWluindexDCExcDynamic}{\SLOWluindexDCExcDynamicCI}		& \sdr{\SLOWluindexDCnoGExc}{\SLOWluindexDCnoGExcCI}{\SLOWluindexDCnoGExcDynamic}{\SLOWluindexDCnoGExcDynamicCI}	& \sdr{\FASTluindexFTODC}{\FASTluindexFTODCCI}{\FASTluindexFTODCDynamic}{\FASTluindexFTODCDynamicCI}		& \sdr{\FASTluindexREDC}{\FASTluindexREDCCI}{\FASTluindexREDCDynamic}{\FASTluindexREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWluindexCAPOExc}{\SLOWluindexCAPOExcCI}{\SLOWluindexCAPOExcDynamic}{\SLOWluindexCAPOExcDynamicCI}	& \sdr{\SLOWluindexCAPOnoGExc}{\SLOWluindexCAPOnoGExcCI}{\SLOWluindexCAPOnoGExcDynamic}{\SLOWluindexCAPOnoGExcDynamicCI}	& \sdr{\FASTluindexFTOCAPO}{\FASTluindexFTOCAPOCI}{\FASTluindexFTOCAPODynamic}{\FASTluindexFTOCAPODynamicCI}	& \sdr{\FASTluindexRECAPO}{\FASTluindexRECAPOCI}{\FASTluindexRECAPODynamic}{\FASTluindexRECAPODynamicCI} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\hfill
% \begin{tabular}{@{}HHlll@{}}
%         & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
% \HB		& \rna													& \sdr{\SLOWlusearchHB}{\SLOWlusearchHBCI}{\SLOWlusearchHBDynamic}{\SLOWlusearchHBDynamicCI}					& \sdr{\FASTlusearchFTOHB}{\FASTlusearchFTOHBCI}{\FASTlusearchFTOHBDynamic}{\FASTlusearchFTOHBDynamicCI}		& \rna \\
% \WCP	& \rna													& \sdr{\SLOWlusearchWCP}{\SLOWlusearchWCPCI}{\SLOWlusearchWCPDynamic}{\SLOWlusearchWCPDynamicCI}				& \sdr{\FASTlusearchFTOWCP}{\FASTlusearchFTOWCPCI}{\FASTlusearchFTOWCPDynamic}{\FASTlusearchFTOWCPDynamicCI}		& \sdr{\FASTlusearchREWCP}{\FASTlusearchREWCPCI}{\FASTlusearchREWCPDynamic}{\FASTlusearchREWCPDynamicCI} \\
% \DC		& \sdr{\SLOWlusearchDCExc}{\SLOWlusearchDCExcCI}{\SLOWlusearchDCExcDynamic}{\SLOWlusearchDCExcDynamicCI}		& \sdr{\SLOWlusearchDCnoGExc}{\SLOWlusearchDCnoGExcCI}{\SLOWlusearchDCnoGExcDynamic}{\SLOWlusearchDCnoGExcDynamicCI}	& \sdr{\FASTlusearchFTODC}{\FASTlusearchFTODCCI}{\FASTlusearchFTODCDynamic}{\FASTlusearchFTODCDynamicCI}		& \sdr{\FASTlusearchREDC}{\FASTlusearchREDCCI}{\FASTlusearchREDCDynamic}{\FASTlusearchREDCDynamicCI} \\
% \CAPO	& \sdr{\SLOWlusearchCAPOExc}{\SLOWlusearchCAPOExcCI}{\SLOWlusearchCAPOExcDynamic}{\SLOWlusearchCAPOExcDynamicCI}	& \sdr{\SLOWlusearchCAPOnoGExc}{\SLOWlusearchCAPOnoGExcCI}{\SLOWlusearchCAPOnoGExcDynamic}{\SLOWlusearchCAPOnoGExcDynamicCI}	& \sdr{\FASTlusearchFTOCAPO}{\FASTlusearchFTOCAPOCI}{\FASTlusearchFTOCAPODynamic}{\FASTlusearchFTOCAPODynamicCI}	& \sdr{\FASTlusearchRECAPO}{\FASTlusearchRECAPOCI}{\FASTlusearchRECAPODynamic}{\FASTlusearchRECAPODynamicCI} \\
% 		& \mc{4}{c}{\bench{lusearch}} \\
% \end{tabular}
% \hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWpmdHB}{\SLOWpmdHBCI}{\SLOWpmdHBDynamic}{\SLOWpmdHBDynamicCI}					& \sdr{\FASTpmdFTOHB}{\FASTpmdFTOHBCI}{\FASTpmdFTOHBDynamic}{\FASTpmdFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWpmdWCP}{\SLOWpmdWCPCI}{\SLOWpmdWCPDynamic}{\SLOWpmdWCPDynamicCI}				& \sdr{\FASTpmdFTOWCP}{\FASTpmdFTOWCPCI}{\FASTpmdFTOWCPDynamic}{\FASTpmdFTOWCPDynamicCI}		& \sdr{\FASTpmdREWCP}{\FASTpmdREWCPCI}{\FASTpmdREWCPDynamic}{\FASTpmdREWCPDynamicCI} \\
\DC		& \sdr{\SLOWpmdDCExc}{\SLOWpmdDCExcCI}{\SLOWpmdDCExcDynamic}{\SLOWpmdDCExcDynamicCI}		& \sdr{\SLOWpmdDCnoGExc}{\SLOWpmdDCnoGExcCI}{\SLOWpmdDCnoGExcDynamic}{\SLOWpmdDCnoGExcDynamicCI}	& \sdr{\FASTpmdFTODC}{\FASTpmdFTODCCI}{\FASTpmdFTODCDynamic}{\FASTpmdFTODCDynamicCI}		& \sdr{\FASTpmdREDC}{\FASTpmdREDCCI}{\FASTpmdREDCDynamic}{\FASTpmdREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWpmdCAPOExc}{\SLOWpmdCAPOExcCI}{\SLOWpmdCAPOExcDynamic}{\SLOWpmdCAPOExcDynamicCI}	& \sdr{\SLOWpmdCAPOnoGExc}{\SLOWpmdCAPOnoGExcCI}{\SLOWpmdCAPOnoGExcDynamic}{\SLOWpmdCAPOnoGExcDynamicCI}	& \sdr{\FASTpmdFTOCAPO}{\FASTpmdFTOCAPOCI}{\FASTpmdFTOCAPODynamic}{\FASTpmdFTOCAPODynamicCI}	& \sdr{\FASTpmdRECAPO}{\FASTpmdRECAPOCI}{\FASTpmdRECAPODynamic}{\FASTpmdRECAPODynamicCI} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWsunflowHB}{\SLOWsunflowHBCI}{\SLOWsunflowHBDynamic}{\SLOWsunflowHBDynamicCI}					& \sdr{\FASTsunflowFTOHB}{\FASTsunflowFTOHBCI}{\FASTsunflowFTOHBDynamic}{\FASTsunflowFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWsunflowWCP}{\SLOWsunflowWCPCI}{\SLOWsunflowWCPDynamic}{\SLOWsunflowWCPDynamicCI}				& \sdr{\FASTsunflowFTOWCP}{\FASTsunflowFTOWCPCI}{\FASTsunflowFTOWCPDynamic}{\FASTsunflowFTOWCPDynamicCI}		& \sdr{\FASTsunflowREWCP}{\FASTsunflowREWCPCI}{\FASTsunflowREWCPDynamic}{\FASTsunflowREWCPDynamicCI} \\
\DC		& \sdr{\SLOWsunflowDCExc}{\SLOWsunflowDCExcCI}{\SLOWsunflowDCExcDynamic}{\SLOWsunflowDCExcDynamicCI}		& \sdr{\SLOWsunflowDCnoGExc}{\SLOWsunflowDCnoGExcCI}{\SLOWsunflowDCnoGExcDynamic}{\SLOWsunflowDCnoGExcDynamicCI}	& \sdr{\FASTsunflowFTODC}{\FASTsunflowFTODCCI}{\FASTsunflowFTODCDynamic}{\FASTsunflowFTODCDynamicCI}		& \sdr{\FASTsunflowREDC}{\FASTsunflowREDCCI}{\FASTsunflowREDCDynamic}{\FASTsunflowREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWsunflowCAPOExc}{\SLOWsunflowCAPOExcCI}{\SLOWsunflowCAPOExcDynamic}{\SLOWsunflowCAPOExcDynamicCI}	& \sdr{\SLOWsunflowCAPOnoGExc}{\SLOWsunflowCAPOnoGExcCI}{\SLOWsunflowCAPOnoGExcDynamic}{\SLOWsunflowCAPOnoGExcDynamicCI}	& \sdr{\FASTsunflowFTOCAPO}{\FASTsunflowFTOCAPOCI}{\FASTsunflowFTOCAPODynamic}{\FASTsunflowFTOCAPODynamicCI}	& \sdr{\FASTsunflowRECAPO}{\FASTsunflowRECAPOCI}{\FASTsunflowRECAPODynamic}{\FASTsunflowRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWtomcatHB}{\SLOWtomcatHBCI}{\SLOWtomcatHBDynamic}{\SLOWtomcatHBDynamicCI}					& \sdr{\FASTtomcatFTOHB}{\FASTtomcatFTOHBCI}{\FASTtomcatFTOHBDynamic}{\FASTtomcatFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWtomcatWCP}{\SLOWtomcatWCPCI}{\SLOWtomcatWCPDynamic}{\SLOWtomcatWCPDynamicCI}				& \sdr{\FASTtomcatFTOWCP}{\FASTtomcatFTOWCPCI}{\FASTtomcatFTOWCPDynamic}{\FASTtomcatFTOWCPDynamicCI}		& \sdr{\FASTtomcatREWCP}{\FASTtomcatREWCPCI}{\FASTtomcatREWCPDynamic}{\FASTtomcatREWCPDynamicCI} \\
\DC		& \sdr{\SLOWtomcatDCExc}{\SLOWtomcatDCExcCI}{\SLOWtomcatDCExcDynamic}{\SLOWtomcatDCExcDynamicCI}		& \sdr{\SLOWtomcatDCnoGExc}{\SLOWtomcatDCnoGExcCI}{\SLOWtomcatDCnoGExcDynamic}{\SLOWtomcatDCnoGExcDynamicCI}	& \sdr{\FASTtomcatFTODC}{\FASTtomcatFTODCCI}{\FASTtomcatFTODCDynamic}{\FASTtomcatFTODCDynamicCI}		& \sdr{\FASTtomcatREDC}{\FASTtomcatREDCCI}{\FASTtomcatREDCDynamic}{\FASTtomcatREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWtomcatCAPOExc}{\SLOWtomcatCAPOExcCI}{\SLOWtomcatCAPOExcDynamic}{\SLOWtomcatCAPOExcDynamicCI}	& \sdr{\SLOWtomcatCAPOnoGExc}{\SLOWtomcatCAPOnoGExcCI}{\SLOWtomcatCAPOnoGExcDynamic}{\SLOWtomcatCAPOnoGExcDynamicCI}	& \sdr{\FASTtomcatFTOCAPO}{\FASTtomcatFTOCAPOCI}{\FASTtomcatFTOCAPODynamic}{\FASTtomcatFTOCAPODynamicCI}	& \sdr{\FASTtomcatRECAPO}{\FASTtomcatRECAPOCI}{\FASTtomcatRECAPODynamic}{\FASTtomcatRECAPODynamicCI} \\
        & \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hlll@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna													& \sdr{\SLOWxalanHB}{\SLOWxalanHBCI}{\SLOWxalanHBDynamic}{\SLOWxalanHBDynamicCI}					& \sdr{\FASTxalanFTOHB}{\FASTxalanFTOHBCI}{\FASTxalanFTOHBDynamic}{\FASTxalanFTOHBDynamicCI}		& \rna \\
\WCP	& \rna													& \sdr{\SLOWxalanWCP}{\SLOWxalanWCPCI}{\SLOWxalanWCPDynamic}{\SLOWxalanWCPDynamicCI}				& \sdr{\FASTxalanFTOWCP}{\FASTxalanFTOWCPCI}{\FASTxalanFTOWCPDynamic}{\FASTxalanFTOWCPDynamicCI}		& \sdr{\FASTxalanREWCP}{\FASTxalanREWCPCI}{\FASTxalanREWCPDynamic}{\FASTxalanREWCPDynamicCI} \\
\DC		& \sdr{\SLOWxalanDCExc}{\SLOWxalanDCExcCI}{\SLOWxalanDCExcDynamic}{\SLOWxalanDCExcDynamicCI}		& \sdr{\SLOWxalanDCnoGExc}{\SLOWxalanDCnoGExcCI}{\SLOWxalanDCnoGExcDynamic}{\SLOWxalanDCnoGExcDynamicCI}	& \sdr{\FASTxalanFTODC}{\FASTxalanFTODCCI}{\FASTxalanFTODCDynamic}{\FASTxalanFTODCDynamicCI}		& \sdr{\FASTxalanREDC}{\FASTxalanREDCCI}{\FASTxalanREDCDynamic}{\FASTxalanREDCDynamicCI} \\
\CAPO	& \sdr{\SLOWxalanCAPOExc}{\SLOWxalanCAPOExcCI}{\SLOWxalanCAPOExcDynamic}{\SLOWxalanCAPOExcDynamicCI}	& \sdr{\SLOWxalanCAPOnoGExc}{\SLOWxalanCAPOnoGExcCI}{\SLOWxalanCAPOnoGExcDynamic}{\SLOWxalanCAPOnoGExcDynamicCI}	& \sdr{\FASTxalanFTOCAPO}{\FASTxalanFTOCAPOCI}{\FASTxalanFTOCAPODynamic}{\FASTxalanFTOCAPODynamicCI}	& \sdr{\FASTxalanRECAPO}{\FASTxalanRECAPOCI}{\FASTxalanRECAPODynamic}{\FASTxalanRECAPODynamicCI} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\caption{Static and Dynamic Race Counts {\bf with no race edge} for counting
races by {\bf field name and array type} for all analyses with 95\% confidence intervals.}
\label{tab:race:allDaCapo:CI}
\end{table*}

==> result-macros/PIP_fastTool_noCoresSet.tex <==
\newcommand{\FASTavroraEvents}{1,400}
\newcommand{\FASTavroraNoFPEvents}{5.7}
\newcommand{\avroraHBEventTotal}{1,400}
\newcommand{\avroraHBNoFPEventTotal}{150}
\newcommand{\avroraHBNoFPAccessTotal}{150}
\newcommand{\avroraHBNoFPOtherTotal}{3.6}
\newcommand{\avroraHBReadTotal}{69.4}
\newcommand{\avroraHBWriteTotal}{28.3}
\newcommand{\avroraHBNoFPAccessInCS}{30.2}
\newcommand{\avroraHBNoFPAccessOutCS}{47.8}
\newcommand{\avroraHBAcqRelTotal}{51.5}
\newcommand{\avroraHBOtherTotal}{11.2}
\newcommand{\avroraHBNoFPReadTotal}{110}
\newcommand{\avroraHBReadInCS}{6.05}
\newcommand{\avroraHBReadOutCS}{94}
\newcommand{\avroraHBReadSameEp}{0.0242}
\newcommand{\avroraHBReadSharedSameEp}{\cna}
\newcommand{\avroraHBReadExclusive}{96.5}
\newcommand{\avroraHBReadOwned}{\cna}
\newcommand{\avroraHBReadShare}{0.0206}
\newcommand{\avroraHBReadShared}{3.51}
\newcommand{\avroraHBReadSharedOwned}{\cna}
\newcommand{\avroraHBNoFPHonestWriteTotal}{44}
\newcommand{\avroraHBWriteInCS}{6.22}
\newcommand{\avroraHBWriteOutCS}{96.2}
\newcommand{\avroraHBNoFPWriteTotal}{44}
\newcommand{\avroraHBWriteSameEp}{2.4}
\newcommand{\avroraHBWriteExclusive}{99.5}
\newcommand{\avroraHBWriteOwned}{\cna}
\newcommand{\avroraHBWriteShared}{0.476}
\newcommand{\avroraHBNoFPOtherEventTotal}{3562882}
\newcommand{\avroraHBAcqRelOtherTotal}{82.1}
\newcommand{\avroraHBNoAcqRelOtherTotal}{638177}
\newcommand{\avroraHBFork}{9.4E-4}
\newcommand{\avroraHBJoin}{9.4E-4}
\newcommand{\avroraHBPreWait}{50.0}
\newcommand{\avroraHBPostWait}{50.0}
\newcommand{\avroraHBVolatileTotal}{0.0}
\newcommand{\avroraHBClassInit}{0.0196}
\newcommand{\avroraHBClassAccess}{0.029}
\newcommand{\avroraHBRaceTotal}{623472}
\newcommand{\avroraHBWrRdRace}{34.9}
\newcommand{\avroraHBWrWrRace}{32.5}
\newcommand{\avroraHBRdWrRace}{0.077}
\newcommand{\avroraHBRdShWrRace}{32.5}
\newcommand{\avroraHBHoldLocksTotal}{9.2}
\newcommand{\avroraHBOneLockHeld}{5.70}
\newcommand{\avroraHBTwoNestedLocks}{<0.1}
\newcommand{\avroraHBThreeNestedLocks}{\cna}
\newcommand{\avroraHBFourNestedLocks}{\cna}
\newcommand{\avroraHBFiveNestedLocks}{\cna}
\newcommand{\avroraHBSixNestedLocks}{\cna}
\newcommand{\avroraHBSevenNestedLocks}{\cna}
\newcommand{\avroraHBEightNestedLocks}{\cna}
\newcommand{\avroraHBNineNestedLocks}{\cna}
\newcommand{\avroraHBTenNestedLocks}{\cna}
\newcommand{\avroraHBHundredNestedLocks}{\cna}
\newcommand{\avroraFTOHBEventTotal}{1,400}
\newcommand{\avroraFTOHBNoFPEventTotal}{140}
\newcommand{\avroraFTOHBNoFPAccessTotal}{140}
\newcommand{\avroraFTOHBNoFPOtherTotal}{3.6}
\newcommand{\avroraFTOHBReadTotal}{66.6}
\newcommand{\avroraFTOHBWriteTotal}{30.9}
\newcommand{\avroraFTOHBNoFPAccessInCS}{28.6}
\newcommand{\avroraFTOHBNoFPAccessOutCS}{48.6}
\newcommand{\avroraFTOHBAcqRelTotal}{52.7}
\newcommand{\avroraFTOHBOtherTotal}{11.8}
\newcommand{\avroraFTOHBNoFPReadTotal}{94}
\newcommand{\avroraFTOHBReadInCS}{6.64}
\newcommand{\avroraFTOHBReadOutCS}{93.4}
\newcommand{\avroraFTOHBReadSameEp}{0.0276}
\newcommand{\avroraFTOHBReadSharedSameEp}{\cna}
\newcommand{\avroraFTOHBReadExclusive}{5.4}
\newcommand{\avroraFTOHBReadOwned}{90.4}
\newcommand{\avroraFTOHBReadShare}{0.216}
\newcommand{\avroraFTOHBReadShared}{0.143}
\newcommand{\avroraFTOHBReadSharedOwned}{3.81}
\newcommand{\avroraFTOHBNoFPHonestWriteTotal}{44}
\newcommand{\avroraFTOHBWriteInCS}{6.22}
\newcommand{\avroraFTOHBWriteOutCS}{96.2}
\newcommand{\avroraFTOHBNoFPWriteTotal}{44}
\newcommand{\avroraFTOHBWriteSameEp}{2.4}
\newcommand{\avroraFTOHBWriteExclusive}{0.377}
\newcommand{\avroraFTOHBWriteOwned}{99.2}
\newcommand{\avroraFTOHBWriteShared}{0.414}
\newcommand{\avroraFTOHBNoFPOtherEventTotal}{3581136}
\newcommand{\avroraFTOHBAcqRelOtherTotal}{81.7}
\newcommand{\avroraFTOHBNoAcqRelOtherTotal}{655636}
\newcommand{\avroraFTOHBFork}{9.15E-4}
\newcommand{\avroraFTOHBJoin}{9.15E-4}
\newcommand{\avroraFTOHBPreWait}{50.0}
\newcommand{\avroraFTOHBPostWait}{50.0}
\newcommand{\avroraFTOHBVolatileTotal}{0.0}
\newcommand{\avroraFTOHBClassInit}{0.0191}
\newcommand{\avroraFTOHBClassAccess}{0.0282}
\newcommand{\avroraFTOHBRaceTotal}{450557}
\newcommand{\avroraFTOHBWrRdRace}{55.2}
\newcommand{\avroraFTOHBWrWrRace}{0.0}
\newcommand{\avroraFTOHBRdWrRace}{5.29}
\newcommand{\avroraFTOHBRdShWrRace}{39.5}
\newcommand{\avroraFTOHBHoldLocksTotal}{8.4}
\newcommand{\avroraFTOHBOneLockHeld}{5.76}
\newcommand{\avroraFTOHBTwoNestedLocks}{<0.1}
\newcommand{\avroraFTOHBThreeNestedLocks}{\cna}
\newcommand{\avroraFTOHBFourNestedLocks}{\cna}
\newcommand{\avroraFTOHBFiveNestedLocks}{\cna}
\newcommand{\avroraFTOHBSixNestedLocks}{\cna}
\newcommand{\avroraFTOHBSevenNestedLocks}{\cna}
\newcommand{\avroraFTOHBEightNestedLocks}{\cna}
\newcommand{\avroraFTOHBNineNestedLocks}{\cna}
\newcommand{\avroraFTOHBTenNestedLocks}{\cna}
\newcommand{\avroraFTOHBHundredNestedLocks}{\cna}
\newcommand{\avroraFTOWCPEventTotal}{1,400}
\newcommand{\avroraFTOWCPNoFPEventTotal}{140}
\newcommand{\avroraFTOWCPNoFPAccessTotal}{140}
\newcommand{\avroraFTOWCPNoFPOtherTotal}{3.7}
\newcommand{\avroraFTOWCPReadTotal}{66.6}
\newcommand{\avroraFTOWCPWriteTotal}{30.8}
\newcommand{\avroraFTOWCPNoFPAccessInCS}{28.6}
\newcommand{\avroraFTOWCPNoFPAccessOutCS}{49.0}
\newcommand{\avroraFTOWCPAcqRelTotal}{52.0}
\newcommand{\avroraFTOWCPOtherTotal}{13.3}
\newcommand{\avroraFTOWCPNoFPReadTotal}{94}
\newcommand{\avroraFTOWCPReadInCS}{6.73}
\newcommand{\avroraFTOWCPReadOutCS}{93.3}
\newcommand{\avroraFTOWCPReadSameEp}{0.0275}
\newcommand{\avroraFTOWCPReadSharedSameEp}{\cna}
\newcommand{\avroraFTOWCPReadExclusive}{2.86}
\newcommand{\avroraFTOWCPReadOwned}{90.3}
\newcommand{\avroraFTOWCPReadShare}{0.532}
\newcommand{\avroraFTOWCPReadShared}{0.454}
\newcommand{\avroraFTOWCPReadSharedOwned}{5.83}
\newcommand{\avroraFTOWCPNoFPHonestWriteTotal}{44}
\newcommand{\avroraFTOWCPWriteInCS}{6.17}
\newcommand{\avroraFTOWCPWriteOutCS}{96.3}
\newcommand{\avroraFTOWCPNoFPWriteTotal}{44}
\newcommand{\avroraFTOWCPWriteSameEp}{2.44}
\newcommand{\avroraFTOWCPWriteExclusive}{0.316}
\newcommand{\avroraFTOWCPWriteOwned}{98.9}
\newcommand{\avroraFTOWCPWriteShared}{0.779}
\newcommand{\avroraFTOWCPNoFPOtherEventTotal}{3717370}
\newcommand{\avroraFTOWCPAcqRelOtherTotal}{79.6}
\newcommand{\avroraFTOWCPNoAcqRelOtherTotal}{757250}
\newcommand{\avroraFTOWCPFork}{7.92E-4}
\newcommand{\avroraFTOWCPJoin}{7.92E-4}
\newcommand{\avroraFTOWCPPreWait}{50.0}
\newcommand{\avroraFTOWCPPostWait}{50.0}
\newcommand{\avroraFTOWCPVolatileTotal}{0.0}
\newcommand{\avroraFTOWCPClassInit}{0.0165}
\newcommand{\avroraFTOWCPClassAccess}{0.0244}
\newcommand{\avroraFTOWCPRaceTotal}{442025}
\newcommand{\avroraFTOWCPWrRdRace}{54.1}
\newcommand{\avroraFTOWCPWrWrRace}{0.0}
\newcommand{\avroraFTOWCPRdWrRace}{4.03}
\newcommand{\avroraFTOWCPRdShWrRace}{41.8}
\newcommand{\avroraFTOWCPHoldLocksTotal}{8.5}
\newcommand{\avroraFTOWCPOneLockHeld}{5.82}
\newcommand{\avroraFTOWCPTwoNestedLocks}{<0.1}
\newcommand{\avroraFTOWCPThreeNestedLocks}{\cna}
\newcommand{\avroraFTOWCPFourNestedLocks}{\cna}
\newcommand{\avroraFTOWCPFiveNestedLocks}{\cna}
\newcommand{\avroraFTOWCPSixNestedLocks}{\cna}
\newcommand{\avroraFTOWCPSevenNestedLocks}{\cna}
\newcommand{\avroraFTOWCPEightNestedLocks}{\cna}
\newcommand{\avroraFTOWCPNineNestedLocks}{\cna}
\newcommand{\avroraFTOWCPTenNestedLocks}{\cna}
\newcommand{\avroraFTOWCPHundredNestedLocks}{\cna}
\newcommand{\avroraREWCPEventTotal}{1,400}
\newcommand{\avroraREWCPNoFPEventTotal}{140}
\newcommand{\avroraREWCPNoFPAccessTotal}{140}
\newcommand{\avroraREWCPNoFPOtherTotal}{3.6}
\newcommand{\avroraREWCPReadTotal}{66.6}
\newcommand{\avroraREWCPWriteTotal}{30.8}
\newcommand{\avroraREWCPNoFPAccessInCS}{33.2}
\newcommand{\avroraREWCPNoFPAccessOutCS}{45.8}
\newcommand{\avroraREWCPAcqRelTotal}{51.4}
\newcommand{\avroraREWCPOtherTotal}{12.1}
\newcommand{\avroraREWCPNoFPReadTotal}{94}
\newcommand{\avroraREWCPReadInCS}{6.66}
\newcommand{\avroraREWCPReadOutCS}{93.4}
\newcommand{\avroraREWCPReadSameEp}{0.0275}
\newcommand{\avroraREWCPReadSharedSameEp}{\cna}
\newcommand{\avroraREWCPReadExclusive}{2.21}
\newcommand{\avroraREWCPReadOwned}{42.3}
\newcommand{\avroraREWCPReadShare}{0.856}
\newcommand{\avroraREWCPReadShared}{0.74}
\newcommand{\avroraREWCPReadSharedOwned}{53.9}
\newcommand{\avroraREWCPNoFPHonestWriteTotal}{44}
\newcommand{\avroraREWCPWriteInCS}{6.19}
\newcommand{\avroraREWCPWriteOutCS}{96.2}
\newcommand{\avroraREWCPNoFPWriteTotal}{44}
\newcommand{\avroraREWCPWriteSameEp}{2.42}
\newcommand{\avroraREWCPWriteExclusive}{0.338}
\newcommand{\avroraREWCPWriteOwned}{98.4}
\newcommand{\avroraREWCPWriteShared}{1.31}
\newcommand{\avroraREWCPNoFPOtherEventTotal}{3634025}
\newcommand{\avroraREWCPAcqRelOtherTotal}{81.0}
\newcommand{\avroraREWCPNoAcqRelOtherTotal}{691596}
\newcommand{\avroraREWCPFork}{8.68E-4}
\newcommand{\avroraREWCPJoin}{8.68E-4}
\newcommand{\avroraREWCPPreWait}{50.0}
\newcommand{\avroraREWCPPostWait}{50.0}
\newcommand{\avroraREWCPVolatileTotal}{0.0}
\newcommand{\avroraREWCPClassInit}{0.0181}
\newcommand{\avroraREWCPClassAccess}{0.0267}
\newcommand{\avroraREWCPRaceTotal}{440210}
\newcommand{\avroraREWCPWrRdRace}{53.9}
\newcommand{\avroraREWCPWrWrRace}{0.0}
\newcommand{\avroraREWCPRdWrRace}{3.77}
\newcommand{\avroraREWCPRdShWrRace}{42.3}
\newcommand{\avroraREWCPHoldLocksTotal}{8.5}
\newcommand{\avroraREWCPOneLockHeld}{5.88}
\newcommand{\avroraREWCPTwoNestedLocks}{<0.1}
\newcommand{\avroraREWCPThreeNestedLocks}{\cna}
\newcommand{\avroraREWCPFourNestedLocks}{\cna}
\newcommand{\avroraREWCPFiveNestedLocks}{\cna}
\newcommand{\avroraREWCPSixNestedLocks}{\cna}
\newcommand{\avroraREWCPSevenNestedLocks}{\cna}
\newcommand{\avroraREWCPEightNestedLocks}{\cna}
\newcommand{\avroraREWCPNineNestedLocks}{\cna}
\newcommand{\avroraREWCPTenNestedLocks}{\cna}
\newcommand{\avroraREWCPHundredNestedLocks}{\cna}
\newcommand{\avroraFTODCEventTotal}{1,400}
\newcommand{\avroraFTODCNoFPEventTotal}{140}
\newcommand{\avroraFTODCNoFPAccessTotal}{140}
\newcommand{\avroraFTODCNoFPOtherTotal}{3.7}
\newcommand{\avroraFTODCReadTotal}{66.6}
\newcommand{\avroraFTODCWriteTotal}{30.8}
\newcommand{\avroraFTODCNoFPAccessInCS}{28.7}
\newcommand{\avroraFTODCNoFPAccessOutCS}{48.9}
\newcommand{\avroraFTODCAcqRelTotal}{52.1}
\newcommand{\avroraFTODCOtherTotal}{13.2}
\newcommand{\avroraFTODCNoFPReadTotal}{94}
\newcommand{\avroraFTODCReadInCS}{6.71}
\newcommand{\avroraFTODCReadOutCS}{93.3}
\newcommand{\avroraFTODCReadSameEp}{0.0275}
\newcommand{\avroraFTODCReadSharedSameEp}{\cna}
\newcommand{\avroraFTODCReadExclusive}{2.6}
\newcommand{\avroraFTODCReadOwned}{90.3}
\newcommand{\avroraFTODCReadShare}{0.668}
\newcommand{\avroraFTODCReadShared}{0.561}
\newcommand{\avroraFTODCReadSharedOwned}{5.83}
\newcommand{\avroraFTODCNoFPHonestWriteTotal}{44}
\newcommand{\avroraFTODCWriteInCS}{6.16}
\newcommand{\avroraFTODCWriteOutCS}{96.3}
\newcommand{\avroraFTODCNoFPWriteTotal}{44}
\newcommand{\avroraFTODCWriteSameEp}{2.43}
\newcommand{\avroraFTODCWriteExclusive}{0.31}
\newcommand{\avroraFTODCWriteOwned}{98.8}
\newcommand{\avroraFTODCWriteShared}{0.937}
\newcommand{\avroraFTODCNoFPOtherEventTotal}{3704010}
\newcommand{\avroraFTODCAcqRelOtherTotal}{79.7}
\newcommand{\avroraFTODCNoAcqRelOtherTotal}{751356}
\newcommand{\avroraFTODCFork}{7.99E-4}
\newcommand{\avroraFTODCJoin}{7.99E-4}
\newcommand{\avroraFTODCPreWait}{50.0}
\newcommand{\avroraFTODCPostWait}{50.0}
\newcommand{\avroraFTODCVolatileTotal}{0.0}
\newcommand{\avroraFTODCClassInit}{0.0166}
\newcommand{\avroraFTODCClassAccess}{0.0246}
\newcommand{\avroraFTODCRaceTotal}{439826}
\newcommand{\avroraFTODCWrRdRace}{53.8}
\newcommand{\avroraFTODCWrWrRace}{0.0}
\newcommand{\avroraFTODCRdWrRace}{3.63}
\newcommand{\avroraFTODCRdShWrRace}{42.6}
\newcommand{\avroraFTODCHoldLocksTotal}{8.5}
\newcommand{\avroraFTODCOneLockHeld}{5.81}
\newcommand{\avroraFTODCTwoNestedLocks}{<0.1}
\newcommand{\avroraFTODCThreeNestedLocks}{\cna}
\newcommand{\avroraFTODCFourNestedLocks}{\cna}
\newcommand{\avroraFTODCFiveNestedLocks}{\cna}
\newcommand{\avroraFTODCSixNestedLocks}{\cna}
\newcommand{\avroraFTODCSevenNestedLocks}{\cna}
\newcommand{\avroraFTODCEightNestedLocks}{\cna}
\newcommand{\avroraFTODCNineNestedLocks}{\cna}
\newcommand{\avroraFTODCTenNestedLocks}{\cna}
\newcommand{\avroraFTODCHundredNestedLocks}{\cna}
\newcommand{\avroraREDCEventTotal}{1,400}
\newcommand{\avroraREDCNoFPEventTotal}{140}
\newcommand{\avroraREDCNoFPAccessTotal}{140}
\newcommand{\avroraREDCNoFPOtherTotal}{3.7}
\newcommand{\avroraREDCReadTotal}{66.6}
\newcommand{\avroraREDCWriteTotal}{30.8}
\newcommand{\avroraREDCNoFPAccessInCS}{34.6}
\newcommand{\avroraREDCNoFPAccessOutCS}{44.7}
\newcommand{\avroraREDCAcqRelTotal}{50.8}
\newcommand{\avroraREDCOtherTotal}{12.3}
\newcommand{\avroraREDCNoFPReadTotal}{94}
\newcommand{\avroraREDCReadInCS}{6.67}
\newcommand{\avroraREDCReadOutCS}{93.4}
\newcommand{\avroraREDCReadSameEp}{0.0275}
\newcommand{\avroraREDCReadSharedSameEp}{\cna}
\newcommand{\avroraREDCReadExclusive}{1.74}
\newcommand{\avroraREDCReadOwned}{42.3}
\newcommand{\avroraREDCReadShare}{1.1}
\newcommand{\avroraREDCReadShared}{0.933}
\newcommand{\avroraREDCReadSharedOwned}{53.9}
\newcommand{\avroraREDCNoFPHonestWriteTotal}{44}
\newcommand{\avroraREDCWriteInCS}{6.17}
\newcommand{\avroraREDCWriteOutCS}{96.3}
\newcommand{\avroraREDCNoFPWriteTotal}{44}
\newcommand{\avroraREDCWriteSameEp}{2.42}
\newcommand{\avroraREDCWriteExclusive}{0.33}
\newcommand{\avroraREDCWriteOwned}{98}
\newcommand{\avroraREDCWriteShared}{1.71}
\newcommand{\avroraREDCNoFPOtherEventTotal}{3650251}
\newcommand{\avroraREDCAcqRelOtherTotal}{80.6}
\newcommand{\avroraREDCNoAcqRelOtherTotal}{709913}
\newcommand{\avroraREDCFork}{8.45E-4}
\newcommand{\avroraREDCJoin}{8.45E-4}
\newcommand{\avroraREDCPreWait}{50.0}
\newcommand{\avroraREDCPostWait}{50.0}
\newcommand{\avroraREDCVolatileTotal}{0.0}
\newcommand{\avroraREDCClassInit}{0.0176}
\newcommand{\avroraREDCClassAccess}{0.0261}
\newcommand{\avroraREDCRaceTotal}{441227}
\newcommand{\avroraREDCWrRdRace}{54.0}
\newcommand{\avroraREDCWrWrRace}{0.0}
\newcommand{\avroraREDCRdWrRace}{3.88}
\newcommand{\avroraREDCRdShWrRace}{42.1}
\newcommand{\avroraREDCHoldLocksTotal}{8.6}
\newcommand{\avroraREDCOneLockHeld}{5.90}
\newcommand{\avroraREDCTwoNestedLocks}{<0.1}
\newcommand{\avroraREDCThreeNestedLocks}{\cna}
\newcommand{\avroraREDCFourNestedLocks}{\cna}
\newcommand{\avroraREDCFiveNestedLocks}{\cna}
\newcommand{\avroraREDCSixNestedLocks}{\cna}
\newcommand{\avroraREDCSevenNestedLocks}{\cna}
\newcommand{\avroraREDCEightNestedLocks}{\cna}
\newcommand{\avroraREDCNineNestedLocks}{\cna}
\newcommand{\avroraREDCTenNestedLocks}{\cna}
\newcommand{\avroraREDCHundredNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOEventTotal}{1,400}
\newcommand{\avroraFTOCAPONoFPEventTotal}{140}
\newcommand{\avroraFTOCAPONoFPAccessTotal}{140}
\newcommand{\avroraFTOCAPONoFPOtherTotal}{3.7}
\newcommand{\avroraFTOCAPOReadTotal}{66.6}
\newcommand{\avroraFTOCAPOWriteTotal}{30.8}
\newcommand{\avroraFTOCAPONoFPAccessInCS}{28.4}
\newcommand{\avroraFTOCAPONoFPAccessOutCS}{49.0}
\newcommand{\avroraFTOCAPOAcqRelTotal}{52.0}
\newcommand{\avroraFTOCAPOOtherTotal}{13.1}
\newcommand{\avroraFTOCAPONoFPReadTotal}{94}
\newcommand{\avroraFTOCAPOReadInCS}{6.72}
\newcommand{\avroraFTOCAPOReadOutCS}{93.3}
\newcommand{\avroraFTOCAPOReadSameEp}{0.0275}
\newcommand{\avroraFTOCAPOReadSharedSameEp}{\cna}
\newcommand{\avroraFTOCAPOReadExclusive}{2.58}
\newcommand{\avroraFTOCAPOReadOwned}{90.3}
\newcommand{\avroraFTOCAPOReadShare}{0.685}
\newcommand{\avroraFTOCAPOReadShared}{0.587}
\newcommand{\avroraFTOCAPOReadSharedOwned}{5.83}
\newcommand{\avroraFTOCAPONoFPHonestWriteTotal}{44}
\newcommand{\avroraFTOCAPOWriteInCS}{6.18}
\newcommand{\avroraFTOCAPOWriteOutCS}{96.3}
\newcommand{\avroraFTOCAPONoFPWriteTotal}{44}
\newcommand{\avroraFTOCAPOWriteSameEp}{2.43}
\newcommand{\avroraFTOCAPOWriteExclusive}{0.334}
\newcommand{\avroraFTOCAPOWriteOwned}{98.7}
\newcommand{\avroraFTOCAPOWriteShared}{0.933}
\newcommand{\avroraFTOCAPONoFPOtherEventTotal}{3698548}
\newcommand{\avroraFTOCAPOAcqRelOtherTotal}{79.9}
\newcommand{\avroraFTOCAPONoAcqRelOtherTotal}{742492}
\newcommand{\avroraFTOCAPOFork}{8.08E-4}
\newcommand{\avroraFTOCAPOJoin}{8.08E-4}
\newcommand{\avroraFTOCAPOPreWait}{50.0}
\newcommand{\avroraFTOCAPOPostWait}{50.0}
\newcommand{\avroraFTOCAPOVolatileTotal}{0.0}
\newcommand{\avroraFTOCAPOClassInit}{0.0168}
\newcommand{\avroraFTOCAPOClassAccess}{0.0249}
\newcommand{\avroraFTOCAPORaceTotal}{448577}
\newcommand{\avroraFTOCAPOWrRdRace}{54.9}
\newcommand{\avroraFTOCAPOWrWrRace}{0.0}
\newcommand{\avroraFTOCAPORdWrRace}{4.76}
\newcommand{\avroraFTOCAPORdShWrRace}{40.4}
\newcommand{\avroraFTOCAPOHoldLocksTotal}{8.5}
\newcommand{\avroraFTOCAPOOneLockHeld}{5.81}
\newcommand{\avroraFTOCAPOTwoNestedLocks}{<0.1}
\newcommand{\avroraFTOCAPOThreeNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOFourNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOSixNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOEightNestedLocks}{\cna}
\newcommand{\avroraFTOCAPONineNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOTenNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\avroraRECAPOEventTotal}{1,400}
\newcommand{\avroraRECAPONoFPEventTotal}{140}
\newcommand{\avroraRECAPONoFPAccessTotal}{140}
\newcommand{\avroraRECAPONoFPOtherTotal}{3.6}
\newcommand{\avroraRECAPOReadTotal}{66.6}
\newcommand{\avroraRECAPOWriteTotal}{30.9}
\newcommand{\avroraRECAPONoFPAccessInCS}{34.6}
\newcommand{\avroraRECAPONoFPAccessOutCS}{44.6}
\newcommand{\avroraRECAPOAcqRelTotal}{51.1}
\newcommand{\avroraRECAPOOtherTotal}{11.4}
\newcommand{\avroraRECAPONoFPReadTotal}{94}
\newcommand{\avroraRECAPOReadInCS}{6.63}
\newcommand{\avroraRECAPOReadOutCS}{93.4}
\newcommand{\avroraRECAPOReadSameEp}{0.0276}
\newcommand{\avroraRECAPOReadSharedSameEp}{\cna}
\newcommand{\avroraRECAPOReadExclusive}{1.79}
\newcommand{\avroraRECAPOReadOwned}{42.2}
\newcommand{\avroraRECAPOReadShare}{1.11}
\newcommand{\avroraRECAPOReadShared}{0.936}
\newcommand{\avroraRECAPOReadSharedOwned}{53.9}
\newcommand{\avroraRECAPONoFPHonestWriteTotal}{44}
\newcommand{\avroraRECAPOWriteInCS}{6.22}
\newcommand{\avroraRECAPOWriteOutCS}{96.2}
\newcommand{\avroraRECAPONoFPWriteTotal}{44}
\newcommand{\avroraRECAPOWriteSameEp}{2.41}
\newcommand{\avroraRECAPOWriteExclusive}{0.37}
\newcommand{\avroraRECAPOWriteOwned}{98}
\newcommand{\avroraRECAPOWriteShared}{1.68}
\newcommand{\avroraRECAPONoFPOtherEventTotal}{3580335}
\newcommand{\avroraRECAPOAcqRelOtherTotal}{81.8}
\newcommand{\avroraRECAPONoAcqRelOtherTotal}{651497}
\newcommand{\avroraRECAPOFork}{9.21E-4}
\newcommand{\avroraRECAPOJoin}{9.21E-4}
\newcommand{\avroraRECAPOPreWait}{50.0}
\newcommand{\avroraRECAPOPostWait}{50.0}
\newcommand{\avroraRECAPOVolatileTotal}{0.0}
\newcommand{\avroraRECAPOClassInit}{0.0192}
\newcommand{\avroraRECAPOClassAccess}{0.0284}
\newcommand{\avroraRECAPORaceTotal}{447814}
\newcommand{\avroraRECAPOWrRdRace}{54.8}
\newcommand{\avroraRECAPOWrWrRace}{0.0}
\newcommand{\avroraRECAPORdWrRace}{4.69}
\newcommand{\avroraRECAPORdShWrRace}{40.5}
\newcommand{\avroraRECAPOHoldLocksTotal}{8.6}
\newcommand{\avroraRECAPOOneLockHeld}{5.89}
\newcommand{\avroraRECAPOTwoNestedLocks}{<0.1}
\newcommand{\avroraRECAPOThreeNestedLocks}{\cna}
\newcommand{\avroraRECAPOFourNestedLocks}{\cna}
\newcommand{\avroraRECAPOFiveNestedLocks}{\cna}
\newcommand{\avroraRECAPOSixNestedLocks}{\cna}
\newcommand{\avroraRECAPOSevenNestedLocks}{\cna}
\newcommand{\avroraRECAPOEightNestedLocks}{\cna}
\newcommand{\avroraRECAPONineNestedLocks}{\cna}
\newcommand{\avroraRECAPOTenNestedLocks}{\cna}
\newcommand{\avroraRECAPOHundredNestedLocks}{\cna}
\newcommand{\FASTavroraMaxLiveThreads}{7}
\newcommand{\FASTavroraTotalThreads}{7}
\newcommand{\FASTavroraBaseTime}{2.4}
\newcommand{\FASTavroraBaseTimeCI}{24}
\newcommand{\FASTavroraEmptyTime}{\rna}
\newcommand{\FASTavroraEmptyTimeCI}{\rna}
\newcommand{\FASTavroraEmptyTimeCIMIN}{\rna}
\newcommand{\FASTavroraEmptyTimeCIMAX}{\rna}
\newcommand{\FASTavroraFTTime}{7.2}
\newcommand{\FASTavroraFTTimeCI}{0.18}
\newcommand{\FASTavroraHBTime}{5.8}
\newcommand{\FASTavroraHBTimeCI}{0.12}
\newcommand{\FASTavroraFTOHBTime}{6.0}
\newcommand{\FASTavroraFTOHBTimeCI}{0.1}
\newcommand{\FASTavroraWCPTime}{\rna}
\newcommand{\FASTavroraWCPTimeCI}{\rna}
\newcommand{\FASTavroraWCPTimeCIMIN}{\rna}
\newcommand{\FASTavroraWCPTimeCIMAX}{\rna}
\newcommand{\FASTavroraFTOWCPTime}{10}
\newcommand{\FASTavroraFTOWCPTimeCI}{0.22}
\newcommand{\FASTavroraREWCPTime}{8.3}
\newcommand{\FASTavroraREWCPTimeCI}{0.2}
\newcommand{\FASTavroraDCTime}{\rna}
\newcommand{\FASTavroraDCTimeCI}{\rna}
\newcommand{\FASTavroraDCTimeCIMIN}{\rna}
\newcommand{\FASTavroraDCTimeCIMAX}{\rna}
\newcommand{\FASTavroraFTODCTime}{11}
\newcommand{\FASTavroraFTODCTimeCI}{0.19}
\newcommand{\FASTavroraREDCTime}{8.9}
\newcommand{\FASTavroraREDCTimeCI}{0.24}
\newcommand{\FASTavroraCAPOTime}{\rna}
\newcommand{\FASTavroraCAPOTimeCI}{\rna}
\newcommand{\FASTavroraCAPOTimeCIMIN}{\rna}
\newcommand{\FASTavroraCAPOTimeCIMAX}{\rna}
\newcommand{\FASTavroraFTOCAPOTime}{9.0}
\newcommand{\FASTavroraFTOCAPOTimeCI}{0.2}
\newcommand{\FASTavroraRECAPOTime}{6.8}
\newcommand{\FASTavroraRECAPOTimeCI}{0.11}
\newcommand{\FASTavroraAGGCAPOTime}{\rna}
\newcommand{\FASTavroraAGGCAPOTimeCI}{\rna}
\newcommand{\FASTavroraAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTavroraAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTavroraStaticTime}{\rzero}
\newcommand{\FASTavroraDynamicTime}{\rzero}
\newcommand{\FASTavroraBaseMem}{150}
\newcommand{\FASTavroraBaseMemCI}{2.7}
\newcommand{\FASTavroraFTMem}{21}
\newcommand{\FASTavroraFTMemCI}{4.4}
\newcommand{\FASTavroraHBMem}{15}
\newcommand{\FASTavroraHBMemCI}{0.3}
\newcommand{\FASTavroraFTOHBMem}{15}
\newcommand{\FASTavroraFTOHBMemCI}{0.28}
\newcommand{\FASTavroraWCPMem}{\memna}
\newcommand{\FASTavroraWCPMemCI}{\memna}
\newcommand{\FASTavroraWCPMemCIMIN}{\memna}
\newcommand{\FASTavroraWCPMemCIMAX}{\memna}
\newcommand{\FASTavroraFTOWCPMem}{32}
\newcommand{\FASTavroraFTOWCPMemCI}{0.63}
\newcommand{\FASTavroraREWCPMem}{24}
\newcommand{\FASTavroraREWCPMemCI}{0.86}
\newcommand{\FASTavroraDCMem}{\memna}
\newcommand{\FASTavroraDCMemCI}{\memna}
\newcommand{\FASTavroraDCMemCIMIN}{\memna}
\newcommand{\FASTavroraDCMemCIMAX}{\memna}
\newcommand{\FASTavroraFTODCMem}{33}
\newcommand{\FASTavroraFTODCMemCI}{0.59}
\newcommand{\FASTavroraREDCMem}{26}
\newcommand{\FASTavroraREDCMemCI}{0.71}
\newcommand{\FASTavroraCAPOMem}{\memna}
\newcommand{\FASTavroraCAPOMemCI}{\memna}
\newcommand{\FASTavroraCAPOMemCIMIN}{\memna}
\newcommand{\FASTavroraCAPOMemCIMAX}{\memna}
\newcommand{\FASTavroraFTOCAPOMem}{29}
\newcommand{\FASTavroraFTOCAPOMemCI}{0.81}
\newcommand{\FASTavroraRECAPOMem}{16}
\newcommand{\FASTavroraRECAPOMemCI}{0.56}
\newcommand{\FASTavroraAGGCAPOMem}{\memna}
\newcommand{\FASTavroraAGGCAPOMemCI}{\memna}
\newcommand{\FASTavroraAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTavroraAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTavroraEventsCI}{21,137}
\newcommand{\FASTavroraEventsCIMIN}{1,437,301,964}
\newcommand{\FASTavroraEventsCIMAX}{1,437,344,238}
\newcommand{\FASTavroraNoFPEventsCI}{3,475}
\newcommand{\FASTavroraNoFPEventsCIMIN}{5,725,692}
\newcommand{\FASTavroraNoFPEventsCIMAX}{5,732,642}
\newcommand{\FASTavroraFT}{3}
\newcommand{\FASTavroraFTCI}{0.0}
\newcommand{\FASTavroraFTCIMIN}{3}
\newcommand{\FASTavroraFTCIMAX}{3}
\newcommand{\FASTavroraFTDynamic}{754,986}
\newcommand{\FASTavroraFTDynamicCI}{1,779}
\newcommand{\FASTavroraFTDynamicCIMIN}{753,207}
\newcommand{\FASTavroraFTDynamicCIMAX}{756,765}
\newcommand{\FASTavroraHB}{6}
\newcommand{\FASTavroraHBCI}{0.0}
\newcommand{\FASTavroraHBCIMIN}{6}
\newcommand{\FASTavroraHBCIMAX}{6}
\newcommand{\FASTavroraHBDynamic}{420,878}
\newcommand{\FASTavroraHBDynamicCI}{398}
\newcommand{\FASTavroraHBDynamicCIMIN}{420,480}
\newcommand{\FASTavroraHBDynamicCIMAX}{421,276}
\newcommand{\FASTavroraFTOHB}{6}
\newcommand{\FASTavroraFTOHBCI}{0.0}
\newcommand{\FASTavroraFTOHBCIMIN}{6}
\newcommand{\FASTavroraFTOHBCIMAX}{6}
\newcommand{\FASTavroraFTOHBDynamic}{450,557}
\newcommand{\FASTavroraFTOHBDynamicCI}{980}
\newcommand{\FASTavroraFTOHBDynamicCIMIN}{449,577}
\newcommand{\FASTavroraFTOHBDynamicCIMAX}{451,537}
\newcommand{\FASTavroraWCP}{\rna}
\newcommand{\FASTavroraWCPCI}{\rna}
\newcommand{\FASTavroraWCPCIMIN}{\rna}
\newcommand{\FASTavroraWCPCIMAX}{\rna}
\newcommand{\FASTavroraWCPDynamic}{\rna}
\newcommand{\FASTavroraWCPDynamicCI}{\rna}
\newcommand{\FASTavroraWCPDynamicCIMIN}{\rna}
\newcommand{\FASTavroraWCPDynamicCIMAX}{\rna}
\newcommand{\FASTavroraFTOWCP}{6}
\newcommand{\FASTavroraFTOWCPCI}{0.0}
\newcommand{\FASTavroraFTOWCPCIMIN}{6}
\newcommand{\FASTavroraFTOWCPCIMAX}{6}
\newcommand{\FASTavroraFTOWCPDynamic}{442,025}
\newcommand{\FASTavroraFTOWCPDynamicCI}{1,921}
\newcommand{\FASTavroraFTOWCPDynamicCIMIN}{440,104}
\newcommand{\FASTavroraFTOWCPDynamicCIMAX}{443,946}
\newcommand{\FASTavroraREWCP}{6}
\newcommand{\FASTavroraREWCPCI}{0.0}
\newcommand{\FASTavroraREWCPCIMIN}{6}
\newcommand{\FASTavroraREWCPCIMAX}{6}
\newcommand{\FASTavroraREWCPDynamic}{440,210}
\newcommand{\FASTavroraREWCPDynamicCI}{2,517}
\newcommand{\FASTavroraREWCPDynamicCIMIN}{437,693}
\newcommand{\FASTavroraREWCPDynamicCIMAX}{442,727}
\newcommand{\FASTavroraDC}{\rna}
\newcommand{\FASTavroraDCCI}{\rna}
\newcommand{\FASTavroraDCCIMIN}{\rna}
\newcommand{\FASTavroraDCCIMAX}{\rna}
\newcommand{\FASTavroraDCDynamic}{\rna}
\newcommand{\FASTavroraDCDynamicCI}{\rna}
\newcommand{\FASTavroraDCDynamicCIMIN}{\rna}
\newcommand{\FASTavroraDCDynamicCIMAX}{\rna}
\newcommand{\FASTavroraFTODC}{6}
\newcommand{\FASTavroraFTODCCI}{0.0}
\newcommand{\FASTavroraFTODCCIMIN}{6}
\newcommand{\FASTavroraFTODCCIMAX}{6}
\newcommand{\FASTavroraFTODCDynamic}{439,826}
\newcommand{\FASTavroraFTODCDynamicCI}{1,410}
\newcommand{\FASTavroraFTODCDynamicCIMIN}{438,416}
\newcommand{\FASTavroraFTODCDynamicCIMAX}{441,236}
\newcommand{\FASTavroraREDC}{6}
\newcommand{\FASTavroraREDCCI}{0.0}
\newcommand{\FASTavroraREDCCIMIN}{6}
\newcommand{\FASTavroraREDCCIMAX}{6}
\newcommand{\FASTavroraREDCDynamic}{441,227}
\newcommand{\FASTavroraREDCDynamicCI}{2,554}
\newcommand{\FASTavroraREDCDynamicCIMIN}{438,673}
\newcommand{\FASTavroraREDCDynamicCIMAX}{443,781}
\newcommand{\FASTavroraCAPO}{\rna}
\newcommand{\FASTavroraCAPOCI}{\rna}
\newcommand{\FASTavroraCAPOCIMIN}{\rna}
\newcommand{\FASTavroraCAPOCIMAX}{\rna}
\newcommand{\FASTavroraCAPODynamic}{\rna}
\newcommand{\FASTavroraCAPODynamicCI}{\rna}
\newcommand{\FASTavroraCAPODynamicCIMIN}{\rna}
\newcommand{\FASTavroraCAPODynamicCIMAX}{\rna}
\newcommand{\FASTavroraFTOCAPO}{6}
\newcommand{\FASTavroraFTOCAPOCI}{0.0}
\newcommand{\FASTavroraFTOCAPOCIMIN}{6}
\newcommand{\FASTavroraFTOCAPOCIMAX}{6}
\newcommand{\FASTavroraFTOCAPODynamic}{448,577}
\newcommand{\FASTavroraFTOCAPODynamicCI}{968}
\newcommand{\FASTavroraFTOCAPODynamicCIMIN}{447,609}
\newcommand{\FASTavroraFTOCAPODynamicCIMAX}{449,545}
\newcommand{\FASTavroraRECAPO}{6}
\newcommand{\FASTavroraRECAPOCI}{0.0}
\newcommand{\FASTavroraRECAPOCIMIN}{6}
\newcommand{\FASTavroraRECAPOCIMAX}{6}
\newcommand{\FASTavroraRECAPODynamic}{447,814}
\newcommand{\FASTavroraRECAPODynamicCI}{1,712}
\newcommand{\FASTavroraRECAPODynamicCIMIN}{446,102}
\newcommand{\FASTavroraRECAPODynamicCIMAX}{449,526}
\newcommand{\FASTavroraAGGCAPO}{\rna}
\newcommand{\FASTavroraAGGCAPOCI}{\rna}
\newcommand{\FASTavroraAGGCAPOCIMIN}{\rna}
\newcommand{\FASTavroraAGGCAPOCIMAX}{\rna}
\newcommand{\FASTavroraAGGCAPODynamic}{\rna}
\newcommand{\FASTavroraAGGCAPODynamicCI}{\rna}
\newcommand{\FASTavroraAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTavroraAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTbatikEvents}{160}
\newcommand{\FASTbatikNoFPEvents}{5.1}
\newcommand{\batikHBEventTotal}{160}
\newcommand{\batikHBNoFPEventTotal}{6.5}
\newcommand{\batikHBNoFPAccessTotal}{6.3}
\newcommand{\batikHBNoFPOtherTotal}{0.22}
\newcommand{\batikHBReadTotal}{60.4}
\newcommand{\batikHBWriteTotal}{36.2}
\newcommand{\batikHBNoFPAccessInCS}{76.2}
\newcommand{\batikHBNoFPAccessOutCS}{23.8}
\newcommand{\batikHBAcqRelTotal}{2.05}
\newcommand{\batikHBOtherTotal}{2.27}
\newcommand{\batikHBNoFPReadTotal}{3.9}
\newcommand{\batikHBReadInCS}{91.8}
\newcommand{\batikHBReadOutCS}{77.1}
\newcommand{\batikHBReadSameEp}{68.9}
\newcommand{\batikHBReadSharedSameEp}{\cna}
\newcommand{\batikHBReadExclusive}{100}
\newcommand{\batikHBReadOwned}{\cna}
\newcommand{\batikHBReadShare}{\cna}
\newcommand{\batikHBReadShared}{\cna}
\newcommand{\batikHBReadSharedOwned}{\cna}
\newcommand{\batikHBNoFPHonestWriteTotal}{2.4}
\newcommand{\batikHBWriteInCS}{134}
\newcommand{\batikHBWriteOutCS}{59.2}
\newcommand{\batikHBNoFPWriteTotal}{2.4}
\newcommand{\batikHBWriteSameEp}{93.3}
\newcommand{\batikHBWriteExclusive}{100}
\newcommand{\batikHBWriteOwned}{\cna}
\newcommand{\batikHBWriteShared}{\cna}
\newcommand{\batikHBNoFPOtherEventTotal}{221213}
\newcommand{\batikHBAcqRelOtherTotal}{47.4}
\newcommand{\batikHBNoAcqRelOtherTotal}{116273}
\newcommand{\batikHBFork}{0.00516}
\newcommand{\batikHBJoin}{0.0}
\newcommand{\batikHBPreWait}{0.0086}
\newcommand{\batikHBPostWait}{0.0086}
\newcommand{\batikHBVolatileTotal}{99.7}
\newcommand{\batikHBClassInit}{0.134}
\newcommand{\batikHBClassAccess}{0.0989}
\newcommand{\batikHBRaceTotal}{\rna}
\newcommand{\batikHBWrRdRace}{\rna}
\newcommand{\batikHBWrWrRace}{\rna}
\newcommand{\batikHBRdWrRace}{\rna}
\newcommand{\batikHBRdShWrRace}{\rna}
\newcommand{\batikHBHoldLocksTotal}{6.8}
\newcommand{\batikHBOneLockHeld}{107.}
\newcommand{\batikHBTwoNestedLocks}{<0.1}
\newcommand{\batikHBThreeNestedLocks}{<0.1}
\newcommand{\batikHBFourNestedLocks}{\cna}
\newcommand{\batikHBFiveNestedLocks}{\cna}
\newcommand{\batikHBSixNestedLocks}{\cna}
\newcommand{\batikHBSevenNestedLocks}{\cna}
\newcommand{\batikHBEightNestedLocks}{\cna}
\newcommand{\batikHBNineNestedLocks}{\cna}
\newcommand{\batikHBTenNestedLocks}{\cna}
\newcommand{\batikHBHundredNestedLocks}{\cna}
\newcommand{\batikFTOHBEventTotal}{160}
\newcommand{\batikFTOHBNoFPEventTotal}{5.8}
\newcommand{\batikFTOHBNoFPAccessTotal}{5.6}
\newcommand{\batikFTOHBNoFPOtherTotal}{0.22}
\newcommand{\batikFTOHBReadTotal}{55.7}
\newcommand{\batikFTOHBWriteTotal}{40.5}
\newcommand{\batikFTOHBNoFPAccessInCS}{76.2}
\newcommand{\batikFTOHBNoFPAccessOutCS}{23.8}
\newcommand{\batikFTOHBAcqRelTotal}{2.05}
\newcommand{\batikFTOHBOtherTotal}{2.27}
\newcommand{\batikFTOHBNoFPReadTotal}{3.2}
\newcommand{\batikFTOHBReadInCS}{97.6}
\newcommand{\batikFTOHBReadOutCS}{86.2}
\newcommand{\batikFTOHBReadSameEp}{83.8}
\newcommand{\batikFTOHBReadSharedSameEp}{\cna}
\newcommand{\batikFTOHBReadExclusive}{0.00708}
\newcommand{\batikFTOHBReadOwned}{100}
\newcommand{\batikFTOHBReadShare}{\cna}
\newcommand{\batikFTOHBReadShared}{\cna}
\newcommand{\batikFTOHBReadSharedOwned}{\cna}
\newcommand{\batikFTOHBNoFPHonestWriteTotal}{2.4}
\newcommand{\batikFTOHBWriteInCS}{134}
\newcommand{\batikFTOHBWriteOutCS}{59.2}
\newcommand{\batikFTOHBNoFPWriteTotal}{2.4}
\newcommand{\batikFTOHBWriteSameEp}{93.3}
\newcommand{\batikFTOHBWriteExclusive}{\cna}
\newcommand{\batikFTOHBWriteOwned}{100}
\newcommand{\batikFTOHBWriteShared}{\cna}
\newcommand{\batikFTOHBNoFPOtherEventTotal}{221213}
\newcommand{\batikFTOHBAcqRelOtherTotal}{47.4}
\newcommand{\batikFTOHBNoAcqRelOtherTotal}{116273}
\newcommand{\batikFTOHBFork}{0.00516}
\newcommand{\batikFTOHBJoin}{0.0}
\newcommand{\batikFTOHBPreWait}{0.0086}
\newcommand{\batikFTOHBPostWait}{0.0086}
\newcommand{\batikFTOHBVolatileTotal}{99.7}
\newcommand{\batikFTOHBClassInit}{0.134}
\newcommand{\batikFTOHBClassAccess}{0.0989}
\newcommand{\batikFTOHBRaceTotal}{\rna}
\newcommand{\batikFTOHBWrRdRace}{\rna}
\newcommand{\batikFTOHBWrWrRace}{\rna}
\newcommand{\batikFTOHBRdWrRace}{\rna}
\newcommand{\batikFTOHBRdShWrRace}{\rna}
\newcommand{\batikFTOHBHoldLocksTotal}{2.6}
\newcommand{\batikFTOHBOneLockHeld}{46.0}
\newcommand{\batikFTOHBTwoNestedLocks}{<0.1}
\newcommand{\batikFTOHBThreeNestedLocks}{<0.1}
\newcommand{\batikFTOHBFourNestedLocks}{\cna}
\newcommand{\batikFTOHBFiveNestedLocks}{\cna}
\newcommand{\batikFTOHBSixNestedLocks}{\cna}
\newcommand{\batikFTOHBSevenNestedLocks}{\cna}
\newcommand{\batikFTOHBEightNestedLocks}{\cna}
\newcommand{\batikFTOHBNineNestedLocks}{\cna}
\newcommand{\batikFTOHBTenNestedLocks}{\cna}
\newcommand{\batikFTOHBHundredNestedLocks}{\cna}
\newcommand{\batikFTOWCPEventTotal}{160}
\newcommand{\batikFTOWCPNoFPEventTotal}{5.8}
\newcommand{\batikFTOWCPNoFPAccessTotal}{5.6}
\newcommand{\batikFTOWCPNoFPOtherTotal}{0.22}
\newcommand{\batikFTOWCPReadTotal}{55.6}
\newcommand{\batikFTOWCPWriteTotal}{40.6}
\newcommand{\batikFTOWCPNoFPAccessInCS}{76.2}
\newcommand{\batikFTOWCPNoFPAccessOutCS}{23.8}
\newcommand{\batikFTOWCPAcqRelTotal}{2.05}
\newcommand{\batikFTOWCPOtherTotal}{2.27}
\newcommand{\batikFTOWCPNoFPReadTotal}{3.2}
\newcommand{\batikFTOWCPReadInCS}{97.6}
\newcommand{\batikFTOWCPReadOutCS}{86.1}
\newcommand{\batikFTOWCPReadSameEp}{83.8}
\newcommand{\batikFTOWCPReadSharedSameEp}{\cna}
\newcommand{\batikFTOWCPReadExclusive}{0.00692}
\newcommand{\batikFTOWCPReadOwned}{100}
\newcommand{\batikFTOWCPReadShare}{<0.001}
\newcommand{\batikFTOWCPReadShared}{\cna}
\newcommand{\batikFTOWCPReadSharedOwned}{\cna}
\newcommand{\batikFTOWCPNoFPHonestWriteTotal}{2.4}
\newcommand{\batikFTOWCPWriteInCS}{134}
\newcommand{\batikFTOWCPWriteOutCS}{59}
\newcommand{\batikFTOWCPNoFPWriteTotal}{2.4}
\newcommand{\batikFTOWCPWriteSameEp}{93}
\newcommand{\batikFTOWCPWriteExclusive}{\cna}
\newcommand{\batikFTOWCPWriteOwned}{100}
\newcommand{\batikFTOWCPWriteShared}{<0.001}
\newcommand{\batikFTOWCPNoFPOtherEventTotal}{221213}
\newcommand{\batikFTOWCPAcqRelOtherTotal}{47.4}
\newcommand{\batikFTOWCPNoAcqRelOtherTotal}{116273}
\newcommand{\batikFTOWCPFork}{0.00516}
\newcommand{\batikFTOWCPJoin}{0.0}
\newcommand{\batikFTOWCPPreWait}{0.0086}
\newcommand{\batikFTOWCPPostWait}{0.0086}
\newcommand{\batikFTOWCPVolatileTotal}{99.7}
\newcommand{\batikFTOWCPClassInit}{0.134}
\newcommand{\batikFTOWCPClassAccess}{0.0989}
\newcommand{\batikFTOWCPRaceTotal}{\rna}
\newcommand{\batikFTOWCPWrRdRace}{\rna}
\newcommand{\batikFTOWCPWrWrRace}{\rna}
\newcommand{\batikFTOWCPRdWrRace}{\rna}
\newcommand{\batikFTOWCPRdShWrRace}{\rna}
\newcommand{\batikFTOWCPHoldLocksTotal}{2.6}
\newcommand{\batikFTOWCPOneLockHeld}{46.1}
\newcommand{\batikFTOWCPTwoNestedLocks}{<0.1}
\newcommand{\batikFTOWCPThreeNestedLocks}{<0.1}
\newcommand{\batikFTOWCPFourNestedLocks}{\cna}
\newcommand{\batikFTOWCPFiveNestedLocks}{\cna}
\newcommand{\batikFTOWCPSixNestedLocks}{\cna}
\newcommand{\batikFTOWCPSevenNestedLocks}{\cna}
\newcommand{\batikFTOWCPEightNestedLocks}{\cna}
\newcommand{\batikFTOWCPNineNestedLocks}{\cna}
\newcommand{\batikFTOWCPTenNestedLocks}{\cna}
\newcommand{\batikFTOWCPHundredNestedLocks}{\cna}
\newcommand{\batikREWCPEventTotal}{160}
\newcommand{\batikREWCPNoFPEventTotal}{5.8}
\newcommand{\batikREWCPNoFPAccessTotal}{5.6}
\newcommand{\batikREWCPNoFPOtherTotal}{0.22}
\newcommand{\batikREWCPReadTotal}{55.6}
\newcommand{\batikREWCPWriteTotal}{40.6}
\newcommand{\batikREWCPNoFPAccessInCS}{76.2}
\newcommand{\batikREWCPNoFPAccessOutCS}{23.8}
\newcommand{\batikREWCPAcqRelTotal}{2.05}
\newcommand{\batikREWCPOtherTotal}{2.27}
\newcommand{\batikREWCPNoFPReadTotal}{3.2}
\newcommand{\batikREWCPReadInCS}{97.6}
\newcommand{\batikREWCPReadOutCS}{86.1}
\newcommand{\batikREWCPReadSameEp}{83.8}
\newcommand{\batikREWCPReadSharedSameEp}{\cna}
\newcommand{\batikREWCPReadExclusive}{0.00692}
\newcommand{\batikREWCPReadOwned}{100}
\newcommand{\batikREWCPReadShare}{<0.001}
\newcommand{\batikREWCPReadShared}{\cna}
\newcommand{\batikREWCPReadSharedOwned}{\cna}
\newcommand{\batikREWCPNoFPHonestWriteTotal}{2.4}
\newcommand{\batikREWCPWriteInCS}{134}
\newcommand{\batikREWCPWriteOutCS}{59}
\newcommand{\batikREWCPNoFPWriteTotal}{2.4}
\newcommand{\batikREWCPWriteSameEp}{93}
\newcommand{\batikREWCPWriteExclusive}{\cna}
\newcommand{\batikREWCPWriteOwned}{100}
\newcommand{\batikREWCPWriteShared}{<0.001}
\newcommand{\batikREWCPNoFPOtherEventTotal}{221213}
\newcommand{\batikREWCPAcqRelOtherTotal}{47.4}
\newcommand{\batikREWCPNoAcqRelOtherTotal}{116273}
\newcommand{\batikREWCPFork}{0.00516}
\newcommand{\batikREWCPJoin}{0.0}
\newcommand{\batikREWCPPreWait}{0.0086}
\newcommand{\batikREWCPPostWait}{0.0086}
\newcommand{\batikREWCPVolatileTotal}{99.7}
\newcommand{\batikREWCPClassInit}{0.134}
\newcommand{\batikREWCPClassAccess}{0.0989}
\newcommand{\batikREWCPRaceTotal}{\rna}
\newcommand{\batikREWCPWrRdRace}{\rna}
\newcommand{\batikREWCPWrWrRace}{\rna}
\newcommand{\batikREWCPRdWrRace}{\rna}
\newcommand{\batikREWCPRdShWrRace}{\rna}
\newcommand{\batikREWCPHoldLocksTotal}{2.6}
\newcommand{\batikREWCPOneLockHeld}{46.1}
\newcommand{\batikREWCPTwoNestedLocks}{<0.1}
\newcommand{\batikREWCPThreeNestedLocks}{<0.1}
\newcommand{\batikREWCPFourNestedLocks}{\cna}
\newcommand{\batikREWCPFiveNestedLocks}{\cna}
\newcommand{\batikREWCPSixNestedLocks}{\cna}
\newcommand{\batikREWCPSevenNestedLocks}{\cna}
\newcommand{\batikREWCPEightNestedLocks}{\cna}
\newcommand{\batikREWCPNineNestedLocks}{\cna}
\newcommand{\batikREWCPTenNestedLocks}{\cna}
\newcommand{\batikREWCPHundredNestedLocks}{\cna}
\newcommand{\batikFTODCEventTotal}{160}
\newcommand{\batikFTODCNoFPEventTotal}{5.8}
\newcommand{\batikFTODCNoFPAccessTotal}{5.6}
\newcommand{\batikFTODCNoFPOtherTotal}{0.22}
\newcommand{\batikFTODCReadTotal}{55.6}
\newcommand{\batikFTODCWriteTotal}{40.6}
\newcommand{\batikFTODCNoFPAccessInCS}{76.2}
\newcommand{\batikFTODCNoFPAccessOutCS}{23.8}
\newcommand{\batikFTODCAcqRelTotal}{2.05}
\newcommand{\batikFTODCOtherTotal}{2.27}
\newcommand{\batikFTODCNoFPReadTotal}{3.2}
\newcommand{\batikFTODCReadInCS}{97.6}
\newcommand{\batikFTODCReadOutCS}{86.1}
\newcommand{\batikFTODCReadSameEp}{83.8}
\newcommand{\batikFTODCReadSharedSameEp}{\cna}
\newcommand{\batikFTODCReadExclusive}{0.00692}
\newcommand{\batikFTODCReadOwned}{100}
\newcommand{\batikFTODCReadShare}{<0.001}
\newcommand{\batikFTODCReadShared}{\cna}
\newcommand{\batikFTODCReadSharedOwned}{\cna}
\newcommand{\batikFTODCNoFPHonestWriteTotal}{2.4}
\newcommand{\batikFTODCWriteInCS}{134}
\newcommand{\batikFTODCWriteOutCS}{59}
\newcommand{\batikFTODCNoFPWriteTotal}{2.4}
\newcommand{\batikFTODCWriteSameEp}{93}
\newcommand{\batikFTODCWriteExclusive}{\cna}
\newcommand{\batikFTODCWriteOwned}{100}
\newcommand{\batikFTODCWriteShared}{<0.001}
\newcommand{\batikFTODCNoFPOtherEventTotal}{221213}
\newcommand{\batikFTODCAcqRelOtherTotal}{47.4}
\newcommand{\batikFTODCNoAcqRelOtherTotal}{116273}
\newcommand{\batikFTODCFork}{0.00516}
\newcommand{\batikFTODCJoin}{0.0}
\newcommand{\batikFTODCPreWait}{0.0086}
\newcommand{\batikFTODCPostWait}{0.0086}
\newcommand{\batikFTODCVolatileTotal}{99.7}
\newcommand{\batikFTODCClassInit}{0.134}
\newcommand{\batikFTODCClassAccess}{0.0989}
\newcommand{\batikFTODCRaceTotal}{\rna}
\newcommand{\batikFTODCWrRdRace}{\rna}
\newcommand{\batikFTODCWrWrRace}{\rna}
\newcommand{\batikFTODCRdWrRace}{\rna}
\newcommand{\batikFTODCRdShWrRace}{\rna}
\newcommand{\batikFTODCHoldLocksTotal}{2.6}
\newcommand{\batikFTODCOneLockHeld}{46.1}
\newcommand{\batikFTODCTwoNestedLocks}{<0.1}
\newcommand{\batikFTODCThreeNestedLocks}{<0.1}
\newcommand{\batikFTODCFourNestedLocks}{\cna}
\newcommand{\batikFTODCFiveNestedLocks}{\cna}
\newcommand{\batikFTODCSixNestedLocks}{\cna}
\newcommand{\batikFTODCSevenNestedLocks}{\cna}
\newcommand{\batikFTODCEightNestedLocks}{\cna}
\newcommand{\batikFTODCNineNestedLocks}{\cna}
\newcommand{\batikFTODCTenNestedLocks}{\cna}
\newcommand{\batikFTODCHundredNestedLocks}{\cna}
\newcommand{\batikREDCEventTotal}{160}
\newcommand{\batikREDCNoFPEventTotal}{5.8}
\newcommand{\batikREDCNoFPAccessTotal}{5.6}
\newcommand{\batikREDCNoFPOtherTotal}{0.22}
\newcommand{\batikREDCReadTotal}{55.6}
\newcommand{\batikREDCWriteTotal}{40.6}
\newcommand{\batikREDCNoFPAccessInCS}{76.2}
\newcommand{\batikREDCNoFPAccessOutCS}{23.8}
\newcommand{\batikREDCAcqRelTotal}{2.05}
\newcommand{\batikREDCOtherTotal}{2.27}
\newcommand{\batikREDCNoFPReadTotal}{3.2}
\newcommand{\batikREDCReadInCS}{97.6}
\newcommand{\batikREDCReadOutCS}{86.1}
\newcommand{\batikREDCReadSameEp}{83.8}
\newcommand{\batikREDCReadSharedSameEp}{\cna}
\newcommand{\batikREDCReadExclusive}{0.00692}
\newcommand{\batikREDCReadOwned}{100}
\newcommand{\batikREDCReadShare}{<0.001}
\newcommand{\batikREDCReadShared}{\cna}
\newcommand{\batikREDCReadSharedOwned}{\cna}
\newcommand{\batikREDCNoFPHonestWriteTotal}{2.4}
\newcommand{\batikREDCWriteInCS}{134}
\newcommand{\batikREDCWriteOutCS}{59}
\newcommand{\batikREDCNoFPWriteTotal}{2.4}
\newcommand{\batikREDCWriteSameEp}{93}
\newcommand{\batikREDCWriteExclusive}{\cna}
\newcommand{\batikREDCWriteOwned}{100}
\newcommand{\batikREDCWriteShared}{<0.001}
\newcommand{\batikREDCNoFPOtherEventTotal}{221213}
\newcommand{\batikREDCAcqRelOtherTotal}{47.4}
\newcommand{\batikREDCNoAcqRelOtherTotal}{116273}
\newcommand{\batikREDCFork}{0.00516}
\newcommand{\batikREDCJoin}{0.0}
\newcommand{\batikREDCPreWait}{0.0086}
\newcommand{\batikREDCPostWait}{0.0086}
\newcommand{\batikREDCVolatileTotal}{99.7}
\newcommand{\batikREDCClassInit}{0.134}
\newcommand{\batikREDCClassAccess}{0.0989}
\newcommand{\batikREDCRaceTotal}{\rna}
\newcommand{\batikREDCWrRdRace}{\rna}
\newcommand{\batikREDCWrWrRace}{\rna}
\newcommand{\batikREDCRdWrRace}{\rna}
\newcommand{\batikREDCRdShWrRace}{\rna}
\newcommand{\batikREDCHoldLocksTotal}{2.6}
\newcommand{\batikREDCOneLockHeld}{46.1}
\newcommand{\batikREDCTwoNestedLocks}{<0.1}
\newcommand{\batikREDCThreeNestedLocks}{<0.1}
\newcommand{\batikREDCFourNestedLocks}{\cna}
\newcommand{\batikREDCFiveNestedLocks}{\cna}
\newcommand{\batikREDCSixNestedLocks}{\cna}
\newcommand{\batikREDCSevenNestedLocks}{\cna}
\newcommand{\batikREDCEightNestedLocks}{\cna}
\newcommand{\batikREDCNineNestedLocks}{\cna}
\newcommand{\batikREDCTenNestedLocks}{\cna}
\newcommand{\batikREDCHundredNestedLocks}{\cna}
\newcommand{\batikFTOCAPOEventTotal}{160}
\newcommand{\batikFTOCAPONoFPEventTotal}{5.8}
\newcommand{\batikFTOCAPONoFPAccessTotal}{5.6}
\newcommand{\batikFTOCAPONoFPOtherTotal}{0.22}
\newcommand{\batikFTOCAPOReadTotal}{55.6}
\newcommand{\batikFTOCAPOWriteTotal}{40.6}
\newcommand{\batikFTOCAPONoFPAccessInCS}{76.2}
\newcommand{\batikFTOCAPONoFPAccessOutCS}{23.8}
\newcommand{\batikFTOCAPOAcqRelTotal}{2.05}
\newcommand{\batikFTOCAPOOtherTotal}{2.27}
\newcommand{\batikFTOCAPONoFPReadTotal}{3.2}
\newcommand{\batikFTOCAPOReadInCS}{97.6}
\newcommand{\batikFTOCAPOReadOutCS}{86.1}
\newcommand{\batikFTOCAPOReadSameEp}{83.8}
\newcommand{\batikFTOCAPOReadSharedSameEp}{\cna}
\newcommand{\batikFTOCAPOReadExclusive}{0.00692}
\newcommand{\batikFTOCAPOReadOwned}{100}
\newcommand{\batikFTOCAPOReadShare}{<0.001}
\newcommand{\batikFTOCAPOReadShared}{\cna}
\newcommand{\batikFTOCAPOReadSharedOwned}{\cna}
\newcommand{\batikFTOCAPONoFPHonestWriteTotal}{2.4}
\newcommand{\batikFTOCAPOWriteInCS}{134}
\newcommand{\batikFTOCAPOWriteOutCS}{59}
\newcommand{\batikFTOCAPONoFPWriteTotal}{2.4}
\newcommand{\batikFTOCAPOWriteSameEp}{93}
\newcommand{\batikFTOCAPOWriteExclusive}{\cna}
\newcommand{\batikFTOCAPOWriteOwned}{100}
\newcommand{\batikFTOCAPOWriteShared}{<0.001}
\newcommand{\batikFTOCAPONoFPOtherEventTotal}{221213}
\newcommand{\batikFTOCAPOAcqRelOtherTotal}{47.4}
\newcommand{\batikFTOCAPONoAcqRelOtherTotal}{116273}
\newcommand{\batikFTOCAPOFork}{0.00516}
\newcommand{\batikFTOCAPOJoin}{0.0}
\newcommand{\batikFTOCAPOPreWait}{0.0086}
\newcommand{\batikFTOCAPOPostWait}{0.0086}
\newcommand{\batikFTOCAPOVolatileTotal}{99.7}
\newcommand{\batikFTOCAPOClassInit}{0.134}
\newcommand{\batikFTOCAPOClassAccess}{0.0989}
\newcommand{\batikFTOCAPORaceTotal}{\rna}
\newcommand{\batikFTOCAPOWrRdRace}{\rna}
\newcommand{\batikFTOCAPOWrWrRace}{\rna}
\newcommand{\batikFTOCAPORdWrRace}{\rna}
\newcommand{\batikFTOCAPORdShWrRace}{\rna}
\newcommand{\batikFTOCAPOHoldLocksTotal}{2.6}
\newcommand{\batikFTOCAPOOneLockHeld}{46.1}
\newcommand{\batikFTOCAPOTwoNestedLocks}{<0.1}
\newcommand{\batikFTOCAPOThreeNestedLocks}{<0.1}
\newcommand{\batikFTOCAPOFourNestedLocks}{\cna}
\newcommand{\batikFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\batikFTOCAPOSixNestedLocks}{\cna}
\newcommand{\batikFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\batikFTOCAPOEightNestedLocks}{\cna}
\newcommand{\batikFTOCAPONineNestedLocks}{\cna}
\newcommand{\batikFTOCAPOTenNestedLocks}{\cna}
\newcommand{\batikFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\batikRECAPOEventTotal}{160}
\newcommand{\batikRECAPONoFPEventTotal}{5.8}
\newcommand{\batikRECAPONoFPAccessTotal}{5.6}
\newcommand{\batikRECAPONoFPOtherTotal}{0.22}
\newcommand{\batikRECAPOReadTotal}{55.6}
\newcommand{\batikRECAPOWriteTotal}{40.6}
\newcommand{\batikRECAPONoFPAccessInCS}{76.2}
\newcommand{\batikRECAPONoFPAccessOutCS}{23.8}
\newcommand{\batikRECAPOAcqRelTotal}{2.05}
\newcommand{\batikRECAPOOtherTotal}{2.27}
\newcommand{\batikRECAPONoFPReadTotal}{3.2}
\newcommand{\batikRECAPOReadInCS}{97.6}
\newcommand{\batikRECAPOReadOutCS}{86.1}
\newcommand{\batikRECAPOReadSameEp}{83.8}
\newcommand{\batikRECAPOReadSharedSameEp}{\cna}
\newcommand{\batikRECAPOReadExclusive}{0.00692}
\newcommand{\batikRECAPOReadOwned}{100}
\newcommand{\batikRECAPOReadShare}{<0.001}
\newcommand{\batikRECAPOReadShared}{\cna}
\newcommand{\batikRECAPOReadSharedOwned}{\cna}
\newcommand{\batikRECAPONoFPHonestWriteTotal}{2.4}
\newcommand{\batikRECAPOWriteInCS}{134}
\newcommand{\batikRECAPOWriteOutCS}{59}
\newcommand{\batikRECAPONoFPWriteTotal}{2.4}
\newcommand{\batikRECAPOWriteSameEp}{93}
\newcommand{\batikRECAPOWriteExclusive}{\cna}
\newcommand{\batikRECAPOWriteOwned}{100}
\newcommand{\batikRECAPOWriteShared}{<0.001}
\newcommand{\batikRECAPONoFPOtherEventTotal}{221213}
\newcommand{\batikRECAPOAcqRelOtherTotal}{47.4}
\newcommand{\batikRECAPONoAcqRelOtherTotal}{116273}
\newcommand{\batikRECAPOFork}{0.00516}
\newcommand{\batikRECAPOJoin}{0.0}
\newcommand{\batikRECAPOPreWait}{0.0086}
\newcommand{\batikRECAPOPostWait}{0.0086}
\newcommand{\batikRECAPOVolatileTotal}{99.7}
\newcommand{\batikRECAPOClassInit}{0.134}
\newcommand{\batikRECAPOClassAccess}{0.0989}
\newcommand{\batikRECAPORaceTotal}{\rna}
\newcommand{\batikRECAPOWrRdRace}{\rna}
\newcommand{\batikRECAPOWrWrRace}{\rna}
\newcommand{\batikRECAPORdWrRace}{\rna}
\newcommand{\batikRECAPORdShWrRace}{\rna}
\newcommand{\batikRECAPOHoldLocksTotal}{2.6}
\newcommand{\batikRECAPOOneLockHeld}{46.1}
\newcommand{\batikRECAPOTwoNestedLocks}{<0.1}
\newcommand{\batikRECAPOThreeNestedLocks}{<0.1}
\newcommand{\batikRECAPOFourNestedLocks}{\cna}
\newcommand{\batikRECAPOFiveNestedLocks}{\cna}
\newcommand{\batikRECAPOSixNestedLocks}{\cna}
\newcommand{\batikRECAPOSevenNestedLocks}{\cna}
\newcommand{\batikRECAPOEightNestedLocks}{\cna}
\newcommand{\batikRECAPONineNestedLocks}{\cna}
\newcommand{\batikRECAPOTenNestedLocks}{\cna}
\newcommand{\batikRECAPOHundredNestedLocks}{\cna}
\newcommand{\FASTbatikMaxLiveThreads}{2}
\newcommand{\FASTbatikTotalThreads}{7}
\newcommand{\FASTbatikBaseTime}{2.6}
\newcommand{\FASTbatikBaseTimeCI}{48}
\newcommand{\FASTbatikEmptyTime}{\rna}
\newcommand{\FASTbatikEmptyTimeCI}{\rna}
\newcommand{\FASTbatikEmptyTimeCIMIN}{\rna}
\newcommand{\FASTbatikEmptyTimeCIMAX}{\rna}
\newcommand{\FASTbatikFTTime}{4.1}
\newcommand{\FASTbatikFTTimeCI}{0.059}
\newcommand{\FASTbatikHBTime}{4.3}
\newcommand{\FASTbatikHBTimeCI}{0.059}
\newcommand{\FASTbatikFTOHBTime}{4.3}
\newcommand{\FASTbatikFTOHBTimeCI}{0.074}
\newcommand{\FASTbatikWCPTime}{\rna}
\newcommand{\FASTbatikWCPTimeCI}{\rna}
\newcommand{\FASTbatikWCPTimeCIMIN}{\rna}
\newcommand{\FASTbatikWCPTimeCIMAX}{\rna}
\newcommand{\FASTbatikFTOWCPTime}{7.2}
\newcommand{\FASTbatikFTOWCPTimeCI}{0.15}
\newcommand{\FASTbatikREWCPTime}{5.0}
\newcommand{\FASTbatikREWCPTimeCI}{0.093}
\newcommand{\FASTbatikDCTime}{\rna}
\newcommand{\FASTbatikDCTimeCI}{\rna}
\newcommand{\FASTbatikDCTimeCIMIN}{\rna}
\newcommand{\FASTbatikDCTimeCIMAX}{\rna}
\newcommand{\FASTbatikFTODCTime}{7.2}
\newcommand{\FASTbatikFTODCTimeCI}{0.13}
\newcommand{\FASTbatikREDCTime}{5.0}
\newcommand{\FASTbatikREDCTimeCI}{0.076}
\newcommand{\FASTbatikCAPOTime}{\rna}
\newcommand{\FASTbatikCAPOTimeCI}{\rna}
\newcommand{\FASTbatikCAPOTimeCIMIN}{\rna}
\newcommand{\FASTbatikCAPOTimeCIMAX}{\rna}
\newcommand{\FASTbatikFTOCAPOTime}{7.3}
\newcommand{\FASTbatikFTOCAPOTimeCI}{0.12}
\newcommand{\FASTbatikRECAPOTime}{4.9}
\newcommand{\FASTbatikRECAPOTimeCI}{0.1}
\newcommand{\FASTbatikAGGCAPOTime}{\rna}
\newcommand{\FASTbatikAGGCAPOTimeCI}{\rna}
\newcommand{\FASTbatikAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTbatikAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTbatikStaticTime}{\rzero}
\newcommand{\FASTbatikDynamicTime}{\rzero}
\newcommand{\FASTbatikBaseMem}{220}
\newcommand{\FASTbatikBaseMemCI}{0.84}
\newcommand{\FASTbatikFTMem}{5.6}
\newcommand{\FASTbatikFTMemCI}{0.1}
\newcommand{\FASTbatikHBMem}{5.6}
\newcommand{\FASTbatikHBMemCI}{0.068}
\newcommand{\FASTbatikFTOHBMem}{5.6}
\newcommand{\FASTbatikFTOHBMemCI}{0.07}
\newcommand{\FASTbatikWCPMem}{\memna}
\newcommand{\FASTbatikWCPMemCI}{\memna}
\newcommand{\FASTbatikWCPMemCIMIN}{\memna}
\newcommand{\FASTbatikWCPMemCIMAX}{\memna}
\newcommand{\FASTbatikFTOWCPMem}{14}
\newcommand{\FASTbatikFTOWCPMemCI}{0.34}
\newcommand{\FASTbatikREWCPMem}{11}
\newcommand{\FASTbatikREWCPMemCI}{0.083}
\newcommand{\FASTbatikDCMem}{\memna}
\newcommand{\FASTbatikDCMemCI}{\memna}
\newcommand{\FASTbatikDCMemCIMIN}{\memna}
\newcommand{\FASTbatikDCMemCIMAX}{\memna}
\newcommand{\FASTbatikFTODCMem}{14}
\newcommand{\FASTbatikFTODCMemCI}{0.34}
\newcommand{\FASTbatikREDCMem}{11}
\newcommand{\FASTbatikREDCMemCI}{0.035}
\newcommand{\FASTbatikCAPOMem}{\memna}
\newcommand{\FASTbatikCAPOMemCI}{\memna}
\newcommand{\FASTbatikCAPOMemCIMIN}{\memna}
\newcommand{\FASTbatikCAPOMemCIMAX}{\memna}
\newcommand{\FASTbatikFTOCAPOMem}{14}
\newcommand{\FASTbatikFTOCAPOMemCI}{0.39}
\newcommand{\FASTbatikRECAPOMem}{12}
\newcommand{\FASTbatikRECAPOMemCI}{0.063}
\newcommand{\FASTbatikAGGCAPOMem}{\memna}
\newcommand{\FASTbatikAGGCAPOMemCI}{\memna}
\newcommand{\FASTbatikAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTbatikAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTbatikEventsCI}{0}
\newcommand{\FASTbatikEventsCIMIN}{155,322,726}
\newcommand{\FASTbatikEventsCIMAX}{155,322,726}
\newcommand{\FASTbatikNoFPEventsCI}{0}
\newcommand{\FASTbatikNoFPEventsCIMIN}{5,127,824}
\newcommand{\FASTbatikNoFPEventsCIMAX}{5,127,824}
\newcommand{\FASTbatikFT}{0}
\newcommand{\FASTbatikFTCI}{0.0}
\newcommand{\FASTbatikFTCIMIN}{0}
\newcommand{\FASTbatikFTCIMAX}{0}
\newcommand{\FASTbatikFTDynamic}{0}
\newcommand{\FASTbatikFTDynamicCI}{0.0}
\newcommand{\FASTbatikFTDynamicCIMIN}{0}
\newcommand{\FASTbatikFTDynamicCIMAX}{0}
\newcommand{\FASTbatikHB}{0}
\newcommand{\FASTbatikHBCI}{0.0}
\newcommand{\FASTbatikHBCIMIN}{0}
\newcommand{\FASTbatikHBCIMAX}{0}
\newcommand{\FASTbatikHBDynamic}{0}
\newcommand{\FASTbatikHBDynamicCI}{0.0}
\newcommand{\FASTbatikHBDynamicCIMIN}{0}
\newcommand{\FASTbatikHBDynamicCIMAX}{0}
\newcommand{\FASTbatikFTOHB}{0}
\newcommand{\FASTbatikFTOHBCI}{0.0}
\newcommand{\FASTbatikFTOHBCIMIN}{0}
\newcommand{\FASTbatikFTOHBCIMAX}{0}
\newcommand{\FASTbatikFTOHBDynamic}{0}
\newcommand{\FASTbatikFTOHBDynamicCI}{0.0}
\newcommand{\FASTbatikFTOHBDynamicCIMIN}{0}
\newcommand{\FASTbatikFTOHBDynamicCIMAX}{0}
\newcommand{\FASTbatikWCP}{\rna}
\newcommand{\FASTbatikWCPCI}{\rna}
\newcommand{\FASTbatikWCPCIMIN}{\rna}
\newcommand{\FASTbatikWCPCIMAX}{\rna}
\newcommand{\FASTbatikWCPDynamic}{\rna}
\newcommand{\FASTbatikWCPDynamicCI}{\rna}
\newcommand{\FASTbatikWCPDynamicCIMIN}{\rna}
\newcommand{\FASTbatikWCPDynamicCIMAX}{\rna}
\newcommand{\FASTbatikFTOWCP}{0}
\newcommand{\FASTbatikFTOWCPCI}{0.0}
\newcommand{\FASTbatikFTOWCPCIMIN}{0}
\newcommand{\FASTbatikFTOWCPCIMAX}{0}
\newcommand{\FASTbatikFTOWCPDynamic}{0}
\newcommand{\FASTbatikFTOWCPDynamicCI}{0.0}
\newcommand{\FASTbatikFTOWCPDynamicCIMIN}{0}
\newcommand{\FASTbatikFTOWCPDynamicCIMAX}{0}
\newcommand{\FASTbatikREWCP}{0}
\newcommand{\FASTbatikREWCPCI}{0.0}
\newcommand{\FASTbatikREWCPCIMIN}{0}
\newcommand{\FASTbatikREWCPCIMAX}{0}
\newcommand{\FASTbatikREWCPDynamic}{0}
\newcommand{\FASTbatikREWCPDynamicCI}{0.0}
\newcommand{\FASTbatikREWCPDynamicCIMIN}{0}
\newcommand{\FASTbatikREWCPDynamicCIMAX}{0}
\newcommand{\FASTbatikDC}{\rna}
\newcommand{\FASTbatikDCCI}{\rna}
\newcommand{\FASTbatikDCCIMIN}{\rna}
\newcommand{\FASTbatikDCCIMAX}{\rna}
\newcommand{\FASTbatikDCDynamic}{\rna}
\newcommand{\FASTbatikDCDynamicCI}{\rna}
\newcommand{\FASTbatikDCDynamicCIMIN}{\rna}
\newcommand{\FASTbatikDCDynamicCIMAX}{\rna}
\newcommand{\FASTbatikFTODC}{0}
\newcommand{\FASTbatikFTODCCI}{0.0}
\newcommand{\FASTbatikFTODCCIMIN}{0}
\newcommand{\FASTbatikFTODCCIMAX}{0}
\newcommand{\FASTbatikFTODCDynamic}{0}
\newcommand{\FASTbatikFTODCDynamicCI}{0.0}
\newcommand{\FASTbatikFTODCDynamicCIMIN}{0}
\newcommand{\FASTbatikFTODCDynamicCIMAX}{0}
\newcommand{\FASTbatikREDC}{0}
\newcommand{\FASTbatikREDCCI}{0.0}
\newcommand{\FASTbatikREDCCIMIN}{0}
\newcommand{\FASTbatikREDCCIMAX}{0}
\newcommand{\FASTbatikREDCDynamic}{0}
\newcommand{\FASTbatikREDCDynamicCI}{0.0}
\newcommand{\FASTbatikREDCDynamicCIMIN}{0}
\newcommand{\FASTbatikREDCDynamicCIMAX}{0}
\newcommand{\FASTbatikCAPO}{\rna}
\newcommand{\FASTbatikCAPOCI}{\rna}
\newcommand{\FASTbatikCAPOCIMIN}{\rna}
\newcommand{\FASTbatikCAPOCIMAX}{\rna}
\newcommand{\FASTbatikCAPODynamic}{\rna}
\newcommand{\FASTbatikCAPODynamicCI}{\rna}
\newcommand{\FASTbatikCAPODynamicCIMIN}{\rna}
\newcommand{\FASTbatikCAPODynamicCIMAX}{\rna}
\newcommand{\FASTbatikFTOCAPO}{0}
\newcommand{\FASTbatikFTOCAPOCI}{0.0}
\newcommand{\FASTbatikFTOCAPOCIMIN}{0}
\newcommand{\FASTbatikFTOCAPOCIMAX}{0}
\newcommand{\FASTbatikFTOCAPODynamic}{0}
\newcommand{\FASTbatikFTOCAPODynamicCI}{0.0}
\newcommand{\FASTbatikFTOCAPODynamicCIMIN}{0}
\newcommand{\FASTbatikFTOCAPODynamicCIMAX}{0}
\newcommand{\FASTbatikRECAPO}{0}
\newcommand{\FASTbatikRECAPOCI}{0.0}
\newcommand{\FASTbatikRECAPOCIMIN}{0}
\newcommand{\FASTbatikRECAPOCIMAX}{0}
\newcommand{\FASTbatikRECAPODynamic}{0}
\newcommand{\FASTbatikRECAPODynamicCI}{0.0}
\newcommand{\FASTbatikRECAPODynamicCIMIN}{0}
\newcommand{\FASTbatikRECAPODynamicCIMAX}{0}
\newcommand{\FASTbatikAGGCAPO}{\rna}
\newcommand{\FASTbatikAGGCAPOCI}{\rna}
\newcommand{\FASTbatikAGGCAPOCIMIN}{\rna}
\newcommand{\FASTbatikAGGCAPOCIMAX}{\rna}
\newcommand{\FASTbatikAGGCAPODynamic}{\rna}
\newcommand{\FASTbatikAGGCAPODynamicCI}{\rna}
\newcommand{\FASTbatikAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTbatikAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASThtwoEvents}{3,800}
\newcommand{\FASThtwoNoFPEvents}{120}
\newcommand{\htwoHBEventTotal}{3,800}
\newcommand{\htwoHBNoFPEventTotal}{340}
\newcommand{\htwoHBNoFPAccessTotal}{340}
\newcommand{\htwoHBNoFPOtherTotal}{5.1}
\newcommand{\htwoHBReadTotal}{84.9}
\newcommand{\htwoHBWriteTotal}{13.6}
\newcommand{\htwoHBNoFPAccessInCS}{96.9}
\newcommand{\htwoHBNoFPAccessOutCS}{3.02}
\newcommand{\htwoHBAcqRelTotal}{3.17}
\newcommand{\htwoHBOtherTotal}{1.13}
\newcommand{\htwoHBNoFPReadTotal}{290}
\newcommand{\htwoHBReadInCS}{94.8}
\newcommand{\htwoHBReadOutCS}{15.2}
\newcommand{\htwoHBReadSameEp}{9.99}
\newcommand{\htwoHBReadSharedSameEp}{\cna}
\newcommand{\htwoHBReadExclusive}{98.7}
\newcommand{\htwoHBReadOwned}{\cna}
\newcommand{\htwoHBReadShare}{<0.001}
\newcommand{\htwoHBReadShared}{1.26}
\newcommand{\htwoHBReadSharedOwned}{\cna}
\newcommand{\htwoHBNoFPHonestWriteTotal}{46}
\newcommand{\htwoHBWriteInCS}{258}
\newcommand{\htwoHBWriteOutCS}{24.3}
\newcommand{\htwoHBNoFPWriteTotal}{46}
\newcommand{\htwoHBWriteSameEp}{182}
\newcommand{\htwoHBWriteExclusive}{99.8}
\newcommand{\htwoHBWriteOwned}{\cna}
\newcommand{\htwoHBWriteShared}{0.24}
\newcommand{\htwoHBNoFPOtherEventTotal}{5100449}
\newcommand{\htwoHBAcqRelOtherTotal}{73.7}
\newcommand{\htwoHBNoAcqRelOtherTotal}{1339844}
\newcommand{\htwoHBFork}{0.00112}
\newcommand{\htwoHBJoin}{0.00112}
\newcommand{\htwoHBPreWait}{0.0555}
\newcommand{\htwoHBPostWait}{0.0555}
\newcommand{\htwoHBVolatileTotal}{99.9}
\newcommand{\htwoHBClassInit}{0.00269}
\newcommand{\htwoHBClassAccess}{0.0214}
\newcommand{\htwoHBRaceTotal}{128394}
\newcommand{\htwoHBWrRdRace}{32.9}
\newcommand{\htwoHBWrWrRace}{31.5}
\newcommand{\htwoHBRdWrRace}{0.0}
\newcommand{\htwoHBRdShWrRace}{35.6}
\newcommand{\htwoHBHoldLocksTotal}{390}
\newcommand{\htwoHBOneLockHeld}{117.}
\newcommand{\htwoHBTwoNestedLocks}{115.}
\newcommand{\htwoHBThreeNestedLocks}{0.14}
\newcommand{\htwoHBFourNestedLocks}{<0.1}
\newcommand{\htwoHBFiveNestedLocks}{\cna}
\newcommand{\htwoHBSixNestedLocks}{\cna}
\newcommand{\htwoHBSevenNestedLocks}{\cna}
\newcommand{\htwoHBEightNestedLocks}{\cna}
\newcommand{\htwoHBNineNestedLocks}{\cna}
\newcommand{\htwoHBTenNestedLocks}{\cna}
\newcommand{\htwoHBHundredNestedLocks}{\cna}
\newcommand{\htwoFTOHBEventTotal}{3,800}
\newcommand{\htwoFTOHBNoFPEventTotal}{300}
\newcommand{\htwoFTOHBNoFPAccessTotal}{300}
\newcommand{\htwoFTOHBNoFPOtherTotal}{5.1}
\newcommand{\htwoFTOHBReadTotal}{82.9}
\newcommand{\htwoFTOHBWriteTotal}{15.4}
\newcommand{\htwoFTOHBNoFPAccessInCS}{96.9}
\newcommand{\htwoFTOHBNoFPAccessOutCS}{3.01}
\newcommand{\htwoFTOHBAcqRelTotal}{3.17}
\newcommand{\htwoFTOHBOtherTotal}{1.13}
\newcommand{\htwoFTOHBNoFPReadTotal}{250}
\newcommand{\htwoFTOHBReadInCS}{94.2}
\newcommand{\htwoFTOHBReadOutCS}{17.3}
\newcommand{\htwoFTOHBReadSameEp}{11.6}
\newcommand{\htwoFTOHBReadSharedSameEp}{\cna}
\newcommand{\htwoFTOHBReadExclusive}{14.4}
\newcommand{\htwoFTOHBReadOwned}{84.2}
\newcommand{\htwoFTOHBReadShare}{0.0163}
\newcommand{\htwoFTOHBReadShared}{0.00632}
\newcommand{\htwoFTOHBReadSharedOwned}{1.39}
\newcommand{\htwoFTOHBNoFPHonestWriteTotal}{46}
\newcommand{\htwoFTOHBWriteInCS}{258}
\newcommand{\htwoFTOHBWriteOutCS}{24.3}
\newcommand{\htwoFTOHBNoFPWriteTotal}{46}
\newcommand{\htwoFTOHBWriteSameEp}{182}
\newcommand{\htwoFTOHBWriteExclusive}{0.302}
\newcommand{\htwoFTOHBWriteOwned}{99.6}
\newcommand{\htwoFTOHBWriteShared}{0.0867}
\newcommand{\htwoFTOHBNoFPOtherEventTotal}{5100481}
\newcommand{\htwoFTOHBAcqRelOtherTotal}{73.7}
\newcommand{\htwoFTOHBNoAcqRelOtherTotal}{1339826}
\newcommand{\htwoFTOHBFork}{0.00112}
\newcommand{\htwoFTOHBJoin}{0.00112}
\newcommand{\htwoFTOHBPreWait}{0.0543}
\newcommand{\htwoFTOHBPostWait}{0.0543}
\newcommand{\htwoFTOHBVolatileTotal}{99.9}
\newcommand{\htwoFTOHBClassInit}{0.00269}
\newcommand{\htwoFTOHBClassAccess}{0.0214}
\newcommand{\htwoFTOHBRaceTotal}{79473}
\newcommand{\htwoFTOHBWrRdRace}{49.9}
\newcommand{\htwoFTOHBWrWrRace}{0.0}
\newcommand{\htwoFTOHBRdWrRace}{0.342}
\newcommand{\htwoFTOHBRdShWrRace}{49.8}
\newcommand{\htwoFTOHBHoldLocksTotal}{250}
\newcommand{\htwoFTOHBOneLockHeld}{82.6}
\newcommand{\htwoFTOHBTwoNestedLocks}{80.6}
\newcommand{\htwoFTOHBThreeNestedLocks}{0.17}
\newcommand{\htwoFTOHBFourNestedLocks}{<0.1}
\newcommand{\htwoFTOHBFiveNestedLocks}{\cna}
\newcommand{\htwoFTOHBSixNestedLocks}{\cna}
\newcommand{\htwoFTOHBSevenNestedLocks}{\cna}
\newcommand{\htwoFTOHBEightNestedLocks}{\cna}
\newcommand{\htwoFTOHBNineNestedLocks}{\cna}
\newcommand{\htwoFTOHBTenNestedLocks}{\cna}
\newcommand{\htwoFTOHBHundredNestedLocks}{\cna}
\newcommand{\htwoFTOWCPEventTotal}{3,800}
\newcommand{\htwoFTOWCPNoFPEventTotal}{310}
\newcommand{\htwoFTOWCPNoFPAccessTotal}{300}
\newcommand{\htwoFTOWCPNoFPOtherTotal}{5.1}
\newcommand{\htwoFTOWCPReadTotal}{83.1}
\newcommand{\htwoFTOWCPWriteTotal}{15.2}
\newcommand{\htwoFTOWCPNoFPAccessInCS}{96.9}
\newcommand{\htwoFTOWCPNoFPAccessOutCS}{3.01}
\newcommand{\htwoFTOWCPAcqRelTotal}{3.17}
\newcommand{\htwoFTOWCPOtherTotal}{1.13}
\newcommand{\htwoFTOWCPNoFPReadTotal}{250}
\newcommand{\htwoFTOWCPReadInCS}{94.3}
\newcommand{\htwoFTOWCPReadOutCS}{17.1}
\newcommand{\htwoFTOWCPReadSameEp}{11.4}
\newcommand{\htwoFTOWCPReadSharedSameEp}{\cna}
\newcommand{\htwoFTOWCPReadExclusive}{11.8}
\newcommand{\htwoFTOWCPReadOwned}{83.5}
\newcommand{\htwoFTOWCPReadShare}{0.0485}
\newcommand{\htwoFTOWCPReadShared}{0.174}
\newcommand{\htwoFTOWCPReadSharedOwned}{4.47}
\newcommand{\htwoFTOWCPNoFPHonestWriteTotal}{46}
\newcommand{\htwoFTOWCPWriteInCS}{258}
\newcommand{\htwoFTOWCPWriteOutCS}{24.3}
\newcommand{\htwoFTOWCPNoFPWriteTotal}{46}
\newcommand{\htwoFTOWCPWriteSameEp}{182}
\newcommand{\htwoFTOWCPWriteExclusive}{0.306}
\newcommand{\htwoFTOWCPWriteOwned}{99.5}
\newcommand{\htwoFTOWCPWriteShared}{0.172}
\newcommand{\htwoFTOWCPNoFPOtherEventTotal}{5103461}
\newcommand{\htwoFTOWCPAcqRelOtherTotal}{73.7}
\newcommand{\htwoFTOWCPNoAcqRelOtherTotal}{1342209}
\newcommand{\htwoFTOWCPFork}{0.00112}
\newcommand{\htwoFTOWCPJoin}{0.00112}
\newcommand{\htwoFTOWCPPreWait}{0.13}
\newcommand{\htwoFTOWCPPostWait}{0.13}
\newcommand{\htwoFTOWCPVolatileTotal}{99.7}
\newcommand{\htwoFTOWCPClassInit}{0.00268}
\newcommand{\htwoFTOWCPClassAccess}{0.0214}
\newcommand{\htwoFTOWCPRaceTotal}{85962}
\newcommand{\htwoFTOWCPWrRdRace}{49.9}
\newcommand{\htwoFTOWCPWrWrRace}{0.0}
\newcommand{\htwoFTOWCPRdWrRace}{0.465}
\newcommand{\htwoFTOWCPRdShWrRace}{49.6}
\newcommand{\htwoFTOWCPHoldLocksTotal}{250}
\newcommand{\htwoFTOWCPOneLockHeld}{82.8}
\newcommand{\htwoFTOWCPTwoNestedLocks}{80.1}
\newcommand{\htwoFTOWCPThreeNestedLocks}{0.17}
\newcommand{\htwoFTOWCPFourNestedLocks}{<0.1}
\newcommand{\htwoFTOWCPFiveNestedLocks}{\cna}
\newcommand{\htwoFTOWCPSixNestedLocks}{\cna}
\newcommand{\htwoFTOWCPSevenNestedLocks}{\cna}
\newcommand{\htwoFTOWCPEightNestedLocks}{\cna}
\newcommand{\htwoFTOWCPNineNestedLocks}{\cna}
\newcommand{\htwoFTOWCPTenNestedLocks}{\cna}
\newcommand{\htwoFTOWCPHundredNestedLocks}{\cna}
\newcommand{\htwoREWCPEventTotal}{3,800}
\newcommand{\htwoREWCPNoFPEventTotal}{300}
\newcommand{\htwoREWCPNoFPAccessTotal}{300}
\newcommand{\htwoREWCPNoFPOtherTotal}{5.1}
\newcommand{\htwoREWCPReadTotal}{83.1}
\newcommand{\htwoREWCPWriteTotal}{15.2}
\newcommand{\htwoREWCPNoFPAccessInCS}{96.9}
\newcommand{\htwoREWCPNoFPAccessOutCS}{3.01}
\newcommand{\htwoREWCPAcqRelTotal}{3.17}
\newcommand{\htwoREWCPOtherTotal}{1.13}
\newcommand{\htwoREWCPNoFPReadTotal}{250}
\newcommand{\htwoREWCPReadInCS}{94.3}
\newcommand{\htwoREWCPReadOutCS}{17.1}
\newcommand{\htwoREWCPReadSameEp}{11.5}
\newcommand{\htwoREWCPReadSharedSameEp}{\cna}
\newcommand{\htwoREWCPReadExclusive}{10}
\newcommand{\htwoREWCPReadOwned}{83.1}
\newcommand{\htwoREWCPReadShare}{0.201}
\newcommand{\htwoREWCPReadShared}{0.374}
\newcommand{\htwoREWCPReadSharedOwned}{6.32}
\newcommand{\htwoREWCPNoFPHonestWriteTotal}{46}
\newcommand{\htwoREWCPWriteInCS}{258}
\newcommand{\htwoREWCPWriteOutCS}{24.2}
\newcommand{\htwoREWCPNoFPWriteTotal}{46}
\newcommand{\htwoREWCPWriteSameEp}{182}
\newcommand{\htwoREWCPWriteExclusive}{0.29}
\newcommand{\htwoREWCPWriteOwned}{98.9}
\newcommand{\htwoREWCPWriteShared}{0.814}
\newcommand{\htwoREWCPNoFPOtherEventTotal}{5100920}
\newcommand{\htwoREWCPAcqRelOtherTotal}{73.7}
\newcommand{\htwoREWCPNoAcqRelOtherTotal}{1340142}
\newcommand{\htwoREWCPFork}{0.00112}
\newcommand{\htwoREWCPJoin}{0.00112}
\newcommand{\htwoREWCPPreWait}{0.0645}
\newcommand{\htwoREWCPPostWait}{0.0645}
\newcommand{\htwoREWCPVolatileTotal}{99.8}
\newcommand{\htwoREWCPClassInit}{0.00269}
\newcommand{\htwoREWCPClassAccess}{0.0214}
\newcommand{\htwoREWCPRaceTotal}{83082}
\newcommand{\htwoREWCPWrRdRace}{49.9}
\newcommand{\htwoREWCPWrWrRace}{0.0}
\newcommand{\htwoREWCPRdWrRace}{0.129}
\newcommand{\htwoREWCPRdShWrRace}{50.0}
\newcommand{\htwoREWCPHoldLocksTotal}{250}
\newcommand{\htwoREWCPOneLockHeld}{82.8}
\newcommand{\htwoREWCPTwoNestedLocks}{80.1}
\newcommand{\htwoREWCPThreeNestedLocks}{0.17}
\newcommand{\htwoREWCPFourNestedLocks}{<0.1}
\newcommand{\htwoREWCPFiveNestedLocks}{\cna}
\newcommand{\htwoREWCPSixNestedLocks}{\cna}
\newcommand{\htwoREWCPSevenNestedLocks}{\cna}
\newcommand{\htwoREWCPEightNestedLocks}{\cna}
\newcommand{\htwoREWCPNineNestedLocks}{\cna}
\newcommand{\htwoREWCPTenNestedLocks}{\cna}
\newcommand{\htwoREWCPHundredNestedLocks}{\cna}
\newcommand{\htwoFTODCEventTotal}{3,800}
\newcommand{\htwoFTODCNoFPEventTotal}{310}
\newcommand{\htwoFTODCNoFPAccessTotal}{300}
\newcommand{\htwoFTODCNoFPOtherTotal}{5.1}
\newcommand{\htwoFTODCReadTotal}{83.1}
\newcommand{\htwoFTODCWriteTotal}{15.2}
\newcommand{\htwoFTODCNoFPAccessInCS}{96.9}
\newcommand{\htwoFTODCNoFPAccessOutCS}{3.02}
\newcommand{\htwoFTODCAcqRelTotal}{3.17}
\newcommand{\htwoFTODCOtherTotal}{1.13}
\newcommand{\htwoFTODCNoFPReadTotal}{250}
\newcommand{\htwoFTODCReadInCS}{94.3}
\newcommand{\htwoFTODCReadOutCS}{17.1}
\newcommand{\htwoFTODCReadSameEp}{11.4}
\newcommand{\htwoFTODCReadSharedSameEp}{\cna}
\newcommand{\htwoFTODCReadExclusive}{10.9}
\newcommand{\htwoFTODCReadOwned}{83.3}
\newcommand{\htwoFTODCReadShare}{0.0794}
\newcommand{\htwoFTODCReadShared}{0.338}
\newcommand{\htwoFTODCReadSharedOwned}{5.35}
\newcommand{\htwoFTODCNoFPHonestWriteTotal}{46}
\newcommand{\htwoFTODCWriteInCS}{258}
\newcommand{\htwoFTODCWriteOutCS}{24.3}
\newcommand{\htwoFTODCNoFPWriteTotal}{46}
\newcommand{\htwoFTODCWriteSameEp}{182}
\newcommand{\htwoFTODCWriteExclusive}{0.302}
\newcommand{\htwoFTODCWriteOwned}{99.5}
\newcommand{\htwoFTODCWriteShared}{0.238}
\newcommand{\htwoFTODCNoFPOtherEventTotal}{5103368}
\newcommand{\htwoFTODCAcqRelOtherTotal}{73.7}
\newcommand{\htwoFTODCNoAcqRelOtherTotal}{1342230}
\newcommand{\htwoFTODCFork}{0.00112}
\newcommand{\htwoFTODCJoin}{0.00112}
\newcommand{\htwoFTODCPreWait}{0.132}
\newcommand{\htwoFTODCPostWait}{0.132}
\newcommand{\htwoFTODCVolatileTotal}{99.7}
\newcommand{\htwoFTODCClassInit}{0.00268}
\newcommand{\htwoFTODCClassAccess}{0.0214}
\newcommand{\htwoFTODCRaceTotal}{86790}
\newcommand{\htwoFTODCWrRdRace}{49.8}
\newcommand{\htwoFTODCWrWrRace}{0.0}
\newcommand{\htwoFTODCRdWrRace}{0.342}
\newcommand{\htwoFTODCRdShWrRace}{49.9}
\newcommand{\htwoFTODCHoldLocksTotal}{250}
\newcommand{\htwoFTODCOneLockHeld}{82.8}
\newcommand{\htwoFTODCTwoNestedLocks}{80.1}
\newcommand{\htwoFTODCThreeNestedLocks}{0.17}
\newcommand{\htwoFTODCFourNestedLocks}{<0.1}
\newcommand{\htwoFTODCFiveNestedLocks}{\cna}
\newcommand{\htwoFTODCSixNestedLocks}{\cna}
\newcommand{\htwoFTODCSevenNestedLocks}{\cna}
\newcommand{\htwoFTODCEightNestedLocks}{\cna}
\newcommand{\htwoFTODCNineNestedLocks}{\cna}
\newcommand{\htwoFTODCTenNestedLocks}{\cna}
\newcommand{\htwoFTODCHundredNestedLocks}{\cna}
\newcommand{\htwoREDCEventTotal}{3,800}
\newcommand{\htwoREDCNoFPEventTotal}{300}
\newcommand{\htwoREDCNoFPAccessTotal}{300}
\newcommand{\htwoREDCNoFPOtherTotal}{5.1}
\newcommand{\htwoREDCReadTotal}{83.1}
\newcommand{\htwoREDCWriteTotal}{15.2}
\newcommand{\htwoREDCNoFPAccessInCS}{96.9}
\newcommand{\htwoREDCNoFPAccessOutCS}{3.01}
\newcommand{\htwoREDCAcqRelTotal}{3.17}
\newcommand{\htwoREDCOtherTotal}{1.13}
\newcommand{\htwoREDCNoFPReadTotal}{250}
\newcommand{\htwoREDCReadInCS}{94.3}
\newcommand{\htwoREDCReadOutCS}{17.1}
\newcommand{\htwoREDCReadSameEp}{11.5}
\newcommand{\htwoREDCReadSharedSameEp}{\cna}
\newcommand{\htwoREDCReadExclusive}{7.4}
\newcommand{\htwoREDCReadOwned}{82.6}
\newcommand{\htwoREDCReadShare}{0.265}
\newcommand{\htwoREDCReadShared}{0.896}
\newcommand{\htwoREDCReadSharedOwned}{8.83}
\newcommand{\htwoREDCNoFPHonestWriteTotal}{46}
\newcommand{\htwoREDCWriteInCS}{258}
\newcommand{\htwoREDCWriteOutCS}{24.2}
\newcommand{\htwoREDCNoFPWriteTotal}{46}
\newcommand{\htwoREDCWriteSameEp}{182}
\newcommand{\htwoREDCWriteExclusive}{0.286}
\newcommand{\htwoREDCWriteOwned}{98.8}
\newcommand{\htwoREDCWriteShared}{0.897}
\newcommand{\htwoREDCNoFPOtherEventTotal}{5100916}
\newcommand{\htwoREDCAcqRelOtherTotal}{73.7}
\newcommand{\htwoREDCNoAcqRelOtherTotal}{1340155}
\newcommand{\htwoREDCFork}{0.00112}
\newcommand{\htwoREDCJoin}{0.00112}
\newcommand{\htwoREDCPreWait}{0.0655}
\newcommand{\htwoREDCPostWait}{0.0655}
\newcommand{\htwoREDCVolatileTotal}{99.8}
\newcommand{\htwoREDCClassInit}{0.00269}
\newcommand{\htwoREDCClassAccess}{0.0214}
\newcommand{\htwoREDCRaceTotal}{84154}
\newcommand{\htwoREDCWrRdRace}{49.8}
\newcommand{\htwoREDCWrWrRace}{0.0}
\newcommand{\htwoREDCRdWrRace}{0.134}
\newcommand{\htwoREDCRdShWrRace}{50.0}
\newcommand{\htwoREDCHoldLocksTotal}{250}
\newcommand{\htwoREDCOneLockHeld}{82.8}
\newcommand{\htwoREDCTwoNestedLocks}{80.1}
\newcommand{\htwoREDCThreeNestedLocks}{0.17}
\newcommand{\htwoREDCFourNestedLocks}{<0.1}
\newcommand{\htwoREDCFiveNestedLocks}{\cna}
\newcommand{\htwoREDCSixNestedLocks}{\cna}
\newcommand{\htwoREDCSevenNestedLocks}{\cna}
\newcommand{\htwoREDCEightNestedLocks}{\cna}
\newcommand{\htwoREDCNineNestedLocks}{\cna}
\newcommand{\htwoREDCTenNestedLocks}{\cna}
\newcommand{\htwoREDCHundredNestedLocks}{\cna}
\newcommand{\htwoFTOCAPOEventTotal}{3,800}
\newcommand{\htwoFTOCAPONoFPEventTotal}{310}
\newcommand{\htwoFTOCAPONoFPAccessTotal}{300}
\newcommand{\htwoFTOCAPONoFPOtherTotal}{5.1}
\newcommand{\htwoFTOCAPOReadTotal}{83.1}
\newcommand{\htwoFTOCAPOWriteTotal}{15.2}
\newcommand{\htwoFTOCAPONoFPAccessInCS}{96.9}
\newcommand{\htwoFTOCAPONoFPAccessOutCS}{3.02}
\newcommand{\htwoFTOCAPOAcqRelTotal}{3.17}
\newcommand{\htwoFTOCAPOOtherTotal}{1.13}
\newcommand{\htwoFTOCAPONoFPReadTotal}{250}
\newcommand{\htwoFTOCAPOReadInCS}{94.3}
\newcommand{\htwoFTOCAPOReadOutCS}{17.1}
\newcommand{\htwoFTOCAPOReadSameEp}{11.4}
\newcommand{\htwoFTOCAPOReadSharedSameEp}{\cna}
\newcommand{\htwoFTOCAPOReadExclusive}{11}
\newcommand{\htwoFTOCAPOReadOwned}{83.3}
\newcommand{\htwoFTOCAPOReadShare}{0.0788}
\newcommand{\htwoFTOCAPOReadShared}{0.338}
\newcommand{\htwoFTOCAPOReadSharedOwned}{5.34}
\newcommand{\htwoFTOCAPONoFPHonestWriteTotal}{46}
\newcommand{\htwoFTOCAPOWriteInCS}{258}
\newcommand{\htwoFTOCAPOWriteOutCS}{24.3}
\newcommand{\htwoFTOCAPONoFPWriteTotal}{46}
\newcommand{\htwoFTOCAPOWriteSameEp}{182}
\newcommand{\htwoFTOCAPOWriteExclusive}{0.303}
\newcommand{\htwoFTOCAPOWriteOwned}{99.5}
\newcommand{\htwoFTOCAPOWriteShared}{0.238}
\newcommand{\htwoFTOCAPONoFPOtherEventTotal}{5103971}
\newcommand{\htwoFTOCAPOAcqRelOtherTotal}{73.7}
\newcommand{\htwoFTOCAPONoAcqRelOtherTotal}{1342240}
\newcommand{\htwoFTOCAPOFork}{0.00112}
\newcommand{\htwoFTOCAPOJoin}{0.00112}
\newcommand{\htwoFTOCAPOPreWait}{0.128}
\newcommand{\htwoFTOCAPOPostWait}{0.128}
\newcommand{\htwoFTOCAPOVolatileTotal}{99.7}
\newcommand{\htwoFTOCAPOClassInit}{0.00268}
\newcommand{\htwoFTOCAPOClassAccess}{0.0214}
\newcommand{\htwoFTOCAPORaceTotal}{86963}
\newcommand{\htwoFTOCAPOWrRdRace}{49.8}
\newcommand{\htwoFTOCAPOWrWrRace}{0.0}
\newcommand{\htwoFTOCAPORdWrRace}{0.448}
\newcommand{\htwoFTOCAPORdShWrRace}{49.7}
\newcommand{\htwoFTOCAPOHoldLocksTotal}{250}
\newcommand{\htwoFTOCAPOOneLockHeld}{82.8}
\newcommand{\htwoFTOCAPOTwoNestedLocks}{80.1}
\newcommand{\htwoFTOCAPOThreeNestedLocks}{0.17}
\newcommand{\htwoFTOCAPOFourNestedLocks}{<0.1}
\newcommand{\htwoFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\htwoFTOCAPOSixNestedLocks}{\cna}
\newcommand{\htwoFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\htwoFTOCAPOEightNestedLocks}{\cna}
\newcommand{\htwoFTOCAPONineNestedLocks}{\cna}
\newcommand{\htwoFTOCAPOTenNestedLocks}{\cna}
\newcommand{\htwoFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\htwoRECAPOEventTotal}{3,800}
\newcommand{\htwoRECAPONoFPEventTotal}{300}
\newcommand{\htwoRECAPONoFPAccessTotal}{300}
\newcommand{\htwoRECAPONoFPOtherTotal}{5.1}
\newcommand{\htwoRECAPOReadTotal}{83.1}
\newcommand{\htwoRECAPOWriteTotal}{15.2}
\newcommand{\htwoRECAPONoFPAccessInCS}{96.9}
\newcommand{\htwoRECAPONoFPAccessOutCS}{3.01}
\newcommand{\htwoRECAPOAcqRelTotal}{3.17}
\newcommand{\htwoRECAPOOtherTotal}{1.13}
\newcommand{\htwoRECAPONoFPReadTotal}{250}
\newcommand{\htwoRECAPOReadInCS}{94.3}
\newcommand{\htwoRECAPOReadOutCS}{17.1}
\newcommand{\htwoRECAPOReadSameEp}{11.5}
\newcommand{\htwoRECAPOReadSharedSameEp}{\cna}
\newcommand{\htwoRECAPOReadExclusive}{7.55}
\newcommand{\htwoRECAPOReadOwned}{82.6}
\newcommand{\htwoRECAPOReadShare}{0.259}
\newcommand{\htwoRECAPOReadShared}{0.863}
\newcommand{\htwoRECAPOReadSharedOwned}{8.7}
\newcommand{\htwoRECAPONoFPHonestWriteTotal}{46}
\newcommand{\htwoRECAPOWriteInCS}{258}
\newcommand{\htwoRECAPOWriteOutCS}{24.2}
\newcommand{\htwoRECAPONoFPWriteTotal}{46}
\newcommand{\htwoRECAPOWriteSameEp}{182}
\newcommand{\htwoRECAPOWriteExclusive}{0.286}
\newcommand{\htwoRECAPOWriteOwned}{98.8}
\newcommand{\htwoRECAPOWriteShared}{0.88}
\newcommand{\htwoRECAPONoFPOtherEventTotal}{5100766}
\newcommand{\htwoRECAPOAcqRelOtherTotal}{73.7}
\newcommand{\htwoRECAPONoAcqRelOtherTotal}{1340025}
\newcommand{\htwoRECAPOFork}{0.00112}
\newcommand{\htwoRECAPOJoin}{0.00112}
\newcommand{\htwoRECAPOPreWait}{0.0613}
\newcommand{\htwoRECAPOPostWait}{0.0613}
\newcommand{\htwoRECAPOVolatileTotal}{99.9}
\newcommand{\htwoRECAPOClassInit}{0.00269}
\newcommand{\htwoRECAPOClassAccess}{0.0214}
\newcommand{\htwoRECAPORaceTotal}{83476}
\newcommand{\htwoRECAPOWrRdRace}{49.9}
\newcommand{\htwoRECAPOWrWrRace}{0.0}
\newcommand{\htwoRECAPORdWrRace}{0.328}
\newcommand{\htwoRECAPORdShWrRace}{49.8}
\newcommand{\htwoRECAPOHoldLocksTotal}{250}
\newcommand{\htwoRECAPOOneLockHeld}{82.8}
\newcommand{\htwoRECAPOTwoNestedLocks}{80.1}
\newcommand{\htwoRECAPOThreeNestedLocks}{0.17}
\newcommand{\htwoRECAPOFourNestedLocks}{<0.1}
\newcommand{\htwoRECAPOFiveNestedLocks}{\cna}
\newcommand{\htwoRECAPOSixNestedLocks}{\cna}
\newcommand{\htwoRECAPOSevenNestedLocks}{\cna}
\newcommand{\htwoRECAPOEightNestedLocks}{\cna}
\newcommand{\htwoRECAPONineNestedLocks}{\cna}
\newcommand{\htwoRECAPOTenNestedLocks}{\cna}
\newcommand{\htwoRECAPOHundredNestedLocks}{\cna}
\newcommand{\FASThtwoMaxLiveThreads}{15}
\newcommand{\FASThtwoTotalThreads}{16}
\newcommand{\FASThtwoBaseTime}{4.9}
\newcommand{\FASThtwoBaseTimeCI}{62}
\newcommand{\FASThtwoEmptyTime}{\rna}
\newcommand{\FASThtwoEmptyTimeCI}{\rna}
\newcommand{\FASThtwoEmptyTimeCIMIN}{\rna}
\newcommand{\FASThtwoEmptyTimeCIMAX}{\rna}
\newcommand{\FASThtwoFTTime}{9.3}
\newcommand{\FASThtwoFTTimeCI}{0.15}
\newcommand{\FASThtwoHBTime}{9.7}
\newcommand{\FASThtwoHBTimeCI}{0.17}
\newcommand{\FASThtwoFTOHBTime}{9.6}
\newcommand{\FASThtwoFTOHBTimeCI}{0.19}
\newcommand{\FASThtwoWCPTime}{\rna}
\newcommand{\FASThtwoWCPTimeCI}{\rna}
\newcommand{\FASThtwoWCPTimeCIMIN}{\rna}
\newcommand{\FASThtwoWCPTimeCIMAX}{\rna}
\newcommand{\FASThtwoFTOWCPTime}{57}
\newcommand{\FASThtwoFTOWCPTimeCI}{4.6}
\newcommand{\FASThtwoREWCPTime}{13}
\newcommand{\FASThtwoREWCPTimeCI}{0.49}
\newcommand{\FASThtwoDCTime}{\rna}
\newcommand{\FASThtwoDCTimeCI}{\rna}
\newcommand{\FASThtwoDCTimeCIMIN}{\rna}
\newcommand{\FASThtwoDCTimeCIMAX}{\rna}
\newcommand{\FASThtwoFTODCTime}{60}
\newcommand{\FASThtwoFTODCTimeCI}{5.4}
\newcommand{\FASThtwoREDCTime}{14}
\newcommand{\FASThtwoREDCTimeCI}{0.17}
\newcommand{\FASThtwoCAPOTime}{\rna}
\newcommand{\FASThtwoCAPOTimeCI}{\rna}
\newcommand{\FASThtwoCAPOTimeCIMIN}{\rna}
\newcommand{\FASThtwoCAPOTimeCIMAX}{\rna}
\newcommand{\FASThtwoFTOCAPOTime}{55}
\newcommand{\FASThtwoFTOCAPOTimeCI}{4.0}
\newcommand{\FASThtwoRECAPOTime}{12}
\newcommand{\FASThtwoRECAPOTimeCI}{0.2}
\newcommand{\FASThtwoAGGCAPOTime}{\rna}
\newcommand{\FASThtwoAGGCAPOTimeCI}{\rna}
\newcommand{\FASThtwoAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASThtwoAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASThtwoStaticTime}{\rzero}
\newcommand{\FASThtwoDynamicTime}{\rzero}
\newcommand{\FASThtwoBaseMem}{1,800}
\newcommand{\FASThtwoBaseMemCI}{43.0}
\newcommand{\FASThtwoFTMem}{3.0}
\newcommand{\FASThtwoFTMemCI}{0.075}
\newcommand{\FASThtwoHBMem}{3.0}
\newcommand{\FASThtwoHBMemCI}{0.074}
\newcommand{\FASThtwoFTOHBMem}{3.0}
\newcommand{\FASThtwoFTOHBMemCI}{0.082}
\newcommand{\FASThtwoWCPMem}{\memna}
\newcommand{\FASThtwoWCPMemCI}{\memna}
\newcommand{\FASThtwoWCPMemCIMIN}{\memna}
\newcommand{\FASThtwoWCPMemCIMAX}{\memna}
\newcommand{\FASThtwoFTOWCPMem}{39}
\newcommand{\FASThtwoFTOWCPMemCI}{2.3}
\newcommand{\FASThtwoREWCPMem}{8.3}
\newcommand{\FASThtwoREWCPMemCI}{0.2}
\newcommand{\FASThtwoDCMem}{\memna}
\newcommand{\FASThtwoDCMemCI}{\memna}
\newcommand{\FASThtwoDCMemCIMIN}{\memna}
\newcommand{\FASThtwoDCMemCIMAX}{\memna}
\newcommand{\FASThtwoFTODCMem}{41}
\newcommand{\FASThtwoFTODCMemCI}{2.0}
\newcommand{\FASThtwoREDCMem}{8.3}
\newcommand{\FASThtwoREDCMemCI}{0.28}
\newcommand{\FASThtwoCAPOMem}{\memna}
\newcommand{\FASThtwoCAPOMemCI}{\memna}
\newcommand{\FASThtwoCAPOMemCIMIN}{\memna}
\newcommand{\FASThtwoCAPOMemCIMAX}{\memna}
\newcommand{\FASThtwoFTOCAPOMem}{40}
\newcommand{\FASThtwoFTOCAPOMemCI}{1.7}
\newcommand{\FASThtwoRECAPOMem}{7.2}
\newcommand{\FASThtwoRECAPOMemCI}{0.22}
\newcommand{\FASThtwoAGGCAPOMem}{\memna}
\newcommand{\FASThtwoAGGCAPOMemCI}{\memna}
\newcommand{\FASThtwoAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASThtwoAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASThtwoEventsCI}{1,140,435}
\newcommand{\FASThtwoEventsCIMIN}{3,811,302,310}
\newcommand{\FASThtwoEventsCIMAX}{3,813,583,180}
\newcommand{\FASThtwoNoFPEventsCI}{7,558}
\newcommand{\FASThtwoNoFPEventsCIMIN}{118,686,985}
\newcommand{\FASThtwoNoFPEventsCIMAX}{118,702,101}
\newcommand{\FASThtwoFT}{11}
\newcommand{\FASThtwoFTCI}{0.0}
\newcommand{\FASThtwoFTCIMIN}{11}
\newcommand{\FASThtwoFTCIMAX}{11}
\newcommand{\FASThtwoFTDynamic}{106,149}
\newcommand{\FASThtwoFTDynamicCI}{604}
\newcommand{\FASThtwoFTDynamicCIMIN}{105,545}
\newcommand{\FASThtwoFTDynamicCIMAX}{106,753}
\newcommand{\FASThtwoHB}{13}
\newcommand{\FASThtwoHBCI}{0.0}
\newcommand{\FASThtwoHBCIMIN}{13}
\newcommand{\FASThtwoHBCIMAX}{13}
\newcommand{\FASThtwoHBDynamic}{87,891}
\newcommand{\FASThtwoHBDynamicCI}{263}
\newcommand{\FASThtwoHBDynamicCIMIN}{87,628}
\newcommand{\FASThtwoHBDynamicCIMAX}{88,154}
\newcommand{\FASThtwoFTOHB}{13}
\newcommand{\FASThtwoFTOHBCI}{0.0}
\newcommand{\FASThtwoFTOHBCIMIN}{13}
\newcommand{\FASThtwoFTOHBCIMAX}{13}
\newcommand{\FASThtwoFTOHBDynamic}{79,473}
\newcommand{\FASThtwoFTOHBDynamicCI}{903}
\newcommand{\FASThtwoFTOHBDynamicCIMIN}{78,570}
\newcommand{\FASThtwoFTOHBDynamicCIMAX}{80,376}
\newcommand{\FASThtwoWCP}{\rna}
\newcommand{\FASThtwoWCPCI}{\rna}
\newcommand{\FASThtwoWCPCIMIN}{\rna}
\newcommand{\FASThtwoWCPCIMAX}{\rna}
\newcommand{\FASThtwoWCPDynamic}{\rna}
\newcommand{\FASThtwoWCPDynamicCI}{\rna}
\newcommand{\FASThtwoWCPDynamicCIMIN}{\rna}
\newcommand{\FASThtwoWCPDynamicCIMAX}{\rna}
\newcommand{\FASThtwoFTOWCP}{13}
\newcommand{\FASThtwoFTOWCPCI}{0.0}
\newcommand{\FASThtwoFTOWCPCIMIN}{13}
\newcommand{\FASThtwoFTOWCPCIMAX}{13}
\newcommand{\FASThtwoFTOWCPDynamic}{85,962}
\newcommand{\FASThtwoFTOWCPDynamicCI}{171}
\newcommand{\FASThtwoFTOWCPDynamicCIMIN}{85,791}
\newcommand{\FASThtwoFTOWCPDynamicCIMAX}{86,133}
\newcommand{\FASThtwoREWCP}{13}
\newcommand{\FASThtwoREWCPCI}{0.26}
\newcommand{\FASThtwoREWCPCIMIN}{13}
\newcommand{\FASThtwoREWCPCIMAX}{13}
\newcommand{\FASThtwoREWCPDynamic}{83,082}
\newcommand{\FASThtwoREWCPDynamicCI}{445}
\newcommand{\FASThtwoREWCPDynamicCIMIN}{82,637}
\newcommand{\FASThtwoREWCPDynamicCIMAX}{83,527}
\newcommand{\FASThtwoDC}{\rna}
\newcommand{\FASThtwoDCCI}{\rna}
\newcommand{\FASThtwoDCCIMIN}{\rna}
\newcommand{\FASThtwoDCCIMAX}{\rna}
\newcommand{\FASThtwoDCDynamic}{\rna}
\newcommand{\FASThtwoDCDynamicCI}{\rna}
\newcommand{\FASThtwoDCDynamicCIMIN}{\rna}
\newcommand{\FASThtwoDCDynamicCIMAX}{\rna}
\newcommand{\FASThtwoFTODC}{13}
\newcommand{\FASThtwoFTODCCI}{0.0}
\newcommand{\FASThtwoFTODCCIMIN}{13}
\newcommand{\FASThtwoFTODCCIMAX}{13}
\newcommand{\FASThtwoFTODCDynamic}{86,790}
\newcommand{\FASThtwoFTODCDynamicCI}{195}
\newcommand{\FASThtwoFTODCDynamicCIMIN}{86,595}
\newcommand{\FASThtwoFTODCDynamicCIMAX}{86,985}
\newcommand{\FASThtwoREDC}{13}
\newcommand{\FASThtwoREDCCI}{0.0}
\newcommand{\FASThtwoREDCCIMIN}{13}
\newcommand{\FASThtwoREDCCIMAX}{13}
\newcommand{\FASThtwoREDCDynamic}{84,154}
\newcommand{\FASThtwoREDCDynamicCI}{303}
\newcommand{\FASThtwoREDCDynamicCIMIN}{83,851}
\newcommand{\FASThtwoREDCDynamicCIMAX}{84,457}
\newcommand{\FASThtwoCAPO}{\rna}
\newcommand{\FASThtwoCAPOCI}{\rna}
\newcommand{\FASThtwoCAPOCIMIN}{\rna}
\newcommand{\FASThtwoCAPOCIMAX}{\rna}
\newcommand{\FASThtwoCAPODynamic}{\rna}
\newcommand{\FASThtwoCAPODynamicCI}{\rna}
\newcommand{\FASThtwoCAPODynamicCIMIN}{\rna}
\newcommand{\FASThtwoCAPODynamicCIMAX}{\rna}
\newcommand{\FASThtwoFTOCAPO}{13}
\newcommand{\FASThtwoFTOCAPOCI}{0.0}
\newcommand{\FASThtwoFTOCAPOCIMIN}{13}
\newcommand{\FASThtwoFTOCAPOCIMAX}{13}
\newcommand{\FASThtwoFTOCAPODynamic}{86,963}
\newcommand{\FASThtwoFTOCAPODynamicCI}{149}
\newcommand{\FASThtwoFTOCAPODynamicCIMIN}{86,814}
\newcommand{\FASThtwoFTOCAPODynamicCIMAX}{87,112}
\newcommand{\FASThtwoRECAPO}{13}
\newcommand{\FASThtwoRECAPOCI}{0.0}
\newcommand{\FASThtwoRECAPOCIMIN}{13}
\newcommand{\FASThtwoRECAPOCIMAX}{13}
\newcommand{\FASThtwoRECAPODynamic}{83,476}
\newcommand{\FASThtwoRECAPODynamicCI}{640}
\newcommand{\FASThtwoRECAPODynamicCIMIN}{82,836}
\newcommand{\FASThtwoRECAPODynamicCIMAX}{84,116}
\newcommand{\FASThtwoAGGCAPO}{\rna}
\newcommand{\FASThtwoAGGCAPOCI}{\rna}
\newcommand{\FASThtwoAGGCAPOCIMIN}{\rna}
\newcommand{\FASThtwoAGGCAPOCIMAX}{\rna}
\newcommand{\FASThtwoAGGCAPODynamic}{\rna}
\newcommand{\FASThtwoAGGCAPODynamicCI}{\rna}
\newcommand{\FASThtwoAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASThtwoAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTjythonEvents}{730}
\newcommand{\FASTjythonNoFPEvents}{130}
\newcommand{\jythonHBEventTotal}{730}
\newcommand{\jythonHBNoFPEventTotal}{190}
\newcommand{\jythonHBNoFPAccessTotal}{170}
\newcommand{\jythonHBNoFPOtherTotal}{27}
\newcommand{\jythonHBReadTotal}{71.5}
\newcommand{\jythonHBWriteTotal}{14.7}
\newcommand{\jythonHBNoFPAccessInCS}{5.42}
\newcommand{\jythonHBNoFPAccessOutCS}{94.6}
\newcommand{\jythonHBAcqRelTotal}{17.2}
\newcommand{\jythonHBOtherTotal}{3.6}
\newcommand{\jythonHBNoFPReadTotal}{140}
\newcommand{\jythonHBReadInCS}{4.18}
\newcommand{\jythonHBReadOutCS}{106}
\newcommand{\jythonHBReadSameEp}{10.3}
\newcommand{\jythonHBReadSharedSameEp}{\cna}
\newcommand{\jythonHBReadExclusive}{97.7}
\newcommand{\jythonHBReadOwned}{\cna}
\newcommand{\jythonHBReadShare}{<0.001}
\newcommand{\jythonHBReadShared}{2.25}
\newcommand{\jythonHBReadSharedOwned}{\cna}
\newcommand{\jythonHBNoFPHonestWriteTotal}{28}
\newcommand{\jythonHBWriteInCS}{19.1}
\newcommand{\jythonHBWriteOutCS}{388}
\newcommand{\jythonHBNoFPWriteTotal}{28}
\newcommand{\jythonHBWriteSameEp}{307}
\newcommand{\jythonHBWriteExclusive}{100}
\newcommand{\jythonHBWriteOwned}{\cna}
\newcommand{\jythonHBWriteShared}{<0.001}
\newcommand{\jythonHBNoFPOtherEventTotal}{26523556}
\newcommand{\jythonHBAcqRelOtherTotal}{82.7}
\newcommand{\jythonHBNoAcqRelOtherTotal}{4594890}
\newcommand{\jythonHBFork}{0.0}
\newcommand{\jythonHBJoin}{0.0}
\newcommand{\jythonHBPreWait}{0.0}
\newcommand{\jythonHBPostWait}{0.0}
\newcommand{\jythonHBVolatileTotal}{100.0}
\newcommand{\jythonHBClassInit}{0.00372}
\newcommand{\jythonHBClassAccess}{0.00303}
\newcommand{\jythonHBRaceTotal}{30}
\newcommand{\jythonHBWrRdRace}{80.0}
\newcommand{\jythonHBWrWrRace}{10.0}
\newcommand{\jythonHBRdWrRace}{6.67}
\newcommand{\jythonHBRdShWrRace}{3.33}
\newcommand{\jythonHBHoldLocksTotal}{11}
\newcommand{\jythonHBOneLockHeld}{6.73}
\newcommand{\jythonHBTwoNestedLocks}{0.26}
\newcommand{\jythonHBThreeNestedLocks}{<0.1}
\newcommand{\jythonHBFourNestedLocks}{\cna}
\newcommand{\jythonHBFiveNestedLocks}{\cna}
\newcommand{\jythonHBSixNestedLocks}{\cna}
\newcommand{\jythonHBSevenNestedLocks}{\cna}
\newcommand{\jythonHBEightNestedLocks}{\cna}
\newcommand{\jythonHBNineNestedLocks}{\cna}
\newcommand{\jythonHBTenNestedLocks}{\cna}
\newcommand{\jythonHBHundredNestedLocks}{\cna}
\newcommand{\jythonFTOHBEventTotal}{730}
\newcommand{\jythonFTOHBNoFPEventTotal}{170}
\newcommand{\jythonFTOHBNoFPAccessTotal}{140}
\newcommand{\jythonFTOHBNoFPOtherTotal}{27}
\newcommand{\jythonFTOHBReadTotal}{67.3}
\newcommand{\jythonFTOHBWriteTotal}{16.9}
\newcommand{\jythonFTOHBNoFPAccessInCS}{5.42}
\newcommand{\jythonFTOHBNoFPAccessOutCS}{94.6}
\newcommand{\jythonFTOHBAcqRelTotal}{17.2}
\newcommand{\jythonFTOHBOtherTotal}{3.6}
\newcommand{\jythonFTOHBNoFPReadTotal}{110}
\newcommand{\jythonFTOHBReadInCS}{4.84}
\newcommand{\jythonFTOHBReadOutCS}{108}
\newcommand{\jythonFTOHBReadSameEp}{12.5}
\newcommand{\jythonFTOHBReadSharedSameEp}{\cna}
\newcommand{\jythonFTOHBReadExclusive}{<0.001}
\newcommand{\jythonFTOHBReadOwned}{97.3}
\newcommand{\jythonFTOHBReadShare}{<0.001}
\newcommand{\jythonFTOHBReadShared}{\cna}
\newcommand{\jythonFTOHBReadSharedOwned}{2.74}
\newcommand{\jythonFTOHBNoFPHonestWriteTotal}{28}
\newcommand{\jythonFTOHBWriteInCS}{19.1}
\newcommand{\jythonFTOHBWriteOutCS}{388}
\newcommand{\jythonFTOHBNoFPWriteTotal}{28}
\newcommand{\jythonFTOHBWriteSameEp}{307}
\newcommand{\jythonFTOHBWriteExclusive}{<0.001}
\newcommand{\jythonFTOHBWriteOwned}{100}
\newcommand{\jythonFTOHBWriteShared}{<0.001}
\newcommand{\jythonFTOHBNoFPOtherEventTotal}{26523557}
\newcommand{\jythonFTOHBAcqRelOtherTotal}{82.7}
\newcommand{\jythonFTOHBNoAcqRelOtherTotal}{4594891}
\newcommand{\jythonFTOHBFork}{0.0}
\newcommand{\jythonFTOHBJoin}{0.0}
\newcommand{\jythonFTOHBPreWait}{0.0}
\newcommand{\jythonFTOHBPostWait}{0.0}
\newcommand{\jythonFTOHBVolatileTotal}{100.0}
\newcommand{\jythonFTOHBClassInit}{0.00372}
\newcommand{\jythonFTOHBClassAccess}{0.00303}
\newcommand{\jythonFTOHBRaceTotal}{27}
\newcommand{\jythonFTOHBWrRdRace}{88.9}
\newcommand{\jythonFTOHBWrWrRace}{0.0}
\newcommand{\jythonFTOHBRdWrRace}{7.41}
\newcommand{\jythonFTOHBRdShWrRace}{3.7}
\newcommand{\jythonFTOHBHoldLocksTotal}{5.4}
\newcommand{\jythonFTOHBOneLockHeld}{3.81}
\newcommand{\jythonFTOHBTwoNestedLocks}{0.23}
\newcommand{\jythonFTOHBThreeNestedLocks}{<0.1}
\newcommand{\jythonFTOHBFourNestedLocks}{\cna}
\newcommand{\jythonFTOHBFiveNestedLocks}{\cna}
\newcommand{\jythonFTOHBSixNestedLocks}{\cna}
\newcommand{\jythonFTOHBSevenNestedLocks}{\cna}
\newcommand{\jythonFTOHBEightNestedLocks}{\cna}
\newcommand{\jythonFTOHBNineNestedLocks}{\cna}
\newcommand{\jythonFTOHBTenNestedLocks}{\cna}
\newcommand{\jythonFTOHBHundredNestedLocks}{\cna}
\newcommand{\jythonFTOWCPEventTotal}{730}
\newcommand{\jythonFTOWCPNoFPEventTotal}{170}
\newcommand{\jythonFTOWCPNoFPAccessTotal}{140}
\newcommand{\jythonFTOWCPNoFPOtherTotal}{27}
\newcommand{\jythonFTOWCPReadTotal}{67.3}
\newcommand{\jythonFTOWCPWriteTotal}{16.9}
\newcommand{\jythonFTOWCPNoFPAccessInCS}{5.42}
\newcommand{\jythonFTOWCPNoFPAccessOutCS}{94.6}
\newcommand{\jythonFTOWCPAcqRelTotal}{17.2}
\newcommand{\jythonFTOWCPOtherTotal}{3.6}
\newcommand{\jythonFTOWCPNoFPReadTotal}{110}
\newcommand{\jythonFTOWCPReadInCS}{4.84}
\newcommand{\jythonFTOWCPReadOutCS}{108}
\newcommand{\jythonFTOWCPReadSameEp}{12.5}
\newcommand{\jythonFTOWCPReadSharedSameEp}{\cna}
\newcommand{\jythonFTOWCPReadExclusive}{<0.001}
\newcommand{\jythonFTOWCPReadOwned}{95.4}
\newcommand{\jythonFTOWCPReadShare}{<0.001}
\newcommand{\jythonFTOWCPReadShared}{\cna}
\newcommand{\jythonFTOWCPReadSharedOwned}{4.6}
\newcommand{\jythonFTOWCPNoFPHonestWriteTotal}{28}
\newcommand{\jythonFTOWCPWriteInCS}{19.1}
\newcommand{\jythonFTOWCPWriteOutCS}{388}
\newcommand{\jythonFTOWCPNoFPWriteTotal}{28}
\newcommand{\jythonFTOWCPWriteSameEp}{307}
\newcommand{\jythonFTOWCPWriteExclusive}{<0.001}
\newcommand{\jythonFTOWCPWriteOwned}{100}
\newcommand{\jythonFTOWCPWriteShared}{<0.001}
\newcommand{\jythonFTOWCPNoFPOtherEventTotal}{26523555}
\newcommand{\jythonFTOWCPAcqRelOtherTotal}{82.7}
\newcommand{\jythonFTOWCPNoAcqRelOtherTotal}{4594889}
\newcommand{\jythonFTOWCPFork}{0.0}
\newcommand{\jythonFTOWCPJoin}{0.0}
\newcommand{\jythonFTOWCPPreWait}{0.0}
\newcommand{\jythonFTOWCPPostWait}{0.0}
\newcommand{\jythonFTOWCPVolatileTotal}{100.0}
\newcommand{\jythonFTOWCPClassInit}{0.00372}
\newcommand{\jythonFTOWCPClassAccess}{0.00303}
\newcommand{\jythonFTOWCPRaceTotal}{19}
\newcommand{\jythonFTOWCPWrRdRace}{84.2}
\newcommand{\jythonFTOWCPWrWrRace}{0.0}
\newcommand{\jythonFTOWCPRdWrRace}{10.5}
\newcommand{\jythonFTOWCPRdShWrRace}{5.26}
\newcommand{\jythonFTOWCPHoldLocksTotal}{5.4}
\newcommand{\jythonFTOWCPOneLockHeld}{3.82}
\newcommand{\jythonFTOWCPTwoNestedLocks}{0.23}
\newcommand{\jythonFTOWCPThreeNestedLocks}{<0.1}
\newcommand{\jythonFTOWCPFourNestedLocks}{\cna}
\newcommand{\jythonFTOWCPFiveNestedLocks}{\cna}
\newcommand{\jythonFTOWCPSixNestedLocks}{\cna}
\newcommand{\jythonFTOWCPSevenNestedLocks}{\cna}
\newcommand{\jythonFTOWCPEightNestedLocks}{\cna}
\newcommand{\jythonFTOWCPNineNestedLocks}{\cna}
\newcommand{\jythonFTOWCPTenNestedLocks}{\cna}
\newcommand{\jythonFTOWCPHundredNestedLocks}{\cna}
\newcommand{\jythonREWCPEventTotal}{730}
\newcommand{\jythonREWCPNoFPEventTotal}{170}
\newcommand{\jythonREWCPNoFPAccessTotal}{140}
\newcommand{\jythonREWCPNoFPOtherTotal}{27}
\newcommand{\jythonREWCPReadTotal}{67.3}
\newcommand{\jythonREWCPWriteTotal}{16.9}
\newcommand{\jythonREWCPNoFPAccessInCS}{5.42}
\newcommand{\jythonREWCPNoFPAccessOutCS}{94.6}
\newcommand{\jythonREWCPAcqRelTotal}{17.2}
\newcommand{\jythonREWCPOtherTotal}{3.6}
\newcommand{\jythonREWCPNoFPReadTotal}{110}
\newcommand{\jythonREWCPReadInCS}{4.84}
\newcommand{\jythonREWCPReadOutCS}{108}
\newcommand{\jythonREWCPReadSameEp}{12.5}
\newcommand{\jythonREWCPReadSharedSameEp}{\cna}
\newcommand{\jythonREWCPReadExclusive}{<0.001}
\newcommand{\jythonREWCPReadOwned}{95.3}
\newcommand{\jythonREWCPReadShare}{<0.001}
\newcommand{\jythonREWCPReadShared}{\cna}
\newcommand{\jythonREWCPReadSharedOwned}{4.73}
\newcommand{\jythonREWCPNoFPHonestWriteTotal}{28}
\newcommand{\jythonREWCPWriteInCS}{19.1}
\newcommand{\jythonREWCPWriteOutCS}{388}
\newcommand{\jythonREWCPNoFPWriteTotal}{28}
\newcommand{\jythonREWCPWriteSameEp}{307}
\newcommand{\jythonREWCPWriteExclusive}{<0.001}
\newcommand{\jythonREWCPWriteOwned}{100}
\newcommand{\jythonREWCPWriteShared}{<0.001}
\newcommand{\jythonREWCPNoFPOtherEventTotal}{26523556}
\newcommand{\jythonREWCPAcqRelOtherTotal}{82.7}
\newcommand{\jythonREWCPNoAcqRelOtherTotal}{4594890}
\newcommand{\jythonREWCPFork}{0.0}
\newcommand{\jythonREWCPJoin}{0.0}
\newcommand{\jythonREWCPPreWait}{0.0}
\newcommand{\jythonREWCPPostWait}{0.0}
\newcommand{\jythonREWCPVolatileTotal}{100.0}
\newcommand{\jythonREWCPClassInit}{0.00372}
\newcommand{\jythonREWCPClassAccess}{0.00303}
\newcommand{\jythonREWCPRaceTotal}{25}
\newcommand{\jythonREWCPWrRdRace}{88.0}
\newcommand{\jythonREWCPWrWrRace}{0.0}
\newcommand{\jythonREWCPRdWrRace}{8.0}
\newcommand{\jythonREWCPRdShWrRace}{4.0}
\newcommand{\jythonREWCPHoldLocksTotal}{5.4}
\newcommand{\jythonREWCPOneLockHeld}{3.82}
\newcommand{\jythonREWCPTwoNestedLocks}{0.23}
\newcommand{\jythonREWCPThreeNestedLocks}{<0.1}
\newcommand{\jythonREWCPFourNestedLocks}{\cna}
\newcommand{\jythonREWCPFiveNestedLocks}{\cna}
\newcommand{\jythonREWCPSixNestedLocks}{\cna}
\newcommand{\jythonREWCPSevenNestedLocks}{\cna}
\newcommand{\jythonREWCPEightNestedLocks}{\cna}
\newcommand{\jythonREWCPNineNestedLocks}{\cna}
\newcommand{\jythonREWCPTenNestedLocks}{\cna}
\newcommand{\jythonREWCPHundredNestedLocks}{\cna}
\newcommand{\jythonFTODCEventTotal}{730}
\newcommand{\jythonFTODCNoFPEventTotal}{170}
\newcommand{\jythonFTODCNoFPAccessTotal}{140}
\newcommand{\jythonFTODCNoFPOtherTotal}{27}
\newcommand{\jythonFTODCReadTotal}{67.3}
\newcommand{\jythonFTODCWriteTotal}{16.9}
\newcommand{\jythonFTODCNoFPAccessInCS}{5.42}
\newcommand{\jythonFTODCNoFPAccessOutCS}{94.6}
\newcommand{\jythonFTODCAcqRelTotal}{17.2}
\newcommand{\jythonFTODCOtherTotal}{3.6}
\newcommand{\jythonFTODCNoFPReadTotal}{110}
\newcommand{\jythonFTODCReadInCS}{4.84}
\newcommand{\jythonFTODCReadOutCS}{108}
\newcommand{\jythonFTODCReadSameEp}{12.5}
\newcommand{\jythonFTODCReadSharedSameEp}{\cna}
\newcommand{\jythonFTODCReadExclusive}{\cna}
\newcommand{\jythonFTODCReadOwned}{95.4}
\newcommand{\jythonFTODCReadShare}{<0.001}
\newcommand{\jythonFTODCReadShared}{\cna}
\newcommand{\jythonFTODCReadSharedOwned}{4.64}
\newcommand{\jythonFTODCNoFPHonestWriteTotal}{28}
\newcommand{\jythonFTODCWriteInCS}{19.1}
\newcommand{\jythonFTODCWriteOutCS}{388}
\newcommand{\jythonFTODCNoFPWriteTotal}{28}
\newcommand{\jythonFTODCWriteSameEp}{307}
\newcommand{\jythonFTODCWriteExclusive}{<0.001}
\newcommand{\jythonFTODCWriteOwned}{100}
\newcommand{\jythonFTODCWriteShared}{<0.001}
\newcommand{\jythonFTODCNoFPOtherEventTotal}{26523556}
\newcommand{\jythonFTODCAcqRelOtherTotal}{82.7}
\newcommand{\jythonFTODCNoAcqRelOtherTotal}{4594890}
\newcommand{\jythonFTODCFork}{0.0}
\newcommand{\jythonFTODCJoin}{0.0}
\newcommand{\jythonFTODCPreWait}{0.0}
\newcommand{\jythonFTODCPostWait}{0.0}
\newcommand{\jythonFTODCVolatileTotal}{100.0}
\newcommand{\jythonFTODCClassInit}{0.00372}
\newcommand{\jythonFTODCClassAccess}{0.00303}
\newcommand{\jythonFTODCRaceTotal}{29}
\newcommand{\jythonFTODCWrRdRace}{79.3}
\newcommand{\jythonFTODCWrWrRace}{0.0}
\newcommand{\jythonFTODCRdWrRace}{6.9}
\newcommand{\jythonFTODCRdShWrRace}{13.8}
\newcommand{\jythonFTODCHoldLocksTotal}{5.4}
\newcommand{\jythonFTODCOneLockHeld}{3.82}
\newcommand{\jythonFTODCTwoNestedLocks}{0.23}
\newcommand{\jythonFTODCThreeNestedLocks}{<0.1}
\newcommand{\jythonFTODCFourNestedLocks}{\cna}
\newcommand{\jythonFTODCFiveNestedLocks}{\cna}
\newcommand{\jythonFTODCSixNestedLocks}{\cna}
\newcommand{\jythonFTODCSevenNestedLocks}{\cna}
\newcommand{\jythonFTODCEightNestedLocks}{\cna}
\newcommand{\jythonFTODCNineNestedLocks}{\cna}
\newcommand{\jythonFTODCTenNestedLocks}{\cna}
\newcommand{\jythonFTODCHundredNestedLocks}{\cna}
\newcommand{\jythonREDCEventTotal}{730}
\newcommand{\jythonREDCNoFPEventTotal}{170}
\newcommand{\jythonREDCNoFPAccessTotal}{140}
\newcommand{\jythonREDCNoFPOtherTotal}{27}
\newcommand{\jythonREDCReadTotal}{67.3}
\newcommand{\jythonREDCWriteTotal}{16.9}
\newcommand{\jythonREDCNoFPAccessInCS}{5.42}
\newcommand{\jythonREDCNoFPAccessOutCS}{94.6}
\newcommand{\jythonREDCAcqRelTotal}{17.2}
\newcommand{\jythonREDCOtherTotal}{3.6}
\newcommand{\jythonREDCNoFPReadTotal}{110}
\newcommand{\jythonREDCReadInCS}{4.84}
\newcommand{\jythonREDCReadOutCS}{108}
\newcommand{\jythonREDCReadSameEp}{12.5}
\newcommand{\jythonREDCReadSharedSameEp}{\cna}
\newcommand{\jythonREDCReadExclusive}{\cna}
\newcommand{\jythonREDCReadOwned}{95.2}
\newcommand{\jythonREDCReadShare}{<0.001}
\newcommand{\jythonREDCReadShared}{\cna}
\newcommand{\jythonREDCReadSharedOwned}{4.76}
\newcommand{\jythonREDCNoFPHonestWriteTotal}{28}
\newcommand{\jythonREDCWriteInCS}{19.1}
\newcommand{\jythonREDCWriteOutCS}{388}
\newcommand{\jythonREDCNoFPWriteTotal}{28}
\newcommand{\jythonREDCWriteSameEp}{307}
\newcommand{\jythonREDCWriteExclusive}{<0.001}
\newcommand{\jythonREDCWriteOwned}{100}
\newcommand{\jythonREDCWriteShared}{<0.001}
\newcommand{\jythonREDCNoFPOtherEventTotal}{26523556}
\newcommand{\jythonREDCAcqRelOtherTotal}{82.7}
\newcommand{\jythonREDCNoAcqRelOtherTotal}{4594890}
\newcommand{\jythonREDCFork}{0.0}
\newcommand{\jythonREDCJoin}{0.0}
\newcommand{\jythonREDCPreWait}{0.0}
\newcommand{\jythonREDCPostWait}{0.0}
\newcommand{\jythonREDCVolatileTotal}{100.0}
\newcommand{\jythonREDCClassInit}{0.00372}
\newcommand{\jythonREDCClassAccess}{0.00303}
\newcommand{\jythonREDCRaceTotal}{32}
\newcommand{\jythonREDCWrRdRace}{81.3}
\newcommand{\jythonREDCWrWrRace}{0.0}
\newcommand{\jythonREDCRdWrRace}{6.25}
\newcommand{\jythonREDCRdShWrRace}{12.5}
\newcommand{\jythonREDCHoldLocksTotal}{5.4}
\newcommand{\jythonREDCOneLockHeld}{3.82}
\newcommand{\jythonREDCTwoNestedLocks}{0.23}
\newcommand{\jythonREDCThreeNestedLocks}{<0.1}
\newcommand{\jythonREDCFourNestedLocks}{\cna}
\newcommand{\jythonREDCFiveNestedLocks}{\cna}
\newcommand{\jythonREDCSixNestedLocks}{\cna}
\newcommand{\jythonREDCSevenNestedLocks}{\cna}
\newcommand{\jythonREDCEightNestedLocks}{\cna}
\newcommand{\jythonREDCNineNestedLocks}{\cna}
\newcommand{\jythonREDCTenNestedLocks}{\cna}
\newcommand{\jythonREDCHundredNestedLocks}{\cna}
\newcommand{\jythonFTOCAPOEventTotal}{730}
\newcommand{\jythonFTOCAPONoFPEventTotal}{170}
\newcommand{\jythonFTOCAPONoFPAccessTotal}{140}
\newcommand{\jythonFTOCAPONoFPOtherTotal}{27}
\newcommand{\jythonFTOCAPOReadTotal}{67.3}
\newcommand{\jythonFTOCAPOWriteTotal}{16.9}
\newcommand{\jythonFTOCAPONoFPAccessInCS}{5.42}
\newcommand{\jythonFTOCAPONoFPAccessOutCS}{94.6}
\newcommand{\jythonFTOCAPOAcqRelTotal}{17.2}
\newcommand{\jythonFTOCAPOOtherTotal}{3.6}
\newcommand{\jythonFTOCAPONoFPReadTotal}{110}
\newcommand{\jythonFTOCAPOReadInCS}{4.84}
\newcommand{\jythonFTOCAPOReadOutCS}{108}
\newcommand{\jythonFTOCAPOReadSameEp}{12.5}
\newcommand{\jythonFTOCAPOReadSharedSameEp}{\cna}
\newcommand{\jythonFTOCAPOReadExclusive}{\cna}
\newcommand{\jythonFTOCAPOReadOwned}{95.3}
\newcommand{\jythonFTOCAPOReadShare}{<0.001}
\newcommand{\jythonFTOCAPOReadShared}{\cna}
\newcommand{\jythonFTOCAPOReadSharedOwned}{4.65}
\newcommand{\jythonFTOCAPONoFPHonestWriteTotal}{28}
\newcommand{\jythonFTOCAPOWriteInCS}{19.1}
\newcommand{\jythonFTOCAPOWriteOutCS}{388}
\newcommand{\jythonFTOCAPONoFPWriteTotal}{28}
\newcommand{\jythonFTOCAPOWriteSameEp}{307}
\newcommand{\jythonFTOCAPOWriteExclusive}{<0.001}
\newcommand{\jythonFTOCAPOWriteOwned}{100}
\newcommand{\jythonFTOCAPOWriteShared}{<0.001}
\newcommand{\jythonFTOCAPONoFPOtherEventTotal}{26523556}
\newcommand{\jythonFTOCAPOAcqRelOtherTotal}{82.7}
\newcommand{\jythonFTOCAPONoAcqRelOtherTotal}{4594890}
\newcommand{\jythonFTOCAPOFork}{0.0}
\newcommand{\jythonFTOCAPOJoin}{0.0}
\newcommand{\jythonFTOCAPOPreWait}{0.0}
\newcommand{\jythonFTOCAPOPostWait}{0.0}
\newcommand{\jythonFTOCAPOVolatileTotal}{100.0}
\newcommand{\jythonFTOCAPOClassInit}{0.00372}
\newcommand{\jythonFTOCAPOClassAccess}{0.00303}
\newcommand{\jythonFTOCAPORaceTotal}{30}
\newcommand{\jythonFTOCAPOWrRdRace}{80.0}
\newcommand{\jythonFTOCAPOWrWrRace}{0.0}
\newcommand{\jythonFTOCAPORdWrRace}{6.67}
\newcommand{\jythonFTOCAPORdShWrRace}{13.3}
\newcommand{\jythonFTOCAPOHoldLocksTotal}{5.4}
\newcommand{\jythonFTOCAPOOneLockHeld}{3.82}
\newcommand{\jythonFTOCAPOTwoNestedLocks}{0.23}
\newcommand{\jythonFTOCAPOThreeNestedLocks}{<0.1}
\newcommand{\jythonFTOCAPOFourNestedLocks}{\cna}
\newcommand{\jythonFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\jythonFTOCAPOSixNestedLocks}{\cna}
\newcommand{\jythonFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\jythonFTOCAPOEightNestedLocks}{\cna}
\newcommand{\jythonFTOCAPONineNestedLocks}{\cna}
\newcommand{\jythonFTOCAPOTenNestedLocks}{\cna}
\newcommand{\jythonFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\jythonRECAPOEventTotal}{730}
\newcommand{\jythonRECAPONoFPEventTotal}{170}
\newcommand{\jythonRECAPONoFPAccessTotal}{140}
\newcommand{\jythonRECAPONoFPOtherTotal}{27}
\newcommand{\jythonRECAPOReadTotal}{67.3}
\newcommand{\jythonRECAPOWriteTotal}{16.9}
\newcommand{\jythonRECAPONoFPAccessInCS}{5.42}
\newcommand{\jythonRECAPONoFPAccessOutCS}{94.6}
\newcommand{\jythonRECAPOAcqRelTotal}{17.2}
\newcommand{\jythonRECAPOOtherTotal}{3.6}
\newcommand{\jythonRECAPONoFPReadTotal}{110}
\newcommand{\jythonRECAPOReadInCS}{4.84}
\newcommand{\jythonRECAPOReadOutCS}{108}
\newcommand{\jythonRECAPOReadSameEp}{12.5}
\newcommand{\jythonRECAPOReadSharedSameEp}{\cna}
\newcommand{\jythonRECAPOReadExclusive}{\cna}
\newcommand{\jythonRECAPOReadOwned}{95.3}
\newcommand{\jythonRECAPOReadShare}{<0.001}
\newcommand{\jythonRECAPOReadShared}{\cna}
\newcommand{\jythonRECAPOReadSharedOwned}{4.65}
\newcommand{\jythonRECAPONoFPHonestWriteTotal}{28}
\newcommand{\jythonRECAPOWriteInCS}{19.1}
\newcommand{\jythonRECAPOWriteOutCS}{388}
\newcommand{\jythonRECAPONoFPWriteTotal}{28}
\newcommand{\jythonRECAPOWriteSameEp}{307}
\newcommand{\jythonRECAPOWriteExclusive}{<0.001}
\newcommand{\jythonRECAPOWriteOwned}{100}
\newcommand{\jythonRECAPOWriteShared}{<0.001}
\newcommand{\jythonRECAPONoFPOtherEventTotal}{26523557}
\newcommand{\jythonRECAPOAcqRelOtherTotal}{82.7}
\newcommand{\jythonRECAPONoAcqRelOtherTotal}{4594891}
\newcommand{\jythonRECAPOFork}{0.0}
\newcommand{\jythonRECAPOJoin}{0.0}
\newcommand{\jythonRECAPOPreWait}{0.0}
\newcommand{\jythonRECAPOPostWait}{0.0}
\newcommand{\jythonRECAPOVolatileTotal}{100.0}
\newcommand{\jythonRECAPOClassInit}{0.00372}
\newcommand{\jythonRECAPOClassAccess}{0.00303}
\newcommand{\jythonRECAPORaceTotal}{32}
\newcommand{\jythonRECAPOWrRdRace}{81.3}
\newcommand{\jythonRECAPOWrWrRace}{0.0}
\newcommand{\jythonRECAPORdWrRace}{6.25}
\newcommand{\jythonRECAPORdShWrRace}{12.5}
\newcommand{\jythonRECAPOHoldLocksTotal}{5.4}
\newcommand{\jythonRECAPOOneLockHeld}{3.82}
\newcommand{\jythonRECAPOTwoNestedLocks}{0.23}
\newcommand{\jythonRECAPOThreeNestedLocks}{<0.1}
\newcommand{\jythonRECAPOFourNestedLocks}{\cna}
\newcommand{\jythonRECAPOFiveNestedLocks}{\cna}
\newcommand{\jythonRECAPOSixNestedLocks}{\cna}
\newcommand{\jythonRECAPOSevenNestedLocks}{\cna}
\newcommand{\jythonRECAPOEightNestedLocks}{\cna}
\newcommand{\jythonRECAPONineNestedLocks}{\cna}
\newcommand{\jythonRECAPOTenNestedLocks}{\cna}
\newcommand{\jythonRECAPOHundredNestedLocks}{\cna}
\newcommand{\FASTjythonMaxLiveThreads}{2}
\newcommand{\FASTjythonTotalThreads}{2}
\newcommand{\FASTjythonBaseTime}{3.8}
\newcommand{\FASTjythonBaseTimeCI}{85}
\newcommand{\FASTjythonEmptyTime}{\rna}
\newcommand{\FASTjythonEmptyTimeCI}{\rna}
\newcommand{\FASTjythonEmptyTimeCIMIN}{\rna}
\newcommand{\FASTjythonEmptyTimeCIMAX}{\rna}
\newcommand{\FASTjythonFTTime}{8.4}
\newcommand{\FASTjythonFTTimeCI}{0.23}
\newcommand{\FASTjythonHBTime}{9.3}
\newcommand{\FASTjythonHBTimeCI}{0.22}
\newcommand{\FASTjythonFTOHBTime}{9.2}
\newcommand{\FASTjythonFTOHBTimeCI}{0.23}
\newcommand{\FASTjythonWCPTime}{\rna}
\newcommand{\FASTjythonWCPTimeCI}{\rna}
\newcommand{\FASTjythonWCPTimeCIMIN}{\rna}
\newcommand{\FASTjythonWCPTimeCIMAX}{\rna}
\newcommand{\FASTjythonFTOWCPTime}{11}
\newcommand{\FASTjythonFTOWCPTimeCI}{0.24}
\newcommand{\FASTjythonREWCPTime}{13}
\newcommand{\FASTjythonREWCPTimeCI}{0.21}
\newcommand{\FASTjythonDCTime}{\rna}
\newcommand{\FASTjythonDCTimeCI}{\rna}
\newcommand{\FASTjythonDCTimeCIMIN}{\rna}
\newcommand{\FASTjythonDCTimeCIMAX}{\rna}
\newcommand{\FASTjythonFTODCTime}{11}
\newcommand{\FASTjythonFTODCTimeCI}{0.25}
\newcommand{\FASTjythonREDCTime}{12}
\newcommand{\FASTjythonREDCTimeCI}{0.48}
\newcommand{\FASTjythonCAPOTime}{\rna}
\newcommand{\FASTjythonCAPOTimeCI}{\rna}
\newcommand{\FASTjythonCAPOTimeCIMIN}{\rna}
\newcommand{\FASTjythonCAPOTimeCIMAX}{\rna}
\newcommand{\FASTjythonFTOCAPOTime}{9.3}
\newcommand{\FASTjythonFTOCAPOTimeCI}{0.17}
\newcommand{\FASTjythonRECAPOTime}{9.9}
\newcommand{\FASTjythonRECAPOTimeCI}{0.19}
\newcommand{\FASTjythonAGGCAPOTime}{\rna}
\newcommand{\FASTjythonAGGCAPOTimeCI}{\rna}
\newcommand{\FASTjythonAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTjythonAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTjythonStaticTime}{\rzero}
\newcommand{\FASTjythonDynamicTime}{\rzero}
\newcommand{\FASTjythonBaseMem}{740}
\newcommand{\FASTjythonBaseMemCI}{4.5}
\newcommand{\FASTjythonFTMem}{6.6}
\newcommand{\FASTjythonFTMemCI}{0.25}
\newcommand{\FASTjythonHBMem}{6.9}
\newcommand{\FASTjythonHBMemCI}{0.16}
\newcommand{\FASTjythonFTOHBMem}{6.6}
\newcommand{\FASTjythonFTOHBMemCI}{0.36}
\newcommand{\FASTjythonWCPMem}{\memna}
\newcommand{\FASTjythonWCPMemCI}{\memna}
\newcommand{\FASTjythonWCPMemCIMIN}{\memna}
\newcommand{\FASTjythonWCPMemCIMAX}{\memna}
\newcommand{\FASTjythonFTOWCPMem}{13}
\newcommand{\FASTjythonFTOWCPMemCI}{0.33}
\newcommand{\FASTjythonREWCPMem}{15}
\newcommand{\FASTjythonREWCPMemCI}{0.63}
\newcommand{\FASTjythonDCMem}{\memna}
\newcommand{\FASTjythonDCMemCI}{\memna}
\newcommand{\FASTjythonDCMemCIMIN}{\memna}
\newcommand{\FASTjythonDCMemCIMAX}{\memna}
\newcommand{\FASTjythonFTODCMem}{13}
\newcommand{\FASTjythonFTODCMemCI}{0.33}
\newcommand{\FASTjythonREDCMem}{15}
\newcommand{\FASTjythonREDCMemCI}{0.85}
\newcommand{\FASTjythonCAPOMem}{\memna}
\newcommand{\FASTjythonCAPOMemCI}{\memna}
\newcommand{\FASTjythonCAPOMemCIMIN}{\memna}
\newcommand{\FASTjythonCAPOMemCIMAX}{\memna}
\newcommand{\FASTjythonFTOCAPOMem}{8.8}
\newcommand{\FASTjythonFTOCAPOMemCI}{0.13}
\newcommand{\FASTjythonRECAPOMem}{11}
\newcommand{\FASTjythonRECAPOMemCI}{0.4}
\newcommand{\FASTjythonAGGCAPOMem}{\memna}
\newcommand{\FASTjythonAGGCAPOMemCI}{\memna}
\newcommand{\FASTjythonAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTjythonAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTjythonEventsCI}{155}
\newcommand{\FASTjythonEventsCIMIN}{728,376,441}
\newcommand{\FASTjythonEventsCIMAX}{728,376,751}
\newcommand{\FASTjythonNoFPEventsCI}{12}
\newcommand{\FASTjythonNoFPEventsCIMIN}{127,785,325}
\newcommand{\FASTjythonNoFPEventsCIMAX}{127,785,349}
\newcommand{\FASTjythonFT}{23}
\newcommand{\FASTjythonFTCI}{1.3}
\newcommand{\FASTjythonFTCIMIN}{22}
\newcommand{\FASTjythonFTCIMAX}{24}
\newcommand{\FASTjythonFTDynamic}{47}
\newcommand{\FASTjythonFTDynamicCI}{1.1}
\newcommand{\FASTjythonFTDynamicCIMIN}{46}
\newcommand{\FASTjythonFTDynamicCIMAX}{48}
\newcommand{\FASTjythonHB}{25}
\newcommand{\FASTjythonHBCI}{1.2}
\newcommand{\FASTjythonHBCIMIN}{24}
\newcommand{\FASTjythonHBCIMAX}{26}
\newcommand{\FASTjythonHBDynamic}{27}
\newcommand{\FASTjythonHBDynamicCI}{1.2}
\newcommand{\FASTjythonHBDynamicCIMIN}{26}
\newcommand{\FASTjythonHBDynamicCIMAX}{28}
\newcommand{\FASTjythonFTOHB}{24}
\newcommand{\FASTjythonFTOHBCI}{1.3}
\newcommand{\FASTjythonFTOHBCIMIN}{23}
\newcommand{\FASTjythonFTOHBCIMAX}{25}
\newcommand{\FASTjythonFTOHBDynamic}{27}
\newcommand{\FASTjythonFTOHBDynamicCI}{1.2}
\newcommand{\FASTjythonFTOHBDynamicCIMIN}{26}
\newcommand{\FASTjythonFTOHBDynamicCIMAX}{28}
\newcommand{\FASTjythonWCP}{\rna}
\newcommand{\FASTjythonWCPCI}{\rna}
\newcommand{\FASTjythonWCPCIMIN}{\rna}
\newcommand{\FASTjythonWCPCIMAX}{\rna}
\newcommand{\FASTjythonWCPDynamic}{\rna}
\newcommand{\FASTjythonWCPDynamicCI}{\rna}
\newcommand{\FASTjythonWCPDynamicCIMIN}{\rna}
\newcommand{\FASTjythonWCPDynamicCIMAX}{\rna}
\newcommand{\FASTjythonFTOWCP}{19}
\newcommand{\FASTjythonFTOWCPCI}{0.33}
\newcommand{\FASTjythonFTOWCPCIMIN}{19}
\newcommand{\FASTjythonFTOWCPCIMAX}{19}
\newcommand{\FASTjythonFTOWCPDynamic}{19}
\newcommand{\FASTjythonFTOWCPDynamicCI}{0.33}
\newcommand{\FASTjythonFTOWCPDynamicCIMIN}{19}
\newcommand{\FASTjythonFTOWCPDynamicCIMAX}{19}
\newcommand{\FASTjythonREWCP}{23}
\newcommand{\FASTjythonREWCPCI}{1.4}
\newcommand{\FASTjythonREWCPCIMIN}{22}
\newcommand{\FASTjythonREWCPCIMAX}{24}
\newcommand{\FASTjythonREWCPDynamic}{25}
\newcommand{\FASTjythonREWCPDynamicCI}{1.8}
\newcommand{\FASTjythonREWCPDynamicCIMIN}{23}
\newcommand{\FASTjythonREWCPDynamicCIMAX}{27}
\newcommand{\FASTjythonDC}{\rna}
\newcommand{\FASTjythonDCCI}{\rna}
\newcommand{\FASTjythonDCCIMIN}{\rna}
\newcommand{\FASTjythonDCCIMAX}{\rna}
\newcommand{\FASTjythonDCDynamic}{\rna}
\newcommand{\FASTjythonDCDynamicCI}{\rna}
\newcommand{\FASTjythonDCDynamicCIMIN}{\rna}
\newcommand{\FASTjythonDCDynamicCIMAX}{\rna}
\newcommand{\FASTjythonFTODC}{27}
\newcommand{\FASTjythonFTODCCI}{0.0}
\newcommand{\FASTjythonFTODCCIMIN}{27}
\newcommand{\FASTjythonFTODCCIMAX}{27}
\newcommand{\FASTjythonFTODCDynamic}{29}
\newcommand{\FASTjythonFTODCDynamicCI}{0.26}
\newcommand{\FASTjythonFTODCDynamicCIMIN}{29}
\newcommand{\FASTjythonFTODCDynamicCIMAX}{29}
\newcommand{\FASTjythonREDC}{29}
\newcommand{\FASTjythonREDCCI}{1.3}
\newcommand{\FASTjythonREDCCIMIN}{28}
\newcommand{\FASTjythonREDCCIMAX}{30}
\newcommand{\FASTjythonREDCDynamic}{32}
\newcommand{\FASTjythonREDCDynamicCI}{1.3}
\newcommand{\FASTjythonREDCDynamicCIMIN}{31}
\newcommand{\FASTjythonREDCDynamicCIMAX}{33}
\newcommand{\FASTjythonCAPO}{\rna}
\newcommand{\FASTjythonCAPOCI}{\rna}
\newcommand{\FASTjythonCAPOCIMIN}{\rna}
\newcommand{\FASTjythonCAPOCIMAX}{\rna}
\newcommand{\FASTjythonCAPODynamic}{\rna}
\newcommand{\FASTjythonCAPODynamicCI}{\rna}
\newcommand{\FASTjythonCAPODynamicCIMIN}{\rna}
\newcommand{\FASTjythonCAPODynamicCIMAX}{\rna}
\newcommand{\FASTjythonFTOCAPO}{27}
\newcommand{\FASTjythonFTOCAPOCI}{0.0}
\newcommand{\FASTjythonFTOCAPOCIMIN}{27}
\newcommand{\FASTjythonFTOCAPOCIMAX}{27}
\newcommand{\FASTjythonFTOCAPODynamic}{30}
\newcommand{\FASTjythonFTOCAPODynamicCI}{0.33}
\newcommand{\FASTjythonFTOCAPODynamicCIMIN}{30}
\newcommand{\FASTjythonFTOCAPODynamicCIMAX}{30}
\newcommand{\FASTjythonRECAPO}{29}
\newcommand{\FASTjythonRECAPOCI}{1.3}
\newcommand{\FASTjythonRECAPOCIMIN}{28}
\newcommand{\FASTjythonRECAPOCIMAX}{30}
\newcommand{\FASTjythonRECAPODynamic}{32}
\newcommand{\FASTjythonRECAPODynamicCI}{1.3}
\newcommand{\FASTjythonRECAPODynamicCIMIN}{31}
\newcommand{\FASTjythonRECAPODynamicCIMAX}{33}
\newcommand{\FASTjythonAGGCAPO}{\rna}
\newcommand{\FASTjythonAGGCAPOCI}{\rna}
\newcommand{\FASTjythonAGGCAPOCIMIN}{\rna}
\newcommand{\FASTjythonAGGCAPOCIMAX}{\rna}
\newcommand{\FASTjythonAGGCAPODynamic}{\rna}
\newcommand{\FASTjythonAGGCAPODynamicCI}{\rna}
\newcommand{\FASTjythonAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTjythonAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTluindexEvents}{400}
\newcommand{\FASTluindexNoFPEvents}{2.9}
\newcommand{\luindexHBEventTotal}{400}
\newcommand{\luindexHBNoFPEventTotal}{43}
\newcommand{\luindexHBNoFPAccessTotal}{42}
\newcommand{\luindexHBNoFPOtherTotal}{0.42}
\newcommand{\luindexHBReadTotal}{67.6}
\newcommand{\luindexHBWriteTotal}{31.4}
\newcommand{\luindexHBNoFPAccessInCS}{8.08}
\newcommand{\luindexHBNoFPAccessOutCS}{91.9}
\newcommand{\luindexHBAcqRelTotal}{14.2}
\newcommand{\luindexHBOtherTotal}{0.0197}
\newcommand{\luindexHBNoFPReadTotal}{29}
\newcommand{\luindexHBReadInCS}{23.8}
\newcommand{\luindexHBReadOutCS}{81.3}
\newcommand{\luindexHBReadSameEp}{5.1}
\newcommand{\luindexHBReadSharedSameEp}{\cna}
\newcommand{\luindexHBReadExclusive}{100}
\newcommand{\luindexHBReadOwned}{\cna}
\newcommand{\luindexHBReadShare}{<0.001}
\newcommand{\luindexHBReadShared}{<0.001}
\newcommand{\luindexHBReadSharedOwned}{\cna}
\newcommand{\luindexHBNoFPHonestWriteTotal}{13}
\newcommand{\luindexHBWriteInCS}{32.1}
\newcommand{\luindexHBWriteOutCS}{75.5}
\newcommand{\luindexHBNoFPWriteTotal}{13}
\newcommand{\luindexHBWriteSameEp}{7.57}
\newcommand{\luindexHBWriteExclusive}{100}
\newcommand{\luindexHBWriteOwned}{\cna}
\newcommand{\luindexHBWriteShared}{<0.001}
\newcommand{\luindexHBNoFPOtherEventTotal}{415314}
\newcommand{\luindexHBAcqRelOtherTotal}{99.9}
\newcommand{\luindexHBNoAcqRelOtherTotal}{574}
\newcommand{\luindexHBFork}{0.174}
\newcommand{\luindexHBJoin}{0.0}
\newcommand{\luindexHBPreWait}{0.348}
\newcommand{\luindexHBPostWait}{0.348}
\newcommand{\luindexHBVolatileTotal}{77.2}
\newcommand{\luindexHBClassInit}{11.5}
\newcommand{\luindexHBClassAccess}{10.5}
\newcommand{\luindexHBRaceTotal}{1}
\newcommand{\luindexHBWrRdRace}{0.0}
\newcommand{\luindexHBWrWrRace}{0.0}
\newcommand{\luindexHBRdWrRace}{0.0}
\newcommand{\luindexHBRdShWrRace}{100.0}
\newcommand{\luindexHBHoldLocksTotal}{11}
\newcommand{\luindexHBOneLockHeld}{26.3}
\newcommand{\luindexHBTwoNestedLocks}{26.0}
\newcommand{\luindexHBThreeNestedLocks}{25.9}
\newcommand{\luindexHBFourNestedLocks}{0.69}
\newcommand{\luindexHBFiveNestedLocks}{<0.1}
\newcommand{\luindexHBSixNestedLocks}{<0.1}
\newcommand{\luindexHBSevenNestedLocks}{\cna}
\newcommand{\luindexHBEightNestedLocks}{\cna}
\newcommand{\luindexHBNineNestedLocks}{\cna}
\newcommand{\luindexHBTenNestedLocks}{\cna}
\newcommand{\luindexHBHundredNestedLocks}{\cna}
\newcommand{\luindexFTOHBEventTotal}{400}
\newcommand{\luindexFTOHBNoFPEventTotal}{41}
\newcommand{\luindexFTOHBNoFPAccessTotal}{40}
\newcommand{\luindexFTOHBNoFPOtherTotal}{0.42}
\newcommand{\luindexFTOHBReadTotal}{66.0}
\newcommand{\luindexFTOHBWriteTotal}{33.0}
\newcommand{\luindexFTOHBNoFPAccessInCS}{8.08}
\newcommand{\luindexFTOHBNoFPAccessOutCS}{91.9}
\newcommand{\luindexFTOHBAcqRelTotal}{14.2}
\newcommand{\luindexFTOHBOtherTotal}{0.0197}
\newcommand{\luindexFTOHBNoFPReadTotal}{27}
\newcommand{\luindexFTOHBReadInCS}{23.4}
\newcommand{\luindexFTOHBReadOutCS}{82}
\newcommand{\luindexFTOHBReadSameEp}{5.48}
\newcommand{\luindexFTOHBReadSharedSameEp}{\cna}
\newcommand{\luindexFTOHBReadExclusive}{<0.001}
\newcommand{\luindexFTOHBReadOwned}{100}
\newcommand{\luindexFTOHBReadShare}{<0.001}
\newcommand{\luindexFTOHBReadShared}{\cna}
\newcommand{\luindexFTOHBReadSharedOwned}{<0.001}
\newcommand{\luindexFTOHBNoFPHonestWriteTotal}{13}
\newcommand{\luindexFTOHBWriteInCS}{32.1}
\newcommand{\luindexFTOHBWriteOutCS}{75.5}
\newcommand{\luindexFTOHBNoFPWriteTotal}{13}
\newcommand{\luindexFTOHBWriteSameEp}{7.57}
\newcommand{\luindexFTOHBWriteExclusive}{<0.001}
\newcommand{\luindexFTOHBWriteOwned}{100}
\newcommand{\luindexFTOHBWriteShared}{<0.001}
\newcommand{\luindexFTOHBNoFPOtherEventTotal}{415314}
\newcommand{\luindexFTOHBAcqRelOtherTotal}{99.9}
\newcommand{\luindexFTOHBNoAcqRelOtherTotal}{574}
\newcommand{\luindexFTOHBFork}{0.174}
\newcommand{\luindexFTOHBJoin}{0.0}
\newcommand{\luindexFTOHBPreWait}{0.348}
\newcommand{\luindexFTOHBPostWait}{0.348}
\newcommand{\luindexFTOHBVolatileTotal}{77.2}
\newcommand{\luindexFTOHBClassInit}{11.5}
\newcommand{\luindexFTOHBClassAccess}{10.5}
\newcommand{\luindexFTOHBRaceTotal}{1}
\newcommand{\luindexFTOHBWrRdRace}{0.0}
\newcommand{\luindexFTOHBWrWrRace}{0.0}
\newcommand{\luindexFTOHBRdWrRace}{0.0}
\newcommand{\luindexFTOHBRdShWrRace}{100.0}
\newcommand{\luindexFTOHBHoldLocksTotal}{10}
\newcommand{\luindexFTOHBOneLockHeld}{25.8}
\newcommand{\luindexFTOHBTwoNestedLocks}{25.4}
\newcommand{\luindexFTOHBThreeNestedLocks}{25.3}
\newcommand{\luindexFTOHBFourNestedLocks}{0.61}
\newcommand{\luindexFTOHBFiveNestedLocks}{<0.1}
\newcommand{\luindexFTOHBSixNestedLocks}{<0.1}
\newcommand{\luindexFTOHBSevenNestedLocks}{\cna}
\newcommand{\luindexFTOHBEightNestedLocks}{\cna}
\newcommand{\luindexFTOHBNineNestedLocks}{\cna}
\newcommand{\luindexFTOHBTenNestedLocks}{\cna}
\newcommand{\luindexFTOHBHundredNestedLocks}{\cna}
\newcommand{\luindexFTOWCPEventTotal}{400}
\newcommand{\luindexFTOWCPNoFPEventTotal}{41}
\newcommand{\luindexFTOWCPNoFPAccessTotal}{40}
\newcommand{\luindexFTOWCPNoFPOtherTotal}{0.42}
\newcommand{\luindexFTOWCPReadTotal}{66.0}
\newcommand{\luindexFTOWCPWriteTotal}{33.0}
\newcommand{\luindexFTOWCPNoFPAccessInCS}{8.08}
\newcommand{\luindexFTOWCPNoFPAccessOutCS}{91.9}
\newcommand{\luindexFTOWCPAcqRelTotal}{14.2}
\newcommand{\luindexFTOWCPOtherTotal}{0.02}
\newcommand{\luindexFTOWCPNoFPReadTotal}{27}
\newcommand{\luindexFTOWCPReadInCS}{23.5}
\newcommand{\luindexFTOWCPReadOutCS}{82}
\newcommand{\luindexFTOWCPReadSameEp}{5.48}
\newcommand{\luindexFTOWCPReadSharedSameEp}{\cna}
\newcommand{\luindexFTOWCPReadExclusive}{<0.001}
\newcommand{\luindexFTOWCPReadOwned}{100}
\newcommand{\luindexFTOWCPReadShare}{<0.001}
\newcommand{\luindexFTOWCPReadShared}{\cna}
\newcommand{\luindexFTOWCPReadSharedOwned}{<0.001}
\newcommand{\luindexFTOWCPNoFPHonestWriteTotal}{13}
\newcommand{\luindexFTOWCPWriteInCS}{32.1}
\newcommand{\luindexFTOWCPWriteOutCS}{75.5}
\newcommand{\luindexFTOWCPNoFPWriteTotal}{13}
\newcommand{\luindexFTOWCPWriteSameEp}{7.57}
\newcommand{\luindexFTOWCPWriteExclusive}{<0.001}
\newcommand{\luindexFTOWCPWriteOwned}{100}
\newcommand{\luindexFTOWCPWriteShared}{<0.001}
\newcommand{\luindexFTOWCPNoFPOtherEventTotal}{415322}
\newcommand{\luindexFTOWCPAcqRelOtherTotal}{99.9}
\newcommand{\luindexFTOWCPNoAcqRelOtherTotal}{582}
\newcommand{\luindexFTOWCPFork}{0.172}
\newcommand{\luindexFTOWCPJoin}{0.0}
\newcommand{\luindexFTOWCPPreWait}{0.344}
\newcommand{\luindexFTOWCPPostWait}{0.344}
\newcommand{\luindexFTOWCPVolatileTotal}{77.5}
\newcommand{\luindexFTOWCPClassInit}{11.3}
\newcommand{\luindexFTOWCPClassAccess}{10.3}
\newcommand{\luindexFTOWCPRaceTotal}{1}
\newcommand{\luindexFTOWCPWrRdRace}{0.0}
\newcommand{\luindexFTOWCPWrWrRace}{0.0}
\newcommand{\luindexFTOWCPRdWrRace}{0.0}
\newcommand{\luindexFTOWCPRdShWrRace}{100.0}
\newcommand{\luindexFTOWCPHoldLocksTotal}{10}
\newcommand{\luindexFTOWCPOneLockHeld}{25.8}
\newcommand{\luindexFTOWCPTwoNestedLocks}{25.4}
\newcommand{\luindexFTOWCPThreeNestedLocks}{25.3}
\newcommand{\luindexFTOWCPFourNestedLocks}{0.61}
\newcommand{\luindexFTOWCPFiveNestedLocks}{<0.1}
\newcommand{\luindexFTOWCPSixNestedLocks}{<0.1}
\newcommand{\luindexFTOWCPSevenNestedLocks}{\cna}
\newcommand{\luindexFTOWCPEightNestedLocks}{\cna}
\newcommand{\luindexFTOWCPNineNestedLocks}{\cna}
\newcommand{\luindexFTOWCPTenNestedLocks}{\cna}
\newcommand{\luindexFTOWCPHundredNestedLocks}{\cna}
\newcommand{\luindexREWCPEventTotal}{400}
\newcommand{\luindexREWCPNoFPEventTotal}{41}
\newcommand{\luindexREWCPNoFPAccessTotal}{40}
\newcommand{\luindexREWCPNoFPOtherTotal}{0.42}
\newcommand{\luindexREWCPReadTotal}{66.0}
\newcommand{\luindexREWCPWriteTotal}{33.0}
\newcommand{\luindexREWCPNoFPAccessInCS}{8.08}
\newcommand{\luindexREWCPNoFPAccessOutCS}{91.9}
\newcommand{\luindexREWCPAcqRelTotal}{14.2}
\newcommand{\luindexREWCPOtherTotal}{0.0197}
\newcommand{\luindexREWCPNoFPReadTotal}{27}
\newcommand{\luindexREWCPReadInCS}{23.5}
\newcommand{\luindexREWCPReadOutCS}{82}
\newcommand{\luindexREWCPReadSameEp}{5.48}
\newcommand{\luindexREWCPReadSharedSameEp}{\cna}
\newcommand{\luindexREWCPReadExclusive}{<0.001}
\newcommand{\luindexREWCPReadOwned}{100}
\newcommand{\luindexREWCPReadShare}{<0.001}
\newcommand{\luindexREWCPReadShared}{\cna}
\newcommand{\luindexREWCPReadSharedOwned}{<0.001}
\newcommand{\luindexREWCPNoFPHonestWriteTotal}{13}
\newcommand{\luindexREWCPWriteInCS}{32.1}
\newcommand{\luindexREWCPWriteOutCS}{75.5}
\newcommand{\luindexREWCPNoFPWriteTotal}{13}
\newcommand{\luindexREWCPWriteSameEp}{7.57}
\newcommand{\luindexREWCPWriteExclusive}{<0.001}
\newcommand{\luindexREWCPWriteOwned}{100}
\newcommand{\luindexREWCPWriteShared}{<0.001}
\newcommand{\luindexREWCPNoFPOtherEventTotal}{415315}
\newcommand{\luindexREWCPAcqRelOtherTotal}{99.9}
\newcommand{\luindexREWCPNoAcqRelOtherTotal}{575}
\newcommand{\luindexREWCPFork}{0.174}
\newcommand{\luindexREWCPJoin}{0.0}
\newcommand{\luindexREWCPPreWait}{0.348}
\newcommand{\luindexREWCPPostWait}{0.348}
\newcommand{\luindexREWCPVolatileTotal}{77.2}
\newcommand{\luindexREWCPClassInit}{11.5}
\newcommand{\luindexREWCPClassAccess}{10.4}
\newcommand{\luindexREWCPRaceTotal}{1}
\newcommand{\luindexREWCPWrRdRace}{0.0}
\newcommand{\luindexREWCPWrWrRace}{0.0}
\newcommand{\luindexREWCPRdWrRace}{0.0}
\newcommand{\luindexREWCPRdShWrRace}{100.0}
\newcommand{\luindexREWCPHoldLocksTotal}{10}
\newcommand{\luindexREWCPOneLockHeld}{25.8}
\newcommand{\luindexREWCPTwoNestedLocks}{25.4}
\newcommand{\luindexREWCPThreeNestedLocks}{25.3}
\newcommand{\luindexREWCPFourNestedLocks}{0.61}
\newcommand{\luindexREWCPFiveNestedLocks}{<0.1}
\newcommand{\luindexREWCPSixNestedLocks}{<0.1}
\newcommand{\luindexREWCPSevenNestedLocks}{\cna}
\newcommand{\luindexREWCPEightNestedLocks}{\cna}
\newcommand{\luindexREWCPNineNestedLocks}{\cna}
\newcommand{\luindexREWCPTenNestedLocks}{\cna}
\newcommand{\luindexREWCPHundredNestedLocks}{\cna}
\newcommand{\luindexFTODCEventTotal}{400}
\newcommand{\luindexFTODCNoFPEventTotal}{41}
\newcommand{\luindexFTODCNoFPAccessTotal}{40}
\newcommand{\luindexFTODCNoFPOtherTotal}{0.42}
\newcommand{\luindexFTODCReadTotal}{66.0}
\newcommand{\luindexFTODCWriteTotal}{33.0}
\newcommand{\luindexFTODCNoFPAccessInCS}{8.08}
\newcommand{\luindexFTODCNoFPAccessOutCS}{91.9}
\newcommand{\luindexFTODCAcqRelTotal}{14.2}
\newcommand{\luindexFTODCOtherTotal}{0.02}
\newcommand{\luindexFTODCNoFPReadTotal}{27}
\newcommand{\luindexFTODCReadInCS}{23.5}
\newcommand{\luindexFTODCReadOutCS}{82}
\newcommand{\luindexFTODCReadSameEp}{5.48}
\newcommand{\luindexFTODCReadSharedSameEp}{\cna}
\newcommand{\luindexFTODCReadExclusive}{<0.001}
\newcommand{\luindexFTODCReadOwned}{100}
\newcommand{\luindexFTODCReadShare}{<0.001}
\newcommand{\luindexFTODCReadShared}{\cna}
\newcommand{\luindexFTODCReadSharedOwned}{<0.001}
\newcommand{\luindexFTODCNoFPHonestWriteTotal}{13}
\newcommand{\luindexFTODCWriteInCS}{32.1}
\newcommand{\luindexFTODCWriteOutCS}{75.5}
\newcommand{\luindexFTODCNoFPWriteTotal}{13}
\newcommand{\luindexFTODCWriteSameEp}{7.57}
\newcommand{\luindexFTODCWriteExclusive}{<0.001}
\newcommand{\luindexFTODCWriteOwned}{100}
\newcommand{\luindexFTODCWriteShared}{<0.001}
\newcommand{\luindexFTODCNoFPOtherEventTotal}{415322}
\newcommand{\luindexFTODCAcqRelOtherTotal}{99.9}
\newcommand{\luindexFTODCNoAcqRelOtherTotal}{582}
\newcommand{\luindexFTODCFork}{0.172}
\newcommand{\luindexFTODCJoin}{0.0}
\newcommand{\luindexFTODCPreWait}{0.344}
\newcommand{\luindexFTODCPostWait}{0.344}
\newcommand{\luindexFTODCVolatileTotal}{77.5}
\newcommand{\luindexFTODCClassInit}{11.3}
\newcommand{\luindexFTODCClassAccess}{10.3}
\newcommand{\luindexFTODCRaceTotal}{1}
\newcommand{\luindexFTODCWrRdRace}{0.0}
\newcommand{\luindexFTODCWrWrRace}{0.0}
\newcommand{\luindexFTODCRdWrRace}{0.0}
\newcommand{\luindexFTODCRdShWrRace}{100.0}
\newcommand{\luindexFTODCHoldLocksTotal}{10}
\newcommand{\luindexFTODCOneLockHeld}{25.8}
\newcommand{\luindexFTODCTwoNestedLocks}{25.4}
\newcommand{\luindexFTODCThreeNestedLocks}{25.3}
\newcommand{\luindexFTODCFourNestedLocks}{0.61}
\newcommand{\luindexFTODCFiveNestedLocks}{<0.1}
\newcommand{\luindexFTODCSixNestedLocks}{<0.1}
\newcommand{\luindexFTODCSevenNestedLocks}{\cna}
\newcommand{\luindexFTODCEightNestedLocks}{\cna}
\newcommand{\luindexFTODCNineNestedLocks}{\cna}
\newcommand{\luindexFTODCTenNestedLocks}{\cna}
\newcommand{\luindexFTODCHundredNestedLocks}{\cna}
\newcommand{\luindexREDCEventTotal}{400}
\newcommand{\luindexREDCNoFPEventTotal}{41}
\newcommand{\luindexREDCNoFPAccessTotal}{40}
\newcommand{\luindexREDCNoFPOtherTotal}{0.42}
\newcommand{\luindexREDCReadTotal}{66.0}
\newcommand{\luindexREDCWriteTotal}{33.0}
\newcommand{\luindexREDCNoFPAccessInCS}{8.08}
\newcommand{\luindexREDCNoFPAccessOutCS}{91.9}
\newcommand{\luindexREDCAcqRelTotal}{14.2}
\newcommand{\luindexREDCOtherTotal}{0.0197}
\newcommand{\luindexREDCNoFPReadTotal}{27}
\newcommand{\luindexREDCReadInCS}{23.5}
\newcommand{\luindexREDCReadOutCS}{82}
\newcommand{\luindexREDCReadSameEp}{5.48}
\newcommand{\luindexREDCReadSharedSameEp}{\cna}
\newcommand{\luindexREDCReadExclusive}{<0.001}
\newcommand{\luindexREDCReadOwned}{100}
\newcommand{\luindexREDCReadShare}{<0.001}
\newcommand{\luindexREDCReadShared}{\cna}
\newcommand{\luindexREDCReadSharedOwned}{<0.001}
\newcommand{\luindexREDCNoFPHonestWriteTotal}{13}
\newcommand{\luindexREDCWriteInCS}{32.1}
\newcommand{\luindexREDCWriteOutCS}{75.5}
\newcommand{\luindexREDCNoFPWriteTotal}{13}
\newcommand{\luindexREDCWriteSameEp}{7.57}
\newcommand{\luindexREDCWriteExclusive}{<0.001}
\newcommand{\luindexREDCWriteOwned}{100}
\newcommand{\luindexREDCWriteShared}{<0.001}
\newcommand{\luindexREDCNoFPOtherEventTotal}{415315}
\newcommand{\luindexREDCAcqRelOtherTotal}{99.9}
\newcommand{\luindexREDCNoAcqRelOtherTotal}{575}
\newcommand{\luindexREDCFork}{0.174}
\newcommand{\luindexREDCJoin}{0.0}
\newcommand{\luindexREDCPreWait}{0.348}
\newcommand{\luindexREDCPostWait}{0.348}
\newcommand{\luindexREDCVolatileTotal}{77.2}
\newcommand{\luindexREDCClassInit}{11.5}
\newcommand{\luindexREDCClassAccess}{10.4}
\newcommand{\luindexREDCRaceTotal}{1}
\newcommand{\luindexREDCWrRdRace}{0.0}
\newcommand{\luindexREDCWrWrRace}{0.0}
\newcommand{\luindexREDCRdWrRace}{0.0}
\newcommand{\luindexREDCRdShWrRace}{100.0}
\newcommand{\luindexREDCHoldLocksTotal}{10}
\newcommand{\luindexREDCOneLockHeld}{25.8}
\newcommand{\luindexREDCTwoNestedLocks}{25.4}
\newcommand{\luindexREDCThreeNestedLocks}{25.3}
\newcommand{\luindexREDCFourNestedLocks}{0.61}
\newcommand{\luindexREDCFiveNestedLocks}{<0.1}
\newcommand{\luindexREDCSixNestedLocks}{<0.1}
\newcommand{\luindexREDCSevenNestedLocks}{\cna}
\newcommand{\luindexREDCEightNestedLocks}{\cna}
\newcommand{\luindexREDCNineNestedLocks}{\cna}
\newcommand{\luindexREDCTenNestedLocks}{\cna}
\newcommand{\luindexREDCHundredNestedLocks}{\cna}
\newcommand{\luindexFTOCAPOEventTotal}{400}
\newcommand{\luindexFTOCAPONoFPEventTotal}{41}
\newcommand{\luindexFTOCAPONoFPAccessTotal}{40}
\newcommand{\luindexFTOCAPONoFPOtherTotal}{0.42}
\newcommand{\luindexFTOCAPOReadTotal}{66.0}
\newcommand{\luindexFTOCAPOWriteTotal}{33.0}
\newcommand{\luindexFTOCAPONoFPAccessInCS}{8.08}
\newcommand{\luindexFTOCAPONoFPAccessOutCS}{91.9}
\newcommand{\luindexFTOCAPOAcqRelTotal}{14.2}
\newcommand{\luindexFTOCAPOOtherTotal}{0.02}
\newcommand{\luindexFTOCAPONoFPReadTotal}{27}
\newcommand{\luindexFTOCAPOReadInCS}{23.5}
\newcommand{\luindexFTOCAPOReadOutCS}{82}
\newcommand{\luindexFTOCAPOReadSameEp}{5.48}
\newcommand{\luindexFTOCAPOReadSharedSameEp}{\cna}
\newcommand{\luindexFTOCAPOReadExclusive}{<0.001}
\newcommand{\luindexFTOCAPOReadOwned}{100}
\newcommand{\luindexFTOCAPOReadShare}{<0.001}
\newcommand{\luindexFTOCAPOReadShared}{\cna}
\newcommand{\luindexFTOCAPOReadSharedOwned}{<0.001}
\newcommand{\luindexFTOCAPONoFPHonestWriteTotal}{13}
\newcommand{\luindexFTOCAPOWriteInCS}{32.1}
\newcommand{\luindexFTOCAPOWriteOutCS}{75.5}
\newcommand{\luindexFTOCAPONoFPWriteTotal}{13}
\newcommand{\luindexFTOCAPOWriteSameEp}{7.57}
\newcommand{\luindexFTOCAPOWriteExclusive}{<0.001}
\newcommand{\luindexFTOCAPOWriteOwned}{100}
\newcommand{\luindexFTOCAPOWriteShared}{<0.001}
\newcommand{\luindexFTOCAPONoFPOtherEventTotal}{415322}
\newcommand{\luindexFTOCAPOAcqRelOtherTotal}{99.9}
\newcommand{\luindexFTOCAPONoAcqRelOtherTotal}{582}
\newcommand{\luindexFTOCAPOFork}{0.172}
\newcommand{\luindexFTOCAPOJoin}{0.0}
\newcommand{\luindexFTOCAPOPreWait}{0.344}
\newcommand{\luindexFTOCAPOPostWait}{0.344}
\newcommand{\luindexFTOCAPOVolatileTotal}{77.5}
\newcommand{\luindexFTOCAPOClassInit}{11.3}
\newcommand{\luindexFTOCAPOClassAccess}{10.3}
\newcommand{\luindexFTOCAPORaceTotal}{1}
\newcommand{\luindexFTOCAPOWrRdRace}{0.0}
\newcommand{\luindexFTOCAPOWrWrRace}{0.0}
\newcommand{\luindexFTOCAPORdWrRace}{0.0}
\newcommand{\luindexFTOCAPORdShWrRace}{100.0}
\newcommand{\luindexFTOCAPOHoldLocksTotal}{10}
\newcommand{\luindexFTOCAPOOneLockHeld}{25.8}
\newcommand{\luindexFTOCAPOTwoNestedLocks}{25.4}
\newcommand{\luindexFTOCAPOThreeNestedLocks}{25.3}
\newcommand{\luindexFTOCAPOFourNestedLocks}{0.61}
\newcommand{\luindexFTOCAPOFiveNestedLocks}{<0.1}
\newcommand{\luindexFTOCAPOSixNestedLocks}{<0.1}
\newcommand{\luindexFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\luindexFTOCAPOEightNestedLocks}{\cna}
\newcommand{\luindexFTOCAPONineNestedLocks}{\cna}
\newcommand{\luindexFTOCAPOTenNestedLocks}{\cna}
\newcommand{\luindexFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\luindexRECAPOEventTotal}{400}
\newcommand{\luindexRECAPONoFPEventTotal}{41}
\newcommand{\luindexRECAPONoFPAccessTotal}{40}
\newcommand{\luindexRECAPONoFPOtherTotal}{0.42}
\newcommand{\luindexRECAPOReadTotal}{66.0}
\newcommand{\luindexRECAPOWriteTotal}{33.0}
\newcommand{\luindexRECAPONoFPAccessInCS}{8.08}
\newcommand{\luindexRECAPONoFPAccessOutCS}{91.9}
\newcommand{\luindexRECAPOAcqRelTotal}{14.2}
\newcommand{\luindexRECAPOOtherTotal}{0.0197}
\newcommand{\luindexRECAPONoFPReadTotal}{27}
\newcommand{\luindexRECAPOReadInCS}{23.5}
\newcommand{\luindexRECAPOReadOutCS}{82}
\newcommand{\luindexRECAPOReadSameEp}{5.48}
\newcommand{\luindexRECAPOReadSharedSameEp}{\cna}
\newcommand{\luindexRECAPOReadExclusive}{<0.001}
\newcommand{\luindexRECAPOReadOwned}{100}
\newcommand{\luindexRECAPOReadShare}{<0.001}
\newcommand{\luindexRECAPOReadShared}{\cna}
\newcommand{\luindexRECAPOReadSharedOwned}{<0.001}
\newcommand{\luindexRECAPONoFPHonestWriteTotal}{13}
\newcommand{\luindexRECAPOWriteInCS}{32.1}
\newcommand{\luindexRECAPOWriteOutCS}{75.5}
\newcommand{\luindexRECAPONoFPWriteTotal}{13}
\newcommand{\luindexRECAPOWriteSameEp}{7.57}
\newcommand{\luindexRECAPOWriteExclusive}{<0.001}
\newcommand{\luindexRECAPOWriteOwned}{100}
\newcommand{\luindexRECAPOWriteShared}{<0.001}
\newcommand{\luindexRECAPONoFPOtherEventTotal}{415315}
\newcommand{\luindexRECAPOAcqRelOtherTotal}{99.9}
\newcommand{\luindexRECAPONoAcqRelOtherTotal}{575}
\newcommand{\luindexRECAPOFork}{0.174}
\newcommand{\luindexRECAPOJoin}{0.0}
\newcommand{\luindexRECAPOPreWait}{0.348}
\newcommand{\luindexRECAPOPostWait}{0.348}
\newcommand{\luindexRECAPOVolatileTotal}{77.2}
\newcommand{\luindexRECAPOClassInit}{11.5}
\newcommand{\luindexRECAPOClassAccess}{10.4}
\newcommand{\luindexRECAPORaceTotal}{1}
\newcommand{\luindexRECAPOWrRdRace}{0.0}
\newcommand{\luindexRECAPOWrWrRace}{0.0}
\newcommand{\luindexRECAPORdWrRace}{0.0}
\newcommand{\luindexRECAPORdShWrRace}{100.0}
\newcommand{\luindexRECAPOHoldLocksTotal}{10}
\newcommand{\luindexRECAPOOneLockHeld}{25.8}
\newcommand{\luindexRECAPOTwoNestedLocks}{25.4}
\newcommand{\luindexRECAPOThreeNestedLocks}{25.3}
\newcommand{\luindexRECAPOFourNestedLocks}{0.61}
\newcommand{\luindexRECAPOFiveNestedLocks}{<0.1}
\newcommand{\luindexRECAPOSixNestedLocks}{<0.1}
\newcommand{\luindexRECAPOSevenNestedLocks}{\cna}
\newcommand{\luindexRECAPOEightNestedLocks}{\cna}
\newcommand{\luindexRECAPONineNestedLocks}{\cna}
\newcommand{\luindexRECAPOTenNestedLocks}{\cna}
\newcommand{\luindexRECAPOHundredNestedLocks}{\cna}
\newcommand{\FASTluindexMaxLiveThreads}{3}
\newcommand{\FASTluindexTotalThreads}{3}
\newcommand{\FASTluindexBaseTime}{1.2}
\newcommand{\FASTluindexBaseTimeCI}{40}
\newcommand{\FASTluindexEmptyTime}{\rna}
\newcommand{\FASTluindexEmptyTimeCI}{\rna}
\newcommand{\FASTluindexEmptyTimeCIMIN}{\rna}
\newcommand{\FASTluindexEmptyTimeCIMAX}{\rna}
\newcommand{\FASTluindexFTTime}{8.1}
\newcommand{\FASTluindexFTTimeCI}{0.28}
\newcommand{\FASTluindexHBTime}{8.4}
\newcommand{\FASTluindexHBTimeCI}{0.24}
\newcommand{\FASTluindexFTOHBTime}{8.3}
\newcommand{\FASTluindexFTOHBTimeCI}{0.27}
\newcommand{\FASTluindexWCPTime}{\rna}
\newcommand{\FASTluindexWCPTimeCI}{\rna}
\newcommand{\FASTluindexWCPTimeCIMIN}{\rna}
\newcommand{\FASTluindexWCPTimeCIMAX}{\rna}
\newcommand{\FASTluindexFTOWCPTime}{25}
\newcommand{\FASTluindexFTOWCPTimeCI}{0.79}
\newcommand{\FASTluindexREWCPTime}{9.8}
\newcommand{\FASTluindexREWCPTimeCI}{0.26}
\newcommand{\FASTluindexDCTime}{\rna}
\newcommand{\FASTluindexDCTimeCI}{\rna}
\newcommand{\FASTluindexDCTimeCIMIN}{\rna}
\newcommand{\FASTluindexDCTimeCIMAX}{\rna}
\newcommand{\FASTluindexFTODCTime}{25}
\newcommand{\FASTluindexFTODCTimeCI}{0.69}
\newcommand{\FASTluindexREDCTime}{9.7}
\newcommand{\FASTluindexREDCTimeCI}{0.25}
\newcommand{\FASTluindexCAPOTime}{\rna}
\newcommand{\FASTluindexCAPOTimeCI}{\rna}
\newcommand{\FASTluindexCAPOTimeCIMIN}{\rna}
\newcommand{\FASTluindexCAPOTimeCIMAX}{\rna}
\newcommand{\FASTluindexFTOCAPOTime}{25}
\newcommand{\FASTluindexFTOCAPOTimeCI}{0.83}
\newcommand{\FASTluindexRECAPOTime}{9.5}
\newcommand{\FASTluindexRECAPOTimeCI}{0.32}
\newcommand{\FASTluindexAGGCAPOTime}{\rna}
\newcommand{\FASTluindexAGGCAPOTimeCI}{\rna}
\newcommand{\FASTluindexAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTluindexAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTluindexStaticTime}{\rzero}
\newcommand{\FASTluindexDynamicTime}{\rzero}
\newcommand{\FASTluindexBaseMem}{130}
\newcommand{\FASTluindexBaseMemCI}{8.1}
\newcommand{\FASTluindexFTMem}{4.8}
\newcommand{\FASTluindexFTMemCI}{0.25}
\newcommand{\FASTluindexHBMem}{4.7}
\newcommand{\FASTluindexHBMemCI}{0.23}
\newcommand{\FASTluindexFTOHBMem}{4.8}
\newcommand{\FASTluindexFTOHBMemCI}{0.25}
\newcommand{\FASTluindexWCPMem}{\memna}
\newcommand{\FASTluindexWCPMemCI}{\memna}
\newcommand{\FASTluindexWCPMemCIMIN}{\memna}
\newcommand{\FASTluindexWCPMemCIMAX}{\memna}
\newcommand{\FASTluindexFTOWCPMem}{23}
\newcommand{\FASTluindexFTOWCPMemCI}{1.4}
\newcommand{\FASTluindexREWCPMem}{8.7}
\newcommand{\FASTluindexREWCPMemCI}{0.67}
\newcommand{\FASTluindexDCMem}{\memna}
\newcommand{\FASTluindexDCMemCI}{\memna}
\newcommand{\FASTluindexDCMemCIMIN}{\memna}
\newcommand{\FASTluindexDCMemCIMAX}{\memna}
\newcommand{\FASTluindexFTODCMem}{22}
\newcommand{\FASTluindexFTODCMemCI}{1.4}
\newcommand{\FASTluindexREDCMem}{10}
\newcommand{\FASTluindexREDCMemCI}{0.6}
\newcommand{\FASTluindexCAPOMem}{\memna}
\newcommand{\FASTluindexCAPOMemCI}{\memna}
\newcommand{\FASTluindexCAPOMemCIMIN}{\memna}
\newcommand{\FASTluindexCAPOMemCIMAX}{\memna}
\newcommand{\FASTluindexFTOCAPOMem}{23}
\newcommand{\FASTluindexFTOCAPOMemCI}{1.3}
\newcommand{\FASTluindexRECAPOMem}{7.9}
\newcommand{\FASTluindexRECAPOMemCI}{0.44}
\newcommand{\FASTluindexAGGCAPOMem}{\memna}
\newcommand{\FASTluindexAGGCAPOMemCI}{\memna}
\newcommand{\FASTluindexAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTluindexAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTluindexEventsCI}{1}
\newcommand{\FASTluindexEventsCIMIN}{396,268,360}
\newcommand{\FASTluindexEventsCIMAX}{396,268,362}
\newcommand{\FASTluindexNoFPEventsCI}{0}
\newcommand{\FASTluindexNoFPEventsCIMIN}{2,915,285}
\newcommand{\FASTluindexNoFPEventsCIMAX}{2,915,285}
\newcommand{\FASTluindexFT}{1}
\newcommand{\FASTluindexFTCI}{0.0}
\newcommand{\FASTluindexFTCIMIN}{1}
\newcommand{\FASTluindexFTCIMAX}{1}
\newcommand{\FASTluindexFTDynamic}{1}
\newcommand{\FASTluindexFTDynamicCI}{0.0}
\newcommand{\FASTluindexFTDynamicCIMIN}{1}
\newcommand{\FASTluindexFTDynamicCIMAX}{1}
\newcommand{\FASTluindexHB}{1}
\newcommand{\FASTluindexHBCI}{0.0}
\newcommand{\FASTluindexHBCIMIN}{1}
\newcommand{\FASTluindexHBCIMAX}{1}
\newcommand{\FASTluindexHBDynamic}{1}
\newcommand{\FASTluindexHBDynamicCI}{0.0}
\newcommand{\FASTluindexHBDynamicCIMIN}{1}
\newcommand{\FASTluindexHBDynamicCIMAX}{1}
\newcommand{\FASTluindexFTOHB}{1}
\newcommand{\FASTluindexFTOHBCI}{0.0}
\newcommand{\FASTluindexFTOHBCIMIN}{1}
\newcommand{\FASTluindexFTOHBCIMAX}{1}
\newcommand{\FASTluindexFTOHBDynamic}{1}
\newcommand{\FASTluindexFTOHBDynamicCI}{0.0}
\newcommand{\FASTluindexFTOHBDynamicCIMIN}{1}
\newcommand{\FASTluindexFTOHBDynamicCIMAX}{1}
\newcommand{\FASTluindexWCP}{\rna}
\newcommand{\FASTluindexWCPCI}{\rna}
\newcommand{\FASTluindexWCPCIMIN}{\rna}
\newcommand{\FASTluindexWCPCIMAX}{\rna}
\newcommand{\FASTluindexWCPDynamic}{\rna}
\newcommand{\FASTluindexWCPDynamicCI}{\rna}
\newcommand{\FASTluindexWCPDynamicCIMIN}{\rna}
\newcommand{\FASTluindexWCPDynamicCIMAX}{\rna}
\newcommand{\FASTluindexFTOWCP}{1}
\newcommand{\FASTluindexFTOWCPCI}{0.0}
\newcommand{\FASTluindexFTOWCPCIMIN}{1}
\newcommand{\FASTluindexFTOWCPCIMAX}{1}
\newcommand{\FASTluindexFTOWCPDynamic}{1}
\newcommand{\FASTluindexFTOWCPDynamicCI}{0.0}
\newcommand{\FASTluindexFTOWCPDynamicCIMIN}{1}
\newcommand{\FASTluindexFTOWCPDynamicCIMAX}{1}
\newcommand{\FASTluindexREWCP}{1}
\newcommand{\FASTluindexREWCPCI}{0.0}
\newcommand{\FASTluindexREWCPCIMIN}{1}
\newcommand{\FASTluindexREWCPCIMAX}{1}
\newcommand{\FASTluindexREWCPDynamic}{1}
\newcommand{\FASTluindexREWCPDynamicCI}{0.0}
\newcommand{\FASTluindexREWCPDynamicCIMIN}{1}
\newcommand{\FASTluindexREWCPDynamicCIMAX}{1}
\newcommand{\FASTluindexDC}{\rna}
\newcommand{\FASTluindexDCCI}{\rna}
\newcommand{\FASTluindexDCCIMIN}{\rna}
\newcommand{\FASTluindexDCCIMAX}{\rna}
\newcommand{\FASTluindexDCDynamic}{\rna}
\newcommand{\FASTluindexDCDynamicCI}{\rna}
\newcommand{\FASTluindexDCDynamicCIMIN}{\rna}
\newcommand{\FASTluindexDCDynamicCIMAX}{\rna}
\newcommand{\FASTluindexFTODC}{1}
\newcommand{\FASTluindexFTODCCI}{0.0}
\newcommand{\FASTluindexFTODCCIMIN}{1}
\newcommand{\FASTluindexFTODCCIMAX}{1}
\newcommand{\FASTluindexFTODCDynamic}{1}
\newcommand{\FASTluindexFTODCDynamicCI}{0.0}
\newcommand{\FASTluindexFTODCDynamicCIMIN}{1}
\newcommand{\FASTluindexFTODCDynamicCIMAX}{1}
\newcommand{\FASTluindexREDC}{1}
\newcommand{\FASTluindexREDCCI}{0.0}
\newcommand{\FASTluindexREDCCIMIN}{1}
\newcommand{\FASTluindexREDCCIMAX}{1}
\newcommand{\FASTluindexREDCDynamic}{1}
\newcommand{\FASTluindexREDCDynamicCI}{0.0}
\newcommand{\FASTluindexREDCDynamicCIMIN}{1}
\newcommand{\FASTluindexREDCDynamicCIMAX}{1}
\newcommand{\FASTluindexCAPO}{\rna}
\newcommand{\FASTluindexCAPOCI}{\rna}
\newcommand{\FASTluindexCAPOCIMIN}{\rna}
\newcommand{\FASTluindexCAPOCIMAX}{\rna}
\newcommand{\FASTluindexCAPODynamic}{\rna}
\newcommand{\FASTluindexCAPODynamicCI}{\rna}
\newcommand{\FASTluindexCAPODynamicCIMIN}{\rna}
\newcommand{\FASTluindexCAPODynamicCIMAX}{\rna}
\newcommand{\FASTluindexFTOCAPO}{1}
\newcommand{\FASTluindexFTOCAPOCI}{0.0}
\newcommand{\FASTluindexFTOCAPOCIMIN}{1}
\newcommand{\FASTluindexFTOCAPOCIMAX}{1}
\newcommand{\FASTluindexFTOCAPODynamic}{1}
\newcommand{\FASTluindexFTOCAPODynamicCI}{0.0}
\newcommand{\FASTluindexFTOCAPODynamicCIMIN}{1}
\newcommand{\FASTluindexFTOCAPODynamicCIMAX}{1}
\newcommand{\FASTluindexRECAPO}{1}
\newcommand{\FASTluindexRECAPOCI}{0.0}
\newcommand{\FASTluindexRECAPOCIMIN}{1}
\newcommand{\FASTluindexRECAPOCIMAX}{1}
\newcommand{\FASTluindexRECAPODynamic}{1}
\newcommand{\FASTluindexRECAPODynamicCI}{0.0}
\newcommand{\FASTluindexRECAPODynamicCIMIN}{1}
\newcommand{\FASTluindexRECAPODynamicCIMAX}{1}
\newcommand{\FASTluindexAGGCAPO}{\rna}
\newcommand{\FASTluindexAGGCAPOCI}{\rna}
\newcommand{\FASTluindexAGGCAPOCIMIN}{\rna}
\newcommand{\FASTluindexAGGCAPOCIMAX}{\rna}
\newcommand{\FASTluindexAGGCAPODynamic}{\rna}
\newcommand{\FASTluindexAGGCAPODynamicCI}{\rna}
\newcommand{\FASTluindexAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTluindexAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTlusearchEvents}{1,400}
\newcommand{\FASTlusearchNoFPEvents}{43}
\newcommand{\lusearchHBEventTotal}{1,400}
\newcommand{\lusearchHBNoFPEventTotal}{150}
\newcommand{\lusearchHBNoFPAccessTotal}{150}
\newcommand{\lusearchHBNoFPOtherTotal}{3.8}
\newcommand{\lusearchHBReadTotal}{79.4}
\newcommand{\lusearchHBWriteTotal}{18.1}
\newcommand{\lusearchHBNoFPAccessInCS}{4.89}
\newcommand{\lusearchHBNoFPAccessOutCS}{95.1}
\newcommand{\lusearchHBAcqRelTotal}{6.23}
\newcommand{\lusearchHBOtherTotal}{2.72}
\newcommand{\lusearchHBNoFPReadTotal}{120}
\newcommand{\lusearchHBReadInCS}{3.36}
\newcommand{\lusearchHBReadOutCS}{103}
\newcommand{\lusearchHBReadSameEp}{6.47}
\newcommand{\lusearchHBReadSharedSameEp}{\cna}
\newcommand{\lusearchHBReadExclusive}{96.6}
\newcommand{\lusearchHBReadOwned}{\cna}
\newcommand{\lusearchHBReadShare}{<0.001}
\newcommand{\lusearchHBReadShared}{3.41}
\newcommand{\lusearchHBReadSharedOwned}{\cna}
\newcommand{\lusearchHBNoFPHonestWriteTotal}{28}
\newcommand{\lusearchHBWriteInCS}{10}
\newcommand{\lusearchHBWriteOutCS}{200}
\newcommand{\lusearchHBNoFPWriteTotal}{28}
\newcommand{\lusearchHBWriteSameEp}{110}
\newcommand{\lusearchHBWriteExclusive}{100}
\newcommand{\lusearchHBWriteOwned}{\cna}
\newcommand{\lusearchHBWriteShared}{\cna}
\newcommand{\lusearchHBNoFPOtherEventTotal}{3816290}
\newcommand{\lusearchHBAcqRelOtherTotal}{69.6}
\newcommand{\lusearchHBNoAcqRelOtherTotal}{1158354}
\newcommand{\lusearchHBFork}{0.00121}
\newcommand{\lusearchHBJoin}{0.0}
\newcommand{\lusearchHBPreWait}{0.00518}
\newcommand{\lusearchHBPostWait}{0.00518}
\newcommand{\lusearchHBVolatileTotal}{100.0}
\newcommand{\lusearchHBClassInit}{0.00311}
\newcommand{\lusearchHBClassAccess}{0.0293}
\newcommand{\lusearchHBRaceTotal}{\rna}
\newcommand{\lusearchHBWrRdRace}{\rna}
\newcommand{\lusearchHBWrWrRace}{\rna}
\newcommand{\lusearchHBRdWrRace}{\rna}
\newcommand{\lusearchHBRdShWrRace}{\rna}
\newcommand{\lusearchHBHoldLocksTotal}{6.9}
\newcommand{\lusearchHBOneLockHeld}{4.60}
\newcommand{\lusearchHBTwoNestedLocks}{0.26}
\newcommand{\lusearchHBThreeNestedLocks}{<0.1}
\newcommand{\lusearchHBFourNestedLocks}{\cna}
\newcommand{\lusearchHBFiveNestedLocks}{\cna}
\newcommand{\lusearchHBSixNestedLocks}{\cna}
\newcommand{\lusearchHBSevenNestedLocks}{\cna}
\newcommand{\lusearchHBEightNestedLocks}{\cna}
\newcommand{\lusearchHBNineNestedLocks}{\cna}
\newcommand{\lusearchHBTenNestedLocks}{\cna}
\newcommand{\lusearchHBHundredNestedLocks}{\cna}
\newcommand{\lusearchFTOHBEventTotal}{1,400}
\newcommand{\lusearchFTOHBNoFPEventTotal}{140}
\newcommand{\lusearchFTOHBNoFPAccessTotal}{130}
\newcommand{\lusearchFTOHBNoFPOtherTotal}{3.8}
\newcommand{\lusearchFTOHBReadTotal}{76.9}
\newcommand{\lusearchFTOHBWriteTotal}{20.3}
\newcommand{\lusearchFTOHBNoFPAccessInCS}{4.89}
\newcommand{\lusearchFTOHBNoFPAccessOutCS}{95.1}
\newcommand{\lusearchFTOHBAcqRelTotal}{6.23}
\newcommand{\lusearchFTOHBOtherTotal}{2.72}
\newcommand{\lusearchFTOHBNoFPReadTotal}{110}
\newcommand{\lusearchFTOHBReadInCS}{3.53}
\newcommand{\lusearchFTOHBReadOutCS}{104}
\newcommand{\lusearchFTOHBReadSameEp}{7.49}
\newcommand{\lusearchFTOHBReadSharedSameEp}{\cna}
\newcommand{\lusearchFTOHBReadExclusive}{<0.001}
\newcommand{\lusearchFTOHBReadOwned}{96.1}
\newcommand{\lusearchFTOHBReadShare}{<0.001}
\newcommand{\lusearchFTOHBReadShared}{0.00113}
\newcommand{\lusearchFTOHBReadSharedOwned}{3.94}
\newcommand{\lusearchFTOHBNoFPHonestWriteTotal}{28}
\newcommand{\lusearchFTOHBWriteInCS}{10}
\newcommand{\lusearchFTOHBWriteOutCS}{200}
\newcommand{\lusearchFTOHBNoFPWriteTotal}{28}
\newcommand{\lusearchFTOHBWriteSameEp}{110}
\newcommand{\lusearchFTOHBWriteExclusive}{\cna}
\newcommand{\lusearchFTOHBWriteOwned}{100}
\newcommand{\lusearchFTOHBWriteShared}{\cna}
\newcommand{\lusearchFTOHBNoFPOtherEventTotal}{3816326}
\newcommand{\lusearchFTOHBAcqRelOtherTotal}{69.6}
\newcommand{\lusearchFTOHBNoAcqRelOtherTotal}{1158390}
\newcommand{\lusearchFTOHBFork}{0.00121}
\newcommand{\lusearchFTOHBJoin}{0.0}
\newcommand{\lusearchFTOHBPreWait}{0.00518}
\newcommand{\lusearchFTOHBPostWait}{0.00518}
\newcommand{\lusearchFTOHBVolatileTotal}{100.0}
\newcommand{\lusearchFTOHBClassInit}{0.00311}
\newcommand{\lusearchFTOHBClassAccess}{0.0293}
\newcommand{\lusearchFTOHBRaceTotal}{\rna}
\newcommand{\lusearchFTOHBWrRdRace}{\rna}
\newcommand{\lusearchFTOHBWrWrRace}{\rna}
\newcommand{\lusearchFTOHBRdWrRace}{\rna}
\newcommand{\lusearchFTOHBRdShWrRace}{\rna}
\newcommand{\lusearchFTOHBHoldLocksTotal}{4.7}
\newcommand{\lusearchFTOHBOneLockHeld}{3.47}
\newcommand{\lusearchFTOHBTwoNestedLocks}{0.29}
\newcommand{\lusearchFTOHBThreeNestedLocks}{<0.1}
\newcommand{\lusearchFTOHBFourNestedLocks}{\cna}
\newcommand{\lusearchFTOHBFiveNestedLocks}{\cna}
\newcommand{\lusearchFTOHBSixNestedLocks}{\cna}
\newcommand{\lusearchFTOHBSevenNestedLocks}{\cna}
\newcommand{\lusearchFTOHBEightNestedLocks}{\cna}
\newcommand{\lusearchFTOHBNineNestedLocks}{\cna}
\newcommand{\lusearchFTOHBTenNestedLocks}{\cna}
\newcommand{\lusearchFTOHBHundredNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPEventTotal}{1,400}
\newcommand{\lusearchFTOWCPNoFPEventTotal}{140}
\newcommand{\lusearchFTOWCPNoFPAccessTotal}{130}
\newcommand{\lusearchFTOWCPNoFPOtherTotal}{3.8}
\newcommand{\lusearchFTOWCPReadTotal}{77.0}
\newcommand{\lusearchFTOWCPWriteTotal}{20.2}
\newcommand{\lusearchFTOWCPNoFPAccessInCS}{4.89}
\newcommand{\lusearchFTOWCPNoFPAccessOutCS}{95.1}
\newcommand{\lusearchFTOWCPAcqRelTotal}{6.23}
\newcommand{\lusearchFTOWCPOtherTotal}{2.72}
\newcommand{\lusearchFTOWCPNoFPReadTotal}{110}
\newcommand{\lusearchFTOWCPReadInCS}{3.94}
\newcommand{\lusearchFTOWCPReadOutCS}{104}
\newcommand{\lusearchFTOWCPReadSameEp}{7.45}
\newcommand{\lusearchFTOWCPReadSharedSameEp}{\cna}
\newcommand{\lusearchFTOWCPReadExclusive}{<0.001}
\newcommand{\lusearchFTOWCPReadOwned}{96.1}
\newcommand{\lusearchFTOWCPReadShare}{<0.001}
\newcommand{\lusearchFTOWCPReadShared}{0.00113}
\newcommand{\lusearchFTOWCPReadSharedOwned}{3.93}
\newcommand{\lusearchFTOWCPNoFPHonestWriteTotal}{28}
\newcommand{\lusearchFTOWCPWriteInCS}{10}
\newcommand{\lusearchFTOWCPWriteOutCS}{200}
\newcommand{\lusearchFTOWCPNoFPWriteTotal}{28}
\newcommand{\lusearchFTOWCPWriteSameEp}{110}
\newcommand{\lusearchFTOWCPWriteExclusive}{\cna}
\newcommand{\lusearchFTOWCPWriteOwned}{100}
\newcommand{\lusearchFTOWCPWriteShared}{<0.001}
\newcommand{\lusearchFTOWCPNoFPOtherEventTotal}{3816265}
\newcommand{\lusearchFTOWCPAcqRelOtherTotal}{69.6}
\newcommand{\lusearchFTOWCPNoAcqRelOtherTotal}{1158329}
\newcommand{\lusearchFTOWCPFork}{0.00121}
\newcommand{\lusearchFTOWCPJoin}{0.0}
\newcommand{\lusearchFTOWCPPreWait}{0.00527}
\newcommand{\lusearchFTOWCPPostWait}{0.00527}
\newcommand{\lusearchFTOWCPVolatileTotal}{100.0}
\newcommand{\lusearchFTOWCPClassInit}{0.00311}
\newcommand{\lusearchFTOWCPClassAccess}{0.0293}
\newcommand{\lusearchFTOWCPRaceTotal}{\rna}
\newcommand{\lusearchFTOWCPWrRdRace}{\rna}
\newcommand{\lusearchFTOWCPWrWrRace}{\rna}
\newcommand{\lusearchFTOWCPRdWrRace}{\rna}
\newcommand{\lusearchFTOWCPRdShWrRace}{\rna}
\newcommand{\lusearchFTOWCPHoldLocksTotal}{5.1}
\newcommand{\lusearchFTOWCPOneLockHeld}{3.79}
\newcommand{\lusearchFTOWCPTwoNestedLocks}{0.39}
\newcommand{\lusearchFTOWCPThreeNestedLocks}{<0.1}
\newcommand{\lusearchFTOWCPFourNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPFiveNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPSixNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPSevenNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPEightNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPNineNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPTenNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPHundredNestedLocks}{\cna}
\newcommand{\lusearchREWCPEventTotal}{1,400}
\newcommand{\lusearchREWCPNoFPEventTotal}{140}
\newcommand{\lusearchREWCPNoFPAccessTotal}{130}
\newcommand{\lusearchREWCPNoFPOtherTotal}{3.8}
\newcommand{\lusearchREWCPReadTotal}{77.0}
\newcommand{\lusearchREWCPWriteTotal}{20.2}
\newcommand{\lusearchREWCPNoFPAccessInCS}{4.89}
\newcommand{\lusearchREWCPNoFPAccessOutCS}{95.1}
\newcommand{\lusearchREWCPAcqRelTotal}{6.23}
\newcommand{\lusearchREWCPOtherTotal}{2.72}
\newcommand{\lusearchREWCPNoFPReadTotal}{110}
\newcommand{\lusearchREWCPReadInCS}{3.94}
\newcommand{\lusearchREWCPReadOutCS}{104}
\newcommand{\lusearchREWCPReadSameEp}{7.45}
\newcommand{\lusearchREWCPReadSharedSameEp}{\cna}
\newcommand{\lusearchREWCPReadExclusive}{<0.001}
\newcommand{\lusearchREWCPReadOwned}{96.1}
\newcommand{\lusearchREWCPReadShare}{<0.001}
\newcommand{\lusearchREWCPReadShared}{0.00113}
\newcommand{\lusearchREWCPReadSharedOwned}{3.93}
\newcommand{\lusearchREWCPNoFPHonestWriteTotal}{28}
\newcommand{\lusearchREWCPWriteInCS}{10}
\newcommand{\lusearchREWCPWriteOutCS}{200}
\newcommand{\lusearchREWCPNoFPWriteTotal}{28}
\newcommand{\lusearchREWCPWriteSameEp}{110}
\newcommand{\lusearchREWCPWriteExclusive}{\cna}
\newcommand{\lusearchREWCPWriteOwned}{100}
\newcommand{\lusearchREWCPWriteShared}{<0.001}
\newcommand{\lusearchREWCPNoFPOtherEventTotal}{3816272}
\newcommand{\lusearchREWCPAcqRelOtherTotal}{69.6}
\newcommand{\lusearchREWCPNoAcqRelOtherTotal}{1158336}
\newcommand{\lusearchREWCPFork}{0.00121}
\newcommand{\lusearchREWCPJoin}{0.0}
\newcommand{\lusearchREWCPPreWait}{0.00527}
\newcommand{\lusearchREWCPPostWait}{0.00527}
\newcommand{\lusearchREWCPVolatileTotal}{100.0}
\newcommand{\lusearchREWCPClassInit}{0.00311}
\newcommand{\lusearchREWCPClassAccess}{0.0293}
\newcommand{\lusearchREWCPRaceTotal}{\rna}
\newcommand{\lusearchREWCPWrRdRace}{\rna}
\newcommand{\lusearchREWCPWrWrRace}{\rna}
\newcommand{\lusearchREWCPRdWrRace}{\rna}
\newcommand{\lusearchREWCPRdShWrRace}{\rna}
\newcommand{\lusearchREWCPHoldLocksTotal}{5.1}
\newcommand{\lusearchREWCPOneLockHeld}{3.79}
\newcommand{\lusearchREWCPTwoNestedLocks}{0.39}
\newcommand{\lusearchREWCPThreeNestedLocks}{<0.1}
\newcommand{\lusearchREWCPFourNestedLocks}{\cna}
\newcommand{\lusearchREWCPFiveNestedLocks}{\cna}
\newcommand{\lusearchREWCPSixNestedLocks}{\cna}
\newcommand{\lusearchREWCPSevenNestedLocks}{\cna}
\newcommand{\lusearchREWCPEightNestedLocks}{\cna}
\newcommand{\lusearchREWCPNineNestedLocks}{\cna}
\newcommand{\lusearchREWCPTenNestedLocks}{\cna}
\newcommand{\lusearchREWCPHundredNestedLocks}{\cna}
\newcommand{\lusearchFTODCEventTotal}{1,400}
\newcommand{\lusearchFTODCNoFPEventTotal}{140}
\newcommand{\lusearchFTODCNoFPAccessTotal}{130}
\newcommand{\lusearchFTODCNoFPOtherTotal}{3.8}
\newcommand{\lusearchFTODCReadTotal}{77.0}
\newcommand{\lusearchFTODCWriteTotal}{20.2}
\newcommand{\lusearchFTODCNoFPAccessInCS}{4.89}
\newcommand{\lusearchFTODCNoFPAccessOutCS}{95.1}
\newcommand{\lusearchFTODCAcqRelTotal}{6.23}
\newcommand{\lusearchFTODCOtherTotal}{2.72}
\newcommand{\lusearchFTODCNoFPReadTotal}{110}
\newcommand{\lusearchFTODCReadInCS}{3.94}
\newcommand{\lusearchFTODCReadOutCS}{104}
\newcommand{\lusearchFTODCReadSameEp}{7.45}
\newcommand{\lusearchFTODCReadSharedSameEp}{\cna}
\newcommand{\lusearchFTODCReadExclusive}{<0.001}
\newcommand{\lusearchFTODCReadOwned}{96.1}
\newcommand{\lusearchFTODCReadShare}{<0.001}
\newcommand{\lusearchFTODCReadShared}{0.00113}
\newcommand{\lusearchFTODCReadSharedOwned}{3.93}
\newcommand{\lusearchFTODCNoFPHonestWriteTotal}{28}
\newcommand{\lusearchFTODCWriteInCS}{10}
\newcommand{\lusearchFTODCWriteOutCS}{200}
\newcommand{\lusearchFTODCNoFPWriteTotal}{28}
\newcommand{\lusearchFTODCWriteSameEp}{110}
\newcommand{\lusearchFTODCWriteExclusive}{\cna}
\newcommand{\lusearchFTODCWriteOwned}{100}
\newcommand{\lusearchFTODCWriteShared}{<0.001}
\newcommand{\lusearchFTODCNoFPOtherEventTotal}{3816265}
\newcommand{\lusearchFTODCAcqRelOtherTotal}{69.6}
\newcommand{\lusearchFTODCNoAcqRelOtherTotal}{1158329}
\newcommand{\lusearchFTODCFork}{0.00121}
\newcommand{\lusearchFTODCJoin}{0.0}
\newcommand{\lusearchFTODCPreWait}{0.00527}
\newcommand{\lusearchFTODCPostWait}{0.00527}
\newcommand{\lusearchFTODCVolatileTotal}{100.0}
\newcommand{\lusearchFTODCClassInit}{0.00311}
\newcommand{\lusearchFTODCClassAccess}{0.0293}
\newcommand{\lusearchFTODCRaceTotal}{\rna}
\newcommand{\lusearchFTODCWrRdRace}{\rna}
\newcommand{\lusearchFTODCWrWrRace}{\rna}
\newcommand{\lusearchFTODCRdWrRace}{\rna}
\newcommand{\lusearchFTODCRdShWrRace}{\rna}
\newcommand{\lusearchFTODCHoldLocksTotal}{5.1}
\newcommand{\lusearchFTODCOneLockHeld}{3.79}
\newcommand{\lusearchFTODCTwoNestedLocks}{0.39}
\newcommand{\lusearchFTODCThreeNestedLocks}{<0.1}
\newcommand{\lusearchFTODCFourNestedLocks}{\cna}
\newcommand{\lusearchFTODCFiveNestedLocks}{\cna}
\newcommand{\lusearchFTODCSixNestedLocks}{\cna}
\newcommand{\lusearchFTODCSevenNestedLocks}{\cna}
\newcommand{\lusearchFTODCEightNestedLocks}{\cna}
\newcommand{\lusearchFTODCNineNestedLocks}{\cna}
\newcommand{\lusearchFTODCTenNestedLocks}{\cna}
\newcommand{\lusearchFTODCHundredNestedLocks}{\cna}
\newcommand{\lusearchREDCEventTotal}{1,400}
\newcommand{\lusearchREDCNoFPEventTotal}{140}
\newcommand{\lusearchREDCNoFPAccessTotal}{130}
\newcommand{\lusearchREDCNoFPOtherTotal}{3.8}
\newcommand{\lusearchREDCReadTotal}{77.0}
\newcommand{\lusearchREDCWriteTotal}{20.2}
\newcommand{\lusearchREDCNoFPAccessInCS}{4.89}
\newcommand{\lusearchREDCNoFPAccessOutCS}{95.1}
\newcommand{\lusearchREDCAcqRelTotal}{6.23}
\newcommand{\lusearchREDCOtherTotal}{2.72}
\newcommand{\lusearchREDCNoFPReadTotal}{110}
\newcommand{\lusearchREDCReadInCS}{3.94}
\newcommand{\lusearchREDCReadOutCS}{104}
\newcommand{\lusearchREDCReadSameEp}{7.45}
\newcommand{\lusearchREDCReadSharedSameEp}{\cna}
\newcommand{\lusearchREDCReadExclusive}{<0.001}
\newcommand{\lusearchREDCReadOwned}{96.1}
\newcommand{\lusearchREDCReadShare}{<0.001}
\newcommand{\lusearchREDCReadShared}{0.00113}
\newcommand{\lusearchREDCReadSharedOwned}{3.93}
\newcommand{\lusearchREDCNoFPHonestWriteTotal}{28}
\newcommand{\lusearchREDCWriteInCS}{10}
\newcommand{\lusearchREDCWriteOutCS}{200}
\newcommand{\lusearchREDCNoFPWriteTotal}{28}
\newcommand{\lusearchREDCWriteSameEp}{110}
\newcommand{\lusearchREDCWriteExclusive}{\cna}
\newcommand{\lusearchREDCWriteOwned}{100}
\newcommand{\lusearchREDCWriteShared}{<0.001}
\newcommand{\lusearchREDCNoFPOtherEventTotal}{3816260}
\newcommand{\lusearchREDCAcqRelOtherTotal}{69.6}
\newcommand{\lusearchREDCNoAcqRelOtherTotal}{1158324}
\newcommand{\lusearchREDCFork}{0.00121}
\newcommand{\lusearchREDCJoin}{0.0}
\newcommand{\lusearchREDCPreWait}{0.00544}
\newcommand{\lusearchREDCPostWait}{0.00544}
\newcommand{\lusearchREDCVolatileTotal}{100.0}
\newcommand{\lusearchREDCClassInit}{0.00311}
\newcommand{\lusearchREDCClassAccess}{0.0293}
\newcommand{\lusearchREDCRaceTotal}{\rna}
\newcommand{\lusearchREDCWrRdRace}{\rna}
\newcommand{\lusearchREDCWrWrRace}{\rna}
\newcommand{\lusearchREDCRdWrRace}{\rna}
\newcommand{\lusearchREDCRdShWrRace}{\rna}
\newcommand{\lusearchREDCHoldLocksTotal}{5.1}
\newcommand{\lusearchREDCOneLockHeld}{3.79}
\newcommand{\lusearchREDCTwoNestedLocks}{0.39}
\newcommand{\lusearchREDCThreeNestedLocks}{<0.1}
\newcommand{\lusearchREDCFourNestedLocks}{\cna}
\newcommand{\lusearchREDCFiveNestedLocks}{\cna}
\newcommand{\lusearchREDCSixNestedLocks}{\cna}
\newcommand{\lusearchREDCSevenNestedLocks}{\cna}
\newcommand{\lusearchREDCEightNestedLocks}{\cna}
\newcommand{\lusearchREDCNineNestedLocks}{\cna}
\newcommand{\lusearchREDCTenNestedLocks}{\cna}
\newcommand{\lusearchREDCHundredNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPOEventTotal}{1,400}
\newcommand{\lusearchFTOCAPONoFPEventTotal}{140}
\newcommand{\lusearchFTOCAPONoFPAccessTotal}{130}
\newcommand{\lusearchFTOCAPONoFPOtherTotal}{3.8}
\newcommand{\lusearchFTOCAPOReadTotal}{77.0}
\newcommand{\lusearchFTOCAPOWriteTotal}{20.2}
\newcommand{\lusearchFTOCAPONoFPAccessInCS}{4.89}
\newcommand{\lusearchFTOCAPONoFPAccessOutCS}{95.1}
\newcommand{\lusearchFTOCAPOAcqRelTotal}{6.23}
\newcommand{\lusearchFTOCAPOOtherTotal}{2.72}
\newcommand{\lusearchFTOCAPONoFPReadTotal}{110}
\newcommand{\lusearchFTOCAPOReadInCS}{3.94}
\newcommand{\lusearchFTOCAPOReadOutCS}{104}
\newcommand{\lusearchFTOCAPOReadSameEp}{7.45}
\newcommand{\lusearchFTOCAPOReadSharedSameEp}{\cna}
\newcommand{\lusearchFTOCAPOReadExclusive}{<0.001}
\newcommand{\lusearchFTOCAPOReadOwned}{96.1}
\newcommand{\lusearchFTOCAPOReadShare}{<0.001}
\newcommand{\lusearchFTOCAPOReadShared}{0.00113}
\newcommand{\lusearchFTOCAPOReadSharedOwned}{3.93}
\newcommand{\lusearchFTOCAPONoFPHonestWriteTotal}{28}
\newcommand{\lusearchFTOCAPOWriteInCS}{10}
\newcommand{\lusearchFTOCAPOWriteOutCS}{200}
\newcommand{\lusearchFTOCAPONoFPWriteTotal}{28}
\newcommand{\lusearchFTOCAPOWriteSameEp}{110}
\newcommand{\lusearchFTOCAPOWriteExclusive}{\cna}
\newcommand{\lusearchFTOCAPOWriteOwned}{100}
\newcommand{\lusearchFTOCAPOWriteShared}{<0.001}
\newcommand{\lusearchFTOCAPONoFPOtherEventTotal}{3816323}
\newcommand{\lusearchFTOCAPOAcqRelOtherTotal}{69.6}
\newcommand{\lusearchFTOCAPONoAcqRelOtherTotal}{1158387}
\newcommand{\lusearchFTOCAPOFork}{0.00121}
\newcommand{\lusearchFTOCAPOJoin}{0.0}
\newcommand{\lusearchFTOCAPOPreWait}{0.00509}
\newcommand{\lusearchFTOCAPOPostWait}{0.00509}
\newcommand{\lusearchFTOCAPOVolatileTotal}{100.0}
\newcommand{\lusearchFTOCAPOClassInit}{0.00311}
\newcommand{\lusearchFTOCAPOClassAccess}{0.0293}
\newcommand{\lusearchFTOCAPORaceTotal}{\rna}
\newcommand{\lusearchFTOCAPOWrRdRace}{\rna}
\newcommand{\lusearchFTOCAPOWrWrRace}{\rna}
\newcommand{\lusearchFTOCAPORdWrRace}{\rna}
\newcommand{\lusearchFTOCAPORdShWrRace}{\rna}
\newcommand{\lusearchFTOCAPOHoldLocksTotal}{5.1}
\newcommand{\lusearchFTOCAPOOneLockHeld}{3.79}
\newcommand{\lusearchFTOCAPOTwoNestedLocks}{0.39}
\newcommand{\lusearchFTOCAPOThreeNestedLocks}{<0.1}
\newcommand{\lusearchFTOCAPOFourNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPOSixNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPOEightNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPONineNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPOTenNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\lusearchRECAPOEventTotal}{1,400}
\newcommand{\lusearchRECAPONoFPEventTotal}{140}
\newcommand{\lusearchRECAPONoFPAccessTotal}{130}
\newcommand{\lusearchRECAPONoFPOtherTotal}{3.8}
\newcommand{\lusearchRECAPOReadTotal}{77.0}
\newcommand{\lusearchRECAPOWriteTotal}{20.2}
\newcommand{\lusearchRECAPONoFPAccessInCS}{4.89}
\newcommand{\lusearchRECAPONoFPAccessOutCS}{95.1}
\newcommand{\lusearchRECAPOAcqRelTotal}{6.23}
\newcommand{\lusearchRECAPOOtherTotal}{2.72}
\newcommand{\lusearchRECAPONoFPReadTotal}{110}
\newcommand{\lusearchRECAPOReadInCS}{3.94}
\newcommand{\lusearchRECAPOReadOutCS}{104}
\newcommand{\lusearchRECAPOReadSameEp}{7.45}
\newcommand{\lusearchRECAPOReadSharedSameEp}{\cna}
\newcommand{\lusearchRECAPOReadExclusive}{<0.001}
\newcommand{\lusearchRECAPOReadOwned}{96.1}
\newcommand{\lusearchRECAPOReadShare}{<0.001}
\newcommand{\lusearchRECAPOReadShared}{0.00113}
\newcommand{\lusearchRECAPOReadSharedOwned}{3.93}
\newcommand{\lusearchRECAPONoFPHonestWriteTotal}{28}
\newcommand{\lusearchRECAPOWriteInCS}{10}
\newcommand{\lusearchRECAPOWriteOutCS}{200}
\newcommand{\lusearchRECAPONoFPWriteTotal}{28}
\newcommand{\lusearchRECAPOWriteSameEp}{110}
\newcommand{\lusearchRECAPOWriteExclusive}{\cna}
\newcommand{\lusearchRECAPOWriteOwned}{100}
\newcommand{\lusearchRECAPOWriteShared}{<0.001}
\newcommand{\lusearchRECAPONoFPOtherEventTotal}{3816288}
\newcommand{\lusearchRECAPOAcqRelOtherTotal}{69.6}
\newcommand{\lusearchRECAPONoAcqRelOtherTotal}{1158352}
\newcommand{\lusearchRECAPOFork}{0.00121}
\newcommand{\lusearchRECAPOJoin}{0.0}
\newcommand{\lusearchRECAPOPreWait}{0.00518}
\newcommand{\lusearchRECAPOPostWait}{0.00518}
\newcommand{\lusearchRECAPOVolatileTotal}{100.0}
\newcommand{\lusearchRECAPOClassInit}{0.00311}
\newcommand{\lusearchRECAPOClassAccess}{0.0293}
\newcommand{\lusearchRECAPORaceTotal}{\rna}
\newcommand{\lusearchRECAPOWrRdRace}{\rna}
\newcommand{\lusearchRECAPOWrWrRace}{\rna}
\newcommand{\lusearchRECAPORdWrRace}{\rna}
\newcommand{\lusearchRECAPORdShWrRace}{\rna}
\newcommand{\lusearchRECAPOHoldLocksTotal}{5.1}
\newcommand{\lusearchRECAPOOneLockHeld}{3.79}
\newcommand{\lusearchRECAPOTwoNestedLocks}{0.39}
\newcommand{\lusearchRECAPOThreeNestedLocks}{<0.1}
\newcommand{\lusearchRECAPOFourNestedLocks}{\cna}
\newcommand{\lusearchRECAPOFiveNestedLocks}{\cna}
\newcommand{\lusearchRECAPOSixNestedLocks}{\cna}
\newcommand{\lusearchRECAPOSevenNestedLocks}{\cna}
\newcommand{\lusearchRECAPOEightNestedLocks}{\cna}
\newcommand{\lusearchRECAPONineNestedLocks}{\cna}
\newcommand{\lusearchRECAPOTenNestedLocks}{\cna}
\newcommand{\lusearchRECAPOHundredNestedLocks}{\cna}
\newcommand{\FASTlusearchMaxLiveThreads}{16}
\newcommand{\FASTlusearchTotalThreads}{16}
\newcommand{\FASTlusearchBaseTime}{0.96}
\newcommand{\FASTlusearchBaseTimeCI}{47}
\newcommand{\FASTlusearchEmptyTime}{\rna}
\newcommand{\FASTlusearchEmptyTimeCI}{\rna}
\newcommand{\FASTlusearchEmptyTimeCIMIN}{\rna}
\newcommand{\FASTlusearchEmptyTimeCIMAX}{\rna}
\newcommand{\FASTlusearchFTTime}{11}
\newcommand{\FASTlusearchFTTimeCI}{0.68}
\newcommand{\FASTlusearchHBTime}{12}
\newcommand{\FASTlusearchHBTimeCI}{0.71}
\newcommand{\FASTlusearchFTOHBTime}{12}
\newcommand{\FASTlusearchFTOHBTimeCI}{0.81}
\newcommand{\FASTlusearchWCPTime}{\rna}
\newcommand{\FASTlusearchWCPTimeCI}{\rna}
\newcommand{\FASTlusearchWCPTimeCIMIN}{\rna}
\newcommand{\FASTlusearchWCPTimeCIMAX}{\rna}
\newcommand{\FASTlusearchFTOWCPTime}{14}
\newcommand{\FASTlusearchFTOWCPTimeCI}{0.85}
\newcommand{\FASTlusearchREWCPTime}{14}
\newcommand{\FASTlusearchREWCPTimeCI}{1.2}
\newcommand{\FASTlusearchDCTime}{\rna}
\newcommand{\FASTlusearchDCTimeCI}{\rna}
\newcommand{\FASTlusearchDCTimeCIMIN}{\rna}
\newcommand{\FASTlusearchDCTimeCIMAX}{\rna}
\newcommand{\FASTlusearchFTODCTime}{15}
\newcommand{\FASTlusearchFTODCTimeCI}{0.87}
\newcommand{\FASTlusearchREDCTime}{14}
\newcommand{\FASTlusearchREDCTimeCI}{0.74}
\newcommand{\FASTlusearchCAPOTime}{\rna}
\newcommand{\FASTlusearchCAPOTimeCI}{\rna}
\newcommand{\FASTlusearchCAPOTimeCIMIN}{\rna}
\newcommand{\FASTlusearchCAPOTimeCIMAX}{\rna}
\newcommand{\FASTlusearchFTOCAPOTime}{13}
\newcommand{\FASTlusearchFTOCAPOTimeCI}{0.73}
\newcommand{\FASTlusearchRECAPOTime}{13}
\newcommand{\FASTlusearchRECAPOTimeCI}{1.2}
\newcommand{\FASTlusearchAGGCAPOTime}{\rna}
\newcommand{\FASTlusearchAGGCAPOTimeCI}{\rna}
\newcommand{\FASTlusearchAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTlusearchAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTlusearchStaticTime}{\rzero}
\newcommand{\FASTlusearchDynamicTime}{\rzero}
\newcommand{\FASTlusearchBaseMem}{1,600}
\newcommand{\FASTlusearchBaseMemCI}{90.0}
\newcommand{\FASTlusearchFTMem}{8.9}
\newcommand{\FASTlusearchFTMemCI}{0.71}
\newcommand{\FASTlusearchHBMem}{8.9}
\newcommand{\FASTlusearchHBMemCI}{0.72}
\newcommand{\FASTlusearchFTOHBMem}{8.9}
\newcommand{\FASTlusearchFTOHBMemCI}{0.89}
\newcommand{\FASTlusearchWCPMem}{\memna}
\newcommand{\FASTlusearchWCPMemCI}{\memna}
\newcommand{\FASTlusearchWCPMemCIMIN}{\memna}
\newcommand{\FASTlusearchWCPMemCIMAX}{\memna}
\newcommand{\FASTlusearchFTOWCPMem}{10}
\newcommand{\FASTlusearchFTOWCPMemCI}{0.92}
\newcommand{\FASTlusearchREWCPMem}{10}
\newcommand{\FASTlusearchREWCPMemCI}{0.73}
\newcommand{\FASTlusearchDCMem}{\memna}
\newcommand{\FASTlusearchDCMemCI}{\memna}
\newcommand{\FASTlusearchDCMemCIMIN}{\memna}
\newcommand{\FASTlusearchDCMemCIMAX}{\memna}
\newcommand{\FASTlusearchFTODCMem}{10}
\newcommand{\FASTlusearchFTODCMemCI}{0.83}
\newcommand{\FASTlusearchREDCMem}{11}
\newcommand{\FASTlusearchREDCMemCI}{0.86}
\newcommand{\FASTlusearchCAPOMem}{\memna}
\newcommand{\FASTlusearchCAPOMemCI}{\memna}
\newcommand{\FASTlusearchCAPOMemCIMIN}{\memna}
\newcommand{\FASTlusearchCAPOMemCIMAX}{\memna}
\newcommand{\FASTlusearchFTOCAPOMem}{9.6}
\newcommand{\FASTlusearchFTOCAPOMemCI}{0.86}
\newcommand{\FASTlusearchRECAPOMem}{9.6}
\newcommand{\FASTlusearchRECAPOMemCI}{0.81}
\newcommand{\FASTlusearchAGGCAPOMem}{\memna}
\newcommand{\FASTlusearchAGGCAPOMemCI}{\memna}
\newcommand{\FASTlusearchAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTlusearchAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTlusearchEventsCI}{13}
\newcommand{\FASTlusearchEventsCIMIN}{1,443,227,412}
\newcommand{\FASTlusearchEventsCIMAX}{1,443,227,438}
\newcommand{\FASTlusearchNoFPEventsCI}{14}
\newcommand{\FASTlusearchNoFPEventsCIMIN}{42,639,899}
\newcommand{\FASTlusearchNoFPEventsCIMAX}{42,639,927}
\newcommand{\FASTlusearchFT}{0}
\newcommand{\FASTlusearchFTCI}{0.0}
\newcommand{\FASTlusearchFTCIMIN}{0}
\newcommand{\FASTlusearchFTCIMAX}{0}
\newcommand{\FASTlusearchFTDynamic}{0}
\newcommand{\FASTlusearchFTDynamicCI}{0.0}
\newcommand{\FASTlusearchFTDynamicCIMIN}{0}
\newcommand{\FASTlusearchFTDynamicCIMAX}{0}
\newcommand{\FASTlusearchHB}{0}
\newcommand{\FASTlusearchHBCI}{0.0}
\newcommand{\FASTlusearchHBCIMIN}{0}
\newcommand{\FASTlusearchHBCIMAX}{0}
\newcommand{\FASTlusearchHBDynamic}{0}
\newcommand{\FASTlusearchHBDynamicCI}{0.0}
\newcommand{\FASTlusearchHBDynamicCIMIN}{0}
\newcommand{\FASTlusearchHBDynamicCIMAX}{0}
\newcommand{\FASTlusearchFTOHB}{0}
\newcommand{\FASTlusearchFTOHBCI}{0.0}
\newcommand{\FASTlusearchFTOHBCIMIN}{0}
\newcommand{\FASTlusearchFTOHBCIMAX}{0}
\newcommand{\FASTlusearchFTOHBDynamic}{0}
\newcommand{\FASTlusearchFTOHBDynamicCI}{0.0}
\newcommand{\FASTlusearchFTOHBDynamicCIMIN}{0}
\newcommand{\FASTlusearchFTOHBDynamicCIMAX}{0}
\newcommand{\FASTlusearchWCP}{\rna}
\newcommand{\FASTlusearchWCPCI}{\rna}
\newcommand{\FASTlusearchWCPCIMIN}{\rna}
\newcommand{\FASTlusearchWCPCIMAX}{\rna}
\newcommand{\FASTlusearchWCPDynamic}{\rna}
\newcommand{\FASTlusearchWCPDynamicCI}{\rna}
\newcommand{\FASTlusearchWCPDynamicCIMIN}{\rna}
\newcommand{\FASTlusearchWCPDynamicCIMAX}{\rna}
\newcommand{\FASTlusearchFTOWCP}{0}
\newcommand{\FASTlusearchFTOWCPCI}{0.0}
\newcommand{\FASTlusearchFTOWCPCIMIN}{0}
\newcommand{\FASTlusearchFTOWCPCIMAX}{0}
\newcommand{\FASTlusearchFTOWCPDynamic}{0}
\newcommand{\FASTlusearchFTOWCPDynamicCI}{0.0}
\newcommand{\FASTlusearchFTOWCPDynamicCIMIN}{0}
\newcommand{\FASTlusearchFTOWCPDynamicCIMAX}{0}
\newcommand{\FASTlusearchREWCP}{0}
\newcommand{\FASTlusearchREWCPCI}{0.0}
\newcommand{\FASTlusearchREWCPCIMIN}{0}
\newcommand{\FASTlusearchREWCPCIMAX}{0}
\newcommand{\FASTlusearchREWCPDynamic}{0}
\newcommand{\FASTlusearchREWCPDynamicCI}{0.0}
\newcommand{\FASTlusearchREWCPDynamicCIMIN}{0}
\newcommand{\FASTlusearchREWCPDynamicCIMAX}{0}
\newcommand{\FASTlusearchDC}{\rna}
\newcommand{\FASTlusearchDCCI}{\rna}
\newcommand{\FASTlusearchDCCIMIN}{\rna}
\newcommand{\FASTlusearchDCCIMAX}{\rna}
\newcommand{\FASTlusearchDCDynamic}{\rna}
\newcommand{\FASTlusearchDCDynamicCI}{\rna}
\newcommand{\FASTlusearchDCDynamicCIMIN}{\rna}
\newcommand{\FASTlusearchDCDynamicCIMAX}{\rna}
\newcommand{\FASTlusearchFTODC}{0}
\newcommand{\FASTlusearchFTODCCI}{0.0}
\newcommand{\FASTlusearchFTODCCIMIN}{0}
\newcommand{\FASTlusearchFTODCCIMAX}{0}
\newcommand{\FASTlusearchFTODCDynamic}{0}
\newcommand{\FASTlusearchFTODCDynamicCI}{0.0}
\newcommand{\FASTlusearchFTODCDynamicCIMIN}{0}
\newcommand{\FASTlusearchFTODCDynamicCIMAX}{0}
\newcommand{\FASTlusearchREDC}{0}
\newcommand{\FASTlusearchREDCCI}{0.0}
\newcommand{\FASTlusearchREDCCIMIN}{0}
\newcommand{\FASTlusearchREDCCIMAX}{0}
\newcommand{\FASTlusearchREDCDynamic}{0}
\newcommand{\FASTlusearchREDCDynamicCI}{0.0}
\newcommand{\FASTlusearchREDCDynamicCIMIN}{0}
\newcommand{\FASTlusearchREDCDynamicCIMAX}{0}
\newcommand{\FASTlusearchCAPO}{\rna}
\newcommand{\FASTlusearchCAPOCI}{\rna}
\newcommand{\FASTlusearchCAPOCIMIN}{\rna}
\newcommand{\FASTlusearchCAPOCIMAX}{\rna}
\newcommand{\FASTlusearchCAPODynamic}{\rna}
\newcommand{\FASTlusearchCAPODynamicCI}{\rna}
\newcommand{\FASTlusearchCAPODynamicCIMIN}{\rna}
\newcommand{\FASTlusearchCAPODynamicCIMAX}{\rna}
\newcommand{\FASTlusearchFTOCAPO}{0}
\newcommand{\FASTlusearchFTOCAPOCI}{0.0}
\newcommand{\FASTlusearchFTOCAPOCIMIN}{0}
\newcommand{\FASTlusearchFTOCAPOCIMAX}{0}
\newcommand{\FASTlusearchFTOCAPODynamic}{0}
\newcommand{\FASTlusearchFTOCAPODynamicCI}{0.0}
\newcommand{\FASTlusearchFTOCAPODynamicCIMIN}{0}
\newcommand{\FASTlusearchFTOCAPODynamicCIMAX}{0}
\newcommand{\FASTlusearchRECAPO}{0}
\newcommand{\FASTlusearchRECAPOCI}{0.0}
\newcommand{\FASTlusearchRECAPOCIMIN}{0}
\newcommand{\FASTlusearchRECAPOCIMAX}{0}
\newcommand{\FASTlusearchRECAPODynamic}{0}
\newcommand{\FASTlusearchRECAPODynamicCI}{0.0}
\newcommand{\FASTlusearchRECAPODynamicCIMIN}{0}
\newcommand{\FASTlusearchRECAPODynamicCIMAX}{0}
\newcommand{\FASTlusearchAGGCAPO}{\rna}
\newcommand{\FASTlusearchAGGCAPOCI}{\rna}
\newcommand{\FASTlusearchAGGCAPOCIMIN}{\rna}
\newcommand{\FASTlusearchAGGCAPOCIMAX}{\rna}
\newcommand{\FASTlusearchAGGCAPODynamic}{\rna}
\newcommand{\FASTlusearchAGGCAPODynamicCI}{\rna}
\newcommand{\FASTlusearchAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTlusearchAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTpmdEvents}{210}
\newcommand{\FASTpmdNoFPEvents}{13}
\newcommand{\pmdHBEventTotal}{210}
\newcommand{\pmdHBNoFPEventTotal}{13}
\newcommand{\pmdHBNoFPAccessTotal}{13}
\newcommand{\pmdHBNoFPOtherTotal}{<0.1}
\newcommand{\pmdHBReadTotal}{95.6}
\newcommand{\pmdHBWriteTotal}{4.27}
\newcommand{\pmdHBNoFPAccessInCS}{10.3}
\newcommand{\pmdHBNoFPAccessOutCS}{89.7}
\newcommand{\pmdHBAcqRelTotal}{0.134}
\newcommand{\pmdHBOtherTotal}{0.00553}
\newcommand{\pmdHBNoFPReadTotal}{12}
\newcommand{\pmdHBReadInCS}{11}
\newcommand{\pmdHBReadOutCS}{110}
\newcommand{\pmdHBReadSameEp}{21.2}
\newcommand{\pmdHBReadSharedSameEp}{\cna}
\newcommand{\pmdHBReadExclusive}{99}
\newcommand{\pmdHBReadOwned}{\cna}
\newcommand{\pmdHBReadShare}{0.0163}
\newcommand{\pmdHBReadShared}{0.949}
\newcommand{\pmdHBReadSharedOwned}{\cna}
\newcommand{\pmdHBNoFPHonestWriteTotal}{0.54}
\newcommand{\pmdHBWriteInCS}{26.4}
\newcommand{\pmdHBWriteOutCS}{2000}
\newcommand{\pmdHBNoFPWriteTotal}{0.54}
\newcommand{\pmdHBWriteSameEp}{1930}
\newcommand{\pmdHBWriteExclusive}{100}
\newcommand{\pmdHBWriteOwned}{\cna}
\newcommand{\pmdHBWriteShared}{<0.001}
\newcommand{\pmdHBNoFPOtherEventTotal}{18326}
\newcommand{\pmdHBAcqRelOtherTotal}{96.0}
\newcommand{\pmdHBNoAcqRelOtherTotal}{724}
\newcommand{\pmdHBFork}{0.0}
\newcommand{\pmdHBJoin}{0.0}
\newcommand{\pmdHBPreWait}{0.0}
\newcommand{\pmdHBPostWait}{0.0}
\newcommand{\pmdHBVolatileTotal}{0.0}
\newcommand{\pmdHBClassInit}{7.87}
\newcommand{\pmdHBClassAccess}{92.1}
\newcommand{\pmdHBRaceTotal}{1802}
\newcommand{\pmdHBWrRdRace}{99.1}
\newcommand{\pmdHBWrWrRace}{0.832}
\newcommand{\pmdHBRdWrRace}{0.0}
\newcommand{\pmdHBRdShWrRace}{0.0555}
\newcommand{\pmdHBHoldLocksTotal}{1.5}
\newcommand{\pmdHBOneLockHeld}{11.6}
\newcommand{\pmdHBTwoNestedLocks}{\cna}
\newcommand{\pmdHBThreeNestedLocks}{\cna}
\newcommand{\pmdHBFourNestedLocks}{\cna}
\newcommand{\pmdHBFiveNestedLocks}{\cna}
\newcommand{\pmdHBSixNestedLocks}{\cna}
\newcommand{\pmdHBSevenNestedLocks}{\cna}
\newcommand{\pmdHBEightNestedLocks}{\cna}
\newcommand{\pmdHBNineNestedLocks}{\cna}
\newcommand{\pmdHBTenNestedLocks}{\cna}
\newcommand{\pmdHBHundredNestedLocks}{\cna}
\newcommand{\pmdFTOHBEventTotal}{210}
\newcommand{\pmdFTOHBNoFPEventTotal}{8.0}
\newcommand{\pmdFTOHBNoFPAccessTotal}{7.9}
\newcommand{\pmdFTOHBNoFPOtherTotal}{<0.1}
\newcommand{\pmdFTOHBReadTotal}{92.9}
\newcommand{\pmdFTOHBWriteTotal}{6.85}
\newcommand{\pmdFTOHBNoFPAccessInCS}{10.3}
\newcommand{\pmdFTOHBNoFPAccessOutCS}{89.7}
\newcommand{\pmdFTOHBAcqRelTotal}{0.134}
\newcommand{\pmdFTOHBOtherTotal}{0.0055}
\newcommand{\pmdFTOHBNoFPReadTotal}{7.4}
\newcommand{\pmdFTOHBReadInCS}{17.5}
\newcommand{\pmdFTOHBReadOutCS}{117}
\newcommand{\pmdFTOHBReadSameEp}{34.9}
\newcommand{\pmdFTOHBReadSharedSameEp}{\cna}
\newcommand{\pmdFTOHBReadExclusive}{0.3}
\newcommand{\pmdFTOHBReadOwned}{98.1}
\newcommand{\pmdFTOHBReadShare}{0.0336}
\newcommand{\pmdFTOHBReadShared}{0.145}
\newcommand{\pmdFTOHBReadSharedOwned}{1.43}
\newcommand{\pmdFTOHBNoFPHonestWriteTotal}{0.54}
\newcommand{\pmdFTOHBWriteInCS}{26.4}
\newcommand{\pmdFTOHBWriteOutCS}{2000}
\newcommand{\pmdFTOHBNoFPWriteTotal}{0.54}
\newcommand{\pmdFTOHBWriteSameEp}{1930}
\newcommand{\pmdFTOHBWriteExclusive}{0.00275}
\newcommand{\pmdFTOHBWriteOwned}{100}
\newcommand{\pmdFTOHBWriteShared}{<0.001}
\newcommand{\pmdFTOHBNoFPOtherEventTotal}{18323}
\newcommand{\pmdFTOHBAcqRelOtherTotal}{96.1}
\newcommand{\pmdFTOHBNoAcqRelOtherTotal}{721}
\newcommand{\pmdFTOHBFork}{0.0}
\newcommand{\pmdFTOHBJoin}{0.0}
\newcommand{\pmdFTOHBPreWait}{0.0}
\newcommand{\pmdFTOHBPostWait}{0.0}
\newcommand{\pmdFTOHBVolatileTotal}{0.0}
\newcommand{\pmdFTOHBClassInit}{7.91}
\newcommand{\pmdFTOHBClassAccess}{92.1}
\newcommand{\pmdFTOHBRaceTotal}{1765}
\newcommand{\pmdFTOHBWrRdRace}{99.0}
\newcommand{\pmdFTOHBWrWrRace}{0.0}
\newcommand{\pmdFTOHBRdWrRace}{0.85}
\newcommand{\pmdFTOHBRdShWrRace}{0.113}
\newcommand{\pmdFTOHBHoldLocksTotal}{0.093}
\newcommand{\pmdFTOHBOneLockHeld}{1.14}
\newcommand{\pmdFTOHBTwoNestedLocks}{\cna}
\newcommand{\pmdFTOHBThreeNestedLocks}{\cna}
\newcommand{\pmdFTOHBFourNestedLocks}{\cna}
\newcommand{\pmdFTOHBFiveNestedLocks}{\cna}
\newcommand{\pmdFTOHBSixNestedLocks}{\cna}
\newcommand{\pmdFTOHBSevenNestedLocks}{\cna}
\newcommand{\pmdFTOHBEightNestedLocks}{\cna}
\newcommand{\pmdFTOHBNineNestedLocks}{\cna}
\newcommand{\pmdFTOHBTenNestedLocks}{\cna}
\newcommand{\pmdFTOHBHundredNestedLocks}{\cna}
\newcommand{\pmdFTOWCPEventTotal}{210}
\newcommand{\pmdFTOWCPNoFPEventTotal}{8.0}
\newcommand{\pmdFTOWCPNoFPAccessTotal}{7.9}
\newcommand{\pmdFTOWCPNoFPOtherTotal}{<0.1}
\newcommand{\pmdFTOWCPReadTotal}{92.9}
\newcommand{\pmdFTOWCPWriteTotal}{6.85}
\newcommand{\pmdFTOWCPNoFPAccessInCS}{10.3}
\newcommand{\pmdFTOWCPNoFPAccessOutCS}{89.7}
\newcommand{\pmdFTOWCPAcqRelTotal}{0.134}
\newcommand{\pmdFTOWCPOtherTotal}{0.00552}
\newcommand{\pmdFTOWCPNoFPReadTotal}{7.4}
\newcommand{\pmdFTOWCPReadInCS}{17.5}
\newcommand{\pmdFTOWCPReadOutCS}{117}
\newcommand{\pmdFTOWCPReadSameEp}{34.9}
\newcommand{\pmdFTOWCPReadSharedSameEp}{\cna}
\newcommand{\pmdFTOWCPReadExclusive}{0.255}
\newcommand{\pmdFTOWCPReadOwned}{98}
\newcommand{\pmdFTOWCPReadShare}{0.0343}
\newcommand{\pmdFTOWCPReadShared}{0.146}
\newcommand{\pmdFTOWCPReadSharedOwned}{1.55}
\newcommand{\pmdFTOWCPNoFPHonestWriteTotal}{0.54}
\newcommand{\pmdFTOWCPWriteInCS}{26.4}
\newcommand{\pmdFTOWCPWriteOutCS}{2000}
\newcommand{\pmdFTOWCPNoFPWriteTotal}{0.54}
\newcommand{\pmdFTOWCPWriteSameEp}{1930}
\newcommand{\pmdFTOWCPWriteExclusive}{0.00276}
\newcommand{\pmdFTOWCPWriteOwned}{100}
\newcommand{\pmdFTOWCPWriteShared}{<0.001}
\newcommand{\pmdFTOWCPNoFPOtherEventTotal}{18325}
\newcommand{\pmdFTOWCPAcqRelOtherTotal}{96.1}
\newcommand{\pmdFTOWCPNoAcqRelOtherTotal}{723}
\newcommand{\pmdFTOWCPFork}{0.0}
\newcommand{\pmdFTOWCPJoin}{0.0}
\newcommand{\pmdFTOWCPPreWait}{0.0}
\newcommand{\pmdFTOWCPPostWait}{0.0}
\newcommand{\pmdFTOWCPVolatileTotal}{0.0}
\newcommand{\pmdFTOWCPClassInit}{7.88}
\newcommand{\pmdFTOWCPClassAccess}{92.1}
\newcommand{\pmdFTOWCPRaceTotal}{1823}
\newcommand{\pmdFTOWCPWrRdRace}{99.1}
\newcommand{\pmdFTOWCPWrWrRace}{0.0}
\newcommand{\pmdFTOWCPRdWrRace}{0.823}
\newcommand{\pmdFTOWCPRdShWrRace}{0.0549}
\newcommand{\pmdFTOWCPHoldLocksTotal}{0.093}
\newcommand{\pmdFTOWCPOneLockHeld}{1.14}
\newcommand{\pmdFTOWCPTwoNestedLocks}{\cna}
\newcommand{\pmdFTOWCPThreeNestedLocks}{\cna}
\newcommand{\pmdFTOWCPFourNestedLocks}{\cna}
\newcommand{\pmdFTOWCPFiveNestedLocks}{\cna}
\newcommand{\pmdFTOWCPSixNestedLocks}{\cna}
\newcommand{\pmdFTOWCPSevenNestedLocks}{\cna}
\newcommand{\pmdFTOWCPEightNestedLocks}{\cna}
\newcommand{\pmdFTOWCPNineNestedLocks}{\cna}
\newcommand{\pmdFTOWCPTenNestedLocks}{\cna}
\newcommand{\pmdFTOWCPHundredNestedLocks}{\cna}
\newcommand{\pmdREWCPEventTotal}{210}
\newcommand{\pmdREWCPNoFPEventTotal}{8.0}
\newcommand{\pmdREWCPNoFPAccessTotal}{7.9}
\newcommand{\pmdREWCPNoFPOtherTotal}{<0.1}
\newcommand{\pmdREWCPReadTotal}{92.9}
\newcommand{\pmdREWCPWriteTotal}{6.85}
\newcommand{\pmdREWCPNoFPAccessInCS}{10.3}
\newcommand{\pmdREWCPNoFPAccessOutCS}{89.7}
\newcommand{\pmdREWCPAcqRelTotal}{0.134}
\newcommand{\pmdREWCPOtherTotal}{0.00553}
\newcommand{\pmdREWCPNoFPReadTotal}{7.4}
\newcommand{\pmdREWCPReadInCS}{17.5}
\newcommand{\pmdREWCPReadOutCS}{117}
\newcommand{\pmdREWCPReadSameEp}{34.9}
\newcommand{\pmdREWCPReadSharedSameEp}{\cna}
\newcommand{\pmdREWCPReadExclusive}{0.222}
\newcommand{\pmdREWCPReadOwned}{98}
\newcommand{\pmdREWCPReadShare}{0.0662}
\newcommand{\pmdREWCPReadShared}{0.147}
\newcommand{\pmdREWCPReadSharedOwned}{1.55}
\newcommand{\pmdREWCPNoFPHonestWriteTotal}{0.54}
\newcommand{\pmdREWCPWriteInCS}{26.4}
\newcommand{\pmdREWCPWriteOutCS}{2000}
\newcommand{\pmdREWCPNoFPWriteTotal}{0.54}
\newcommand{\pmdREWCPWriteSameEp}{1930}
\newcommand{\pmdREWCPWriteExclusive}{0.00257}
\newcommand{\pmdREWCPWriteOwned}{99.6}
\newcommand{\pmdREWCPWriteShared}{0.441}
\newcommand{\pmdREWCPNoFPOtherEventTotal}{18326}
\newcommand{\pmdREWCPAcqRelOtherTotal}{96.0}
\newcommand{\pmdREWCPNoAcqRelOtherTotal}{724}
\newcommand{\pmdREWCPFork}{0.0}
\newcommand{\pmdREWCPJoin}{0.0}
\newcommand{\pmdREWCPPreWait}{0.0}
\newcommand{\pmdREWCPPostWait}{0.0}
\newcommand{\pmdREWCPVolatileTotal}{0.0}
\newcommand{\pmdREWCPClassInit}{7.87}
\newcommand{\pmdREWCPClassAccess}{92.1}
\newcommand{\pmdREWCPRaceTotal}{1750}
\newcommand{\pmdREWCPWrRdRace}{99.1}
\newcommand{\pmdREWCPWrWrRace}{0.0}
\newcommand{\pmdREWCPRdWrRace}{0.8}
\newcommand{\pmdREWCPRdShWrRace}{0.0571}
\newcommand{\pmdREWCPHoldLocksTotal}{0.093}
\newcommand{\pmdREWCPOneLockHeld}{1.14}
\newcommand{\pmdREWCPTwoNestedLocks}{\cna}
\newcommand{\pmdREWCPThreeNestedLocks}{\cna}
\newcommand{\pmdREWCPFourNestedLocks}{\cna}
\newcommand{\pmdREWCPFiveNestedLocks}{\cna}
\newcommand{\pmdREWCPSixNestedLocks}{\cna}
\newcommand{\pmdREWCPSevenNestedLocks}{\cna}
\newcommand{\pmdREWCPEightNestedLocks}{\cna}
\newcommand{\pmdREWCPNineNestedLocks}{\cna}
\newcommand{\pmdREWCPTenNestedLocks}{\cna}
\newcommand{\pmdREWCPHundredNestedLocks}{\cna}
\newcommand{\pmdFTODCEventTotal}{210}
\newcommand{\pmdFTODCNoFPEventTotal}{8.0}
\newcommand{\pmdFTODCNoFPAccessTotal}{7.9}
\newcommand{\pmdFTODCNoFPOtherTotal}{<0.1}
\newcommand{\pmdFTODCReadTotal}{92.9}
\newcommand{\pmdFTODCWriteTotal}{6.84}
\newcommand{\pmdFTODCNoFPAccessInCS}{10.3}
\newcommand{\pmdFTODCNoFPAccessOutCS}{89.7}
\newcommand{\pmdFTODCAcqRelTotal}{0.134}
\newcommand{\pmdFTODCOtherTotal}{0.00553}
\newcommand{\pmdFTODCNoFPReadTotal}{7.4}
\newcommand{\pmdFTODCReadInCS}{17.5}
\newcommand{\pmdFTODCReadOutCS}{117}
\newcommand{\pmdFTODCReadSameEp}{34.9}
\newcommand{\pmdFTODCReadSharedSameEp}{\cna}
\newcommand{\pmdFTODCReadExclusive}{0.229}
\newcommand{\pmdFTODCReadOwned}{98}
\newcommand{\pmdFTODCReadShare}{0.053}
\newcommand{\pmdFTODCReadShared}{0.149}
\newcommand{\pmdFTODCReadSharedOwned}{1.56}
\newcommand{\pmdFTODCNoFPHonestWriteTotal}{0.54}
\newcommand{\pmdFTODCWriteInCS}{26.4}
\newcommand{\pmdFTODCWriteOutCS}{2000}
\newcommand{\pmdFTODCNoFPWriteTotal}{0.54}
\newcommand{\pmdFTODCWriteSameEp}{1930}
\newcommand{\pmdFTODCWriteExclusive}{0.00257}
\newcommand{\pmdFTODCWriteOwned}{100}
\newcommand{\pmdFTODCWriteShared}{<0.001}
\newcommand{\pmdFTODCNoFPOtherEventTotal}{18326}
\newcommand{\pmdFTODCAcqRelOtherTotal}{96.0}
\newcommand{\pmdFTODCNoAcqRelOtherTotal}{724}
\newcommand{\pmdFTODCFork}{0.0}
\newcommand{\pmdFTODCJoin}{0.0}
\newcommand{\pmdFTODCPreWait}{0.0}
\newcommand{\pmdFTODCPostWait}{0.0}
\newcommand{\pmdFTODCVolatileTotal}{0.0}
\newcommand{\pmdFTODCClassInit}{7.87}
\newcommand{\pmdFTODCClassAccess}{92.1}
\newcommand{\pmdFTODCRaceTotal}{3660}
\newcommand{\pmdFTODCWrRdRace}{99.6}
\newcommand{\pmdFTODCWrWrRace}{0.0}
\newcommand{\pmdFTODCRdWrRace}{0.383}
\newcommand{\pmdFTODCRdShWrRace}{0.0273}
\newcommand{\pmdFTODCHoldLocksTotal}{0.093}
\newcommand{\pmdFTODCOneLockHeld}{1.12}
\newcommand{\pmdFTODCTwoNestedLocks}{\cna}
\newcommand{\pmdFTODCThreeNestedLocks}{\cna}
\newcommand{\pmdFTODCFourNestedLocks}{\cna}
\newcommand{\pmdFTODCFiveNestedLocks}{\cna}
\newcommand{\pmdFTODCSixNestedLocks}{\cna}
\newcommand{\pmdFTODCSevenNestedLocks}{\cna}
\newcommand{\pmdFTODCEightNestedLocks}{\cna}
\newcommand{\pmdFTODCNineNestedLocks}{\cna}
\newcommand{\pmdFTODCTenNestedLocks}{\cna}
\newcommand{\pmdFTODCHundredNestedLocks}{\cna}
\newcommand{\pmdREDCEventTotal}{210}
\newcommand{\pmdREDCNoFPEventTotal}{8.0}
\newcommand{\pmdREDCNoFPAccessTotal}{7.9}
\newcommand{\pmdREDCNoFPOtherTotal}{<0.1}
\newcommand{\pmdREDCReadTotal}{92.9}
\newcommand{\pmdREDCWriteTotal}{6.85}
\newcommand{\pmdREDCNoFPAccessInCS}{10.3}
\newcommand{\pmdREDCNoFPAccessOutCS}{89.7}
\newcommand{\pmdREDCAcqRelTotal}{0.134}
\newcommand{\pmdREDCOtherTotal}{0.0055}
\newcommand{\pmdREDCNoFPReadTotal}{7.4}
\newcommand{\pmdREDCReadInCS}{17.5}
\newcommand{\pmdREDCReadOutCS}{117}
\newcommand{\pmdREDCReadSameEp}{34.9}
\newcommand{\pmdREDCReadSharedSameEp}{\cna}
\newcommand{\pmdREDCReadExclusive}{0.118}
\newcommand{\pmdREDCReadOwned}{98}
\newcommand{\pmdREDCReadShare}{0.16}
\newcommand{\pmdREDCReadShared}{0.15}
\newcommand{\pmdREDCReadSharedOwned}{1.56}
\newcommand{\pmdREDCNoFPHonestWriteTotal}{0.54}
\newcommand{\pmdREDCWriteInCS}{26.4}
\newcommand{\pmdREDCWriteOutCS}{2000}
\newcommand{\pmdREDCNoFPWriteTotal}{0.54}
\newcommand{\pmdREDCWriteSameEp}{1930}
\newcommand{\pmdREDCWriteExclusive}{0.00257}
\newcommand{\pmdREDCWriteOwned}{98.5}
\newcommand{\pmdREDCWriteShared}{1.47}
\newcommand{\pmdREDCNoFPOtherEventTotal}{18323}
\newcommand{\pmdREDCAcqRelOtherTotal}{96.1}
\newcommand{\pmdREDCNoAcqRelOtherTotal}{721}
\newcommand{\pmdREDCFork}{0.0}
\newcommand{\pmdREDCJoin}{0.0}
\newcommand{\pmdREDCPreWait}{0.0}
\newcommand{\pmdREDCPostWait}{0.0}
\newcommand{\pmdREDCVolatileTotal}{0.0}
\newcommand{\pmdREDCClassInit}{7.91}
\newcommand{\pmdREDCClassAccess}{92.1}
\newcommand{\pmdREDCRaceTotal}{3731}
\newcommand{\pmdREDCWrRdRace}{99.6}
\newcommand{\pmdREDCWrWrRace}{0.0}
\newcommand{\pmdREDCRdWrRace}{0.375}
\newcommand{\pmdREDCRdShWrRace}{0.0268}
\newcommand{\pmdREDCHoldLocksTotal}{0.093}
\newcommand{\pmdREDCOneLockHeld}{1.12}
\newcommand{\pmdREDCTwoNestedLocks}{\cna}
\newcommand{\pmdREDCThreeNestedLocks}{\cna}
\newcommand{\pmdREDCFourNestedLocks}{\cna}
\newcommand{\pmdREDCFiveNestedLocks}{\cna}
\newcommand{\pmdREDCSixNestedLocks}{\cna}
\newcommand{\pmdREDCSevenNestedLocks}{\cna}
\newcommand{\pmdREDCEightNestedLocks}{\cna}
\newcommand{\pmdREDCNineNestedLocks}{\cna}
\newcommand{\pmdREDCTenNestedLocks}{\cna}
\newcommand{\pmdREDCHundredNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOEventTotal}{210}
\newcommand{\pmdFTOCAPONoFPEventTotal}{8.0}
\newcommand{\pmdFTOCAPONoFPAccessTotal}{7.9}
\newcommand{\pmdFTOCAPONoFPOtherTotal}{<0.1}
\newcommand{\pmdFTOCAPOReadTotal}{92.9}
\newcommand{\pmdFTOCAPOWriteTotal}{6.85}
\newcommand{\pmdFTOCAPONoFPAccessInCS}{10.3}
\newcommand{\pmdFTOCAPONoFPAccessOutCS}{89.7}
\newcommand{\pmdFTOCAPOAcqRelTotal}{0.134}
\newcommand{\pmdFTOCAPOOtherTotal}{0.00554}
\newcommand{\pmdFTOCAPONoFPReadTotal}{7.4}
\newcommand{\pmdFTOCAPOReadInCS}{17.5}
\newcommand{\pmdFTOCAPOReadOutCS}{117}
\newcommand{\pmdFTOCAPOReadSameEp}{34.9}
\newcommand{\pmdFTOCAPOReadSharedSameEp}{\cna}
\newcommand{\pmdFTOCAPOReadExclusive}{0.226}
\newcommand{\pmdFTOCAPOReadOwned}{98}
\newcommand{\pmdFTOCAPOReadShare}{0.0533}
\newcommand{\pmdFTOCAPOReadShared}{0.149}
\newcommand{\pmdFTOCAPOReadSharedOwned}{1.56}
\newcommand{\pmdFTOCAPONoFPHonestWriteTotal}{0.54}
\newcommand{\pmdFTOCAPOWriteInCS}{26.4}
\newcommand{\pmdFTOCAPOWriteOutCS}{2000}
\newcommand{\pmdFTOCAPONoFPWriteTotal}{0.54}
\newcommand{\pmdFTOCAPOWriteSameEp}{1930}
\newcommand{\pmdFTOCAPOWriteExclusive}{0.00257}
\newcommand{\pmdFTOCAPOWriteOwned}{100}
\newcommand{\pmdFTOCAPOWriteShared}{<0.001}
\newcommand{\pmdFTOCAPONoFPOtherEventTotal}{18328}
\newcommand{\pmdFTOCAPOAcqRelOtherTotal}{96.0}
\newcommand{\pmdFTOCAPONoAcqRelOtherTotal}{726}
\newcommand{\pmdFTOCAPOFork}{0.0}
\newcommand{\pmdFTOCAPOJoin}{0.0}
\newcommand{\pmdFTOCAPOPreWait}{0.0}
\newcommand{\pmdFTOCAPOPostWait}{0.0}
\newcommand{\pmdFTOCAPOVolatileTotal}{0.0}
\newcommand{\pmdFTOCAPOClassInit}{7.85}
\newcommand{\pmdFTOCAPOClassAccess}{92.1}
\newcommand{\pmdFTOCAPORaceTotal}{3785}
\newcommand{\pmdFTOCAPOWrRdRace}{99.6}
\newcommand{\pmdFTOCAPOWrWrRace}{0.0}
\newcommand{\pmdFTOCAPORdWrRace}{0.37}
\newcommand{\pmdFTOCAPORdShWrRace}{0.0264}
\newcommand{\pmdFTOCAPOHoldLocksTotal}{0.093}
\newcommand{\pmdFTOCAPOOneLockHeld}{1.12}
\newcommand{\pmdFTOCAPOTwoNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOThreeNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOFourNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOSixNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOEightNestedLocks}{\cna}
\newcommand{\pmdFTOCAPONineNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOTenNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\pmdRECAPOEventTotal}{210}
\newcommand{\pmdRECAPONoFPEventTotal}{8.0}
\newcommand{\pmdRECAPONoFPAccessTotal}{7.9}
\newcommand{\pmdRECAPONoFPOtherTotal}{<0.1}
\newcommand{\pmdRECAPOReadTotal}{92.9}
\newcommand{\pmdRECAPOWriteTotal}{6.85}
\newcommand{\pmdRECAPONoFPAccessInCS}{10.3}
\newcommand{\pmdRECAPONoFPAccessOutCS}{89.7}
\newcommand{\pmdRECAPOAcqRelTotal}{0.134}
\newcommand{\pmdRECAPOOtherTotal}{0.00549}
\newcommand{\pmdRECAPONoFPReadTotal}{7.4}
\newcommand{\pmdRECAPOReadInCS}{17.5}
\newcommand{\pmdRECAPOReadOutCS}{117}
\newcommand{\pmdRECAPOReadSameEp}{34.9}
\newcommand{\pmdRECAPOReadSharedSameEp}{\cna}
\newcommand{\pmdRECAPOReadExclusive}{0.118}
\newcommand{\pmdRECAPOReadOwned}{98}
\newcommand{\pmdRECAPOReadShare}{0.16}
\newcommand{\pmdRECAPOReadShared}{0.151}
\newcommand{\pmdRECAPOReadSharedOwned}{1.56}
\newcommand{\pmdRECAPONoFPHonestWriteTotal}{0.54}
\newcommand{\pmdRECAPOWriteInCS}{26.4}
\newcommand{\pmdRECAPOWriteOutCS}{2000}
\newcommand{\pmdRECAPONoFPWriteTotal}{0.54}
\newcommand{\pmdRECAPOWriteSameEp}{1930}
\newcommand{\pmdRECAPOWriteExclusive}{0.00275}
\newcommand{\pmdRECAPOWriteOwned}{98.5}
\newcommand{\pmdRECAPOWriteShared}{1.47}
\newcommand{\pmdRECAPONoFPOtherEventTotal}{18322}
\newcommand{\pmdRECAPOAcqRelOtherTotal}{96.1}
\newcommand{\pmdRECAPONoAcqRelOtherTotal}{720}
\newcommand{\pmdRECAPOFork}{0.0}
\newcommand{\pmdRECAPOJoin}{0.0}
\newcommand{\pmdRECAPOPreWait}{0.0}
\newcommand{\pmdRECAPOPostWait}{0.0}
\newcommand{\pmdRECAPOVolatileTotal}{0.0}
\newcommand{\pmdRECAPOClassInit}{7.92}
\newcommand{\pmdRECAPOClassAccess}{92.1}
\newcommand{\pmdRECAPORaceTotal}{3700}
\newcommand{\pmdRECAPOWrRdRace}{99.6}
\newcommand{\pmdRECAPOWrWrRace}{0.0}
\newcommand{\pmdRECAPORdWrRace}{0.405}
\newcommand{\pmdRECAPORdShWrRace}{0.027}
\newcommand{\pmdRECAPOHoldLocksTotal}{0.093}
\newcommand{\pmdRECAPOOneLockHeld}{1.12}
\newcommand{\pmdRECAPOTwoNestedLocks}{\cna}
\newcommand{\pmdRECAPOThreeNestedLocks}{\cna}
\newcommand{\pmdRECAPOFourNestedLocks}{\cna}
\newcommand{\pmdRECAPOFiveNestedLocks}{\cna}
\newcommand{\pmdRECAPOSixNestedLocks}{\cna}
\newcommand{\pmdRECAPOSevenNestedLocks}{\cna}
\newcommand{\pmdRECAPOEightNestedLocks}{\cna}
\newcommand{\pmdRECAPONineNestedLocks}{\cna}
\newcommand{\pmdRECAPOTenNestedLocks}{\cna}
\newcommand{\pmdRECAPOHundredNestedLocks}{\cna}
\newcommand{\FASTpmdMaxLiveThreads}{15}
\newcommand{\FASTpmdTotalThreads}{15}
\newcommand{\FASTpmdBaseTime}{1.4}
\newcommand{\FASTpmdBaseTimeCI}{24}
\newcommand{\FASTpmdEmptyTime}{\rna}
\newcommand{\FASTpmdEmptyTimeCI}{\rna}
\newcommand{\FASTpmdEmptyTimeCIMIN}{\rna}
\newcommand{\FASTpmdEmptyTimeCIMAX}{\rna}
\newcommand{\FASTpmdFTTime}{6.9}
\newcommand{\FASTpmdFTTimeCI}{0.32}
\newcommand{\FASTpmdHBTime}{6.5}
\newcommand{\FASTpmdHBTimeCI}{0.17}
\newcommand{\FASTpmdFTOHBTime}{6.4}
\newcommand{\FASTpmdFTOHBTimeCI}{0.24}
\newcommand{\FASTpmdWCPTime}{\rna}
\newcommand{\FASTpmdWCPTimeCI}{\rna}
\newcommand{\FASTpmdWCPTimeCIMIN}{\rna}
\newcommand{\FASTpmdWCPTimeCIMAX}{\rna}
\newcommand{\FASTpmdFTOWCPTime}{6.6}
\newcommand{\FASTpmdFTOWCPTimeCI}{0.15}
\newcommand{\FASTpmdREWCPTime}{7.6}
\newcommand{\FASTpmdREWCPTimeCI}{0.25}
\newcommand{\FASTpmdDCTime}{\rna}
\newcommand{\FASTpmdDCTimeCI}{\rna}
\newcommand{\FASTpmdDCTimeCIMIN}{\rna}
\newcommand{\FASTpmdDCTimeCIMAX}{\rna}
\newcommand{\FASTpmdFTODCTime}{6.7}
\newcommand{\FASTpmdFTODCTimeCI}{0.14}
\newcommand{\FASTpmdREDCTime}{7.5}
\newcommand{\FASTpmdREDCTimeCI}{0.17}
\newcommand{\FASTpmdCAPOTime}{\rna}
\newcommand{\FASTpmdCAPOTimeCI}{\rna}
\newcommand{\FASTpmdCAPOTimeCIMIN}{\rna}
\newcommand{\FASTpmdCAPOTimeCIMAX}{\rna}
\newcommand{\FASTpmdFTOCAPOTime}{6.6}
\newcommand{\FASTpmdFTOCAPOTimeCI}{0.14}
\newcommand{\FASTpmdRECAPOTime}{7.4}
\newcommand{\FASTpmdRECAPOTimeCI}{0.12}
\newcommand{\FASTpmdAGGCAPOTime}{\rna}
\newcommand{\FASTpmdAGGCAPOTimeCI}{\rna}
\newcommand{\FASTpmdAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTpmdAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTpmdStaticTime}{\rzero}
\newcommand{\FASTpmdDynamicTime}{\rzero}
\newcommand{\FASTpmdBaseMem}{590}
\newcommand{\FASTpmdBaseMemCI}{10.0}
\newcommand{\FASTpmdFTMem}{2.5}
\newcommand{\FASTpmdFTMemCI}{0.15}
\newcommand{\FASTpmdHBMem}{2.7}
\newcommand{\FASTpmdHBMemCI}{0.15}
\newcommand{\FASTpmdFTOHBMem}{2.5}
\newcommand{\FASTpmdFTOHBMemCI}{0.17}
\newcommand{\FASTpmdWCPMem}{\memna}
\newcommand{\FASTpmdWCPMemCI}{\memna}
\newcommand{\FASTpmdWCPMemCIMIN}{\memna}
\newcommand{\FASTpmdWCPMemCIMAX}{\memna}
\newcommand{\FASTpmdFTOWCPMem}{3.0}
\newcommand{\FASTpmdFTOWCPMemCI}{0.21}
\newcommand{\FASTpmdREWCPMem}{5.1}
\newcommand{\FASTpmdREWCPMemCI}{0.11}
\newcommand{\FASTpmdDCMem}{\memna}
\newcommand{\FASTpmdDCMemCI}{\memna}
\newcommand{\FASTpmdDCMemCIMIN}{\memna}
\newcommand{\FASTpmdDCMemCIMAX}{\memna}
\newcommand{\FASTpmdFTODCMem}{2.9}
\newcommand{\FASTpmdFTODCMemCI}{0.11}
\newcommand{\FASTpmdREDCMem}{5.1}
\newcommand{\FASTpmdREDCMemCI}{0.12}
\newcommand{\FASTpmdCAPOMem}{\memna}
\newcommand{\FASTpmdCAPOMemCI}{\memna}
\newcommand{\FASTpmdCAPOMemCIMIN}{\memna}
\newcommand{\FASTpmdCAPOMemCIMAX}{\memna}
\newcommand{\FASTpmdFTOCAPOMem}{2.9}
\newcommand{\FASTpmdFTOCAPOMemCI}{0.16}
\newcommand{\FASTpmdRECAPOMem}{4.9}
\newcommand{\FASTpmdRECAPOMemCI}{0.13}
\newcommand{\FASTpmdAGGCAPOMem}{\memna}
\newcommand{\FASTpmdAGGCAPOMemCI}{\memna}
\newcommand{\FASTpmdAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTpmdAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTpmdEventsCI}{1,038}
\newcommand{\FASTpmdEventsCIMIN}{207,312,729}
\newcommand{\FASTpmdEventsCIMAX}{207,314,805}
\newcommand{\FASTpmdNoFPEventsCI}{893}
\newcommand{\FASTpmdNoFPEventsCIMIN}{13,101,938}
\newcommand{\FASTpmdNoFPEventsCIMAX}{13,103,724}
\newcommand{\FASTpmdFT}{17}
\newcommand{\FASTpmdFTCI}{0.64}
\newcommand{\FASTpmdFTCIMIN}{16}
\newcommand{\FASTpmdFTCIMAX}{18}
\newcommand{\FASTpmdFTDynamic}{3,772}
\newcommand{\FASTpmdFTDynamicCI}{400}
\newcommand{\FASTpmdFTDynamicCIMIN}{3,372}
\newcommand{\FASTpmdFTDynamicCIMAX}{4,172}
\newcommand{\FASTpmdHB}{18}
\newcommand{\FASTpmdHBCI}{0.26}
\newcommand{\FASTpmdHBCIMIN}{18}
\newcommand{\FASTpmdHBCIMAX}{18}
\newcommand{\FASTpmdHBDynamic}{1,801}
\newcommand{\FASTpmdHBDynamicCI}{111}
\newcommand{\FASTpmdHBDynamicCIMIN}{1,690}
\newcommand{\FASTpmdHBDynamicCIMAX}{1,912}
\newcommand{\FASTpmdFTOHB}{18}
\newcommand{\FASTpmdFTOHBCI}{0.32}
\newcommand{\FASTpmdFTOHBCIMIN}{18}
\newcommand{\FASTpmdFTOHBCIMAX}{18}
\newcommand{\FASTpmdFTOHBDynamic}{1,765}
\newcommand{\FASTpmdFTOHBDynamicCI}{139}
\newcommand{\FASTpmdFTOHBDynamicCIMIN}{1,626}
\newcommand{\FASTpmdFTOHBDynamicCIMAX}{1,904}
\newcommand{\FASTpmdWCP}{\rna}
\newcommand{\FASTpmdWCPCI}{\rna}
\newcommand{\FASTpmdWCPCIMIN}{\rna}
\newcommand{\FASTpmdWCPCIMAX}{\rna}
\newcommand{\FASTpmdWCPDynamic}{\rna}
\newcommand{\FASTpmdWCPDynamicCI}{\rna}
\newcommand{\FASTpmdWCPDynamicCIMIN}{\rna}
\newcommand{\FASTpmdWCPDynamicCIMAX}{\rna}
\newcommand{\FASTpmdFTOWCP}{18}
\newcommand{\FASTpmdFTOWCPCI}{0.43}
\newcommand{\FASTpmdFTOWCPCIMIN}{18}
\newcommand{\FASTpmdFTOWCPCIMAX}{18}
\newcommand{\FASTpmdFTOWCPDynamic}{1,823}
\newcommand{\FASTpmdFTOWCPDynamicCI}{126}
\newcommand{\FASTpmdFTOWCPDynamicCIMIN}{1,697}
\newcommand{\FASTpmdFTOWCPDynamicCIMAX}{1,949}
\newcommand{\FASTpmdREWCP}{18}
\newcommand{\FASTpmdREWCPCI}{0.3}
\newcommand{\FASTpmdREWCPCIMIN}{18}
\newcommand{\FASTpmdREWCPCIMAX}{18}
\newcommand{\FASTpmdREWCPDynamic}{1,750}
\newcommand{\FASTpmdREWCPDynamicCI}{96}
\newcommand{\FASTpmdREWCPDynamicCIMIN}{1,654}
\newcommand{\FASTpmdREWCPDynamicCIMAX}{1,846}
\newcommand{\FASTpmdDC}{\rna}
\newcommand{\FASTpmdDCCI}{\rna}
\newcommand{\FASTpmdDCCIMIN}{\rna}
\newcommand{\FASTpmdDCCIMAX}{\rna}
\newcommand{\FASTpmdDCDynamic}{\rna}
\newcommand{\FASTpmdDCDynamicCI}{\rna}
\newcommand{\FASTpmdDCDynamicCIMIN}{\rna}
\newcommand{\FASTpmdDCDynamicCIMAX}{\rna}
\newcommand{\FASTpmdFTODC}{18}
\newcommand{\FASTpmdFTODCCI}{0.43}
\newcommand{\FASTpmdFTODCCIMIN}{18}
\newcommand{\FASTpmdFTODCCIMAX}{18}
\newcommand{\FASTpmdFTODCDynamic}{3,660}
\newcommand{\FASTpmdFTODCDynamicCI}{185}
\newcommand{\FASTpmdFTODCDynamicCIMIN}{3,475}
\newcommand{\FASTpmdFTODCDynamicCIMAX}{3,845}
\newcommand{\FASTpmdREDC}{18}
\newcommand{\FASTpmdREDCCI}{0.26}
\newcommand{\FASTpmdREDCCIMIN}{18}
\newcommand{\FASTpmdREDCCIMAX}{18}
\newcommand{\FASTpmdREDCDynamic}{3,731}
\newcommand{\FASTpmdREDCDynamicCI}{128}
\newcommand{\FASTpmdREDCDynamicCIMIN}{3,603}
\newcommand{\FASTpmdREDCDynamicCIMAX}{3,859}
\newcommand{\FASTpmdCAPO}{\rna}
\newcommand{\FASTpmdCAPOCI}{\rna}
\newcommand{\FASTpmdCAPOCIMIN}{\rna}
\newcommand{\FASTpmdCAPOCIMAX}{\rna}
\newcommand{\FASTpmdCAPODynamic}{\rna}
\newcommand{\FASTpmdCAPODynamicCI}{\rna}
\newcommand{\FASTpmdCAPODynamicCIMIN}{\rna}
\newcommand{\FASTpmdCAPODynamicCIMAX}{\rna}
\newcommand{\FASTpmdFTOCAPO}{18}
\newcommand{\FASTpmdFTOCAPOCI}{0.26}
\newcommand{\FASTpmdFTOCAPOCIMIN}{18}
\newcommand{\FASTpmdFTOCAPOCIMAX}{18}
\newcommand{\FASTpmdFTOCAPODynamic}{3,785}
\newcommand{\FASTpmdFTOCAPODynamicCI}{196}
\newcommand{\FASTpmdFTOCAPODynamicCIMIN}{3,589}
\newcommand{\FASTpmdFTOCAPODynamicCIMAX}{3,981}
\newcommand{\FASTpmdRECAPO}{19}
\newcommand{\FASTpmdRECAPOCI}{0.33}
\newcommand{\FASTpmdRECAPOCIMIN}{19}
\newcommand{\FASTpmdRECAPOCIMAX}{19}
\newcommand{\FASTpmdRECAPODynamic}{3,700}
\newcommand{\FASTpmdRECAPODynamicCI}{211}
\newcommand{\FASTpmdRECAPODynamicCIMIN}{3,489}
\newcommand{\FASTpmdRECAPODynamicCIMAX}{3,911}
\newcommand{\FASTpmdAGGCAPO}{\rna}
\newcommand{\FASTpmdAGGCAPOCI}{\rna}
\newcommand{\FASTpmdAGGCAPOCIMIN}{\rna}
\newcommand{\FASTpmdAGGCAPOCIMAX}{\rna}
\newcommand{\FASTpmdAGGCAPODynamic}{\rna}
\newcommand{\FASTpmdAGGCAPODynamicCI}{\rna}
\newcommand{\FASTpmdAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTpmdAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTsunflowEvents}{9,700}
\newcommand{\FASTsunflowNoFPEvents}{400}
\newcommand{\sunflowHBEventTotal}{9,700}
\newcommand{\sunflowHBNoFPEventTotal}{370}
\newcommand{\sunflowHBNoFPAccessTotal}{370}
\newcommand{\sunflowHBNoFPOtherTotal}{<0.1}
\newcommand{\sunflowHBReadTotal}{99.7}
\newcommand{\sunflowHBWriteTotal}{0.26}
\newcommand{\sunflowHBNoFPAccessInCS}{0.229}
\newcommand{\sunflowHBNoFPAccessOutCS}{99.8}
\newcommand{\sunflowHBAcqRelTotal}{4.05E-4}
\newcommand{\sunflowHBOtherTotal}{5.27E-5}
\newcommand{\sunflowHBNoFPReadTotal}{370}
\newcommand{\sunflowHBReadInCS}{0.235}
\newcommand{\sunflowHBReadOutCS}{100}
\newcommand{\sunflowHBReadSameEp}{0.277}
\newcommand{\sunflowHBReadSharedSameEp}{<0.001}
\newcommand{\sunflowHBReadExclusive}{99.4}
\newcommand{\sunflowHBReadOwned}{\cna}
\newcommand{\sunflowHBReadShare}{0.0223}
\newcommand{\sunflowHBReadShared}{0.595}
\newcommand{\sunflowHBReadSharedOwned}{\cna}
\newcommand{\sunflowHBNoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowHBWriteInCS}{95.1}
\newcommand{\sunflowHBWriteOutCS}{41400}
\newcommand{\sunflowHBNoFPWriteTotal}{0.96}
\newcommand{\sunflowHBWriteSameEp}{41400}
\newcommand{\sunflowHBWriteExclusive}{100}
\newcommand{\sunflowHBWriteOwned}{\cna}
\newcommand{\sunflowHBWriteShared}{<0.001}
\newcommand{\sunflowHBNoFPOtherEventTotal}{1815}
\newcommand{\sunflowHBAcqRelOtherTotal}{88.5}
\newcommand{\sunflowHBNoAcqRelOtherTotal}{209}
\newcommand{\sunflowHBFork}{13.4}
\newcommand{\sunflowHBJoin}{13.4}
\newcommand{\sunflowHBPreWait}{0.0}
\newcommand{\sunflowHBPostWait}{0.0}
\newcommand{\sunflowHBVolatileTotal}{0.0}
\newcommand{\sunflowHBClassInit}{9.09}
\newcommand{\sunflowHBClassAccess}{64.1}
\newcommand{\sunflowHBRaceTotal}{59}
\newcommand{\sunflowHBWrRdRace}{93.2}
\newcommand{\sunflowHBWrWrRace}{0.0}
\newcommand{\sunflowHBRdWrRace}{0.0}
\newcommand{\sunflowHBRdShWrRace}{6.78}
\newcommand{\sunflowHBHoldLocksTotal}{1.8}
\newcommand{\sunflowHBOneLockHeld}{0.48}
\newcommand{\sunflowHBTwoNestedLocks}{<0.1}
\newcommand{\sunflowHBThreeNestedLocks}{\cna}
\newcommand{\sunflowHBFourNestedLocks}{\cna}
\newcommand{\sunflowHBFiveNestedLocks}{\cna}
\newcommand{\sunflowHBSixNestedLocks}{\cna}
\newcommand{\sunflowHBSevenNestedLocks}{\cna}
\newcommand{\sunflowHBEightNestedLocks}{\cna}
\newcommand{\sunflowHBNineNestedLocks}{\cna}
\newcommand{\sunflowHBTenNestedLocks}{\cna}
\newcommand{\sunflowHBHundredNestedLocks}{\cna}
\newcommand{\sunflowFTOHBEventTotal}{9,700}
\newcommand{\sunflowFTOHBNoFPEventTotal}{3.5}
\newcommand{\sunflowFTOHBNoFPAccessTotal}{3.5}
\newcommand{\sunflowFTOHBNoFPOtherTotal}{<0.1}
\newcommand{\sunflowFTOHBReadTotal}{72.3}
\newcommand{\sunflowFTOHBWriteTotal}{27.6}
\newcommand{\sunflowFTOHBNoFPAccessInCS}{0.229}
\newcommand{\sunflowFTOHBNoFPAccessOutCS}{99.8}
\newcommand{\sunflowFTOHBAcqRelTotal}{4.05E-4}
\newcommand{\sunflowFTOHBOtherTotal}{5.27E-5}
\newcommand{\sunflowFTOHBNoFPReadTotal}{2.5}
\newcommand{\sunflowFTOHBReadInCS}{1.09}
\newcommand{\sunflowFTOHBReadOutCS}{139}
\newcommand{\sunflowFTOHBReadSameEp}{40.5}
\newcommand{\sunflowFTOHBReadSharedSameEp}{<0.001}
\newcommand{\sunflowFTOHBReadExclusive}{5.77}
\newcommand{\sunflowFTOHBReadOwned}{3.94}
\newcommand{\sunflowFTOHBReadShare}{3.27}
\newcommand{\sunflowFTOHBReadShared}{31.1}
\newcommand{\sunflowFTOHBReadSharedOwned}{56}
\newcommand{\sunflowFTOHBNoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowFTOHBWriteInCS}{95.1}
\newcommand{\sunflowFTOHBWriteOutCS}{41400}
\newcommand{\sunflowFTOHBNoFPWriteTotal}{0.96}
\newcommand{\sunflowFTOHBWriteSameEp}{41400}
\newcommand{\sunflowFTOHBWriteExclusive}{<0.001}
\newcommand{\sunflowFTOHBWriteOwned}{100}
\newcommand{\sunflowFTOHBWriteShared}{<0.001}
\newcommand{\sunflowFTOHBNoFPOtherEventTotal}{1815}
\newcommand{\sunflowFTOHBAcqRelOtherTotal}{88.5}
\newcommand{\sunflowFTOHBNoAcqRelOtherTotal}{209}
\newcommand{\sunflowFTOHBFork}{13.4}
\newcommand{\sunflowFTOHBJoin}{13.4}
\newcommand{\sunflowFTOHBPreWait}{0.0}
\newcommand{\sunflowFTOHBPostWait}{0.0}
\newcommand{\sunflowFTOHBVolatileTotal}{0.0}
\newcommand{\sunflowFTOHBClassInit}{9.09}
\newcommand{\sunflowFTOHBClassAccess}{64.1}
\newcommand{\sunflowFTOHBRaceTotal}{55}
\newcommand{\sunflowFTOHBWrRdRace}{92.7}
\newcommand{\sunflowFTOHBWrWrRace}{0.0}
\newcommand{\sunflowFTOHBRdWrRace}{0.0}
\newcommand{\sunflowFTOHBRdShWrRace}{7.27}
\newcommand{\sunflowFTOHBHoldLocksTotal}{0.027}
\newcommand{\sunflowFTOHBOneLockHeld}{0.79}
\newcommand{\sunflowFTOHBTwoNestedLocks}{<0.1}
\newcommand{\sunflowFTOHBThreeNestedLocks}{\cna}
\newcommand{\sunflowFTOHBFourNestedLocks}{\cna}
\newcommand{\sunflowFTOHBFiveNestedLocks}{\cna}
\newcommand{\sunflowFTOHBSixNestedLocks}{\cna}
\newcommand{\sunflowFTOHBSevenNestedLocks}{\cna}
\newcommand{\sunflowFTOHBEightNestedLocks}{\cna}
\newcommand{\sunflowFTOHBNineNestedLocks}{\cna}
\newcommand{\sunflowFTOHBTenNestedLocks}{\cna}
\newcommand{\sunflowFTOHBHundredNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPEventTotal}{9,700}
\newcommand{\sunflowFTOWCPNoFPEventTotal}{3.5}
\newcommand{\sunflowFTOWCPNoFPAccessTotal}{3.5}
\newcommand{\sunflowFTOWCPNoFPOtherTotal}{<0.1}
\newcommand{\sunflowFTOWCPReadTotal}{72.3}
\newcommand{\sunflowFTOWCPWriteTotal}{27.6}
\newcommand{\sunflowFTOWCPNoFPAccessInCS}{0.229}
\newcommand{\sunflowFTOWCPNoFPAccessOutCS}{99.8}
\newcommand{\sunflowFTOWCPAcqRelTotal}{4.06E-4}
\newcommand{\sunflowFTOWCPOtherTotal}{5.29E-5}
\newcommand{\sunflowFTOWCPNoFPReadTotal}{2.5}
\newcommand{\sunflowFTOWCPReadInCS}{1.09}
\newcommand{\sunflowFTOWCPReadOutCS}{139}
\newcommand{\sunflowFTOWCPReadSameEp}{40.5}
\newcommand{\sunflowFTOWCPReadSharedSameEp}{<0.001}
\newcommand{\sunflowFTOWCPReadExclusive}{5.98}
\newcommand{\sunflowFTOWCPReadOwned}{3.7}
\newcommand{\sunflowFTOWCPReadShare}{3.27}
\newcommand{\sunflowFTOWCPReadShared}{31.1}
\newcommand{\sunflowFTOWCPReadSharedOwned}{55.9}
\newcommand{\sunflowFTOWCPNoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowFTOWCPWriteInCS}{95.1}
\newcommand{\sunflowFTOWCPWriteOutCS}{41400}
\newcommand{\sunflowFTOWCPNoFPWriteTotal}{0.96}
\newcommand{\sunflowFTOWCPWriteSameEp}{41400}
\newcommand{\sunflowFTOWCPWriteExclusive}{<0.001}
\newcommand{\sunflowFTOWCPWriteOwned}{100}
\newcommand{\sunflowFTOWCPWriteShared}{<0.001}
\newcommand{\sunflowFTOWCPNoFPOtherEventTotal}{1819}
\newcommand{\sunflowFTOWCPAcqRelOtherTotal}{88.5}
\newcommand{\sunflowFTOWCPNoAcqRelOtherTotal}{210}
\newcommand{\sunflowFTOWCPFork}{13.3}
\newcommand{\sunflowFTOWCPJoin}{13.3}
\newcommand{\sunflowFTOWCPPreWait}{0.0}
\newcommand{\sunflowFTOWCPPostWait}{0.0}
\newcommand{\sunflowFTOWCPVolatileTotal}{0.0}
\newcommand{\sunflowFTOWCPClassInit}{9.05}
\newcommand{\sunflowFTOWCPClassAccess}{64.3}
\newcommand{\sunflowFTOWCPRaceTotal}{210}
\newcommand{\sunflowFTOWCPWrRdRace}{97.6}
\newcommand{\sunflowFTOWCPWrWrRace}{0.0}
\newcommand{\sunflowFTOWCPRdWrRace}{0.0}
\newcommand{\sunflowFTOWCPRdShWrRace}{2.38}
\newcommand{\sunflowFTOWCPHoldLocksTotal}{0.027}
\newcommand{\sunflowFTOWCPOneLockHeld}{0.78}
\newcommand{\sunflowFTOWCPTwoNestedLocks}{<0.1}
\newcommand{\sunflowFTOWCPThreeNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPFourNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPFiveNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPSixNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPSevenNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPEightNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPNineNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPTenNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPHundredNestedLocks}{\cna}
\newcommand{\sunflowREWCPEventTotal}{9,700}
\newcommand{\sunflowREWCPNoFPEventTotal}{3.5}
\newcommand{\sunflowREWCPNoFPAccessTotal}{3.5}
\newcommand{\sunflowREWCPNoFPOtherTotal}{<0.1}
\newcommand{\sunflowREWCPReadTotal}{72.3}
\newcommand{\sunflowREWCPWriteTotal}{27.6}
\newcommand{\sunflowREWCPNoFPAccessInCS}{0.229}
\newcommand{\sunflowREWCPNoFPAccessOutCS}{99.8}
\newcommand{\sunflowREWCPAcqRelTotal}{4.05E-4}
\newcommand{\sunflowREWCPOtherTotal}{5.27E-5}
\newcommand{\sunflowREWCPNoFPReadTotal}{2.5}
\newcommand{\sunflowREWCPReadInCS}{1.09}
\newcommand{\sunflowREWCPReadOutCS}{139}
\newcommand{\sunflowREWCPReadSameEp}{40.5}
\newcommand{\sunflowREWCPReadSharedSameEp}{\cna}
\newcommand{\sunflowREWCPReadExclusive}{5.74}
\newcommand{\sunflowREWCPReadOwned}{3.93}
\newcommand{\sunflowREWCPReadShare}{3.27}
\newcommand{\sunflowREWCPReadShared}{31.2}
\newcommand{\sunflowREWCPReadSharedOwned}{55.8}
\newcommand{\sunflowREWCPNoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowREWCPWriteInCS}{95.1}
\newcommand{\sunflowREWCPWriteOutCS}{41400}
\newcommand{\sunflowREWCPNoFPWriteTotal}{0.96}
\newcommand{\sunflowREWCPWriteSameEp}{41400}
\newcommand{\sunflowREWCPWriteExclusive}{<0.001}
\newcommand{\sunflowREWCPWriteOwned}{100}
\newcommand{\sunflowREWCPWriteShared}{0.0162}
\newcommand{\sunflowREWCPNoFPOtherEventTotal}{1817}
\newcommand{\sunflowREWCPAcqRelOtherTotal}{88.5}
\newcommand{\sunflowREWCPNoAcqRelOtherTotal}{209}
\newcommand{\sunflowREWCPFork}{13.4}
\newcommand{\sunflowREWCPJoin}{13.4}
\newcommand{\sunflowREWCPPreWait}{0.0}
\newcommand{\sunflowREWCPPostWait}{0.0}
\newcommand{\sunflowREWCPVolatileTotal}{0.0}
\newcommand{\sunflowREWCPClassInit}{9.09}
\newcommand{\sunflowREWCPClassAccess}{64.1}
\newcommand{\sunflowREWCPRaceTotal}{246}
\newcommand{\sunflowREWCPWrRdRace}{98.4}
\newcommand{\sunflowREWCPWrWrRace}{0.0}
\newcommand{\sunflowREWCPRdWrRace}{0.0}
\newcommand{\sunflowREWCPRdShWrRace}{1.63}
\newcommand{\sunflowREWCPHoldLocksTotal}{0.027}
\newcommand{\sunflowREWCPOneLockHeld}{0.78}
\newcommand{\sunflowREWCPTwoNestedLocks}{<0.1}
\newcommand{\sunflowREWCPThreeNestedLocks}{\cna}
\newcommand{\sunflowREWCPFourNestedLocks}{\cna}
\newcommand{\sunflowREWCPFiveNestedLocks}{\cna}
\newcommand{\sunflowREWCPSixNestedLocks}{\cna}
\newcommand{\sunflowREWCPSevenNestedLocks}{\cna}
\newcommand{\sunflowREWCPEightNestedLocks}{\cna}
\newcommand{\sunflowREWCPNineNestedLocks}{\cna}
\newcommand{\sunflowREWCPTenNestedLocks}{\cna}
\newcommand{\sunflowREWCPHundredNestedLocks}{\cna}
\newcommand{\sunflowFTODCEventTotal}{9,700}
\newcommand{\sunflowFTODCNoFPEventTotal}{3.5}
\newcommand{\sunflowFTODCNoFPAccessTotal}{3.5}
\newcommand{\sunflowFTODCNoFPOtherTotal}{<0.1}
\newcommand{\sunflowFTODCReadTotal}{72.3}
\newcommand{\sunflowFTODCWriteTotal}{27.6}
\newcommand{\sunflowFTODCNoFPAccessInCS}{0.229}
\newcommand{\sunflowFTODCNoFPAccessOutCS}{99.8}
\newcommand{\sunflowFTODCAcqRelTotal}{4.05E-4}
\newcommand{\sunflowFTODCOtherTotal}{5.27E-5}
\newcommand{\sunflowFTODCNoFPReadTotal}{2.5}
\newcommand{\sunflowFTODCReadInCS}{1.09}
\newcommand{\sunflowFTODCReadOutCS}{139}
\newcommand{\sunflowFTODCReadSameEp}{40.5}
\newcommand{\sunflowFTODCReadSharedSameEp}{<0.001}
\newcommand{\sunflowFTODCReadExclusive}{5.82}
\newcommand{\sunflowFTODCReadOwned}{3.86}
\newcommand{\sunflowFTODCReadShare}{3.27}
\newcommand{\sunflowFTODCReadShared}{31.1}
\newcommand{\sunflowFTODCReadSharedOwned}{56}
\newcommand{\sunflowFTODCNoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowFTODCWriteInCS}{95.1}
\newcommand{\sunflowFTODCWriteOutCS}{41400}
\newcommand{\sunflowFTODCNoFPWriteTotal}{0.96}
\newcommand{\sunflowFTODCWriteSameEp}{41400}
\newcommand{\sunflowFTODCWriteExclusive}{<0.001}
\newcommand{\sunflowFTODCWriteOwned}{100}
\newcommand{\sunflowFTODCWriteShared}{<0.001}
\newcommand{\sunflowFTODCNoFPOtherEventTotal}{1818}
\newcommand{\sunflowFTODCAcqRelOtherTotal}{88.5}
\newcommand{\sunflowFTODCNoAcqRelOtherTotal}{209}
\newcommand{\sunflowFTODCFork}{13.4}
\newcommand{\sunflowFTODCJoin}{13.4}
\newcommand{\sunflowFTODCPreWait}{0.0}
\newcommand{\sunflowFTODCPostWait}{0.0}
\newcommand{\sunflowFTODCVolatileTotal}{0.0}
\newcommand{\sunflowFTODCClassInit}{9.09}
\newcommand{\sunflowFTODCClassAccess}{64.1}
\newcommand{\sunflowFTODCRaceTotal}{403}
\newcommand{\sunflowFTODCWrRdRace}{98.8}
\newcommand{\sunflowFTODCWrWrRace}{0.0}
\newcommand{\sunflowFTODCRdWrRace}{0.0}
\newcommand{\sunflowFTODCRdShWrRace}{1.24}
\newcommand{\sunflowFTODCHoldLocksTotal}{0.027}
\newcommand{\sunflowFTODCOneLockHeld}{0.78}
\newcommand{\sunflowFTODCTwoNestedLocks}{<0.1}
\newcommand{\sunflowFTODCThreeNestedLocks}{\cna}
\newcommand{\sunflowFTODCFourNestedLocks}{\cna}
\newcommand{\sunflowFTODCFiveNestedLocks}{\cna}
\newcommand{\sunflowFTODCSixNestedLocks}{\cna}
\newcommand{\sunflowFTODCSevenNestedLocks}{\cna}
\newcommand{\sunflowFTODCEightNestedLocks}{\cna}
\newcommand{\sunflowFTODCNineNestedLocks}{\cna}
\newcommand{\sunflowFTODCTenNestedLocks}{\cna}
\newcommand{\sunflowFTODCHundredNestedLocks}{\cna}
\newcommand{\sunflowREDCEventTotal}{9,700}
\newcommand{\sunflowREDCNoFPEventTotal}{3.5}
\newcommand{\sunflowREDCNoFPAccessTotal}{3.5}
\newcommand{\sunflowREDCNoFPOtherTotal}{<0.1}
\newcommand{\sunflowREDCReadTotal}{72.3}
\newcommand{\sunflowREDCWriteTotal}{27.6}
\newcommand{\sunflowREDCNoFPAccessInCS}{0.229}
\newcommand{\sunflowREDCNoFPAccessOutCS}{99.8}
\newcommand{\sunflowREDCAcqRelTotal}{4.05E-4}
\newcommand{\sunflowREDCOtherTotal}{5.27E-5}
\newcommand{\sunflowREDCNoFPReadTotal}{2.5}
\newcommand{\sunflowREDCReadInCS}{1.09}
\newcommand{\sunflowREDCReadOutCS}{139}
\newcommand{\sunflowREDCReadSameEp}{40.5}
\newcommand{\sunflowREDCReadSharedSameEp}{<0.001}
\newcommand{\sunflowREDCReadExclusive}{5.72}
\newcommand{\sunflowREDCReadOwned}{3.94}
\newcommand{\sunflowREDCReadShare}{3.27}
\newcommand{\sunflowREDCReadShared}{31.1}
\newcommand{\sunflowREDCReadSharedOwned}{55.9}
\newcommand{\sunflowREDCNoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowREDCWriteInCS}{95.1}
\newcommand{\sunflowREDCWriteOutCS}{41400}
\newcommand{\sunflowREDCNoFPWriteTotal}{0.96}
\newcommand{\sunflowREDCWriteSameEp}{41400}
\newcommand{\sunflowREDCWriteExclusive}{<0.001}
\newcommand{\sunflowREDCWriteOwned}{100}
\newcommand{\sunflowREDCWriteShared}{0.0161}
\newcommand{\sunflowREDCNoFPOtherEventTotal}{1816}
\newcommand{\sunflowREDCAcqRelOtherTotal}{88.5}
\newcommand{\sunflowREDCNoAcqRelOtherTotal}{209}
\newcommand{\sunflowREDCFork}{13.4}
\newcommand{\sunflowREDCJoin}{13.4}
\newcommand{\sunflowREDCPreWait}{0.0}
\newcommand{\sunflowREDCPostWait}{0.0}
\newcommand{\sunflowREDCVolatileTotal}{0.0}
\newcommand{\sunflowREDCClassInit}{9.09}
\newcommand{\sunflowREDCClassAccess}{64.1}
\newcommand{\sunflowREDCRaceTotal}{412}
\newcommand{\sunflowREDCWrRdRace}{99.0}
\newcommand{\sunflowREDCWrWrRace}{0.0}
\newcommand{\sunflowREDCRdWrRace}{0.0}
\newcommand{\sunflowREDCRdShWrRace}{0.971}
\newcommand{\sunflowREDCHoldLocksTotal}{0.027}
\newcommand{\sunflowREDCOneLockHeld}{0.78}
\newcommand{\sunflowREDCTwoNestedLocks}{<0.1}
\newcommand{\sunflowREDCThreeNestedLocks}{\cna}
\newcommand{\sunflowREDCFourNestedLocks}{\cna}
\newcommand{\sunflowREDCFiveNestedLocks}{\cna}
\newcommand{\sunflowREDCSixNestedLocks}{\cna}
\newcommand{\sunflowREDCSevenNestedLocks}{\cna}
\newcommand{\sunflowREDCEightNestedLocks}{\cna}
\newcommand{\sunflowREDCNineNestedLocks}{\cna}
\newcommand{\sunflowREDCTenNestedLocks}{\cna}
\newcommand{\sunflowREDCHundredNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOEventTotal}{9,700}
\newcommand{\sunflowFTOCAPONoFPEventTotal}{3.5}
\newcommand{\sunflowFTOCAPONoFPAccessTotal}{3.5}
\newcommand{\sunflowFTOCAPONoFPOtherTotal}{<0.1}
\newcommand{\sunflowFTOCAPOReadTotal}{72.3}
\newcommand{\sunflowFTOCAPOWriteTotal}{27.6}
\newcommand{\sunflowFTOCAPONoFPAccessInCS}{0.229}
\newcommand{\sunflowFTOCAPONoFPAccessOutCS}{99.8}
\newcommand{\sunflowFTOCAPOAcqRelTotal}{4.05E-4}
\newcommand{\sunflowFTOCAPOOtherTotal}{5.27E-5}
\newcommand{\sunflowFTOCAPONoFPReadTotal}{2.5}
\newcommand{\sunflowFTOCAPOReadInCS}{1.09}
\newcommand{\sunflowFTOCAPOReadOutCS}{139}
\newcommand{\sunflowFTOCAPOReadSameEp}{40.5}
\newcommand{\sunflowFTOCAPOReadSharedSameEp}{<0.001}
\newcommand{\sunflowFTOCAPOReadExclusive}{5.74}
\newcommand{\sunflowFTOCAPOReadOwned}{3.94}
\newcommand{\sunflowFTOCAPOReadShare}{3.27}
\newcommand{\sunflowFTOCAPOReadShared}{31.1}
\newcommand{\sunflowFTOCAPOReadSharedOwned}{56}
\newcommand{\sunflowFTOCAPONoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowFTOCAPOWriteInCS}{95.1}
\newcommand{\sunflowFTOCAPOWriteOutCS}{41400}
\newcommand{\sunflowFTOCAPONoFPWriteTotal}{0.96}
\newcommand{\sunflowFTOCAPOWriteSameEp}{41400}
\newcommand{\sunflowFTOCAPOWriteExclusive}{<0.001}
\newcommand{\sunflowFTOCAPOWriteOwned}{100}
\newcommand{\sunflowFTOCAPOWriteShared}{<0.001}
\newcommand{\sunflowFTOCAPONoFPOtherEventTotal}{1816}
\newcommand{\sunflowFTOCAPOAcqRelOtherTotal}{88.5}
\newcommand{\sunflowFTOCAPONoAcqRelOtherTotal}{209}
\newcommand{\sunflowFTOCAPOFork}{13.4}
\newcommand{\sunflowFTOCAPOJoin}{13.4}
\newcommand{\sunflowFTOCAPOPreWait}{0.0}
\newcommand{\sunflowFTOCAPOPostWait}{0.0}
\newcommand{\sunflowFTOCAPOVolatileTotal}{0.0}
\newcommand{\sunflowFTOCAPOClassInit}{9.09}
\newcommand{\sunflowFTOCAPOClassAccess}{64.1}
\newcommand{\sunflowFTOCAPORaceTotal}{416}
\newcommand{\sunflowFTOCAPOWrRdRace}{98.8}
\newcommand{\sunflowFTOCAPOWrWrRace}{0.0}
\newcommand{\sunflowFTOCAPORdWrRace}{0.0}
\newcommand{\sunflowFTOCAPORdShWrRace}{0.962}
\newcommand{\sunflowFTOCAPOHoldLocksTotal}{0.027}
\newcommand{\sunflowFTOCAPOOneLockHeld}{0.78}
\newcommand{\sunflowFTOCAPOTwoNestedLocks}{<0.1}
\newcommand{\sunflowFTOCAPOThreeNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOFourNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOSixNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOEightNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPONineNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOTenNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\sunflowRECAPOEventTotal}{9,700}
\newcommand{\sunflowRECAPONoFPEventTotal}{3.5}
\newcommand{\sunflowRECAPONoFPAccessTotal}{3.5}
\newcommand{\sunflowRECAPONoFPOtherTotal}{<0.1}
\newcommand{\sunflowRECAPOReadTotal}{72.3}
\newcommand{\sunflowRECAPOWriteTotal}{27.6}
\newcommand{\sunflowRECAPONoFPAccessInCS}{0.229}
\newcommand{\sunflowRECAPONoFPAccessOutCS}{99.8}
\newcommand{\sunflowRECAPOAcqRelTotal}{4.05E-4}
\newcommand{\sunflowRECAPOOtherTotal}{5.27E-5}
\newcommand{\sunflowRECAPONoFPReadTotal}{2.5}
\newcommand{\sunflowRECAPOReadInCS}{1.09}
\newcommand{\sunflowRECAPOReadOutCS}{139}
\newcommand{\sunflowRECAPOReadSameEp}{40.5}
\newcommand{\sunflowRECAPOReadSharedSameEp}{<0.001}
\newcommand{\sunflowRECAPOReadExclusive}{5.73}
\newcommand{\sunflowRECAPOReadOwned}{3.93}
\newcommand{\sunflowRECAPOReadShare}{3.27}
\newcommand{\sunflowRECAPOReadShared}{31.2}
\newcommand{\sunflowRECAPOReadSharedOwned}{55.9}
\newcommand{\sunflowRECAPONoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowRECAPOWriteInCS}{95.1}
\newcommand{\sunflowRECAPOWriteOutCS}{41400}
\newcommand{\sunflowRECAPONoFPWriteTotal}{0.96}
\newcommand{\sunflowRECAPOWriteSameEp}{41400}
\newcommand{\sunflowRECAPOWriteExclusive}{<0.001}
\newcommand{\sunflowRECAPOWriteOwned}{100}
\newcommand{\sunflowRECAPOWriteShared}{0.0158}
\newcommand{\sunflowRECAPONoFPOtherEventTotal}{1816}
\newcommand{\sunflowRECAPOAcqRelOtherTotal}{88.5}
\newcommand{\sunflowRECAPONoAcqRelOtherTotal}{209}
\newcommand{\sunflowRECAPOFork}{13.4}
\newcommand{\sunflowRECAPOJoin}{13.4}
\newcommand{\sunflowRECAPOPreWait}{0.0}
\newcommand{\sunflowRECAPOPostWait}{0.0}
\newcommand{\sunflowRECAPOVolatileTotal}{0.0}
\newcommand{\sunflowRECAPOClassInit}{9.09}
\newcommand{\sunflowRECAPOClassAccess}{64.1}
\newcommand{\sunflowRECAPORaceTotal}{415}
\newcommand{\sunflowRECAPOWrRdRace}{99.0}
\newcommand{\sunflowRECAPOWrWrRace}{0.0}
\newcommand{\sunflowRECAPORdWrRace}{0.0}
\newcommand{\sunflowRECAPORdShWrRace}{0.964}
\newcommand{\sunflowRECAPOHoldLocksTotal}{0.027}
\newcommand{\sunflowRECAPOOneLockHeld}{0.78}
\newcommand{\sunflowRECAPOTwoNestedLocks}{<0.1}
\newcommand{\sunflowRECAPOThreeNestedLocks}{\cna}
\newcommand{\sunflowRECAPOFourNestedLocks}{\cna}
\newcommand{\sunflowRECAPOFiveNestedLocks}{\cna}
\newcommand{\sunflowRECAPOSixNestedLocks}{\cna}
\newcommand{\sunflowRECAPOSevenNestedLocks}{\cna}
\newcommand{\sunflowRECAPOEightNestedLocks}{\cna}
\newcommand{\sunflowRECAPONineNestedLocks}{\cna}
\newcommand{\sunflowRECAPOTenNestedLocks}{\cna}
\newcommand{\sunflowRECAPOHundredNestedLocks}{\cna}
\newcommand{\FASTsunflowMaxLiveThreads}{29}
\newcommand{\FASTsunflowTotalThreads}{29}
\newcommand{\FASTsunflowBaseTime}{1.3}
\newcommand{\FASTsunflowBaseTimeCI}{29}
\newcommand{\FASTsunflowEmptyTime}{\rna}
\newcommand{\FASTsunflowEmptyTimeCI}{\rna}
\newcommand{\FASTsunflowEmptyTimeCIMIN}{\rna}
\newcommand{\FASTsunflowEmptyTimeCIMAX}{\rna}
\newcommand{\FASTsunflowFTTime}{18}
\newcommand{\FASTsunflowFTTimeCI}{0.7}
\newcommand{\FASTsunflowHBTime}{20}
\newcommand{\FASTsunflowHBTimeCI}{0.58}
\newcommand{\FASTsunflowFTOHBTime}{19}
\newcommand{\FASTsunflowFTOHBTimeCI}{0.55}
\newcommand{\FASTsunflowWCPTime}{\rna}
\newcommand{\FASTsunflowWCPTimeCI}{\rna}
\newcommand{\FASTsunflowWCPTimeCIMIN}{\rna}
\newcommand{\FASTsunflowWCPTimeCIMAX}{\rna}
\newcommand{\FASTsunflowFTOWCPTime}{21}
\newcommand{\FASTsunflowFTOWCPTimeCI}{0.87}
\newcommand{\FASTsunflowREWCPTime}{21}
\newcommand{\FASTsunflowREWCPTimeCI}{0.67}
\newcommand{\FASTsunflowDCTime}{\rna}
\newcommand{\FASTsunflowDCTimeCI}{\rna}
\newcommand{\FASTsunflowDCTimeCIMIN}{\rna}
\newcommand{\FASTsunflowDCTimeCIMAX}{\rna}
\newcommand{\FASTsunflowFTODCTime}{21}
\newcommand{\FASTsunflowFTODCTimeCI}{0.91}
\newcommand{\FASTsunflowREDCTime}{22}
\newcommand{\FASTsunflowREDCTimeCI}{1.2}
\newcommand{\FASTsunflowCAPOTime}{\rna}
\newcommand{\FASTsunflowCAPOTimeCI}{\rna}
\newcommand{\FASTsunflowCAPOTimeCIMIN}{\rna}
\newcommand{\FASTsunflowCAPOTimeCIMAX}{\rna}
\newcommand{\FASTsunflowFTOCAPOTime}{21}
\newcommand{\FASTsunflowFTOCAPOTimeCI}{0.76}
\newcommand{\FASTsunflowRECAPOTime}{22}
\newcommand{\FASTsunflowRECAPOTimeCI}{0.95}
\newcommand{\FASTsunflowAGGCAPOTime}{\rna}
\newcommand{\FASTsunflowAGGCAPOTimeCI}{\rna}
\newcommand{\FASTsunflowAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTsunflowAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTsunflowStaticTime}{\rzero}
\newcommand{\FASTsunflowDynamicTime}{\rzero}
\newcommand{\FASTsunflowBaseMem}{610}
\newcommand{\FASTsunflowBaseMemCI}{4.8}
\newcommand{\FASTsunflowFTMem}{8.6}
\newcommand{\FASTsunflowFTMemCI}{0.079}
\newcommand{\FASTsunflowHBMem}{8.5}
\newcommand{\FASTsunflowHBMemCI}{0.086}
\newcommand{\FASTsunflowFTOHBMem}{8.6}
\newcommand{\FASTsunflowFTOHBMemCI}{0.073}
\newcommand{\FASTsunflowWCPMem}{\memna}
\newcommand{\FASTsunflowWCPMemCI}{\memna}
\newcommand{\FASTsunflowWCPMemCIMIN}{\memna}
\newcommand{\FASTsunflowWCPMemCIMAX}{\memna}
\newcommand{\FASTsunflowFTOWCPMem}{9.3}
\newcommand{\FASTsunflowFTOWCPMemCI}{0.089}
\newcommand{\FASTsunflowREWCPMem}{38}
\newcommand{\FASTsunflowREWCPMemCI}{0.31}
\newcommand{\FASTsunflowDCMem}{\memna}
\newcommand{\FASTsunflowDCMemCI}{\memna}
\newcommand{\FASTsunflowDCMemCIMIN}{\memna}
\newcommand{\FASTsunflowDCMemCIMAX}{\memna}
\newcommand{\FASTsunflowFTODCMem}{9.3}
\newcommand{\FASTsunflowFTODCMemCI}{0.076}
\newcommand{\FASTsunflowREDCMem}{38}
\newcommand{\FASTsunflowREDCMemCI}{0.32}
\newcommand{\FASTsunflowCAPOMem}{\memna}
\newcommand{\FASTsunflowCAPOMemCI}{\memna}
\newcommand{\FASTsunflowCAPOMemCIMIN}{\memna}
\newcommand{\FASTsunflowCAPOMemCIMAX}{\memna}
\newcommand{\FASTsunflowFTOCAPOMem}{9.3}
\newcommand{\FASTsunflowFTOCAPOMemCI}{0.084}
\newcommand{\FASTsunflowRECAPOMem}{38}
\newcommand{\FASTsunflowRECAPOMemCI}{0.3}
\newcommand{\FASTsunflowAGGCAPOMem}{\memna}
\newcommand{\FASTsunflowAGGCAPOMemCI}{\memna}
\newcommand{\FASTsunflowAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTsunflowAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTsunflowEventsCI}{7}
\newcommand{\FASTsunflowEventsCIMIN}{9,681,323,549}
\newcommand{\FASTsunflowEventsCIMAX}{9,681,323,563}
\newcommand{\FASTsunflowNoFPEventsCI}{17}
\newcommand{\FASTsunflowNoFPEventsCIMIN}{396,882,632}
\newcommand{\FASTsunflowNoFPEventsCIMAX}{396,882,666}
\newcommand{\FASTsunflowFT}{5}
\newcommand{\FASTsunflowFTCI}{0.0}
\newcommand{\FASTsunflowFTCIMIN}{5}
\newcommand{\FASTsunflowFTCIMAX}{5}
\newcommand{\FASTsunflowFTDynamic}{115}
\newcommand{\FASTsunflowFTDynamicCI}{7.1}
\newcommand{\FASTsunflowFTDynamicCIMIN}{108}
\newcommand{\FASTsunflowFTDynamicCIMAX}{122}
\newcommand{\FASTsunflowHB}{6}
\newcommand{\FASTsunflowHBCI}{0.0}
\newcommand{\FASTsunflowHBCIMIN}{6}
\newcommand{\FASTsunflowHBCIMAX}{6}
\newcommand{\FASTsunflowHBDynamic}{59}
\newcommand{\FASTsunflowHBDynamicCI}{4.9}
\newcommand{\FASTsunflowHBDynamicCIMIN}{54}
\newcommand{\FASTsunflowHBDynamicCIMAX}{64}
\newcommand{\FASTsunflowFTOHB}{6}
\newcommand{\FASTsunflowFTOHBCI}{0.0}
\newcommand{\FASTsunflowFTOHBCIMIN}{6}
\newcommand{\FASTsunflowFTOHBCIMAX}{6}
\newcommand{\FASTsunflowFTOHBDynamic}{55}
\newcommand{\FASTsunflowFTOHBDynamicCI}{1.7}
\newcommand{\FASTsunflowFTOHBDynamicCIMIN}{53}
\newcommand{\FASTsunflowFTOHBDynamicCIMAX}{57}
\newcommand{\FASTsunflowWCP}{\rna}
\newcommand{\FASTsunflowWCPCI}{\rna}
\newcommand{\FASTsunflowWCPCIMIN}{\rna}
\newcommand{\FASTsunflowWCPCIMAX}{\rna}
\newcommand{\FASTsunflowWCPDynamic}{\rna}
\newcommand{\FASTsunflowWCPDynamicCI}{\rna}
\newcommand{\FASTsunflowWCPDynamicCIMIN}{\rna}
\newcommand{\FASTsunflowWCPDynamicCIMAX}{\rna}
\newcommand{\FASTsunflowFTOWCP}{18}
\newcommand{\FASTsunflowFTOWCPCI}{0.0}
\newcommand{\FASTsunflowFTOWCPCIMIN}{18}
\newcommand{\FASTsunflowFTOWCPCIMAX}{18}
\newcommand{\FASTsunflowFTOWCPDynamic}{210}
\newcommand{\FASTsunflowFTOWCPDynamicCI}{15}
\newcommand{\FASTsunflowFTOWCPDynamicCIMIN}{195}
\newcommand{\FASTsunflowFTOWCPDynamicCIMAX}{225}
\newcommand{\FASTsunflowREWCP}{19}
\newcommand{\FASTsunflowREWCPCI}{0.0}
\newcommand{\FASTsunflowREWCPCIMIN}{19}
\newcommand{\FASTsunflowREWCPCIMAX}{19}
\newcommand{\FASTsunflowREWCPDynamic}{246}
\newcommand{\FASTsunflowREWCPDynamicCI}{5.0}
\newcommand{\FASTsunflowREWCPDynamicCIMIN}{241}
\newcommand{\FASTsunflowREWCPDynamicCIMAX}{251}
\newcommand{\FASTsunflowDC}{\rna}
\newcommand{\FASTsunflowDCCI}{\rna}
\newcommand{\FASTsunflowDCCIMIN}{\rna}
\newcommand{\FASTsunflowDCCIMAX}{\rna}
\newcommand{\FASTsunflowDCDynamic}{\rna}
\newcommand{\FASTsunflowDCDynamicCI}{\rna}
\newcommand{\FASTsunflowDCDynamicCIMIN}{\rna}
\newcommand{\FASTsunflowDCDynamicCIMAX}{\rna}
\newcommand{\FASTsunflowFTODC}{19}
\newcommand{\FASTsunflowFTODCCI}{0.0}
\newcommand{\FASTsunflowFTODCCIMIN}{19}
\newcommand{\FASTsunflowFTODCCIMAX}{19}
\newcommand{\FASTsunflowFTODCDynamic}{403}
\newcommand{\FASTsunflowFTODCDynamicCI}{11}
\newcommand{\FASTsunflowFTODCDynamicCIMIN}{392}
\newcommand{\FASTsunflowFTODCDynamicCIMAX}{414}
\newcommand{\FASTsunflowREDC}{19}
\newcommand{\FASTsunflowREDCCI}{0.0}
\newcommand{\FASTsunflowREDCCIMIN}{19}
\newcommand{\FASTsunflowREDCCIMAX}{19}
\newcommand{\FASTsunflowREDCDynamic}{412}
\newcommand{\FASTsunflowREDCDynamicCI}{8.5}
\newcommand{\FASTsunflowREDCDynamicCIMIN}{403}
\newcommand{\FASTsunflowREDCDynamicCIMAX}{421}
\newcommand{\FASTsunflowCAPO}{\rna}
\newcommand{\FASTsunflowCAPOCI}{\rna}
\newcommand{\FASTsunflowCAPOCIMIN}{\rna}
\newcommand{\FASTsunflowCAPOCIMAX}{\rna}
\newcommand{\FASTsunflowCAPODynamic}{\rna}
\newcommand{\FASTsunflowCAPODynamicCI}{\rna}
\newcommand{\FASTsunflowCAPODynamicCIMIN}{\rna}
\newcommand{\FASTsunflowCAPODynamicCIMAX}{\rna}
\newcommand{\FASTsunflowFTOCAPO}{19}
\newcommand{\FASTsunflowFTOCAPOCI}{0.0}
\newcommand{\FASTsunflowFTOCAPOCIMIN}{19}
\newcommand{\FASTsunflowFTOCAPOCIMAX}{19}
\newcommand{\FASTsunflowFTOCAPODynamic}{416}
\newcommand{\FASTsunflowFTOCAPODynamicCI}{10}
\newcommand{\FASTsunflowFTOCAPODynamicCIMIN}{406}
\newcommand{\FASTsunflowFTOCAPODynamicCIMAX}{426}
\newcommand{\FASTsunflowRECAPO}{19}
\newcommand{\FASTsunflowRECAPOCI}{0.0}
\newcommand{\FASTsunflowRECAPOCIMIN}{19}
\newcommand{\FASTsunflowRECAPOCIMAX}{19}
\newcommand{\FASTsunflowRECAPODynamic}{415}
\newcommand{\FASTsunflowRECAPODynamicCI}{8.1}
\newcommand{\FASTsunflowRECAPODynamicCIMIN}{407}
\newcommand{\FASTsunflowRECAPODynamicCIMAX}{423}
\newcommand{\FASTsunflowAGGCAPO}{\rna}
\newcommand{\FASTsunflowAGGCAPOCI}{\rna}
\newcommand{\FASTsunflowAGGCAPOCIMIN}{\rna}
\newcommand{\FASTsunflowAGGCAPOCIMAX}{\rna}
\newcommand{\FASTsunflowAGGCAPODynamic}{\rna}
\newcommand{\FASTsunflowAGGCAPODynamicCI}{\rna}
\newcommand{\FASTsunflowAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTsunflowAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTtomcatEvents}{43}
\newcommand{\FASTtomcatNoFPEvents}{10}
\newcommand{\tomcatHBEventTotal}{44}
\newcommand{\tomcatHBNoFPEventTotal}{10}
\newcommand{\tomcatHBNoFPAccessTotal}{9.6}
\newcommand{\tomcatHBNoFPOtherTotal}{0.77}
\newcommand{\tomcatHBReadTotal}{54.9}
\newcommand{\tomcatHBWriteTotal}{37.6}
\newcommand{\tomcatHBNoFPAccessInCS}{2.87}
\newcommand{\tomcatHBNoFPAccessOutCS}{86.0}
\newcommand{\tomcatHBAcqRelTotal}{6.53}
\newcommand{\tomcatHBOtherTotal}{0.583}
\newcommand{\tomcatHBNoFPReadTotal}{5.7}
\newcommand{\tomcatHBReadInCS}{21.9}
\newcommand{\tomcatHBReadOutCS}{163}
\newcommand{\tomcatHBReadSameEp}{84.9}
\newcommand{\tomcatHBReadSharedSameEp}{<0.001}
\newcommand{\tomcatHBReadExclusive}{38}
\newcommand{\tomcatHBReadOwned}{\cna}
\newcommand{\tomcatHBReadShare}{0.301}
\newcommand{\tomcatHBReadShared}{61.7}
\newcommand{\tomcatHBReadSharedOwned}{\cna}
\newcommand{\tomcatHBNoFPHonestWriteTotal}{3.9}
\newcommand{\tomcatHBWriteInCS}{5.3}
\newcommand{\tomcatHBWriteOutCS}{114}
\newcommand{\tomcatHBNoFPWriteTotal}{3.9}
\newcommand{\tomcatHBWriteSameEp}{19.6}
\newcommand{\tomcatHBWriteExclusive}{66}
\newcommand{\tomcatHBWriteOwned}{\cna}
\newcommand{\tomcatHBWriteShared}{34}
\newcommand{\tomcatHBNoFPOtherEventTotal}{774544}
\newcommand{\tomcatHBAcqRelOtherTotal}{91.8}
\newcommand{\tomcatHBNoAcqRelOtherTotal}{63439}
\newcommand{\tomcatHBFork}{0.0583}
\newcommand{\tomcatHBJoin}{0.0236}
\newcommand{\tomcatHBPreWait}{0.011}
\newcommand{\tomcatHBPostWait}{0.00946}
\newcommand{\tomcatHBVolatileTotal}{96.9}
\newcommand{\tomcatHBClassInit}{0.389}
\newcommand{\tomcatHBClassAccess}{2.61}
\newcommand{\tomcatHBRaceTotal}{2499163}
\newcommand{\tomcatHBWrRdRace}{16.8}
\newcommand{\tomcatHBWrWrRace}{61.9}
\newcommand{\tomcatHBRdWrRace}{1.25}
\newcommand{\tomcatHBRdShWrRace}{20.0}
\newcommand{\tomcatHBHoldLocksTotal}{1.5}
\newcommand{\tomcatHBOneLockHeld}{<0.1}
\newcommand{\tomcatHBTwoNestedLocks}{<0.1}
\newcommand{\tomcatHBThreeNestedLocks}{<0.1}
\newcommand{\tomcatHBFourNestedLocks}{<0.1}
\newcommand{\tomcatHBFiveNestedLocks}{<0.1}
\newcommand{\tomcatHBSixNestedLocks}{<0.1}
\newcommand{\tomcatHBSevenNestedLocks}{<0.1}
\newcommand{\tomcatHBEightNestedLocks}{<0.1}
\newcommand{\tomcatHBNineNestedLocks}{<0.1}
\newcommand{\tomcatHBTenNestedLocks}{<0.1}
\newcommand{\tomcatHBHundredNestedLocks}{\cna}
\newcommand{\tomcatFTOHBEventTotal}{43}
\newcommand{\tomcatFTOHBNoFPEventTotal}{9.6}
\newcommand{\tomcatFTOHBNoFPAccessTotal}{8.8}
\newcommand{\tomcatFTOHBNoFPOtherTotal}{0.78}
\newcommand{\tomcatFTOHBReadTotal}{51.4}
\newcommand{\tomcatFTOHBWriteTotal}{40.5}
\newcommand{\tomcatFTOHBNoFPAccessInCS}{2.37}
\newcommand{\tomcatFTOHBNoFPAccessOutCS}{77.5}
\newcommand{\tomcatFTOHBAcqRelTotal}{7.03}
\newcommand{\tomcatFTOHBOtherTotal}{0.628}
\newcommand{\tomcatFTOHBNoFPReadTotal}{4.9}
\newcommand{\tomcatFTOHBReadInCS}{24.9}
\newcommand{\tomcatFTOHBReadOutCS}{173}
\newcommand{\tomcatFTOHBReadSameEp}{97.6}
\newcommand{\tomcatFTOHBReadSharedSameEp}{<0.001}
\newcommand{\tomcatFTOHBReadExclusive}{6.6}
\newcommand{\tomcatFTOHBReadOwned}{38.9}
\newcommand{\tomcatFTOHBReadShare}{6.87}
\newcommand{\tomcatFTOHBReadShared}{3.04}
\newcommand{\tomcatFTOHBReadSharedOwned}{44.6}
\newcommand{\tomcatFTOHBNoFPHonestWriteTotal}{3.9}
\newcommand{\tomcatFTOHBWriteInCS}{5.31}
\newcommand{\tomcatFTOHBWriteOutCS}{114}
\newcommand{\tomcatFTOHBNoFPWriteTotal}{3.9}
\newcommand{\tomcatFTOHBWriteSameEp}{19.6}
\newcommand{\tomcatFTOHBWriteExclusive}{50.6}
\newcommand{\tomcatFTOHBWriteOwned}{40.9}
\newcommand{\tomcatFTOHBWriteShared}{8.51}
\newcommand{\tomcatFTOHBNoFPOtherEventTotal}{775577}
\newcommand{\tomcatFTOHBAcqRelOtherTotal}{91.8}
\newcommand{\tomcatFTOHBNoAcqRelOtherTotal}{63558}
\newcommand{\tomcatFTOHBFork}{0.0582}
\newcommand{\tomcatFTOHBJoin}{0.0236}
\newcommand{\tomcatFTOHBPreWait}{0.011}
\newcommand{\tomcatFTOHBPostWait}{0.00944}
\newcommand{\tomcatFTOHBVolatileTotal}{96.9}
\newcommand{\tomcatFTOHBClassInit}{0.389}
\newcommand{\tomcatFTOHBClassAccess}{2.57}
\newcommand{\tomcatFTOHBRaceTotal}{1880304}
\newcommand{\tomcatFTOHBWrRdRace}{17.6}
\newcommand{\tomcatFTOHBWrWrRace}{0.0}
\newcommand{\tomcatFTOHBRdWrRace}{66.4}
\newcommand{\tomcatFTOHBRdShWrRace}{16.1}
\newcommand{\tomcatFTOHBHoldLocksTotal}{1.2}
\newcommand{\tomcatFTOHBOneLockHeld}{<0.1}
\newcommand{\tomcatFTOHBTwoNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBThreeNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBFourNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBFiveNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBSixNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBSevenNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBEightNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBNineNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBTenNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBHundredNestedLocks}{\cna}
\newcommand{\tomcatFTOWCPEventTotal}{43}
\newcommand{\tomcatFTOWCPNoFPEventTotal}{9.6}
\newcommand{\tomcatFTOWCPNoFPAccessTotal}{8.9}
\newcommand{\tomcatFTOWCPNoFPOtherTotal}{0.77}
\newcommand{\tomcatFTOWCPReadTotal}{51.6}
\newcommand{\tomcatFTOWCPWriteTotal}{40.3}
\newcommand{\tomcatFTOWCPNoFPAccessInCS}{2.41}
\newcommand{\tomcatFTOWCPNoFPAccessOutCS}{78.0}
\newcommand{\tomcatFTOWCPAcqRelTotal}{7.13}
\newcommand{\tomcatFTOWCPOtherTotal}{0.636}
\newcommand{\tomcatFTOWCPNoFPReadTotal}{5.0}
\newcommand{\tomcatFTOWCPReadInCS}{25.5}
\newcommand{\tomcatFTOWCPReadOutCS}{171}
\newcommand{\tomcatFTOWCPReadSameEp}{96.9}
\newcommand{\tomcatFTOWCPReadSharedSameEp}{<0.001}
\newcommand{\tomcatFTOWCPReadExclusive}{6.02}
\newcommand{\tomcatFTOWCPReadOwned}{36.9}
\newcommand{\tomcatFTOWCPReadShare}{6.56}
\newcommand{\tomcatFTOWCPReadShared}{2.88}
\newcommand{\tomcatFTOWCPReadSharedOwned}{47.6}
\newcommand{\tomcatFTOWCPNoFPHonestWriteTotal}{3.9}
\newcommand{\tomcatFTOWCPWriteInCS}{5.32}
\newcommand{\tomcatFTOWCPWriteOutCS}{114}
\newcommand{\tomcatFTOWCPNoFPWriteTotal}{3.9}
\newcommand{\tomcatFTOWCPWriteSameEp}{19.6}
\newcommand{\tomcatFTOWCPWriteExclusive}{49.8}
\newcommand{\tomcatFTOWCPWriteOwned}{42.1}
\newcommand{\tomcatFTOWCPWriteShared}{8.19}
\newcommand{\tomcatFTOWCPNoFPOtherEventTotal}{774203}
\newcommand{\tomcatFTOWCPAcqRelOtherTotal}{91.8}
\newcommand{\tomcatFTOWCPNoAcqRelOtherTotal}{63377}
\newcommand{\tomcatFTOWCPFork}{0.0584}
\newcommand{\tomcatFTOWCPJoin}{0.0237}
\newcommand{\tomcatFTOWCPPreWait}{0.011}
\newcommand{\tomcatFTOWCPPostWait}{0.00947}
\newcommand{\tomcatFTOWCPVolatileTotal}{97.0}
\newcommand{\tomcatFTOWCPClassInit}{0.39}
\newcommand{\tomcatFTOWCPClassAccess}{2.55}
\newcommand{\tomcatFTOWCPRaceTotal}{1805906}
\newcommand{\tomcatFTOWCPWrRdRace}{17.5}
\newcommand{\tomcatFTOWCPWrWrRace}{0.0}
\newcommand{\tomcatFTOWCPRdWrRace}{66.5}
\newcommand{\tomcatFTOWCPRdShWrRace}{16.0}
\newcommand{\tomcatFTOWCPHoldLocksTotal}{1.3}
\newcommand{\tomcatFTOWCPOneLockHeld}{<0.1}
\newcommand{\tomcatFTOWCPTwoNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPThreeNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPFourNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPFiveNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPSixNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPSevenNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPEightNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPNineNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPTenNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPHundredNestedLocks}{\cna}
\newcommand{\tomcatREWCPEventTotal}{45}
\newcommand{\tomcatREWCPNoFPEventTotal}{9.7}
\newcommand{\tomcatREWCPNoFPAccessTotal}{8.9}
\newcommand{\tomcatREWCPNoFPOtherTotal}{0.78}
\newcommand{\tomcatREWCPReadTotal}{51.7}
\newcommand{\tomcatREWCPWriteTotal}{40.3}
\newcommand{\tomcatREWCPNoFPAccessInCS}{5.95}
\newcommand{\tomcatREWCPNoFPAccessOutCS}{74.7}
\newcommand{\tomcatREWCPAcqRelTotal}{6.81}
\newcommand{\tomcatREWCPOtherTotal}{0.608}
\newcommand{\tomcatREWCPNoFPReadTotal}{5.0}
\newcommand{\tomcatREWCPReadInCS}{28.5}
\newcommand{\tomcatREWCPReadOutCS}{171}
\newcommand{\tomcatREWCPReadSameEp}{99}
\newcommand{\tomcatREWCPReadSharedSameEp}{<0.001}
\newcommand{\tomcatREWCPReadExclusive}{5.77}
\newcommand{\tomcatREWCPReadOwned}{36.6}
\newcommand{\tomcatREWCPReadShare}{6.86}
\newcommand{\tomcatREWCPReadShared}{3.0}
\newcommand{\tomcatREWCPReadSharedOwned}{47.8}
\newcommand{\tomcatREWCPNoFPHonestWriteTotal}{3.9}
\newcommand{\tomcatREWCPWriteInCS}{11.1}
\newcommand{\tomcatREWCPWriteOutCS}{114}
\newcommand{\tomcatREWCPNoFPWriteTotal}{3.9}
\newcommand{\tomcatREWCPWriteSameEp}{25.2}
\newcommand{\tomcatREWCPWriteExclusive}{50.4}
\newcommand{\tomcatREWCPWriteOwned}{41}
\newcommand{\tomcatREWCPWriteShared}{8.55}
\newcommand{\tomcatREWCPNoFPOtherEventTotal}{776723}
\newcommand{\tomcatREWCPAcqRelOtherTotal}{91.8}
\newcommand{\tomcatREWCPNoAcqRelOtherTotal}{63627}
\newcommand{\tomcatREWCPFork}{0.0582}
\newcommand{\tomcatREWCPJoin}{0.0236}
\newcommand{\tomcatREWCPPreWait}{0.011}
\newcommand{\tomcatREWCPPostWait}{0.00943}
\newcommand{\tomcatREWCPVolatileTotal}{96.9}
\newcommand{\tomcatREWCPClassInit}{0.404}
\newcommand{\tomcatREWCPClassAccess}{2.6}
\newcommand{\tomcatREWCPRaceTotal}{1870127}
\newcommand{\tomcatREWCPWrRdRace}{17.5}
\newcommand{\tomcatREWCPWrWrRace}{0.0}
\newcommand{\tomcatREWCPRdWrRace}{66.5}
\newcommand{\tomcatREWCPRdShWrRace}{16.0}
\newcommand{\tomcatREWCPHoldLocksTotal}{1.3}
\newcommand{\tomcatREWCPOneLockHeld}{<0.1}
\newcommand{\tomcatREWCPTwoNestedLocks}{<0.1}
\newcommand{\tomcatREWCPThreeNestedLocks}{<0.1}
\newcommand{\tomcatREWCPFourNestedLocks}{<0.1}
\newcommand{\tomcatREWCPFiveNestedLocks}{<0.1}
\newcommand{\tomcatREWCPSixNestedLocks}{<0.1}
\newcommand{\tomcatREWCPSevenNestedLocks}{<0.1}
\newcommand{\tomcatREWCPEightNestedLocks}{<0.1}
\newcommand{\tomcatREWCPNineNestedLocks}{<0.1}
\newcommand{\tomcatREWCPTenNestedLocks}{<0.1}
\newcommand{\tomcatREWCPHundredNestedLocks}{\cna}
\newcommand{\tomcatFTODCEventTotal}{43}
\newcommand{\tomcatFTODCNoFPEventTotal}{9.7}
\newcommand{\tomcatFTODCNoFPAccessTotal}{8.9}
\newcommand{\tomcatFTODCNoFPOtherTotal}{0.78}
\newcommand{\tomcatFTODCReadTotal}{51.6}
\newcommand{\tomcatFTODCWriteTotal}{40.3}
\newcommand{\tomcatFTODCNoFPAccessInCS}{2.4}
\newcommand{\tomcatFTODCNoFPAccessOutCS}{77.8}
\newcommand{\tomcatFTODCAcqRelTotal}{7.11}
\newcommand{\tomcatFTODCOtherTotal}{0.635}
\newcommand{\tomcatFTODCNoFPReadTotal}{5.0}
\newcommand{\tomcatFTODCReadInCS}{25.5}
\newcommand{\tomcatFTODCReadOutCS}{171}
\newcommand{\tomcatFTODCReadSameEp}{96.6}
\newcommand{\tomcatFTODCReadSharedSameEp}{<0.001}
\newcommand{\tomcatFTODCReadExclusive}{6.02}
\newcommand{\tomcatFTODCReadOwned}{36.9}
\newcommand{\tomcatFTODCReadShare}{6.61}
\newcommand{\tomcatFTODCReadShared}{2.96}
\newcommand{\tomcatFTODCReadSharedOwned}{47.5}
\newcommand{\tomcatFTODCNoFPHonestWriteTotal}{3.9}
\newcommand{\tomcatFTODCWriteInCS}{5.34}
\newcommand{\tomcatFTODCWriteOutCS}{114}
\newcommand{\tomcatFTODCNoFPWriteTotal}{3.9}
\newcommand{\tomcatFTODCWriteSameEp}{19.6}
\newcommand{\tomcatFTODCWriteExclusive}{50}
\newcommand{\tomcatFTODCWriteOwned}{41.8}
\newcommand{\tomcatFTODCWriteShared}{8.25}
\newcommand{\tomcatFTODCNoFPOtherEventTotal}{776460}
\newcommand{\tomcatFTODCAcqRelOtherTotal}{91.8}
\newcommand{\tomcatFTODCNoAcqRelOtherTotal}{63641}
\newcommand{\tomcatFTODCFork}{0.0581}
\newcommand{\tomcatFTODCJoin}{0.0236}
\newcommand{\tomcatFTODCPreWait}{0.011}
\newcommand{\tomcatFTODCPostWait}{0.00943}
\newcommand{\tomcatFTODCVolatileTotal}{96.9}
\newcommand{\tomcatFTODCClassInit}{0.388}
\newcommand{\tomcatFTODCClassAccess}{2.57}
\newcommand{\tomcatFTODCRaceTotal}{1828079}
\newcommand{\tomcatFTODCWrRdRace}{17.5}
\newcommand{\tomcatFTODCWrWrRace}{0.0}
\newcommand{\tomcatFTODCRdWrRace}{66.5}
\newcommand{\tomcatFTODCRdShWrRace}{16.0}
\newcommand{\tomcatFTODCHoldLocksTotal}{1.3}
\newcommand{\tomcatFTODCOneLockHeld}{<0.1}
\newcommand{\tomcatFTODCTwoNestedLocks}{<0.1}
\newcommand{\tomcatFTODCThreeNestedLocks}{<0.1}
\newcommand{\tomcatFTODCFourNestedLocks}{<0.1}
\newcommand{\tomcatFTODCFiveNestedLocks}{<0.1}
\newcommand{\tomcatFTODCSixNestedLocks}{<0.1}
\newcommand{\tomcatFTODCSevenNestedLocks}{<0.1}
\newcommand{\tomcatFTODCEightNestedLocks}{<0.1}
\newcommand{\tomcatFTODCNineNestedLocks}{<0.1}
\newcommand{\tomcatFTODCTenNestedLocks}{<0.1}
\newcommand{\tomcatFTODCHundredNestedLocks}{\cna}
\newcommand{\tomcatREDCEventTotal}{45}
\newcommand{\tomcatREDCNoFPEventTotal}{9.7}
\newcommand{\tomcatREDCNoFPAccessTotal}{8.9}
\newcommand{\tomcatREDCNoFPOtherTotal}{0.77}
\newcommand{\tomcatREDCReadTotal}{51.8}
\newcommand{\tomcatREDCWriteTotal}{40.2}
\newcommand{\tomcatREDCNoFPAccessInCS}{7.25}
\newcommand{\tomcatREDCNoFPAccessOutCS}{73.8}
\newcommand{\tomcatREDCAcqRelTotal}{6.73}
\newcommand{\tomcatREDCOtherTotal}{0.602}
\newcommand{\tomcatREDCNoFPReadTotal}{5.0}
\newcommand{\tomcatREDCReadInCS}{30}
\newcommand{\tomcatREDCReadOutCS}{170}
\newcommand{\tomcatREDCReadSameEp}{100}
\newcommand{\tomcatREDCReadSharedSameEp}{<0.001}
\newcommand{\tomcatREDCReadExclusive}{5.8}
\newcommand{\tomcatREDCReadOwned}{36.9}
\newcommand{\tomcatREDCReadShare}{6.82}
\newcommand{\tomcatREDCReadShared}{2.98}
\newcommand{\tomcatREDCReadSharedOwned}{47.6}
\newcommand{\tomcatREDCNoFPHonestWriteTotal}{3.9}
\newcommand{\tomcatREDCWriteInCS}{12.9}
\newcommand{\tomcatREDCWriteOutCS}{114}
\newcommand{\tomcatREDCNoFPWriteTotal}{3.9}
\newcommand{\tomcatREDCWriteSameEp}{27}
\newcommand{\tomcatREDCWriteExclusive}{50.3}
\newcommand{\tomcatREDCWriteOwned}{41.2}
\newcommand{\tomcatREDCWriteShared}{8.52}
\newcommand{\tomcatREDCNoFPOtherEventTotal}{774174}
\newcommand{\tomcatREDCAcqRelOtherTotal}{91.8}
\newcommand{\tomcatREDCNoAcqRelOtherTotal}{63564}
\newcommand{\tomcatREDCFork}{0.0582}
\newcommand{\tomcatREDCJoin}{0.0236}
\newcommand{\tomcatREDCPreWait}{0.011}
\newcommand{\tomcatREDCPostWait}{0.00944}
\newcommand{\tomcatREDCVolatileTotal}{96.9}
\newcommand{\tomcatREDCClassInit}{0.42}
\newcommand{\tomcatREDCClassAccess}{2.6}
\newcommand{\tomcatREDCRaceTotal}{1853955}
\newcommand{\tomcatREDCWrRdRace}{17.5}
\newcommand{\tomcatREDCWrWrRace}{0.0}
\newcommand{\tomcatREDCRdWrRace}{66.4}
\newcommand{\tomcatREDCRdShWrRace}{16.0}
\newcommand{\tomcatREDCHoldLocksTotal}{1.3}
\newcommand{\tomcatREDCOneLockHeld}{<0.1}
\newcommand{\tomcatREDCTwoNestedLocks}{<0.1}
\newcommand{\tomcatREDCThreeNestedLocks}{<0.1}
\newcommand{\tomcatREDCFourNestedLocks}{<0.1}
\newcommand{\tomcatREDCFiveNestedLocks}{<0.1}
\newcommand{\tomcatREDCSixNestedLocks}{<0.1}
\newcommand{\tomcatREDCSevenNestedLocks}{<0.1}
\newcommand{\tomcatREDCEightNestedLocks}{<0.1}
\newcommand{\tomcatREDCNineNestedLocks}{<0.1}
\newcommand{\tomcatREDCTenNestedLocks}{<0.1}
\newcommand{\tomcatREDCHundredNestedLocks}{\cna}
\newcommand{\tomcatFTOCAPOEventTotal}{43}
\newcommand{\tomcatFTOCAPONoFPEventTotal}{9.6}
\newcommand{\tomcatFTOCAPONoFPAccessTotal}{8.9}
\newcommand{\tomcatFTOCAPONoFPOtherTotal}{0.77}
\newcommand{\tomcatFTOCAPOReadTotal}{51.6}
\newcommand{\tomcatFTOCAPOWriteTotal}{40.3}
\newcommand{\tomcatFTOCAPONoFPAccessInCS}{2.36}
\newcommand{\tomcatFTOCAPONoFPAccessOutCS}{77.4}
\newcommand{\tomcatFTOCAPOAcqRelTotal}{7.01}
\newcommand{\tomcatFTOCAPOOtherTotal}{0.625}
\newcommand{\tomcatFTOCAPONoFPReadTotal}{5.0}
\newcommand{\tomcatFTOCAPOReadInCS}{25.5}
\newcommand{\tomcatFTOCAPOReadOutCS}{171}
\newcommand{\tomcatFTOCAPOReadSameEp}{96.8}
\newcommand{\tomcatFTOCAPOReadSharedSameEp}{<0.001}
\newcommand{\tomcatFTOCAPOReadExclusive}{5.87}
\newcommand{\tomcatFTOCAPOReadOwned}{36.6}
\newcommand{\tomcatFTOCAPOReadShare}{6.87}
\newcommand{\tomcatFTOCAPOReadShared}{3.02}
\newcommand{\tomcatFTOCAPOReadSharedOwned}{47.6}
\newcommand{\tomcatFTOCAPONoFPHonestWriteTotal}{3.9}
\newcommand{\tomcatFTOCAPOWriteInCS}{5.33}
\newcommand{\tomcatFTOCAPOWriteOutCS}{114}
\newcommand{\tomcatFTOCAPONoFPWriteTotal}{3.9}
\newcommand{\tomcatFTOCAPOWriteSameEp}{19.6}
\newcommand{\tomcatFTOCAPOWriteExclusive}{51}
\newcommand{\tomcatFTOCAPOWriteOwned}{40.5}
\newcommand{\tomcatFTOCAPOWriteShared}{8.57}
\newcommand{\tomcatFTOCAPONoFPOtherEventTotal}{774586}
\newcommand{\tomcatFTOCAPOAcqRelOtherTotal}{91.8}
\newcommand{\tomcatFTOCAPONoAcqRelOtherTotal}{63465}
\newcommand{\tomcatFTOCAPOFork}{0.0583}
\newcommand{\tomcatFTOCAPOJoin}{0.0236}
\newcommand{\tomcatFTOCAPOPreWait}{0.011}
\newcommand{\tomcatFTOCAPOPostWait}{0.00945}
\newcommand{\tomcatFTOCAPOVolatileTotal}{96.9}
\newcommand{\tomcatFTOCAPOClassInit}{0.389}
\newcommand{\tomcatFTOCAPOClassAccess}{2.6}
\newcommand{\tomcatFTOCAPORaceTotal}{1893071}
\newcommand{\tomcatFTOCAPOWrRdRace}{17.6}
\newcommand{\tomcatFTOCAPOWrWrRace}{0.0}
\newcommand{\tomcatFTOCAPORdWrRace}{66.4}
\newcommand{\tomcatFTOCAPORdShWrRace}{16.0}
\newcommand{\tomcatFTOCAPOHoldLocksTotal}{1.3}
\newcommand{\tomcatFTOCAPOOneLockHeld}{<0.1}
\newcommand{\tomcatFTOCAPOTwoNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOThreeNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOFourNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOFiveNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOSixNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOSevenNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOEightNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPONineNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOTenNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\tomcatRECAPOEventTotal}{43}
\newcommand{\tomcatRECAPONoFPEventTotal}{9.6}
\newcommand{\tomcatRECAPONoFPAccessTotal}{8.9}
\newcommand{\tomcatRECAPONoFPOtherTotal}{0.77}
\newcommand{\tomcatRECAPOReadTotal}{51.7}
\newcommand{\tomcatRECAPOWriteTotal}{40.3}
\newcommand{\tomcatRECAPONoFPAccessInCS}{3.44}
\newcommand{\tomcatRECAPONoFPAccessOutCS}{76.6}
\newcommand{\tomcatRECAPOAcqRelTotal}{6.94}
\newcommand{\tomcatRECAPOOtherTotal}{0.62}
\newcommand{\tomcatRECAPONoFPReadTotal}{5.0}
\newcommand{\tomcatRECAPOReadInCS}{26.6}
\newcommand{\tomcatRECAPOReadOutCS}{171}
\newcommand{\tomcatRECAPOReadSameEp}{97.7}
\newcommand{\tomcatRECAPOReadSharedSameEp}{<0.001}
\newcommand{\tomcatRECAPOReadExclusive}{5.66}
\newcommand{\tomcatRECAPOReadOwned}{36.6}
\newcommand{\tomcatRECAPOReadShare}{6.96}
\newcommand{\tomcatRECAPOReadShared}{3.02}
\newcommand{\tomcatRECAPOReadSharedOwned}{47.8}
\newcommand{\tomcatRECAPONoFPHonestWriteTotal}{3.9}
\newcommand{\tomcatRECAPOWriteInCS}{6.88}
\newcommand{\tomcatRECAPOWriteOutCS}{114}
\newcommand{\tomcatRECAPONoFPWriteTotal}{3.9}
\newcommand{\tomcatRECAPOWriteSameEp}{21.1}
\newcommand{\tomcatRECAPOWriteExclusive}{50.6}
\newcommand{\tomcatRECAPOWriteOwned}{40.7}
\newcommand{\tomcatRECAPOWriteShared}{8.68}
\newcommand{\tomcatRECAPONoFPOtherEventTotal}{774087}
\newcommand{\tomcatRECAPOAcqRelOtherTotal}{91.8}
\newcommand{\tomcatRECAPONoAcqRelOtherTotal}{63520}
\newcommand{\tomcatRECAPOFork}{0.0582}
\newcommand{\tomcatRECAPOJoin}{0.0236}
\newcommand{\tomcatRECAPOPreWait}{0.011}
\newcommand{\tomcatRECAPOPostWait}{0.00945}
\newcommand{\tomcatRECAPOVolatileTotal}{96.9}
\newcommand{\tomcatRECAPOClassInit}{0.403}
\newcommand{\tomcatRECAPOClassAccess}{2.6}
\newcommand{\tomcatRECAPORaceTotal}{1888210}
\newcommand{\tomcatRECAPOWrRdRace}{17.6}
\newcommand{\tomcatRECAPOWrWrRace}{0.0}
\newcommand{\tomcatRECAPORdWrRace}{66.4}
\newcommand{\tomcatRECAPORdShWrRace}{16.1}
\newcommand{\tomcatRECAPOHoldLocksTotal}{1.3}
\newcommand{\tomcatRECAPOOneLockHeld}{<0.1}
\newcommand{\tomcatRECAPOTwoNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOThreeNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOFourNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOFiveNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOSixNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOSevenNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOEightNestedLocks}{<0.1}
\newcommand{\tomcatRECAPONineNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOTenNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOHundredNestedLocks}{\cna}
\newcommand{\FASTtomcatMaxLiveThreads}{55}
\newcommand{\FASTtomcatTotalThreads}{55}
\newcommand{\FASTtomcatBaseTime}{0.92}
\newcommand{\FASTtomcatBaseTimeCI}{5.4}
\newcommand{\FASTtomcatEmptyTime}{\rna}
\newcommand{\FASTtomcatEmptyTimeCI}{\rna}
\newcommand{\FASTtomcatEmptyTimeCIMIN}{\rna}
\newcommand{\FASTtomcatEmptyTimeCIMAX}{\rna}
\newcommand{\FASTtomcatFTTime}{29}
\newcommand{\FASTtomcatFTTimeCI}{1.2}
\newcommand{\FASTtomcatHBTime}{18}
\newcommand{\FASTtomcatHBTimeCI}{0.53}
\newcommand{\FASTtomcatFTOHBTime}{18}
\newcommand{\FASTtomcatFTOHBTimeCI}{0.58}
\newcommand{\FASTtomcatWCPTime}{\rna}
\newcommand{\FASTtomcatWCPTimeCI}{\rna}
\newcommand{\FASTtomcatWCPTimeCIMIN}{\rna}
\newcommand{\FASTtomcatWCPTimeCIMAX}{\rna}
\newcommand{\FASTtomcatFTOWCPTime}{20}
\newcommand{\FASTtomcatFTOWCPTimeCI}{0.77}
\newcommand{\FASTtomcatREWCPTime}{23}
\newcommand{\FASTtomcatREWCPTimeCI}{1.2}
\newcommand{\FASTtomcatDCTime}{\rna}
\newcommand{\FASTtomcatDCTimeCI}{\rna}
\newcommand{\FASTtomcatDCTimeCIMIN}{\rna}
\newcommand{\FASTtomcatDCTimeCIMAX}{\rna}
\newcommand{\FASTtomcatFTODCTime}{22}
\newcommand{\FASTtomcatFTODCTimeCI}{0.74}
\newcommand{\FASTtomcatREDCTime}{24}
\newcommand{\FASTtomcatREDCTimeCI}{1.4}
\newcommand{\FASTtomcatCAPOTime}{\rna}
\newcommand{\FASTtomcatCAPOTimeCI}{\rna}
\newcommand{\FASTtomcatCAPOTimeCIMIN}{\rna}
\newcommand{\FASTtomcatCAPOTimeCIMAX}{\rna}
\newcommand{\FASTtomcatFTOCAPOTime}{19}
\newcommand{\FASTtomcatFTOCAPOTimeCI}{0.45}
\newcommand{\FASTtomcatRECAPOTime}{20}
\newcommand{\FASTtomcatRECAPOTimeCI}{1.1}
\newcommand{\FASTtomcatAGGCAPOTime}{\rna}
\newcommand{\FASTtomcatAGGCAPOTimeCI}{\rna}
\newcommand{\FASTtomcatAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTtomcatAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTtomcatStaticTime}{\rzero}
\newcommand{\FASTtomcatDynamicTime}{\rzero}
\newcommand{\FASTtomcatBaseMem}{510}
\newcommand{\FASTtomcatBaseMemCI}{3.0}
\newcommand{\FASTtomcatFTMem}{81}
\newcommand{\FASTtomcatFTMemCI}{13.0}
\newcommand{\FASTtomcatHBMem}{59}
\newcommand{\FASTtomcatHBMemCI}{7.8}
\newcommand{\FASTtomcatFTOHBMem}{67}
\newcommand{\FASTtomcatFTOHBMemCI}{7.9}
\newcommand{\FASTtomcatWCPMem}{\memna}
\newcommand{\FASTtomcatWCPMemCI}{\memna}
\newcommand{\FASTtomcatWCPMemCIMIN}{\memna}
\newcommand{\FASTtomcatWCPMemCIMAX}{\memna}
\newcommand{\FASTtomcatFTOWCPMem}{75}
\newcommand{\FASTtomcatFTOWCPMemCI}{10.0}
\newcommand{\FASTtomcatREWCPMem}{63}
\newcommand{\FASTtomcatREWCPMemCI}{2.5}
\newcommand{\FASTtomcatDCMem}{\memna}
\newcommand{\FASTtomcatDCMemCI}{\memna}
\newcommand{\FASTtomcatDCMemCIMIN}{\memna}
\newcommand{\FASTtomcatDCMemCIMAX}{\memna}
\newcommand{\FASTtomcatFTODCMem}{79}
\newcommand{\FASTtomcatFTODCMemCI}{6.3}
\newcommand{\FASTtomcatREDCMem}{75}
\newcommand{\FASTtomcatREDCMemCI}{4.5}
\newcommand{\FASTtomcatCAPOMem}{\memna}
\newcommand{\FASTtomcatCAPOMemCI}{\memna}
\newcommand{\FASTtomcatCAPOMemCIMIN}{\memna}
\newcommand{\FASTtomcatCAPOMemCIMAX}{\memna}
\newcommand{\FASTtomcatFTOCAPOMem}{81}
\newcommand{\FASTtomcatFTOCAPOMemCI}{13.0}
\newcommand{\FASTtomcatRECAPOMem}{77}
\newcommand{\FASTtomcatRECAPOMemCI}{7.1}
\newcommand{\FASTtomcatAGGCAPOMem}{\memna}
\newcommand{\FASTtomcatAGGCAPOMemCI}{\memna}
\newcommand{\FASTtomcatAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTtomcatAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTtomcatEventsCI}{510,908}
\newcommand{\FASTtomcatEventsCIMIN}{42,824,037}
\newcommand{\FASTtomcatEventsCIMAX}{43,845,853}
\newcommand{\FASTtomcatNoFPEventsCI}{240,869}
\newcommand{\FASTtomcatNoFPEventsCIMIN}{9,999,117}
\newcommand{\FASTtomcatNoFPEventsCIMAX}{10,480,855}
\newcommand{\FASTtomcatFT}{422}
\newcommand{\FASTtomcatFTCI}{6.9}
\newcommand{\FASTtomcatFTCIMIN}{415}
\newcommand{\FASTtomcatFTCIMAX}{429}
\newcommand{\FASTtomcatFTDynamic}{3,569,142}
\newcommand{\FASTtomcatFTDynamicCI}{97,807}
\newcommand{\FASTtomcatFTDynamicCIMIN}{3,471,335}
\newcommand{\FASTtomcatFTDynamicCIMAX}{3,666,949}
\newcommand{\FASTtomcatHB}{640}
\newcommand{\FASTtomcatHBCI}{5.7}
\newcommand{\FASTtomcatHBCIMIN}{634}
\newcommand{\FASTtomcatHBCIMAX}{646}
\newcommand{\FASTtomcatHBDynamic}{2,019,955}
\newcommand{\FASTtomcatHBDynamicCI}{59,948}
\newcommand{\FASTtomcatHBDynamicCIMIN}{1,960,007}
\newcommand{\FASTtomcatHBDynamicCIMAX}{2,079,903}
\newcommand{\FASTtomcatFTOHB}{597}
\newcommand{\FASTtomcatFTOHBCI}{1.6}
\newcommand{\FASTtomcatFTOHBCIMIN}{595}
\newcommand{\FASTtomcatFTOHBCIMAX}{599}
\newcommand{\FASTtomcatFTOHBDynamic}{1,880,275}
\newcommand{\FASTtomcatFTOHBDynamicCI}{63,435}
\newcommand{\FASTtomcatFTOHBDynamicCIMIN}{1,816,840}
\newcommand{\FASTtomcatFTOHBDynamicCIMAX}{1,943,710}
\newcommand{\FASTtomcatWCP}{\rna}
\newcommand{\FASTtomcatWCPCI}{\rna}
\newcommand{\FASTtomcatWCPCIMIN}{\rna}
\newcommand{\FASTtomcatWCPCIMAX}{\rna}
\newcommand{\FASTtomcatWCPDynamic}{\rna}
\newcommand{\FASTtomcatWCPDynamicCI}{\rna}
\newcommand{\FASTtomcatWCPDynamicCIMIN}{\rna}
\newcommand{\FASTtomcatWCPDynamicCIMAX}{\rna}
\newcommand{\FASTtomcatFTOWCP}{599}
\newcommand{\FASTtomcatFTOWCPCI}{2.2}
\newcommand{\FASTtomcatFTOWCPCIMIN}{597}
\newcommand{\FASTtomcatFTOWCPCIMAX}{601}
\newcommand{\FASTtomcatFTOWCPDynamic}{1,805,906}
\newcommand{\FASTtomcatFTOWCPDynamicCI}{30,438}
\newcommand{\FASTtomcatFTOWCPDynamicCIMIN}{1,775,468}
\newcommand{\FASTtomcatFTOWCPDynamicCIMAX}{1,836,344}
\newcommand{\FASTtomcatREWCP}{603}
\newcommand{\FASTtomcatREWCPCI}{4.9}
\newcommand{\FASTtomcatREWCPCIMIN}{598}
\newcommand{\FASTtomcatREWCPCIMAX}{608}
\newcommand{\FASTtomcatREWCPDynamic}{1,870,062}
\newcommand{\FASTtomcatREWCPDynamicCI}{70,056}
\newcommand{\FASTtomcatREWCPDynamicCIMIN}{1,800,006}
\newcommand{\FASTtomcatREWCPDynamicCIMAX}{1,940,118}
\newcommand{\FASTtomcatDC}{\rna}
\newcommand{\FASTtomcatDCCI}{\rna}
\newcommand{\FASTtomcatDCCIMIN}{\rna}
\newcommand{\FASTtomcatDCCIMAX}{\rna}
\newcommand{\FASTtomcatDCDynamic}{\rna}
\newcommand{\FASTtomcatDCDynamicCI}{\rna}
\newcommand{\FASTtomcatDCDynamicCIMIN}{\rna}
\newcommand{\FASTtomcatDCDynamicCIMAX}{\rna}
\newcommand{\FASTtomcatFTODC}{603}
\newcommand{\FASTtomcatFTODCCI}{1.9}
\newcommand{\FASTtomcatFTODCCIMIN}{601}
\newcommand{\FASTtomcatFTODCCIMAX}{605}
\newcommand{\FASTtomcatFTODCDynamic}{1,828,079}
\newcommand{\FASTtomcatFTODCDynamicCI}{74,474}
\newcommand{\FASTtomcatFTODCDynamicCIMIN}{1,753,605}
\newcommand{\FASTtomcatFTODCDynamicCIMAX}{1,902,553}
\newcommand{\FASTtomcatREDC}{605}
\newcommand{\FASTtomcatREDCCI}{2.9}
\newcommand{\FASTtomcatREDCCIMIN}{602}
\newcommand{\FASTtomcatREDCCIMAX}{608}
\newcommand{\FASTtomcatREDCDynamic}{1,853,955}
\newcommand{\FASTtomcatREDCDynamicCI}{72,503}
\newcommand{\FASTtomcatREDCDynamicCIMIN}{1,781,452}
\newcommand{\FASTtomcatREDCDynamicCIMAX}{1,926,458}
\newcommand{\FASTtomcatCAPO}{\rna}
\newcommand{\FASTtomcatCAPOCI}{\rna}
\newcommand{\FASTtomcatCAPOCIMIN}{\rna}
\newcommand{\FASTtomcatCAPOCIMAX}{\rna}
\newcommand{\FASTtomcatCAPODynamic}{\rna}
\newcommand{\FASTtomcatCAPODynamicCI}{\rna}
\newcommand{\FASTtomcatCAPODynamicCIMIN}{\rna}
\newcommand{\FASTtomcatCAPODynamicCIMAX}{\rna}
\newcommand{\FASTtomcatFTOCAPO}{608}
\newcommand{\FASTtomcatFTOCAPOCI}{4.6}
\newcommand{\FASTtomcatFTOCAPOCIMIN}{603}
\newcommand{\FASTtomcatFTOCAPOCIMAX}{613}
\newcommand{\FASTtomcatFTOCAPODynamic}{1,893,071}
\newcommand{\FASTtomcatFTOCAPODynamicCI}{55,409}
\newcommand{\FASTtomcatFTOCAPODynamicCIMIN}{1,837,662}
\newcommand{\FASTtomcatFTOCAPODynamicCIMAX}{1,948,480}
\newcommand{\FASTtomcatRECAPO}{608}
\newcommand{\FASTtomcatRECAPOCI}{4.7}
\newcommand{\FASTtomcatRECAPOCIMIN}{603}
\newcommand{\FASTtomcatRECAPOCIMAX}{613}
\newcommand{\FASTtomcatRECAPODynamic}{1,888,181}
\newcommand{\FASTtomcatRECAPODynamicCI}{84,583}
\newcommand{\FASTtomcatRECAPODynamicCIMIN}{1,803,598}
\newcommand{\FASTtomcatRECAPODynamicCIMAX}{1,972,764}
\newcommand{\FASTtomcatAGGCAPO}{\rna}
\newcommand{\FASTtomcatAGGCAPOCI}{\rna}
\newcommand{\FASTtomcatAGGCAPOCIMIN}{\rna}
\newcommand{\FASTtomcatAGGCAPOCIMAX}{\rna}
\newcommand{\FASTtomcatAGGCAPODynamic}{\rna}
\newcommand{\FASTtomcatAGGCAPODynamicCI}{\rna}
\newcommand{\FASTtomcatAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTtomcatAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTxalanEvents}{630}
\newcommand{\FASTxalanNoFPEvents}{48}
\newcommand{\xalanHBEventTotal}{630}
\newcommand{\xalanHBNoFPEventTotal}{240}
\newcommand{\xalanHBNoFPAccessTotal}{230}
\newcommand{\xalanHBNoFPOtherTotal}{8.9}
\newcommand{\xalanHBReadTotal}{79.5}
\newcommand{\xalanHBWriteTotal}{16.7}
\newcommand{\xalanHBNoFPAccessInCS}{98.5}
\newcommand{\xalanHBNoFPAccessOutCS}{1.49}
\newcommand{\xalanHBAcqRelTotal}{22.1}
\newcommand{\xalanHBOtherTotal}{7.63E-4}
\newcommand{\xalanHBNoFPReadTotal}{190}
\newcommand{\xalanHBReadInCS}{110}
\newcommand{\xalanHBReadOutCS}{0.0808}
\newcommand{\xalanHBReadSameEp}{10}
\newcommand{\xalanHBReadSharedSameEp}{\cna}
\newcommand{\xalanHBReadExclusive}{85}
\newcommand{\xalanHBReadOwned}{\cna}
\newcommand{\xalanHBReadShare}{0.00196}
\newcommand{\xalanHBReadShared}{15}
\newcommand{\xalanHBReadSharedOwned}{\cna}
\newcommand{\xalanHBNoFPHonestWriteTotal}{40}
\newcommand{\xalanHBWriteInCS}{130}
\newcommand{\xalanHBWriteOutCS}{1.16}
\newcommand{\xalanHBNoFPWriteTotal}{40}
\newcommand{\xalanHBWriteSameEp}{31}
\newcommand{\xalanHBWriteExclusive}{100}
\newcommand{\xalanHBWriteOwned}{\cna}
\newcommand{\xalanHBWriteShared}{<0.001}
\newcommand{\xalanHBNoFPOtherEventTotal}{8928580}
\newcommand{\xalanHBAcqRelOtherTotal}{100.0}
\newcommand{\xalanHBNoAcqRelOtherTotal}{308}
\newcommand{\xalanHBFork}{4.55}
\newcommand{\xalanHBJoin}{4.55}
\newcommand{\xalanHBPreWait}{4.55}
\newcommand{\xalanHBPostWait}{4.55}
\newcommand{\xalanHBVolatileTotal}{0.0}
\newcommand{\xalanHBClassInit}{10.4}
\newcommand{\xalanHBClassAccess}{71.4}
\newcommand{\xalanHBRaceTotal}{2595}
\newcommand{\xalanHBWrRdRace}{98.8}
\newcommand{\xalanHBWrWrRace}{0.539}
\newcommand{\xalanHBRdWrRace}{0.0}
\newcommand{\xalanHBRdShWrRace}{0.617}
\newcommand{\xalanHBHoldLocksTotal}{260}
\newcommand{\xalanHBOneLockHeld}{113.}
\newcommand{\xalanHBTwoNestedLocks}{113.}
\newcommand{\xalanHBThreeNestedLocks}{1.17}
\newcommand{\xalanHBFourNestedLocks}{<0.1}
\newcommand{\xalanHBFiveNestedLocks}{\cna}
\newcommand{\xalanHBSixNestedLocks}{\cna}
\newcommand{\xalanHBSevenNestedLocks}{\cna}
\newcommand{\xalanHBEightNestedLocks}{\cna}
\newcommand{\xalanHBNineNestedLocks}{\cna}
\newcommand{\xalanHBTenNestedLocks}{\cna}
\newcommand{\xalanHBHundredNestedLocks}{\cna}
\newcommand{\xalanFTOHBEventTotal}{630}
\newcommand{\xalanFTOHBNoFPEventTotal}{230}
\newcommand{\xalanFTOHBNoFPAccessTotal}{220}
\newcommand{\xalanFTOHBNoFPOtherTotal}{8.9}
\newcommand{\xalanFTOHBReadTotal}{79.1}
\newcommand{\xalanFTOHBWriteTotal}{17.1}
\newcommand{\xalanFTOHBNoFPAccessInCS}{98.5}
\newcommand{\xalanFTOHBNoFPAccessOutCS}{1.49}
\newcommand{\xalanFTOHBAcqRelTotal}{22.1}
\newcommand{\xalanFTOHBOtherTotal}{7.63E-4}
\newcommand{\xalanFTOHBNoFPReadTotal}{180}
\newcommand{\xalanFTOHBReadInCS}{110}
\newcommand{\xalanFTOHBReadOutCS}{0.0477}
\newcommand{\xalanFTOHBReadSameEp}{10.3}
\newcommand{\xalanFTOHBReadSharedSameEp}{\cna}
\newcommand{\xalanFTOHBReadExclusive}{1.67}
\newcommand{\xalanFTOHBReadOwned}{82.9}
\newcommand{\xalanFTOHBReadShare}{0.00197}
\newcommand{\xalanFTOHBReadShared}{0.0236}
\newcommand{\xalanFTOHBReadSharedOwned}{15.4}
\newcommand{\xalanFTOHBNoFPHonestWriteTotal}{40}
\newcommand{\xalanFTOHBWriteInCS}{130}
\newcommand{\xalanFTOHBWriteOutCS}{1.16}
\newcommand{\xalanFTOHBNoFPWriteTotal}{40}
\newcommand{\xalanFTOHBWriteSameEp}{31}
\newcommand{\xalanFTOHBWriteExclusive}{10.6}
\newcommand{\xalanFTOHBWriteOwned}{89.4}
\newcommand{\xalanFTOHBWriteShared}{<0.001}
\newcommand{\xalanFTOHBNoFPOtherEventTotal}{8928580}
\newcommand{\xalanFTOHBAcqRelOtherTotal}{100.0}
\newcommand{\xalanFTOHBNoAcqRelOtherTotal}{308}
\newcommand{\xalanFTOHBFork}{4.55}
\newcommand{\xalanFTOHBJoin}{4.55}
\newcommand{\xalanFTOHBPreWait}{4.55}
\newcommand{\xalanFTOHBPostWait}{4.55}
\newcommand{\xalanFTOHBVolatileTotal}{0.0}
\newcommand{\xalanFTOHBClassInit}{10.4}
\newcommand{\xalanFTOHBClassAccess}{71.8}
\newcommand{\xalanFTOHBRaceTotal}{2600}
\newcommand{\xalanFTOHBWrRdRace}{99.4}
\newcommand{\xalanFTOHBWrWrRace}{0.0}
\newcommand{\xalanFTOHBRdWrRace}{0.538}
\newcommand{\xalanFTOHBRdShWrRace}{0.0769}
\newcommand{\xalanFTOHBHoldLocksTotal}{220}
\newcommand{\xalanFTOHBOneLockHeld}{99.9}
\newcommand{\xalanFTOHBTwoNestedLocks}{99.7}
\newcommand{\xalanFTOHBThreeNestedLocks}{1.10}
\newcommand{\xalanFTOHBFourNestedLocks}{\cna}
\newcommand{\xalanFTOHBFiveNestedLocks}{\cna}
\newcommand{\xalanFTOHBSixNestedLocks}{\cna}
\newcommand{\xalanFTOHBSevenNestedLocks}{\cna}
\newcommand{\xalanFTOHBEightNestedLocks}{\cna}
\newcommand{\xalanFTOHBNineNestedLocks}{\cna}
\newcommand{\xalanFTOHBTenNestedLocks}{\cna}
\newcommand{\xalanFTOHBHundredNestedLocks}{\cna}
\newcommand{\xalanFTOWCPEventTotal}{630}
\newcommand{\xalanFTOWCPNoFPEventTotal}{240}
\newcommand{\xalanFTOWCPNoFPAccessTotal}{230}
\newcommand{\xalanFTOWCPNoFPOtherTotal}{8.9}
\newcommand{\xalanFTOWCPReadTotal}{79.4}
\newcommand{\xalanFTOWCPWriteTotal}{16.8}
\newcommand{\xalanFTOWCPNoFPAccessInCS}{89.4}
\newcommand{\xalanFTOWCPNoFPAccessOutCS}{1.21}
\newcommand{\xalanFTOWCPAcqRelTotal}{18.8}
\newcommand{\xalanFTOWCPOtherTotal}{6.43E-4}
\newcommand{\xalanFTOWCPNoFPReadTotal}{190}
\newcommand{\xalanFTOWCPReadInCS}{110}
\newcommand{\xalanFTOWCPReadOutCS}{0.0467}
\newcommand{\xalanFTOWCPReadSameEp}{10.1}
\newcommand{\xalanFTOWCPReadSharedSameEp}{<0.001}
\newcommand{\xalanFTOWCPReadExclusive}{0.0383}
\newcommand{\xalanFTOWCPReadOwned}{82.4}
\newcommand{\xalanFTOWCPReadShare}{0.0185}
\newcommand{\xalanFTOWCPReadShared}{0.036}
\newcommand{\xalanFTOWCPReadSharedOwned}{17.5}
\newcommand{\xalanFTOWCPNoFPHonestWriteTotal}{40}
\newcommand{\xalanFTOWCPWriteInCS}{130}
\newcommand{\xalanFTOWCPWriteOutCS}{1.15}
\newcommand{\xalanFTOWCPNoFPWriteTotal}{40}
\newcommand{\xalanFTOWCPWriteSameEp}{31}
\newcommand{\xalanFTOWCPWriteExclusive}{10.8}
\newcommand{\xalanFTOWCPWriteOwned}{89.1}
\newcommand{\xalanFTOWCPWriteShared}{0.0726}
\newcommand{\xalanFTOWCPNoFPOtherEventTotal}{8928578}
\newcommand{\xalanFTOWCPAcqRelOtherTotal}{100.0}
\newcommand{\xalanFTOWCPNoAcqRelOtherTotal}{306}
\newcommand{\xalanFTOWCPFork}{4.58}
\newcommand{\xalanFTOWCPJoin}{4.58}
\newcommand{\xalanFTOWCPPreWait}{4.58}
\newcommand{\xalanFTOWCPPostWait}{4.58}
\newcommand{\xalanFTOWCPVolatileTotal}{0.0}
\newcommand{\xalanFTOWCPClassInit}{10.5}
\newcommand{\xalanFTOWCPClassAccess}{71.2}
\newcommand{\xalanFTOWCPRaceTotal}{3624975}
\newcommand{\xalanFTOWCPWrRdRace}{0.874}
\newcommand{\xalanFTOWCPWrWrRace}{0.0}
\newcommand{\xalanFTOWCPRdWrRace}{98.7}
\newcommand{\xalanFTOWCPRdShWrRace}{0.4}
\newcommand{\xalanFTOWCPHoldLocksTotal}{230}
\newcommand{\xalanFTOWCPOneLockHeld}{99.9}
\newcommand{\xalanFTOWCPTwoNestedLocks}{99.7}
\newcommand{\xalanFTOWCPThreeNestedLocks}{1.27}
\newcommand{\xalanFTOWCPFourNestedLocks}{\cna}
\newcommand{\xalanFTOWCPFiveNestedLocks}{\cna}
\newcommand{\xalanFTOWCPSixNestedLocks}{\cna}
\newcommand{\xalanFTOWCPSevenNestedLocks}{\cna}
\newcommand{\xalanFTOWCPEightNestedLocks}{\cna}
\newcommand{\xalanFTOWCPNineNestedLocks}{\cna}
\newcommand{\xalanFTOWCPTenNestedLocks}{\cna}
\newcommand{\xalanFTOWCPHundredNestedLocks}{\cna}
\newcommand{\xalanREWCPEventTotal}{630}
\newcommand{\xalanREWCPNoFPEventTotal}{240}
\newcommand{\xalanREWCPNoFPAccessTotal}{230}
\newcommand{\xalanREWCPNoFPOtherTotal}{8.9}
\newcommand{\xalanREWCPReadTotal}{79.4}
\newcommand{\xalanREWCPWriteTotal}{16.8}
\newcommand{\xalanREWCPNoFPAccessInCS}{89.5}
\newcommand{\xalanREWCPNoFPAccessOutCS}{1.21}
\newcommand{\xalanREWCPAcqRelTotal}{18.8}
\newcommand{\xalanREWCPOtherTotal}{6.41E-4}
\newcommand{\xalanREWCPNoFPReadTotal}{190}
\newcommand{\xalanREWCPReadInCS}{110}
\newcommand{\xalanREWCPReadOutCS}{0.0467}
\newcommand{\xalanREWCPReadSameEp}{10.1}
\newcommand{\xalanREWCPReadSharedSameEp}{<0.001}
\newcommand{\xalanREWCPReadExclusive}{0.0181}
\newcommand{\xalanREWCPReadOwned}{82.4}
\newcommand{\xalanREWCPReadShare}{0.0198}
\newcommand{\xalanREWCPReadShared}{0.0375}
\newcommand{\xalanREWCPReadSharedOwned}{17.5}
\newcommand{\xalanREWCPNoFPHonestWriteTotal}{40}
\newcommand{\xalanREWCPWriteInCS}{130}
\newcommand{\xalanREWCPWriteOutCS}{1.15}
\newcommand{\xalanREWCPNoFPWriteTotal}{40}
\newcommand{\xalanREWCPWriteSameEp}{31}
\newcommand{\xalanREWCPWriteExclusive}{10.8}
\newcommand{\xalanREWCPWriteOwned}{89.1}
\newcommand{\xalanREWCPWriteShared}{0.0784}
\newcommand{\xalanREWCPNoFPOtherEventTotal}{8928577}
\newcommand{\xalanREWCPAcqRelOtherTotal}{100.0}
\newcommand{\xalanREWCPNoAcqRelOtherTotal}{305}
\newcommand{\xalanREWCPFork}{4.59}
\newcommand{\xalanREWCPJoin}{4.59}
\newcommand{\xalanREWCPPreWait}{4.59}
\newcommand{\xalanREWCPPostWait}{4.59}
\newcommand{\xalanREWCPVolatileTotal}{0.0}
\newcommand{\xalanREWCPClassInit}{10.5}
\newcommand{\xalanREWCPClassAccess}{71.1}
\newcommand{\xalanREWCPRaceTotal}{3603126}
\newcommand{\xalanREWCPWrRdRace}{0.868}
\newcommand{\xalanREWCPWrWrRace}{0.0}
\newcommand{\xalanREWCPRdWrRace}{98.7}
\newcommand{\xalanREWCPRdShWrRace}{0.395}
\newcommand{\xalanREWCPHoldLocksTotal}{230}
\newcommand{\xalanREWCPOneLockHeld}{99.9}
\newcommand{\xalanREWCPTwoNestedLocks}{99.7}
\newcommand{\xalanREWCPThreeNestedLocks}{1.29}
\newcommand{\xalanREWCPFourNestedLocks}{\cna}
\newcommand{\xalanREWCPFiveNestedLocks}{\cna}
\newcommand{\xalanREWCPSixNestedLocks}{\cna}
\newcommand{\xalanREWCPSevenNestedLocks}{\cna}
\newcommand{\xalanREWCPEightNestedLocks}{\cna}
\newcommand{\xalanREWCPNineNestedLocks}{\cna}
\newcommand{\xalanREWCPTenNestedLocks}{\cna}
\newcommand{\xalanREWCPHundredNestedLocks}{\cna}
\newcommand{\xalanFTODCEventTotal}{630}
\newcommand{\xalanFTODCNoFPEventTotal}{240}
\newcommand{\xalanFTODCNoFPAccessTotal}{230}
\newcommand{\xalanFTODCNoFPOtherTotal}{8.9}
\newcommand{\xalanFTODCReadTotal}{79.4}
\newcommand{\xalanFTODCWriteTotal}{16.8}
\newcommand{\xalanFTODCNoFPAccessInCS}{88.6}
\newcommand{\xalanFTODCNoFPAccessOutCS}{1.18}
\newcommand{\xalanFTODCAcqRelTotal}{18.4}
\newcommand{\xalanFTODCOtherTotal}{6.3E-4}
\newcommand{\xalanFTODCNoFPReadTotal}{190}
\newcommand{\xalanFTODCReadInCS}{110}
\newcommand{\xalanFTODCReadOutCS}{0.0467}
\newcommand{\xalanFTODCReadSameEp}{10.1}
\newcommand{\xalanFTODCReadSharedSameEp}{<0.001}
\newcommand{\xalanFTODCReadExclusive}{0.0202}
\newcommand{\xalanFTODCReadOwned}{82.3}
\newcommand{\xalanFTODCReadShare}{0.0196}
\newcommand{\xalanFTODCReadShared}{0.0372}
\newcommand{\xalanFTODCReadSharedOwned}{17.6}
\newcommand{\xalanFTODCNoFPHonestWriteTotal}{40}
\newcommand{\xalanFTODCWriteInCS}{130}
\newcommand{\xalanFTODCWriteOutCS}{1.15}
\newcommand{\xalanFTODCNoFPWriteTotal}{40}
\newcommand{\xalanFTODCWriteSameEp}{31}
\newcommand{\xalanFTODCWriteExclusive}{10.8}
\newcommand{\xalanFTODCWriteOwned}{89.1}
\newcommand{\xalanFTODCWriteShared}{0.0778}
\newcommand{\xalanFTODCNoFPOtherEventTotal}{8928577}
\newcommand{\xalanFTODCAcqRelOtherTotal}{100.0}
\newcommand{\xalanFTODCNoAcqRelOtherTotal}{305}
\newcommand{\xalanFTODCFork}{4.59}
\newcommand{\xalanFTODCJoin}{4.59}
\newcommand{\xalanFTODCPreWait}{4.59}
\newcommand{\xalanFTODCPostWait}{4.59}
\newcommand{\xalanFTODCVolatileTotal}{0.0}
\newcommand{\xalanFTODCClassInit}{10.5}
\newcommand{\xalanFTODCClassAccess}{71.5}
\newcommand{\xalanFTODCRaceTotal}{4042745}
\newcommand{\xalanFTODCWrRdRace}{0.851}
\newcommand{\xalanFTODCWrWrRace}{0.0}
\newcommand{\xalanFTODCRdWrRace}{98.8}
\newcommand{\xalanFTODCRdShWrRace}{0.384}
\newcommand{\xalanFTODCHoldLocksTotal}{230}
\newcommand{\xalanFTODCOneLockHeld}{99.9}
\newcommand{\xalanFTODCTwoNestedLocks}{99.7}
\newcommand{\xalanFTODCThreeNestedLocks}{1.09}
\newcommand{\xalanFTODCFourNestedLocks}{\cna}
\newcommand{\xalanFTODCFiveNestedLocks}{\cna}
\newcommand{\xalanFTODCSixNestedLocks}{\cna}
\newcommand{\xalanFTODCSevenNestedLocks}{\cna}
\newcommand{\xalanFTODCEightNestedLocks}{\cna}
\newcommand{\xalanFTODCNineNestedLocks}{\cna}
\newcommand{\xalanFTODCTenNestedLocks}{\cna}
\newcommand{\xalanFTODCHundredNestedLocks}{\cna}
\newcommand{\xalanREDCEventTotal}{630}
\newcommand{\xalanREDCNoFPEventTotal}{240}
\newcommand{\xalanREDCNoFPAccessTotal}{230}
\newcommand{\xalanREDCNoFPOtherTotal}{8.9}
\newcommand{\xalanREDCReadTotal}{79.4}
\newcommand{\xalanREDCWriteTotal}{16.8}
\newcommand{\xalanREDCNoFPAccessInCS}{88.6}
\newcommand{\xalanREDCNoFPAccessOutCS}{1.18}
\newcommand{\xalanREDCAcqRelTotal}{18.4}
\newcommand{\xalanREDCOtherTotal}{6.3E-4}
\newcommand{\xalanREDCNoFPReadTotal}{190}
\newcommand{\xalanREDCReadInCS}{110}
\newcommand{\xalanREDCReadOutCS}{0.0467}
\newcommand{\xalanREDCReadSameEp}{10.1}
\newcommand{\xalanREDCReadSharedSameEp}{\cna}
\newcommand{\xalanREDCReadExclusive}{0.0161}
\newcommand{\xalanREDCReadOwned}{82.4}
\newcommand{\xalanREDCReadShare}{0.02}
\newcommand{\xalanREDCReadShared}{0.0382}
\newcommand{\xalanREDCReadSharedOwned}{17.6}
\newcommand{\xalanREDCNoFPHonestWriteTotal}{40}
\newcommand{\xalanREDCWriteInCS}{130}
\newcommand{\xalanREDCWriteOutCS}{1.15}
\newcommand{\xalanREDCNoFPWriteTotal}{40}
\newcommand{\xalanREDCWriteSameEp}{31}
\newcommand{\xalanREDCWriteExclusive}{10.8}
\newcommand{\xalanREDCWriteOwned}{89.1}
\newcommand{\xalanREDCWriteShared}{0.0787}
\newcommand{\xalanREDCNoFPOtherEventTotal}{8928577}
\newcommand{\xalanREDCAcqRelOtherTotal}{100.0}
\newcommand{\xalanREDCNoAcqRelOtherTotal}{305}
\newcommand{\xalanREDCFork}{4.59}
\newcommand{\xalanREDCJoin}{4.59}
\newcommand{\xalanREDCPreWait}{4.59}
\newcommand{\xalanREDCPostWait}{4.59}
\newcommand{\xalanREDCVolatileTotal}{0.0}
\newcommand{\xalanREDCClassInit}{10.5}
\newcommand{\xalanREDCClassAccess}{71.1}
\newcommand{\xalanREDCRaceTotal}{4031899}
\newcommand{\xalanREDCWrRdRace}{0.856}
\newcommand{\xalanREDCWrWrRace}{0.0}
\newcommand{\xalanREDCRdWrRace}{98.8}
\newcommand{\xalanREDCRdShWrRace}{0.385}
\newcommand{\xalanREDCHoldLocksTotal}{230}
\newcommand{\xalanREDCOneLockHeld}{99.9}
\newcommand{\xalanREDCTwoNestedLocks}{99.7}
\newcommand{\xalanREDCThreeNestedLocks}{1.10}
\newcommand{\xalanREDCFourNestedLocks}{\cna}
\newcommand{\xalanREDCFiveNestedLocks}{\cna}
\newcommand{\xalanREDCSixNestedLocks}{\cna}
\newcommand{\xalanREDCSevenNestedLocks}{\cna}
\newcommand{\xalanREDCEightNestedLocks}{\cna}
\newcommand{\xalanREDCNineNestedLocks}{\cna}
\newcommand{\xalanREDCTenNestedLocks}{\cna}
\newcommand{\xalanREDCHundredNestedLocks}{\cna}
\newcommand{\xalanFTOCAPOEventTotal}{630}
\newcommand{\xalanFTOCAPONoFPEventTotal}{240}
\newcommand{\xalanFTOCAPONoFPAccessTotal}{230}
\newcommand{\xalanFTOCAPONoFPOtherTotal}{8.9}
\newcommand{\xalanFTOCAPOReadTotal}{79.4}
\newcommand{\xalanFTOCAPOWriteTotal}{16.8}
\newcommand{\xalanFTOCAPONoFPAccessInCS}{88.6}
\newcommand{\xalanFTOCAPONoFPAccessOutCS}{1.18}
\newcommand{\xalanFTOCAPOAcqRelTotal}{18.5}
\newcommand{\xalanFTOCAPOOtherTotal}{6.37E-4}
\newcommand{\xalanFTOCAPONoFPReadTotal}{190}
\newcommand{\xalanFTOCAPOReadInCS}{110}
\newcommand{\xalanFTOCAPOReadOutCS}{0.0467}
\newcommand{\xalanFTOCAPOReadSameEp}{10.1}
\newcommand{\xalanFTOCAPOReadSharedSameEp}{<0.001}
\newcommand{\xalanFTOCAPOReadExclusive}{0.0188}
\newcommand{\xalanFTOCAPOReadOwned}{82.3}
\newcommand{\xalanFTOCAPOReadShare}{0.0195}
\newcommand{\xalanFTOCAPOReadShared}{0.0373}
\newcommand{\xalanFTOCAPOReadSharedOwned}{17.6}
\newcommand{\xalanFTOCAPONoFPHonestWriteTotal}{40}
\newcommand{\xalanFTOCAPOWriteInCS}{130}
\newcommand{\xalanFTOCAPOWriteOutCS}{1.15}
\newcommand{\xalanFTOCAPONoFPWriteTotal}{40}
\newcommand{\xalanFTOCAPOWriteSameEp}{31}
\newcommand{\xalanFTOCAPOWriteExclusive}{10.8}
\newcommand{\xalanFTOCAPOWriteOwned}{89.2}
\newcommand{\xalanFTOCAPOWriteShared}{0.0773}
\newcommand{\xalanFTOCAPONoFPOtherEventTotal}{8928580}
\newcommand{\xalanFTOCAPOAcqRelOtherTotal}{100.0}
\newcommand{\xalanFTOCAPONoAcqRelOtherTotal}{308}
\newcommand{\xalanFTOCAPOFork}{4.55}
\newcommand{\xalanFTOCAPOJoin}{4.55}
\newcommand{\xalanFTOCAPOPreWait}{4.55}
\newcommand{\xalanFTOCAPOPostWait}{4.55}
\newcommand{\xalanFTOCAPOVolatileTotal}{0.0}
\newcommand{\xalanFTOCAPOClassInit}{10.4}
\newcommand{\xalanFTOCAPOClassAccess}{71.4}
\newcommand{\xalanFTOCAPORaceTotal}{4012365}
\newcommand{\xalanFTOCAPOWrRdRace}{0.853}
\newcommand{\xalanFTOCAPOWrWrRace}{0.0}
\newcommand{\xalanFTOCAPORdWrRace}{98.8}
\newcommand{\xalanFTOCAPORdShWrRace}{0.384}
\newcommand{\xalanFTOCAPOHoldLocksTotal}{230}
\newcommand{\xalanFTOCAPOOneLockHeld}{99.9}
\newcommand{\xalanFTOCAPOTwoNestedLocks}{99.7}
\newcommand{\xalanFTOCAPOThreeNestedLocks}{1.10}
\newcommand{\xalanFTOCAPOFourNestedLocks}{\cna}
\newcommand{\xalanFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\xalanFTOCAPOSixNestedLocks}{\cna}
\newcommand{\xalanFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\xalanFTOCAPOEightNestedLocks}{\cna}
\newcommand{\xalanFTOCAPONineNestedLocks}{\cna}
\newcommand{\xalanFTOCAPOTenNestedLocks}{\cna}
\newcommand{\xalanFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\xalanRECAPOEventTotal}{630}
\newcommand{\xalanRECAPONoFPEventTotal}{240}
\newcommand{\xalanRECAPONoFPAccessTotal}{230}
\newcommand{\xalanRECAPONoFPOtherTotal}{8.9}
\newcommand{\xalanRECAPOReadTotal}{79.4}
\newcommand{\xalanRECAPOWriteTotal}{16.8}
\newcommand{\xalanRECAPONoFPAccessInCS}{88.6}
\newcommand{\xalanRECAPONoFPAccessOutCS}{1.18}
\newcommand{\xalanRECAPOAcqRelTotal}{18.4}
\newcommand{\xalanRECAPOOtherTotal}{6.36E-4}
\newcommand{\xalanRECAPONoFPReadTotal}{190}
\newcommand{\xalanRECAPOReadInCS}{110}
\newcommand{\xalanRECAPOReadOutCS}{0.0467}
\newcommand{\xalanRECAPOReadSameEp}{10.1}
\newcommand{\xalanRECAPOReadSharedSameEp}{\cna}
\newcommand{\xalanRECAPOReadExclusive}{0.0113}
\newcommand{\xalanRECAPOReadOwned}{82.3}
\newcommand{\xalanRECAPOReadShare}{0.0199}
\newcommand{\xalanRECAPOReadShared}{0.0388}
\newcommand{\xalanRECAPOReadSharedOwned}{17.6}
\newcommand{\xalanRECAPONoFPHonestWriteTotal}{40}
\newcommand{\xalanRECAPOWriteInCS}{130}
\newcommand{\xalanRECAPOWriteOutCS}{1.15}
\newcommand{\xalanRECAPONoFPWriteTotal}{40}
\newcommand{\xalanRECAPOWriteSameEp}{31}
\newcommand{\xalanRECAPOWriteExclusive}{10.8}
\newcommand{\xalanRECAPOWriteOwned}{89.1}
\newcommand{\xalanRECAPOWriteShared}{0.0785}
\newcommand{\xalanRECAPONoFPOtherEventTotal}{8928580}
\newcommand{\xalanRECAPOAcqRelOtherTotal}{100.0}
\newcommand{\xalanRECAPONoAcqRelOtherTotal}{308}
\newcommand{\xalanRECAPOFork}{4.55}
\newcommand{\xalanRECAPOJoin}{4.55}
\newcommand{\xalanRECAPOPreWait}{4.55}
\newcommand{\xalanRECAPOPostWait}{4.55}
\newcommand{\xalanRECAPOVolatileTotal}{0.0}
\newcommand{\xalanRECAPOClassInit}{10.4}
\newcommand{\xalanRECAPOClassAccess}{71.8}
\newcommand{\xalanRECAPORaceTotal}{4030712}
\newcommand{\xalanRECAPOWrRdRace}{0.854}
\newcommand{\xalanRECAPOWrWrRace}{0.0}
\newcommand{\xalanRECAPORdWrRace}{98.8}
\newcommand{\xalanRECAPORdShWrRace}{0.384}
\newcommand{\xalanRECAPOHoldLocksTotal}{230}
\newcommand{\xalanRECAPOOneLockHeld}{99.9}
\newcommand{\xalanRECAPOTwoNestedLocks}{99.7}
\newcommand{\xalanRECAPOThreeNestedLocks}{1.10}
\newcommand{\xalanRECAPOFourNestedLocks}{\cna}
\newcommand{\xalanRECAPOFiveNestedLocks}{\cna}
\newcommand{\xalanRECAPOSixNestedLocks}{\cna}
\newcommand{\xalanRECAPOSevenNestedLocks}{\cna}
\newcommand{\xalanRECAPOEightNestedLocks}{\cna}
\newcommand{\xalanRECAPONineNestedLocks}{\cna}
\newcommand{\xalanRECAPOTenNestedLocks}{\cna}
\newcommand{\xalanRECAPOHundredNestedLocks}{\cna}
\newcommand{\FASTxalanMaxLiveThreads}{15}
\newcommand{\FASTxalanTotalThreads}{15}
\newcommand{\FASTxalanBaseTime}{2.0}
\newcommand{\FASTxalanBaseTimeCI}{120}
\newcommand{\FASTxalanEmptyTime}{\rna}
\newcommand{\FASTxalanEmptyTimeCI}{\rna}
\newcommand{\FASTxalanEmptyTimeCIMIN}{\rna}
\newcommand{\FASTxalanEmptyTimeCIMAX}{\rna}
\newcommand{\FASTxalanFTTime}{4.7}
\newcommand{\FASTxalanFTTimeCI}{0.31}
\newcommand{\FASTxalanHBTime}{4.9}
\newcommand{\FASTxalanHBTimeCI}{0.33}
\newcommand{\FASTxalanFTOHBTime}{4.9}
\newcommand{\FASTxalanFTOHBTimeCI}{0.3}
\newcommand{\FASTxalanWCPTime}{\rna}
\newcommand{\FASTxalanWCPTimeCI}{\rna}
\newcommand{\FASTxalanWCPTimeCIMIN}{\rna}
\newcommand{\FASTxalanWCPTimeCIMAX}{\rna}
\newcommand{\FASTxalanFTOWCPTime}{37}
\newcommand{\FASTxalanFTOWCPTimeCI}{2.1}
\newcommand{\FASTxalanREWCPTime}{14}
\newcommand{\FASTxalanREWCPTimeCI}{0.76}
\newcommand{\FASTxalanDCTime}{\rna}
\newcommand{\FASTxalanDCTimeCI}{\rna}
\newcommand{\FASTxalanDCTimeCIMIN}{\rna}
\newcommand{\FASTxalanDCTimeCIMAX}{\rna}
\newcommand{\FASTxalanFTODCTime}{35}
\newcommand{\FASTxalanFTODCTimeCI}{2.0}
\newcommand{\FASTxalanREDCTime}{16}
\newcommand{\FASTxalanREDCTimeCI}{0.72}
\newcommand{\FASTxalanCAPOTime}{\rna}
\newcommand{\FASTxalanCAPOTimeCI}{\rna}
\newcommand{\FASTxalanCAPOTimeCIMIN}{\rna}
\newcommand{\FASTxalanCAPOTimeCIMAX}{\rna}
\newcommand{\FASTxalanFTOCAPOTime}{32}
\newcommand{\FASTxalanFTOCAPOTimeCI}{2.8}
\newcommand{\FASTxalanRECAPOTime}{11}
\newcommand{\FASTxalanRECAPOTimeCI}{0.55}
\newcommand{\FASTxalanAGGCAPOTime}{\rna}
\newcommand{\FASTxalanAGGCAPOTimeCI}{\rna}
\newcommand{\FASTxalanAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTxalanAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTxalanStaticTime}{\rzero}
\newcommand{\FASTxalanDynamicTime}{\rzero}
\newcommand{\FASTxalanBaseMem}{670}
\newcommand{\FASTxalanBaseMemCI}{8.5}
\newcommand{\FASTxalanFTMem}{6.6}
\newcommand{\FASTxalanFTMemCI}{0.088}
\newcommand{\FASTxalanHBMem}{6.6}
\newcommand{\FASTxalanHBMemCI}{0.1}
\newcommand{\FASTxalanFTOHBMem}{6.6}
\newcommand{\FASTxalanFTOHBMemCI}{0.091}
\newcommand{\FASTxalanWCPMem}{\memna}
\newcommand{\FASTxalanWCPMemCI}{\memna}
\newcommand{\FASTxalanWCPMemCIMIN}{\memna}
\newcommand{\FASTxalanWCPMemCIMAX}{\memna}
\newcommand{\FASTxalanFTOWCPMem}{58}
\newcommand{\FASTxalanFTOWCPMemCI}{0.7}
\newcommand{\FASTxalanREWCPMem}{48}
\newcommand{\FASTxalanREWCPMemCI}{0.83}
\newcommand{\FASTxalanDCMem}{\memna}
\newcommand{\FASTxalanDCMemCI}{\memna}
\newcommand{\FASTxalanDCMemCIMIN}{\memna}
\newcommand{\FASTxalanDCMemCIMAX}{\memna}
\newcommand{\FASTxalanFTODCMem}{60}
\newcommand{\FASTxalanFTODCMemCI}{1.9}
\newcommand{\FASTxalanREDCMem}{49}
\newcommand{\FASTxalanREDCMemCI}{0.93}
\newcommand{\FASTxalanCAPOMem}{\memna}
\newcommand{\FASTxalanCAPOMemCI}{\memna}
\newcommand{\FASTxalanCAPOMemCIMIN}{\memna}
\newcommand{\FASTxalanCAPOMemCIMAX}{\memna}
\newcommand{\FASTxalanFTOCAPOMem}{60}
\newcommand{\FASTxalanFTOCAPOMemCI}{2.1}
\newcommand{\FASTxalanRECAPOMem}{48}
\newcommand{\FASTxalanRECAPOMemCI}{1.2}
\newcommand{\FASTxalanAGGCAPOMem}{\memna}
\newcommand{\FASTxalanAGGCAPOMemCI}{\memna}
\newcommand{\FASTxalanAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTxalanAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTxalanEventsCI}{8,427}
\newcommand{\FASTxalanEventsCIMIN}{630,384,503}
\newcommand{\FASTxalanEventsCIMAX}{630,401,357}
\newcommand{\FASTxalanNoFPEventsCI}{16,894}
\newcommand{\FASTxalanNoFPEventsCIMIN}{48,397,580}
\newcommand{\FASTxalanNoFPEventsCIMAX}{48,431,368}
\newcommand{\FASTxalanFT}{8}
\newcommand{\FASTxalanFTCI}{0.59}
\newcommand{\FASTxalanFTCIMIN}{7}
\newcommand{\FASTxalanFTCIMAX}{9}
\newcommand{\FASTxalanFTDynamic}{2,814}
\newcommand{\FASTxalanFTDynamicCI}{34}
\newcommand{\FASTxalanFTDynamicCIMIN}{2,780}
\newcommand{\FASTxalanFTDynamicCIMAX}{2,848}
\newcommand{\FASTxalanHB}{8}
\newcommand{\FASTxalanHBCI}{0.43}
\newcommand{\FASTxalanHBCIMIN}{8}
\newcommand{\FASTxalanHBCIMAX}{8}
\newcommand{\FASTxalanHBDynamic}{2,581}
\newcommand{\FASTxalanHBDynamicCI}{38}
\newcommand{\FASTxalanHBDynamicCIMIN}{2,543}
\newcommand{\FASTxalanHBDynamicCIMAX}{2,619}
\newcommand{\FASTxalanFTOHB}{8}
\newcommand{\FASTxalanFTOHBCI}{0.26}
\newcommand{\FASTxalanFTOHBCIMIN}{8}
\newcommand{\FASTxalanFTOHBCIMAX}{8}
\newcommand{\FASTxalanFTOHBDynamic}{2,600}
\newcommand{\FASTxalanFTOHBDynamicCI}{7.3}
\newcommand{\FASTxalanFTOHBDynamicCIMIN}{2,593}
\newcommand{\FASTxalanFTOHBDynamicCIMAX}{2,607}
\newcommand{\FASTxalanWCP}{\rna}
\newcommand{\FASTxalanWCPCI}{\rna}
\newcommand{\FASTxalanWCPCIMIN}{\rna}
\newcommand{\FASTxalanWCPCIMAX}{\rna}
\newcommand{\FASTxalanWCPDynamic}{\rna}
\newcommand{\FASTxalanWCPDynamicCI}{\rna}
\newcommand{\FASTxalanWCPDynamicCIMIN}{\rna}
\newcommand{\FASTxalanWCPDynamicCIMAX}{\rna}
\newcommand{\FASTxalanFTOWCP}{44}
\newcommand{\FASTxalanFTOWCPCI}{0.3}
\newcommand{\FASTxalanFTOWCPCIMIN}{44}
\newcommand{\FASTxalanFTOWCPCIMAX}{44}
\newcommand{\FASTxalanFTOWCPDynamic}{3,624,975}
\newcommand{\FASTxalanFTOWCPDynamicCI}{13,330}
\newcommand{\FASTxalanFTOWCPDynamicCIMIN}{3,611,645}
\newcommand{\FASTxalanFTOWCPDynamicCIMAX}{3,638,305}
\newcommand{\FASTxalanREWCP}{50}
\newcommand{\FASTxalanREWCPCI}{1.3}
\newcommand{\FASTxalanREWCPCIMIN}{49}
\newcommand{\FASTxalanREWCPCIMAX}{51}
\newcommand{\FASTxalanREWCPDynamic}{3,603,126}
\newcommand{\FASTxalanREWCPDynamicCI}{12,208}
\newcommand{\FASTxalanREWCPDynamicCIMIN}{3,590,918}
\newcommand{\FASTxalanREWCPDynamicCIMAX}{3,615,334}
\newcommand{\FASTxalanDC}{\rna}
\newcommand{\FASTxalanDCCI}{\rna}
\newcommand{\FASTxalanDCCIMIN}{\rna}
\newcommand{\FASTxalanDCCIMAX}{\rna}
\newcommand{\FASTxalanDCDynamic}{\rna}
\newcommand{\FASTxalanDCDynamicCI}{\rna}
\newcommand{\FASTxalanDCDynamicCIMIN}{\rna}
\newcommand{\FASTxalanDCDynamicCIMAX}{\rna}
\newcommand{\FASTxalanFTODC}{53}
\newcommand{\FASTxalanFTODCCI}{0.78}
\newcommand{\FASTxalanFTODCCIMIN}{52}
\newcommand{\FASTxalanFTODCCIMAX}{54}
\newcommand{\FASTxalanFTODCDynamic}{4,042,745}
\newcommand{\FASTxalanFTODCDynamicCI}{7,602}
\newcommand{\FASTxalanFTODCDynamicCIMIN}{4,035,143}
\newcommand{\FASTxalanFTODCDynamicCIMAX}{4,050,347}
\newcommand{\FASTxalanREDC}{53}
\newcommand{\FASTxalanREDCCI}{0.74}
\newcommand{\FASTxalanREDCCIMIN}{52}
\newcommand{\FASTxalanREDCCIMAX}{54}
\newcommand{\FASTxalanREDCDynamic}{4,031,899}
\newcommand{\FASTxalanREDCDynamicCI}{13,734}
\newcommand{\FASTxalanREDCDynamicCIMIN}{4,018,165}
\newcommand{\FASTxalanREDCDynamicCIMAX}{4,045,633}
\newcommand{\FASTxalanCAPO}{\rna}
\newcommand{\FASTxalanCAPOCI}{\rna}
\newcommand{\FASTxalanCAPOCIMIN}{\rna}
\newcommand{\FASTxalanCAPOCIMAX}{\rna}
\newcommand{\FASTxalanCAPODynamic}{\rna}
\newcommand{\FASTxalanCAPODynamicCI}{\rna}
\newcommand{\FASTxalanCAPODynamicCIMIN}{\rna}
\newcommand{\FASTxalanCAPODynamicCIMAX}{\rna}
\newcommand{\FASTxalanFTOCAPO}{53}
\newcommand{\FASTxalanFTOCAPOCI}{0.51}
\newcommand{\FASTxalanFTOCAPOCIMIN}{52}
\newcommand{\FASTxalanFTOCAPOCIMAX}{54}
\newcommand{\FASTxalanFTOCAPODynamic}{4,012,365}
\newcommand{\FASTxalanFTOCAPODynamicCI}{9,910}
\newcommand{\FASTxalanFTOCAPODynamicCIMIN}{4,002,455}
\newcommand{\FASTxalanFTOCAPODynamicCIMAX}{4,022,275}
\newcommand{\FASTxalanRECAPO}{53}
\newcommand{\FASTxalanRECAPOCI}{0.88}
\newcommand{\FASTxalanRECAPOCIMIN}{52}
\newcommand{\FASTxalanRECAPOCIMAX}{54}
\newcommand{\FASTxalanRECAPODynamic}{4,030,712}
\newcommand{\FASTxalanRECAPODynamicCI}{8,501}
\newcommand{\FASTxalanRECAPODynamicCIMIN}{4,022,211}
\newcommand{\FASTxalanRECAPODynamicCIMAX}{4,039,213}
\newcommand{\FASTxalanAGGCAPO}{\rna}
\newcommand{\FASTxalanAGGCAPOCI}{\rna}
\newcommand{\FASTxalanAGGCAPOCIMIN}{\rna}
\newcommand{\FASTxalanAGGCAPOCIMAX}{\rna}
\newcommand{\FASTxalanAGGCAPODynamic}{\rna}
\newcommand{\FASTxalanAGGCAPODynamicCI}{\rna}
\newcommand{\FASTxalanAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTxalanAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTBaseTimeGeoMean}{1800}
\newcommand{\FASTEmptyTimeGeoMean}{\rna}
\newcommand{\FASTFTTimeGeoMean}{9.0}
\newcommand{\FASTHBTimeGeoMean}{8.7}
\newcommand{\FASTFTOHBTimeGeoMean}{8.6}
\newcommand{\FASTWCPTimeGeoMean}{\rna}
\newcommand{\FASTFTOWCPTimeGeoMean}{17}
\newcommand{\FASTREWCPTimeGeoMean}{12}
\newcommand{\FASTDCTimeGeoMean}{\rna}
\newcommand{\FASTFTODCTimeGeoMean}{17}
\newcommand{\FASTREDCTimeGeoMean}{12}
\newcommand{\FASTCAPOTimeGeoMean}{\rna}
\newcommand{\FASTFTOCAPOTimeGeoMean}{16}
\newcommand{\FASTRECAPOTimeGeoMean}{11}
\newcommand{\FASTAGGCAPOTimeGeoMean}{\rna}
\newcommand{\FASTBaseMemGeoMean}{510}
\newcommand{\FASTEmptyMemGeoMean}{0.0}
\newcommand{\FASTFTMemGeoMean}{8.1}
\newcommand{\FASTHBMemGeoMean}{7.6}
\newcommand{\FASTFTOHBMemGeoMean}{7.6}
\newcommand{\FASTWCPMemGeoMean}{\memna}
\newcommand{\FASTFTOWCPMemGeoMean}{19}
\newcommand{\FASTREWCPMemGeoMean}{17}
\newcommand{\FASTDCMemGeoMean}{\memna}
\newcommand{\FASTFTODCMemGeoMean}{19}
\newcommand{\FASTREDCMemGeoMean}{18}
\newcommand{\FASTCAPOMemGeoMean}{\memna}
\newcommand{\FASTFTOCAPOMemGeoMean}{18}
\newcommand{\FASTRECAPOMemGeoMean}{15}
\newcommand{\FASTAGGCAPOMemGeoMean}{\memna}
\newcommand{\FASTWCPDynamicTotal}{0}
\newcommand{\FASTFTODCTotal}{740}
\newcommand{\FASTCAPOTotal}{0}
\newcommand{\FASTWCPTotal}{0}
\newcommand{\FASTAGGCAPODynamicTotal}{0}
\newcommand{\FASTRECAPOTotal}{748}
\newcommand{\FASTFTTotal}{490}
\newcommand{\FASTHBDynamicTotal}{2,533,193}
\newcommand{\FASTREDCTotal}{744}
\newcommand{\FASTREWCPTotal}{733}
\newcommand{\FASTFTOWCPDynamicTotal}{5,960,921}
\newcommand{\FASTRECAPODynamicTotal}{6,454,331}
\newcommand{\FASTFTOWCPTotal}{718}
\newcommand{\FASTAGGCAPOTotal}{0}
\newcommand{\FASTCAPODynamicTotal}{0}
\newcommand{\FASTFTOCAPOTotal}{745}
\newcommand{\FASTFTODCDynamicTotal}{6,401,533}
\newcommand{\FASTFTDynamicTotal}{4,437,026}
\newcommand{\FASTREWCPDynamicTotal}{5,998,502}
\newcommand{\FASTREDCDynamicTotal}{6,415,411}
\newcommand{\FASTFTOCAPODynamicTotal}{6,445,208}
\newcommand{\FASTFTOHBDynamicTotal}{2,414,753}
\newcommand{\FASTHBTotal}{717}
\newcommand{\FASTFTOHBTotal}{673}
\newcommand{\FASTDCDynamicTotal}{0}
\newcommand{\FASTDCTotal}{0}



==> result-macros/PIP_fastTool_noWriteOrReadRaceEdge.tex <==
\newcommand{\FASTavroraEvents}{1,400}
\newcommand{\FASTavroraNoFPEvents}{5.3}
\newcommand{\avroraHBEventTotal}{1,400}
\newcommand{\avroraHBNoFPEventTotal}{150}
\newcommand{\avroraHBNoFPAccessTotal}{150}
\newcommand{\avroraHBNoFPOtherTotal}{3.6}
\newcommand{\avroraHBReadTotal}{69.4}
\newcommand{\avroraHBWriteTotal}{28.3}
\newcommand{\avroraHBNoFPAccessInCS}{34.8}
\newcommand{\avroraHBNoFPAccessOutCS}{55.5}
\newcommand{\avroraHBAcqRelTotal}{55.3}
\newcommand{\avroraHBOtherTotal}{12.4}
\newcommand{\avroraHBNoFPReadTotal}{110}
\newcommand{\avroraHBReadInCS}{6.07}
\newcommand{\avroraHBReadOutCS}{94.2}
\newcommand{\avroraHBReadSameEp}{0.0242}
\newcommand{\avroraHBReadSharedSameEp}{\cna}
\newcommand{\avroraHBReadExclusive}{96.6}
\newcommand{\avroraHBReadOwned}{\cna}
\newcommand{\avroraHBReadShare}{0.0206}
\newcommand{\avroraHBReadShared}{3.42}
\newcommand{\avroraHBReadSharedOwned}{\cna}
\newcommand{\avroraHBNoFPHonestWriteTotal}{44}
\newcommand{\avroraHBWriteInCS}{6.22}
\newcommand{\avroraHBWriteOutCS}{96.2}
\newcommand{\avroraHBNoFPWriteTotal}{44}
\newcommand{\avroraHBWriteSameEp}{2.41}
\newcommand{\avroraHBWriteExclusive}{99.5}
\newcommand{\avroraHBWriteOwned}{\cna}
\newcommand{\avroraHBWriteShared}{0.474}
\newcommand{\avroraHBNoFPOtherEventTotal}{3584765}
\newcommand{\avroraHBAcqRelOtherTotal}{81.6}
\newcommand{\avroraHBNoAcqRelOtherTotal}{659001}
\newcommand{\avroraHBFork}{9.1E-4}
\newcommand{\avroraHBJoin}{9.1E-4}
\newcommand{\avroraHBPreWait}{50.0}
\newcommand{\avroraHBPostWait}{50.0}
\newcommand{\avroraHBVolatileTotal}{0.0}
\newcommand{\avroraHBClassInit}{0.019}
\newcommand{\avroraHBClassAccess}{0.0281}
\newcommand{\avroraHBRaceTotal}{480029}
\newcommand{\avroraHBWrRdRace}{47.7}
\newcommand{\avroraHBWrWrRace}{19.7}
\newcommand{\avroraHBRdWrRace}{0.158}
\newcommand{\avroraHBRdShWrRace}{32.5}
\newcommand{\avroraHBHoldLocksTotal}{9.2}
\newcommand{\avroraHBOneLockHeld}{5.79}
\newcommand{\avroraHBTwoNestedLocks}{<0.1}
\newcommand{\avroraHBThreeNestedLocks}{\cna}
\newcommand{\avroraHBFourNestedLocks}{\cna}
\newcommand{\avroraHBFiveNestedLocks}{\cna}
\newcommand{\avroraHBSixNestedLocks}{\cna}
\newcommand{\avroraHBSevenNestedLocks}{\cna}
\newcommand{\avroraHBEightNestedLocks}{\cna}
\newcommand{\avroraHBNineNestedLocks}{\cna}
\newcommand{\avroraHBTenNestedLocks}{\cna}
\newcommand{\avroraHBHundredNestedLocks}{\cna}
\newcommand{\avroraFTOHBEventTotal}{1,400}
\newcommand{\avroraFTOHBNoFPEventTotal}{140}
\newcommand{\avroraFTOHBNoFPAccessTotal}{140}
\newcommand{\avroraFTOHBNoFPOtherTotal}{3.6}
\newcommand{\avroraFTOHBReadTotal}{66.6}
\newcommand{\avroraFTOHBWriteTotal}{30.8}
\newcommand{\avroraFTOHBNoFPAccessInCS}{38.6}
\newcommand{\avroraFTOHBNoFPAccessOutCS}{61.4}
\newcommand{\avroraFTOHBAcqRelTotal}{58.0}
\newcommand{\avroraFTOHBOtherTotal}{13.1}
\newcommand{\avroraFTOHBNoFPReadTotal}{94}
\newcommand{\avroraFTOHBReadInCS}{6.65}
\newcommand{\avroraFTOHBReadOutCS}{93.6}
\newcommand{\avroraFTOHBReadSameEp}{0.0276}
\newcommand{\avroraFTOHBReadSharedSameEp}{\cna}
\newcommand{\avroraFTOHBReadExclusive}{5.54}
\newcommand{\avroraFTOHBReadOwned}{90.6}
\newcommand{\avroraFTOHBReadShare}{0.0246}
\newcommand{\avroraFTOHBReadShared}{0.0683}
\newcommand{\avroraFTOHBReadSharedOwned}{3.77}
\newcommand{\avroraFTOHBNoFPHonestWriteTotal}{43}
\newcommand{\avroraFTOHBWriteInCS}{6.24}
\newcommand{\avroraFTOHBWriteOutCS}{96.5}
\newcommand{\avroraFTOHBNoFPWriteTotal}{43}
\newcommand{\avroraFTOHBWriteSameEp}{2.42}
\newcommand{\avroraFTOHBWriteExclusive}{0.326}
\newcommand{\avroraFTOHBWriteOwned}{99.7}
\newcommand{\avroraFTOHBWriteShared}{0.00256}
\newcommand{\avroraFTOHBNoFPOtherEventTotal}{3590617}
\newcommand{\avroraFTOHBAcqRelOtherTotal}{81.5}
\newcommand{\avroraFTOHBNoAcqRelOtherTotal}{662731}
\newcommand{\avroraFTOHBFork}{9.05E-4}
\newcommand{\avroraFTOHBJoin}{9.05E-4}
\newcommand{\avroraFTOHBPreWait}{50.0}
\newcommand{\avroraFTOHBPostWait}{50.0}
\newcommand{\avroraFTOHBVolatileTotal}{0.0}
\newcommand{\avroraFTOHBClassInit}{0.0189}
\newcommand{\avroraFTOHBClassAccess}{0.0279}
\newcommand{\avroraFTOHBRaceTotal}{383548}
\newcommand{\avroraFTOHBWrRdRace}{59.2}
\newcommand{\avroraFTOHBWrWrRace}{0.0}
\newcommand{\avroraFTOHBRdWrRace}{24.4}
\newcommand{\avroraFTOHBRdShWrRace}{16.4}
\newcommand{\avroraFTOHBHoldLocksTotal}{8.4}
\newcommand{\avroraFTOHBOneLockHeld}{5.83}
\newcommand{\avroraFTOHBTwoNestedLocks}{<0.1}
\newcommand{\avroraFTOHBThreeNestedLocks}{\cna}
\newcommand{\avroraFTOHBFourNestedLocks}{\cna}
\newcommand{\avroraFTOHBFiveNestedLocks}{\cna}
\newcommand{\avroraFTOHBSixNestedLocks}{\cna}
\newcommand{\avroraFTOHBSevenNestedLocks}{\cna}
\newcommand{\avroraFTOHBEightNestedLocks}{\cna}
\newcommand{\avroraFTOHBNineNestedLocks}{\cna}
\newcommand{\avroraFTOHBTenNestedLocks}{\cna}
\newcommand{\avroraFTOHBHundredNestedLocks}{\cna}
\newcommand{\avroraWCPEventTotal}{1,400}
\newcommand{\avroraWCPNoFPEventTotal}{150}
\newcommand{\avroraWCPNoFPAccessTotal}{150}
\newcommand{\avroraWCPNoFPOtherTotal}{3.7}
\newcommand{\avroraWCPReadTotal}{69.3}
\newcommand{\avroraWCPWriteTotal}{28.3}
\newcommand{\avroraWCPNoFPAccessInCS}{89.5}
\newcommand{\avroraWCPNoFPAccessOutCS}{8.97}
\newcommand{\avroraWCPAcqRelTotal}{20.9}
\newcommand{\avroraWCPOtherTotal}{5.32}
\newcommand{\avroraWCPNoFPReadTotal}{110}
\newcommand{\avroraWCPReadInCS}{6.13}
\newcommand{\avroraWCPReadOutCS}{94.1}
\newcommand{\avroraWCPReadSameEp}{0.0242}
\newcommand{\avroraWCPReadSharedSameEp}{\cna}
\newcommand{\avroraWCPReadExclusive}{93.7}
\newcommand{\avroraWCPReadOwned}{\cna}
\newcommand{\avroraWCPReadShare}{0.235}
\newcommand{\avroraWCPReadShared}{6.06}
\newcommand{\avroraWCPReadSharedOwned}{\cna}
\newcommand{\avroraWCPNoFPHonestWriteTotal}{44}
\newcommand{\avroraWCPWriteInCS}{6.16}
\newcommand{\avroraWCPWriteOutCS}{96.3}
\newcommand{\avroraWCPNoFPWriteTotal}{44}
\newcommand{\avroraWCPWriteSameEp}{2.43}
\newcommand{\avroraWCPWriteExclusive}{98.6}
\newcommand{\avroraWCPWriteOwned}{\cna}
\newcommand{\avroraWCPWriteShared}{1.37}
\newcommand{\avroraWCPNoFPOtherEventTotal}{3700337}
\newcommand{\avroraWCPAcqRelOtherTotal}{79.7}
\newcommand{\avroraWCPNoAcqRelOtherTotal}{752293}
\newcommand{\avroraWCPFork}{7.98E-4}
\newcommand{\avroraWCPJoin}{7.98E-4}
\newcommand{\avroraWCPPreWait}{50.0}
\newcommand{\avroraWCPPostWait}{50.0}
\newcommand{\avroraWCPVolatileTotal}{0.0}
\newcommand{\avroraWCPClassInit}{0.0166}
\newcommand{\avroraWCPClassAccess}{0.0246}
\newcommand{\avroraWCPRaceTotal}{505092}
\newcommand{\avroraWCPWrRdRace}{48.9}
\newcommand{\avroraWCPWrWrRace}{20.2}
\newcommand{\avroraWCPRdWrRace}{0.0552}
\newcommand{\avroraWCPRdShWrRace}{30.8}
\newcommand{\avroraWCPHoldLocksTotal}{18}
\newcommand{\avroraWCPOneLockHeld}{11.5}
\newcommand{\avroraWCPTwoNestedLocks}{<0.1}
\newcommand{\avroraWCPThreeNestedLocks}{\cna}
\newcommand{\avroraWCPFourNestedLocks}{\cna}
\newcommand{\avroraWCPFiveNestedLocks}{\cna}
\newcommand{\avroraWCPSixNestedLocks}{\cna}
\newcommand{\avroraWCPSevenNestedLocks}{\cna}
\newcommand{\avroraWCPEightNestedLocks}{\cna}
\newcommand{\avroraWCPNineNestedLocks}{\cna}
\newcommand{\avroraWCPTenNestedLocks}{\cna}
\newcommand{\avroraWCPHundredNestedLocks}{\cna}
\newcommand{\avroraFTOWCPEventTotal}{1,400}
\newcommand{\avroraFTOWCPNoFPEventTotal}{140}
\newcommand{\avroraFTOWCPNoFPAccessTotal}{140}
\newcommand{\avroraFTOWCPNoFPOtherTotal}{3.7}
\newcommand{\avroraFTOWCPReadTotal}{66.6}
\newcommand{\avroraFTOWCPWriteTotal}{30.8}
\newcommand{\avroraFTOWCPNoFPAccessInCS}{37.5}
\newcommand{\avroraFTOWCPNoFPAccessOutCS}{62.5}
\newcommand{\avroraFTOWCPAcqRelTotal}{56.6}
\newcommand{\avroraFTOWCPOtherTotal}{14.7}
\newcommand{\avroraFTOWCPNoFPReadTotal}{94}
\newcommand{\avroraFTOWCPReadInCS}{6.75}
\newcommand{\avroraFTOWCPReadOutCS}{93.5}
\newcommand{\avroraFTOWCPReadSameEp}{0.0275}
\newcommand{\avroraFTOWCPReadSharedSameEp}{\cna}
\newcommand{\avroraFTOWCPReadExclusive}{2.9}
\newcommand{\avroraFTOWCPReadOwned}{90.5}
\newcommand{\avroraFTOWCPReadShare}{0.343}
\newcommand{\avroraFTOWCPReadShared}{0.399}
\newcommand{\avroraFTOWCPReadSharedOwned}{5.89}
\newcommand{\avroraFTOWCPNoFPHonestWriteTotal}{44}
\newcommand{\avroraFTOWCPWriteInCS}{6.19}
\newcommand{\avroraFTOWCPWriteOutCS}{96.6}
\newcommand{\avroraFTOWCPNoFPWriteTotal}{44}
\newcommand{\avroraFTOWCPWriteSameEp}{2.45}
\newcommand{\avroraFTOWCPWriteExclusive}{0.281}
\newcommand{\avroraFTOWCPWriteOwned}{99.4}
\newcommand{\avroraFTOWCPWriteShared}{0.368}
\newcommand{\avroraFTOWCPNoFPOtherEventTotal}{3732975}
\newcommand{\avroraFTOWCPAcqRelOtherTotal}{79.4}
\newcommand{\avroraFTOWCPNoAcqRelOtherTotal}{769992}
\newcommand{\avroraFTOWCPFork}{7.79E-4}
\newcommand{\avroraFTOWCPJoin}{7.79E-4}
\newcommand{\avroraFTOWCPPreWait}{50.0}
\newcommand{\avroraFTOWCPPostWait}{50.0}
\newcommand{\avroraFTOWCPVolatileTotal}{0.0}
\newcommand{\avroraFTOWCPClassInit}{0.0162}
\newcommand{\avroraFTOWCPClassAccess}{0.024}
\newcommand{\avroraFTOWCPRaceTotal}{404774}
\newcommand{\avroraFTOWCPWrRdRace}{61.6}
\newcommand{\avroraFTOWCPWrWrRace}{0.0}
\newcommand{\avroraFTOWCPRdWrRace}{25.4}
\newcommand{\avroraFTOWCPRdShWrRace}{13.0}
\newcommand{\avroraFTOWCPHoldLocksTotal}{8.5}
\newcommand{\avroraFTOWCPOneLockHeld}{5.87}
\newcommand{\avroraFTOWCPTwoNestedLocks}{<0.1}
\newcommand{\avroraFTOWCPThreeNestedLocks}{\cna}
\newcommand{\avroraFTOWCPFourNestedLocks}{\cna}
\newcommand{\avroraFTOWCPFiveNestedLocks}{\cna}
\newcommand{\avroraFTOWCPSixNestedLocks}{\cna}
\newcommand{\avroraFTOWCPSevenNestedLocks}{\cna}
\newcommand{\avroraFTOWCPEightNestedLocks}{\cna}
\newcommand{\avroraFTOWCPNineNestedLocks}{\cna}
\newcommand{\avroraFTOWCPTenNestedLocks}{\cna}
\newcommand{\avroraFTOWCPHundredNestedLocks}{\cna}
\newcommand{\avroraREWCPEventTotal}{1,400}
\newcommand{\avroraREWCPNoFPEventTotal}{140}
\newcommand{\avroraREWCPNoFPAccessTotal}{140}
\newcommand{\avroraREWCPNoFPOtherTotal}{3.6}
\newcommand{\avroraREWCPReadTotal}{66.6}
\newcommand{\avroraREWCPWriteTotal}{30.8}
\newcommand{\avroraREWCPNoFPAccessInCS}{42.6}
\newcommand{\avroraREWCPNoFPAccessOutCS}{57.4}
\newcommand{\avroraREWCPAcqRelTotal}{55.8}
\newcommand{\avroraREWCPOtherTotal}{13.3}
\newcommand{\avroraREWCPNoFPReadTotal}{94}
\newcommand{\avroraREWCPReadInCS}{6.69}
\newcommand{\avroraREWCPReadOutCS}{93.6}
\newcommand{\avroraREWCPReadSameEp}{0.0276}
\newcommand{\avroraREWCPReadSharedSameEp}{\cna}
\newcommand{\avroraREWCPReadExclusive}{2.26}
\newcommand{\avroraREWCPReadOwned}{42.4}
\newcommand{\avroraREWCPReadShare}{0.658}
\newcommand{\avroraREWCPReadShared}{0.685}
\newcommand{\avroraREWCPReadSharedOwned}{54}
\newcommand{\avroraREWCPNoFPHonestWriteTotal}{43}
\newcommand{\avroraREWCPWriteInCS}{6.21}
\newcommand{\avroraREWCPWriteOutCS}{96.6}
\newcommand{\avroraREWCPNoFPWriteTotal}{43}
\newcommand{\avroraREWCPWriteSameEp}{2.43}
\newcommand{\avroraREWCPWriteExclusive}{0.307}
\newcommand{\avroraREWCPWriteOwned}{98.8}
\newcommand{\avroraREWCPWriteShared}{0.883}
\newcommand{\avroraREWCPNoFPOtherEventTotal}{3647522}
\newcommand{\avroraREWCPAcqRelOtherTotal}{80.7}
\newcommand{\avroraREWCPNoAcqRelOtherTotal}{702782}
\newcommand{\avroraREWCPFork}{8.54E-4}
\newcommand{\avroraREWCPJoin}{8.54E-4}
\newcommand{\avroraREWCPPreWait}{50.0}
\newcommand{\avroraREWCPPostWait}{50.0}
\newcommand{\avroraREWCPVolatileTotal}{0.0}
\newcommand{\avroraREWCPClassInit}{0.0178}
\newcommand{\avroraREWCPClassAccess}{0.0263}
\newcommand{\avroraREWCPRaceTotal}{416112}
\newcommand{\avroraREWCPWrRdRace}{62.8}
\newcommand{\avroraREWCPWrWrRace}{0.0}
\newcommand{\avroraREWCPRdWrRace}{25.9}
\newcommand{\avroraREWCPRdShWrRace}{11.3}
\newcommand{\avroraREWCPHoldLocksTotal}{8.6}
\newcommand{\avroraREWCPOneLockHeld}{5.92}
\newcommand{\avroraREWCPTwoNestedLocks}{<0.1}
\newcommand{\avroraREWCPThreeNestedLocks}{\cna}
\newcommand{\avroraREWCPFourNestedLocks}{\cna}
\newcommand{\avroraREWCPFiveNestedLocks}{\cna}
\newcommand{\avroraREWCPSixNestedLocks}{\cna}
\newcommand{\avroraREWCPSevenNestedLocks}{\cna}
\newcommand{\avroraREWCPEightNestedLocks}{\cna}
\newcommand{\avroraREWCPNineNestedLocks}{\cna}
\newcommand{\avroraREWCPTenNestedLocks}{\cna}
\newcommand{\avroraREWCPHundredNestedLocks}{\cna}
\newcommand{\avroraDCEventTotal}{1,400}
\newcommand{\avroraDCNoFPEventTotal}{150}
\newcommand{\avroraDCNoFPAccessTotal}{150}
\newcommand{\avroraDCNoFPOtherTotal}{3.7}
\newcommand{\avroraDCReadTotal}{69.4}
\newcommand{\avroraDCWriteTotal}{28.2}
\newcommand{\avroraDCNoFPAccessInCS}{89.5}
\newcommand{\avroraDCNoFPAccessOutCS}{9.01}
\newcommand{\avroraDCAcqRelTotal}{20.8}
\newcommand{\avroraDCOtherTotal}{5.37}
\newcommand{\avroraDCNoFPReadTotal}{110}
\newcommand{\avroraDCReadInCS}{6.13}
\newcommand{\avroraDCReadOutCS}{94.1}
\newcommand{\avroraDCReadSameEp}{0.0242}
\newcommand{\avroraDCReadSharedSameEp}{\cna}
\newcommand{\avroraDCReadExclusive}{93.4}
\newcommand{\avroraDCReadOwned}{\cna}
\newcommand{\avroraDCReadShare}{0.306}
\newcommand{\avroraDCReadShared}{6.32}
\newcommand{\avroraDCReadSharedOwned}{\cna}
\newcommand{\avroraDCNoFPHonestWriteTotal}{44}
\newcommand{\avroraDCWriteInCS}{6.15}
\newcommand{\avroraDCWriteOutCS}{96.3}
\newcommand{\avroraDCNoFPWriteTotal}{44}
\newcommand{\avroraDCWriteSameEp}{2.43}
\newcommand{\avroraDCWriteExclusive}{98.4}
\newcommand{\avroraDCWriteOwned}{\cna}
\newcommand{\avroraDCWriteShared}{1.59}
\newcommand{\avroraDCNoFPOtherEventTotal}{3702169}
\newcommand{\avroraDCAcqRelOtherTotal}{79.5}
\newcommand{\avroraDCNoAcqRelOtherTotal}{759138}
\newcommand{\avroraDCFork}{7.9E-4}
\newcommand{\avroraDCJoin}{7.9E-4}
\newcommand{\avroraDCPreWait}{50.0}
\newcommand{\avroraDCPostWait}{50.0}
\newcommand{\avroraDCVolatileTotal}{0.0}
\newcommand{\avroraDCClassInit}{0.0165}
\newcommand{\avroraDCClassAccess}{0.0244}
\newcommand{\avroraDCRaceTotal}{514203}
\newcommand{\avroraDCWrRdRace}{49.2}
\newcommand{\avroraDCWrWrRace}{20.3}
\newcommand{\avroraDCRdWrRace}{0.0463}
\newcommand{\avroraDCRdShWrRace}{30.5}
\newcommand{\avroraDCHoldLocksTotal}{18}
\newcommand{\avroraDCOneLockHeld}{11.5}
\newcommand{\avroraDCTwoNestedLocks}{<0.1}
\newcommand{\avroraDCThreeNestedLocks}{\cna}
\newcommand{\avroraDCFourNestedLocks}{\cna}
\newcommand{\avroraDCFiveNestedLocks}{\cna}
\newcommand{\avroraDCSixNestedLocks}{\cna}
\newcommand{\avroraDCSevenNestedLocks}{\cna}
\newcommand{\avroraDCEightNestedLocks}{\cna}
\newcommand{\avroraDCNineNestedLocks}{\cna}
\newcommand{\avroraDCTenNestedLocks}{\cna}
\newcommand{\avroraDCHundredNestedLocks}{\cna}
\newcommand{\avroraFTODCEventTotal}{1,400}
\newcommand{\avroraFTODCNoFPEventTotal}{140}
\newcommand{\avroraFTODCNoFPAccessTotal}{140}
\newcommand{\avroraFTODCNoFPOtherTotal}{3.7}
\newcommand{\avroraFTODCReadTotal}{66.6}
\newcommand{\avroraFTODCWriteTotal}{30.8}
\newcommand{\avroraFTODCNoFPAccessInCS}{37.5}
\newcommand{\avroraFTODCNoFPAccessOutCS}{62.5}
\newcommand{\avroraFTODCAcqRelTotal}{56.6}
\newcommand{\avroraFTODCOtherTotal}{14.7}
\newcommand{\avroraFTODCNoFPReadTotal}{94}
\newcommand{\avroraFTODCReadInCS}{6.74}
\newcommand{\avroraFTODCReadOutCS}{93.6}
\newcommand{\avroraFTODCReadSameEp}{0.0275}
\newcommand{\avroraFTODCReadSharedSameEp}{\cna}
\newcommand{\avroraFTODCReadExclusive}{2.63}
\newcommand{\avroraFTODCReadOwned}{90.5}
\newcommand{\avroraFTODCReadShare}{0.48}
\newcommand{\avroraFTODCReadShared}{0.521}
\newcommand{\avroraFTODCReadSharedOwned}{5.9}
\newcommand{\avroraFTODCNoFPHonestWriteTotal}{43}
\newcommand{\avroraFTODCWriteInCS}{6.19}
\newcommand{\avroraFTODCWriteOutCS}{96.6}
\newcommand{\avroraFTODCNoFPWriteTotal}{43}
\newcommand{\avroraFTODCWriteSameEp}{2.45}
\newcommand{\avroraFTODCWriteExclusive}{0.279}
\newcommand{\avroraFTODCWriteOwned}{99.2}
\newcommand{\avroraFTODCWriteShared}{0.522}
\newcommand{\avroraFTODCNoFPOtherEventTotal}{3722819}
\newcommand{\avroraFTODCAcqRelOtherTotal}{79.4}
\newcommand{\avroraFTODCNoAcqRelOtherTotal}{765540}
\newcommand{\avroraFTODCFork}{7.84E-4}
\newcommand{\avroraFTODCJoin}{7.84E-4}
\newcommand{\avroraFTODCPreWait}{50.0}
\newcommand{\avroraFTODCPostWait}{50.0}
\newcommand{\avroraFTODCVolatileTotal}{0.0}
\newcommand{\avroraFTODCClassInit}{0.0163}
\newcommand{\avroraFTODCClassAccess}{0.0242}
\newcommand{\avroraFTODCRaceTotal}{408940}
\newcommand{\avroraFTODCWrRdRace}{61.7}
\newcommand{\avroraFTODCWrWrRace}{0.0}
\newcommand{\avroraFTODCRdWrRace}{25.4}
\newcommand{\avroraFTODCRdShWrRace}{12.9}
\newcommand{\avroraFTODCHoldLocksTotal}{8.5}
\newcommand{\avroraFTODCOneLockHeld}{5.86}
\newcommand{\avroraFTODCTwoNestedLocks}{<0.1}
\newcommand{\avroraFTODCThreeNestedLocks}{\cna}
\newcommand{\avroraFTODCFourNestedLocks}{\cna}
\newcommand{\avroraFTODCFiveNestedLocks}{\cna}
\newcommand{\avroraFTODCSixNestedLocks}{\cna}
\newcommand{\avroraFTODCSevenNestedLocks}{\cna}
\newcommand{\avroraFTODCEightNestedLocks}{\cna}
\newcommand{\avroraFTODCNineNestedLocks}{\cna}
\newcommand{\avroraFTODCTenNestedLocks}{\cna}
\newcommand{\avroraFTODCHundredNestedLocks}{\cna}
\newcommand{\avroraREDCEventTotal}{1,400}
\newcommand{\avroraREDCNoFPEventTotal}{140}
\newcommand{\avroraREDCNoFPAccessTotal}{140}
\newcommand{\avroraREDCNoFPOtherTotal}{3.7}
\newcommand{\avroraREDCReadTotal}{66.6}
\newcommand{\avroraREDCWriteTotal}{30.8}
\newcommand{\avroraREDCNoFPAccessInCS}{44.2}
\newcommand{\avroraREDCNoFPAccessOutCS}{55.8}
\newcommand{\avroraREDCAcqRelTotal}{55.0}
\newcommand{\avroraREDCOtherTotal}{13.5}
\newcommand{\avroraREDCNoFPReadTotal}{94}
\newcommand{\avroraREDCReadInCS}{6.69}
\newcommand{\avroraREDCReadOutCS}{93.6}
\newcommand{\avroraREDCReadSameEp}{0.0276}
\newcommand{\avroraREDCReadSharedSameEp}{\cna}
\newcommand{\avroraREDCReadExclusive}{1.79}
\newcommand{\avroraREDCReadOwned}{42.4}
\newcommand{\avroraREDCReadShare}{0.901}
\newcommand{\avroraREDCReadShared}{0.875}
\newcommand{\avroraREDCReadSharedOwned}{54}
\newcommand{\avroraREDCNoFPHonestWriteTotal}{43}
\newcommand{\avroraREDCWriteInCS}{6.19}
\newcommand{\avroraREDCWriteOutCS}{96.6}
\newcommand{\avroraREDCNoFPWriteTotal}{43}
\newcommand{\avroraREDCWriteSameEp}{2.44}
\newcommand{\avroraREDCWriteExclusive}{0.295}
\newcommand{\avroraREDCWriteOwned}{98.4}
\newcommand{\avroraREDCWriteShared}{1.29}
\newcommand{\avroraREDCNoFPOtherEventTotal}{3668806}
\newcommand{\avroraREDCAcqRelOtherTotal}{80.2}
\newcommand{\avroraREDCNoAcqRelOtherTotal}{724656}
\newcommand{\avroraREDCFork}{8.28E-4}
\newcommand{\avroraREDCJoin}{8.28E-4}
\newcommand{\avroraREDCPreWait}{50.0}
\newcommand{\avroraREDCPostWait}{50.0}
\newcommand{\avroraREDCVolatileTotal}{0.0}
\newcommand{\avroraREDCClassInit}{0.0172}
\newcommand{\avroraREDCClassAccess}{0.0255}
\newcommand{\avroraREDCRaceTotal}{417100}
\newcommand{\avroraREDCWrRdRace}{62.6}
\newcommand{\avroraREDCWrWrRace}{0.0}
\newcommand{\avroraREDCRdWrRace}{25.8}
\newcommand{\avroraREDCRdShWrRace}{11.7}
\newcommand{\avroraREDCHoldLocksTotal}{8.6}
\newcommand{\avroraREDCOneLockHeld}{5.95}
\newcommand{\avroraREDCTwoNestedLocks}{<0.1}
\newcommand{\avroraREDCThreeNestedLocks}{\cna}
\newcommand{\avroraREDCFourNestedLocks}{\cna}
\newcommand{\avroraREDCFiveNestedLocks}{\cna}
\newcommand{\avroraREDCSixNestedLocks}{\cna}
\newcommand{\avroraREDCSevenNestedLocks}{\cna}
\newcommand{\avroraREDCEightNestedLocks}{\cna}
\newcommand{\avroraREDCNineNestedLocks}{\cna}
\newcommand{\avroraREDCTenNestedLocks}{\cna}
\newcommand{\avroraREDCHundredNestedLocks}{\cna}
\newcommand{\avroraCAPOEventTotal}{1,400}
\newcommand{\avroraCAPONoFPEventTotal}{150}
\newcommand{\avroraCAPONoFPAccessTotal}{150}
\newcommand{\avroraCAPONoFPOtherTotal}{3.7}
\newcommand{\avroraCAPOReadTotal}{69.4}
\newcommand{\avroraCAPOWriteTotal}{28.3}
\newcommand{\avroraCAPONoFPAccessInCS}{89.6}
\newcommand{\avroraCAPONoFPAccessOutCS}{8.88}
\newcommand{\avroraCAPOAcqRelTotal}{20.9}
\newcommand{\avroraCAPOOtherTotal}{5.13}
\newcommand{\avroraCAPONoFPReadTotal}{110}
\newcommand{\avroraCAPOReadInCS}{6.11}
\newcommand{\avroraCAPOReadOutCS}{94.1}
\newcommand{\avroraCAPOReadSameEp}{0.0242}
\newcommand{\avroraCAPOReadSharedSameEp}{\cna}
\newcommand{\avroraCAPOReadExclusive}{93.4}
\newcommand{\avroraCAPOReadOwned}{\cna}
\newcommand{\avroraCAPOReadShare}{0.317}
\newcommand{\avroraCAPOReadShared}{6.28}
\newcommand{\avroraCAPOReadSharedOwned}{\cna}
\newcommand{\avroraCAPONoFPHonestWriteTotal}{44}
\newcommand{\avroraCAPOWriteInCS}{6.17}
\newcommand{\avroraCAPOWriteOutCS}{96.3}
\newcommand{\avroraCAPONoFPWriteTotal}{44}
\newcommand{\avroraCAPOWriteSameEp}{2.42}
\newcommand{\avroraCAPOWriteExclusive}{98.4}
\newcommand{\avroraCAPOWriteOwned}{\cna}
\newcommand{\avroraCAPOWriteShared}{1.58}
\newcommand{\avroraCAPONoFPOtherEventTotal}{3662266}
\newcommand{\avroraCAPOAcqRelOtherTotal}{80.3}
\newcommand{\avroraCAPONoAcqRelOtherTotal}{720571}
\newcommand{\avroraCAPOFork}{8.33E-4}
\newcommand{\avroraCAPOJoin}{8.33E-4}
\newcommand{\avroraCAPOPreWait}{50.0}
\newcommand{\avroraCAPOPostWait}{50.0}
\newcommand{\avroraCAPOVolatileTotal}{0.0}
\newcommand{\avroraCAPOClassInit}{0.0173}
\newcommand{\avroraCAPOClassAccess}{0.0257}
\newcommand{\avroraCAPORaceTotal}{490830}
\newcommand{\avroraCAPOWrRdRace}{47.9}
\newcommand{\avroraCAPOWrWrRace}{19.8}
\newcommand{\avroraCAPORdWrRace}{0.0487}
\newcommand{\avroraCAPORdShWrRace}{32.3}
\newcommand{\avroraCAPOHoldLocksTotal}{18}
\newcommand{\avroraCAPOOneLockHeld}{11.5}
\newcommand{\avroraCAPOTwoNestedLocks}{<0.1}
\newcommand{\avroraCAPOThreeNestedLocks}{\cna}
\newcommand{\avroraCAPOFourNestedLocks}{\cna}
\newcommand{\avroraCAPOFiveNestedLocks}{\cna}
\newcommand{\avroraCAPOSixNestedLocks}{\cna}
\newcommand{\avroraCAPOSevenNestedLocks}{\cna}
\newcommand{\avroraCAPOEightNestedLocks}{\cna}
\newcommand{\avroraCAPONineNestedLocks}{\cna}
\newcommand{\avroraCAPOTenNestedLocks}{\cna}
\newcommand{\avroraCAPOHundredNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOEventTotal}{1,400}
\newcommand{\avroraFTOCAPONoFPEventTotal}{140}
\newcommand{\avroraFTOCAPONoFPAccessTotal}{140}
\newcommand{\avroraFTOCAPONoFPOtherTotal}{3.7}
\newcommand{\avroraFTOCAPOReadTotal}{66.6}
\newcommand{\avroraFTOCAPOWriteTotal}{30.8}
\newcommand{\avroraFTOCAPONoFPAccessInCS}{37.8}
\newcommand{\avroraFTOCAPONoFPAccessOutCS}{62.2}
\newcommand{\avroraFTOCAPOAcqRelTotal}{57.0}
\newcommand{\avroraFTOCAPOOtherTotal}{14.5}
\newcommand{\avroraFTOCAPONoFPReadTotal}{94}
\newcommand{\avroraFTOCAPOReadInCS}{6.74}
\newcommand{\avroraFTOCAPOReadOutCS}{93.5}
\newcommand{\avroraFTOCAPOReadSameEp}{0.0275}
\newcommand{\avroraFTOCAPOReadSharedSameEp}{\cna}
\newcommand{\avroraFTOCAPOReadExclusive}{2.61}
\newcommand{\avroraFTOCAPOReadOwned}{90.5}
\newcommand{\avroraFTOCAPOReadShare}{0.5}
\newcommand{\avroraFTOCAPOReadShared}{0.526}
\newcommand{\avroraFTOCAPOReadSharedOwned}{5.9}
\newcommand{\avroraFTOCAPONoFPHonestWriteTotal}{44}
\newcommand{\avroraFTOCAPOWriteInCS}{6.2}
\newcommand{\avroraFTOCAPOWriteOutCS}{96.6}
\newcommand{\avroraFTOCAPONoFPWriteTotal}{44}
\newcommand{\avroraFTOCAPOWriteSameEp}{2.45}
\newcommand{\avroraFTOCAPOWriteExclusive}{0.289}
\newcommand{\avroraFTOCAPOWriteOwned}{99.2}
\newcommand{\avroraFTOCAPOWriteShared}{0.527}
\newcommand{\avroraFTOCAPONoFPOtherEventTotal}{3710669}
\newcommand{\avroraFTOCAPOAcqRelOtherTotal}{79.7}
\newcommand{\avroraFTOCAPONoAcqRelOtherTotal}{751529}
\newcommand{\avroraFTOCAPOFork}{7.98E-4}
\newcommand{\avroraFTOCAPOJoin}{7.98E-4}
\newcommand{\avroraFTOCAPOPreWait}{50.0}
\newcommand{\avroraFTOCAPOPostWait}{50.0}
\newcommand{\avroraFTOCAPOVolatileTotal}{0.0}
\newcommand{\avroraFTOCAPOClassInit}{0.0166}
\newcommand{\avroraFTOCAPOClassAccess}{0.0246}
\newcommand{\avroraFTOCAPORaceTotal}{393971}
\newcommand{\avroraFTOCAPOWrRdRace}{59.7}
\newcommand{\avroraFTOCAPOWrWrRace}{0.0}
\newcommand{\avroraFTOCAPORdWrRace}{24.6}
\newcommand{\avroraFTOCAPORdShWrRace}{15.6}
\newcommand{\avroraFTOCAPOHoldLocksTotal}{8.5}
\newcommand{\avroraFTOCAPOOneLockHeld}{5.87}
\newcommand{\avroraFTOCAPOTwoNestedLocks}{<0.1}
\newcommand{\avroraFTOCAPOThreeNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOFourNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOSixNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOEightNestedLocks}{\cna}
\newcommand{\avroraFTOCAPONineNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOTenNestedLocks}{\cna}
\newcommand{\avroraFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\avroraRECAPOEventTotal}{1,400}
\newcommand{\avroraRECAPONoFPEventTotal}{140}
\newcommand{\avroraRECAPONoFPAccessTotal}{140}
\newcommand{\avroraRECAPONoFPOtherTotal}{3.6}
\newcommand{\avroraRECAPOReadTotal}{66.6}
\newcommand{\avroraRECAPOWriteTotal}{30.8}
\newcommand{\avroraRECAPONoFPAccessInCS}{44.9}
\newcommand{\avroraRECAPONoFPAccessOutCS}{55.1}
\newcommand{\avroraRECAPOAcqRelTotal}{55.8}
\newcommand{\avroraRECAPOOtherTotal}{12.6}
\newcommand{\avroraRECAPONoFPReadTotal}{94}
\newcommand{\avroraRECAPOReadInCS}{6.65}
\newcommand{\avroraRECAPOReadOutCS}{93.6}
\newcommand{\avroraRECAPOReadSameEp}{0.0276}
\newcommand{\avroraRECAPOReadSharedSameEp}{\cna}
\newcommand{\avroraRECAPOReadExclusive}{1.84}
\newcommand{\avroraRECAPOReadOwned}{42.3}
\newcommand{\avroraRECAPOReadShare}{0.92}
\newcommand{\avroraRECAPOReadShared}{0.862}
\newcommand{\avroraRECAPOReadSharedOwned}{54}
\newcommand{\avroraRECAPONoFPHonestWriteTotal}{43}
\newcommand{\avroraRECAPOWriteInCS}{6.24}
\newcommand{\avroraRECAPOWriteOutCS}{96.5}
\newcommand{\avroraRECAPONoFPWriteTotal}{43}
\newcommand{\avroraRECAPOWriteSameEp}{2.42}
\newcommand{\avroraRECAPOWriteExclusive}{0.326}
\newcommand{\avroraRECAPOWriteOwned}{98.4}
\newcommand{\avroraRECAPOWriteShared}{1.27}
\newcommand{\avroraRECAPONoFPOtherEventTotal}{3590229}
\newcommand{\avroraRECAPOAcqRelOtherTotal}{81.6}
\newcommand{\avroraRECAPONoAcqRelOtherTotal}{659696}
\newcommand{\avroraRECAPOFork}{9.1E-4}
\newcommand{\avroraRECAPOJoin}{9.1E-4}
\newcommand{\avroraRECAPOPreWait}{50.0}
\newcommand{\avroraRECAPOPostWait}{50.0}
\newcommand{\avroraRECAPOVolatileTotal}{0.0}
\newcommand{\avroraRECAPOClassInit}{0.0189}
\newcommand{\avroraRECAPOClassAccess}{0.028}
\newcommand{\avroraRECAPORaceTotal}{401530}
\newcommand{\avroraRECAPOWrRdRace}{60.8}
\newcommand{\avroraRECAPOWrWrRace}{0.0}
\newcommand{\avroraRECAPORdWrRace}{25.0}
\newcommand{\avroraRECAPORdShWrRace}{14.2}
\newcommand{\avroraRECAPOHoldLocksTotal}{8.6}
\newcommand{\avroraRECAPOOneLockHeld}{5.95}
\newcommand{\avroraRECAPOTwoNestedLocks}{<0.1}
\newcommand{\avroraRECAPOThreeNestedLocks}{\cna}
\newcommand{\avroraRECAPOFourNestedLocks}{\cna}
\newcommand{\avroraRECAPOFiveNestedLocks}{\cna}
\newcommand{\avroraRECAPOSixNestedLocks}{\cna}
\newcommand{\avroraRECAPOSevenNestedLocks}{\cna}
\newcommand{\avroraRECAPOEightNestedLocks}{\cna}
\newcommand{\avroraRECAPONineNestedLocks}{\cna}
\newcommand{\avroraRECAPOTenNestedLocks}{\cna}
\newcommand{\avroraRECAPOHundredNestedLocks}{\cna}
\newcommand{\avroraCAPOTotalSetClears}{1.8}
\newcommand{\avroraCAPOReadSetZero}{5.46E-5}
\newcommand{\avroraCAPOReadSetOne}{31.7}
\newcommand{\avroraCAPOReadSetGtOne}{68.3}
\newcommand{\avroraCAPOWriteSetZero}{58.2}
\newcommand{\avroraCAPOWriteSetOne}{1.42}
\newcommand{\avroraCAPOWriteSetGtOne}{40.3}
\newcommand{\avroraCAPOTotalMapClears}{1.8}
\newcommand{\avroraCAPOReadMapZero}{0.0}
\newcommand{\avroraCAPOReadMapOne}{0.236}
\newcommand{\avroraCAPOReadMapTen}{1.52}
\newcommand{\avroraCAPOReadMapHund}{31.6}
\newcommand{\avroraCAPOReadMapThou}{5.93}
\newcommand{\avroraCAPOReadMapGtThou}{60.8}
\newcommand{\avroraCAPOWriteMapZero}{0.285}
\newcommand{\avroraCAPOWriteMapOne}{0.0}
\newcommand{\avroraCAPOWriteMapTen}{1.36}
\newcommand{\avroraCAPOWriteMapHund}{14.6}
\newcommand{\avroraCAPOWriteMapThou}{23.0}
\newcommand{\avroraCAPOWriteMapGtThou}{60.8}
\newcommand{\FASTavroraMaxLiveThreads}{7}
\newcommand{\FASTavroraTotalThreads}{7}
\newcommand{\FASTavroraBaseTime}{2.4}
\newcommand{\FASTavroraBaseTimeCI}{20}
\newcommand{\FASTavroraEmptyTime}{\rna}
\newcommand{\FASTavroraEmptyTimeCI}{\rna}
\newcommand{\FASTavroraEmptyTimeCIMIN}{\rna}
\newcommand{\FASTavroraEmptyTimeCIMAX}{\rna}
\newcommand{\FASTavroraFTTime}{7.2}
\newcommand{\FASTavroraFTTimeCI}{0.2}
\newcommand{\FASTavroraHBTime}{6.0}
\newcommand{\FASTavroraHBTimeCI}{0.12}
\newcommand{\FASTavroraFTOHBTime}{6.0}
\newcommand{\FASTavroraFTOHBTimeCI}{0.083}
\newcommand{\FASTavroraWCPTime}{9.7}
\newcommand{\FASTavroraWCPTimeCI}{0.15}
\newcommand{\FASTavroraFTOWCPTime}{10}
\newcommand{\FASTavroraFTOWCPTimeCI}{0.069}
\newcommand{\FASTavroraREWCPTime}{8.2}
\newcommand{\FASTavroraREWCPTimeCI}{0.086}
\newcommand{\FASTavroraDCTime}{10}
\newcommand{\FASTavroraDCTimeCI}{0.14}
\newcommand{\FASTavroraFTODCTime}{11}
\newcommand{\FASTavroraFTODCTimeCI}{0.1}
\newcommand{\FASTavroraREDCTime}{9.0}
\newcommand{\FASTavroraREDCTimeCI}{0.17}
\newcommand{\FASTavroraCAPOTime}{8.0}
\newcommand{\FASTavroraCAPOTimeCI}{0.17}
\newcommand{\FASTavroraFTOCAPOTime}{8.7}
\newcommand{\FASTavroraFTOCAPOTimeCI}{0.089}
\newcommand{\FASTavroraRECAPOTime}{6.8}
\newcommand{\FASTavroraRECAPOTimeCI}{0.073}
\newcommand{\FASTavroraAGGCAPOTime}{\rna}
\newcommand{\FASTavroraAGGCAPOTimeCI}{\rna}
\newcommand{\FASTavroraAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTavroraAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTavroraStaticTime}{\rzero}
\newcommand{\FASTavroraDynamicTime}{\rzero}
\newcommand{\FASTavroraBaseMem}{160}
\newcommand{\FASTavroraBaseMemCI}{6.1}
\newcommand{\FASTavroraFTMem}{21}
\newcommand{\FASTavroraFTMemCI}{4.5}
\newcommand{\FASTavroraHBMem}{14}
\newcommand{\FASTavroraHBMemCI}{0.53}
\newcommand{\FASTavroraFTOHBMem}{14}
\newcommand{\FASTavroraFTOHBMemCI}{0.51}
\newcommand{\FASTavroraWCPMem}{32}
\newcommand{\FASTavroraWCPMemCI}{1.2}
\newcommand{\FASTavroraFTOWCPMem}{32}
\newcommand{\FASTavroraFTOWCPMemCI}{1.1}
\newcommand{\FASTavroraREWCPMem}{20}
\newcommand{\FASTavroraREWCPMemCI}{0.82}
\newcommand{\FASTavroraDCMem}{32}
\newcommand{\FASTavroraDCMemCI}{1.2}
\newcommand{\FASTavroraFTODCMem}{32}
\newcommand{\FASTavroraFTODCMemCI}{1.2}
\newcommand{\FASTavroraREDCMem}{23}
\newcommand{\FASTavroraREDCMemCI}{1.2}
\newcommand{\FASTavroraCAPOMem}{21}
\newcommand{\FASTavroraCAPOMemCI}{0.52}
\newcommand{\FASTavroraFTOCAPOMem}{20}
\newcommand{\FASTavroraFTOCAPOMemCI}{1.1}
\newcommand{\FASTavroraRECAPOMem}{15}
\newcommand{\FASTavroraRECAPOMemCI}{0.58}
\newcommand{\FASTavroraAGGCAPOMem}{\memna}
\newcommand{\FASTavroraAGGCAPOMemCI}{\memna}
\newcommand{\FASTavroraAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTavroraAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTavroraEventsCI}{32,318}
\newcommand{\FASTavroraEventsCIMIN}{1,436,881,947}
\newcommand{\FASTavroraEventsCIMAX}{1,436,946,583}
\newcommand{\FASTavroraNoFPEventsCI}{4,751}
\newcommand{\FASTavroraNoFPEventsCIMIN}{5,245,796}
\newcommand{\FASTavroraNoFPEventsCIMAX}{5,255,298}
\newcommand{\FASTavroraFT}{3}
\newcommand{\FASTavroraFTCI}{0}
\newcommand{\FASTavroraFTCIMIN}{3}
\newcommand{\FASTavroraFTCIMAX}{3}
\newcommand{\FASTavroraFTDynamic}{755,475}
\newcommand{\FASTavroraFTDynamicCI}{3,253}
\newcommand{\FASTavroraFTDynamicCIMIN}{752,222}
\newcommand{\FASTavroraFTDynamicCIMAX}{758,728}
\newcommand{\FASTavroraHB}{6}
\newcommand{\FASTavroraHBCI}{0}
\newcommand{\FASTavroraHBCIMIN}{6}
\newcommand{\FASTavroraHBCIMAX}{6}
\newcommand{\FASTavroraHBDynamic}{385,599}
\newcommand{\FASTavroraHBDynamicCI}{2,694}
\newcommand{\FASTavroraHBDynamicCIMIN}{382,905}
\newcommand{\FASTavroraHBDynamicCIMAX}{388,293}
\newcommand{\FASTavroraFTOHB}{6}
\newcommand{\FASTavroraFTOHBCI}{0}
\newcommand{\FASTavroraFTOHBCIMIN}{6}
\newcommand{\FASTavroraFTOHBCIMAX}{6}
\newcommand{\FASTavroraFTOHBDynamic}{383,548}
\newcommand{\FASTavroraFTOHBDynamicCI}{3,337}
\newcommand{\FASTavroraFTOHBDynamicCIMIN}{380,211}
\newcommand{\FASTavroraFTOHBDynamicCIMAX}{386,885}
\newcommand{\FASTavroraWCP}{5}
\newcommand{\FASTavroraWCPCI}{0}
\newcommand{\FASTavroraWCPCIMIN}{5}
\newcommand{\FASTavroraWCPCIMAX}{5}
\newcommand{\FASTavroraWCPDynamic}{402,905}
\newcommand{\FASTavroraWCPDynamicCI}{4,887}
\newcommand{\FASTavroraWCPDynamicCIMIN}{398,018}
\newcommand{\FASTavroraWCPDynamicCIMAX}{407,792}
\newcommand{\FASTavroraFTOWCP}{6}
\newcommand{\FASTavroraFTOWCPCI}{0}
\newcommand{\FASTavroraFTOWCPCIMIN}{6}
\newcommand{\FASTavroraFTOWCPCIMAX}{6}
\newcommand{\FASTavroraFTOWCPDynamic}{404,774}
\newcommand{\FASTavroraFTOWCPDynamicCI}{4,051}
\newcommand{\FASTavroraFTOWCPDynamicCIMIN}{400,723}
\newcommand{\FASTavroraFTOWCPDynamicCIMAX}{408,825}
\newcommand{\FASTavroraREWCP}{6}
\newcommand{\FASTavroraREWCPCI}{0}
\newcommand{\FASTavroraREWCPCIMIN}{6}
\newcommand{\FASTavroraREWCPCIMAX}{6}
\newcommand{\FASTavroraREWCPDynamic}{416,112}
\newcommand{\FASTavroraREWCPDynamicCI}{3,306}
\newcommand{\FASTavroraREWCPDynamicCIMIN}{412,806}
\newcommand{\FASTavroraREWCPDynamicCIMAX}{419,418}
\newcommand{\FASTavroraDC}{5}
\newcommand{\FASTavroraDCCI}{0}
\newcommand{\FASTavroraDCCIMIN}{5}
\newcommand{\FASTavroraDCCIMAX}{5}
\newcommand{\FASTavroraDCDynamic}{409,692}
\newcommand{\FASTavroraDCDynamicCI}{2,820}
\newcommand{\FASTavroraDCDynamicCIMIN}{406,872}
\newcommand{\FASTavroraDCDynamicCIMAX}{412,512}
\newcommand{\FASTavroraFTODC}{5}
\newcommand{\FASTavroraFTODCCI}{0}
\newcommand{\FASTavroraFTODCCIMIN}{5}
\newcommand{\FASTavroraFTODCCIMAX}{5}
\newcommand{\FASTavroraFTODCDynamic}{408,940}
\newcommand{\FASTavroraFTODCDynamicCI}{5,563}
\newcommand{\FASTavroraFTODCDynamicCIMIN}{403,377}
\newcommand{\FASTavroraFTODCDynamicCIMAX}{414,503}
\newcommand{\FASTavroraREDC}{5}
\newcommand{\FASTavroraREDCCI}{0}
\newcommand{\FASTavroraREDCCIMIN}{5}
\newcommand{\FASTavroraREDCCIMAX}{5}
\newcommand{\FASTavroraREDCDynamic}{417,100}
\newcommand{\FASTavroraREDCDynamicCI}{3,422}
\newcommand{\FASTavroraREDCDynamicCIMIN}{413,678}
\newcommand{\FASTavroraREDCDynamicCIMAX}{420,522}
\newcommand{\FASTavroraCAPO}{5}
\newcommand{\FASTavroraCAPOCI}{0}
\newcommand{\FASTavroraCAPOCIMIN}{5}
\newcommand{\FASTavroraCAPOCIMAX}{5}
\newcommand{\FASTavroraCAPODynamic}{393,756}
\newcommand{\FASTavroraCAPODynamicCI}{3,888}
\newcommand{\FASTavroraCAPODynamicCIMIN}{389,868}
\newcommand{\FASTavroraCAPODynamicCIMAX}{397,644}
\newcommand{\FASTavroraFTOCAPO}{5}
\newcommand{\FASTavroraFTOCAPOCI}{0}
\newcommand{\FASTavroraFTOCAPOCIMIN}{5}
\newcommand{\FASTavroraFTOCAPOCIMAX}{5}
\newcommand{\FASTavroraFTOCAPODynamic}{393,971}
\newcommand{\FASTavroraFTOCAPODynamicCI}{4,759}
\newcommand{\FASTavroraFTOCAPODynamicCIMIN}{389,212}
\newcommand{\FASTavroraFTOCAPODynamicCIMAX}{398,730}
\newcommand{\FASTavroraRECAPO}{5}
\newcommand{\FASTavroraRECAPOCI}{0}
\newcommand{\FASTavroraRECAPOCIMIN}{5}
\newcommand{\FASTavroraRECAPOCIMAX}{5}
\newcommand{\FASTavroraRECAPODynamic}{401,530}
\newcommand{\FASTavroraRECAPODynamicCI}{3,102}
\newcommand{\FASTavroraRECAPODynamicCIMIN}{398,428}
\newcommand{\FASTavroraRECAPODynamicCIMAX}{404,632}
\newcommand{\FASTavroraAGGCAPO}{\rna}
\newcommand{\FASTavroraAGGCAPOCI}{\rna}
\newcommand{\FASTavroraAGGCAPOCIMIN}{\rna}
\newcommand{\FASTavroraAGGCAPOCIMAX}{\rna}
\newcommand{\FASTavroraAGGCAPODynamic}{\rna}
\newcommand{\FASTavroraAGGCAPODynamicCI}{\rna}
\newcommand{\FASTavroraAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTavroraAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTbatikEvents}{160}
\newcommand{\FASTbatikNoFPEvents}{5.1}
\newcommand{\batikHBEventTotal}{160}
\newcommand{\batikHBNoFPEventTotal}{6.5}
\newcommand{\batikHBNoFPAccessTotal}{6.3}
\newcommand{\batikHBNoFPOtherTotal}{0.22}
\newcommand{\batikHBReadTotal}{60.4}
\newcommand{\batikHBWriteTotal}{36.2}
\newcommand{\batikHBNoFPAccessInCS}{76.2}
\newcommand{\batikHBNoFPAccessOutCS}{23.8}
\newcommand{\batikHBAcqRelTotal}{2.05}
\newcommand{\batikHBOtherTotal}{2.27}
\newcommand{\batikHBNoFPReadTotal}{3.9}
\newcommand{\batikHBReadInCS}{91.8}
\newcommand{\batikHBReadOutCS}{77.1}
\newcommand{\batikHBReadSameEp}{68.9}
\newcommand{\batikHBReadSharedSameEp}{\cna}
\newcommand{\batikHBReadExclusive}{100}
\newcommand{\batikHBReadOwned}{\cna}
\newcommand{\batikHBReadShare}{\cna}
\newcommand{\batikHBReadShared}{\cna}
\newcommand{\batikHBReadSharedOwned}{\cna}
\newcommand{\batikHBNoFPHonestWriteTotal}{2.4}
\newcommand{\batikHBWriteInCS}{134}
\newcommand{\batikHBWriteOutCS}{59.2}
\newcommand{\batikHBNoFPWriteTotal}{2.4}
\newcommand{\batikHBWriteSameEp}{93.3}
\newcommand{\batikHBWriteExclusive}{100}
\newcommand{\batikHBWriteOwned}{\cna}
\newcommand{\batikHBWriteShared}{\cna}
\newcommand{\batikHBNoFPOtherEventTotal}{221213}
\newcommand{\batikHBAcqRelOtherTotal}{47.4}
\newcommand{\batikHBNoAcqRelOtherTotal}{116273}
\newcommand{\batikHBFork}{0.00516}
\newcommand{\batikHBJoin}{0.0}
\newcommand{\batikHBPreWait}{0.0086}
\newcommand{\batikHBPostWait}{0.0086}
\newcommand{\batikHBVolatileTotal}{99.7}
\newcommand{\batikHBClassInit}{0.134}
\newcommand{\batikHBClassAccess}{0.0989}
\newcommand{\batikHBRaceTotal}{\rna}
\newcommand{\batikHBWrRdRace}{\rna}
\newcommand{\batikHBWrWrRace}{\rna}
\newcommand{\batikHBRdWrRace}{\rna}
\newcommand{\batikHBRdShWrRace}{\rna}
\newcommand{\batikHBHoldLocksTotal}{6.8}
\newcommand{\batikHBOneLockHeld}{107.}
\newcommand{\batikHBTwoNestedLocks}{<0.1}
\newcommand{\batikHBThreeNestedLocks}{<0.1}
\newcommand{\batikHBFourNestedLocks}{\cna}
\newcommand{\batikHBFiveNestedLocks}{\cna}
\newcommand{\batikHBSixNestedLocks}{\cna}
\newcommand{\batikHBSevenNestedLocks}{\cna}
\newcommand{\batikHBEightNestedLocks}{\cna}
\newcommand{\batikHBNineNestedLocks}{\cna}
\newcommand{\batikHBTenNestedLocks}{\cna}
\newcommand{\batikHBHundredNestedLocks}{\cna}
\newcommand{\batikFTOHBEventTotal}{160}
\newcommand{\batikFTOHBNoFPEventTotal}{5.8}
\newcommand{\batikFTOHBNoFPAccessTotal}{5.6}
\newcommand{\batikFTOHBNoFPOtherTotal}{0.22}
\newcommand{\batikFTOHBReadTotal}{55.7}
\newcommand{\batikFTOHBWriteTotal}{40.5}
\newcommand{\batikFTOHBNoFPAccessInCS}{76.2}
\newcommand{\batikFTOHBNoFPAccessOutCS}{23.8}
\newcommand{\batikFTOHBAcqRelTotal}{2.05}
\newcommand{\batikFTOHBOtherTotal}{2.27}
\newcommand{\batikFTOHBNoFPReadTotal}{3.2}
\newcommand{\batikFTOHBReadInCS}{97.6}
\newcommand{\batikFTOHBReadOutCS}{86.2}
\newcommand{\batikFTOHBReadSameEp}{83.8}
\newcommand{\batikFTOHBReadSharedSameEp}{\cna}
\newcommand{\batikFTOHBReadExclusive}{0.00708}
\newcommand{\batikFTOHBReadOwned}{100}
\newcommand{\batikFTOHBReadShare}{\cna}
\newcommand{\batikFTOHBReadShared}{\cna}
\newcommand{\batikFTOHBReadSharedOwned}{\cna}
\newcommand{\batikFTOHBNoFPHonestWriteTotal}{2.4}
\newcommand{\batikFTOHBWriteInCS}{134}
\newcommand{\batikFTOHBWriteOutCS}{59.2}
\newcommand{\batikFTOHBNoFPWriteTotal}{2.4}
\newcommand{\batikFTOHBWriteSameEp}{93.3}
\newcommand{\batikFTOHBWriteExclusive}{\cna}
\newcommand{\batikFTOHBWriteOwned}{100}
\newcommand{\batikFTOHBWriteShared}{\cna}
\newcommand{\batikFTOHBNoFPOtherEventTotal}{221213}
\newcommand{\batikFTOHBAcqRelOtherTotal}{47.4}
\newcommand{\batikFTOHBNoAcqRelOtherTotal}{116273}
\newcommand{\batikFTOHBFork}{0.00516}
\newcommand{\batikFTOHBJoin}{0.0}
\newcommand{\batikFTOHBPreWait}{0.0086}
\newcommand{\batikFTOHBPostWait}{0.0086}
\newcommand{\batikFTOHBVolatileTotal}{99.7}
\newcommand{\batikFTOHBClassInit}{0.134}
\newcommand{\batikFTOHBClassAccess}{0.0989}
\newcommand{\batikFTOHBRaceTotal}{\rna}
\newcommand{\batikFTOHBWrRdRace}{\rna}
\newcommand{\batikFTOHBWrWrRace}{\rna}
\newcommand{\batikFTOHBRdWrRace}{\rna}
\newcommand{\batikFTOHBRdShWrRace}{\rna}
\newcommand{\batikFTOHBHoldLocksTotal}{2.6}
\newcommand{\batikFTOHBOneLockHeld}{46.0}
\newcommand{\batikFTOHBTwoNestedLocks}{<0.1}
\newcommand{\batikFTOHBThreeNestedLocks}{<0.1}
\newcommand{\batikFTOHBFourNestedLocks}{\cna}
\newcommand{\batikFTOHBFiveNestedLocks}{\cna}
\newcommand{\batikFTOHBSixNestedLocks}{\cna}
\newcommand{\batikFTOHBSevenNestedLocks}{\cna}
\newcommand{\batikFTOHBEightNestedLocks}{\cna}
\newcommand{\batikFTOHBNineNestedLocks}{\cna}
\newcommand{\batikFTOHBTenNestedLocks}{\cna}
\newcommand{\batikFTOHBHundredNestedLocks}{\cna}
\newcommand{\batikWCPEventTotal}{160}
\newcommand{\batikWCPNoFPEventTotal}{6.5}
\newcommand{\batikWCPNoFPAccessTotal}{6.3}
\newcommand{\batikWCPNoFPOtherTotal}{0.22}
\newcommand{\batikWCPReadTotal}{60.4}
\newcommand{\batikWCPWriteTotal}{36.2}
\newcommand{\batikWCPNoFPAccessInCS}{85.3}
\newcommand{\batikWCPNoFPAccessOutCS}{14.7}
\newcommand{\batikWCPAcqRelTotal}{1.29}
\newcommand{\batikWCPOtherTotal}{1.42}
\newcommand{\batikWCPNoFPReadTotal}{3.9}
\newcommand{\batikWCPReadInCS}{91.8}
\newcommand{\batikWCPReadOutCS}{77.1}
\newcommand{\batikWCPReadSameEp}{68.9}
\newcommand{\batikWCPReadSharedSameEp}{\cna}
\newcommand{\batikWCPReadExclusive}{100}
\newcommand{\batikWCPReadOwned}{\cna}
\newcommand{\batikWCPReadShare}{<0.001}
\newcommand{\batikWCPReadShared}{0.00163}
\newcommand{\batikWCPReadSharedOwned}{\cna}
\newcommand{\batikWCPNoFPHonestWriteTotal}{2.4}
\newcommand{\batikWCPWriteInCS}{134}
\newcommand{\batikWCPWriteOutCS}{59}
\newcommand{\batikWCPNoFPWriteTotal}{2.4}
\newcommand{\batikWCPWriteSameEp}{93}
\newcommand{\batikWCPWriteExclusive}{100}
\newcommand{\batikWCPWriteOwned}{\cna}
\newcommand{\batikWCPWriteShared}{<0.001}
\newcommand{\batikWCPNoFPOtherEventTotal}{221213}
\newcommand{\batikWCPAcqRelOtherTotal}{47.4}
\newcommand{\batikWCPNoAcqRelOtherTotal}{116273}
\newcommand{\batikWCPFork}{0.00516}
\newcommand{\batikWCPJoin}{0.0}
\newcommand{\batikWCPPreWait}{0.0086}
\newcommand{\batikWCPPostWait}{0.0086}
\newcommand{\batikWCPVolatileTotal}{99.7}
\newcommand{\batikWCPClassInit}{0.134}
\newcommand{\batikWCPClassAccess}{0.0989}
\newcommand{\batikWCPRaceTotal}{\rna}
\newcommand{\batikWCPWrRdRace}{\rna}
\newcommand{\batikWCPWrWrRace}{\rna}
\newcommand{\batikWCPRdWrRace}{\rna}
\newcommand{\batikWCPRdShWrRace}{\rna}
\newcommand{\batikWCPHoldLocksTotal}{9.8}
\newcommand{\batikWCPOneLockHeld}{155.}
\newcommand{\batikWCPTwoNestedLocks}{<0.1}
\newcommand{\batikWCPThreeNestedLocks}{<0.1}
\newcommand{\batikWCPFourNestedLocks}{\cna}
\newcommand{\batikWCPFiveNestedLocks}{\cna}
\newcommand{\batikWCPSixNestedLocks}{\cna}
\newcommand{\batikWCPSevenNestedLocks}{\cna}
\newcommand{\batikWCPEightNestedLocks}{\cna}
\newcommand{\batikWCPNineNestedLocks}{\cna}
\newcommand{\batikWCPTenNestedLocks}{\cna}
\newcommand{\batikWCPHundredNestedLocks}{\cna}
\newcommand{\batikFTOWCPEventTotal}{160}
\newcommand{\batikFTOWCPNoFPEventTotal}{5.8}
\newcommand{\batikFTOWCPNoFPAccessTotal}{5.6}
\newcommand{\batikFTOWCPNoFPOtherTotal}{0.22}
\newcommand{\batikFTOWCPReadTotal}{55.6}
\newcommand{\batikFTOWCPWriteTotal}{40.6}
\newcommand{\batikFTOWCPNoFPAccessInCS}{76.2}
\newcommand{\batikFTOWCPNoFPAccessOutCS}{23.8}
\newcommand{\batikFTOWCPAcqRelTotal}{2.05}
\newcommand{\batikFTOWCPOtherTotal}{2.27}
\newcommand{\batikFTOWCPNoFPReadTotal}{3.2}
\newcommand{\batikFTOWCPReadInCS}{97.6}
\newcommand{\batikFTOWCPReadOutCS}{86.1}
\newcommand{\batikFTOWCPReadSameEp}{83.8}
\newcommand{\batikFTOWCPReadSharedSameEp}{\cna}
\newcommand{\batikFTOWCPReadExclusive}{0.00692}
\newcommand{\batikFTOWCPReadOwned}{100}
\newcommand{\batikFTOWCPReadShare}{<0.001}
\newcommand{\batikFTOWCPReadShared}{\cna}
\newcommand{\batikFTOWCPReadSharedOwned}{\cna}
\newcommand{\batikFTOWCPNoFPHonestWriteTotal}{2.4}
\newcommand{\batikFTOWCPWriteInCS}{134}
\newcommand{\batikFTOWCPWriteOutCS}{59}
\newcommand{\batikFTOWCPNoFPWriteTotal}{2.4}
\newcommand{\batikFTOWCPWriteSameEp}{93}
\newcommand{\batikFTOWCPWriteExclusive}{\cna}
\newcommand{\batikFTOWCPWriteOwned}{100}
\newcommand{\batikFTOWCPWriteShared}{<0.001}
\newcommand{\batikFTOWCPNoFPOtherEventTotal}{221213}
\newcommand{\batikFTOWCPAcqRelOtherTotal}{47.4}
\newcommand{\batikFTOWCPNoAcqRelOtherTotal}{116273}
\newcommand{\batikFTOWCPFork}{0.00516}
\newcommand{\batikFTOWCPJoin}{0.0}
\newcommand{\batikFTOWCPPreWait}{0.0086}
\newcommand{\batikFTOWCPPostWait}{0.0086}
\newcommand{\batikFTOWCPVolatileTotal}{99.7}
\newcommand{\batikFTOWCPClassInit}{0.134}
\newcommand{\batikFTOWCPClassAccess}{0.0989}
\newcommand{\batikFTOWCPRaceTotal}{\rna}
\newcommand{\batikFTOWCPWrRdRace}{\rna}
\newcommand{\batikFTOWCPWrWrRace}{\rna}
\newcommand{\batikFTOWCPRdWrRace}{\rna}
\newcommand{\batikFTOWCPRdShWrRace}{\rna}
\newcommand{\batikFTOWCPHoldLocksTotal}{2.6}
\newcommand{\batikFTOWCPOneLockHeld}{46.1}
\newcommand{\batikFTOWCPTwoNestedLocks}{<0.1}
\newcommand{\batikFTOWCPThreeNestedLocks}{<0.1}
\newcommand{\batikFTOWCPFourNestedLocks}{\cna}
\newcommand{\batikFTOWCPFiveNestedLocks}{\cna}
\newcommand{\batikFTOWCPSixNestedLocks}{\cna}
\newcommand{\batikFTOWCPSevenNestedLocks}{\cna}
\newcommand{\batikFTOWCPEightNestedLocks}{\cna}
\newcommand{\batikFTOWCPNineNestedLocks}{\cna}
\newcommand{\batikFTOWCPTenNestedLocks}{\cna}
\newcommand{\batikFTOWCPHundredNestedLocks}{\cna}
\newcommand{\batikREWCPEventTotal}{160}
\newcommand{\batikREWCPNoFPEventTotal}{5.8}
\newcommand{\batikREWCPNoFPAccessTotal}{5.6}
\newcommand{\batikREWCPNoFPOtherTotal}{0.22}
\newcommand{\batikREWCPReadTotal}{55.6}
\newcommand{\batikREWCPWriteTotal}{40.6}
\newcommand{\batikREWCPNoFPAccessInCS}{76.2}
\newcommand{\batikREWCPNoFPAccessOutCS}{23.8}
\newcommand{\batikREWCPAcqRelTotal}{2.05}
\newcommand{\batikREWCPOtherTotal}{2.27}
\newcommand{\batikREWCPNoFPReadTotal}{3.2}
\newcommand{\batikREWCPReadInCS}{97.6}
\newcommand{\batikREWCPReadOutCS}{86.1}
\newcommand{\batikREWCPReadSameEp}{83.8}
\newcommand{\batikREWCPReadSharedSameEp}{\cna}
\newcommand{\batikREWCPReadExclusive}{0.00692}
\newcommand{\batikREWCPReadOwned}{100}
\newcommand{\batikREWCPReadShare}{<0.001}
\newcommand{\batikREWCPReadShared}{\cna}
\newcommand{\batikREWCPReadSharedOwned}{\cna}
\newcommand{\batikREWCPNoFPHonestWriteTotal}{2.4}
\newcommand{\batikREWCPWriteInCS}{134}
\newcommand{\batikREWCPWriteOutCS}{59}
\newcommand{\batikREWCPNoFPWriteTotal}{2.4}
\newcommand{\batikREWCPWriteSameEp}{93}
\newcommand{\batikREWCPWriteExclusive}{\cna}
\newcommand{\batikREWCPWriteOwned}{100}
\newcommand{\batikREWCPWriteShared}{<0.001}
\newcommand{\batikREWCPNoFPOtherEventTotal}{221213}
\newcommand{\batikREWCPAcqRelOtherTotal}{47.4}
\newcommand{\batikREWCPNoAcqRelOtherTotal}{116273}
\newcommand{\batikREWCPFork}{0.00516}
\newcommand{\batikREWCPJoin}{0.0}
\newcommand{\batikREWCPPreWait}{0.0086}
\newcommand{\batikREWCPPostWait}{0.0086}
\newcommand{\batikREWCPVolatileTotal}{99.7}
\newcommand{\batikREWCPClassInit}{0.134}
\newcommand{\batikREWCPClassAccess}{0.0989}
\newcommand{\batikREWCPRaceTotal}{\rna}
\newcommand{\batikREWCPWrRdRace}{\rna}
\newcommand{\batikREWCPWrWrRace}{\rna}
\newcommand{\batikREWCPRdWrRace}{\rna}
\newcommand{\batikREWCPRdShWrRace}{\rna}
\newcommand{\batikREWCPHoldLocksTotal}{2.6}
\newcommand{\batikREWCPOneLockHeld}{46.1}
\newcommand{\batikREWCPTwoNestedLocks}{<0.1}
\newcommand{\batikREWCPThreeNestedLocks}{<0.1}
\newcommand{\batikREWCPFourNestedLocks}{\cna}
\newcommand{\batikREWCPFiveNestedLocks}{\cna}
\newcommand{\batikREWCPSixNestedLocks}{\cna}
\newcommand{\batikREWCPSevenNestedLocks}{\cna}
\newcommand{\batikREWCPEightNestedLocks}{\cna}
\newcommand{\batikREWCPNineNestedLocks}{\cna}
\newcommand{\batikREWCPTenNestedLocks}{\cna}
\newcommand{\batikREWCPHundredNestedLocks}{\cna}
\newcommand{\batikDCEventTotal}{160}
\newcommand{\batikDCNoFPEventTotal}{6.5}
\newcommand{\batikDCNoFPAccessTotal}{6.3}
\newcommand{\batikDCNoFPOtherTotal}{0.22}
\newcommand{\batikDCReadTotal}{60.4}
\newcommand{\batikDCWriteTotal}{36.2}
\newcommand{\batikDCNoFPAccessInCS}{85.3}
\newcommand{\batikDCNoFPAccessOutCS}{14.7}
\newcommand{\batikDCAcqRelTotal}{1.29}
\newcommand{\batikDCOtherTotal}{1.42}
\newcommand{\batikDCNoFPReadTotal}{3.9}
\newcommand{\batikDCReadInCS}{91.8}
\newcommand{\batikDCReadOutCS}{77.1}
\newcommand{\batikDCReadSameEp}{68.9}
\newcommand{\batikDCReadSharedSameEp}{\cna}
\newcommand{\batikDCReadExclusive}{100}
\newcommand{\batikDCReadOwned}{\cna}
\newcommand{\batikDCReadShare}{<0.001}
\newcommand{\batikDCReadShared}{0.00163}
\newcommand{\batikDCReadSharedOwned}{\cna}
\newcommand{\batikDCNoFPHonestWriteTotal}{2.4}
\newcommand{\batikDCWriteInCS}{134}
\newcommand{\batikDCWriteOutCS}{59}
\newcommand{\batikDCNoFPWriteTotal}{2.4}
\newcommand{\batikDCWriteSameEp}{93}
\newcommand{\batikDCWriteExclusive}{100}
\newcommand{\batikDCWriteOwned}{\cna}
\newcommand{\batikDCWriteShared}{<0.001}
\newcommand{\batikDCNoFPOtherEventTotal}{221213}
\newcommand{\batikDCAcqRelOtherTotal}{47.4}
\newcommand{\batikDCNoAcqRelOtherTotal}{116273}
\newcommand{\batikDCFork}{0.00516}
\newcommand{\batikDCJoin}{0.0}
\newcommand{\batikDCPreWait}{0.0086}
\newcommand{\batikDCPostWait}{0.0086}
\newcommand{\batikDCVolatileTotal}{99.7}
\newcommand{\batikDCClassInit}{0.134}
\newcommand{\batikDCClassAccess}{0.0989}
\newcommand{\batikDCRaceTotal}{\rna}
\newcommand{\batikDCWrRdRace}{\rna}
\newcommand{\batikDCWrWrRace}{\rna}
\newcommand{\batikDCRdWrRace}{\rna}
\newcommand{\batikDCRdShWrRace}{\rna}
\newcommand{\batikDCHoldLocksTotal}{9.8}
\newcommand{\batikDCOneLockHeld}{155.}
\newcommand{\batikDCTwoNestedLocks}{<0.1}
\newcommand{\batikDCThreeNestedLocks}{<0.1}
\newcommand{\batikDCFourNestedLocks}{\cna}
\newcommand{\batikDCFiveNestedLocks}{\cna}
\newcommand{\batikDCSixNestedLocks}{\cna}
\newcommand{\batikDCSevenNestedLocks}{\cna}
\newcommand{\batikDCEightNestedLocks}{\cna}
\newcommand{\batikDCNineNestedLocks}{\cna}
\newcommand{\batikDCTenNestedLocks}{\cna}
\newcommand{\batikDCHundredNestedLocks}{\cna}
\newcommand{\batikFTODCEventTotal}{160}
\newcommand{\batikFTODCNoFPEventTotal}{5.8}
\newcommand{\batikFTODCNoFPAccessTotal}{5.6}
\newcommand{\batikFTODCNoFPOtherTotal}{0.22}
\newcommand{\batikFTODCReadTotal}{55.6}
\newcommand{\batikFTODCWriteTotal}{40.6}
\newcommand{\batikFTODCNoFPAccessInCS}{76.2}
\newcommand{\batikFTODCNoFPAccessOutCS}{23.8}
\newcommand{\batikFTODCAcqRelTotal}{2.05}
\newcommand{\batikFTODCOtherTotal}{2.27}
\newcommand{\batikFTODCNoFPReadTotal}{3.2}
\newcommand{\batikFTODCReadInCS}{97.6}
\newcommand{\batikFTODCReadOutCS}{86.1}
\newcommand{\batikFTODCReadSameEp}{83.8}
\newcommand{\batikFTODCReadSharedSameEp}{\cna}
\newcommand{\batikFTODCReadExclusive}{0.00692}
\newcommand{\batikFTODCReadOwned}{100}
\newcommand{\batikFTODCReadShare}{<0.001}
\newcommand{\batikFTODCReadShared}{\cna}
\newcommand{\batikFTODCReadSharedOwned}{\cna}
\newcommand{\batikFTODCNoFPHonestWriteTotal}{2.4}
\newcommand{\batikFTODCWriteInCS}{134}
\newcommand{\batikFTODCWriteOutCS}{59}
\newcommand{\batikFTODCNoFPWriteTotal}{2.4}
\newcommand{\batikFTODCWriteSameEp}{93}
\newcommand{\batikFTODCWriteExclusive}{\cna}
\newcommand{\batikFTODCWriteOwned}{100}
\newcommand{\batikFTODCWriteShared}{<0.001}
\newcommand{\batikFTODCNoFPOtherEventTotal}{221213}
\newcommand{\batikFTODCAcqRelOtherTotal}{47.4}
\newcommand{\batikFTODCNoAcqRelOtherTotal}{116273}
\newcommand{\batikFTODCFork}{0.00516}
\newcommand{\batikFTODCJoin}{0.0}
\newcommand{\batikFTODCPreWait}{0.0086}
\newcommand{\batikFTODCPostWait}{0.0086}
\newcommand{\batikFTODCVolatileTotal}{99.7}
\newcommand{\batikFTODCClassInit}{0.134}
\newcommand{\batikFTODCClassAccess}{0.0989}
\newcommand{\batikFTODCRaceTotal}{\rna}
\newcommand{\batikFTODCWrRdRace}{\rna}
\newcommand{\batikFTODCWrWrRace}{\rna}
\newcommand{\batikFTODCRdWrRace}{\rna}
\newcommand{\batikFTODCRdShWrRace}{\rna}
\newcommand{\batikFTODCHoldLocksTotal}{2.6}
\newcommand{\batikFTODCOneLockHeld}{46.1}
\newcommand{\batikFTODCTwoNestedLocks}{<0.1}
\newcommand{\batikFTODCThreeNestedLocks}{<0.1}
\newcommand{\batikFTODCFourNestedLocks}{\cna}
\newcommand{\batikFTODCFiveNestedLocks}{\cna}
\newcommand{\batikFTODCSixNestedLocks}{\cna}
\newcommand{\batikFTODCSevenNestedLocks}{\cna}
\newcommand{\batikFTODCEightNestedLocks}{\cna}
\newcommand{\batikFTODCNineNestedLocks}{\cna}
\newcommand{\batikFTODCTenNestedLocks}{\cna}
\newcommand{\batikFTODCHundredNestedLocks}{\cna}
\newcommand{\batikREDCEventTotal}{160}
\newcommand{\batikREDCNoFPEventTotal}{5.8}
\newcommand{\batikREDCNoFPAccessTotal}{5.6}
\newcommand{\batikREDCNoFPOtherTotal}{0.22}
\newcommand{\batikREDCReadTotal}{55.6}
\newcommand{\batikREDCWriteTotal}{40.6}
\newcommand{\batikREDCNoFPAccessInCS}{76.2}
\newcommand{\batikREDCNoFPAccessOutCS}{23.8}
\newcommand{\batikREDCAcqRelTotal}{2.05}
\newcommand{\batikREDCOtherTotal}{2.27}
\newcommand{\batikREDCNoFPReadTotal}{3.2}
\newcommand{\batikREDCReadInCS}{97.6}
\newcommand{\batikREDCReadOutCS}{86.1}
\newcommand{\batikREDCReadSameEp}{83.8}
\newcommand{\batikREDCReadSharedSameEp}{\cna}
\newcommand{\batikREDCReadExclusive}{0.00692}
\newcommand{\batikREDCReadOwned}{100}
\newcommand{\batikREDCReadShare}{<0.001}
\newcommand{\batikREDCReadShared}{\cna}
\newcommand{\batikREDCReadSharedOwned}{\cna}
\newcommand{\batikREDCNoFPHonestWriteTotal}{2.4}
\newcommand{\batikREDCWriteInCS}{134}
\newcommand{\batikREDCWriteOutCS}{59}
\newcommand{\batikREDCNoFPWriteTotal}{2.4}
\newcommand{\batikREDCWriteSameEp}{93}
\newcommand{\batikREDCWriteExclusive}{\cna}
\newcommand{\batikREDCWriteOwned}{100}
\newcommand{\batikREDCWriteShared}{<0.001}
\newcommand{\batikREDCNoFPOtherEventTotal}{221213}
\newcommand{\batikREDCAcqRelOtherTotal}{47.4}
\newcommand{\batikREDCNoAcqRelOtherTotal}{116273}
\newcommand{\batikREDCFork}{0.00516}
\newcommand{\batikREDCJoin}{0.0}
\newcommand{\batikREDCPreWait}{0.0086}
\newcommand{\batikREDCPostWait}{0.0086}
\newcommand{\batikREDCVolatileTotal}{99.7}
\newcommand{\batikREDCClassInit}{0.134}
\newcommand{\batikREDCClassAccess}{0.0989}
\newcommand{\batikREDCRaceTotal}{\rna}
\newcommand{\batikREDCWrRdRace}{\rna}
\newcommand{\batikREDCWrWrRace}{\rna}
\newcommand{\batikREDCRdWrRace}{\rna}
\newcommand{\batikREDCRdShWrRace}{\rna}
\newcommand{\batikREDCHoldLocksTotal}{2.6}
\newcommand{\batikREDCOneLockHeld}{46.1}
\newcommand{\batikREDCTwoNestedLocks}{<0.1}
\newcommand{\batikREDCThreeNestedLocks}{<0.1}
\newcommand{\batikREDCFourNestedLocks}{\cna}
\newcommand{\batikREDCFiveNestedLocks}{\cna}
\newcommand{\batikREDCSixNestedLocks}{\cna}
\newcommand{\batikREDCSevenNestedLocks}{\cna}
\newcommand{\batikREDCEightNestedLocks}{\cna}
\newcommand{\batikREDCNineNestedLocks}{\cna}
\newcommand{\batikREDCTenNestedLocks}{\cna}
\newcommand{\batikREDCHundredNestedLocks}{\cna}
\newcommand{\batikCAPOEventTotal}{160}
\newcommand{\batikCAPONoFPEventTotal}{6.5}
\newcommand{\batikCAPONoFPAccessTotal}{6.3}
\newcommand{\batikCAPONoFPOtherTotal}{0.22}
\newcommand{\batikCAPOReadTotal}{60.4}
\newcommand{\batikCAPOWriteTotal}{36.2}
\newcommand{\batikCAPONoFPAccessInCS}{85.3}
\newcommand{\batikCAPONoFPAccessOutCS}{14.7}
\newcommand{\batikCAPOAcqRelTotal}{1.29}
\newcommand{\batikCAPOOtherTotal}{1.42}
\newcommand{\batikCAPONoFPReadTotal}{3.9}
\newcommand{\batikCAPOReadInCS}{91.8}
\newcommand{\batikCAPOReadOutCS}{77.1}
\newcommand{\batikCAPOReadSameEp}{68.9}
\newcommand{\batikCAPOReadSharedSameEp}{\cna}
\newcommand{\batikCAPOReadExclusive}{100}
\newcommand{\batikCAPOReadOwned}{\cna}
\newcommand{\batikCAPOReadShare}{<0.001}
\newcommand{\batikCAPOReadShared}{0.00163}
\newcommand{\batikCAPOReadSharedOwned}{\cna}
\newcommand{\batikCAPONoFPHonestWriteTotal}{2.4}
\newcommand{\batikCAPOWriteInCS}{134}
\newcommand{\batikCAPOWriteOutCS}{59}
\newcommand{\batikCAPONoFPWriteTotal}{2.4}
\newcommand{\batikCAPOWriteSameEp}{93}
\newcommand{\batikCAPOWriteExclusive}{100}
\newcommand{\batikCAPOWriteOwned}{\cna}
\newcommand{\batikCAPOWriteShared}{<0.001}
\newcommand{\batikCAPONoFPOtherEventTotal}{221213}
\newcommand{\batikCAPOAcqRelOtherTotal}{47.4}
\newcommand{\batikCAPONoAcqRelOtherTotal}{116273}
\newcommand{\batikCAPOFork}{0.00516}
\newcommand{\batikCAPOJoin}{0.0}
\newcommand{\batikCAPOPreWait}{0.0086}
\newcommand{\batikCAPOPostWait}{0.0086}
\newcommand{\batikCAPOVolatileTotal}{99.7}
\newcommand{\batikCAPOClassInit}{0.134}
\newcommand{\batikCAPOClassAccess}{0.0989}
\newcommand{\batikCAPORaceTotal}{\rna}
\newcommand{\batikCAPOWrRdRace}{\rna}
\newcommand{\batikCAPOWrWrRace}{\rna}
\newcommand{\batikCAPORdWrRace}{\rna}
\newcommand{\batikCAPORdShWrRace}{\rna}
\newcommand{\batikCAPOHoldLocksTotal}{9.8}
\newcommand{\batikCAPOOneLockHeld}{155.}
\newcommand{\batikCAPOTwoNestedLocks}{<0.1}
\newcommand{\batikCAPOThreeNestedLocks}{<0.1}
\newcommand{\batikCAPOFourNestedLocks}{\cna}
\newcommand{\batikCAPOFiveNestedLocks}{\cna}
\newcommand{\batikCAPOSixNestedLocks}{\cna}
\newcommand{\batikCAPOSevenNestedLocks}{\cna}
\newcommand{\batikCAPOEightNestedLocks}{\cna}
\newcommand{\batikCAPONineNestedLocks}{\cna}
\newcommand{\batikCAPOTenNestedLocks}{\cna}
\newcommand{\batikCAPOHundredNestedLocks}{\cna}
\newcommand{\batikFTOCAPOEventTotal}{160}
\newcommand{\batikFTOCAPONoFPEventTotal}{5.8}
\newcommand{\batikFTOCAPONoFPAccessTotal}{5.6}
\newcommand{\batikFTOCAPONoFPOtherTotal}{0.22}
\newcommand{\batikFTOCAPOReadTotal}{55.6}
\newcommand{\batikFTOCAPOWriteTotal}{40.6}
\newcommand{\batikFTOCAPONoFPAccessInCS}{76.2}
\newcommand{\batikFTOCAPONoFPAccessOutCS}{23.8}
\newcommand{\batikFTOCAPOAcqRelTotal}{2.05}
\newcommand{\batikFTOCAPOOtherTotal}{2.27}
\newcommand{\batikFTOCAPONoFPReadTotal}{3.2}
\newcommand{\batikFTOCAPOReadInCS}{97.6}
\newcommand{\batikFTOCAPOReadOutCS}{86.1}
\newcommand{\batikFTOCAPOReadSameEp}{83.8}
\newcommand{\batikFTOCAPOReadSharedSameEp}{\cna}
\newcommand{\batikFTOCAPOReadExclusive}{0.00692}
\newcommand{\batikFTOCAPOReadOwned}{100}
\newcommand{\batikFTOCAPOReadShare}{<0.001}
\newcommand{\batikFTOCAPOReadShared}{\cna}
\newcommand{\batikFTOCAPOReadSharedOwned}{\cna}
\newcommand{\batikFTOCAPONoFPHonestWriteTotal}{2.4}
\newcommand{\batikFTOCAPOWriteInCS}{134}
\newcommand{\batikFTOCAPOWriteOutCS}{59}
\newcommand{\batikFTOCAPONoFPWriteTotal}{2.4}
\newcommand{\batikFTOCAPOWriteSameEp}{93}
\newcommand{\batikFTOCAPOWriteExclusive}{\cna}
\newcommand{\batikFTOCAPOWriteOwned}{100}
\newcommand{\batikFTOCAPOWriteShared}{<0.001}
\newcommand{\batikFTOCAPONoFPOtherEventTotal}{221213}
\newcommand{\batikFTOCAPOAcqRelOtherTotal}{47.4}
\newcommand{\batikFTOCAPONoAcqRelOtherTotal}{116273}
\newcommand{\batikFTOCAPOFork}{0.00516}
\newcommand{\batikFTOCAPOJoin}{0.0}
\newcommand{\batikFTOCAPOPreWait}{0.0086}
\newcommand{\batikFTOCAPOPostWait}{0.0086}
\newcommand{\batikFTOCAPOVolatileTotal}{99.7}
\newcommand{\batikFTOCAPOClassInit}{0.134}
\newcommand{\batikFTOCAPOClassAccess}{0.0989}
\newcommand{\batikFTOCAPORaceTotal}{\rna}
\newcommand{\batikFTOCAPOWrRdRace}{\rna}
\newcommand{\batikFTOCAPOWrWrRace}{\rna}
\newcommand{\batikFTOCAPORdWrRace}{\rna}
\newcommand{\batikFTOCAPORdShWrRace}{\rna}
\newcommand{\batikFTOCAPOHoldLocksTotal}{2.6}
\newcommand{\batikFTOCAPOOneLockHeld}{46.1}
\newcommand{\batikFTOCAPOTwoNestedLocks}{<0.1}
\newcommand{\batikFTOCAPOThreeNestedLocks}{<0.1}
\newcommand{\batikFTOCAPOFourNestedLocks}{\cna}
\newcommand{\batikFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\batikFTOCAPOSixNestedLocks}{\cna}
\newcommand{\batikFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\batikFTOCAPOEightNestedLocks}{\cna}
\newcommand{\batikFTOCAPONineNestedLocks}{\cna}
\newcommand{\batikFTOCAPOTenNestedLocks}{\cna}
\newcommand{\batikFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\batikRECAPOEventTotal}{160}
\newcommand{\batikRECAPONoFPEventTotal}{5.8}
\newcommand{\batikRECAPONoFPAccessTotal}{5.6}
\newcommand{\batikRECAPONoFPOtherTotal}{0.22}
\newcommand{\batikRECAPOReadTotal}{55.6}
\newcommand{\batikRECAPOWriteTotal}{40.6}
\newcommand{\batikRECAPONoFPAccessInCS}{76.2}
\newcommand{\batikRECAPONoFPAccessOutCS}{23.8}
\newcommand{\batikRECAPOAcqRelTotal}{2.05}
\newcommand{\batikRECAPOOtherTotal}{2.27}
\newcommand{\batikRECAPONoFPReadTotal}{3.2}
\newcommand{\batikRECAPOReadInCS}{97.6}
\newcommand{\batikRECAPOReadOutCS}{86.1}
\newcommand{\batikRECAPOReadSameEp}{83.8}
\newcommand{\batikRECAPOReadSharedSameEp}{\cna}
\newcommand{\batikRECAPOReadExclusive}{0.00692}
\newcommand{\batikRECAPOReadOwned}{100}
\newcommand{\batikRECAPOReadShare}{<0.001}
\newcommand{\batikRECAPOReadShared}{\cna}
\newcommand{\batikRECAPOReadSharedOwned}{\cna}
\newcommand{\batikRECAPONoFPHonestWriteTotal}{2.4}
\newcommand{\batikRECAPOWriteInCS}{134}
\newcommand{\batikRECAPOWriteOutCS}{59}
\newcommand{\batikRECAPONoFPWriteTotal}{2.4}
\newcommand{\batikRECAPOWriteSameEp}{93}
\newcommand{\batikRECAPOWriteExclusive}{\cna}
\newcommand{\batikRECAPOWriteOwned}{100}
\newcommand{\batikRECAPOWriteShared}{<0.001}
\newcommand{\batikRECAPONoFPOtherEventTotal}{221213}
\newcommand{\batikRECAPOAcqRelOtherTotal}{47.4}
\newcommand{\batikRECAPONoAcqRelOtherTotal}{116273}
\newcommand{\batikRECAPOFork}{0.00516}
\newcommand{\batikRECAPOJoin}{0.0}
\newcommand{\batikRECAPOPreWait}{0.0086}
\newcommand{\batikRECAPOPostWait}{0.0086}
\newcommand{\batikRECAPOVolatileTotal}{99.7}
\newcommand{\batikRECAPOClassInit}{0.134}
\newcommand{\batikRECAPOClassAccess}{0.0989}
\newcommand{\batikRECAPORaceTotal}{\rna}
\newcommand{\batikRECAPOWrRdRace}{\rna}
\newcommand{\batikRECAPOWrWrRace}{\rna}
\newcommand{\batikRECAPORdWrRace}{\rna}
\newcommand{\batikRECAPORdShWrRace}{\rna}
\newcommand{\batikRECAPOHoldLocksTotal}{2.6}
\newcommand{\batikRECAPOOneLockHeld}{46.1}
\newcommand{\batikRECAPOTwoNestedLocks}{<0.1}
\newcommand{\batikRECAPOThreeNestedLocks}{<0.1}
\newcommand{\batikRECAPOFourNestedLocks}{\cna}
\newcommand{\batikRECAPOFiveNestedLocks}{\cna}
\newcommand{\batikRECAPOSixNestedLocks}{\cna}
\newcommand{\batikRECAPOSevenNestedLocks}{\cna}
\newcommand{\batikRECAPOEightNestedLocks}{\cna}
\newcommand{\batikRECAPONineNestedLocks}{\cna}
\newcommand{\batikRECAPOTenNestedLocks}{\cna}
\newcommand{\batikRECAPOHundredNestedLocks}{\cna}
\newcommand{\batikCAPOTotalSetClears}{0.052}
\newcommand{\batikCAPOReadSetZero}{0.00381}
\newcommand{\batikCAPOReadSetOne}{2.24}
\newcommand{\batikCAPOReadSetGtOne}{97.8}
\newcommand{\batikCAPOWriteSetZero}{4.98}
\newcommand{\batikCAPOWriteSetOne}{0.112}
\newcommand{\batikCAPOWriteSetGtOne}{94.9}
\newcommand{\batikCAPOTotalMapClears}{0.052}
\newcommand{\batikCAPOReadMapZero}{0.00381}
\newcommand{\batikCAPOReadMapOne}{0.242}
\newcommand{\batikCAPOReadMapTen}{14.2}
\newcommand{\batikCAPOReadMapHund}{68.9}
\newcommand{\batikCAPOReadMapThou}{16.5}
\newcommand{\batikCAPOReadMapGtThou}{0.16}
\newcommand{\batikCAPOWriteMapZero}{0.158}
\newcommand{\batikCAPOWriteMapOne}{0.0514}
\newcommand{\batikCAPOWriteMapTen}{0.32}
\newcommand{\batikCAPOWriteMapHund}{57.5}
\newcommand{\batikCAPOWriteMapThou}{37.3}
\newcommand{\batikCAPOWriteMapGtThou}{4.63}
\newcommand{\FASTbatikMaxLiveThreads}{2}
\newcommand{\FASTbatikTotalThreads}{7}
\newcommand{\FASTbatikBaseTime}{2.6}
\newcommand{\FASTbatikBaseTimeCI}{37}
\newcommand{\FASTbatikEmptyTime}{\rna}
\newcommand{\FASTbatikEmptyTimeCI}{\rna}
\newcommand{\FASTbatikEmptyTimeCIMIN}{\rna}
\newcommand{\FASTbatikEmptyTimeCIMAX}{\rna}
\newcommand{\FASTbatikFTTime}{4.1}
\newcommand{\FASTbatikFTTimeCI}{0.064}
\newcommand{\FASTbatikHBTime}{4.2}
\newcommand{\FASTbatikHBTimeCI}{0.1}
\newcommand{\FASTbatikFTOHBTime}{4.2}
\newcommand{\FASTbatikFTOHBTimeCI}{0.064}
\newcommand{\FASTbatikWCPTime}{7.0}
\newcommand{\FASTbatikWCPTimeCI}{0.13}
\newcommand{\FASTbatikFTOWCPTime}{7.2}
\newcommand{\FASTbatikFTOWCPTimeCI}{0.12}
\newcommand{\FASTbatikREWCPTime}{4.9}
\newcommand{\FASTbatikREWCPTimeCI}{0.066}
\newcommand{\FASTbatikDCTime}{7.0}
\newcommand{\FASTbatikDCTimeCI}{0.14}
\newcommand{\FASTbatikFTODCTime}{7.2}
\newcommand{\FASTbatikFTODCTimeCI}{0.14}
\newcommand{\FASTbatikREDCTime}{4.9}
\newcommand{\FASTbatikREDCTimeCI}{0.074}
\newcommand{\FASTbatikCAPOTime}{6.7}
\newcommand{\FASTbatikCAPOTimeCI}{0.31}
\newcommand{\FASTbatikFTOCAPOTime}{7.2}
\newcommand{\FASTbatikFTOCAPOTimeCI}{0.13}
\newcommand{\FASTbatikRECAPOTime}{4.9}
\newcommand{\FASTbatikRECAPOTimeCI}{0.087}
\newcommand{\FASTbatikAGGCAPOTime}{\rna}
\newcommand{\FASTbatikAGGCAPOTimeCI}{\rna}
\newcommand{\FASTbatikAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTbatikAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTbatikStaticTime}{\rzero}
\newcommand{\FASTbatikDynamicTime}{\rzero}
\newcommand{\FASTbatikBaseMem}{220}
\newcommand{\FASTbatikBaseMemCI}{3.6}
\newcommand{\FASTbatikFTMem}{5.5}
\newcommand{\FASTbatikFTMemCI}{0.12}
\newcommand{\FASTbatikHBMem}{5.5}
\newcommand{\FASTbatikHBMemCI}{0.096}
\newcommand{\FASTbatikFTOHBMem}{5.5}
\newcommand{\FASTbatikFTOHBMemCI}{0.13}
\newcommand{\FASTbatikWCPMem}{14}
\newcommand{\FASTbatikWCPMemCI}{0.69}
\newcommand{\FASTbatikFTOWCPMem}{14}
\newcommand{\FASTbatikFTOWCPMemCI}{0.36}
\newcommand{\FASTbatikREWCPMem}{11}
\newcommand{\FASTbatikREWCPMemCI}{0.19}
\newcommand{\FASTbatikDCMem}{12}
\newcommand{\FASTbatikDCMemCI}{1.1}
\newcommand{\FASTbatikFTODCMem}{14}
\newcommand{\FASTbatikFTODCMemCI}{0.32}
\newcommand{\FASTbatikREDCMem}{12}
\newcommand{\FASTbatikREDCMemCI}{0.14}
\newcommand{\FASTbatikCAPOMem}{13}
\newcommand{\FASTbatikCAPOMemCI}{1.0}
\newcommand{\FASTbatikFTOCAPOMem}{14}
\newcommand{\FASTbatikFTOCAPOMemCI}{0.41}
\newcommand{\FASTbatikRECAPOMem}{12}
\newcommand{\FASTbatikRECAPOMemCI}{0.19}
\newcommand{\FASTbatikAGGCAPOMem}{\memna}
\newcommand{\FASTbatikAGGCAPOMemCI}{\memna}
\newcommand{\FASTbatikAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTbatikAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTbatikEventsCI}{0}
\newcommand{\FASTbatikEventsCIMIN}{155,322,726}
\newcommand{\FASTbatikEventsCIMAX}{155,322,726}
\newcommand{\FASTbatikNoFPEventsCI}{0}
\newcommand{\FASTbatikNoFPEventsCIMIN}{5,127,824}
\newcommand{\FASTbatikNoFPEventsCIMAX}{5,127,824}
\newcommand{\FASTbatikFT}{0}
\newcommand{\FASTbatikFTCI}{0}
\newcommand{\FASTbatikFTCIMIN}{0}
\newcommand{\FASTbatikFTCIMAX}{0}
\newcommand{\FASTbatikFTDynamic}{0}
\newcommand{\FASTbatikFTDynamicCI}{0}
\newcommand{\FASTbatikFTDynamicCIMIN}{0}
\newcommand{\FASTbatikFTDynamicCIMAX}{0}
\newcommand{\FASTbatikHB}{0}
\newcommand{\FASTbatikHBCI}{0}
\newcommand{\FASTbatikHBCIMIN}{0}
\newcommand{\FASTbatikHBCIMAX}{0}
\newcommand{\FASTbatikHBDynamic}{0}
\newcommand{\FASTbatikHBDynamicCI}{0}
\newcommand{\FASTbatikHBDynamicCIMIN}{0}
\newcommand{\FASTbatikHBDynamicCIMAX}{0}
\newcommand{\FASTbatikFTOHB}{0}
\newcommand{\FASTbatikFTOHBCI}{0}
\newcommand{\FASTbatikFTOHBCIMIN}{0}
\newcommand{\FASTbatikFTOHBCIMAX}{0}
\newcommand{\FASTbatikFTOHBDynamic}{0}
\newcommand{\FASTbatikFTOHBDynamicCI}{0}
\newcommand{\FASTbatikFTOHBDynamicCIMIN}{0}
\newcommand{\FASTbatikFTOHBDynamicCIMAX}{0}
\newcommand{\FASTbatikWCP}{0}
\newcommand{\FASTbatikWCPCI}{0}
\newcommand{\FASTbatikWCPCIMIN}{0}
\newcommand{\FASTbatikWCPCIMAX}{0}
\newcommand{\FASTbatikWCPDynamic}{0}
\newcommand{\FASTbatikWCPDynamicCI}{0}
\newcommand{\FASTbatikWCPDynamicCIMIN}{0}
\newcommand{\FASTbatikWCPDynamicCIMAX}{0}
\newcommand{\FASTbatikFTOWCP}{0}
\newcommand{\FASTbatikFTOWCPCI}{0}
\newcommand{\FASTbatikFTOWCPCIMIN}{0}
\newcommand{\FASTbatikFTOWCPCIMAX}{0}
\newcommand{\FASTbatikFTOWCPDynamic}{0}
\newcommand{\FASTbatikFTOWCPDynamicCI}{0}
\newcommand{\FASTbatikFTOWCPDynamicCIMIN}{0}
\newcommand{\FASTbatikFTOWCPDynamicCIMAX}{0}
\newcommand{\FASTbatikREWCP}{0}
\newcommand{\FASTbatikREWCPCI}{0}
\newcommand{\FASTbatikREWCPCIMIN}{0}
\newcommand{\FASTbatikREWCPCIMAX}{0}
\newcommand{\FASTbatikREWCPDynamic}{0}
\newcommand{\FASTbatikREWCPDynamicCI}{0}
\newcommand{\FASTbatikREWCPDynamicCIMIN}{0}
\newcommand{\FASTbatikREWCPDynamicCIMAX}{0}
\newcommand{\FASTbatikDC}{0}
\newcommand{\FASTbatikDCCI}{0}
\newcommand{\FASTbatikDCCIMIN}{0}
\newcommand{\FASTbatikDCCIMAX}{0}
\newcommand{\FASTbatikDCDynamic}{0}
\newcommand{\FASTbatikDCDynamicCI}{0}
\newcommand{\FASTbatikDCDynamicCIMIN}{0}
\newcommand{\FASTbatikDCDynamicCIMAX}{0}
\newcommand{\FASTbatikFTODC}{0}
\newcommand{\FASTbatikFTODCCI}{0}
\newcommand{\FASTbatikFTODCCIMIN}{0}
\newcommand{\FASTbatikFTODCCIMAX}{0}
\newcommand{\FASTbatikFTODCDynamic}{0}
\newcommand{\FASTbatikFTODCDynamicCI}{0}
\newcommand{\FASTbatikFTODCDynamicCIMIN}{0}
\newcommand{\FASTbatikFTODCDynamicCIMAX}{0}
\newcommand{\FASTbatikREDC}{0}
\newcommand{\FASTbatikREDCCI}{0}
\newcommand{\FASTbatikREDCCIMIN}{0}
\newcommand{\FASTbatikREDCCIMAX}{0}
\newcommand{\FASTbatikREDCDynamic}{0}
\newcommand{\FASTbatikREDCDynamicCI}{0}
\newcommand{\FASTbatikREDCDynamicCIMIN}{0}
\newcommand{\FASTbatikREDCDynamicCIMAX}{0}
\newcommand{\FASTbatikCAPO}{0}
\newcommand{\FASTbatikCAPOCI}{0}
\newcommand{\FASTbatikCAPOCIMIN}{0}
\newcommand{\FASTbatikCAPOCIMAX}{0}
\newcommand{\FASTbatikCAPODynamic}{0}
\newcommand{\FASTbatikCAPODynamicCI}{0}
\newcommand{\FASTbatikCAPODynamicCIMIN}{0}
\newcommand{\FASTbatikCAPODynamicCIMAX}{0}
\newcommand{\FASTbatikFTOCAPO}{0}
\newcommand{\FASTbatikFTOCAPOCI}{0}
\newcommand{\FASTbatikFTOCAPOCIMIN}{0}
\newcommand{\FASTbatikFTOCAPOCIMAX}{0}
\newcommand{\FASTbatikFTOCAPODynamic}{0}
\newcommand{\FASTbatikFTOCAPODynamicCI}{0}
\newcommand{\FASTbatikFTOCAPODynamicCIMIN}{0}
\newcommand{\FASTbatikFTOCAPODynamicCIMAX}{0}
\newcommand{\FASTbatikRECAPO}{0}
\newcommand{\FASTbatikRECAPOCI}{0}
\newcommand{\FASTbatikRECAPOCIMIN}{0}
\newcommand{\FASTbatikRECAPOCIMAX}{0}
\newcommand{\FASTbatikRECAPODynamic}{0}
\newcommand{\FASTbatikRECAPODynamicCI}{0}
\newcommand{\FASTbatikRECAPODynamicCIMIN}{0}
\newcommand{\FASTbatikRECAPODynamicCIMAX}{0}
\newcommand{\FASTbatikAGGCAPO}{\rna}
\newcommand{\FASTbatikAGGCAPOCI}{\rna}
\newcommand{\FASTbatikAGGCAPOCIMIN}{\rna}
\newcommand{\FASTbatikAGGCAPOCIMAX}{\rna}
\newcommand{\FASTbatikAGGCAPODynamic}{\rna}
\newcommand{\FASTbatikAGGCAPODynamicCI}{\rna}
\newcommand{\FASTbatikAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTbatikAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASThtwoEvents}{3,800}
\newcommand{\FASThtwoNoFPEvents}{120}
\newcommand{\htwoHBEventTotal}{3,800}
\newcommand{\htwoHBNoFPEventTotal}{340}
\newcommand{\htwoHBNoFPAccessTotal}{340}
\newcommand{\htwoHBNoFPOtherTotal}{5.1}
\newcommand{\htwoHBReadTotal}{84.9}
\newcommand{\htwoHBWriteTotal}{13.6}
\newcommand{\htwoHBNoFPAccessInCS}{97.0}
\newcommand{\htwoHBNoFPAccessOutCS}{2.93}
\newcommand{\htwoHBAcqRelTotal}{3.17}
\newcommand{\htwoHBOtherTotal}{1.13}
\newcommand{\htwoHBNoFPReadTotal}{290}
\newcommand{\htwoHBReadInCS}{94.9}
\newcommand{\htwoHBReadOutCS}{15.2}
\newcommand{\htwoHBReadSameEp}{10}
\newcommand{\htwoHBReadSharedSameEp}{\cna}
\newcommand{\htwoHBReadExclusive}{98.8}
\newcommand{\htwoHBReadOwned}{\cna}
\newcommand{\htwoHBReadShare}{<0.001}
\newcommand{\htwoHBReadShared}{1.2}
\newcommand{\htwoHBReadSharedOwned}{\cna}
\newcommand{\htwoHBNoFPHonestWriteTotal}{46}
\newcommand{\htwoHBWriteInCS}{258}
\newcommand{\htwoHBWriteOutCS}{24.2}
\newcommand{\htwoHBNoFPWriteTotal}{46}
\newcommand{\htwoHBWriteSameEp}{182}
\newcommand{\htwoHBWriteExclusive}{99.9}
\newcommand{\htwoHBWriteOwned}{\cna}
\newcommand{\htwoHBWriteShared}{0.108}
\newcommand{\htwoHBNoFPOtherEventTotal}{5098225}
\newcommand{\htwoHBAcqRelOtherTotal}{73.7}
\newcommand{\htwoHBNoAcqRelOtherTotal}{1338987}
\newcommand{\htwoHBFork}{6.72E-4}
\newcommand{\htwoHBJoin}{6.72E-4}
\newcommand{\htwoHBPreWait}{0.0227}
\newcommand{\htwoHBPostWait}{0.0227}
\newcommand{\htwoHBVolatileTotal}{99.9}
\newcommand{\htwoHBClassInit}{0.00269}
\newcommand{\htwoHBClassAccess}{0.0134}
\newcommand{\htwoHBRaceTotal}{87091}
\newcommand{\htwoHBWrRdRace}{33.5}
\newcommand{\htwoHBWrWrRace}{32.5}
\newcommand{\htwoHBRdWrRace}{22.9}
\newcommand{\htwoHBRdShWrRace}{11.0}
\newcommand{\htwoHBHoldLocksTotal}{390}
\newcommand{\htwoHBOneLockHeld}{117.}
\newcommand{\htwoHBTwoNestedLocks}{115.}
\newcommand{\htwoHBThreeNestedLocks}{0.15}
\newcommand{\htwoHBFourNestedLocks}{<0.1}
\newcommand{\htwoHBFiveNestedLocks}{\cna}
\newcommand{\htwoHBSixNestedLocks}{\cna}
\newcommand{\htwoHBSevenNestedLocks}{\cna}
\newcommand{\htwoHBEightNestedLocks}{\cna}
\newcommand{\htwoHBNineNestedLocks}{\cna}
\newcommand{\htwoHBTenNestedLocks}{\cna}
\newcommand{\htwoHBHundredNestedLocks}{\cna}
\newcommand{\htwoFTOHBEventTotal}{3,800}
\newcommand{\htwoFTOHBNoFPEventTotal}{300}
\newcommand{\htwoFTOHBNoFPAccessTotal}{300}
\newcommand{\htwoFTOHBNoFPOtherTotal}{5.1}
\newcommand{\htwoFTOHBReadTotal}{82.9}
\newcommand{\htwoFTOHBWriteTotal}{15.4}
\newcommand{\htwoFTOHBNoFPAccessInCS}{97.1}
\newcommand{\htwoFTOHBNoFPAccessOutCS}{2.93}
\newcommand{\htwoFTOHBAcqRelTotal}{3.17}
\newcommand{\htwoFTOHBOtherTotal}{1.13}
\newcommand{\htwoFTOHBNoFPReadTotal}{250}
\newcommand{\htwoFTOHBReadInCS}{94.2}
\newcommand{\htwoFTOHBReadOutCS}{17.4}
\newcommand{\htwoFTOHBReadSameEp}{11.6}
\newcommand{\htwoFTOHBReadSharedSameEp}{\cna}
\newcommand{\htwoFTOHBReadExclusive}{13.2}
\newcommand{\htwoFTOHBReadOwned}{85.4}
\newcommand{\htwoFTOHBReadShare}{<0.001}
\newcommand{\htwoFTOHBReadShared}{0.00252}
\newcommand{\htwoFTOHBReadSharedOwned}{1.38}
\newcommand{\htwoFTOHBNoFPHonestWriteTotal}{46}
\newcommand{\htwoFTOHBWriteInCS}{258}
\newcommand{\htwoFTOHBWriteOutCS}{24.2}
\newcommand{\htwoFTOHBNoFPWriteTotal}{46}
\newcommand{\htwoFTOHBWriteSameEp}{183}
\newcommand{\htwoFTOHBWriteExclusive}{0.272}
\newcommand{\htwoFTOHBWriteOwned}{99.7}
\newcommand{\htwoFTOHBWriteShared}{0.00201}
\newcommand{\htwoFTOHBNoFPOtherEventTotal}{5098302}
\newcommand{\htwoFTOHBAcqRelOtherTotal}{73.7}
\newcommand{\htwoFTOHBNoAcqRelOtherTotal}{1339005}
\newcommand{\htwoFTOHBFork}{6.72E-4}
\newcommand{\htwoFTOHBJoin}{6.72E-4}
\newcommand{\htwoFTOHBPreWait}{0.0227}
\newcommand{\htwoFTOHBPostWait}{0.0227}
\newcommand{\htwoFTOHBVolatileTotal}{99.9}
\newcommand{\htwoFTOHBClassInit}{0.00269}
\newcommand{\htwoFTOHBClassAccess}{0.0133}
\newcommand{\htwoFTOHBRaceTotal}{59691}
\newcommand{\htwoFTOHBWrRdRace}{49.7}
\newcommand{\htwoFTOHBWrWrRace}{0.0}
\newcommand{\htwoFTOHBRdWrRace}{48.3}
\newcommand{\htwoFTOHBRdShWrRace}{2.02}
\newcommand{\htwoFTOHBHoldLocksTotal}{240}
\newcommand{\htwoFTOHBOneLockHeld}{82.6}
\newcommand{\htwoFTOHBTwoNestedLocks}{80.5}
\newcommand{\htwoFTOHBThreeNestedLocks}{0.18}
\newcommand{\htwoFTOHBFourNestedLocks}{<0.1}
\newcommand{\htwoFTOHBFiveNestedLocks}{\cna}
\newcommand{\htwoFTOHBSixNestedLocks}{\cna}
\newcommand{\htwoFTOHBSevenNestedLocks}{\cna}
\newcommand{\htwoFTOHBEightNestedLocks}{\cna}
\newcommand{\htwoFTOHBNineNestedLocks}{\cna}
\newcommand{\htwoFTOHBTenNestedLocks}{\cna}
\newcommand{\htwoFTOHBHundredNestedLocks}{\cna}
\newcommand{\htwoWCPEventTotal}{3,800}
\newcommand{\htwoWCPNoFPEventTotal}{340}
\newcommand{\htwoWCPNoFPAccessTotal}{340}
\newcommand{\htwoWCPNoFPOtherTotal}{5.1}
\newcommand{\htwoWCPReadTotal}{85.0}
\newcommand{\htwoWCPWriteTotal}{13.5}
\newcommand{\htwoWCPNoFPAccessInCS}{99.2}
\newcommand{\htwoWCPNoFPAccessOutCS}{0.832}
\newcommand{\htwoWCPAcqRelTotal}{0.927}
\newcommand{\htwoWCPOtherTotal}{0.33}
\newcommand{\htwoWCPNoFPReadTotal}{290}
\newcommand{\htwoWCPReadInCS}{94.9}
\newcommand{\htwoWCPReadOutCS}{15}
\newcommand{\htwoWCPReadSameEp}{9.91}
\newcommand{\htwoWCPReadSharedSameEp}{\cna}
\newcommand{\htwoWCPReadExclusive}{96.1}
\newcommand{\htwoWCPReadOwned}{\cna}
\newcommand{\htwoWCPReadShare}{0.0162}
\newcommand{\htwoWCPReadShared}{3.9}
\newcommand{\htwoWCPReadSharedOwned}{\cna}
\newcommand{\htwoWCPNoFPHonestWriteTotal}{46}
\newcommand{\htwoWCPWriteInCS}{258}
\newcommand{\htwoWCPWriteOutCS}{24.2}
\newcommand{\htwoWCPNoFPWriteTotal}{46}
\newcommand{\htwoWCPWriteSameEp}{182}
\newcommand{\htwoWCPWriteExclusive}{99.7}
\newcommand{\htwoWCPWriteOwned}{\cna}
\newcommand{\htwoWCPWriteShared}{0.346}
\newcommand{\htwoWCPNoFPOtherEventTotal}{5098998}
\newcommand{\htwoWCPAcqRelOtherTotal}{73.7}
\newcommand{\htwoWCPNoAcqRelOtherTotal}{1339621}
\newcommand{\htwoWCPFork}{6.72E-4}
\newcommand{\htwoWCPJoin}{6.72E-4}
\newcommand{\htwoWCPPreWait}{0.0439}
\newcommand{\htwoWCPPostWait}{0.0439}
\newcommand{\htwoWCPVolatileTotal}{99.9}
\newcommand{\htwoWCPClassInit}{0.00269}
\newcommand{\htwoWCPClassAccess}{0.0133}
\newcommand{\htwoWCPRaceTotal}{100695}
\newcommand{\htwoWCPWrRdRace}{33.4}
\newcommand{\htwoWCPWrWrRace}{32.6}
\newcommand{\htwoWCPRdWrRace}{3.89}
\newcommand{\htwoWCPRdShWrRace}{30.1}
\newcommand{\htwoWCPHoldLocksTotal}{680}
\newcommand{\htwoWCPOneLockHeld}{201.}
\newcommand{\htwoWCPTwoNestedLocks}{197.}
\newcommand{\htwoWCPThreeNestedLocks}{0.32}
\newcommand{\htwoWCPFourNestedLocks}{<0.1}
\newcommand{\htwoWCPFiveNestedLocks}{\cna}
\newcommand{\htwoWCPSixNestedLocks}{\cna}
\newcommand{\htwoWCPSevenNestedLocks}{\cna}
\newcommand{\htwoWCPEightNestedLocks}{\cna}
\newcommand{\htwoWCPNineNestedLocks}{\cna}
\newcommand{\htwoWCPTenNestedLocks}{\cna}
\newcommand{\htwoWCPHundredNestedLocks}{\cna}
\newcommand{\htwoFTOWCPEventTotal}{3,800}
\newcommand{\htwoFTOWCPNoFPEventTotal}{300}
\newcommand{\htwoFTOWCPNoFPAccessTotal}{300}
\newcommand{\htwoFTOWCPNoFPOtherTotal}{5.1}
\newcommand{\htwoFTOWCPReadTotal}{83.1}
\newcommand{\htwoFTOWCPWriteTotal}{15.2}
\newcommand{\htwoFTOWCPNoFPAccessInCS}{97.1}
\newcommand{\htwoFTOWCPNoFPAccessOutCS}{2.94}
\newcommand{\htwoFTOWCPAcqRelTotal}{3.17}
\newcommand{\htwoFTOWCPOtherTotal}{1.13}
\newcommand{\htwoFTOWCPNoFPReadTotal}{250}
\newcommand{\htwoFTOWCPReadInCS}{94.3}
\newcommand{\htwoFTOWCPReadOutCS}{17.2}
\newcommand{\htwoFTOWCPReadSameEp}{11.5}
\newcommand{\htwoFTOWCPReadSharedSameEp}{\cna}
\newcommand{\htwoFTOWCPReadExclusive}{11}
\newcommand{\htwoFTOWCPReadOwned}{84.5}
\newcommand{\htwoFTOWCPReadShare}{0.0299}
\newcommand{\htwoFTOWCPReadShared}{0.0906}
\newcommand{\htwoFTOWCPReadSharedOwned}{4.35}
\newcommand{\htwoFTOWCPNoFPHonestWriteTotal}{46}
\newcommand{\htwoFTOWCPWriteInCS}{258}
\newcommand{\htwoFTOWCPWriteOutCS}{24.2}
\newcommand{\htwoFTOWCPNoFPWriteTotal}{46}
\newcommand{\htwoFTOWCPWriteSameEp}{182}
\newcommand{\htwoFTOWCPWriteExclusive}{0.275}
\newcommand{\htwoFTOWCPWriteOwned}{99.6}
\newcommand{\htwoFTOWCPWriteShared}{0.0812}
\newcommand{\htwoFTOWCPNoFPOtherEventTotal}{5099089}
\newcommand{\htwoFTOWCPAcqRelOtherTotal}{73.7}
\newcommand{\htwoFTOWCPNoAcqRelOtherTotal}{1339679}
\newcommand{\htwoFTOWCPFork}{6.72E-4}
\newcommand{\htwoFTOWCPJoin}{6.72E-4}
\newcommand{\htwoFTOWCPPreWait}{0.046}
\newcommand{\htwoFTOWCPPostWait}{0.046}
\newcommand{\htwoFTOWCPVolatileTotal}{99.9}
\newcommand{\htwoFTOWCPClassInit}{0.00269}
\newcommand{\htwoFTOWCPClassAccess}{0.0134}
\newcommand{\htwoFTOWCPRaceTotal}{67930}
\newcommand{\htwoFTOWCPWrRdRace}{49.6}
\newcommand{\htwoFTOWCPWrWrRace}{0.0}
\newcommand{\htwoFTOWCPRdWrRace}{48.4}
\newcommand{\htwoFTOWCPRdShWrRace}{1.99}
\newcommand{\htwoFTOWCPHoldLocksTotal}{250}
\newcommand{\htwoFTOWCPOneLockHeld}{82.8}
\newcommand{\htwoFTOWCPTwoNestedLocks}{80.1}
\newcommand{\htwoFTOWCPThreeNestedLocks}{0.18}
\newcommand{\htwoFTOWCPFourNestedLocks}{<0.1}
\newcommand{\htwoFTOWCPFiveNestedLocks}{\cna}
\newcommand{\htwoFTOWCPSixNestedLocks}{\cna}
\newcommand{\htwoFTOWCPSevenNestedLocks}{\cna}
\newcommand{\htwoFTOWCPEightNestedLocks}{\cna}
\newcommand{\htwoFTOWCPNineNestedLocks}{\cna}
\newcommand{\htwoFTOWCPTenNestedLocks}{\cna}
\newcommand{\htwoFTOWCPHundredNestedLocks}{\cna}
\newcommand{\htwoREWCPEventTotal}{3,800}
\newcommand{\htwoREWCPNoFPEventTotal}{300}
\newcommand{\htwoREWCPNoFPAccessTotal}{300}
\newcommand{\htwoREWCPNoFPOtherTotal}{5.1}
\newcommand{\htwoREWCPReadTotal}{83.1}
\newcommand{\htwoREWCPWriteTotal}{15.2}
\newcommand{\htwoREWCPNoFPAccessInCS}{97.1}
\newcommand{\htwoREWCPNoFPAccessOutCS}{2.93}
\newcommand{\htwoREWCPAcqRelTotal}{3.17}
\newcommand{\htwoREWCPOtherTotal}{1.13}
\newcommand{\htwoREWCPNoFPReadTotal}{250}
\newcommand{\htwoREWCPReadInCS}{94.3}
\newcommand{\htwoREWCPReadOutCS}{17.2}
\newcommand{\htwoREWCPReadSameEp}{11.5}
\newcommand{\htwoREWCPReadSharedSameEp}{\cna}
\newcommand{\htwoREWCPReadExclusive}{9.66}
\newcommand{\htwoREWCPReadOwned}{84}
\newcommand{\htwoREWCPReadShare}{0.145}
\newcommand{\htwoREWCPReadShared}{0.193}
\newcommand{\htwoREWCPReadSharedOwned}{6.02}
\newcommand{\htwoREWCPNoFPHonestWriteTotal}{46}
\newcommand{\htwoREWCPWriteInCS}{258}
\newcommand{\htwoREWCPWriteOutCS}{24.2}
\newcommand{\htwoREWCPNoFPWriteTotal}{46}
\newcommand{\htwoREWCPWriteSameEp}{182}
\newcommand{\htwoREWCPWriteExclusive}{0.262}
\newcommand{\htwoREWCPWriteOwned}{99.2}
\newcommand{\htwoREWCPWriteShared}{0.543}
\newcommand{\htwoREWCPNoFPOtherEventTotal}{5098305}
\newcommand{\htwoREWCPAcqRelOtherTotal}{73.7}
\newcommand{\htwoREWCPNoAcqRelOtherTotal}{1339054}
\newcommand{\htwoREWCPFork}{6.72E-4}
\newcommand{\htwoREWCPJoin}{6.72E-4}
\newcommand{\htwoREWCPPreWait}{0.025}
\newcommand{\htwoREWCPPostWait}{0.025}
\newcommand{\htwoREWCPVolatileTotal}{99.9}
\newcommand{\htwoREWCPClassInit}{0.00269}
\newcommand{\htwoREWCPClassAccess}{0.0133}
\newcommand{\htwoREWCPRaceTotal}{64688}
\newcommand{\htwoREWCPWrRdRace}{49.7}
\newcommand{\htwoREWCPWrWrRace}{0.0}
\newcommand{\htwoREWCPRdWrRace}{48.3}
\newcommand{\htwoREWCPRdShWrRace}{1.95}
\newcommand{\htwoREWCPHoldLocksTotal}{250}
\newcommand{\htwoREWCPOneLockHeld}{82.8}
\newcommand{\htwoREWCPTwoNestedLocks}{80.1}
\newcommand{\htwoREWCPThreeNestedLocks}{0.18}
\newcommand{\htwoREWCPFourNestedLocks}{<0.1}
\newcommand{\htwoREWCPFiveNestedLocks}{\cna}
\newcommand{\htwoREWCPSixNestedLocks}{\cna}
\newcommand{\htwoREWCPSevenNestedLocks}{\cna}
\newcommand{\htwoREWCPEightNestedLocks}{\cna}
\newcommand{\htwoREWCPNineNestedLocks}{\cna}
\newcommand{\htwoREWCPTenNestedLocks}{\cna}
\newcommand{\htwoREWCPHundredNestedLocks}{\cna}
\newcommand{\htwoDCEventTotal}{3,800}
\newcommand{\htwoDCNoFPEventTotal}{340}
\newcommand{\htwoDCNoFPAccessTotal}{340}
\newcommand{\htwoDCNoFPOtherTotal}{5.1}
\newcommand{\htwoDCReadTotal}{85.0}
\newcommand{\htwoDCWriteTotal}{13.5}
\newcommand{\htwoDCNoFPAccessInCS}{99.2}
\newcommand{\htwoDCNoFPAccessOutCS}{0.832}
\newcommand{\htwoDCAcqRelTotal}{0.927}
\newcommand{\htwoDCOtherTotal}{0.33}
\newcommand{\htwoDCNoFPReadTotal}{290}
\newcommand{\htwoDCReadInCS}{94.9}
\newcommand{\htwoDCReadOutCS}{15}
\newcommand{\htwoDCReadSameEp}{9.91}
\newcommand{\htwoDCReadSharedSameEp}{\cna}
\newcommand{\htwoDCReadExclusive}{95.1}
\newcommand{\htwoDCReadOwned}{\cna}
\newcommand{\htwoDCReadShare}{0.0356}
\newcommand{\htwoDCReadShared}{4.89}
\newcommand{\htwoDCReadSharedOwned}{\cna}
\newcommand{\htwoDCNoFPHonestWriteTotal}{46}
\newcommand{\htwoDCWriteInCS}{258}
\newcommand{\htwoDCWriteOutCS}{24.2}
\newcommand{\htwoDCNoFPWriteTotal}{46}
\newcommand{\htwoDCWriteSameEp}{182}
\newcommand{\htwoDCWriteExclusive}{99.6}
\newcommand{\htwoDCWriteOwned}{\cna}
\newcommand{\htwoDCWriteShared}{0.402}
\newcommand{\htwoDCNoFPOtherEventTotal}{5099199}
\newcommand{\htwoDCAcqRelOtherTotal}{73.7}
\newcommand{\htwoDCNoAcqRelOtherTotal}{1339689}
\newcommand{\htwoDCFork}{6.72E-4}
\newcommand{\htwoDCJoin}{6.72E-4}
\newcommand{\htwoDCPreWait}{0.0442}
\newcommand{\htwoDCPostWait}{0.0442}
\newcommand{\htwoDCVolatileTotal}{99.9}
\newcommand{\htwoDCClassInit}{0.00269}
\newcommand{\htwoDCClassAccess}{0.0134}
\newcommand{\htwoDCRaceTotal}{101104}
\newcommand{\htwoDCWrRdRace}{33.4}
\newcommand{\htwoDCWrWrRace}{32.6}
\newcommand{\htwoDCRdWrRace}{10.0}
\newcommand{\htwoDCRdShWrRace}{24.0}
\newcommand{\htwoDCHoldLocksTotal}{680}
\newcommand{\htwoDCOneLockHeld}{201.}
\newcommand{\htwoDCTwoNestedLocks}{197.}
\newcommand{\htwoDCThreeNestedLocks}{0.32}
\newcommand{\htwoDCFourNestedLocks}{<0.1}
\newcommand{\htwoDCFiveNestedLocks}{\cna}
\newcommand{\htwoDCSixNestedLocks}{\cna}
\newcommand{\htwoDCSevenNestedLocks}{\cna}
\newcommand{\htwoDCEightNestedLocks}{\cna}
\newcommand{\htwoDCNineNestedLocks}{\cna}
\newcommand{\htwoDCTenNestedLocks}{\cna}
\newcommand{\htwoDCHundredNestedLocks}{\cna}
\newcommand{\htwoFTODCEventTotal}{3,800}
\newcommand{\htwoFTODCNoFPEventTotal}{300}
\newcommand{\htwoFTODCNoFPAccessTotal}{300}
\newcommand{\htwoFTODCNoFPOtherTotal}{5.1}
\newcommand{\htwoFTODCReadTotal}{83.1}
\newcommand{\htwoFTODCWriteTotal}{15.2}
\newcommand{\htwoFTODCNoFPAccessInCS}{97.1}
\newcommand{\htwoFTODCNoFPAccessOutCS}{2.94}
\newcommand{\htwoFTODCAcqRelTotal}{3.17}
\newcommand{\htwoFTODCOtherTotal}{1.13}
\newcommand{\htwoFTODCNoFPReadTotal}{250}
\newcommand{\htwoFTODCReadInCS}{94.3}
\newcommand{\htwoFTODCReadOutCS}{17.2}
\newcommand{\htwoFTODCReadSameEp}{11.5}
\newcommand{\htwoFTODCReadSharedSameEp}{\cna}
\newcommand{\htwoFTODCReadExclusive}{10.3}
\newcommand{\htwoFTODCReadOwned}{84.3}
\newcommand{\htwoFTODCReadShare}{0.0553}
\newcommand{\htwoFTODCReadShared}{0.175}
\newcommand{\htwoFTODCReadSharedOwned}{5.15}
\newcommand{\htwoFTODCNoFPHonestWriteTotal}{46}
\newcommand{\htwoFTODCWriteInCS}{258}
\newcommand{\htwoFTODCWriteOutCS}{24.2}
\newcommand{\htwoFTODCNoFPWriteTotal}{46}
\newcommand{\htwoFTODCWriteSameEp}{182}
\newcommand{\htwoFTODCWriteExclusive}{0.273}
\newcommand{\htwoFTODCWriteOwned}{99.6}
\newcommand{\htwoFTODCWriteShared}{0.129}
\newcommand{\htwoFTODCNoFPOtherEventTotal}{5099243}
\newcommand{\htwoFTODCAcqRelOtherTotal}{73.7}
\newcommand{\htwoFTODCNoAcqRelOtherTotal}{1339745}
\newcommand{\htwoFTODCFork}{6.72E-4}
\newcommand{\htwoFTODCJoin}{6.72E-4}
\newcommand{\htwoFTODCPreWait}{0.0469}
\newcommand{\htwoFTODCPostWait}{0.0469}
\newcommand{\htwoFTODCVolatileTotal}{99.9}
\newcommand{\htwoFTODCClassInit}{0.00269}
\newcommand{\htwoFTODCClassAccess}{0.0133}
\newcommand{\htwoFTODCRaceTotal}{68318}
\newcommand{\htwoFTODCWrRdRace}{49.5}
\newcommand{\htwoFTODCWrWrRace}{0.0}
\newcommand{\htwoFTODCRdWrRace}{48.2}
\newcommand{\htwoFTODCRdShWrRace}{2.27}
\newcommand{\htwoFTODCHoldLocksTotal}{250}
\newcommand{\htwoFTODCOneLockHeld}{82.8}
\newcommand{\htwoFTODCTwoNestedLocks}{80.1}
\newcommand{\htwoFTODCThreeNestedLocks}{0.18}
\newcommand{\htwoFTODCFourNestedLocks}{<0.1}
\newcommand{\htwoFTODCFiveNestedLocks}{\cna}
\newcommand{\htwoFTODCSixNestedLocks}{\cna}
\newcommand{\htwoFTODCSevenNestedLocks}{\cna}
\newcommand{\htwoFTODCEightNestedLocks}{\cna}
\newcommand{\htwoFTODCNineNestedLocks}{\cna}
\newcommand{\htwoFTODCTenNestedLocks}{\cna}
\newcommand{\htwoFTODCHundredNestedLocks}{\cna}
\newcommand{\htwoREDCEventTotal}{3,800}
\newcommand{\htwoREDCNoFPEventTotal}{300}
\newcommand{\htwoREDCNoFPAccessTotal}{300}
\newcommand{\htwoREDCNoFPOtherTotal}{5.1}
\newcommand{\htwoREDCReadTotal}{83.1}
\newcommand{\htwoREDCWriteTotal}{15.2}
\newcommand{\htwoREDCNoFPAccessInCS}{97.1}
\newcommand{\htwoREDCNoFPAccessOutCS}{2.93}
\newcommand{\htwoREDCAcqRelTotal}{3.17}
\newcommand{\htwoREDCOtherTotal}{1.13}
\newcommand{\htwoREDCNoFPReadTotal}{250}
\newcommand{\htwoREDCReadInCS}{94.3}
\newcommand{\htwoREDCReadOutCS}{17.2}
\newcommand{\htwoREDCReadSameEp}{11.5}
\newcommand{\htwoREDCReadSharedSameEp}{\cna}
\newcommand{\htwoREDCReadExclusive}{8.11}
\newcommand{\htwoREDCReadOwned}{83.5}
\newcommand{\htwoREDCReadShare}{0.185}
\newcommand{\htwoREDCReadShared}{0.374}
\newcommand{\htwoREDCReadSharedOwned}{7.8}
\newcommand{\htwoREDCNoFPHonestWriteTotal}{46}
\newcommand{\htwoREDCWriteInCS}{258}
\newcommand{\htwoREDCWriteOutCS}{24.2}
\newcommand{\htwoREDCNoFPWriteTotal}{46}
\newcommand{\htwoREDCWriteSameEp}{182}
\newcommand{\htwoREDCWriteExclusive}{0.26}
\newcommand{\htwoREDCWriteOwned}{99.1}
\newcommand{\htwoREDCWriteShared}{0.603}
\newcommand{\htwoREDCNoFPOtherEventTotal}{5098464}
\newcommand{\htwoREDCAcqRelOtherTotal}{73.7}
\newcommand{\htwoREDCNoAcqRelOtherTotal}{1339098}
\newcommand{\htwoREDCFork}{6.72E-4}
\newcommand{\htwoREDCJoin}{6.72E-4}
\newcommand{\htwoREDCPreWait}{0.0256}
\newcommand{\htwoREDCPostWait}{0.0256}
\newcommand{\htwoREDCVolatileTotal}{99.9}
\newcommand{\htwoREDCClassInit}{0.00269}
\newcommand{\htwoREDCClassAccess}{0.0133}
\newcommand{\htwoREDCRaceTotal}{65747}
\newcommand{\htwoREDCWrRdRace}{49.7}
\newcommand{\htwoREDCWrWrRace}{0.0}
\newcommand{\htwoREDCRdWrRace}{48.2}
\newcommand{\htwoREDCRdShWrRace}{2.1}
\newcommand{\htwoREDCHoldLocksTotal}{250}
\newcommand{\htwoREDCOneLockHeld}{82.8}
\newcommand{\htwoREDCTwoNestedLocks}{80.1}
\newcommand{\htwoREDCThreeNestedLocks}{0.18}
\newcommand{\htwoREDCFourNestedLocks}{<0.1}
\newcommand{\htwoREDCFiveNestedLocks}{\cna}
\newcommand{\htwoREDCSixNestedLocks}{\cna}
\newcommand{\htwoREDCSevenNestedLocks}{\cna}
\newcommand{\htwoREDCEightNestedLocks}{\cna}
\newcommand{\htwoREDCNineNestedLocks}{\cna}
\newcommand{\htwoREDCTenNestedLocks}{\cna}
\newcommand{\htwoREDCHundredNestedLocks}{\cna}
\newcommand{\htwoCAPOEventTotal}{3,800}
\newcommand{\htwoCAPONoFPEventTotal}{340}
\newcommand{\htwoCAPONoFPAccessTotal}{340}
\newcommand{\htwoCAPONoFPOtherTotal}{5.1}
\newcommand{\htwoCAPOReadTotal}{85.0}
\newcommand{\htwoCAPOWriteTotal}{13.5}
\newcommand{\htwoCAPONoFPAccessInCS}{99.2}
\newcommand{\htwoCAPONoFPAccessOutCS}{0.832}
\newcommand{\htwoCAPOAcqRelTotal}{0.927}
\newcommand{\htwoCAPOOtherTotal}{0.33}
\newcommand{\htwoCAPONoFPReadTotal}{290}
\newcommand{\htwoCAPOReadInCS}{94.9}
\newcommand{\htwoCAPOReadOutCS}{15}
\newcommand{\htwoCAPOReadSameEp}{9.91}
\newcommand{\htwoCAPOReadSharedSameEp}{\cna}
\newcommand{\htwoCAPOReadExclusive}{95.2}
\newcommand{\htwoCAPOReadOwned}{\cna}
\newcommand{\htwoCAPOReadShare}{0.0331}
\newcommand{\htwoCAPOReadShared}{4.75}
\newcommand{\htwoCAPOReadSharedOwned}{\cna}
\newcommand{\htwoCAPONoFPHonestWriteTotal}{46}
\newcommand{\htwoCAPOWriteInCS}{258}
\newcommand{\htwoCAPOWriteOutCS}{24.2}
\newcommand{\htwoCAPONoFPWriteTotal}{46}
\newcommand{\htwoCAPOWriteSameEp}{182}
\newcommand{\htwoCAPOWriteExclusive}{99.6}
\newcommand{\htwoCAPOWriteOwned}{\cna}
\newcommand{\htwoCAPOWriteShared}{0.379}
\newcommand{\htwoCAPONoFPOtherEventTotal}{5099099}
\newcommand{\htwoCAPOAcqRelOtherTotal}{73.7}
\newcommand{\htwoCAPONoAcqRelOtherTotal}{1339636}
\newcommand{\htwoCAPOFork}{6.72E-4}
\newcommand{\htwoCAPOJoin}{6.72E-4}
\newcommand{\htwoCAPOPreWait}{0.0433}
\newcommand{\htwoCAPOPostWait}{0.0433}
\newcommand{\htwoCAPOVolatileTotal}{99.9}
\newcommand{\htwoCAPOClassInit}{0.00269}
\newcommand{\htwoCAPOClassAccess}{0.0133}
\newcommand{\htwoCAPORaceTotal}{101343}
\newcommand{\htwoCAPOWrRdRace}{33.5}
\newcommand{\htwoCAPOWrWrRace}{32.6}
\newcommand{\htwoCAPORdWrRace}{17.1}
\newcommand{\htwoCAPORdShWrRace}{16.8}
\newcommand{\htwoCAPOHoldLocksTotal}{680}
\newcommand{\htwoCAPOOneLockHeld}{201.}
\newcommand{\htwoCAPOTwoNestedLocks}{197.}
\newcommand{\htwoCAPOThreeNestedLocks}{0.32}
\newcommand{\htwoCAPOFourNestedLocks}{<0.1}
\newcommand{\htwoCAPOFiveNestedLocks}{\cna}
\newcommand{\htwoCAPOSixNestedLocks}{\cna}
\newcommand{\htwoCAPOSevenNestedLocks}{\cna}
\newcommand{\htwoCAPOEightNestedLocks}{\cna}
\newcommand{\htwoCAPONineNestedLocks}{\cna}
\newcommand{\htwoCAPOTenNestedLocks}{\cna}
\newcommand{\htwoCAPOHundredNestedLocks}{\cna}
\newcommand{\htwoFTOCAPOEventTotal}{3,800}
\newcommand{\htwoFTOCAPONoFPEventTotal}{300}
\newcommand{\htwoFTOCAPONoFPAccessTotal}{300}
\newcommand{\htwoFTOCAPONoFPOtherTotal}{5.1}
\newcommand{\htwoFTOCAPOReadTotal}{83.1}
\newcommand{\htwoFTOCAPOWriteTotal}{15.2}
\newcommand{\htwoFTOCAPONoFPAccessInCS}{97.1}
\newcommand{\htwoFTOCAPONoFPAccessOutCS}{2.94}
\newcommand{\htwoFTOCAPOAcqRelTotal}{3.17}
\newcommand{\htwoFTOCAPOOtherTotal}{1.13}
\newcommand{\htwoFTOCAPONoFPReadTotal}{250}
\newcommand{\htwoFTOCAPOReadInCS}{94.3}
\newcommand{\htwoFTOCAPOReadOutCS}{17.2}
\newcommand{\htwoFTOCAPOReadSameEp}{11.5}
\newcommand{\htwoFTOCAPOReadSharedSameEp}{\cna}
\newcommand{\htwoFTOCAPOReadExclusive}{10.5}
\newcommand{\htwoFTOCAPOReadOwned}{84.3}
\newcommand{\htwoFTOCAPOReadShare}{0.0509}
\newcommand{\htwoFTOCAPOReadShared}{0.152}
\newcommand{\htwoFTOCAPOReadSharedOwned}{5.01}
\newcommand{\htwoFTOCAPONoFPHonestWriteTotal}{46}
\newcommand{\htwoFTOCAPOWriteInCS}{258}
\newcommand{\htwoFTOCAPOWriteOutCS}{24.2}
\newcommand{\htwoFTOCAPONoFPWriteTotal}{46}
\newcommand{\htwoFTOCAPOWriteSameEp}{182}
\newcommand{\htwoFTOCAPOWriteExclusive}{0.274}
\newcommand{\htwoFTOCAPOWriteOwned}{99.6}
\newcommand{\htwoFTOCAPOWriteShared}{0.127}
\newcommand{\htwoFTOCAPONoFPOtherEventTotal}{5099103}
\newcommand{\htwoFTOCAPOAcqRelOtherTotal}{73.7}
\newcommand{\htwoFTOCAPONoAcqRelOtherTotal}{1339668}
\newcommand{\htwoFTOCAPOFork}{6.72E-4}
\newcommand{\htwoFTOCAPOJoin}{6.72E-4}
\newcommand{\htwoFTOCAPOPreWait}{0.0451}
\newcommand{\htwoFTOCAPOPostWait}{0.0451}
\newcommand{\htwoFTOCAPOVolatileTotal}{99.9}
\newcommand{\htwoFTOCAPOClassInit}{0.00269}
\newcommand{\htwoFTOCAPOClassAccess}{0.0133}
\newcommand{\htwoFTOCAPORaceTotal}{68560}
\newcommand{\htwoFTOCAPOWrRdRace}{49.6}
\newcommand{\htwoFTOCAPOWrWrRace}{0.0}
\newcommand{\htwoFTOCAPORdWrRace}{48.2}
\newcommand{\htwoFTOCAPORdShWrRace}{2.19}
\newcommand{\htwoFTOCAPOHoldLocksTotal}{250}
\newcommand{\htwoFTOCAPOOneLockHeld}{82.8}
\newcommand{\htwoFTOCAPOTwoNestedLocks}{80.1}
\newcommand{\htwoFTOCAPOThreeNestedLocks}{0.18}
\newcommand{\htwoFTOCAPOFourNestedLocks}{<0.1}
\newcommand{\htwoFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\htwoFTOCAPOSixNestedLocks}{\cna}
\newcommand{\htwoFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\htwoFTOCAPOEightNestedLocks}{\cna}
\newcommand{\htwoFTOCAPONineNestedLocks}{\cna}
\newcommand{\htwoFTOCAPOTenNestedLocks}{\cna}
\newcommand{\htwoFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\htwoRECAPOEventTotal}{3,800}
\newcommand{\htwoRECAPONoFPEventTotal}{300}
\newcommand{\htwoRECAPONoFPAccessTotal}{300}
\newcommand{\htwoRECAPONoFPOtherTotal}{5.1}
\newcommand{\htwoRECAPOReadTotal}{83.1}
\newcommand{\htwoRECAPOWriteTotal}{15.2}
\newcommand{\htwoRECAPONoFPAccessInCS}{97.1}
\newcommand{\htwoRECAPONoFPAccessOutCS}{2.93}
\newcommand{\htwoRECAPOAcqRelTotal}{3.17}
\newcommand{\htwoRECAPOOtherTotal}{1.13}
\newcommand{\htwoRECAPONoFPReadTotal}{250}
\newcommand{\htwoRECAPOReadInCS}{94.3}
\newcommand{\htwoRECAPOReadOutCS}{17.2}
\newcommand{\htwoRECAPOReadSameEp}{11.5}
\newcommand{\htwoRECAPOReadSharedSameEp}{\cna}
\newcommand{\htwoRECAPOReadExclusive}{8.13}
\newcommand{\htwoRECAPOReadOwned}{83.6}
\newcommand{\htwoRECAPOReadShare}{0.181}
\newcommand{\htwoRECAPOReadShared}{0.37}
\newcommand{\htwoRECAPOReadSharedOwned}{7.74}
\newcommand{\htwoRECAPONoFPHonestWriteTotal}{46}
\newcommand{\htwoRECAPOWriteInCS}{258}
\newcommand{\htwoRECAPOWriteOutCS}{24.2}
\newcommand{\htwoRECAPONoFPWriteTotal}{46}
\newcommand{\htwoRECAPOWriteSameEp}{182}
\newcommand{\htwoRECAPOWriteExclusive}{0.26}
\newcommand{\htwoRECAPOWriteOwned}{99.2}
\newcommand{\htwoRECAPOWriteShared}{0.584}
\newcommand{\htwoRECAPONoFPOtherEventTotal}{5098449}
\newcommand{\htwoRECAPOAcqRelOtherTotal}{73.7}
\newcommand{\htwoRECAPONoAcqRelOtherTotal}{1339073}
\newcommand{\htwoRECAPOFork}{6.72E-4}
\newcommand{\htwoRECAPOJoin}{6.72E-4}
\newcommand{\htwoRECAPOPreWait}{0.0246}
\newcommand{\htwoRECAPOPostWait}{0.0246}
\newcommand{\htwoRECAPOVolatileTotal}{99.9}
\newcommand{\htwoRECAPOClassInit}{0.00269}
\newcommand{\htwoRECAPOClassAccess}{0.0134}
\newcommand{\htwoRECAPORaceTotal}{63127}
\newcommand{\htwoRECAPOWrRdRace}{49.7}
\newcommand{\htwoRECAPOWrWrRace}{0.0}
\newcommand{\htwoRECAPORdWrRace}{48.1}
\newcommand{\htwoRECAPORdShWrRace}{2.17}
\newcommand{\htwoRECAPOHoldLocksTotal}{250}
\newcommand{\htwoRECAPOOneLockHeld}{82.8}
\newcommand{\htwoRECAPOTwoNestedLocks}{80.1}
\newcommand{\htwoRECAPOThreeNestedLocks}{0.18}
\newcommand{\htwoRECAPOFourNestedLocks}{<0.1}
\newcommand{\htwoRECAPOFiveNestedLocks}{\cna}
\newcommand{\htwoRECAPOSixNestedLocks}{\cna}
\newcommand{\htwoRECAPOSevenNestedLocks}{\cna}
\newcommand{\htwoRECAPOEightNestedLocks}{\cna}
\newcommand{\htwoRECAPONineNestedLocks}{\cna}
\newcommand{\htwoRECAPOTenNestedLocks}{\cna}
\newcommand{\htwoRECAPOHundredNestedLocks}{\cna}
\newcommand{\htwoCAPOTotalSetClears}{1.9}
\newcommand{\htwoCAPOReadSetZero}{3.19E-4}
\newcommand{\htwoCAPOReadSetOne}{35.2}
\newcommand{\htwoCAPOReadSetGtOne}{64.8}
\newcommand{\htwoCAPOWriteSetZero}{34.8}
\newcommand{\htwoCAPOWriteSetOne}{0.426}
\newcommand{\htwoCAPOWriteSetGtOne}{64.8}
\newcommand{\htwoCAPOTotalMapClears}{1.9}
\newcommand{\htwoCAPOReadMapZero}{1.6E-4}
\newcommand{\htwoCAPOReadMapOne}{0.433}
\newcommand{\htwoCAPOReadMapTen}{34.8}
\newcommand{\htwoCAPOReadMapHund}{6.91E-4}
\newcommand{\htwoCAPOReadMapThou}{0.00649}
\newcommand{\htwoCAPOReadMapGtThou}{64.8}
\newcommand{\htwoCAPOWriteMapZero}{0.00718}
\newcommand{\htwoCAPOWriteMapOne}{0.426}
\newcommand{\htwoCAPOWriteMapTen}{5.85E-4}
\newcommand{\htwoCAPOWriteMapHund}{34.8}
\newcommand{\htwoCAPOWriteMapThou}{0.0143}
\newcommand{\htwoCAPOWriteMapGtThou}{64.8}
\newcommand{\FASThtwoMaxLiveThreads}{9}
\newcommand{\FASThtwoTotalThreads}{10}
\newcommand{\FASThtwoBaseTime}{4.9}
\newcommand{\FASThtwoBaseTimeCI}{76}
\newcommand{\FASThtwoEmptyTime}{\rna}
\newcommand{\FASThtwoEmptyTimeCI}{\rna}
\newcommand{\FASThtwoEmptyTimeCIMIN}{\rna}
\newcommand{\FASThtwoEmptyTimeCIMAX}{\rna}
\newcommand{\FASThtwoFTTime}{9.3}
\newcommand{\FASThtwoFTTimeCI}{0.43}
\newcommand{\FASThtwoHBTime}{9.2}
\newcommand{\FASThtwoHBTimeCI}{0.19}
\newcommand{\FASThtwoFTOHBTime}{9.6}
\newcommand{\FASThtwoFTOHBTimeCI}{0.085}
\newcommand{\FASThtwoWCPTime}{54}
\newcommand{\FASThtwoWCPTimeCI}{4.3}
\newcommand{\FASThtwoFTOWCPTime}{59}
\newcommand{\FASThtwoFTOWCPTimeCI}{4.9}
\newcommand{\FASThtwoREWCPTime}{12}
\newcommand{\FASThtwoREWCPTimeCI}{0.51}
\newcommand{\FASThtwoDCTime}{53}
\newcommand{\FASThtwoDCTimeCI}{5.0}
\newcommand{\FASThtwoFTODCTime}{56}
\newcommand{\FASThtwoFTODCTimeCI}{4.4}
\newcommand{\FASThtwoREDCTime}{13}
\newcommand{\FASThtwoREDCTimeCI}{0.61}
\newcommand{\FASThtwoCAPOTime}{52}
\newcommand{\FASThtwoCAPOTimeCI}{4.3}
\newcommand{\FASThtwoFTOCAPOTime}{56}
\newcommand{\FASThtwoFTOCAPOTimeCI}{6.8}
\newcommand{\FASThtwoRECAPOTime}{11}
\newcommand{\FASThtwoRECAPOTimeCI}{0.17}
\newcommand{\FASThtwoAGGCAPOTime}{\rna}
\newcommand{\FASThtwoAGGCAPOTimeCI}{\rna}
\newcommand{\FASThtwoAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASThtwoAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASThtwoStaticTime}{\rzero}
\newcommand{\FASThtwoDynamicTime}{\rzero}
\newcommand{\FASThtwoBaseMem}{1,800}
\newcommand{\FASThtwoBaseMemCI}{28.0}
\newcommand{\FASThtwoFTMem}{3.0}
\newcommand{\FASThtwoFTMemCI}{0.063}
\newcommand{\FASThtwoHBMem}{3.2}
\newcommand{\FASThtwoHBMemCI}{0.069}
\newcommand{\FASThtwoFTOHBMem}{3.3}
\newcommand{\FASThtwoFTOHBMemCI}{0.13}
\newcommand{\FASThtwoWCPMem}{37}
\newcommand{\FASThtwoWCPMemCI}{1.4}
\newcommand{\FASThtwoFTOWCPMem}{40}
\newcommand{\FASThtwoFTOWCPMemCI}{1.6}
\newcommand{\FASThtwoREWCPMem}{7.8}
\newcommand{\FASThtwoREWCPMemCI}{0.15}
\newcommand{\FASThtwoDCMem}{36}
\newcommand{\FASThtwoDCMemCI}{0.7}
\newcommand{\FASThtwoFTODCMem}{38}
\newcommand{\FASThtwoFTODCMemCI}{2.1}
\newcommand{\FASThtwoREDCMem}{8.3}
\newcommand{\FASThtwoREDCMemCI}{0.31}
\newcommand{\FASThtwoCAPOMem}{36}
\newcommand{\FASThtwoCAPOMemCI}{1.9}
\newcommand{\FASThtwoFTOCAPOMem}{41}
\newcommand{\FASThtwoFTOCAPOMemCI}{1.8}
\newcommand{\FASThtwoRECAPOMem}{7.2}
\newcommand{\FASThtwoRECAPOMemCI}{0.31}
\newcommand{\FASThtwoAGGCAPOMem}{\memna}
\newcommand{\FASThtwoAGGCAPOMemCI}{\memna}
\newcommand{\FASThtwoAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASThtwoAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASThtwoEventsCI}{1,098,542}
\newcommand{\FASThtwoEventsCIMIN}{3,799,732,093}
\newcommand{\FASThtwoEventsCIMAX}{3,801,929,177}
\newcommand{\FASThtwoNoFPEventsCI}{7,285}
\newcommand{\FASThtwoNoFPEventsCIMIN}{118,475,954}
\newcommand{\FASThtwoNoFPEventsCIMAX}{118,490,524}
\newcommand{\FASThtwoFT}{11}
\newcommand{\FASThtwoFTCI}{0}
\newcommand{\FASThtwoFTCIMIN}{11}
\newcommand{\FASThtwoFTCIMAX}{11}
\newcommand{\FASThtwoFTDynamic}{92,275}
\newcommand{\FASThtwoFTDynamicCI}{855}
\newcommand{\FASThtwoFTDynamicCIMIN}{91,420}
\newcommand{\FASThtwoFTDynamicCIMAX}{93,130}
\newcommand{\FASThtwoHB}{13}
\newcommand{\FASThtwoHBCI}{0}
\newcommand{\FASThtwoHBCIMIN}{13}
\newcommand{\FASThtwoHBCIMAX}{13}
\newcommand{\FASThtwoHBDynamic}{58,756}
\newcommand{\FASThtwoHBDynamicCI}{1,153}
\newcommand{\FASThtwoHBDynamicCIMIN}{57,603}
\newcommand{\FASThtwoHBDynamicCIMAX}{59,909}
\newcommand{\FASThtwoFTOHB}{13}
\newcommand{\FASThtwoFTOHBCI}{0}
\newcommand{\FASThtwoFTOHBCIMIN}{13}
\newcommand{\FASThtwoFTOHBCIMAX}{13}
\newcommand{\FASThtwoFTOHBDynamic}{59,691}
\newcommand{\FASThtwoFTOHBDynamicCI}{979}
\newcommand{\FASThtwoFTOHBDynamicCIMIN}{58,712}
\newcommand{\FASThtwoFTOHBDynamicCIMAX}{60,670}
\newcommand{\FASThtwoWCP}{13}
\newcommand{\FASThtwoWCPCI}{0}
\newcommand{\FASThtwoWCPCIMIN}{13}
\newcommand{\FASThtwoWCPCIMAX}{13}
\newcommand{\FASThtwoWCPDynamic}{67,850}
\newcommand{\FASThtwoWCPDynamicCI}{233}
\newcommand{\FASThtwoWCPDynamicCIMIN}{67,617}
\newcommand{\FASThtwoWCPDynamicCIMAX}{68,083}
\newcommand{\FASThtwoFTOWCP}{13}
\newcommand{\FASThtwoFTOWCPCI}{0}
\newcommand{\FASThtwoFTOWCPCIMIN}{13}
\newcommand{\FASThtwoFTOWCPCIMAX}{13}
\newcommand{\FASThtwoFTOWCPDynamic}{67,930}
\newcommand{\FASThtwoFTOWCPDynamicCI}{167}
\newcommand{\FASThtwoFTOWCPDynamicCIMIN}{67,763}
\newcommand{\FASThtwoFTOWCPDynamicCIMAX}{68,097}
\newcommand{\FASThtwoREWCP}{13}
\newcommand{\FASThtwoREWCPCI}{0}
\newcommand{\FASThtwoREWCPCIMIN}{13}
\newcommand{\FASThtwoREWCPCIMAX}{13}
\newcommand{\FASThtwoREWCPDynamic}{64,688}
\newcommand{\FASThtwoREWCPDynamicCI}{909}
\newcommand{\FASThtwoREWCPDynamicCIMIN}{63,779}
\newcommand{\FASThtwoREWCPDynamicCIMAX}{65,597}
\newcommand{\FASThtwoDC}{13}
\newcommand{\FASThtwoDCCI}{0}
\newcommand{\FASThtwoDCCIMIN}{13}
\newcommand{\FASThtwoDCCIMAX}{13}
\newcommand{\FASThtwoDCDynamic}{68,193}
\newcommand{\FASThtwoDCDynamicCI}{165}
\newcommand{\FASThtwoDCDynamicCIMIN}{68,028}
\newcommand{\FASThtwoDCDynamicCIMAX}{68,358}
\newcommand{\FASThtwoFTODC}{13}
\newcommand{\FASThtwoFTODCCI}{0}
\newcommand{\FASThtwoFTODCCIMIN}{13}
\newcommand{\FASThtwoFTODCCIMAX}{13}
\newcommand{\FASThtwoFTODCDynamic}{68,318}
\newcommand{\FASThtwoFTODCDynamicCI}{163}
\newcommand{\FASThtwoFTODCDynamicCIMIN}{68,155}
\newcommand{\FASThtwoFTODCDynamicCIMAX}{68,481}
\newcommand{\FASThtwoREDC}{13}
\newcommand{\FASThtwoREDCCI}{0}
\newcommand{\FASThtwoREDCCIMIN}{13}
\newcommand{\FASThtwoREDCCIMAX}{13}
\newcommand{\FASThtwoREDCDynamic}{65,747}
\newcommand{\FASThtwoREDCDynamicCI}{1,094}
\newcommand{\FASThtwoREDCDynamicCIMIN}{64,653}
\newcommand{\FASThtwoREDCDynamicCIMAX}{66,841}
\newcommand{\FASThtwoCAPO}{13}
\newcommand{\FASThtwoCAPOCI}{0}
\newcommand{\FASThtwoCAPOCIMIN}{13}
\newcommand{\FASThtwoCAPOCIMAX}{13}
\newcommand{\FASThtwoCAPODynamic}{68,346}
\newcommand{\FASThtwoCAPODynamicCI}{239}
\newcommand{\FASThtwoCAPODynamicCIMIN}{68,107}
\newcommand{\FASThtwoCAPODynamicCIMAX}{68,585}
\newcommand{\FASThtwoFTOCAPO}{13}
\newcommand{\FASThtwoFTOCAPOCI}{0}
\newcommand{\FASThtwoFTOCAPOCIMIN}{13}
\newcommand{\FASThtwoFTOCAPOCIMAX}{13}
\newcommand{\FASThtwoFTOCAPODynamic}{68,560}
\newcommand{\FASThtwoFTOCAPODynamicCI}{203}
\newcommand{\FASThtwoFTOCAPODynamicCIMIN}{68,357}
\newcommand{\FASThtwoFTOCAPODynamicCIMAX}{68,763}
\newcommand{\FASThtwoRECAPO}{13}
\newcommand{\FASThtwoRECAPOCI}{0}
\newcommand{\FASThtwoRECAPOCIMIN}{13}
\newcommand{\FASThtwoRECAPOCIMAX}{13}
\newcommand{\FASThtwoRECAPODynamic}{63,127}
\newcommand{\FASThtwoRECAPODynamicCI}{1,038}
\newcommand{\FASThtwoRECAPODynamicCIMIN}{62,089}
\newcommand{\FASThtwoRECAPODynamicCIMAX}{64,165}
\newcommand{\FASThtwoAGGCAPO}{\rna}
\newcommand{\FASThtwoAGGCAPOCI}{\rna}
\newcommand{\FASThtwoAGGCAPOCIMIN}{\rna}
\newcommand{\FASThtwoAGGCAPOCIMAX}{\rna}
\newcommand{\FASThtwoAGGCAPODynamic}{\rna}
\newcommand{\FASThtwoAGGCAPODynamicCI}{\rna}
\newcommand{\FASThtwoAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASThtwoAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTjythonEvents}{730}
\newcommand{\FASTjythonNoFPEvents}{130}
\newcommand{\jythonHBEventTotal}{640}
\newcommand{\jythonHBNoFPEventTotal}{180}
\newcommand{\jythonHBNoFPAccessTotal}{160}
\newcommand{\jythonHBNoFPOtherTotal}{26}
\newcommand{\jythonHBReadTotal}{71.9}
\newcommand{\jythonHBWriteTotal}{14.0}
\newcommand{\jythonHBNoFPAccessInCS}{6.42}
\newcommand{\jythonHBNoFPAccessOutCS}{93.6}
\newcommand{\jythonHBAcqRelTotal}{19.0}
\newcommand{\jythonHBOtherTotal}{4.14}
\newcommand{\jythonHBNoFPReadTotal}{130}
\newcommand{\jythonHBReadInCS}{4.08}
\newcommand{\jythonHBReadOutCS}{106}
\newcommand{\jythonHBReadSameEp}{10.2}
\newcommand{\jythonHBReadSharedSameEp}{\cna}
\newcommand{\jythonHBReadExclusive}{97.7}
\newcommand{\jythonHBReadOwned}{\cna}
\newcommand{\jythonHBReadShare}{<0.001}
\newcommand{\jythonHBReadShared}{2.29}
\newcommand{\jythonHBReadSharedOwned}{\cna}
\newcommand{\jythonHBNoFPHonestWriteTotal}{26}
\newcommand{\jythonHBWriteInCS}{21.2}
\newcommand{\jythonHBWriteOutCS}{360}
\newcommand{\jythonHBNoFPWriteTotal}{26}
\newcommand{\jythonHBWriteSameEp}{281}
\newcommand{\jythonHBWriteExclusive}{100}
\newcommand{\jythonHBWriteOwned}{\cna}
\newcommand{\jythonHBWriteShared}{\cna}
\newcommand{\jythonHBNoFPOtherEventTotal}{25722405}
\newcommand{\jythonHBAcqRelOtherTotal}{82.1}
\newcommand{\jythonHBNoAcqRelOtherTotal}{4594751}
\newcommand{\jythonHBFork}{0.0}
\newcommand{\jythonHBJoin}{0.0}
\newcommand{\jythonHBPreWait}{0.0}
\newcommand{\jythonHBPostWait}{0.0}
\newcommand{\jythonHBVolatileTotal}{100.0}
\newcommand{\jythonHBClassInit}{0.00372}
\newcommand{\jythonHBClassAccess}{0.00303}
\newcommand{\jythonHBRaceTotal}{51}
\newcommand{\jythonHBWrRdRace}{84.3}
\newcommand{\jythonHBWrWrRace}{7.84}
\newcommand{\jythonHBRdWrRace}{7.84}
\newcommand{\jythonHBRdShWrRace}{0.0}
\newcommand{\jythonHBHoldLocksTotal}{11}
\newcommand{\jythonHBOneLockHeld}{6.86}
\newcommand{\jythonHBTwoNestedLocks}{0.28}
\newcommand{\jythonHBThreeNestedLocks}{<0.1}
\newcommand{\jythonHBFourNestedLocks}{\cna}
\newcommand{\jythonHBFiveNestedLocks}{\cna}
\newcommand{\jythonHBSixNestedLocks}{\cna}
\newcommand{\jythonHBSevenNestedLocks}{\cna}
\newcommand{\jythonHBEightNestedLocks}{\cna}
\newcommand{\jythonHBNineNestedLocks}{\cna}
\newcommand{\jythonHBTenNestedLocks}{\cna}
\newcommand{\jythonHBHundredNestedLocks}{\cna}
\newcommand{\jythonFTOHBEventTotal}{730}
\newcommand{\jythonFTOHBNoFPEventTotal}{170}
\newcommand{\jythonFTOHBNoFPAccessTotal}{140}
\newcommand{\jythonFTOHBNoFPOtherTotal}{27}
\newcommand{\jythonFTOHBReadTotal}{67.3}
\newcommand{\jythonFTOHBWriteTotal}{16.9}
\newcommand{\jythonFTOHBNoFPAccessInCS}{5.42}
\newcommand{\jythonFTOHBNoFPAccessOutCS}{94.6}
\newcommand{\jythonFTOHBAcqRelTotal}{17.2}
\newcommand{\jythonFTOHBOtherTotal}{3.6}
\newcommand{\jythonFTOHBNoFPReadTotal}{110}
\newcommand{\jythonFTOHBReadInCS}{4.84}
\newcommand{\jythonFTOHBReadOutCS}{108}
\newcommand{\jythonFTOHBReadSameEp}{12.5}
\newcommand{\jythonFTOHBReadSharedSameEp}{\cna}
\newcommand{\jythonFTOHBReadExclusive}{<0.001}
\newcommand{\jythonFTOHBReadOwned}{97.3}
\newcommand{\jythonFTOHBReadShare}{<0.001}
\newcommand{\jythonFTOHBReadShared}{\cna}
\newcommand{\jythonFTOHBReadSharedOwned}{2.66}
\newcommand{\jythonFTOHBNoFPHonestWriteTotal}{28}
\newcommand{\jythonFTOHBWriteInCS}{19.1}
\newcommand{\jythonFTOHBWriteOutCS}{388}
\newcommand{\jythonFTOHBNoFPWriteTotal}{28}
\newcommand{\jythonFTOHBWriteSameEp}{307}
\newcommand{\jythonFTOHBWriteExclusive}{<0.001}
\newcommand{\jythonFTOHBWriteOwned}{100}
\newcommand{\jythonFTOHBWriteShared}{\cna}
\newcommand{\jythonFTOHBNoFPOtherEventTotal}{26523556}
\newcommand{\jythonFTOHBAcqRelOtherTotal}{82.7}
\newcommand{\jythonFTOHBNoAcqRelOtherTotal}{4594890}
\newcommand{\jythonFTOHBFork}{0.0}
\newcommand{\jythonFTOHBJoin}{0.0}
\newcommand{\jythonFTOHBPreWait}{0.0}
\newcommand{\jythonFTOHBPostWait}{0.0}
\newcommand{\jythonFTOHBVolatileTotal}{100.0}
\newcommand{\jythonFTOHBClassInit}{0.00372}
\newcommand{\jythonFTOHBClassAccess}{0.00303}
\newcommand{\jythonFTOHBRaceTotal}{47}
\newcommand{\jythonFTOHBWrRdRace}{91.5}
\newcommand{\jythonFTOHBWrWrRace}{0.0}
\newcommand{\jythonFTOHBRdWrRace}{8.51}
\newcommand{\jythonFTOHBRdShWrRace}{0.0}
\newcommand{\jythonFTOHBHoldLocksTotal}{5.4}
\newcommand{\jythonFTOHBOneLockHeld}{3.81}
\newcommand{\jythonFTOHBTwoNestedLocks}{0.23}
\newcommand{\jythonFTOHBThreeNestedLocks}{<0.1}
\newcommand{\jythonFTOHBFourNestedLocks}{\cna}
\newcommand{\jythonFTOHBFiveNestedLocks}{\cna}
\newcommand{\jythonFTOHBSixNestedLocks}{\cna}
\newcommand{\jythonFTOHBSevenNestedLocks}{\cna}
\newcommand{\jythonFTOHBEightNestedLocks}{\cna}
\newcommand{\jythonFTOHBNineNestedLocks}{\cna}
\newcommand{\jythonFTOHBTenNestedLocks}{\cna}
\newcommand{\jythonFTOHBHundredNestedLocks}{\cna}
\newcommand{\jythonWCPEventTotal}{730}
\newcommand{\jythonWCPNoFPEventTotal}{190}
\newcommand{\jythonWCPNoFPAccessTotal}{170}
\newcommand{\jythonWCPNoFPOtherTotal}{27}
\newcommand{\jythonWCPReadTotal}{71.5}
\newcommand{\jythonWCPWriteTotal}{14.7}
\newcommand{\jythonWCPNoFPAccessInCS}{10.5}
\newcommand{\jythonWCPNoFPAccessOutCS}{89.5}
\newcommand{\jythonWCPAcqRelTotal}{16.4}
\newcommand{\jythonWCPOtherTotal}{3.44}
\newcommand{\jythonWCPNoFPReadTotal}{140}
\newcommand{\jythonWCPReadInCS}{4.18}
\newcommand{\jythonWCPReadOutCS}{106}
\newcommand{\jythonWCPReadSameEp}{10.3}
\newcommand{\jythonWCPReadSharedSameEp}{\cna}
\newcommand{\jythonWCPReadExclusive}{96.2}
\newcommand{\jythonWCPReadOwned}{\cna}
\newcommand{\jythonWCPReadShare}{<0.001}
\newcommand{\jythonWCPReadShared}{3.82}
\newcommand{\jythonWCPReadSharedOwned}{\cna}
\newcommand{\jythonWCPNoFPHonestWriteTotal}{28}
\newcommand{\jythonWCPWriteInCS}{19.1}
\newcommand{\jythonWCPWriteOutCS}{388}
\newcommand{\jythonWCPNoFPWriteTotal}{28}
\newcommand{\jythonWCPWriteSameEp}{307}
\newcommand{\jythonWCPWriteExclusive}{100}
\newcommand{\jythonWCPWriteOwned}{\cna}
\newcommand{\jythonWCPWriteShared}{\cna}
\newcommand{\jythonWCPNoFPOtherEventTotal}{26523557}
\newcommand{\jythonWCPAcqRelOtherTotal}{82.7}
\newcommand{\jythonWCPNoAcqRelOtherTotal}{4594891}
\newcommand{\jythonWCPFork}{0.0}
\newcommand{\jythonWCPJoin}{0.0}
\newcommand{\jythonWCPPreWait}{0.0}
\newcommand{\jythonWCPPostWait}{0.0}
\newcommand{\jythonWCPVolatileTotal}{100.0}
\newcommand{\jythonWCPClassInit}{0.00372}
\newcommand{\jythonWCPClassAccess}{0.00303}
\newcommand{\jythonWCPRaceTotal}{49}
\newcommand{\jythonWCPWrRdRace}{83.7}
\newcommand{\jythonWCPWrWrRace}{8.16}
\newcommand{\jythonWCPRdWrRace}{8.16}
\newcommand{\jythonWCPRdShWrRace}{0.0}
\newcommand{\jythonWCPHoldLocksTotal}{17}
\newcommand{\jythonWCPOneLockHeld}{10.1}
\newcommand{\jythonWCPTwoNestedLocks}{0.48}
\newcommand{\jythonWCPThreeNestedLocks}{<0.1}
\newcommand{\jythonWCPFourNestedLocks}{\cna}
\newcommand{\jythonWCPFiveNestedLocks}{\cna}
\newcommand{\jythonWCPSixNestedLocks}{\cna}
\newcommand{\jythonWCPSevenNestedLocks}{\cna}
\newcommand{\jythonWCPEightNestedLocks}{\cna}
\newcommand{\jythonWCPNineNestedLocks}{\cna}
\newcommand{\jythonWCPTenNestedLocks}{\cna}
\newcommand{\jythonWCPHundredNestedLocks}{\cna}
\newcommand{\jythonFTOWCPEventTotal}{730}
\newcommand{\jythonFTOWCPNoFPEventTotal}{170}
\newcommand{\jythonFTOWCPNoFPAccessTotal}{140}
\newcommand{\jythonFTOWCPNoFPOtherTotal}{27}
\newcommand{\jythonFTOWCPReadTotal}{67.3}
\newcommand{\jythonFTOWCPWriteTotal}{16.9}
\newcommand{\jythonFTOWCPNoFPAccessInCS}{5.42}
\newcommand{\jythonFTOWCPNoFPAccessOutCS}{94.6}
\newcommand{\jythonFTOWCPAcqRelTotal}{17.2}
\newcommand{\jythonFTOWCPOtherTotal}{3.6}
\newcommand{\jythonFTOWCPNoFPReadTotal}{110}
\newcommand{\jythonFTOWCPReadInCS}{4.84}
\newcommand{\jythonFTOWCPReadOutCS}{108}
\newcommand{\jythonFTOWCPReadSameEp}{12.5}
\newcommand{\jythonFTOWCPReadSharedSameEp}{\cna}
\newcommand{\jythonFTOWCPReadExclusive}{<0.001}
\newcommand{\jythonFTOWCPReadOwned}{95.4}
\newcommand{\jythonFTOWCPReadShare}{<0.001}
\newcommand{\jythonFTOWCPReadShared}{\cna}
\newcommand{\jythonFTOWCPReadSharedOwned}{4.61}
\newcommand{\jythonFTOWCPNoFPHonestWriteTotal}{28}
\newcommand{\jythonFTOWCPWriteInCS}{19.1}
\newcommand{\jythonFTOWCPWriteOutCS}{388}
\newcommand{\jythonFTOWCPNoFPWriteTotal}{28}
\newcommand{\jythonFTOWCPWriteSameEp}{307}
\newcommand{\jythonFTOWCPWriteExclusive}{<0.001}
\newcommand{\jythonFTOWCPWriteOwned}{100}
\newcommand{\jythonFTOWCPWriteShared}{\cna}
\newcommand{\jythonFTOWCPNoFPOtherEventTotal}{26523557}
\newcommand{\jythonFTOWCPAcqRelOtherTotal}{82.7}
\newcommand{\jythonFTOWCPNoAcqRelOtherTotal}{4594891}
\newcommand{\jythonFTOWCPFork}{0.0}
\newcommand{\jythonFTOWCPJoin}{0.0}
\newcommand{\jythonFTOWCPPreWait}{0.0}
\newcommand{\jythonFTOWCPPostWait}{0.0}
\newcommand{\jythonFTOWCPVolatileTotal}{100.0}
\newcommand{\jythonFTOWCPClassInit}{0.00372}
\newcommand{\jythonFTOWCPClassAccess}{0.00303}
\newcommand{\jythonFTOWCPRaceTotal}{34}
\newcommand{\jythonFTOWCPWrRdRace}{88.2}
\newcommand{\jythonFTOWCPWrWrRace}{0.0}
\newcommand{\jythonFTOWCPRdWrRace}{11.8}
\newcommand{\jythonFTOWCPRdShWrRace}{0.0}
\newcommand{\jythonFTOWCPHoldLocksTotal}{5.4}
\newcommand{\jythonFTOWCPOneLockHeld}{3.82}
\newcommand{\jythonFTOWCPTwoNestedLocks}{0.23}
\newcommand{\jythonFTOWCPThreeNestedLocks}{<0.1}
\newcommand{\jythonFTOWCPFourNestedLocks}{\cna}
\newcommand{\jythonFTOWCPFiveNestedLocks}{\cna}
\newcommand{\jythonFTOWCPSixNestedLocks}{\cna}
\newcommand{\jythonFTOWCPSevenNestedLocks}{\cna}
\newcommand{\jythonFTOWCPEightNestedLocks}{\cna}
\newcommand{\jythonFTOWCPNineNestedLocks}{\cna}
\newcommand{\jythonFTOWCPTenNestedLocks}{\cna}
\newcommand{\jythonFTOWCPHundredNestedLocks}{\cna}
\newcommand{\jythonREWCPEventTotal}{730}
\newcommand{\jythonREWCPNoFPEventTotal}{170}
\newcommand{\jythonREWCPNoFPAccessTotal}{140}
\newcommand{\jythonREWCPNoFPOtherTotal}{27}
\newcommand{\jythonREWCPReadTotal}{67.3}
\newcommand{\jythonREWCPWriteTotal}{16.9}
\newcommand{\jythonREWCPNoFPAccessInCS}{5.42}
\newcommand{\jythonREWCPNoFPAccessOutCS}{94.6}
\newcommand{\jythonREWCPAcqRelTotal}{17.2}
\newcommand{\jythonREWCPOtherTotal}{3.6}
\newcommand{\jythonREWCPNoFPReadTotal}{110}
\newcommand{\jythonREWCPReadInCS}{4.84}
\newcommand{\jythonREWCPReadOutCS}{108}
\newcommand{\jythonREWCPReadSameEp}{12.5}
\newcommand{\jythonREWCPReadSharedSameEp}{\cna}
\newcommand{\jythonREWCPReadExclusive}{<0.001}
\newcommand{\jythonREWCPReadOwned}{95.4}
\newcommand{\jythonREWCPReadShare}{<0.001}
\newcommand{\jythonREWCPReadShared}{\cna}
\newcommand{\jythonREWCPReadSharedOwned}{4.61}
\newcommand{\jythonREWCPNoFPHonestWriteTotal}{28}
\newcommand{\jythonREWCPWriteInCS}{19.1}
\newcommand{\jythonREWCPWriteOutCS}{388}
\newcommand{\jythonREWCPNoFPWriteTotal}{28}
\newcommand{\jythonREWCPWriteSameEp}{307}
\newcommand{\jythonREWCPWriteExclusive}{<0.001}
\newcommand{\jythonREWCPWriteOwned}{100}
\newcommand{\jythonREWCPWriteShared}{\cna}
\newcommand{\jythonREWCPNoFPOtherEventTotal}{26523556}
\newcommand{\jythonREWCPAcqRelOtherTotal}{82.7}
\newcommand{\jythonREWCPNoAcqRelOtherTotal}{4594890}
\newcommand{\jythonREWCPFork}{0.0}
\newcommand{\jythonREWCPJoin}{0.0}
\newcommand{\jythonREWCPPreWait}{0.0}
\newcommand{\jythonREWCPPostWait}{0.0}
\newcommand{\jythonREWCPVolatileTotal}{100.0}
\newcommand{\jythonREWCPClassInit}{0.00372}
\newcommand{\jythonREWCPClassAccess}{0.00303}
\newcommand{\jythonREWCPRaceTotal}{45}
\newcommand{\jythonREWCPWrRdRace}{91.1}
\newcommand{\jythonREWCPWrWrRace}{0.0}
\newcommand{\jythonREWCPRdWrRace}{8.89}
\newcommand{\jythonREWCPRdShWrRace}{0.0}
\newcommand{\jythonREWCPHoldLocksTotal}{5.4}
\newcommand{\jythonREWCPOneLockHeld}{3.82}
\newcommand{\jythonREWCPTwoNestedLocks}{0.23}
\newcommand{\jythonREWCPThreeNestedLocks}{<0.1}
\newcommand{\jythonREWCPFourNestedLocks}{\cna}
\newcommand{\jythonREWCPFiveNestedLocks}{\cna}
\newcommand{\jythonREWCPSixNestedLocks}{\cna}
\newcommand{\jythonREWCPSevenNestedLocks}{\cna}
\newcommand{\jythonREWCPEightNestedLocks}{\cna}
\newcommand{\jythonREWCPNineNestedLocks}{\cna}
\newcommand{\jythonREWCPTenNestedLocks}{\cna}
\newcommand{\jythonREWCPHundredNestedLocks}{\cna}
\newcommand{\jythonDCEventTotal}{730}
\newcommand{\jythonDCNoFPEventTotal}{190}
\newcommand{\jythonDCNoFPAccessTotal}{170}
\newcommand{\jythonDCNoFPOtherTotal}{27}
\newcommand{\jythonDCReadTotal}{71.5}
\newcommand{\jythonDCWriteTotal}{14.7}
\newcommand{\jythonDCNoFPAccessInCS}{10.5}
\newcommand{\jythonDCNoFPAccessOutCS}{89.5}
\newcommand{\jythonDCAcqRelTotal}{16.4}
\newcommand{\jythonDCOtherTotal}{3.44}
\newcommand{\jythonDCNoFPReadTotal}{140}
\newcommand{\jythonDCReadInCS}{4.18}
\newcommand{\jythonDCReadOutCS}{106}
\newcommand{\jythonDCReadSameEp}{10.3}
\newcommand{\jythonDCReadSharedSameEp}{\cna}
\newcommand{\jythonDCReadExclusive}{98.4}
\newcommand{\jythonDCReadOwned}{\cna}
\newcommand{\jythonDCReadShare}{<0.001}
\newcommand{\jythonDCReadShared}{1.62}
\newcommand{\jythonDCReadSharedOwned}{\cna}
\newcommand{\jythonDCNoFPHonestWriteTotal}{28}
\newcommand{\jythonDCWriteInCS}{19.1}
\newcommand{\jythonDCWriteOutCS}{388}
\newcommand{\jythonDCNoFPWriteTotal}{28}
\newcommand{\jythonDCWriteSameEp}{307}
\newcommand{\jythonDCWriteExclusive}{100}
\newcommand{\jythonDCWriteOwned}{\cna}
\newcommand{\jythonDCWriteShared}{\cna}
\newcommand{\jythonDCNoFPOtherEventTotal}{26523556}
\newcommand{\jythonDCAcqRelOtherTotal}{82.7}
\newcommand{\jythonDCNoAcqRelOtherTotal}{4594890}
\newcommand{\jythonDCFork}{0.0}
\newcommand{\jythonDCJoin}{0.0}
\newcommand{\jythonDCPreWait}{0.0}
\newcommand{\jythonDCPostWait}{0.0}
\newcommand{\jythonDCVolatileTotal}{100.0}
\newcommand{\jythonDCClassInit}{0.00372}
\newcommand{\jythonDCClassAccess}{0.00303}
\newcommand{\jythonDCRaceTotal}{70}
\newcommand{\jythonDCWrRdRace}{78.6}
\newcommand{\jythonDCWrWrRace}{11.4}
\newcommand{\jythonDCRdWrRace}{10.0}
\newcommand{\jythonDCRdShWrRace}{0.0}
\newcommand{\jythonDCHoldLocksTotal}{17}
\newcommand{\jythonDCOneLockHeld}{10.1}
\newcommand{\jythonDCTwoNestedLocks}{0.48}
\newcommand{\jythonDCThreeNestedLocks}{<0.1}
\newcommand{\jythonDCFourNestedLocks}{\cna}
\newcommand{\jythonDCFiveNestedLocks}{\cna}
\newcommand{\jythonDCSixNestedLocks}{\cna}
\newcommand{\jythonDCSevenNestedLocks}{\cna}
\newcommand{\jythonDCEightNestedLocks}{\cna}
\newcommand{\jythonDCNineNestedLocks}{\cna}
\newcommand{\jythonDCTenNestedLocks}{\cna}
\newcommand{\jythonDCHundredNestedLocks}{\cna}
\newcommand{\jythonFTODCEventTotal}{730}
\newcommand{\jythonFTODCNoFPEventTotal}{170}
\newcommand{\jythonFTODCNoFPAccessTotal}{140}
\newcommand{\jythonFTODCNoFPOtherTotal}{27}
\newcommand{\jythonFTODCReadTotal}{67.3}
\newcommand{\jythonFTODCWriteTotal}{16.9}
\newcommand{\jythonFTODCNoFPAccessInCS}{5.42}
\newcommand{\jythonFTODCNoFPAccessOutCS}{94.6}
\newcommand{\jythonFTODCAcqRelTotal}{17.2}
\newcommand{\jythonFTODCOtherTotal}{3.6}
\newcommand{\jythonFTODCNoFPReadTotal}{110}
\newcommand{\jythonFTODCReadInCS}{4.84}
\newcommand{\jythonFTODCReadOutCS}{108}
\newcommand{\jythonFTODCReadSameEp}{12.5}
\newcommand{\jythonFTODCReadSharedSameEp}{\cna}
\newcommand{\jythonFTODCReadExclusive}{\cna}
\newcommand{\jythonFTODCReadOwned}{98}
\newcommand{\jythonFTODCReadShare}{<0.001}
\newcommand{\jythonFTODCReadShared}{\cna}
\newcommand{\jythonFTODCReadSharedOwned}{1.99}
\newcommand{\jythonFTODCNoFPHonestWriteTotal}{28}
\newcommand{\jythonFTODCWriteInCS}{19.1}
\newcommand{\jythonFTODCWriteOutCS}{388}
\newcommand{\jythonFTODCNoFPWriteTotal}{28}
\newcommand{\jythonFTODCWriteSameEp}{307}
\newcommand{\jythonFTODCWriteExclusive}{\cna}
\newcommand{\jythonFTODCWriteOwned}{100}
\newcommand{\jythonFTODCWriteShared}{\cna}
\newcommand{\jythonFTODCNoFPOtherEventTotal}{26523557}
\newcommand{\jythonFTODCAcqRelOtherTotal}{82.7}
\newcommand{\jythonFTODCNoAcqRelOtherTotal}{4594891}
\newcommand{\jythonFTODCFork}{0.0}
\newcommand{\jythonFTODCJoin}{0.0}
\newcommand{\jythonFTODCPreWait}{0.0}
\newcommand{\jythonFTODCPostWait}{0.0}
\newcommand{\jythonFTODCVolatileTotal}{100.0}
\newcommand{\jythonFTODCClassInit}{0.00372}
\newcommand{\jythonFTODCClassAccess}{0.00303}
\newcommand{\jythonFTODCRaceTotal}{60}
\newcommand{\jythonFTODCWrRdRace}{86.7}
\newcommand{\jythonFTODCWrWrRace}{0.0}
\newcommand{\jythonFTODCRdWrRace}{13.3}
\newcommand{\jythonFTODCRdShWrRace}{0.0}
\newcommand{\jythonFTODCHoldLocksTotal}{5.4}
\newcommand{\jythonFTODCOneLockHeld}{3.82}
\newcommand{\jythonFTODCTwoNestedLocks}{0.23}
\newcommand{\jythonFTODCThreeNestedLocks}{<0.1}
\newcommand{\jythonFTODCFourNestedLocks}{\cna}
\newcommand{\jythonFTODCFiveNestedLocks}{\cna}
\newcommand{\jythonFTODCSixNestedLocks}{\cna}
\newcommand{\jythonFTODCSevenNestedLocks}{\cna}
\newcommand{\jythonFTODCEightNestedLocks}{\cna}
\newcommand{\jythonFTODCNineNestedLocks}{\cna}
\newcommand{\jythonFTODCTenNestedLocks}{\cna}
\newcommand{\jythonFTODCHundredNestedLocks}{\cna}
\newcommand{\jythonREDCEventTotal}{730}
\newcommand{\jythonREDCNoFPEventTotal}{170}
\newcommand{\jythonREDCNoFPAccessTotal}{140}
\newcommand{\jythonREDCNoFPOtherTotal}{27}
\newcommand{\jythonREDCReadTotal}{67.3}
\newcommand{\jythonREDCWriteTotal}{16.9}
\newcommand{\jythonREDCNoFPAccessInCS}{5.42}
\newcommand{\jythonREDCNoFPAccessOutCS}{94.6}
\newcommand{\jythonREDCAcqRelTotal}{17.2}
\newcommand{\jythonREDCOtherTotal}{3.6}
\newcommand{\jythonREDCNoFPReadTotal}{110}
\newcommand{\jythonREDCReadInCS}{4.84}
\newcommand{\jythonREDCReadOutCS}{108}
\newcommand{\jythonREDCReadSameEp}{12.5}
\newcommand{\jythonREDCReadSharedSameEp}{\cna}
\newcommand{\jythonREDCReadExclusive}{\cna}
\newcommand{\jythonREDCReadOwned}{98}
\newcommand{\jythonREDCReadShare}{<0.001}
\newcommand{\jythonREDCReadShared}{\cna}
\newcommand{\jythonREDCReadSharedOwned}{2.02}
\newcommand{\jythonREDCNoFPHonestWriteTotal}{28}
\newcommand{\jythonREDCWriteInCS}{19.1}
\newcommand{\jythonREDCWriteOutCS}{388}
\newcommand{\jythonREDCNoFPWriteTotal}{28}
\newcommand{\jythonREDCWriteSameEp}{307}
\newcommand{\jythonREDCWriteExclusive}{\cna}
\newcommand{\jythonREDCWriteOwned}{100}
\newcommand{\jythonREDCWriteShared}{\cna}
\newcommand{\jythonREDCNoFPOtherEventTotal}{26523556}
\newcommand{\jythonREDCAcqRelOtherTotal}{82.7}
\newcommand{\jythonREDCNoAcqRelOtherTotal}{4594890}
\newcommand{\jythonREDCFork}{0.0}
\newcommand{\jythonREDCJoin}{0.0}
\newcommand{\jythonREDCPreWait}{0.0}
\newcommand{\jythonREDCPostWait}{0.0}
\newcommand{\jythonREDCVolatileTotal}{100.0}
\newcommand{\jythonREDCClassInit}{0.00372}
\newcommand{\jythonREDCClassAccess}{0.00303}
\newcommand{\jythonREDCRaceTotal}{63}
\newcommand{\jythonREDCWrRdRace}{87.3}
\newcommand{\jythonREDCWrWrRace}{0.0}
\newcommand{\jythonREDCRdWrRace}{12.7}
\newcommand{\jythonREDCRdShWrRace}{0.0}
\newcommand{\jythonREDCHoldLocksTotal}{5.4}
\newcommand{\jythonREDCOneLockHeld}{3.82}
\newcommand{\jythonREDCTwoNestedLocks}{0.23}
\newcommand{\jythonREDCThreeNestedLocks}{<0.1}
\newcommand{\jythonREDCFourNestedLocks}{\cna}
\newcommand{\jythonREDCFiveNestedLocks}{\cna}
\newcommand{\jythonREDCSixNestedLocks}{\cna}
\newcommand{\jythonREDCSevenNestedLocks}{\cna}
\newcommand{\jythonREDCEightNestedLocks}{\cna}
\newcommand{\jythonREDCNineNestedLocks}{\cna}
\newcommand{\jythonREDCTenNestedLocks}{\cna}
\newcommand{\jythonREDCHundredNestedLocks}{\cna}
\newcommand{\jythonCAPOEventTotal}{730}
\newcommand{\jythonCAPONoFPEventTotal}{190}
\newcommand{\jythonCAPONoFPAccessTotal}{170}
\newcommand{\jythonCAPONoFPOtherTotal}{27}
\newcommand{\jythonCAPOReadTotal}{71.5}
\newcommand{\jythonCAPOWriteTotal}{14.7}
\newcommand{\jythonCAPONoFPAccessInCS}{10.5}
\newcommand{\jythonCAPONoFPAccessOutCS}{89.5}
\newcommand{\jythonCAPOAcqRelTotal}{16.4}
\newcommand{\jythonCAPOOtherTotal}{3.44}
\newcommand{\jythonCAPONoFPReadTotal}{140}
\newcommand{\jythonCAPOReadInCS}{4.18}
\newcommand{\jythonCAPOReadOutCS}{106}
\newcommand{\jythonCAPOReadSameEp}{10.3}
\newcommand{\jythonCAPOReadSharedSameEp}{\cna}
\newcommand{\jythonCAPOReadExclusive}{98.4}
\newcommand{\jythonCAPOReadOwned}{\cna}
\newcommand{\jythonCAPOReadShare}{<0.001}
\newcommand{\jythonCAPOReadShared}{1.64}
\newcommand{\jythonCAPOReadSharedOwned}{\cna}
\newcommand{\jythonCAPONoFPHonestWriteTotal}{28}
\newcommand{\jythonCAPOWriteInCS}{19.1}
\newcommand{\jythonCAPOWriteOutCS}{388}
\newcommand{\jythonCAPONoFPWriteTotal}{28}
\newcommand{\jythonCAPOWriteSameEp}{307}
\newcommand{\jythonCAPOWriteExclusive}{100}
\newcommand{\jythonCAPOWriteOwned}{\cna}
\newcommand{\jythonCAPOWriteShared}{\cna}
\newcommand{\jythonCAPONoFPOtherEventTotal}{26523557}
\newcommand{\jythonCAPOAcqRelOtherTotal}{82.7}
\newcommand{\jythonCAPONoAcqRelOtherTotal}{4594891}
\newcommand{\jythonCAPOFork}{0.0}
\newcommand{\jythonCAPOJoin}{0.0}
\newcommand{\jythonCAPOPreWait}{0.0}
\newcommand{\jythonCAPOPostWait}{0.0}
\newcommand{\jythonCAPOVolatileTotal}{100.0}
\newcommand{\jythonCAPOClassInit}{0.00372}
\newcommand{\jythonCAPOClassAccess}{0.00303}
\newcommand{\jythonCAPORaceTotal}{68}
\newcommand{\jythonCAPOWrRdRace}{77.9}
\newcommand{\jythonCAPOWrWrRace}{11.8}
\newcommand{\jythonCAPORdWrRace}{10.3}
\newcommand{\jythonCAPORdShWrRace}{0.0}
\newcommand{\jythonCAPOHoldLocksTotal}{17}
\newcommand{\jythonCAPOOneLockHeld}{10.1}
\newcommand{\jythonCAPOTwoNestedLocks}{0.48}
\newcommand{\jythonCAPOThreeNestedLocks}{<0.1}
\newcommand{\jythonCAPOFourNestedLocks}{\cna}
\newcommand{\jythonCAPOFiveNestedLocks}{\cna}
\newcommand{\jythonCAPOSixNestedLocks}{\cna}
\newcommand{\jythonCAPOSevenNestedLocks}{\cna}
\newcommand{\jythonCAPOEightNestedLocks}{\cna}
\newcommand{\jythonCAPONineNestedLocks}{\cna}
\newcommand{\jythonCAPOTenNestedLocks}{\cna}
\newcommand{\jythonCAPOHundredNestedLocks}{\cna}
\newcommand{\jythonFTOCAPOEventTotal}{730}
\newcommand{\jythonFTOCAPONoFPEventTotal}{170}
\newcommand{\jythonFTOCAPONoFPAccessTotal}{140}
\newcommand{\jythonFTOCAPONoFPOtherTotal}{27}
\newcommand{\jythonFTOCAPOReadTotal}{67.3}
\newcommand{\jythonFTOCAPOWriteTotal}{16.9}
\newcommand{\jythonFTOCAPONoFPAccessInCS}{5.42}
\newcommand{\jythonFTOCAPONoFPAccessOutCS}{94.6}
\newcommand{\jythonFTOCAPOAcqRelTotal}{17.2}
\newcommand{\jythonFTOCAPOOtherTotal}{3.6}
\newcommand{\jythonFTOCAPONoFPReadTotal}{110}
\newcommand{\jythonFTOCAPOReadInCS}{4.84}
\newcommand{\jythonFTOCAPOReadOutCS}{108}
\newcommand{\jythonFTOCAPOReadSameEp}{12.5}
\newcommand{\jythonFTOCAPOReadSharedSameEp}{\cna}
\newcommand{\jythonFTOCAPOReadExclusive}{\cna}
\newcommand{\jythonFTOCAPOReadOwned}{98.1}
\newcommand{\jythonFTOCAPOReadShare}{<0.001}
\newcommand{\jythonFTOCAPOReadShared}{\cna}
\newcommand{\jythonFTOCAPOReadSharedOwned}{1.95}
\newcommand{\jythonFTOCAPONoFPHonestWriteTotal}{28}
\newcommand{\jythonFTOCAPOWriteInCS}{19.1}
\newcommand{\jythonFTOCAPOWriteOutCS}{388}
\newcommand{\jythonFTOCAPONoFPWriteTotal}{28}
\newcommand{\jythonFTOCAPOWriteSameEp}{307}
\newcommand{\jythonFTOCAPOWriteExclusive}{\cna}
\newcommand{\jythonFTOCAPOWriteOwned}{100}
\newcommand{\jythonFTOCAPOWriteShared}{\cna}
\newcommand{\jythonFTOCAPONoFPOtherEventTotal}{26523556}
\newcommand{\jythonFTOCAPOAcqRelOtherTotal}{82.7}
\newcommand{\jythonFTOCAPONoAcqRelOtherTotal}{4594890}
\newcommand{\jythonFTOCAPOFork}{0.0}
\newcommand{\jythonFTOCAPOJoin}{0.0}
\newcommand{\jythonFTOCAPOPreWait}{0.0}
\newcommand{\jythonFTOCAPOPostWait}{0.0}
\newcommand{\jythonFTOCAPOVolatileTotal}{100.0}
\newcommand{\jythonFTOCAPOClassInit}{0.00372}
\newcommand{\jythonFTOCAPOClassAccess}{0.00303}
\newcommand{\jythonFTOCAPORaceTotal}{61}
\newcommand{\jythonFTOCAPOWrRdRace}{86.9}
\newcommand{\jythonFTOCAPOWrWrRace}{0.0}
\newcommand{\jythonFTOCAPORdWrRace}{13.1}
\newcommand{\jythonFTOCAPORdShWrRace}{0.0}
\newcommand{\jythonFTOCAPOHoldLocksTotal}{5.4}
\newcommand{\jythonFTOCAPOOneLockHeld}{3.82}
\newcommand{\jythonFTOCAPOTwoNestedLocks}{0.23}
\newcommand{\jythonFTOCAPOThreeNestedLocks}{<0.1}
\newcommand{\jythonFTOCAPOFourNestedLocks}{\cna}
\newcommand{\jythonFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\jythonFTOCAPOSixNestedLocks}{\cna}
\newcommand{\jythonFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\jythonFTOCAPOEightNestedLocks}{\cna}
\newcommand{\jythonFTOCAPONineNestedLocks}{\cna}
\newcommand{\jythonFTOCAPOTenNestedLocks}{\cna}
\newcommand{\jythonFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\jythonRECAPOEventTotal}{730}
\newcommand{\jythonRECAPONoFPEventTotal}{170}
\newcommand{\jythonRECAPONoFPAccessTotal}{140}
\newcommand{\jythonRECAPONoFPOtherTotal}{27}
\newcommand{\jythonRECAPOReadTotal}{67.3}
\newcommand{\jythonRECAPOWriteTotal}{16.9}
\newcommand{\jythonRECAPONoFPAccessInCS}{5.42}
\newcommand{\jythonRECAPONoFPAccessOutCS}{94.6}
\newcommand{\jythonRECAPOAcqRelTotal}{17.2}
\newcommand{\jythonRECAPOOtherTotal}{3.6}
\newcommand{\jythonRECAPONoFPReadTotal}{110}
\newcommand{\jythonRECAPOReadInCS}{4.84}
\newcommand{\jythonRECAPOReadOutCS}{108}
\newcommand{\jythonRECAPOReadSameEp}{12.5}
\newcommand{\jythonRECAPOReadSharedSameEp}{\cna}
\newcommand{\jythonRECAPOReadExclusive}{\cna}
\newcommand{\jythonRECAPOReadOwned}{98}
\newcommand{\jythonRECAPOReadShare}{<0.001}
\newcommand{\jythonRECAPOReadShared}{\cna}
\newcommand{\jythonRECAPOReadSharedOwned}{1.98}
\newcommand{\jythonRECAPONoFPHonestWriteTotal}{28}
\newcommand{\jythonRECAPOWriteInCS}{19.1}
\newcommand{\jythonRECAPOWriteOutCS}{388}
\newcommand{\jythonRECAPONoFPWriteTotal}{28}
\newcommand{\jythonRECAPOWriteSameEp}{307}
\newcommand{\jythonRECAPOWriteExclusive}{\cna}
\newcommand{\jythonRECAPOWriteOwned}{100}
\newcommand{\jythonRECAPOWriteShared}{\cna}
\newcommand{\jythonRECAPONoFPOtherEventTotal}{26523556}
\newcommand{\jythonRECAPOAcqRelOtherTotal}{82.7}
\newcommand{\jythonRECAPONoAcqRelOtherTotal}{4594890}
\newcommand{\jythonRECAPOFork}{0.0}
\newcommand{\jythonRECAPOJoin}{0.0}
\newcommand{\jythonRECAPOPreWait}{0.0}
\newcommand{\jythonRECAPOPostWait}{0.0}
\newcommand{\jythonRECAPOVolatileTotal}{100.0}
\newcommand{\jythonRECAPOClassInit}{0.00372}
\newcommand{\jythonRECAPOClassAccess}{0.00303}
\newcommand{\jythonRECAPORaceTotal}{63}
\newcommand{\jythonRECAPOWrRdRace}{87.3}
\newcommand{\jythonRECAPOWrWrRace}{0.0}
\newcommand{\jythonRECAPORdWrRace}{12.7}
\newcommand{\jythonRECAPORdShWrRace}{0.0}
\newcommand{\jythonRECAPOHoldLocksTotal}{5.4}
\newcommand{\jythonRECAPOOneLockHeld}{3.82}
\newcommand{\jythonRECAPOTwoNestedLocks}{0.23}
\newcommand{\jythonRECAPOThreeNestedLocks}{<0.1}
\newcommand{\jythonRECAPOFourNestedLocks}{\cna}
\newcommand{\jythonRECAPOFiveNestedLocks}{\cna}
\newcommand{\jythonRECAPOSixNestedLocks}{\cna}
\newcommand{\jythonRECAPOSevenNestedLocks}{\cna}
\newcommand{\jythonRECAPOEightNestedLocks}{\cna}
\newcommand{\jythonRECAPONineNestedLocks}{\cna}
\newcommand{\jythonRECAPOTenNestedLocks}{\cna}
\newcommand{\jythonRECAPOHundredNestedLocks}{\cna}
\newcommand{\jythonCAPOTotalSetClears}{11}
\newcommand{\jythonCAPOReadSetZero}{69.6}
\newcommand{\jythonCAPOReadSetOne}{30.4}
\newcommand{\jythonCAPOReadSetGtOne}{0.00461}
\newcommand{\jythonCAPOWriteSetZero}{98.0}
\newcommand{\jythonCAPOWriteSetOne}{0.00178}
\newcommand{\jythonCAPOWriteSetGtOne}{1.97}
\newcommand{\jythonCAPOTotalMapClears}{11}
\newcommand{\jythonCAPOReadMapZero}{25.2}
\newcommand{\jythonCAPOReadMapOne}{46.4}
\newcommand{\jythonCAPOReadMapTen}{0.00334}
\newcommand{\jythonCAPOReadMapHund}{0.00165}
\newcommand{\jythonCAPOReadMapThou}{0.00389}
\newcommand{\jythonCAPOReadMapGtThou}{28.4}
\newcommand{\jythonCAPOWriteMapZero}{25.2}
\newcommand{\jythonCAPOWriteMapOne}{0.00417}
\newcommand{\jythonCAPOWriteMapTen}{3.7}
\newcommand{\jythonCAPOWriteMapHund}{0.27}
\newcommand{\jythonCAPOWriteMapThou}{0.659}
\newcommand{\jythonCAPOWriteMapGtThou}{70.1}
\newcommand{\FASTjythonMaxLiveThreads}{2}
\newcommand{\FASTjythonTotalThreads}{2}
\newcommand{\FASTjythonBaseTime}{3.8}
\newcommand{\FASTjythonBaseTimeCI}{76}
\newcommand{\FASTjythonEmptyTime}{\rna}
\newcommand{\FASTjythonEmptyTimeCI}{\rna}
\newcommand{\FASTjythonEmptyTimeCIMIN}{\rna}
\newcommand{\FASTjythonEmptyTimeCIMAX}{\rna}
\newcommand{\FASTjythonFTTime}{8.5}
\newcommand{\FASTjythonFTTimeCI}{0.19}
\newcommand{\FASTjythonHBTime}{9.0}
\newcommand{\FASTjythonHBTimeCI}{0.23}
\newcommand{\FASTjythonFTOHBTime}{9.2}
\newcommand{\FASTjythonFTOHBTimeCI}{0.19}
\newcommand{\FASTjythonWCPTime}{12}
\newcommand{\FASTjythonWCPTimeCI}{0.4}
\newcommand{\FASTjythonFTOWCPTime}{11}
\newcommand{\FASTjythonFTOWCPTimeCI}{0.22}
\newcommand{\FASTjythonREWCPTime}{13}
\newcommand{\FASTjythonREWCPTimeCI}{0.32}
\newcommand{\FASTjythonDCTime}{12}
\newcommand{\FASTjythonDCTimeCI}{0.43}
\newcommand{\FASTjythonFTODCTime}{11}
\newcommand{\FASTjythonFTODCTimeCI}{0.2}
\newcommand{\FASTjythonREDCTime}{13}
\newcommand{\FASTjythonREDCTimeCI}{0.34}
\newcommand{\FASTjythonCAPOTime}{9.4}
\newcommand{\FASTjythonCAPOTimeCI}{0.18}
\newcommand{\FASTjythonFTOCAPOTime}{9.4}
\newcommand{\FASTjythonFTOCAPOTimeCI}{0.17}
\newcommand{\FASTjythonRECAPOTime}{10}
\newcommand{\FASTjythonRECAPOTimeCI}{0.28}
\newcommand{\FASTjythonAGGCAPOTime}{\rna}
\newcommand{\FASTjythonAGGCAPOTimeCI}{\rna}
\newcommand{\FASTjythonAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTjythonAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTjythonStaticTime}{\rzero}
\newcommand{\FASTjythonDynamicTime}{\rzero}
\newcommand{\FASTjythonBaseMem}{740}
\newcommand{\FASTjythonBaseMemCI}{5.2}
\newcommand{\FASTjythonFTMem}{6.2}
\newcommand{\FASTjythonFTMemCI}{0.38}
\newcommand{\FASTjythonHBMem}{6.2}
\newcommand{\FASTjythonHBMemCI}{0.091}
\newcommand{\FASTjythonFTOHBMem}{6.8}
\newcommand{\FASTjythonFTOHBMemCI}{0.15}
\newcommand{\FASTjythonWCPMem}{12}
\newcommand{\FASTjythonWCPMemCI}{0.38}
\newcommand{\FASTjythonFTOWCPMem}{13}
\newcommand{\FASTjythonFTOWCPMemCI}{0.34}
\newcommand{\FASTjythonREWCPMem}{16}
\newcommand{\FASTjythonREWCPMemCI}{0.28}
\newcommand{\FASTjythonDCMem}{13}
\newcommand{\FASTjythonDCMemCI}{0.32}
\newcommand{\FASTjythonFTODCMem}{13}
\newcommand{\FASTjythonFTODCMemCI}{0.45}
\newcommand{\FASTjythonREDCMem}{15}
\newcommand{\FASTjythonREDCMemCI}{0.42}
\newcommand{\FASTjythonCAPOMem}{7.7}
\newcommand{\FASTjythonCAPOMemCI}{0.14}
\newcommand{\FASTjythonFTOCAPOMem}{9.0}
\newcommand{\FASTjythonFTOCAPOMemCI}{0.13}
\newcommand{\FASTjythonRECAPOMem}{11}
\newcommand{\FASTjythonRECAPOMemCI}{0.38}
\newcommand{\FASTjythonAGGCAPOMem}{\memna}
\newcommand{\FASTjythonAGGCAPOMemCI}{\memna}
\newcommand{\FASTjythonAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTjythonAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTjythonEventsCI}{140}
\newcommand{\FASTjythonEventsCIMIN}{728,376,855}
\newcommand{\FASTjythonEventsCIMAX}{728,377,135}
\newcommand{\FASTjythonNoFPEventsCI}{10}
\newcommand{\FASTjythonNoFPEventsCIMIN}{127,785,801}
\newcommand{\FASTjythonNoFPEventsCIMAX}{127,785,821}
\newcommand{\FASTjythonFT}{22}
\newcommand{\FASTjythonFTCI}{1}
\newcommand{\FASTjythonFTCIMIN}{21}
\newcommand{\FASTjythonFTCIMAX}{23}
\newcommand{\FASTjythonFTDynamic}{47}
\newcommand{\FASTjythonFTDynamicCI}{1}
\newcommand{\FASTjythonFTDynamicCIMIN}{46}
\newcommand{\FASTjythonFTDynamicCIMAX}{48}
\newcommand{\FASTjythonHB}{42}
\newcommand{\FASTjythonHBCI}{1}
\newcommand{\FASTjythonHBCIMIN}{41}
\newcommand{\FASTjythonHBCIMAX}{43}
\newcommand{\FASTjythonHBDynamic}{47}
\newcommand{\FASTjythonHBDynamicCI}{1}
\newcommand{\FASTjythonHBDynamicCIMIN}{46}
\newcommand{\FASTjythonHBDynamicCIMAX}{48}
\newcommand{\FASTjythonFTOHB}{41}
\newcommand{\FASTjythonFTOHBCI}{1}
\newcommand{\FASTjythonFTOHBCIMIN}{40}
\newcommand{\FASTjythonFTOHBCIMAX}{42}
\newcommand{\FASTjythonFTOHBDynamic}{47}
\newcommand{\FASTjythonFTOHBDynamicCI}{1}
\newcommand{\FASTjythonFTOHBDynamicCIMIN}{46}
\newcommand{\FASTjythonFTOHBDynamicCIMAX}{48}
\newcommand{\FASTjythonWCP}{40}
\newcommand{\FASTjythonWCPCI}{1}
\newcommand{\FASTjythonWCPCIMIN}{39}
\newcommand{\FASTjythonWCPCIMAX}{41}
\newcommand{\FASTjythonWCPDynamic}{45}
\newcommand{\FASTjythonWCPDynamicCI}{1}
\newcommand{\FASTjythonWCPDynamicCIMIN}{44}
\newcommand{\FASTjythonWCPDynamicCIMAX}{46}
\newcommand{\FASTjythonFTOWCP}{34}
\newcommand{\FASTjythonFTOWCPCI}{0}
\newcommand{\FASTjythonFTOWCPCIMIN}{34}
\newcommand{\FASTjythonFTOWCPCIMAX}{34}
\newcommand{\FASTjythonFTOWCPDynamic}{34}
\newcommand{\FASTjythonFTOWCPDynamicCI}{0}
\newcommand{\FASTjythonFTOWCPDynamicCIMIN}{34}
\newcommand{\FASTjythonFTOWCPDynamicCIMAX}{34}
\newcommand{\FASTjythonREWCP}{41}
\newcommand{\FASTjythonREWCPCI}{1}
\newcommand{\FASTjythonREWCPCIMIN}{40}
\newcommand{\FASTjythonREWCPCIMAX}{42}
\newcommand{\FASTjythonREWCPDynamic}{45}
\newcommand{\FASTjythonREWCPDynamicCI}{2}
\newcommand{\FASTjythonREWCPDynamicCIMIN}{43}
\newcommand{\FASTjythonREWCPDynamicCIMAX}{47}
\newcommand{\FASTjythonDC}{52}
\newcommand{\FASTjythonDCCI}{1}
\newcommand{\FASTjythonDCCIMIN}{51}
\newcommand{\FASTjythonDCCIMAX}{53}
\newcommand{\FASTjythonDCDynamic}{63}
\newcommand{\FASTjythonDCDynamicCI}{1}
\newcommand{\FASTjythonDCDynamicCIMIN}{62}
\newcommand{\FASTjythonDCDynamicCIMAX}{64}
\newcommand{\FASTjythonFTODC}{50}
\newcommand{\FASTjythonFTODCCI}{0}
\newcommand{\FASTjythonFTODCCIMIN}{50}
\newcommand{\FASTjythonFTODCCIMAX}{50}
\newcommand{\FASTjythonFTODCDynamic}{60}
\newcommand{\FASTjythonFTODCDynamicCI}{0}
\newcommand{\FASTjythonFTODCDynamicCIMIN}{60}
\newcommand{\FASTjythonFTODCDynamicCIMAX}{60}
\newcommand{\FASTjythonREDC}{52}
\newcommand{\FASTjythonREDCCI}{1}
\newcommand{\FASTjythonREDCCIMIN}{51}
\newcommand{\FASTjythonREDCCIMAX}{53}
\newcommand{\FASTjythonREDCDynamic}{63}
\newcommand{\FASTjythonREDCDynamicCI}{1}
\newcommand{\FASTjythonREDCDynamicCIMIN}{62}
\newcommand{\FASTjythonREDCDynamicCIMAX}{64}
\newcommand{\FASTjythonCAPO}{50}
\newcommand{\FASTjythonCAPOCI}{0}
\newcommand{\FASTjythonCAPOCIMIN}{50}
\newcommand{\FASTjythonCAPOCIMAX}{50}
\newcommand{\FASTjythonCAPODynamic}{61}
\newcommand{\FASTjythonCAPODynamicCI}{0}
\newcommand{\FASTjythonCAPODynamicCIMIN}{61}
\newcommand{\FASTjythonCAPODynamicCIMAX}{61}
\newcommand{\FASTjythonFTOCAPO}{51}
\newcommand{\FASTjythonFTOCAPOCI}{1}
\newcommand{\FASTjythonFTOCAPOCIMIN}{50}
\newcommand{\FASTjythonFTOCAPOCIMAX}{52}
\newcommand{\FASTjythonFTOCAPODynamic}{61}
\newcommand{\FASTjythonFTOCAPODynamicCI}{1}
\newcommand{\FASTjythonFTOCAPODynamicCIMIN}{60}
\newcommand{\FASTjythonFTOCAPODynamicCIMAX}{62}
\newcommand{\FASTjythonRECAPO}{52}
\newcommand{\FASTjythonRECAPOCI}{1}
\newcommand{\FASTjythonRECAPOCIMIN}{51}
\newcommand{\FASTjythonRECAPOCIMAX}{53}
\newcommand{\FASTjythonRECAPODynamic}{63}
\newcommand{\FASTjythonRECAPODynamicCI}{1}
\newcommand{\FASTjythonRECAPODynamicCIMIN}{62}
\newcommand{\FASTjythonRECAPODynamicCIMAX}{64}
\newcommand{\FASTjythonAGGCAPO}{\rna}
\newcommand{\FASTjythonAGGCAPOCI}{\rna}
\newcommand{\FASTjythonAGGCAPOCIMIN}{\rna}
\newcommand{\FASTjythonAGGCAPOCIMAX}{\rna}
\newcommand{\FASTjythonAGGCAPODynamic}{\rna}
\newcommand{\FASTjythonAGGCAPODynamicCI}{\rna}
\newcommand{\FASTjythonAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTjythonAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTluindexEvents}{400}
\newcommand{\FASTluindexNoFPEvents}{2.9}
\newcommand{\luindexHBEventTotal}{400}
\newcommand{\luindexHBNoFPEventTotal}{43}
\newcommand{\luindexHBNoFPAccessTotal}{42}
\newcommand{\luindexHBNoFPOtherTotal}{0.42}
\newcommand{\luindexHBReadTotal}{67.6}
\newcommand{\luindexHBWriteTotal}{31.4}
\newcommand{\luindexHBNoFPAccessInCS}{8.08}
\newcommand{\luindexHBNoFPAccessOutCS}{91.9}
\newcommand{\luindexHBAcqRelTotal}{14.2}
\newcommand{\luindexHBOtherTotal}{0.0202}
\newcommand{\luindexHBNoFPReadTotal}{29}
\newcommand{\luindexHBReadInCS}{23.8}
\newcommand{\luindexHBReadOutCS}{81.3}
\newcommand{\luindexHBReadSameEp}{5.1}
\newcommand{\luindexHBReadSharedSameEp}{\cna}
\newcommand{\luindexHBReadExclusive}{100}
\newcommand{\luindexHBReadOwned}{\cna}
\newcommand{\luindexHBReadShare}{<0.001}
\newcommand{\luindexHBReadShared}{<0.001}
\newcommand{\luindexHBReadSharedOwned}{\cna}
\newcommand{\luindexHBNoFPHonestWriteTotal}{13}
\newcommand{\luindexHBWriteInCS}{32.1}
\newcommand{\luindexHBWriteOutCS}{75.5}
\newcommand{\luindexHBNoFPWriteTotal}{13}
\newcommand{\luindexHBWriteSameEp}{7.57}
\newcommand{\luindexHBWriteExclusive}{100}
\newcommand{\luindexHBWriteOwned}{\cna}
\newcommand{\luindexHBWriteShared}{<0.001}
\newcommand{\luindexHBNoFPOtherEventTotal}{415336}
\newcommand{\luindexHBAcqRelOtherTotal}{99.9}
\newcommand{\luindexHBNoAcqRelOtherTotal}{590}
\newcommand{\luindexHBFork}{0.169}
\newcommand{\luindexHBJoin}{0.0}
\newcommand{\luindexHBPreWait}{0.339}
\newcommand{\luindexHBPostWait}{0.339}
\newcommand{\luindexHBVolatileTotal}{77.8}
\newcommand{\luindexHBClassInit}{11.2}
\newcommand{\luindexHBClassAccess}{10.2}
\newcommand{\luindexHBRaceTotal}{1}
\newcommand{\luindexHBWrRdRace}{0.0}
\newcommand{\luindexHBWrWrRace}{0.0}
\newcommand{\luindexHBRdWrRace}{0.0}
\newcommand{\luindexHBRdShWrRace}{100.0}
\newcommand{\luindexHBHoldLocksTotal}{11}
\newcommand{\luindexHBOneLockHeld}{26.3}
\newcommand{\luindexHBTwoNestedLocks}{26.0}
\newcommand{\luindexHBThreeNestedLocks}{25.9}
\newcommand{\luindexHBFourNestedLocks}{0.69}
\newcommand{\luindexHBFiveNestedLocks}{<0.1}
\newcommand{\luindexHBSixNestedLocks}{<0.1}
\newcommand{\luindexHBSevenNestedLocks}{\cna}
\newcommand{\luindexHBEightNestedLocks}{\cna}
\newcommand{\luindexHBNineNestedLocks}{\cna}
\newcommand{\luindexHBTenNestedLocks}{\cna}
\newcommand{\luindexHBHundredNestedLocks}{\cna}
\newcommand{\luindexFTOHBEventTotal}{400}
\newcommand{\luindexFTOHBNoFPEventTotal}{41}
\newcommand{\luindexFTOHBNoFPAccessTotal}{40}
\newcommand{\luindexFTOHBNoFPOtherTotal}{0.42}
\newcommand{\luindexFTOHBReadTotal}{66.0}
\newcommand{\luindexFTOHBWriteTotal}{33.0}
\newcommand{\luindexFTOHBNoFPAccessInCS}{8.08}
\newcommand{\luindexFTOHBNoFPAccessOutCS}{91.9}
\newcommand{\luindexFTOHBAcqRelTotal}{14.2}
\newcommand{\luindexFTOHBOtherTotal}{0.0197}
\newcommand{\luindexFTOHBNoFPReadTotal}{27}
\newcommand{\luindexFTOHBReadInCS}{23.4}
\newcommand{\luindexFTOHBReadOutCS}{82}
\newcommand{\luindexFTOHBReadSameEp}{5.48}
\newcommand{\luindexFTOHBReadSharedSameEp}{\cna}
\newcommand{\luindexFTOHBReadExclusive}{<0.001}
\newcommand{\luindexFTOHBReadOwned}{100}
\newcommand{\luindexFTOHBReadShare}{<0.001}
\newcommand{\luindexFTOHBReadShared}{\cna}
\newcommand{\luindexFTOHBReadSharedOwned}{<0.001}
\newcommand{\luindexFTOHBNoFPHonestWriteTotal}{13}
\newcommand{\luindexFTOHBWriteInCS}{32.1}
\newcommand{\luindexFTOHBWriteOutCS}{75.5}
\newcommand{\luindexFTOHBNoFPWriteTotal}{13}
\newcommand{\luindexFTOHBWriteSameEp}{7.57}
\newcommand{\luindexFTOHBWriteExclusive}{<0.001}
\newcommand{\luindexFTOHBWriteOwned}{100}
\newcommand{\luindexFTOHBWriteShared}{\cna}
\newcommand{\luindexFTOHBNoFPOtherEventTotal}{415314}
\newcommand{\luindexFTOHBAcqRelOtherTotal}{99.9}
\newcommand{\luindexFTOHBNoAcqRelOtherTotal}{574}
\newcommand{\luindexFTOHBFork}{0.174}
\newcommand{\luindexFTOHBJoin}{0.0}
\newcommand{\luindexFTOHBPreWait}{0.348}
\newcommand{\luindexFTOHBPostWait}{0.348}
\newcommand{\luindexFTOHBVolatileTotal}{77.2}
\newcommand{\luindexFTOHBClassInit}{11.5}
\newcommand{\luindexFTOHBClassAccess}{10.5}
\newcommand{\luindexFTOHBRaceTotal}{1}
\newcommand{\luindexFTOHBWrRdRace}{0.0}
\newcommand{\luindexFTOHBWrWrRace}{0.0}
\newcommand{\luindexFTOHBRdWrRace}{0.0}
\newcommand{\luindexFTOHBRdShWrRace}{100.0}
\newcommand{\luindexFTOHBHoldLocksTotal}{10}
\newcommand{\luindexFTOHBOneLockHeld}{25.8}
\newcommand{\luindexFTOHBTwoNestedLocks}{25.4}
\newcommand{\luindexFTOHBThreeNestedLocks}{25.3}
\newcommand{\luindexFTOHBFourNestedLocks}{0.61}
\newcommand{\luindexFTOHBFiveNestedLocks}{<0.1}
\newcommand{\luindexFTOHBSixNestedLocks}{<0.1}
\newcommand{\luindexFTOHBSevenNestedLocks}{\cna}
\newcommand{\luindexFTOHBEightNestedLocks}{\cna}
\newcommand{\luindexFTOHBNineNestedLocks}{\cna}
\newcommand{\luindexFTOHBTenNestedLocks}{\cna}
\newcommand{\luindexFTOHBHundredNestedLocks}{\cna}
\newcommand{\luindexWCPEventTotal}{400}
\newcommand{\luindexWCPNoFPEventTotal}{43}
\newcommand{\luindexWCPNoFPAccessTotal}{42}
\newcommand{\luindexWCPNoFPOtherTotal}{0.42}
\newcommand{\luindexWCPReadTotal}{67.6}
\newcommand{\luindexWCPWriteTotal}{31.4}
\newcommand{\luindexWCPNoFPAccessInCS}{83.0}
\newcommand{\luindexWCPNoFPAccessOutCS}{17.0}
\newcommand{\luindexWCPAcqRelTotal}{2.98}
\newcommand{\luindexWCPOtherTotal}{0.00418}
\newcommand{\luindexWCPNoFPReadTotal}{29}
\newcommand{\luindexWCPReadInCS}{23.8}
\newcommand{\luindexWCPReadOutCS}{81.3}
\newcommand{\luindexWCPReadSameEp}{5.1}
\newcommand{\luindexWCPReadSharedSameEp}{\cna}
\newcommand{\luindexWCPReadExclusive}{100}
\newcommand{\luindexWCPReadOwned}{\cna}
\newcommand{\luindexWCPReadShare}{<0.001}
\newcommand{\luindexWCPReadShared}{<0.001}
\newcommand{\luindexWCPReadSharedOwned}{\cna}
\newcommand{\luindexWCPNoFPHonestWriteTotal}{13}
\newcommand{\luindexWCPWriteInCS}{32.1}
\newcommand{\luindexWCPWriteOutCS}{75.5}
\newcommand{\luindexWCPNoFPWriteTotal}{13}
\newcommand{\luindexWCPWriteSameEp}{7.57}
\newcommand{\luindexWCPWriteExclusive}{100}
\newcommand{\luindexWCPWriteOwned}{\cna}
\newcommand{\luindexWCPWriteShared}{<0.001}
\newcommand{\luindexWCPNoFPOtherEventTotal}{415322}
\newcommand{\luindexWCPAcqRelOtherTotal}{99.9}
\newcommand{\luindexWCPNoAcqRelOtherTotal}{582}
\newcommand{\luindexWCPFork}{0.172}
\newcommand{\luindexWCPJoin}{0.0}
\newcommand{\luindexWCPPreWait}{0.344}
\newcommand{\luindexWCPPostWait}{0.344}
\newcommand{\luindexWCPVolatileTotal}{77.5}
\newcommand{\luindexWCPClassInit}{11.3}
\newcommand{\luindexWCPClassAccess}{10.3}
\newcommand{\luindexWCPRaceTotal}{1}
\newcommand{\luindexWCPWrRdRace}{0.0}
\newcommand{\luindexWCPWrWrRace}{0.0}
\newcommand{\luindexWCPRdWrRace}{0.0}
\newcommand{\luindexWCPRdShWrRace}{100.0}
\newcommand{\luindexWCPHoldLocksTotal}{22}
\newcommand{\luindexWCPOneLockHeld}{52.3}
\newcommand{\luindexWCPTwoNestedLocks}{51.5}
\newcommand{\luindexWCPThreeNestedLocks}{51.4}
\newcommand{\luindexWCPFourNestedLocks}{1.28}
\newcommand{\luindexWCPFiveNestedLocks}{<0.1}
\newcommand{\luindexWCPSixNestedLocks}{<0.1}
\newcommand{\luindexWCPSevenNestedLocks}{\cna}
\newcommand{\luindexWCPEightNestedLocks}{\cna}
\newcommand{\luindexWCPNineNestedLocks}{\cna}
\newcommand{\luindexWCPTenNestedLocks}{\cna}
\newcommand{\luindexWCPHundredNestedLocks}{\cna}
\newcommand{\luindexFTOWCPEventTotal}{400}
\newcommand{\luindexFTOWCPNoFPEventTotal}{41}
\newcommand{\luindexFTOWCPNoFPAccessTotal}{40}
\newcommand{\luindexFTOWCPNoFPOtherTotal}{0.42}
\newcommand{\luindexFTOWCPReadTotal}{66.0}
\newcommand{\luindexFTOWCPWriteTotal}{33.0}
\newcommand{\luindexFTOWCPNoFPAccessInCS}{8.08}
\newcommand{\luindexFTOWCPNoFPAccessOutCS}{91.9}
\newcommand{\luindexFTOWCPAcqRelTotal}{14.2}
\newcommand{\luindexFTOWCPOtherTotal}{0.02}
\newcommand{\luindexFTOWCPNoFPReadTotal}{27}
\newcommand{\luindexFTOWCPReadInCS}{23.5}
\newcommand{\luindexFTOWCPReadOutCS}{82}
\newcommand{\luindexFTOWCPReadSameEp}{5.48}
\newcommand{\luindexFTOWCPReadSharedSameEp}{\cna}
\newcommand{\luindexFTOWCPReadExclusive}{<0.001}
\newcommand{\luindexFTOWCPReadOwned}{100}
\newcommand{\luindexFTOWCPReadShare}{<0.001}
\newcommand{\luindexFTOWCPReadShared}{\cna}
\newcommand{\luindexFTOWCPReadSharedOwned}{<0.001}
\newcommand{\luindexFTOWCPNoFPHonestWriteTotal}{13}
\newcommand{\luindexFTOWCPWriteInCS}{32.1}
\newcommand{\luindexFTOWCPWriteOutCS}{75.5}
\newcommand{\luindexFTOWCPNoFPWriteTotal}{13}
\newcommand{\luindexFTOWCPWriteSameEp}{7.57}
\newcommand{\luindexFTOWCPWriteExclusive}{<0.001}
\newcommand{\luindexFTOWCPWriteOwned}{100}
\newcommand{\luindexFTOWCPWriteShared}{\cna}
\newcommand{\luindexFTOWCPNoFPOtherEventTotal}{415322}
\newcommand{\luindexFTOWCPAcqRelOtherTotal}{99.9}
\newcommand{\luindexFTOWCPNoAcqRelOtherTotal}{582}
\newcommand{\luindexFTOWCPFork}{0.172}
\newcommand{\luindexFTOWCPJoin}{0.0}
\newcommand{\luindexFTOWCPPreWait}{0.344}
\newcommand{\luindexFTOWCPPostWait}{0.344}
\newcommand{\luindexFTOWCPVolatileTotal}{77.5}
\newcommand{\luindexFTOWCPClassInit}{11.3}
\newcommand{\luindexFTOWCPClassAccess}{10.3}
\newcommand{\luindexFTOWCPRaceTotal}{1}
\newcommand{\luindexFTOWCPWrRdRace}{0.0}
\newcommand{\luindexFTOWCPWrWrRace}{0.0}
\newcommand{\luindexFTOWCPRdWrRace}{0.0}
\newcommand{\luindexFTOWCPRdShWrRace}{100.0}
\newcommand{\luindexFTOWCPHoldLocksTotal}{10}
\newcommand{\luindexFTOWCPOneLockHeld}{25.8}
\newcommand{\luindexFTOWCPTwoNestedLocks}{25.4}
\newcommand{\luindexFTOWCPThreeNestedLocks}{25.3}
\newcommand{\luindexFTOWCPFourNestedLocks}{0.61}
\newcommand{\luindexFTOWCPFiveNestedLocks}{<0.1}
\newcommand{\luindexFTOWCPSixNestedLocks}{<0.1}
\newcommand{\luindexFTOWCPSevenNestedLocks}{\cna}
\newcommand{\luindexFTOWCPEightNestedLocks}{\cna}
\newcommand{\luindexFTOWCPNineNestedLocks}{\cna}
\newcommand{\luindexFTOWCPTenNestedLocks}{\cna}
\newcommand{\luindexFTOWCPHundredNestedLocks}{\cna}
\newcommand{\luindexREWCPEventTotal}{400}
\newcommand{\luindexREWCPNoFPEventTotal}{41}
\newcommand{\luindexREWCPNoFPAccessTotal}{40}
\newcommand{\luindexREWCPNoFPOtherTotal}{0.42}
\newcommand{\luindexREWCPReadTotal}{66.0}
\newcommand{\luindexREWCPWriteTotal}{33.0}
\newcommand{\luindexREWCPNoFPAccessInCS}{8.08}
\newcommand{\luindexREWCPNoFPAccessOutCS}{91.9}
\newcommand{\luindexREWCPAcqRelTotal}{14.2}
\newcommand{\luindexREWCPOtherTotal}{0.0197}
\newcommand{\luindexREWCPNoFPReadTotal}{27}
\newcommand{\luindexREWCPReadInCS}{23.5}
\newcommand{\luindexREWCPReadOutCS}{82}
\newcommand{\luindexREWCPReadSameEp}{5.48}
\newcommand{\luindexREWCPReadSharedSameEp}{\cna}
\newcommand{\luindexREWCPReadExclusive}{<0.001}
\newcommand{\luindexREWCPReadOwned}{100}
\newcommand{\luindexREWCPReadShare}{<0.001}
\newcommand{\luindexREWCPReadShared}{\cna}
\newcommand{\luindexREWCPReadSharedOwned}{<0.001}
\newcommand{\luindexREWCPNoFPHonestWriteTotal}{13}
\newcommand{\luindexREWCPWriteInCS}{32.1}
\newcommand{\luindexREWCPWriteOutCS}{75.5}
\newcommand{\luindexREWCPNoFPWriteTotal}{13}
\newcommand{\luindexREWCPWriteSameEp}{7.57}
\newcommand{\luindexREWCPWriteExclusive}{<0.001}
\newcommand{\luindexREWCPWriteOwned}{100}
\newcommand{\luindexREWCPWriteShared}{\cna}
\newcommand{\luindexREWCPNoFPOtherEventTotal}{415315}
\newcommand{\luindexREWCPAcqRelOtherTotal}{99.9}
\newcommand{\luindexREWCPNoAcqRelOtherTotal}{575}
\newcommand{\luindexREWCPFork}{0.174}
\newcommand{\luindexREWCPJoin}{0.0}
\newcommand{\luindexREWCPPreWait}{0.348}
\newcommand{\luindexREWCPPostWait}{0.348}
\newcommand{\luindexREWCPVolatileTotal}{77.2}
\newcommand{\luindexREWCPClassInit}{11.5}
\newcommand{\luindexREWCPClassAccess}{10.4}
\newcommand{\luindexREWCPRaceTotal}{1}
\newcommand{\luindexREWCPWrRdRace}{0.0}
\newcommand{\luindexREWCPWrWrRace}{0.0}
\newcommand{\luindexREWCPRdWrRace}{0.0}
\newcommand{\luindexREWCPRdShWrRace}{100.0}
\newcommand{\luindexREWCPHoldLocksTotal}{10}
\newcommand{\luindexREWCPOneLockHeld}{25.8}
\newcommand{\luindexREWCPTwoNestedLocks}{25.4}
\newcommand{\luindexREWCPThreeNestedLocks}{25.3}
\newcommand{\luindexREWCPFourNestedLocks}{0.61}
\newcommand{\luindexREWCPFiveNestedLocks}{<0.1}
\newcommand{\luindexREWCPSixNestedLocks}{<0.1}
\newcommand{\luindexREWCPSevenNestedLocks}{\cna}
\newcommand{\luindexREWCPEightNestedLocks}{\cna}
\newcommand{\luindexREWCPNineNestedLocks}{\cna}
\newcommand{\luindexREWCPTenNestedLocks}{\cna}
\newcommand{\luindexREWCPHundredNestedLocks}{\cna}
\newcommand{\luindexDCEventTotal}{400}
\newcommand{\luindexDCNoFPEventTotal}{43}
\newcommand{\luindexDCNoFPAccessTotal}{42}
\newcommand{\luindexDCNoFPOtherTotal}{0.42}
\newcommand{\luindexDCReadTotal}{67.6}
\newcommand{\luindexDCWriteTotal}{31.4}
\newcommand{\luindexDCNoFPAccessInCS}{83.0}
\newcommand{\luindexDCNoFPAccessOutCS}{17.0}
\newcommand{\luindexDCAcqRelTotal}{2.98}
\newcommand{\luindexDCOtherTotal}{0.00418}
\newcommand{\luindexDCNoFPReadTotal}{29}
\newcommand{\luindexDCReadInCS}{23.8}
\newcommand{\luindexDCReadOutCS}{81.3}
\newcommand{\luindexDCReadSameEp}{5.1}
\newcommand{\luindexDCReadSharedSameEp}{\cna}
\newcommand{\luindexDCReadExclusive}{100}
\newcommand{\luindexDCReadOwned}{\cna}
\newcommand{\luindexDCReadShare}{<0.001}
\newcommand{\luindexDCReadShared}{<0.001}
\newcommand{\luindexDCReadSharedOwned}{\cna}
\newcommand{\luindexDCNoFPHonestWriteTotal}{13}
\newcommand{\luindexDCWriteInCS}{32.1}
\newcommand{\luindexDCWriteOutCS}{75.5}
\newcommand{\luindexDCNoFPWriteTotal}{13}
\newcommand{\luindexDCWriteSameEp}{7.57}
\newcommand{\luindexDCWriteExclusive}{100}
\newcommand{\luindexDCWriteOwned}{\cna}
\newcommand{\luindexDCWriteShared}{<0.001}
\newcommand{\luindexDCNoFPOtherEventTotal}{415322}
\newcommand{\luindexDCAcqRelOtherTotal}{99.9}
\newcommand{\luindexDCNoAcqRelOtherTotal}{582}
\newcommand{\luindexDCFork}{0.172}
\newcommand{\luindexDCJoin}{0.0}
\newcommand{\luindexDCPreWait}{0.344}
\newcommand{\luindexDCPostWait}{0.344}
\newcommand{\luindexDCVolatileTotal}{77.5}
\newcommand{\luindexDCClassInit}{11.3}
\newcommand{\luindexDCClassAccess}{10.3}
\newcommand{\luindexDCRaceTotal}{1}
\newcommand{\luindexDCWrRdRace}{0.0}
\newcommand{\luindexDCWrWrRace}{0.0}
\newcommand{\luindexDCRdWrRace}{0.0}
\newcommand{\luindexDCRdShWrRace}{100.0}
\newcommand{\luindexDCHoldLocksTotal}{22}
\newcommand{\luindexDCOneLockHeld}{52.3}
\newcommand{\luindexDCTwoNestedLocks}{51.5}
\newcommand{\luindexDCThreeNestedLocks}{51.4}
\newcommand{\luindexDCFourNestedLocks}{1.28}
\newcommand{\luindexDCFiveNestedLocks}{<0.1}
\newcommand{\luindexDCSixNestedLocks}{<0.1}
\newcommand{\luindexDCSevenNestedLocks}{\cna}
\newcommand{\luindexDCEightNestedLocks}{\cna}
\newcommand{\luindexDCNineNestedLocks}{\cna}
\newcommand{\luindexDCTenNestedLocks}{\cna}
\newcommand{\luindexDCHundredNestedLocks}{\cna}
\newcommand{\luindexFTODCEventTotal}{400}
\newcommand{\luindexFTODCNoFPEventTotal}{41}
\newcommand{\luindexFTODCNoFPAccessTotal}{40}
\newcommand{\luindexFTODCNoFPOtherTotal}{0.42}
\newcommand{\luindexFTODCReadTotal}{66.0}
\newcommand{\luindexFTODCWriteTotal}{33.0}
\newcommand{\luindexFTODCNoFPAccessInCS}{8.08}
\newcommand{\luindexFTODCNoFPAccessOutCS}{91.9}
\newcommand{\luindexFTODCAcqRelTotal}{14.2}
\newcommand{\luindexFTODCOtherTotal}{0.02}
\newcommand{\luindexFTODCNoFPReadTotal}{27}
\newcommand{\luindexFTODCReadInCS}{23.5}
\newcommand{\luindexFTODCReadOutCS}{82}
\newcommand{\luindexFTODCReadSameEp}{5.48}
\newcommand{\luindexFTODCReadSharedSameEp}{\cna}
\newcommand{\luindexFTODCReadExclusive}{<0.001}
\newcommand{\luindexFTODCReadOwned}{100}
\newcommand{\luindexFTODCReadShare}{<0.001}
\newcommand{\luindexFTODCReadShared}{\cna}
\newcommand{\luindexFTODCReadSharedOwned}{<0.001}
\newcommand{\luindexFTODCNoFPHonestWriteTotal}{13}
\newcommand{\luindexFTODCWriteInCS}{32.1}
\newcommand{\luindexFTODCWriteOutCS}{75.5}
\newcommand{\luindexFTODCNoFPWriteTotal}{13}
\newcommand{\luindexFTODCWriteSameEp}{7.57}
\newcommand{\luindexFTODCWriteExclusive}{<0.001}
\newcommand{\luindexFTODCWriteOwned}{100}
\newcommand{\luindexFTODCWriteShared}{\cna}
\newcommand{\luindexFTODCNoFPOtherEventTotal}{415322}
\newcommand{\luindexFTODCAcqRelOtherTotal}{99.9}
\newcommand{\luindexFTODCNoAcqRelOtherTotal}{582}
\newcommand{\luindexFTODCFork}{0.172}
\newcommand{\luindexFTODCJoin}{0.0}
\newcommand{\luindexFTODCPreWait}{0.344}
\newcommand{\luindexFTODCPostWait}{0.344}
\newcommand{\luindexFTODCVolatileTotal}{77.5}
\newcommand{\luindexFTODCClassInit}{11.3}
\newcommand{\luindexFTODCClassAccess}{10.3}
\newcommand{\luindexFTODCRaceTotal}{1}
\newcommand{\luindexFTODCWrRdRace}{0.0}
\newcommand{\luindexFTODCWrWrRace}{0.0}
\newcommand{\luindexFTODCRdWrRace}{0.0}
\newcommand{\luindexFTODCRdShWrRace}{100.0}
\newcommand{\luindexFTODCHoldLocksTotal}{10}
\newcommand{\luindexFTODCOneLockHeld}{25.8}
\newcommand{\luindexFTODCTwoNestedLocks}{25.4}
\newcommand{\luindexFTODCThreeNestedLocks}{25.3}
\newcommand{\luindexFTODCFourNestedLocks}{0.61}
\newcommand{\luindexFTODCFiveNestedLocks}{<0.1}
\newcommand{\luindexFTODCSixNestedLocks}{<0.1}
\newcommand{\luindexFTODCSevenNestedLocks}{\cna}
\newcommand{\luindexFTODCEightNestedLocks}{\cna}
\newcommand{\luindexFTODCNineNestedLocks}{\cna}
\newcommand{\luindexFTODCTenNestedLocks}{\cna}
\newcommand{\luindexFTODCHundredNestedLocks}{\cna}
\newcommand{\luindexREDCEventTotal}{400}
\newcommand{\luindexREDCNoFPEventTotal}{41}
\newcommand{\luindexREDCNoFPAccessTotal}{40}
\newcommand{\luindexREDCNoFPOtherTotal}{0.42}
\newcommand{\luindexREDCReadTotal}{66.0}
\newcommand{\luindexREDCWriteTotal}{33.0}
\newcommand{\luindexREDCNoFPAccessInCS}{8.08}
\newcommand{\luindexREDCNoFPAccessOutCS}{91.9}
\newcommand{\luindexREDCAcqRelTotal}{14.2}
\newcommand{\luindexREDCOtherTotal}{0.0197}
\newcommand{\luindexREDCNoFPReadTotal}{27}
\newcommand{\luindexREDCReadInCS}{23.5}
\newcommand{\luindexREDCReadOutCS}{82}
\newcommand{\luindexREDCReadSameEp}{5.48}
\newcommand{\luindexREDCReadSharedSameEp}{\cna}
\newcommand{\luindexREDCReadExclusive}{<0.001}
\newcommand{\luindexREDCReadOwned}{100}
\newcommand{\luindexREDCReadShare}{<0.001}
\newcommand{\luindexREDCReadShared}{\cna}
\newcommand{\luindexREDCReadSharedOwned}{<0.001}
\newcommand{\luindexREDCNoFPHonestWriteTotal}{13}
\newcommand{\luindexREDCWriteInCS}{32.1}
\newcommand{\luindexREDCWriteOutCS}{75.5}
\newcommand{\luindexREDCNoFPWriteTotal}{13}
\newcommand{\luindexREDCWriteSameEp}{7.57}
\newcommand{\luindexREDCWriteExclusive}{<0.001}
\newcommand{\luindexREDCWriteOwned}{100}
\newcommand{\luindexREDCWriteShared}{\cna}
\newcommand{\luindexREDCNoFPOtherEventTotal}{415315}
\newcommand{\luindexREDCAcqRelOtherTotal}{99.9}
\newcommand{\luindexREDCNoAcqRelOtherTotal}{575}
\newcommand{\luindexREDCFork}{0.174}
\newcommand{\luindexREDCJoin}{0.0}
\newcommand{\luindexREDCPreWait}{0.348}
\newcommand{\luindexREDCPostWait}{0.348}
\newcommand{\luindexREDCVolatileTotal}{77.2}
\newcommand{\luindexREDCClassInit}{11.5}
\newcommand{\luindexREDCClassAccess}{10.4}
\newcommand{\luindexREDCRaceTotal}{1}
\newcommand{\luindexREDCWrRdRace}{0.0}
\newcommand{\luindexREDCWrWrRace}{0.0}
\newcommand{\luindexREDCRdWrRace}{0.0}
\newcommand{\luindexREDCRdShWrRace}{100.0}
\newcommand{\luindexREDCHoldLocksTotal}{10}
\newcommand{\luindexREDCOneLockHeld}{25.8}
\newcommand{\luindexREDCTwoNestedLocks}{25.4}
\newcommand{\luindexREDCThreeNestedLocks}{25.3}
\newcommand{\luindexREDCFourNestedLocks}{0.61}
\newcommand{\luindexREDCFiveNestedLocks}{<0.1}
\newcommand{\luindexREDCSixNestedLocks}{<0.1}
\newcommand{\luindexREDCSevenNestedLocks}{\cna}
\newcommand{\luindexREDCEightNestedLocks}{\cna}
\newcommand{\luindexREDCNineNestedLocks}{\cna}
\newcommand{\luindexREDCTenNestedLocks}{\cna}
\newcommand{\luindexREDCHundredNestedLocks}{\cna}
\newcommand{\luindexCAPOEventTotal}{400}
\newcommand{\luindexCAPONoFPEventTotal}{43}
\newcommand{\luindexCAPONoFPAccessTotal}{42}
\newcommand{\luindexCAPONoFPOtherTotal}{0.42}
\newcommand{\luindexCAPOReadTotal}{67.6}
\newcommand{\luindexCAPOWriteTotal}{31.4}
\newcommand{\luindexCAPONoFPAccessInCS}{83.0}
\newcommand{\luindexCAPONoFPAccessOutCS}{17.0}
\newcommand{\luindexCAPOAcqRelTotal}{2.98}
\newcommand{\luindexCAPOOtherTotal}{0.00418}
\newcommand{\luindexCAPONoFPReadTotal}{29}
\newcommand{\luindexCAPOReadInCS}{23.8}
\newcommand{\luindexCAPOReadOutCS}{81.3}
\newcommand{\luindexCAPOReadSameEp}{5.1}
\newcommand{\luindexCAPOReadSharedSameEp}{\cna}
\newcommand{\luindexCAPOReadExclusive}{100}
\newcommand{\luindexCAPOReadOwned}{\cna}
\newcommand{\luindexCAPOReadShare}{<0.001}
\newcommand{\luindexCAPOReadShared}{<0.001}
\newcommand{\luindexCAPOReadSharedOwned}{\cna}
\newcommand{\luindexCAPONoFPHonestWriteTotal}{13}
\newcommand{\luindexCAPOWriteInCS}{32.1}
\newcommand{\luindexCAPOWriteOutCS}{75.5}
\newcommand{\luindexCAPONoFPWriteTotal}{13}
\newcommand{\luindexCAPOWriteSameEp}{7.57}
\newcommand{\luindexCAPOWriteExclusive}{100}
\newcommand{\luindexCAPOWriteOwned}{\cna}
\newcommand{\luindexCAPOWriteShared}{<0.001}
\newcommand{\luindexCAPONoFPOtherEventTotal}{415322}
\newcommand{\luindexCAPOAcqRelOtherTotal}{99.9}
\newcommand{\luindexCAPONoAcqRelOtherTotal}{582}
\newcommand{\luindexCAPOFork}{0.172}
\newcommand{\luindexCAPOJoin}{0.0}
\newcommand{\luindexCAPOPreWait}{0.344}
\newcommand{\luindexCAPOPostWait}{0.344}
\newcommand{\luindexCAPOVolatileTotal}{77.5}
\newcommand{\luindexCAPOClassInit}{11.3}
\newcommand{\luindexCAPOClassAccess}{10.3}
\newcommand{\luindexCAPORaceTotal}{1}
\newcommand{\luindexCAPOWrRdRace}{0.0}
\newcommand{\luindexCAPOWrWrRace}{0.0}
\newcommand{\luindexCAPORdWrRace}{0.0}
\newcommand{\luindexCAPORdShWrRace}{100.0}
\newcommand{\luindexCAPOHoldLocksTotal}{22}
\newcommand{\luindexCAPOOneLockHeld}{52.3}
\newcommand{\luindexCAPOTwoNestedLocks}{51.5}
\newcommand{\luindexCAPOThreeNestedLocks}{51.4}
\newcommand{\luindexCAPOFourNestedLocks}{1.28}
\newcommand{\luindexCAPOFiveNestedLocks}{<0.1}
\newcommand{\luindexCAPOSixNestedLocks}{<0.1}
\newcommand{\luindexCAPOSevenNestedLocks}{\cna}
\newcommand{\luindexCAPOEightNestedLocks}{\cna}
\newcommand{\luindexCAPONineNestedLocks}{\cna}
\newcommand{\luindexCAPOTenNestedLocks}{\cna}
\newcommand{\luindexCAPOHundredNestedLocks}{\cna}
\newcommand{\luindexFTOCAPOEventTotal}{400}
\newcommand{\luindexFTOCAPONoFPEventTotal}{41}
\newcommand{\luindexFTOCAPONoFPAccessTotal}{40}
\newcommand{\luindexFTOCAPONoFPOtherTotal}{0.42}
\newcommand{\luindexFTOCAPOReadTotal}{66.0}
\newcommand{\luindexFTOCAPOWriteTotal}{33.0}
\newcommand{\luindexFTOCAPONoFPAccessInCS}{8.08}
\newcommand{\luindexFTOCAPONoFPAccessOutCS}{91.9}
\newcommand{\luindexFTOCAPOAcqRelTotal}{14.2}
\newcommand{\luindexFTOCAPOOtherTotal}{0.02}
\newcommand{\luindexFTOCAPONoFPReadTotal}{27}
\newcommand{\luindexFTOCAPOReadInCS}{23.5}
\newcommand{\luindexFTOCAPOReadOutCS}{82}
\newcommand{\luindexFTOCAPOReadSameEp}{5.48}
\newcommand{\luindexFTOCAPOReadSharedSameEp}{\cna}
\newcommand{\luindexFTOCAPOReadExclusive}{<0.001}
\newcommand{\luindexFTOCAPOReadOwned}{100}
\newcommand{\luindexFTOCAPOReadShare}{<0.001}
\newcommand{\luindexFTOCAPOReadShared}{\cna}
\newcommand{\luindexFTOCAPOReadSharedOwned}{<0.001}
\newcommand{\luindexFTOCAPONoFPHonestWriteTotal}{13}
\newcommand{\luindexFTOCAPOWriteInCS}{32.1}
\newcommand{\luindexFTOCAPOWriteOutCS}{75.5}
\newcommand{\luindexFTOCAPONoFPWriteTotal}{13}
\newcommand{\luindexFTOCAPOWriteSameEp}{7.57}
\newcommand{\luindexFTOCAPOWriteExclusive}{<0.001}
\newcommand{\luindexFTOCAPOWriteOwned}{100}
\newcommand{\luindexFTOCAPOWriteShared}{\cna}
\newcommand{\luindexFTOCAPONoFPOtherEventTotal}{415322}
\newcommand{\luindexFTOCAPOAcqRelOtherTotal}{99.9}
\newcommand{\luindexFTOCAPONoAcqRelOtherTotal}{582}
\newcommand{\luindexFTOCAPOFork}{0.172}
\newcommand{\luindexFTOCAPOJoin}{0.0}
\newcommand{\luindexFTOCAPOPreWait}{0.344}
\newcommand{\luindexFTOCAPOPostWait}{0.344}
\newcommand{\luindexFTOCAPOVolatileTotal}{77.5}
\newcommand{\luindexFTOCAPOClassInit}{11.3}
\newcommand{\luindexFTOCAPOClassAccess}{10.3}
\newcommand{\luindexFTOCAPORaceTotal}{1}
\newcommand{\luindexFTOCAPOWrRdRace}{0.0}
\newcommand{\luindexFTOCAPOWrWrRace}{0.0}
\newcommand{\luindexFTOCAPORdWrRace}{0.0}
\newcommand{\luindexFTOCAPORdShWrRace}{100.0}
\newcommand{\luindexFTOCAPOHoldLocksTotal}{10}
\newcommand{\luindexFTOCAPOOneLockHeld}{25.8}
\newcommand{\luindexFTOCAPOTwoNestedLocks}{25.4}
\newcommand{\luindexFTOCAPOThreeNestedLocks}{25.3}
\newcommand{\luindexFTOCAPOFourNestedLocks}{0.61}
\newcommand{\luindexFTOCAPOFiveNestedLocks}{<0.1}
\newcommand{\luindexFTOCAPOSixNestedLocks}{<0.1}
\newcommand{\luindexFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\luindexFTOCAPOEightNestedLocks}{\cna}
\newcommand{\luindexFTOCAPONineNestedLocks}{\cna}
\newcommand{\luindexFTOCAPOTenNestedLocks}{\cna}
\newcommand{\luindexFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\luindexRECAPOEventTotal}{400}
\newcommand{\luindexRECAPONoFPEventTotal}{41}
\newcommand{\luindexRECAPONoFPAccessTotal}{40}
\newcommand{\luindexRECAPONoFPOtherTotal}{0.42}
\newcommand{\luindexRECAPOReadTotal}{66.0}
\newcommand{\luindexRECAPOWriteTotal}{33.0}
\newcommand{\luindexRECAPONoFPAccessInCS}{8.08}
\newcommand{\luindexRECAPONoFPAccessOutCS}{91.9}
\newcommand{\luindexRECAPOAcqRelTotal}{14.2}
\newcommand{\luindexRECAPOOtherTotal}{0.0197}
\newcommand{\luindexRECAPONoFPReadTotal}{27}
\newcommand{\luindexRECAPOReadInCS}{23.5}
\newcommand{\luindexRECAPOReadOutCS}{82}
\newcommand{\luindexRECAPOReadSameEp}{5.48}
\newcommand{\luindexRECAPOReadSharedSameEp}{\cna}
\newcommand{\luindexRECAPOReadExclusive}{<0.001}
\newcommand{\luindexRECAPOReadOwned}{100}
\newcommand{\luindexRECAPOReadShare}{<0.001}
\newcommand{\luindexRECAPOReadShared}{\cna}
\newcommand{\luindexRECAPOReadSharedOwned}{<0.001}
\newcommand{\luindexRECAPONoFPHonestWriteTotal}{13}
\newcommand{\luindexRECAPOWriteInCS}{32.1}
\newcommand{\luindexRECAPOWriteOutCS}{75.5}
\newcommand{\luindexRECAPONoFPWriteTotal}{13}
\newcommand{\luindexRECAPOWriteSameEp}{7.57}
\newcommand{\luindexRECAPOWriteExclusive}{<0.001}
\newcommand{\luindexRECAPOWriteOwned}{100}
\newcommand{\luindexRECAPOWriteShared}{\cna}
\newcommand{\luindexRECAPONoFPOtherEventTotal}{415315}
\newcommand{\luindexRECAPOAcqRelOtherTotal}{99.9}
\newcommand{\luindexRECAPONoAcqRelOtherTotal}{575}
\newcommand{\luindexRECAPOFork}{0.174}
\newcommand{\luindexRECAPOJoin}{0.0}
\newcommand{\luindexRECAPOPreWait}{0.348}
\newcommand{\luindexRECAPOPostWait}{0.348}
\newcommand{\luindexRECAPOVolatileTotal}{77.2}
\newcommand{\luindexRECAPOClassInit}{11.5}
\newcommand{\luindexRECAPOClassAccess}{10.4}
\newcommand{\luindexRECAPORaceTotal}{1}
\newcommand{\luindexRECAPOWrRdRace}{0.0}
\newcommand{\luindexRECAPOWrWrRace}{0.0}
\newcommand{\luindexRECAPORdWrRace}{0.0}
\newcommand{\luindexRECAPORdShWrRace}{100.0}
\newcommand{\luindexRECAPOHoldLocksTotal}{10}
\newcommand{\luindexRECAPOOneLockHeld}{25.8}
\newcommand{\luindexRECAPOTwoNestedLocks}{25.4}
\newcommand{\luindexRECAPOThreeNestedLocks}{25.3}
\newcommand{\luindexRECAPOFourNestedLocks}{0.61}
\newcommand{\luindexRECAPOFiveNestedLocks}{<0.1}
\newcommand{\luindexRECAPOSixNestedLocks}{<0.1}
\newcommand{\luindexRECAPOSevenNestedLocks}{\cna}
\newcommand{\luindexRECAPOEightNestedLocks}{\cna}
\newcommand{\luindexRECAPONineNestedLocks}{\cna}
\newcommand{\luindexRECAPOTenNestedLocks}{\cna}
\newcommand{\luindexRECAPOHundredNestedLocks}{\cna}
\newcommand{\luindexCAPOTotalSetClears}{0.21}
\newcommand{\luindexCAPOReadSetZero}{90.0}
\newcommand{\luindexCAPOReadSetOne}{4.62}
\newcommand{\luindexCAPOReadSetGtOne}{5.37}
\newcommand{\luindexCAPOWriteSetZero}{6.91}
\newcommand{\luindexCAPOWriteSetOne}{90.6}
\newcommand{\luindexCAPOWriteSetGtOne}{2.51}
\newcommand{\luindexCAPOTotalMapClears}{0.21}
\newcommand{\luindexCAPOReadMapZero}{0.597}
\newcommand{\luindexCAPOReadMapOne}{0.0203}
\newcommand{\luindexCAPOReadMapTen}{94.1}
\newcommand{\luindexCAPOReadMapHund}{2.28}
\newcommand{\luindexCAPOReadMapThou}{9.64E-4}
\newcommand{\luindexCAPOReadMapGtThou}{3.0}
\newcommand{\luindexCAPOWriteMapZero}{0.619}
\newcommand{\luindexCAPOWriteMapOne}{0.437}
\newcommand{\luindexCAPOWriteMapTen}{93.9}
\newcommand{\luindexCAPOWriteMapHund}{0.0227}
\newcommand{\luindexCAPOWriteMapThou}{0.437}
\newcommand{\luindexCAPOWriteMapGtThou}{4.57}
\newcommand{\FASTluindexMaxLiveThreads}{3}
\newcommand{\FASTluindexTotalThreads}{3}
\newcommand{\FASTluindexBaseTime}{1.3}
\newcommand{\FASTluindexBaseTimeCI}{120}
\newcommand{\FASTluindexEmptyTime}{\rna}
\newcommand{\FASTluindexEmptyTimeCI}{\rna}
\newcommand{\FASTluindexEmptyTimeCIMIN}{\rna}
\newcommand{\FASTluindexEmptyTimeCIMAX}{\rna}
\newcommand{\FASTluindexFTTime}{7.4}
\newcommand{\FASTluindexFTTimeCI}{0.54}
\newcommand{\FASTluindexHBTime}{7.7}
\newcommand{\FASTluindexHBTimeCI}{0.58}
\newcommand{\FASTluindexFTOHBTime}{7.7}
\newcommand{\FASTluindexFTOHBTimeCI}{0.58}
\newcommand{\FASTluindexWCPTime}{18}
\newcommand{\FASTluindexWCPTimeCI}{1.4}
\newcommand{\FASTluindexFTOWCPTime}{23}
\newcommand{\FASTluindexFTOWCPTimeCI}{1.6}
\newcommand{\FASTluindexREWCPTime}{9.1}
\newcommand{\FASTluindexREWCPTimeCI}{0.68}
\newcommand{\FASTluindexDCTime}{18}
\newcommand{\FASTluindexDCTimeCI}{1.3}
\newcommand{\FASTluindexFTODCTime}{23}
\newcommand{\FASTluindexFTODCTimeCI}{1.7}
\newcommand{\FASTluindexREDCTime}{9.0}
\newcommand{\FASTluindexREDCTimeCI}{0.6}
\newcommand{\FASTluindexCAPOTime}{18}
\newcommand{\FASTluindexCAPOTimeCI}{1.3}
\newcommand{\FASTluindexFTOCAPOTime}{23}
\newcommand{\FASTluindexFTOCAPOTimeCI}{1.6}
\newcommand{\FASTluindexRECAPOTime}{8.8}
\newcommand{\FASTluindexRECAPOTimeCI}{0.64}
\newcommand{\FASTluindexAGGCAPOTime}{\rna}
\newcommand{\FASTluindexAGGCAPOTimeCI}{\rna}
\newcommand{\FASTluindexAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTluindexAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTluindexStaticTime}{\rzero}
\newcommand{\FASTluindexDynamicTime}{\rzero}
\newcommand{\FASTluindexBaseMem}{120}
\newcommand{\FASTluindexBaseMemCI}{2.9}
\newcommand{\FASTluindexFTMem}{4.9}
\newcommand{\FASTluindexFTMemCI}{0.12}
\newcommand{\FASTluindexHBMem}{4.9}
\newcommand{\FASTluindexHBMemCI}{0.097}
\newcommand{\FASTluindexFTOHBMem}{4.9}
\newcommand{\FASTluindexFTOHBMemCI}{0.14}
\newcommand{\FASTluindexWCPMem}{23}
\newcommand{\FASTluindexWCPMemCI}{0.5}
\newcommand{\FASTluindexFTOWCPMem}{24}
\newcommand{\FASTluindexFTOWCPMemCI}{0.58}
\newcommand{\FASTluindexREWCPMem}{9.0}
\newcommand{\FASTluindexREWCPMemCI}{0.7}
\newcommand{\FASTluindexDCMem}{23}
\newcommand{\FASTluindexDCMemCI}{0.53}
\newcommand{\FASTluindexFTODCMem}{24}
\newcommand{\FASTluindexFTODCMemCI}{0.49}
\newcommand{\FASTluindexREDCMem}{9.8}
\newcommand{\FASTluindexREDCMemCI}{0.85}
\newcommand{\FASTluindexCAPOMem}{23}
\newcommand{\FASTluindexCAPOMemCI}{0.58}
\newcommand{\FASTluindexFTOCAPOMem}{24}
\newcommand{\FASTluindexFTOCAPOMemCI}{0.51}
\newcommand{\FASTluindexRECAPOMem}{8.2}
\newcommand{\FASTluindexRECAPOMemCI}{0.21}
\newcommand{\FASTluindexAGGCAPOMem}{\memna}
\newcommand{\FASTluindexAGGCAPOMemCI}{\memna}
\newcommand{\FASTluindexAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTluindexAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTluindexEventsCI}{0}
\newcommand{\FASTluindexEventsCIMIN}{396,268,367}
\newcommand{\FASTluindexEventsCIMAX}{396,268,367}
\newcommand{\FASTluindexNoFPEventsCI}{0}
\newcommand{\FASTluindexNoFPEventsCIMIN}{2,915,284}
\newcommand{\FASTluindexNoFPEventsCIMAX}{2,915,284}
\newcommand{\FASTluindexFT}{1}
\newcommand{\FASTluindexFTCI}{0}
\newcommand{\FASTluindexFTCIMIN}{1}
\newcommand{\FASTluindexFTCIMAX}{1}
\newcommand{\FASTluindexFTDynamic}{1}
\newcommand{\FASTluindexFTDynamicCI}{0}
\newcommand{\FASTluindexFTDynamicCIMIN}{1}
\newcommand{\FASTluindexFTDynamicCIMAX}{1}
\newcommand{\FASTluindexHB}{1}
\newcommand{\FASTluindexHBCI}{0}
\newcommand{\FASTluindexHBCIMIN}{1}
\newcommand{\FASTluindexHBCIMAX}{1}
\newcommand{\FASTluindexHBDynamic}{1}
\newcommand{\FASTluindexHBDynamicCI}{0}
\newcommand{\FASTluindexHBDynamicCIMIN}{1}
\newcommand{\FASTluindexHBDynamicCIMAX}{1}
\newcommand{\FASTluindexFTOHB}{1}
\newcommand{\FASTluindexFTOHBCI}{0}
\newcommand{\FASTluindexFTOHBCIMIN}{1}
\newcommand{\FASTluindexFTOHBCIMAX}{1}
\newcommand{\FASTluindexFTOHBDynamic}{1}
\newcommand{\FASTluindexFTOHBDynamicCI}{0}
\newcommand{\FASTluindexFTOHBDynamicCIMIN}{1}
\newcommand{\FASTluindexFTOHBDynamicCIMAX}{1}
\newcommand{\FASTluindexWCP}{1}
\newcommand{\FASTluindexWCPCI}{0}
\newcommand{\FASTluindexWCPCIMIN}{1}
\newcommand{\FASTluindexWCPCIMAX}{1}
\newcommand{\FASTluindexWCPDynamic}{1}
\newcommand{\FASTluindexWCPDynamicCI}{0}
\newcommand{\FASTluindexWCPDynamicCIMIN}{1}
\newcommand{\FASTluindexWCPDynamicCIMAX}{1}
\newcommand{\FASTluindexFTOWCP}{1}
\newcommand{\FASTluindexFTOWCPCI}{0}
\newcommand{\FASTluindexFTOWCPCIMIN}{1}
\newcommand{\FASTluindexFTOWCPCIMAX}{1}
\newcommand{\FASTluindexFTOWCPDynamic}{1}
\newcommand{\FASTluindexFTOWCPDynamicCI}{0}
\newcommand{\FASTluindexFTOWCPDynamicCIMIN}{1}
\newcommand{\FASTluindexFTOWCPDynamicCIMAX}{1}
\newcommand{\FASTluindexREWCP}{1}
\newcommand{\FASTluindexREWCPCI}{0}
\newcommand{\FASTluindexREWCPCIMIN}{1}
\newcommand{\FASTluindexREWCPCIMAX}{1}
\newcommand{\FASTluindexREWCPDynamic}{1}
\newcommand{\FASTluindexREWCPDynamicCI}{0}
\newcommand{\FASTluindexREWCPDynamicCIMIN}{1}
\newcommand{\FASTluindexREWCPDynamicCIMAX}{1}
\newcommand{\FASTluindexDC}{1}
\newcommand{\FASTluindexDCCI}{0}
\newcommand{\FASTluindexDCCIMIN}{1}
\newcommand{\FASTluindexDCCIMAX}{1}
\newcommand{\FASTluindexDCDynamic}{1}
\newcommand{\FASTluindexDCDynamicCI}{0}
\newcommand{\FASTluindexDCDynamicCIMIN}{1}
\newcommand{\FASTluindexDCDynamicCIMAX}{1}
\newcommand{\FASTluindexFTODC}{1}
\newcommand{\FASTluindexFTODCCI}{0}
\newcommand{\FASTluindexFTODCCIMIN}{1}
\newcommand{\FASTluindexFTODCCIMAX}{1}
\newcommand{\FASTluindexFTODCDynamic}{1}
\newcommand{\FASTluindexFTODCDynamicCI}{0}
\newcommand{\FASTluindexFTODCDynamicCIMIN}{1}
\newcommand{\FASTluindexFTODCDynamicCIMAX}{1}
\newcommand{\FASTluindexREDC}{1}
\newcommand{\FASTluindexREDCCI}{0}
\newcommand{\FASTluindexREDCCIMIN}{1}
\newcommand{\FASTluindexREDCCIMAX}{1}
\newcommand{\FASTluindexREDCDynamic}{1}
\newcommand{\FASTluindexREDCDynamicCI}{0}
\newcommand{\FASTluindexREDCDynamicCIMIN}{1}
\newcommand{\FASTluindexREDCDynamicCIMAX}{1}
\newcommand{\FASTluindexCAPO}{1}
\newcommand{\FASTluindexCAPOCI}{0}
\newcommand{\FASTluindexCAPOCIMIN}{1}
\newcommand{\FASTluindexCAPOCIMAX}{1}
\newcommand{\FASTluindexCAPODynamic}{1}
\newcommand{\FASTluindexCAPODynamicCI}{0}
\newcommand{\FASTluindexCAPODynamicCIMIN}{1}
\newcommand{\FASTluindexCAPODynamicCIMAX}{1}
\newcommand{\FASTluindexFTOCAPO}{1}
\newcommand{\FASTluindexFTOCAPOCI}{0}
\newcommand{\FASTluindexFTOCAPOCIMIN}{1}
\newcommand{\FASTluindexFTOCAPOCIMAX}{1}
\newcommand{\FASTluindexFTOCAPODynamic}{1}
\newcommand{\FASTluindexFTOCAPODynamicCI}{0}
\newcommand{\FASTluindexFTOCAPODynamicCIMIN}{1}
\newcommand{\FASTluindexFTOCAPODynamicCIMAX}{1}
\newcommand{\FASTluindexRECAPO}{1}
\newcommand{\FASTluindexRECAPOCI}{0}
\newcommand{\FASTluindexRECAPOCIMIN}{1}
\newcommand{\FASTluindexRECAPOCIMAX}{1}
\newcommand{\FASTluindexRECAPODynamic}{1}
\newcommand{\FASTluindexRECAPODynamicCI}{0}
\newcommand{\FASTluindexRECAPODynamicCIMIN}{1}
\newcommand{\FASTluindexRECAPODynamicCIMAX}{1}
\newcommand{\FASTluindexAGGCAPO}{\rna}
\newcommand{\FASTluindexAGGCAPOCI}{\rna}
\newcommand{\FASTluindexAGGCAPOCIMIN}{\rna}
\newcommand{\FASTluindexAGGCAPOCIMAX}{\rna}
\newcommand{\FASTluindexAGGCAPODynamic}{\rna}
\newcommand{\FASTluindexAGGCAPODynamicCI}{\rna}
\newcommand{\FASTluindexAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTluindexAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTlusearchEvents}{1,400}
\newcommand{\FASTlusearchNoFPEvents}{43}
\newcommand{\lusearchHBEventTotal}{1,400}
\newcommand{\lusearchHBNoFPEventTotal}{150}
\newcommand{\lusearchHBNoFPAccessTotal}{150}
\newcommand{\lusearchHBNoFPOtherTotal}{3.8}
\newcommand{\lusearchHBReadTotal}{79.4}
\newcommand{\lusearchHBWriteTotal}{18.1}
\newcommand{\lusearchHBNoFPAccessInCS}{4.89}
\newcommand{\lusearchHBNoFPAccessOutCS}{95.1}
\newcommand{\lusearchHBAcqRelTotal}{6.23}
\newcommand{\lusearchHBOtherTotal}{2.72}
\newcommand{\lusearchHBNoFPReadTotal}{120}
\newcommand{\lusearchHBReadInCS}{3.36}
\newcommand{\lusearchHBReadOutCS}{103}
\newcommand{\lusearchHBReadSameEp}{6.47}
\newcommand{\lusearchHBReadSharedSameEp}{\cna}
\newcommand{\lusearchHBReadExclusive}{96.6}
\newcommand{\lusearchHBReadOwned}{\cna}
\newcommand{\lusearchHBReadShare}{<0.001}
\newcommand{\lusearchHBReadShared}{3.41}
\newcommand{\lusearchHBReadSharedOwned}{\cna}
\newcommand{\lusearchHBNoFPHonestWriteTotal}{28}
\newcommand{\lusearchHBWriteInCS}{10}
\newcommand{\lusearchHBWriteOutCS}{200}
\newcommand{\lusearchHBNoFPWriteTotal}{28}
\newcommand{\lusearchHBWriteSameEp}{110}
\newcommand{\lusearchHBWriteExclusive}{100}
\newcommand{\lusearchHBWriteOwned}{\cna}
\newcommand{\lusearchHBWriteShared}{\cna}
\newcommand{\lusearchHBNoFPOtherEventTotal}{3816174}
\newcommand{\lusearchHBAcqRelOtherTotal}{69.6}
\newcommand{\lusearchHBNoAcqRelOtherTotal}{1158238}
\newcommand{\lusearchHBFork}{6.91E-4}
\newcommand{\lusearchHBJoin}{0.0}
\newcommand{\lusearchHBPreWait}{0.00553}
\newcommand{\lusearchHBPostWait}{0.00553}
\newcommand{\lusearchHBVolatileTotal}{100.0}
\newcommand{\lusearchHBClassInit}{0.00311}
\newcommand{\lusearchHBClassAccess}{0.0168}
\newcommand{\lusearchHBRaceTotal}{\rna}
\newcommand{\lusearchHBWrRdRace}{\rna}
\newcommand{\lusearchHBWrWrRace}{\rna}
\newcommand{\lusearchHBRdWrRace}{\rna}
\newcommand{\lusearchHBRdShWrRace}{\rna}
\newcommand{\lusearchHBHoldLocksTotal}{6.9}
\newcommand{\lusearchHBOneLockHeld}{4.60}
\newcommand{\lusearchHBTwoNestedLocks}{0.26}
\newcommand{\lusearchHBThreeNestedLocks}{<0.1}
\newcommand{\lusearchHBFourNestedLocks}{\cna}
\newcommand{\lusearchHBFiveNestedLocks}{\cna}
\newcommand{\lusearchHBSixNestedLocks}{\cna}
\newcommand{\lusearchHBSevenNestedLocks}{\cna}
\newcommand{\lusearchHBEightNestedLocks}{\cna}
\newcommand{\lusearchHBNineNestedLocks}{\cna}
\newcommand{\lusearchHBTenNestedLocks}{\cna}
\newcommand{\lusearchHBHundredNestedLocks}{\cna}
\newcommand{\lusearchFTOHBEventTotal}{1,400}
\newcommand{\lusearchFTOHBNoFPEventTotal}{140}
\newcommand{\lusearchFTOHBNoFPAccessTotal}{130}
\newcommand{\lusearchFTOHBNoFPOtherTotal}{3.8}
\newcommand{\lusearchFTOHBReadTotal}{76.9}
\newcommand{\lusearchFTOHBWriteTotal}{20.3}
\newcommand{\lusearchFTOHBNoFPAccessInCS}{4.89}
\newcommand{\lusearchFTOHBNoFPAccessOutCS}{95.1}
\newcommand{\lusearchFTOHBAcqRelTotal}{6.23}
\newcommand{\lusearchFTOHBOtherTotal}{2.72}
\newcommand{\lusearchFTOHBNoFPReadTotal}{110}
\newcommand{\lusearchFTOHBReadInCS}{3.53}
\newcommand{\lusearchFTOHBReadOutCS}{104}
\newcommand{\lusearchFTOHBReadSameEp}{7.49}
\newcommand{\lusearchFTOHBReadSharedSameEp}{\cna}
\newcommand{\lusearchFTOHBReadExclusive}{<0.001}
\newcommand{\lusearchFTOHBReadOwned}{96.1}
\newcommand{\lusearchFTOHBReadShare}{<0.001}
\newcommand{\lusearchFTOHBReadShared}{<0.001}
\newcommand{\lusearchFTOHBReadSharedOwned}{3.94}
\newcommand{\lusearchFTOHBNoFPHonestWriteTotal}{28}
\newcommand{\lusearchFTOHBWriteInCS}{10}
\newcommand{\lusearchFTOHBWriteOutCS}{200}
\newcommand{\lusearchFTOHBNoFPWriteTotal}{28}
\newcommand{\lusearchFTOHBWriteSameEp}{110}
\newcommand{\lusearchFTOHBWriteExclusive}{\cna}
\newcommand{\lusearchFTOHBWriteOwned}{100}
\newcommand{\lusearchFTOHBWriteShared}{\cna}
\newcommand{\lusearchFTOHBNoFPOtherEventTotal}{3816148}
\newcommand{\lusearchFTOHBAcqRelOtherTotal}{69.6}
\newcommand{\lusearchFTOHBNoAcqRelOtherTotal}{1158212}
\newcommand{\lusearchFTOHBFork}{6.91E-4}
\newcommand{\lusearchFTOHBJoin}{0.0}
\newcommand{\lusearchFTOHBPreWait}{0.00544}
\newcommand{\lusearchFTOHBPostWait}{0.00544}
\newcommand{\lusearchFTOHBVolatileTotal}{100.0}
\newcommand{\lusearchFTOHBClassInit}{0.00311}
\newcommand{\lusearchFTOHBClassAccess}{0.0168}
\newcommand{\lusearchFTOHBRaceTotal}{\rna}
\newcommand{\lusearchFTOHBWrRdRace}{\rna}
\newcommand{\lusearchFTOHBWrWrRace}{\rna}
\newcommand{\lusearchFTOHBRdWrRace}{\rna}
\newcommand{\lusearchFTOHBRdShWrRace}{\rna}
\newcommand{\lusearchFTOHBHoldLocksTotal}{4.7}
\newcommand{\lusearchFTOHBOneLockHeld}{3.47}
\newcommand{\lusearchFTOHBTwoNestedLocks}{0.29}
\newcommand{\lusearchFTOHBThreeNestedLocks}{<0.1}
\newcommand{\lusearchFTOHBFourNestedLocks}{\cna}
\newcommand{\lusearchFTOHBFiveNestedLocks}{\cna}
\newcommand{\lusearchFTOHBSixNestedLocks}{\cna}
\newcommand{\lusearchFTOHBSevenNestedLocks}{\cna}
\newcommand{\lusearchFTOHBEightNestedLocks}{\cna}
\newcommand{\lusearchFTOHBNineNestedLocks}{\cna}
\newcommand{\lusearchFTOHBTenNestedLocks}{\cna}
\newcommand{\lusearchFTOHBHundredNestedLocks}{\cna}
\newcommand{\lusearchWCPEventTotal}{1,400}
\newcommand{\lusearchWCPNoFPEventTotal}{160}
\newcommand{\lusearchWCPNoFPAccessTotal}{150}
\newcommand{\lusearchWCPNoFPOtherTotal}{3.8}
\newcommand{\lusearchWCPReadTotal}{79.5}
\newcommand{\lusearchWCPWriteTotal}{18.0}
\newcommand{\lusearchWCPNoFPAccessInCS}{16.7}
\newcommand{\lusearchWCPNoFPAccessOutCS}{83.3}
\newcommand{\lusearchWCPAcqRelTotal}{5.52}
\newcommand{\lusearchWCPOtherTotal}{2.41}
\newcommand{\lusearchWCPNoFPReadTotal}{120}
\newcommand{\lusearchWCPReadInCS}{3.72}
\newcommand{\lusearchWCPReadOutCS}{103}
\newcommand{\lusearchWCPReadSameEp}{6.44}
\newcommand{\lusearchWCPReadSharedSameEp}{\cna}
\newcommand{\lusearchWCPReadExclusive}{96.6}
\newcommand{\lusearchWCPReadOwned}{\cna}
\newcommand{\lusearchWCPReadShare}{<0.001}
\newcommand{\lusearchWCPReadShared}{3.39}
\newcommand{\lusearchWCPReadSharedOwned}{\cna}
\newcommand{\lusearchWCPNoFPHonestWriteTotal}{28}
\newcommand{\lusearchWCPWriteInCS}{10}
\newcommand{\lusearchWCPWriteOutCS}{200}
\newcommand{\lusearchWCPNoFPWriteTotal}{28}
\newcommand{\lusearchWCPWriteSameEp}{110}
\newcommand{\lusearchWCPWriteExclusive}{100}
\newcommand{\lusearchWCPWriteOwned}{\cna}
\newcommand{\lusearchWCPWriteShared}{<0.001}
\newcommand{\lusearchWCPNoFPOtherEventTotal}{3816190}
\newcommand{\lusearchWCPAcqRelOtherTotal}{69.6}
\newcommand{\lusearchWCPNoAcqRelOtherTotal}{1158254}
\newcommand{\lusearchWCPFork}{6.91E-4}
\newcommand{\lusearchWCPJoin}{0.0}
\newcommand{\lusearchWCPPreWait}{0.00553}
\newcommand{\lusearchWCPPostWait}{0.00553}
\newcommand{\lusearchWCPVolatileTotal}{100.0}
\newcommand{\lusearchWCPClassInit}{0.00311}
\newcommand{\lusearchWCPClassAccess}{0.0168}
\newcommand{\lusearchWCPRaceTotal}{\rna}
\newcommand{\lusearchWCPWrRdRace}{\rna}
\newcommand{\lusearchWCPWrWrRace}{\rna}
\newcommand{\lusearchWCPRdWrRace}{\rna}
\newcommand{\lusearchWCPRdShWrRace}{\rna}
\newcommand{\lusearchWCPHoldLocksTotal}{13}
\newcommand{\lusearchWCPOneLockHeld}{8.51}
\newcommand{\lusearchWCPTwoNestedLocks}{0.70}
\newcommand{\lusearchWCPThreeNestedLocks}{<0.1}
\newcommand{\lusearchWCPFourNestedLocks}{\cna}
\newcommand{\lusearchWCPFiveNestedLocks}{\cna}
\newcommand{\lusearchWCPSixNestedLocks}{\cna}
\newcommand{\lusearchWCPSevenNestedLocks}{\cna}
\newcommand{\lusearchWCPEightNestedLocks}{\cna}
\newcommand{\lusearchWCPNineNestedLocks}{\cna}
\newcommand{\lusearchWCPTenNestedLocks}{\cna}
\newcommand{\lusearchWCPHundredNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPEventTotal}{1,400}
\newcommand{\lusearchFTOWCPNoFPEventTotal}{140}
\newcommand{\lusearchFTOWCPNoFPAccessTotal}{130}
\newcommand{\lusearchFTOWCPNoFPOtherTotal}{3.8}
\newcommand{\lusearchFTOWCPReadTotal}{77.0}
\newcommand{\lusearchFTOWCPWriteTotal}{20.2}
\newcommand{\lusearchFTOWCPNoFPAccessInCS}{4.89}
\newcommand{\lusearchFTOWCPNoFPAccessOutCS}{95.1}
\newcommand{\lusearchFTOWCPAcqRelTotal}{6.23}
\newcommand{\lusearchFTOWCPOtherTotal}{2.72}
\newcommand{\lusearchFTOWCPNoFPReadTotal}{110}
\newcommand{\lusearchFTOWCPReadInCS}{3.94}
\newcommand{\lusearchFTOWCPReadOutCS}{104}
\newcommand{\lusearchFTOWCPReadSameEp}{7.45}
\newcommand{\lusearchFTOWCPReadSharedSameEp}{\cna}
\newcommand{\lusearchFTOWCPReadExclusive}{<0.001}
\newcommand{\lusearchFTOWCPReadOwned}{96.1}
\newcommand{\lusearchFTOWCPReadShare}{<0.001}
\newcommand{\lusearchFTOWCPReadShared}{<0.001}
\newcommand{\lusearchFTOWCPReadSharedOwned}{3.93}
\newcommand{\lusearchFTOWCPNoFPHonestWriteTotal}{28}
\newcommand{\lusearchFTOWCPWriteInCS}{10}
\newcommand{\lusearchFTOWCPWriteOutCS}{200}
\newcommand{\lusearchFTOWCPNoFPWriteTotal}{28}
\newcommand{\lusearchFTOWCPWriteSameEp}{110}
\newcommand{\lusearchFTOWCPWriteExclusive}{\cna}
\newcommand{\lusearchFTOWCPWriteOwned}{100}
\newcommand{\lusearchFTOWCPWriteShared}{<0.001}
\newcommand{\lusearchFTOWCPNoFPOtherEventTotal}{3816204}
\newcommand{\lusearchFTOWCPAcqRelOtherTotal}{69.6}
\newcommand{\lusearchFTOWCPNoAcqRelOtherTotal}{1158268}
\newcommand{\lusearchFTOWCPFork}{6.91E-4}
\newcommand{\lusearchFTOWCPJoin}{0.0}
\newcommand{\lusearchFTOWCPPreWait}{0.00553}
\newcommand{\lusearchFTOWCPPostWait}{0.00553}
\newcommand{\lusearchFTOWCPVolatileTotal}{100.0}
\newcommand{\lusearchFTOWCPClassInit}{0.00311}
\newcommand{\lusearchFTOWCPClassAccess}{0.0168}
\newcommand{\lusearchFTOWCPRaceTotal}{\rna}
\newcommand{\lusearchFTOWCPWrRdRace}{\rna}
\newcommand{\lusearchFTOWCPWrWrRace}{\rna}
\newcommand{\lusearchFTOWCPRdWrRace}{\rna}
\newcommand{\lusearchFTOWCPRdShWrRace}{\rna}
\newcommand{\lusearchFTOWCPHoldLocksTotal}{5.1}
\newcommand{\lusearchFTOWCPOneLockHeld}{3.79}
\newcommand{\lusearchFTOWCPTwoNestedLocks}{0.39}
\newcommand{\lusearchFTOWCPThreeNestedLocks}{<0.1}
\newcommand{\lusearchFTOWCPFourNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPFiveNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPSixNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPSevenNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPEightNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPNineNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPTenNestedLocks}{\cna}
\newcommand{\lusearchFTOWCPHundredNestedLocks}{\cna}
\newcommand{\lusearchREWCPEventTotal}{1,400}
\newcommand{\lusearchREWCPNoFPEventTotal}{140}
\newcommand{\lusearchREWCPNoFPAccessTotal}{130}
\newcommand{\lusearchREWCPNoFPOtherTotal}{3.8}
\newcommand{\lusearchREWCPReadTotal}{77.0}
\newcommand{\lusearchREWCPWriteTotal}{20.2}
\newcommand{\lusearchREWCPNoFPAccessInCS}{4.89}
\newcommand{\lusearchREWCPNoFPAccessOutCS}{95.1}
\newcommand{\lusearchREWCPAcqRelTotal}{6.23}
\newcommand{\lusearchREWCPOtherTotal}{2.72}
\newcommand{\lusearchREWCPNoFPReadTotal}{110}
\newcommand{\lusearchREWCPReadInCS}{3.94}
\newcommand{\lusearchREWCPReadOutCS}{104}
\newcommand{\lusearchREWCPReadSameEp}{7.45}
\newcommand{\lusearchREWCPReadSharedSameEp}{\cna}
\newcommand{\lusearchREWCPReadExclusive}{<0.001}
\newcommand{\lusearchREWCPReadOwned}{96.1}
\newcommand{\lusearchREWCPReadShare}{<0.001}
\newcommand{\lusearchREWCPReadShared}{<0.001}
\newcommand{\lusearchREWCPReadSharedOwned}{3.93}
\newcommand{\lusearchREWCPNoFPHonestWriteTotal}{28}
\newcommand{\lusearchREWCPWriteInCS}{10}
\newcommand{\lusearchREWCPWriteOutCS}{200}
\newcommand{\lusearchREWCPNoFPWriteTotal}{28}
\newcommand{\lusearchREWCPWriteSameEp}{110}
\newcommand{\lusearchREWCPWriteExclusive}{\cna}
\newcommand{\lusearchREWCPWriteOwned}{100}
\newcommand{\lusearchREWCPWriteShared}{<0.001}
\newcommand{\lusearchREWCPNoFPOtherEventTotal}{3816150}
\newcommand{\lusearchREWCPAcqRelOtherTotal}{69.6}
\newcommand{\lusearchREWCPNoAcqRelOtherTotal}{1158214}
\newcommand{\lusearchREWCPFork}{6.91E-4}
\newcommand{\lusearchREWCPJoin}{0.0}
\newcommand{\lusearchREWCPPreWait}{0.00544}
\newcommand{\lusearchREWCPPostWait}{0.00544}
\newcommand{\lusearchREWCPVolatileTotal}{100.0}
\newcommand{\lusearchREWCPClassInit}{0.00311}
\newcommand{\lusearchREWCPClassAccess}{0.0168}
\newcommand{\lusearchREWCPRaceTotal}{\rna}
\newcommand{\lusearchREWCPWrRdRace}{\rna}
\newcommand{\lusearchREWCPWrWrRace}{\rna}
\newcommand{\lusearchREWCPRdWrRace}{\rna}
\newcommand{\lusearchREWCPRdShWrRace}{\rna}
\newcommand{\lusearchREWCPHoldLocksTotal}{5.1}
\newcommand{\lusearchREWCPOneLockHeld}{3.79}
\newcommand{\lusearchREWCPTwoNestedLocks}{0.39}
\newcommand{\lusearchREWCPThreeNestedLocks}{<0.1}
\newcommand{\lusearchREWCPFourNestedLocks}{\cna}
\newcommand{\lusearchREWCPFiveNestedLocks}{\cna}
\newcommand{\lusearchREWCPSixNestedLocks}{\cna}
\newcommand{\lusearchREWCPSevenNestedLocks}{\cna}
\newcommand{\lusearchREWCPEightNestedLocks}{\cna}
\newcommand{\lusearchREWCPNineNestedLocks}{\cna}
\newcommand{\lusearchREWCPTenNestedLocks}{\cna}
\newcommand{\lusearchREWCPHundredNestedLocks}{\cna}
\newcommand{\lusearchDCEventTotal}{1,400}
\newcommand{\lusearchDCNoFPEventTotal}{160}
\newcommand{\lusearchDCNoFPAccessTotal}{150}
\newcommand{\lusearchDCNoFPOtherTotal}{3.8}
\newcommand{\lusearchDCReadTotal}{79.5}
\newcommand{\lusearchDCWriteTotal}{18.0}
\newcommand{\lusearchDCNoFPAccessInCS}{16.7}
\newcommand{\lusearchDCNoFPAccessOutCS}{83.3}
\newcommand{\lusearchDCAcqRelTotal}{5.52}
\newcommand{\lusearchDCOtherTotal}{2.41}
\newcommand{\lusearchDCNoFPReadTotal}{120}
\newcommand{\lusearchDCReadInCS}{3.72}
\newcommand{\lusearchDCReadOutCS}{103}
\newcommand{\lusearchDCReadSameEp}{6.44}
\newcommand{\lusearchDCReadSharedSameEp}{\cna}
\newcommand{\lusearchDCReadExclusive}{96.6}
\newcommand{\lusearchDCReadOwned}{\cna}
\newcommand{\lusearchDCReadShare}{<0.001}
\newcommand{\lusearchDCReadShared}{3.39}
\newcommand{\lusearchDCReadSharedOwned}{\cna}
\newcommand{\lusearchDCNoFPHonestWriteTotal}{28}
\newcommand{\lusearchDCWriteInCS}{10}
\newcommand{\lusearchDCWriteOutCS}{200}
\newcommand{\lusearchDCNoFPWriteTotal}{28}
\newcommand{\lusearchDCWriteSameEp}{110}
\newcommand{\lusearchDCWriteExclusive}{100}
\newcommand{\lusearchDCWriteOwned}{\cna}
\newcommand{\lusearchDCWriteShared}{<0.001}
\newcommand{\lusearchDCNoFPOtherEventTotal}{3816192}
\newcommand{\lusearchDCAcqRelOtherTotal}{69.6}
\newcommand{\lusearchDCNoAcqRelOtherTotal}{1158256}
\newcommand{\lusearchDCFork}{6.91E-4}
\newcommand{\lusearchDCJoin}{0.0}
\newcommand{\lusearchDCPreWait}{0.00553}
\newcommand{\lusearchDCPostWait}{0.00553}
\newcommand{\lusearchDCVolatileTotal}{100.0}
\newcommand{\lusearchDCClassInit}{0.00311}
\newcommand{\lusearchDCClassAccess}{0.0168}
\newcommand{\lusearchDCRaceTotal}{\rna}
\newcommand{\lusearchDCWrRdRace}{\rna}
\newcommand{\lusearchDCWrWrRace}{\rna}
\newcommand{\lusearchDCRdWrRace}{\rna}
\newcommand{\lusearchDCRdShWrRace}{\rna}
\newcommand{\lusearchDCHoldLocksTotal}{13}
\newcommand{\lusearchDCOneLockHeld}{8.51}
\newcommand{\lusearchDCTwoNestedLocks}{0.70}
\newcommand{\lusearchDCThreeNestedLocks}{<0.1}
\newcommand{\lusearchDCFourNestedLocks}{\cna}
\newcommand{\lusearchDCFiveNestedLocks}{\cna}
\newcommand{\lusearchDCSixNestedLocks}{\cna}
\newcommand{\lusearchDCSevenNestedLocks}{\cna}
\newcommand{\lusearchDCEightNestedLocks}{\cna}
\newcommand{\lusearchDCNineNestedLocks}{\cna}
\newcommand{\lusearchDCTenNestedLocks}{\cna}
\newcommand{\lusearchDCHundredNestedLocks}{\cna}
\newcommand{\lusearchFTODCEventTotal}{1,400}
\newcommand{\lusearchFTODCNoFPEventTotal}{140}
\newcommand{\lusearchFTODCNoFPAccessTotal}{130}
\newcommand{\lusearchFTODCNoFPOtherTotal}{3.8}
\newcommand{\lusearchFTODCReadTotal}{77.0}
\newcommand{\lusearchFTODCWriteTotal}{20.2}
\newcommand{\lusearchFTODCNoFPAccessInCS}{4.89}
\newcommand{\lusearchFTODCNoFPAccessOutCS}{95.1}
\newcommand{\lusearchFTODCAcqRelTotal}{6.23}
\newcommand{\lusearchFTODCOtherTotal}{2.72}
\newcommand{\lusearchFTODCNoFPReadTotal}{110}
\newcommand{\lusearchFTODCReadInCS}{3.94}
\newcommand{\lusearchFTODCReadOutCS}{104}
\newcommand{\lusearchFTODCReadSameEp}{7.45}
\newcommand{\lusearchFTODCReadSharedSameEp}{\cna}
\newcommand{\lusearchFTODCReadExclusive}{<0.001}
\newcommand{\lusearchFTODCReadOwned}{96.1}
\newcommand{\lusearchFTODCReadShare}{<0.001}
\newcommand{\lusearchFTODCReadShared}{<0.001}
\newcommand{\lusearchFTODCReadSharedOwned}{3.93}
\newcommand{\lusearchFTODCNoFPHonestWriteTotal}{28}
\newcommand{\lusearchFTODCWriteInCS}{10}
\newcommand{\lusearchFTODCWriteOutCS}{200}
\newcommand{\lusearchFTODCNoFPWriteTotal}{28}
\newcommand{\lusearchFTODCWriteSameEp}{110}
\newcommand{\lusearchFTODCWriteExclusive}{\cna}
\newcommand{\lusearchFTODCWriteOwned}{100}
\newcommand{\lusearchFTODCWriteShared}{<0.001}
\newcommand{\lusearchFTODCNoFPOtherEventTotal}{3816185}
\newcommand{\lusearchFTODCAcqRelOtherTotal}{69.6}
\newcommand{\lusearchFTODCNoAcqRelOtherTotal}{1158249}
\newcommand{\lusearchFTODCFork}{6.91E-4}
\newcommand{\lusearchFTODCJoin}{0.0}
\newcommand{\lusearchFTODCPreWait}{0.00553}
\newcommand{\lusearchFTODCPostWait}{0.00553}
\newcommand{\lusearchFTODCVolatileTotal}{100.0}
\newcommand{\lusearchFTODCClassInit}{0.00311}
\newcommand{\lusearchFTODCClassAccess}{0.0168}
\newcommand{\lusearchFTODCRaceTotal}{\rna}
\newcommand{\lusearchFTODCWrRdRace}{\rna}
\newcommand{\lusearchFTODCWrWrRace}{\rna}
\newcommand{\lusearchFTODCRdWrRace}{\rna}
\newcommand{\lusearchFTODCRdShWrRace}{\rna}
\newcommand{\lusearchFTODCHoldLocksTotal}{5.1}
\newcommand{\lusearchFTODCOneLockHeld}{3.79}
\newcommand{\lusearchFTODCTwoNestedLocks}{0.39}
\newcommand{\lusearchFTODCThreeNestedLocks}{<0.1}
\newcommand{\lusearchFTODCFourNestedLocks}{\cna}
\newcommand{\lusearchFTODCFiveNestedLocks}{\cna}
\newcommand{\lusearchFTODCSixNestedLocks}{\cna}
\newcommand{\lusearchFTODCSevenNestedLocks}{\cna}
\newcommand{\lusearchFTODCEightNestedLocks}{\cna}
\newcommand{\lusearchFTODCNineNestedLocks}{\cna}
\newcommand{\lusearchFTODCTenNestedLocks}{\cna}
\newcommand{\lusearchFTODCHundredNestedLocks}{\cna}
\newcommand{\lusearchREDCEventTotal}{1,400}
\newcommand{\lusearchREDCNoFPEventTotal}{140}
\newcommand{\lusearchREDCNoFPAccessTotal}{130}
\newcommand{\lusearchREDCNoFPOtherTotal}{3.8}
\newcommand{\lusearchREDCReadTotal}{77.0}
\newcommand{\lusearchREDCWriteTotal}{20.2}
\newcommand{\lusearchREDCNoFPAccessInCS}{4.89}
\newcommand{\lusearchREDCNoFPAccessOutCS}{95.1}
\newcommand{\lusearchREDCAcqRelTotal}{6.23}
\newcommand{\lusearchREDCOtherTotal}{2.72}
\newcommand{\lusearchREDCNoFPReadTotal}{110}
\newcommand{\lusearchREDCReadInCS}{3.94}
\newcommand{\lusearchREDCReadOutCS}{104}
\newcommand{\lusearchREDCReadSameEp}{7.45}
\newcommand{\lusearchREDCReadSharedSameEp}{\cna}
\newcommand{\lusearchREDCReadExclusive}{<0.001}
\newcommand{\lusearchREDCReadOwned}{96.1}
\newcommand{\lusearchREDCReadShare}{<0.001}
\newcommand{\lusearchREDCReadShared}{<0.001}
\newcommand{\lusearchREDCReadSharedOwned}{3.93}
\newcommand{\lusearchREDCNoFPHonestWriteTotal}{28}
\newcommand{\lusearchREDCWriteInCS}{10}
\newcommand{\lusearchREDCWriteOutCS}{200}
\newcommand{\lusearchREDCNoFPWriteTotal}{28}
\newcommand{\lusearchREDCWriteSameEp}{110}
\newcommand{\lusearchREDCWriteExclusive}{\cna}
\newcommand{\lusearchREDCWriteOwned}{100}
\newcommand{\lusearchREDCWriteShared}{<0.001}
\newcommand{\lusearchREDCNoFPOtherEventTotal}{3816157}
\newcommand{\lusearchREDCAcqRelOtherTotal}{69.6}
\newcommand{\lusearchREDCNoAcqRelOtherTotal}{1158221}
\newcommand{\lusearchREDCFork}{6.91E-4}
\newcommand{\lusearchREDCJoin}{0.0}
\newcommand{\lusearchREDCPreWait}{0.00553}
\newcommand{\lusearchREDCPostWait}{0.00553}
\newcommand{\lusearchREDCVolatileTotal}{100.0}
\newcommand{\lusearchREDCClassInit}{0.00311}
\newcommand{\lusearchREDCClassAccess}{0.0168}
\newcommand{\lusearchREDCRaceTotal}{\rna}
\newcommand{\lusearchREDCWrRdRace}{\rna}
\newcommand{\lusearchREDCWrWrRace}{\rna}
\newcommand{\lusearchREDCRdWrRace}{\rna}
\newcommand{\lusearchREDCRdShWrRace}{\rna}
\newcommand{\lusearchREDCHoldLocksTotal}{5.1}
\newcommand{\lusearchREDCOneLockHeld}{3.79}
\newcommand{\lusearchREDCTwoNestedLocks}{0.39}
\newcommand{\lusearchREDCThreeNestedLocks}{<0.1}
\newcommand{\lusearchREDCFourNestedLocks}{\cna}
\newcommand{\lusearchREDCFiveNestedLocks}{\cna}
\newcommand{\lusearchREDCSixNestedLocks}{\cna}
\newcommand{\lusearchREDCSevenNestedLocks}{\cna}
\newcommand{\lusearchREDCEightNestedLocks}{\cna}
\newcommand{\lusearchREDCNineNestedLocks}{\cna}
\newcommand{\lusearchREDCTenNestedLocks}{\cna}
\newcommand{\lusearchREDCHundredNestedLocks}{\cna}
\newcommand{\lusearchCAPOEventTotal}{1,400}
\newcommand{\lusearchCAPONoFPEventTotal}{160}
\newcommand{\lusearchCAPONoFPAccessTotal}{150}
\newcommand{\lusearchCAPONoFPOtherTotal}{3.8}
\newcommand{\lusearchCAPOReadTotal}{79.5}
\newcommand{\lusearchCAPOWriteTotal}{18.0}
\newcommand{\lusearchCAPONoFPAccessInCS}{16.7}
\newcommand{\lusearchCAPONoFPAccessOutCS}{83.3}
\newcommand{\lusearchCAPOAcqRelTotal}{5.52}
\newcommand{\lusearchCAPOOtherTotal}{2.41}
\newcommand{\lusearchCAPONoFPReadTotal}{120}
\newcommand{\lusearchCAPOReadInCS}{3.72}
\newcommand{\lusearchCAPOReadOutCS}{103}
\newcommand{\lusearchCAPOReadSameEp}{6.44}
\newcommand{\lusearchCAPOReadSharedSameEp}{\cna}
\newcommand{\lusearchCAPOReadExclusive}{96.6}
\newcommand{\lusearchCAPOReadOwned}{\cna}
\newcommand{\lusearchCAPOReadShare}{<0.001}
\newcommand{\lusearchCAPOReadShared}{3.39}
\newcommand{\lusearchCAPOReadSharedOwned}{\cna}
\newcommand{\lusearchCAPONoFPHonestWriteTotal}{28}
\newcommand{\lusearchCAPOWriteInCS}{10}
\newcommand{\lusearchCAPOWriteOutCS}{200}
\newcommand{\lusearchCAPONoFPWriteTotal}{28}
\newcommand{\lusearchCAPOWriteSameEp}{110}
\newcommand{\lusearchCAPOWriteExclusive}{100}
\newcommand{\lusearchCAPOWriteOwned}{\cna}
\newcommand{\lusearchCAPOWriteShared}{<0.001}
\newcommand{\lusearchCAPONoFPOtherEventTotal}{3816201}
\newcommand{\lusearchCAPOAcqRelOtherTotal}{69.6}
\newcommand{\lusearchCAPONoAcqRelOtherTotal}{1158265}
\newcommand{\lusearchCAPOFork}{6.91E-4}
\newcommand{\lusearchCAPOJoin}{0.0}
\newcommand{\lusearchCAPOPreWait}{0.00553}
\newcommand{\lusearchCAPOPostWait}{0.00553}
\newcommand{\lusearchCAPOVolatileTotal}{100.0}
\newcommand{\lusearchCAPOClassInit}{0.00311}
\newcommand{\lusearchCAPOClassAccess}{0.0168}
\newcommand{\lusearchCAPORaceTotal}{\rna}
\newcommand{\lusearchCAPOWrRdRace}{\rna}
\newcommand{\lusearchCAPOWrWrRace}{\rna}
\newcommand{\lusearchCAPORdWrRace}{\rna}
\newcommand{\lusearchCAPORdShWrRace}{\rna}
\newcommand{\lusearchCAPOHoldLocksTotal}{13}
\newcommand{\lusearchCAPOOneLockHeld}{8.51}
\newcommand{\lusearchCAPOTwoNestedLocks}{0.70}
\newcommand{\lusearchCAPOThreeNestedLocks}{<0.1}
\newcommand{\lusearchCAPOFourNestedLocks}{\cna}
\newcommand{\lusearchCAPOFiveNestedLocks}{\cna}
\newcommand{\lusearchCAPOSixNestedLocks}{\cna}
\newcommand{\lusearchCAPOSevenNestedLocks}{\cna}
\newcommand{\lusearchCAPOEightNestedLocks}{\cna}
\newcommand{\lusearchCAPONineNestedLocks}{\cna}
\newcommand{\lusearchCAPOTenNestedLocks}{\cna}
\newcommand{\lusearchCAPOHundredNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPOEventTotal}{1,400}
\newcommand{\lusearchFTOCAPONoFPEventTotal}{140}
\newcommand{\lusearchFTOCAPONoFPAccessTotal}{130}
\newcommand{\lusearchFTOCAPONoFPOtherTotal}{3.8}
\newcommand{\lusearchFTOCAPOReadTotal}{77.0}
\newcommand{\lusearchFTOCAPOWriteTotal}{20.2}
\newcommand{\lusearchFTOCAPONoFPAccessInCS}{4.89}
\newcommand{\lusearchFTOCAPONoFPAccessOutCS}{95.1}
\newcommand{\lusearchFTOCAPOAcqRelTotal}{6.23}
\newcommand{\lusearchFTOCAPOOtherTotal}{2.72}
\newcommand{\lusearchFTOCAPONoFPReadTotal}{110}
\newcommand{\lusearchFTOCAPOReadInCS}{3.94}
\newcommand{\lusearchFTOCAPOReadOutCS}{104}
\newcommand{\lusearchFTOCAPOReadSameEp}{7.45}
\newcommand{\lusearchFTOCAPOReadSharedSameEp}{\cna}
\newcommand{\lusearchFTOCAPOReadExclusive}{<0.001}
\newcommand{\lusearchFTOCAPOReadOwned}{96.1}
\newcommand{\lusearchFTOCAPOReadShare}{<0.001}
\newcommand{\lusearchFTOCAPOReadShared}{<0.001}
\newcommand{\lusearchFTOCAPOReadSharedOwned}{3.93}
\newcommand{\lusearchFTOCAPONoFPHonestWriteTotal}{28}
\newcommand{\lusearchFTOCAPOWriteInCS}{10}
\newcommand{\lusearchFTOCAPOWriteOutCS}{200}
\newcommand{\lusearchFTOCAPONoFPWriteTotal}{28}
\newcommand{\lusearchFTOCAPOWriteSameEp}{110}
\newcommand{\lusearchFTOCAPOWriteExclusive}{\cna}
\newcommand{\lusearchFTOCAPOWriteOwned}{100}
\newcommand{\lusearchFTOCAPOWriteShared}{<0.001}
\newcommand{\lusearchFTOCAPONoFPOtherEventTotal}{3816214}
\newcommand{\lusearchFTOCAPOAcqRelOtherTotal}{69.6}
\newcommand{\lusearchFTOCAPONoAcqRelOtherTotal}{1158278}
\newcommand{\lusearchFTOCAPOFork}{6.91E-4}
\newcommand{\lusearchFTOCAPOJoin}{0.0}
\newcommand{\lusearchFTOCAPOPreWait}{0.00553}
\newcommand{\lusearchFTOCAPOPostWait}{0.00553}
\newcommand{\lusearchFTOCAPOVolatileTotal}{100.0}
\newcommand{\lusearchFTOCAPOClassInit}{0.00311}
\newcommand{\lusearchFTOCAPOClassAccess}{0.0168}
\newcommand{\lusearchFTOCAPORaceTotal}{\rna}
\newcommand{\lusearchFTOCAPOWrRdRace}{\rna}
\newcommand{\lusearchFTOCAPOWrWrRace}{\rna}
\newcommand{\lusearchFTOCAPORdWrRace}{\rna}
\newcommand{\lusearchFTOCAPORdShWrRace}{\rna}
\newcommand{\lusearchFTOCAPOHoldLocksTotal}{5.1}
\newcommand{\lusearchFTOCAPOOneLockHeld}{3.79}
\newcommand{\lusearchFTOCAPOTwoNestedLocks}{0.39}
\newcommand{\lusearchFTOCAPOThreeNestedLocks}{<0.1}
\newcommand{\lusearchFTOCAPOFourNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPOSixNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPOEightNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPONineNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPOTenNestedLocks}{\cna}
\newcommand{\lusearchFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\lusearchRECAPOEventTotal}{1,400}
\newcommand{\lusearchRECAPONoFPEventTotal}{140}
\newcommand{\lusearchRECAPONoFPAccessTotal}{130}
\newcommand{\lusearchRECAPONoFPOtherTotal}{3.8}
\newcommand{\lusearchRECAPOReadTotal}{77.0}
\newcommand{\lusearchRECAPOWriteTotal}{20.2}
\newcommand{\lusearchRECAPONoFPAccessInCS}{4.89}
\newcommand{\lusearchRECAPONoFPAccessOutCS}{95.1}
\newcommand{\lusearchRECAPOAcqRelTotal}{6.23}
\newcommand{\lusearchRECAPOOtherTotal}{2.72}
\newcommand{\lusearchRECAPONoFPReadTotal}{110}
\newcommand{\lusearchRECAPOReadInCS}{3.94}
\newcommand{\lusearchRECAPOReadOutCS}{104}
\newcommand{\lusearchRECAPOReadSameEp}{7.45}
\newcommand{\lusearchRECAPOReadSharedSameEp}{\cna}
\newcommand{\lusearchRECAPOReadExclusive}{<0.001}
\newcommand{\lusearchRECAPOReadOwned}{96.1}
\newcommand{\lusearchRECAPOReadShare}{<0.001}
\newcommand{\lusearchRECAPOReadShared}{<0.001}
\newcommand{\lusearchRECAPOReadSharedOwned}{3.93}
\newcommand{\lusearchRECAPONoFPHonestWriteTotal}{28}
\newcommand{\lusearchRECAPOWriteInCS}{10}
\newcommand{\lusearchRECAPOWriteOutCS}{200}
\newcommand{\lusearchRECAPONoFPWriteTotal}{28}
\newcommand{\lusearchRECAPOWriteSameEp}{110}
\newcommand{\lusearchRECAPOWriteExclusive}{\cna}
\newcommand{\lusearchRECAPOWriteOwned}{100}
\newcommand{\lusearchRECAPOWriteShared}{<0.001}
\newcommand{\lusearchRECAPONoFPOtherEventTotal}{3816194}
\newcommand{\lusearchRECAPOAcqRelOtherTotal}{69.6}
\newcommand{\lusearchRECAPONoAcqRelOtherTotal}{1158258}
\newcommand{\lusearchRECAPOFork}{6.91E-4}
\newcommand{\lusearchRECAPOJoin}{0.0}
\newcommand{\lusearchRECAPOPreWait}{0.00553}
\newcommand{\lusearchRECAPOPostWait}{0.00553}
\newcommand{\lusearchRECAPOVolatileTotal}{100.0}
\newcommand{\lusearchRECAPOClassInit}{0.00311}
\newcommand{\lusearchRECAPOClassAccess}{0.0168}
\newcommand{\lusearchRECAPORaceTotal}{\rna}
\newcommand{\lusearchRECAPOWrRdRace}{\rna}
\newcommand{\lusearchRECAPOWrWrRace}{\rna}
\newcommand{\lusearchRECAPORdWrRace}{\rna}
\newcommand{\lusearchRECAPORdShWrRace}{\rna}
\newcommand{\lusearchRECAPOHoldLocksTotal}{5.1}
\newcommand{\lusearchRECAPOOneLockHeld}{3.79}
\newcommand{\lusearchRECAPOTwoNestedLocks}{0.39}
\newcommand{\lusearchRECAPOThreeNestedLocks}{<0.1}
\newcommand{\lusearchRECAPOFourNestedLocks}{\cna}
\newcommand{\lusearchRECAPOFiveNestedLocks}{\cna}
\newcommand{\lusearchRECAPOSixNestedLocks}{\cna}
\newcommand{\lusearchRECAPOSevenNestedLocks}{\cna}
\newcommand{\lusearchRECAPOEightNestedLocks}{\cna}
\newcommand{\lusearchRECAPONineNestedLocks}{\cna}
\newcommand{\lusearchRECAPOTenNestedLocks}{\cna}
\newcommand{\lusearchRECAPOHundredNestedLocks}{\cna}
\newcommand{\lusearchCAPOTotalSetClears}{1.3}
\newcommand{\lusearchCAPOReadSetZero}{0.00474}
\newcommand{\lusearchCAPOReadSetOne}{59.2}
\newcommand{\lusearchCAPOReadSetGtOne}{40.8}
\newcommand{\lusearchCAPOWriteSetZero}{78.9}
\newcommand{\lusearchCAPOWriteSetOne}{17.1}
\newcommand{\lusearchCAPOWriteSetGtOne}{4.06}
\newcommand{\lusearchCAPOTotalMapClears}{1.3}
\newcommand{\lusearchCAPOReadMapZero}{0.0}
\newcommand{\lusearchCAPOReadMapOne}{0.0145}
\newcommand{\lusearchCAPOReadMapTen}{9.37}
\newcommand{\lusearchCAPOReadMapHund}{25.5}
\newcommand{\lusearchCAPOReadMapThou}{13.6}
\newcommand{\lusearchCAPOReadMapGtThou}{51.5}
\newcommand{\lusearchCAPOWriteMapZero}{0.00497}
\newcommand{\lusearchCAPOWriteMapOne}{17.0}
\newcommand{\lusearchCAPOWriteMapTen}{19.9}
\newcommand{\lusearchCAPOWriteMapHund}{0.291}
\newcommand{\lusearchCAPOWriteMapThou}{1.77}
\newcommand{\lusearchCAPOWriteMapGtThou}{61.0}
\newcommand{\FASTlusearchMaxLiveThreads}{10}
\newcommand{\FASTlusearchTotalThreads}{10}
\newcommand{\FASTlusearchBaseTime}{0.98}
\newcommand{\FASTlusearchBaseTimeCI}{34}
\newcommand{\FASTlusearchEmptyTime}{\rna}
\newcommand{\FASTlusearchEmptyTimeCI}{\rna}
\newcommand{\FASTlusearchEmptyTimeCIMIN}{\rna}
\newcommand{\FASTlusearchEmptyTimeCIMAX}{\rna}
\newcommand{\FASTlusearchFTTime}{12}
\newcommand{\FASTlusearchFTTimeCI}{0.46}
\newcommand{\FASTlusearchHBTime}{12}
\newcommand{\FASTlusearchHBTimeCI}{0.56}
\newcommand{\FASTlusearchFTOHBTime}{12}
\newcommand{\FASTlusearchFTOHBTimeCI}{0.69}
\newcommand{\FASTlusearchWCPTime}{15}
\newcommand{\FASTlusearchWCPTimeCI}{0.56}
\newcommand{\FASTlusearchFTOWCPTime}{15}
\newcommand{\FASTlusearchFTOWCPTimeCI}{0.58}
\newcommand{\FASTlusearchREWCPTime}{15}
\newcommand{\FASTlusearchREWCPTimeCI}{0.6}
\newcommand{\FASTlusearchDCTime}{15}
\newcommand{\FASTlusearchDCTimeCI}{0.43}
\newcommand{\FASTlusearchFTODCTime}{15}
\newcommand{\FASTlusearchFTODCTimeCI}{0.58}
\newcommand{\FASTlusearchREDCTime}{15}
\newcommand{\FASTlusearchREDCTimeCI}{0.55}
\newcommand{\FASTlusearchCAPOTime}{13}
\newcommand{\FASTlusearchCAPOTimeCI}{0.42}
\newcommand{\FASTlusearchFTOCAPOTime}{14}
\newcommand{\FASTlusearchFTOCAPOTimeCI}{0.59}
\newcommand{\FASTlusearchRECAPOTime}{14}
\newcommand{\FASTlusearchRECAPOTimeCI}{0.69}
\newcommand{\FASTlusearchAGGCAPOTime}{\rna}
\newcommand{\FASTlusearchAGGCAPOTimeCI}{\rna}
\newcommand{\FASTlusearchAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTlusearchAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTlusearchStaticTime}{\rzero}
\newcommand{\FASTlusearchDynamicTime}{\rzero}
\newcommand{\FASTlusearchBaseMem}{1,600}
\newcommand{\FASTlusearchBaseMemCI}{9.2}
\newcommand{\FASTlusearchFTMem}{8.8}
\newcommand{\FASTlusearchFTMemCI}{0.23}
\newcommand{\FASTlusearchHBMem}{8.8}
\newcommand{\FASTlusearchHBMemCI}{0.37}
\newcommand{\FASTlusearchFTOHBMem}{8.1}
\newcommand{\FASTlusearchFTOHBMemCI}{0.32}
\newcommand{\FASTlusearchWCPMem}{9.4}
\newcommand{\FASTlusearchWCPMemCI}{0.31}
\newcommand{\FASTlusearchFTOWCPMem}{9.4}
\newcommand{\FASTlusearchFTOWCPMemCI}{0.36}
\newcommand{\FASTlusearchREWCPMem}{10}
\newcommand{\FASTlusearchREWCPMemCI}{0.17}
\newcommand{\FASTlusearchDCMem}{9.4}
\newcommand{\FASTlusearchDCMemCI}{0.35}
\newcommand{\FASTlusearchFTODCMem}{9.4}
\newcommand{\FASTlusearchFTODCMemCI}{0.28}
\newcommand{\FASTlusearchREDCMem}{10}
\newcommand{\FASTlusearchREDCMemCI}{0.37}
\newcommand{\FASTlusearchCAPOMem}{8.8}
\newcommand{\FASTlusearchCAPOMemCI}{0.25}
\newcommand{\FASTlusearchFTOCAPOMem}{9.4}
\newcommand{\FASTlusearchFTOCAPOMemCI}{0.13}
\newcommand{\FASTlusearchRECAPOMem}{9.4}
\newcommand{\FASTlusearchRECAPOMemCI}{0.13}
\newcommand{\FASTlusearchAGGCAPOMem}{\memna}
\newcommand{\FASTlusearchAGGCAPOMemCI}{\memna}
\newcommand{\FASTlusearchAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTlusearchAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTlusearchEventsCI}{18}
\newcommand{\FASTlusearchEventsCIMIN}{1,443,227,220}
\newcommand{\FASTlusearchEventsCIMAX}{1,443,227,256}
\newcommand{\FASTlusearchNoFPEventsCI}{19}
\newcommand{\FASTlusearchNoFPEventsCIMIN}{42,639,706}
\newcommand{\FASTlusearchNoFPEventsCIMAX}{42,639,744}
\newcommand{\FASTlusearchFT}{0}
\newcommand{\FASTlusearchFTCI}{0}
\newcommand{\FASTlusearchFTCIMIN}{0}
\newcommand{\FASTlusearchFTCIMAX}{0}
\newcommand{\FASTlusearchFTDynamic}{0}
\newcommand{\FASTlusearchFTDynamicCI}{0}
\newcommand{\FASTlusearchFTDynamicCIMIN}{0}
\newcommand{\FASTlusearchFTDynamicCIMAX}{0}
\newcommand{\FASTlusearchHB}{0}
\newcommand{\FASTlusearchHBCI}{0}
\newcommand{\FASTlusearchHBCIMIN}{0}
\newcommand{\FASTlusearchHBCIMAX}{0}
\newcommand{\FASTlusearchHBDynamic}{0}
\newcommand{\FASTlusearchHBDynamicCI}{0}
\newcommand{\FASTlusearchHBDynamicCIMIN}{0}
\newcommand{\FASTlusearchHBDynamicCIMAX}{0}
\newcommand{\FASTlusearchFTOHB}{0}
\newcommand{\FASTlusearchFTOHBCI}{0}
\newcommand{\FASTlusearchFTOHBCIMIN}{0}
\newcommand{\FASTlusearchFTOHBCIMAX}{0}
\newcommand{\FASTlusearchFTOHBDynamic}{0}
\newcommand{\FASTlusearchFTOHBDynamicCI}{0}
\newcommand{\FASTlusearchFTOHBDynamicCIMIN}{0}
\newcommand{\FASTlusearchFTOHBDynamicCIMAX}{0}
\newcommand{\FASTlusearchWCP}{0}
\newcommand{\FASTlusearchWCPCI}{0}
\newcommand{\FASTlusearchWCPCIMIN}{0}
\newcommand{\FASTlusearchWCPCIMAX}{0}
\newcommand{\FASTlusearchWCPDynamic}{0}
\newcommand{\FASTlusearchWCPDynamicCI}{0}
\newcommand{\FASTlusearchWCPDynamicCIMIN}{0}
\newcommand{\FASTlusearchWCPDynamicCIMAX}{0}
\newcommand{\FASTlusearchFTOWCP}{0}
\newcommand{\FASTlusearchFTOWCPCI}{0}
\newcommand{\FASTlusearchFTOWCPCIMIN}{0}
\newcommand{\FASTlusearchFTOWCPCIMAX}{0}
\newcommand{\FASTlusearchFTOWCPDynamic}{0}
\newcommand{\FASTlusearchFTOWCPDynamicCI}{0}
\newcommand{\FASTlusearchFTOWCPDynamicCIMIN}{0}
\newcommand{\FASTlusearchFTOWCPDynamicCIMAX}{0}
\newcommand{\FASTlusearchREWCP}{0}
\newcommand{\FASTlusearchREWCPCI}{0}
\newcommand{\FASTlusearchREWCPCIMIN}{0}
\newcommand{\FASTlusearchREWCPCIMAX}{0}
\newcommand{\FASTlusearchREWCPDynamic}{0}
\newcommand{\FASTlusearchREWCPDynamicCI}{0}
\newcommand{\FASTlusearchREWCPDynamicCIMIN}{0}
\newcommand{\FASTlusearchREWCPDynamicCIMAX}{0}
\newcommand{\FASTlusearchDC}{0}
\newcommand{\FASTlusearchDCCI}{0}
\newcommand{\FASTlusearchDCCIMIN}{0}
\newcommand{\FASTlusearchDCCIMAX}{0}
\newcommand{\FASTlusearchDCDynamic}{0}
\newcommand{\FASTlusearchDCDynamicCI}{0}
\newcommand{\FASTlusearchDCDynamicCIMIN}{0}
\newcommand{\FASTlusearchDCDynamicCIMAX}{0}
\newcommand{\FASTlusearchFTODC}{0}
\newcommand{\FASTlusearchFTODCCI}{0}
\newcommand{\FASTlusearchFTODCCIMIN}{0}
\newcommand{\FASTlusearchFTODCCIMAX}{0}
\newcommand{\FASTlusearchFTODCDynamic}{0}
\newcommand{\FASTlusearchFTODCDynamicCI}{0}
\newcommand{\FASTlusearchFTODCDynamicCIMIN}{0}
\newcommand{\FASTlusearchFTODCDynamicCIMAX}{0}
\newcommand{\FASTlusearchREDC}{0}
\newcommand{\FASTlusearchREDCCI}{0}
\newcommand{\FASTlusearchREDCCIMIN}{0}
\newcommand{\FASTlusearchREDCCIMAX}{0}
\newcommand{\FASTlusearchREDCDynamic}{0}
\newcommand{\FASTlusearchREDCDynamicCI}{0}
\newcommand{\FASTlusearchREDCDynamicCIMIN}{0}
\newcommand{\FASTlusearchREDCDynamicCIMAX}{0}
\newcommand{\FASTlusearchCAPO}{0}
\newcommand{\FASTlusearchCAPOCI}{0}
\newcommand{\FASTlusearchCAPOCIMIN}{0}
\newcommand{\FASTlusearchCAPOCIMAX}{0}
\newcommand{\FASTlusearchCAPODynamic}{0}
\newcommand{\FASTlusearchCAPODynamicCI}{0}
\newcommand{\FASTlusearchCAPODynamicCIMIN}{0}
\newcommand{\FASTlusearchCAPODynamicCIMAX}{0}
\newcommand{\FASTlusearchFTOCAPO}{0}
\newcommand{\FASTlusearchFTOCAPOCI}{0}
\newcommand{\FASTlusearchFTOCAPOCIMIN}{0}
\newcommand{\FASTlusearchFTOCAPOCIMAX}{0}
\newcommand{\FASTlusearchFTOCAPODynamic}{0}
\newcommand{\FASTlusearchFTOCAPODynamicCI}{0}
\newcommand{\FASTlusearchFTOCAPODynamicCIMIN}{0}
\newcommand{\FASTlusearchFTOCAPODynamicCIMAX}{0}
\newcommand{\FASTlusearchRECAPO}{0}
\newcommand{\FASTlusearchRECAPOCI}{0}
\newcommand{\FASTlusearchRECAPOCIMIN}{0}
\newcommand{\FASTlusearchRECAPOCIMAX}{0}
\newcommand{\FASTlusearchRECAPODynamic}{0}
\newcommand{\FASTlusearchRECAPODynamicCI}{0}
\newcommand{\FASTlusearchRECAPODynamicCIMIN}{0}
\newcommand{\FASTlusearchRECAPODynamicCIMAX}{0}
\newcommand{\FASTlusearchAGGCAPO}{\rna}
\newcommand{\FASTlusearchAGGCAPOCI}{\rna}
\newcommand{\FASTlusearchAGGCAPOCIMIN}{\rna}
\newcommand{\FASTlusearchAGGCAPOCIMAX}{\rna}
\newcommand{\FASTlusearchAGGCAPODynamic}{\rna}
\newcommand{\FASTlusearchAGGCAPODynamicCI}{\rna}
\newcommand{\FASTlusearchAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTlusearchAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTpmdEvents}{200}
\newcommand{\FASTpmdNoFPEvents}{13}
\newcommand{\pmdHBEventTotal}{200}
\newcommand{\pmdHBNoFPEventTotal}{13}
\newcommand{\pmdHBNoFPAccessTotal}{13}
\newcommand{\pmdHBNoFPOtherTotal}{<0.1}
\newcommand{\pmdHBReadTotal}{95.9}
\newcommand{\pmdHBWriteTotal}{3.91}
\newcommand{\pmdHBNoFPAccessInCS}{10.5}
\newcommand{\pmdHBNoFPAccessOutCS}{89.5}
\newcommand{\pmdHBAcqRelTotal}{0.137}
\newcommand{\pmdHBOtherTotal}{0.00357}
\newcommand{\pmdHBNoFPReadTotal}{12}
\newcommand{\pmdHBReadInCS}{11.1}
\newcommand{\pmdHBReadOutCS}{110}
\newcommand{\pmdHBReadSameEp}{20.7}
\newcommand{\pmdHBReadSharedSameEp}{\cna}
\newcommand{\pmdHBReadExclusive}{99.1}
\newcommand{\pmdHBReadOwned}{\cna}
\newcommand{\pmdHBReadShare}{0.00787}
\newcommand{\pmdHBReadShared}{0.938}
\newcommand{\pmdHBReadSharedOwned}{\cna}
\newcommand{\pmdHBNoFPHonestWriteTotal}{0.49}
\newcommand{\pmdHBWriteInCS}{29.2}
\newcommand{\pmdHBWriteOutCS}{2170}
\newcommand{\pmdHBNoFPWriteTotal}{0.49}
\newcommand{\pmdHBWriteSameEp}{2100}
\newcommand{\pmdHBWriteExclusive}{100}
\newcommand{\pmdHBWriteOwned}{\cna}
\newcommand{\pmdHBWriteShared}{\cna}
\newcommand{\pmdHBNoFPOtherEventTotal}{18037}
\newcommand{\pmdHBAcqRelOtherTotal}{97.5}
\newcommand{\pmdHBNoAcqRelOtherTotal}{459}
\newcommand{\pmdHBFork}{0.0}
\newcommand{\pmdHBJoin}{0.0}
\newcommand{\pmdHBPreWait}{0.0}
\newcommand{\pmdHBPostWait}{0.0}
\newcommand{\pmdHBVolatileTotal}{0.0}
\newcommand{\pmdHBClassInit}{12.4}
\newcommand{\pmdHBClassAccess}{87.6}
\newcommand{\pmdHBRaceTotal}{3889}
\newcommand{\pmdHBWrRdRace}{99.5}
\newcommand{\pmdHBWrWrRace}{0.489}
\newcommand{\pmdHBRdWrRace}{0.0}
\newcommand{\pmdHBRdShWrRace}{0.0}
\newcommand{\pmdHBHoldLocksTotal}{1.5}
\newcommand{\pmdHBOneLockHeld}{11.8}
\newcommand{\pmdHBTwoNestedLocks}{\cna}
\newcommand{\pmdHBThreeNestedLocks}{\cna}
\newcommand{\pmdHBFourNestedLocks}{\cna}
\newcommand{\pmdHBFiveNestedLocks}{\cna}
\newcommand{\pmdHBSixNestedLocks}{\cna}
\newcommand{\pmdHBSevenNestedLocks}{\cna}
\newcommand{\pmdHBEightNestedLocks}{\cna}
\newcommand{\pmdHBNineNestedLocks}{\cna}
\newcommand{\pmdHBTenNestedLocks}{\cna}
\newcommand{\pmdHBHundredNestedLocks}{\cna}
\newcommand{\pmdFTOHBEventTotal}{200}
\newcommand{\pmdFTOHBNoFPEventTotal}{7.9}
\newcommand{\pmdFTOHBNoFPAccessTotal}{7.9}
\newcommand{\pmdFTOHBNoFPOtherTotal}{<0.1}
\newcommand{\pmdFTOHBReadTotal}{93.5}
\newcommand{\pmdFTOHBWriteTotal}{6.23}
\newcommand{\pmdFTOHBNoFPAccessInCS}{10.5}
\newcommand{\pmdFTOHBNoFPAccessOutCS}{89.5}
\newcommand{\pmdFTOHBAcqRelTotal}{0.137}
\newcommand{\pmdFTOHBOtherTotal}{0.00357}
\newcommand{\pmdFTOHBNoFPReadTotal}{7.4}
\newcommand{\pmdFTOHBReadInCS}{17.5}
\newcommand{\pmdFTOHBReadOutCS}{116}
\newcommand{\pmdFTOHBReadSameEp}{33.9}
\newcommand{\pmdFTOHBReadSharedSameEp}{\cna}
\newcommand{\pmdFTOHBReadExclusive}{0.286}
\newcommand{\pmdFTOHBReadOwned}{98.1}
\newcommand{\pmdFTOHBReadShare}{0.0131}
\newcommand{\pmdFTOHBReadShared}{0.0748}
\newcommand{\pmdFTOHBReadSharedOwned}{1.48}
\newcommand{\pmdFTOHBNoFPHonestWriteTotal}{0.49}
\newcommand{\pmdFTOHBWriteInCS}{29.2}
\newcommand{\pmdFTOHBWriteOutCS}{2170}
\newcommand{\pmdFTOHBNoFPWriteTotal}{0.49}
\newcommand{\pmdFTOHBWriteSameEp}{2100}
\newcommand{\pmdFTOHBWriteExclusive}{0.00163}
\newcommand{\pmdFTOHBWriteOwned}{100}
\newcommand{\pmdFTOHBWriteShared}{\cna}
\newcommand{\pmdFTOHBNoFPOtherEventTotal}{18036}
\newcommand{\pmdFTOHBAcqRelOtherTotal}{97.5}
\newcommand{\pmdFTOHBNoAcqRelOtherTotal}{458}
\newcommand{\pmdFTOHBFork}{0.0}
\newcommand{\pmdFTOHBJoin}{0.0}
\newcommand{\pmdFTOHBPreWait}{0.0}
\newcommand{\pmdFTOHBPostWait}{0.0}
\newcommand{\pmdFTOHBVolatileTotal}{0.0}
\newcommand{\pmdFTOHBClassInit}{12.4}
\newcommand{\pmdFTOHBClassAccess}{87.6}
\newcommand{\pmdFTOHBRaceTotal}{3969}
\newcommand{\pmdFTOHBWrRdRace}{99.6}
\newcommand{\pmdFTOHBWrWrRace}{0.0}
\newcommand{\pmdFTOHBRdWrRace}{0.428}
\newcommand{\pmdFTOHBRdShWrRace}{0.0}
\newcommand{\pmdFTOHBHoldLocksTotal}{0.093}
\newcommand{\pmdFTOHBOneLockHeld}{1.12}
\newcommand{\pmdFTOHBTwoNestedLocks}{\cna}
\newcommand{\pmdFTOHBThreeNestedLocks}{\cna}
\newcommand{\pmdFTOHBFourNestedLocks}{\cna}
\newcommand{\pmdFTOHBFiveNestedLocks}{\cna}
\newcommand{\pmdFTOHBSixNestedLocks}{\cna}
\newcommand{\pmdFTOHBSevenNestedLocks}{\cna}
\newcommand{\pmdFTOHBEightNestedLocks}{\cna}
\newcommand{\pmdFTOHBNineNestedLocks}{\cna}
\newcommand{\pmdFTOHBTenNestedLocks}{\cna}
\newcommand{\pmdFTOHBHundredNestedLocks}{\cna}
\newcommand{\pmdWCPEventTotal}{200}
\newcommand{\pmdWCPNoFPEventTotal}{13}
\newcommand{\pmdWCPNoFPAccessTotal}{13}
\newcommand{\pmdWCPNoFPOtherTotal}{<0.1}
\newcommand{\pmdWCPReadTotal}{95.9}
\newcommand{\pmdWCPWriteTotal}{3.91}
\newcommand{\pmdWCPNoFPAccessInCS}{11.5}
\newcommand{\pmdWCPNoFPAccessOutCS}{88.5}
\newcommand{\pmdWCPAcqRelTotal}{0.135}
\newcommand{\pmdWCPOtherTotal}{0.00353}
\newcommand{\pmdWCPNoFPReadTotal}{12}
\newcommand{\pmdWCPReadInCS}{11.1}
\newcommand{\pmdWCPReadOutCS}{110}
\newcommand{\pmdWCPReadSameEp}{20.7}
\newcommand{\pmdWCPReadSharedSameEp}{\cna}
\newcommand{\pmdWCPReadExclusive}{99}
\newcommand{\pmdWCPReadOwned}{\cna}
\newcommand{\pmdWCPReadShare}{0.00828}
\newcommand{\pmdWCPReadShared}{1.02}
\newcommand{\pmdWCPReadSharedOwned}{\cna}
\newcommand{\pmdWCPNoFPHonestWriteTotal}{0.49}
\newcommand{\pmdWCPWriteInCS}{29.2}
\newcommand{\pmdWCPWriteOutCS}{2170}
\newcommand{\pmdWCPNoFPWriteTotal}{0.49}
\newcommand{\pmdWCPWriteSameEp}{2100}
\newcommand{\pmdWCPWriteExclusive}{100}
\newcommand{\pmdWCPWriteOwned}{\cna}
\newcommand{\pmdWCPWriteShared}{\cna}
\newcommand{\pmdWCPNoFPOtherEventTotal}{18037}
\newcommand{\pmdWCPAcqRelOtherTotal}{97.5}
\newcommand{\pmdWCPNoAcqRelOtherTotal}{459}
\newcommand{\pmdWCPFork}{0.0}
\newcommand{\pmdWCPJoin}{0.0}
\newcommand{\pmdWCPPreWait}{0.0}
\newcommand{\pmdWCPPostWait}{0.0}
\newcommand{\pmdWCPVolatileTotal}{0.0}
\newcommand{\pmdWCPClassInit}{12.4}
\newcommand{\pmdWCPClassAccess}{87.6}
\newcommand{\pmdWCPRaceTotal}{5243}
\newcommand{\pmdWCPWrRdRace}{99.7}
\newcommand{\pmdWCPWrWrRace}{0.343}
\newcommand{\pmdWCPRdWrRace}{0.0}
\newcommand{\pmdWCPRdShWrRace}{0.0}
\newcommand{\pmdWCPHoldLocksTotal}{1.6}
\newcommand{\pmdWCPOneLockHeld}{12.9}
\newcommand{\pmdWCPTwoNestedLocks}{\cna}
\newcommand{\pmdWCPThreeNestedLocks}{\cna}
\newcommand{\pmdWCPFourNestedLocks}{\cna}
\newcommand{\pmdWCPFiveNestedLocks}{\cna}
\newcommand{\pmdWCPSixNestedLocks}{\cna}
\newcommand{\pmdWCPSevenNestedLocks}{\cna}
\newcommand{\pmdWCPEightNestedLocks}{\cna}
\newcommand{\pmdWCPNineNestedLocks}{\cna}
\newcommand{\pmdWCPTenNestedLocks}{\cna}
\newcommand{\pmdWCPHundredNestedLocks}{\cna}
\newcommand{\pmdFTOWCPEventTotal}{200}
\newcommand{\pmdFTOWCPNoFPEventTotal}{7.9}
\newcommand{\pmdFTOWCPNoFPAccessTotal}{7.9}
\newcommand{\pmdFTOWCPNoFPOtherTotal}{<0.1}
\newcommand{\pmdFTOWCPReadTotal}{93.5}
\newcommand{\pmdFTOWCPWriteTotal}{6.23}
\newcommand{\pmdFTOWCPNoFPAccessInCS}{10.5}
\newcommand{\pmdFTOWCPNoFPAccessOutCS}{89.5}
\newcommand{\pmdFTOWCPAcqRelTotal}{0.137}
\newcommand{\pmdFTOWCPOtherTotal}{0.00357}
\newcommand{\pmdFTOWCPNoFPReadTotal}{7.4}
\newcommand{\pmdFTOWCPReadInCS}{17.5}
\newcommand{\pmdFTOWCPReadOutCS}{116}
\newcommand{\pmdFTOWCPReadSameEp}{33.9}
\newcommand{\pmdFTOWCPReadSharedSameEp}{\cna}
\newcommand{\pmdFTOWCPReadExclusive}{0.244}
\newcommand{\pmdFTOWCPReadOwned}{98.1}
\newcommand{\pmdFTOWCPReadShare}{0.0135}
\newcommand{\pmdFTOWCPReadShared}{0.0763}
\newcommand{\pmdFTOWCPReadSharedOwned}{1.6}
\newcommand{\pmdFTOWCPNoFPHonestWriteTotal}{0.49}
\newcommand{\pmdFTOWCPWriteInCS}{29.2}
\newcommand{\pmdFTOWCPWriteOutCS}{2170}
\newcommand{\pmdFTOWCPNoFPWriteTotal}{0.49}
\newcommand{\pmdFTOWCPWriteSameEp}{2100}
\newcommand{\pmdFTOWCPWriteExclusive}{0.00163}
\newcommand{\pmdFTOWCPWriteOwned}{100}
\newcommand{\pmdFTOWCPWriteShared}{\cna}
\newcommand{\pmdFTOWCPNoFPOtherEventTotal}{18037}
\newcommand{\pmdFTOWCPAcqRelOtherTotal}{97.5}
\newcommand{\pmdFTOWCPNoAcqRelOtherTotal}{459}
\newcommand{\pmdFTOWCPFork}{0.0}
\newcommand{\pmdFTOWCPJoin}{0.0}
\newcommand{\pmdFTOWCPPreWait}{0.0}
\newcommand{\pmdFTOWCPPostWait}{0.0}
\newcommand{\pmdFTOWCPVolatileTotal}{0.0}
\newcommand{\pmdFTOWCPClassInit}{12.4}
\newcommand{\pmdFTOWCPClassAccess}{87.6}
\newcommand{\pmdFTOWCPRaceTotal}{3884}
\newcommand{\pmdFTOWCPWrRdRace}{99.5}
\newcommand{\pmdFTOWCPWrWrRace}{0.0}
\newcommand{\pmdFTOWCPRdWrRace}{0.489}
\newcommand{\pmdFTOWCPRdShWrRace}{0.0}
\newcommand{\pmdFTOWCPHoldLocksTotal}{0.093}
\newcommand{\pmdFTOWCPOneLockHeld}{1.12}
\newcommand{\pmdFTOWCPTwoNestedLocks}{\cna}
\newcommand{\pmdFTOWCPThreeNestedLocks}{\cna}
\newcommand{\pmdFTOWCPFourNestedLocks}{\cna}
\newcommand{\pmdFTOWCPFiveNestedLocks}{\cna}
\newcommand{\pmdFTOWCPSixNestedLocks}{\cna}
\newcommand{\pmdFTOWCPSevenNestedLocks}{\cna}
\newcommand{\pmdFTOWCPEightNestedLocks}{\cna}
\newcommand{\pmdFTOWCPNineNestedLocks}{\cna}
\newcommand{\pmdFTOWCPTenNestedLocks}{\cna}
\newcommand{\pmdFTOWCPHundredNestedLocks}{\cna}
\newcommand{\pmdREWCPEventTotal}{200}
\newcommand{\pmdREWCPNoFPEventTotal}{7.9}
\newcommand{\pmdREWCPNoFPAccessTotal}{7.9}
\newcommand{\pmdREWCPNoFPOtherTotal}{<0.1}
\newcommand{\pmdREWCPReadTotal}{93.5}
\newcommand{\pmdREWCPWriteTotal}{6.23}
\newcommand{\pmdREWCPNoFPAccessInCS}{10.5}
\newcommand{\pmdREWCPNoFPAccessOutCS}{89.5}
\newcommand{\pmdREWCPAcqRelTotal}{0.137}
\newcommand{\pmdREWCPOtherTotal}{0.00357}
\newcommand{\pmdREWCPNoFPReadTotal}{7.4}
\newcommand{\pmdREWCPReadInCS}{17.5}
\newcommand{\pmdREWCPReadOutCS}{116}
\newcommand{\pmdREWCPReadSameEp}{33.9}
\newcommand{\pmdREWCPReadSharedSameEp}{\cna}
\newcommand{\pmdREWCPReadExclusive}{0.208}
\newcommand{\pmdREWCPReadOwned}{98.1}
\newcommand{\pmdREWCPReadShare}{0.0489}
\newcommand{\pmdREWCPReadShared}{0.076}
\newcommand{\pmdREWCPReadSharedOwned}{1.6}
\newcommand{\pmdREWCPNoFPHonestWriteTotal}{0.49}
\newcommand{\pmdREWCPWriteInCS}{29.2}
\newcommand{\pmdREWCPWriteOutCS}{2170}
\newcommand{\pmdREWCPNoFPWriteTotal}{0.49}
\newcommand{\pmdREWCPWriteSameEp}{2100}
\newcommand{\pmdREWCPWriteExclusive}{0.00163}
\newcommand{\pmdREWCPWriteOwned}{99.5}
\newcommand{\pmdREWCPWriteShared}{0.532}
\newcommand{\pmdREWCPNoFPOtherEventTotal}{18037}
\newcommand{\pmdREWCPAcqRelOtherTotal}{97.5}
\newcommand{\pmdREWCPNoAcqRelOtherTotal}{459}
\newcommand{\pmdREWCPFork}{0.0}
\newcommand{\pmdREWCPJoin}{0.0}
\newcommand{\pmdREWCPPreWait}{0.0}
\newcommand{\pmdREWCPPostWait}{0.0}
\newcommand{\pmdREWCPVolatileTotal}{0.0}
\newcommand{\pmdREWCPClassInit}{12.4}
\newcommand{\pmdREWCPClassAccess}{87.6}
\newcommand{\pmdREWCPRaceTotal}{5135}
\newcommand{\pmdREWCPWrRdRace}{99.6}
\newcommand{\pmdREWCPWrWrRace}{0.0}
\newcommand{\pmdREWCPRdWrRace}{0.389}
\newcommand{\pmdREWCPRdShWrRace}{0.0}
\newcommand{\pmdREWCPHoldLocksTotal}{0.093}
\newcommand{\pmdREWCPOneLockHeld}{1.11}
\newcommand{\pmdREWCPTwoNestedLocks}{\cna}
\newcommand{\pmdREWCPThreeNestedLocks}{\cna}
\newcommand{\pmdREWCPFourNestedLocks}{\cna}
\newcommand{\pmdREWCPFiveNestedLocks}{\cna}
\newcommand{\pmdREWCPSixNestedLocks}{\cna}
\newcommand{\pmdREWCPSevenNestedLocks}{\cna}
\newcommand{\pmdREWCPEightNestedLocks}{\cna}
\newcommand{\pmdREWCPNineNestedLocks}{\cna}
\newcommand{\pmdREWCPTenNestedLocks}{\cna}
\newcommand{\pmdREWCPHundredNestedLocks}{\cna}
\newcommand{\pmdDCEventTotal}{200}
\newcommand{\pmdDCNoFPEventTotal}{13}
\newcommand{\pmdDCNoFPAccessTotal}{13}
\newcommand{\pmdDCNoFPOtherTotal}{<0.1}
\newcommand{\pmdDCReadTotal}{95.9}
\newcommand{\pmdDCWriteTotal}{3.91}
\newcommand{\pmdDCNoFPAccessInCS}{11.5}
\newcommand{\pmdDCNoFPAccessOutCS}{88.5}
\newcommand{\pmdDCAcqRelTotal}{0.135}
\newcommand{\pmdDCOtherTotal}{0.00354}
\newcommand{\pmdDCNoFPReadTotal}{12}
\newcommand{\pmdDCReadInCS}{11.1}
\newcommand{\pmdDCReadOutCS}{110}
\newcommand{\pmdDCReadSameEp}{20.7}
\newcommand{\pmdDCReadSharedSameEp}{\cna}
\newcommand{\pmdDCReadExclusive}{99}
\newcommand{\pmdDCReadOwned}{\cna}
\newcommand{\pmdDCReadShare}{0.0104}
\newcommand{\pmdDCReadShared}{1.03}
\newcommand{\pmdDCReadSharedOwned}{\cna}
\newcommand{\pmdDCNoFPHonestWriteTotal}{0.49}
\newcommand{\pmdDCWriteInCS}{29.2}
\newcommand{\pmdDCWriteOutCS}{2170}
\newcommand{\pmdDCNoFPWriteTotal}{0.49}
\newcommand{\pmdDCWriteSameEp}{2100}
\newcommand{\pmdDCWriteExclusive}{100}
\newcommand{\pmdDCWriteOwned}{\cna}
\newcommand{\pmdDCWriteShared}{\cna}
\newcommand{\pmdDCNoFPOtherEventTotal}{18038}
\newcommand{\pmdDCAcqRelOtherTotal}{97.4}
\newcommand{\pmdDCNoAcqRelOtherTotal}{460}
\newcommand{\pmdDCFork}{0.0}
\newcommand{\pmdDCJoin}{0.0}
\newcommand{\pmdDCPreWait}{0.0}
\newcommand{\pmdDCPostWait}{0.0}
\newcommand{\pmdDCVolatileTotal}{0.0}
\newcommand{\pmdDCClassInit}{12.4}
\newcommand{\pmdDCClassAccess}{87.6}
\newcommand{\pmdDCRaceTotal}{8439}
\newcommand{\pmdDCWrRdRace}{97.4}
\newcommand{\pmdDCWrWrRace}{2.61}
\newcommand{\pmdDCRdWrRace}{0.0}
\newcommand{\pmdDCRdShWrRace}{0.0}
\newcommand{\pmdDCHoldLocksTotal}{1.6}
\newcommand{\pmdDCOneLockHeld}{12.9}
\newcommand{\pmdDCTwoNestedLocks}{\cna}
\newcommand{\pmdDCThreeNestedLocks}{\cna}
\newcommand{\pmdDCFourNestedLocks}{\cna}
\newcommand{\pmdDCFiveNestedLocks}{\cna}
\newcommand{\pmdDCSixNestedLocks}{\cna}
\newcommand{\pmdDCSevenNestedLocks}{\cna}
\newcommand{\pmdDCEightNestedLocks}{\cna}
\newcommand{\pmdDCNineNestedLocks}{\cna}
\newcommand{\pmdDCTenNestedLocks}{\cna}
\newcommand{\pmdDCHundredNestedLocks}{\cna}
\newcommand{\pmdFTODCEventTotal}{200}
\newcommand{\pmdFTODCNoFPEventTotal}{7.9}
\newcommand{\pmdFTODCNoFPAccessTotal}{7.9}
\newcommand{\pmdFTODCNoFPOtherTotal}{<0.1}
\newcommand{\pmdFTODCReadTotal}{93.5}
\newcommand{\pmdFTODCWriteTotal}{6.23}
\newcommand{\pmdFTODCNoFPAccessInCS}{10.5}
\newcommand{\pmdFTODCNoFPAccessOutCS}{89.5}
\newcommand{\pmdFTODCAcqRelTotal}{0.137}
\newcommand{\pmdFTODCOtherTotal}{0.00358}
\newcommand{\pmdFTODCNoFPReadTotal}{7.4}
\newcommand{\pmdFTODCReadInCS}{17.5}
\newcommand{\pmdFTODCReadOutCS}{117}
\newcommand{\pmdFTODCReadSameEp}{33.9}
\newcommand{\pmdFTODCReadSharedSameEp}{\cna}
\newcommand{\pmdFTODCReadExclusive}{0.217}
\newcommand{\pmdFTODCReadOwned}{98.1}
\newcommand{\pmdFTODCReadShare}{0.0169}
\newcommand{\pmdFTODCReadShared}{0.0784}
\newcommand{\pmdFTODCReadSharedOwned}{1.6}
\newcommand{\pmdFTODCNoFPHonestWriteTotal}{0.49}
\newcommand{\pmdFTODCWriteInCS}{29.2}
\newcommand{\pmdFTODCWriteOutCS}{2170}
\newcommand{\pmdFTODCNoFPWriteTotal}{0.49}
\newcommand{\pmdFTODCWriteSameEp}{2100}
\newcommand{\pmdFTODCWriteExclusive}{\cna}
\newcommand{\pmdFTODCWriteOwned}{100}
\newcommand{\pmdFTODCWriteShared}{\cna}
\newcommand{\pmdFTODCNoFPOtherEventTotal}{18038}
\newcommand{\pmdFTODCAcqRelOtherTotal}{97.4}
\newcommand{\pmdFTODCNoAcqRelOtherTotal}{460}
\newcommand{\pmdFTODCFork}{0.0}
\newcommand{\pmdFTODCJoin}{0.0}
\newcommand{\pmdFTODCPreWait}{0.0}
\newcommand{\pmdFTODCPostWait}{0.0}
\newcommand{\pmdFTODCVolatileTotal}{0.0}
\newcommand{\pmdFTODCClassInit}{12.4}
\newcommand{\pmdFTODCClassAccess}{87.6}
\newcommand{\pmdFTODCRaceTotal}{8697}
\newcommand{\pmdFTODCWrRdRace}{97.5}
\newcommand{\pmdFTODCWrWrRace}{0.0}
\newcommand{\pmdFTODCRdWrRace}{2.53}
\newcommand{\pmdFTODCRdShWrRace}{0.0}
\newcommand{\pmdFTODCHoldLocksTotal}{0.093}
\newcommand{\pmdFTODCOneLockHeld}{1.06}
\newcommand{\pmdFTODCTwoNestedLocks}{\cna}
\newcommand{\pmdFTODCThreeNestedLocks}{\cna}
\newcommand{\pmdFTODCFourNestedLocks}{\cna}
\newcommand{\pmdFTODCFiveNestedLocks}{\cna}
\newcommand{\pmdFTODCSixNestedLocks}{\cna}
\newcommand{\pmdFTODCSevenNestedLocks}{\cna}
\newcommand{\pmdFTODCEightNestedLocks}{\cna}
\newcommand{\pmdFTODCNineNestedLocks}{\cna}
\newcommand{\pmdFTODCTenNestedLocks}{\cna}
\newcommand{\pmdFTODCHundredNestedLocks}{\cna}
\newcommand{\pmdREDCEventTotal}{200}
\newcommand{\pmdREDCNoFPEventTotal}{7.9}
\newcommand{\pmdREDCNoFPAccessTotal}{7.9}
\newcommand{\pmdREDCNoFPOtherTotal}{<0.1}
\newcommand{\pmdREDCReadTotal}{93.5}
\newcommand{\pmdREDCWriteTotal}{6.23}
\newcommand{\pmdREDCNoFPAccessInCS}{10.5}
\newcommand{\pmdREDCNoFPAccessOutCS}{89.5}
\newcommand{\pmdREDCAcqRelTotal}{0.137}
\newcommand{\pmdREDCOtherTotal}{0.00357}
\newcommand{\pmdREDCNoFPReadTotal}{7.4}
\newcommand{\pmdREDCReadInCS}{17.5}
\newcommand{\pmdREDCReadOutCS}{117}
\newcommand{\pmdREDCReadSameEp}{33.9}
\newcommand{\pmdREDCReadSharedSameEp}{\cna}
\newcommand{\pmdREDCReadExclusive}{0.115}
\newcommand{\pmdREDCReadOwned}{98.1}
\newcommand{\pmdREDCReadShare}{0.117}
\newcommand{\pmdREDCReadShared}{0.0786}
\newcommand{\pmdREDCReadSharedOwned}{1.6}
\newcommand{\pmdREDCNoFPHonestWriteTotal}{0.49}
\newcommand{\pmdREDCWriteInCS}{29.2}
\newcommand{\pmdREDCWriteOutCS}{2170}
\newcommand{\pmdREDCNoFPWriteTotal}{0.49}
\newcommand{\pmdREDCWriteSameEp}{2100}
\newcommand{\pmdREDCWriteExclusive}{\cna}
\newcommand{\pmdREDCWriteOwned}{98.5}
\newcommand{\pmdREDCWriteShared}{1.5}
\newcommand{\pmdREDCNoFPOtherEventTotal}{18036}
\newcommand{\pmdREDCAcqRelOtherTotal}{97.5}
\newcommand{\pmdREDCNoAcqRelOtherTotal}{458}
\newcommand{\pmdREDCFork}{0.0}
\newcommand{\pmdREDCJoin}{0.0}
\newcommand{\pmdREDCPreWait}{0.0}
\newcommand{\pmdREDCPostWait}{0.0}
\newcommand{\pmdREDCVolatileTotal}{0.0}
\newcommand{\pmdREDCClassInit}{12.4}
\newcommand{\pmdREDCClassAccess}{87.6}
\newcommand{\pmdREDCRaceTotal}{8684}
\newcommand{\pmdREDCWrRdRace}{97.5}
\newcommand{\pmdREDCWrWrRace}{0.0}
\newcommand{\pmdREDCRdWrRace}{2.53}
\newcommand{\pmdREDCRdShWrRace}{0.0}
\newcommand{\pmdREDCHoldLocksTotal}{0.093}
\newcommand{\pmdREDCOneLockHeld}{1.06}
\newcommand{\pmdREDCTwoNestedLocks}{\cna}
\newcommand{\pmdREDCThreeNestedLocks}{\cna}
\newcommand{\pmdREDCFourNestedLocks}{\cna}
\newcommand{\pmdREDCFiveNestedLocks}{\cna}
\newcommand{\pmdREDCSixNestedLocks}{\cna}
\newcommand{\pmdREDCSevenNestedLocks}{\cna}
\newcommand{\pmdREDCEightNestedLocks}{\cna}
\newcommand{\pmdREDCNineNestedLocks}{\cna}
\newcommand{\pmdREDCTenNestedLocks}{\cna}
\newcommand{\pmdREDCHundredNestedLocks}{\cna}
\newcommand{\pmdCAPOEventTotal}{200}
\newcommand{\pmdCAPONoFPEventTotal}{13}
\newcommand{\pmdCAPONoFPAccessTotal}{13}
\newcommand{\pmdCAPONoFPOtherTotal}{<0.1}
\newcommand{\pmdCAPOReadTotal}{95.9}
\newcommand{\pmdCAPOWriteTotal}{3.91}
\newcommand{\pmdCAPONoFPAccessInCS}{11.5}
\newcommand{\pmdCAPONoFPAccessOutCS}{88.5}
\newcommand{\pmdCAPOAcqRelTotal}{0.135}
\newcommand{\pmdCAPOOtherTotal}{0.00353}
\newcommand{\pmdCAPONoFPReadTotal}{12}
\newcommand{\pmdCAPOReadInCS}{11.1}
\newcommand{\pmdCAPOReadOutCS}{110}
\newcommand{\pmdCAPOReadSameEp}{20.7}
\newcommand{\pmdCAPOReadSharedSameEp}{\cna}
\newcommand{\pmdCAPOReadExclusive}{99}
\newcommand{\pmdCAPOReadOwned}{\cna}
\newcommand{\pmdCAPOReadShare}{0.0103}
\newcommand{\pmdCAPOReadShared}{1.03}
\newcommand{\pmdCAPOReadSharedOwned}{\cna}
\newcommand{\pmdCAPONoFPHonestWriteTotal}{0.49}
\newcommand{\pmdCAPOWriteInCS}{29.2}
\newcommand{\pmdCAPOWriteOutCS}{2170}
\newcommand{\pmdCAPONoFPWriteTotal}{0.49}
\newcommand{\pmdCAPOWriteSameEp}{2100}
\newcommand{\pmdCAPOWriteExclusive}{100}
\newcommand{\pmdCAPOWriteOwned}{\cna}
\newcommand{\pmdCAPOWriteShared}{\cna}
\newcommand{\pmdCAPONoFPOtherEventTotal}{18037}
\newcommand{\pmdCAPOAcqRelOtherTotal}{97.5}
\newcommand{\pmdCAPONoAcqRelOtherTotal}{459}
\newcommand{\pmdCAPOFork}{0.0}
\newcommand{\pmdCAPOJoin}{0.0}
\newcommand{\pmdCAPOPreWait}{0.0}
\newcommand{\pmdCAPOPostWait}{0.0}
\newcommand{\pmdCAPOVolatileTotal}{0.0}
\newcommand{\pmdCAPOClassInit}{12.4}
\newcommand{\pmdCAPOClassAccess}{87.6}
\newcommand{\pmdCAPORaceTotal}{7852}
\newcommand{\pmdCAPOWrRdRace}{97.2}
\newcommand{\pmdCAPOWrWrRace}{2.8}
\newcommand{\pmdCAPORdWrRace}{0.0}
\newcommand{\pmdCAPORdShWrRace}{0.0}
\newcommand{\pmdCAPOHoldLocksTotal}{1.6}
\newcommand{\pmdCAPOOneLockHeld}{12.9}
\newcommand{\pmdCAPOTwoNestedLocks}{\cna}
\newcommand{\pmdCAPOThreeNestedLocks}{\cna}
\newcommand{\pmdCAPOFourNestedLocks}{\cna}
\newcommand{\pmdCAPOFiveNestedLocks}{\cna}
\newcommand{\pmdCAPOSixNestedLocks}{\cna}
\newcommand{\pmdCAPOSevenNestedLocks}{\cna}
\newcommand{\pmdCAPOEightNestedLocks}{\cna}
\newcommand{\pmdCAPONineNestedLocks}{\cna}
\newcommand{\pmdCAPOTenNestedLocks}{\cna}
\newcommand{\pmdCAPOHundredNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOEventTotal}{200}
\newcommand{\pmdFTOCAPONoFPEventTotal}{7.9}
\newcommand{\pmdFTOCAPONoFPAccessTotal}{7.9}
\newcommand{\pmdFTOCAPONoFPOtherTotal}{<0.1}
\newcommand{\pmdFTOCAPOReadTotal}{93.5}
\newcommand{\pmdFTOCAPOWriteTotal}{6.23}
\newcommand{\pmdFTOCAPONoFPAccessInCS}{10.5}
\newcommand{\pmdFTOCAPONoFPAccessOutCS}{89.5}
\newcommand{\pmdFTOCAPOAcqRelTotal}{0.137}
\newcommand{\pmdFTOCAPOOtherTotal}{0.00357}
\newcommand{\pmdFTOCAPONoFPReadTotal}{7.4}
\newcommand{\pmdFTOCAPOReadInCS}{17.5}
\newcommand{\pmdFTOCAPOReadOutCS}{117}
\newcommand{\pmdFTOCAPOReadSameEp}{33.9}
\newcommand{\pmdFTOCAPOReadSharedSameEp}{\cna}
\newcommand{\pmdFTOCAPOReadExclusive}{0.216}
\newcommand{\pmdFTOCAPOReadOwned}{98.1}
\newcommand{\pmdFTOCAPOReadShare}{0.0171}
\newcommand{\pmdFTOCAPOReadShared}{0.0789}
\newcommand{\pmdFTOCAPOReadSharedOwned}{1.6}
\newcommand{\pmdFTOCAPONoFPHonestWriteTotal}{0.49}
\newcommand{\pmdFTOCAPOWriteInCS}{29.2}
\newcommand{\pmdFTOCAPOWriteOutCS}{2170}
\newcommand{\pmdFTOCAPONoFPWriteTotal}{0.49}
\newcommand{\pmdFTOCAPOWriteSameEp}{2100}
\newcommand{\pmdFTOCAPOWriteExclusive}{\cna}
\newcommand{\pmdFTOCAPOWriteOwned}{100}
\newcommand{\pmdFTOCAPOWriteShared}{\cna}
\newcommand{\pmdFTOCAPONoFPOtherEventTotal}{18037}
\newcommand{\pmdFTOCAPOAcqRelOtherTotal}{97.5}
\newcommand{\pmdFTOCAPONoAcqRelOtherTotal}{459}
\newcommand{\pmdFTOCAPOFork}{0.0}
\newcommand{\pmdFTOCAPOJoin}{0.0}
\newcommand{\pmdFTOCAPOPreWait}{0.0}
\newcommand{\pmdFTOCAPOPostWait}{0.0}
\newcommand{\pmdFTOCAPOVolatileTotal}{0.0}
\newcommand{\pmdFTOCAPOClassInit}{12.4}
\newcommand{\pmdFTOCAPOClassAccess}{87.6}
\newcommand{\pmdFTOCAPORaceTotal}{9337}
\newcommand{\pmdFTOCAPOWrRdRace}{97.6}
\newcommand{\pmdFTOCAPOWrWrRace}{0.0}
\newcommand{\pmdFTOCAPORdWrRace}{2.36}
\newcommand{\pmdFTOCAPORdShWrRace}{0.0}
\newcommand{\pmdFTOCAPOHoldLocksTotal}{0.093}
\newcommand{\pmdFTOCAPOOneLockHeld}{1.05}
\newcommand{\pmdFTOCAPOTwoNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOThreeNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOFourNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOSixNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOEightNestedLocks}{\cna}
\newcommand{\pmdFTOCAPONineNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOTenNestedLocks}{\cna}
\newcommand{\pmdFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\pmdRECAPOEventTotal}{200}
\newcommand{\pmdRECAPONoFPEventTotal}{7.9}
\newcommand{\pmdRECAPONoFPAccessTotal}{7.9}
\newcommand{\pmdRECAPONoFPOtherTotal}{<0.1}
\newcommand{\pmdRECAPOReadTotal}{93.5}
\newcommand{\pmdRECAPOWriteTotal}{6.23}
\newcommand{\pmdRECAPONoFPAccessInCS}{10.5}
\newcommand{\pmdRECAPONoFPAccessOutCS}{89.5}
\newcommand{\pmdRECAPOAcqRelTotal}{0.137}
\newcommand{\pmdRECAPOOtherTotal}{0.00358}
\newcommand{\pmdRECAPONoFPReadTotal}{7.4}
\newcommand{\pmdRECAPOReadInCS}{17.5}
\newcommand{\pmdRECAPOReadOutCS}{117}
\newcommand{\pmdRECAPOReadSameEp}{33.9}
\newcommand{\pmdRECAPOReadSharedSameEp}{\cna}
\newcommand{\pmdRECAPOReadExclusive}{0.115}
\newcommand{\pmdRECAPOReadOwned}{98.1}
\newcommand{\pmdRECAPOReadShare}{0.117}
\newcommand{\pmdRECAPOReadShared}{0.0789}
\newcommand{\pmdRECAPOReadSharedOwned}{1.6}
\newcommand{\pmdRECAPONoFPHonestWriteTotal}{0.49}
\newcommand{\pmdRECAPOWriteInCS}{29.2}
\newcommand{\pmdRECAPOWriteOutCS}{2170}
\newcommand{\pmdRECAPONoFPWriteTotal}{0.49}
\newcommand{\pmdRECAPOWriteSameEp}{2100}
\newcommand{\pmdRECAPOWriteExclusive}{\cna}
\newcommand{\pmdRECAPOWriteOwned}{98.5}
\newcommand{\pmdRECAPOWriteShared}{1.5}
\newcommand{\pmdRECAPONoFPOtherEventTotal}{18038}
\newcommand{\pmdRECAPOAcqRelOtherTotal}{97.4}
\newcommand{\pmdRECAPONoAcqRelOtherTotal}{460}
\newcommand{\pmdRECAPOFork}{0.0}
\newcommand{\pmdRECAPOJoin}{0.0}
\newcommand{\pmdRECAPOPreWait}{0.0}
\newcommand{\pmdRECAPOPostWait}{0.0}
\newcommand{\pmdRECAPOVolatileTotal}{0.0}
\newcommand{\pmdRECAPOClassInit}{12.4}
\newcommand{\pmdRECAPOClassAccess}{87.6}
\newcommand{\pmdRECAPORaceTotal}{9245}
\newcommand{\pmdRECAPOWrRdRace}{97.6}
\newcommand{\pmdRECAPOWrWrRace}{0.0}
\newcommand{\pmdRECAPORdWrRace}{2.38}
\newcommand{\pmdRECAPORdShWrRace}{0.0}
\newcommand{\pmdRECAPOHoldLocksTotal}{0.093}
\newcommand{\pmdRECAPOOneLockHeld}{1.06}
\newcommand{\pmdRECAPOTwoNestedLocks}{\cna}
\newcommand{\pmdRECAPOThreeNestedLocks}{\cna}
\newcommand{\pmdRECAPOFourNestedLocks}{\cna}
\newcommand{\pmdRECAPOFiveNestedLocks}{\cna}
\newcommand{\pmdRECAPOSixNestedLocks}{\cna}
\newcommand{\pmdRECAPOSevenNestedLocks}{\cna}
\newcommand{\pmdRECAPOEightNestedLocks}{\cna}
\newcommand{\pmdRECAPONineNestedLocks}{\cna}
\newcommand{\pmdRECAPOTenNestedLocks}{\cna}
\newcommand{\pmdRECAPOHundredNestedLocks}{\cna}
\newcommand{\pmdCAPOTotalSetClears}{0.0088}
\newcommand{\pmdCAPOReadSetZero}{0.0}
\newcommand{\pmdCAPOReadSetOne}{0.216}
\newcommand{\pmdCAPOReadSetGtOne}{99.8}
\newcommand{\pmdCAPOWriteSetZero}{0.216}
\newcommand{\pmdCAPOWriteSetOne}{0.0}
\newcommand{\pmdCAPOWriteSetGtOne}{99.8}
\newcommand{\pmdCAPOTotalMapClears}{0.0088}
\newcommand{\pmdCAPOReadMapZero}{0.0}
\newcommand{\pmdCAPOReadMapOne}{0.114}
\newcommand{\pmdCAPOReadMapTen}{0.148}
\newcommand{\pmdCAPOReadMapHund}{97.2}
\newcommand{\pmdCAPOReadMapThou}{0.33}
\newcommand{\pmdCAPOReadMapGtThou}{2.17}
\newcommand{\pmdCAPOWriteMapZero}{0.114}
\newcommand{\pmdCAPOWriteMapOne}{0.0}
\newcommand{\pmdCAPOWriteMapTen}{0.216}
\newcommand{\pmdCAPOWriteMapHund}{97.3}
\newcommand{\pmdCAPOWriteMapThou}{2.09}
\newcommand{\pmdCAPOWriteMapGtThou}{0.25}
\newcommand{\FASTpmdMaxLiveThreads}{9}
\newcommand{\FASTpmdTotalThreads}{9}
\newcommand{\FASTpmdBaseTime}{1.4}
\newcommand{\FASTpmdBaseTimeCI}{20}
\newcommand{\FASTpmdEmptyTime}{\rna}
\newcommand{\FASTpmdEmptyTimeCI}{\rna}
\newcommand{\FASTpmdEmptyTimeCIMIN}{\rna}
\newcommand{\FASTpmdEmptyTimeCIMAX}{\rna}
\newcommand{\FASTpmdFTTime}{6.2}
\newcommand{\FASTpmdFTTimeCI}{0.26}
\newcommand{\FASTpmdHBTime}{6.1}
\newcommand{\FASTpmdHBTimeCI}{0.13}
\newcommand{\FASTpmdFTOHBTime}{6.2}
\newcommand{\FASTpmdFTOHBTimeCI}{0.18}
\newcommand{\FASTpmdWCPTime}{6.2}
\newcommand{\FASTpmdWCPTimeCI}{0.11}
\newcommand{\FASTpmdFTOWCPTime}{6.3}
\newcommand{\FASTpmdFTOWCPTimeCI}{0.11}
\newcommand{\FASTpmdREWCPTime}{7.2}
\newcommand{\FASTpmdREWCPTimeCI}{0.17}
\newcommand{\FASTpmdDCTime}{6.1}
\newcommand{\FASTpmdDCTimeCI}{0.17}
\newcommand{\FASTpmdFTODCTime}{6.4}
\newcommand{\FASTpmdFTODCTimeCI}{0.093}
\newcommand{\FASTpmdREDCTime}{7.3}
\newcommand{\FASTpmdREDCTimeCI}{0.11}
\newcommand{\FASTpmdCAPOTime}{6.0}
\newcommand{\FASTpmdCAPOTimeCI}{0.15}
\newcommand{\FASTpmdFTOCAPOTime}{6.4}
\newcommand{\FASTpmdFTOCAPOTimeCI}{0.12}
\newcommand{\FASTpmdRECAPOTime}{7.2}
\newcommand{\FASTpmdRECAPOTimeCI}{0.19}
\newcommand{\FASTpmdAGGCAPOTime}{\rna}
\newcommand{\FASTpmdAGGCAPOTimeCI}{\rna}
\newcommand{\FASTpmdAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTpmdAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTpmdStaticTime}{\rzero}
\newcommand{\FASTpmdDynamicTime}{\rzero}
\newcommand{\FASTpmdBaseMem}{590}
\newcommand{\FASTpmdBaseMemCI}{13.0}
\newcommand{\FASTpmdFTMem}{2.7}
\newcommand{\FASTpmdFTMemCI}{0.19}
\newcommand{\FASTpmdHBMem}{2.7}
\newcommand{\FASTpmdHBMemCI}{0.21}
\newcommand{\FASTpmdFTOHBMem}{2.5}
\newcommand{\FASTpmdFTOHBMemCI}{0.18}
\newcommand{\FASTpmdWCPMem}{2.9}
\newcommand{\FASTpmdWCPMemCI}{0.18}
\newcommand{\FASTpmdFTOWCPMem}{2.7}
\newcommand{\FASTpmdFTOWCPMemCI}{0.17}
\newcommand{\FASTpmdREWCPMem}{4.9}
\newcommand{\FASTpmdREWCPMemCI}{0.16}
\newcommand{\FASTpmdDCMem}{3.1}
\newcommand{\FASTpmdDCMemCI}{0.17}
\newcommand{\FASTpmdFTODCMem}{2.9}
\newcommand{\FASTpmdFTODCMemCI}{0.11}
\newcommand{\FASTpmdREDCMem}{4.9}
\newcommand{\FASTpmdREDCMemCI}{0.15}
\newcommand{\FASTpmdCAPOMem}{2.7}
\newcommand{\FASTpmdCAPOMemCI}{0.13}
\newcommand{\FASTpmdFTOCAPOMem}{2.9}
\newcommand{\FASTpmdFTOCAPOMemCI}{0.16}
\newcommand{\FASTpmdRECAPOMem}{4.9}
\newcommand{\FASTpmdRECAPOMemCI}{0.16}
\newcommand{\FASTpmdAGGCAPOMem}{\memna}
\newcommand{\FASTpmdAGGCAPOMemCI}{\memna}
\newcommand{\FASTpmdAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTpmdAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTpmdEventsCI}{803}
\newcommand{\FASTpmdEventsCIMIN}{200,051,558}
\newcommand{\FASTpmdEventsCIMAX}{200,053,164}
\newcommand{\FASTpmdNoFPEventsCI}{1,316}
\newcommand{\FASTpmdNoFPEventsCIMIN}{12,845,467}
\newcommand{\FASTpmdNoFPEventsCIMAX}{12,848,099}
\newcommand{\FASTpmdFT}{18}
\newcommand{\FASTpmdFTCI}{0}
\newcommand{\FASTpmdFTCIMIN}{18}
\newcommand{\FASTpmdFTCIMAX}{18}
\newcommand{\FASTpmdFTDynamic}{3,820}
\newcommand{\FASTpmdFTDynamicCI}{523}
\newcommand{\FASTpmdFTDynamicCIMIN}{3,297}
\newcommand{\FASTpmdFTDynamicCIMAX}{4,343}
\newcommand{\FASTpmdHB}{24}
\newcommand{\FASTpmdHBCI}{0}
\newcommand{\FASTpmdHBCIMIN}{24}
\newcommand{\FASTpmdHBCIMAX}{24}
\newcommand{\FASTpmdHBDynamic}{3,889}
\newcommand{\FASTpmdHBDynamicCI}{572}
\newcommand{\FASTpmdHBDynamicCIMIN}{3,317}
\newcommand{\FASTpmdHBDynamicCIMAX}{4,461}
\newcommand{\FASTpmdFTOHB}{24}
\newcommand{\FASTpmdFTOHBCI}{0}
\newcommand{\FASTpmdFTOHBCIMIN}{24}
\newcommand{\FASTpmdFTOHBCIMAX}{24}
\newcommand{\FASTpmdFTOHBDynamic}{3,969}
\newcommand{\FASTpmdFTOHBDynamicCI}{526}
\newcommand{\FASTpmdFTOHBDynamicCIMIN}{3,443}
\newcommand{\FASTpmdFTOHBDynamicCIMAX}{4,495}
\newcommand{\FASTpmdWCP}{24}
\newcommand{\FASTpmdWCPCI}{0}
\newcommand{\FASTpmdWCPCIMIN}{24}
\newcommand{\FASTpmdWCPCIMAX}{24}
\newcommand{\FASTpmdWCPDynamic}{5,243}
\newcommand{\FASTpmdWCPDynamicCI}{931}
\newcommand{\FASTpmdWCPDynamicCIMIN}{4,312}
\newcommand{\FASTpmdWCPDynamicCIMAX}{6,174}
\newcommand{\FASTpmdFTOWCP}{24}
\newcommand{\FASTpmdFTOWCPCI}{0}
\newcommand{\FASTpmdFTOWCPCIMIN}{24}
\newcommand{\FASTpmdFTOWCPCIMAX}{24}
\newcommand{\FASTpmdFTOWCPDynamic}{3,884}
\newcommand{\FASTpmdFTOWCPDynamicCI}{1,018}
\newcommand{\FASTpmdFTOWCPDynamicCIMIN}{2,866}
\newcommand{\FASTpmdFTOWCPDynamicCIMAX}{4,902}
\newcommand{\FASTpmdREWCP}{24}
\newcommand{\FASTpmdREWCPCI}{0}
\newcommand{\FASTpmdREWCPCIMIN}{24}
\newcommand{\FASTpmdREWCPCIMAX}{24}
\newcommand{\FASTpmdREWCPDynamic}{5,135}
\newcommand{\FASTpmdREWCPDynamicCI}{540}
\newcommand{\FASTpmdREWCPDynamicCIMIN}{4,595}
\newcommand{\FASTpmdREWCPDynamicCIMAX}{5,675}
\newcommand{\FASTpmdDC}{27}
\newcommand{\FASTpmdDCCI}{0}
\newcommand{\FASTpmdDCCIMIN}{27}
\newcommand{\FASTpmdDCCIMAX}{27}
\newcommand{\FASTpmdDCDynamic}{8,439}
\newcommand{\FASTpmdDCDynamicCI}{1,072}
\newcommand{\FASTpmdDCDynamicCIMIN}{7,367}
\newcommand{\FASTpmdDCDynamicCIMAX}{9,511}
\newcommand{\FASTpmdFTODC}{27}
\newcommand{\FASTpmdFTODCCI}{0}
\newcommand{\FASTpmdFTODCCIMIN}{27}
\newcommand{\FASTpmdFTODCCIMAX}{27}
\newcommand{\FASTpmdFTODCDynamic}{8,697}
\newcommand{\FASTpmdFTODCDynamicCI}{1,241}
\newcommand{\FASTpmdFTODCDynamicCIMIN}{7,456}
\newcommand{\FASTpmdFTODCDynamicCIMAX}{9,938}
\newcommand{\FASTpmdREDC}{27}
\newcommand{\FASTpmdREDCCI}{0}
\newcommand{\FASTpmdREDCCIMIN}{27}
\newcommand{\FASTpmdREDCCIMAX}{27}
\newcommand{\FASTpmdREDCDynamic}{8,684}
\newcommand{\FASTpmdREDCDynamicCI}{933}
\newcommand{\FASTpmdREDCDynamicCIMIN}{7,751}
\newcommand{\FASTpmdREDCDynamicCIMAX}{9,617}
\newcommand{\FASTpmdCAPO}{27}
\newcommand{\FASTpmdCAPOCI}{0}
\newcommand{\FASTpmdCAPOCIMIN}{27}
\newcommand{\FASTpmdCAPOCIMAX}{27}
\newcommand{\FASTpmdCAPODynamic}{7,852}
\newcommand{\FASTpmdCAPODynamicCI}{795}
\newcommand{\FASTpmdCAPODynamicCIMIN}{7,057}
\newcommand{\FASTpmdCAPODynamicCIMAX}{8,647}
\newcommand{\FASTpmdFTOCAPO}{27}
\newcommand{\FASTpmdFTOCAPOCI}{0}
\newcommand{\FASTpmdFTOCAPOCIMIN}{27}
\newcommand{\FASTpmdFTOCAPOCIMAX}{27}
\newcommand{\FASTpmdFTOCAPODynamic}{9,337}
\newcommand{\FASTpmdFTOCAPODynamicCI}{2,105}
\newcommand{\FASTpmdFTOCAPODynamicCIMIN}{7,232}
\newcommand{\FASTpmdFTOCAPODynamicCIMAX}{11,442}
\newcommand{\FASTpmdRECAPO}{27}
\newcommand{\FASTpmdRECAPOCI}{0}
\newcommand{\FASTpmdRECAPOCIMIN}{27}
\newcommand{\FASTpmdRECAPOCIMAX}{27}
\newcommand{\FASTpmdRECAPODynamic}{9,245}
\newcommand{\FASTpmdRECAPODynamicCI}{1,154}
\newcommand{\FASTpmdRECAPODynamicCIMIN}{8,091}
\newcommand{\FASTpmdRECAPODynamicCIMAX}{10,399}
\newcommand{\FASTpmdAGGCAPO}{\rna}
\newcommand{\FASTpmdAGGCAPOCI}{\rna}
\newcommand{\FASTpmdAGGCAPOCIMIN}{\rna}
\newcommand{\FASTpmdAGGCAPOCIMAX}{\rna}
\newcommand{\FASTpmdAGGCAPODynamic}{\rna}
\newcommand{\FASTpmdAGGCAPODynamicCI}{\rna}
\newcommand{\FASTpmdAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTpmdAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTsunflowEvents}{9,700}
\newcommand{\FASTsunflowNoFPEvents}{400}
\newcommand{\sunflowHBEventTotal}{9,700}
\newcommand{\sunflowHBNoFPEventTotal}{370}
\newcommand{\sunflowHBNoFPAccessTotal}{370}
\newcommand{\sunflowHBNoFPOtherTotal}{<0.1}
\newcommand{\sunflowHBReadTotal}{99.7}
\newcommand{\sunflowHBWriteTotal}{0.26}
\newcommand{\sunflowHBNoFPAccessInCS}{0.229}
\newcommand{\sunflowHBNoFPAccessOutCS}{99.8}
\newcommand{\sunflowHBAcqRelTotal}{3.94E-4}
\newcommand{\sunflowHBOtherTotal}{3.45E-5}
\newcommand{\sunflowHBNoFPReadTotal}{370}
\newcommand{\sunflowHBReadInCS}{0.235}
\newcommand{\sunflowHBReadOutCS}{100}
\newcommand{\sunflowHBReadSameEp}{0.277}
\newcommand{\sunflowHBReadSharedSameEp}{<0.001}
\newcommand{\sunflowHBReadExclusive}{99.4}
\newcommand{\sunflowHBReadOwned}{\cna}
\newcommand{\sunflowHBReadShare}{0.0222}
\newcommand{\sunflowHBReadShared}{0.594}
\newcommand{\sunflowHBReadSharedOwned}{\cna}
\newcommand{\sunflowHBNoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowHBWriteInCS}{95.1}
\newcommand{\sunflowHBWriteOutCS}{41400}
\newcommand{\sunflowHBNoFPWriteTotal}{0.96}
\newcommand{\sunflowHBWriteSameEp}{41400}
\newcommand{\sunflowHBWriteExclusive}{100}
\newcommand{\sunflowHBWriteOwned}{\cna}
\newcommand{\sunflowHBWriteShared}{<0.001}
\newcommand{\sunflowHBNoFPOtherEventTotal}{1701}
\newcommand{\sunflowHBAcqRelOtherTotal}{92.0}
\newcommand{\sunflowHBNoAcqRelOtherTotal}{137}
\newcommand{\sunflowHBFork}{11.7}
\newcommand{\sunflowHBJoin}{11.7}
\newcommand{\sunflowHBPreWait}{0.0}
\newcommand{\sunflowHBPostWait}{0.0}
\newcommand{\sunflowHBVolatileTotal}{0.0}
\newcommand{\sunflowHBClassInit}{13.9}
\newcommand{\sunflowHBClassAccess}{62.8}
\newcommand{\sunflowHBRaceTotal}{45}
\newcommand{\sunflowHBWrRdRace}{88.9}
\newcommand{\sunflowHBWrWrRace}{0.0}
\newcommand{\sunflowHBRdWrRace}{0.0}
\newcommand{\sunflowHBRdShWrRace}{8.89}
\newcommand{\sunflowHBHoldLocksTotal}{1.8}
\newcommand{\sunflowHBOneLockHeld}{0.48}
\newcommand{\sunflowHBTwoNestedLocks}{<0.1}
\newcommand{\sunflowHBThreeNestedLocks}{\cna}
\newcommand{\sunflowHBFourNestedLocks}{\cna}
\newcommand{\sunflowHBFiveNestedLocks}{\cna}
\newcommand{\sunflowHBSixNestedLocks}{\cna}
\newcommand{\sunflowHBSevenNestedLocks}{\cna}
\newcommand{\sunflowHBEightNestedLocks}{\cna}
\newcommand{\sunflowHBNineNestedLocks}{\cna}
\newcommand{\sunflowHBTenNestedLocks}{\cna}
\newcommand{\sunflowHBHundredNestedLocks}{\cna}
\newcommand{\sunflowFTOHBEventTotal}{9,700}
\newcommand{\sunflowFTOHBNoFPEventTotal}{3.5}
\newcommand{\sunflowFTOHBNoFPAccessTotal}{3.5}
\newcommand{\sunflowFTOHBNoFPOtherTotal}{<0.1}
\newcommand{\sunflowFTOHBReadTotal}{72.3}
\newcommand{\sunflowFTOHBWriteTotal}{27.6}
\newcommand{\sunflowFTOHBNoFPAccessInCS}{0.229}
\newcommand{\sunflowFTOHBNoFPAccessOutCS}{99.8}
\newcommand{\sunflowFTOHBAcqRelTotal}{3.94E-4}
\newcommand{\sunflowFTOHBOtherTotal}{3.45E-5}
\newcommand{\sunflowFTOHBNoFPReadTotal}{2.5}
\newcommand{\sunflowFTOHBReadInCS}{1.09}
\newcommand{\sunflowFTOHBReadOutCS}{139}
\newcommand{\sunflowFTOHBReadSameEp}{40.5}
\newcommand{\sunflowFTOHBReadSharedSameEp}{<0.001}
\newcommand{\sunflowFTOHBReadExclusive}{5.82}
\newcommand{\sunflowFTOHBReadOwned}{4.05}
\newcommand{\sunflowFTOHBReadShare}{3.24}
\newcommand{\sunflowFTOHBReadShared}{16.7}
\newcommand{\sunflowFTOHBReadSharedOwned}{70.2}
\newcommand{\sunflowFTOHBNoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowFTOHBWriteInCS}{95.1}
\newcommand{\sunflowFTOHBWriteOutCS}{41400}
\newcommand{\sunflowFTOHBNoFPWriteTotal}{0.96}
\newcommand{\sunflowFTOHBWriteSameEp}{41400}
\newcommand{\sunflowFTOHBWriteExclusive}{<0.001}
\newcommand{\sunflowFTOHBWriteOwned}{100}
\newcommand{\sunflowFTOHBWriteShared}{<0.001}
\newcommand{\sunflowFTOHBNoFPOtherEventTotal}{1702}
\newcommand{\sunflowFTOHBAcqRelOtherTotal}{92.0}
\newcommand{\sunflowFTOHBNoAcqRelOtherTotal}{137}
\newcommand{\sunflowFTOHBFork}{11.7}
\newcommand{\sunflowFTOHBJoin}{11.7}
\newcommand{\sunflowFTOHBPreWait}{0.0}
\newcommand{\sunflowFTOHBPostWait}{0.0}
\newcommand{\sunflowFTOHBVolatileTotal}{0.0}
\newcommand{\sunflowFTOHBClassInit}{13.9}
\newcommand{\sunflowFTOHBClassAccess}{62.8}
\newcommand{\sunflowFTOHBRaceTotal}{44}
\newcommand{\sunflowFTOHBWrRdRace}{90.9}
\newcommand{\sunflowFTOHBWrWrRace}{0.0}
\newcommand{\sunflowFTOHBRdWrRace}{0.0}
\newcommand{\sunflowFTOHBRdShWrRace}{11.4}
\newcommand{\sunflowFTOHBHoldLocksTotal}{0.027}
\newcommand{\sunflowFTOHBOneLockHeld}{0.78}
\newcommand{\sunflowFTOHBTwoNestedLocks}{<0.1}
\newcommand{\sunflowFTOHBThreeNestedLocks}{\cna}
\newcommand{\sunflowFTOHBFourNestedLocks}{\cna}
\newcommand{\sunflowFTOHBFiveNestedLocks}{\cna}
\newcommand{\sunflowFTOHBSixNestedLocks}{\cna}
\newcommand{\sunflowFTOHBSevenNestedLocks}{\cna}
\newcommand{\sunflowFTOHBEightNestedLocks}{\cna}
\newcommand{\sunflowFTOHBNineNestedLocks}{\cna}
\newcommand{\sunflowFTOHBTenNestedLocks}{\cna}
\newcommand{\sunflowFTOHBHundredNestedLocks}{\cna}
\newcommand{\sunflowWCPEventTotal}{9,700}
\newcommand{\sunflowWCPNoFPEventTotal}{370}
\newcommand{\sunflowWCPNoFPAccessTotal}{370}
\newcommand{\sunflowWCPNoFPOtherTotal}{<0.1}
\newcommand{\sunflowWCPReadTotal}{99.7}
\newcommand{\sunflowWCPWriteTotal}{0.26}
\newcommand{\sunflowWCPNoFPAccessInCS}{0.445}
\newcommand{\sunflowWCPNoFPAccessOutCS}{99.6}
\newcommand{\sunflowWCPAcqRelTotal}{3.94E-4}
\newcommand{\sunflowWCPOtherTotal}{3.44E-5}
\newcommand{\sunflowWCPNoFPReadTotal}{370}
\newcommand{\sunflowWCPReadInCS}{0.235}
\newcommand{\sunflowWCPReadOutCS}{100}
\newcommand{\sunflowWCPReadSameEp}{0.277}
\newcommand{\sunflowWCPReadSharedSameEp}{<0.001}
\newcommand{\sunflowWCPReadExclusive}{99.4}
\newcommand{\sunflowWCPReadOwned}{\cna}
\newcommand{\sunflowWCPReadShare}{0.0221}
\newcommand{\sunflowWCPReadShared}{0.594}
\newcommand{\sunflowWCPReadSharedOwned}{\cna}
\newcommand{\sunflowWCPNoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowWCPWriteInCS}{95.1}
\newcommand{\sunflowWCPWriteOutCS}{41400}
\newcommand{\sunflowWCPNoFPWriteTotal}{0.96}
\newcommand{\sunflowWCPWriteSameEp}{41400}
\newcommand{\sunflowWCPWriteExclusive}{100}
\newcommand{\sunflowWCPWriteOwned}{\cna}
\newcommand{\sunflowWCPWriteShared}{<0.001}
\newcommand{\sunflowWCPNoFPOtherEventTotal}{1703}
\newcommand{\sunflowWCPAcqRelOtherTotal}{92.0}
\newcommand{\sunflowWCPNoAcqRelOtherTotal}{137}
\newcommand{\sunflowWCPFork}{11.7}
\newcommand{\sunflowWCPJoin}{11.7}
\newcommand{\sunflowWCPPreWait}{0.0}
\newcommand{\sunflowWCPPostWait}{0.0}
\newcommand{\sunflowWCPVolatileTotal}{0.0}
\newcommand{\sunflowWCPClassInit}{13.9}
\newcommand{\sunflowWCPClassAccess}{62.8}
\newcommand{\sunflowWCPRaceTotal}{718}
\newcommand{\sunflowWCPWrRdRace}{99.3}
\newcommand{\sunflowWCPWrWrRace}{0.0}
\newcommand{\sunflowWCPRdWrRace}{0.0}
\newcommand{\sunflowWCPRdShWrRace}{0.696}
\newcommand{\sunflowWCPHoldLocksTotal}{2.6}
\newcommand{\sunflowWCPOneLockHeld}{0.71}
\newcommand{\sunflowWCPTwoNestedLocks}{<0.1}
\newcommand{\sunflowWCPThreeNestedLocks}{\cna}
\newcommand{\sunflowWCPFourNestedLocks}{\cna}
\newcommand{\sunflowWCPFiveNestedLocks}{\cna}
\newcommand{\sunflowWCPSixNestedLocks}{\cna}
\newcommand{\sunflowWCPSevenNestedLocks}{\cna}
\newcommand{\sunflowWCPEightNestedLocks}{\cna}
\newcommand{\sunflowWCPNineNestedLocks}{\cna}
\newcommand{\sunflowWCPTenNestedLocks}{\cna}
\newcommand{\sunflowWCPHundredNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPEventTotal}{9,700}
\newcommand{\sunflowFTOWCPNoFPEventTotal}{3.5}
\newcommand{\sunflowFTOWCPNoFPAccessTotal}{3.5}
\newcommand{\sunflowFTOWCPNoFPOtherTotal}{<0.1}
\newcommand{\sunflowFTOWCPReadTotal}{72.3}
\newcommand{\sunflowFTOWCPWriteTotal}{27.6}
\newcommand{\sunflowFTOWCPNoFPAccessInCS}{0.229}
\newcommand{\sunflowFTOWCPNoFPAccessOutCS}{99.8}
\newcommand{\sunflowFTOWCPAcqRelTotal}{3.95E-4}
\newcommand{\sunflowFTOWCPOtherTotal}{3.45E-5}
\newcommand{\sunflowFTOWCPNoFPReadTotal}{2.5}
\newcommand{\sunflowFTOWCPReadInCS}{1.09}
\newcommand{\sunflowFTOWCPReadOutCS}{139}
\newcommand{\sunflowFTOWCPReadSameEp}{40.5}
\newcommand{\sunflowFTOWCPReadSharedSameEp}{<0.001}
\newcommand{\sunflowFTOWCPReadExclusive}{5.94}
\newcommand{\sunflowFTOWCPReadOwned}{3.9}
\newcommand{\sunflowFTOWCPReadShare}{3.24}
\newcommand{\sunflowFTOWCPReadShared}{16.7}
\newcommand{\sunflowFTOWCPReadSharedOwned}{70.3}
\newcommand{\sunflowFTOWCPNoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowFTOWCPWriteInCS}{95.1}
\newcommand{\sunflowFTOWCPWriteOutCS}{41400}
\newcommand{\sunflowFTOWCPNoFPWriteTotal}{0.96}
\newcommand{\sunflowFTOWCPWriteSameEp}{41400}
\newcommand{\sunflowFTOWCPWriteExclusive}{<0.001}
\newcommand{\sunflowFTOWCPWriteOwned}{100}
\newcommand{\sunflowFTOWCPWriteShared}{<0.001}
\newcommand{\sunflowFTOWCPNoFPOtherEventTotal}{1703}
\newcommand{\sunflowFTOWCPAcqRelOtherTotal}{92.0}
\newcommand{\sunflowFTOWCPNoAcqRelOtherTotal}{137}
\newcommand{\sunflowFTOWCPFork}{11.7}
\newcommand{\sunflowFTOWCPJoin}{11.7}
\newcommand{\sunflowFTOWCPPreWait}{0.0}
\newcommand{\sunflowFTOWCPPostWait}{0.0}
\newcommand{\sunflowFTOWCPVolatileTotal}{0.0}
\newcommand{\sunflowFTOWCPClassInit}{13.9}
\newcommand{\sunflowFTOWCPClassAccess}{62.8}
\newcommand{\sunflowFTOWCPRaceTotal}{637}
\newcommand{\sunflowFTOWCPWrRdRace}{99.1}
\newcommand{\sunflowFTOWCPWrWrRace}{0.0}
\newcommand{\sunflowFTOWCPRdWrRace}{0.0}
\newcommand{\sunflowFTOWCPRdShWrRace}{0.785}
\newcommand{\sunflowFTOWCPHoldLocksTotal}{0.027}
\newcommand{\sunflowFTOWCPOneLockHeld}{0.77}
\newcommand{\sunflowFTOWCPTwoNestedLocks}{<0.1}
\newcommand{\sunflowFTOWCPThreeNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPFourNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPFiveNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPSixNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPSevenNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPEightNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPNineNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPTenNestedLocks}{\cna}
\newcommand{\sunflowFTOWCPHundredNestedLocks}{\cna}
\newcommand{\sunflowREWCPEventTotal}{9,700}
\newcommand{\sunflowREWCPNoFPEventTotal}{3.5}
\newcommand{\sunflowREWCPNoFPAccessTotal}{3.5}
\newcommand{\sunflowREWCPNoFPOtherTotal}{<0.1}
\newcommand{\sunflowREWCPReadTotal}{72.3}
\newcommand{\sunflowREWCPWriteTotal}{27.6}
\newcommand{\sunflowREWCPNoFPAccessInCS}{0.229}
\newcommand{\sunflowREWCPNoFPAccessOutCS}{99.8}
\newcommand{\sunflowREWCPAcqRelTotal}{3.94E-4}
\newcommand{\sunflowREWCPOtherTotal}{3.43E-5}
\newcommand{\sunflowREWCPNoFPReadTotal}{2.5}
\newcommand{\sunflowREWCPReadInCS}{1.09}
\newcommand{\sunflowREWCPReadOutCS}{140}
\newcommand{\sunflowREWCPReadSameEp}{40.5}
\newcommand{\sunflowREWCPReadSharedSameEp}{<0.001}
\newcommand{\sunflowREWCPReadExclusive}{5.79}
\newcommand{\sunflowREWCPReadOwned}{4.07}
\newcommand{\sunflowREWCPReadShare}{3.23}
\newcommand{\sunflowREWCPReadShared}{16.7}
\newcommand{\sunflowREWCPReadSharedOwned}{70.3}
\newcommand{\sunflowREWCPNoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowREWCPWriteInCS}{95.1}
\newcommand{\sunflowREWCPWriteOutCS}{41400}
\newcommand{\sunflowREWCPNoFPWriteTotal}{0.96}
\newcommand{\sunflowREWCPWriteSameEp}{41400}
\newcommand{\sunflowREWCPWriteExclusive}{<0.001}
\newcommand{\sunflowREWCPWriteOwned}{100}
\newcommand{\sunflowREWCPWriteShared}{0.0145}
\newcommand{\sunflowREWCPNoFPOtherEventTotal}{1701}
\newcommand{\sunflowREWCPAcqRelOtherTotal}{91.9}
\newcommand{\sunflowREWCPNoAcqRelOtherTotal}{136}
\newcommand{\sunflowREWCPFork}{11.8}
\newcommand{\sunflowREWCPJoin}{11.8}
\newcommand{\sunflowREWCPPreWait}{0.0}
\newcommand{\sunflowREWCPPostWait}{0.0}
\newcommand{\sunflowREWCPVolatileTotal}{0.0}
\newcommand{\sunflowREWCPClassInit}{14.0}
\newcommand{\sunflowREWCPClassAccess}{62.5}
\newcommand{\sunflowREWCPRaceTotal}{2012}
\newcommand{\sunflowREWCPWrRdRace}{99.8}
\newcommand{\sunflowREWCPWrWrRace}{0.0}
\newcommand{\sunflowREWCPRdWrRace}{0.0}
\newcommand{\sunflowREWCPRdShWrRace}{0.199}
\newcommand{\sunflowREWCPHoldLocksTotal}{0.027}
\newcommand{\sunflowREWCPOneLockHeld}{0.73}
\newcommand{\sunflowREWCPTwoNestedLocks}{<0.1}
\newcommand{\sunflowREWCPThreeNestedLocks}{\cna}
\newcommand{\sunflowREWCPFourNestedLocks}{\cna}
\newcommand{\sunflowREWCPFiveNestedLocks}{\cna}
\newcommand{\sunflowREWCPSixNestedLocks}{\cna}
\newcommand{\sunflowREWCPSevenNestedLocks}{\cna}
\newcommand{\sunflowREWCPEightNestedLocks}{\cna}
\newcommand{\sunflowREWCPNineNestedLocks}{\cna}
\newcommand{\sunflowREWCPTenNestedLocks}{\cna}
\newcommand{\sunflowREWCPHundredNestedLocks}{\cna}
\newcommand{\sunflowDCEventTotal}{9,700}
\newcommand{\sunflowDCNoFPEventTotal}{370}
\newcommand{\sunflowDCNoFPAccessTotal}{370}
\newcommand{\sunflowDCNoFPOtherTotal}{<0.1}
\newcommand{\sunflowDCReadTotal}{99.7}
\newcommand{\sunflowDCWriteTotal}{0.26}
\newcommand{\sunflowDCNoFPAccessInCS}{0.445}
\newcommand{\sunflowDCNoFPAccessOutCS}{99.6}
\newcommand{\sunflowDCAcqRelTotal}{3.94E-4}
\newcommand{\sunflowDCOtherTotal}{3.44E-5}
\newcommand{\sunflowDCNoFPReadTotal}{370}
\newcommand{\sunflowDCReadInCS}{0.235}
\newcommand{\sunflowDCReadOutCS}{100}
\newcommand{\sunflowDCReadSameEp}{0.277}
\newcommand{\sunflowDCReadSharedSameEp}{<0.001}
\newcommand{\sunflowDCReadExclusive}{99.4}
\newcommand{\sunflowDCReadOwned}{\cna}
\newcommand{\sunflowDCReadShare}{0.0221}
\newcommand{\sunflowDCReadShared}{0.594}
\newcommand{\sunflowDCReadSharedOwned}{\cna}
\newcommand{\sunflowDCNoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowDCWriteInCS}{95.1}
\newcommand{\sunflowDCWriteOutCS}{41400}
\newcommand{\sunflowDCNoFPWriteTotal}{0.96}
\newcommand{\sunflowDCWriteSameEp}{41400}
\newcommand{\sunflowDCWriteExclusive}{100}
\newcommand{\sunflowDCWriteOwned}{\cna}
\newcommand{\sunflowDCWriteShared}{<0.001}
\newcommand{\sunflowDCNoFPOtherEventTotal}{1702}
\newcommand{\sunflowDCAcqRelOtherTotal}{92.0}
\newcommand{\sunflowDCNoAcqRelOtherTotal}{137}
\newcommand{\sunflowDCFork}{11.7}
\newcommand{\sunflowDCJoin}{11.7}
\newcommand{\sunflowDCPreWait}{0.0}
\newcommand{\sunflowDCPostWait}{0.0}
\newcommand{\sunflowDCVolatileTotal}{0.0}
\newcommand{\sunflowDCClassInit}{13.9}
\newcommand{\sunflowDCClassAccess}{62.8}
\newcommand{\sunflowDCRaceTotal}{1406}
\newcommand{\sunflowDCWrRdRace}{99.7}
\newcommand{\sunflowDCWrWrRace}{0.0}
\newcommand{\sunflowDCRdWrRace}{0.0}
\newcommand{\sunflowDCRdShWrRace}{0.356}
\newcommand{\sunflowDCHoldLocksTotal}{2.6}
\newcommand{\sunflowDCOneLockHeld}{0.71}
\newcommand{\sunflowDCTwoNestedLocks}{<0.1}
\newcommand{\sunflowDCThreeNestedLocks}{\cna}
\newcommand{\sunflowDCFourNestedLocks}{\cna}
\newcommand{\sunflowDCFiveNestedLocks}{\cna}
\newcommand{\sunflowDCSixNestedLocks}{\cna}
\newcommand{\sunflowDCSevenNestedLocks}{\cna}
\newcommand{\sunflowDCEightNestedLocks}{\cna}
\newcommand{\sunflowDCNineNestedLocks}{\cna}
\newcommand{\sunflowDCTenNestedLocks}{\cna}
\newcommand{\sunflowDCHundredNestedLocks}{\cna}
\newcommand{\sunflowFTODCEventTotal}{9,700}
\newcommand{\sunflowFTODCNoFPEventTotal}{3.5}
\newcommand{\sunflowFTODCNoFPAccessTotal}{3.5}
\newcommand{\sunflowFTODCNoFPOtherTotal}{<0.1}
\newcommand{\sunflowFTODCReadTotal}{72.3}
\newcommand{\sunflowFTODCWriteTotal}{27.6}
\newcommand{\sunflowFTODCNoFPAccessInCS}{0.229}
\newcommand{\sunflowFTODCNoFPAccessOutCS}{99.8}
\newcommand{\sunflowFTODCAcqRelTotal}{3.95E-4}
\newcommand{\sunflowFTODCOtherTotal}{3.43E-5}
\newcommand{\sunflowFTODCNoFPReadTotal}{2.5}
\newcommand{\sunflowFTODCReadInCS}{1.09}
\newcommand{\sunflowFTODCReadOutCS}{139}
\newcommand{\sunflowFTODCReadSameEp}{40.5}
\newcommand{\sunflowFTODCReadSharedSameEp}{<0.001}
\newcommand{\sunflowFTODCReadExclusive}{5.96}
\newcommand{\sunflowFTODCReadOwned}{3.91}
\newcommand{\sunflowFTODCReadShare}{3.23}
\newcommand{\sunflowFTODCReadShared}{16.7}
\newcommand{\sunflowFTODCReadSharedOwned}{70.2}
\newcommand{\sunflowFTODCNoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowFTODCWriteInCS}{95.1}
\newcommand{\sunflowFTODCWriteOutCS}{41400}
\newcommand{\sunflowFTODCNoFPWriteTotal}{0.96}
\newcommand{\sunflowFTODCWriteSameEp}{41400}
\newcommand{\sunflowFTODCWriteExclusive}{<0.001}
\newcommand{\sunflowFTODCWriteOwned}{100}
\newcommand{\sunflowFTODCWriteShared}{<0.001}
\newcommand{\sunflowFTODCNoFPOtherEventTotal}{1702}
\newcommand{\sunflowFTODCAcqRelOtherTotal}{92.0}
\newcommand{\sunflowFTODCNoAcqRelOtherTotal}{136}
\newcommand{\sunflowFTODCFork}{11.8}
\newcommand{\sunflowFTODCJoin}{11.8}
\newcommand{\sunflowFTODCPreWait}{0.0}
\newcommand{\sunflowFTODCPostWait}{0.0}
\newcommand{\sunflowFTODCVolatileTotal}{0.0}
\newcommand{\sunflowFTODCClassInit}{14.0}
\newcommand{\sunflowFTODCClassAccess}{62.5}
\newcommand{\sunflowFTODCRaceTotal}{1332}
\newcommand{\sunflowFTODCWrRdRace}{99.6}
\newcommand{\sunflowFTODCWrWrRace}{0.0}
\newcommand{\sunflowFTODCRdWrRace}{0.0}
\newcommand{\sunflowFTODCRdShWrRace}{0.375}
\newcommand{\sunflowFTODCHoldLocksTotal}{0.027}
\newcommand{\sunflowFTODCOneLockHeld}{0.75}
\newcommand{\sunflowFTODCTwoNestedLocks}{<0.1}
\newcommand{\sunflowFTODCThreeNestedLocks}{\cna}
\newcommand{\sunflowFTODCFourNestedLocks}{\cna}
\newcommand{\sunflowFTODCFiveNestedLocks}{\cna}
\newcommand{\sunflowFTODCSixNestedLocks}{\cna}
\newcommand{\sunflowFTODCSevenNestedLocks}{\cna}
\newcommand{\sunflowFTODCEightNestedLocks}{\cna}
\newcommand{\sunflowFTODCNineNestedLocks}{\cna}
\newcommand{\sunflowFTODCTenNestedLocks}{\cna}
\newcommand{\sunflowFTODCHundredNestedLocks}{\cna}
\newcommand{\sunflowREDCEventTotal}{9,700}
\newcommand{\sunflowREDCNoFPEventTotal}{3.5}
\newcommand{\sunflowREDCNoFPAccessTotal}{3.5}
\newcommand{\sunflowREDCNoFPOtherTotal}{<0.1}
\newcommand{\sunflowREDCReadTotal}{72.3}
\newcommand{\sunflowREDCWriteTotal}{27.6}
\newcommand{\sunflowREDCNoFPAccessInCS}{0.229}
\newcommand{\sunflowREDCNoFPAccessOutCS}{99.8}
\newcommand{\sunflowREDCAcqRelTotal}{3.94E-4}
\newcommand{\sunflowREDCOtherTotal}{3.43E-5}
\newcommand{\sunflowREDCNoFPReadTotal}{2.5}
\newcommand{\sunflowREDCReadInCS}{1.09}
\newcommand{\sunflowREDCReadOutCS}{140}
\newcommand{\sunflowREDCReadSameEp}{40.5}
\newcommand{\sunflowREDCReadSharedSameEp}{<0.001}
\newcommand{\sunflowREDCReadExclusive}{5.79}
\newcommand{\sunflowREDCReadOwned}{4.05}
\newcommand{\sunflowREDCReadShare}{3.24}
\newcommand{\sunflowREDCReadShared}{16.7}
\newcommand{\sunflowREDCReadSharedOwned}{70.2}
\newcommand{\sunflowREDCNoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowREDCWriteInCS}{95.1}
\newcommand{\sunflowREDCWriteOutCS}{41400}
\newcommand{\sunflowREDCNoFPWriteTotal}{0.96}
\newcommand{\sunflowREDCWriteSameEp}{41400}
\newcommand{\sunflowREDCWriteExclusive}{<0.001}
\newcommand{\sunflowREDCWriteOwned}{100}
\newcommand{\sunflowREDCWriteShared}{0.0143}
\newcommand{\sunflowREDCNoFPOtherEventTotal}{1701}
\newcommand{\sunflowREDCAcqRelOtherTotal}{91.9}
\newcommand{\sunflowREDCNoAcqRelOtherTotal}{136}
\newcommand{\sunflowREDCFork}{11.8}
\newcommand{\sunflowREDCJoin}{11.8}
\newcommand{\sunflowREDCPreWait}{0.0}
\newcommand{\sunflowREDCPostWait}{0.0}
\newcommand{\sunflowREDCVolatileTotal}{0.0}
\newcommand{\sunflowREDCClassInit}{14.0}
\newcommand{\sunflowREDCClassAccess}{62.5}
\newcommand{\sunflowREDCRaceTotal}{4175}
\newcommand{\sunflowREDCWrRdRace}{99.9}
\newcommand{\sunflowREDCWrWrRace}{0.0}
\newcommand{\sunflowREDCRdWrRace}{0.0}
\newcommand{\sunflowREDCRdShWrRace}{0.0958}
\newcommand{\sunflowREDCHoldLocksTotal}{0.027}
\newcommand{\sunflowREDCOneLockHeld}{0.67}
\newcommand{\sunflowREDCTwoNestedLocks}{<0.1}
\newcommand{\sunflowREDCThreeNestedLocks}{\cna}
\newcommand{\sunflowREDCFourNestedLocks}{\cna}
\newcommand{\sunflowREDCFiveNestedLocks}{\cna}
\newcommand{\sunflowREDCSixNestedLocks}{\cna}
\newcommand{\sunflowREDCSevenNestedLocks}{\cna}
\newcommand{\sunflowREDCEightNestedLocks}{\cna}
\newcommand{\sunflowREDCNineNestedLocks}{\cna}
\newcommand{\sunflowREDCTenNestedLocks}{\cna}
\newcommand{\sunflowREDCHundredNestedLocks}{\cna}
\newcommand{\sunflowCAPOEventTotal}{9,700}
\newcommand{\sunflowCAPONoFPEventTotal}{370}
\newcommand{\sunflowCAPONoFPAccessTotal}{370}
\newcommand{\sunflowCAPONoFPOtherTotal}{<0.1}
\newcommand{\sunflowCAPOReadTotal}{99.7}
\newcommand{\sunflowCAPOWriteTotal}{0.26}
\newcommand{\sunflowCAPONoFPAccessInCS}{0.445}
\newcommand{\sunflowCAPONoFPAccessOutCS}{99.6}
\newcommand{\sunflowCAPOAcqRelTotal}{3.94E-4}
\newcommand{\sunflowCAPOOtherTotal}{3.44E-5}
\newcommand{\sunflowCAPONoFPReadTotal}{370}
\newcommand{\sunflowCAPOReadInCS}{0.235}
\newcommand{\sunflowCAPOReadOutCS}{100}
\newcommand{\sunflowCAPOReadSameEp}{0.277}
\newcommand{\sunflowCAPOReadSharedSameEp}{<0.001}
\newcommand{\sunflowCAPOReadExclusive}{99.4}
\newcommand{\sunflowCAPOReadOwned}{\cna}
\newcommand{\sunflowCAPOReadShare}{0.0221}
\newcommand{\sunflowCAPOReadShared}{0.594}
\newcommand{\sunflowCAPOReadSharedOwned}{\cna}
\newcommand{\sunflowCAPONoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowCAPOWriteInCS}{95.1}
\newcommand{\sunflowCAPOWriteOutCS}{41400}
\newcommand{\sunflowCAPONoFPWriteTotal}{0.96}
\newcommand{\sunflowCAPOWriteSameEp}{41400}
\newcommand{\sunflowCAPOWriteExclusive}{100}
\newcommand{\sunflowCAPOWriteOwned}{\cna}
\newcommand{\sunflowCAPOWriteShared}{<0.001}
\newcommand{\sunflowCAPONoFPOtherEventTotal}{1703}
\newcommand{\sunflowCAPOAcqRelOtherTotal}{92.0}
\newcommand{\sunflowCAPONoAcqRelOtherTotal}{137}
\newcommand{\sunflowCAPOFork}{11.7}
\newcommand{\sunflowCAPOJoin}{11.7}
\newcommand{\sunflowCAPOPreWait}{0.0}
\newcommand{\sunflowCAPOPostWait}{0.0}
\newcommand{\sunflowCAPOVolatileTotal}{0.0}
\newcommand{\sunflowCAPOClassInit}{13.9}
\newcommand{\sunflowCAPOClassAccess}{62.8}
\newcommand{\sunflowCAPORaceTotal}{1538}
\newcommand{\sunflowCAPOWrRdRace}{99.7}
\newcommand{\sunflowCAPOWrWrRace}{0.0}
\newcommand{\sunflowCAPORdWrRace}{0.0}
\newcommand{\sunflowCAPORdShWrRace}{0.325}
\newcommand{\sunflowCAPOHoldLocksTotal}{2.6}
\newcommand{\sunflowCAPOOneLockHeld}{0.71}
\newcommand{\sunflowCAPOTwoNestedLocks}{<0.1}
\newcommand{\sunflowCAPOThreeNestedLocks}{\cna}
\newcommand{\sunflowCAPOFourNestedLocks}{\cna}
\newcommand{\sunflowCAPOFiveNestedLocks}{\cna}
\newcommand{\sunflowCAPOSixNestedLocks}{\cna}
\newcommand{\sunflowCAPOSevenNestedLocks}{\cna}
\newcommand{\sunflowCAPOEightNestedLocks}{\cna}
\newcommand{\sunflowCAPONineNestedLocks}{\cna}
\newcommand{\sunflowCAPOTenNestedLocks}{\cna}
\newcommand{\sunflowCAPOHundredNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOEventTotal}{9,700}
\newcommand{\sunflowFTOCAPONoFPEventTotal}{3.5}
\newcommand{\sunflowFTOCAPONoFPAccessTotal}{3.5}
\newcommand{\sunflowFTOCAPONoFPOtherTotal}{<0.1}
\newcommand{\sunflowFTOCAPOReadTotal}{72.3}
\newcommand{\sunflowFTOCAPOWriteTotal}{27.6}
\newcommand{\sunflowFTOCAPONoFPAccessInCS}{0.229}
\newcommand{\sunflowFTOCAPONoFPAccessOutCS}{99.8}
\newcommand{\sunflowFTOCAPOAcqRelTotal}{3.95E-4}
\newcommand{\sunflowFTOCAPOOtherTotal}{3.45E-5}
\newcommand{\sunflowFTOCAPONoFPReadTotal}{2.5}
\newcommand{\sunflowFTOCAPOReadInCS}{1.09}
\newcommand{\sunflowFTOCAPOReadOutCS}{139}
\newcommand{\sunflowFTOCAPOReadSameEp}{40.5}
\newcommand{\sunflowFTOCAPOReadSharedSameEp}{<0.001}
\newcommand{\sunflowFTOCAPOReadExclusive}{6.11}
\newcommand{\sunflowFTOCAPOReadOwned}{3.72}
\newcommand{\sunflowFTOCAPOReadShare}{3.24}
\newcommand{\sunflowFTOCAPOReadShared}{16.7}
\newcommand{\sunflowFTOCAPOReadSharedOwned}{70.2}
\newcommand{\sunflowFTOCAPONoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowFTOCAPOWriteInCS}{95.1}
\newcommand{\sunflowFTOCAPOWriteOutCS}{41400}
\newcommand{\sunflowFTOCAPONoFPWriteTotal}{0.96}
\newcommand{\sunflowFTOCAPOWriteSameEp}{41400}
\newcommand{\sunflowFTOCAPOWriteExclusive}{<0.001}
\newcommand{\sunflowFTOCAPOWriteOwned}{100}
\newcommand{\sunflowFTOCAPOWriteShared}{<0.001}
\newcommand{\sunflowFTOCAPONoFPOtherEventTotal}{1704}
\newcommand{\sunflowFTOCAPOAcqRelOtherTotal}{92.0}
\newcommand{\sunflowFTOCAPONoAcqRelOtherTotal}{137}
\newcommand{\sunflowFTOCAPOFork}{11.7}
\newcommand{\sunflowFTOCAPOJoin}{11.7}
\newcommand{\sunflowFTOCAPOPreWait}{0.0}
\newcommand{\sunflowFTOCAPOPostWait}{0.0}
\newcommand{\sunflowFTOCAPOVolatileTotal}{0.0}
\newcommand{\sunflowFTOCAPOClassInit}{13.9}
\newcommand{\sunflowFTOCAPOClassAccess}{62.8}
\newcommand{\sunflowFTOCAPORaceTotal}{1315}
\newcommand{\sunflowFTOCAPOWrRdRace}{99.6}
\newcommand{\sunflowFTOCAPOWrWrRace}{0.0}
\newcommand{\sunflowFTOCAPORdWrRace}{0.0}
\newcommand{\sunflowFTOCAPORdShWrRace}{0.38}
\newcommand{\sunflowFTOCAPOHoldLocksTotal}{0.027}
\newcommand{\sunflowFTOCAPOOneLockHeld}{0.75}
\newcommand{\sunflowFTOCAPOTwoNestedLocks}{<0.1}
\newcommand{\sunflowFTOCAPOThreeNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOFourNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOSixNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOEightNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPONineNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOTenNestedLocks}{\cna}
\newcommand{\sunflowFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\sunflowRECAPOEventTotal}{9,700}
\newcommand{\sunflowRECAPONoFPEventTotal}{3.5}
\newcommand{\sunflowRECAPONoFPAccessTotal}{3.5}
\newcommand{\sunflowRECAPONoFPOtherTotal}{<0.1}
\newcommand{\sunflowRECAPOReadTotal}{72.3}
\newcommand{\sunflowRECAPOWriteTotal}{27.6}
\newcommand{\sunflowRECAPONoFPAccessInCS}{0.229}
\newcommand{\sunflowRECAPONoFPAccessOutCS}{99.8}
\newcommand{\sunflowRECAPOAcqRelTotal}{3.94E-4}
\newcommand{\sunflowRECAPOOtherTotal}{3.45E-5}
\newcommand{\sunflowRECAPONoFPReadTotal}{2.5}
\newcommand{\sunflowRECAPOReadInCS}{1.09}
\newcommand{\sunflowRECAPOReadOutCS}{140}
\newcommand{\sunflowRECAPOReadSameEp}{40.5}
\newcommand{\sunflowRECAPOReadSharedSameEp}{<0.001}
\newcommand{\sunflowRECAPOReadExclusive}{5.79}
\newcommand{\sunflowRECAPOReadOwned}{4.05}
\newcommand{\sunflowRECAPOReadShare}{3.24}
\newcommand{\sunflowRECAPOReadShared}{16.7}
\newcommand{\sunflowRECAPOReadSharedOwned}{70.3}
\newcommand{\sunflowRECAPONoFPHonestWriteTotal}{0.96}
\newcommand{\sunflowRECAPOWriteInCS}{95.1}
\newcommand{\sunflowRECAPOWriteOutCS}{41400}
\newcommand{\sunflowRECAPONoFPWriteTotal}{0.96}
\newcommand{\sunflowRECAPOWriteSameEp}{41400}
\newcommand{\sunflowRECAPOWriteExclusive}{<0.001}
\newcommand{\sunflowRECAPOWriteOwned}{100}
\newcommand{\sunflowRECAPOWriteShared}{0.0137}
\newcommand{\sunflowRECAPONoFPOtherEventTotal}{1701}
\newcommand{\sunflowRECAPOAcqRelOtherTotal}{91.9}
\newcommand{\sunflowRECAPONoAcqRelOtherTotal}{137}
\newcommand{\sunflowRECAPOFork}{11.7}
\newcommand{\sunflowRECAPOJoin}{11.7}
\newcommand{\sunflowRECAPOPreWait}{0.0}
\newcommand{\sunflowRECAPOPostWait}{0.0}
\newcommand{\sunflowRECAPOVolatileTotal}{0.0}
\newcommand{\sunflowRECAPOClassInit}{13.9}
\newcommand{\sunflowRECAPOClassAccess}{62.8}
\newcommand{\sunflowRECAPORaceTotal}{3394}
\newcommand{\sunflowRECAPOWrRdRace}{99.9}
\newcommand{\sunflowRECAPOWrWrRace}{0.0}
\newcommand{\sunflowRECAPORdWrRace}{0.0}
\newcommand{\sunflowRECAPORdShWrRace}{0.118}
\newcommand{\sunflowRECAPOHoldLocksTotal}{0.027}
\newcommand{\sunflowRECAPOOneLockHeld}{0.69}
\newcommand{\sunflowRECAPOTwoNestedLocks}{<0.1}
\newcommand{\sunflowRECAPOThreeNestedLocks}{\cna}
\newcommand{\sunflowRECAPOFourNestedLocks}{\cna}
\newcommand{\sunflowRECAPOFiveNestedLocks}{\cna}
\newcommand{\sunflowRECAPOSixNestedLocks}{\cna}
\newcommand{\sunflowRECAPOSevenNestedLocks}{\cna}
\newcommand{\sunflowRECAPOEightNestedLocks}{\cna}
\newcommand{\sunflowRECAPONineNestedLocks}{\cna}
\newcommand{\sunflowRECAPOTenNestedLocks}{\cna}
\newcommand{\sunflowRECAPOHundredNestedLocks}{\cna}
\newcommand{\sunflowCAPOTotalSetClears}{7.8E-4}
\newcommand{\sunflowCAPOReadSetZero}{0.0}
\newcommand{\sunflowCAPOReadSetOne}{72.2}
\newcommand{\sunflowCAPOReadSetGtOne}{27.8}
\newcommand{\sunflowCAPOWriteSetZero}{78.9}
\newcommand{\sunflowCAPOWriteSetOne}{19.9}
\newcommand{\sunflowCAPOWriteSetGtOne}{1.15}
\newcommand{\sunflowCAPOTotalMapClears}{7.8E-4}
\newcommand{\sunflowCAPOReadMapZero}{0.0}
\newcommand{\sunflowCAPOReadMapOne}{16.9}
\newcommand{\sunflowCAPOReadMapTen}{48.8}
\newcommand{\sunflowCAPOReadMapHund}{29.6}
\newcommand{\sunflowCAPOReadMapThou}{3.07}
\newcommand{\sunflowCAPOReadMapGtThou}{1.66}
\newcommand{\sunflowCAPOWriteMapZero}{16.9}
\newcommand{\sunflowCAPOWriteMapOne}{20.7}
\newcommand{\sunflowCAPOWriteMapTen}{8.05}
\newcommand{\sunflowCAPOWriteMapHund}{52.7}
\newcommand{\sunflowCAPOWriteMapThou}{0.0}
\newcommand{\sunflowCAPOWriteMapGtThou}{1.66}
\newcommand{\FASTsunflowMaxLiveThreads}{17}
\newcommand{\FASTsunflowTotalThreads}{17}
\newcommand{\FASTsunflowBaseTime}{1.4}
\newcommand{\FASTsunflowBaseTimeCI}{43}
\newcommand{\FASTsunflowEmptyTime}{\rna}
\newcommand{\FASTsunflowEmptyTimeCI}{\rna}
\newcommand{\FASTsunflowEmptyTimeCIMIN}{\rna}
\newcommand{\FASTsunflowEmptyTimeCIMAX}{\rna}
\newcommand{\FASTsunflowFTTime}{22}
\newcommand{\FASTsunflowFTTimeCI}{1.0}
\newcommand{\FASTsunflowHBTime}{26}
\newcommand{\FASTsunflowHBTimeCI}{1.7}
\newcommand{\FASTsunflowFTOHBTime}{24}
\newcommand{\FASTsunflowFTOHBTimeCI}{0.73}
\newcommand{\FASTsunflowWCPTime}{27}
\newcommand{\FASTsunflowWCPTimeCI}{0.75}
\newcommand{\FASTsunflowFTOWCPTime}{25}
\newcommand{\FASTsunflowFTOWCPTimeCI}{0.72}
\newcommand{\FASTsunflowREWCPTime}{29}
\newcommand{\FASTsunflowREWCPTimeCI}{1.0}
\newcommand{\FASTsunflowDCTime}{27}
\newcommand{\FASTsunflowDCTimeCI}{1.0}
\newcommand{\FASTsunflowFTODCTime}{25}
\newcommand{\FASTsunflowFTODCTimeCI}{0.71}
\newcommand{\FASTsunflowREDCTime}{30}
\newcommand{\FASTsunflowREDCTimeCI}{1.3}
\newcommand{\FASTsunflowCAPOTime}{27}
\newcommand{\FASTsunflowCAPOTimeCI}{0.95}
\newcommand{\FASTsunflowFTOCAPOTime}{25}
\newcommand{\FASTsunflowFTOCAPOTimeCI}{0.96}
\newcommand{\FASTsunflowRECAPOTime}{28}
\newcommand{\FASTsunflowRECAPOTimeCI}{1.2}
\newcommand{\FASTsunflowAGGCAPOTime}{\rna}
\newcommand{\FASTsunflowAGGCAPOTimeCI}{\rna}
\newcommand{\FASTsunflowAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTsunflowAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTsunflowStaticTime}{\rzero}
\newcommand{\FASTsunflowDynamicTime}{\rzero}
\newcommand{\FASTsunflowBaseMem}{610}
\newcommand{\FASTsunflowBaseMemCI}{0.86}
\newcommand{\FASTsunflowFTMem}{8.2}
\newcommand{\FASTsunflowFTMemCI}{0.051}
\newcommand{\FASTsunflowHBMem}{8.2}
\newcommand{\FASTsunflowHBMemCI}{0.023}
\newcommand{\FASTsunflowFTOHBMem}{8.2}
\newcommand{\FASTsunflowFTOHBMemCI}{0.045}
\newcommand{\FASTsunflowWCPMem}{9.0}
\newcommand{\FASTsunflowWCPMemCI}{0.05}
\newcommand{\FASTsunflowFTOWCPMem}{9.0}
\newcommand{\FASTsunflowFTOWCPMemCI}{0.02}
\newcommand{\FASTsunflowREWCPMem}{38}
\newcommand{\FASTsunflowREWCPMemCI}{0.066}
\newcommand{\FASTsunflowDCMem}{9.0}
\newcommand{\FASTsunflowDCMemCI}{0.029}
\newcommand{\FASTsunflowFTODCMem}{9.0}
\newcommand{\FASTsunflowFTODCMemCI}{0.042}
\newcommand{\FASTsunflowREDCMem}{38}
\newcommand{\FASTsunflowREDCMemCI}{0.089}
\newcommand{\FASTsunflowCAPOMem}{9.0}
\newcommand{\FASTsunflowCAPOMemCI}{0.035}
\newcommand{\FASTsunflowFTOCAPOMem}{9.0}
\newcommand{\FASTsunflowFTOCAPOMemCI}{0.037}
\newcommand{\FASTsunflowRECAPOMem}{38}
\newcommand{\FASTsunflowRECAPOMemCI}{0.12}
\newcommand{\FASTsunflowAGGCAPOMem}{\memna}
\newcommand{\FASTsunflowAGGCAPOMemCI}{\memna}
\newcommand{\FASTsunflowAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTsunflowAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTsunflowEventsCI}{0}
\newcommand{\FASTsunflowEventsCIMIN}{9,681,321,385}
\newcommand{\FASTsunflowEventsCIMAX}{9,681,321,385}
\newcommand{\FASTsunflowNoFPEventsCI}{611}
\newcommand{\FASTsunflowNoFPEventsCIMIN}{396,882,543}
\newcommand{\FASTsunflowNoFPEventsCIMAX}{396,883,765}
\newcommand{\FASTsunflowFT}{5}
\newcommand{\FASTsunflowFTCI}{0}
\newcommand{\FASTsunflowFTCIMIN}{5}
\newcommand{\FASTsunflowFTCIMAX}{5}
\newcommand{\FASTsunflowFTDynamic}{60}
\newcommand{\FASTsunflowFTDynamicCI}{2}
\newcommand{\FASTsunflowFTDynamicCIMIN}{58}
\newcommand{\FASTsunflowFTDynamicCIMAX}{62}
\newcommand{\FASTsunflowHB}{6}
\newcommand{\FASTsunflowHBCI}{0}
\newcommand{\FASTsunflowHBCIMIN}{6}
\newcommand{\FASTsunflowHBCIMAX}{6}
\newcommand{\FASTsunflowHBDynamic}{45}
\newcommand{\FASTsunflowHBDynamicCI}{6}
\newcommand{\FASTsunflowHBDynamicCIMIN}{39}
\newcommand{\FASTsunflowHBDynamicCIMAX}{51}
\newcommand{\FASTsunflowFTOHB}{6}
\newcommand{\FASTsunflowFTOHBCI}{0}
\newcommand{\FASTsunflowFTOHBCIMIN}{6}
\newcommand{\FASTsunflowFTOHBCIMAX}{6}
\newcommand{\FASTsunflowFTOHBDynamic}{44}
\newcommand{\FASTsunflowFTOHBDynamicCI}{3}
\newcommand{\FASTsunflowFTOHBDynamicCIMIN}{41}
\newcommand{\FASTsunflowFTOHBDynamicCIMAX}{47}
\newcommand{\FASTsunflowWCP}{27}
\newcommand{\FASTsunflowWCPCI}{0}
\newcommand{\FASTsunflowWCPCIMIN}{27}
\newcommand{\FASTsunflowWCPCIMAX}{27}
\newcommand{\FASTsunflowWCPDynamic}{718}
\newcommand{\FASTsunflowWCPDynamicCI}{79}
\newcommand{\FASTsunflowWCPDynamicCIMIN}{639}
\newcommand{\FASTsunflowWCPDynamicCIMAX}{797}
\newcommand{\FASTsunflowFTOWCP}{27}
\newcommand{\FASTsunflowFTOWCPCI}{0}
\newcommand{\FASTsunflowFTOWCPCIMIN}{27}
\newcommand{\FASTsunflowFTOWCPCIMAX}{27}
\newcommand{\FASTsunflowFTOWCPDynamic}{637}
\newcommand{\FASTsunflowFTOWCPDynamicCI}{84}
\newcommand{\FASTsunflowFTOWCPDynamicCIMIN}{553}
\newcommand{\FASTsunflowFTOWCPDynamicCIMAX}{721}
\newcommand{\FASTsunflowREWCP}{69}
\newcommand{\FASTsunflowREWCPCI}{7}
\newcommand{\FASTsunflowREWCPCIMIN}{62}
\newcommand{\FASTsunflowREWCPCIMAX}{76}
\newcommand{\FASTsunflowREWCPDynamic}{2,012}
\newcommand{\FASTsunflowREWCPDynamicCI}{298}
\newcommand{\FASTsunflowREWCPDynamicCIMIN}{1,714}
\newcommand{\FASTsunflowREWCPDynamicCIMAX}{2,310}
\newcommand{\FASTsunflowDC}{28}
\newcommand{\FASTsunflowDCCI}{0}
\newcommand{\FASTsunflowDCCIMIN}{28}
\newcommand{\FASTsunflowDCCIMAX}{28}
\newcommand{\FASTsunflowDCDynamic}{1,406}
\newcommand{\FASTsunflowDCDynamicCI}{124}
\newcommand{\FASTsunflowDCDynamicCIMIN}{1,282}
\newcommand{\FASTsunflowDCDynamicCIMAX}{1,530}
\newcommand{\FASTsunflowFTODC}{28}
\newcommand{\FASTsunflowFTODCCI}{0}
\newcommand{\FASTsunflowFTODCCIMIN}{28}
\newcommand{\FASTsunflowFTODCCIMAX}{28}
\newcommand{\FASTsunflowFTODCDynamic}{1,332}
\newcommand{\FASTsunflowFTODCDynamicCI}{205}
\newcommand{\FASTsunflowFTODCDynamicCIMIN}{1,127}
\newcommand{\FASTsunflowFTODCDynamicCIMAX}{1,537}
\newcommand{\FASTsunflowREDC}{93}
\newcommand{\FASTsunflowREDCCI}{5}
\newcommand{\FASTsunflowREDCCIMIN}{88}
\newcommand{\FASTsunflowREDCCIMAX}{98}
\newcommand{\FASTsunflowREDCDynamic}{4,175}
\newcommand{\FASTsunflowREDCDynamicCI}{448}
\newcommand{\FASTsunflowREDCDynamicCIMIN}{3,727}
\newcommand{\FASTsunflowREDCDynamicCIMAX}{4,623}
\newcommand{\FASTsunflowCAPO}{28}
\newcommand{\FASTsunflowCAPOCI}{0}
\newcommand{\FASTsunflowCAPOCIMIN}{28}
\newcommand{\FASTsunflowCAPOCIMAX}{28}
\newcommand{\FASTsunflowCAPODynamic}{1,538}
\newcommand{\FASTsunflowCAPODynamicCI}{145}
\newcommand{\FASTsunflowCAPODynamicCIMIN}{1,393}
\newcommand{\FASTsunflowCAPODynamicCIMAX}{1,683}
\newcommand{\FASTsunflowFTOCAPO}{28}
\newcommand{\FASTsunflowFTOCAPOCI}{0}
\newcommand{\FASTsunflowFTOCAPOCIMIN}{28}
\newcommand{\FASTsunflowFTOCAPOCIMAX}{28}
\newcommand{\FASTsunflowFTOCAPODynamic}{1,315}
\newcommand{\FASTsunflowFTOCAPODynamicCI}{227}
\newcommand{\FASTsunflowFTOCAPODynamicCIMIN}{1,088}
\newcommand{\FASTsunflowFTOCAPODynamicCIMAX}{1,542}
\newcommand{\FASTsunflowRECAPO}{90}
\newcommand{\FASTsunflowRECAPOCI}{8}
\newcommand{\FASTsunflowRECAPOCIMIN}{82}
\newcommand{\FASTsunflowRECAPOCIMAX}{98}
\newcommand{\FASTsunflowRECAPODynamic}{3,394}
\newcommand{\FASTsunflowRECAPODynamicCI}{612}
\newcommand{\FASTsunflowRECAPODynamicCIMIN}{2,782}
\newcommand{\FASTsunflowRECAPODynamicCIMAX}{4,006}
\newcommand{\FASTsunflowAGGCAPO}{\rna}
\newcommand{\FASTsunflowAGGCAPOCI}{\rna}
\newcommand{\FASTsunflowAGGCAPOCIMIN}{\rna}
\newcommand{\FASTsunflowAGGCAPOCIMAX}{\rna}
\newcommand{\FASTsunflowAGGCAPODynamic}{\rna}
\newcommand{\FASTsunflowAGGCAPODynamicCI}{\rna}
\newcommand{\FASTsunflowAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTsunflowAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTtomcatEvents}{63}
\newcommand{\FASTtomcatNoFPEvents}{22}
\newcommand{\tomcatHBEventTotal}{51}
\newcommand{\tomcatHBNoFPEventTotal}{13}
\newcommand{\tomcatHBNoFPAccessTotal}{12}
\newcommand{\tomcatHBNoFPOtherTotal}{0.88}
\newcommand{\tomcatHBReadTotal}{45.5}
\newcommand{\tomcatHBWriteTotal}{47.5}
\newcommand{\tomcatHBNoFPAccessInCS}{1.86}
\newcommand{\tomcatHBNoFPAccessOutCS}{91.4}
\newcommand{\tomcatHBAcqRelTotal}{3.48}
\newcommand{\tomcatHBOtherTotal}{0.306}
\newcommand{\tomcatHBNoFPReadTotal}{5.8}
\newcommand{\tomcatHBReadInCS}{25.9}
\newcommand{\tomcatHBReadOutCS}{309}
\newcommand{\tomcatHBReadSameEp}{95.3}
\newcommand{\tomcatHBReadSharedSameEp}{<0.001}
\newcommand{\tomcatHBReadExclusive}{49.8}
\newcommand{\tomcatHBReadOwned}{\cna}
\newcommand{\tomcatHBReadShare}{0.126}
\newcommand{\tomcatHBReadShared}{50.1}
\newcommand{\tomcatHBReadSharedOwned}{\cna}
\newcommand{\tomcatHBNoFPHonestWriteTotal}{6.0}
\newcommand{\tomcatHBWriteInCS}{4.0}
\newcommand{\tomcatHBWriteOutCS}{110}
\newcommand{\tomcatHBNoFPWriteTotal}{6.0}
\newcommand{\tomcatHBWriteSameEp}{14}
\newcommand{\tomcatHBWriteExclusive}{94.8}
\newcommand{\tomcatHBWriteOwned}{\cna}
\newcommand{\tomcatHBWriteShared}{5.15}
\newcommand{\tomcatHBNoFPOtherEventTotal}{883115}
\newcommand{\tomcatHBAcqRelOtherTotal}{91.9}
\newcommand{\tomcatHBNoAcqRelOtherTotal}{71356}
\newcommand{\tomcatHBFork}{0.035}
\newcommand{\tomcatHBJoin}{0.0126}
\newcommand{\tomcatHBPreWait}{0.0112}
\newcommand{\tomcatHBPostWait}{0.00981}
\newcommand{\tomcatHBVolatileTotal}{98.1}
\newcommand{\tomcatHBClassInit}{0.346}
\newcommand{\tomcatHBClassAccess}{1.5}
\newcommand{\tomcatHBRaceTotal}{12641710}
\newcommand{\tomcatHBWrRdRace}{63.5}
\newcommand{\tomcatHBWrWrRace}{26.4}
\newcommand{\tomcatHBRdWrRace}{8.66}
\newcommand{\tomcatHBRdShWrRace}{1.44}
\newcommand{\tomcatHBHoldLocksTotal}{2.0}
\newcommand{\tomcatHBOneLockHeld}{<0.1}
\newcommand{\tomcatHBTwoNestedLocks}{<0.1}
\newcommand{\tomcatHBThreeNestedLocks}{<0.1}
\newcommand{\tomcatHBFourNestedLocks}{<0.1}
\newcommand{\tomcatHBFiveNestedLocks}{<0.1}
\newcommand{\tomcatHBSixNestedLocks}{<0.1}
\newcommand{\tomcatHBSevenNestedLocks}{<0.1}
\newcommand{\tomcatHBEightNestedLocks}{<0.1}
\newcommand{\tomcatHBNineNestedLocks}{<0.1}
\newcommand{\tomcatHBTenNestedLocks}{<0.1}
\newcommand{\tomcatHBHundredNestedLocks}{\cna}
\newcommand{\tomcatFTOHBEventTotal}{47}
\newcommand{\tomcatFTOHBNoFPEventTotal}{8.6}
\newcommand{\tomcatFTOHBNoFPAccessTotal}{7.7}
\newcommand{\tomcatFTOHBNoFPOtherTotal}{0.88}
\newcommand{\tomcatFTOHBReadTotal}{60.4}
\newcommand{\tomcatFTOHBWriteTotal}{29.3}
\newcommand{\tomcatFTOHBNoFPAccessInCS}{1.97}
\newcommand{\tomcatFTOHBNoFPAccessOutCS}{98.0}
\newcommand{\tomcatFTOHBAcqRelTotal}{4.29}
\newcommand{\tomcatFTOHBOtherTotal}{0.377}
\newcommand{\tomcatFTOHBNoFPReadTotal}{5.2}
\newcommand{\tomcatFTOHBReadInCS}{28.3}
\newcommand{\tomcatFTOHBReadOutCS}{335}
\newcommand{\tomcatFTOHBReadSameEp}{106}
\newcommand{\tomcatFTOHBReadSharedSameEp}{<0.001}
\newcommand{\tomcatFTOHBReadExclusive}{8.53}
\newcommand{\tomcatFTOHBReadOwned}{38.2}
\newcommand{\tomcatFTOHBReadShare}{0.534}
\newcommand{\tomcatFTOHBReadShared}{2.26}
\newcommand{\tomcatFTOHBReadSharedOwned}{50.4}
\newcommand{\tomcatFTOHBNoFPHonestWriteTotal}{2.5}
\newcommand{\tomcatFTOHBWriteInCS}{9.56}
\newcommand{\tomcatFTOHBWriteOutCS}{264}
\newcommand{\tomcatFTOHBNoFPWriteTotal}{2.5}
\newcommand{\tomcatFTOHBWriteSameEp}{33.5}
\newcommand{\tomcatFTOHBWriteExclusive}{53.8}
\newcommand{\tomcatFTOHBWriteOwned}{45.3}
\newcommand{\tomcatFTOHBWriteShared}{0.845}
\newcommand{\tomcatFTOHBNoFPOtherEventTotal}{884020}
\newcommand{\tomcatFTOHBAcqRelOtherTotal}{91.9}
\newcommand{\tomcatFTOHBNoAcqRelOtherTotal}{71434}
\newcommand{\tomcatFTOHBFork}{0.035}
\newcommand{\tomcatFTOHBJoin}{0.0126}
\newcommand{\tomcatFTOHBPreWait}{0.0112}
\newcommand{\tomcatFTOHBPostWait}{0.0098}
\newcommand{\tomcatFTOHBVolatileTotal}{98.1}
\newcommand{\tomcatFTOHBClassInit}{0.346}
\newcommand{\tomcatFTOHBClassAccess}{1.52}
\newcommand{\tomcatFTOHBRaceTotal}{11696379}
\newcommand{\tomcatFTOHBWrRdRace}{69.9}
\newcommand{\tomcatFTOHBWrWrRace}{0.0}
\newcommand{\tomcatFTOHBRdWrRace}{29.3}
\newcommand{\tomcatFTOHBRdShWrRace}{0.836}
\newcommand{\tomcatFTOHBHoldLocksTotal}{1.6}
\newcommand{\tomcatFTOHBOneLockHeld}{<0.1}
\newcommand{\tomcatFTOHBTwoNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBThreeNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBFourNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBFiveNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBSixNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBSevenNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBEightNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBNineNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBTenNestedLocks}{<0.1}
\newcommand{\tomcatFTOHBHundredNestedLocks}{\cna}
\newcommand{\tomcatFTOWCPEventTotal}{47}
\newcommand{\tomcatFTOWCPNoFPEventTotal}{8.8}
\newcommand{\tomcatFTOWCPNoFPAccessTotal}{7.9}
\newcommand{\tomcatFTOWCPNoFPOtherTotal}{0.89}
\newcommand{\tomcatFTOWCPReadTotal}{60.2}
\newcommand{\tomcatFTOWCPWriteTotal}{29.7}
\newcommand{\tomcatFTOWCPNoFPAccessInCS}{2.02}
\newcommand{\tomcatFTOWCPNoFPAccessOutCS}{98.0}
\newcommand{\tomcatFTOWCPAcqRelTotal}{4.38}
\newcommand{\tomcatFTOWCPOtherTotal}{0.385}
\newcommand{\tomcatFTOWCPNoFPReadTotal}{5.3}
\newcommand{\tomcatFTOWCPReadInCS}{29}
\newcommand{\tomcatFTOWCPReadOutCS}{326}
\newcommand{\tomcatFTOWCPReadSameEp}{104}
\newcommand{\tomcatFTOWCPReadSharedSameEp}{<0.001}
\newcommand{\tomcatFTOWCPReadExclusive}{8.06}
\newcommand{\tomcatFTOWCPReadOwned}{35.9}
\newcommand{\tomcatFTOWCPReadShare}{0.533}
\newcommand{\tomcatFTOWCPReadShared}{2.16}
\newcommand{\tomcatFTOWCPReadSharedOwned}{53.3}
\newcommand{\tomcatFTOWCPNoFPHonestWriteTotal}{2.6}
\newcommand{\tomcatFTOWCPWriteInCS}{9.38}
\newcommand{\tomcatFTOWCPWriteOutCS}{254}
\newcommand{\tomcatFTOWCPNoFPWriteTotal}{2.6}
\newcommand{\tomcatFTOWCPWriteSameEp}{32.6}
\newcommand{\tomcatFTOWCPWriteExclusive}{51.7}
\newcommand{\tomcatFTOWCPWriteOwned}{47.4}
\newcommand{\tomcatFTOWCPWriteShared}{0.83}
\newcommand{\tomcatFTOWCPNoFPOtherEventTotal}{885521}
\newcommand{\tomcatFTOWCPAcqRelOtherTotal}{91.9}
\newcommand{\tomcatFTOWCPNoAcqRelOtherTotal}{71545}
\newcommand{\tomcatFTOWCPFork}{0.0349}
\newcommand{\tomcatFTOWCPJoin}{0.0126}
\newcommand{\tomcatFTOWCPPreWait}{0.0112}
\newcommand{\tomcatFTOWCPPostWait}{0.00978}
\newcommand{\tomcatFTOWCPVolatileTotal}{98.1}
\newcommand{\tomcatFTOWCPClassInit}{0.345}
\newcommand{\tomcatFTOWCPClassAccess}{1.5}
\newcommand{\tomcatFTOWCPRaceTotal}{11360288}
\newcommand{\tomcatFTOWCPWrRdRace}{70.0}
\newcommand{\tomcatFTOWCPWrWrRace}{0.0}
\newcommand{\tomcatFTOWCPRdWrRace}{29.2}
\newcommand{\tomcatFTOWCPRdShWrRace}{0.811}
\newcommand{\tomcatFTOWCPHoldLocksTotal}{1.6}
\newcommand{\tomcatFTOWCPOneLockHeld}{<0.1}
\newcommand{\tomcatFTOWCPTwoNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPThreeNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPFourNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPFiveNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPSixNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPSevenNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPEightNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPNineNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPTenNestedLocks}{<0.1}
\newcommand{\tomcatFTOWCPHundredNestedLocks}{\cna}
\newcommand{\tomcatREWCPEventTotal}{70}
\newcommand{\tomcatREWCPNoFPEventTotal}{9.0}
\newcommand{\tomcatREWCPNoFPAccessTotal}{8.1}
\newcommand{\tomcatREWCPNoFPOtherTotal}{0.88}
\newcommand{\tomcatREWCPReadTotal}{60.3}
\newcommand{\tomcatREWCPWriteTotal}{29.9}
\newcommand{\tomcatREWCPNoFPAccessInCS}{23.9}
\newcommand{\tomcatREWCPNoFPAccessOutCS}{76.1}
\newcommand{\tomcatREWCPAcqRelTotal}{3.43}
\newcommand{\tomcatREWCPOtherTotal}{0.303}
\newcommand{\tomcatREWCPNoFPReadTotal}{5.4}
\newcommand{\tomcatREWCPReadInCS}{65.5}
\newcommand{\tomcatREWCPReadOutCS}{318}
\newcommand{\tomcatREWCPReadSameEp}{136}
\newcommand{\tomcatREWCPReadSharedSameEp}{0.00189}
\newcommand{\tomcatREWCPReadExclusive}{7.76}
\newcommand{\tomcatREWCPReadOwned}{36.8}
\newcommand{\tomcatREWCPReadShare}{0.644}
\newcommand{\tomcatREWCPReadShared}{2.19}
\newcommand{\tomcatREWCPReadSharedOwned}{52.6}
\newcommand{\tomcatREWCPNoFPHonestWriteTotal}{2.7}
\newcommand{\tomcatREWCPWriteInCS}{133}
\newcommand{\tomcatREWCPWriteOutCS}{246}
\newcommand{\tomcatREWCPNoFPWriteTotal}{2.7}
\newcommand{\tomcatREWCPWriteSameEp}{152}
\newcommand{\tomcatREWCPWriteExclusive}{50.7}
\newcommand{\tomcatREWCPWriteOwned}{48.3}
\newcommand{\tomcatREWCPWriteShared}{1.01}
\newcommand{\tomcatREWCPNoFPOtherEventTotal}{883993}
\newcommand{\tomcatREWCPAcqRelOtherTotal}{91.9}
\newcommand{\tomcatREWCPNoAcqRelOtherTotal}{71650}
\newcommand{\tomcatREWCPFork}{0.0349}
\newcommand{\tomcatREWCPJoin}{0.0126}
\newcommand{\tomcatREWCPPreWait}{0.0112}
\newcommand{\tomcatREWCPPostWait}{0.00977}
\newcommand{\tomcatREWCPVolatileTotal}{97.8}
\newcommand{\tomcatREWCPClassInit}{0.401}
\newcommand{\tomcatREWCPClassAccess}{1.74}
\newcommand{\tomcatREWCPRaceTotal}{11362682}
\newcommand{\tomcatREWCPWrRdRace}{70.1}
\newcommand{\tomcatREWCPWrWrRace}{0.0}
\newcommand{\tomcatREWCPRdWrRace}{29.1}
\newcommand{\tomcatREWCPRdShWrRace}{0.838}
\newcommand{\tomcatREWCPHoldLocksTotal}{1.9}
\newcommand{\tomcatREWCPOneLockHeld}{<0.1}
\newcommand{\tomcatREWCPTwoNestedLocks}{<0.1}
\newcommand{\tomcatREWCPThreeNestedLocks}{<0.1}
\newcommand{\tomcatREWCPFourNestedLocks}{<0.1}
\newcommand{\tomcatREWCPFiveNestedLocks}{<0.1}
\newcommand{\tomcatREWCPSixNestedLocks}{<0.1}
\newcommand{\tomcatREWCPSevenNestedLocks}{<0.1}
\newcommand{\tomcatREWCPEightNestedLocks}{<0.1}
\newcommand{\tomcatREWCPNineNestedLocks}{<0.1}
\newcommand{\tomcatREWCPTenNestedLocks}{<0.1}
\newcommand{\tomcatREWCPHundredNestedLocks}{\cna}
\newcommand{\tomcatFTODCEventTotal}{47}
\newcommand{\tomcatFTODCNoFPEventTotal}{8.8}
\newcommand{\tomcatFTODCNoFPAccessTotal}{7.9}
\newcommand{\tomcatFTODCNoFPOtherTotal}{0.88}
\newcommand{\tomcatFTODCReadTotal}{59.8}
\newcommand{\tomcatFTODCWriteTotal}{30.1}
\newcommand{\tomcatFTODCNoFPAccessInCS}{2.04}
\newcommand{\tomcatFTODCNoFPAccessOutCS}{98.0}
\newcommand{\tomcatFTODCAcqRelTotal}{4.41}
\newcommand{\tomcatFTODCOtherTotal}{0.388}
\newcommand{\tomcatFTODCNoFPReadTotal}{5.3}
\newcommand{\tomcatFTODCReadInCS}{28.9}
\newcommand{\tomcatFTODCReadOutCS}{325}
\newcommand{\tomcatFTODCReadSameEp}{105}
\newcommand{\tomcatFTODCReadSharedSameEp}{<0.001}
\newcommand{\tomcatFTODCReadExclusive}{8.17}
\newcommand{\tomcatFTODCReadOwned}{35.9}
\newcommand{\tomcatFTODCReadShare}{0.547}
\newcommand{\tomcatFTODCReadShared}{2.09}
\newcommand{\tomcatFTODCReadSharedOwned}{53.3}
\newcommand{\tomcatFTODCNoFPHonestWriteTotal}{2.6}
\newcommand{\tomcatFTODCWriteInCS}{9.16}
\newcommand{\tomcatFTODCWriteOutCS}{249}
\newcommand{\tomcatFTODCNoFPWriteTotal}{2.6}
\newcommand{\tomcatFTODCWriteSameEp}{32}
\newcommand{\tomcatFTODCWriteExclusive}{51.8}
\newcommand{\tomcatFTODCWriteOwned}{47.3}
\newcommand{\tomcatFTODCWriteShared}{0.842}
\newcommand{\tomcatFTODCNoFPOtherEventTotal}{882559}
\newcommand{\tomcatFTODCAcqRelOtherTotal}{91.9}
\newcommand{\tomcatFTODCNoAcqRelOtherTotal}{71307}
\newcommand{\tomcatFTODCFork}{0.0351}
\newcommand{\tomcatFTODCJoin}{0.0126}
\newcommand{\tomcatFTODCPreWait}{0.0112}
\newcommand{\tomcatFTODCPostWait}{0.00982}
\newcommand{\tomcatFTODCVolatileTotal}{98.1}
\newcommand{\tomcatFTODCClassInit}{0.346}
\newcommand{\tomcatFTODCClassAccess}{1.48}
\newcommand{\tomcatFTODCRaceTotal}{11173794}
\newcommand{\tomcatFTODCWrRdRace}{70.3}
\newcommand{\tomcatFTODCWrWrRace}{0.0}
\newcommand{\tomcatFTODCRdWrRace}{29.0}
\newcommand{\tomcatFTODCRdShWrRace}{0.784}
\newcommand{\tomcatFTODCHoldLocksTotal}{1.6}
\newcommand{\tomcatFTODCOneLockHeld}{<0.1}
\newcommand{\tomcatFTODCTwoNestedLocks}{<0.1}
\newcommand{\tomcatFTODCThreeNestedLocks}{<0.1}
\newcommand{\tomcatFTODCFourNestedLocks}{<0.1}
\newcommand{\tomcatFTODCFiveNestedLocks}{<0.1}
\newcommand{\tomcatFTODCSixNestedLocks}{<0.1}
\newcommand{\tomcatFTODCSevenNestedLocks}{<0.1}
\newcommand{\tomcatFTODCEightNestedLocks}{<0.1}
\newcommand{\tomcatFTODCNineNestedLocks}{<0.1}
\newcommand{\tomcatFTODCTenNestedLocks}{<0.1}
\newcommand{\tomcatFTODCHundredNestedLocks}{\cna}
\newcommand{\tomcatREDCEventTotal}{58}
\newcommand{\tomcatREDCNoFPEventTotal}{8.8}
\newcommand{\tomcatREDCNoFPAccessTotal}{7.9}
\newcommand{\tomcatREDCNoFPOtherTotal}{0.88}
\newcommand{\tomcatREDCReadTotal}{60.2}
\newcommand{\tomcatREDCWriteTotal}{29.8}
\newcommand{\tomcatREDCNoFPAccessInCS}{14.3}
\newcommand{\tomcatREDCNoFPAccessOutCS}{85.7}
\newcommand{\tomcatREDCAcqRelTotal}{3.83}
\newcommand{\tomcatREDCOtherTotal}{0.337}
\newcommand{\tomcatREDCNoFPReadTotal}{5.3}
\newcommand{\tomcatREDCReadInCS}{46.8}
\newcommand{\tomcatREDCReadOutCS}{324}
\newcommand{\tomcatREDCReadSameEp}{120}
\newcommand{\tomcatREDCReadSharedSameEp}{0.00132}
\newcommand{\tomcatREDCReadExclusive}{7.88}
\newcommand{\tomcatREDCReadOwned}{36}
\newcommand{\tomcatREDCReadShare}{0.661}
\newcommand{\tomcatREDCReadShared}{2.19}
\newcommand{\tomcatREDCReadSharedOwned}{53.3}
\newcommand{\tomcatREDCNoFPHonestWriteTotal}{2.6}
\newcommand{\tomcatREDCWriteInCS}{73.7}
\newcommand{\tomcatREDCWriteOutCS}{251}
\newcommand{\tomcatREDCNoFPWriteTotal}{2.6}
\newcommand{\tomcatREDCWriteSameEp}{95.2}
\newcommand{\tomcatREDCWriteExclusive}{51.9}
\newcommand{\tomcatREDCWriteOwned}{47.1}
\newcommand{\tomcatREDCWriteShared}{1.05}
\newcommand{\tomcatREDCNoFPOtherEventTotal}{882681}
\newcommand{\tomcatREDCAcqRelOtherTotal}{91.9}
\newcommand{\tomcatREDCNoAcqRelOtherTotal}{71484}
\newcommand{\tomcatREDCFork}{0.035}
\newcommand{\tomcatREDCJoin}{0.0126}
\newcommand{\tomcatREDCPreWait}{0.0112}
\newcommand{\tomcatREDCPostWait}{0.00979}
\newcommand{\tomcatREDCVolatileTotal}{97.9}
\newcommand{\tomcatREDCClassInit}{0.392}
\newcommand{\tomcatREDCClassAccess}{1.65}
\newcommand{\tomcatREDCRaceTotal}{11407952}
\newcommand{\tomcatREDCWrRdRace}{70.1}
\newcommand{\tomcatREDCWrWrRace}{0.0}
\newcommand{\tomcatREDCRdWrRace}{29.1}
\newcommand{\tomcatREDCRdShWrRace}{0.813}
\newcommand{\tomcatREDCHoldLocksTotal}{1.7}
\newcommand{\tomcatREDCOneLockHeld}{<0.1}
\newcommand{\tomcatREDCTwoNestedLocks}{<0.1}
\newcommand{\tomcatREDCThreeNestedLocks}{<0.1}
\newcommand{\tomcatREDCFourNestedLocks}{<0.1}
\newcommand{\tomcatREDCFiveNestedLocks}{<0.1}
\newcommand{\tomcatREDCSixNestedLocks}{<0.1}
\newcommand{\tomcatREDCSevenNestedLocks}{<0.1}
\newcommand{\tomcatREDCEightNestedLocks}{<0.1}
\newcommand{\tomcatREDCNineNestedLocks}{<0.1}
\newcommand{\tomcatREDCTenNestedLocks}{<0.1}
\newcommand{\tomcatREDCHundredNestedLocks}{\cna}
\newcommand{\tomcatFTOCAPOEventTotal}{47}
\newcommand{\tomcatFTOCAPONoFPEventTotal}{8.7}
\newcommand{\tomcatFTOCAPONoFPAccessTotal}{7.8}
\newcommand{\tomcatFTOCAPONoFPOtherTotal}{0.88}
\newcommand{\tomcatFTOCAPOReadTotal}{60.2}
\newcommand{\tomcatFTOCAPOWriteTotal}{29.7}
\newcommand{\tomcatFTOCAPONoFPAccessInCS}{2.02}
\newcommand{\tomcatFTOCAPONoFPAccessOutCS}{98.0}
\newcommand{\tomcatFTOCAPOAcqRelTotal}{4.36}
\newcommand{\tomcatFTOCAPOOtherTotal}{0.384}
\newcommand{\tomcatFTOCAPONoFPReadTotal}{5.3}
\newcommand{\tomcatFTOCAPOReadInCS}{29}
\newcommand{\tomcatFTOCAPOReadOutCS}{327}
\newcommand{\tomcatFTOCAPOReadSameEp}{105}
\newcommand{\tomcatFTOCAPOReadSharedSameEp}{<0.001}
\newcommand{\tomcatFTOCAPOReadExclusive}{8.03}
\newcommand{\tomcatFTOCAPOReadOwned}{35.8}
\newcommand{\tomcatFTOCAPOReadShare}{0.538}
\newcommand{\tomcatFTOCAPOReadShared}{2.16}
\newcommand{\tomcatFTOCAPOReadSharedOwned}{53.5}
\newcommand{\tomcatFTOCAPONoFPHonestWriteTotal}{2.6}
\newcommand{\tomcatFTOCAPOWriteInCS}{9.37}
\newcommand{\tomcatFTOCAPOWriteOutCS}{255}
\newcommand{\tomcatFTOCAPONoFPWriteTotal}{2.6}
\newcommand{\tomcatFTOCAPOWriteSameEp}{32.7}
\newcommand{\tomcatFTOCAPOWriteExclusive}{52.3}
\newcommand{\tomcatFTOCAPOWriteOwned}{46.9}
\newcommand{\tomcatFTOCAPOWriteShared}{0.839}
\newcommand{\tomcatFTOCAPONoFPOtherEventTotal}{883330}
\newcommand{\tomcatFTOCAPOAcqRelOtherTotal}{91.9}
\newcommand{\tomcatFTOCAPONoAcqRelOtherTotal}{71391}
\newcommand{\tomcatFTOCAPOFork}{0.035}
\newcommand{\tomcatFTOCAPOJoin}{0.0126}
\newcommand{\tomcatFTOCAPOPreWait}{0.0112}
\newcommand{\tomcatFTOCAPOPostWait}{0.00981}
\newcommand{\tomcatFTOCAPOVolatileTotal}{98.1}
\newcommand{\tomcatFTOCAPOClassInit}{0.346}
\newcommand{\tomcatFTOCAPOClassAccess}{1.51}
\newcommand{\tomcatFTOCAPORaceTotal}{11374205}
\newcommand{\tomcatFTOCAPOWrRdRace}{70.0}
\newcommand{\tomcatFTOCAPOWrWrRace}{0.0}
\newcommand{\tomcatFTOCAPORdWrRace}{29.1}
\newcommand{\tomcatFTOCAPORdShWrRace}{0.814}
\newcommand{\tomcatFTOCAPOHoldLocksTotal}{1.6}
\newcommand{\tomcatFTOCAPOOneLockHeld}{<0.1}
\newcommand{\tomcatFTOCAPOTwoNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOThreeNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOFourNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOFiveNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOSixNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOSevenNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOEightNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPONineNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOTenNestedLocks}{<0.1}
\newcommand{\tomcatFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\tomcatRECAPOEventTotal}{63}
\newcommand{\tomcatRECAPONoFPEventTotal}{8.8}
\newcommand{\tomcatRECAPONoFPAccessTotal}{7.9}
\newcommand{\tomcatRECAPONoFPOtherTotal}{0.88}
\newcommand{\tomcatRECAPOReadTotal}{60.4}
\newcommand{\tomcatRECAPOWriteTotal}{29.6}
\newcommand{\tomcatRECAPONoFPAccessInCS}{18.2}
\newcommand{\tomcatRECAPONoFPAccessOutCS}{81.8}
\newcommand{\tomcatRECAPOAcqRelTotal}{3.65}
\newcommand{\tomcatRECAPOOtherTotal}{0.321}
\newcommand{\tomcatRECAPONoFPReadTotal}{5.3}
\newcommand{\tomcatRECAPOReadInCS}{53.3}
\newcommand{\tomcatRECAPOReadOutCS}{323}
\newcommand{\tomcatRECAPOReadSameEp}{126}
\newcommand{\tomcatRECAPOReadSharedSameEp}{0.00176}
\newcommand{\tomcatRECAPOReadExclusive}{7.76}
\newcommand{\tomcatRECAPOReadOwned}{36.2}
\newcommand{\tomcatRECAPOReadShare}{0.646}
\newcommand{\tomcatRECAPOReadShared}{2.22}
\newcommand{\tomcatRECAPOReadSharedOwned}{53.2}
\newcommand{\tomcatRECAPONoFPHonestWriteTotal}{2.6}
\newcommand{\tomcatRECAPOWriteInCS}{99.8}
\newcommand{\tomcatRECAPOWriteOutCS}{253}
\newcommand{\tomcatRECAPONoFPWriteTotal}{2.6}
\newcommand{\tomcatRECAPOWriteSameEp}{121}
\newcommand{\tomcatRECAPOWriteExclusive}{51.7}
\newcommand{\tomcatRECAPOWriteOwned}{47.2}
\newcommand{\tomcatRECAPOWriteShared}{1.03}
\newcommand{\tomcatRECAPONoFPOtherEventTotal}{882799}
\newcommand{\tomcatRECAPOAcqRelOtherTotal}{91.9}
\newcommand{\tomcatRECAPONoAcqRelOtherTotal}{71487}
\newcommand{\tomcatRECAPOFork}{0.035}
\newcommand{\tomcatRECAPOJoin}{0.0126}
\newcommand{\tomcatRECAPOPreWait}{0.0112}
\newcommand{\tomcatRECAPOPostWait}{0.00979}
\newcommand{\tomcatRECAPOVolatileTotal}{97.9}
\newcommand{\tomcatRECAPOClassInit}{0.38}
\newcommand{\tomcatRECAPOClassAccess}{1.64}
\newcommand{\tomcatRECAPORaceTotal}{11489536}
\newcommand{\tomcatRECAPOWrRdRace}{69.9}
\newcommand{\tomcatRECAPOWrWrRace}{0.0}
\newcommand{\tomcatRECAPORdWrRace}{29.2}
\newcommand{\tomcatRECAPORdShWrRace}{0.869}
\newcommand{\tomcatRECAPOHoldLocksTotal}{1.8}
\newcommand{\tomcatRECAPOOneLockHeld}{<0.1}
\newcommand{\tomcatRECAPOTwoNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOThreeNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOFourNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOFiveNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOSixNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOSevenNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOEightNestedLocks}{<0.1}
\newcommand{\tomcatRECAPONineNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOTenNestedLocks}{<0.1}
\newcommand{\tomcatRECAPOHundredNestedLocks}{\cna}
\newcommand{\FASTtomcatMaxLiveThreads}{37}
\newcommand{\FASTtomcatTotalThreads}{37}
\newcommand{\FASTtomcatBaseTime}{0.92}
\newcommand{\FASTtomcatBaseTimeCI}{4.8}
\newcommand{\FASTtomcatEmptyTime}{\rna}
\newcommand{\FASTtomcatEmptyTimeCI}{\rna}
\newcommand{\FASTtomcatEmptyTimeCIMIN}{\rna}
\newcommand{\FASTtomcatEmptyTimeCIMAX}{\rna}
\newcommand{\FASTtomcatFTTime}{41}
\newcommand{\FASTtomcatFTTimeCI}{1.2}
\newcommand{\FASTtomcatHBTime}{93}
\newcommand{\FASTtomcatHBTimeCI}{4.4}
\newcommand{\FASTtomcatFTOHBTime}{100}
\newcommand{\FASTtomcatFTOHBTimeCI}{2.8}
\newcommand{\FASTtomcatWCPTime}{\rna}
\newcommand{\FASTtomcatWCPTimeCI}{\rna}
\newcommand{\FASTtomcatWCPTimeCIMIN}{\rna}
\newcommand{\FASTtomcatWCPTimeCIMAX}{\rna}
\newcommand{\FASTtomcatFTOWCPTime}{100}
\newcommand{\FASTtomcatFTOWCPTimeCI}{3.2}
\newcommand{\FASTtomcatREWCPTime}{96}
\newcommand{\FASTtomcatREWCPTimeCI}{5.0}
\newcommand{\FASTtomcatDCTime}{\rna}
\newcommand{\FASTtomcatDCTimeCI}{\rna}
\newcommand{\FASTtomcatDCTimeCIMIN}{\rna}
\newcommand{\FASTtomcatDCTimeCIMAX}{\rna}
\newcommand{\FASTtomcatFTODCTime}{100}
\newcommand{\FASTtomcatFTODCTimeCI}{4.4}
\newcommand{\FASTtomcatREDCTime}{96}
\newcommand{\FASTtomcatREDCTimeCI}{4.0}
\newcommand{\FASTtomcatCAPOTime}{\rna}
\newcommand{\FASTtomcatCAPOTimeCI}{\rna}
\newcommand{\FASTtomcatCAPOTimeCIMIN}{\rna}
\newcommand{\FASTtomcatCAPOTimeCIMAX}{\rna}
\newcommand{\FASTtomcatFTOCAPOTime}{100}
\newcommand{\FASTtomcatFTOCAPOTimeCI}{3.4}
\newcommand{\FASTtomcatRECAPOTime}{96}
\newcommand{\FASTtomcatRECAPOTimeCI}{7.9}
\newcommand{\FASTtomcatAGGCAPOTime}{\rna}
\newcommand{\FASTtomcatAGGCAPOTimeCI}{\rna}
\newcommand{\FASTtomcatAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTtomcatAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTtomcatStaticTime}{\rzero}
\newcommand{\FASTtomcatDynamicTime}{\rzero}
\newcommand{\FASTtomcatBaseMem}{510}
\newcommand{\FASTtomcatBaseMemCI}{2.5}
\newcommand{\FASTtomcatFTMem}{51}
\newcommand{\FASTtomcatFTMemCI}{5.1}
\newcommand{\FASTtomcatHBMem}{100}
\newcommand{\FASTtomcatHBMemCI}{17.0}
\newcommand{\FASTtomcatFTOHBMem}{95}
\newcommand{\FASTtomcatFTOHBMemCI}{16.0}
\newcommand{\FASTtomcatWCPMem}{\memna}
\newcommand{\FASTtomcatWCPMemCI}{\memna}
\newcommand{\FASTtomcatWCPMemCIMIN}{\memna}
\newcommand{\FASTtomcatWCPMemCIMAX}{\memna}
\newcommand{\FASTtomcatFTOWCPMem}{140}
\newcommand{\FASTtomcatFTOWCPMemCI}{0.77}
\newcommand{\FASTtomcatREWCPMem}{140}
\newcommand{\FASTtomcatREWCPMemCI}{3.8}
\newcommand{\FASTtomcatDCMem}{\memna}
\newcommand{\FASTtomcatDCMemCI}{\memna}
\newcommand{\FASTtomcatDCMemCIMIN}{\memna}
\newcommand{\FASTtomcatDCMemCIMAX}{\memna}
\newcommand{\FASTtomcatFTODCMem}{140}
\newcommand{\FASTtomcatFTODCMemCI}{0.44}
\newcommand{\FASTtomcatREDCMem}{140}
\newcommand{\FASTtomcatREDCMemCI}{4.4}
\newcommand{\FASTtomcatCAPOMem}{\memna}
\newcommand{\FASTtomcatCAPOMemCI}{\memna}
\newcommand{\FASTtomcatCAPOMemCIMIN}{\memna}
\newcommand{\FASTtomcatCAPOMemCIMAX}{\memna}
\newcommand{\FASTtomcatFTOCAPOMem}{110}
\newcommand{\FASTtomcatFTOCAPOMemCI}{15.0}
\newcommand{\FASTtomcatRECAPOMem}{130}
\newcommand{\FASTtomcatRECAPOMemCI}{6.4}
\newcommand{\FASTtomcatAGGCAPOMem}{\memna}
\newcommand{\FASTtomcatAGGCAPOMemCI}{\memna}
\newcommand{\FASTtomcatAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTtomcatAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTtomcatEventsCI}{16,981,722}
\newcommand{\FASTtomcatEventsCIMIN}{45,707,104}
\newcommand{\FASTtomcatEventsCIMAX}{79,670,548}
\newcommand{\FASTtomcatNoFPEventsCI}{3,896,752}
\newcommand{\FASTtomcatNoFPEventsCIMIN}{18,356,790}
\newcommand{\FASTtomcatNoFPEventsCIMAX}{26,150,294}
\newcommand{\FASTtomcatFT}{422}
\newcommand{\FASTtomcatFTCI}{4}
\newcommand{\FASTtomcatFTCIMIN}{418}
\newcommand{\FASTtomcatFTCIMAX}{426}
\newcommand{\FASTtomcatFTDynamic}{4,926,017}
\newcommand{\FASTtomcatFTDynamicCI}{124,800}
\newcommand{\FASTtomcatFTDynamicCIMIN}{4,801,217}
\newcommand{\FASTtomcatFTDynamicCIMAX}{5,050,817}
\newcommand{\FASTtomcatHB}{1,356}
\newcommand{\FASTtomcatHBCI}{17}
\newcommand{\FASTtomcatHBCIMIN}{1,339}
\newcommand{\FASTtomcatHBCIMAX}{1,373}
\newcommand{\FASTtomcatHBDynamic}{11,473,007}
\newcommand{\FASTtomcatHBDynamicCI}{454,089}
\newcommand{\FASTtomcatHBDynamicCIMIN}{11,018,918}
\newcommand{\FASTtomcatHBDynamicCIMAX}{11,927,096}
\newcommand{\FASTtomcatFTOHB}{1,359}
\newcommand{\FASTtomcatFTOHBCI}{19}
\newcommand{\FASTtomcatFTOHBCIMIN}{1,340}
\newcommand{\FASTtomcatFTOHBCIMAX}{1,378}
\newcommand{\FASTtomcatFTOHBDynamic}{11,696,340}
\newcommand{\FASTtomcatFTOHBDynamicCI}{275,750}
\newcommand{\FASTtomcatFTOHBDynamicCIMIN}{11,420,590}
\newcommand{\FASTtomcatFTOHBDynamicCIMAX}{11,972,090}
\newcommand{\FASTtomcatWCP}{\rna}
\newcommand{\FASTtomcatWCPCI}{\rna}
\newcommand{\FASTtomcatWCPCIMIN}{\rna}
\newcommand{\FASTtomcatWCPCIMAX}{\rna}
\newcommand{\FASTtomcatWCPDynamic}{\rna}
\newcommand{\FASTtomcatWCPDynamicCI}{\rna}
\newcommand{\FASTtomcatWCPDynamicCIMIN}{\rna}
\newcommand{\FASTtomcatWCPDynamicCIMAX}{\rna}
\newcommand{\FASTtomcatFTOWCP}{1,363}
\newcommand{\FASTtomcatFTOWCPCI}{16}
\newcommand{\FASTtomcatFTOWCPCIMIN}{1,347}
\newcommand{\FASTtomcatFTOWCPCIMAX}{1,379}
\newcommand{\FASTtomcatFTOWCPDynamic}{11,360,254}
\newcommand{\FASTtomcatFTOWCPDynamicCI}{401,808}
\newcommand{\FASTtomcatFTOWCPDynamicCIMIN}{10,958,446}
\newcommand{\FASTtomcatFTOWCPDynamicCIMAX}{11,762,062}
\newcommand{\FASTtomcatREWCP}{1,357}
\newcommand{\FASTtomcatREWCPCI}{20}
\newcommand{\FASTtomcatREWCPCIMIN}{1,337}
\newcommand{\FASTtomcatREWCPCIMAX}{1,377}
\newcommand{\FASTtomcatREWCPDynamic}{11,362,682}
\newcommand{\FASTtomcatREWCPDynamicCI}{434,073}
\newcommand{\FASTtomcatREWCPDynamicCIMIN}{10,928,609}
\newcommand{\FASTtomcatREWCPDynamicCIMAX}{11,796,755}
\newcommand{\FASTtomcatDC}{\rna}
\newcommand{\FASTtomcatDCCI}{\rna}
\newcommand{\FASTtomcatDCCIMIN}{\rna}
\newcommand{\FASTtomcatDCCIMAX}{\rna}
\newcommand{\FASTtomcatDCDynamic}{\rna}
\newcommand{\FASTtomcatDCDynamicCI}{\rna}
\newcommand{\FASTtomcatDCDynamicCIMIN}{\rna}
\newcommand{\FASTtomcatDCDynamicCIMAX}{\rna}
\newcommand{\FASTtomcatFTODC}{1,397}
\newcommand{\FASTtomcatFTODCCI}{18}
\newcommand{\FASTtomcatFTODCCIMIN}{1,379}
\newcommand{\FASTtomcatFTODCCIMAX}{1,415}
\newcommand{\FASTtomcatFTODCDynamic}{11,173,794}
\newcommand{\FASTtomcatFTODCDynamicCI}{453,049}
\newcommand{\FASTtomcatFTODCDynamicCIMIN}{10,720,745}
\newcommand{\FASTtomcatFTODCDynamicCIMAX}{11,626,843}
\newcommand{\FASTtomcatREDC}{1,418}
\newcommand{\FASTtomcatREDCCI}{14}
\newcommand{\FASTtomcatREDCCIMIN}{1,404}
\newcommand{\FASTtomcatREDCCIMAX}{1,432}
\newcommand{\FASTtomcatREDCDynamic}{11,407,916}
\newcommand{\FASTtomcatREDCDynamicCI}{476,781}
\newcommand{\FASTtomcatREDCDynamicCIMIN}{10,931,135}
\newcommand{\FASTtomcatREDCDynamicCIMAX}{11,884,697}
\newcommand{\FASTtomcatCAPO}{\rna}
\newcommand{\FASTtomcatCAPOCI}{\rna}
\newcommand{\FASTtomcatCAPOCIMIN}{\rna}
\newcommand{\FASTtomcatCAPOCIMAX}{\rna}
\newcommand{\FASTtomcatCAPODynamic}{\rna}
\newcommand{\FASTtomcatCAPODynamicCI}{\rna}
\newcommand{\FASTtomcatCAPODynamicCIMIN}{\rna}
\newcommand{\FASTtomcatCAPODynamicCIMAX}{\rna}
\newcommand{\FASTtomcatFTOCAPO}{1,393}
\newcommand{\FASTtomcatFTOCAPOCI}{18}
\newcommand{\FASTtomcatFTOCAPOCIMIN}{1,375}
\newcommand{\FASTtomcatFTOCAPOCIMAX}{1,411}
\newcommand{\FASTtomcatFTOCAPODynamic}{11,374,198}
\newcommand{\FASTtomcatFTOCAPODynamicCI}{394,202}
\newcommand{\FASTtomcatFTOCAPODynamicCIMIN}{10,979,996}
\newcommand{\FASTtomcatFTOCAPODynamicCIMAX}{11,768,400}
\newcommand{\FASTtomcatRECAPO}{1,420}
\newcommand{\FASTtomcatRECAPOCI}{21}
\newcommand{\FASTtomcatRECAPOCIMIN}{1,399}
\newcommand{\FASTtomcatRECAPOCIMAX}{1,441}
\newcommand{\FASTtomcatRECAPODynamic}{11,489,501}
\newcommand{\FASTtomcatRECAPODynamicCI}{463,620}
\newcommand{\FASTtomcatRECAPODynamicCIMIN}{11,025,881}
\newcommand{\FASTtomcatRECAPODynamicCIMAX}{11,953,121}
\newcommand{\FASTtomcatAGGCAPO}{\rna}
\newcommand{\FASTtomcatAGGCAPOCI}{\rna}
\newcommand{\FASTtomcatAGGCAPOCIMIN}{\rna}
\newcommand{\FASTtomcatAGGCAPOCIMAX}{\rna}
\newcommand{\FASTtomcatAGGCAPODynamic}{\rna}
\newcommand{\FASTtomcatAGGCAPODynamicCI}{\rna}
\newcommand{\FASTtomcatAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTtomcatAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTxalanEvents}{630}
\newcommand{\FASTxalanNoFPEvents}{53}
\newcommand{\xalanHBEventTotal}{630}
\newcommand{\xalanHBNoFPEventTotal}{240}
\newcommand{\xalanHBNoFPAccessTotal}{230}
\newcommand{\xalanHBNoFPOtherTotal}{8.9}
\newcommand{\xalanHBReadTotal}{79.5}
\newcommand{\xalanHBWriteTotal}{16.7}
\newcommand{\xalanHBNoFPAccessInCS}{98.5}
\newcommand{\xalanHBNoFPAccessOutCS}{1.49}
\newcommand{\xalanHBAcqRelTotal}{22.1}
\newcommand{\xalanHBOtherTotal}{4.78E-4}
\newcommand{\xalanHBNoFPReadTotal}{190}
\newcommand{\xalanHBReadInCS}{110}
\newcommand{\xalanHBReadOutCS}{0.0807}
\newcommand{\xalanHBReadSameEp}{10}
\newcommand{\xalanHBReadSharedSameEp}{\cna}
\newcommand{\xalanHBReadExclusive}{85.5}
\newcommand{\xalanHBReadOwned}{\cna}
\newcommand{\xalanHBReadShare}{0.00156}
\newcommand{\xalanHBReadShared}{14.5}
\newcommand{\xalanHBReadSharedOwned}{\cna}
\newcommand{\xalanHBNoFPHonestWriteTotal}{40}
\newcommand{\xalanHBWriteInCS}{130}
\newcommand{\xalanHBWriteOutCS}{1.16}
\newcommand{\xalanHBNoFPWriteTotal}{40}
\newcommand{\xalanHBWriteSameEp}{31}
\newcommand{\xalanHBWriteExclusive}{100}
\newcommand{\xalanHBWriteOwned}{\cna}
\newcommand{\xalanHBWriteShared}{<0.001}
\newcommand{\xalanHBNoFPOtherEventTotal}{8928441}
\newcommand{\xalanHBAcqRelOtherTotal}{100.0}
\newcommand{\xalanHBNoAcqRelOtherTotal}{193}
\newcommand{\xalanHBFork}{4.15}
\newcommand{\xalanHBJoin}{4.15}
\newcommand{\xalanHBPreWait}{3.63}
\newcommand{\xalanHBPostWait}{3.63}
\newcommand{\xalanHBVolatileTotal}{0.0}
\newcommand{\xalanHBClassInit}{16.6}
\newcommand{\xalanHBClassAccess}{67.9}
\newcommand{\xalanHBRaceTotal}{1428}
\newcommand{\xalanHBWrRdRace}{99.3}
\newcommand{\xalanHBWrWrRace}{0.0}
\newcommand{\xalanHBRdWrRace}{0.0}
\newcommand{\xalanHBRdShWrRace}{0.7}
\newcommand{\xalanHBHoldLocksTotal}{260}
\newcommand{\xalanHBOneLockHeld}{113.}
\newcommand{\xalanHBTwoNestedLocks}{113.}
\newcommand{\xalanHBThreeNestedLocks}{1.17}
\newcommand{\xalanHBFourNestedLocks}{<0.1}
\newcommand{\xalanHBFiveNestedLocks}{\cna}
\newcommand{\xalanHBSixNestedLocks}{\cna}
\newcommand{\xalanHBSevenNestedLocks}{\cna}
\newcommand{\xalanHBEightNestedLocks}{\cna}
\newcommand{\xalanHBNineNestedLocks}{\cna}
\newcommand{\xalanHBTenNestedLocks}{\cna}
\newcommand{\xalanHBHundredNestedLocks}{\cna}
\newcommand{\xalanFTOHBEventTotal}{630}
\newcommand{\xalanFTOHBNoFPEventTotal}{230}
\newcommand{\xalanFTOHBNoFPAccessTotal}{220}
\newcommand{\xalanFTOHBNoFPOtherTotal}{8.9}
\newcommand{\xalanFTOHBReadTotal}{79.1}
\newcommand{\xalanFTOHBWriteTotal}{17.1}
\newcommand{\xalanFTOHBNoFPAccessInCS}{98.5}
\newcommand{\xalanFTOHBNoFPAccessOutCS}{1.49}
\newcommand{\xalanFTOHBAcqRelTotal}{22.1}
\newcommand{\xalanFTOHBOtherTotal}{4.83E-4}
\newcommand{\xalanFTOHBNoFPReadTotal}{180}
\newcommand{\xalanFTOHBReadInCS}{110}
\newcommand{\xalanFTOHBReadOutCS}{0.0477}
\newcommand{\xalanFTOHBReadSameEp}{10.3}
\newcommand{\xalanFTOHBReadSharedSameEp}{<0.001}
\newcommand{\xalanFTOHBReadExclusive}{1.59}
\newcommand{\xalanFTOHBReadOwned}{83.6}
\newcommand{\xalanFTOHBReadShare}{0.00155}
\newcommand{\xalanFTOHBReadShared}{0.0093}
\newcommand{\xalanFTOHBReadSharedOwned}{14.8}
\newcommand{\xalanFTOHBNoFPHonestWriteTotal}{40}
\newcommand{\xalanFTOHBWriteInCS}{130}
\newcommand{\xalanFTOHBWriteOutCS}{1.16}
\newcommand{\xalanFTOHBNoFPWriteTotal}{40}
\newcommand{\xalanFTOHBWriteSameEp}{31}
\newcommand{\xalanFTOHBWriteExclusive}{9.73}
\newcommand{\xalanFTOHBWriteOwned}{90.3}
\newcommand{\xalanFTOHBWriteShared}{\cna}
\newcommand{\xalanFTOHBNoFPOtherEventTotal}{8928443}
\newcommand{\xalanFTOHBAcqRelOtherTotal}{100.0}
\newcommand{\xalanFTOHBNoAcqRelOtherTotal}{195}
\newcommand{\xalanFTOHBFork}{4.1}
\newcommand{\xalanFTOHBJoin}{4.1}
\newcommand{\xalanFTOHBPreWait}{4.1}
\newcommand{\xalanFTOHBPostWait}{4.1}
\newcommand{\xalanFTOHBVolatileTotal}{0.0}
\newcommand{\xalanFTOHBClassInit}{16.4}
\newcommand{\xalanFTOHBClassAccess}{67.2}
\newcommand{\xalanFTOHBRaceTotal}{1428}
\newcommand{\xalanFTOHBWrRdRace}{99.3}
\newcommand{\xalanFTOHBWrWrRace}{0.0}
\newcommand{\xalanFTOHBRdWrRace}{0.0}
\newcommand{\xalanFTOHBRdShWrRace}{0.7}
\newcommand{\xalanFTOHBHoldLocksTotal}{220}
\newcommand{\xalanFTOHBOneLockHeld}{99.9}
\newcommand{\xalanFTOHBTwoNestedLocks}{99.7}
\newcommand{\xalanFTOHBThreeNestedLocks}{1.10}
\newcommand{\xalanFTOHBFourNestedLocks}{\cna}
\newcommand{\xalanFTOHBFiveNestedLocks}{\cna}
\newcommand{\xalanFTOHBSixNestedLocks}{\cna}
\newcommand{\xalanFTOHBSevenNestedLocks}{\cna}
\newcommand{\xalanFTOHBEightNestedLocks}{\cna}
\newcommand{\xalanFTOHBNineNestedLocks}{\cna}
\newcommand{\xalanFTOHBTenNestedLocks}{\cna}
\newcommand{\xalanFTOHBHundredNestedLocks}{\cna}
\newcommand{\xalanWCPEventTotal}{640}
\newcommand{\xalanWCPNoFPEventTotal}{240}
\newcommand{\xalanWCPNoFPAccessTotal}{230}
\newcommand{\xalanWCPNoFPOtherTotal}{8.9}
\newcommand{\xalanWCPReadTotal}{79.3}
\newcommand{\xalanWCPWriteTotal}{17.0}
\newcommand{\xalanWCPNoFPAccessInCS}{98.5}
\newcommand{\xalanWCPNoFPAccessOutCS}{0.172}
\newcommand{\xalanWCPAcqRelTotal}{3.13}
\newcommand{\xalanWCPOtherTotal}{6.79E-5}
\newcommand{\xalanWCPNoFPReadTotal}{190}
\newcommand{\xalanWCPReadInCS}{112}
\newcommand{\xalanWCPReadOutCS}{0.0801}
\newcommand{\xalanWCPReadSameEp}{9.96}
\newcommand{\xalanWCPReadSharedSameEp}{<0.001}
\newcommand{\xalanWCPReadExclusive}{83.4}
\newcommand{\xalanWCPReadOwned}{\cna}
\newcommand{\xalanWCPReadShare}{0.00244}
\newcommand{\xalanWCPReadShared}{16.6}
\newcommand{\xalanWCPReadSharedOwned}{\cna}
\newcommand{\xalanWCPNoFPHonestWriteTotal}{41}
\newcommand{\xalanWCPWriteInCS}{129}
\newcommand{\xalanWCPWriteOutCS}{1.12}
\newcommand{\xalanWCPNoFPWriteTotal}{41}
\newcommand{\xalanWCPWriteSameEp}{30.2}
\newcommand{\xalanWCPWriteExclusive}{100}
\newcommand{\xalanWCPWriteOwned}{\cna}
\newcommand{\xalanWCPWriteShared}{0.0403}
\newcommand{\xalanWCPNoFPOtherEventTotal}{8928442}
\newcommand{\xalanWCPAcqRelOtherTotal}{100.0}
\newcommand{\xalanWCPNoAcqRelOtherTotal}{194}
\newcommand{\xalanWCPFork}{4.12}
\newcommand{\xalanWCPJoin}{4.12}
\newcommand{\xalanWCPPreWait}{4.12}
\newcommand{\xalanWCPPostWait}{4.12}
\newcommand{\xalanWCPVolatileTotal}{0.0}
\newcommand{\xalanWCPClassInit}{16.5}
\newcommand{\xalanWCPClassAccess}{67.5}
\newcommand{\xalanWCPRaceTotal}{13229787}
\newcommand{\xalanWCPWrRdRace}{28.0}
\newcommand{\xalanWCPWrWrRace}{44.3}
\newcommand{\xalanWCPRdWrRace}{27.6}
\newcommand{\xalanWCPRdShWrRace}{0.0831}
\newcommand{\xalanWCPHoldLocksTotal}{500}
\newcommand{\xalanWCPOneLockHeld}{210.}
\newcommand{\xalanWCPTwoNestedLocks}{210.}
\newcommand{\xalanWCPThreeNestedLocks}{<0.1}
\newcommand{\xalanWCPFourNestedLocks}{<0.1}
\newcommand{\xalanWCPFiveNestedLocks}{\cna}
\newcommand{\xalanWCPSixNestedLocks}{\cna}
\newcommand{\xalanWCPSevenNestedLocks}{\cna}
\newcommand{\xalanWCPEightNestedLocks}{\cna}
\newcommand{\xalanWCPNineNestedLocks}{\cna}
\newcommand{\xalanWCPTenNestedLocks}{\cna}
\newcommand{\xalanWCPHundredNestedLocks}{\cna}
\newcommand{\xalanFTOWCPEventTotal}{630}
\newcommand{\xalanFTOWCPNoFPEventTotal}{230}
\newcommand{\xalanFTOWCPNoFPAccessTotal}{220}
\newcommand{\xalanFTOWCPNoFPOtherTotal}{8.9}
\newcommand{\xalanFTOWCPReadTotal}{80.9}
\newcommand{\xalanFTOWCPWriteTotal}{15.2}
\newcommand{\xalanFTOWCPNoFPAccessInCS}{98.9}
\newcommand{\xalanFTOWCPNoFPAccessOutCS}{1.14}
\newcommand{\xalanFTOWCPAcqRelTotal}{17.9}
\newcommand{\xalanFTOWCPOtherTotal}{3.84E-4}
\newcommand{\xalanFTOWCPNoFPReadTotal}{190}
\newcommand{\xalanFTOWCPReadInCS}{112}
\newcommand{\xalanFTOWCPReadOutCS}{0.0472}
\newcommand{\xalanFTOWCPReadSameEp}{10.2}
\newcommand{\xalanFTOWCPReadSharedSameEp}{<0.001}
\newcommand{\xalanFTOWCPReadExclusive}{0.122}
\newcommand{\xalanFTOWCPReadOwned}{82.9}
\newcommand{\xalanFTOWCPReadShare}{0.00365}
\newcommand{\xalanFTOWCPReadShared}{0.0163}
\newcommand{\xalanFTOWCPReadSharedOwned}{17}
\newcommand{\xalanFTOWCPNoFPHonestWriteTotal}{35}
\newcommand{\xalanFTOWCPWriteInCS}{151}
\newcommand{\xalanFTOWCPWriteOutCS}{1.31}
\newcommand{\xalanFTOWCPNoFPWriteTotal}{35}
\newcommand{\xalanFTOWCPWriteSameEp}{35.3}
\newcommand{\xalanFTOWCPWriteExclusive}{3.48}
\newcommand{\xalanFTOWCPWriteOwned}{96.5}
\newcommand{\xalanFTOWCPWriteShared}{0.00632}
\newcommand{\xalanFTOWCPNoFPOtherEventTotal}{8928440}
\newcommand{\xalanFTOWCPAcqRelOtherTotal}{100.0}
\newcommand{\xalanFTOWCPNoAcqRelOtherTotal}{192}
\newcommand{\xalanFTOWCPFork}{4.17}
\newcommand{\xalanFTOWCPJoin}{4.17}
\newcommand{\xalanFTOWCPPreWait}{3.65}
\newcommand{\xalanFTOWCPPostWait}{3.65}
\newcommand{\xalanFTOWCPVolatileTotal}{0.0}
\newcommand{\xalanFTOWCPClassInit}{16.7}
\newcommand{\xalanFTOWCPClassAccess}{67.7}
\newcommand{\xalanFTOWCPRaceTotal}{9674981}
\newcommand{\xalanFTOWCPWrRdRace}{38.7}
\newcommand{\xalanFTOWCPWrWrRace}{0.0}
\newcommand{\xalanFTOWCPRdWrRace}{61.2}
\newcommand{\xalanFTOWCPRdShWrRace}{0.0824}
\newcommand{\xalanFTOWCPHoldLocksTotal}{240}
\newcommand{\xalanFTOWCPOneLockHeld}{104.}
\newcommand{\xalanFTOWCPTwoNestedLocks}{104.}
\newcommand{\xalanFTOWCPThreeNestedLocks}{<0.1}
\newcommand{\xalanFTOWCPFourNestedLocks}{\cna}
\newcommand{\xalanFTOWCPFiveNestedLocks}{\cna}
\newcommand{\xalanFTOWCPSixNestedLocks}{\cna}
\newcommand{\xalanFTOWCPSevenNestedLocks}{\cna}
\newcommand{\xalanFTOWCPEightNestedLocks}{\cna}
\newcommand{\xalanFTOWCPNineNestedLocks}{\cna}
\newcommand{\xalanFTOWCPTenNestedLocks}{\cna}
\newcommand{\xalanFTOWCPHundredNestedLocks}{\cna}
\newcommand{\xalanREWCPEventTotal}{630}
\newcommand{\xalanREWCPNoFPEventTotal}{230}
\newcommand{\xalanREWCPNoFPAccessTotal}{220}
\newcommand{\xalanREWCPNoFPOtherTotal}{8.9}
\newcommand{\xalanREWCPReadTotal}{80.8}
\newcommand{\xalanREWCPWriteTotal}{15.3}
\newcommand{\xalanREWCPNoFPAccessInCS}{98.8}
\newcommand{\xalanREWCPNoFPAccessOutCS}{1.16}
\newcommand{\xalanREWCPAcqRelTotal}{18.1}
\newcommand{\xalanREWCPOtherTotal}{3.95E-4}
\newcommand{\xalanREWCPNoFPReadTotal}{190}
\newcommand{\xalanREWCPReadInCS}{112}
\newcommand{\xalanREWCPReadOutCS}{0.0471}
\newcommand{\xalanREWCPReadSameEp}{10.2}
\newcommand{\xalanREWCPReadSharedSameEp}{<0.001}
\newcommand{\xalanREWCPReadExclusive}{0.0644}
\newcommand{\xalanREWCPReadOwned}{82.6}
\newcommand{\xalanREWCPReadShare}{0.0356}
\newcommand{\xalanREWCPReadShared}{0.0177}
\newcommand{\xalanREWCPReadSharedOwned}{17.3}
\newcommand{\xalanREWCPNoFPHonestWriteTotal}{35}
\newcommand{\xalanREWCPWriteInCS}{150}
\newcommand{\xalanREWCPWriteOutCS}{1.3}
\newcommand{\xalanREWCPNoFPWriteTotal}{35}
\newcommand{\xalanREWCPWriteSameEp}{35}
\newcommand{\xalanREWCPWriteExclusive}{3.9}
\newcommand{\xalanREWCPWriteOwned}{95.9}
\newcommand{\xalanREWCPWriteShared}{0.173}
\newcommand{\xalanREWCPNoFPOtherEventTotal}{8928443}
\newcommand{\xalanREWCPAcqRelOtherTotal}{100.0}
\newcommand{\xalanREWCPNoAcqRelOtherTotal}{195}
\newcommand{\xalanREWCPFork}{4.1}
\newcommand{\xalanREWCPJoin}{4.1}
\newcommand{\xalanREWCPPreWait}{4.1}
\newcommand{\xalanREWCPPostWait}{4.1}
\newcommand{\xalanREWCPVolatileTotal}{0.0}
\newcommand{\xalanREWCPClassInit}{16.4}
\newcommand{\xalanREWCPClassAccess}{67.2}
\newcommand{\xalanREWCPRaceTotal}{9008212}
\newcommand{\xalanREWCPWrRdRace}{37.8}
\newcommand{\xalanREWCPWrWrRace}{0.0}
\newcommand{\xalanREWCPRdWrRace}{62.1}
\newcommand{\xalanREWCPRdShWrRace}{0.0897}
\newcommand{\xalanREWCPHoldLocksTotal}{240}
\newcommand{\xalanREWCPOneLockHeld}{104.}
\newcommand{\xalanREWCPTwoNestedLocks}{103.}
\newcommand{\xalanREWCPThreeNestedLocks}{<0.1}
\newcommand{\xalanREWCPFourNestedLocks}{\cna}
\newcommand{\xalanREWCPFiveNestedLocks}{\cna}
\newcommand{\xalanREWCPSixNestedLocks}{\cna}
\newcommand{\xalanREWCPSevenNestedLocks}{\cna}
\newcommand{\xalanREWCPEightNestedLocks}{\cna}
\newcommand{\xalanREWCPNineNestedLocks}{\cna}
\newcommand{\xalanREWCPTenNestedLocks}{\cna}
\newcommand{\xalanREWCPHundredNestedLocks}{\cna}
\newcommand{\xalanDCEventTotal}{640}
\newcommand{\xalanDCNoFPEventTotal}{240}
\newcommand{\xalanDCNoFPAccessTotal}{230}
\newcommand{\xalanDCNoFPOtherTotal}{8.9}
\newcommand{\xalanDCReadTotal}{79.2}
\newcommand{\xalanDCWriteTotal}{17.1}
\newcommand{\xalanDCNoFPAccessInCS}{98.1}
\newcommand{\xalanDCNoFPAccessOutCS}{0.171}
\newcommand{\xalanDCAcqRelTotal}{3.09}
\newcommand{\xalanDCOtherTotal}{6.68E-5}
\newcommand{\xalanDCNoFPReadTotal}{190}
\newcommand{\xalanDCReadInCS}{112}
\newcommand{\xalanDCReadOutCS}{0.0804}
\newcommand{\xalanDCReadSameEp}{10}
\newcommand{\xalanDCReadSharedSameEp}{<0.001}
\newcommand{\xalanDCReadExclusive}{83.1}
\newcommand{\xalanDCReadOwned}{\cna}
\newcommand{\xalanDCReadShare}{0.00254}
\newcommand{\xalanDCReadShared}{16.9}
\newcommand{\xalanDCReadSharedOwned}{\cna}
\newcommand{\xalanDCNoFPHonestWriteTotal}{41}
\newcommand{\xalanDCWriteInCS}{129}
\newcommand{\xalanDCWriteOutCS}{1.12}
\newcommand{\xalanDCNoFPWriteTotal}{41}
\newcommand{\xalanDCWriteSameEp}{30}
\newcommand{\xalanDCWriteExclusive}{100}
\newcommand{\xalanDCWriteOwned}{\cna}
\newcommand{\xalanDCWriteShared}{0.0388}
\newcommand{\xalanDCNoFPOtherEventTotal}{8928441}
\newcommand{\xalanDCAcqRelOtherTotal}{100.0}
\newcommand{\xalanDCNoAcqRelOtherTotal}{193}
\newcommand{\xalanDCFork}{4.15}
\newcommand{\xalanDCJoin}{4.15}
\newcommand{\xalanDCPreWait}{4.15}
\newcommand{\xalanDCPostWait}{4.15}
\newcommand{\xalanDCVolatileTotal}{0.0}
\newcommand{\xalanDCClassInit}{16.6}
\newcommand{\xalanDCClassAccess}{67.4}
\newcommand{\xalanDCRaceTotal}{17005466}
\newcommand{\xalanDCWrRdRace}{28.1}
\newcommand{\xalanDCWrWrRace}{44.0}
\newcommand{\xalanDCRdWrRace}{27.8}
\newcommand{\xalanDCRdShWrRace}{0.0809}
\newcommand{\xalanDCHoldLocksTotal}{500}
\newcommand{\xalanDCOneLockHeld}{210.}
\newcommand{\xalanDCTwoNestedLocks}{209.}
\newcommand{\xalanDCThreeNestedLocks}{<0.1}
\newcommand{\xalanDCFourNestedLocks}{<0.1}
\newcommand{\xalanDCFiveNestedLocks}{\cna}
\newcommand{\xalanDCSixNestedLocks}{\cna}
\newcommand{\xalanDCSevenNestedLocks}{\cna}
\newcommand{\xalanDCEightNestedLocks}{\cna}
\newcommand{\xalanDCNineNestedLocks}{\cna}
\newcommand{\xalanDCTenNestedLocks}{\cna}
\newcommand{\xalanDCHundredNestedLocks}{\cna}
\newcommand{\xalanFTODCEventTotal}{630}
\newcommand{\xalanFTODCNoFPEventTotal}{230}
\newcommand{\xalanFTODCNoFPAccessTotal}{220}
\newcommand{\xalanFTODCNoFPOtherTotal}{8.9}
\newcommand{\xalanFTODCReadTotal}{81.4}
\newcommand{\xalanFTODCWriteTotal}{14.7}
\newcommand{\xalanFTODCNoFPAccessInCS}{98.9}
\newcommand{\xalanFTODCNoFPAccessOutCS}{1.07}
\newcommand{\xalanFTODCAcqRelTotal}{17.0}
\newcommand{\xalanFTODCOtherTotal}{3.67E-4}
\newcommand{\xalanFTODCNoFPReadTotal}{190}
\newcommand{\xalanFTODCReadInCS}{113}
\newcommand{\xalanFTODCReadOutCS}{0.0473}
\newcommand{\xalanFTODCReadSameEp}{10.2}
\newcommand{\xalanFTODCReadSharedSameEp}{<0.001}
\newcommand{\xalanFTODCReadExclusive}{0.0875}
\newcommand{\xalanFTODCReadOwned}{82.7}
\newcommand{\xalanFTODCReadShare}{0.00312}
\newcommand{\xalanFTODCReadShared}{0.0167}
\newcommand{\xalanFTODCReadSharedOwned}{17.2}
\newcommand{\xalanFTODCNoFPHonestWriteTotal}{34}
\newcommand{\xalanFTODCWriteInCS}{158}
\newcommand{\xalanFTODCWriteOutCS}{1.37}
\newcommand{\xalanFTODCNoFPWriteTotal}{34}
\newcommand{\xalanFTODCWriteSameEp}{36.7}
\newcommand{\xalanFTODCWriteExclusive}{2.02}
\newcommand{\xalanFTODCWriteOwned}{98}
\newcommand{\xalanFTODCWriteShared}{0.00269}
\newcommand{\xalanFTODCNoFPOtherEventTotal}{8928441}
\newcommand{\xalanFTODCAcqRelOtherTotal}{100.0}
\newcommand{\xalanFTODCNoAcqRelOtherTotal}{193}
\newcommand{\xalanFTODCFork}{4.15}
\newcommand{\xalanFTODCJoin}{4.15}
\newcommand{\xalanFTODCPreWait}{3.63}
\newcommand{\xalanFTODCPostWait}{3.63}
\newcommand{\xalanFTODCVolatileTotal}{0.0}
\newcommand{\xalanFTODCClassInit}{16.6}
\newcommand{\xalanFTODCClassAccess}{67.9}
\newcommand{\xalanFTODCRaceTotal}{12295329}
\newcommand{\xalanFTODCWrRdRace}{39.0}
\newcommand{\xalanFTODCWrWrRace}{0.0}
\newcommand{\xalanFTODCRdWrRace}{60.9}
\newcommand{\xalanFTODCRdShWrRace}{0.0996}
\newcommand{\xalanFTODCHoldLocksTotal}{240}
\newcommand{\xalanFTODCOneLockHeld}{105.}
\newcommand{\xalanFTODCTwoNestedLocks}{105.}
\newcommand{\xalanFTODCThreeNestedLocks}{<0.1}
\newcommand{\xalanFTODCFourNestedLocks}{\cna}
\newcommand{\xalanFTODCFiveNestedLocks}{\cna}
\newcommand{\xalanFTODCSixNestedLocks}{\cna}
\newcommand{\xalanFTODCSevenNestedLocks}{\cna}
\newcommand{\xalanFTODCEightNestedLocks}{\cna}
\newcommand{\xalanFTODCNineNestedLocks}{\cna}
\newcommand{\xalanFTODCTenNestedLocks}{\cna}
\newcommand{\xalanFTODCHundredNestedLocks}{\cna}
\newcommand{\xalanREDCEventTotal}{630}
\newcommand{\xalanREDCNoFPEventTotal}{230}
\newcommand{\xalanREDCNoFPAccessTotal}{220}
\newcommand{\xalanREDCNoFPOtherTotal}{8.9}
\newcommand{\xalanREDCReadTotal}{81.4}
\newcommand{\xalanREDCWriteTotal}{14.7}
\newcommand{\xalanREDCNoFPAccessInCS}{98.9}
\newcommand{\xalanREDCNoFPAccessOutCS}{1.07}
\newcommand{\xalanREDCAcqRelTotal}{17.0}
\newcommand{\xalanREDCOtherTotal}{3.69E-4}
\newcommand{\xalanREDCNoFPReadTotal}{190}
\newcommand{\xalanREDCReadInCS}{113}
\newcommand{\xalanREDCReadOutCS}{0.0473}
\newcommand{\xalanREDCReadSameEp}{10.2}
\newcommand{\xalanREDCReadSharedSameEp}{<0.001}
\newcommand{\xalanREDCReadExclusive}{0.0615}
\newcommand{\xalanREDCReadOwned}{82.5}
\newcommand{\xalanREDCReadShare}{0.00839}
\newcommand{\xalanREDCReadShared}{0.0175}
\newcommand{\xalanREDCReadSharedOwned}{17.4}
\newcommand{\xalanREDCNoFPHonestWriteTotal}{34}
\newcommand{\xalanREDCWriteInCS}{158}
\newcommand{\xalanREDCWriteOutCS}{1.37}
\newcommand{\xalanREDCNoFPWriteTotal}{34}
\newcommand{\xalanREDCWriteSameEp}{36.7}
\newcommand{\xalanREDCWriteExclusive}{2.05}
\newcommand{\xalanREDCWriteOwned}{97.9}
\newcommand{\xalanREDCWriteShared}{0.0309}
\newcommand{\xalanREDCNoFPOtherEventTotal}{8928442}
\newcommand{\xalanREDCAcqRelOtherTotal}{100.0}
\newcommand{\xalanREDCNoAcqRelOtherTotal}{194}
\newcommand{\xalanREDCFork}{4.12}
\newcommand{\xalanREDCJoin}{4.12}
\newcommand{\xalanREDCPreWait}{4.12}
\newcommand{\xalanREDCPostWait}{4.12}
\newcommand{\xalanREDCVolatileTotal}{0.0}
\newcommand{\xalanREDCClassInit}{16.5}
\newcommand{\xalanREDCClassAccess}{67.5}
\newcommand{\xalanREDCRaceTotal}{12239088}
\newcommand{\xalanREDCWrRdRace}{38.9}
\newcommand{\xalanREDCWrWrRace}{0.0}
\newcommand{\xalanREDCRdWrRace}{61.0}
\newcommand{\xalanREDCRdShWrRace}{0.1}
\newcommand{\xalanREDCHoldLocksTotal}{240}
\newcommand{\xalanREDCOneLockHeld}{105.}
\newcommand{\xalanREDCTwoNestedLocks}{105.}
\newcommand{\xalanREDCThreeNestedLocks}{<0.1}
\newcommand{\xalanREDCFourNestedLocks}{\cna}
\newcommand{\xalanREDCFiveNestedLocks}{\cna}
\newcommand{\xalanREDCSixNestedLocks}{\cna}
\newcommand{\xalanREDCSevenNestedLocks}{\cna}
\newcommand{\xalanREDCEightNestedLocks}{\cna}
\newcommand{\xalanREDCNineNestedLocks}{\cna}
\newcommand{\xalanREDCTenNestedLocks}{\cna}
\newcommand{\xalanREDCHundredNestedLocks}{\cna}
\newcommand{\xalanCAPOEventTotal}{640}
\newcommand{\xalanCAPONoFPEventTotal}{240}
\newcommand{\xalanCAPONoFPAccessTotal}{230}
\newcommand{\xalanCAPONoFPOtherTotal}{8.9}
\newcommand{\xalanCAPOReadTotal}{79.2}
\newcommand{\xalanCAPOWriteTotal}{17.1}
\newcommand{\xalanCAPONoFPAccessInCS}{98.1}
\newcommand{\xalanCAPONoFPAccessOutCS}{0.171}
\newcommand{\xalanCAPOAcqRelTotal}{3.09}
\newcommand{\xalanCAPOOtherTotal}{6.72E-5}
\newcommand{\xalanCAPONoFPReadTotal}{190}
\newcommand{\xalanCAPOReadInCS}{112}
\newcommand{\xalanCAPOReadOutCS}{0.0804}
\newcommand{\xalanCAPOReadSameEp}{10}
\newcommand{\xalanCAPOReadSharedSameEp}{<0.001}
\newcommand{\xalanCAPOReadExclusive}{83.1}
\newcommand{\xalanCAPOReadOwned}{\cna}
\newcommand{\xalanCAPOReadShare}{0.00259}
\newcommand{\xalanCAPOReadShared}{16.9}
\newcommand{\xalanCAPOReadSharedOwned}{\cna}
\newcommand{\xalanCAPONoFPHonestWriteTotal}{41}
\newcommand{\xalanCAPOWriteInCS}{129}
\newcommand{\xalanCAPOWriteOutCS}{1.12}
\newcommand{\xalanCAPONoFPWriteTotal}{41}
\newcommand{\xalanCAPOWriteSameEp}{30}
\newcommand{\xalanCAPOWriteExclusive}{100}
\newcommand{\xalanCAPOWriteOwned}{\cna}
\newcommand{\xalanCAPOWriteShared}{0.0389}
\newcommand{\xalanCAPONoFPOtherEventTotal}{8928442}
\newcommand{\xalanCAPOAcqRelOtherTotal}{100.0}
\newcommand{\xalanCAPONoAcqRelOtherTotal}{194}
\newcommand{\xalanCAPOFork}{4.12}
\newcommand{\xalanCAPOJoin}{4.12}
\newcommand{\xalanCAPOPreWait}{4.12}
\newcommand{\xalanCAPOPostWait}{4.12}
\newcommand{\xalanCAPOVolatileTotal}{0.0}
\newcommand{\xalanCAPOClassInit}{16.5}
\newcommand{\xalanCAPOClassAccess}{67.5}
\newcommand{\xalanCAPORaceTotal}{17016558}
\newcommand{\xalanCAPOWrRdRace}{28.2}
\newcommand{\xalanCAPOWrWrRace}{44.0}
\newcommand{\xalanCAPORdWrRace}{27.8}
\newcommand{\xalanCAPORdShWrRace}{0.0808}
\newcommand{\xalanCAPOHoldLocksTotal}{500}
\newcommand{\xalanCAPOOneLockHeld}{210.}
\newcommand{\xalanCAPOTwoNestedLocks}{209.}
\newcommand{\xalanCAPOThreeNestedLocks}{<0.1}
\newcommand{\xalanCAPOFourNestedLocks}{<0.1}
\newcommand{\xalanCAPOFiveNestedLocks}{\cna}
\newcommand{\xalanCAPOSixNestedLocks}{\cna}
\newcommand{\xalanCAPOSevenNestedLocks}{\cna}
\newcommand{\xalanCAPOEightNestedLocks}{\cna}
\newcommand{\xalanCAPONineNestedLocks}{\cna}
\newcommand{\xalanCAPOTenNestedLocks}{\cna}
\newcommand{\xalanCAPOHundredNestedLocks}{\cna}
\newcommand{\xalanFTOCAPOEventTotal}{630}
\newcommand{\xalanFTOCAPONoFPEventTotal}{230}
\newcommand{\xalanFTOCAPONoFPAccessTotal}{220}
\newcommand{\xalanFTOCAPONoFPOtherTotal}{8.9}
\newcommand{\xalanFTOCAPOReadTotal}{81.4}
\newcommand{\xalanFTOCAPOWriteTotal}{14.7}
\newcommand{\xalanFTOCAPONoFPAccessInCS}{98.9}
\newcommand{\xalanFTOCAPONoFPAccessOutCS}{1.07}
\newcommand{\xalanFTOCAPOAcqRelTotal}{17.0}
\newcommand{\xalanFTOCAPOOtherTotal}{3.71E-4}
\newcommand{\xalanFTOCAPONoFPReadTotal}{190}
\newcommand{\xalanFTOCAPOReadInCS}{113}
\newcommand{\xalanFTOCAPOReadOutCS}{0.0473}
\newcommand{\xalanFTOCAPOReadSameEp}{10.2}
\newcommand{\xalanFTOCAPOReadSharedSameEp}{<0.001}
\newcommand{\xalanFTOCAPOReadExclusive}{0.0864}
\newcommand{\xalanFTOCAPOReadOwned}{82.7}
\newcommand{\xalanFTOCAPOReadShare}{0.0031}
\newcommand{\xalanFTOCAPOReadShared}{0.0168}
\newcommand{\xalanFTOCAPOReadSharedOwned}{17.2}
\newcommand{\xalanFTOCAPONoFPHonestWriteTotal}{34}
\newcommand{\xalanFTOCAPOWriteInCS}{158}
\newcommand{\xalanFTOCAPOWriteOutCS}{1.37}
\newcommand{\xalanFTOCAPONoFPWriteTotal}{34}
\newcommand{\xalanFTOCAPOWriteSameEp}{36.7}
\newcommand{\xalanFTOCAPOWriteExclusive}{2.02}
\newcommand{\xalanFTOCAPOWriteOwned}{98}
\newcommand{\xalanFTOCAPOWriteShared}{0.00263}
\newcommand{\xalanFTOCAPONoFPOtherEventTotal}{8928443}
\newcommand{\xalanFTOCAPOAcqRelOtherTotal}{100.0}
\newcommand{\xalanFTOCAPONoAcqRelOtherTotal}{195}
\newcommand{\xalanFTOCAPOFork}{4.1}
\newcommand{\xalanFTOCAPOJoin}{4.1}
\newcommand{\xalanFTOCAPOPreWait}{4.1}
\newcommand{\xalanFTOCAPOPostWait}{4.1}
\newcommand{\xalanFTOCAPOVolatileTotal}{0.0}
\newcommand{\xalanFTOCAPOClassInit}{16.4}
\newcommand{\xalanFTOCAPOClassAccess}{67.2}
\newcommand{\xalanFTOCAPORaceTotal}{12287643}
\newcommand{\xalanFTOCAPOWrRdRace}{39.0}
\newcommand{\xalanFTOCAPOWrWrRace}{0.0}
\newcommand{\xalanFTOCAPORdWrRace}{60.9}
\newcommand{\xalanFTOCAPORdShWrRace}{0.1}
\newcommand{\xalanFTOCAPOHoldLocksTotal}{240}
\newcommand{\xalanFTOCAPOOneLockHeld}{105.}
\newcommand{\xalanFTOCAPOTwoNestedLocks}{105.}
\newcommand{\xalanFTOCAPOThreeNestedLocks}{<0.1}
\newcommand{\xalanFTOCAPOFourNestedLocks}{\cna}
\newcommand{\xalanFTOCAPOFiveNestedLocks}{\cna}
\newcommand{\xalanFTOCAPOSixNestedLocks}{\cna}
\newcommand{\xalanFTOCAPOSevenNestedLocks}{\cna}
\newcommand{\xalanFTOCAPOEightNestedLocks}{\cna}
\newcommand{\xalanFTOCAPONineNestedLocks}{\cna}
\newcommand{\xalanFTOCAPOTenNestedLocks}{\cna}
\newcommand{\xalanFTOCAPOHundredNestedLocks}{\cna}
\newcommand{\xalanRECAPOEventTotal}{630}
\newcommand{\xalanRECAPONoFPEventTotal}{230}
\newcommand{\xalanRECAPONoFPAccessTotal}{220}
\newcommand{\xalanRECAPONoFPOtherTotal}{8.9}
\newcommand{\xalanRECAPOReadTotal}{81.3}
\newcommand{\xalanRECAPOWriteTotal}{14.7}
\newcommand{\xalanRECAPONoFPAccessInCS}{98.9}
\newcommand{\xalanRECAPONoFPAccessOutCS}{1.07}
\newcommand{\xalanRECAPOAcqRelTotal}{17.0}
\newcommand{\xalanRECAPOOtherTotal}{3.71E-4}
\newcommand{\xalanRECAPONoFPReadTotal}{190}
\newcommand{\xalanRECAPOReadInCS}{113}
\newcommand{\xalanRECAPOReadOutCS}{0.0473}
\newcommand{\xalanRECAPOReadSameEp}{10.2}
\newcommand{\xalanRECAPOReadSharedSameEp}{<0.001}
\newcommand{\xalanRECAPOReadExclusive}{0.0515}
\newcommand{\xalanRECAPOReadOwned}{82.5}
\newcommand{\xalanRECAPOReadShare}{0.00826}
\newcommand{\xalanRECAPOReadShared}{0.0176}
\newcommand{\xalanRECAPOReadSharedOwned}{17.5}
\newcommand{\xalanRECAPONoFPHonestWriteTotal}{34}
\newcommand{\xalanRECAPOWriteInCS}{157}
\newcommand{\xalanRECAPOWriteOutCS}{1.37}
\newcommand{\xalanRECAPONoFPWriteTotal}{34}
\newcommand{\xalanRECAPOWriteSameEp}{36.7}
\newcommand{\xalanRECAPOWriteExclusive}{2.05}
\newcommand{\xalanRECAPOWriteOwned}{97.9}
\newcommand{\xalanRECAPOWriteShared}{0.0301}
\newcommand{\xalanRECAPONoFPOtherEventTotal}{8928443}
\newcommand{\xalanRECAPOAcqRelOtherTotal}{100.0}
\newcommand{\xalanRECAPONoAcqRelOtherTotal}{195}
\newcommand{\xalanRECAPOFork}{4.1}
\newcommand{\xalanRECAPOJoin}{4.1}
\newcommand{\xalanRECAPOPreWait}{4.1}
\newcommand{\xalanRECAPOPostWait}{4.1}
\newcommand{\xalanRECAPOVolatileTotal}{0.0}
\newcommand{\xalanRECAPOClassInit}{16.4}
\newcommand{\xalanRECAPOClassAccess}{67.2}
\newcommand{\xalanRECAPORaceTotal}{12199514}
\newcommand{\xalanRECAPOWrRdRace}{38.8}
\newcommand{\xalanRECAPOWrWrRace}{0.0}
\newcommand{\xalanRECAPORdWrRace}{61.1}
\newcommand{\xalanRECAPORdShWrRace}{0.101}
\newcommand{\xalanRECAPOHoldLocksTotal}{240}
\newcommand{\xalanRECAPOOneLockHeld}{105.}
\newcommand{\xalanRECAPOTwoNestedLocks}{105.}
\newcommand{\xalanRECAPOThreeNestedLocks}{<0.1}
\newcommand{\xalanRECAPOFourNestedLocks}{\cna}
\newcommand{\xalanRECAPOFiveNestedLocks}{\cna}
\newcommand{\xalanRECAPOSixNestedLocks}{\cna}
\newcommand{\xalanRECAPOSevenNestedLocks}{\cna}
\newcommand{\xalanRECAPOEightNestedLocks}{\cna}
\newcommand{\xalanRECAPONineNestedLocks}{\cna}
\newcommand{\xalanRECAPOTenNestedLocks}{\cna}
\newcommand{\xalanRECAPOHundredNestedLocks}{\cna}
\newcommand{\xalanCAPOTotalSetClears}{4.5}
\newcommand{\xalanCAPOReadSetZero}{27.8}
\newcommand{\xalanCAPOReadSetOne}{0.59}
\newcommand{\xalanCAPOReadSetGtOne}{71.6}
\newcommand{\xalanCAPOWriteSetZero}{98.3}
\newcommand{\xalanCAPOWriteSetOne}{0.968}
\newcommand{\xalanCAPOWriteSetGtOne}{0.754}
\newcommand{\xalanCAPOTotalMapClears}{4.5}
\newcommand{\xalanCAPOReadMapZero}{1.77}
\newcommand{\xalanCAPOReadMapOne}{20.1}
\newcommand{\xalanCAPOReadMapTen}{4.01}
\newcommand{\xalanCAPOReadMapHund}{3.09}
\newcommand{\xalanCAPOReadMapThou}{58.6}
\newcommand{\xalanCAPOReadMapGtThou}{12.4}
\newcommand{\xalanCAPOWriteMapZero}{20.1}
\newcommand{\xalanCAPOWriteMapOne}{0.835}
\newcommand{\xalanCAPOWriteMapTen}{2.73}
\newcommand{\xalanCAPOWriteMapHund}{5.32}
\newcommand{\xalanCAPOWriteMapThou}{1.36}
\newcommand{\xalanCAPOWriteMapGtThou}{69.6}
\newcommand{\FASTxalanMaxLiveThreads}{9}
\newcommand{\FASTxalanTotalThreads}{9}
\newcommand{\FASTxalanBaseTime}{2.0}
\newcommand{\FASTxalanBaseTimeCI}{220}
\newcommand{\FASTxalanEmptyTime}{\rna}
\newcommand{\FASTxalanEmptyTimeCI}{\rna}
\newcommand{\FASTxalanEmptyTimeCIMIN}{\rna}
\newcommand{\FASTxalanEmptyTimeCIMAX}{\rna}
\newcommand{\FASTxalanFTTime}{5.0}
\newcommand{\FASTxalanFTTimeCI}{0.94}
\newcommand{\FASTxalanHBTime}{5.1}
\newcommand{\FASTxalanHBTimeCI}{0.99}
\newcommand{\FASTxalanFTOHBTime}{5.2}
\newcommand{\FASTxalanFTOHBTimeCI}{1.0}
\newcommand{\FASTxalanWCPTime}{35}
\newcommand{\FASTxalanWCPTimeCI}{7.6}
\newcommand{\FASTxalanFTOWCPTime}{41}
\newcommand{\FASTxalanFTOWCPTimeCI}{8.5}
\newcommand{\FASTxalanREWCPTime}{19}
\newcommand{\FASTxalanREWCPTimeCI}{4.5}
\newcommand{\FASTxalanDCTime}{42}
\newcommand{\FASTxalanDCTimeCI}{7.9}
\newcommand{\FASTxalanFTODCTime}{44}
\newcommand{\FASTxalanFTODCTimeCI}{9.0}
\newcommand{\FASTxalanREDCTime}{23}
\newcommand{\FASTxalanREDCTimeCI}{4.3}
\newcommand{\FASTxalanCAPOTime}{40}
\newcommand{\FASTxalanCAPOTimeCI}{6.9}
\newcommand{\FASTxalanFTOCAPOTime}{42}
\newcommand{\FASTxalanFTOCAPOTimeCI}{10}
\newcommand{\FASTxalanRECAPOTime}{21}
\newcommand{\FASTxalanRECAPOTimeCI}{3.9}
\newcommand{\FASTxalanAGGCAPOTime}{\rna}
\newcommand{\FASTxalanAGGCAPOTimeCI}{\rna}
\newcommand{\FASTxalanAGGCAPOTimeCIMIN}{\rna}
\newcommand{\FASTxalanAGGCAPOTimeCIMAX}{\rna}
\newcommand{\FASTxalanStaticTime}{\rzero}
\newcommand{\FASTxalanDynamicTime}{\rzero}
\newcommand{\FASTxalanBaseMem}{660}
\newcommand{\FASTxalanBaseMemCI}{7.1}
\newcommand{\FASTxalanFTMem}{6.8}
\newcommand{\FASTxalanFTMemCI}{0.069}
\newcommand{\FASTxalanHBMem}{6.8}
\newcommand{\FASTxalanHBMemCI}{0.079}
\newcommand{\FASTxalanFTOHBMem}{6.8}
\newcommand{\FASTxalanFTOHBMemCI}{0.069}
\newcommand{\FASTxalanWCPMem}{69}
\newcommand{\FASTxalanWCPMemCI}{2.6}
\newcommand{\FASTxalanFTOWCPMem}{69}
\newcommand{\FASTxalanFTOWCPMemCI}{0.98}
\newcommand{\FASTxalanREWCPMem}{60}
\newcommand{\FASTxalanREWCPMemCI}{1.8}
\newcommand{\FASTxalanDCMem}{78}
\newcommand{\FASTxalanDCMemCI}{1.5}
\newcommand{\FASTxalanFTODCMem}{80}
\newcommand{\FASTxalanFTODCMemCI}{2.1}
\newcommand{\FASTxalanREDCMem}{69}
\newcommand{\FASTxalanREDCMemCI}{2.0}
\newcommand{\FASTxalanCAPOMem}{78}
\newcommand{\FASTxalanCAPOMemCI}{1.2}
\newcommand{\FASTxalanFTOCAPOMem}{78}
\newcommand{\FASTxalanFTOCAPOMemCI}{2.2}
\newcommand{\FASTxalanRECAPOMem}{75}
\newcommand{\FASTxalanRECAPOMemCI}{6.7}
\newcommand{\FASTxalanAGGCAPOMem}{\memna}
\newcommand{\FASTxalanAGGCAPOMemCI}{\memna}
\newcommand{\FASTxalanAGGCAPOMemCIMIN}{\memna}
\newcommand{\FASTxalanAGGCAPOMemCIMAX}{\memna}
\newcommand{\FASTxalanEventsCI}{98}
\newcommand{\FASTxalanEventsCIMIN}{626,353,956}
\newcommand{\FASTxalanEventsCIMAX}{626,354,152}
\newcommand{\FASTxalanNoFPEventsCI}{10,103}
\newcommand{\FASTxalanNoFPEventsCIMIN}{52,523,875}
\newcommand{\FASTxalanNoFPEventsCIMAX}{52,544,081}
\newcommand{\FASTxalanFT}{8}
\newcommand{\FASTxalanFTCI}{0}
\newcommand{\FASTxalanFTCIMIN}{8}
\newcommand{\FASTxalanFTCIMAX}{8}
\newcommand{\FASTxalanFTDynamic}{1,484}
\newcommand{\FASTxalanFTDynamicCI}{0}
\newcommand{\FASTxalanFTDynamicCIMIN}{1,484}
\newcommand{\FASTxalanFTDynamicCIMAX}{1,484}
\newcommand{\FASTxalanHB}{9}
\newcommand{\FASTxalanHBCI}{0}
\newcommand{\FASTxalanHBCIMIN}{9}
\newcommand{\FASTxalanHBCIMAX}{9}
\newcommand{\FASTxalanHBDynamic}{1,428}
\newcommand{\FASTxalanHBDynamicCI}{0}
\newcommand{\FASTxalanHBDynamicCIMIN}{1,428}
\newcommand{\FASTxalanHBDynamicCIMAX}{1,428}
\newcommand{\FASTxalanFTOHB}{9}
\newcommand{\FASTxalanFTOHBCI}{0}
\newcommand{\FASTxalanFTOHBCIMIN}{9}
\newcommand{\FASTxalanFTOHBCIMAX}{9}
\newcommand{\FASTxalanFTOHBDynamic}{1,428}
\newcommand{\FASTxalanFTOHBDynamicCI}{0}
\newcommand{\FASTxalanFTOHBDynamicCIMIN}{1,428}
\newcommand{\FASTxalanFTOHBDynamicCIMAX}{1,428}
\newcommand{\FASTxalanWCP}{149}
\newcommand{\FASTxalanWCPCI}{1}
\newcommand{\FASTxalanWCPCIMIN}{148}
\newcommand{\FASTxalanWCPCIMAX}{150}
\newcommand{\FASTxalanWCPDynamic}{9,573,623}
\newcommand{\FASTxalanWCPDynamicCI}{5,682}
\newcommand{\FASTxalanWCPDynamicCIMIN}{9,567,941}
\newcommand{\FASTxalanWCPDynamicCIMAX}{9,579,305}
\newcommand{\FASTxalanFTOWCP}{146}
\newcommand{\FASTxalanFTOWCPCI}{0}
\newcommand{\FASTxalanFTOWCPCIMIN}{146}
\newcommand{\FASTxalanFTOWCPCIMAX}{146}
\newcommand{\FASTxalanFTOWCPDynamic}{9,674,981}
\newcommand{\FASTxalanFTOWCPDynamicCI}{10,912}
\newcommand{\FASTxalanFTOWCPDynamicCIMIN}{9,664,069}
\newcommand{\FASTxalanFTOWCPDynamicCIMAX}{9,685,893}
\newcommand{\FASTxalanREWCP}{159}
\newcommand{\FASTxalanREWCPCI}{1}
\newcommand{\FASTxalanREWCPCIMIN}{158}
\newcommand{\FASTxalanREWCPCIMAX}{160}
\newcommand{\FASTxalanREWCPDynamic}{9,008,212}
\newcommand{\FASTxalanREWCPDynamicCI}{31,988}
\newcommand{\FASTxalanREWCPDynamicCIMIN}{8,976,224}
\newcommand{\FASTxalanREWCPDynamicCIMAX}{9,040,200}
\newcommand{\FASTxalanDC}{167}
\newcommand{\FASTxalanDCCI}{1}
\newcommand{\FASTxalanDCCIMIN}{166}
\newcommand{\FASTxalanDCCIMAX}{168}
\newcommand{\FASTxalanDCDynamic}{12,281,140}
\newcommand{\FASTxalanDCDynamicCI}{15,781}
\newcommand{\FASTxalanDCDynamicCIMIN}{12,265,359}
\newcommand{\FASTxalanDCDynamicCIMAX}{12,296,921}
\newcommand{\FASTxalanFTODC}{168}
\newcommand{\FASTxalanFTODCCI}{0}
\newcommand{\FASTxalanFTODCCIMIN}{168}
\newcommand{\FASTxalanFTODCCIMAX}{168}
\newcommand{\FASTxalanFTODCDynamic}{12,295,329}
\newcommand{\FASTxalanFTODCDynamicCI}{14,215}
\newcommand{\FASTxalanFTODCDynamicCIMIN}{12,281,114}
\newcommand{\FASTxalanFTODCDynamicCIMAX}{12,309,544}
\newcommand{\FASTxalanREDC}{166}
\newcommand{\FASTxalanREDCCI}{2}
\newcommand{\FASTxalanREDCCIMIN}{164}
\newcommand{\FASTxalanREDCCIMAX}{168}
\newcommand{\FASTxalanREDCDynamic}{12,239,088}
\newcommand{\FASTxalanREDCDynamicCI}{17,961}
\newcommand{\FASTxalanREDCDynamicCIMIN}{12,221,127}
\newcommand{\FASTxalanREDCDynamicCIMAX}{12,257,049}
\newcommand{\FASTxalanCAPO}{167}
\newcommand{\FASTxalanCAPOCI}{1}
\newcommand{\FASTxalanCAPOCIMIN}{166}
\newcommand{\FASTxalanCAPOCIMAX}{168}
\newcommand{\FASTxalanCAPODynamic}{12,288,823}
\newcommand{\FASTxalanCAPODynamicCI}{13,359}
\newcommand{\FASTxalanCAPODynamicCIMIN}{12,275,464}
\newcommand{\FASTxalanCAPODynamicCIMAX}{12,302,182}
\newcommand{\FASTxalanFTOCAPO}{168}
\newcommand{\FASTxalanFTOCAPOCI}{0}
\newcommand{\FASTxalanFTOCAPOCIMIN}{168}
\newcommand{\FASTxalanFTOCAPOCIMAX}{168}
\newcommand{\FASTxalanFTOCAPODynamic}{12,287,643}
\newcommand{\FASTxalanFTOCAPODynamicCI}{14,847}
\newcommand{\FASTxalanFTOCAPODynamicCIMIN}{12,272,796}
\newcommand{\FASTxalanFTOCAPODynamicCIMAX}{12,302,490}
\newcommand{\FASTxalanRECAPO}{166}
\newcommand{\FASTxalanRECAPOCI}{2}
\newcommand{\FASTxalanRECAPOCIMIN}{164}
\newcommand{\FASTxalanRECAPOCIMAX}{168}
\newcommand{\FASTxalanRECAPODynamic}{12,199,514}
\newcommand{\FASTxalanRECAPODynamicCI}{10,196}
\newcommand{\FASTxalanRECAPODynamicCIMIN}{12,189,318}
\newcommand{\FASTxalanRECAPODynamicCIMAX}{12,209,710}
\newcommand{\FASTxalanAGGCAPO}{\rna}
\newcommand{\FASTxalanAGGCAPOCI}{\rna}
\newcommand{\FASTxalanAGGCAPOCIMIN}{\rna}
\newcommand{\FASTxalanAGGCAPOCIMAX}{\rna}
\newcommand{\FASTxalanAGGCAPODynamic}{\rna}
\newcommand{\FASTxalanAGGCAPODynamicCI}{\rna}
\newcommand{\FASTxalanAGGCAPODynamicCIMIN}{\rna}
\newcommand{\FASTxalanAGGCAPODynamicCIMAX}{\rna}
\newcommand{\FASTBaseTimeGeoMean}{1900}
\newcommand{\FASTEmptyTimeGeoMean}{\rna}
\newcommand{\FASTFTTimeGeoMean}{9.5}
\newcommand{\FASTHBTimeGeoMean}{10}
\newcommand{\FASTFTOHBTimeGeoMean}{10}
\newcommand{\FASTWCPTimeGeoMean}{16}
\newcommand{\FASTFTOWCPTimeGeoMean}{20}
\newcommand{\FASTREWCPTimeGeoMean}{14}
\newcommand{\FASTDCTimeGeoMean}{16}
\newcommand{\FASTFTODCTimeGeoMean}{20}
\newcommand{\FASTREDCTimeGeoMean}{15}
\newcommand{\FASTCAPOTimeGeoMean}{15}
\newcommand{\FASTFTOCAPOTimeGeoMean}{19}
\newcommand{\FASTRECAPOTimeGeoMean}{13}
\newcommand{\FASTAGGCAPOTimeGeoMean}{\rna}
\newcommand{\FASTBaseMemGeoMean}{510}
\newcommand{\FASTEmptyMemGeoMean}{0.0}
\newcommand{\FASTFTMemGeoMean}{7.7}
\newcommand{\FASTHBMemGeoMean}{8.0}
\newcommand{\FASTFTOHBMemGeoMean}{7.9}
\newcommand{\FASTWCPMemGeoMean}{16}
\newcommand{\FASTFTOWCPMemGeoMean}{20}
\newcommand{\FASTREWCPMemGeoMean}{18}
\newcommand{\FASTDCMemGeoMean}{16}
\newcommand{\FASTFTODCMemGeoMean}{21}
\newcommand{\FASTREDCMemGeoMean}{19}
\newcommand{\FASTCAPOMemGeoMean}{15}
\newcommand{\FASTFTOCAPOMemGeoMean}{19}
\newcommand{\FASTRECAPOMemGeoMean}{17}
\newcommand{\FASTAGGCAPOMemGeoMean}{\memna}
\newcommand{\FASTWCPDynamicTotal}{10,050,385}
\newcommand{\FASTFTODCTotal}{1689}
\newcommand{\FASTCAPOTotal}{291}
\newcommand{\FASTWCPTotal}{259}
\newcommand{\FASTAGGCAPODynamicTotal}{0}
\newcommand{\FASTRECAPOTotal}{1774}
\newcommand{\FASTFTTotal}{490}
\newcommand{\FASTHBDynamicTotal}{11,922,772}
\newcommand{\FASTREDCTotal}{1775}
\newcommand{\FASTREWCPTotal}{1670}
\newcommand{\FASTFTOWCPDynamicTotal}{21,512,495}
\newcommand{\FASTRECAPODynamicTotal}{24,166,375}
\newcommand{\FASTFTOWCPTotal}{1614}
\newcommand{\FASTAGGCAPOTotal}{0}
\newcommand{\FASTCAPODynamicTotal}{12,760,377}
\newcommand{\FASTFTOCAPOTotal}{1686}
\newcommand{\FASTFTODCDynamicTotal}{23,956,471}
\newcommand{\FASTFTDynamicTotal}{5,779,179}
\newcommand{\FASTREWCPDynamicTotal}{20,858,887}
\newcommand{\FASTREDCDynamicTotal}{24,142,774}
\newcommand{\FASTFTOCAPODynamicTotal}{24,135,086}
\newcommand{\FASTFTOHBDynamicTotal}{12,145,068}
\newcommand{\FASTHBTotal}{1457}
\newcommand{\FASTFTOHBTotal}{1459}
\newcommand{\FASTDCDynamicTotal}{12,768,934}
\newcommand{\FASTDCTotal}{293}



==> result-macros/PIP_slowTool_noWriteOrReadRaceEdge_accessMetaUpdate.tex <==
\newcommand{\SLOWavroraEvents}{1,400}
\newcommand{\SLOWavroraNoFPEvents}{160}
\newcommand{\SLOWavroraMaxLiveThreads}{7}
\newcommand{\SLOWavroraTotalThreads}{7}
\newcommand{\SLOWavroraBaseTime}{2.4}
\newcommand{\SLOWavroraBaseTimeCI}{20}
\newcommand{\SLOWavroraEmptyTime}{\rna}
\newcommand{\SLOWavroraEmptyTimeCI}{\rna}
\newcommand{\SLOWavroraEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWavroraEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWavroraFTTime}{7.2}
\newcommand{\SLOWavroraFTTimeCI}{0.13}
\newcommand{\SLOWavroraHBTime}{18}
\newcommand{\SLOWavroraHBTimeCI}{0.53}
\newcommand{\SLOWavroraWCPTime}{24}
\newcommand{\SLOWavroraWCPTimeCI}{0.35}
\newcommand{\SLOWavroraDCnoGExcTime}{22}
\newcommand{\SLOWavroraDCnoGExcTimeCI}{0.45}
\newcommand{\SLOWavroraDCnoGTime}{\rna}
\newcommand{\SLOWavroraDCnoGTimeCI}{\rna}
\newcommand{\SLOWavroraDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWavroraDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWavroraDCExcTime}{26}
\newcommand{\SLOWavroraDCExcTimeCI}{0.29}
\newcommand{\SLOWavroraDCTime}{\rna}
\newcommand{\SLOWavroraDCTimeCI}{\rna}
\newcommand{\SLOWavroraDCTimeCIMIN}{\rna}
\newcommand{\SLOWavroraDCTimeCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGExcTime}{20}
\newcommand{\SLOWavroraCAPOnoGExcTimeCI}{0.36}
\newcommand{\SLOWavroraCAPOnoGTime}{\rna}
\newcommand{\SLOWavroraCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOExcTime}{23}
\newcommand{\SLOWavroraCAPOExcTimeCI}{0.40}
\newcommand{\SLOWavroraCAPOTime}{\rna}
\newcommand{\SLOWavroraCAPOTimeCI}{\rna}
\newcommand{\SLOWavroraCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWavroraStaticTime}{\rzero}
\newcommand{\SLOWavroraDynamicTime}{\rzero}
\newcommand{\SLOWavroraBaseMem}{150}
\newcommand{\SLOWavroraBaseMemCI}{6.2}
\newcommand{\SLOWavroraHBMem}{32}
\newcommand{\SLOWavroraHBMemCI}{1.4}
\newcommand{\SLOWavroraFTMem}{20}
\newcommand{\SLOWavroraFTMemCI}{3.5}
\newcommand{\SLOWavroraWCPMem}{99}
\newcommand{\SLOWavroraWCPMemCI}{3.9}
\newcommand{\SLOWavroraDCnoGExcMem}{41}
\newcommand{\SLOWavroraDCnoGExcMemCI}{1.9}
\newcommand{\SLOWavroraDCnoGMem}{\memna}
\newcommand{\SLOWavroraDCnoGMemCI}{\memna}
\newcommand{\SLOWavroraDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWavroraDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWavroraDCExcMem}{72}
\newcommand{\SLOWavroraDCExcMemCI}{3.1}
\newcommand{\SLOWavroraDCMem}{\memna}
\newcommand{\SLOWavroraDCMemCI}{\memna}
\newcommand{\SLOWavroraDCMemCIMIN}{\memna}
\newcommand{\SLOWavroraDCMemCIMAX}{\memna}
\newcommand{\SLOWavroraCAPOnoGExcMem}{37}
\newcommand{\SLOWavroraCAPOnoGExcMemCI}{2.2}
\newcommand{\SLOWavroraCAPOnoGMem}{\memna}
\newcommand{\SLOWavroraCAPOnoGMemCI}{\memna}
\newcommand{\SLOWavroraCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWavroraCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWavroraCAPOExcMem}{72}
\newcommand{\SLOWavroraCAPOExcMemCI}{3.0}
\newcommand{\SLOWavroraCAPOMem}{\memna}
\newcommand{\SLOWavroraCAPOMemCI}{\memna}
\newcommand{\SLOWavroraCAPOMemCIMIN}{\memna}
\newcommand{\SLOWavroraCAPOMemCIMAX}{\memna}
\newcommand{\SLOWavroraEventsCI}{107,189}
\newcommand{\SLOWavroraEventsCIMIN}{1,438,491,676}
\newcommand{\SLOWavroraEventsCIMAX}{1,438,706,054}
\newcommand{\SLOWavroraNoFPEventsCI}{91,458}
\newcommand{\SLOWavroraNoFPEventsCIMIN}{156,345,614}
\newcommand{\SLOWavroraNoFPEventsCIMAX}{156,528,530}
\newcommand{\SLOWavroraHB}{6}
\newcommand{\SLOWavroraHBCI}{0}
\newcommand{\SLOWavroraHBCIMIN}{6}
\newcommand{\SLOWavroraHBCIMAX}{6}
\newcommand{\SLOWavroraHBDynamic}{425,515}
\newcommand{\SLOWavroraHBDynamicCI}{1,885}
\newcommand{\SLOWavroraHBDynamicCIMIN}{423,630}
\newcommand{\SLOWavroraHBDynamicCIMAX}{427,400}
\newcommand{\SLOWavroraFT}{3}
\newcommand{\SLOWavroraFTCI}{0}
\newcommand{\SLOWavroraFTCIMIN}{3}
\newcommand{\SLOWavroraFTCIMAX}{3}
\newcommand{\SLOWavroraFTDynamic}{755,780}
\newcommand{\SLOWavroraFTDynamicCI}{3,115}
\newcommand{\SLOWavroraFTDynamicCIMIN}{752,665}
\newcommand{\SLOWavroraFTDynamicCIMAX}{758,895}
\newcommand{\SLOWavroraWCP}{6}
\newcommand{\SLOWavroraWCPCI}{0}
\newcommand{\SLOWavroraWCPCIMIN}{6}
\newcommand{\SLOWavroraWCPCIMAX}{6}
\newcommand{\SLOWavroraWCPDynamic}{423,457}
\newcommand{\SLOWavroraWCPDynamicCI}{553}
\newcommand{\SLOWavroraWCPDynamicCIMIN}{422,904}
\newcommand{\SLOWavroraWCPDynamicCIMAX}{424,010}
\newcommand{\SLOWavroraDCnoGExc}{6}
\newcommand{\SLOWavroraDCnoGExcCI}{0}
\newcommand{\SLOWavroraDCnoGExcCIMIN}{6}
\newcommand{\SLOWavroraDCnoGExcCIMAX}{6}
\newcommand{\SLOWavroraDCnoGExcDynamic}{443,207}
\newcommand{\SLOWavroraDCnoGExcDynamicCI}{584}
\newcommand{\SLOWavroraDCnoGExcDynamicCIMIN}{442,623}
\newcommand{\SLOWavroraDCnoGExcDynamicCIMAX}{443,791}
\newcommand{\SLOWavroraDCnoG}{\rna}
\newcommand{\SLOWavroraDCnoGCI}{\rna}
\newcommand{\SLOWavroraDCnoGCIMIN}{\rna}
\newcommand{\SLOWavroraDCnoGCIMAX}{\rna}
\newcommand{\SLOWavroraDCnoGDynamic}{\rna}
\newcommand{\SLOWavroraDCnoGDynamicCI}{\rna}
\newcommand{\SLOWavroraDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraDCExc}{6}
\newcommand{\SLOWavroraDCExcCI}{0}
\newcommand{\SLOWavroraDCExcCIMIN}{6}
\newcommand{\SLOWavroraDCExcCIMAX}{6}
\newcommand{\SLOWavroraDCExcDynamic}{154,673}
\newcommand{\SLOWavroraDCExcDynamicCI}{3,886}
\newcommand{\SLOWavroraDCExcDynamicCIMIN}{150,787}
\newcommand{\SLOWavroraDCExcDynamicCIMAX}{158,559}
\newcommand{\SLOWavroraDC}{\rna}
\newcommand{\SLOWavroraDCCI}{\rna}
\newcommand{\SLOWavroraDCCIMIN}{\rna}
\newcommand{\SLOWavroraDCCIMAX}{\rna}
\newcommand{\SLOWavroraDCDynamic}{\rna}
\newcommand{\SLOWavroraDCDynamicCI}{\rna}
\newcommand{\SLOWavroraDCDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraDCDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGExc}{6}
\newcommand{\SLOWavroraCAPOnoGExcCI}{0}
\newcommand{\SLOWavroraCAPOnoGExcCIMIN}{6}
\newcommand{\SLOWavroraCAPOnoGExcCIMAX}{6}
\newcommand{\SLOWavroraCAPOnoGExcDynamic}{441,420}
\newcommand{\SLOWavroraCAPOnoGExcDynamicCI}{615}
\newcommand{\SLOWavroraCAPOnoGExcDynamicCIMIN}{440,805}
\newcommand{\SLOWavroraCAPOnoGExcDynamicCIMAX}{442,035}
\newcommand{\SLOWavroraCAPOnoG}{\rna}
\newcommand{\SLOWavroraCAPOnoGCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamic}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOExc}{6}
\newcommand{\SLOWavroraCAPOExcCI}{0}
\newcommand{\SLOWavroraCAPOExcCIMIN}{6}
\newcommand{\SLOWavroraCAPOExcCIMAX}{6}
\newcommand{\SLOWavroraCAPOExcDynamic}{217,518}
\newcommand{\SLOWavroraCAPOExcDynamicCI}{2,377}
\newcommand{\SLOWavroraCAPOExcDynamicCIMIN}{215,141}
\newcommand{\SLOWavroraCAPOExcDynamicCIMAX}{219,895}
\newcommand{\SLOWavroraCAPO}{\rna}
\newcommand{\SLOWavroraCAPOCI}{\rna}
\newcommand{\SLOWavroraCAPOCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOCIMAX}{\rna}
\newcommand{\SLOWavroraCAPODynamic}{\rna}
\newcommand{\SLOWavroraCAPODynamicCI}{\rna}
\newcommand{\SLOWavroraCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWavroraCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIP}{\rna}
\newcommand{\SLOWavroraPIPCI}{\rna}
\newcommand{\SLOWavroraPIPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPDynamic}{\rna}
\newcommand{\SLOWavroraPIPDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraHBUP}{3}
\newcommand{\SLOWavroraHBUPCI}{0}
\newcommand{\SLOWavroraHBUPCIMIN}{3}
\newcommand{\SLOWavroraHBUPCIMAX}{3}
\newcommand{\SLOWavroraHBDynamicUP}{425,515}
\newcommand{\SLOWavroraHBDynamicUPCI}{1,885}
\newcommand{\SLOWavroraHBDynamicUPCIMIN}{423,630}
\newcommand{\SLOWavroraHBDynamicUPCIMAX}{427,400}
\newcommand{\SLOWavroraWCPUP}{3}
\newcommand{\SLOWavroraWCPUPCI}{0}
\newcommand{\SLOWavroraWCPUPCIMIN}{3}
\newcommand{\SLOWavroraWCPUPCIMAX}{3}
\newcommand{\SLOWavroraWCPDynamicUP}{423,457}
\newcommand{\SLOWavroraWCPDynamicUPCI}{553}
\newcommand{\SLOWavroraWCPDynamicUPCIMIN}{422,904}
\newcommand{\SLOWavroraWCPDynamicUPCIMAX}{424,010}
\newcommand{\SLOWavroraWDCnoGUP}{\rna}
\newcommand{\SLOWavroraWDCnoGUPCI}{\rna}
\newcommand{\SLOWavroraWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWavroraWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWavroraWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWavroraWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWavroraWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraWDCUP}{\rna}
\newcommand{\SLOWavroraWDCUPCI}{\rna}
\newcommand{\SLOWavroraWDCUPCIMIN}{\rna}
\newcommand{\SLOWavroraWDCUPCIMAX}{\rna}
\newcommand{\SLOWavroraWDCDynamicUP}{\rna}
\newcommand{\SLOWavroraWDCDynamicUPCI}{\rna}
\newcommand{\SLOWavroraWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGUP}{\rna}
\newcommand{\SLOWavroraCAPOnoGUPCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOUP}{\rna}
\newcommand{\SLOWavroraCAPOUPCI}{\rna}
\newcommand{\SLOWavroraCAPOUPCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOUPCIMAX}{\rna}
\newcommand{\SLOWavroraCAPODynamicUP}{\rna}
\newcommand{\SLOWavroraCAPODynamicUPCI}{\rna}
\newcommand{\SLOWavroraCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPUP}{\rna}
\newcommand{\SLOWavroraPIPUPCI}{\rna}
\newcommand{\SLOWavroraPIPUPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPUPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPDynamicUP}{\rna}
\newcommand{\SLOWavroraPIPDynamicUPCI}{\rna}
\newcommand{\SLOWavroraPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPHB}{\rna}
\newcommand{\SLOWavroraPIPHBCI}{\rna}
\newcommand{\SLOWavroraPIPHBCIMIN}{\rna}
\newcommand{\SLOWavroraPIPHBCIMAX}{\rna}
\newcommand{\SLOWavroraPIPHBDynamic}{\rna}
\newcommand{\SLOWavroraPIPHBDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIPWCP}{\rna}
\newcommand{\SLOWavroraPIPWCPCI}{\rna}
\newcommand{\SLOWavroraPIPWCPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPWCPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPWCPDynamic}{\rna}
\newcommand{\SLOWavroraPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIPWDC}{\rna}
\newcommand{\SLOWavroraPIPWDCCI}{\rna}
\newcommand{\SLOWavroraPIPWDCCIMIN}{\rna}
\newcommand{\SLOWavroraPIPWDCCIMAX}{\rna}
\newcommand{\SLOWavroraPIPWDCDynamic}{\rna}
\newcommand{\SLOWavroraPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIPCAPO}{\rna}
\newcommand{\SLOWavroraPIPCAPOCI}{\rna}
\newcommand{\SLOWavroraPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWavroraPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWavroraPIPCAPODynamic}{\rna}
\newcommand{\SLOWavroraPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWavroraPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIPPIP}{\rna}
\newcommand{\SLOWavroraPIPPIPCI}{\rna}
\newcommand{\SLOWavroraPIPPIPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPPIPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPPIPDynamic}{\rna}
\newcommand{\SLOWavroraPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikEvents}{160}
\newcommand{\SLOWbatikNoFPEvents}{11}
\newcommand{\SLOWbatikMaxLiveThreads}{7}
\newcommand{\SLOWbatikTotalThreads}{7}
\newcommand{\SLOWbatikBaseTime}{2.6}
\newcommand{\SLOWbatikBaseTimeCI}{37}
\newcommand{\SLOWbatikEmptyTime}{\rna}
\newcommand{\SLOWbatikEmptyTimeCI}{\rna}
\newcommand{\SLOWbatikEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWbatikEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWbatikFTTime}{4.1}
\newcommand{\SLOWbatikFTTimeCI}{0.067}
\newcommand{\SLOWbatikHBTime}{8.1}
\newcommand{\SLOWbatikHBTimeCI}{0.081}
\newcommand{\SLOWbatikWCPTime}{13}
\newcommand{\SLOWbatikWCPTimeCI}{0.26}
\newcommand{\SLOWbatikDCnoGExcTime}{11}
\newcommand{\SLOWbatikDCnoGExcTimeCI}{0.16}
\newcommand{\SLOWbatikDCnoGTime}{\rna}
\newcommand{\SLOWbatikDCnoGTimeCI}{\rna}
\newcommand{\SLOWbatikDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWbatikDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWbatikDCExcTime}{12}
\newcommand{\SLOWbatikDCExcTimeCI}{0.13}
\newcommand{\SLOWbatikDCTime}{\rna}
\newcommand{\SLOWbatikDCTimeCI}{\rna}
\newcommand{\SLOWbatikDCTimeCIMIN}{\rna}
\newcommand{\SLOWbatikDCTimeCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGExcTime}{10}
\newcommand{\SLOWbatikCAPOnoGExcTimeCI}{0.17}
\newcommand{\SLOWbatikCAPOnoGTime}{\rna}
\newcommand{\SLOWbatikCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOExcTime}{12}
\newcommand{\SLOWbatikCAPOExcTimeCI}{0.22}
\newcommand{\SLOWbatikCAPOTime}{\rna}
\newcommand{\SLOWbatikCAPOTimeCI}{\rna}
\newcommand{\SLOWbatikCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWbatikStaticTime}{\rzero}
\newcommand{\SLOWbatikDynamicTime}{\rzero}
\newcommand{\SLOWbatikBaseMem}{220}
\newcommand{\SLOWbatikBaseMemCI}{5.0}
\newcommand{\SLOWbatikHBMem}{30}
\newcommand{\SLOWbatikHBMemCI}{0.76}
\newcommand{\SLOWbatikFTMem}{5.5}
\newcommand{\SLOWbatikFTMemCI}{0.11}
\newcommand{\SLOWbatikWCPMem}{50}
\newcommand{\SLOWbatikWCPMemCI}{2.3}
\newcommand{\SLOWbatikDCnoGExcMem}{44}
\newcommand{\SLOWbatikDCnoGExcMemCI}{2.7}
\newcommand{\SLOWbatikDCnoGMem}{\memna}
\newcommand{\SLOWbatikDCnoGMemCI}{\memna}
\newcommand{\SLOWbatikDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWbatikDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWbatikDCExcMem}{46}
\newcommand{\SLOWbatikDCExcMemCI}{1.5}
\newcommand{\SLOWbatikDCMem}{\memna}
\newcommand{\SLOWbatikDCMemCI}{\memna}
\newcommand{\SLOWbatikDCMemCIMIN}{\memna}
\newcommand{\SLOWbatikDCMemCIMAX}{\memna}
\newcommand{\SLOWbatikCAPOnoGExcMem}{41}
\newcommand{\SLOWbatikCAPOnoGExcMemCI}{3.3}
\newcommand{\SLOWbatikCAPOnoGMem}{\memna}
\newcommand{\SLOWbatikCAPOnoGMemCI}{\memna}
\newcommand{\SLOWbatikCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWbatikCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWbatikCAPOExcMem}{44}
\newcommand{\SLOWbatikCAPOExcMemCI}{1.1}
\newcommand{\SLOWbatikCAPOMem}{\memna}
\newcommand{\SLOWbatikCAPOMemCI}{\memna}
\newcommand{\SLOWbatikCAPOMemCIMIN}{\memna}
\newcommand{\SLOWbatikCAPOMemCIMAX}{\memna}
\newcommand{\SLOWbatikEventsCI}{0}
\newcommand{\SLOWbatikEventsCIMIN}{155,322,726}
\newcommand{\SLOWbatikEventsCIMAX}{155,322,726}
\newcommand{\SLOWbatikNoFPEventsCI}{0}
\newcommand{\SLOWbatikNoFPEventsCIMIN}{11,422,601}
\newcommand{\SLOWbatikNoFPEventsCIMAX}{11,422,601}
\newcommand{\SLOWbatikHB}{0}
\newcommand{\SLOWbatikHBCI}{0}
\newcommand{\SLOWbatikHBCIMIN}{0}
\newcommand{\SLOWbatikHBCIMAX}{0}
\newcommand{\SLOWbatikHBDynamic}{0}
\newcommand{\SLOWbatikHBDynamicCI}{0}
\newcommand{\SLOWbatikHBDynamicCIMIN}{0}
\newcommand{\SLOWbatikHBDynamicCIMAX}{0}
\newcommand{\SLOWbatikFT}{0}
\newcommand{\SLOWbatikFTCI}{0}
\newcommand{\SLOWbatikFTCIMIN}{0}
\newcommand{\SLOWbatikFTCIMAX}{0}
\newcommand{\SLOWbatikFTDynamic}{0}
\newcommand{\SLOWbatikFTDynamicCI}{0}
\newcommand{\SLOWbatikFTDynamicCIMIN}{0}
\newcommand{\SLOWbatikFTDynamicCIMAX}{0}
\newcommand{\SLOWbatikWCP}{0}
\newcommand{\SLOWbatikWCPCI}{0}
\newcommand{\SLOWbatikWCPCIMIN}{0}
\newcommand{\SLOWbatikWCPCIMAX}{0}
\newcommand{\SLOWbatikWCPDynamic}{0}
\newcommand{\SLOWbatikWCPDynamicCI}{0}
\newcommand{\SLOWbatikWCPDynamicCIMIN}{0}
\newcommand{\SLOWbatikWCPDynamicCIMAX}{0}
\newcommand{\SLOWbatikDCnoGExc}{0}
\newcommand{\SLOWbatikDCnoGExcCI}{0}
\newcommand{\SLOWbatikDCnoGExcCIMIN}{0}
\newcommand{\SLOWbatikDCnoGExcCIMAX}{0}
\newcommand{\SLOWbatikDCnoGExcDynamic}{0}
\newcommand{\SLOWbatikDCnoGExcDynamicCI}{0}
\newcommand{\SLOWbatikDCnoGExcDynamicCIMIN}{0}
\newcommand{\SLOWbatikDCnoGExcDynamicCIMAX}{0}
\newcommand{\SLOWbatikDCnoG}{\rna}
\newcommand{\SLOWbatikDCnoGCI}{\rna}
\newcommand{\SLOWbatikDCnoGCIMIN}{\rna}
\newcommand{\SLOWbatikDCnoGCIMAX}{\rna}
\newcommand{\SLOWbatikDCnoGDynamic}{\rna}
\newcommand{\SLOWbatikDCnoGDynamicCI}{\rna}
\newcommand{\SLOWbatikDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikDCExc}{0}
\newcommand{\SLOWbatikDCExcCI}{0}
\newcommand{\SLOWbatikDCExcCIMIN}{0}
\newcommand{\SLOWbatikDCExcCIMAX}{0}
\newcommand{\SLOWbatikDCExcDynamic}{0}
\newcommand{\SLOWbatikDCExcDynamicCI}{0}
\newcommand{\SLOWbatikDCExcDynamicCIMIN}{0}
\newcommand{\SLOWbatikDCExcDynamicCIMAX}{0}
\newcommand{\SLOWbatikDC}{\rna}
\newcommand{\SLOWbatikDCCI}{\rna}
\newcommand{\SLOWbatikDCCIMIN}{\rna}
\newcommand{\SLOWbatikDCCIMAX}{\rna}
\newcommand{\SLOWbatikDCDynamic}{\rna}
\newcommand{\SLOWbatikDCDynamicCI}{\rna}
\newcommand{\SLOWbatikDCDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikDCDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGExc}{0}
\newcommand{\SLOWbatikCAPOnoGExcCI}{0}
\newcommand{\SLOWbatikCAPOnoGExcCIMIN}{0}
\newcommand{\SLOWbatikCAPOnoGExcCIMAX}{0}
\newcommand{\SLOWbatikCAPOnoGExcDynamic}{0}
\newcommand{\SLOWbatikCAPOnoGExcDynamicCI}{0}
\newcommand{\SLOWbatikCAPOnoGExcDynamicCIMIN}{0}
\newcommand{\SLOWbatikCAPOnoGExcDynamicCIMAX}{0}
\newcommand{\SLOWbatikCAPOnoG}{\rna}
\newcommand{\SLOWbatikCAPOnoGCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamic}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOExc}{0}
\newcommand{\SLOWbatikCAPOExcCI}{0}
\newcommand{\SLOWbatikCAPOExcCIMIN}{0}
\newcommand{\SLOWbatikCAPOExcCIMAX}{0}
\newcommand{\SLOWbatikCAPOExcDynamic}{0}
\newcommand{\SLOWbatikCAPOExcDynamicCI}{0}
\newcommand{\SLOWbatikCAPOExcDynamicCIMIN}{0}
\newcommand{\SLOWbatikCAPOExcDynamicCIMAX}{0}
\newcommand{\SLOWbatikCAPO}{\rna}
\newcommand{\SLOWbatikCAPOCI}{\rna}
\newcommand{\SLOWbatikCAPOCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOCIMAX}{\rna}
\newcommand{\SLOWbatikCAPODynamic}{\rna}
\newcommand{\SLOWbatikCAPODynamicCI}{\rna}
\newcommand{\SLOWbatikCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWbatikCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIP}{\rna}
\newcommand{\SLOWbatikPIPCI}{\rna}
\newcommand{\SLOWbatikPIPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPDynamic}{\rna}
\newcommand{\SLOWbatikPIPDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikHBUP}{0}
\newcommand{\SLOWbatikHBUPCI}{0}
\newcommand{\SLOWbatikHBUPCIMIN}{0}
\newcommand{\SLOWbatikHBUPCIMAX}{0}
\newcommand{\SLOWbatikHBDynamicUP}{0}
\newcommand{\SLOWbatikHBDynamicUPCI}{0}
\newcommand{\SLOWbatikHBDynamicUPCIMIN}{0}
\newcommand{\SLOWbatikHBDynamicUPCIMAX}{0}
\newcommand{\SLOWbatikWCPUP}{0}
\newcommand{\SLOWbatikWCPUPCI}{0}
\newcommand{\SLOWbatikWCPUPCIMIN}{0}
\newcommand{\SLOWbatikWCPUPCIMAX}{0}
\newcommand{\SLOWbatikWCPDynamicUP}{0}
\newcommand{\SLOWbatikWCPDynamicUPCI}{0}
\newcommand{\SLOWbatikWCPDynamicUPCIMIN}{0}
\newcommand{\SLOWbatikWCPDynamicUPCIMAX}{0}
\newcommand{\SLOWbatikWDCnoGUP}{\rna}
\newcommand{\SLOWbatikWDCnoGUPCI}{\rna}
\newcommand{\SLOWbatikWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWbatikWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWbatikWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWbatikWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWbatikWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikWDCUP}{\rna}
\newcommand{\SLOWbatikWDCUPCI}{\rna}
\newcommand{\SLOWbatikWDCUPCIMIN}{\rna}
\newcommand{\SLOWbatikWDCUPCIMAX}{\rna}
\newcommand{\SLOWbatikWDCDynamicUP}{\rna}
\newcommand{\SLOWbatikWDCDynamicUPCI}{\rna}
\newcommand{\SLOWbatikWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGUP}{\rna}
\newcommand{\SLOWbatikCAPOnoGUPCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOUP}{\rna}
\newcommand{\SLOWbatikCAPOUPCI}{\rna}
\newcommand{\SLOWbatikCAPOUPCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOUPCIMAX}{\rna}
\newcommand{\SLOWbatikCAPODynamicUP}{\rna}
\newcommand{\SLOWbatikCAPODynamicUPCI}{\rna}
\newcommand{\SLOWbatikCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPUP}{\rna}
\newcommand{\SLOWbatikPIPUPCI}{\rna}
\newcommand{\SLOWbatikPIPUPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPUPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPDynamicUP}{\rna}
\newcommand{\SLOWbatikPIPDynamicUPCI}{\rna}
\newcommand{\SLOWbatikPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPHB}{\rna}
\newcommand{\SLOWbatikPIPHBCI}{\rna}
\newcommand{\SLOWbatikPIPHBCIMIN}{\rna}
\newcommand{\SLOWbatikPIPHBCIMAX}{\rna}
\newcommand{\SLOWbatikPIPHBDynamic}{\rna}
\newcommand{\SLOWbatikPIPHBDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIPWCP}{\rna}
\newcommand{\SLOWbatikPIPWCPCI}{\rna}
\newcommand{\SLOWbatikPIPWCPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPWCPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPWCPDynamic}{\rna}
\newcommand{\SLOWbatikPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIPWDC}{\rna}
\newcommand{\SLOWbatikPIPWDCCI}{\rna}
\newcommand{\SLOWbatikPIPWDCCIMIN}{\rna}
\newcommand{\SLOWbatikPIPWDCCIMAX}{\rna}
\newcommand{\SLOWbatikPIPWDCDynamic}{\rna}
\newcommand{\SLOWbatikPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIPCAPO}{\rna}
\newcommand{\SLOWbatikPIPCAPOCI}{\rna}
\newcommand{\SLOWbatikPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWbatikPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWbatikPIPCAPODynamic}{\rna}
\newcommand{\SLOWbatikPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWbatikPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIPPIP}{\rna}
\newcommand{\SLOWbatikPIPPIPCI}{\rna}
\newcommand{\SLOWbatikPIPPIPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPPIPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPPIPDynamic}{\rna}
\newcommand{\SLOWbatikPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoEvents}{3,800}
\newcommand{\SLOWhtwoNoFPEvents}{460}
\newcommand{\SLOWhtwoMaxLiveThreads}{9}
\newcommand{\SLOWhtwoTotalThreads}{10}
\newcommand{\SLOWhtwoBaseTime}{4.9}
\newcommand{\SLOWhtwoBaseTimeCI}{65}
\newcommand{\SLOWhtwoEmptyTime}{\rna}
\newcommand{\SLOWhtwoEmptyTimeCI}{\rna}
\newcommand{\SLOWhtwoEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoFTTime}{9.5}
\newcommand{\SLOWhtwoFTTimeCI}{0.54}
\newcommand{\SLOWhtwoHBTime}{32}
\newcommand{\SLOWhtwoHBTimeCI}{1.1}
\newcommand{\SLOWhtwoWCPTime}{79}
\newcommand{\SLOWhtwoWCPTimeCI}{6.0}
\newcommand{\SLOWhtwoDCnoGExcTime}{77}
\newcommand{\SLOWhtwoDCnoGExcTimeCI}{5.5}
\newcommand{\SLOWhtwoDCnoGTime}{\rna}
\newcommand{\SLOWhtwoDCnoGTimeCI}{\rna}
\newcommand{\SLOWhtwoDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoDCExcTime}{77}
\newcommand{\SLOWhtwoDCExcTimeCI}{4.2}
\newcommand{\SLOWhtwoDCTime}{\rna}
\newcommand{\SLOWhtwoDCTimeCI}{\rna}
\newcommand{\SLOWhtwoDCTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoDCTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGExcTime}{73}
\newcommand{\SLOWhtwoCAPOnoGExcTimeCI}{4.1}
\newcommand{\SLOWhtwoCAPOnoGTime}{\rna}
\newcommand{\SLOWhtwoCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOExcTime}{77}
\newcommand{\SLOWhtwoCAPOExcTimeCI}{3.7}
\newcommand{\SLOWhtwoCAPOTime}{\rna}
\newcommand{\SLOWhtwoCAPOTimeCI}{\rna}
\newcommand{\SLOWhtwoCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoStaticTime}{\rzero}
\newcommand{\SLOWhtwoDynamicTime}{\rzero}
\newcommand{\SLOWhtwoBaseMem}{1,800}
\newcommand{\SLOWhtwoBaseMemCI}{48.0}
\newcommand{\SLOWhtwoHBMem}{17}
\newcommand{\SLOWhtwoHBMemCI}{1.2}
\newcommand{\SLOWhtwoFTMem}{3.1}
\newcommand{\SLOWhtwoFTMemCI}{0.076}
\newcommand{\SLOWhtwoWCPMem}{63}
\newcommand{\SLOWhtwoWCPMemCI}{1.5}
\newcommand{\SLOWhtwoDCnoGExcMem}{55}
\newcommand{\SLOWhtwoDCnoGExcMemCI}{2.9}
\newcommand{\SLOWhtwoDCnoGMem}{\memna}
\newcommand{\SLOWhtwoDCnoGMemCI}{\memna}
\newcommand{\SLOWhtwoDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWhtwoDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWhtwoDCExcMem}{57}
\newcommand{\SLOWhtwoDCExcMemCI}{2.5}
\newcommand{\SLOWhtwoDCMem}{\memna}
\newcommand{\SLOWhtwoDCMemCI}{\memna}
\newcommand{\SLOWhtwoDCMemCIMIN}{\memna}
\newcommand{\SLOWhtwoDCMemCIMAX}{\memna}
\newcommand{\SLOWhtwoCAPOnoGExcMem}{53}
\newcommand{\SLOWhtwoCAPOnoGExcMemCI}{3.3}
\newcommand{\SLOWhtwoCAPOnoGMem}{\memna}
\newcommand{\SLOWhtwoCAPOnoGMemCI}{\memna}
\newcommand{\SLOWhtwoCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWhtwoCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWhtwoCAPOExcMem}{57}
\newcommand{\SLOWhtwoCAPOExcMemCI}{3.0}
\newcommand{\SLOWhtwoCAPOMem}{\memna}
\newcommand{\SLOWhtwoCAPOMemCI}{\memna}
\newcommand{\SLOWhtwoCAPOMemCIMIN}{\memna}
\newcommand{\SLOWhtwoCAPOMemCIMAX}{\memna}
\newcommand{\SLOWhtwoEventsCI}{1,258,655}
\newcommand{\SLOWhtwoEventsCIMIN}{3,801,406,538}
\newcommand{\SLOWhtwoEventsCIMAX}{3,803,923,848}
\newcommand{\SLOWhtwoNoFPEventsCI}{41,806}
\newcommand{\SLOWhtwoNoFPEventsCIMIN}{457,193,918}
\newcommand{\SLOWhtwoNoFPEventsCIMAX}{457,277,530}
\newcommand{\SLOWhtwoHB}{13}
\newcommand{\SLOWhtwoHBCI}{0.2}
\newcommand{\SLOWhtwoHBCIMIN}{13}
\newcommand{\SLOWhtwoHBCIMAX}{13}
\newcommand{\SLOWhtwoHBDynamic}{83,739}
\newcommand{\SLOWhtwoHBDynamicCI}{156}
\newcommand{\SLOWhtwoHBDynamicCIMIN}{83,583}
\newcommand{\SLOWhtwoHBDynamicCIMAX}{83,895}
\newcommand{\SLOWhtwoFT}{11}
\newcommand{\SLOWhtwoFTCI}{0.30}
\newcommand{\SLOWhtwoFTCIMIN}{11}
\newcommand{\SLOWhtwoFTCIMAX}{11}
\newcommand{\SLOWhtwoFTDynamic}{92,746}
\newcommand{\SLOWhtwoFTDynamicCI}{872}
\newcommand{\SLOWhtwoFTDynamicCIMIN}{91,874}
\newcommand{\SLOWhtwoFTDynamicCIMAX}{93,618}
\newcommand{\SLOWhtwoWCP}{13}
\newcommand{\SLOWhtwoWCPCI}{0.3}
\newcommand{\SLOWhtwoWCPCIMIN}{13}
\newcommand{\SLOWhtwoWCPCIMAX}{13}
\newcommand{\SLOWhtwoWCPDynamic}{83,926}
\newcommand{\SLOWhtwoWCPDynamicCI}{130}
\newcommand{\SLOWhtwoWCPDynamicCIMIN}{83,796}
\newcommand{\SLOWhtwoWCPDynamicCIMAX}{84,056}
\newcommand{\SLOWhtwoDCnoGExc}{13}
\newcommand{\SLOWhtwoDCnoGExcCI}{0}
\newcommand{\SLOWhtwoDCnoGExcCIMIN}{13}
\newcommand{\SLOWhtwoDCnoGExcCIMAX}{13}
\newcommand{\SLOWhtwoDCnoGExcDynamic}{84,442}
\newcommand{\SLOWhtwoDCnoGExcDynamicCI}{196}
\newcommand{\SLOWhtwoDCnoGExcDynamicCIMIN}{84,246}
\newcommand{\SLOWhtwoDCnoGExcDynamicCIMAX}{84,638}
\newcommand{\SLOWhtwoDCnoG}{\rna}
\newcommand{\SLOWhtwoDCnoGCI}{\rna}
\newcommand{\SLOWhtwoDCnoGCIMIN}{\rna}
\newcommand{\SLOWhtwoDCnoGCIMAX}{\rna}
\newcommand{\SLOWhtwoDCnoGDynamic}{\rna}
\newcommand{\SLOWhtwoDCnoGDynamicCI}{\rna}
\newcommand{\SLOWhtwoDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoDCExc}{13}
\newcommand{\SLOWhtwoDCExcCI}{0.30}
\newcommand{\SLOWhtwoDCExcCIMIN}{13}
\newcommand{\SLOWhtwoDCExcCIMAX}{13}
\newcommand{\SLOWhtwoDCExcDynamic}{41,383}
\newcommand{\SLOWhtwoDCExcDynamicCI}{125}
\newcommand{\SLOWhtwoDCExcDynamicCIMIN}{41,258}
\newcommand{\SLOWhtwoDCExcDynamicCIMAX}{41,508}
\newcommand{\SLOWhtwoDC}{\rna}
\newcommand{\SLOWhtwoDCCI}{\rna}
\newcommand{\SLOWhtwoDCCIMIN}{\rna}
\newcommand{\SLOWhtwoDCCIMAX}{\rna}
\newcommand{\SLOWhtwoDCDynamic}{\rna}
\newcommand{\SLOWhtwoDCDynamicCI}{\rna}
\newcommand{\SLOWhtwoDCDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoDCDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGExc}{13}
\newcommand{\SLOWhtwoCAPOnoGExcCI}{0}
\newcommand{\SLOWhtwoCAPOnoGExcCIMIN}{13}
\newcommand{\SLOWhtwoCAPOnoGExcCIMAX}{13}
\newcommand{\SLOWhtwoCAPOnoGExcDynamic}{84,153}
\newcommand{\SLOWhtwoCAPOnoGExcDynamicCI}{296}
\newcommand{\SLOWhtwoCAPOnoGExcDynamicCIMIN}{83,857}
\newcommand{\SLOWhtwoCAPOnoGExcDynamicCIMAX}{84,449}
\newcommand{\SLOWhtwoCAPOnoG}{\rna}
\newcommand{\SLOWhtwoCAPOnoGCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamic}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOExc}{13}
\newcommand{\SLOWhtwoCAPOExcCI}{0.26}
\newcommand{\SLOWhtwoCAPOExcCIMIN}{13}
\newcommand{\SLOWhtwoCAPOExcCIMAX}{13}
\newcommand{\SLOWhtwoCAPOExcDynamic}{41,426}
\newcommand{\SLOWhtwoCAPOExcDynamicCI}{158}
\newcommand{\SLOWhtwoCAPOExcDynamicCIMIN}{41,268}
\newcommand{\SLOWhtwoCAPOExcDynamicCIMAX}{41,584}
\newcommand{\SLOWhtwoCAPO}{\rna}
\newcommand{\SLOWhtwoCAPOCI}{\rna}
\newcommand{\SLOWhtwoCAPOCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPODynamic}{\rna}
\newcommand{\SLOWhtwoCAPODynamicCI}{\rna}
\newcommand{\SLOWhtwoCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIP}{\rna}
\newcommand{\SLOWhtwoPIPCI}{\rna}
\newcommand{\SLOWhtwoPIPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPDynamic}{\rna}
\newcommand{\SLOWhtwoPIPDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoHBUP}{9}
\newcommand{\SLOWhtwoHBUPCI}{0.20}
\newcommand{\SLOWhtwoHBUPCIMIN}{9}
\newcommand{\SLOWhtwoHBUPCIMAX}{9}
\newcommand{\SLOWhtwoHBDynamicUP}{83,739}
\newcommand{\SLOWhtwoHBDynamicUPCI}{156}
\newcommand{\SLOWhtwoHBDynamicUPCIMIN}{83,583}
\newcommand{\SLOWhtwoHBDynamicUPCIMAX}{83,895}
\newcommand{\SLOWhtwoWCPUP}{9}
\newcommand{\SLOWhtwoWCPUPCI}{0.59}
\newcommand{\SLOWhtwoWCPUPCIMIN}{8}
\newcommand{\SLOWhtwoWCPUPCIMAX}{10}
\newcommand{\SLOWhtwoWCPDynamicUP}{83,926}
\newcommand{\SLOWhtwoWCPDynamicUPCI}{130}
\newcommand{\SLOWhtwoWCPDynamicUPCIMIN}{83,796}
\newcommand{\SLOWhtwoWCPDynamicUPCIMAX}{84,056}
\newcommand{\SLOWhtwoWDCnoGUP}{\rna}
\newcommand{\SLOWhtwoWDCnoGUPCI}{\rna}
\newcommand{\SLOWhtwoWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWhtwoWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWhtwoWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWhtwoWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWhtwoWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoWDCUP}{\rna}
\newcommand{\SLOWhtwoWDCUPCI}{\rna}
\newcommand{\SLOWhtwoWDCUPCIMIN}{\rna}
\newcommand{\SLOWhtwoWDCUPCIMAX}{\rna}
\newcommand{\SLOWhtwoWDCDynamicUP}{\rna}
\newcommand{\SLOWhtwoWDCDynamicUPCI}{\rna}
\newcommand{\SLOWhtwoWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGUP}{\rna}
\newcommand{\SLOWhtwoCAPOnoGUPCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOUP}{\rna}
\newcommand{\SLOWhtwoCAPOUPCI}{\rna}
\newcommand{\SLOWhtwoCAPOUPCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOUPCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPODynamicUP}{\rna}
\newcommand{\SLOWhtwoCAPODynamicUPCI}{\rna}
\newcommand{\SLOWhtwoCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPUP}{\rna}
\newcommand{\SLOWhtwoPIPUPCI}{\rna}
\newcommand{\SLOWhtwoPIPUPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPUPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPDynamicUP}{\rna}
\newcommand{\SLOWhtwoPIPDynamicUPCI}{\rna}
\newcommand{\SLOWhtwoPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPHB}{\rna}
\newcommand{\SLOWhtwoPIPHBCI}{\rna}
\newcommand{\SLOWhtwoPIPHBCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPHBCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPHBDynamic}{\rna}
\newcommand{\SLOWhtwoPIPHBDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPWCP}{\rna}
\newcommand{\SLOWhtwoPIPWCPCI}{\rna}
\newcommand{\SLOWhtwoPIPWCPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPWCPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPWCPDynamic}{\rna}
\newcommand{\SLOWhtwoPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPWDC}{\rna}
\newcommand{\SLOWhtwoPIPWDCCI}{\rna}
\newcommand{\SLOWhtwoPIPWDCCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPWDCCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPWDCDynamic}{\rna}
\newcommand{\SLOWhtwoPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPCAPO}{\rna}
\newcommand{\SLOWhtwoPIPCAPOCI}{\rna}
\newcommand{\SLOWhtwoPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPCAPODynamic}{\rna}
\newcommand{\SLOWhtwoPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPPIP}{\rna}
\newcommand{\SLOWhtwoPIPPIPCI}{\rna}
\newcommand{\SLOWhtwoPIPPIPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPPIPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPPIPDynamic}{\rna}
\newcommand{\SLOWhtwoPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonEvents}{730}
\newcommand{\SLOWjythonNoFPEvents}{290}
\newcommand{\SLOWjythonMaxLiveThreads}{2}
\newcommand{\SLOWjythonTotalThreads}{2}
\newcommand{\SLOWjythonBaseTime}{4.0}
\newcommand{\SLOWjythonBaseTimeCI}{98}
\newcommand{\SLOWjythonEmptyTime}{\rna}
\newcommand{\SLOWjythonEmptyTimeCI}{\rna}
\newcommand{\SLOWjythonEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWjythonEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWjythonFTTime}{8.1}
\newcommand{\SLOWjythonFTTimeCI}{0.23}
\newcommand{\SLOWjythonHBTime}{23}
\newcommand{\SLOWjythonHBTimeCI}{0.38}
\newcommand{\SLOWjythonWCPTime}{33}
\newcommand{\SLOWjythonWCPTimeCI}{1.1}
\newcommand{\SLOWjythonDCnoGExcTime}{26}
\newcommand{\SLOWjythonDCnoGExcTimeCI}{0.70}
\newcommand{\SLOWjythonDCnoGTime}{\rna}
\newcommand{\SLOWjythonDCnoGTimeCI}{\rna}
\newcommand{\SLOWjythonDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWjythonDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWjythonDCExcTime}{31}
\newcommand{\SLOWjythonDCExcTimeCI}{0.88}
\newcommand{\SLOWjythonDCTime}{\rna}
\newcommand{\SLOWjythonDCTimeCI}{\rna}
\newcommand{\SLOWjythonDCTimeCIMIN}{\rna}
\newcommand{\SLOWjythonDCTimeCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGExcTime}{23}
\newcommand{\SLOWjythonCAPOnoGExcTimeCI}{0.50}
\newcommand{\SLOWjythonCAPOnoGTime}{\rna}
\newcommand{\SLOWjythonCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOExcTime}{28}
\newcommand{\SLOWjythonCAPOExcTimeCI}{0.84}
\newcommand{\SLOWjythonCAPOTime}{\rna}
\newcommand{\SLOWjythonCAPOTimeCI}{\rna}
\newcommand{\SLOWjythonCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWjythonStaticTime}{\rzero}
\newcommand{\SLOWjythonDynamicTime}{\rzero}
\newcommand{\SLOWjythonBaseMem}{740}
\newcommand{\SLOWjythonBaseMemCI}{6.3}
\newcommand{\SLOWjythonHBMem}{22}
\newcommand{\SLOWjythonHBMemCI}{0.47}
\newcommand{\SLOWjythonFTMem}{6.4}
\newcommand{\SLOWjythonFTMemCI}{0.33}
\newcommand{\SLOWjythonWCPMem}{20}
\newcommand{\SLOWjythonWCPMemCI}{0.80}
\newcommand{\SLOWjythonDCnoGExcMem}{18}
\newcommand{\SLOWjythonDCnoGExcMemCI}{0.75}
\newcommand{\SLOWjythonDCnoGMem}{\memna}
\newcommand{\SLOWjythonDCnoGMemCI}{\memna}
\newcommand{\SLOWjythonDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWjythonDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWjythonDCExcMem}{31}
\newcommand{\SLOWjythonDCExcMemCI}{0.83}
\newcommand{\SLOWjythonDCMem}{\memna}
\newcommand{\SLOWjythonDCMemCI}{\memna}
\newcommand{\SLOWjythonDCMemCIMIN}{\memna}
\newcommand{\SLOWjythonDCMemCIMAX}{\memna}
\newcommand{\SLOWjythonCAPOnoGExcMem}{16}
\newcommand{\SLOWjythonCAPOnoGExcMemCI}{0.60}
\newcommand{\SLOWjythonCAPOnoGMem}{\memna}
\newcommand{\SLOWjythonCAPOnoGMemCI}{\memna}
\newcommand{\SLOWjythonCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWjythonCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWjythonCAPOExcMem}{24}
\newcommand{\SLOWjythonCAPOExcMemCI}{0.28}
\newcommand{\SLOWjythonCAPOMem}{\memna}
\newcommand{\SLOWjythonCAPOMemCI}{\memna}
\newcommand{\SLOWjythonCAPOMemCIMIN}{\memna}
\newcommand{\SLOWjythonCAPOMemCIMAX}{\memna}
\newcommand{\SLOWjythonEventsCI}{211}
\newcommand{\SLOWjythonEventsCIMIN}{728,376,678}
\newcommand{\SLOWjythonEventsCIMAX}{728,377,100}
\newcommand{\SLOWjythonNoFPEventsCI}{18}
\newcommand{\SLOWjythonNoFPEventsCIMIN}{293,898,196}
\newcommand{\SLOWjythonNoFPEventsCIMAX}{293,898,232}
\newcommand{\SLOWjythonHB}{21}
\newcommand{\SLOWjythonHBCI}{1}
\newcommand{\SLOWjythonHBCIMIN}{20}
\newcommand{\SLOWjythonHBCIMAX}{22}
\newcommand{\SLOWjythonHBDynamic}{22}
\newcommand{\SLOWjythonHBDynamicCI}{2}
\newcommand{\SLOWjythonHBDynamicCIMIN}{20}
\newcommand{\SLOWjythonHBDynamicCIMAX}{24}
\newcommand{\SLOWjythonFT}{22}
\newcommand{\SLOWjythonFTCI}{1.2}
\newcommand{\SLOWjythonFTCIMIN}{21}
\newcommand{\SLOWjythonFTCIMAX}{23}
\newcommand{\SLOWjythonFTDynamic}{47}
\newcommand{\SLOWjythonFTDynamicCI}{1.1}
\newcommand{\SLOWjythonFTDynamicCIMIN}{46}
\newcommand{\SLOWjythonFTDynamicCIMAX}{48}
\newcommand{\SLOWjythonWCP}{22}
\newcommand{\SLOWjythonWCPCI}{0}
\newcommand{\SLOWjythonWCPCIMIN}{22}
\newcommand{\SLOWjythonWCPCIMAX}{22}
\newcommand{\SLOWjythonWCPDynamic}{25}
\newcommand{\SLOWjythonWCPDynamicCI}{0.3}
\newcommand{\SLOWjythonWCPDynamicCIMIN}{25}
\newcommand{\SLOWjythonWCPDynamicCIMAX}{25}
\newcommand{\SLOWjythonDCnoGExc}{31}
\newcommand{\SLOWjythonDCnoGExcCI}{0}
\newcommand{\SLOWjythonDCnoGExcCIMIN}{31}
\newcommand{\SLOWjythonDCnoGExcCIMAX}{31}
\newcommand{\SLOWjythonDCnoGExcDynamic}{35}
\newcommand{\SLOWjythonDCnoGExcDynamicCI}{0}
\newcommand{\SLOWjythonDCnoGExcDynamicCIMIN}{35}
\newcommand{\SLOWjythonDCnoGExcDynamicCIMAX}{35}
\newcommand{\SLOWjythonDCnoG}{\rna}
\newcommand{\SLOWjythonDCnoGCI}{\rna}
\newcommand{\SLOWjythonDCnoGCIMIN}{\rna}
\newcommand{\SLOWjythonDCnoGCIMAX}{\rna}
\newcommand{\SLOWjythonDCnoGDynamic}{\rna}
\newcommand{\SLOWjythonDCnoGDynamicCI}{\rna}
\newcommand{\SLOWjythonDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonDCExc}{3}
\newcommand{\SLOWjythonDCExcCI}{0.30}
\newcommand{\SLOWjythonDCExcCIMIN}{3}
\newcommand{\SLOWjythonDCExcCIMAX}{3}
\newcommand{\SLOWjythonDCExcDynamic}{4}
\newcommand{\SLOWjythonDCExcDynamicCI}{0.60}
\newcommand{\SLOWjythonDCExcDynamicCIMIN}{3}
\newcommand{\SLOWjythonDCExcDynamicCIMAX}{5}
\newcommand{\SLOWjythonDC}{\rna}
\newcommand{\SLOWjythonDCCI}{\rna}
\newcommand{\SLOWjythonDCCIMIN}{\rna}
\newcommand{\SLOWjythonDCCIMAX}{\rna}
\newcommand{\SLOWjythonDCDynamic}{\rna}
\newcommand{\SLOWjythonDCDynamicCI}{\rna}
\newcommand{\SLOWjythonDCDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonDCDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGExc}{31}
\newcommand{\SLOWjythonCAPOnoGExcCI}{0}
\newcommand{\SLOWjythonCAPOnoGExcCIMIN}{31}
\newcommand{\SLOWjythonCAPOnoGExcCIMAX}{31}
\newcommand{\SLOWjythonCAPOnoGExcDynamic}{35}
\newcommand{\SLOWjythonCAPOnoGExcDynamicCI}{0}
\newcommand{\SLOWjythonCAPOnoGExcDynamicCIMIN}{35}
\newcommand{\SLOWjythonCAPOnoGExcDynamicCIMAX}{35}
\newcommand{\SLOWjythonCAPOnoG}{\rna}
\newcommand{\SLOWjythonCAPOnoGCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamic}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOExc}{3}
\newcommand{\SLOWjythonCAPOExcCI}{0.32}
\newcommand{\SLOWjythonCAPOExcCIMIN}{3}
\newcommand{\SLOWjythonCAPOExcCIMAX}{3}
\newcommand{\SLOWjythonCAPOExcDynamic}{4}
\newcommand{\SLOWjythonCAPOExcDynamicCI}{0.64}
\newcommand{\SLOWjythonCAPOExcDynamicCIMIN}{3}
\newcommand{\SLOWjythonCAPOExcDynamicCIMAX}{5}
\newcommand{\SLOWjythonCAPO}{\rna}
\newcommand{\SLOWjythonCAPOCI}{\rna}
\newcommand{\SLOWjythonCAPOCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOCIMAX}{\rna}
\newcommand{\SLOWjythonCAPODynamic}{\rna}
\newcommand{\SLOWjythonCAPODynamicCI}{\rna}
\newcommand{\SLOWjythonCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWjythonCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIP}{\rna}
\newcommand{\SLOWjythonPIPCI}{\rna}
\newcommand{\SLOWjythonPIPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPDynamic}{\rna}
\newcommand{\SLOWjythonPIPDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonHBUP}{21}
\newcommand{\SLOWjythonHBUPCI}{0.98}
\newcommand{\SLOWjythonHBUPCIMIN}{20}
\newcommand{\SLOWjythonHBUPCIMAX}{22}
\newcommand{\SLOWjythonHBDynamicUP}{22}
\newcommand{\SLOWjythonHBDynamicUPCI}{1.6}
\newcommand{\SLOWjythonHBDynamicUPCIMIN}{20}
\newcommand{\SLOWjythonHBDynamicUPCIMAX}{24}
\newcommand{\SLOWjythonWCPUP}{22}
\newcommand{\SLOWjythonWCPUPCI}{0}
\newcommand{\SLOWjythonWCPUPCIMIN}{22}
\newcommand{\SLOWjythonWCPUPCIMAX}{22}
\newcommand{\SLOWjythonWCPDynamicUP}{25}
\newcommand{\SLOWjythonWCPDynamicUPCI}{0.32}
\newcommand{\SLOWjythonWCPDynamicUPCIMIN}{25}
\newcommand{\SLOWjythonWCPDynamicUPCIMAX}{25}
\newcommand{\SLOWjythonWDCnoGUP}{\rna}
\newcommand{\SLOWjythonWDCnoGUPCI}{\rna}
\newcommand{\SLOWjythonWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWjythonWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWjythonWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWjythonWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWjythonWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonWDCUP}{\rna}
\newcommand{\SLOWjythonWDCUPCI}{\rna}
\newcommand{\SLOWjythonWDCUPCIMIN}{\rna}
\newcommand{\SLOWjythonWDCUPCIMAX}{\rna}
\newcommand{\SLOWjythonWDCDynamicUP}{\rna}
\newcommand{\SLOWjythonWDCDynamicUPCI}{\rna}
\newcommand{\SLOWjythonWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGUP}{\rna}
\newcommand{\SLOWjythonCAPOnoGUPCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOUP}{\rna}
\newcommand{\SLOWjythonCAPOUPCI}{\rna}
\newcommand{\SLOWjythonCAPOUPCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOUPCIMAX}{\rna}
\newcommand{\SLOWjythonCAPODynamicUP}{\rna}
\newcommand{\SLOWjythonCAPODynamicUPCI}{\rna}
\newcommand{\SLOWjythonCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPUP}{\rna}
\newcommand{\SLOWjythonPIPUPCI}{\rna}
\newcommand{\SLOWjythonPIPUPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPUPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPDynamicUP}{\rna}
\newcommand{\SLOWjythonPIPDynamicUPCI}{\rna}
\newcommand{\SLOWjythonPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPHB}{\rna}
\newcommand{\SLOWjythonPIPHBCI}{\rna}
\newcommand{\SLOWjythonPIPHBCIMIN}{\rna}
\newcommand{\SLOWjythonPIPHBCIMAX}{\rna}
\newcommand{\SLOWjythonPIPHBDynamic}{\rna}
\newcommand{\SLOWjythonPIPHBDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIPWCP}{\rna}
\newcommand{\SLOWjythonPIPWCPCI}{\rna}
\newcommand{\SLOWjythonPIPWCPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPWCPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPWCPDynamic}{\rna}
\newcommand{\SLOWjythonPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIPWDC}{\rna}
\newcommand{\SLOWjythonPIPWDCCI}{\rna}
\newcommand{\SLOWjythonPIPWDCCIMIN}{\rna}
\newcommand{\SLOWjythonPIPWDCCIMAX}{\rna}
\newcommand{\SLOWjythonPIPWDCDynamic}{\rna}
\newcommand{\SLOWjythonPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIPCAPO}{\rna}
\newcommand{\SLOWjythonPIPCAPOCI}{\rna}
\newcommand{\SLOWjythonPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWjythonPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWjythonPIPCAPODynamic}{\rna}
\newcommand{\SLOWjythonPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWjythonPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIPPIP}{\rna}
\newcommand{\SLOWjythonPIPPIPCI}{\rna}
\newcommand{\SLOWjythonPIPPIPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPPIPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPPIPDynamic}{\rna}
\newcommand{\SLOWjythonPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexEvents}{400}
\newcommand{\SLOWluindexNoFPEvents}{45}
\newcommand{\SLOWluindexMaxLiveThreads}{3}
\newcommand{\SLOWluindexTotalThreads}{3}
\newcommand{\SLOWluindexBaseTime}{1.2}
\newcommand{\SLOWluindexBaseTimeCI}{78}
\newcommand{\SLOWluindexEmptyTime}{\rna}
\newcommand{\SLOWluindexEmptyTimeCI}{\rna}
\newcommand{\SLOWluindexEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWluindexEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWluindexFTTime}{7.8}
\newcommand{\SLOWluindexFTTimeCI}{0.35}
\newcommand{\SLOWluindexHBTime}{28}
\newcommand{\SLOWluindexHBTimeCI}{1.3}
\newcommand{\SLOWluindexWCPTime}{47}
\newcommand{\SLOWluindexWCPTimeCI}{2.5}
\newcommand{\SLOWluindexDCnoGExcTime}{40}
\newcommand{\SLOWluindexDCnoGExcTimeCI}{2.0}
\newcommand{\SLOWluindexDCnoGTime}{\rna}
\newcommand{\SLOWluindexDCnoGTimeCI}{\rna}
\newcommand{\SLOWluindexDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWluindexDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWluindexDCExcTime}{44}
\newcommand{\SLOWluindexDCExcTimeCI}{2.3}
\newcommand{\SLOWluindexDCTime}{\rna}
\newcommand{\SLOWluindexDCTimeCI}{\rna}
\newcommand{\SLOWluindexDCTimeCIMIN}{\rna}
\newcommand{\SLOWluindexDCTimeCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGExcTime}{39}
\newcommand{\SLOWluindexCAPOnoGExcTimeCI}{2.1}
\newcommand{\SLOWluindexCAPOnoGTime}{\rna}
\newcommand{\SLOWluindexCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOExcTime}{44}
\newcommand{\SLOWluindexCAPOExcTimeCI}{2.5}
\newcommand{\SLOWluindexCAPOTime}{\rna}
\newcommand{\SLOWluindexCAPOTimeCI}{\rna}
\newcommand{\SLOWluindexCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWluindexStaticTime}{\rzero}
\newcommand{\SLOWluindexDynamicTime}{\rzero}
\newcommand{\SLOWluindexBaseMem}{120}
\newcommand{\SLOWluindexBaseMemCI}{8.9}
\newcommand{\SLOWluindexHBMem}{34}
\newcommand{\SLOWluindexHBMemCI}{2.2}
\newcommand{\SLOWluindexFTMem}{4.9}
\newcommand{\SLOWluindexFTMemCI}{0.31}
\newcommand{\SLOWluindexWCPMem}{71}
\newcommand{\SLOWluindexWCPMemCI}{4.5}
\newcommand{\SLOWluindexDCnoGExcMem}{51}
\newcommand{\SLOWluindexDCnoGExcMemCI}{3.5}
\newcommand{\SLOWluindexDCnoGMem}{\memna}
\newcommand{\SLOWluindexDCnoGMemCI}{\memna}
\newcommand{\SLOWluindexDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWluindexDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWluindexDCExcMem}{65}
\newcommand{\SLOWluindexDCExcMemCI}{4.4}
\newcommand{\SLOWluindexDCMem}{\memna}
\newcommand{\SLOWluindexDCMemCI}{\memna}
\newcommand{\SLOWluindexDCMemCIMIN}{\memna}
\newcommand{\SLOWluindexDCMemCIMAX}{\memna}
\newcommand{\SLOWluindexCAPOnoGExcMem}{50}
\newcommand{\SLOWluindexCAPOnoGExcMemCI}{3.3}
\newcommand{\SLOWluindexCAPOnoGMem}{\memna}
\newcommand{\SLOWluindexCAPOnoGMemCI}{\memna}
\newcommand{\SLOWluindexCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWluindexCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWluindexCAPOExcMem}{65}
\newcommand{\SLOWluindexCAPOExcMemCI}{4.1}
\newcommand{\SLOWluindexCAPOMem}{\memna}
\newcommand{\SLOWluindexCAPOMemCI}{\memna}
\newcommand{\SLOWluindexCAPOMemCIMIN}{\memna}
\newcommand{\SLOWluindexCAPOMemCIMAX}{\memna}
\newcommand{\SLOWluindexEventsCI}{4}
\newcommand{\SLOWluindexEventsCIMIN}{396,268,397}
\newcommand{\SLOWluindexEventsCIMAX}{396,268,405}
\newcommand{\SLOWluindexNoFPEventsCI}{3}
\newcommand{\SLOWluindexNoFPEventsCIMIN}{45,411,630}
\newcommand{\SLOWluindexNoFPEventsCIMAX}{45,411,636}
\newcommand{\SLOWluindexHB}{1}
\newcommand{\SLOWluindexHBCI}{0}
\newcommand{\SLOWluindexHBCIMIN}{1}
\newcommand{\SLOWluindexHBCIMAX}{1}
\newcommand{\SLOWluindexHBDynamic}{1}
\newcommand{\SLOWluindexHBDynamicCI}{0}
\newcommand{\SLOWluindexHBDynamicCIMIN}{1}
\newcommand{\SLOWluindexHBDynamicCIMAX}{1}
\newcommand{\SLOWluindexFT}{1}
\newcommand{\SLOWluindexFTCI}{0}
\newcommand{\SLOWluindexFTCIMIN}{1}
\newcommand{\SLOWluindexFTCIMAX}{1}
\newcommand{\SLOWluindexFTDynamic}{1}
\newcommand{\SLOWluindexFTDynamicCI}{0}
\newcommand{\SLOWluindexFTDynamicCIMIN}{1}
\newcommand{\SLOWluindexFTDynamicCIMAX}{1}
\newcommand{\SLOWluindexWCP}{1}
\newcommand{\SLOWluindexWCPCI}{0}
\newcommand{\SLOWluindexWCPCIMIN}{1}
\newcommand{\SLOWluindexWCPCIMAX}{1}
\newcommand{\SLOWluindexWCPDynamic}{1}
\newcommand{\SLOWluindexWCPDynamicCI}{0}
\newcommand{\SLOWluindexWCPDynamicCIMIN}{1}
\newcommand{\SLOWluindexWCPDynamicCIMAX}{1}
\newcommand{\SLOWluindexDCnoGExc}{1}
\newcommand{\SLOWluindexDCnoGExcCI}{0}
\newcommand{\SLOWluindexDCnoGExcCIMIN}{1}
\newcommand{\SLOWluindexDCnoGExcCIMAX}{1}
\newcommand{\SLOWluindexDCnoGExcDynamic}{1}
\newcommand{\SLOWluindexDCnoGExcDynamicCI}{0}
\newcommand{\SLOWluindexDCnoGExcDynamicCIMIN}{1}
\newcommand{\SLOWluindexDCnoGExcDynamicCIMAX}{1}
\newcommand{\SLOWluindexDCnoG}{\rna}
\newcommand{\SLOWluindexDCnoGCI}{\rna}
\newcommand{\SLOWluindexDCnoGCIMIN}{\rna}
\newcommand{\SLOWluindexDCnoGCIMAX}{\rna}
\newcommand{\SLOWluindexDCnoGDynamic}{\rna}
\newcommand{\SLOWluindexDCnoGDynamicCI}{\rna}
\newcommand{\SLOWluindexDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexDCExc}{1}
\newcommand{\SLOWluindexDCExcCI}{0}
\newcommand{\SLOWluindexDCExcCIMIN}{1}
\newcommand{\SLOWluindexDCExcCIMAX}{1}
\newcommand{\SLOWluindexDCExcDynamic}{1}
\newcommand{\SLOWluindexDCExcDynamicCI}{0}
\newcommand{\SLOWluindexDCExcDynamicCIMIN}{1}
\newcommand{\SLOWluindexDCExcDynamicCIMAX}{1}
\newcommand{\SLOWluindexDC}{\rna}
\newcommand{\SLOWluindexDCCI}{\rna}
\newcommand{\SLOWluindexDCCIMIN}{\rna}
\newcommand{\SLOWluindexDCCIMAX}{\rna}
\newcommand{\SLOWluindexDCDynamic}{\rna}
\newcommand{\SLOWluindexDCDynamicCI}{\rna}
\newcommand{\SLOWluindexDCDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexDCDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGExc}{1}
\newcommand{\SLOWluindexCAPOnoGExcCI}{0}
\newcommand{\SLOWluindexCAPOnoGExcCIMIN}{1}
\newcommand{\SLOWluindexCAPOnoGExcCIMAX}{1}
\newcommand{\SLOWluindexCAPOnoGExcDynamic}{1}
\newcommand{\SLOWluindexCAPOnoGExcDynamicCI}{0}
\newcommand{\SLOWluindexCAPOnoGExcDynamicCIMIN}{1}
\newcommand{\SLOWluindexCAPOnoGExcDynamicCIMAX}{1}
\newcommand{\SLOWluindexCAPOnoG}{\rna}
\newcommand{\SLOWluindexCAPOnoGCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamic}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOExc}{1}
\newcommand{\SLOWluindexCAPOExcCI}{0}
\newcommand{\SLOWluindexCAPOExcCIMIN}{1}
\newcommand{\SLOWluindexCAPOExcCIMAX}{1}
\newcommand{\SLOWluindexCAPOExcDynamic}{1}
\newcommand{\SLOWluindexCAPOExcDynamicCI}{0}
\newcommand{\SLOWluindexCAPOExcDynamicCIMIN}{1}
\newcommand{\SLOWluindexCAPOExcDynamicCIMAX}{1}
\newcommand{\SLOWluindexCAPO}{\rna}
\newcommand{\SLOWluindexCAPOCI}{\rna}
\newcommand{\SLOWluindexCAPOCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOCIMAX}{\rna}
\newcommand{\SLOWluindexCAPODynamic}{\rna}
\newcommand{\SLOWluindexCAPODynamicCI}{\rna}
\newcommand{\SLOWluindexCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWluindexCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIP}{\rna}
\newcommand{\SLOWluindexPIPCI}{\rna}
\newcommand{\SLOWluindexPIPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPDynamic}{\rna}
\newcommand{\SLOWluindexPIPDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexHBUP}{1}
\newcommand{\SLOWluindexHBUPCI}{0}
\newcommand{\SLOWluindexHBUPCIMIN}{1}
\newcommand{\SLOWluindexHBUPCIMAX}{1}
\newcommand{\SLOWluindexHBDynamicUP}{1}
\newcommand{\SLOWluindexHBDynamicUPCI}{0}
\newcommand{\SLOWluindexHBDynamicUPCIMIN}{1}
\newcommand{\SLOWluindexHBDynamicUPCIMAX}{1}
\newcommand{\SLOWluindexWCPUP}{1}
\newcommand{\SLOWluindexWCPUPCI}{0}
\newcommand{\SLOWluindexWCPUPCIMIN}{1}
\newcommand{\SLOWluindexWCPUPCIMAX}{1}
\newcommand{\SLOWluindexWCPDynamicUP}{1}
\newcommand{\SLOWluindexWCPDynamicUPCI}{0}
\newcommand{\SLOWluindexWCPDynamicUPCIMIN}{1}
\newcommand{\SLOWluindexWCPDynamicUPCIMAX}{1}
\newcommand{\SLOWluindexWDCnoGUP}{\rna}
\newcommand{\SLOWluindexWDCnoGUPCI}{\rna}
\newcommand{\SLOWluindexWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWluindexWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWluindexWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWluindexWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWluindexWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexWDCUP}{\rna}
\newcommand{\SLOWluindexWDCUPCI}{\rna}
\newcommand{\SLOWluindexWDCUPCIMIN}{\rna}
\newcommand{\SLOWluindexWDCUPCIMAX}{\rna}
\newcommand{\SLOWluindexWDCDynamicUP}{\rna}
\newcommand{\SLOWluindexWDCDynamicUPCI}{\rna}
\newcommand{\SLOWluindexWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGUP}{\rna}
\newcommand{\SLOWluindexCAPOnoGUPCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOUP}{\rna}
\newcommand{\SLOWluindexCAPOUPCI}{\rna}
\newcommand{\SLOWluindexCAPOUPCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOUPCIMAX}{\rna}
\newcommand{\SLOWluindexCAPODynamicUP}{\rna}
\newcommand{\SLOWluindexCAPODynamicUPCI}{\rna}
\newcommand{\SLOWluindexCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPUP}{\rna}
\newcommand{\SLOWluindexPIPUPCI}{\rna}
\newcommand{\SLOWluindexPIPUPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPUPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPDynamicUP}{\rna}
\newcommand{\SLOWluindexPIPDynamicUPCI}{\rna}
\newcommand{\SLOWluindexPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPHB}{\rna}
\newcommand{\SLOWluindexPIPHBCI}{\rna}
\newcommand{\SLOWluindexPIPHBCIMIN}{\rna}
\newcommand{\SLOWluindexPIPHBCIMAX}{\rna}
\newcommand{\SLOWluindexPIPHBDynamic}{\rna}
\newcommand{\SLOWluindexPIPHBDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIPWCP}{\rna}
\newcommand{\SLOWluindexPIPWCPCI}{\rna}
\newcommand{\SLOWluindexPIPWCPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPWCPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPWCPDynamic}{\rna}
\newcommand{\SLOWluindexPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIPWDC}{\rna}
\newcommand{\SLOWluindexPIPWDCCI}{\rna}
\newcommand{\SLOWluindexPIPWDCCIMIN}{\rna}
\newcommand{\SLOWluindexPIPWDCCIMAX}{\rna}
\newcommand{\SLOWluindexPIPWDCDynamic}{\rna}
\newcommand{\SLOWluindexPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIPCAPO}{\rna}
\newcommand{\SLOWluindexPIPCAPOCI}{\rna}
\newcommand{\SLOWluindexPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWluindexPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWluindexPIPCAPODynamic}{\rna}
\newcommand{\SLOWluindexPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWluindexPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIPPIP}{\rna}
\newcommand{\SLOWluindexPIPPIPCI}{\rna}
\newcommand{\SLOWluindexPIPPIPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPPIPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPPIPDynamic}{\rna}
\newcommand{\SLOWluindexPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchEvents}{1,400}
\newcommand{\SLOWlusearchNoFPEvents}{190}
\newcommand{\SLOWlusearchMaxLiveThreads}{10}
\newcommand{\SLOWlusearchTotalThreads}{10}
\newcommand{\SLOWlusearchBaseTime}{0.96}
\newcommand{\SLOWlusearchBaseTimeCI}{42}
\newcommand{\SLOWlusearchEmptyTime}{\rna}
\newcommand{\SLOWlusearchEmptyTimeCI}{\rna}
\newcommand{\SLOWlusearchEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchFTTime}{12}
\newcommand{\SLOWlusearchFTTimeCI}{0.61}
\newcommand{\SLOWlusearchHBTime}{30}
\newcommand{\SLOWlusearchHBTimeCI}{2.3}
\newcommand{\SLOWlusearchWCPTime}{40}
\newcommand{\SLOWlusearchWCPTimeCI}{3.3}
\newcommand{\SLOWlusearchDCnoGExcTime}{32}
\newcommand{\SLOWlusearchDCnoGExcTimeCI}{3.2}
\newcommand{\SLOWlusearchDCnoGTime}{\rna}
\newcommand{\SLOWlusearchDCnoGTimeCI}{\rna}
\newcommand{\SLOWlusearchDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchDCExcTime}{33}
\newcommand{\SLOWlusearchDCExcTimeCI}{1.3}
\newcommand{\SLOWlusearchDCTime}{\rna}
\newcommand{\SLOWlusearchDCTimeCI}{\rna}
\newcommand{\SLOWlusearchDCTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchDCTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGExcTime}{30}
\newcommand{\SLOWlusearchCAPOnoGExcTimeCI}{1.4}
\newcommand{\SLOWlusearchCAPOnoGTime}{\rna}
\newcommand{\SLOWlusearchCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOExcTime}{32}
\newcommand{\SLOWlusearchCAPOExcTimeCI}{1.1}
\newcommand{\SLOWlusearchCAPOTime}{\rna}
\newcommand{\SLOWlusearchCAPOTimeCI}{\rna}
\newcommand{\SLOWlusearchCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchStaticTime}{\rzero}
\newcommand{\SLOWlusearchDynamicTime}{\rzero}
\newcommand{\SLOWlusearchBaseMem}{1,600}
\newcommand{\SLOWlusearchBaseMemCI}{16.0}
\newcommand{\SLOWlusearchHBMem}{11}
\newcommand{\SLOWlusearchHBMemCI}{0.31}
\newcommand{\SLOWlusearchFTMem}{8.8}
\newcommand{\SLOWlusearchFTMemCI}{0.46}
\newcommand{\SLOWlusearchWCPMem}{16}
\newcommand{\SLOWlusearchWCPMemCI}{0.68}
\newcommand{\SLOWlusearchDCnoGExcMem}{12}
\newcommand{\SLOWlusearchDCnoGExcMemCI}{0.33}
\newcommand{\SLOWlusearchDCnoGMem}{\memna}
\newcommand{\SLOWlusearchDCnoGMemCI}{\memna}
\newcommand{\SLOWlusearchDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWlusearchDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWlusearchDCExcMem}{13}
\newcommand{\SLOWlusearchDCExcMemCI}{0.37}
\newcommand{\SLOWlusearchDCMem}{\memna}
\newcommand{\SLOWlusearchDCMemCI}{\memna}
\newcommand{\SLOWlusearchDCMemCIMIN}{\memna}
\newcommand{\SLOWlusearchDCMemCIMAX}{\memna}
\newcommand{\SLOWlusearchCAPOnoGExcMem}{12}
\newcommand{\SLOWlusearchCAPOnoGExcMemCI}{0.20}
\newcommand{\SLOWlusearchCAPOnoGMem}{\memna}
\newcommand{\SLOWlusearchCAPOnoGMemCI}{\memna}
\newcommand{\SLOWlusearchCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWlusearchCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWlusearchCAPOExcMem}{13}
\newcommand{\SLOWlusearchCAPOExcMemCI}{0.30}
\newcommand{\SLOWlusearchCAPOMem}{\memna}
\newcommand{\SLOWlusearchCAPOMemCI}{\memna}
\newcommand{\SLOWlusearchCAPOMemCIMIN}{\memna}
\newcommand{\SLOWlusearchCAPOMemCIMAX}{\memna}
\newcommand{\SLOWlusearchEventsCI}{21}
\newcommand{\SLOWlusearchEventsCIMIN}{1,443,227,212}
\newcommand{\SLOWlusearchEventsCIMAX}{1,443,227,254}
\newcommand{\SLOWlusearchNoFPEventsCI}{22}
\newcommand{\SLOWlusearchNoFPEventsCIMIN}{194,058,044}
\newcommand{\SLOWlusearchNoFPEventsCIMAX}{194,058,088}
\newcommand{\SLOWlusearchHB}{0}
\newcommand{\SLOWlusearchHBCI}{0}
\newcommand{\SLOWlusearchHBCIMIN}{0}
\newcommand{\SLOWlusearchHBCIMAX}{0}
\newcommand{\SLOWlusearchHBDynamic}{0}
\newcommand{\SLOWlusearchHBDynamicCI}{0}
\newcommand{\SLOWlusearchHBDynamicCIMIN}{0}
\newcommand{\SLOWlusearchHBDynamicCIMAX}{0}
\newcommand{\SLOWlusearchFT}{0}
\newcommand{\SLOWlusearchFTCI}{0}
\newcommand{\SLOWlusearchFTCIMIN}{0}
\newcommand{\SLOWlusearchFTCIMAX}{0}
\newcommand{\SLOWlusearchFTDynamic}{0}
\newcommand{\SLOWlusearchFTDynamicCI}{0}
\newcommand{\SLOWlusearchFTDynamicCIMIN}{0}
\newcommand{\SLOWlusearchFTDynamicCIMAX}{0}
\newcommand{\SLOWlusearchWCP}{0}
\newcommand{\SLOWlusearchWCPCI}{0}
\newcommand{\SLOWlusearchWCPCIMIN}{0}
\newcommand{\SLOWlusearchWCPCIMAX}{0}
\newcommand{\SLOWlusearchWCPDynamic}{0}
\newcommand{\SLOWlusearchWCPDynamicCI}{0}
\newcommand{\SLOWlusearchWCPDynamicCIMIN}{0}
\newcommand{\SLOWlusearchWCPDynamicCIMAX}{0}
\newcommand{\SLOWlusearchDCnoGExc}{0}
\newcommand{\SLOWlusearchDCnoGExcCI}{0}
\newcommand{\SLOWlusearchDCnoGExcCIMIN}{0}
\newcommand{\SLOWlusearchDCnoGExcCIMAX}{0}
\newcommand{\SLOWlusearchDCnoGExcDynamic}{0}
\newcommand{\SLOWlusearchDCnoGExcDynamicCI}{0}
\newcommand{\SLOWlusearchDCnoGExcDynamicCIMIN}{0}
\newcommand{\SLOWlusearchDCnoGExcDynamicCIMAX}{0}
\newcommand{\SLOWlusearchDCnoG}{\rna}
\newcommand{\SLOWlusearchDCnoGCI}{\rna}
\newcommand{\SLOWlusearchDCnoGCIMIN}{\rna}
\newcommand{\SLOWlusearchDCnoGCIMAX}{\rna}
\newcommand{\SLOWlusearchDCnoGDynamic}{\rna}
\newcommand{\SLOWlusearchDCnoGDynamicCI}{\rna}
\newcommand{\SLOWlusearchDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchDCExc}{0}
\newcommand{\SLOWlusearchDCExcCI}{0}
\newcommand{\SLOWlusearchDCExcCIMIN}{0}
\newcommand{\SLOWlusearchDCExcCIMAX}{0}
\newcommand{\SLOWlusearchDCExcDynamic}{0}
\newcommand{\SLOWlusearchDCExcDynamicCI}{0}
\newcommand{\SLOWlusearchDCExcDynamicCIMIN}{0}
\newcommand{\SLOWlusearchDCExcDynamicCIMAX}{0}
\newcommand{\SLOWlusearchDC}{\rna}
\newcommand{\SLOWlusearchDCCI}{\rna}
\newcommand{\SLOWlusearchDCCIMIN}{\rna}
\newcommand{\SLOWlusearchDCCIMAX}{\rna}
\newcommand{\SLOWlusearchDCDynamic}{\rna}
\newcommand{\SLOWlusearchDCDynamicCI}{\rna}
\newcommand{\SLOWlusearchDCDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchDCDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGExc}{0}
\newcommand{\SLOWlusearchCAPOnoGExcCI}{0}
\newcommand{\SLOWlusearchCAPOnoGExcCIMIN}{0}
\newcommand{\SLOWlusearchCAPOnoGExcCIMAX}{0}
\newcommand{\SLOWlusearchCAPOnoGExcDynamic}{0}
\newcommand{\SLOWlusearchCAPOnoGExcDynamicCI}{0}
\newcommand{\SLOWlusearchCAPOnoGExcDynamicCIMIN}{0}
\newcommand{\SLOWlusearchCAPOnoGExcDynamicCIMAX}{0}
\newcommand{\SLOWlusearchCAPOnoG}{\rna}
\newcommand{\SLOWlusearchCAPOnoGCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamic}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOExc}{0}
\newcommand{\SLOWlusearchCAPOExcCI}{0}
\newcommand{\SLOWlusearchCAPOExcCIMIN}{0}
\newcommand{\SLOWlusearchCAPOExcCIMAX}{0}
\newcommand{\SLOWlusearchCAPOExcDynamic}{0}
\newcommand{\SLOWlusearchCAPOExcDynamicCI}{0}
\newcommand{\SLOWlusearchCAPOExcDynamicCIMIN}{0}
\newcommand{\SLOWlusearchCAPOExcDynamicCIMAX}{0}
\newcommand{\SLOWlusearchCAPO}{\rna}
\newcommand{\SLOWlusearchCAPOCI}{\rna}
\newcommand{\SLOWlusearchCAPOCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPODynamic}{\rna}
\newcommand{\SLOWlusearchCAPODynamicCI}{\rna}
\newcommand{\SLOWlusearchCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIP}{\rna}
\newcommand{\SLOWlusearchPIPCI}{\rna}
\newcommand{\SLOWlusearchPIPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPDynamic}{\rna}
\newcommand{\SLOWlusearchPIPDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchHBUP}{0}
\newcommand{\SLOWlusearchHBUPCI}{0}
\newcommand{\SLOWlusearchHBUPCIMIN}{0}
\newcommand{\SLOWlusearchHBUPCIMAX}{0}
\newcommand{\SLOWlusearchHBDynamicUP}{0}
\newcommand{\SLOWlusearchHBDynamicUPCI}{0}
\newcommand{\SLOWlusearchHBDynamicUPCIMIN}{0}
\newcommand{\SLOWlusearchHBDynamicUPCIMAX}{0}
\newcommand{\SLOWlusearchWCPUP}{0}
\newcommand{\SLOWlusearchWCPUPCI}{0}
\newcommand{\SLOWlusearchWCPUPCIMIN}{0}
\newcommand{\SLOWlusearchWCPUPCIMAX}{0}
\newcommand{\SLOWlusearchWCPDynamicUP}{0}
\newcommand{\SLOWlusearchWCPDynamicUPCI}{0}
\newcommand{\SLOWlusearchWCPDynamicUPCIMIN}{0}
\newcommand{\SLOWlusearchWCPDynamicUPCIMAX}{0}
\newcommand{\SLOWlusearchWDCnoGUP}{\rna}
\newcommand{\SLOWlusearchWDCnoGUPCI}{\rna}
\newcommand{\SLOWlusearchWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWlusearchWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWlusearchWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWlusearchWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWlusearchWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchWDCUP}{\rna}
\newcommand{\SLOWlusearchWDCUPCI}{\rna}
\newcommand{\SLOWlusearchWDCUPCIMIN}{\rna}
\newcommand{\SLOWlusearchWDCUPCIMAX}{\rna}
\newcommand{\SLOWlusearchWDCDynamicUP}{\rna}
\newcommand{\SLOWlusearchWDCDynamicUPCI}{\rna}
\newcommand{\SLOWlusearchWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGUP}{\rna}
\newcommand{\SLOWlusearchCAPOnoGUPCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOUP}{\rna}
\newcommand{\SLOWlusearchCAPOUPCI}{\rna}
\newcommand{\SLOWlusearchCAPOUPCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOUPCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPODynamicUP}{\rna}
\newcommand{\SLOWlusearchCAPODynamicUPCI}{\rna}
\newcommand{\SLOWlusearchCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPUP}{\rna}
\newcommand{\SLOWlusearchPIPUPCI}{\rna}
\newcommand{\SLOWlusearchPIPUPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPUPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPDynamicUP}{\rna}
\newcommand{\SLOWlusearchPIPDynamicUPCI}{\rna}
\newcommand{\SLOWlusearchPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPHB}{\rna}
\newcommand{\SLOWlusearchPIPHBCI}{\rna}
\newcommand{\SLOWlusearchPIPHBCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPHBCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPHBDynamic}{\rna}
\newcommand{\SLOWlusearchPIPHBDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPWCP}{\rna}
\newcommand{\SLOWlusearchPIPWCPCI}{\rna}
\newcommand{\SLOWlusearchPIPWCPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPWCPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPWCPDynamic}{\rna}
\newcommand{\SLOWlusearchPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPWDC}{\rna}
\newcommand{\SLOWlusearchPIPWDCCI}{\rna}
\newcommand{\SLOWlusearchPIPWDCCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPWDCCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPWDCDynamic}{\rna}
\newcommand{\SLOWlusearchPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPCAPO}{\rna}
\newcommand{\SLOWlusearchPIPCAPOCI}{\rna}
\newcommand{\SLOWlusearchPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPCAPODynamic}{\rna}
\newcommand{\SLOWlusearchPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPPIP}{\rna}
\newcommand{\SLOWlusearchPIPPIPCI}{\rna}
\newcommand{\SLOWlusearchPIPPIPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPPIPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPPIPDynamic}{\rna}
\newcommand{\SLOWlusearchPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdEvents}{200}
\newcommand{\SLOWpmdNoFPEvents}{25}
\newcommand{\SLOWpmdMaxLiveThreads}{9}
\newcommand{\SLOWpmdTotalThreads}{9}
\newcommand{\SLOWpmdBaseTime}{1.4}
\newcommand{\SLOWpmdBaseTimeCI}{22}
\newcommand{\SLOWpmdEmptyTime}{\rna}
\newcommand{\SLOWpmdEmptyTimeCI}{\rna}
\newcommand{\SLOWpmdEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWpmdEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWpmdFTTime}{6.0}
\newcommand{\SLOWpmdFTTimeCI}{0.16}
\newcommand{\SLOWpmdHBTime}{13}
\newcommand{\SLOWpmdHBTimeCI}{0.27}
\newcommand{\SLOWpmdWCPTime}{16}
\newcommand{\SLOWpmdWCPTimeCI}{0.50}
\newcommand{\SLOWpmdDCnoGExcTime}{14}
\newcommand{\SLOWpmdDCnoGExcTimeCI}{0.33}
\newcommand{\SLOWpmdDCnoGTime}{\rna}
\newcommand{\SLOWpmdDCnoGTimeCI}{\rna}
\newcommand{\SLOWpmdDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWpmdDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWpmdDCExcTime}{15}
\newcommand{\SLOWpmdDCExcTimeCI}{0.30}
\newcommand{\SLOWpmdDCTime}{\rna}
\newcommand{\SLOWpmdDCTimeCI}{\rna}
\newcommand{\SLOWpmdDCTimeCIMIN}{\rna}
\newcommand{\SLOWpmdDCTimeCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGExcTime}{14}
\newcommand{\SLOWpmdCAPOnoGExcTimeCI}{0.36}
\newcommand{\SLOWpmdCAPOnoGTime}{\rna}
\newcommand{\SLOWpmdCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOExcTime}{15}
\newcommand{\SLOWpmdCAPOExcTimeCI}{0.33}
\newcommand{\SLOWpmdCAPOTime}{\rna}
\newcommand{\SLOWpmdCAPOTimeCI}{\rna}
\newcommand{\SLOWpmdCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWpmdStaticTime}{\rzero}
\newcommand{\SLOWpmdDynamicTime}{\rzero}
\newcommand{\SLOWpmdBaseMem}{590}
\newcommand{\SLOWpmdBaseMemCI}{13.0}
\newcommand{\SLOWpmdHBMem}{11}
\newcommand{\SLOWpmdHBMemCI}{0.38}
\newcommand{\SLOWpmdFTMem}{2.7}
\newcommand{\SLOWpmdFTMemCI}{0.17}
\newcommand{\SLOWpmdWCPMem}{17}
\newcommand{\SLOWpmdWCPMemCI}{0.71}
\newcommand{\SLOWpmdDCnoGExcMem}{11}
\newcommand{\SLOWpmdDCnoGExcMemCI}{0.20}
\newcommand{\SLOWpmdDCnoGMem}{\memna}
\newcommand{\SLOWpmdDCnoGMemCI}{\memna}
\newcommand{\SLOWpmdDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWpmdDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWpmdDCExcMem}{13}
\newcommand{\SLOWpmdDCExcMemCI}{0.30}
\newcommand{\SLOWpmdDCMem}{\memna}
\newcommand{\SLOWpmdDCMemCI}{\memna}
\newcommand{\SLOWpmdDCMemCIMIN}{\memna}
\newcommand{\SLOWpmdDCMemCIMAX}{\memna}
\newcommand{\SLOWpmdCAPOnoGExcMem}{11}
\newcommand{\SLOWpmdCAPOnoGExcMemCI}{0.28}
\newcommand{\SLOWpmdCAPOnoGMem}{\memna}
\newcommand{\SLOWpmdCAPOnoGMemCI}{\memna}
\newcommand{\SLOWpmdCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWpmdCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWpmdCAPOExcMem}{13}
\newcommand{\SLOWpmdCAPOExcMemCI}{0.33}
\newcommand{\SLOWpmdCAPOMem}{\memna}
\newcommand{\SLOWpmdCAPOMemCI}{\memna}
\newcommand{\SLOWpmdCAPOMemCIMIN}{\memna}
\newcommand{\SLOWpmdCAPOMemCIMAX}{\memna}
\newcommand{\SLOWpmdEventsCI}{455}
\newcommand{\SLOWpmdEventsCIMIN}{200,051,915}
\newcommand{\SLOWpmdEventsCIMAX}{200,052,825}
\newcommand{\SLOWpmdNoFPEventsCI}{55}
\newcommand{\SLOWpmdNoFPEventsCIMIN}{25,405,134}
\newcommand{\SLOWpmdNoFPEventsCIMAX}{25,405,244}
\newcommand{\SLOWpmdHB}{6}
\newcommand{\SLOWpmdHBCI}{0}
\newcommand{\SLOWpmdHBCIMIN}{6}
\newcommand{\SLOWpmdHBCIMAX}{6}
\newcommand{\SLOWpmdHBDynamic}{203}
\newcommand{\SLOWpmdHBDynamicCI}{57}
\newcommand{\SLOWpmdHBDynamicCIMIN}{146}
\newcommand{\SLOWpmdHBDynamicCIMAX}{260}
\newcommand{\SLOWpmdFT}{18}
\newcommand{\SLOWpmdFTCI}{0}
\newcommand{\SLOWpmdFTCIMIN}{18}
\newcommand{\SLOWpmdFTCIMAX}{18}
\newcommand{\SLOWpmdFTDynamic}{4,450}
\newcommand{\SLOWpmdFTDynamicCI}{972}
\newcommand{\SLOWpmdFTDynamicCIMIN}{3,478}
\newcommand{\SLOWpmdFTDynamicCIMAX}{5,422}
\newcommand{\SLOWpmdWCP}{6}
\newcommand{\SLOWpmdWCPCI}{0}
\newcommand{\SLOWpmdWCPCIMIN}{6}
\newcommand{\SLOWpmdWCPCIMAX}{6}
\newcommand{\SLOWpmdWCPDynamic}{147}
\newcommand{\SLOWpmdWCPDynamicCI}{17}
\newcommand{\SLOWpmdWCPDynamicCIMIN}{130}
\newcommand{\SLOWpmdWCPDynamicCIMAX}{164}
\newcommand{\SLOWpmdDCnoGExc}{10}
\newcommand{\SLOWpmdDCnoGExcCI}{0}
\newcommand{\SLOWpmdDCnoGExcCIMIN}{10}
\newcommand{\SLOWpmdDCnoGExcCIMAX}{10}
\newcommand{\SLOWpmdDCnoGExcDynamic}{1,391}
\newcommand{\SLOWpmdDCnoGExcDynamicCI}{137}
\newcommand{\SLOWpmdDCnoGExcDynamicCIMIN}{1,254}
\newcommand{\SLOWpmdDCnoGExcDynamicCIMAX}{1,528}
\newcommand{\SLOWpmdDCnoG}{\rna}
\newcommand{\SLOWpmdDCnoGCI}{\rna}
\newcommand{\SLOWpmdDCnoGCIMIN}{\rna}
\newcommand{\SLOWpmdDCnoGCIMAX}{\rna}
\newcommand{\SLOWpmdDCnoGDynamic}{\rna}
\newcommand{\SLOWpmdDCnoGDynamicCI}{\rna}
\newcommand{\SLOWpmdDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdDCExc}{5}
\newcommand{\SLOWpmdDCExcCI}{0.20}
\newcommand{\SLOWpmdDCExcCIMIN}{5}
\newcommand{\SLOWpmdDCExcCIMAX}{5}
\newcommand{\SLOWpmdDCExcDynamic}{28}
\newcommand{\SLOWpmdDCExcDynamicCI}{2.9}
\newcommand{\SLOWpmdDCExcDynamicCIMIN}{25}
\newcommand{\SLOWpmdDCExcDynamicCIMAX}{31}
\newcommand{\SLOWpmdDC}{\rna}
\newcommand{\SLOWpmdDCCI}{\rna}
\newcommand{\SLOWpmdDCCIMIN}{\rna}
\newcommand{\SLOWpmdDCCIMAX}{\rna}
\newcommand{\SLOWpmdDCDynamic}{\rna}
\newcommand{\SLOWpmdDCDynamicCI}{\rna}
\newcommand{\SLOWpmdDCDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdDCDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGExc}{10}
\newcommand{\SLOWpmdCAPOnoGExcCI}{0}
\newcommand{\SLOWpmdCAPOnoGExcCIMIN}{10}
\newcommand{\SLOWpmdCAPOnoGExcCIMAX}{10}
\newcommand{\SLOWpmdCAPOnoGExcDynamic}{1,376}
\newcommand{\SLOWpmdCAPOnoGExcDynamicCI}{156}
\newcommand{\SLOWpmdCAPOnoGExcDynamicCIMIN}{1,220}
\newcommand{\SLOWpmdCAPOnoGExcDynamicCIMAX}{1,532}
\newcommand{\SLOWpmdCAPOnoG}{\rna}
\newcommand{\SLOWpmdCAPOnoGCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamic}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOExc}{6}
\newcommand{\SLOWpmdCAPOExcCI}{0.32}
\newcommand{\SLOWpmdCAPOExcCIMIN}{6}
\newcommand{\SLOWpmdCAPOExcCIMAX}{6}
\newcommand{\SLOWpmdCAPOExcDynamic}{32}
\newcommand{\SLOWpmdCAPOExcDynamicCI}{3.1}
\newcommand{\SLOWpmdCAPOExcDynamicCIMIN}{29}
\newcommand{\SLOWpmdCAPOExcDynamicCIMAX}{35}
\newcommand{\SLOWpmdCAPO}{\rna}
\newcommand{\SLOWpmdCAPOCI}{\rna}
\newcommand{\SLOWpmdCAPOCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOCIMAX}{\rna}
\newcommand{\SLOWpmdCAPODynamic}{\rna}
\newcommand{\SLOWpmdCAPODynamicCI}{\rna}
\newcommand{\SLOWpmdCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWpmdCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIP}{\rna}
\newcommand{\SLOWpmdPIPCI}{\rna}
\newcommand{\SLOWpmdPIPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPDynamic}{\rna}
\newcommand{\SLOWpmdPIPDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdHBUP}{6}
\newcommand{\SLOWpmdHBUPCI}{0}
\newcommand{\SLOWpmdHBUPCIMIN}{6}
\newcommand{\SLOWpmdHBUPCIMAX}{6}
\newcommand{\SLOWpmdHBDynamicUP}{202}
\newcommand{\SLOWpmdHBDynamicUPCI}{57}
\newcommand{\SLOWpmdHBDynamicUPCIMIN}{145}
\newcommand{\SLOWpmdHBDynamicUPCIMAX}{259}
\newcommand{\SLOWpmdWCPUP}{6}
\newcommand{\SLOWpmdWCPUPCI}{0}
\newcommand{\SLOWpmdWCPUPCIMIN}{6}
\newcommand{\SLOWpmdWCPUPCIMAX}{6}
\newcommand{\SLOWpmdWCPDynamicUP}{147}
\newcommand{\SLOWpmdWCPDynamicUPCI}{17}
\newcommand{\SLOWpmdWCPDynamicUPCIMIN}{130}
\newcommand{\SLOWpmdWCPDynamicUPCIMAX}{164}
\newcommand{\SLOWpmdWDCnoGUP}{\rna}
\newcommand{\SLOWpmdWDCnoGUPCI}{\rna}
\newcommand{\SLOWpmdWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWpmdWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWpmdWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWpmdWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWpmdWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdWDCUP}{\rna}
\newcommand{\SLOWpmdWDCUPCI}{\rna}
\newcommand{\SLOWpmdWDCUPCIMIN}{\rna}
\newcommand{\SLOWpmdWDCUPCIMAX}{\rna}
\newcommand{\SLOWpmdWDCDynamicUP}{\rna}
\newcommand{\SLOWpmdWDCDynamicUPCI}{\rna}
\newcommand{\SLOWpmdWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGUP}{\rna}
\newcommand{\SLOWpmdCAPOnoGUPCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOUP}{\rna}
\newcommand{\SLOWpmdCAPOUPCI}{\rna}
\newcommand{\SLOWpmdCAPOUPCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOUPCIMAX}{\rna}
\newcommand{\SLOWpmdCAPODynamicUP}{\rna}
\newcommand{\SLOWpmdCAPODynamicUPCI}{\rna}
\newcommand{\SLOWpmdCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPUP}{\rna}
\newcommand{\SLOWpmdPIPUPCI}{\rna}
\newcommand{\SLOWpmdPIPUPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPUPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPDynamicUP}{\rna}
\newcommand{\SLOWpmdPIPDynamicUPCI}{\rna}
\newcommand{\SLOWpmdPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPHB}{\rna}
\newcommand{\SLOWpmdPIPHBCI}{\rna}
\newcommand{\SLOWpmdPIPHBCIMIN}{\rna}
\newcommand{\SLOWpmdPIPHBCIMAX}{\rna}
\newcommand{\SLOWpmdPIPHBDynamic}{\rna}
\newcommand{\SLOWpmdPIPHBDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIPWCP}{\rna}
\newcommand{\SLOWpmdPIPWCPCI}{\rna}
\newcommand{\SLOWpmdPIPWCPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPWCPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPWCPDynamic}{\rna}
\newcommand{\SLOWpmdPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIPWDC}{\rna}
\newcommand{\SLOWpmdPIPWDCCI}{\rna}
\newcommand{\SLOWpmdPIPWDCCIMIN}{\rna}
\newcommand{\SLOWpmdPIPWDCCIMAX}{\rna}
\newcommand{\SLOWpmdPIPWDCDynamic}{\rna}
\newcommand{\SLOWpmdPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIPCAPO}{\rna}
\newcommand{\SLOWpmdPIPCAPOCI}{\rna}
\newcommand{\SLOWpmdPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWpmdPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWpmdPIPCAPODynamic}{\rna}
\newcommand{\SLOWpmdPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWpmdPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIPPIP}{\rna}
\newcommand{\SLOWpmdPIPPIPCI}{\rna}
\newcommand{\SLOWpmdPIPPIPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPPIPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPPIPDynamic}{\rna}
\newcommand{\SLOWpmdPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowEvents}{9,700}
\newcommand{\SLOWsunflowNoFPEvents}{760}
\newcommand{\SLOWsunflowMaxLiveThreads}{17}
\newcommand{\SLOWsunflowTotalThreads}{17}
\newcommand{\SLOWsunflowBaseTime}{1.4}
\newcommand{\SLOWsunflowBaseTimeCI}{33}
\newcommand{\SLOWsunflowEmptyTime}{\rna}
\newcommand{\SLOWsunflowEmptyTimeCI}{\rna}
\newcommand{\SLOWsunflowEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowFTTime}{23}
\newcommand{\SLOWsunflowFTTimeCI}{0.74}
\newcommand{\SLOWsunflowHBTime}{89}
\newcommand{\SLOWsunflowHBTimeCI}{2.6}
\newcommand{\SLOWsunflowWCPTime}{110}
\newcommand{\SLOWsunflowWCPTimeCI}{3.2}
\newcommand{\SLOWsunflowDCnoGExcTime}{88}
\newcommand{\SLOWsunflowDCnoGExcTimeCI}{2.1}
\newcommand{\SLOWsunflowDCnoGTime}{\rna}
\newcommand{\SLOWsunflowDCnoGTimeCI}{\rna}
\newcommand{\SLOWsunflowDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowDCExcTime}{100}
\newcommand{\SLOWsunflowDCExcTimeCI}{9.5}
\newcommand{\SLOWsunflowDCTime}{\rna}
\newcommand{\SLOWsunflowDCTimeCI}{\rna}
\newcommand{\SLOWsunflowDCTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowDCTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGExcTime}{88}
\newcommand{\SLOWsunflowCAPOnoGExcTimeCI}{2.4}
\newcommand{\SLOWsunflowCAPOnoGTime}{\rna}
\newcommand{\SLOWsunflowCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOExcTime}{110}
\newcommand{\SLOWsunflowCAPOExcTimeCI}{12}
\newcommand{\SLOWsunflowCAPOTime}{\rna}
\newcommand{\SLOWsunflowCAPOTimeCI}{\rna}
\newcommand{\SLOWsunflowCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowStaticTime}{\rzero}
\newcommand{\SLOWsunflowDynamicTime}{\rzero}
\newcommand{\SLOWsunflowBaseMem}{610}
\newcommand{\SLOWsunflowBaseMemCI}{4.2}
\newcommand{\SLOWsunflowHBMem}{23}
\newcommand{\SLOWsunflowHBMemCI}{0.87}
\newcommand{\SLOWsunflowFTMem}{8.2}
\newcommand{\SLOWsunflowFTMemCI}{0.062}
\newcommand{\SLOWsunflowWCPMem}{54}
\newcommand{\SLOWsunflowWCPMemCI}{1.3}
\newcommand{\SLOWsunflowDCnoGExcMem}{24}
\newcommand{\SLOWsunflowDCnoGExcMemCI}{0.35}
\newcommand{\SLOWsunflowDCnoGMem}{\memna}
\newcommand{\SLOWsunflowDCnoGMemCI}{\memna}
\newcommand{\SLOWsunflowDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWsunflowDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWsunflowDCExcMem}{26}
\newcommand{\SLOWsunflowDCExcMemCI}{0.68}
\newcommand{\SLOWsunflowDCMem}{\memna}
\newcommand{\SLOWsunflowDCMemCI}{\memna}
\newcommand{\SLOWsunflowDCMemCIMIN}{\memna}
\newcommand{\SLOWsunflowDCMemCIMAX}{\memna}
\newcommand{\SLOWsunflowCAPOnoGExcMem}{24}
\newcommand{\SLOWsunflowCAPOnoGExcMemCI}{0.41}
\newcommand{\SLOWsunflowCAPOnoGMem}{\memna}
\newcommand{\SLOWsunflowCAPOnoGMemCI}{\memna}
\newcommand{\SLOWsunflowCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWsunflowCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWsunflowCAPOExcMem}{26}
\newcommand{\SLOWsunflowCAPOExcMemCI}{0.87}
\newcommand{\SLOWsunflowCAPOMem}{\memna}
\newcommand{\SLOWsunflowCAPOMemCI}{\memna}
\newcommand{\SLOWsunflowCAPOMemCIMIN}{\memna}
\newcommand{\SLOWsunflowCAPOMemCIMAX}{\memna}
\newcommand{\SLOWsunflowEventsCI}{1}
\newcommand{\SLOWsunflowEventsCIMIN}{9,681,321,388}
\newcommand{\SLOWsunflowEventsCIMAX}{9,681,321,390}
\newcommand{\SLOWsunflowNoFPEventsCI}{5}
\newcommand{\SLOWsunflowNoFPEventsCIMIN}{764,388,873}
\newcommand{\SLOWsunflowNoFPEventsCIMAX}{764,388,883}
\newcommand{\SLOWsunflowHB}{6}
\newcommand{\SLOWsunflowHBCI}{0}
\newcommand{\SLOWsunflowHBCIMIN}{6}
\newcommand{\SLOWsunflowHBCIMAX}{6}
\newcommand{\SLOWsunflowHBDynamic}{32}
\newcommand{\SLOWsunflowHBDynamicCI}{3}
\newcommand{\SLOWsunflowHBDynamicCIMIN}{29}
\newcommand{\SLOWsunflowHBDynamicCIMAX}{35}
\newcommand{\SLOWsunflowFT}{5}
\newcommand{\SLOWsunflowFTCI}{0}
\newcommand{\SLOWsunflowFTCIMIN}{5}
\newcommand{\SLOWsunflowFTCIMAX}{5}
\newcommand{\SLOWsunflowFTDynamic}{61}
\newcommand{\SLOWsunflowFTDynamicCI}{6.1}
\newcommand{\SLOWsunflowFTDynamicCIMIN}{55}
\newcommand{\SLOWsunflowFTDynamicCIMAX}{67}
\newcommand{\SLOWsunflowWCP}{18}
\newcommand{\SLOWsunflowWCPCI}{0}
\newcommand{\SLOWsunflowWCPCIMIN}{18}
\newcommand{\SLOWsunflowWCPCIMAX}{18}
\newcommand{\SLOWsunflowWCPDynamic}{153}
\newcommand{\SLOWsunflowWCPDynamicCI}{4}
\newcommand{\SLOWsunflowWCPDynamicCIMIN}{149}
\newcommand{\SLOWsunflowWCPDynamicCIMAX}{157}
\newcommand{\SLOWsunflowDCnoGExc}{19}
\newcommand{\SLOWsunflowDCnoGExcCI}{0}
\newcommand{\SLOWsunflowDCnoGExcCIMIN}{19}
\newcommand{\SLOWsunflowDCnoGExcCIMAX}{19}
\newcommand{\SLOWsunflowDCnoGExcDynamic}{417}
\newcommand{\SLOWsunflowDCnoGExcDynamicCI}{38}
\newcommand{\SLOWsunflowDCnoGExcDynamicCIMIN}{379}
\newcommand{\SLOWsunflowDCnoGExcDynamicCIMAX}{455}
\newcommand{\SLOWsunflowDCnoG}{\rna}
\newcommand{\SLOWsunflowDCnoGCI}{\rna}
\newcommand{\SLOWsunflowDCnoGCIMIN}{\rna}
\newcommand{\SLOWsunflowDCnoGCIMAX}{\rna}
\newcommand{\SLOWsunflowDCnoGDynamic}{\rna}
\newcommand{\SLOWsunflowDCnoGDynamicCI}{\rna}
\newcommand{\SLOWsunflowDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowDCExc}{3}
\newcommand{\SLOWsunflowDCExcCI}{0}
\newcommand{\SLOWsunflowDCExcCIMIN}{3}
\newcommand{\SLOWsunflowDCExcCIMAX}{3}
\newcommand{\SLOWsunflowDCExcDynamic}{14}
\newcommand{\SLOWsunflowDCExcDynamicCI}{0}
\newcommand{\SLOWsunflowDCExcDynamicCIMIN}{14}
\newcommand{\SLOWsunflowDCExcDynamicCIMAX}{14}
\newcommand{\SLOWsunflowDC}{\rna}
\newcommand{\SLOWsunflowDCCI}{\rna}
\newcommand{\SLOWsunflowDCCIMIN}{\rna}
\newcommand{\SLOWsunflowDCCIMAX}{\rna}
\newcommand{\SLOWsunflowDCDynamic}{\rna}
\newcommand{\SLOWsunflowDCDynamicCI}{\rna}
\newcommand{\SLOWsunflowDCDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowDCDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGExc}{19}
\newcommand{\SLOWsunflowCAPOnoGExcCI}{0}
\newcommand{\SLOWsunflowCAPOnoGExcCIMIN}{19}
\newcommand{\SLOWsunflowCAPOnoGExcCIMAX}{19}
\newcommand{\SLOWsunflowCAPOnoGExcDynamic}{345}
\newcommand{\SLOWsunflowCAPOnoGExcDynamicCI}{81}
\newcommand{\SLOWsunflowCAPOnoGExcDynamicCIMIN}{264}
\newcommand{\SLOWsunflowCAPOnoGExcDynamicCIMAX}{426}
\newcommand{\SLOWsunflowCAPOnoG}{\rna}
\newcommand{\SLOWsunflowCAPOnoGCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamic}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOExc}{3}
\newcommand{\SLOWsunflowCAPOExcCI}{0}
\newcommand{\SLOWsunflowCAPOExcCIMIN}{3}
\newcommand{\SLOWsunflowCAPOExcCIMAX}{3}
\newcommand{\SLOWsunflowCAPOExcDynamic}{14}
\newcommand{\SLOWsunflowCAPOExcDynamicCI}{0}
\newcommand{\SLOWsunflowCAPOExcDynamicCIMIN}{14}
\newcommand{\SLOWsunflowCAPOExcDynamicCIMAX}{14}
\newcommand{\SLOWsunflowCAPO}{\rna}
\newcommand{\SLOWsunflowCAPOCI}{\rna}
\newcommand{\SLOWsunflowCAPOCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPODynamic}{\rna}
\newcommand{\SLOWsunflowCAPODynamicCI}{\rna}
\newcommand{\SLOWsunflowCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIP}{\rna}
\newcommand{\SLOWsunflowPIPCI}{\rna}
\newcommand{\SLOWsunflowPIPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPDynamic}{\rna}
\newcommand{\SLOWsunflowPIPDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowHBUP}{5}
\newcommand{\SLOWsunflowHBUPCI}{0}
\newcommand{\SLOWsunflowHBUPCIMIN}{5}
\newcommand{\SLOWsunflowHBUPCIMAX}{5}
\newcommand{\SLOWsunflowHBDynamicUP}{32}
\newcommand{\SLOWsunflowHBDynamicUPCI}{2.8}
\newcommand{\SLOWsunflowHBDynamicUPCIMIN}{29}
\newcommand{\SLOWsunflowHBDynamicUPCIMAX}{35}
\newcommand{\SLOWsunflowWCPUP}{17}
\newcommand{\SLOWsunflowWCPUPCI}{0}
\newcommand{\SLOWsunflowWCPUPCIMIN}{17}
\newcommand{\SLOWsunflowWCPUPCIMAX}{17}
\newcommand{\SLOWsunflowWCPDynamicUP}{154}
\newcommand{\SLOWsunflowWCPDynamicUPCI}{3.9}
\newcommand{\SLOWsunflowWCPDynamicUPCIMIN}{150}
\newcommand{\SLOWsunflowWCPDynamicUPCIMAX}{158}
\newcommand{\SLOWsunflowWDCnoGUP}{\rna}
\newcommand{\SLOWsunflowWDCnoGUPCI}{\rna}
\newcommand{\SLOWsunflowWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWsunflowWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWsunflowWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWsunflowWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWsunflowWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowWDCUP}{\rna}
\newcommand{\SLOWsunflowWDCUPCI}{\rna}
\newcommand{\SLOWsunflowWDCUPCIMIN}{\rna}
\newcommand{\SLOWsunflowWDCUPCIMAX}{\rna}
\newcommand{\SLOWsunflowWDCDynamicUP}{\rna}
\newcommand{\SLOWsunflowWDCDynamicUPCI}{\rna}
\newcommand{\SLOWsunflowWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGUP}{\rna}
\newcommand{\SLOWsunflowCAPOnoGUPCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOUP}{\rna}
\newcommand{\SLOWsunflowCAPOUPCI}{\rna}
\newcommand{\SLOWsunflowCAPOUPCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOUPCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPODynamicUP}{\rna}
\newcommand{\SLOWsunflowCAPODynamicUPCI}{\rna}
\newcommand{\SLOWsunflowCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPUP}{\rna}
\newcommand{\SLOWsunflowPIPUPCI}{\rna}
\newcommand{\SLOWsunflowPIPUPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPUPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPDynamicUP}{\rna}
\newcommand{\SLOWsunflowPIPDynamicUPCI}{\rna}
\newcommand{\SLOWsunflowPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPHB}{\rna}
\newcommand{\SLOWsunflowPIPHBCI}{\rna}
\newcommand{\SLOWsunflowPIPHBCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPHBCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPHBDynamic}{\rna}
\newcommand{\SLOWsunflowPIPHBDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPWCP}{\rna}
\newcommand{\SLOWsunflowPIPWCPCI}{\rna}
\newcommand{\SLOWsunflowPIPWCPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPWCPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPWCPDynamic}{\rna}
\newcommand{\SLOWsunflowPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPWDC}{\rna}
\newcommand{\SLOWsunflowPIPWDCCI}{\rna}
\newcommand{\SLOWsunflowPIPWDCCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPWDCCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPWDCDynamic}{\rna}
\newcommand{\SLOWsunflowPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPCAPO}{\rna}
\newcommand{\SLOWsunflowPIPCAPOCI}{\rna}
\newcommand{\SLOWsunflowPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPCAPODynamic}{\rna}
\newcommand{\SLOWsunflowPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPPIP}{\rna}
\newcommand{\SLOWsunflowPIPPIPCI}{\rna}
\newcommand{\SLOWsunflowPIPPIPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPPIPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPPIPDynamic}{\rna}
\newcommand{\SLOWsunflowPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatEvents}{47}
\newcommand{\SLOWtomcatNoFPEvents}{18}
\newcommand{\SLOWtomcatMaxLiveThreads}{33}
\newcommand{\SLOWtomcatTotalThreads}{35}
\newcommand{\SLOWtomcatBaseTime}{0.93}
\newcommand{\SLOWtomcatBaseTimeCI}{5.2}
\newcommand{\SLOWtomcatEmptyTime}{\rna}
\newcommand{\SLOWtomcatEmptyTimeCI}{\rna}
\newcommand{\SLOWtomcatEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatFTTime}{42}
\newcommand{\SLOWtomcatFTTimeCI}{2.0}
\newcommand{\SLOWtomcatHBTime}{11}
\newcommand{\SLOWtomcatHBTimeCI}{0.36}
\newcommand{\SLOWtomcatWCPTime}{15}
\newcommand{\SLOWtomcatWCPTimeCI}{0.59}
\newcommand{\SLOWtomcatDCnoGExcTime}{14}
\newcommand{\SLOWtomcatDCnoGExcTimeCI}{0.27}
\newcommand{\SLOWtomcatDCnoGTime}{\rna}
\newcommand{\SLOWtomcatDCnoGTimeCI}{\rna}
\newcommand{\SLOWtomcatDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatDCExcTime}{14}
\newcommand{\SLOWtomcatDCExcTimeCI}{0.75}
\newcommand{\SLOWtomcatDCTime}{\rna}
\newcommand{\SLOWtomcatDCTimeCI}{\rna}
\newcommand{\SLOWtomcatDCTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatDCTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGExcTime}{12}
\newcommand{\SLOWtomcatCAPOnoGExcTimeCI}{0.36}
\newcommand{\SLOWtomcatCAPOnoGTime}{\rna}
\newcommand{\SLOWtomcatCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOExcTime}{9.4}
\newcommand{\SLOWtomcatCAPOExcTimeCI}{0.28}
\newcommand{\SLOWtomcatCAPOTime}{\rna}
\newcommand{\SLOWtomcatCAPOTimeCI}{\rna}
\newcommand{\SLOWtomcatCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatStaticTime}{\rzero}
\newcommand{\SLOWtomcatDynamicTime}{\rzero}
\newcommand{\SLOWtomcatBaseMem}{510}
\newcommand{\SLOWtomcatBaseMemCI}{2.9}
\newcommand{\SLOWtomcatHBMem}{27}
\newcommand{\SLOWtomcatHBMemCI}{1.3}
\newcommand{\SLOWtomcatFTMem}{57}
\newcommand{\SLOWtomcatFTMemCI}{6.5}
\newcommand{\SLOWtomcatWCPMem}{35}
\newcommand{\SLOWtomcatWCPMemCI}{1.3}
\newcommand{\SLOWtomcatDCnoGExcMem}{27}
\newcommand{\SLOWtomcatDCnoGExcMemCI}{1.7}
\newcommand{\SLOWtomcatDCnoGMem}{\memna}
\newcommand{\SLOWtomcatDCnoGMemCI}{\memna}
\newcommand{\SLOWtomcatDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWtomcatDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWtomcatDCExcMem}{24}
\newcommand{\SLOWtomcatDCExcMemCI}{0.80}
\newcommand{\SLOWtomcatDCMem}{\memna}
\newcommand{\SLOWtomcatDCMemCI}{\memna}
\newcommand{\SLOWtomcatDCMemCIMIN}{\memna}
\newcommand{\SLOWtomcatDCMemCIMAX}{\memna}
\newcommand{\SLOWtomcatCAPOnoGExcMem}{27}
\newcommand{\SLOWtomcatCAPOnoGExcMemCI}{1.2}
\newcommand{\SLOWtomcatCAPOnoGMem}{\memna}
\newcommand{\SLOWtomcatCAPOnoGMemCI}{\memna}
\newcommand{\SLOWtomcatCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWtomcatCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWtomcatCAPOExcMem}{22}
\newcommand{\SLOWtomcatCAPOExcMemCI}{0.97}
\newcommand{\SLOWtomcatCAPOMem}{\memna}
\newcommand{\SLOWtomcatCAPOMemCI}{\memna}
\newcommand{\SLOWtomcatCAPOMemCIMIN}{\memna}
\newcommand{\SLOWtomcatCAPOMemCIMAX}{\memna}
\newcommand{\SLOWtomcatEventsCI}{131,702}
\newcommand{\SLOWtomcatEventsCIMIN}{46,958,604}
\newcommand{\SLOWtomcatEventsCIMAX}{47,222,008}
\newcommand{\SLOWtomcatNoFPEventsCI}{21,346}
\newcommand{\SLOWtomcatNoFPEventsCIMIN}{18,266,398}
\newcommand{\SLOWtomcatNoFPEventsCIMAX}{18,309,090}
\newcommand{\SLOWtomcatHB}{585}
\newcommand{\SLOWtomcatHBCI}{19}
\newcommand{\SLOWtomcatHBCIMIN}{566}
\newcommand{\SLOWtomcatHBCIMAX}{604}
\newcommand{\SLOWtomcatHBDynamic}{2,043,203}
\newcommand{\SLOWtomcatHBDynamicCI}{233,462}
\newcommand{\SLOWtomcatHBDynamicCIMIN}{1,809,741}
\newcommand{\SLOWtomcatHBDynamicCIMAX}{2,276,665}
\newcommand{\SLOWtomcatFT}{408}
\newcommand{\SLOWtomcatFTCI}{7.0}
\newcommand{\SLOWtomcatFTCIMIN}{401}
\newcommand{\SLOWtomcatFTCIMAX}{415}
\newcommand{\SLOWtomcatFTDynamic}{5,158,890}
\newcommand{\SLOWtomcatFTDynamicCI}{238,708}
\newcommand{\SLOWtomcatFTDynamicCIMIN}{4,920,182}
\newcommand{\SLOWtomcatFTDynamicCIMAX}{5,397,598}
\newcommand{\SLOWtomcatWCP}{578}
\newcommand{\SLOWtomcatWCPCI}{17}
\newcommand{\SLOWtomcatWCPCIMIN}{561}
\newcommand{\SLOWtomcatWCPCIMAX}{595}
\newcommand{\SLOWtomcatWCPDynamic}{1,555,862}
\newcommand{\SLOWtomcatWCPDynamicCI}{109,775}
\newcommand{\SLOWtomcatWCPDynamicCIMIN}{1,446,087}
\newcommand{\SLOWtomcatWCPDynamicCIMAX}{1,665,637}
\newcommand{\SLOWtomcatDCnoGExc}{585}
\newcommand{\SLOWtomcatDCnoGExcCI}{6}
\newcommand{\SLOWtomcatDCnoGExcCIMIN}{579}
\newcommand{\SLOWtomcatDCnoGExcCIMAX}{591}
\newcommand{\SLOWtomcatDCnoGExcDynamic}{1,533,538}
\newcommand{\SLOWtomcatDCnoGExcDynamicCI}{109,296}
\newcommand{\SLOWtomcatDCnoGExcDynamicCIMIN}{1,424,242}
\newcommand{\SLOWtomcatDCnoGExcDynamicCIMAX}{1,642,834}
\newcommand{\SLOWtomcatDCnoG}{\rna}
\newcommand{\SLOWtomcatDCnoGCI}{\rna}
\newcommand{\SLOWtomcatDCnoGCIMIN}{\rna}
\newcommand{\SLOWtomcatDCnoGCIMAX}{\rna}
\newcommand{\SLOWtomcatDCnoGDynamic}{\rna}
\newcommand{\SLOWtomcatDCnoGDynamicCI}{\rna}
\newcommand{\SLOWtomcatDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatDCExc}{65}
\newcommand{\SLOWtomcatDCExcCI}{1.3}
\newcommand{\SLOWtomcatDCExcCIMIN}{64}
\newcommand{\SLOWtomcatDCExcCIMAX}{66}
\newcommand{\SLOWtomcatDCExcDynamic}{11,991}
\newcommand{\SLOWtomcatDCExcDynamicCI}{577}
\newcommand{\SLOWtomcatDCExcDynamicCIMIN}{11,414}
\newcommand{\SLOWtomcatDCExcDynamicCIMAX}{12,568}
\newcommand{\SLOWtomcatDC}{\rna}
\newcommand{\SLOWtomcatDCCI}{\rna}
\newcommand{\SLOWtomcatDCCIMIN}{\rna}
\newcommand{\SLOWtomcatDCCIMAX}{\rna}
\newcommand{\SLOWtomcatDCDynamic}{\rna}
\newcommand{\SLOWtomcatDCDynamicCI}{\rna}
\newcommand{\SLOWtomcatDCDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatDCDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGExc}{598}
\newcommand{\SLOWtomcatCAPOnoGExcCI}{22}
\newcommand{\SLOWtomcatCAPOnoGExcCIMIN}{576}
\newcommand{\SLOWtomcatCAPOnoGExcCIMAX}{620}
\newcommand{\SLOWtomcatCAPOnoGExcDynamic}{1,949,913}
\newcommand{\SLOWtomcatCAPOnoGExcDynamicCI}{123,875}
\newcommand{\SLOWtomcatCAPOnoGExcDynamicCIMIN}{1,826,038}
\newcommand{\SLOWtomcatCAPOnoGExcDynamicCIMAX}{2,073,788}
\newcommand{\SLOWtomcatCAPOnoG}{\rna}
\newcommand{\SLOWtomcatCAPOnoGCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamic}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOExc}{65}
\newcommand{\SLOWtomcatCAPOExcCI}{2.7}
\newcommand{\SLOWtomcatCAPOExcCIMIN}{62}
\newcommand{\SLOWtomcatCAPOExcCIMAX}{68}
\newcommand{\SLOWtomcatCAPOExcDynamic}{13,225}
\newcommand{\SLOWtomcatCAPOExcDynamicCI}{228}
\newcommand{\SLOWtomcatCAPOExcDynamicCIMIN}{12,997}
\newcommand{\SLOWtomcatCAPOExcDynamicCIMAX}{13,453}
\newcommand{\SLOWtomcatCAPO}{\rna}
\newcommand{\SLOWtomcatCAPOCI}{\rna}
\newcommand{\SLOWtomcatCAPOCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPODynamic}{\rna}
\newcommand{\SLOWtomcatCAPODynamicCI}{\rna}
\newcommand{\SLOWtomcatCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIP}{\rna}
\newcommand{\SLOWtomcatPIPCI}{\rna}
\newcommand{\SLOWtomcatPIPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPDynamic}{\rna}
\newcommand{\SLOWtomcatPIPDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatHBUP}{777}
\newcommand{\SLOWtomcatHBUPCI}{22}
\newcommand{\SLOWtomcatHBUPCIMIN}{755}
\newcommand{\SLOWtomcatHBUPCIMAX}{799}
\newcommand{\SLOWtomcatHBDynamicUP}{2,042,424}
\newcommand{\SLOWtomcatHBDynamicUPCI}{233,060}
\newcommand{\SLOWtomcatHBDynamicUPCIMIN}{1,809,364}
\newcommand{\SLOWtomcatHBDynamicUPCIMAX}{2,275,484}
\newcommand{\SLOWtomcatWCPUP}{773}
\newcommand{\SLOWtomcatWCPUPCI}{21}
\newcommand{\SLOWtomcatWCPUPCIMIN}{752}
\newcommand{\SLOWtomcatWCPUPCIMAX}{794}
\newcommand{\SLOWtomcatWCPDynamicUP}{1,555,601}
\newcommand{\SLOWtomcatWCPDynamicUPCI}{109,761}
\newcommand{\SLOWtomcatWCPDynamicUPCIMIN}{1,445,840}
\newcommand{\SLOWtomcatWCPDynamicUPCIMAX}{1,665,362}
\newcommand{\SLOWtomcatWDCnoGUP}{\rna}
\newcommand{\SLOWtomcatWDCnoGUPCI}{\rna}
\newcommand{\SLOWtomcatWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWtomcatWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWtomcatWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWtomcatWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWtomcatWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatWDCUP}{\rna}
\newcommand{\SLOWtomcatWDCUPCI}{\rna}
\newcommand{\SLOWtomcatWDCUPCIMIN}{\rna}
\newcommand{\SLOWtomcatWDCUPCIMAX}{\rna}
\newcommand{\SLOWtomcatWDCDynamicUP}{\rna}
\newcommand{\SLOWtomcatWDCDynamicUPCI}{\rna}
\newcommand{\SLOWtomcatWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGUP}{\rna}
\newcommand{\SLOWtomcatCAPOnoGUPCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOUP}{\rna}
\newcommand{\SLOWtomcatCAPOUPCI}{\rna}
\newcommand{\SLOWtomcatCAPOUPCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOUPCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPODynamicUP}{\rna}
\newcommand{\SLOWtomcatCAPODynamicUPCI}{\rna}
\newcommand{\SLOWtomcatCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPUP}{\rna}
\newcommand{\SLOWtomcatPIPUPCI}{\rna}
\newcommand{\SLOWtomcatPIPUPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPUPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPDynamicUP}{\rna}
\newcommand{\SLOWtomcatPIPDynamicUPCI}{\rna}
\newcommand{\SLOWtomcatPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPHB}{\rna}
\newcommand{\SLOWtomcatPIPHBCI}{\rna}
\newcommand{\SLOWtomcatPIPHBCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPHBCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPHBDynamic}{\rna}
\newcommand{\SLOWtomcatPIPHBDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPWCP}{\rna}
\newcommand{\SLOWtomcatPIPWCPCI}{\rna}
\newcommand{\SLOWtomcatPIPWCPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPWCPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPWCPDynamic}{\rna}
\newcommand{\SLOWtomcatPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPWDC}{\rna}
\newcommand{\SLOWtomcatPIPWDCCI}{\rna}
\newcommand{\SLOWtomcatPIPWDCCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPWDCCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPWDCDynamic}{\rna}
\newcommand{\SLOWtomcatPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPCAPO}{\rna}
\newcommand{\SLOWtomcatPIPCAPOCI}{\rna}
\newcommand{\SLOWtomcatPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPCAPODynamic}{\rna}
\newcommand{\SLOWtomcatPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPPIP}{\rna}
\newcommand{\SLOWtomcatPIPPIPCI}{\rna}
\newcommand{\SLOWtomcatPIPPIPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPPIPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPPIPDynamic}{\rna}
\newcommand{\SLOWtomcatPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanEvents}{630}
\newcommand{\SLOWxalanNoFPEvents}{270}
\newcommand{\SLOWxalanMaxLiveThreads}{9}
\newcommand{\SLOWxalanTotalThreads}{9}
\newcommand{\SLOWxalanBaseTime}{2.0}
\newcommand{\SLOWxalanBaseTimeCI}{72}
\newcommand{\SLOWxalanEmptyTime}{\rna}
\newcommand{\SLOWxalanEmptyTimeCI}{\rna}
\newcommand{\SLOWxalanEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWxalanEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWxalanFTTime}{4.8}
\newcommand{\SLOWxalanFTTimeCI}{0.31}
\newcommand{\SLOWxalanHBTime}{16}
\newcommand{\SLOWxalanHBTimeCI}{2.5}
\newcommand{\SLOWxalanWCPTime}{48}
\newcommand{\SLOWxalanWCPTimeCI}{3.0}
\newcommand{\SLOWxalanDCnoGExcTime}{44}
\newcommand{\SLOWxalanDCnoGExcTimeCI}{2.8}
\newcommand{\SLOWxalanDCnoGTime}{\rna}
\newcommand{\SLOWxalanDCnoGTimeCI}{\rna}
\newcommand{\SLOWxalanDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWxalanDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWxalanDCExcTime}{58}
\newcommand{\SLOWxalanDCExcTimeCI}{2.0}
\newcommand{\SLOWxalanDCTime}{\rna}
\newcommand{\SLOWxalanDCTimeCI}{\rna}
\newcommand{\SLOWxalanDCTimeCIMIN}{\rna}
\newcommand{\SLOWxalanDCTimeCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGExcTime}{40}
\newcommand{\SLOWxalanCAPOnoGExcTimeCI}{2.3}
\newcommand{\SLOWxalanCAPOnoGTime}{\rna}
\newcommand{\SLOWxalanCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOExcTime}{51}
\newcommand{\SLOWxalanCAPOExcTimeCI}{2.8}
\newcommand{\SLOWxalanCAPOTime}{\rna}
\newcommand{\SLOWxalanCAPOTimeCI}{\rna}
\newcommand{\SLOWxalanCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWxalanStaticTime}{\rzero}
\newcommand{\SLOWxalanDynamicTime}{\rzero}
\newcommand{\SLOWxalanBaseMem}{670}
\newcommand{\SLOWxalanBaseMemCI}{7.4}
\newcommand{\SLOWxalanHBMem}{22}
\newcommand{\SLOWxalanHBMemCI}{0.85}
\newcommand{\SLOWxalanFTMem}{6.7}
\newcommand{\SLOWxalanFTMemCI}{0.088}
\newcommand{\SLOWxalanWCPMem}{57}
\newcommand{\SLOWxalanWCPMemCI}{2.2}
\newcommand{\SLOWxalanDCnoGExcMem}{48}
\newcommand{\SLOWxalanDCnoGExcMemCI}{2.0}
\newcommand{\SLOWxalanDCnoGMem}{\memna}
\newcommand{\SLOWxalanDCnoGMemCI}{\memna}
\newcommand{\SLOWxalanDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWxalanDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWxalanDCExcMem}{61}
\newcommand{\SLOWxalanDCExcMemCI}{0.84}
\newcommand{\SLOWxalanDCMem}{\memna}
\newcommand{\SLOWxalanDCMemCI}{\memna}
\newcommand{\SLOWxalanDCMemCIMIN}{\memna}
\newcommand{\SLOWxalanDCMemCIMAX}{\memna}
\newcommand{\SLOWxalanCAPOnoGExcMem}{48}
\newcommand{\SLOWxalanCAPOnoGExcMemCI}{0.93}
\newcommand{\SLOWxalanCAPOnoGMem}{\memna}
\newcommand{\SLOWxalanCAPOnoGMemCI}{\memna}
\newcommand{\SLOWxalanCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWxalanCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWxalanCAPOExcMem}{57}
\newcommand{\SLOWxalanCAPOExcMemCI}{1.5}
\newcommand{\SLOWxalanCAPOMem}{\memna}
\newcommand{\SLOWxalanCAPOMemCI}{\memna}
\newcommand{\SLOWxalanCAPOMemCIMIN}{\memna}
\newcommand{\SLOWxalanCAPOMemCIMAX}{\memna}
\newcommand{\SLOWxalanEventsCI}{18}
\newcommand{\SLOWxalanEventsCIMIN}{626,353,750}
\newcommand{\SLOWxalanEventsCIMAX}{626,353,786}
\newcommand{\SLOWxalanNoFPEventsCI}{15}
\newcommand{\SLOWxalanNoFPEventsCIMIN}{273,861,865}
\newcommand{\SLOWxalanNoFPEventsCIMAX}{273,861,895}
\newcommand{\SLOWxalanHB}{8}
\newcommand{\SLOWxalanHBCI}{0}
\newcommand{\SLOWxalanHBCIMIN}{8}
\newcommand{\SLOWxalanHBCIMAX}{8}
\newcommand{\SLOWxalanHBDynamic}{1,230}
\newcommand{\SLOWxalanHBDynamicCI}{23}
\newcommand{\SLOWxalanHBDynamicCIMIN}{1,207}
\newcommand{\SLOWxalanHBDynamicCIMAX}{1,253}
\newcommand{\SLOWxalanFT}{8}
\newcommand{\SLOWxalanFTCI}{0}
\newcommand{\SLOWxalanFTCIMIN}{8}
\newcommand{\SLOWxalanFTCIMAX}{8}
\newcommand{\SLOWxalanFTDynamic}{1,484}
\newcommand{\SLOWxalanFTDynamicCI}{0}
\newcommand{\SLOWxalanFTDynamicCIMIN}{1,484}
\newcommand{\SLOWxalanFTDynamicCIMAX}{1,484}
\newcommand{\SLOWxalanWCP}{63}
\newcommand{\SLOWxalanWCPCI}{0}
\newcommand{\SLOWxalanWCPCIMIN}{63}
\newcommand{\SLOWxalanWCPCIMAX}{63}
\newcommand{\SLOWxalanWCPDynamic}{4,746,687}
\newcommand{\SLOWxalanWCPDynamicCI}{35,989}
\newcommand{\SLOWxalanWCPDynamicCIMIN}{4,710,698}
\newcommand{\SLOWxalanWCPDynamicCIMAX}{4,782,676}
\newcommand{\SLOWxalanDCnoGExc}{74}
\newcommand{\SLOWxalanDCnoGExcCI}{0.2}
\newcommand{\SLOWxalanDCnoGExcCIMIN}{74}
\newcommand{\SLOWxalanDCnoGExcCIMAX}{74}
\newcommand{\SLOWxalanDCnoGExcDynamic}{6,711,435}
\newcommand{\SLOWxalanDCnoGExcDynamicCI}{6,996}
\newcommand{\SLOWxalanDCnoGExcDynamicCIMIN}{6,704,439}
\newcommand{\SLOWxalanDCnoGExcDynamicCIMAX}{6,718,431}
\newcommand{\SLOWxalanDCnoG}{\rna}
\newcommand{\SLOWxalanDCnoGCI}{\rna}
\newcommand{\SLOWxalanDCnoGCIMIN}{\rna}
\newcommand{\SLOWxalanDCnoGCIMAX}{\rna}
\newcommand{\SLOWxalanDCnoGDynamic}{\rna}
\newcommand{\SLOWxalanDCnoGDynamicCI}{\rna}
\newcommand{\SLOWxalanDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanDCExc}{8}
\newcommand{\SLOWxalanDCExcCI}{0.32}
\newcommand{\SLOWxalanDCExcCIMIN}{8}
\newcommand{\SLOWxalanDCExcCIMAX}{8}
\newcommand{\SLOWxalanDCExcDynamic}{262,419}
\newcommand{\SLOWxalanDCExcDynamicCI}{841}
\newcommand{\SLOWxalanDCExcDynamicCIMIN}{261,578}
\newcommand{\SLOWxalanDCExcDynamicCIMAX}{263,260}
\newcommand{\SLOWxalanDC}{\rna}
\newcommand{\SLOWxalanDCCI}{\rna}
\newcommand{\SLOWxalanDCCIMIN}{\rna}
\newcommand{\SLOWxalanDCCIMAX}{\rna}
\newcommand{\SLOWxalanDCDynamic}{\rna}
\newcommand{\SLOWxalanDCDynamicCI}{\rna}
\newcommand{\SLOWxalanDCDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanDCDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGExc}{74}
\newcommand{\SLOWxalanCAPOnoGExcCI}{0.6}
\newcommand{\SLOWxalanCAPOnoGExcCIMIN}{73}
\newcommand{\SLOWxalanCAPOnoGExcCIMAX}{75}
\newcommand{\SLOWxalanCAPOnoGExcDynamic}{6,701,028}
\newcommand{\SLOWxalanCAPOnoGExcDynamicCI}{8,132}
\newcommand{\SLOWxalanCAPOnoGExcDynamicCIMIN}{6,692,896}
\newcommand{\SLOWxalanCAPOnoGExcDynamicCIMAX}{6,709,160}
\newcommand{\SLOWxalanCAPOnoG}{\rna}
\newcommand{\SLOWxalanCAPOnoGCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamic}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOExc}{7}
\newcommand{\SLOWxalanCAPOExcCI}{0}
\newcommand{\SLOWxalanCAPOExcCIMIN}{7}
\newcommand{\SLOWxalanCAPOExcCIMAX}{7}
\newcommand{\SLOWxalanCAPOExcDynamic}{259,955}
\newcommand{\SLOWxalanCAPOExcDynamicCI}{736}
\newcommand{\SLOWxalanCAPOExcDynamicCIMIN}{259,219}
\newcommand{\SLOWxalanCAPOExcDynamicCIMAX}{260,691}
\newcommand{\SLOWxalanCAPO}{\rna}
\newcommand{\SLOWxalanCAPOCI}{\rna}
\newcommand{\SLOWxalanCAPOCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOCIMAX}{\rna}
\newcommand{\SLOWxalanCAPODynamic}{\rna}
\newcommand{\SLOWxalanCAPODynamicCI}{\rna}
\newcommand{\SLOWxalanCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWxalanCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIP}{\rna}
\newcommand{\SLOWxalanPIPCI}{\rna}
\newcommand{\SLOWxalanPIPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPDynamic}{\rna}
\newcommand{\SLOWxalanPIPDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanHBUP}{33}
\newcommand{\SLOWxalanHBUPCI}{0}
\newcommand{\SLOWxalanHBUPCIMIN}{33}
\newcommand{\SLOWxalanHBUPCIMAX}{33}
\newcommand{\SLOWxalanHBDynamicUP}{1,206}
\newcommand{\SLOWxalanHBDynamicUPCI}{20}
\newcommand{\SLOWxalanHBDynamicUPCIMIN}{1,186}
\newcommand{\SLOWxalanHBDynamicUPCIMAX}{1,226}
\newcommand{\SLOWxalanWCPUP}{158}
\newcommand{\SLOWxalanWCPUPCI}{0.54}
\newcommand{\SLOWxalanWCPUPCIMIN}{157}
\newcommand{\SLOWxalanWCPUPCIMAX}{159}
\newcommand{\SLOWxalanWCPDynamicUP}{4,748,509}
\newcommand{\SLOWxalanWCPDynamicUPCI}{36,128}
\newcommand{\SLOWxalanWCPDynamicUPCIMIN}{4,712,381}
\newcommand{\SLOWxalanWCPDynamicUPCIMAX}{4,784,637}
\newcommand{\SLOWxalanWDCnoGUP}{\rna}
\newcommand{\SLOWxalanWDCnoGUPCI}{\rna}
\newcommand{\SLOWxalanWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWxalanWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWxalanWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWxalanWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWxalanWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanWDCUP}{\rna}
\newcommand{\SLOWxalanWDCUPCI}{\rna}
\newcommand{\SLOWxalanWDCUPCIMIN}{\rna}
\newcommand{\SLOWxalanWDCUPCIMAX}{\rna}
\newcommand{\SLOWxalanWDCDynamicUP}{\rna}
\newcommand{\SLOWxalanWDCDynamicUPCI}{\rna}
\newcommand{\SLOWxalanWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGUP}{\rna}
\newcommand{\SLOWxalanCAPOnoGUPCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOUP}{\rna}
\newcommand{\SLOWxalanCAPOUPCI}{\rna}
\newcommand{\SLOWxalanCAPOUPCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOUPCIMAX}{\rna}
\newcommand{\SLOWxalanCAPODynamicUP}{\rna}
\newcommand{\SLOWxalanCAPODynamicUPCI}{\rna}
\newcommand{\SLOWxalanCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPUP}{\rna}
\newcommand{\SLOWxalanPIPUPCI}{\rna}
\newcommand{\SLOWxalanPIPUPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPUPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPDynamicUP}{\rna}
\newcommand{\SLOWxalanPIPDynamicUPCI}{\rna}
\newcommand{\SLOWxalanPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPHB}{\rna}
\newcommand{\SLOWxalanPIPHBCI}{\rna}
\newcommand{\SLOWxalanPIPHBCIMIN}{\rna}
\newcommand{\SLOWxalanPIPHBCIMAX}{\rna}
\newcommand{\SLOWxalanPIPHBDynamic}{\rna}
\newcommand{\SLOWxalanPIPHBDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIPWCP}{\rna}
\newcommand{\SLOWxalanPIPWCPCI}{\rna}
\newcommand{\SLOWxalanPIPWCPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPWCPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPWCPDynamic}{\rna}
\newcommand{\SLOWxalanPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIPWDC}{\rna}
\newcommand{\SLOWxalanPIPWDCCI}{\rna}
\newcommand{\SLOWxalanPIPWDCCIMIN}{\rna}
\newcommand{\SLOWxalanPIPWDCCIMAX}{\rna}
\newcommand{\SLOWxalanPIPWDCDynamic}{\rna}
\newcommand{\SLOWxalanPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIPCAPO}{\rna}
\newcommand{\SLOWxalanPIPCAPOCI}{\rna}
\newcommand{\SLOWxalanPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWxalanPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWxalanPIPCAPODynamic}{\rna}
\newcommand{\SLOWxalanPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWxalanPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIPPIP}{\rna}
\newcommand{\SLOWxalanPIPPIPCI}{\rna}
\newcommand{\SLOWxalanPIPPIPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPPIPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPPIPDynamic}{\rna}
\newcommand{\SLOWxalanPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWBaseTimeGeoMean}{1900}
\newcommand{\SLOWEmptyTimeGeoMean}{\rna}
\newcommand{\SLOWFTTimeGeoMean}{9.5}
\newcommand{\SLOWHBTimeGeoMean}{21}
\newcommand{\SLOWWCPTimeGeoMean}{34}
\newcommand{\SLOWDCnoGExcTimeGeoMean}{29}
\newcommand{\SLOWDCnoGTimeGeoMean}{\rna}
\newcommand{\SLOWDCExcTimeGeoMean}{32}
\newcommand{\SLOWDCTimeGeoMean}{\rna}
\newcommand{\SLOWCAPOnoGExcTimeGeoMean}{27}
\newcommand{\SLOWCAPOnoGTimeGeoMean}{\rna}
\newcommand{\SLOWCAPOExcTimeGeoMean}{30}
\newcommand{\SLOWCAPOTimeGeoMean}{\rna}
\newcommand{\SLOWBaseMemGeoMean}{500}
\newcommand{\SLOWEmptyMemGeoMean}{0}
\newcommand{\SLOWFTMemGeoMean}{7.8}
\newcommand{\SLOWHBMemGeoMean}{22}
\newcommand{\SLOWWCPMemGeoMean}{41}
\newcommand{\SLOWDCnoGExcMemGeoMean}{29}
\newcommand{\SLOWDCnoGMemGeoMean}{\memna}
\newcommand{\SLOWDCExcMemGeoMean}{34}
\newcommand{\SLOWDCMemGeoMean}{\memna}
\newcommand{\SLOWCAPOnoGExcMemGeoMean}{28}
\newcommand{\SLOWCAPOnoGMemGeoMean}{\memna}
\newcommand{\SLOWCAPOExcMemGeoMean}{33}
\newcommand{\SLOWCAPOMemGeoMean}{\memna}
\newcommand{\SLOWWCPDynamicTotal}{6,810,258}
\newcommand{\SLOWHBDynamicUPTotal}{2,553,141}
\newcommand{\SLOWPIPWDCDynamicTotal}{0}
\newcommand{\SLOWCAPOTotal}{0}
\newcommand{\SLOWPIPWCPTotal}{0}
\newcommand{\SLOWWCPTotal}{707}
\newcommand{\SLOWWDCnoGDynamicUPTotal}{0}
\newcommand{\SLOWCAPOnoGExcDynamicTotal}{9,178,271}
\newcommand{\SLOWCAPOExcTotal}{104}
\newcommand{\SLOWDCExcTotal}{104}
\newcommand{\SLOWDCnoGExcTotal}{739}
\newcommand{\SLOWPIPDynamicUPTotal}{0}
\newcommand{\SLOWPIPPIPTotal}{0}
\newcommand{\SLOWFTTotal}{476}
\newcommand{\SLOWHBDynamicTotal}{2,553,945}
\newcommand{\SLOWCAPOnoGDynamicUPTotal}{0}
\newcommand{\SLOWDCnoGExcDynamicTotal}{8,774,466}
\newcommand{\SLOWCAPOnoGTotal}{0}
\newcommand{\SLOWPIPWDCTotal}{0}
\newcommand{\SLOWCAPOnoGExcTotal}{752}
\newcommand{\SLOWPIPHBDynamicTotal}{0}
\newcommand{\SLOWWDCUPTotal}{0}
\newcommand{\SLOWDCnoGTotal}{0}
\newcommand{\SLOWWCPDynamicUPTotal}{6,811,820}
\newcommand{\SLOWPIPUPTotal}{0}
\newcommand{\SLOWCAPODynamicTotal}{0}
\newcommand{\SLOWCAPOnoGUPTotal}{0}
\newcommand{\SLOWPIPCAPOTotal}{0}
\newcommand{\SLOWCAPOnoGDynamicTotal}{0}
\newcommand{\SLOWFTDynamicTotal}{6,013,459}
\newcommand{\SLOWPIPCAPODynamicTotal}{0}
\newcommand{\SLOWDCnoGDynamicTotal}{0}
\newcommand{\SLOWWDCnoGUPTotal}{0}
\newcommand{\SLOWDCExcDynamicTotal}{470,513}
\newcommand{\SLOWWDCDynamicUPTotal}{0}
\newcommand{\SLOWHBUPTotal}{855}
\newcommand{\SLOWCAPOExcDynamicTotal}{532,175}
\newcommand{\SLOWPIPTotal}{0}
\newcommand{\SLOWWCPUPTotal}{989}
\newcommand{\SLOWCAPOUPTotal}{0}
\newcommand{\SLOWPIPHBTotal}{0}
\newcommand{\SLOWHBTotal}{646}
\newcommand{\SLOWDCDynamicTotal}{0}
\newcommand{\SLOWPIPDynamicTotal}{0}
\newcommand{\SLOWCAPODynamicUPTotal}{0}
\newcommand{\SLOWPIPPIPDynamicTotal}{0}
\newcommand{\SLOWPIPWCPDynamicTotal}{0}
\newcommand{\SLOWDCTotal}{0}



==> result-macros/PIP_slowTool_raceEdgeFix.tex <==
\newcommand{\SLOWavroraEvents}{1,400}
\newcommand{\SLOWavroraNoFPEvents}{160}
\newcommand{\SLOWavroraMaxLiveThreads}{7}
\newcommand{\SLOWavroraTotalThreads}{7}
\newcommand{\SLOWavroraBaseTime}{2.3}
\newcommand{\SLOWavroraBaseTimeCI}{10}
\newcommand{\SLOWavroraEmptyTime}{\rna}
\newcommand{\SLOWavroraEmptyTimeCI}{\rna}
\newcommand{\SLOWavroraEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWavroraEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWavroraFTTime}{\rna}
\newcommand{\SLOWavroraFTTimeCI}{\rna}
\newcommand{\SLOWavroraFTTimeCIMIN}{\rna}
\newcommand{\SLOWavroraFTTimeCIMAX}{\rna}
\newcommand{\SLOWavroraHBTime}{17}
\newcommand{\SLOWavroraHBTimeCI}{0.18}
\newcommand{\SLOWavroraWCPTime}{23}
\newcommand{\SLOWavroraWCPTimeCI}{0.56}
\newcommand{\SLOWavroraDCnoGExcTime}{21}
\newcommand{\SLOWavroraDCnoGExcTimeCI}{0.39}
\newcommand{\SLOWavroraDCnoGTime}{\rna}
\newcommand{\SLOWavroraDCnoGTimeCI}{\rna}
\newcommand{\SLOWavroraDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWavroraDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWavroraDCExcTime}{25}
\newcommand{\SLOWavroraDCExcTimeCI}{0.54}
\newcommand{\SLOWavroraDCTime}{\rna}
\newcommand{\SLOWavroraDCTimeCI}{\rna}
\newcommand{\SLOWavroraDCTimeCIMIN}{\rna}
\newcommand{\SLOWavroraDCTimeCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGExcTime}{18}
\newcommand{\SLOWavroraCAPOnoGExcTimeCI}{0.25}
\newcommand{\SLOWavroraCAPOnoGTime}{\rna}
\newcommand{\SLOWavroraCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOExcTime}{22}
\newcommand{\SLOWavroraCAPOExcTimeCI}{0.30}
\newcommand{\SLOWavroraCAPOTime}{\rna}
\newcommand{\SLOWavroraCAPOTimeCI}{\rna}
\newcommand{\SLOWavroraCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWavroraStaticTime}{\rzero}
\newcommand{\SLOWavroraDynamicTime}{\rzero}
\newcommand{\SLOWavroraBaseMem}{180}
\newcommand{\SLOWavroraBaseMemCI}{5.4}
\newcommand{\SLOWavroraHBMem}{28}
\newcommand{\SLOWavroraHBMemCI}{0.83}
\newcommand{\SLOWavroraFTMem}{\memna}
\newcommand{\SLOWavroraFTMemCI}{\memna}
\newcommand{\SLOWavroraFTMemCIMIN}{\memna}
\newcommand{\SLOWavroraFTMemCIMAX}{\memna}
\newcommand{\SLOWavroraWCPMem}{83}
\newcommand{\SLOWavroraWCPMemCI}{2.8}
\newcommand{\SLOWavroraDCnoGExcMem}{36}
\newcommand{\SLOWavroraDCnoGExcMemCI}{1.1}
\newcommand{\SLOWavroraDCnoGMem}{\memna}
\newcommand{\SLOWavroraDCnoGMemCI}{\memna}
\newcommand{\SLOWavroraDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWavroraDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWavroraDCExcMem}{61}
\newcommand{\SLOWavroraDCExcMemCI}{2.0}
\newcommand{\SLOWavroraDCMem}{\memna}
\newcommand{\SLOWavroraDCMemCI}{\memna}
\newcommand{\SLOWavroraDCMemCIMIN}{\memna}
\newcommand{\SLOWavroraDCMemCIMAX}{\memna}
\newcommand{\SLOWavroraCAPOnoGExcMem}{32}
\newcommand{\SLOWavroraCAPOnoGExcMemCI}{1.4}
\newcommand{\SLOWavroraCAPOnoGMem}{\memna}
\newcommand{\SLOWavroraCAPOnoGMemCI}{\memna}
\newcommand{\SLOWavroraCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWavroraCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWavroraCAPOExcMem}{61}
\newcommand{\SLOWavroraCAPOExcMemCI}{1.9}
\newcommand{\SLOWavroraCAPOMem}{\memna}
\newcommand{\SLOWavroraCAPOMemCI}{\memna}
\newcommand{\SLOWavroraCAPOMemCIMIN}{\memna}
\newcommand{\SLOWavroraCAPOMemCIMAX}{\memna}
\newcommand{\SLOWavroraEventsCI}{100,577}
\newcommand{\SLOWavroraEventsCIMIN}{1,438,646,762}
\newcommand{\SLOWavroraEventsCIMAX}{1,438,847,916}
\newcommand{\SLOWavroraNoFPEventsCI}{87,377}
\newcommand{\SLOWavroraNoFPEventsCIMIN}{156,476,384}
\newcommand{\SLOWavroraNoFPEventsCIMAX}{156,651,138}
\newcommand{\SLOWavroraHB}{6}
\newcommand{\SLOWavroraHBCI}{0}
\newcommand{\SLOWavroraHBCIMIN}{6}
\newcommand{\SLOWavroraHBCIMAX}{6}
\newcommand{\SLOWavroraHBDynamic}{129,204}
\newcommand{\SLOWavroraHBDynamicCI}{805}
\newcommand{\SLOWavroraHBDynamicCIMIN}{128,399}
\newcommand{\SLOWavroraHBDynamicCIMAX}{130,009}
\newcommand{\SLOWavroraFT}{\rna}
\newcommand{\SLOWavroraFTCI}{\rna}
\newcommand{\SLOWavroraFTCIMIN}{\rna}
\newcommand{\SLOWavroraFTCIMAX}{\rna}
\newcommand{\SLOWavroraFTDynamic}{\rna}
\newcommand{\SLOWavroraFTDynamicCI}{\rna}
\newcommand{\SLOWavroraFTDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraFTDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraWCP}{5}
\newcommand{\SLOWavroraWCPCI}{0}
\newcommand{\SLOWavroraWCPCIMIN}{5}
\newcommand{\SLOWavroraWCPCIMAX}{5}
\newcommand{\SLOWavroraWCPDynamic}{109,148}
\newcommand{\SLOWavroraWCPDynamicCI}{307}
\newcommand{\SLOWavroraWCPDynamicCIMIN}{108,841}
\newcommand{\SLOWavroraWCPDynamicCIMAX}{109,455}
\newcommand{\SLOWavroraDCnoGExc}{6}
\newcommand{\SLOWavroraDCnoGExcCI}{0}
\newcommand{\SLOWavroraDCnoGExcCIMIN}{6}
\newcommand{\SLOWavroraDCnoGExcCIMAX}{6}
\newcommand{\SLOWavroraDCnoGExcDynamic}{207,647}
\newcommand{\SLOWavroraDCnoGExcDynamicCI}{214}
\newcommand{\SLOWavroraDCnoGExcDynamicCIMIN}{207,433}
\newcommand{\SLOWavroraDCnoGExcDynamicCIMAX}{207,861}
\newcommand{\SLOWavroraDCnoG}{\rna}
\newcommand{\SLOWavroraDCnoGCI}{\rna}
\newcommand{\SLOWavroraDCnoGCIMIN}{\rna}
\newcommand{\SLOWavroraDCnoGCIMAX}{\rna}
\newcommand{\SLOWavroraDCnoGDynamic}{\rna}
\newcommand{\SLOWavroraDCnoGDynamicCI}{\rna}
\newcommand{\SLOWavroraDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraDCExc}{6}
\newcommand{\SLOWavroraDCExcCI}{0}
\newcommand{\SLOWavroraDCExcCIMIN}{6}
\newcommand{\SLOWavroraDCExcCIMAX}{6}
\newcommand{\SLOWavroraDCExcDynamic}{149,875}
\newcommand{\SLOWavroraDCExcDynamicCI}{2,229}
\newcommand{\SLOWavroraDCExcDynamicCIMIN}{147,646}
\newcommand{\SLOWavroraDCExcDynamicCIMAX}{152,104}
\newcommand{\SLOWavroraDC}{\rna}
\newcommand{\SLOWavroraDCCI}{\rna}
\newcommand{\SLOWavroraDCCIMIN}{\rna}
\newcommand{\SLOWavroraDCCIMAX}{\rna}
\newcommand{\SLOWavroraDCDynamic}{\rna}
\newcommand{\SLOWavroraDCDynamicCI}{\rna}
\newcommand{\SLOWavroraDCDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraDCDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGExc}{6}
\newcommand{\SLOWavroraCAPOnoGExcCI}{0}
\newcommand{\SLOWavroraCAPOnoGExcCIMIN}{6}
\newcommand{\SLOWavroraCAPOnoGExcCIMAX}{6}
\newcommand{\SLOWavroraCAPOnoGExcDynamic}{236,067}
\newcommand{\SLOWavroraCAPOnoGExcDynamicCI}{1,645}
\newcommand{\SLOWavroraCAPOnoGExcDynamicCIMIN}{234,422}
\newcommand{\SLOWavroraCAPOnoGExcDynamicCIMAX}{237,712}
\newcommand{\SLOWavroraCAPOnoG}{\rna}
\newcommand{\SLOWavroraCAPOnoGCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamic}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOExc}{6}
\newcommand{\SLOWavroraCAPOExcCI}{0}
\newcommand{\SLOWavroraCAPOExcCIMIN}{6}
\newcommand{\SLOWavroraCAPOExcCIMAX}{6}
\newcommand{\SLOWavroraCAPOExcDynamic}{216,435}
\newcommand{\SLOWavroraCAPOExcDynamicCI}{3,317}
\newcommand{\SLOWavroraCAPOExcDynamicCIMIN}{213,118}
\newcommand{\SLOWavroraCAPOExcDynamicCIMAX}{219,752}
\newcommand{\SLOWavroraCAPO}{\rna}
\newcommand{\SLOWavroraCAPOCI}{\rna}
\newcommand{\SLOWavroraCAPOCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOCIMAX}{\rna}
\newcommand{\SLOWavroraCAPODynamic}{\rna}
\newcommand{\SLOWavroraCAPODynamicCI}{\rna}
\newcommand{\SLOWavroraCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWavroraCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIP}{\rna}
\newcommand{\SLOWavroraPIPCI}{\rna}
\newcommand{\SLOWavroraPIPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPDynamic}{\rna}
\newcommand{\SLOWavroraPIPDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraHBUP}{3}
\newcommand{\SLOWavroraHBUPCI}{0}
\newcommand{\SLOWavroraHBUPCIMIN}{3}
\newcommand{\SLOWavroraHBUPCIMAX}{3}
\newcommand{\SLOWavroraHBDynamicUP}{129,204}
\newcommand{\SLOWavroraHBDynamicUPCI}{805}
\newcommand{\SLOWavroraHBDynamicUPCIMIN}{128,399}
\newcommand{\SLOWavroraHBDynamicUPCIMAX}{130,009}
\newcommand{\SLOWavroraWCPUP}{4}
\newcommand{\SLOWavroraWCPUPCI}{0}
\newcommand{\SLOWavroraWCPUPCIMIN}{4}
\newcommand{\SLOWavroraWCPUPCIMAX}{4}
\newcommand{\SLOWavroraWCPDynamicUP}{109,148}
\newcommand{\SLOWavroraWCPDynamicUPCI}{307}
\newcommand{\SLOWavroraWCPDynamicUPCIMIN}{108,841}
\newcommand{\SLOWavroraWCPDynamicUPCIMAX}{109,455}
\newcommand{\SLOWavroraWDCnoGUP}{\rna}
\newcommand{\SLOWavroraWDCnoGUPCI}{\rna}
\newcommand{\SLOWavroraWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWavroraWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWavroraWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWavroraWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWavroraWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraWDCUP}{\rna}
\newcommand{\SLOWavroraWDCUPCI}{\rna}
\newcommand{\SLOWavroraWDCUPCIMIN}{\rna}
\newcommand{\SLOWavroraWDCUPCIMAX}{\rna}
\newcommand{\SLOWavroraWDCDynamicUP}{\rna}
\newcommand{\SLOWavroraWDCDynamicUPCI}{\rna}
\newcommand{\SLOWavroraWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGUP}{\rna}
\newcommand{\SLOWavroraCAPOnoGUPCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOUP}{\rna}
\newcommand{\SLOWavroraCAPOUPCI}{\rna}
\newcommand{\SLOWavroraCAPOUPCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOUPCIMAX}{\rna}
\newcommand{\SLOWavroraCAPODynamicUP}{\rna}
\newcommand{\SLOWavroraCAPODynamicUPCI}{\rna}
\newcommand{\SLOWavroraCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPUP}{\rna}
\newcommand{\SLOWavroraPIPUPCI}{\rna}
\newcommand{\SLOWavroraPIPUPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPUPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPDynamicUP}{\rna}
\newcommand{\SLOWavroraPIPDynamicUPCI}{\rna}
\newcommand{\SLOWavroraPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPHB}{\rna}
\newcommand{\SLOWavroraPIPHBCI}{\rna}
\newcommand{\SLOWavroraPIPHBCIMIN}{\rna}
\newcommand{\SLOWavroraPIPHBCIMAX}{\rna}
\newcommand{\SLOWavroraPIPHBDynamic}{\rna}
\newcommand{\SLOWavroraPIPHBDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIPWCP}{\rna}
\newcommand{\SLOWavroraPIPWCPCI}{\rna}
\newcommand{\SLOWavroraPIPWCPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPWCPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPWCPDynamic}{\rna}
\newcommand{\SLOWavroraPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIPWDC}{\rna}
\newcommand{\SLOWavroraPIPWDCCI}{\rna}
\newcommand{\SLOWavroraPIPWDCCIMIN}{\rna}
\newcommand{\SLOWavroraPIPWDCCIMAX}{\rna}
\newcommand{\SLOWavroraPIPWDCDynamic}{\rna}
\newcommand{\SLOWavroraPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIPCAPO}{\rna}
\newcommand{\SLOWavroraPIPCAPOCI}{\rna}
\newcommand{\SLOWavroraPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWavroraPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWavroraPIPCAPODynamic}{\rna}
\newcommand{\SLOWavroraPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWavroraPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIPPIP}{\rna}
\newcommand{\SLOWavroraPIPPIPCI}{\rna}
\newcommand{\SLOWavroraPIPPIPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPPIPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPPIPDynamic}{\rna}
\newcommand{\SLOWavroraPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikEvents}{160}
\newcommand{\SLOWbatikNoFPEvents}{11}
\newcommand{\SLOWbatikMaxLiveThreads}{7}
\newcommand{\SLOWbatikTotalThreads}{7}
\newcommand{\SLOWbatikBaseTime}{2.5}
\newcommand{\SLOWbatikBaseTimeCI}{33}
\newcommand{\SLOWbatikEmptyTime}{\rna}
\newcommand{\SLOWbatikEmptyTimeCI}{\rna}
\newcommand{\SLOWbatikEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWbatikEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWbatikFTTime}{\rna}
\newcommand{\SLOWbatikFTTimeCI}{\rna}
\newcommand{\SLOWbatikFTTimeCIMIN}{\rna}
\newcommand{\SLOWbatikFTTimeCIMAX}{\rna}
\newcommand{\SLOWbatikHBTime}{8.0}
\newcommand{\SLOWbatikHBTimeCI}{0.086}
\newcommand{\SLOWbatikWCPTime}{12}
\newcommand{\SLOWbatikWCPTimeCI}{0.11}
\newcommand{\SLOWbatikDCnoGExcTime}{10}
\newcommand{\SLOWbatikDCnoGExcTimeCI}{0.10}
\newcommand{\SLOWbatikDCnoGTime}{\rna}
\newcommand{\SLOWbatikDCnoGTimeCI}{\rna}
\newcommand{\SLOWbatikDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWbatikDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWbatikDCExcTime}{11}
\newcommand{\SLOWbatikDCExcTimeCI}{0.14}
\newcommand{\SLOWbatikDCTime}{\rna}
\newcommand{\SLOWbatikDCTimeCI}{\rna}
\newcommand{\SLOWbatikDCTimeCIMIN}{\rna}
\newcommand{\SLOWbatikDCTimeCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGExcTime}{9.8}
\newcommand{\SLOWbatikCAPOnoGExcTimeCI}{0.099}
\newcommand{\SLOWbatikCAPOnoGTime}{\rna}
\newcommand{\SLOWbatikCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOExcTime}{11}
\newcommand{\SLOWbatikCAPOExcTimeCI}{0.096}
\newcommand{\SLOWbatikCAPOTime}{\rna}
\newcommand{\SLOWbatikCAPOTimeCI}{\rna}
\newcommand{\SLOWbatikCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWbatikStaticTime}{\rzero}
\newcommand{\SLOWbatikDynamicTime}{\rzero}
\newcommand{\SLOWbatikBaseMem}{240}
\newcommand{\SLOWbatikBaseMemCI}{0.64}
\newcommand{\SLOWbatikHBMem}{28}
\newcommand{\SLOWbatikHBMemCI}{0.081}
\newcommand{\SLOWbatikFTMem}{\memna}
\newcommand{\SLOWbatikFTMemCI}{\memna}
\newcommand{\SLOWbatikFTMemCIMIN}{\memna}
\newcommand{\SLOWbatikFTMemCIMAX}{\memna}
\newcommand{\SLOWbatikWCPMem}{45}
\newcommand{\SLOWbatikWCPMemCI}{0.25}
\newcommand{\SLOWbatikDCnoGExcMem}{36}
\newcommand{\SLOWbatikDCnoGExcMemCI}{1.6}
\newcommand{\SLOWbatikDCnoGMem}{\memna}
\newcommand{\SLOWbatikDCnoGMemCI}{\memna}
\newcommand{\SLOWbatikDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWbatikDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWbatikDCExcMem}{41}
\newcommand{\SLOWbatikDCExcMemCI}{0.15}
\newcommand{\SLOWbatikDCMem}{\memna}
\newcommand{\SLOWbatikDCMemCI}{\memna}
\newcommand{\SLOWbatikDCMemCIMIN}{\memna}
\newcommand{\SLOWbatikDCMemCIMAX}{\memna}
\newcommand{\SLOWbatikCAPOnoGExcMem}{35}
\newcommand{\SLOWbatikCAPOnoGExcMemCI}{0.18}
\newcommand{\SLOWbatikCAPOnoGMem}{\memna}
\newcommand{\SLOWbatikCAPOnoGMemCI}{\memna}
\newcommand{\SLOWbatikCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWbatikCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWbatikCAPOExcMem}{41}
\newcommand{\SLOWbatikCAPOExcMemCI}{1.8}
\newcommand{\SLOWbatikCAPOMem}{\memna}
\newcommand{\SLOWbatikCAPOMemCI}{\memna}
\newcommand{\SLOWbatikCAPOMemCIMIN}{\memna}
\newcommand{\SLOWbatikCAPOMemCIMAX}{\memna}
\newcommand{\SLOWbatikEventsCI}{0}
\newcommand{\SLOWbatikEventsCIMIN}{155,322,726}
\newcommand{\SLOWbatikEventsCIMAX}{155,322,726}
\newcommand{\SLOWbatikNoFPEventsCI}{0}
\newcommand{\SLOWbatikNoFPEventsCIMIN}{11,422,601}
\newcommand{\SLOWbatikNoFPEventsCIMAX}{11,422,601}
\newcommand{\SLOWbatikHB}{0}
\newcommand{\SLOWbatikHBCI}{0}
\newcommand{\SLOWbatikHBCIMIN}{0}
\newcommand{\SLOWbatikHBCIMAX}{0}
\newcommand{\SLOWbatikHBDynamic}{0}
\newcommand{\SLOWbatikHBDynamicCI}{0}
\newcommand{\SLOWbatikHBDynamicCIMIN}{0}
\newcommand{\SLOWbatikHBDynamicCIMAX}{0}
\newcommand{\SLOWbatikFT}{\rna}
\newcommand{\SLOWbatikFTCI}{\rna}
\newcommand{\SLOWbatikFTCIMIN}{\rna}
\newcommand{\SLOWbatikFTCIMAX}{\rna}
\newcommand{\SLOWbatikFTDynamic}{\rna}
\newcommand{\SLOWbatikFTDynamicCI}{\rna}
\newcommand{\SLOWbatikFTDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikFTDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikWCP}{0}
\newcommand{\SLOWbatikWCPCI}{0}
\newcommand{\SLOWbatikWCPCIMIN}{0}
\newcommand{\SLOWbatikWCPCIMAX}{0}
\newcommand{\SLOWbatikWCPDynamic}{0}
\newcommand{\SLOWbatikWCPDynamicCI}{0}
\newcommand{\SLOWbatikWCPDynamicCIMIN}{0}
\newcommand{\SLOWbatikWCPDynamicCIMAX}{0}
\newcommand{\SLOWbatikDCnoGExc}{0}
\newcommand{\SLOWbatikDCnoGExcCI}{0}
\newcommand{\SLOWbatikDCnoGExcCIMIN}{0}
\newcommand{\SLOWbatikDCnoGExcCIMAX}{0}
\newcommand{\SLOWbatikDCnoGExcDynamic}{0}
\newcommand{\SLOWbatikDCnoGExcDynamicCI}{0}
\newcommand{\SLOWbatikDCnoGExcDynamicCIMIN}{0}
\newcommand{\SLOWbatikDCnoGExcDynamicCIMAX}{0}
\newcommand{\SLOWbatikDCnoG}{\rna}
\newcommand{\SLOWbatikDCnoGCI}{\rna}
\newcommand{\SLOWbatikDCnoGCIMIN}{\rna}
\newcommand{\SLOWbatikDCnoGCIMAX}{\rna}
\newcommand{\SLOWbatikDCnoGDynamic}{\rna}
\newcommand{\SLOWbatikDCnoGDynamicCI}{\rna}
\newcommand{\SLOWbatikDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikDCExc}{0}
\newcommand{\SLOWbatikDCExcCI}{0}
\newcommand{\SLOWbatikDCExcCIMIN}{0}
\newcommand{\SLOWbatikDCExcCIMAX}{0}
\newcommand{\SLOWbatikDCExcDynamic}{0}
\newcommand{\SLOWbatikDCExcDynamicCI}{0}
\newcommand{\SLOWbatikDCExcDynamicCIMIN}{0}
\newcommand{\SLOWbatikDCExcDynamicCIMAX}{0}
\newcommand{\SLOWbatikDC}{\rna}
\newcommand{\SLOWbatikDCCI}{\rna}
\newcommand{\SLOWbatikDCCIMIN}{\rna}
\newcommand{\SLOWbatikDCCIMAX}{\rna}
\newcommand{\SLOWbatikDCDynamic}{\rna}
\newcommand{\SLOWbatikDCDynamicCI}{\rna}
\newcommand{\SLOWbatikDCDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikDCDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGExc}{0}
\newcommand{\SLOWbatikCAPOnoGExcCI}{0}
\newcommand{\SLOWbatikCAPOnoGExcCIMIN}{0}
\newcommand{\SLOWbatikCAPOnoGExcCIMAX}{0}
\newcommand{\SLOWbatikCAPOnoGExcDynamic}{0}
\newcommand{\SLOWbatikCAPOnoGExcDynamicCI}{0}
\newcommand{\SLOWbatikCAPOnoGExcDynamicCIMIN}{0}
\newcommand{\SLOWbatikCAPOnoGExcDynamicCIMAX}{0}
\newcommand{\SLOWbatikCAPOnoG}{\rna}
\newcommand{\SLOWbatikCAPOnoGCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamic}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOExc}{0}
\newcommand{\SLOWbatikCAPOExcCI}{0}
\newcommand{\SLOWbatikCAPOExcCIMIN}{0}
\newcommand{\SLOWbatikCAPOExcCIMAX}{0}
\newcommand{\SLOWbatikCAPOExcDynamic}{0}
\newcommand{\SLOWbatikCAPOExcDynamicCI}{0}
\newcommand{\SLOWbatikCAPOExcDynamicCIMIN}{0}
\newcommand{\SLOWbatikCAPOExcDynamicCIMAX}{0}
\newcommand{\SLOWbatikCAPO}{\rna}
\newcommand{\SLOWbatikCAPOCI}{\rna}
\newcommand{\SLOWbatikCAPOCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOCIMAX}{\rna}
\newcommand{\SLOWbatikCAPODynamic}{\rna}
\newcommand{\SLOWbatikCAPODynamicCI}{\rna}
\newcommand{\SLOWbatikCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWbatikCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIP}{\rna}
\newcommand{\SLOWbatikPIPCI}{\rna}
\newcommand{\SLOWbatikPIPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPDynamic}{\rna}
\newcommand{\SLOWbatikPIPDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikHBUP}{0}
\newcommand{\SLOWbatikHBUPCI}{0}
\newcommand{\SLOWbatikHBUPCIMIN}{0}
\newcommand{\SLOWbatikHBUPCIMAX}{0}
\newcommand{\SLOWbatikHBDynamicUP}{0}
\newcommand{\SLOWbatikHBDynamicUPCI}{0}
\newcommand{\SLOWbatikHBDynamicUPCIMIN}{0}
\newcommand{\SLOWbatikHBDynamicUPCIMAX}{0}
\newcommand{\SLOWbatikWCPUP}{0}
\newcommand{\SLOWbatikWCPUPCI}{0}
\newcommand{\SLOWbatikWCPUPCIMIN}{0}
\newcommand{\SLOWbatikWCPUPCIMAX}{0}
\newcommand{\SLOWbatikWCPDynamicUP}{0}
\newcommand{\SLOWbatikWCPDynamicUPCI}{0}
\newcommand{\SLOWbatikWCPDynamicUPCIMIN}{0}
\newcommand{\SLOWbatikWCPDynamicUPCIMAX}{0}
\newcommand{\SLOWbatikWDCnoGUP}{\rna}
\newcommand{\SLOWbatikWDCnoGUPCI}{\rna}
\newcommand{\SLOWbatikWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWbatikWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWbatikWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWbatikWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWbatikWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikWDCUP}{\rna}
\newcommand{\SLOWbatikWDCUPCI}{\rna}
\newcommand{\SLOWbatikWDCUPCIMIN}{\rna}
\newcommand{\SLOWbatikWDCUPCIMAX}{\rna}
\newcommand{\SLOWbatikWDCDynamicUP}{\rna}
\newcommand{\SLOWbatikWDCDynamicUPCI}{\rna}
\newcommand{\SLOWbatikWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGUP}{\rna}
\newcommand{\SLOWbatikCAPOnoGUPCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOUP}{\rna}
\newcommand{\SLOWbatikCAPOUPCI}{\rna}
\newcommand{\SLOWbatikCAPOUPCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOUPCIMAX}{\rna}
\newcommand{\SLOWbatikCAPODynamicUP}{\rna}
\newcommand{\SLOWbatikCAPODynamicUPCI}{\rna}
\newcommand{\SLOWbatikCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPUP}{\rna}
\newcommand{\SLOWbatikPIPUPCI}{\rna}
\newcommand{\SLOWbatikPIPUPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPUPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPDynamicUP}{\rna}
\newcommand{\SLOWbatikPIPDynamicUPCI}{\rna}
\newcommand{\SLOWbatikPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPHB}{\rna}
\newcommand{\SLOWbatikPIPHBCI}{\rna}
\newcommand{\SLOWbatikPIPHBCIMIN}{\rna}
\newcommand{\SLOWbatikPIPHBCIMAX}{\rna}
\newcommand{\SLOWbatikPIPHBDynamic}{\rna}
\newcommand{\SLOWbatikPIPHBDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIPWCP}{\rna}
\newcommand{\SLOWbatikPIPWCPCI}{\rna}
\newcommand{\SLOWbatikPIPWCPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPWCPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPWCPDynamic}{\rna}
\newcommand{\SLOWbatikPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIPWDC}{\rna}
\newcommand{\SLOWbatikPIPWDCCI}{\rna}
\newcommand{\SLOWbatikPIPWDCCIMIN}{\rna}
\newcommand{\SLOWbatikPIPWDCCIMAX}{\rna}
\newcommand{\SLOWbatikPIPWDCDynamic}{\rna}
\newcommand{\SLOWbatikPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIPCAPO}{\rna}
\newcommand{\SLOWbatikPIPCAPOCI}{\rna}
\newcommand{\SLOWbatikPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWbatikPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWbatikPIPCAPODynamic}{\rna}
\newcommand{\SLOWbatikPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWbatikPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIPPIP}{\rna}
\newcommand{\SLOWbatikPIPPIPCI}{\rna}
\newcommand{\SLOWbatikPIPPIPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPPIPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPPIPDynamic}{\rna}
\newcommand{\SLOWbatikPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoEvents}{3,800}
\newcommand{\SLOWhtwoNoFPEvents}{460}
\newcommand{\SLOWhtwoMaxLiveThreads}{9}
\newcommand{\SLOWhtwoTotalThreads}{10}
\newcommand{\SLOWhtwoBaseTime}{4.7}
\newcommand{\SLOWhtwoBaseTimeCI}{68}
\newcommand{\SLOWhtwoEmptyTime}{\rna}
\newcommand{\SLOWhtwoEmptyTimeCI}{\rna}
\newcommand{\SLOWhtwoEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoFTTime}{\rna}
\newcommand{\SLOWhtwoFTTimeCI}{\rna}
\newcommand{\SLOWhtwoFTTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoFTTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoHBTime}{27}
\newcommand{\SLOWhtwoHBTimeCI}{0.59}
\newcommand{\SLOWhtwoWCPTime}{77}
\newcommand{\SLOWhtwoWCPTimeCI}{4.9}
\newcommand{\SLOWhtwoDCnoGExcTime}{74}
\newcommand{\SLOWhtwoDCnoGExcTimeCI}{6.3}
\newcommand{\SLOWhtwoDCnoGTime}{\rna}
\newcommand{\SLOWhtwoDCnoGTimeCI}{\rna}
\newcommand{\SLOWhtwoDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoDCExcTime}{74}
\newcommand{\SLOWhtwoDCExcTimeCI}{3.8}
\newcommand{\SLOWhtwoDCTime}{\rna}
\newcommand{\SLOWhtwoDCTimeCI}{\rna}
\newcommand{\SLOWhtwoDCTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoDCTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGExcTime}{69}
\newcommand{\SLOWhtwoCAPOnoGExcTimeCI}{3.5}
\newcommand{\SLOWhtwoCAPOnoGTime}{\rna}
\newcommand{\SLOWhtwoCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOExcTime}{78}
\newcommand{\SLOWhtwoCAPOExcTimeCI}{4.6}
\newcommand{\SLOWhtwoCAPOTime}{\rna}
\newcommand{\SLOWhtwoCAPOTimeCI}{\rna}
\newcommand{\SLOWhtwoCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoStaticTime}{\rzero}
\newcommand{\SLOWhtwoDynamicTime}{\rzero}
\newcommand{\SLOWhtwoBaseMem}{1,800}
\newcommand{\SLOWhtwoBaseMemCI}{53.0}
\newcommand{\SLOWhtwoHBMem}{17}
\newcommand{\SLOWhtwoHBMemCI}{0.88}
\newcommand{\SLOWhtwoFTMem}{\memna}
\newcommand{\SLOWhtwoFTMemCI}{\memna}
\newcommand{\SLOWhtwoFTMemCIMIN}{\memna}
\newcommand{\SLOWhtwoFTMemCIMAX}{\memna}
\newcommand{\SLOWhtwoWCPMem}{61}
\newcommand{\SLOWhtwoWCPMemCI}{3.4}
\newcommand{\SLOWhtwoDCnoGExcMem}{54}
\newcommand{\SLOWhtwoDCnoGExcMemCI}{2.6}
\newcommand{\SLOWhtwoDCnoGMem}{\memna}
\newcommand{\SLOWhtwoDCnoGMemCI}{\memna}
\newcommand{\SLOWhtwoDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWhtwoDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWhtwoDCExcMem}{55}
\newcommand{\SLOWhtwoDCExcMemCI}{2.2}
\newcommand{\SLOWhtwoDCMem}{\memna}
\newcommand{\SLOWhtwoDCMemCI}{\memna}
\newcommand{\SLOWhtwoDCMemCIMIN}{\memna}
\newcommand{\SLOWhtwoDCMemCIMAX}{\memna}
\newcommand{\SLOWhtwoCAPOnoGExcMem}{54}
\newcommand{\SLOWhtwoCAPOnoGExcMemCI}{3.1}
\newcommand{\SLOWhtwoCAPOnoGMem}{\memna}
\newcommand{\SLOWhtwoCAPOnoGMemCI}{\memna}
\newcommand{\SLOWhtwoCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWhtwoCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWhtwoCAPOExcMem}{55}
\newcommand{\SLOWhtwoCAPOExcMemCI}{3.6}
\newcommand{\SLOWhtwoCAPOMem}{\memna}
\newcommand{\SLOWhtwoCAPOMemCI}{\memna}
\newcommand{\SLOWhtwoCAPOMemCIMIN}{\memna}
\newcommand{\SLOWhtwoCAPOMemCIMAX}{\memna}
\newcommand{\SLOWhtwoEventsCI}{1,191,230}
\newcommand{\SLOWhtwoEventsCIMIN}{3,801,486,163}
\newcommand{\SLOWhtwoEventsCIMAX}{3,803,868,623}
\newcommand{\SLOWhtwoNoFPEventsCI}{36,284}
\newcommand{\SLOWhtwoNoFPEventsCIMIN}{457,126,637}
\newcommand{\SLOWhtwoNoFPEventsCIMAX}{457,199,205}
\newcommand{\SLOWhtwoHB}{13}
\newcommand{\SLOWhtwoHBCI}{0}
\newcommand{\SLOWhtwoHBCIMIN}{13}
\newcommand{\SLOWhtwoHBCIMAX}{13}
\newcommand{\SLOWhtwoHBDynamic}{40,609}
\newcommand{\SLOWhtwoHBDynamicCI}{120}
\newcommand{\SLOWhtwoHBDynamicCIMIN}{40,489}
\newcommand{\SLOWhtwoHBDynamicCIMAX}{40,729}
\newcommand{\SLOWhtwoFT}{\rna}
\newcommand{\SLOWhtwoFTCI}{\rna}
\newcommand{\SLOWhtwoFTCIMIN}{\rna}
\newcommand{\SLOWhtwoFTCIMAX}{\rna}
\newcommand{\SLOWhtwoFTDynamic}{\rna}
\newcommand{\SLOWhtwoFTDynamicCI}{\rna}
\newcommand{\SLOWhtwoFTDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoFTDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoWCP}{12}
\newcommand{\SLOWhtwoWCPCI}{0}
\newcommand{\SLOWhtwoWCPCIMIN}{12}
\newcommand{\SLOWhtwoWCPCIMAX}{12}
\newcommand{\SLOWhtwoWCPDynamic}{41,053}
\newcommand{\SLOWhtwoWCPDynamicCI}{128}
\newcommand{\SLOWhtwoWCPDynamicCIMIN}{40,925}
\newcommand{\SLOWhtwoWCPDynamicCIMAX}{41,181}
\newcommand{\SLOWhtwoDCnoGExc}{13}
\newcommand{\SLOWhtwoDCnoGExcCI}{0}
\newcommand{\SLOWhtwoDCnoGExcCIMIN}{13}
\newcommand{\SLOWhtwoDCnoGExcCIMAX}{13}
\newcommand{\SLOWhtwoDCnoGExcDynamic}{41,382}
\newcommand{\SLOWhtwoDCnoGExcDynamicCI}{150}
\newcommand{\SLOWhtwoDCnoGExcDynamicCIMIN}{41,232}
\newcommand{\SLOWhtwoDCnoGExcDynamicCIMAX}{41,532}
\newcommand{\SLOWhtwoDCnoG}{\rna}
\newcommand{\SLOWhtwoDCnoGCI}{\rna}
\newcommand{\SLOWhtwoDCnoGCIMIN}{\rna}
\newcommand{\SLOWhtwoDCnoGCIMAX}{\rna}
\newcommand{\SLOWhtwoDCnoGDynamic}{\rna}
\newcommand{\SLOWhtwoDCnoGDynamicCI}{\rna}
\newcommand{\SLOWhtwoDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoDCExc}{13}
\newcommand{\SLOWhtwoDCExcCI}{0}
\newcommand{\SLOWhtwoDCExcCIMIN}{13}
\newcommand{\SLOWhtwoDCExcCIMAX}{13}
\newcommand{\SLOWhtwoDCExcDynamic}{41,391}
\newcommand{\SLOWhtwoDCExcDynamicCI}{71}
\newcommand{\SLOWhtwoDCExcDynamicCIMIN}{41,320}
\newcommand{\SLOWhtwoDCExcDynamicCIMAX}{41,462}
\newcommand{\SLOWhtwoDC}{\rna}
\newcommand{\SLOWhtwoDCCI}{\rna}
\newcommand{\SLOWhtwoDCCIMIN}{\rna}
\newcommand{\SLOWhtwoDCCIMAX}{\rna}
\newcommand{\SLOWhtwoDCDynamic}{\rna}
\newcommand{\SLOWhtwoDCDynamicCI}{\rna}
\newcommand{\SLOWhtwoDCDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoDCDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGExc}{13}
\newcommand{\SLOWhtwoCAPOnoGExcCI}{0}
\newcommand{\SLOWhtwoCAPOnoGExcCIMIN}{13}
\newcommand{\SLOWhtwoCAPOnoGExcCIMAX}{13}
\newcommand{\SLOWhtwoCAPOnoGExcDynamic}{41,443}
\newcommand{\SLOWhtwoCAPOnoGExcDynamicCI}{88}
\newcommand{\SLOWhtwoCAPOnoGExcDynamicCIMIN}{41,355}
\newcommand{\SLOWhtwoCAPOnoGExcDynamicCIMAX}{41,531}
\newcommand{\SLOWhtwoCAPOnoG}{\rna}
\newcommand{\SLOWhtwoCAPOnoGCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamic}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOExc}{13}
\newcommand{\SLOWhtwoCAPOExcCI}{0}
\newcommand{\SLOWhtwoCAPOExcCIMIN}{13}
\newcommand{\SLOWhtwoCAPOExcCIMAX}{13}
\newcommand{\SLOWhtwoCAPOExcDynamic}{41,429}
\newcommand{\SLOWhtwoCAPOExcDynamicCI}{86}
\newcommand{\SLOWhtwoCAPOExcDynamicCIMIN}{41,343}
\newcommand{\SLOWhtwoCAPOExcDynamicCIMAX}{41,515}
\newcommand{\SLOWhtwoCAPO}{\rna}
\newcommand{\SLOWhtwoCAPOCI}{\rna}
\newcommand{\SLOWhtwoCAPOCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPODynamic}{\rna}
\newcommand{\SLOWhtwoCAPODynamicCI}{\rna}
\newcommand{\SLOWhtwoCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIP}{\rna}
\newcommand{\SLOWhtwoPIPCI}{\rna}
\newcommand{\SLOWhtwoPIPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPDynamic}{\rna}
\newcommand{\SLOWhtwoPIPDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoHBUP}{8}
\newcommand{\SLOWhtwoHBUPCI}{0}
\newcommand{\SLOWhtwoHBUPCIMIN}{8}
\newcommand{\SLOWhtwoHBUPCIMAX}{8}
\newcommand{\SLOWhtwoHBDynamicUP}{40,609}
\newcommand{\SLOWhtwoHBDynamicUPCI}{120}
\newcommand{\SLOWhtwoHBDynamicUPCIMIN}{40,489}
\newcommand{\SLOWhtwoHBDynamicUPCIMAX}{40,729}
\newcommand{\SLOWhtwoWCPUP}{8}
\newcommand{\SLOWhtwoWCPUPCI}{0}
\newcommand{\SLOWhtwoWCPUPCIMIN}{8}
\newcommand{\SLOWhtwoWCPUPCIMAX}{8}
\newcommand{\SLOWhtwoWCPDynamicUP}{41,053}
\newcommand{\SLOWhtwoWCPDynamicUPCI}{128}
\newcommand{\SLOWhtwoWCPDynamicUPCIMIN}{40,925}
\newcommand{\SLOWhtwoWCPDynamicUPCIMAX}{41,181}
\newcommand{\SLOWhtwoWDCnoGUP}{\rna}
\newcommand{\SLOWhtwoWDCnoGUPCI}{\rna}
\newcommand{\SLOWhtwoWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWhtwoWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWhtwoWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWhtwoWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWhtwoWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoWDCUP}{\rna}
\newcommand{\SLOWhtwoWDCUPCI}{\rna}
\newcommand{\SLOWhtwoWDCUPCIMIN}{\rna}
\newcommand{\SLOWhtwoWDCUPCIMAX}{\rna}
\newcommand{\SLOWhtwoWDCDynamicUP}{\rna}
\newcommand{\SLOWhtwoWDCDynamicUPCI}{\rna}
\newcommand{\SLOWhtwoWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGUP}{\rna}
\newcommand{\SLOWhtwoCAPOnoGUPCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOUP}{\rna}
\newcommand{\SLOWhtwoCAPOUPCI}{\rna}
\newcommand{\SLOWhtwoCAPOUPCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOUPCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPODynamicUP}{\rna}
\newcommand{\SLOWhtwoCAPODynamicUPCI}{\rna}
\newcommand{\SLOWhtwoCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPUP}{\rna}
\newcommand{\SLOWhtwoPIPUPCI}{\rna}
\newcommand{\SLOWhtwoPIPUPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPUPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPDynamicUP}{\rna}
\newcommand{\SLOWhtwoPIPDynamicUPCI}{\rna}
\newcommand{\SLOWhtwoPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPHB}{\rna}
\newcommand{\SLOWhtwoPIPHBCI}{\rna}
\newcommand{\SLOWhtwoPIPHBCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPHBCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPHBDynamic}{\rna}
\newcommand{\SLOWhtwoPIPHBDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPWCP}{\rna}
\newcommand{\SLOWhtwoPIPWCPCI}{\rna}
\newcommand{\SLOWhtwoPIPWCPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPWCPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPWCPDynamic}{\rna}
\newcommand{\SLOWhtwoPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPWDC}{\rna}
\newcommand{\SLOWhtwoPIPWDCCI}{\rna}
\newcommand{\SLOWhtwoPIPWDCCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPWDCCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPWDCDynamic}{\rna}
\newcommand{\SLOWhtwoPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPCAPO}{\rna}
\newcommand{\SLOWhtwoPIPCAPOCI}{\rna}
\newcommand{\SLOWhtwoPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPCAPODynamic}{\rna}
\newcommand{\SLOWhtwoPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPPIP}{\rna}
\newcommand{\SLOWhtwoPIPPIPCI}{\rna}
\newcommand{\SLOWhtwoPIPPIPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPPIPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPPIPDynamic}{\rna}
\newcommand{\SLOWhtwoPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonEvents}{730}
\newcommand{\SLOWjythonNoFPEvents}{290}
\newcommand{\SLOWjythonMaxLiveThreads}{2}
\newcommand{\SLOWjythonTotalThreads}{2}
\newcommand{\SLOWjythonBaseTime}{3.8}
\newcommand{\SLOWjythonBaseTimeCI}{110}
\newcommand{\SLOWjythonEmptyTime}{\rna}
\newcommand{\SLOWjythonEmptyTimeCI}{\rna}
\newcommand{\SLOWjythonEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWjythonEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWjythonFTTime}{\rna}
\newcommand{\SLOWjythonFTTimeCI}{\rna}
\newcommand{\SLOWjythonFTTimeCIMIN}{\rna}
\newcommand{\SLOWjythonFTTimeCIMAX}{\rna}
\newcommand{\SLOWjythonHBTime}{23}
\newcommand{\SLOWjythonHBTimeCI}{0.58}
\newcommand{\SLOWjythonWCPTime}{33}
\newcommand{\SLOWjythonWCPTimeCI}{3.0}
\newcommand{\SLOWjythonDCnoGExcTime}{26}
\newcommand{\SLOWjythonDCnoGExcTimeCI}{0.89}
\newcommand{\SLOWjythonDCnoGTime}{\rna}
\newcommand{\SLOWjythonDCnoGTimeCI}{\rna}
\newcommand{\SLOWjythonDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWjythonDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWjythonDCExcTime}{31}
\newcommand{\SLOWjythonDCExcTimeCI}{0.84}
\newcommand{\SLOWjythonDCTime}{\rna}
\newcommand{\SLOWjythonDCTimeCI}{\rna}
\newcommand{\SLOWjythonDCTimeCIMIN}{\rna}
\newcommand{\SLOWjythonDCTimeCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGExcTime}{24}
\newcommand{\SLOWjythonCAPOnoGExcTimeCI}{0.59}
\newcommand{\SLOWjythonCAPOnoGTime}{\rna}
\newcommand{\SLOWjythonCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOExcTime}{28}
\newcommand{\SLOWjythonCAPOExcTimeCI}{0.76}
\newcommand{\SLOWjythonCAPOTime}{\rna}
\newcommand{\SLOWjythonCAPOTimeCI}{\rna}
\newcommand{\SLOWjythonCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWjythonStaticTime}{\rzero}
\newcommand{\SLOWjythonDynamicTime}{\rzero}
\newcommand{\SLOWjythonBaseMem}{760}
\newcommand{\SLOWjythonBaseMemCI}{6.7}
\newcommand{\SLOWjythonHBMem}{22}
\newcommand{\SLOWjythonHBMemCI}{0.55}
\newcommand{\SLOWjythonFTMem}{\memna}
\newcommand{\SLOWjythonFTMemCI}{\memna}
\newcommand{\SLOWjythonFTMemCIMIN}{\memna}
\newcommand{\SLOWjythonFTMemCIMAX}{\memna}
\newcommand{\SLOWjythonWCPMem}{21}
\newcommand{\SLOWjythonWCPMemCI}{0.74}
\newcommand{\SLOWjythonDCnoGExcMem}{18}
\newcommand{\SLOWjythonDCnoGExcMemCI}{0.37}
\newcommand{\SLOWjythonDCnoGMem}{\memna}
\newcommand{\SLOWjythonDCnoGMemCI}{\memna}
\newcommand{\SLOWjythonDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWjythonDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWjythonDCExcMem}{30}
\newcommand{\SLOWjythonDCExcMemCI}{0.51}
\newcommand{\SLOWjythonDCMem}{\memna}
\newcommand{\SLOWjythonDCMemCI}{\memna}
\newcommand{\SLOWjythonDCMemCIMIN}{\memna}
\newcommand{\SLOWjythonDCMemCIMAX}{\memna}
\newcommand{\SLOWjythonCAPOnoGExcMem}{17}
\newcommand{\SLOWjythonCAPOnoGExcMemCI}{0.51}
\newcommand{\SLOWjythonCAPOnoGMem}{\memna}
\newcommand{\SLOWjythonCAPOnoGMemCI}{\memna}
\newcommand{\SLOWjythonCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWjythonCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWjythonCAPOExcMem}{25}
\newcommand{\SLOWjythonCAPOExcMemCI}{0.37}
\newcommand{\SLOWjythonCAPOMem}{\memna}
\newcommand{\SLOWjythonCAPOMemCI}{\memna}
\newcommand{\SLOWjythonCAPOMemCIMIN}{\memna}
\newcommand{\SLOWjythonCAPOMemCIMAX}{\memna}
\newcommand{\SLOWjythonEventsCI}{368}
\newcommand{\SLOWjythonEventsCIMIN}{728,376,235}
\newcommand{\SLOWjythonEventsCIMAX}{728,376,971}
\newcommand{\SLOWjythonNoFPEventsCI}{13}
\newcommand{\SLOWjythonNoFPEventsCIMIN}{293,897,752}
\newcommand{\SLOWjythonNoFPEventsCIMAX}{293,897,778}
\newcommand{\SLOWjythonHB}{3}
\newcommand{\SLOWjythonHBCI}{0}
\newcommand{\SLOWjythonHBCIMIN}{3}
\newcommand{\SLOWjythonHBCIMAX}{3}
\newcommand{\SLOWjythonHBDynamic}{3}
\newcommand{\SLOWjythonHBDynamicCI}{0}
\newcommand{\SLOWjythonHBDynamicCIMIN}{3}
\newcommand{\SLOWjythonHBDynamicCIMAX}{3}
\newcommand{\SLOWjythonFT}{\rna}
\newcommand{\SLOWjythonFTCI}{\rna}
\newcommand{\SLOWjythonFTCIMIN}{\rna}
\newcommand{\SLOWjythonFTCIMAX}{\rna}
\newcommand{\SLOWjythonFTDynamic}{\rna}
\newcommand{\SLOWjythonFTDynamicCI}{\rna}
\newcommand{\SLOWjythonFTDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonFTDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonWCP}{3}
\newcommand{\SLOWjythonWCPCI}{0}
\newcommand{\SLOWjythonWCPCIMIN}{3}
\newcommand{\SLOWjythonWCPCIMAX}{3}
\newcommand{\SLOWjythonWCPDynamic}{4}
\newcommand{\SLOWjythonWCPDynamicCI}{0}
\newcommand{\SLOWjythonWCPDynamicCIMIN}{4}
\newcommand{\SLOWjythonWCPDynamicCIMAX}{4}
\newcommand{\SLOWjythonDCnoGExc}{4}
\newcommand{\SLOWjythonDCnoGExcCI}{1}
\newcommand{\SLOWjythonDCnoGExcCIMIN}{3}
\newcommand{\SLOWjythonDCnoGExcCIMAX}{5}
\newcommand{\SLOWjythonDCnoGExcDynamic}{5}
\newcommand{\SLOWjythonDCnoGExcDynamicCI}{1}
\newcommand{\SLOWjythonDCnoGExcDynamicCIMIN}{4}
\newcommand{\SLOWjythonDCnoGExcDynamicCIMAX}{6}
\newcommand{\SLOWjythonDCnoG}{\rna}
\newcommand{\SLOWjythonDCnoGCI}{\rna}
\newcommand{\SLOWjythonDCnoGCIMIN}{\rna}
\newcommand{\SLOWjythonDCnoGCIMAX}{\rna}
\newcommand{\SLOWjythonDCnoGDynamic}{\rna}
\newcommand{\SLOWjythonDCnoGDynamicCI}{\rna}
\newcommand{\SLOWjythonDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonDCExc}{2}
\newcommand{\SLOWjythonDCExcCI}{0}
\newcommand{\SLOWjythonDCExcCIMIN}{2}
\newcommand{\SLOWjythonDCExcCIMAX}{2}
\newcommand{\SLOWjythonDCExcDynamic}{4}
\newcommand{\SLOWjythonDCExcDynamicCI}{1}
\newcommand{\SLOWjythonDCExcDynamicCIMIN}{3}
\newcommand{\SLOWjythonDCExcDynamicCIMAX}{5}
\newcommand{\SLOWjythonDC}{\rna}
\newcommand{\SLOWjythonDCCI}{\rna}
\newcommand{\SLOWjythonDCCIMIN}{\rna}
\newcommand{\SLOWjythonDCCIMAX}{\rna}
\newcommand{\SLOWjythonDCDynamic}{\rna}
\newcommand{\SLOWjythonDCDynamicCI}{\rna}
\newcommand{\SLOWjythonDCDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonDCDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGExc}{3}
\newcommand{\SLOWjythonCAPOnoGExcCI}{1}
\newcommand{\SLOWjythonCAPOnoGExcCIMIN}{2}
\newcommand{\SLOWjythonCAPOnoGExcCIMAX}{4}
\newcommand{\SLOWjythonCAPOnoGExcDynamic}{5}
\newcommand{\SLOWjythonCAPOnoGExcDynamicCI}{1}
\newcommand{\SLOWjythonCAPOnoGExcDynamicCIMIN}{4}
\newcommand{\SLOWjythonCAPOnoGExcDynamicCIMAX}{6}
\newcommand{\SLOWjythonCAPOnoG}{\rna}
\newcommand{\SLOWjythonCAPOnoGCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamic}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOExc}{2}
\newcommand{\SLOWjythonCAPOExcCI}{0}
\newcommand{\SLOWjythonCAPOExcCIMIN}{2}
\newcommand{\SLOWjythonCAPOExcCIMAX}{2}
\newcommand{\SLOWjythonCAPOExcDynamic}{4}
\newcommand{\SLOWjythonCAPOExcDynamicCI}{1}
\newcommand{\SLOWjythonCAPOExcDynamicCIMIN}{3}
\newcommand{\SLOWjythonCAPOExcDynamicCIMAX}{5}
\newcommand{\SLOWjythonCAPO}{\rna}
\newcommand{\SLOWjythonCAPOCI}{\rna}
\newcommand{\SLOWjythonCAPOCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOCIMAX}{\rna}
\newcommand{\SLOWjythonCAPODynamic}{\rna}
\newcommand{\SLOWjythonCAPODynamicCI}{\rna}
\newcommand{\SLOWjythonCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWjythonCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIP}{\rna}
\newcommand{\SLOWjythonPIPCI}{\rna}
\newcommand{\SLOWjythonPIPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPDynamic}{\rna}
\newcommand{\SLOWjythonPIPDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonHBUP}{3}
\newcommand{\SLOWjythonHBUPCI}{0}
\newcommand{\SLOWjythonHBUPCIMIN}{3}
\newcommand{\SLOWjythonHBUPCIMAX}{3}
\newcommand{\SLOWjythonHBDynamicUP}{3}
\newcommand{\SLOWjythonHBDynamicUPCI}{0}
\newcommand{\SLOWjythonHBDynamicUPCIMIN}{3}
\newcommand{\SLOWjythonHBDynamicUPCIMAX}{3}
\newcommand{\SLOWjythonWCPUP}{3}
\newcommand{\SLOWjythonWCPUPCI}{0}
\newcommand{\SLOWjythonWCPUPCIMIN}{3}
\newcommand{\SLOWjythonWCPUPCIMAX}{3}
\newcommand{\SLOWjythonWCPDynamicUP}{4}
\newcommand{\SLOWjythonWCPDynamicUPCI}{0}
\newcommand{\SLOWjythonWCPDynamicUPCIMIN}{4}
\newcommand{\SLOWjythonWCPDynamicUPCIMAX}{4}
\newcommand{\SLOWjythonWDCnoGUP}{\rna}
\newcommand{\SLOWjythonWDCnoGUPCI}{\rna}
\newcommand{\SLOWjythonWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWjythonWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWjythonWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWjythonWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWjythonWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonWDCUP}{\rna}
\newcommand{\SLOWjythonWDCUPCI}{\rna}
\newcommand{\SLOWjythonWDCUPCIMIN}{\rna}
\newcommand{\SLOWjythonWDCUPCIMAX}{\rna}
\newcommand{\SLOWjythonWDCDynamicUP}{\rna}
\newcommand{\SLOWjythonWDCDynamicUPCI}{\rna}
\newcommand{\SLOWjythonWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGUP}{\rna}
\newcommand{\SLOWjythonCAPOnoGUPCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOUP}{\rna}
\newcommand{\SLOWjythonCAPOUPCI}{\rna}
\newcommand{\SLOWjythonCAPOUPCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOUPCIMAX}{\rna}
\newcommand{\SLOWjythonCAPODynamicUP}{\rna}
\newcommand{\SLOWjythonCAPODynamicUPCI}{\rna}
\newcommand{\SLOWjythonCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPUP}{\rna}
\newcommand{\SLOWjythonPIPUPCI}{\rna}
\newcommand{\SLOWjythonPIPUPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPUPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPDynamicUP}{\rna}
\newcommand{\SLOWjythonPIPDynamicUPCI}{\rna}
\newcommand{\SLOWjythonPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPHB}{\rna}
\newcommand{\SLOWjythonPIPHBCI}{\rna}
\newcommand{\SLOWjythonPIPHBCIMIN}{\rna}
\newcommand{\SLOWjythonPIPHBCIMAX}{\rna}
\newcommand{\SLOWjythonPIPHBDynamic}{\rna}
\newcommand{\SLOWjythonPIPHBDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIPWCP}{\rna}
\newcommand{\SLOWjythonPIPWCPCI}{\rna}
\newcommand{\SLOWjythonPIPWCPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPWCPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPWCPDynamic}{\rna}
\newcommand{\SLOWjythonPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIPWDC}{\rna}
\newcommand{\SLOWjythonPIPWDCCI}{\rna}
\newcommand{\SLOWjythonPIPWDCCIMIN}{\rna}
\newcommand{\SLOWjythonPIPWDCCIMAX}{\rna}
\newcommand{\SLOWjythonPIPWDCDynamic}{\rna}
\newcommand{\SLOWjythonPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIPCAPO}{\rna}
\newcommand{\SLOWjythonPIPCAPOCI}{\rna}
\newcommand{\SLOWjythonPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWjythonPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWjythonPIPCAPODynamic}{\rna}
\newcommand{\SLOWjythonPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWjythonPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIPPIP}{\rna}
\newcommand{\SLOWjythonPIPPIPCI}{\rna}
\newcommand{\SLOWjythonPIPPIPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPPIPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPPIPDynamic}{\rna}
\newcommand{\SLOWjythonPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexEvents}{400}
\newcommand{\SLOWluindexNoFPEvents}{45}
\newcommand{\SLOWluindexMaxLiveThreads}{3}
\newcommand{\SLOWluindexTotalThreads}{3}
\newcommand{\SLOWluindexBaseTime}{1.2}
\newcommand{\SLOWluindexBaseTimeCI}{59}
\newcommand{\SLOWluindexEmptyTime}{\rna}
\newcommand{\SLOWluindexEmptyTimeCI}{\rna}
\newcommand{\SLOWluindexEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWluindexEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWluindexFTTime}{\rna}
\newcommand{\SLOWluindexFTTimeCI}{\rna}
\newcommand{\SLOWluindexFTTimeCIMIN}{\rna}
\newcommand{\SLOWluindexFTTimeCIMAX}{\rna}
\newcommand{\SLOWluindexHBTime}{27}
\newcommand{\SLOWluindexHBTimeCI}{1.1}
\newcommand{\SLOWluindexWCPTime}{43}
\newcommand{\SLOWluindexWCPTimeCI}{1.7}
\newcommand{\SLOWluindexDCnoGExcTime}{36}
\newcommand{\SLOWluindexDCnoGExcTimeCI}{1.6}
\newcommand{\SLOWluindexDCnoGTime}{\rna}
\newcommand{\SLOWluindexDCnoGTimeCI}{\rna}
\newcommand{\SLOWluindexDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWluindexDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWluindexDCExcTime}{40}
\newcommand{\SLOWluindexDCExcTimeCI}{1.7}
\newcommand{\SLOWluindexDCTime}{\rna}
\newcommand{\SLOWluindexDCTimeCI}{\rna}
\newcommand{\SLOWluindexDCTimeCIMIN}{\rna}
\newcommand{\SLOWluindexDCTimeCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGExcTime}{36}
\newcommand{\SLOWluindexCAPOnoGExcTimeCI}{1.6}
\newcommand{\SLOWluindexCAPOnoGTime}{\rna}
\newcommand{\SLOWluindexCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOExcTime}{39}
\newcommand{\SLOWluindexCAPOExcTimeCI}{1.6}
\newcommand{\SLOWluindexCAPOTime}{\rna}
\newcommand{\SLOWluindexCAPOTimeCI}{\rna}
\newcommand{\SLOWluindexCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWluindexStaticTime}{\rzero}
\newcommand{\SLOWluindexDynamicTime}{\rzero}
\newcommand{\SLOWluindexBaseMem}{150}
\newcommand{\SLOWluindexBaseMemCI}{1.1}
\newcommand{\SLOWluindexHBMem}{29}
\newcommand{\SLOWluindexHBMemCI}{0.22}
\newcommand{\SLOWluindexFTMem}{\memna}
\newcommand{\SLOWluindexFTMemCI}{\memna}
\newcommand{\SLOWluindexFTMemCIMIN}{\memna}
\newcommand{\SLOWluindexFTMemCIMAX}{\memna}
\newcommand{\SLOWluindexWCPMem}{60}
\newcommand{\SLOWluindexWCPMemCI}{0.56}
\newcommand{\SLOWluindexDCnoGExcMem}{42}
\newcommand{\SLOWluindexDCnoGExcMemCI}{0.35}
\newcommand{\SLOWluindexDCnoGMem}{\memna}
\newcommand{\SLOWluindexDCnoGMemCI}{\memna}
\newcommand{\SLOWluindexDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWluindexDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWluindexDCExcMem}{50}
\newcommand{\SLOWluindexDCExcMemCI}{2.4}
\newcommand{\SLOWluindexDCMem}{\memna}
\newcommand{\SLOWluindexDCMemCI}{\memna}
\newcommand{\SLOWluindexDCMemCIMIN}{\memna}
\newcommand{\SLOWluindexDCMemCIMAX}{\memna}
\newcommand{\SLOWluindexCAPOnoGExcMem}{42}
\newcommand{\SLOWluindexCAPOnoGExcMemCI}{0.33}
\newcommand{\SLOWluindexCAPOnoGMem}{\memna}
\newcommand{\SLOWluindexCAPOnoGMemCI}{\memna}
\newcommand{\SLOWluindexCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWluindexCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWluindexCAPOExcMem}{47}
\newcommand{\SLOWluindexCAPOExcMemCI}{0.35}
\newcommand{\SLOWluindexCAPOMem}{\memna}
\newcommand{\SLOWluindexCAPOMemCI}{\memna}
\newcommand{\SLOWluindexCAPOMemCIMIN}{\memna}
\newcommand{\SLOWluindexCAPOMemCIMAX}{\memna}
\newcommand{\SLOWluindexEventsCI}{3}
\newcommand{\SLOWluindexEventsCIMIN}{396,268,394}
\newcommand{\SLOWluindexEventsCIMAX}{396,268,400}
\newcommand{\SLOWluindexNoFPEventsCI}{3}
\newcommand{\SLOWluindexNoFPEventsCIMIN}{45,411,630}
\newcommand{\SLOWluindexNoFPEventsCIMAX}{45,411,636}
\newcommand{\SLOWluindexHB}{1}
\newcommand{\SLOWluindexHBCI}{0}
\newcommand{\SLOWluindexHBCIMIN}{1}
\newcommand{\SLOWluindexHBCIMAX}{1}
\newcommand{\SLOWluindexHBDynamic}{1}
\newcommand{\SLOWluindexHBDynamicCI}{0}
\newcommand{\SLOWluindexHBDynamicCIMIN}{1}
\newcommand{\SLOWluindexHBDynamicCIMAX}{1}
\newcommand{\SLOWluindexFT}{\rna}
\newcommand{\SLOWluindexFTCI}{\rna}
\newcommand{\SLOWluindexFTCIMIN}{\rna}
\newcommand{\SLOWluindexFTCIMAX}{\rna}
\newcommand{\SLOWluindexFTDynamic}{\rna}
\newcommand{\SLOWluindexFTDynamicCI}{\rna}
\newcommand{\SLOWluindexFTDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexFTDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexWCP}{1}
\newcommand{\SLOWluindexWCPCI}{0}
\newcommand{\SLOWluindexWCPCIMIN}{1}
\newcommand{\SLOWluindexWCPCIMAX}{1}
\newcommand{\SLOWluindexWCPDynamic}{1}
\newcommand{\SLOWluindexWCPDynamicCI}{0}
\newcommand{\SLOWluindexWCPDynamicCIMIN}{1}
\newcommand{\SLOWluindexWCPDynamicCIMAX}{1}
\newcommand{\SLOWluindexDCnoGExc}{1}
\newcommand{\SLOWluindexDCnoGExcCI}{0}
\newcommand{\SLOWluindexDCnoGExcCIMIN}{1}
\newcommand{\SLOWluindexDCnoGExcCIMAX}{1}
\newcommand{\SLOWluindexDCnoGExcDynamic}{1}
\newcommand{\SLOWluindexDCnoGExcDynamicCI}{0}
\newcommand{\SLOWluindexDCnoGExcDynamicCIMIN}{1}
\newcommand{\SLOWluindexDCnoGExcDynamicCIMAX}{1}
\newcommand{\SLOWluindexDCnoG}{\rna}
\newcommand{\SLOWluindexDCnoGCI}{\rna}
\newcommand{\SLOWluindexDCnoGCIMIN}{\rna}
\newcommand{\SLOWluindexDCnoGCIMAX}{\rna}
\newcommand{\SLOWluindexDCnoGDynamic}{\rna}
\newcommand{\SLOWluindexDCnoGDynamicCI}{\rna}
\newcommand{\SLOWluindexDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexDCExc}{1}
\newcommand{\SLOWluindexDCExcCI}{0}
\newcommand{\SLOWluindexDCExcCIMIN}{1}
\newcommand{\SLOWluindexDCExcCIMAX}{1}
\newcommand{\SLOWluindexDCExcDynamic}{1}
\newcommand{\SLOWluindexDCExcDynamicCI}{0}
\newcommand{\SLOWluindexDCExcDynamicCIMIN}{1}
\newcommand{\SLOWluindexDCExcDynamicCIMAX}{1}
\newcommand{\SLOWluindexDC}{\rna}
\newcommand{\SLOWluindexDCCI}{\rna}
\newcommand{\SLOWluindexDCCIMIN}{\rna}
\newcommand{\SLOWluindexDCCIMAX}{\rna}
\newcommand{\SLOWluindexDCDynamic}{\rna}
\newcommand{\SLOWluindexDCDynamicCI}{\rna}
\newcommand{\SLOWluindexDCDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexDCDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGExc}{1}
\newcommand{\SLOWluindexCAPOnoGExcCI}{0}
\newcommand{\SLOWluindexCAPOnoGExcCIMIN}{1}
\newcommand{\SLOWluindexCAPOnoGExcCIMAX}{1}
\newcommand{\SLOWluindexCAPOnoGExcDynamic}{1}
\newcommand{\SLOWluindexCAPOnoGExcDynamicCI}{0}
\newcommand{\SLOWluindexCAPOnoGExcDynamicCIMIN}{1}
\newcommand{\SLOWluindexCAPOnoGExcDynamicCIMAX}{1}
\newcommand{\SLOWluindexCAPOnoG}{\rna}
\newcommand{\SLOWluindexCAPOnoGCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamic}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOExc}{1}
\newcommand{\SLOWluindexCAPOExcCI}{0}
\newcommand{\SLOWluindexCAPOExcCIMIN}{1}
\newcommand{\SLOWluindexCAPOExcCIMAX}{1}
\newcommand{\SLOWluindexCAPOExcDynamic}{1}
\newcommand{\SLOWluindexCAPOExcDynamicCI}{0}
\newcommand{\SLOWluindexCAPOExcDynamicCIMIN}{1}
\newcommand{\SLOWluindexCAPOExcDynamicCIMAX}{1}
\newcommand{\SLOWluindexCAPO}{\rna}
\newcommand{\SLOWluindexCAPOCI}{\rna}
\newcommand{\SLOWluindexCAPOCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOCIMAX}{\rna}
\newcommand{\SLOWluindexCAPODynamic}{\rna}
\newcommand{\SLOWluindexCAPODynamicCI}{\rna}
\newcommand{\SLOWluindexCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWluindexCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIP}{\rna}
\newcommand{\SLOWluindexPIPCI}{\rna}
\newcommand{\SLOWluindexPIPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPDynamic}{\rna}
\newcommand{\SLOWluindexPIPDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexHBUP}{1}
\newcommand{\SLOWluindexHBUPCI}{0}
\newcommand{\SLOWluindexHBUPCIMIN}{1}
\newcommand{\SLOWluindexHBUPCIMAX}{1}
\newcommand{\SLOWluindexHBDynamicUP}{1}
\newcommand{\SLOWluindexHBDynamicUPCI}{0}
\newcommand{\SLOWluindexHBDynamicUPCIMIN}{1}
\newcommand{\SLOWluindexHBDynamicUPCIMAX}{1}
\newcommand{\SLOWluindexWCPUP}{1}
\newcommand{\SLOWluindexWCPUPCI}{0}
\newcommand{\SLOWluindexWCPUPCIMIN}{1}
\newcommand{\SLOWluindexWCPUPCIMAX}{1}
\newcommand{\SLOWluindexWCPDynamicUP}{1}
\newcommand{\SLOWluindexWCPDynamicUPCI}{0}
\newcommand{\SLOWluindexWCPDynamicUPCIMIN}{1}
\newcommand{\SLOWluindexWCPDynamicUPCIMAX}{1}
\newcommand{\SLOWluindexWDCnoGUP}{\rna}
\newcommand{\SLOWluindexWDCnoGUPCI}{\rna}
\newcommand{\SLOWluindexWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWluindexWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWluindexWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWluindexWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWluindexWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexWDCUP}{\rna}
\newcommand{\SLOWluindexWDCUPCI}{\rna}
\newcommand{\SLOWluindexWDCUPCIMIN}{\rna}
\newcommand{\SLOWluindexWDCUPCIMAX}{\rna}
\newcommand{\SLOWluindexWDCDynamicUP}{\rna}
\newcommand{\SLOWluindexWDCDynamicUPCI}{\rna}
\newcommand{\SLOWluindexWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGUP}{\rna}
\newcommand{\SLOWluindexCAPOnoGUPCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOUP}{\rna}
\newcommand{\SLOWluindexCAPOUPCI}{\rna}
\newcommand{\SLOWluindexCAPOUPCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOUPCIMAX}{\rna}
\newcommand{\SLOWluindexCAPODynamicUP}{\rna}
\newcommand{\SLOWluindexCAPODynamicUPCI}{\rna}
\newcommand{\SLOWluindexCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPUP}{\rna}
\newcommand{\SLOWluindexPIPUPCI}{\rna}
\newcommand{\SLOWluindexPIPUPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPUPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPDynamicUP}{\rna}
\newcommand{\SLOWluindexPIPDynamicUPCI}{\rna}
\newcommand{\SLOWluindexPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPHB}{\rna}
\newcommand{\SLOWluindexPIPHBCI}{\rna}
\newcommand{\SLOWluindexPIPHBCIMIN}{\rna}
\newcommand{\SLOWluindexPIPHBCIMAX}{\rna}
\newcommand{\SLOWluindexPIPHBDynamic}{\rna}
\newcommand{\SLOWluindexPIPHBDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIPWCP}{\rna}
\newcommand{\SLOWluindexPIPWCPCI}{\rna}
\newcommand{\SLOWluindexPIPWCPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPWCPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPWCPDynamic}{\rna}
\newcommand{\SLOWluindexPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIPWDC}{\rna}
\newcommand{\SLOWluindexPIPWDCCI}{\rna}
\newcommand{\SLOWluindexPIPWDCCIMIN}{\rna}
\newcommand{\SLOWluindexPIPWDCCIMAX}{\rna}
\newcommand{\SLOWluindexPIPWDCDynamic}{\rna}
\newcommand{\SLOWluindexPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIPCAPO}{\rna}
\newcommand{\SLOWluindexPIPCAPOCI}{\rna}
\newcommand{\SLOWluindexPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWluindexPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWluindexPIPCAPODynamic}{\rna}
\newcommand{\SLOWluindexPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWluindexPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIPPIP}{\rna}
\newcommand{\SLOWluindexPIPPIPCI}{\rna}
\newcommand{\SLOWluindexPIPPIPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPPIPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPPIPDynamic}{\rna}
\newcommand{\SLOWluindexPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchEvents}{1,400}
\newcommand{\SLOWlusearchNoFPEvents}{190}
\newcommand{\SLOWlusearchMaxLiveThreads}{10}
\newcommand{\SLOWlusearchTotalThreads}{10}
\newcommand{\SLOWlusearchBaseTime}{0.96}
\newcommand{\SLOWlusearchBaseTimeCI}{83}
\newcommand{\SLOWlusearchEmptyTime}{\rna}
\newcommand{\SLOWlusearchEmptyTimeCI}{\rna}
\newcommand{\SLOWlusearchEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchFTTime}{\rna}
\newcommand{\SLOWlusearchFTTimeCI}{\rna}
\newcommand{\SLOWlusearchFTTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchFTTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchHBTime}{28}
\newcommand{\SLOWlusearchHBTimeCI}{2.6}
\newcommand{\SLOWlusearchWCPTime}{41}
\newcommand{\SLOWlusearchWCPTimeCI}{4.0}
\newcommand{\SLOWlusearchDCnoGExcTime}{30}
\newcommand{\SLOWlusearchDCnoGExcTimeCI}{2.8}
\newcommand{\SLOWlusearchDCnoGTime}{\rna}
\newcommand{\SLOWlusearchDCnoGTimeCI}{\rna}
\newcommand{\SLOWlusearchDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchDCExcTime}{36}
\newcommand{\SLOWlusearchDCExcTimeCI}{6.4}
\newcommand{\SLOWlusearchDCTime}{\rna}
\newcommand{\SLOWlusearchDCTimeCI}{\rna}
\newcommand{\SLOWlusearchDCTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchDCTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGExcTime}{29}
\newcommand{\SLOWlusearchCAPOnoGExcTimeCI}{2.4}
\newcommand{\SLOWlusearchCAPOnoGTime}{\rna}
\newcommand{\SLOWlusearchCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOExcTime}{33}
\newcommand{\SLOWlusearchCAPOExcTimeCI}{3.1}
\newcommand{\SLOWlusearchCAPOTime}{\rna}
\newcommand{\SLOWlusearchCAPOTimeCI}{\rna}
\newcommand{\SLOWlusearchCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchStaticTime}{\rzero}
\newcommand{\SLOWlusearchDynamicTime}{\rzero}
\newcommand{\SLOWlusearchBaseMem}{1,600}
\newcommand{\SLOWlusearchBaseMemCI}{11.0}
\newcommand{\SLOWlusearchHBMem}{14}
\newcommand{\SLOWlusearchHBMemCI}{0.51}
\newcommand{\SLOWlusearchFTMem}{\memna}
\newcommand{\SLOWlusearchFTMemCI}{\memna}
\newcommand{\SLOWlusearchFTMemCIMIN}{\memna}
\newcommand{\SLOWlusearchFTMemCIMAX}{\memna}
\newcommand{\SLOWlusearchWCPMem}{18}
\newcommand{\SLOWlusearchWCPMemCI}{0.59}
\newcommand{\SLOWlusearchDCnoGExcMem}{14}
\newcommand{\SLOWlusearchDCnoGExcMemCI}{0.35}
\newcommand{\SLOWlusearchDCnoGMem}{\memna}
\newcommand{\SLOWlusearchDCnoGMemCI}{\memna}
\newcommand{\SLOWlusearchDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWlusearchDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWlusearchDCExcMem}{15}
\newcommand{\SLOWlusearchDCExcMemCI}{0.54}
\newcommand{\SLOWlusearchDCMem}{\memna}
\newcommand{\SLOWlusearchDCMemCI}{\memna}
\newcommand{\SLOWlusearchDCMemCIMIN}{\memna}
\newcommand{\SLOWlusearchDCMemCIMAX}{\memna}
\newcommand{\SLOWlusearchCAPOnoGExcMem}{13}
\newcommand{\SLOWlusearchCAPOnoGExcMemCI}{0.59}
\newcommand{\SLOWlusearchCAPOnoGMem}{\memna}
\newcommand{\SLOWlusearchCAPOnoGMemCI}{\memna}
\newcommand{\SLOWlusearchCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWlusearchCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWlusearchCAPOExcMem}{15}
\newcommand{\SLOWlusearchCAPOExcMemCI}{0.49}
\newcommand{\SLOWlusearchCAPOMem}{\memna}
\newcommand{\SLOWlusearchCAPOMemCI}{\memna}
\newcommand{\SLOWlusearchCAPOMemCIMIN}{\memna}
\newcommand{\SLOWlusearchCAPOMemCIMAX}{\memna}
\newcommand{\SLOWlusearchEventsCI}{22}
\newcommand{\SLOWlusearchEventsCIMIN}{1,443,227,310}
\newcommand{\SLOWlusearchEventsCIMAX}{1,443,227,354}
\newcommand{\SLOWlusearchNoFPEventsCI}{22}
\newcommand{\SLOWlusearchNoFPEventsCIMIN}{194,058,140}
\newcommand{\SLOWlusearchNoFPEventsCIMAX}{194,058,184}
\newcommand{\SLOWlusearchHB}{0}
\newcommand{\SLOWlusearchHBCI}{0}
\newcommand{\SLOWlusearchHBCIMIN}{0}
\newcommand{\SLOWlusearchHBCIMAX}{0}
\newcommand{\SLOWlusearchHBDynamic}{0}
\newcommand{\SLOWlusearchHBDynamicCI}{0}
\newcommand{\SLOWlusearchHBDynamicCIMIN}{0}
\newcommand{\SLOWlusearchHBDynamicCIMAX}{0}
\newcommand{\SLOWlusearchFT}{\rna}
\newcommand{\SLOWlusearchFTCI}{\rna}
\newcommand{\SLOWlusearchFTCIMIN}{\rna}
\newcommand{\SLOWlusearchFTCIMAX}{\rna}
\newcommand{\SLOWlusearchFTDynamic}{\rna}
\newcommand{\SLOWlusearchFTDynamicCI}{\rna}
\newcommand{\SLOWlusearchFTDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchFTDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchWCP}{0}
\newcommand{\SLOWlusearchWCPCI}{0}
\newcommand{\SLOWlusearchWCPCIMIN}{0}
\newcommand{\SLOWlusearchWCPCIMAX}{0}
\newcommand{\SLOWlusearchWCPDynamic}{0}
\newcommand{\SLOWlusearchWCPDynamicCI}{0}
\newcommand{\SLOWlusearchWCPDynamicCIMIN}{0}
\newcommand{\SLOWlusearchWCPDynamicCIMAX}{0}
\newcommand{\SLOWlusearchDCnoGExc}{0}
\newcommand{\SLOWlusearchDCnoGExcCI}{0}
\newcommand{\SLOWlusearchDCnoGExcCIMIN}{0}
\newcommand{\SLOWlusearchDCnoGExcCIMAX}{0}
\newcommand{\SLOWlusearchDCnoGExcDynamic}{0}
\newcommand{\SLOWlusearchDCnoGExcDynamicCI}{0}
\newcommand{\SLOWlusearchDCnoGExcDynamicCIMIN}{0}
\newcommand{\SLOWlusearchDCnoGExcDynamicCIMAX}{0}
\newcommand{\SLOWlusearchDCnoG}{\rna}
\newcommand{\SLOWlusearchDCnoGCI}{\rna}
\newcommand{\SLOWlusearchDCnoGCIMIN}{\rna}
\newcommand{\SLOWlusearchDCnoGCIMAX}{\rna}
\newcommand{\SLOWlusearchDCnoGDynamic}{\rna}
\newcommand{\SLOWlusearchDCnoGDynamicCI}{\rna}
\newcommand{\SLOWlusearchDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchDCExc}{0}
\newcommand{\SLOWlusearchDCExcCI}{0}
\newcommand{\SLOWlusearchDCExcCIMIN}{0}
\newcommand{\SLOWlusearchDCExcCIMAX}{0}
\newcommand{\SLOWlusearchDCExcDynamic}{0}
\newcommand{\SLOWlusearchDCExcDynamicCI}{0}
\newcommand{\SLOWlusearchDCExcDynamicCIMIN}{0}
\newcommand{\SLOWlusearchDCExcDynamicCIMAX}{0}
\newcommand{\SLOWlusearchDC}{\rna}
\newcommand{\SLOWlusearchDCCI}{\rna}
\newcommand{\SLOWlusearchDCCIMIN}{\rna}
\newcommand{\SLOWlusearchDCCIMAX}{\rna}
\newcommand{\SLOWlusearchDCDynamic}{\rna}
\newcommand{\SLOWlusearchDCDynamicCI}{\rna}
\newcommand{\SLOWlusearchDCDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchDCDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGExc}{0}
\newcommand{\SLOWlusearchCAPOnoGExcCI}{0}
\newcommand{\SLOWlusearchCAPOnoGExcCIMIN}{0}
\newcommand{\SLOWlusearchCAPOnoGExcCIMAX}{0}
\newcommand{\SLOWlusearchCAPOnoGExcDynamic}{0}
\newcommand{\SLOWlusearchCAPOnoGExcDynamicCI}{0}
\newcommand{\SLOWlusearchCAPOnoGExcDynamicCIMIN}{0}
\newcommand{\SLOWlusearchCAPOnoGExcDynamicCIMAX}{0}
\newcommand{\SLOWlusearchCAPOnoG}{\rna}
\newcommand{\SLOWlusearchCAPOnoGCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamic}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOExc}{0}
\newcommand{\SLOWlusearchCAPOExcCI}{0}
\newcommand{\SLOWlusearchCAPOExcCIMIN}{0}
\newcommand{\SLOWlusearchCAPOExcCIMAX}{0}
\newcommand{\SLOWlusearchCAPOExcDynamic}{0}
\newcommand{\SLOWlusearchCAPOExcDynamicCI}{0}
\newcommand{\SLOWlusearchCAPOExcDynamicCIMIN}{0}
\newcommand{\SLOWlusearchCAPOExcDynamicCIMAX}{0}
\newcommand{\SLOWlusearchCAPO}{\rna}
\newcommand{\SLOWlusearchCAPOCI}{\rna}
\newcommand{\SLOWlusearchCAPOCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPODynamic}{\rna}
\newcommand{\SLOWlusearchCAPODynamicCI}{\rna}
\newcommand{\SLOWlusearchCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIP}{\rna}
\newcommand{\SLOWlusearchPIPCI}{\rna}
\newcommand{\SLOWlusearchPIPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPDynamic}{\rna}
\newcommand{\SLOWlusearchPIPDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchHBUP}{0}
\newcommand{\SLOWlusearchHBUPCI}{0}
\newcommand{\SLOWlusearchHBUPCIMIN}{0}
\newcommand{\SLOWlusearchHBUPCIMAX}{0}
\newcommand{\SLOWlusearchHBDynamicUP}{0}
\newcommand{\SLOWlusearchHBDynamicUPCI}{0}
\newcommand{\SLOWlusearchHBDynamicUPCIMIN}{0}
\newcommand{\SLOWlusearchHBDynamicUPCIMAX}{0}
\newcommand{\SLOWlusearchWCPUP}{0}
\newcommand{\SLOWlusearchWCPUPCI}{0}
\newcommand{\SLOWlusearchWCPUPCIMIN}{0}
\newcommand{\SLOWlusearchWCPUPCIMAX}{0}
\newcommand{\SLOWlusearchWCPDynamicUP}{0}
\newcommand{\SLOWlusearchWCPDynamicUPCI}{0}
\newcommand{\SLOWlusearchWCPDynamicUPCIMIN}{0}
\newcommand{\SLOWlusearchWCPDynamicUPCIMAX}{0}
\newcommand{\SLOWlusearchWDCnoGUP}{\rna}
\newcommand{\SLOWlusearchWDCnoGUPCI}{\rna}
\newcommand{\SLOWlusearchWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWlusearchWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWlusearchWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWlusearchWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWlusearchWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchWDCUP}{\rna}
\newcommand{\SLOWlusearchWDCUPCI}{\rna}
\newcommand{\SLOWlusearchWDCUPCIMIN}{\rna}
\newcommand{\SLOWlusearchWDCUPCIMAX}{\rna}
\newcommand{\SLOWlusearchWDCDynamicUP}{\rna}
\newcommand{\SLOWlusearchWDCDynamicUPCI}{\rna}
\newcommand{\SLOWlusearchWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGUP}{\rna}
\newcommand{\SLOWlusearchCAPOnoGUPCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOUP}{\rna}
\newcommand{\SLOWlusearchCAPOUPCI}{\rna}
\newcommand{\SLOWlusearchCAPOUPCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOUPCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPODynamicUP}{\rna}
\newcommand{\SLOWlusearchCAPODynamicUPCI}{\rna}
\newcommand{\SLOWlusearchCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPUP}{\rna}
\newcommand{\SLOWlusearchPIPUPCI}{\rna}
\newcommand{\SLOWlusearchPIPUPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPUPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPDynamicUP}{\rna}
\newcommand{\SLOWlusearchPIPDynamicUPCI}{\rna}
\newcommand{\SLOWlusearchPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPHB}{\rna}
\newcommand{\SLOWlusearchPIPHBCI}{\rna}
\newcommand{\SLOWlusearchPIPHBCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPHBCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPHBDynamic}{\rna}
\newcommand{\SLOWlusearchPIPHBDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPWCP}{\rna}
\newcommand{\SLOWlusearchPIPWCPCI}{\rna}
\newcommand{\SLOWlusearchPIPWCPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPWCPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPWCPDynamic}{\rna}
\newcommand{\SLOWlusearchPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPWDC}{\rna}
\newcommand{\SLOWlusearchPIPWDCCI}{\rna}
\newcommand{\SLOWlusearchPIPWDCCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPWDCCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPWDCDynamic}{\rna}
\newcommand{\SLOWlusearchPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPCAPO}{\rna}
\newcommand{\SLOWlusearchPIPCAPOCI}{\rna}
\newcommand{\SLOWlusearchPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPCAPODynamic}{\rna}
\newcommand{\SLOWlusearchPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPPIP}{\rna}
\newcommand{\SLOWlusearchPIPPIPCI}{\rna}
\newcommand{\SLOWlusearchPIPPIPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPPIPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPPIPDynamic}{\rna}
\newcommand{\SLOWlusearchPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdEvents}{200}
\newcommand{\SLOWpmdNoFPEvents}{25}
\newcommand{\SLOWpmdMaxLiveThreads}{9}
\newcommand{\SLOWpmdTotalThreads}{9}
\newcommand{\SLOWpmdBaseTime}{1.2}
\newcommand{\SLOWpmdBaseTimeCI}{15}
\newcommand{\SLOWpmdEmptyTime}{\rna}
\newcommand{\SLOWpmdEmptyTimeCI}{\rna}
\newcommand{\SLOWpmdEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWpmdEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWpmdFTTime}{\rna}
\newcommand{\SLOWpmdFTTimeCI}{\rna}
\newcommand{\SLOWpmdFTTimeCIMIN}{\rna}
\newcommand{\SLOWpmdFTTimeCIMAX}{\rna}
\newcommand{\SLOWpmdHBTime}{14}
\newcommand{\SLOWpmdHBTimeCI}{0.40}
\newcommand{\SLOWpmdWCPTime}{18}
\newcommand{\SLOWpmdWCPTimeCI}{0.83}
\newcommand{\SLOWpmdDCnoGExcTime}{15}
\newcommand{\SLOWpmdDCnoGExcTimeCI}{0.31}
\newcommand{\SLOWpmdDCnoGTime}{\rna}
\newcommand{\SLOWpmdDCnoGTimeCI}{\rna}
\newcommand{\SLOWpmdDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWpmdDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWpmdDCExcTime}{15}
\newcommand{\SLOWpmdDCExcTimeCI}{0.42}
\newcommand{\SLOWpmdDCTime}{\rna}
\newcommand{\SLOWpmdDCTimeCI}{\rna}
\newcommand{\SLOWpmdDCTimeCIMIN}{\rna}
\newcommand{\SLOWpmdDCTimeCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGExcTime}{15}
\newcommand{\SLOWpmdCAPOnoGExcTimeCI}{0.36}
\newcommand{\SLOWpmdCAPOnoGTime}{\rna}
\newcommand{\SLOWpmdCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOExcTime}{15}
\newcommand{\SLOWpmdCAPOExcTimeCI}{0.39}
\newcommand{\SLOWpmdCAPOTime}{\rna}
\newcommand{\SLOWpmdCAPOTimeCI}{\rna}
\newcommand{\SLOWpmdCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWpmdStaticTime}{\rzero}
\newcommand{\SLOWpmdDynamicTime}{\rzero}
\newcommand{\SLOWpmdBaseMem}{630}
\newcommand{\SLOWpmdBaseMemCI}{12.0}
\newcommand{\SLOWpmdHBMem}{11}
\newcommand{\SLOWpmdHBMemCI}{0.33}
\newcommand{\SLOWpmdFTMem}{\memna}
\newcommand{\SLOWpmdFTMemCI}{\memna}
\newcommand{\SLOWpmdFTMemCIMIN}{\memna}
\newcommand{\SLOWpmdFTMemCIMAX}{\memna}
\newcommand{\SLOWpmdWCPMem}{17}
\newcommand{\SLOWpmdWCPMemCI}{0.56}
\newcommand{\SLOWpmdDCnoGExcMem}{11}
\newcommand{\SLOWpmdDCnoGExcMemCI}{0.35}
\newcommand{\SLOWpmdDCnoGMem}{\memna}
\newcommand{\SLOWpmdDCnoGMemCI}{\memna}
\newcommand{\SLOWpmdDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWpmdDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWpmdDCExcMem}{12}
\newcommand{\SLOWpmdDCExcMemCI}{0.25}
\newcommand{\SLOWpmdDCMem}{\memna}
\newcommand{\SLOWpmdDCMemCI}{\memna}
\newcommand{\SLOWpmdDCMemCIMIN}{\memna}
\newcommand{\SLOWpmdDCMemCIMAX}{\memna}
\newcommand{\SLOWpmdCAPOnoGExcMem}{11}
\newcommand{\SLOWpmdCAPOnoGExcMemCI}{0.33}
\newcommand{\SLOWpmdCAPOnoGMem}{\memna}
\newcommand{\SLOWpmdCAPOnoGMemCI}{\memna}
\newcommand{\SLOWpmdCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWpmdCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWpmdCAPOExcMem}{12}
\newcommand{\SLOWpmdCAPOExcMemCI}{0.21}
\newcommand{\SLOWpmdCAPOMem}{\memna}
\newcommand{\SLOWpmdCAPOMemCI}{\memna}
\newcommand{\SLOWpmdCAPOMemCIMIN}{\memna}
\newcommand{\SLOWpmdCAPOMemCIMAX}{\memna}
\newcommand{\SLOWpmdEventsCI}{631}
\newcommand{\SLOWpmdEventsCIMIN}{200,052,280}
\newcommand{\SLOWpmdEventsCIMAX}{200,053,542}
\newcommand{\SLOWpmdNoFPEventsCI}{116}
\newcommand{\SLOWpmdNoFPEventsCIMIN}{25,405,240}
\newcommand{\SLOWpmdNoFPEventsCIMAX}{25,405,472}
\newcommand{\SLOWpmdHB}{4}
\newcommand{\SLOWpmdHBCI}{0}
\newcommand{\SLOWpmdHBCIMIN}{4}
\newcommand{\SLOWpmdHBCIMAX}{4}
\newcommand{\SLOWpmdHBDynamic}{21}
\newcommand{\SLOWpmdHBDynamicCI}{2}
\newcommand{\SLOWpmdHBDynamicCIMIN}{19}
\newcommand{\SLOWpmdHBDynamicCIMAX}{23}
\newcommand{\SLOWpmdFT}{\rna}
\newcommand{\SLOWpmdFTCI}{\rna}
\newcommand{\SLOWpmdFTCIMIN}{\rna}
\newcommand{\SLOWpmdFTCIMAX}{\rna}
\newcommand{\SLOWpmdFTDynamic}{\rna}
\newcommand{\SLOWpmdFTDynamicCI}{\rna}
\newcommand{\SLOWpmdFTDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdFTDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdWCP}{4}
\newcommand{\SLOWpmdWCPCI}{0}
\newcommand{\SLOWpmdWCPCIMIN}{4}
\newcommand{\SLOWpmdWCPCIMAX}{4}
\newcommand{\SLOWpmdWCPDynamic}{19}
\newcommand{\SLOWpmdWCPDynamicCI}{4}
\newcommand{\SLOWpmdWCPDynamicCIMIN}{15}
\newcommand{\SLOWpmdWCPDynamicCIMAX}{23}
\newcommand{\SLOWpmdDCnoGExc}{8}
\newcommand{\SLOWpmdDCnoGExcCI}{0}
\newcommand{\SLOWpmdDCnoGExcCIMIN}{8}
\newcommand{\SLOWpmdDCnoGExcCIMAX}{8}
\newcommand{\SLOWpmdDCnoGExcDynamic}{523}
\newcommand{\SLOWpmdDCnoGExcDynamicCI}{27}
\newcommand{\SLOWpmdDCnoGExcDynamicCIMIN}{496}
\newcommand{\SLOWpmdDCnoGExcDynamicCIMAX}{550}
\newcommand{\SLOWpmdDCnoG}{\rna}
\newcommand{\SLOWpmdDCnoGCI}{\rna}
\newcommand{\SLOWpmdDCnoGCIMIN}{\rna}
\newcommand{\SLOWpmdDCnoGCIMAX}{\rna}
\newcommand{\SLOWpmdDCnoGDynamic}{\rna}
\newcommand{\SLOWpmdDCnoGDynamicCI}{\rna}
\newcommand{\SLOWpmdDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdDCExc}{5}
\newcommand{\SLOWpmdDCExcCI}{0}
\newcommand{\SLOWpmdDCExcCIMIN}{5}
\newcommand{\SLOWpmdDCExcCIMAX}{5}
\newcommand{\SLOWpmdDCExcDynamic}{34}
\newcommand{\SLOWpmdDCExcDynamicCI}{2}
\newcommand{\SLOWpmdDCExcDynamicCIMIN}{32}
\newcommand{\SLOWpmdDCExcDynamicCIMAX}{36}
\newcommand{\SLOWpmdDC}{\rna}
\newcommand{\SLOWpmdDCCI}{\rna}
\newcommand{\SLOWpmdDCCIMIN}{\rna}
\newcommand{\SLOWpmdDCCIMAX}{\rna}
\newcommand{\SLOWpmdDCDynamic}{\rna}
\newcommand{\SLOWpmdDCDynamicCI}{\rna}
\newcommand{\SLOWpmdDCDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdDCDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGExc}{7}
\newcommand{\SLOWpmdCAPOnoGExcCI}{0}
\newcommand{\SLOWpmdCAPOnoGExcCIMIN}{7}
\newcommand{\SLOWpmdCAPOnoGExcCIMAX}{7}
\newcommand{\SLOWpmdCAPOnoGExcDynamic}{563}
\newcommand{\SLOWpmdCAPOnoGExcDynamicCI}{42}
\newcommand{\SLOWpmdCAPOnoGExcDynamicCIMIN}{521}
\newcommand{\SLOWpmdCAPOnoGExcDynamicCIMAX}{605}
\newcommand{\SLOWpmdCAPOnoG}{\rna}
\newcommand{\SLOWpmdCAPOnoGCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamic}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOExc}{5}
\newcommand{\SLOWpmdCAPOExcCI}{0}
\newcommand{\SLOWpmdCAPOExcCIMIN}{5}
\newcommand{\SLOWpmdCAPOExcCIMAX}{5}
\newcommand{\SLOWpmdCAPOExcDynamic}{34}
\newcommand{\SLOWpmdCAPOExcDynamicCI}{2}
\newcommand{\SLOWpmdCAPOExcDynamicCIMIN}{32}
\newcommand{\SLOWpmdCAPOExcDynamicCIMAX}{36}
\newcommand{\SLOWpmdCAPO}{\rna}
\newcommand{\SLOWpmdCAPOCI}{\rna}
\newcommand{\SLOWpmdCAPOCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOCIMAX}{\rna}
\newcommand{\SLOWpmdCAPODynamic}{\rna}
\newcommand{\SLOWpmdCAPODynamicCI}{\rna}
\newcommand{\SLOWpmdCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWpmdCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIP}{\rna}
\newcommand{\SLOWpmdPIPCI}{\rna}
\newcommand{\SLOWpmdPIPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPDynamic}{\rna}
\newcommand{\SLOWpmdPIPDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdHBUP}{4}
\newcommand{\SLOWpmdHBUPCI}{0}
\newcommand{\SLOWpmdHBUPCIMIN}{4}
\newcommand{\SLOWpmdHBUPCIMAX}{4}
\newcommand{\SLOWpmdHBDynamicUP}{21}
\newcommand{\SLOWpmdHBDynamicUPCI}{2}
\newcommand{\SLOWpmdHBDynamicUPCIMIN}{19}
\newcommand{\SLOWpmdHBDynamicUPCIMAX}{23}
\newcommand{\SLOWpmdWCPUP}{4}
\newcommand{\SLOWpmdWCPUPCI}{0}
\newcommand{\SLOWpmdWCPUPCIMIN}{4}
\newcommand{\SLOWpmdWCPUPCIMAX}{4}
\newcommand{\SLOWpmdWCPDynamicUP}{19}
\newcommand{\SLOWpmdWCPDynamicUPCI}{4}
\newcommand{\SLOWpmdWCPDynamicUPCIMIN}{15}
\newcommand{\SLOWpmdWCPDynamicUPCIMAX}{23}
\newcommand{\SLOWpmdWDCnoGUP}{\rna}
\newcommand{\SLOWpmdWDCnoGUPCI}{\rna}
\newcommand{\SLOWpmdWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWpmdWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWpmdWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWpmdWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWpmdWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdWDCUP}{\rna}
\newcommand{\SLOWpmdWDCUPCI}{\rna}
\newcommand{\SLOWpmdWDCUPCIMIN}{\rna}
\newcommand{\SLOWpmdWDCUPCIMAX}{\rna}
\newcommand{\SLOWpmdWDCDynamicUP}{\rna}
\newcommand{\SLOWpmdWDCDynamicUPCI}{\rna}
\newcommand{\SLOWpmdWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGUP}{\rna}
\newcommand{\SLOWpmdCAPOnoGUPCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOUP}{\rna}
\newcommand{\SLOWpmdCAPOUPCI}{\rna}
\newcommand{\SLOWpmdCAPOUPCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOUPCIMAX}{\rna}
\newcommand{\SLOWpmdCAPODynamicUP}{\rna}
\newcommand{\SLOWpmdCAPODynamicUPCI}{\rna}
\newcommand{\SLOWpmdCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPUP}{\rna}
\newcommand{\SLOWpmdPIPUPCI}{\rna}
\newcommand{\SLOWpmdPIPUPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPUPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPDynamicUP}{\rna}
\newcommand{\SLOWpmdPIPDynamicUPCI}{\rna}
\newcommand{\SLOWpmdPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPHB}{\rna}
\newcommand{\SLOWpmdPIPHBCI}{\rna}
\newcommand{\SLOWpmdPIPHBCIMIN}{\rna}
\newcommand{\SLOWpmdPIPHBCIMAX}{\rna}
\newcommand{\SLOWpmdPIPHBDynamic}{\rna}
\newcommand{\SLOWpmdPIPHBDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIPWCP}{\rna}
\newcommand{\SLOWpmdPIPWCPCI}{\rna}
\newcommand{\SLOWpmdPIPWCPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPWCPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPWCPDynamic}{\rna}
\newcommand{\SLOWpmdPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIPWDC}{\rna}
\newcommand{\SLOWpmdPIPWDCCI}{\rna}
\newcommand{\SLOWpmdPIPWDCCIMIN}{\rna}
\newcommand{\SLOWpmdPIPWDCCIMAX}{\rna}
\newcommand{\SLOWpmdPIPWDCDynamic}{\rna}
\newcommand{\SLOWpmdPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIPCAPO}{\rna}
\newcommand{\SLOWpmdPIPCAPOCI}{\rna}
\newcommand{\SLOWpmdPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWpmdPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWpmdPIPCAPODynamic}{\rna}
\newcommand{\SLOWpmdPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWpmdPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIPPIP}{\rna}
\newcommand{\SLOWpmdPIPPIPCI}{\rna}
\newcommand{\SLOWpmdPIPPIPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPPIPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPPIPDynamic}{\rna}
\newcommand{\SLOWpmdPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowEvents}{9,700}
\newcommand{\SLOWsunflowNoFPEvents}{760}
\newcommand{\SLOWsunflowMaxLiveThreads}{17}
\newcommand{\SLOWsunflowTotalThreads}{17}
\newcommand{\SLOWsunflowBaseTime}{1.7}
\newcommand{\SLOWsunflowBaseTimeCI}{93}
\newcommand{\SLOWsunflowEmptyTime}{\rna}
\newcommand{\SLOWsunflowEmptyTimeCI}{\rna}
\newcommand{\SLOWsunflowEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowFTTime}{\rna}
\newcommand{\SLOWsunflowFTTimeCI}{\rna}
\newcommand{\SLOWsunflowFTTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowFTTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowHBTime}{75}
\newcommand{\SLOWsunflowHBTimeCI}{8.7}
\newcommand{\SLOWsunflowWCPTime}{90}
\newcommand{\SLOWsunflowWCPTimeCI}{5.8}
\newcommand{\SLOWsunflowDCnoGExcTime}{74}
\newcommand{\SLOWsunflowDCnoGExcTimeCI}{13}
\newcommand{\SLOWsunflowDCnoGTime}{\rna}
\newcommand{\SLOWsunflowDCnoGTimeCI}{\rna}
\newcommand{\SLOWsunflowDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowDCExcTime}{77}
\newcommand{\SLOWsunflowDCExcTimeCI}{4.3}
\newcommand{\SLOWsunflowDCTime}{\rna}
\newcommand{\SLOWsunflowDCTimeCI}{\rna}
\newcommand{\SLOWsunflowDCTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowDCTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGExcTime}{70}
\newcommand{\SLOWsunflowCAPOnoGExcTimeCI}{4.0}
\newcommand{\SLOWsunflowCAPOnoGTime}{\rna}
\newcommand{\SLOWsunflowCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOExcTime}{82}
\newcommand{\SLOWsunflowCAPOExcTimeCI}{8.9}
\newcommand{\SLOWsunflowCAPOTime}{\rna}
\newcommand{\SLOWsunflowCAPOTimeCI}{\rna}
\newcommand{\SLOWsunflowCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowStaticTime}{\rzero}
\newcommand{\SLOWsunflowDynamicTime}{\rzero}
\newcommand{\SLOWsunflowBaseMem}{630}
\newcommand{\SLOWsunflowBaseMemCI}{0.86}
\newcommand{\SLOWsunflowHBMem}{25}
\newcommand{\SLOWsunflowHBMemCI}{0.94}
\newcommand{\SLOWsunflowFTMem}{\memna}
\newcommand{\SLOWsunflowFTMemCI}{\memna}
\newcommand{\SLOWsunflowFTMemCIMIN}{\memna}
\newcommand{\SLOWsunflowFTMemCIMAX}{\memna}
\newcommand{\SLOWsunflowWCPMem}{51}
\newcommand{\SLOWsunflowWCPMemCI}{0.81}
\newcommand{\SLOWsunflowDCnoGExcMem}{24}
\newcommand{\SLOWsunflowDCnoGExcMemCI}{0.84}
\newcommand{\SLOWsunflowDCnoGMem}{\memna}
\newcommand{\SLOWsunflowDCnoGMemCI}{\memna}
\newcommand{\SLOWsunflowDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWsunflowDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWsunflowDCExcMem}{27}
\newcommand{\SLOWsunflowDCExcMemCI}{0.51}
\newcommand{\SLOWsunflowDCMem}{\memna}
\newcommand{\SLOWsunflowDCMemCI}{\memna}
\newcommand{\SLOWsunflowDCMemCIMIN}{\memna}
\newcommand{\SLOWsunflowDCMemCIMAX}{\memna}
\newcommand{\SLOWsunflowCAPOnoGExcMem}{24}
\newcommand{\SLOWsunflowCAPOnoGExcMemCI}{0.41}
\newcommand{\SLOWsunflowCAPOnoGMem}{\memna}
\newcommand{\SLOWsunflowCAPOnoGMemCI}{\memna}
\newcommand{\SLOWsunflowCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWsunflowCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWsunflowCAPOExcMem}{25}
\newcommand{\SLOWsunflowCAPOExcMemCI}{0.64}
\newcommand{\SLOWsunflowCAPOMem}{\memna}
\newcommand{\SLOWsunflowCAPOMemCI}{\memna}
\newcommand{\SLOWsunflowCAPOMemCIMIN}{\memna}
\newcommand{\SLOWsunflowCAPOMemCIMAX}{\memna}
\newcommand{\SLOWsunflowEventsCI}{2}
\newcommand{\SLOWsunflowEventsCIMIN}{9,681,321,387}
\newcommand{\SLOWsunflowEventsCIMAX}{9,681,321,391}
\newcommand{\SLOWsunflowNoFPEventsCI}{7}
\newcommand{\SLOWsunflowNoFPEventsCIMIN}{764,388,867}
\newcommand{\SLOWsunflowNoFPEventsCIMAX}{764,388,881}
\newcommand{\SLOWsunflowHB}{3}
\newcommand{\SLOWsunflowHBCI}{0}
\newcommand{\SLOWsunflowHBCIMIN}{3}
\newcommand{\SLOWsunflowHBCIMAX}{3}
\newcommand{\SLOWsunflowHBDynamic}{7}
\newcommand{\SLOWsunflowHBDynamicCI}{0}
\newcommand{\SLOWsunflowHBDynamicCIMIN}{7}
\newcommand{\SLOWsunflowHBDynamicCIMAX}{7}
\newcommand{\SLOWsunflowFT}{\rna}
\newcommand{\SLOWsunflowFTCI}{\rna}
\newcommand{\SLOWsunflowFTCIMIN}{\rna}
\newcommand{\SLOWsunflowFTCIMAX}{\rna}
\newcommand{\SLOWsunflowFTDynamic}{\rna}
\newcommand{\SLOWsunflowFTDynamicCI}{\rna}
\newcommand{\SLOWsunflowFTDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowFTDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowWCP}{3}
\newcommand{\SLOWsunflowWCPCI}{0}
\newcommand{\SLOWsunflowWCPCIMIN}{3}
\newcommand{\SLOWsunflowWCPCIMAX}{3}
\newcommand{\SLOWsunflowWCPDynamic}{10}
\newcommand{\SLOWsunflowWCPDynamicCI}{2}
\newcommand{\SLOWsunflowWCPDynamicCIMIN}{8}
\newcommand{\SLOWsunflowWCPDynamicCIMAX}{12}
\newcommand{\SLOWsunflowDCnoGExc}{3}
\newcommand{\SLOWsunflowDCnoGExcCI}{0}
\newcommand{\SLOWsunflowDCnoGExcCIMIN}{3}
\newcommand{\SLOWsunflowDCnoGExcCIMAX}{3}
\newcommand{\SLOWsunflowDCnoGExcDynamic}{14}
\newcommand{\SLOWsunflowDCnoGExcDynamicCI}{0}
\newcommand{\SLOWsunflowDCnoGExcDynamicCIMIN}{14}
\newcommand{\SLOWsunflowDCnoGExcDynamicCIMAX}{14}
\newcommand{\SLOWsunflowDCnoG}{\rna}
\newcommand{\SLOWsunflowDCnoGCI}{\rna}
\newcommand{\SLOWsunflowDCnoGCIMIN}{\rna}
\newcommand{\SLOWsunflowDCnoGCIMAX}{\rna}
\newcommand{\SLOWsunflowDCnoGDynamic}{\rna}
\newcommand{\SLOWsunflowDCnoGDynamicCI}{\rna}
\newcommand{\SLOWsunflowDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowDCExc}{3}
\newcommand{\SLOWsunflowDCExcCI}{0}
\newcommand{\SLOWsunflowDCExcCIMIN}{3}
\newcommand{\SLOWsunflowDCExcCIMAX}{3}
\newcommand{\SLOWsunflowDCExcDynamic}{14}
\newcommand{\SLOWsunflowDCExcDynamicCI}{0}
\newcommand{\SLOWsunflowDCExcDynamicCIMIN}{14}
\newcommand{\SLOWsunflowDCExcDynamicCIMAX}{14}
\newcommand{\SLOWsunflowDC}{\rna}
\newcommand{\SLOWsunflowDCCI}{\rna}
\newcommand{\SLOWsunflowDCCIMIN}{\rna}
\newcommand{\SLOWsunflowDCCIMAX}{\rna}
\newcommand{\SLOWsunflowDCDynamic}{\rna}
\newcommand{\SLOWsunflowDCDynamicCI}{\rna}
\newcommand{\SLOWsunflowDCDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowDCDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGExc}{3}
\newcommand{\SLOWsunflowCAPOnoGExcCI}{0}
\newcommand{\SLOWsunflowCAPOnoGExcCIMIN}{3}
\newcommand{\SLOWsunflowCAPOnoGExcCIMAX}{3}
\newcommand{\SLOWsunflowCAPOnoGExcDynamic}{14}
\newcommand{\SLOWsunflowCAPOnoGExcDynamicCI}{0}
\newcommand{\SLOWsunflowCAPOnoGExcDynamicCIMIN}{14}
\newcommand{\SLOWsunflowCAPOnoGExcDynamicCIMAX}{14}
\newcommand{\SLOWsunflowCAPOnoG}{\rna}
\newcommand{\SLOWsunflowCAPOnoGCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamic}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOExc}{3}
\newcommand{\SLOWsunflowCAPOExcCI}{0}
\newcommand{\SLOWsunflowCAPOExcCIMIN}{3}
\newcommand{\SLOWsunflowCAPOExcCIMAX}{3}
\newcommand{\SLOWsunflowCAPOExcDynamic}{14}
\newcommand{\SLOWsunflowCAPOExcDynamicCI}{0}
\newcommand{\SLOWsunflowCAPOExcDynamicCIMIN}{14}
\newcommand{\SLOWsunflowCAPOExcDynamicCIMAX}{14}
\newcommand{\SLOWsunflowCAPO}{\rna}
\newcommand{\SLOWsunflowCAPOCI}{\rna}
\newcommand{\SLOWsunflowCAPOCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPODynamic}{\rna}
\newcommand{\SLOWsunflowCAPODynamicCI}{\rna}
\newcommand{\SLOWsunflowCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIP}{\rna}
\newcommand{\SLOWsunflowPIPCI}{\rna}
\newcommand{\SLOWsunflowPIPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPDynamic}{\rna}
\newcommand{\SLOWsunflowPIPDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowHBUP}{2}
\newcommand{\SLOWsunflowHBUPCI}{0}
\newcommand{\SLOWsunflowHBUPCIMIN}{2}
\newcommand{\SLOWsunflowHBUPCIMAX}{2}
\newcommand{\SLOWsunflowHBDynamicUP}{7}
\newcommand{\SLOWsunflowHBDynamicUPCI}{0}
\newcommand{\SLOWsunflowHBDynamicUPCIMIN}{7}
\newcommand{\SLOWsunflowHBDynamicUPCIMAX}{7}
\newcommand{\SLOWsunflowWCPUP}{2}
\newcommand{\SLOWsunflowWCPUPCI}{0}
\newcommand{\SLOWsunflowWCPUPCIMIN}{2}
\newcommand{\SLOWsunflowWCPUPCIMAX}{2}
\newcommand{\SLOWsunflowWCPDynamicUP}{10}
\newcommand{\SLOWsunflowWCPDynamicUPCI}{2}
\newcommand{\SLOWsunflowWCPDynamicUPCIMIN}{8}
\newcommand{\SLOWsunflowWCPDynamicUPCIMAX}{12}
\newcommand{\SLOWsunflowWDCnoGUP}{\rna}
\newcommand{\SLOWsunflowWDCnoGUPCI}{\rna}
\newcommand{\SLOWsunflowWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWsunflowWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWsunflowWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWsunflowWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWsunflowWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowWDCUP}{\rna}
\newcommand{\SLOWsunflowWDCUPCI}{\rna}
\newcommand{\SLOWsunflowWDCUPCIMIN}{\rna}
\newcommand{\SLOWsunflowWDCUPCIMAX}{\rna}
\newcommand{\SLOWsunflowWDCDynamicUP}{\rna}
\newcommand{\SLOWsunflowWDCDynamicUPCI}{\rna}
\newcommand{\SLOWsunflowWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGUP}{\rna}
\newcommand{\SLOWsunflowCAPOnoGUPCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOUP}{\rna}
\newcommand{\SLOWsunflowCAPOUPCI}{\rna}
\newcommand{\SLOWsunflowCAPOUPCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOUPCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPODynamicUP}{\rna}
\newcommand{\SLOWsunflowCAPODynamicUPCI}{\rna}
\newcommand{\SLOWsunflowCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPUP}{\rna}
\newcommand{\SLOWsunflowPIPUPCI}{\rna}
\newcommand{\SLOWsunflowPIPUPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPUPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPDynamicUP}{\rna}
\newcommand{\SLOWsunflowPIPDynamicUPCI}{\rna}
\newcommand{\SLOWsunflowPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPHB}{\rna}
\newcommand{\SLOWsunflowPIPHBCI}{\rna}
\newcommand{\SLOWsunflowPIPHBCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPHBCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPHBDynamic}{\rna}
\newcommand{\SLOWsunflowPIPHBDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPWCP}{\rna}
\newcommand{\SLOWsunflowPIPWCPCI}{\rna}
\newcommand{\SLOWsunflowPIPWCPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPWCPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPWCPDynamic}{\rna}
\newcommand{\SLOWsunflowPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPWDC}{\rna}
\newcommand{\SLOWsunflowPIPWDCCI}{\rna}
\newcommand{\SLOWsunflowPIPWDCCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPWDCCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPWDCDynamic}{\rna}
\newcommand{\SLOWsunflowPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPCAPO}{\rna}
\newcommand{\SLOWsunflowPIPCAPOCI}{\rna}
\newcommand{\SLOWsunflowPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPCAPODynamic}{\rna}
\newcommand{\SLOWsunflowPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPPIP}{\rna}
\newcommand{\SLOWsunflowPIPPIPCI}{\rna}
\newcommand{\SLOWsunflowPIPPIPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPPIPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPPIPDynamic}{\rna}
\newcommand{\SLOWsunflowPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatEvents}{47}
\newcommand{\SLOWtomcatNoFPEvents}{18}
\newcommand{\SLOWtomcatMaxLiveThreads}{28}
\newcommand{\SLOWtomcatTotalThreads}{35}
\newcommand{\SLOWtomcatBaseTime}{0.93}
\newcommand{\SLOWtomcatBaseTimeCI}{11}
\newcommand{\SLOWtomcatEmptyTime}{\rna}
\newcommand{\SLOWtomcatEmptyTimeCI}{\rna}
\newcommand{\SLOWtomcatEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatFTTime}{\rna}
\newcommand{\SLOWtomcatFTTimeCI}{\rna}
\newcommand{\SLOWtomcatFTTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatFTTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatHBTime}{9.0}
\newcommand{\SLOWtomcatHBTimeCI}{0.13}
\newcommand{\SLOWtomcatWCPTime}{12}
\newcommand{\SLOWtomcatWCPTimeCI}{0.29}
\newcommand{\SLOWtomcatDCnoGExcTime}{12}
\newcommand{\SLOWtomcatDCnoGExcTimeCI}{0.83}
\newcommand{\SLOWtomcatDCnoGTime}{\rna}
\newcommand{\SLOWtomcatDCnoGTimeCI}{\rna}
\newcommand{\SLOWtomcatDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatDCExcTime}{13}
\newcommand{\SLOWtomcatDCExcTimeCI}{0.75}
\newcommand{\SLOWtomcatDCTime}{\rna}
\newcommand{\SLOWtomcatDCTimeCI}{\rna}
\newcommand{\SLOWtomcatDCTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatDCTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGExcTime}{9.4}
\newcommand{\SLOWtomcatCAPOnoGExcTimeCI}{0.13}
\newcommand{\SLOWtomcatCAPOnoGTime}{\rna}
\newcommand{\SLOWtomcatCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOExcTime}{9.6}
\newcommand{\SLOWtomcatCAPOExcTimeCI}{0.26}
\newcommand{\SLOWtomcatCAPOTime}{\rna}
\newcommand{\SLOWtomcatCAPOTimeCI}{\rna}
\newcommand{\SLOWtomcatCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatStaticTime}{\rzero}
\newcommand{\SLOWtomcatDynamicTime}{\rzero}
\newcommand{\SLOWtomcatBaseMem}{510}
\newcommand{\SLOWtomcatBaseMemCI}{3.9}
\newcommand{\SLOWtomcatHBMem}{16}
\newcommand{\SLOWtomcatHBMemCI}{0.82}
\newcommand{\SLOWtomcatFTMem}{\memna}
\newcommand{\SLOWtomcatFTMemCI}{\memna}
\newcommand{\SLOWtomcatFTMemCIMIN}{\memna}
\newcommand{\SLOWtomcatFTMemCIMAX}{\memna}
\newcommand{\SLOWtomcatWCPMem}{22}
\newcommand{\SLOWtomcatWCPMemCI}{0.78}
\newcommand{\SLOWtomcatDCnoGExcMem}{22}
\newcommand{\SLOWtomcatDCnoGExcMemCI}{0.57}
\newcommand{\SLOWtomcatDCnoGMem}{\memna}
\newcommand{\SLOWtomcatDCnoGMemCI}{\memna}
\newcommand{\SLOWtomcatDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWtomcatDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWtomcatDCExcMem}{24}
\newcommand{\SLOWtomcatDCExcMemCI}{1.2}
\newcommand{\SLOWtomcatDCMem}{\memna}
\newcommand{\SLOWtomcatDCMemCI}{\memna}
\newcommand{\SLOWtomcatDCMemCIMIN}{\memna}
\newcommand{\SLOWtomcatDCMemCIMAX}{\memna}
\newcommand{\SLOWtomcatCAPOnoGExcMem}{18}
\newcommand{\SLOWtomcatCAPOnoGExcMemCI}{0.39}
\newcommand{\SLOWtomcatCAPOnoGMem}{\memna}
\newcommand{\SLOWtomcatCAPOnoGMemCI}{\memna}
\newcommand{\SLOWtomcatCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWtomcatCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWtomcatCAPOExcMem}{22}
\newcommand{\SLOWtomcatCAPOExcMemCI}{0.52}
\newcommand{\SLOWtomcatCAPOMem}{\memna}
\newcommand{\SLOWtomcatCAPOMemCI}{\memna}
\newcommand{\SLOWtomcatCAPOMemCIMIN}{\memna}
\newcommand{\SLOWtomcatCAPOMemCIMAX}{\memna}
\newcommand{\SLOWtomcatEventsCI}{44,311}
\newcommand{\SLOWtomcatEventsCIMIN}{46,955,082}
\newcommand{\SLOWtomcatEventsCIMAX}{47,043,704}
\newcommand{\SLOWtomcatNoFPEventsCI}{14,677}
\newcommand{\SLOWtomcatNoFPEventsCIMIN}{18,262,814}
\newcommand{\SLOWtomcatNoFPEventsCIMAX}{18,292,168}
\newcommand{\SLOWtomcatHB}{55}
\newcommand{\SLOWtomcatHBCI}{2}
\newcommand{\SLOWtomcatHBCIMIN}{53}
\newcommand{\SLOWtomcatHBCIMAX}{57}
\newcommand{\SLOWtomcatHBDynamic}{12,412}
\newcommand{\SLOWtomcatHBDynamicCI}{274}
\newcommand{\SLOWtomcatHBDynamicCIMIN}{12,138}
\newcommand{\SLOWtomcatHBDynamicCIMAX}{12,686}
\newcommand{\SLOWtomcatFT}{\rna}
\newcommand{\SLOWtomcatFTCI}{\rna}
\newcommand{\SLOWtomcatFTCIMIN}{\rna}
\newcommand{\SLOWtomcatFTCIMAX}{\rna}
\newcommand{\SLOWtomcatFTDynamic}{\rna}
\newcommand{\SLOWtomcatFTDynamicCI}{\rna}
\newcommand{\SLOWtomcatFTDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatFTDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatWCP}{56}
\newcommand{\SLOWtomcatWCPCI}{2}
\newcommand{\SLOWtomcatWCPCIMIN}{54}
\newcommand{\SLOWtomcatWCPCIMAX}{58}
\newcommand{\SLOWtomcatWCPDynamic}{11,803}
\newcommand{\SLOWtomcatWCPDynamicCI}{380}
\newcommand{\SLOWtomcatWCPDynamicCIMIN}{11,423}
\newcommand{\SLOWtomcatWCPDynamicCIMAX}{12,183}
\newcommand{\SLOWtomcatDCnoGExc}{95}
\newcommand{\SLOWtomcatDCnoGExcCI}{2}
\newcommand{\SLOWtomcatDCnoGExcCIMIN}{93}
\newcommand{\SLOWtomcatDCnoGExcCIMAX}{97}
\newcommand{\SLOWtomcatDCnoGExcDynamic}{26,960}
\newcommand{\SLOWtomcatDCnoGExcDynamicCI}{773}
\newcommand{\SLOWtomcatDCnoGExcDynamicCIMIN}{26,187}
\newcommand{\SLOWtomcatDCnoGExcDynamicCIMAX}{27,733}
\newcommand{\SLOWtomcatDCnoG}{\rna}
\newcommand{\SLOWtomcatDCnoGCI}{\rna}
\newcommand{\SLOWtomcatDCnoGCIMIN}{\rna}
\newcommand{\SLOWtomcatDCnoGCIMAX}{\rna}
\newcommand{\SLOWtomcatDCnoGDynamic}{\rna}
\newcommand{\SLOWtomcatDCnoGDynamicCI}{\rna}
\newcommand{\SLOWtomcatDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatDCExc}{64}
\newcommand{\SLOWtomcatDCExcCI}{1}
\newcommand{\SLOWtomcatDCExcCIMIN}{63}
\newcommand{\SLOWtomcatDCExcCIMAX}{65}
\newcommand{\SLOWtomcatDCExcDynamic}{12,402}
\newcommand{\SLOWtomcatDCExcDynamicCI}{352}
\newcommand{\SLOWtomcatDCExcDynamicCIMIN}{12,050}
\newcommand{\SLOWtomcatDCExcDynamicCIMAX}{12,754}
\newcommand{\SLOWtomcatDC}{\rna}
\newcommand{\SLOWtomcatDCCI}{\rna}
\newcommand{\SLOWtomcatDCCIMIN}{\rna}
\newcommand{\SLOWtomcatDCCIMAX}{\rna}
\newcommand{\SLOWtomcatDCDynamic}{\rna}
\newcommand{\SLOWtomcatDCDynamicCI}{\rna}
\newcommand{\SLOWtomcatDCDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatDCDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGExc}{91}
\newcommand{\SLOWtomcatCAPOnoGExcCI}{2}
\newcommand{\SLOWtomcatCAPOnoGExcCIMIN}{89}
\newcommand{\SLOWtomcatCAPOnoGExcCIMAX}{93}
\newcommand{\SLOWtomcatCAPOnoGExcDynamic}{27,090}
\newcommand{\SLOWtomcatCAPOnoGExcDynamicCI}{393}
\newcommand{\SLOWtomcatCAPOnoGExcDynamicCIMIN}{26,697}
\newcommand{\SLOWtomcatCAPOnoGExcDynamicCIMAX}{27,483}
\newcommand{\SLOWtomcatCAPOnoG}{\rna}
\newcommand{\SLOWtomcatCAPOnoGCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamic}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOExc}{67}
\newcommand{\SLOWtomcatCAPOExcCI}{2}
\newcommand{\SLOWtomcatCAPOExcCIMIN}{65}
\newcommand{\SLOWtomcatCAPOExcCIMAX}{69}
\newcommand{\SLOWtomcatCAPOExcDynamic}{13,080}
\newcommand{\SLOWtomcatCAPOExcDynamicCI}{185}
\newcommand{\SLOWtomcatCAPOExcDynamicCIMIN}{12,895}
\newcommand{\SLOWtomcatCAPOExcDynamicCIMAX}{13,265}
\newcommand{\SLOWtomcatCAPO}{\rna}
\newcommand{\SLOWtomcatCAPOCI}{\rna}
\newcommand{\SLOWtomcatCAPOCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPODynamic}{\rna}
\newcommand{\SLOWtomcatCAPODynamicCI}{\rna}
\newcommand{\SLOWtomcatCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIP}{\rna}
\newcommand{\SLOWtomcatPIPCI}{\rna}
\newcommand{\SLOWtomcatPIPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPDynamic}{\rna}
\newcommand{\SLOWtomcatPIPDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatHBUP}{48}
\newcommand{\SLOWtomcatHBUPCI}{2}
\newcommand{\SLOWtomcatHBUPCIMIN}{46}
\newcommand{\SLOWtomcatHBUPCIMAX}{50}
\newcommand{\SLOWtomcatHBDynamicUP}{12,414}
\newcommand{\SLOWtomcatHBDynamicUPCI}{273}
\newcommand{\SLOWtomcatHBDynamicUPCIMIN}{12,141}
\newcommand{\SLOWtomcatHBDynamicUPCIMAX}{12,687}
\newcommand{\SLOWtomcatWCPUP}{50}
\newcommand{\SLOWtomcatWCPUPCI}{1}
\newcommand{\SLOWtomcatWCPUPCIMIN}{49}
\newcommand{\SLOWtomcatWCPUPCIMAX}{51}
\newcommand{\SLOWtomcatWCPDynamicUP}{11,805}
\newcommand{\SLOWtomcatWCPDynamicUPCI}{379}
\newcommand{\SLOWtomcatWCPDynamicUPCIMIN}{11,426}
\newcommand{\SLOWtomcatWCPDynamicUPCIMAX}{12,184}
\newcommand{\SLOWtomcatWDCnoGUP}{\rna}
\newcommand{\SLOWtomcatWDCnoGUPCI}{\rna}
\newcommand{\SLOWtomcatWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWtomcatWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWtomcatWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWtomcatWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWtomcatWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatWDCUP}{\rna}
\newcommand{\SLOWtomcatWDCUPCI}{\rna}
\newcommand{\SLOWtomcatWDCUPCIMIN}{\rna}
\newcommand{\SLOWtomcatWDCUPCIMAX}{\rna}
\newcommand{\SLOWtomcatWDCDynamicUP}{\rna}
\newcommand{\SLOWtomcatWDCDynamicUPCI}{\rna}
\newcommand{\SLOWtomcatWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGUP}{\rna}
\newcommand{\SLOWtomcatCAPOnoGUPCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOUP}{\rna}
\newcommand{\SLOWtomcatCAPOUPCI}{\rna}
\newcommand{\SLOWtomcatCAPOUPCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOUPCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPODynamicUP}{\rna}
\newcommand{\SLOWtomcatCAPODynamicUPCI}{\rna}
\newcommand{\SLOWtomcatCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPUP}{\rna}
\newcommand{\SLOWtomcatPIPUPCI}{\rna}
\newcommand{\SLOWtomcatPIPUPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPUPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPDynamicUP}{\rna}
\newcommand{\SLOWtomcatPIPDynamicUPCI}{\rna}
\newcommand{\SLOWtomcatPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPHB}{\rna}
\newcommand{\SLOWtomcatPIPHBCI}{\rna}
\newcommand{\SLOWtomcatPIPHBCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPHBCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPHBDynamic}{\rna}
\newcommand{\SLOWtomcatPIPHBDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPWCP}{\rna}
\newcommand{\SLOWtomcatPIPWCPCI}{\rna}
\newcommand{\SLOWtomcatPIPWCPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPWCPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPWCPDynamic}{\rna}
\newcommand{\SLOWtomcatPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPWDC}{\rna}
\newcommand{\SLOWtomcatPIPWDCCI}{\rna}
\newcommand{\SLOWtomcatPIPWDCCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPWDCCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPWDCDynamic}{\rna}
\newcommand{\SLOWtomcatPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPCAPO}{\rna}
\newcommand{\SLOWtomcatPIPCAPOCI}{\rna}
\newcommand{\SLOWtomcatPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPCAPODynamic}{\rna}
\newcommand{\SLOWtomcatPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPPIP}{\rna}
\newcommand{\SLOWtomcatPIPPIPCI}{\rna}
\newcommand{\SLOWtomcatPIPPIPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPPIPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPPIPDynamic}{\rna}
\newcommand{\SLOWtomcatPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanEvents}{630}
\newcommand{\SLOWxalanNoFPEvents}{270}
\newcommand{\SLOWxalanMaxLiveThreads}{9}
\newcommand{\SLOWxalanTotalThreads}{9}
\newcommand{\SLOWxalanBaseTime}{2.0}
\newcommand{\SLOWxalanBaseTimeCI}{220}
\newcommand{\SLOWxalanEmptyTime}{\rna}
\newcommand{\SLOWxalanEmptyTimeCI}{\rna}
\newcommand{\SLOWxalanEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWxalanEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWxalanFTTime}{\rna}
\newcommand{\SLOWxalanFTTimeCI}{\rna}
\newcommand{\SLOWxalanFTTimeCIMIN}{\rna}
\newcommand{\SLOWxalanFTTimeCIMAX}{\rna}
\newcommand{\SLOWxalanHBTime}{15}
\newcommand{\SLOWxalanHBTimeCI}{3.7}
\newcommand{\SLOWxalanWCPTime}{40}
\newcommand{\SLOWxalanWCPTimeCI}{8.1}
\newcommand{\SLOWxalanDCnoGExcTime}{38}
\newcommand{\SLOWxalanDCnoGExcTimeCI}{6.7}
\newcommand{\SLOWxalanDCnoGTime}{\rna}
\newcommand{\SLOWxalanDCnoGTimeCI}{\rna}
\newcommand{\SLOWxalanDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWxalanDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWxalanDCExcTime}{60}
\newcommand{\SLOWxalanDCExcTimeCI}{11}
\newcommand{\SLOWxalanDCTime}{\rna}
\newcommand{\SLOWxalanDCTimeCI}{\rna}
\newcommand{\SLOWxalanDCTimeCIMIN}{\rna}
\newcommand{\SLOWxalanDCTimeCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGExcTime}{35}
\newcommand{\SLOWxalanCAPOnoGExcTimeCI}{6.4}
\newcommand{\SLOWxalanCAPOnoGTime}{\rna}
\newcommand{\SLOWxalanCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOExcTime}{49}
\newcommand{\SLOWxalanCAPOExcTimeCI}{9.8}
\newcommand{\SLOWxalanCAPOTime}{\rna}
\newcommand{\SLOWxalanCAPOTimeCI}{\rna}
\newcommand{\SLOWxalanCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWxalanStaticTime}{\rzero}
\newcommand{\SLOWxalanDynamicTime}{\rzero}
\newcommand{\SLOWxalanBaseMem}{700}
\newcommand{\SLOWxalanBaseMemCI}{6.8}
\newcommand{\SLOWxalanHBMem}{22}
\newcommand{\SLOWxalanHBMemCI}{0.72}
\newcommand{\SLOWxalanFTMem}{\memna}
\newcommand{\SLOWxalanFTMemCI}{\memna}
\newcommand{\SLOWxalanFTMemCIMIN}{\memna}
\newcommand{\SLOWxalanFTMemCIMAX}{\memna}
\newcommand{\SLOWxalanWCPMem}{49}
\newcommand{\SLOWxalanWCPMemCI}{1.3}
\newcommand{\SLOWxalanDCnoGExcMem}{40}
\newcommand{\SLOWxalanDCnoGExcMemCI}{1.8}
\newcommand{\SLOWxalanDCnoGMem}{\memna}
\newcommand{\SLOWxalanDCnoGMemCI}{\memna}
\newcommand{\SLOWxalanDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWxalanDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWxalanDCExcMem}{60}
\newcommand{\SLOWxalanDCExcMemCI}{2.3}
\newcommand{\SLOWxalanDCMem}{\memna}
\newcommand{\SLOWxalanDCMemCI}{\memna}
\newcommand{\SLOWxalanDCMemCIMIN}{\memna}
\newcommand{\SLOWxalanDCMemCIMAX}{\memna}
\newcommand{\SLOWxalanCAPOnoGExcMem}{39}
\newcommand{\SLOWxalanCAPOnoGExcMemCI}{1.2}
\newcommand{\SLOWxalanCAPOnoGMem}{\memna}
\newcommand{\SLOWxalanCAPOnoGMemCI}{\memna}
\newcommand{\SLOWxalanCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWxalanCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWxalanCAPOExcMem}{56}
\newcommand{\SLOWxalanCAPOExcMemCI}{1.7}
\newcommand{\SLOWxalanCAPOMem}{\memna}
\newcommand{\SLOWxalanCAPOMemCI}{\memna}
\newcommand{\SLOWxalanCAPOMemCIMIN}{\memna}
\newcommand{\SLOWxalanCAPOMemCIMAX}{\memna}
\newcommand{\SLOWxalanEventsCI}{43}
\newcommand{\SLOWxalanEventsCIMIN}{626,353,783}
\newcommand{\SLOWxalanEventsCIMAX}{626,353,869}
\newcommand{\SLOWxalanNoFPEventsCI}{38}
\newcommand{\SLOWxalanNoFPEventsCIMIN}{273,861,897}
\newcommand{\SLOWxalanNoFPEventsCIMAX}{273,861,973}
\newcommand{\SLOWxalanHB}{3}
\newcommand{\SLOWxalanHBCI}{0}
\newcommand{\SLOWxalanHBCIMIN}{3}
\newcommand{\SLOWxalanHBCIMAX}{3}
\newcommand{\SLOWxalanHBDynamic}{17}
\newcommand{\SLOWxalanHBDynamicCI}{0}
\newcommand{\SLOWxalanHBDynamicCIMIN}{17}
\newcommand{\SLOWxalanHBDynamicCIMAX}{17}
\newcommand{\SLOWxalanFT}{\rna}
\newcommand{\SLOWxalanFTCI}{\rna}
\newcommand{\SLOWxalanFTCIMIN}{\rna}
\newcommand{\SLOWxalanFTCIMAX}{\rna}
\newcommand{\SLOWxalanFTDynamic}{\rna}
\newcommand{\SLOWxalanFTDynamicCI}{\rna}
\newcommand{\SLOWxalanFTDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanFTDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanWCP}{6}
\newcommand{\SLOWxalanWCPCI}{0}
\newcommand{\SLOWxalanWCPCIMIN}{6}
\newcommand{\SLOWxalanWCPCIMAX}{6}
\newcommand{\SLOWxalanWCPDynamic}{238,434}
\newcommand{\SLOWxalanWCPDynamicCI}{2,043}
\newcommand{\SLOWxalanWCPDynamicCIMIN}{236,391}
\newcommand{\SLOWxalanWCPDynamicCIMAX}{240,477}
\newcommand{\SLOWxalanDCnoGExc}{15}
\newcommand{\SLOWxalanDCnoGExcCI}{0}
\newcommand{\SLOWxalanDCnoGExcCIMIN}{15}
\newcommand{\SLOWxalanDCnoGExcCIMAX}{15}
\newcommand{\SLOWxalanDCnoGExcDynamic}{412,813}
\newcommand{\SLOWxalanDCnoGExcDynamicCI}{3,233}
\newcommand{\SLOWxalanDCnoGExcDynamicCIMIN}{409,580}
\newcommand{\SLOWxalanDCnoGExcDynamicCIMAX}{416,046}
\newcommand{\SLOWxalanDCnoG}{\rna}
\newcommand{\SLOWxalanDCnoGCI}{\rna}
\newcommand{\SLOWxalanDCnoGCIMIN}{\rna}
\newcommand{\SLOWxalanDCnoGCIMAX}{\rna}
\newcommand{\SLOWxalanDCnoGDynamic}{\rna}
\newcommand{\SLOWxalanDCnoGDynamicCI}{\rna}
\newcommand{\SLOWxalanDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanDCExc}{8}
\newcommand{\SLOWxalanDCExcCI}{0}
\newcommand{\SLOWxalanDCExcCIMIN}{8}
\newcommand{\SLOWxalanDCExcCIMAX}{8}
\newcommand{\SLOWxalanDCExcDynamic}{261,296}
\newcommand{\SLOWxalanDCExcDynamicCI}{1,089}
\newcommand{\SLOWxalanDCExcDynamicCIMIN}{260,207}
\newcommand{\SLOWxalanDCExcDynamicCIMAX}{262,385}
\newcommand{\SLOWxalanDC}{\rna}
\newcommand{\SLOWxalanDCCI}{\rna}
\newcommand{\SLOWxalanDCCIMIN}{\rna}
\newcommand{\SLOWxalanDCCIMAX}{\rna}
\newcommand{\SLOWxalanDCDynamic}{\rna}
\newcommand{\SLOWxalanDCDynamicCI}{\rna}
\newcommand{\SLOWxalanDCDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanDCDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGExc}{14}
\newcommand{\SLOWxalanCAPOnoGExcCI}{0}
\newcommand{\SLOWxalanCAPOnoGExcCIMIN}{14}
\newcommand{\SLOWxalanCAPOnoGExcCIMAX}{14}
\newcommand{\SLOWxalanCAPOnoGExcDynamic}{409,729}
\newcommand{\SLOWxalanCAPOnoGExcDynamicCI}{2,104}
\newcommand{\SLOWxalanCAPOnoGExcDynamicCIMIN}{407,625}
\newcommand{\SLOWxalanCAPOnoGExcDynamicCIMAX}{411,833}
\newcommand{\SLOWxalanCAPOnoG}{\rna}
\newcommand{\SLOWxalanCAPOnoGCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamic}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOExc}{7}
\newcommand{\SLOWxalanCAPOExcCI}{0}
\newcommand{\SLOWxalanCAPOExcCIMIN}{7}
\newcommand{\SLOWxalanCAPOExcCIMAX}{7}
\newcommand{\SLOWxalanCAPOExcDynamic}{260,369}
\newcommand{\SLOWxalanCAPOExcDynamicCI}{258}
\newcommand{\SLOWxalanCAPOExcDynamicCIMIN}{260,111}
\newcommand{\SLOWxalanCAPOExcDynamicCIMAX}{260,627}
\newcommand{\SLOWxalanCAPO}{\rna}
\newcommand{\SLOWxalanCAPOCI}{\rna}
\newcommand{\SLOWxalanCAPOCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOCIMAX}{\rna}
\newcommand{\SLOWxalanCAPODynamic}{\rna}
\newcommand{\SLOWxalanCAPODynamicCI}{\rna}
\newcommand{\SLOWxalanCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWxalanCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIP}{\rna}
\newcommand{\SLOWxalanPIPCI}{\rna}
\newcommand{\SLOWxalanPIPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPDynamic}{\rna}
\newcommand{\SLOWxalanPIPDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanHBUP}{3}
\newcommand{\SLOWxalanHBUPCI}{0}
\newcommand{\SLOWxalanHBUPCIMIN}{3}
\newcommand{\SLOWxalanHBUPCIMAX}{3}
\newcommand{\SLOWxalanHBDynamicUP}{17}
\newcommand{\SLOWxalanHBDynamicUPCI}{0}
\newcommand{\SLOWxalanHBDynamicUPCIMIN}{17}
\newcommand{\SLOWxalanHBDynamicUPCIMAX}{17}
\newcommand{\SLOWxalanWCPUP}{11}
\newcommand{\SLOWxalanWCPUPCI}{0}
\newcommand{\SLOWxalanWCPUPCIMIN}{11}
\newcommand{\SLOWxalanWCPUPCIMAX}{11}
\newcommand{\SLOWxalanWCPDynamicUP}{238,765}
\newcommand{\SLOWxalanWCPDynamicUPCI}{2,082}
\newcommand{\SLOWxalanWCPDynamicUPCIMIN}{236,683}
\newcommand{\SLOWxalanWCPDynamicUPCIMAX}{240,847}
\newcommand{\SLOWxalanWDCnoGUP}{\rna}
\newcommand{\SLOWxalanWDCnoGUPCI}{\rna}
\newcommand{\SLOWxalanWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWxalanWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWxalanWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWxalanWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWxalanWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanWDCUP}{\rna}
\newcommand{\SLOWxalanWDCUPCI}{\rna}
\newcommand{\SLOWxalanWDCUPCIMIN}{\rna}
\newcommand{\SLOWxalanWDCUPCIMAX}{\rna}
\newcommand{\SLOWxalanWDCDynamicUP}{\rna}
\newcommand{\SLOWxalanWDCDynamicUPCI}{\rna}
\newcommand{\SLOWxalanWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGUP}{\rna}
\newcommand{\SLOWxalanCAPOnoGUPCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOUP}{\rna}
\newcommand{\SLOWxalanCAPOUPCI}{\rna}
\newcommand{\SLOWxalanCAPOUPCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOUPCIMAX}{\rna}
\newcommand{\SLOWxalanCAPODynamicUP}{\rna}
\newcommand{\SLOWxalanCAPODynamicUPCI}{\rna}
\newcommand{\SLOWxalanCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPUP}{\rna}
\newcommand{\SLOWxalanPIPUPCI}{\rna}
\newcommand{\SLOWxalanPIPUPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPUPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPDynamicUP}{\rna}
\newcommand{\SLOWxalanPIPDynamicUPCI}{\rna}
\newcommand{\SLOWxalanPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPHB}{\rna}
\newcommand{\SLOWxalanPIPHBCI}{\rna}
\newcommand{\SLOWxalanPIPHBCIMIN}{\rna}
\newcommand{\SLOWxalanPIPHBCIMAX}{\rna}
\newcommand{\SLOWxalanPIPHBDynamic}{\rna}
\newcommand{\SLOWxalanPIPHBDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIPWCP}{\rna}
\newcommand{\SLOWxalanPIPWCPCI}{\rna}
\newcommand{\SLOWxalanPIPWCPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPWCPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPWCPDynamic}{\rna}
\newcommand{\SLOWxalanPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIPWDC}{\rna}
\newcommand{\SLOWxalanPIPWDCCI}{\rna}
\newcommand{\SLOWxalanPIPWDCCIMIN}{\rna}
\newcommand{\SLOWxalanPIPWDCCIMAX}{\rna}
\newcommand{\SLOWxalanPIPWDCDynamic}{\rna}
\newcommand{\SLOWxalanPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIPCAPO}{\rna}
\newcommand{\SLOWxalanPIPCAPOCI}{\rna}
\newcommand{\SLOWxalanPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWxalanPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWxalanPIPCAPODynamic}{\rna}
\newcommand{\SLOWxalanPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWxalanPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIPPIP}{\rna}
\newcommand{\SLOWxalanPIPPIPCI}{\rna}
\newcommand{\SLOWxalanPIPPIPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPPIPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPPIPDynamic}{\rna}
\newcommand{\SLOWxalanPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWBaseTimeGeoMean}{1800}
\newcommand{\SLOWEmptyTimeGeoMean}{\rna}
\newcommand{\SLOWFTTimeGeoMean}{\rna}
\newcommand{\SLOWHBTimeGeoMean}{20}
\newcommand{\SLOWWCPTimeGeoMean}{32}
\newcommand{\SLOWDCnoGExcTimeGeoMean}{27}
\newcommand{\SLOWDCnoGTimeGeoMean}{\rna}
\newcommand{\SLOWDCExcTimeGeoMean}{31}
\newcommand{\SLOWDCTimeGeoMean}{\rna}
\newcommand{\SLOWCAPOnoGExcTimeGeoMean}{25}
\newcommand{\SLOWCAPOnoGTimeGeoMean}{\rna}
\newcommand{\SLOWCAPOExcTimeGeoMean}{29}
\newcommand{\SLOWCAPOTimeGeoMean}{\rna}
\newcommand{\SLOWBaseMemGeoMean}{540}
\newcommand{\SLOWEmptyMemGeoMean}{0.0}
\newcommand{\SLOWFTMemGeoMean}{\memna}
\newcommand{\SLOWHBMemGeoMean}{20}
\newcommand{\SLOWWCPMemGeoMean}{37}
\newcommand{\SLOWDCnoGExcMemGeoMean}{26}
\newcommand{\SLOWDCnoGMemGeoMean}{\memna}
\newcommand{\SLOWDCExcMemGeoMean}{33}
\newcommand{\SLOWDCMemGeoMean}{\memna}
\newcommand{\SLOWCAPOnoGExcMemGeoMean}{25}
\newcommand{\SLOWCAPOnoGMemGeoMean}{\memna}
\newcommand{\SLOWCAPOExcMemGeoMean}{31}
\newcommand{\SLOWCAPOMemGeoMean}{\memna}
\newcommand{\SLOWWCPDynamicTotal}{400,472}
\newcommand{\SLOWHBDynamicUPTotal}{182,276}
\newcommand{\SLOWPIPWDCDynamicTotal}{0}
\newcommand{\SLOWCAPOTotal}{0}
\newcommand{\SLOWPIPWCPTotal}{0}
\newcommand{\SLOWWCPTotal}{90}
\newcommand{\SLOWWDCnoGDynamicUPTotal}{0}
\newcommand{\SLOWCAPOnoGExcDynamicTotal}{714,912}
\newcommand{\SLOWCAPOExcTotal}{104}
\newcommand{\SLOWDCExcTotal}{102}
\newcommand{\SLOWDCnoGExcTotal}{145}
\newcommand{\SLOWPIPDynamicUPTotal}{0}
\newcommand{\SLOWPIPPIPTotal}{0}
\newcommand{\SLOWFTTotal}{0}
\newcommand{\SLOWHBDynamicTotal}{182,274}
\newcommand{\SLOWCAPOnoGDynamicUPTotal}{0}
\newcommand{\SLOWDCnoGExcDynamicTotal}{689,345}
\newcommand{\SLOWCAPOnoGTotal}{0}
\newcommand{\SLOWPIPWDCTotal}{0}
\newcommand{\SLOWCAPOnoGExcTotal}{138}
\newcommand{\SLOWPIPHBDynamicTotal}{0}
\newcommand{\SLOWWDCUPTotal}{0}
\newcommand{\SLOWDCnoGTotal}{0}
\newcommand{\SLOWWCPDynamicUPTotal}{400,805}
\newcommand{\SLOWPIPUPTotal}{0}
\newcommand{\SLOWCAPODynamicTotal}{0}
\newcommand{\SLOWCAPOnoGUPTotal}{0}
\newcommand{\SLOWPIPCAPOTotal}{0}
\newcommand{\SLOWCAPOnoGDynamicTotal}{0}
\newcommand{\SLOWFTDynamicTotal}{0}
\newcommand{\SLOWPIPCAPODynamicTotal}{0}
\newcommand{\SLOWDCnoGDynamicTotal}{0}
\newcommand{\SLOWWDCnoGUPTotal}{0}
\newcommand{\SLOWDCExcDynamicTotal}{465,017}
\newcommand{\SLOWWDCDynamicUPTotal}{0}
\newcommand{\SLOWHBUPTotal}{72}
\newcommand{\SLOWCAPOExcDynamicTotal}{531,366}
\newcommand{\SLOWPIPTotal}{0}
\newcommand{\SLOWWCPUPTotal}{83}
\newcommand{\SLOWCAPOUPTotal}{0}
\newcommand{\SLOWPIPHBTotal}{0}
\newcommand{\SLOWHBTotal}{88}
\newcommand{\SLOWDCDynamicTotal}{0}
\newcommand{\SLOWPIPDynamicTotal}{0}
\newcommand{\SLOWCAPODynamicUPTotal}{0}
\newcommand{\SLOWPIPPIPDynamicTotal}{0}
\newcommand{\SLOWPIPWCPDynamicTotal}{0}
\newcommand{\SLOWDCTotal}{0}



==> result-macros/PIP_slowTool_raceEdgeFix_fieldName.tex <==
\newcommand{\SLOWavroraEvents}{1,400}
\newcommand{\SLOWavroraNoFPEvents}{160}
\newcommand{\SLOWavroraMaxLiveThreads}{7}
\newcommand{\SLOWavroraTotalThreads}{7}
\newcommand{\SLOWavroraBaseTime}{2.3}
\newcommand{\SLOWavroraBaseTimeCI}{10}
\newcommand{\SLOWavroraEmptyTime}{\rna}
\newcommand{\SLOWavroraEmptyTimeCI}{\rna}
\newcommand{\SLOWavroraEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWavroraEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWavroraFTTime}{\rna}
\newcommand{\SLOWavroraFTTimeCI}{\rna}
\newcommand{\SLOWavroraFTTimeCIMIN}{\rna}
\newcommand{\SLOWavroraFTTimeCIMAX}{\rna}
\newcommand{\SLOWavroraHBTime}{17}
\newcommand{\SLOWavroraHBTimeCI}{0.18}
\newcommand{\SLOWavroraWCPTime}{23}
\newcommand{\SLOWavroraWCPTimeCI}{0.56}
\newcommand{\SLOWavroraDCnoGExcTime}{21}
\newcommand{\SLOWavroraDCnoGExcTimeCI}{0.39}
\newcommand{\SLOWavroraDCnoGTime}{\rna}
\newcommand{\SLOWavroraDCnoGTimeCI}{\rna}
\newcommand{\SLOWavroraDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWavroraDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWavroraDCExcTime}{25}
\newcommand{\SLOWavroraDCExcTimeCI}{0.54}
\newcommand{\SLOWavroraDCTime}{\rna}
\newcommand{\SLOWavroraDCTimeCI}{\rna}
\newcommand{\SLOWavroraDCTimeCIMIN}{\rna}
\newcommand{\SLOWavroraDCTimeCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGExcTime}{18}
\newcommand{\SLOWavroraCAPOnoGExcTimeCI}{0.25}
\newcommand{\SLOWavroraCAPOnoGTime}{\rna}
\newcommand{\SLOWavroraCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOExcTime}{22}
\newcommand{\SLOWavroraCAPOExcTimeCI}{0.3}
\newcommand{\SLOWavroraCAPOTime}{\rna}
\newcommand{\SLOWavroraCAPOTimeCI}{\rna}
\newcommand{\SLOWavroraCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWavroraStaticTime}{\rzero}
\newcommand{\SLOWavroraDynamicTime}{\rzero}
\newcommand{\SLOWavroraBaseMem}{180}
\newcommand{\SLOWavroraBaseMemCI}{5.4}
\newcommand{\SLOWavroraHBMem}{28}
\newcommand{\SLOWavroraHBMemCI}{0.83}
\newcommand{\SLOWavroraFTMem}{\memna}
\newcommand{\SLOWavroraFTMemCI}{\memna}
\newcommand{\SLOWavroraFTMemCIMIN}{\memna}
\newcommand{\SLOWavroraFTMemCIMAX}{\memna}
\newcommand{\SLOWavroraWCPMem}{83}
\newcommand{\SLOWavroraWCPMemCI}{2.8}
\newcommand{\SLOWavroraDCnoGExcMem}{36}
\newcommand{\SLOWavroraDCnoGExcMemCI}{1.1}
\newcommand{\SLOWavroraDCnoGMem}{\memna}
\newcommand{\SLOWavroraDCnoGMemCI}{\memna}
\newcommand{\SLOWavroraDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWavroraDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWavroraDCExcMem}{61}
\newcommand{\SLOWavroraDCExcMemCI}{2.0}
\newcommand{\SLOWavroraDCMem}{\memna}
\newcommand{\SLOWavroraDCMemCI}{\memna}
\newcommand{\SLOWavroraDCMemCIMIN}{\memna}
\newcommand{\SLOWavroraDCMemCIMAX}{\memna}
\newcommand{\SLOWavroraCAPOnoGExcMem}{32}
\newcommand{\SLOWavroraCAPOnoGExcMemCI}{1.4}
\newcommand{\SLOWavroraCAPOnoGMem}{\memna}
\newcommand{\SLOWavroraCAPOnoGMemCI}{\memna}
\newcommand{\SLOWavroraCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWavroraCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWavroraCAPOExcMem}{61}
\newcommand{\SLOWavroraCAPOExcMemCI}{1.9}
\newcommand{\SLOWavroraCAPOMem}{\memna}
\newcommand{\SLOWavroraCAPOMemCI}{\memna}
\newcommand{\SLOWavroraCAPOMemCIMIN}{\memna}
\newcommand{\SLOWavroraCAPOMemCIMAX}{\memna}
\newcommand{\SLOWavroraEventsCI}{100,577}
\newcommand{\SLOWavroraEventsCIMIN}{1,438,646,762}
\newcommand{\SLOWavroraEventsCIMAX}{1,438,847,916}
\newcommand{\SLOWavroraNoFPEventsCI}{87,377}
\newcommand{\SLOWavroraNoFPEventsCIMIN}{156,476,384}
\newcommand{\SLOWavroraNoFPEventsCIMAX}{156,651,138}
\newcommand{\SLOWavroraHB}{3}
\newcommand{\SLOWavroraHBCI}{0}
\newcommand{\SLOWavroraHBCIMIN}{3}
\newcommand{\SLOWavroraHBCIMAX}{3}
\newcommand{\SLOWavroraHBDynamic}{129,204}
\newcommand{\SLOWavroraHBDynamicCI}{805}
\newcommand{\SLOWavroraHBDynamicCIMIN}{128,399}
\newcommand{\SLOWavroraHBDynamicCIMAX}{130,009}
\newcommand{\SLOWavroraFT}{\rna}
\newcommand{\SLOWavroraFTCI}{\rna}
\newcommand{\SLOWavroraFTCIMIN}{\rna}
\newcommand{\SLOWavroraFTCIMAX}{\rna}
\newcommand{\SLOWavroraFTDynamic}{\rna}
\newcommand{\SLOWavroraFTDynamicCI}{\rna}
\newcommand{\SLOWavroraFTDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraFTDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraWCP}{3}
\newcommand{\SLOWavroraWCPCI}{0}
\newcommand{\SLOWavroraWCPCIMIN}{3}
\newcommand{\SLOWavroraWCPCIMAX}{3}
\newcommand{\SLOWavroraWCPDynamic}{109,148}
\newcommand{\SLOWavroraWCPDynamicCI}{307}
\newcommand{\SLOWavroraWCPDynamicCIMIN}{108,841}
\newcommand{\SLOWavroraWCPDynamicCIMAX}{109,455}
\newcommand{\SLOWavroraDCnoGExc}{3}
\newcommand{\SLOWavroraDCnoGExcCI}{0}
\newcommand{\SLOWavroraDCnoGExcCIMIN}{3}
\newcommand{\SLOWavroraDCnoGExcCIMAX}{3}
\newcommand{\SLOWavroraDCnoGExcDynamic}{207,647}
\newcommand{\SLOWavroraDCnoGExcDynamicCI}{214}
\newcommand{\SLOWavroraDCnoGExcDynamicCIMIN}{207,433}
\newcommand{\SLOWavroraDCnoGExcDynamicCIMAX}{207,861}
\newcommand{\SLOWavroraDCnoG}{\rna}
\newcommand{\SLOWavroraDCnoGCI}{\rna}
\newcommand{\SLOWavroraDCnoGCIMIN}{\rna}
\newcommand{\SLOWavroraDCnoGCIMAX}{\rna}
\newcommand{\SLOWavroraDCnoGDynamic}{\rna}
\newcommand{\SLOWavroraDCnoGDynamicCI}{\rna}
\newcommand{\SLOWavroraDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraDCExc}{3}
\newcommand{\SLOWavroraDCExcCI}{0}
\newcommand{\SLOWavroraDCExcCIMIN}{3}
\newcommand{\SLOWavroraDCExcCIMAX}{3}
\newcommand{\SLOWavroraDCExcDynamic}{149,875}
\newcommand{\SLOWavroraDCExcDynamicCI}{2,229}
\newcommand{\SLOWavroraDCExcDynamicCIMIN}{147,646}
\newcommand{\SLOWavroraDCExcDynamicCIMAX}{152,104}
\newcommand{\SLOWavroraDC}{\rna}
\newcommand{\SLOWavroraDCCI}{\rna}
\newcommand{\SLOWavroraDCCIMIN}{\rna}
\newcommand{\SLOWavroraDCCIMAX}{\rna}
\newcommand{\SLOWavroraDCDynamic}{\rna}
\newcommand{\SLOWavroraDCDynamicCI}{\rna}
\newcommand{\SLOWavroraDCDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraDCDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGExc}{3}
\newcommand{\SLOWavroraCAPOnoGExcCI}{0}
\newcommand{\SLOWavroraCAPOnoGExcCIMIN}{3}
\newcommand{\SLOWavroraCAPOnoGExcCIMAX}{3}
\newcommand{\SLOWavroraCAPOnoGExcDynamic}{236,067}
\newcommand{\SLOWavroraCAPOnoGExcDynamicCI}{1,645}
\newcommand{\SLOWavroraCAPOnoGExcDynamicCIMIN}{234,422}
\newcommand{\SLOWavroraCAPOnoGExcDynamicCIMAX}{237,712}
\newcommand{\SLOWavroraCAPOnoG}{\rna}
\newcommand{\SLOWavroraCAPOnoGCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamic}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOExc}{3}
\newcommand{\SLOWavroraCAPOExcCI}{0}
\newcommand{\SLOWavroraCAPOExcCIMIN}{3}
\newcommand{\SLOWavroraCAPOExcCIMAX}{3}
\newcommand{\SLOWavroraCAPOExcDynamic}{216,435}
\newcommand{\SLOWavroraCAPOExcDynamicCI}{3,317}
\newcommand{\SLOWavroraCAPOExcDynamicCIMIN}{213,118}
\newcommand{\SLOWavroraCAPOExcDynamicCIMAX}{219,752}
\newcommand{\SLOWavroraCAPO}{\rna}
\newcommand{\SLOWavroraCAPOCI}{\rna}
\newcommand{\SLOWavroraCAPOCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOCIMAX}{\rna}
\newcommand{\SLOWavroraCAPODynamic}{\rna}
\newcommand{\SLOWavroraCAPODynamicCI}{\rna}
\newcommand{\SLOWavroraCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWavroraCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIP}{\rna}
\newcommand{\SLOWavroraPIPCI}{\rna}
\newcommand{\SLOWavroraPIPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPDynamic}{\rna}
\newcommand{\SLOWavroraPIPDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraHBUP}{\rna}
\newcommand{\SLOWavroraHBUPCI}{\rna}
\newcommand{\SLOWavroraHBUPCIMIN}{\rna}
\newcommand{\SLOWavroraHBUPCIMAX}{\rna}
\newcommand{\SLOWavroraHBDynamicUP}{\rna}
\newcommand{\SLOWavroraHBDynamicUPCI}{\rna}
\newcommand{\SLOWavroraHBDynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraHBDynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraWCPUP}{\rna}
\newcommand{\SLOWavroraWCPUPCI}{\rna}
\newcommand{\SLOWavroraWCPUPCIMIN}{\rna}
\newcommand{\SLOWavroraWCPUPCIMAX}{\rna}
\newcommand{\SLOWavroraWCPDynamicUP}{\rna}
\newcommand{\SLOWavroraWCPDynamicUPCI}{\rna}
\newcommand{\SLOWavroraWCPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraWCPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraWDCnoGUP}{\rna}
\newcommand{\SLOWavroraWDCnoGUPCI}{\rna}
\newcommand{\SLOWavroraWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWavroraWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWavroraWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWavroraWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWavroraWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraWDCUP}{\rna}
\newcommand{\SLOWavroraWDCUPCI}{\rna}
\newcommand{\SLOWavroraWDCUPCIMIN}{\rna}
\newcommand{\SLOWavroraWDCUPCIMAX}{\rna}
\newcommand{\SLOWavroraWDCDynamicUP}{\rna}
\newcommand{\SLOWavroraWDCDynamicUPCI}{\rna}
\newcommand{\SLOWavroraWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGUP}{\rna}
\newcommand{\SLOWavroraCAPOnoGUPCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraCAPOUP}{\rna}
\newcommand{\SLOWavroraCAPOUPCI}{\rna}
\newcommand{\SLOWavroraCAPOUPCIMIN}{\rna}
\newcommand{\SLOWavroraCAPOUPCIMAX}{\rna}
\newcommand{\SLOWavroraCAPODynamicUP}{\rna}
\newcommand{\SLOWavroraCAPODynamicUPCI}{\rna}
\newcommand{\SLOWavroraCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPUP}{\rna}
\newcommand{\SLOWavroraPIPUPCI}{\rna}
\newcommand{\SLOWavroraPIPUPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPUPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPDynamicUP}{\rna}
\newcommand{\SLOWavroraPIPDynamicUPCI}{\rna}
\newcommand{\SLOWavroraPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPHB}{\rna}
\newcommand{\SLOWavroraPIPHBCI}{\rna}
\newcommand{\SLOWavroraPIPHBCIMIN}{\rna}
\newcommand{\SLOWavroraPIPHBCIMAX}{\rna}
\newcommand{\SLOWavroraPIPHBDynamic}{\rna}
\newcommand{\SLOWavroraPIPHBDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIPWCP}{\rna}
\newcommand{\SLOWavroraPIPWCPCI}{\rna}
\newcommand{\SLOWavroraPIPWCPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPWCPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPWCPDynamic}{\rna}
\newcommand{\SLOWavroraPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIPWDC}{\rna}
\newcommand{\SLOWavroraPIPWDCCI}{\rna}
\newcommand{\SLOWavroraPIPWDCCIMIN}{\rna}
\newcommand{\SLOWavroraPIPWDCCIMAX}{\rna}
\newcommand{\SLOWavroraPIPWDCDynamic}{\rna}
\newcommand{\SLOWavroraPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIPCAPO}{\rna}
\newcommand{\SLOWavroraPIPCAPOCI}{\rna}
\newcommand{\SLOWavroraPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWavroraPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWavroraPIPCAPODynamic}{\rna}
\newcommand{\SLOWavroraPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWavroraPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWavroraPIPPIP}{\rna}
\newcommand{\SLOWavroraPIPPIPCI}{\rna}
\newcommand{\SLOWavroraPIPPIPCIMIN}{\rna}
\newcommand{\SLOWavroraPIPPIPCIMAX}{\rna}
\newcommand{\SLOWavroraPIPPIPDynamic}{\rna}
\newcommand{\SLOWavroraPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWavroraPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWavroraPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikEvents}{160}
\newcommand{\SLOWbatikNoFPEvents}{11}
\newcommand{\SLOWbatikMaxLiveThreads}{7}
\newcommand{\SLOWbatikTotalThreads}{7}
\newcommand{\SLOWbatikBaseTime}{2.5}
\newcommand{\SLOWbatikBaseTimeCI}{33}
\newcommand{\SLOWbatikEmptyTime}{\rna}
\newcommand{\SLOWbatikEmptyTimeCI}{\rna}
\newcommand{\SLOWbatikEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWbatikEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWbatikFTTime}{\rna}
\newcommand{\SLOWbatikFTTimeCI}{\rna}
\newcommand{\SLOWbatikFTTimeCIMIN}{\rna}
\newcommand{\SLOWbatikFTTimeCIMAX}{\rna}
\newcommand{\SLOWbatikHBTime}{8.0}
\newcommand{\SLOWbatikHBTimeCI}{0.086}
\newcommand{\SLOWbatikWCPTime}{12}
\newcommand{\SLOWbatikWCPTimeCI}{0.11}
\newcommand{\SLOWbatikDCnoGExcTime}{10}
\newcommand{\SLOWbatikDCnoGExcTimeCI}{0.1}
\newcommand{\SLOWbatikDCnoGTime}{\rna}
\newcommand{\SLOWbatikDCnoGTimeCI}{\rna}
\newcommand{\SLOWbatikDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWbatikDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWbatikDCExcTime}{11}
\newcommand{\SLOWbatikDCExcTimeCI}{0.14}
\newcommand{\SLOWbatikDCTime}{\rna}
\newcommand{\SLOWbatikDCTimeCI}{\rna}
\newcommand{\SLOWbatikDCTimeCIMIN}{\rna}
\newcommand{\SLOWbatikDCTimeCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGExcTime}{9.8}
\newcommand{\SLOWbatikCAPOnoGExcTimeCI}{0.099}
\newcommand{\SLOWbatikCAPOnoGTime}{\rna}
\newcommand{\SLOWbatikCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOExcTime}{11}
\newcommand{\SLOWbatikCAPOExcTimeCI}{0.096}
\newcommand{\SLOWbatikCAPOTime}{\rna}
\newcommand{\SLOWbatikCAPOTimeCI}{\rna}
\newcommand{\SLOWbatikCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWbatikStaticTime}{\rzero}
\newcommand{\SLOWbatikDynamicTime}{\rzero}
\newcommand{\SLOWbatikBaseMem}{240}
\newcommand{\SLOWbatikBaseMemCI}{0.64}
\newcommand{\SLOWbatikHBMem}{28}
\newcommand{\SLOWbatikHBMemCI}{0.081}
\newcommand{\SLOWbatikFTMem}{\memna}
\newcommand{\SLOWbatikFTMemCI}{\memna}
\newcommand{\SLOWbatikFTMemCIMIN}{\memna}
\newcommand{\SLOWbatikFTMemCIMAX}{\memna}
\newcommand{\SLOWbatikWCPMem}{45}
\newcommand{\SLOWbatikWCPMemCI}{0.25}
\newcommand{\SLOWbatikDCnoGExcMem}{36}
\newcommand{\SLOWbatikDCnoGExcMemCI}{1.6}
\newcommand{\SLOWbatikDCnoGMem}{\memna}
\newcommand{\SLOWbatikDCnoGMemCI}{\memna}
\newcommand{\SLOWbatikDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWbatikDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWbatikDCExcMem}{41}
\newcommand{\SLOWbatikDCExcMemCI}{0.15}
\newcommand{\SLOWbatikDCMem}{\memna}
\newcommand{\SLOWbatikDCMemCI}{\memna}
\newcommand{\SLOWbatikDCMemCIMIN}{\memna}
\newcommand{\SLOWbatikDCMemCIMAX}{\memna}
\newcommand{\SLOWbatikCAPOnoGExcMem}{35}
\newcommand{\SLOWbatikCAPOnoGExcMemCI}{0.18}
\newcommand{\SLOWbatikCAPOnoGMem}{\memna}
\newcommand{\SLOWbatikCAPOnoGMemCI}{\memna}
\newcommand{\SLOWbatikCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWbatikCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWbatikCAPOExcMem}{41}
\newcommand{\SLOWbatikCAPOExcMemCI}{1.8}
\newcommand{\SLOWbatikCAPOMem}{\memna}
\newcommand{\SLOWbatikCAPOMemCI}{\memna}
\newcommand{\SLOWbatikCAPOMemCIMIN}{\memna}
\newcommand{\SLOWbatikCAPOMemCIMAX}{\memna}
\newcommand{\SLOWbatikEventsCI}{0}
\newcommand{\SLOWbatikEventsCIMIN}{155,322,726}
\newcommand{\SLOWbatikEventsCIMAX}{155,322,726}
\newcommand{\SLOWbatikNoFPEventsCI}{0}
\newcommand{\SLOWbatikNoFPEventsCIMIN}{11,422,601}
\newcommand{\SLOWbatikNoFPEventsCIMAX}{11,422,601}
\newcommand{\SLOWbatikHB}{0}
\newcommand{\SLOWbatikHBCI}{0}
\newcommand{\SLOWbatikHBCIMIN}{0}
\newcommand{\SLOWbatikHBCIMAX}{0}
\newcommand{\SLOWbatikHBDynamic}{0}
\newcommand{\SLOWbatikHBDynamicCI}{0}
\newcommand{\SLOWbatikHBDynamicCIMIN}{0}
\newcommand{\SLOWbatikHBDynamicCIMAX}{0}
\newcommand{\SLOWbatikFT}{\rna}
\newcommand{\SLOWbatikFTCI}{\rna}
\newcommand{\SLOWbatikFTCIMIN}{\rna}
\newcommand{\SLOWbatikFTCIMAX}{\rna}
\newcommand{\SLOWbatikFTDynamic}{\rna}
\newcommand{\SLOWbatikFTDynamicCI}{\rna}
\newcommand{\SLOWbatikFTDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikFTDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikWCP}{0}
\newcommand{\SLOWbatikWCPCI}{0}
\newcommand{\SLOWbatikWCPCIMIN}{0}
\newcommand{\SLOWbatikWCPCIMAX}{0}
\newcommand{\SLOWbatikWCPDynamic}{0}
\newcommand{\SLOWbatikWCPDynamicCI}{0}
\newcommand{\SLOWbatikWCPDynamicCIMIN}{0}
\newcommand{\SLOWbatikWCPDynamicCIMAX}{0}
\newcommand{\SLOWbatikDCnoGExc}{0}
\newcommand{\SLOWbatikDCnoGExcCI}{0}
\newcommand{\SLOWbatikDCnoGExcCIMIN}{0}
\newcommand{\SLOWbatikDCnoGExcCIMAX}{0}
\newcommand{\SLOWbatikDCnoGExcDynamic}{0}
\newcommand{\SLOWbatikDCnoGExcDynamicCI}{0}
\newcommand{\SLOWbatikDCnoGExcDynamicCIMIN}{0}
\newcommand{\SLOWbatikDCnoGExcDynamicCIMAX}{0}
\newcommand{\SLOWbatikDCnoG}{\rna}
\newcommand{\SLOWbatikDCnoGCI}{\rna}
\newcommand{\SLOWbatikDCnoGCIMIN}{\rna}
\newcommand{\SLOWbatikDCnoGCIMAX}{\rna}
\newcommand{\SLOWbatikDCnoGDynamic}{\rna}
\newcommand{\SLOWbatikDCnoGDynamicCI}{\rna}
\newcommand{\SLOWbatikDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikDCExc}{0}
\newcommand{\SLOWbatikDCExcCI}{0}
\newcommand{\SLOWbatikDCExcCIMIN}{0}
\newcommand{\SLOWbatikDCExcCIMAX}{0}
\newcommand{\SLOWbatikDCExcDynamic}{0}
\newcommand{\SLOWbatikDCExcDynamicCI}{0}
\newcommand{\SLOWbatikDCExcDynamicCIMIN}{0}
\newcommand{\SLOWbatikDCExcDynamicCIMAX}{0}
\newcommand{\SLOWbatikDC}{\rna}
\newcommand{\SLOWbatikDCCI}{\rna}
\newcommand{\SLOWbatikDCCIMIN}{\rna}
\newcommand{\SLOWbatikDCCIMAX}{\rna}
\newcommand{\SLOWbatikDCDynamic}{\rna}
\newcommand{\SLOWbatikDCDynamicCI}{\rna}
\newcommand{\SLOWbatikDCDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikDCDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGExc}{0}
\newcommand{\SLOWbatikCAPOnoGExcCI}{0}
\newcommand{\SLOWbatikCAPOnoGExcCIMIN}{0}
\newcommand{\SLOWbatikCAPOnoGExcCIMAX}{0}
\newcommand{\SLOWbatikCAPOnoGExcDynamic}{0}
\newcommand{\SLOWbatikCAPOnoGExcDynamicCI}{0}
\newcommand{\SLOWbatikCAPOnoGExcDynamicCIMIN}{0}
\newcommand{\SLOWbatikCAPOnoGExcDynamicCIMAX}{0}
\newcommand{\SLOWbatikCAPOnoG}{\rna}
\newcommand{\SLOWbatikCAPOnoGCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamic}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOExc}{0}
\newcommand{\SLOWbatikCAPOExcCI}{0}
\newcommand{\SLOWbatikCAPOExcCIMIN}{0}
\newcommand{\SLOWbatikCAPOExcCIMAX}{0}
\newcommand{\SLOWbatikCAPOExcDynamic}{0}
\newcommand{\SLOWbatikCAPOExcDynamicCI}{0}
\newcommand{\SLOWbatikCAPOExcDynamicCIMIN}{0}
\newcommand{\SLOWbatikCAPOExcDynamicCIMAX}{0}
\newcommand{\SLOWbatikCAPO}{\rna}
\newcommand{\SLOWbatikCAPOCI}{\rna}
\newcommand{\SLOWbatikCAPOCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOCIMAX}{\rna}
\newcommand{\SLOWbatikCAPODynamic}{\rna}
\newcommand{\SLOWbatikCAPODynamicCI}{\rna}
\newcommand{\SLOWbatikCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWbatikCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIP}{\rna}
\newcommand{\SLOWbatikPIPCI}{\rna}
\newcommand{\SLOWbatikPIPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPDynamic}{\rna}
\newcommand{\SLOWbatikPIPDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikHBUP}{\rna}
\newcommand{\SLOWbatikHBUPCI}{\rna}
\newcommand{\SLOWbatikHBUPCIMIN}{\rna}
\newcommand{\SLOWbatikHBUPCIMAX}{\rna}
\newcommand{\SLOWbatikHBDynamicUP}{\rna}
\newcommand{\SLOWbatikHBDynamicUPCI}{\rna}
\newcommand{\SLOWbatikHBDynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikHBDynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikWCPUP}{\rna}
\newcommand{\SLOWbatikWCPUPCI}{\rna}
\newcommand{\SLOWbatikWCPUPCIMIN}{\rna}
\newcommand{\SLOWbatikWCPUPCIMAX}{\rna}
\newcommand{\SLOWbatikWCPDynamicUP}{\rna}
\newcommand{\SLOWbatikWCPDynamicUPCI}{\rna}
\newcommand{\SLOWbatikWCPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikWCPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikWDCnoGUP}{\rna}
\newcommand{\SLOWbatikWDCnoGUPCI}{\rna}
\newcommand{\SLOWbatikWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWbatikWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWbatikWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWbatikWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWbatikWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikWDCUP}{\rna}
\newcommand{\SLOWbatikWDCUPCI}{\rna}
\newcommand{\SLOWbatikWDCUPCIMIN}{\rna}
\newcommand{\SLOWbatikWDCUPCIMAX}{\rna}
\newcommand{\SLOWbatikWDCDynamicUP}{\rna}
\newcommand{\SLOWbatikWDCDynamicUPCI}{\rna}
\newcommand{\SLOWbatikWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGUP}{\rna}
\newcommand{\SLOWbatikCAPOnoGUPCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikCAPOUP}{\rna}
\newcommand{\SLOWbatikCAPOUPCI}{\rna}
\newcommand{\SLOWbatikCAPOUPCIMIN}{\rna}
\newcommand{\SLOWbatikCAPOUPCIMAX}{\rna}
\newcommand{\SLOWbatikCAPODynamicUP}{\rna}
\newcommand{\SLOWbatikCAPODynamicUPCI}{\rna}
\newcommand{\SLOWbatikCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPUP}{\rna}
\newcommand{\SLOWbatikPIPUPCI}{\rna}
\newcommand{\SLOWbatikPIPUPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPUPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPDynamicUP}{\rna}
\newcommand{\SLOWbatikPIPDynamicUPCI}{\rna}
\newcommand{\SLOWbatikPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPHB}{\rna}
\newcommand{\SLOWbatikPIPHBCI}{\rna}
\newcommand{\SLOWbatikPIPHBCIMIN}{\rna}
\newcommand{\SLOWbatikPIPHBCIMAX}{\rna}
\newcommand{\SLOWbatikPIPHBDynamic}{\rna}
\newcommand{\SLOWbatikPIPHBDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIPWCP}{\rna}
\newcommand{\SLOWbatikPIPWCPCI}{\rna}
\newcommand{\SLOWbatikPIPWCPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPWCPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPWCPDynamic}{\rna}
\newcommand{\SLOWbatikPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIPWDC}{\rna}
\newcommand{\SLOWbatikPIPWDCCI}{\rna}
\newcommand{\SLOWbatikPIPWDCCIMIN}{\rna}
\newcommand{\SLOWbatikPIPWDCCIMAX}{\rna}
\newcommand{\SLOWbatikPIPWDCDynamic}{\rna}
\newcommand{\SLOWbatikPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIPCAPO}{\rna}
\newcommand{\SLOWbatikPIPCAPOCI}{\rna}
\newcommand{\SLOWbatikPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWbatikPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWbatikPIPCAPODynamic}{\rna}
\newcommand{\SLOWbatikPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWbatikPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWbatikPIPPIP}{\rna}
\newcommand{\SLOWbatikPIPPIPCI}{\rna}
\newcommand{\SLOWbatikPIPPIPCIMIN}{\rna}
\newcommand{\SLOWbatikPIPPIPCIMAX}{\rna}
\newcommand{\SLOWbatikPIPPIPDynamic}{\rna}
\newcommand{\SLOWbatikPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWbatikPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWbatikPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoEvents}{3,800}
\newcommand{\SLOWhtwoNoFPEvents}{460}
\newcommand{\SLOWhtwoMaxLiveThreads}{9}
\newcommand{\SLOWhtwoTotalThreads}{10}
\newcommand{\SLOWhtwoBaseTime}{4.7}
\newcommand{\SLOWhtwoBaseTimeCI}{68}
\newcommand{\SLOWhtwoEmptyTime}{\rna}
\newcommand{\SLOWhtwoEmptyTimeCI}{\rna}
\newcommand{\SLOWhtwoEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoFTTime}{\rna}
\newcommand{\SLOWhtwoFTTimeCI}{\rna}
\newcommand{\SLOWhtwoFTTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoFTTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoHBTime}{27}
\newcommand{\SLOWhtwoHBTimeCI}{0.59}
\newcommand{\SLOWhtwoWCPTime}{77}
\newcommand{\SLOWhtwoWCPTimeCI}{4.9}
\newcommand{\SLOWhtwoDCnoGExcTime}{74}
\newcommand{\SLOWhtwoDCnoGExcTimeCI}{6.3}
\newcommand{\SLOWhtwoDCnoGTime}{\rna}
\newcommand{\SLOWhtwoDCnoGTimeCI}{\rna}
\newcommand{\SLOWhtwoDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoDCExcTime}{74}
\newcommand{\SLOWhtwoDCExcTimeCI}{3.8}
\newcommand{\SLOWhtwoDCTime}{\rna}
\newcommand{\SLOWhtwoDCTimeCI}{\rna}
\newcommand{\SLOWhtwoDCTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoDCTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGExcTime}{69}
\newcommand{\SLOWhtwoCAPOnoGExcTimeCI}{3.5}
\newcommand{\SLOWhtwoCAPOnoGTime}{\rna}
\newcommand{\SLOWhtwoCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOExcTime}{78}
\newcommand{\SLOWhtwoCAPOExcTimeCI}{4.6}
\newcommand{\SLOWhtwoCAPOTime}{\rna}
\newcommand{\SLOWhtwoCAPOTimeCI}{\rna}
\newcommand{\SLOWhtwoCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWhtwoStaticTime}{\rzero}
\newcommand{\SLOWhtwoDynamicTime}{\rzero}
\newcommand{\SLOWhtwoBaseMem}{1,800}
\newcommand{\SLOWhtwoBaseMemCI}{53.0}
\newcommand{\SLOWhtwoHBMem}{17}
\newcommand{\SLOWhtwoHBMemCI}{0.88}
\newcommand{\SLOWhtwoFTMem}{\memna}
\newcommand{\SLOWhtwoFTMemCI}{\memna}
\newcommand{\SLOWhtwoFTMemCIMIN}{\memna}
\newcommand{\SLOWhtwoFTMemCIMAX}{\memna}
\newcommand{\SLOWhtwoWCPMem}{61}
\newcommand{\SLOWhtwoWCPMemCI}{3.4}
\newcommand{\SLOWhtwoDCnoGExcMem}{54}
\newcommand{\SLOWhtwoDCnoGExcMemCI}{2.6}
\newcommand{\SLOWhtwoDCnoGMem}{\memna}
\newcommand{\SLOWhtwoDCnoGMemCI}{\memna}
\newcommand{\SLOWhtwoDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWhtwoDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWhtwoDCExcMem}{55}
\newcommand{\SLOWhtwoDCExcMemCI}{2.2}
\newcommand{\SLOWhtwoDCMem}{\memna}
\newcommand{\SLOWhtwoDCMemCI}{\memna}
\newcommand{\SLOWhtwoDCMemCIMIN}{\memna}
\newcommand{\SLOWhtwoDCMemCIMAX}{\memna}
\newcommand{\SLOWhtwoCAPOnoGExcMem}{54}
\newcommand{\SLOWhtwoCAPOnoGExcMemCI}{3.1}
\newcommand{\SLOWhtwoCAPOnoGMem}{\memna}
\newcommand{\SLOWhtwoCAPOnoGMemCI}{\memna}
\newcommand{\SLOWhtwoCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWhtwoCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWhtwoCAPOExcMem}{55}
\newcommand{\SLOWhtwoCAPOExcMemCI}{3.6}
\newcommand{\SLOWhtwoCAPOMem}{\memna}
\newcommand{\SLOWhtwoCAPOMemCI}{\memna}
\newcommand{\SLOWhtwoCAPOMemCIMIN}{\memna}
\newcommand{\SLOWhtwoCAPOMemCIMAX}{\memna}
\newcommand{\SLOWhtwoEventsCI}{1,191,230}
\newcommand{\SLOWhtwoEventsCIMIN}{3,801,486,163}
\newcommand{\SLOWhtwoEventsCIMAX}{3,803,868,623}
\newcommand{\SLOWhtwoNoFPEventsCI}{36,284}
\newcommand{\SLOWhtwoNoFPEventsCIMIN}{457,126,637}
\newcommand{\SLOWhtwoNoFPEventsCIMAX}{457,199,205}
\newcommand{\SLOWhtwoHB}{11}
\newcommand{\SLOWhtwoHBCI}{0}
\newcommand{\SLOWhtwoHBCIMIN}{11}
\newcommand{\SLOWhtwoHBCIMAX}{11}
\newcommand{\SLOWhtwoHBDynamic}{40,609}
\newcommand{\SLOWhtwoHBDynamicCI}{120}
\newcommand{\SLOWhtwoHBDynamicCIMIN}{40,489}
\newcommand{\SLOWhtwoHBDynamicCIMAX}{40,729}
\newcommand{\SLOWhtwoFT}{\rna}
\newcommand{\SLOWhtwoFTCI}{\rna}
\newcommand{\SLOWhtwoFTCIMIN}{\rna}
\newcommand{\SLOWhtwoFTCIMAX}{\rna}
\newcommand{\SLOWhtwoFTDynamic}{\rna}
\newcommand{\SLOWhtwoFTDynamicCI}{\rna}
\newcommand{\SLOWhtwoFTDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoFTDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoWCP}{11}
\newcommand{\SLOWhtwoWCPCI}{0}
\newcommand{\SLOWhtwoWCPCIMIN}{11}
\newcommand{\SLOWhtwoWCPCIMAX}{11}
\newcommand{\SLOWhtwoWCPDynamic}{41,053}
\newcommand{\SLOWhtwoWCPDynamicCI}{128}
\newcommand{\SLOWhtwoWCPDynamicCIMIN}{40,925}
\newcommand{\SLOWhtwoWCPDynamicCIMAX}{41,181}
\newcommand{\SLOWhtwoDCnoGExc}{11}
\newcommand{\SLOWhtwoDCnoGExcCI}{0}
\newcommand{\SLOWhtwoDCnoGExcCIMIN}{11}
\newcommand{\SLOWhtwoDCnoGExcCIMAX}{11}
\newcommand{\SLOWhtwoDCnoGExcDynamic}{41,382}
\newcommand{\SLOWhtwoDCnoGExcDynamicCI}{150}
\newcommand{\SLOWhtwoDCnoGExcDynamicCIMIN}{41,232}
\newcommand{\SLOWhtwoDCnoGExcDynamicCIMAX}{41,532}
\newcommand{\SLOWhtwoDCnoG}{\rna}
\newcommand{\SLOWhtwoDCnoGCI}{\rna}
\newcommand{\SLOWhtwoDCnoGCIMIN}{\rna}
\newcommand{\SLOWhtwoDCnoGCIMAX}{\rna}
\newcommand{\SLOWhtwoDCnoGDynamic}{\rna}
\newcommand{\SLOWhtwoDCnoGDynamicCI}{\rna}
\newcommand{\SLOWhtwoDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoDCExc}{11}
\newcommand{\SLOWhtwoDCExcCI}{0}
\newcommand{\SLOWhtwoDCExcCIMIN}{11}
\newcommand{\SLOWhtwoDCExcCIMAX}{11}
\newcommand{\SLOWhtwoDCExcDynamic}{41,392}
\newcommand{\SLOWhtwoDCExcDynamicCI}{71}
\newcommand{\SLOWhtwoDCExcDynamicCIMIN}{41,321}
\newcommand{\SLOWhtwoDCExcDynamicCIMAX}{41,463}
\newcommand{\SLOWhtwoDC}{\rna}
\newcommand{\SLOWhtwoDCCI}{\rna}
\newcommand{\SLOWhtwoDCCIMIN}{\rna}
\newcommand{\SLOWhtwoDCCIMAX}{\rna}
\newcommand{\SLOWhtwoDCDynamic}{\rna}
\newcommand{\SLOWhtwoDCDynamicCI}{\rna}
\newcommand{\SLOWhtwoDCDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoDCDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGExc}{11}
\newcommand{\SLOWhtwoCAPOnoGExcCI}{0}
\newcommand{\SLOWhtwoCAPOnoGExcCIMIN}{11}
\newcommand{\SLOWhtwoCAPOnoGExcCIMAX}{11}
\newcommand{\SLOWhtwoCAPOnoGExcDynamic}{41,444}
\newcommand{\SLOWhtwoCAPOnoGExcDynamicCI}{88}
\newcommand{\SLOWhtwoCAPOnoGExcDynamicCIMIN}{41,356}
\newcommand{\SLOWhtwoCAPOnoGExcDynamicCIMAX}{41,532}
\newcommand{\SLOWhtwoCAPOnoG}{\rna}
\newcommand{\SLOWhtwoCAPOnoGCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamic}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOExc}{11}
\newcommand{\SLOWhtwoCAPOExcCI}{0}
\newcommand{\SLOWhtwoCAPOExcCIMIN}{11}
\newcommand{\SLOWhtwoCAPOExcCIMAX}{11}
\newcommand{\SLOWhtwoCAPOExcDynamic}{41,429}
\newcommand{\SLOWhtwoCAPOExcDynamicCI}{86}
\newcommand{\SLOWhtwoCAPOExcDynamicCIMIN}{41,343}
\newcommand{\SLOWhtwoCAPOExcDynamicCIMAX}{41,515}
\newcommand{\SLOWhtwoCAPO}{\rna}
\newcommand{\SLOWhtwoCAPOCI}{\rna}
\newcommand{\SLOWhtwoCAPOCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPODynamic}{\rna}
\newcommand{\SLOWhtwoCAPODynamicCI}{\rna}
\newcommand{\SLOWhtwoCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIP}{\rna}
\newcommand{\SLOWhtwoPIPCI}{\rna}
\newcommand{\SLOWhtwoPIPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPDynamic}{\rna}
\newcommand{\SLOWhtwoPIPDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoHBUP}{\rna}
\newcommand{\SLOWhtwoHBUPCI}{\rna}
\newcommand{\SLOWhtwoHBUPCIMIN}{\rna}
\newcommand{\SLOWhtwoHBUPCIMAX}{\rna}
\newcommand{\SLOWhtwoHBDynamicUP}{\rna}
\newcommand{\SLOWhtwoHBDynamicUPCI}{\rna}
\newcommand{\SLOWhtwoHBDynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoHBDynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoWCPUP}{\rna}
\newcommand{\SLOWhtwoWCPUPCI}{\rna}
\newcommand{\SLOWhtwoWCPUPCIMIN}{\rna}
\newcommand{\SLOWhtwoWCPUPCIMAX}{\rna}
\newcommand{\SLOWhtwoWCPDynamicUP}{\rna}
\newcommand{\SLOWhtwoWCPDynamicUPCI}{\rna}
\newcommand{\SLOWhtwoWCPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoWCPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoWDCnoGUP}{\rna}
\newcommand{\SLOWhtwoWDCnoGUPCI}{\rna}
\newcommand{\SLOWhtwoWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWhtwoWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWhtwoWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWhtwoWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWhtwoWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoWDCUP}{\rna}
\newcommand{\SLOWhtwoWDCUPCI}{\rna}
\newcommand{\SLOWhtwoWDCUPCIMIN}{\rna}
\newcommand{\SLOWhtwoWDCUPCIMAX}{\rna}
\newcommand{\SLOWhtwoWDCDynamicUP}{\rna}
\newcommand{\SLOWhtwoWDCDynamicUPCI}{\rna}
\newcommand{\SLOWhtwoWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGUP}{\rna}
\newcommand{\SLOWhtwoCAPOnoGUPCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPOUP}{\rna}
\newcommand{\SLOWhtwoCAPOUPCI}{\rna}
\newcommand{\SLOWhtwoCAPOUPCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPOUPCIMAX}{\rna}
\newcommand{\SLOWhtwoCAPODynamicUP}{\rna}
\newcommand{\SLOWhtwoCAPODynamicUPCI}{\rna}
\newcommand{\SLOWhtwoCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPUP}{\rna}
\newcommand{\SLOWhtwoPIPUPCI}{\rna}
\newcommand{\SLOWhtwoPIPUPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPUPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPDynamicUP}{\rna}
\newcommand{\SLOWhtwoPIPDynamicUPCI}{\rna}
\newcommand{\SLOWhtwoPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPHB}{\rna}
\newcommand{\SLOWhtwoPIPHBCI}{\rna}
\newcommand{\SLOWhtwoPIPHBCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPHBCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPHBDynamic}{\rna}
\newcommand{\SLOWhtwoPIPHBDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPWCP}{\rna}
\newcommand{\SLOWhtwoPIPWCPCI}{\rna}
\newcommand{\SLOWhtwoPIPWCPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPWCPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPWCPDynamic}{\rna}
\newcommand{\SLOWhtwoPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPWDC}{\rna}
\newcommand{\SLOWhtwoPIPWDCCI}{\rna}
\newcommand{\SLOWhtwoPIPWDCCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPWDCCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPWDCDynamic}{\rna}
\newcommand{\SLOWhtwoPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPCAPO}{\rna}
\newcommand{\SLOWhtwoPIPCAPOCI}{\rna}
\newcommand{\SLOWhtwoPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPCAPODynamic}{\rna}
\newcommand{\SLOWhtwoPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPPIP}{\rna}
\newcommand{\SLOWhtwoPIPPIPCI}{\rna}
\newcommand{\SLOWhtwoPIPPIPCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPPIPCIMAX}{\rna}
\newcommand{\SLOWhtwoPIPPIPDynamic}{\rna}
\newcommand{\SLOWhtwoPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWhtwoPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWhtwoPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonEvents}{730}
\newcommand{\SLOWjythonNoFPEvents}{290}
\newcommand{\SLOWjythonMaxLiveThreads}{2}
\newcommand{\SLOWjythonTotalThreads}{2}
\newcommand{\SLOWjythonBaseTime}{3.8}
\newcommand{\SLOWjythonBaseTimeCI}{110}
\newcommand{\SLOWjythonEmptyTime}{\rna}
\newcommand{\SLOWjythonEmptyTimeCI}{\rna}
\newcommand{\SLOWjythonEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWjythonEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWjythonFTTime}{\rna}
\newcommand{\SLOWjythonFTTimeCI}{\rna}
\newcommand{\SLOWjythonFTTimeCIMIN}{\rna}
\newcommand{\SLOWjythonFTTimeCIMAX}{\rna}
\newcommand{\SLOWjythonHBTime}{23}
\newcommand{\SLOWjythonHBTimeCI}{0.58}
\newcommand{\SLOWjythonWCPTime}{33}
\newcommand{\SLOWjythonWCPTimeCI}{3.0}
\newcommand{\SLOWjythonDCnoGExcTime}{26}
\newcommand{\SLOWjythonDCnoGExcTimeCI}{0.89}
\newcommand{\SLOWjythonDCnoGTime}{\rna}
\newcommand{\SLOWjythonDCnoGTimeCI}{\rna}
\newcommand{\SLOWjythonDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWjythonDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWjythonDCExcTime}{31}
\newcommand{\SLOWjythonDCExcTimeCI}{0.84}
\newcommand{\SLOWjythonDCTime}{\rna}
\newcommand{\SLOWjythonDCTimeCI}{\rna}
\newcommand{\SLOWjythonDCTimeCIMIN}{\rna}
\newcommand{\SLOWjythonDCTimeCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGExcTime}{24}
\newcommand{\SLOWjythonCAPOnoGExcTimeCI}{0.59}
\newcommand{\SLOWjythonCAPOnoGTime}{\rna}
\newcommand{\SLOWjythonCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOExcTime}{28}
\newcommand{\SLOWjythonCAPOExcTimeCI}{0.76}
\newcommand{\SLOWjythonCAPOTime}{\rna}
\newcommand{\SLOWjythonCAPOTimeCI}{\rna}
\newcommand{\SLOWjythonCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWjythonStaticTime}{\rzero}
\newcommand{\SLOWjythonDynamicTime}{\rzero}
\newcommand{\SLOWjythonBaseMem}{760}
\newcommand{\SLOWjythonBaseMemCI}{6.7}
\newcommand{\SLOWjythonHBMem}{22}
\newcommand{\SLOWjythonHBMemCI}{0.55}
\newcommand{\SLOWjythonFTMem}{\memna}
\newcommand{\SLOWjythonFTMemCI}{\memna}
\newcommand{\SLOWjythonFTMemCIMIN}{\memna}
\newcommand{\SLOWjythonFTMemCIMAX}{\memna}
\newcommand{\SLOWjythonWCPMem}{21}
\newcommand{\SLOWjythonWCPMemCI}{0.74}
\newcommand{\SLOWjythonDCnoGExcMem}{18}
\newcommand{\SLOWjythonDCnoGExcMemCI}{0.37}
\newcommand{\SLOWjythonDCnoGMem}{\memna}
\newcommand{\SLOWjythonDCnoGMemCI}{\memna}
\newcommand{\SLOWjythonDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWjythonDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWjythonDCExcMem}{30}
\newcommand{\SLOWjythonDCExcMemCI}{0.51}
\newcommand{\SLOWjythonDCMem}{\memna}
\newcommand{\SLOWjythonDCMemCI}{\memna}
\newcommand{\SLOWjythonDCMemCIMIN}{\memna}
\newcommand{\SLOWjythonDCMemCIMAX}{\memna}
\newcommand{\SLOWjythonCAPOnoGExcMem}{17}
\newcommand{\SLOWjythonCAPOnoGExcMemCI}{0.51}
\newcommand{\SLOWjythonCAPOnoGMem}{\memna}
\newcommand{\SLOWjythonCAPOnoGMemCI}{\memna}
\newcommand{\SLOWjythonCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWjythonCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWjythonCAPOExcMem}{25}
\newcommand{\SLOWjythonCAPOExcMemCI}{0.37}
\newcommand{\SLOWjythonCAPOMem}{\memna}
\newcommand{\SLOWjythonCAPOMemCI}{\memna}
\newcommand{\SLOWjythonCAPOMemCIMIN}{\memna}
\newcommand{\SLOWjythonCAPOMemCIMAX}{\memna}
\newcommand{\SLOWjythonEventsCI}{368}
\newcommand{\SLOWjythonEventsCIMIN}{728,376,235}
\newcommand{\SLOWjythonEventsCIMAX}{728,376,971}
\newcommand{\SLOWjythonNoFPEventsCI}{13}
\newcommand{\SLOWjythonNoFPEventsCIMIN}{293,897,752}
\newcommand{\SLOWjythonNoFPEventsCIMAX}{293,897,778}
\newcommand{\SLOWjythonHB}{3}
\newcommand{\SLOWjythonHBCI}{0}
\newcommand{\SLOWjythonHBCIMIN}{3}
\newcommand{\SLOWjythonHBCIMAX}{3}
\newcommand{\SLOWjythonHBDynamic}{3}
\newcommand{\SLOWjythonHBDynamicCI}{0}
\newcommand{\SLOWjythonHBDynamicCIMIN}{3}
\newcommand{\SLOWjythonHBDynamicCIMAX}{3}
\newcommand{\SLOWjythonFT}{\rna}
\newcommand{\SLOWjythonFTCI}{\rna}
\newcommand{\SLOWjythonFTCIMIN}{\rna}
\newcommand{\SLOWjythonFTCIMAX}{\rna}
\newcommand{\SLOWjythonFTDynamic}{\rna}
\newcommand{\SLOWjythonFTDynamicCI}{\rna}
\newcommand{\SLOWjythonFTDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonFTDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonWCP}{3}
\newcommand{\SLOWjythonWCPCI}{0}
\newcommand{\SLOWjythonWCPCIMIN}{3}
\newcommand{\SLOWjythonWCPCIMAX}{3}
\newcommand{\SLOWjythonWCPDynamic}{4}
\newcommand{\SLOWjythonWCPDynamicCI}{0}
\newcommand{\SLOWjythonWCPDynamicCIMIN}{4}
\newcommand{\SLOWjythonWCPDynamicCIMAX}{4}
\newcommand{\SLOWjythonDCnoGExc}{4}
\newcommand{\SLOWjythonDCnoGExcCI}{1}
\newcommand{\SLOWjythonDCnoGExcCIMIN}{3}
\newcommand{\SLOWjythonDCnoGExcCIMAX}{5}
\newcommand{\SLOWjythonDCnoGExcDynamic}{5}
\newcommand{\SLOWjythonDCnoGExcDynamicCI}{1}
\newcommand{\SLOWjythonDCnoGExcDynamicCIMIN}{4}
\newcommand{\SLOWjythonDCnoGExcDynamicCIMAX}{6}
\newcommand{\SLOWjythonDCnoG}{\rna}
\newcommand{\SLOWjythonDCnoGCI}{\rna}
\newcommand{\SLOWjythonDCnoGCIMIN}{\rna}
\newcommand{\SLOWjythonDCnoGCIMAX}{\rna}
\newcommand{\SLOWjythonDCnoGDynamic}{\rna}
\newcommand{\SLOWjythonDCnoGDynamicCI}{\rna}
\newcommand{\SLOWjythonDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonDCExc}{2}
\newcommand{\SLOWjythonDCExcCI}{0}
\newcommand{\SLOWjythonDCExcCIMIN}{2}
\newcommand{\SLOWjythonDCExcCIMAX}{2}
\newcommand{\SLOWjythonDCExcDynamic}{4}
\newcommand{\SLOWjythonDCExcDynamicCI}{1}
\newcommand{\SLOWjythonDCExcDynamicCIMIN}{3}
\newcommand{\SLOWjythonDCExcDynamicCIMAX}{5}
\newcommand{\SLOWjythonDC}{\rna}
\newcommand{\SLOWjythonDCCI}{\rna}
\newcommand{\SLOWjythonDCCIMIN}{\rna}
\newcommand{\SLOWjythonDCCIMAX}{\rna}
\newcommand{\SLOWjythonDCDynamic}{\rna}
\newcommand{\SLOWjythonDCDynamicCI}{\rna}
\newcommand{\SLOWjythonDCDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonDCDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGExc}{3}
\newcommand{\SLOWjythonCAPOnoGExcCI}{1}
\newcommand{\SLOWjythonCAPOnoGExcCIMIN}{2}
\newcommand{\SLOWjythonCAPOnoGExcCIMAX}{4}
\newcommand{\SLOWjythonCAPOnoGExcDynamic}{5}
\newcommand{\SLOWjythonCAPOnoGExcDynamicCI}{1}
\newcommand{\SLOWjythonCAPOnoGExcDynamicCIMIN}{4}
\newcommand{\SLOWjythonCAPOnoGExcDynamicCIMAX}{6}
\newcommand{\SLOWjythonCAPOnoG}{\rna}
\newcommand{\SLOWjythonCAPOnoGCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamic}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOExc}{2}
\newcommand{\SLOWjythonCAPOExcCI}{0}
\newcommand{\SLOWjythonCAPOExcCIMIN}{2}
\newcommand{\SLOWjythonCAPOExcCIMAX}{2}
\newcommand{\SLOWjythonCAPOExcDynamic}{4}
\newcommand{\SLOWjythonCAPOExcDynamicCI}{1}
\newcommand{\SLOWjythonCAPOExcDynamicCIMIN}{3}
\newcommand{\SLOWjythonCAPOExcDynamicCIMAX}{5}
\newcommand{\SLOWjythonCAPO}{\rna}
\newcommand{\SLOWjythonCAPOCI}{\rna}
\newcommand{\SLOWjythonCAPOCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOCIMAX}{\rna}
\newcommand{\SLOWjythonCAPODynamic}{\rna}
\newcommand{\SLOWjythonCAPODynamicCI}{\rna}
\newcommand{\SLOWjythonCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWjythonCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIP}{\rna}
\newcommand{\SLOWjythonPIPCI}{\rna}
\newcommand{\SLOWjythonPIPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPDynamic}{\rna}
\newcommand{\SLOWjythonPIPDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonHBUP}{\rna}
\newcommand{\SLOWjythonHBUPCI}{\rna}
\newcommand{\SLOWjythonHBUPCIMIN}{\rna}
\newcommand{\SLOWjythonHBUPCIMAX}{\rna}
\newcommand{\SLOWjythonHBDynamicUP}{\rna}
\newcommand{\SLOWjythonHBDynamicUPCI}{\rna}
\newcommand{\SLOWjythonHBDynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonHBDynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonWCPUP}{\rna}
\newcommand{\SLOWjythonWCPUPCI}{\rna}
\newcommand{\SLOWjythonWCPUPCIMIN}{\rna}
\newcommand{\SLOWjythonWCPUPCIMAX}{\rna}
\newcommand{\SLOWjythonWCPDynamicUP}{\rna}
\newcommand{\SLOWjythonWCPDynamicUPCI}{\rna}
\newcommand{\SLOWjythonWCPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonWCPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonWDCnoGUP}{\rna}
\newcommand{\SLOWjythonWDCnoGUPCI}{\rna}
\newcommand{\SLOWjythonWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWjythonWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWjythonWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWjythonWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWjythonWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonWDCUP}{\rna}
\newcommand{\SLOWjythonWDCUPCI}{\rna}
\newcommand{\SLOWjythonWDCUPCIMIN}{\rna}
\newcommand{\SLOWjythonWDCUPCIMAX}{\rna}
\newcommand{\SLOWjythonWDCDynamicUP}{\rna}
\newcommand{\SLOWjythonWDCDynamicUPCI}{\rna}
\newcommand{\SLOWjythonWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGUP}{\rna}
\newcommand{\SLOWjythonCAPOnoGUPCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonCAPOUP}{\rna}
\newcommand{\SLOWjythonCAPOUPCI}{\rna}
\newcommand{\SLOWjythonCAPOUPCIMIN}{\rna}
\newcommand{\SLOWjythonCAPOUPCIMAX}{\rna}
\newcommand{\SLOWjythonCAPODynamicUP}{\rna}
\newcommand{\SLOWjythonCAPODynamicUPCI}{\rna}
\newcommand{\SLOWjythonCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPUP}{\rna}
\newcommand{\SLOWjythonPIPUPCI}{\rna}
\newcommand{\SLOWjythonPIPUPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPUPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPDynamicUP}{\rna}
\newcommand{\SLOWjythonPIPDynamicUPCI}{\rna}
\newcommand{\SLOWjythonPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPHB}{\rna}
\newcommand{\SLOWjythonPIPHBCI}{\rna}
\newcommand{\SLOWjythonPIPHBCIMIN}{\rna}
\newcommand{\SLOWjythonPIPHBCIMAX}{\rna}
\newcommand{\SLOWjythonPIPHBDynamic}{\rna}
\newcommand{\SLOWjythonPIPHBDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIPWCP}{\rna}
\newcommand{\SLOWjythonPIPWCPCI}{\rna}
\newcommand{\SLOWjythonPIPWCPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPWCPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPWCPDynamic}{\rna}
\newcommand{\SLOWjythonPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIPWDC}{\rna}
\newcommand{\SLOWjythonPIPWDCCI}{\rna}
\newcommand{\SLOWjythonPIPWDCCIMIN}{\rna}
\newcommand{\SLOWjythonPIPWDCCIMAX}{\rna}
\newcommand{\SLOWjythonPIPWDCDynamic}{\rna}
\newcommand{\SLOWjythonPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIPCAPO}{\rna}
\newcommand{\SLOWjythonPIPCAPOCI}{\rna}
\newcommand{\SLOWjythonPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWjythonPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWjythonPIPCAPODynamic}{\rna}
\newcommand{\SLOWjythonPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWjythonPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWjythonPIPPIP}{\rna}
\newcommand{\SLOWjythonPIPPIPCI}{\rna}
\newcommand{\SLOWjythonPIPPIPCIMIN}{\rna}
\newcommand{\SLOWjythonPIPPIPCIMAX}{\rna}
\newcommand{\SLOWjythonPIPPIPDynamic}{\rna}
\newcommand{\SLOWjythonPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWjythonPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWjythonPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexEvents}{400}
\newcommand{\SLOWluindexNoFPEvents}{45}
\newcommand{\SLOWluindexMaxLiveThreads}{3}
\newcommand{\SLOWluindexTotalThreads}{3}
\newcommand{\SLOWluindexBaseTime}{1.2}
\newcommand{\SLOWluindexBaseTimeCI}{59}
\newcommand{\SLOWluindexEmptyTime}{\rna}
\newcommand{\SLOWluindexEmptyTimeCI}{\rna}
\newcommand{\SLOWluindexEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWluindexEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWluindexFTTime}{\rna}
\newcommand{\SLOWluindexFTTimeCI}{\rna}
\newcommand{\SLOWluindexFTTimeCIMIN}{\rna}
\newcommand{\SLOWluindexFTTimeCIMAX}{\rna}
\newcommand{\SLOWluindexHBTime}{27}
\newcommand{\SLOWluindexHBTimeCI}{1.1}
\newcommand{\SLOWluindexWCPTime}{43}
\newcommand{\SLOWluindexWCPTimeCI}{1.7}
\newcommand{\SLOWluindexDCnoGExcTime}{36}
\newcommand{\SLOWluindexDCnoGExcTimeCI}{1.6}
\newcommand{\SLOWluindexDCnoGTime}{\rna}
\newcommand{\SLOWluindexDCnoGTimeCI}{\rna}
\newcommand{\SLOWluindexDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWluindexDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWluindexDCExcTime}{40}
\newcommand{\SLOWluindexDCExcTimeCI}{1.7}
\newcommand{\SLOWluindexDCTime}{\rna}
\newcommand{\SLOWluindexDCTimeCI}{\rna}
\newcommand{\SLOWluindexDCTimeCIMIN}{\rna}
\newcommand{\SLOWluindexDCTimeCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGExcTime}{36}
\newcommand{\SLOWluindexCAPOnoGExcTimeCI}{1.6}
\newcommand{\SLOWluindexCAPOnoGTime}{\rna}
\newcommand{\SLOWluindexCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOExcTime}{39}
\newcommand{\SLOWluindexCAPOExcTimeCI}{1.6}
\newcommand{\SLOWluindexCAPOTime}{\rna}
\newcommand{\SLOWluindexCAPOTimeCI}{\rna}
\newcommand{\SLOWluindexCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWluindexStaticTime}{\rzero}
\newcommand{\SLOWluindexDynamicTime}{\rzero}
\newcommand{\SLOWluindexBaseMem}{150}
\newcommand{\SLOWluindexBaseMemCI}{1.1}
\newcommand{\SLOWluindexHBMem}{29}
\newcommand{\SLOWluindexHBMemCI}{0.22}
\newcommand{\SLOWluindexFTMem}{\memna}
\newcommand{\SLOWluindexFTMemCI}{\memna}
\newcommand{\SLOWluindexFTMemCIMIN}{\memna}
\newcommand{\SLOWluindexFTMemCIMAX}{\memna}
\newcommand{\SLOWluindexWCPMem}{60}
\newcommand{\SLOWluindexWCPMemCI}{0.56}
\newcommand{\SLOWluindexDCnoGExcMem}{42}
\newcommand{\SLOWluindexDCnoGExcMemCI}{0.35}
\newcommand{\SLOWluindexDCnoGMem}{\memna}
\newcommand{\SLOWluindexDCnoGMemCI}{\memna}
\newcommand{\SLOWluindexDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWluindexDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWluindexDCExcMem}{50}
\newcommand{\SLOWluindexDCExcMemCI}{2.4}
\newcommand{\SLOWluindexDCMem}{\memna}
\newcommand{\SLOWluindexDCMemCI}{\memna}
\newcommand{\SLOWluindexDCMemCIMIN}{\memna}
\newcommand{\SLOWluindexDCMemCIMAX}{\memna}
\newcommand{\SLOWluindexCAPOnoGExcMem}{42}
\newcommand{\SLOWluindexCAPOnoGExcMemCI}{0.33}
\newcommand{\SLOWluindexCAPOnoGMem}{\memna}
\newcommand{\SLOWluindexCAPOnoGMemCI}{\memna}
\newcommand{\SLOWluindexCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWluindexCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWluindexCAPOExcMem}{47}
\newcommand{\SLOWluindexCAPOExcMemCI}{0.35}
\newcommand{\SLOWluindexCAPOMem}{\memna}
\newcommand{\SLOWluindexCAPOMemCI}{\memna}
\newcommand{\SLOWluindexCAPOMemCIMIN}{\memna}
\newcommand{\SLOWluindexCAPOMemCIMAX}{\memna}
\newcommand{\SLOWluindexEventsCI}{3}
\newcommand{\SLOWluindexEventsCIMIN}{396,268,394}
\newcommand{\SLOWluindexEventsCIMAX}{396,268,400}
\newcommand{\SLOWluindexNoFPEventsCI}{3}
\newcommand{\SLOWluindexNoFPEventsCIMIN}{45,411,630}
\newcommand{\SLOWluindexNoFPEventsCIMAX}{45,411,636}
\newcommand{\SLOWluindexHB}{1}
\newcommand{\SLOWluindexHBCI}{0}
\newcommand{\SLOWluindexHBCIMIN}{1}
\newcommand{\SLOWluindexHBCIMAX}{1}
\newcommand{\SLOWluindexHBDynamic}{1}
\newcommand{\SLOWluindexHBDynamicCI}{0}
\newcommand{\SLOWluindexHBDynamicCIMIN}{1}
\newcommand{\SLOWluindexHBDynamicCIMAX}{1}
\newcommand{\SLOWluindexFT}{\rna}
\newcommand{\SLOWluindexFTCI}{\rna}
\newcommand{\SLOWluindexFTCIMIN}{\rna}
\newcommand{\SLOWluindexFTCIMAX}{\rna}
\newcommand{\SLOWluindexFTDynamic}{\rna}
\newcommand{\SLOWluindexFTDynamicCI}{\rna}
\newcommand{\SLOWluindexFTDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexFTDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexWCP}{1}
\newcommand{\SLOWluindexWCPCI}{0}
\newcommand{\SLOWluindexWCPCIMIN}{1}
\newcommand{\SLOWluindexWCPCIMAX}{1}
\newcommand{\SLOWluindexWCPDynamic}{1}
\newcommand{\SLOWluindexWCPDynamicCI}{0}
\newcommand{\SLOWluindexWCPDynamicCIMIN}{1}
\newcommand{\SLOWluindexWCPDynamicCIMAX}{1}
\newcommand{\SLOWluindexDCnoGExc}{1}
\newcommand{\SLOWluindexDCnoGExcCI}{0}
\newcommand{\SLOWluindexDCnoGExcCIMIN}{1}
\newcommand{\SLOWluindexDCnoGExcCIMAX}{1}
\newcommand{\SLOWluindexDCnoGExcDynamic}{1}
\newcommand{\SLOWluindexDCnoGExcDynamicCI}{0}
\newcommand{\SLOWluindexDCnoGExcDynamicCIMIN}{1}
\newcommand{\SLOWluindexDCnoGExcDynamicCIMAX}{1}
\newcommand{\SLOWluindexDCnoG}{\rna}
\newcommand{\SLOWluindexDCnoGCI}{\rna}
\newcommand{\SLOWluindexDCnoGCIMIN}{\rna}
\newcommand{\SLOWluindexDCnoGCIMAX}{\rna}
\newcommand{\SLOWluindexDCnoGDynamic}{\rna}
\newcommand{\SLOWluindexDCnoGDynamicCI}{\rna}
\newcommand{\SLOWluindexDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexDCExc}{1}
\newcommand{\SLOWluindexDCExcCI}{0}
\newcommand{\SLOWluindexDCExcCIMIN}{1}
\newcommand{\SLOWluindexDCExcCIMAX}{1}
\newcommand{\SLOWluindexDCExcDynamic}{1}
\newcommand{\SLOWluindexDCExcDynamicCI}{0}
\newcommand{\SLOWluindexDCExcDynamicCIMIN}{1}
\newcommand{\SLOWluindexDCExcDynamicCIMAX}{1}
\newcommand{\SLOWluindexDC}{\rna}
\newcommand{\SLOWluindexDCCI}{\rna}
\newcommand{\SLOWluindexDCCIMIN}{\rna}
\newcommand{\SLOWluindexDCCIMAX}{\rna}
\newcommand{\SLOWluindexDCDynamic}{\rna}
\newcommand{\SLOWluindexDCDynamicCI}{\rna}
\newcommand{\SLOWluindexDCDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexDCDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGExc}{1}
\newcommand{\SLOWluindexCAPOnoGExcCI}{0}
\newcommand{\SLOWluindexCAPOnoGExcCIMIN}{1}
\newcommand{\SLOWluindexCAPOnoGExcCIMAX}{1}
\newcommand{\SLOWluindexCAPOnoGExcDynamic}{1}
\newcommand{\SLOWluindexCAPOnoGExcDynamicCI}{0}
\newcommand{\SLOWluindexCAPOnoGExcDynamicCIMIN}{1}
\newcommand{\SLOWluindexCAPOnoGExcDynamicCIMAX}{1}
\newcommand{\SLOWluindexCAPOnoG}{\rna}
\newcommand{\SLOWluindexCAPOnoGCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamic}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOExc}{1}
\newcommand{\SLOWluindexCAPOExcCI}{0}
\newcommand{\SLOWluindexCAPOExcCIMIN}{1}
\newcommand{\SLOWluindexCAPOExcCIMAX}{1}
\newcommand{\SLOWluindexCAPOExcDynamic}{1}
\newcommand{\SLOWluindexCAPOExcDynamicCI}{0}
\newcommand{\SLOWluindexCAPOExcDynamicCIMIN}{1}
\newcommand{\SLOWluindexCAPOExcDynamicCIMAX}{1}
\newcommand{\SLOWluindexCAPO}{\rna}
\newcommand{\SLOWluindexCAPOCI}{\rna}
\newcommand{\SLOWluindexCAPOCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOCIMAX}{\rna}
\newcommand{\SLOWluindexCAPODynamic}{\rna}
\newcommand{\SLOWluindexCAPODynamicCI}{\rna}
\newcommand{\SLOWluindexCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWluindexCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIP}{\rna}
\newcommand{\SLOWluindexPIPCI}{\rna}
\newcommand{\SLOWluindexPIPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPDynamic}{\rna}
\newcommand{\SLOWluindexPIPDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexHBUP}{\rna}
\newcommand{\SLOWluindexHBUPCI}{\rna}
\newcommand{\SLOWluindexHBUPCIMIN}{\rna}
\newcommand{\SLOWluindexHBUPCIMAX}{\rna}
\newcommand{\SLOWluindexHBDynamicUP}{\rna}
\newcommand{\SLOWluindexHBDynamicUPCI}{\rna}
\newcommand{\SLOWluindexHBDynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexHBDynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexWCPUP}{\rna}
\newcommand{\SLOWluindexWCPUPCI}{\rna}
\newcommand{\SLOWluindexWCPUPCIMIN}{\rna}
\newcommand{\SLOWluindexWCPUPCIMAX}{\rna}
\newcommand{\SLOWluindexWCPDynamicUP}{\rna}
\newcommand{\SLOWluindexWCPDynamicUPCI}{\rna}
\newcommand{\SLOWluindexWCPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexWCPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexWDCnoGUP}{\rna}
\newcommand{\SLOWluindexWDCnoGUPCI}{\rna}
\newcommand{\SLOWluindexWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWluindexWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWluindexWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWluindexWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWluindexWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexWDCUP}{\rna}
\newcommand{\SLOWluindexWDCUPCI}{\rna}
\newcommand{\SLOWluindexWDCUPCIMIN}{\rna}
\newcommand{\SLOWluindexWDCUPCIMAX}{\rna}
\newcommand{\SLOWluindexWDCDynamicUP}{\rna}
\newcommand{\SLOWluindexWDCDynamicUPCI}{\rna}
\newcommand{\SLOWluindexWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGUP}{\rna}
\newcommand{\SLOWluindexCAPOnoGUPCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexCAPOUP}{\rna}
\newcommand{\SLOWluindexCAPOUPCI}{\rna}
\newcommand{\SLOWluindexCAPOUPCIMIN}{\rna}
\newcommand{\SLOWluindexCAPOUPCIMAX}{\rna}
\newcommand{\SLOWluindexCAPODynamicUP}{\rna}
\newcommand{\SLOWluindexCAPODynamicUPCI}{\rna}
\newcommand{\SLOWluindexCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPUP}{\rna}
\newcommand{\SLOWluindexPIPUPCI}{\rna}
\newcommand{\SLOWluindexPIPUPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPUPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPDynamicUP}{\rna}
\newcommand{\SLOWluindexPIPDynamicUPCI}{\rna}
\newcommand{\SLOWluindexPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPHB}{\rna}
\newcommand{\SLOWluindexPIPHBCI}{\rna}
\newcommand{\SLOWluindexPIPHBCIMIN}{\rna}
\newcommand{\SLOWluindexPIPHBCIMAX}{\rna}
\newcommand{\SLOWluindexPIPHBDynamic}{\rna}
\newcommand{\SLOWluindexPIPHBDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIPWCP}{\rna}
\newcommand{\SLOWluindexPIPWCPCI}{\rna}
\newcommand{\SLOWluindexPIPWCPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPWCPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPWCPDynamic}{\rna}
\newcommand{\SLOWluindexPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIPWDC}{\rna}
\newcommand{\SLOWluindexPIPWDCCI}{\rna}
\newcommand{\SLOWluindexPIPWDCCIMIN}{\rna}
\newcommand{\SLOWluindexPIPWDCCIMAX}{\rna}
\newcommand{\SLOWluindexPIPWDCDynamic}{\rna}
\newcommand{\SLOWluindexPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIPCAPO}{\rna}
\newcommand{\SLOWluindexPIPCAPOCI}{\rna}
\newcommand{\SLOWluindexPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWluindexPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWluindexPIPCAPODynamic}{\rna}
\newcommand{\SLOWluindexPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWluindexPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWluindexPIPPIP}{\rna}
\newcommand{\SLOWluindexPIPPIPCI}{\rna}
\newcommand{\SLOWluindexPIPPIPCIMIN}{\rna}
\newcommand{\SLOWluindexPIPPIPCIMAX}{\rna}
\newcommand{\SLOWluindexPIPPIPDynamic}{\rna}
\newcommand{\SLOWluindexPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWluindexPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWluindexPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchEvents}{1,400}
\newcommand{\SLOWlusearchNoFPEvents}{190}
\newcommand{\SLOWlusearchMaxLiveThreads}{10}
\newcommand{\SLOWlusearchTotalThreads}{10}
\newcommand{\SLOWlusearchBaseTime}{0.96}
\newcommand{\SLOWlusearchBaseTimeCI}{83}
\newcommand{\SLOWlusearchEmptyTime}{\rna}
\newcommand{\SLOWlusearchEmptyTimeCI}{\rna}
\newcommand{\SLOWlusearchEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchFTTime}{\rna}
\newcommand{\SLOWlusearchFTTimeCI}{\rna}
\newcommand{\SLOWlusearchFTTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchFTTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchHBTime}{28}
\newcommand{\SLOWlusearchHBTimeCI}{2.6}
\newcommand{\SLOWlusearchWCPTime}{41}
\newcommand{\SLOWlusearchWCPTimeCI}{4.0}
\newcommand{\SLOWlusearchDCnoGExcTime}{30}
\newcommand{\SLOWlusearchDCnoGExcTimeCI}{2.8}
\newcommand{\SLOWlusearchDCnoGTime}{\rna}
\newcommand{\SLOWlusearchDCnoGTimeCI}{\rna}
\newcommand{\SLOWlusearchDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchDCExcTime}{36}
\newcommand{\SLOWlusearchDCExcTimeCI}{6.4}
\newcommand{\SLOWlusearchDCTime}{\rna}
\newcommand{\SLOWlusearchDCTimeCI}{\rna}
\newcommand{\SLOWlusearchDCTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchDCTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGExcTime}{29}
\newcommand{\SLOWlusearchCAPOnoGExcTimeCI}{2.4}
\newcommand{\SLOWlusearchCAPOnoGTime}{\rna}
\newcommand{\SLOWlusearchCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOExcTime}{33}
\newcommand{\SLOWlusearchCAPOExcTimeCI}{3.1}
\newcommand{\SLOWlusearchCAPOTime}{\rna}
\newcommand{\SLOWlusearchCAPOTimeCI}{\rna}
\newcommand{\SLOWlusearchCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWlusearchStaticTime}{\rzero}
\newcommand{\SLOWlusearchDynamicTime}{\rzero}
\newcommand{\SLOWlusearchBaseMem}{1,600}
\newcommand{\SLOWlusearchBaseMemCI}{11.0}
\newcommand{\SLOWlusearchHBMem}{14}
\newcommand{\SLOWlusearchHBMemCI}{0.51}
\newcommand{\SLOWlusearchFTMem}{\memna}
\newcommand{\SLOWlusearchFTMemCI}{\memna}
\newcommand{\SLOWlusearchFTMemCIMIN}{\memna}
\newcommand{\SLOWlusearchFTMemCIMAX}{\memna}
\newcommand{\SLOWlusearchWCPMem}{18}
\newcommand{\SLOWlusearchWCPMemCI}{0.59}
\newcommand{\SLOWlusearchDCnoGExcMem}{14}
\newcommand{\SLOWlusearchDCnoGExcMemCI}{0.35}
\newcommand{\SLOWlusearchDCnoGMem}{\memna}
\newcommand{\SLOWlusearchDCnoGMemCI}{\memna}
\newcommand{\SLOWlusearchDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWlusearchDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWlusearchDCExcMem}{15}
\newcommand{\SLOWlusearchDCExcMemCI}{0.54}
\newcommand{\SLOWlusearchDCMem}{\memna}
\newcommand{\SLOWlusearchDCMemCI}{\memna}
\newcommand{\SLOWlusearchDCMemCIMIN}{\memna}
\newcommand{\SLOWlusearchDCMemCIMAX}{\memna}
\newcommand{\SLOWlusearchCAPOnoGExcMem}{13}
\newcommand{\SLOWlusearchCAPOnoGExcMemCI}{0.59}
\newcommand{\SLOWlusearchCAPOnoGMem}{\memna}
\newcommand{\SLOWlusearchCAPOnoGMemCI}{\memna}
\newcommand{\SLOWlusearchCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWlusearchCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWlusearchCAPOExcMem}{15}
\newcommand{\SLOWlusearchCAPOExcMemCI}{0.49}
\newcommand{\SLOWlusearchCAPOMem}{\memna}
\newcommand{\SLOWlusearchCAPOMemCI}{\memna}
\newcommand{\SLOWlusearchCAPOMemCIMIN}{\memna}
\newcommand{\SLOWlusearchCAPOMemCIMAX}{\memna}
\newcommand{\SLOWlusearchEventsCI}{22}
\newcommand{\SLOWlusearchEventsCIMIN}{1,443,227,310}
\newcommand{\SLOWlusearchEventsCIMAX}{1,443,227,354}
\newcommand{\SLOWlusearchNoFPEventsCI}{22}
\newcommand{\SLOWlusearchNoFPEventsCIMIN}{194,058,140}
\newcommand{\SLOWlusearchNoFPEventsCIMAX}{194,058,184}
\newcommand{\SLOWlusearchHB}{0}
\newcommand{\SLOWlusearchHBCI}{0}
\newcommand{\SLOWlusearchHBCIMIN}{0}
\newcommand{\SLOWlusearchHBCIMAX}{0}
\newcommand{\SLOWlusearchHBDynamic}{0}
\newcommand{\SLOWlusearchHBDynamicCI}{0}
\newcommand{\SLOWlusearchHBDynamicCIMIN}{0}
\newcommand{\SLOWlusearchHBDynamicCIMAX}{0}
\newcommand{\SLOWlusearchFT}{\rna}
\newcommand{\SLOWlusearchFTCI}{\rna}
\newcommand{\SLOWlusearchFTCIMIN}{\rna}
\newcommand{\SLOWlusearchFTCIMAX}{\rna}
\newcommand{\SLOWlusearchFTDynamic}{\rna}
\newcommand{\SLOWlusearchFTDynamicCI}{\rna}
\newcommand{\SLOWlusearchFTDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchFTDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchWCP}{0}
\newcommand{\SLOWlusearchWCPCI}{0}
\newcommand{\SLOWlusearchWCPCIMIN}{0}
\newcommand{\SLOWlusearchWCPCIMAX}{0}
\newcommand{\SLOWlusearchWCPDynamic}{0}
\newcommand{\SLOWlusearchWCPDynamicCI}{0}
\newcommand{\SLOWlusearchWCPDynamicCIMIN}{0}
\newcommand{\SLOWlusearchWCPDynamicCIMAX}{0}
\newcommand{\SLOWlusearchDCnoGExc}{0}
\newcommand{\SLOWlusearchDCnoGExcCI}{0}
\newcommand{\SLOWlusearchDCnoGExcCIMIN}{0}
\newcommand{\SLOWlusearchDCnoGExcCIMAX}{0}
\newcommand{\SLOWlusearchDCnoGExcDynamic}{0}
\newcommand{\SLOWlusearchDCnoGExcDynamicCI}{0}
\newcommand{\SLOWlusearchDCnoGExcDynamicCIMIN}{0}
\newcommand{\SLOWlusearchDCnoGExcDynamicCIMAX}{0}
\newcommand{\SLOWlusearchDCnoG}{\rna}
\newcommand{\SLOWlusearchDCnoGCI}{\rna}
\newcommand{\SLOWlusearchDCnoGCIMIN}{\rna}
\newcommand{\SLOWlusearchDCnoGCIMAX}{\rna}
\newcommand{\SLOWlusearchDCnoGDynamic}{\rna}
\newcommand{\SLOWlusearchDCnoGDynamicCI}{\rna}
\newcommand{\SLOWlusearchDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchDCExc}{0}
\newcommand{\SLOWlusearchDCExcCI}{0}
\newcommand{\SLOWlusearchDCExcCIMIN}{0}
\newcommand{\SLOWlusearchDCExcCIMAX}{0}
\newcommand{\SLOWlusearchDCExcDynamic}{0}
\newcommand{\SLOWlusearchDCExcDynamicCI}{0}
\newcommand{\SLOWlusearchDCExcDynamicCIMIN}{0}
\newcommand{\SLOWlusearchDCExcDynamicCIMAX}{0}
\newcommand{\SLOWlusearchDC}{\rna}
\newcommand{\SLOWlusearchDCCI}{\rna}
\newcommand{\SLOWlusearchDCCIMIN}{\rna}
\newcommand{\SLOWlusearchDCCIMAX}{\rna}
\newcommand{\SLOWlusearchDCDynamic}{\rna}
\newcommand{\SLOWlusearchDCDynamicCI}{\rna}
\newcommand{\SLOWlusearchDCDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchDCDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGExc}{0}
\newcommand{\SLOWlusearchCAPOnoGExcCI}{0}
\newcommand{\SLOWlusearchCAPOnoGExcCIMIN}{0}
\newcommand{\SLOWlusearchCAPOnoGExcCIMAX}{0}
\newcommand{\SLOWlusearchCAPOnoGExcDynamic}{0}
\newcommand{\SLOWlusearchCAPOnoGExcDynamicCI}{0}
\newcommand{\SLOWlusearchCAPOnoGExcDynamicCIMIN}{0}
\newcommand{\SLOWlusearchCAPOnoGExcDynamicCIMAX}{0}
\newcommand{\SLOWlusearchCAPOnoG}{\rna}
\newcommand{\SLOWlusearchCAPOnoGCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamic}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOExc}{0}
\newcommand{\SLOWlusearchCAPOExcCI}{0}
\newcommand{\SLOWlusearchCAPOExcCIMIN}{0}
\newcommand{\SLOWlusearchCAPOExcCIMAX}{0}
\newcommand{\SLOWlusearchCAPOExcDynamic}{0}
\newcommand{\SLOWlusearchCAPOExcDynamicCI}{0}
\newcommand{\SLOWlusearchCAPOExcDynamicCIMIN}{0}
\newcommand{\SLOWlusearchCAPOExcDynamicCIMAX}{0}
\newcommand{\SLOWlusearchCAPO}{\rna}
\newcommand{\SLOWlusearchCAPOCI}{\rna}
\newcommand{\SLOWlusearchCAPOCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPODynamic}{\rna}
\newcommand{\SLOWlusearchCAPODynamicCI}{\rna}
\newcommand{\SLOWlusearchCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIP}{\rna}
\newcommand{\SLOWlusearchPIPCI}{\rna}
\newcommand{\SLOWlusearchPIPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPDynamic}{\rna}
\newcommand{\SLOWlusearchPIPDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchHBUP}{\rna}
\newcommand{\SLOWlusearchHBUPCI}{\rna}
\newcommand{\SLOWlusearchHBUPCIMIN}{\rna}
\newcommand{\SLOWlusearchHBUPCIMAX}{\rna}
\newcommand{\SLOWlusearchHBDynamicUP}{\rna}
\newcommand{\SLOWlusearchHBDynamicUPCI}{\rna}
\newcommand{\SLOWlusearchHBDynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchHBDynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchWCPUP}{\rna}
\newcommand{\SLOWlusearchWCPUPCI}{\rna}
\newcommand{\SLOWlusearchWCPUPCIMIN}{\rna}
\newcommand{\SLOWlusearchWCPUPCIMAX}{\rna}
\newcommand{\SLOWlusearchWCPDynamicUP}{\rna}
\newcommand{\SLOWlusearchWCPDynamicUPCI}{\rna}
\newcommand{\SLOWlusearchWCPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchWCPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchWDCnoGUP}{\rna}
\newcommand{\SLOWlusearchWDCnoGUPCI}{\rna}
\newcommand{\SLOWlusearchWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWlusearchWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWlusearchWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWlusearchWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWlusearchWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchWDCUP}{\rna}
\newcommand{\SLOWlusearchWDCUPCI}{\rna}
\newcommand{\SLOWlusearchWDCUPCIMIN}{\rna}
\newcommand{\SLOWlusearchWDCUPCIMAX}{\rna}
\newcommand{\SLOWlusearchWDCDynamicUP}{\rna}
\newcommand{\SLOWlusearchWDCDynamicUPCI}{\rna}
\newcommand{\SLOWlusearchWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGUP}{\rna}
\newcommand{\SLOWlusearchCAPOnoGUPCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPOUP}{\rna}
\newcommand{\SLOWlusearchCAPOUPCI}{\rna}
\newcommand{\SLOWlusearchCAPOUPCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPOUPCIMAX}{\rna}
\newcommand{\SLOWlusearchCAPODynamicUP}{\rna}
\newcommand{\SLOWlusearchCAPODynamicUPCI}{\rna}
\newcommand{\SLOWlusearchCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPUP}{\rna}
\newcommand{\SLOWlusearchPIPUPCI}{\rna}
\newcommand{\SLOWlusearchPIPUPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPUPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPDynamicUP}{\rna}
\newcommand{\SLOWlusearchPIPDynamicUPCI}{\rna}
\newcommand{\SLOWlusearchPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPHB}{\rna}
\newcommand{\SLOWlusearchPIPHBCI}{\rna}
\newcommand{\SLOWlusearchPIPHBCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPHBCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPHBDynamic}{\rna}
\newcommand{\SLOWlusearchPIPHBDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPWCP}{\rna}
\newcommand{\SLOWlusearchPIPWCPCI}{\rna}
\newcommand{\SLOWlusearchPIPWCPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPWCPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPWCPDynamic}{\rna}
\newcommand{\SLOWlusearchPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPWDC}{\rna}
\newcommand{\SLOWlusearchPIPWDCCI}{\rna}
\newcommand{\SLOWlusearchPIPWDCCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPWDCCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPWDCDynamic}{\rna}
\newcommand{\SLOWlusearchPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPCAPO}{\rna}
\newcommand{\SLOWlusearchPIPCAPOCI}{\rna}
\newcommand{\SLOWlusearchPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPCAPODynamic}{\rna}
\newcommand{\SLOWlusearchPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPPIP}{\rna}
\newcommand{\SLOWlusearchPIPPIPCI}{\rna}
\newcommand{\SLOWlusearchPIPPIPCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPPIPCIMAX}{\rna}
\newcommand{\SLOWlusearchPIPPIPDynamic}{\rna}
\newcommand{\SLOWlusearchPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWlusearchPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWlusearchPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdEvents}{200}
\newcommand{\SLOWpmdNoFPEvents}{25}
\newcommand{\SLOWpmdMaxLiveThreads}{9}
\newcommand{\SLOWpmdTotalThreads}{9}
\newcommand{\SLOWpmdBaseTime}{1.2}
\newcommand{\SLOWpmdBaseTimeCI}{15}
\newcommand{\SLOWpmdEmptyTime}{\rna}
\newcommand{\SLOWpmdEmptyTimeCI}{\rna}
\newcommand{\SLOWpmdEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWpmdEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWpmdFTTime}{\rna}
\newcommand{\SLOWpmdFTTimeCI}{\rna}
\newcommand{\SLOWpmdFTTimeCIMIN}{\rna}
\newcommand{\SLOWpmdFTTimeCIMAX}{\rna}
\newcommand{\SLOWpmdHBTime}{14}
\newcommand{\SLOWpmdHBTimeCI}{0.4}
\newcommand{\SLOWpmdWCPTime}{18}
\newcommand{\SLOWpmdWCPTimeCI}{0.83}
\newcommand{\SLOWpmdDCnoGExcTime}{15}
\newcommand{\SLOWpmdDCnoGExcTimeCI}{0.31}
\newcommand{\SLOWpmdDCnoGTime}{\rna}
\newcommand{\SLOWpmdDCnoGTimeCI}{\rna}
\newcommand{\SLOWpmdDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWpmdDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWpmdDCExcTime}{15}
\newcommand{\SLOWpmdDCExcTimeCI}{0.42}
\newcommand{\SLOWpmdDCTime}{\rna}
\newcommand{\SLOWpmdDCTimeCI}{\rna}
\newcommand{\SLOWpmdDCTimeCIMIN}{\rna}
\newcommand{\SLOWpmdDCTimeCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGExcTime}{15}
\newcommand{\SLOWpmdCAPOnoGExcTimeCI}{0.36}
\newcommand{\SLOWpmdCAPOnoGTime}{\rna}
\newcommand{\SLOWpmdCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOExcTime}{15}
\newcommand{\SLOWpmdCAPOExcTimeCI}{0.39}
\newcommand{\SLOWpmdCAPOTime}{\rna}
\newcommand{\SLOWpmdCAPOTimeCI}{\rna}
\newcommand{\SLOWpmdCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWpmdStaticTime}{\rzero}
\newcommand{\SLOWpmdDynamicTime}{\rzero}
\newcommand{\SLOWpmdBaseMem}{630}
\newcommand{\SLOWpmdBaseMemCI}{12.0}
\newcommand{\SLOWpmdHBMem}{11}
\newcommand{\SLOWpmdHBMemCI}{0.33}
\newcommand{\SLOWpmdFTMem}{\memna}
\newcommand{\SLOWpmdFTMemCI}{\memna}
\newcommand{\SLOWpmdFTMemCIMIN}{\memna}
\newcommand{\SLOWpmdFTMemCIMAX}{\memna}
\newcommand{\SLOWpmdWCPMem}{17}
\newcommand{\SLOWpmdWCPMemCI}{0.56}
\newcommand{\SLOWpmdDCnoGExcMem}{11}
\newcommand{\SLOWpmdDCnoGExcMemCI}{0.35}
\newcommand{\SLOWpmdDCnoGMem}{\memna}
\newcommand{\SLOWpmdDCnoGMemCI}{\memna}
\newcommand{\SLOWpmdDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWpmdDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWpmdDCExcMem}{12}
\newcommand{\SLOWpmdDCExcMemCI}{0.25}
\newcommand{\SLOWpmdDCMem}{\memna}
\newcommand{\SLOWpmdDCMemCI}{\memna}
\newcommand{\SLOWpmdDCMemCIMIN}{\memna}
\newcommand{\SLOWpmdDCMemCIMAX}{\memna}
\newcommand{\SLOWpmdCAPOnoGExcMem}{11}
\newcommand{\SLOWpmdCAPOnoGExcMemCI}{0.33}
\newcommand{\SLOWpmdCAPOnoGMem}{\memna}
\newcommand{\SLOWpmdCAPOnoGMemCI}{\memna}
\newcommand{\SLOWpmdCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWpmdCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWpmdCAPOExcMem}{12}
\newcommand{\SLOWpmdCAPOExcMemCI}{0.21}
\newcommand{\SLOWpmdCAPOMem}{\memna}
\newcommand{\SLOWpmdCAPOMemCI}{\memna}
\newcommand{\SLOWpmdCAPOMemCIMIN}{\memna}
\newcommand{\SLOWpmdCAPOMemCIMAX}{\memna}
\newcommand{\SLOWpmdEventsCI}{631}
\newcommand{\SLOWpmdEventsCIMIN}{200,052,280}
\newcommand{\SLOWpmdEventsCIMAX}{200,053,542}
\newcommand{\SLOWpmdNoFPEventsCI}{116}
\newcommand{\SLOWpmdNoFPEventsCIMIN}{25,405,240}
\newcommand{\SLOWpmdNoFPEventsCIMAX}{25,405,472}
\newcommand{\SLOWpmdHB}{4}
\newcommand{\SLOWpmdHBCI}{0}
\newcommand{\SLOWpmdHBCIMIN}{4}
\newcommand{\SLOWpmdHBCIMAX}{4}
\newcommand{\SLOWpmdHBDynamic}{21}
\newcommand{\SLOWpmdHBDynamicCI}{2}
\newcommand{\SLOWpmdHBDynamicCIMIN}{19}
\newcommand{\SLOWpmdHBDynamicCIMAX}{23}
\newcommand{\SLOWpmdFT}{\rna}
\newcommand{\SLOWpmdFTCI}{\rna}
\newcommand{\SLOWpmdFTCIMIN}{\rna}
\newcommand{\SLOWpmdFTCIMAX}{\rna}
\newcommand{\SLOWpmdFTDynamic}{\rna}
\newcommand{\SLOWpmdFTDynamicCI}{\rna}
\newcommand{\SLOWpmdFTDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdFTDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdWCP}{4}
\newcommand{\SLOWpmdWCPCI}{0}
\newcommand{\SLOWpmdWCPCIMIN}{4}
\newcommand{\SLOWpmdWCPCIMAX}{4}
\newcommand{\SLOWpmdWCPDynamic}{19}
\newcommand{\SLOWpmdWCPDynamicCI}{4}
\newcommand{\SLOWpmdWCPDynamicCIMIN}{15}
\newcommand{\SLOWpmdWCPDynamicCIMAX}{23}
\newcommand{\SLOWpmdDCnoGExc}{8}
\newcommand{\SLOWpmdDCnoGExcCI}{0}
\newcommand{\SLOWpmdDCnoGExcCIMIN}{8}
\newcommand{\SLOWpmdDCnoGExcCIMAX}{8}
\newcommand{\SLOWpmdDCnoGExcDynamic}{528}
\newcommand{\SLOWpmdDCnoGExcDynamicCI}{28}
\newcommand{\SLOWpmdDCnoGExcDynamicCIMIN}{500}
\newcommand{\SLOWpmdDCnoGExcDynamicCIMAX}{556}
\newcommand{\SLOWpmdDCnoG}{\rna}
\newcommand{\SLOWpmdDCnoGCI}{\rna}
\newcommand{\SLOWpmdDCnoGCIMIN}{\rna}
\newcommand{\SLOWpmdDCnoGCIMAX}{\rna}
\newcommand{\SLOWpmdDCnoGDynamic}{\rna}
\newcommand{\SLOWpmdDCnoGDynamicCI}{\rna}
\newcommand{\SLOWpmdDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdDCExc}{5}
\newcommand{\SLOWpmdDCExcCI}{0}
\newcommand{\SLOWpmdDCExcCIMIN}{5}
\newcommand{\SLOWpmdDCExcCIMAX}{5}
\newcommand{\SLOWpmdDCExcDynamic}{34}
\newcommand{\SLOWpmdDCExcDynamicCI}{2}
\newcommand{\SLOWpmdDCExcDynamicCIMIN}{32}
\newcommand{\SLOWpmdDCExcDynamicCIMAX}{36}
\newcommand{\SLOWpmdDC}{\rna}
\newcommand{\SLOWpmdDCCI}{\rna}
\newcommand{\SLOWpmdDCCIMIN}{\rna}
\newcommand{\SLOWpmdDCCIMAX}{\rna}
\newcommand{\SLOWpmdDCDynamic}{\rna}
\newcommand{\SLOWpmdDCDynamicCI}{\rna}
\newcommand{\SLOWpmdDCDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdDCDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGExc}{7}
\newcommand{\SLOWpmdCAPOnoGExcCI}{0}
\newcommand{\SLOWpmdCAPOnoGExcCIMIN}{7}
\newcommand{\SLOWpmdCAPOnoGExcCIMAX}{7}
\newcommand{\SLOWpmdCAPOnoGExcDynamic}{571}
\newcommand{\SLOWpmdCAPOnoGExcDynamicCI}{46}
\newcommand{\SLOWpmdCAPOnoGExcDynamicCIMIN}{525}
\newcommand{\SLOWpmdCAPOnoGExcDynamicCIMAX}{617}
\newcommand{\SLOWpmdCAPOnoG}{\rna}
\newcommand{\SLOWpmdCAPOnoGCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamic}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOExc}{5}
\newcommand{\SLOWpmdCAPOExcCI}{0}
\newcommand{\SLOWpmdCAPOExcCIMIN}{5}
\newcommand{\SLOWpmdCAPOExcCIMAX}{5}
\newcommand{\SLOWpmdCAPOExcDynamic}{34}
\newcommand{\SLOWpmdCAPOExcDynamicCI}{2}
\newcommand{\SLOWpmdCAPOExcDynamicCIMIN}{32}
\newcommand{\SLOWpmdCAPOExcDynamicCIMAX}{36}
\newcommand{\SLOWpmdCAPO}{\rna}
\newcommand{\SLOWpmdCAPOCI}{\rna}
\newcommand{\SLOWpmdCAPOCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOCIMAX}{\rna}
\newcommand{\SLOWpmdCAPODynamic}{\rna}
\newcommand{\SLOWpmdCAPODynamicCI}{\rna}
\newcommand{\SLOWpmdCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWpmdCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIP}{\rna}
\newcommand{\SLOWpmdPIPCI}{\rna}
\newcommand{\SLOWpmdPIPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPDynamic}{\rna}
\newcommand{\SLOWpmdPIPDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdHBUP}{\rna}
\newcommand{\SLOWpmdHBUPCI}{\rna}
\newcommand{\SLOWpmdHBUPCIMIN}{\rna}
\newcommand{\SLOWpmdHBUPCIMAX}{\rna}
\newcommand{\SLOWpmdHBDynamicUP}{\rna}
\newcommand{\SLOWpmdHBDynamicUPCI}{\rna}
\newcommand{\SLOWpmdHBDynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdHBDynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdWCPUP}{\rna}
\newcommand{\SLOWpmdWCPUPCI}{\rna}
\newcommand{\SLOWpmdWCPUPCIMIN}{\rna}
\newcommand{\SLOWpmdWCPUPCIMAX}{\rna}
\newcommand{\SLOWpmdWCPDynamicUP}{\rna}
\newcommand{\SLOWpmdWCPDynamicUPCI}{\rna}
\newcommand{\SLOWpmdWCPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdWCPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdWDCnoGUP}{\rna}
\newcommand{\SLOWpmdWDCnoGUPCI}{\rna}
\newcommand{\SLOWpmdWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWpmdWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWpmdWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWpmdWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWpmdWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdWDCUP}{\rna}
\newcommand{\SLOWpmdWDCUPCI}{\rna}
\newcommand{\SLOWpmdWDCUPCIMIN}{\rna}
\newcommand{\SLOWpmdWDCUPCIMAX}{\rna}
\newcommand{\SLOWpmdWDCDynamicUP}{\rna}
\newcommand{\SLOWpmdWDCDynamicUPCI}{\rna}
\newcommand{\SLOWpmdWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGUP}{\rna}
\newcommand{\SLOWpmdCAPOnoGUPCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdCAPOUP}{\rna}
\newcommand{\SLOWpmdCAPOUPCI}{\rna}
\newcommand{\SLOWpmdCAPOUPCIMIN}{\rna}
\newcommand{\SLOWpmdCAPOUPCIMAX}{\rna}
\newcommand{\SLOWpmdCAPODynamicUP}{\rna}
\newcommand{\SLOWpmdCAPODynamicUPCI}{\rna}
\newcommand{\SLOWpmdCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPUP}{\rna}
\newcommand{\SLOWpmdPIPUPCI}{\rna}
\newcommand{\SLOWpmdPIPUPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPUPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPDynamicUP}{\rna}
\newcommand{\SLOWpmdPIPDynamicUPCI}{\rna}
\newcommand{\SLOWpmdPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPHB}{\rna}
\newcommand{\SLOWpmdPIPHBCI}{\rna}
\newcommand{\SLOWpmdPIPHBCIMIN}{\rna}
\newcommand{\SLOWpmdPIPHBCIMAX}{\rna}
\newcommand{\SLOWpmdPIPHBDynamic}{\rna}
\newcommand{\SLOWpmdPIPHBDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIPWCP}{\rna}
\newcommand{\SLOWpmdPIPWCPCI}{\rna}
\newcommand{\SLOWpmdPIPWCPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPWCPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPWCPDynamic}{\rna}
\newcommand{\SLOWpmdPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIPWDC}{\rna}
\newcommand{\SLOWpmdPIPWDCCI}{\rna}
\newcommand{\SLOWpmdPIPWDCCIMIN}{\rna}
\newcommand{\SLOWpmdPIPWDCCIMAX}{\rna}
\newcommand{\SLOWpmdPIPWDCDynamic}{\rna}
\newcommand{\SLOWpmdPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIPCAPO}{\rna}
\newcommand{\SLOWpmdPIPCAPOCI}{\rna}
\newcommand{\SLOWpmdPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWpmdPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWpmdPIPCAPODynamic}{\rna}
\newcommand{\SLOWpmdPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWpmdPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWpmdPIPPIP}{\rna}
\newcommand{\SLOWpmdPIPPIPCI}{\rna}
\newcommand{\SLOWpmdPIPPIPCIMIN}{\rna}
\newcommand{\SLOWpmdPIPPIPCIMAX}{\rna}
\newcommand{\SLOWpmdPIPPIPDynamic}{\rna}
\newcommand{\SLOWpmdPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWpmdPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWpmdPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowEvents}{9,700}
\newcommand{\SLOWsunflowNoFPEvents}{760}
\newcommand{\SLOWsunflowMaxLiveThreads}{17}
\newcommand{\SLOWsunflowTotalThreads}{17}
\newcommand{\SLOWsunflowBaseTime}{1.7}
\newcommand{\SLOWsunflowBaseTimeCI}{93}
\newcommand{\SLOWsunflowEmptyTime}{\rna}
\newcommand{\SLOWsunflowEmptyTimeCI}{\rna}
\newcommand{\SLOWsunflowEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowFTTime}{\rna}
\newcommand{\SLOWsunflowFTTimeCI}{\rna}
\newcommand{\SLOWsunflowFTTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowFTTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowHBTime}{75}
\newcommand{\SLOWsunflowHBTimeCI}{8.7}
\newcommand{\SLOWsunflowWCPTime}{90}
\newcommand{\SLOWsunflowWCPTimeCI}{5.8}
\newcommand{\SLOWsunflowDCnoGExcTime}{74}
\newcommand{\SLOWsunflowDCnoGExcTimeCI}{13}
\newcommand{\SLOWsunflowDCnoGTime}{\rna}
\newcommand{\SLOWsunflowDCnoGTimeCI}{\rna}
\newcommand{\SLOWsunflowDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowDCExcTime}{77}
\newcommand{\SLOWsunflowDCExcTimeCI}{4.3}
\newcommand{\SLOWsunflowDCTime}{\rna}
\newcommand{\SLOWsunflowDCTimeCI}{\rna}
\newcommand{\SLOWsunflowDCTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowDCTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGExcTime}{70}
\newcommand{\SLOWsunflowCAPOnoGExcTimeCI}{4.0}
\newcommand{\SLOWsunflowCAPOnoGTime}{\rna}
\newcommand{\SLOWsunflowCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOExcTime}{82}
\newcommand{\SLOWsunflowCAPOExcTimeCI}{8.9}
\newcommand{\SLOWsunflowCAPOTime}{\rna}
\newcommand{\SLOWsunflowCAPOTimeCI}{\rna}
\newcommand{\SLOWsunflowCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWsunflowStaticTime}{\rzero}
\newcommand{\SLOWsunflowDynamicTime}{\rzero}
\newcommand{\SLOWsunflowBaseMem}{630}
\newcommand{\SLOWsunflowBaseMemCI}{0.86}
\newcommand{\SLOWsunflowHBMem}{25}
\newcommand{\SLOWsunflowHBMemCI}{0.94}
\newcommand{\SLOWsunflowFTMem}{\memna}
\newcommand{\SLOWsunflowFTMemCI}{\memna}
\newcommand{\SLOWsunflowFTMemCIMIN}{\memna}
\newcommand{\SLOWsunflowFTMemCIMAX}{\memna}
\newcommand{\SLOWsunflowWCPMem}{51}
\newcommand{\SLOWsunflowWCPMemCI}{0.81}
\newcommand{\SLOWsunflowDCnoGExcMem}{24}
\newcommand{\SLOWsunflowDCnoGExcMemCI}{0.84}
\newcommand{\SLOWsunflowDCnoGMem}{\memna}
\newcommand{\SLOWsunflowDCnoGMemCI}{\memna}
\newcommand{\SLOWsunflowDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWsunflowDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWsunflowDCExcMem}{27}
\newcommand{\SLOWsunflowDCExcMemCI}{0.51}
\newcommand{\SLOWsunflowDCMem}{\memna}
\newcommand{\SLOWsunflowDCMemCI}{\memna}
\newcommand{\SLOWsunflowDCMemCIMIN}{\memna}
\newcommand{\SLOWsunflowDCMemCIMAX}{\memna}
\newcommand{\SLOWsunflowCAPOnoGExcMem}{24}
\newcommand{\SLOWsunflowCAPOnoGExcMemCI}{0.41}
\newcommand{\SLOWsunflowCAPOnoGMem}{\memna}
\newcommand{\SLOWsunflowCAPOnoGMemCI}{\memna}
\newcommand{\SLOWsunflowCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWsunflowCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWsunflowCAPOExcMem}{25}
\newcommand{\SLOWsunflowCAPOExcMemCI}{0.64}
\newcommand{\SLOWsunflowCAPOMem}{\memna}
\newcommand{\SLOWsunflowCAPOMemCI}{\memna}
\newcommand{\SLOWsunflowCAPOMemCIMIN}{\memna}
\newcommand{\SLOWsunflowCAPOMemCIMAX}{\memna}
\newcommand{\SLOWsunflowEventsCI}{2}
\newcommand{\SLOWsunflowEventsCIMIN}{9,681,321,387}
\newcommand{\SLOWsunflowEventsCIMAX}{9,681,321,391}
\newcommand{\SLOWsunflowNoFPEventsCI}{7}
\newcommand{\SLOWsunflowNoFPEventsCIMIN}{764,388,867}
\newcommand{\SLOWsunflowNoFPEventsCIMAX}{764,388,881}
\newcommand{\SLOWsunflowHB}{2}
\newcommand{\SLOWsunflowHBCI}{0}
\newcommand{\SLOWsunflowHBCIMIN}{2}
\newcommand{\SLOWsunflowHBCIMAX}{2}
\newcommand{\SLOWsunflowHBDynamic}{8}
\newcommand{\SLOWsunflowHBDynamicCI}{0}
\newcommand{\SLOWsunflowHBDynamicCIMIN}{8}
\newcommand{\SLOWsunflowHBDynamicCIMAX}{8}
\newcommand{\SLOWsunflowFT}{\rna}
\newcommand{\SLOWsunflowFTCI}{\rna}
\newcommand{\SLOWsunflowFTCIMIN}{\rna}
\newcommand{\SLOWsunflowFTCIMAX}{\rna}
\newcommand{\SLOWsunflowFTDynamic}{\rna}
\newcommand{\SLOWsunflowFTDynamicCI}{\rna}
\newcommand{\SLOWsunflowFTDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowFTDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowWCP}{2}
\newcommand{\SLOWsunflowWCPCI}{0}
\newcommand{\SLOWsunflowWCPCIMIN}{2}
\newcommand{\SLOWsunflowWCPCIMAX}{2}
\newcommand{\SLOWsunflowWCPDynamic}{11}
\newcommand{\SLOWsunflowWCPDynamicCI}{2}
\newcommand{\SLOWsunflowWCPDynamicCIMIN}{9}
\newcommand{\SLOWsunflowWCPDynamicCIMAX}{13}
\newcommand{\SLOWsunflowDCnoGExc}{2}
\newcommand{\SLOWsunflowDCnoGExcCI}{0}
\newcommand{\SLOWsunflowDCnoGExcCIMIN}{2}
\newcommand{\SLOWsunflowDCnoGExcCIMAX}{2}
\newcommand{\SLOWsunflowDCnoGExcDynamic}{15}
\newcommand{\SLOWsunflowDCnoGExcDynamicCI}{0}
\newcommand{\SLOWsunflowDCnoGExcDynamicCIMIN}{15}
\newcommand{\SLOWsunflowDCnoGExcDynamicCIMAX}{15}
\newcommand{\SLOWsunflowDCnoG}{\rna}
\newcommand{\SLOWsunflowDCnoGCI}{\rna}
\newcommand{\SLOWsunflowDCnoGCIMIN}{\rna}
\newcommand{\SLOWsunflowDCnoGCIMAX}{\rna}
\newcommand{\SLOWsunflowDCnoGDynamic}{\rna}
\newcommand{\SLOWsunflowDCnoGDynamicCI}{\rna}
\newcommand{\SLOWsunflowDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowDCExc}{2}
\newcommand{\SLOWsunflowDCExcCI}{0}
\newcommand{\SLOWsunflowDCExcCIMIN}{2}
\newcommand{\SLOWsunflowDCExcCIMAX}{2}
\newcommand{\SLOWsunflowDCExcDynamic}{15}
\newcommand{\SLOWsunflowDCExcDynamicCI}{0}
\newcommand{\SLOWsunflowDCExcDynamicCIMIN}{15}
\newcommand{\SLOWsunflowDCExcDynamicCIMAX}{15}
\newcommand{\SLOWsunflowDC}{\rna}
\newcommand{\SLOWsunflowDCCI}{\rna}
\newcommand{\SLOWsunflowDCCIMIN}{\rna}
\newcommand{\SLOWsunflowDCCIMAX}{\rna}
\newcommand{\SLOWsunflowDCDynamic}{\rna}
\newcommand{\SLOWsunflowDCDynamicCI}{\rna}
\newcommand{\SLOWsunflowDCDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowDCDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGExc}{2}
\newcommand{\SLOWsunflowCAPOnoGExcCI}{0}
\newcommand{\SLOWsunflowCAPOnoGExcCIMIN}{2}
\newcommand{\SLOWsunflowCAPOnoGExcCIMAX}{2}
\newcommand{\SLOWsunflowCAPOnoGExcDynamic}{15}
\newcommand{\SLOWsunflowCAPOnoGExcDynamicCI}{0}
\newcommand{\SLOWsunflowCAPOnoGExcDynamicCIMIN}{15}
\newcommand{\SLOWsunflowCAPOnoGExcDynamicCIMAX}{15}
\newcommand{\SLOWsunflowCAPOnoG}{\rna}
\newcommand{\SLOWsunflowCAPOnoGCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamic}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOExc}{2}
\newcommand{\SLOWsunflowCAPOExcCI}{0}
\newcommand{\SLOWsunflowCAPOExcCIMIN}{2}
\newcommand{\SLOWsunflowCAPOExcCIMAX}{2}
\newcommand{\SLOWsunflowCAPOExcDynamic}{15}
\newcommand{\SLOWsunflowCAPOExcDynamicCI}{0}
\newcommand{\SLOWsunflowCAPOExcDynamicCIMIN}{15}
\newcommand{\SLOWsunflowCAPOExcDynamicCIMAX}{15}
\newcommand{\SLOWsunflowCAPO}{\rna}
\newcommand{\SLOWsunflowCAPOCI}{\rna}
\newcommand{\SLOWsunflowCAPOCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPODynamic}{\rna}
\newcommand{\SLOWsunflowCAPODynamicCI}{\rna}
\newcommand{\SLOWsunflowCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIP}{\rna}
\newcommand{\SLOWsunflowPIPCI}{\rna}
\newcommand{\SLOWsunflowPIPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPDynamic}{\rna}
\newcommand{\SLOWsunflowPIPDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowHBUP}{\rna}
\newcommand{\SLOWsunflowHBUPCI}{\rna}
\newcommand{\SLOWsunflowHBUPCIMIN}{\rna}
\newcommand{\SLOWsunflowHBUPCIMAX}{\rna}
\newcommand{\SLOWsunflowHBDynamicUP}{\rna}
\newcommand{\SLOWsunflowHBDynamicUPCI}{\rna}
\newcommand{\SLOWsunflowHBDynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowHBDynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowWCPUP}{\rna}
\newcommand{\SLOWsunflowWCPUPCI}{\rna}
\newcommand{\SLOWsunflowWCPUPCIMIN}{\rna}
\newcommand{\SLOWsunflowWCPUPCIMAX}{\rna}
\newcommand{\SLOWsunflowWCPDynamicUP}{\rna}
\newcommand{\SLOWsunflowWCPDynamicUPCI}{\rna}
\newcommand{\SLOWsunflowWCPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowWCPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowWDCnoGUP}{\rna}
\newcommand{\SLOWsunflowWDCnoGUPCI}{\rna}
\newcommand{\SLOWsunflowWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWsunflowWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWsunflowWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWsunflowWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWsunflowWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowWDCUP}{\rna}
\newcommand{\SLOWsunflowWDCUPCI}{\rna}
\newcommand{\SLOWsunflowWDCUPCIMIN}{\rna}
\newcommand{\SLOWsunflowWDCUPCIMAX}{\rna}
\newcommand{\SLOWsunflowWDCDynamicUP}{\rna}
\newcommand{\SLOWsunflowWDCDynamicUPCI}{\rna}
\newcommand{\SLOWsunflowWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGUP}{\rna}
\newcommand{\SLOWsunflowCAPOnoGUPCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPOUP}{\rna}
\newcommand{\SLOWsunflowCAPOUPCI}{\rna}
\newcommand{\SLOWsunflowCAPOUPCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPOUPCIMAX}{\rna}
\newcommand{\SLOWsunflowCAPODynamicUP}{\rna}
\newcommand{\SLOWsunflowCAPODynamicUPCI}{\rna}
\newcommand{\SLOWsunflowCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPUP}{\rna}
\newcommand{\SLOWsunflowPIPUPCI}{\rna}
\newcommand{\SLOWsunflowPIPUPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPUPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPDynamicUP}{\rna}
\newcommand{\SLOWsunflowPIPDynamicUPCI}{\rna}
\newcommand{\SLOWsunflowPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPHB}{\rna}
\newcommand{\SLOWsunflowPIPHBCI}{\rna}
\newcommand{\SLOWsunflowPIPHBCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPHBCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPHBDynamic}{\rna}
\newcommand{\SLOWsunflowPIPHBDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPWCP}{\rna}
\newcommand{\SLOWsunflowPIPWCPCI}{\rna}
\newcommand{\SLOWsunflowPIPWCPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPWCPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPWCPDynamic}{\rna}
\newcommand{\SLOWsunflowPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPWDC}{\rna}
\newcommand{\SLOWsunflowPIPWDCCI}{\rna}
\newcommand{\SLOWsunflowPIPWDCCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPWDCCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPWDCDynamic}{\rna}
\newcommand{\SLOWsunflowPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPCAPO}{\rna}
\newcommand{\SLOWsunflowPIPCAPOCI}{\rna}
\newcommand{\SLOWsunflowPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPCAPODynamic}{\rna}
\newcommand{\SLOWsunflowPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPPIP}{\rna}
\newcommand{\SLOWsunflowPIPPIPCI}{\rna}
\newcommand{\SLOWsunflowPIPPIPCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPPIPCIMAX}{\rna}
\newcommand{\SLOWsunflowPIPPIPDynamic}{\rna}
\newcommand{\SLOWsunflowPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWsunflowPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWsunflowPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatEvents}{47}
\newcommand{\SLOWtomcatNoFPEvents}{18}
\newcommand{\SLOWtomcatMaxLiveThreads}{28}
\newcommand{\SLOWtomcatTotalThreads}{35}
\newcommand{\SLOWtomcatBaseTime}{0.93}
\newcommand{\SLOWtomcatBaseTimeCI}{11}
\newcommand{\SLOWtomcatEmptyTime}{\rna}
\newcommand{\SLOWtomcatEmptyTimeCI}{\rna}
\newcommand{\SLOWtomcatEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatFTTime}{\rna}
\newcommand{\SLOWtomcatFTTimeCI}{\rna}
\newcommand{\SLOWtomcatFTTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatFTTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatHBTime}{9.0}
\newcommand{\SLOWtomcatHBTimeCI}{0.13}
\newcommand{\SLOWtomcatWCPTime}{12}
\newcommand{\SLOWtomcatWCPTimeCI}{0.29}
\newcommand{\SLOWtomcatDCnoGExcTime}{12}
\newcommand{\SLOWtomcatDCnoGExcTimeCI}{0.83}
\newcommand{\SLOWtomcatDCnoGTime}{\rna}
\newcommand{\SLOWtomcatDCnoGTimeCI}{\rna}
\newcommand{\SLOWtomcatDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatDCExcTime}{13}
\newcommand{\SLOWtomcatDCExcTimeCI}{0.75}
\newcommand{\SLOWtomcatDCTime}{\rna}
\newcommand{\SLOWtomcatDCTimeCI}{\rna}
\newcommand{\SLOWtomcatDCTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatDCTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGExcTime}{9.4}
\newcommand{\SLOWtomcatCAPOnoGExcTimeCI}{0.13}
\newcommand{\SLOWtomcatCAPOnoGTime}{\rna}
\newcommand{\SLOWtomcatCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOExcTime}{9.6}
\newcommand{\SLOWtomcatCAPOExcTimeCI}{0.26}
\newcommand{\SLOWtomcatCAPOTime}{\rna}
\newcommand{\SLOWtomcatCAPOTimeCI}{\rna}
\newcommand{\SLOWtomcatCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWtomcatStaticTime}{\rzero}
\newcommand{\SLOWtomcatDynamicTime}{\rzero}
\newcommand{\SLOWtomcatBaseMem}{510}
\newcommand{\SLOWtomcatBaseMemCI}{3.9}
\newcommand{\SLOWtomcatHBMem}{16}
\newcommand{\SLOWtomcatHBMemCI}{0.82}
\newcommand{\SLOWtomcatFTMem}{\memna}
\newcommand{\SLOWtomcatFTMemCI}{\memna}
\newcommand{\SLOWtomcatFTMemCIMIN}{\memna}
\newcommand{\SLOWtomcatFTMemCIMAX}{\memna}
\newcommand{\SLOWtomcatWCPMem}{22}
\newcommand{\SLOWtomcatWCPMemCI}{0.78}
\newcommand{\SLOWtomcatDCnoGExcMem}{22}
\newcommand{\SLOWtomcatDCnoGExcMemCI}{0.57}
\newcommand{\SLOWtomcatDCnoGMem}{\memna}
\newcommand{\SLOWtomcatDCnoGMemCI}{\memna}
\newcommand{\SLOWtomcatDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWtomcatDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWtomcatDCExcMem}{24}
\newcommand{\SLOWtomcatDCExcMemCI}{1.2}
\newcommand{\SLOWtomcatDCMem}{\memna}
\newcommand{\SLOWtomcatDCMemCI}{\memna}
\newcommand{\SLOWtomcatDCMemCIMIN}{\memna}
\newcommand{\SLOWtomcatDCMemCIMAX}{\memna}
\newcommand{\SLOWtomcatCAPOnoGExcMem}{18}
\newcommand{\SLOWtomcatCAPOnoGExcMemCI}{0.39}
\newcommand{\SLOWtomcatCAPOnoGMem}{\memna}
\newcommand{\SLOWtomcatCAPOnoGMemCI}{\memna}
\newcommand{\SLOWtomcatCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWtomcatCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWtomcatCAPOExcMem}{22}
\newcommand{\SLOWtomcatCAPOExcMemCI}{0.52}
\newcommand{\SLOWtomcatCAPOMem}{\memna}
\newcommand{\SLOWtomcatCAPOMemCI}{\memna}
\newcommand{\SLOWtomcatCAPOMemCIMIN}{\memna}
\newcommand{\SLOWtomcatCAPOMemCIMAX}{\memna}
\newcommand{\SLOWtomcatEventsCI}{44,311}
\newcommand{\SLOWtomcatEventsCIMIN}{46,955,082}
\newcommand{\SLOWtomcatEventsCIMAX}{47,043,704}
\newcommand{\SLOWtomcatNoFPEventsCI}{14,677}
\newcommand{\SLOWtomcatNoFPEventsCIMIN}{18,262,814}
\newcommand{\SLOWtomcatNoFPEventsCIMAX}{18,292,168}
\newcommand{\SLOWtomcatHB}{39}
\newcommand{\SLOWtomcatHBCI}{2}
\newcommand{\SLOWtomcatHBCIMIN}{37}
\newcommand{\SLOWtomcatHBCIMAX}{41}
\newcommand{\SLOWtomcatHBDynamic}{12,427}
\newcommand{\SLOWtomcatHBDynamicCI}{275}
\newcommand{\SLOWtomcatHBDynamicCIMIN}{12,152}
\newcommand{\SLOWtomcatHBDynamicCIMAX}{12,702}
\newcommand{\SLOWtomcatFT}{\rna}
\newcommand{\SLOWtomcatFTCI}{\rna}
\newcommand{\SLOWtomcatFTCIMIN}{\rna}
\newcommand{\SLOWtomcatFTCIMAX}{\rna}
\newcommand{\SLOWtomcatFTDynamic}{\rna}
\newcommand{\SLOWtomcatFTDynamicCI}{\rna}
\newcommand{\SLOWtomcatFTDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatFTDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatWCP}{41}
\newcommand{\SLOWtomcatWCPCI}{1}
\newcommand{\SLOWtomcatWCPCIMIN}{40}
\newcommand{\SLOWtomcatWCPCIMAX}{42}
\newcommand{\SLOWtomcatWCPDynamic}{11,820}
\newcommand{\SLOWtomcatWCPDynamicCI}{380}
\newcommand{\SLOWtomcatWCPDynamicCIMIN}{11,440}
\newcommand{\SLOWtomcatWCPDynamicCIMAX}{12,200}
\newcommand{\SLOWtomcatDCnoGExc}{69}
\newcommand{\SLOWtomcatDCnoGExcCI}{1}
\newcommand{\SLOWtomcatDCnoGExcCIMIN}{68}
\newcommand{\SLOWtomcatDCnoGExcCIMAX}{70}
\newcommand{\SLOWtomcatDCnoGExcDynamic}{26,983}
\newcommand{\SLOWtomcatDCnoGExcDynamicCI}{770}
\newcommand{\SLOWtomcatDCnoGExcDynamicCIMIN}{26,213}
\newcommand{\SLOWtomcatDCnoGExcDynamicCIMAX}{27,753}
\newcommand{\SLOWtomcatDCnoG}{\rna}
\newcommand{\SLOWtomcatDCnoGCI}{\rna}
\newcommand{\SLOWtomcatDCnoGCIMIN}{\rna}
\newcommand{\SLOWtomcatDCnoGCIMAX}{\rna}
\newcommand{\SLOWtomcatDCnoGDynamic}{\rna}
\newcommand{\SLOWtomcatDCnoGDynamicCI}{\rna}
\newcommand{\SLOWtomcatDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatDCExc}{47}
\newcommand{\SLOWtomcatDCExcCI}{0}
\newcommand{\SLOWtomcatDCExcCIMIN}{47}
\newcommand{\SLOWtomcatDCExcCIMAX}{47}
\newcommand{\SLOWtomcatDCExcDynamic}{12,432}
\newcommand{\SLOWtomcatDCExcDynamicCI}{351}
\newcommand{\SLOWtomcatDCExcDynamicCIMIN}{12,081}
\newcommand{\SLOWtomcatDCExcDynamicCIMAX}{12,783}
\newcommand{\SLOWtomcatDC}{\rna}
\newcommand{\SLOWtomcatDCCI}{\rna}
\newcommand{\SLOWtomcatDCCIMIN}{\rna}
\newcommand{\SLOWtomcatDCCIMAX}{\rna}
\newcommand{\SLOWtomcatDCDynamic}{\rna}
\newcommand{\SLOWtomcatDCDynamicCI}{\rna}
\newcommand{\SLOWtomcatDCDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatDCDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGExc}{65}
\newcommand{\SLOWtomcatCAPOnoGExcCI}{2}
\newcommand{\SLOWtomcatCAPOnoGExcCIMIN}{63}
\newcommand{\SLOWtomcatCAPOnoGExcCIMAX}{67}
\newcommand{\SLOWtomcatCAPOnoGExcDynamic}{27,112}
\newcommand{\SLOWtomcatCAPOnoGExcDynamicCI}{393}
\newcommand{\SLOWtomcatCAPOnoGExcDynamicCIMIN}{26,719}
\newcommand{\SLOWtomcatCAPOnoGExcDynamicCIMAX}{27,505}
\newcommand{\SLOWtomcatCAPOnoG}{\rna}
\newcommand{\SLOWtomcatCAPOnoGCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamic}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOExc}{47}
\newcommand{\SLOWtomcatCAPOExcCI}{1}
\newcommand{\SLOWtomcatCAPOExcCIMIN}{46}
\newcommand{\SLOWtomcatCAPOExcCIMAX}{48}
\newcommand{\SLOWtomcatCAPOExcDynamic}{13,106}
\newcommand{\SLOWtomcatCAPOExcDynamicCI}{196}
\newcommand{\SLOWtomcatCAPOExcDynamicCIMIN}{12,910}
\newcommand{\SLOWtomcatCAPOExcDynamicCIMAX}{13,302}
\newcommand{\SLOWtomcatCAPO}{\rna}
\newcommand{\SLOWtomcatCAPOCI}{\rna}
\newcommand{\SLOWtomcatCAPOCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPODynamic}{\rna}
\newcommand{\SLOWtomcatCAPODynamicCI}{\rna}
\newcommand{\SLOWtomcatCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIP}{\rna}
\newcommand{\SLOWtomcatPIPCI}{\rna}
\newcommand{\SLOWtomcatPIPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPDynamic}{\rna}
\newcommand{\SLOWtomcatPIPDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatHBUP}{\rna}
\newcommand{\SLOWtomcatHBUPCI}{\rna}
\newcommand{\SLOWtomcatHBUPCIMIN}{\rna}
\newcommand{\SLOWtomcatHBUPCIMAX}{\rna}
\newcommand{\SLOWtomcatHBDynamicUP}{\rna}
\newcommand{\SLOWtomcatHBDynamicUPCI}{\rna}
\newcommand{\SLOWtomcatHBDynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatHBDynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatWCPUP}{\rna}
\newcommand{\SLOWtomcatWCPUPCI}{\rna}
\newcommand{\SLOWtomcatWCPUPCIMIN}{\rna}
\newcommand{\SLOWtomcatWCPUPCIMAX}{\rna}
\newcommand{\SLOWtomcatWCPDynamicUP}{\rna}
\newcommand{\SLOWtomcatWCPDynamicUPCI}{\rna}
\newcommand{\SLOWtomcatWCPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatWCPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatWDCnoGUP}{\rna}
\newcommand{\SLOWtomcatWDCnoGUPCI}{\rna}
\newcommand{\SLOWtomcatWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWtomcatWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWtomcatWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWtomcatWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWtomcatWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatWDCUP}{\rna}
\newcommand{\SLOWtomcatWDCUPCI}{\rna}
\newcommand{\SLOWtomcatWDCUPCIMIN}{\rna}
\newcommand{\SLOWtomcatWDCUPCIMAX}{\rna}
\newcommand{\SLOWtomcatWDCDynamicUP}{\rna}
\newcommand{\SLOWtomcatWDCDynamicUPCI}{\rna}
\newcommand{\SLOWtomcatWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGUP}{\rna}
\newcommand{\SLOWtomcatCAPOnoGUPCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPOUP}{\rna}
\newcommand{\SLOWtomcatCAPOUPCI}{\rna}
\newcommand{\SLOWtomcatCAPOUPCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPOUPCIMAX}{\rna}
\newcommand{\SLOWtomcatCAPODynamicUP}{\rna}
\newcommand{\SLOWtomcatCAPODynamicUPCI}{\rna}
\newcommand{\SLOWtomcatCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPUP}{\rna}
\newcommand{\SLOWtomcatPIPUPCI}{\rna}
\newcommand{\SLOWtomcatPIPUPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPUPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPDynamicUP}{\rna}
\newcommand{\SLOWtomcatPIPDynamicUPCI}{\rna}
\newcommand{\SLOWtomcatPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPHB}{\rna}
\newcommand{\SLOWtomcatPIPHBCI}{\rna}
\newcommand{\SLOWtomcatPIPHBCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPHBCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPHBDynamic}{\rna}
\newcommand{\SLOWtomcatPIPHBDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPWCP}{\rna}
\newcommand{\SLOWtomcatPIPWCPCI}{\rna}
\newcommand{\SLOWtomcatPIPWCPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPWCPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPWCPDynamic}{\rna}
\newcommand{\SLOWtomcatPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPWDC}{\rna}
\newcommand{\SLOWtomcatPIPWDCCI}{\rna}
\newcommand{\SLOWtomcatPIPWDCCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPWDCCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPWDCDynamic}{\rna}
\newcommand{\SLOWtomcatPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPCAPO}{\rna}
\newcommand{\SLOWtomcatPIPCAPOCI}{\rna}
\newcommand{\SLOWtomcatPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPCAPODynamic}{\rna}
\newcommand{\SLOWtomcatPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPPIP}{\rna}
\newcommand{\SLOWtomcatPIPPIPCI}{\rna}
\newcommand{\SLOWtomcatPIPPIPCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPPIPCIMAX}{\rna}
\newcommand{\SLOWtomcatPIPPIPDynamic}{\rna}
\newcommand{\SLOWtomcatPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWtomcatPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWtomcatPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanEvents}{630}
\newcommand{\SLOWxalanNoFPEvents}{270}
\newcommand{\SLOWxalanMaxLiveThreads}{9}
\newcommand{\SLOWxalanTotalThreads}{9}
\newcommand{\SLOWxalanBaseTime}{2.0}
\newcommand{\SLOWxalanBaseTimeCI}{220}
\newcommand{\SLOWxalanEmptyTime}{\rna}
\newcommand{\SLOWxalanEmptyTimeCI}{\rna}
\newcommand{\SLOWxalanEmptyTimeCIMIN}{\rna}
\newcommand{\SLOWxalanEmptyTimeCIMAX}{\rna}
\newcommand{\SLOWxalanFTTime}{\rna}
\newcommand{\SLOWxalanFTTimeCI}{\rna}
\newcommand{\SLOWxalanFTTimeCIMIN}{\rna}
\newcommand{\SLOWxalanFTTimeCIMAX}{\rna}
\newcommand{\SLOWxalanHBTime}{15}
\newcommand{\SLOWxalanHBTimeCI}{3.7}
\newcommand{\SLOWxalanWCPTime}{40}
\newcommand{\SLOWxalanWCPTimeCI}{8.1}
\newcommand{\SLOWxalanDCnoGExcTime}{38}
\newcommand{\SLOWxalanDCnoGExcTimeCI}{6.7}
\newcommand{\SLOWxalanDCnoGTime}{\rna}
\newcommand{\SLOWxalanDCnoGTimeCI}{\rna}
\newcommand{\SLOWxalanDCnoGTimeCIMIN}{\rna}
\newcommand{\SLOWxalanDCnoGTimeCIMAX}{\rna}
\newcommand{\SLOWxalanDCExcTime}{60}
\newcommand{\SLOWxalanDCExcTimeCI}{11}
\newcommand{\SLOWxalanDCTime}{\rna}
\newcommand{\SLOWxalanDCTimeCI}{\rna}
\newcommand{\SLOWxalanDCTimeCIMIN}{\rna}
\newcommand{\SLOWxalanDCTimeCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGExcTime}{35}
\newcommand{\SLOWxalanCAPOnoGExcTimeCI}{6.4}
\newcommand{\SLOWxalanCAPOnoGTime}{\rna}
\newcommand{\SLOWxalanCAPOnoGTimeCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGTimeCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGTimeCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOExcTime}{49}
\newcommand{\SLOWxalanCAPOExcTimeCI}{9.8}
\newcommand{\SLOWxalanCAPOTime}{\rna}
\newcommand{\SLOWxalanCAPOTimeCI}{\rna}
\newcommand{\SLOWxalanCAPOTimeCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOTimeCIMAX}{\rna}
\newcommand{\SLOWxalanStaticTime}{\rzero}
\newcommand{\SLOWxalanDynamicTime}{\rzero}
\newcommand{\SLOWxalanBaseMem}{700}
\newcommand{\SLOWxalanBaseMemCI}{6.8}
\newcommand{\SLOWxalanHBMem}{22}
\newcommand{\SLOWxalanHBMemCI}{0.72}
\newcommand{\SLOWxalanFTMem}{\memna}
\newcommand{\SLOWxalanFTMemCI}{\memna}
\newcommand{\SLOWxalanFTMemCIMIN}{\memna}
\newcommand{\SLOWxalanFTMemCIMAX}{\memna}
\newcommand{\SLOWxalanWCPMem}{49}
\newcommand{\SLOWxalanWCPMemCI}{1.3}
\newcommand{\SLOWxalanDCnoGExcMem}{40}
\newcommand{\SLOWxalanDCnoGExcMemCI}{1.8}
\newcommand{\SLOWxalanDCnoGMem}{\memna}
\newcommand{\SLOWxalanDCnoGMemCI}{\memna}
\newcommand{\SLOWxalanDCnoGMemCIMIN}{\memna}
\newcommand{\SLOWxalanDCnoGMemCIMAX}{\memna}
\newcommand{\SLOWxalanDCExcMem}{60}
\newcommand{\SLOWxalanDCExcMemCI}{2.3}
\newcommand{\SLOWxalanDCMem}{\memna}
\newcommand{\SLOWxalanDCMemCI}{\memna}
\newcommand{\SLOWxalanDCMemCIMIN}{\memna}
\newcommand{\SLOWxalanDCMemCIMAX}{\memna}
\newcommand{\SLOWxalanCAPOnoGExcMem}{39}
\newcommand{\SLOWxalanCAPOnoGExcMemCI}{1.2}
\newcommand{\SLOWxalanCAPOnoGMem}{\memna}
\newcommand{\SLOWxalanCAPOnoGMemCI}{\memna}
\newcommand{\SLOWxalanCAPOnoGMemCIMIN}{\memna}
\newcommand{\SLOWxalanCAPOnoGMemCIMAX}{\memna}
\newcommand{\SLOWxalanCAPOExcMem}{56}
\newcommand{\SLOWxalanCAPOExcMemCI}{1.7}
\newcommand{\SLOWxalanCAPOMem}{\memna}
\newcommand{\SLOWxalanCAPOMemCI}{\memna}
\newcommand{\SLOWxalanCAPOMemCIMIN}{\memna}
\newcommand{\SLOWxalanCAPOMemCIMAX}{\memna}
\newcommand{\SLOWxalanEventsCI}{43}
\newcommand{\SLOWxalanEventsCIMIN}{626,353,783}
\newcommand{\SLOWxalanEventsCIMAX}{626,353,869}
\newcommand{\SLOWxalanNoFPEventsCI}{38}
\newcommand{\SLOWxalanNoFPEventsCIMIN}{273,861,897}
\newcommand{\SLOWxalanNoFPEventsCIMAX}{273,861,973}
\newcommand{\SLOWxalanHB}{3}
\newcommand{\SLOWxalanHBCI}{0}
\newcommand{\SLOWxalanHBCIMIN}{3}
\newcommand{\SLOWxalanHBCIMAX}{3}
\newcommand{\SLOWxalanHBDynamic}{17}
\newcommand{\SLOWxalanHBDynamicCI}{0}
\newcommand{\SLOWxalanHBDynamicCIMIN}{17}
\newcommand{\SLOWxalanHBDynamicCIMAX}{17}
\newcommand{\SLOWxalanFT}{\rna}
\newcommand{\SLOWxalanFTCI}{\rna}
\newcommand{\SLOWxalanFTCIMIN}{\rna}
\newcommand{\SLOWxalanFTCIMAX}{\rna}
\newcommand{\SLOWxalanFTDynamic}{\rna}
\newcommand{\SLOWxalanFTDynamicCI}{\rna}
\newcommand{\SLOWxalanFTDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanFTDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanWCP}{5}
\newcommand{\SLOWxalanWCPCI}{0}
\newcommand{\SLOWxalanWCPCIMIN}{5}
\newcommand{\SLOWxalanWCPCIMAX}{5}
\newcommand{\SLOWxalanWCPDynamic}{238,858}
\newcommand{\SLOWxalanWCPDynamicCI}{2,092}
\newcommand{\SLOWxalanWCPDynamicCIMIN}{236,766}
\newcommand{\SLOWxalanWCPDynamicCIMAX}{240,950}
\newcommand{\SLOWxalanDCnoGExc}{10}
\newcommand{\SLOWxalanDCnoGExcCI}{0}
\newcommand{\SLOWxalanDCnoGExcCIMIN}{10}
\newcommand{\SLOWxalanDCnoGExcCIMAX}{10}
\newcommand{\SLOWxalanDCnoGExcDynamic}{413,420}
\newcommand{\SLOWxalanDCnoGExcDynamicCI}{3,277}
\newcommand{\SLOWxalanDCnoGExcDynamicCIMIN}{410,143}
\newcommand{\SLOWxalanDCnoGExcDynamicCIMAX}{416,697}
\newcommand{\SLOWxalanDCnoG}{\rna}
\newcommand{\SLOWxalanDCnoGCI}{\rna}
\newcommand{\SLOWxalanDCnoGCIMIN}{\rna}
\newcommand{\SLOWxalanDCnoGCIMAX}{\rna}
\newcommand{\SLOWxalanDCnoGDynamic}{\rna}
\newcommand{\SLOWxalanDCnoGDynamicCI}{\rna}
\newcommand{\SLOWxalanDCnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanDCnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanDCExc}{6}
\newcommand{\SLOWxalanDCExcCI}{0}
\newcommand{\SLOWxalanDCExcCIMIN}{6}
\newcommand{\SLOWxalanDCExcCIMAX}{6}
\newcommand{\SLOWxalanDCExcDynamic}{261,709}
\newcommand{\SLOWxalanDCExcDynamicCI}{1,155}
\newcommand{\SLOWxalanDCExcDynamicCIMIN}{260,554}
\newcommand{\SLOWxalanDCExcDynamicCIMAX}{262,864}
\newcommand{\SLOWxalanDC}{\rna}
\newcommand{\SLOWxalanDCCI}{\rna}
\newcommand{\SLOWxalanDCCIMIN}{\rna}
\newcommand{\SLOWxalanDCCIMAX}{\rna}
\newcommand{\SLOWxalanDCDynamic}{\rna}
\newcommand{\SLOWxalanDCDynamicCI}{\rna}
\newcommand{\SLOWxalanDCDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanDCDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGExc}{10}
\newcommand{\SLOWxalanCAPOnoGExcCI}{0}
\newcommand{\SLOWxalanCAPOnoGExcCIMIN}{10}
\newcommand{\SLOWxalanCAPOnoGExcCIMAX}{10}
\newcommand{\SLOWxalanCAPOnoGExcDynamic}{410,492}
\newcommand{\SLOWxalanCAPOnoGExcDynamicCI}{2,123}
\newcommand{\SLOWxalanCAPOnoGExcDynamicCIMIN}{408,369}
\newcommand{\SLOWxalanCAPOnoGExcDynamicCIMAX}{412,615}
\newcommand{\SLOWxalanCAPOnoG}{\rna}
\newcommand{\SLOWxalanCAPOnoGCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamic}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOExc}{6}
\newcommand{\SLOWxalanCAPOExcCI}{0}
\newcommand{\SLOWxalanCAPOExcCIMIN}{6}
\newcommand{\SLOWxalanCAPOExcCIMAX}{6}
\newcommand{\SLOWxalanCAPOExcDynamic}{260,879}
\newcommand{\SLOWxalanCAPOExcDynamicCI}{235}
\newcommand{\SLOWxalanCAPOExcDynamicCIMIN}{260,644}
\newcommand{\SLOWxalanCAPOExcDynamicCIMAX}{261,114}
\newcommand{\SLOWxalanCAPO}{\rna}
\newcommand{\SLOWxalanCAPOCI}{\rna}
\newcommand{\SLOWxalanCAPOCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOCIMAX}{\rna}
\newcommand{\SLOWxalanCAPODynamic}{\rna}
\newcommand{\SLOWxalanCAPODynamicCI}{\rna}
\newcommand{\SLOWxalanCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWxalanCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIP}{\rna}
\newcommand{\SLOWxalanPIPCI}{\rna}
\newcommand{\SLOWxalanPIPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPDynamic}{\rna}
\newcommand{\SLOWxalanPIPDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanHBUP}{\rna}
\newcommand{\SLOWxalanHBUPCI}{\rna}
\newcommand{\SLOWxalanHBUPCIMIN}{\rna}
\newcommand{\SLOWxalanHBUPCIMAX}{\rna}
\newcommand{\SLOWxalanHBDynamicUP}{\rna}
\newcommand{\SLOWxalanHBDynamicUPCI}{\rna}
\newcommand{\SLOWxalanHBDynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanHBDynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanWCPUP}{\rna}
\newcommand{\SLOWxalanWCPUPCI}{\rna}
\newcommand{\SLOWxalanWCPUPCIMIN}{\rna}
\newcommand{\SLOWxalanWCPUPCIMAX}{\rna}
\newcommand{\SLOWxalanWCPDynamicUP}{\rna}
\newcommand{\SLOWxalanWCPDynamicUPCI}{\rna}
\newcommand{\SLOWxalanWCPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanWCPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanWDCnoGUP}{\rna}
\newcommand{\SLOWxalanWDCnoGUPCI}{\rna}
\newcommand{\SLOWxalanWDCnoGUPCIMIN}{\rna}
\newcommand{\SLOWxalanWDCnoGUPCIMAX}{\rna}
\newcommand{\SLOWxalanWDCnoGDynamicUP}{\rna}
\newcommand{\SLOWxalanWDCnoGDynamicUPCI}{\rna}
\newcommand{\SLOWxalanWDCnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanWDCnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanWDCUP}{\rna}
\newcommand{\SLOWxalanWDCUPCI}{\rna}
\newcommand{\SLOWxalanWDCUPCIMIN}{\rna}
\newcommand{\SLOWxalanWDCUPCIMAX}{\rna}
\newcommand{\SLOWxalanWDCDynamicUP}{\rna}
\newcommand{\SLOWxalanWDCDynamicUPCI}{\rna}
\newcommand{\SLOWxalanWDCDynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanWDCDynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGUP}{\rna}
\newcommand{\SLOWxalanCAPOnoGUPCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGUPCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGUPCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicUP}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicUPCI}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOnoGDynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanCAPOUP}{\rna}
\newcommand{\SLOWxalanCAPOUPCI}{\rna}
\newcommand{\SLOWxalanCAPOUPCIMIN}{\rna}
\newcommand{\SLOWxalanCAPOUPCIMAX}{\rna}
\newcommand{\SLOWxalanCAPODynamicUP}{\rna}
\newcommand{\SLOWxalanCAPODynamicUPCI}{\rna}
\newcommand{\SLOWxalanCAPODynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanCAPODynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPUP}{\rna}
\newcommand{\SLOWxalanPIPUPCI}{\rna}
\newcommand{\SLOWxalanPIPUPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPUPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPDynamicUP}{\rna}
\newcommand{\SLOWxalanPIPDynamicUPCI}{\rna}
\newcommand{\SLOWxalanPIPDynamicUPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPDynamicUPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPHB}{\rna}
\newcommand{\SLOWxalanPIPHBCI}{\rna}
\newcommand{\SLOWxalanPIPHBCIMIN}{\rna}
\newcommand{\SLOWxalanPIPHBCIMAX}{\rna}
\newcommand{\SLOWxalanPIPHBDynamic}{\rna}
\newcommand{\SLOWxalanPIPHBDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPHBDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPHBDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIPWCP}{\rna}
\newcommand{\SLOWxalanPIPWCPCI}{\rna}
\newcommand{\SLOWxalanPIPWCPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPWCPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPWCPDynamic}{\rna}
\newcommand{\SLOWxalanPIPWCPDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPWCPDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPWCPDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIPWDC}{\rna}
\newcommand{\SLOWxalanPIPWDCCI}{\rna}
\newcommand{\SLOWxalanPIPWDCCIMIN}{\rna}
\newcommand{\SLOWxalanPIPWDCCIMAX}{\rna}
\newcommand{\SLOWxalanPIPWDCDynamic}{\rna}
\newcommand{\SLOWxalanPIPWDCDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPWDCDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPWDCDynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIPCAPO}{\rna}
\newcommand{\SLOWxalanPIPCAPOCI}{\rna}
\newcommand{\SLOWxalanPIPCAPOCIMIN}{\rna}
\newcommand{\SLOWxalanPIPCAPOCIMAX}{\rna}
\newcommand{\SLOWxalanPIPCAPODynamic}{\rna}
\newcommand{\SLOWxalanPIPCAPODynamicCI}{\rna}
\newcommand{\SLOWxalanPIPCAPODynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPCAPODynamicCIMAX}{\rna}
\newcommand{\SLOWxalanPIPPIP}{\rna}
\newcommand{\SLOWxalanPIPPIPCI}{\rna}
\newcommand{\SLOWxalanPIPPIPCIMIN}{\rna}
\newcommand{\SLOWxalanPIPPIPCIMAX}{\rna}
\newcommand{\SLOWxalanPIPPIPDynamic}{\rna}
\newcommand{\SLOWxalanPIPPIPDynamicCI}{\rna}
\newcommand{\SLOWxalanPIPPIPDynamicCIMIN}{\rna}
\newcommand{\SLOWxalanPIPPIPDynamicCIMAX}{\rna}
\newcommand{\SLOWBaseTimeGeoMean}{1800}
\newcommand{\SLOWEmptyTimeGeoMean}{\rna}
\newcommand{\SLOWFTTimeGeoMean}{\rna}
\newcommand{\SLOWHBTimeGeoMean}{20}
\newcommand{\SLOWWCPTimeGeoMean}{32}
\newcommand{\SLOWDCnoGExcTimeGeoMean}{27}
\newcommand{\SLOWDCnoGTimeGeoMean}{\rna}
\newcommand{\SLOWDCExcTimeGeoMean}{31}
\newcommand{\SLOWDCTimeGeoMean}{\rna}
\newcommand{\SLOWCAPOnoGExcTimeGeoMean}{25}
\newcommand{\SLOWCAPOnoGTimeGeoMean}{\rna}
\newcommand{\SLOWCAPOExcTimeGeoMean}{29}
\newcommand{\SLOWCAPOTimeGeoMean}{\rna}
\newcommand{\SLOWBaseMemGeoMean}{540}
\newcommand{\SLOWEmptyMemGeoMean}{0.0}
\newcommand{\SLOWFTMemGeoMean}{\memna}
\newcommand{\SLOWHBMemGeoMean}{20}
\newcommand{\SLOWWCPMemGeoMean}{37}
\newcommand{\SLOWDCnoGExcMemGeoMean}{26}
\newcommand{\SLOWDCnoGMemGeoMean}{\memna}
\newcommand{\SLOWDCExcMemGeoMean}{33}
\newcommand{\SLOWDCMemGeoMean}{\memna}
\newcommand{\SLOWCAPOnoGExcMemGeoMean}{25}
\newcommand{\SLOWCAPOnoGMemGeoMean}{\memna}
\newcommand{\SLOWCAPOExcMemGeoMean}{31}
\newcommand{\SLOWCAPOMemGeoMean}{\memna}
\newcommand{\SLOWWCPDynamicTotal}{400,914}
\newcommand{\SLOWHBDynamicUPTotal}{0}
\newcommand{\SLOWPIPWDCDynamicTotal}{0}
\newcommand{\SLOWCAPOTotal}{0}
\newcommand{\SLOWPIPWCPTotal}{0}
\newcommand{\SLOWWCPTotal}{70}
\newcommand{\SLOWWDCnoGDynamicUPTotal}{0}
\newcommand{\SLOWCAPOnoGExcDynamicTotal}{715,707}
\newcommand{\SLOWCAPOExcTotal}{77}
\newcommand{\SLOWDCExcTotal}{77}
\newcommand{\SLOWDCnoGExcTotal}{108}
\newcommand{\SLOWPIPDynamicUPTotal}{0}
\newcommand{\SLOWPIPPIPTotal}{0}
\newcommand{\SLOWFTTotal}{0}
\newcommand{\SLOWHBDynamicTotal}{182,290}
\newcommand{\SLOWCAPOnoGDynamicUPTotal}{0}
\newcommand{\SLOWDCnoGExcDynamicTotal}{689,981}
\newcommand{\SLOWCAPOnoGTotal}{0}
\newcommand{\SLOWPIPWDCTotal}{0}
\newcommand{\SLOWCAPOnoGExcTotal}{102}
\newcommand{\SLOWPIPHBDynamicTotal}{0}
\newcommand{\SLOWWDCUPTotal}{0}
\newcommand{\SLOWDCnoGTotal}{0}
\newcommand{\SLOWWCPDynamicUPTotal}{0}
\newcommand{\SLOWPIPUPTotal}{0}
\newcommand{\SLOWCAPODynamicTotal}{0}
\newcommand{\SLOWCAPOnoGUPTotal}{0}
\newcommand{\SLOWPIPCAPOTotal}{0}
\newcommand{\SLOWCAPOnoGDynamicTotal}{0}
\newcommand{\SLOWFTDynamicTotal}{0}
\newcommand{\SLOWPIPCAPODynamicTotal}{0}
\newcommand{\SLOWDCnoGDynamicTotal}{0}
\newcommand{\SLOWWDCnoGUPTotal}{0}
\newcommand{\SLOWDCExcDynamicTotal}{465,462}
\newcommand{\SLOWWDCDynamicUPTotal}{0}
\newcommand{\SLOWHBUPTotal}{0}
\newcommand{\SLOWCAPOExcDynamicTotal}{531,903}
\newcommand{\SLOWPIPTotal}{0}
\newcommand{\SLOWWCPUPTotal}{0}
\newcommand{\SLOWCAPOUPTotal}{0}
\newcommand{\SLOWPIPHBTotal}{0}
\newcommand{\SLOWHBTotal}{66}
\newcommand{\SLOWDCDynamicTotal}{0}
\newcommand{\SLOWPIPDynamicTotal}{0}
\newcommand{\SLOWCAPODynamicUPTotal}{0}
\newcommand{\SLOWPIPPIPDynamicTotal}{0}
\newcommand{\SLOWPIPWCPDynamicTotal}{0}
\newcommand{\SLOWDCTotal}{0}



==> result-tables.tex <==
% Table for geometric mean of all relations with various optimizations for all DaCapo benchmarks
\begin{table}[t]
\begin{empty}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$\;\!\times$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
% \input{result-macros/PIP_slowTool_noWriteOrReadRaceEdge_accessMetaUpdate}
% \input{result-macros/PIP_fastTool_noWriteOrReadRaceEdge_accessMetaUpdate}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOpt2Quiet}
%
\small
\centering
\begin{tabular}{@{}l|Hrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWHBTimeGeoMean}			& \roh{\FASTFTOHBTimeGeoMean}	& \rna \\
\WCP	& \rna							& \roh{\SLOWWCPTimeGeoMean}			& \roh{\FASTFTOWCPTimeGeoMean}	& \roh{\FASTREWCPTimeGeoMean} \\
\DC		& \roh{\SLOWDCExcTimeGeoMean}	& \roh{\SLOWDCnoGExcTimeGeoMean}	& \roh{\FASTFTODCTimeGeoMean}	& \roh{\FASTREDCTimeGeoMean} \\
\CAPO	& \roh{\SLOWCAPOExcTimeGeoMean}	& \roh{\SLOWCAPOnoGExcTimeGeoMean}	& \roh{\FASTFTOCAPOTimeGeoMean}	& \roh{\FASTRECAPOTimeGeoMean} \\
\mc{2}{H}{} & \mc{3}{c}{Run time} \\
\end{tabular}
\hspace*{1em}
\begin{tabular}{@{}HHrrr@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \mem{\SLOWHBMemGeoMean}			& \mem{\FASTFTOHBMemGeoMean}	& \rna \\
\WCP	& \rna							& \mem{\SLOWWCPMemGeoMean}			& \mem{\FASTFTOWCPMemGeoMean}	& \mem{\FASTREWCPMemGeoMean} \\
\DC		& \mem{\SLOWDCExcMemGeoMean}	& \mem{\SLOWDCnoGExcMemGeoMean}	& \mem{\FASTFTODCMemGeoMean}	& \mem{\FASTREDCMemGeoMean} \\
\CAPO	& \mem{\SLOWCAPOExcMemGeoMean}	& \mem{\SLOWCAPOnoGExcMemGeoMean}	& \mem{\FASTFTOCAPOMemGeoMean}	& \mem{\FASTRECAPOMemGeoMean} \\
\mc{2}{H}{} & \mc{3}{c}{Memory usage} \\
\end{tabular}

\caption{Geometric mean of run time and memory usage across the evaluated programs.}
\label{tab:runtime-memory:geoMean}
\end{empty}
% \end{table}
\medskip
% Combined benchmarks table for 10 trials of all relations with various optimizations
% \begin{table*}[t]
\begin{empty}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{#1} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
\newcommand{\vci}[2]{\ifthenelse{\equal{#1}{\rna}}{\rna}{\roh{#1}{\;}\ci{#2}}}
\newcommand{\ci}[1]{\ensuremath{\pm}{\;}\roh{#1}}
% \input{result-macros/PIP_slowTool_noWriteOrReadRaceEdge_accessMetaUpdate}
% \input{result-macros/PIP_fastTool_noWriteOrReadRaceEdge_accessMetaUpdate}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOpt2Quiet}
%
\smaller
\centering
\begin{tabular}{@{}l|Hr@{$\;\;$}r@{$\;\;$}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWavroraHBTime}			& \roh{\FASTavroraFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWavroraWCPTime}			& \roh{\FASTavroraFTOWCPTime}	& \roh{\FASTavroraREWCPTime} \\
\DC		& \roh{\SLOWavroraDCExcTime}	& \roh{\SLOWavroraDCnoGExcTime}	& \roh{\FASTavroraFTODCTime}	& \roh{\FASTavroraREDCTime} \\
\CAPO	& \roh{\SLOWavroraCAPOExcTime}	& \roh{\SLOWavroraCAPOnoGExcTime}	& \roh{\FASTavroraFTOCAPOTime}	& \roh{\FASTavroraRECAPOTime} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWbatikHBTime}			& \roh{\FASTbatikFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWbatikWCPTime}			& \roh{\FASTbatikFTOWCPTime}	& \roh{\FASTbatikREWCPTime} \\
\DC		& \roh{\SLOWbatikDCExcTime}	& \roh{\SLOWbatikDCnoGExcTime}	& \roh{\FASTbatikFTODCTime}	& \roh{\FASTbatikREDCTime} \\
\CAPO	& \roh{\SLOWbatikCAPOExcTime}	& \roh{\SLOWbatikCAPOnoGExcTime}	& \roh{\FASTbatikFTOCAPOTime}	& \roh{\FASTbatikRECAPOTime} \\
		& \mc{4}{c}{\bench{batik}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWhtwoHBTime}			& \roh{\FASThtwoFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWhtwoWCPTime}			& \roh{\FASThtwoFTOWCPTime}	& \roh{\FASThtwoREWCPTime} \\
\DC		& \roh{\SLOWhtwoDCExcTime}	& \roh{\SLOWhtwoDCnoGExcTime}	& \roh{\FASThtwoFTODCTime}	& \roh{\FASThtwoREDCTime} \\
\CAPO	& \roh{\SLOWhtwoCAPOExcTime}	& \roh{\SLOWhtwoCAPOnoGExcTime}	& \roh{\FASThtwoFTOCAPOTime}	& \roh{\FASThtwoRECAPOTime} \\
		& \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWjythonHBTime}			& \roh{\FASTjythonFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWjythonWCPTime}			& \roh{\FASTjythonFTOWCPTime}	& \roh{\FASTjythonREWCPTime} \\
\DC		& \roh{\SLOWjythonDCExcTime}	& \roh{\SLOWjythonDCnoGExcTime}	& \roh{\FASTjythonFTODCTime}	& \roh{\FASTjythonREDCTime} \\
\CAPO	& \roh{\SLOWjythonCAPOExcTime}	& \roh{\SLOWjythonCAPOnoGExcTime}	& \roh{\FASTjythonFTOCAPOTime}	& \roh{\FASTjythonRECAPOTime} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWluindexHBTime}			& \roh{\FASTluindexFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWluindexWCPTime}			& \roh{\FASTluindexFTOWCPTime}	& \roh{\FASTluindexREWCPTime} \\
\DC		& \roh{\SLOWluindexDCExcTime}	& \roh{\SLOWluindexDCnoGExcTime}	& \roh{\FASTluindexFTODCTime}	& \roh{\FASTluindexREDCTime} \\
\CAPO	& \roh{\SLOWluindexCAPOExcTime}	& \roh{\SLOWluindexCAPOnoGExcTime}	& \roh{\FASTluindexFTOCAPOTime}	& \roh{\FASTluindexRECAPOTime} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWlusearchHBTime}			& \roh{\FASTlusearchFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWlusearchWCPTime}			& \roh{\FASTlusearchFTOWCPTime}	& \roh{\FASTlusearchREWCPTime} \\
\DC		& \roh{\SLOWlusearchDCExcTime}	& \roh{\SLOWlusearchDCnoGExcTime}	& \roh{\FASTlusearchFTODCTime}	& \roh{\FASTlusearchREDCTime} \\
\CAPO	& \roh{\SLOWlusearchCAPOExcTime}	& \roh{\SLOWlusearchCAPOnoGExcTime}	& \roh{\FASTlusearchFTOCAPOTime}	& \roh{\FASTlusearchRECAPOTime} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{lusearch}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWpmdHBTime}			& \roh{\FASTpmdFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWpmdWCPTime}			& \roh{\FASTpmdFTOWCPTime}	& \roh{\FASTpmdREWCPTime} \\
\DC		& \roh{\SLOWpmdDCExcTime}	& \roh{\SLOWpmdDCnoGExcTime}	& \roh{\FASTpmdFTODCTime}	& \roh{\FASTpmdREDCTime} \\
\CAPO	& \roh{\SLOWpmdCAPOExcTime}	& \roh{\SLOWpmdCAPOnoGExcTime}	& \roh{\FASTpmdFTOCAPOTime}	& \roh{\FASTpmdRECAPOTime} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWsunflowHBTime}			& \roh{\FASTsunflowFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWsunflowWCPTime}			& \roh{\FASTsunflowFTOWCPTime}	& \roh{\FASTsunflowREWCPTime} \\
\DC		& \roh{\SLOWsunflowDCExcTime}	& \roh{\SLOWsunflowDCnoGExcTime}	& \roh{\FASTsunflowFTODCTime}	& \roh{\FASTsunflowREDCTime} \\
\CAPO	& \roh{\SLOWsunflowCAPOExcTime}	& \roh{\SLOWsunflowCAPOnoGExcTime}	& \roh{\FASTsunflowFTOCAPOTime}	& \roh{\FASTsunflowRECAPOTime} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWtomcatHBTime}			& \roh{\FASTtomcatFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWtomcatWCPTime}			& \roh{\FASTtomcatFTOWCPTime}	& \roh{\FASTtomcatREWCPTime} \\
\DC		& \roh{\SLOWtomcatDCExcTime}	& \roh{\SLOWtomcatDCnoGExcTime}	& \roh{\FASTtomcatFTODCTime}	& \roh{\FASTtomcatREDCTime} \\
\CAPO	& \roh{\SLOWtomcatCAPOExcTime}	& \roh{\SLOWtomcatCAPOnoGExcTime}	& \roh{\FASTtomcatFTOCAPOTime}	& \roh{\FASTtomcatRECAPOTime} \\
		& \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline
\HB		& \rna							& \roh{\SLOWxalanHBTime}			& \roh{\FASTxalanFTOHBTime}	& \rna \\
\WCP	& \rna							& \roh{\SLOWxalanWCPTime}			& \roh{\FASTxalanFTOWCPTime}	& \roh{\FASTxalanREWCPTime} \\
\DC		& \roh{\SLOWxalanDCExcTime}	& \roh{\SLOWxalanDCnoGExcTime}	& \roh{\FASTxalanFTODCTime}	& \roh{\FASTxalanREDCTime} \\
\CAPO	& \roh{\SLOWxalanCAPOExcTime}	& \roh{\SLOWxalanCAPOnoGExcTime}	& \roh{\FASTxalanFTOCAPOTime}	& \roh{\FASTxalanRECAPOTime} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\end{empty}
% \begin{tabular}{@{}l|r|r|r|r||r|r|r|r||r|r|r|r}
% 		& \mc{4}{c||}{\bench{avrora}} & \mc{4}{c||}{\bench{batik}} & \mc{4}{c}{\bench{h2}} \\
% 		& \mc{2}{c|}{Unopt-} & \mc{2}{c||}{} & \mc{2}{c|}{Unopt-} & \mc{2}{c||}{} & \mc{2}{c|}{Unopt-} & \mc{2}{c}{} \\
% Relation& w/ G & w/o G & \FTO- & \RE- & w/ G & w/o G & \FTO- & \RE- & w/ G & w/o G & \FTO- & \RE- \\\hline
% \HB		& \rna							& \roh{\SLOWavroraHBTime}			& \roh{\FASTavroraFTOHBTime}	& \rna							& \rna							& \roh{\SLOWbatikHBTime}		& \roh{\FASTbatikFTOHBTime}		& \rna						& \rna						& \roh{\SLOWhtwoHBTime}			& \roh{\FASThtwoFTOHBTime}	& \rna \\
% \WCP	& \rna							& \roh{\SLOWavroraWCPTime}			& \roh{\FASTavroraFTOWCPTime}	& \roh{\FASTavroraREWCPTime} 	& \rna							& \roh{\SLOWbatikWCPTime}		& \roh{\FASTbatikFTOWCPTime}	& \roh{\FASTbatikREWCPTime} & \rna						& \roh{\SLOWhtwoWCPTime}		& \roh{\FASThtwoFTOWCPTime}	& \roh{\FASThtwoREWCPTime} \\
% \DC		& \roh{\SLOWavroraWDCExcTime}	& \roh{\SLOWavroraWDCnoGExcTime}	& \roh{\FASTavroraFTODCTime}	& \roh{\FASTavroraREDCTime}		& \roh{\SLOWbatikWDCExcTime}	& \roh{\SLOWbatikWDCnoGExcTime}	& \roh{\FASTbatikFTODCTime}		& \roh{\FASTbatikREDCTime}	& \roh{\SLOWhtwoWDCExcTime}	& \roh{\SLOWhtwoWDCnoGExcTime}	& \roh{\FASThtwoFTODCTime}	& \roh{\FASThtwoREDCTime} \\
% \CAPO	& \roh{\SLOWavroraCAPOExcTime}	& \roh{\SLOWavroraCAPOnoGExcTime}	& \roh{\FASTavroraFTOCAPOTime}	& \roh{\FASTavroraRECAPOTime}	& \roh{\SLOWbatikCAPOExcTime}	& \roh{\SLOWbatikCAPOnoGExcTime}& \roh{\FASTbatikFTOCAPOTime}	& \roh{\FASTbatikRECAPOTime}& \roh{\SLOWhtwoCAPOExcTime}& \roh{\SLOWhtwoCAPOnoGExcTime}	& \roh{\FASThtwoFTOCAPOTime}& \roh{\FASThtwoRECAPOTime} \\\hline
% \hline
% \end{tabular}
% \begin{tabular}{@{}l|r|r|r|r||r|r|r|r||r|r|r|r}
% 		& \mc{4}{c||}{\bench{jython}} & \mc{4}{c||}{\bench{luindex}} & \mc{4}{c}{\bench{lusearch}} \\
% 		& \mc{2}{c|}{Unopt-} & \mc{2}{c||}{} & \mc{2}{c|}{Unopt-} & \mc{2}{c||}{} & \mc{2}{c|}{Unopt-} & \mc{2}{c}{} \\
% Relation& w/ G & w/o G & \FTO- & \RE- & w/ G & w/o G & \FTO- & \RE- & w/ G & w/o G & \FTO- & \RE- \\\hline
% \HB		& \rna							& \roh{\SLOWjythonHBTime}			& \roh{\FASTjythonFTOHBTime}	& \rna							& \rna							& \roh{\SLOWluindexHBTime}			& \roh{\FASTluindexFTOHBTime}	& \rna							& \rna							& \roh{\SLOWlusearchHBTime}			& \roh{\FASTlusearchFTOHBTime}	& \rna \\
% \WCP	& \rna							& \roh{\SLOWjythonWCPTime}			& \roh{\FASTjythonFTOWCPTime}	& \roh{\FASTjythonREWCPTime} 	& \rna							& \roh{\SLOWluindexWCPTime}			& \roh{\FASTluindexFTOWCPTime}	& \roh{\FASTluindexREWCPTime}	& \rna							& \roh{\SLOWlusearchWCPTime}		& \roh{\FASTlusearchFTOWCPTime}	& \roh{\FASTlusearchREWCPTime} \\
% \DC		& \roh{\SLOWjythonWDCExcTime}	& \roh{\SLOWjythonWDCnoGExcTime}	& \roh{\FASTjythonFTODCTime}	& \roh{\FASTjythonREDCTime}		& \roh{\SLOWluindexWDCExcTime}	& \roh{\SLOWluindexWDCnoGExcTime}	& \roh{\FASTluindexFTODCTime}	& \roh{\FASTluindexREDCTime}	& \roh{\SLOWlusearchWDCExcTime}	& \roh{\SLOWlusearchWDCnoGExcTime}	& \roh{\FASTlusearchFTODCTime}	& \roh{\FASTlusearchREDCTime} \\
% \CAPO	& \roh{\SLOWjythonCAPOExcTime}	& \roh{\SLOWjythonCAPOnoGExcTime}	& \roh{\FASTjythonFTOCAPOTime}	& \roh{\FASTjythonRECAPOTime}	& \roh{\SLOWluindexCAPOExcTime}	& \roh{\SLOWluindexCAPOnoGExcTime}	& \roh{\FASTluindexFTOCAPOTime}	& \roh{\FASTluindexRECAPOTime}	& \roh{\SLOWlusearchCAPOExcTime}& \roh{\SLOWlusearchCAPOnoGExcTime}	& \roh{\FASTlusearchFTOCAPOTime}& \roh{\FASTlusearchRECAPOTime} \\\hline
% \hline
% \end{tabular}
% \begin{tabular}{@{}l|r|r|r|r||r|r|r|r||r|r|r|r||r|r|r|r}
% 		& \mc{4}{c||}{\bench{pmd}} & \mc{4}{c||}{\bench{sunflow}} & \mc{4}{c||}{\bench{tomcat}} & \mc{4}{c}{\bench{xalan}} \\
% 		& \mc{2}{c|}{Unopt-} & \mc{2}{c||}{} & \mc{2}{c|}{Unopt-} & \mc{2}{c||}{} & \mc{2}{c|}{Unopt-} & \mc{2}{c||}{} & \mc{2}{c|}{Unopt-} & \mc{2}{c}{} \\
% Relation& w/ G & w/o G & \FTO- & \RE- & w/ G & w/o G & \FTO- & \RE- & w/ G & w/o G & \FTO- & \RE- & w/ G & w/o G & \FTO- & \RE- \\\hline
% \HB		& \rna						& \roh{\SLOWpmdHBTime}			& \roh{\FASTpmdFTOHBTime}	& \rna						& \rna							& \roh{\SLOWsunflowHBTime}			& \roh{\FASTsunflowFTOHBTime}	& \rna							& \rna							& \roh{\SLOWtomcatHBTime}			& \roh{\FASTtomcatFTOHBTime}	& \rna 							& \rna							& \roh{\SLOWxalanHBTime}			& \roh{\FASTxalanFTOHBTime}		& \rna \\
% \WCP	& \rna						& \roh{\SLOWpmdWCPTime}			& \roh{\FASTpmdFTOWCPTime}	& \roh{\FASTpmdREWCPTime} 	& \rna							& \roh{\SLOWsunflowWCPTime}			& \roh{\FASTsunflowFTOWCPTime}	& \roh{\FASTsunflowREWCPTime} 	& \rna							& \roh{\SLOWtomcatWCPTime}			& \roh{\FASTtomcatFTOWCPTime}	& \roh{\FASTtomcatREWCPTime} 	& \rna							& \roh{\SLOWxalanWCPTime}			& \roh{\FASTxalanFTOWCPTime}	& \roh{\FASTxalanREWCPTime} \\
% \DC		& \roh{\SLOWpmdWDCExcTime}	& \roh{\SLOWpmdWDCnoGExcTime}	& \roh{\FASTpmdFTODCTime}	& \roh{\FASTpmdREDCTime}	& \roh{\SLOWsunflowWDCExcTime}	& \roh{\SLOWsunflowWDCnoGExcTime}	& \roh{\FASTsunflowFTODCTime}	& \roh{\FASTsunflowREDCTime}	& \roh{\SLOWtomcatWDCExcTime}	& \roh{\SLOWtomcatWDCnoGExcTime}	& \roh{\FASTtomcatFTODCTime}	& \roh{\FASTtomcatREDCTime} 	& \roh{\SLOWxalanWDCExcTime}	& \roh{\SLOWxalanWDCnoGExcTime}		& \roh{\FASTxalanFTODCTime}		& \roh{\FASTxalanREDCTime} \\
% \CAPO	& \roh{\SLOWpmdCAPOExcTime}	& \roh{\SLOWpmdCAPOnoGExcTime}	& \roh{\FASTpmdFTOCAPOTime}	& \roh{\FASTpmdRECAPOTime}	& \roh{\SLOWsunflowCAPOExcTime}	& \roh{\SLOWsunflowCAPOnoGExcTime}	& \roh{\FASTsunflowFTOCAPOTime}	& \roh{\FASTsunflowRECAPOTime}	& \roh{\SLOWtomcatCAPOExcTime}	& \roh{\SLOWtomcatCAPOnoGExcTime}	& \roh{\FASTtomcatFTOCAPOTime}	& \roh{\FASTtomcatRECAPOTime}	& \roh{\SLOWxalanCAPOExcTime}	& \roh{\SLOWxalanCAPOnoGExcTime}	& \roh{\FASTxalanFTOCAPOTime}	& \roh{\FASTxalanRECAPOTime} \\\hline
% \end{tabular}

% \mike{Some results in this table and next are only 1 sig fig, \eg, 7x}

\caption{Run time, relative to uninstrumented execution, of various analyses for each evaluated program.}
\label{tab:performance:allDaCapo}
% \end{table*}
\medskip
% Table for 10 trials of all relations with various optimizations for all DaCapo benchmarks
% \begin{table*}[t]
\begin{empty}
\newcommand{\rzero}{0\xspace}
\newcommand{\roh}[1]{\ifthenelse{\equal{#1}{\rna}}{\rna}{#1$\;\!\times$}} %runtime overhead
\newcommand{\rna}{N/A}
\newcommand{\memna}{N/A} %\newcommand{\memna}{$<\,$2}
\newcommand{\st}[1]{(#1~s)} %static time
\newcommand{\dt}[1]{#1~s} %dynamic time
\newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\rna}{#1$\;\!\times$}}
%memory \newcommand{\mem}[1]{\ifthenelse{\equal{#1}{\memna}}{\memna}{#1$Gb$}} %memory
\newcommand{\et}[1]{#1M} %event total
\newcommand{\enfp}[1]{(#1M)} %event total, no fast path
\newcommand{\base}[1]{#1~s} %base time
% \input{result-macros/PIP_slowTool_noWriteOrReadRaceEdge_accessMetaUpdate}
% \input{result-macros/PIP_fastTool_noWriteOrReadRaceEdge_accessMetaUpdate}
\input{result-macros/PIP_slowTool_noCoresSet}
\input{result-macros/PIP_fastTool_extraOpt2Quiet}
%
\smaller
\centering
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWavroraHBMem}		& \mem{\FASTavroraFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWavroraWCPMem}		& \mem{\FASTavroraFTOWCPMem}	& \mem{\FASTavroraREWCPMem} \\
\DC		& \mem{\SLOWavroraDCExcMem}	& \mem{\SLOWavroraDCnoGExcMem}	& \mem{\FASTavroraFTODCMem}		& \mem{\FASTavroraREDCMem} \\
\CAPO	& \mem{\SLOWavroraCAPOExcMem}	& \mem{\SLOWavroraCAPOnoGExcMem}& \mem{\FASTavroraFTOCAPOMem}	& \mem{\FASTavroraRECAPOMem} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{avrora}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWbatikHBMem}		& \mem{\FASTbatikFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWbatikWCPMem}		& \mem{\FASTbatikFTOWCPMem}	& \mem{\FASTbatikREWCPMem} \\
\DC		& \mem{\SLOWbatikDCExcMem}	& \mem{\SLOWbatikDCnoGExcMem}	& \mem{\FASTbatikFTODCMem}		& \mem{\FASTbatikREDCMem} \\
\CAPO	& \mem{\SLOWbatikCAPOExcMem}	& \mem{\SLOWbatikCAPOnoGExcMem}& \mem{\FASTbatikFTOCAPOMem}	& \mem{\FASTbatikRECAPOMem} \\
		& \mc{4}{c}{\bench{batik}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWhtwoHBMem}		& \mem{\FASThtwoFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWhtwoWCPMem}		& \mem{\FASThtwoFTOWCPMem}	& \mem{\FASThtwoREWCPMem} \\
\DC		& \mem{\SLOWhtwoDCExcMem}	& \mem{\SLOWhtwoDCnoGExcMem}	& \mem{\FASThtwoFTODCMem}		& \mem{\FASThtwoREDCMem} \\
\CAPO	& \mem{\SLOWhtwoCAPOExcMem}	& \mem{\SLOWhtwoCAPOnoGExcMem}& \mem{\FASThtwoFTOCAPOMem}	& \mem{\FASThtwoRECAPOMem} \\
		& \mc{4}{c}{\bench{h2}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWjythonHBMem}		& \mem{\FASTjythonFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWjythonWCPMem}		& \mem{\FASTjythonFTOWCPMem}	& \mem{\FASTjythonREWCPMem} \\
\DC		& \mem{\SLOWjythonDCExcMem}	& \mem{\SLOWjythonDCnoGExcMem}	& \mem{\FASTjythonFTODCMem}		& \mem{\FASTjythonREDCMem} \\
\CAPO	& \mem{\SLOWjythonCAPOExcMem}	& \mem{\SLOWjythonCAPOnoGExcMem}& \mem{\FASTjythonFTOCAPOMem}	& \mem{\FASTjythonRECAPOMem} \\
		& \mc{4}{c}{\bench{jython}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWluindexHBMem}		& \mem{\FASTluindexFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWluindexWCPMem}		& \mem{\FASTluindexFTOWCPMem}	& \mem{\FASTluindexREWCPMem} \\
\DC		& \mem{\SLOWluindexDCExcMem}	& \mem{\SLOWluindexDCnoGExcMem}	& \mem{\FASTluindexFTODCMem}		& \mem{\FASTluindexREDCMem} \\
\CAPO	& \mem{\SLOWluindexCAPOExcMem}	& \mem{\SLOWluindexCAPOnoGExcMem}& \mem{\FASTluindexFTOCAPOMem}	& \mem{\FASTluindexRECAPOMem} \\
		& \mc{4}{c}{\bench{luindex}} \\
\end{tabular}
\medskip\\
\begin{tabular}{@{}l|Hr@{\;\;}r@{\;\;}r@{}}
        & w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWlusearchHBMem}		& \mem{\FASTlusearchFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWlusearchWCPMem}		& \mem{\FASTlusearchFTOWCPMem}	& \mem{\FASTlusearchREWCPMem} \\
\DC		& \mem{\SLOWlusearchDCExcMem}	& \mem{\SLOWlusearchDCnoGExcMem}	& \mem{\FASTlusearchFTODCMem}		& \mem{\FASTlusearchREDCMem} \\
\CAPO	& \mem{\SLOWlusearchCAPOExcMem}	& \mem{\SLOWlusearchCAPOnoGExcMem}& \mem{\FASTlusearchFTOCAPOMem}	& \mem{\FASTlusearchRECAPOMem} \\
\mc{1}{c}{} & \mc{4}{c}{\bench{lusearch}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWpmdHBMem}		& \mem{\FASTpmdFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWpmdWCPMem}		& \mem{\FASTpmdFTOWCPMem}	& \mem{\FASTpmdREWCPMem} \\
\DC		& \mem{\SLOWpmdDCExcMem}	& \mem{\SLOWpmdDCnoGExcMem}	& \mem{\FASTpmdFTODCMem}		& \mem{\FASTpmdREDCMem} \\
\CAPO	& \mem{\SLOWpmdCAPOExcMem}	& \mem{\SLOWpmdCAPOnoGExcMem}& \mem{\FASTpmdFTOCAPOMem}	& \mem{\FASTpmdRECAPOMem} \\
		& \mc{4}{c}{\bench{pmd}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWsunflowHBMem}		& \mem{\FASTsunflowFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWsunflowWCPMem}		& \mem{\FASTsunflowFTOWCPMem}	& \mem{\FASTsunflowREWCPMem} \\
\DC		& \mem{\SLOWsunflowDCExcMem}	& \mem{\SLOWsunflowDCnoGExcMem}	& \mem{\FASTsunflowFTODCMem}		& \mem{\FASTsunflowREDCMem} \\
\CAPO	& \mem{\SLOWsunflowCAPOExcMem}	& \mem{\SLOWsunflowCAPOnoGExcMem}& \mem{\FASTsunflowFTOCAPOMem}	& \mem{\FASTsunflowRECAPOMem} \\
		& \mc{4}{c}{\bench{sunflow}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWtomcatHBMem}		& \mem{\FASTtomcatFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWtomcatWCPMem}		& \mem{\FASTtomcatFTOWCPMem}	& \mem{\FASTtomcatREWCPMem} \\
\DC		& \mem{\SLOWtomcatDCExcMem}	& \mem{\SLOWtomcatDCnoGExcMem}	& \mem{\FASTtomcatFTODCMem}		& \mem{\FASTtomcatREDCMem} \\
\CAPO	& \mem{\SLOWtomcatCAPOExcMem}	& \mem{\SLOWtomcatCAPOnoGExcMem}& \mem{\FASTtomcatFTOCAPOMem}	& \mem{\FASTtomcatRECAPOMem} \\
		& \mc{4}{c}{\bench{tomcat}} \\
\end{tabular}
\hfill
\begin{tabular}{@{}HHr@{\;\;}r@{\;\;}r@{}}
Relation& w/ G & Unopt- & \FTO- & \REAbbrv- \\\hline 
\HB		& \rna							& \mem{\SLOWxalanHBMem}		& \mem{\FASTxalanFTOHBMem}		& \rna \\
\WCP	& \rna							& \mem{\SLOWxalanWCPMem}		& \mem{\FASTxalanFTOWCPMem}	& \mem{\FASTxalanREWCPMem} \\
\DC		& \mem{\SLOWxalanDCExcMem}	& \mem{\SLOWxalanDCnoGExcMem}	& \mem{\FASTxalanFTODCMem}		& \mem{\FASTxalanREDCMem} \\
\CAPO	& \mem{\SLOWxalanCAPOExcMem}	& \mem{\SLOWxalanCAPOnoGExcMem}& \mem{\FASTxalanFTOCAPOMem}	& \mem{\FASTxalanRECAPOMem} \\
		& \mc{4}{c}{\bench{xalan}} \\
\end{tabular}
\end{empty}
% \begin{tabular}{@{}l|r|r|r|r||r|r|r|r||r|r|r|r}
% 		& \mc{4}{c||}{\bench{avrora}} & \mc{4}{c||}{\bench{batik}} & \mc{4}{c}{\bench{h2}} \\
% 		& \mc{2}{c|}{Unopt-} & \mc{2}{c||}{} & \mc{2}{c|}{Unopt-} & \mc{2}{c||}{} & \mc{2}{c|}{Unopt-} & \mc{2}{c}{} \\
% Relation& w/ G & w/o G & \FTO- & \RE- & w/ G & w/o G & \FTO- & \RE- & w/ G & w/o G & \FTO- & \RE- \\\hline
% \HB		& \rna							& \mem{\SLOWavroraHBMem}		& \mem{\FASTavroraFTOHBMem}		& \rna 						& \rna						& \mem{\SLOWbatikHBMem}			& \mem{\FASTbatikFTOHBMem}	& \rna 						& \rna						& \mem{\SLOWhtwoHBMem}			& \mem{\FASThtwoFTOHBMem}	& \rna \\
% \WCP	& \rna							& \mem{\SLOWavroraWCPMem}		& \mem{\FASTavroraFTOWCPMem}	& \mem{\FASTavroraREWCPMem} & \rna						& \mem{\SLOWbatikWCPMem}		& \mem{\FASTbatikFTOWCPMem}	& \mem{\FASTbatikREWCPMem} 	& \rna						& \mem{\SLOWhtwoWCPMem}			& \mem{\FASThtwoFTOWCPMem}	& \mem{\FASThtwoREWCPMem} \\
% \DC		& \mem{\SLOWavroraWDCExcMem}	& \mem{\SLOWavroraWDCnoGExcMem}	& \mem{\FASTavroraFTODCMem}		& \mem{\FASTavroraREDCMem} 	& \mem{\SLOWbatikWDCExcMem}	& \mem{\SLOWbatikWDCnoGExcMem}	& \mem{\FASTbatikFTODCMem}	& \mem{\FASTbatikREDCMem} 	& \mem{\SLOWhtwoWDCExcMem}	& \mem{\SLOWhtwoWDCnoGExcMem}	& \mem{\FASThtwoFTODCMem}	& \mem{\FASThtwoREDCMem} \\
% \CAPO	& \mem{\SLOWavroraCAPOExcMem}	& \mem{\SLOWavroraCAPOnoGExcMem}& \mem{\FASTavroraFTOCAPOMem}	& \mem{\FASTavroraRECAPOMem}& \mem{\SLOWbatikCAPOExcMem}& \mem{\SLOWbatikCAPOnoGExcMem}	& \mem{\FASTbatikFTOCAPOMem}& \mem{\FASTbatikRECAPOMem} & \mem{\SLOWhtwoCAPOExcMem}	& \mem{\SLOWhtwoCAPOnoGExcMem}	& \mem{\FASThtwoFTOCAPOMem}	& \mem{\FASThtwoRECAPOMem} \\\hline
% \end{tabular}
% \begin{tabular}{@{}l|r|r|r|r||r|r|r|r||r|r|r|r}
% 		& \mc{4}{c||}{\bench{jython}} & \mc{4}{c||}{\bench{luindex}} & \mc{4}{c}{\bench{lusearch}} \\
% 		& \mc{2}{c|}{Unopt-} & \mc{2}{c||}{} & \mc{2}{c|}{Unopt-} & \mc{2}{c||}{} & \mc{2}{c|}{Unopt-} & \mc{2}{c}{} \\
% Relation& w/ G & w/o G & \FTO- & \RE- & w/ G & w/o G & \FTO- & \RE- & w/ G & w/o G & \FTO- & \RE- \\\hline
% \HB		& \rna							& \mem{\SLOWjythonHBMem}		& \mem{\FASTjythonFTOHBMem}		& \rna 						& \rna							& \mem{\SLOWluindexHBMem}			& \mem{\FASTluindexFTOHBMem}	& \rna 							& \rna							& \mem{\SLOWlusearchHBMem}			& \mem{\FASTlusearchFTOHBMem}	& \rna \\
% \WCP	& \rna							& \mem{\SLOWjythonWCPMem}		& \mem{\FASTjythonFTOWCPMem}	& \mem{\FASTjythonREWCPMem} & \rna							& \mem{\SLOWluindexWCPMem}			& \mem{\FASTluindexFTOWCPMem}	& \mem{\FASTluindexREWCPMem} 	& \rna							& \mem{\SLOWlusearchWCPMem}			& \mem{\FASTlusearchFTOWCPMem}	& \mem{\FASTlusearchREWCPMem} \\
% \DC		& \mem{\SLOWjythonWDCExcMem}	& \mem{\SLOWjythonWDCnoGExcMem}	& \mem{\FASTjythonFTODCMem}		& \mem{\FASTjythonREDCMem} 	& \mem{\SLOWluindexWDCExcMem}	& \mem{\SLOWluindexWDCnoGExcMem}	& \mem{\FASTluindexFTODCMem}	& \mem{\FASTluindexREDCMem} 	& \mem{\SLOWlusearchWDCExcMem}	& \mem{\SLOWlusearchWDCnoGExcMem}	& \mem{\FASTlusearchFTODCMem}	& \mem{\FASTlusearchREDCMem} \\
% \CAPO	& \mem{\SLOWjythonCAPOExcMem}	& \mem{\SLOWjythonCAPOnoGExcMem}& \mem{\FASTjythonFTOCAPOMem}	& \mem{\FASTjythonRECAPOMem}& \mem{\SLOWluindexCAPOExcMem}	& \mem{\SLOWluindexCAPOnoGExcMem}	& \mem{\FASTluindexFTOCAPOMem}	& \mem{\FASTluindexRECAPOMem}	& \mem{\SLOWlusearchCAPOExcMem}	& \mem{\SLOWlusearchCAPOnoGExcMem}	& \mem{\FASTlusearchFTOCAPOMem}	& \mem{\FASTlusearchRECAPOMem} \\\hline
% \hline
% \end{tabular}
% \begin{tabular}{@{}l|r|r|r|r||r|r|r|r||r|r|r|r||r|r|r|r}
% 		& \mc{4}{c||}{\bench{pmd}} & \mc{4}{c||}{\bench{sunflow}} & \mc{4}{c||}{\bench{tomcat}} & \mc{4}{c}{\bench{xalan}} \\
% 		& \mc{2}{c|}{Unopt-} & \mc{2}{c||}{} & \mc{2}{c|}{Unopt-} & \mc{2}{c||}{} & \mc{2}{c|}{Unopt-} & \mc{2}{c||}{} & \mc{2}{c|}{Unopt-} & \mc{2}{c}{} \\
% Relation& w/ G & w/o G & \FTO- & \RE- & w/ G & w/o G & \FTO- & \RE- & w/ G & w/o G & \FTO- & \RE- & w/ G & w/o G & \FTO- & \RE- \\\hline
% \HB		& \rna						& \mem{\SLOWpmdHBMem}			& \mem{\FASTpmdFTOHBMem}	& \rna 						& \rna							& \mem{\SLOWsunflowHBMem}			& \mem{\FASTsunflowFTOHBMem}	& \rna 							& \rna							& \mem{\SLOWtomcatHBMem}		& \mem{\FASTtomcatFTOHBMem}		& \rna 						& \rna						& \mem{\SLOWxalanHBMem}			& \mem{\FASTxalanFTOHBMem}	& \rna \\
% \WCP	& \rna						& \mem{\SLOWpmdWCPMem}			& \mem{\FASTpmdFTOWCPMem}	& \mem{\FASTpmdREWCPMem} 	& \rna							& \mem{\SLOWsunflowWCPMem}			& \mem{\FASTsunflowFTOWCPMem}	& \mem{\FASTsunflowREWCPMem} 	& \rna							& \mem{\SLOWtomcatWCPMem}		& \mem{\FASTtomcatFTOWCPMem}	& \mem{\FASTtomcatREWCPMem} & \rna						& \mem{\SLOWxalanWCPMem}		& \mem{\FASTxalanFTOWCPMem}	& \mem{\FASTxalanREWCPMem} \\
% \DC		& \mem{\SLOWpmdWDCExcMem}	& \mem{\SLOWpmdWDCnoGExcMem}	& \mem{\FASTpmdFTODCMem}	& \mem{\FASTpmdREDCMem} 	& \mem{\SLOWsunflowWDCExcMem}	& \mem{\SLOWsunflowWDCnoGExcMem}	& \mem{\FASTsunflowFTODCMem}	& \mem{\FASTsunflowREDCMem} 	& \mem{\SLOWtomcatWDCExcMem}	& \mem{\SLOWtomcatWDCnoGExcMem}	& \mem{\FASTtomcatFTODCMem}		& \mem{\FASTtomcatREDCMem} 	& \mem{\SLOWxalanWDCExcMem}	& \mem{\SLOWxalanWDCnoGExcMem}	& \mem{\FASTxalanFTODCMem}	& \mem{\FASTxalanREDCMem} \\
% \CAPO	& \mem{\SLOWpmdCAPOExcMem}	& \mem{\SLOWpmdCAPOnoGExcMem}	& \mem{\FASTpmdFTOCAPOMem}	& \mem{\FASTpmdRECAPOMem}	& \mem{\SLOWsunflowCAPOExcMem}	& \mem{\SLOWsunflowCAPOnoGExcMem}	& \mem{\FASTsunflowFTOCAPOMem}	& \mem{\FASTsunflowRECAPOMem} 	& \mem{\SLOWtomcatCAPOExcMem}	& \mem{\SLOWtomcatCAPOnoGExcMem}& \mem{\FASTtomcatFTOCAPOMem}	& \mem{\FASTtomcatRECAPOMem}& \mem{\SLOWxalanCAPOExcMem}& \mem{\SLOWxalanCAPOnoGExcMem}	& \mem{\FASTxalanFTOCAPOMem}& \mem{\FASTxalanRECAPOMem} \\\hline
% \end{tabular}
\caption{Memory usage, relative to uninstrumented execution, of various analyses for each evaluated program.}
\label{tab:memory:allDaCapo}
\end{table}
